Improving Hyperparameter Learning under Approximate Inference in Gaussian Process Models

Approximate inference in Gaussian process (GP) models with non-conjugate likelihoods gets entangled with the learning of the model hyperparameters. We improve hyperparameter learning in GP models and focus on the interplay between variational inference (VI) and the learning target. While VI's lower bound to the marginal likelihood is a suitable objective for inferring the approximate posterior, we show that a direct approximation of the marginal likelihood as in Expectation Propagation (EP) is a better learning objective for hyperparameter optimization. We design a hybrid training procedure to bring the best of both worlds: it leverages conjugate-computation VI for inference and uses an EP-like marginal likelihood approximation for hyperparameter learning. We compare VI, EP, Laplace approximation, and our proposed training procedure and empirically demonstrate the effectiveness of our proposal across a wide range of data sets.

==> fig/tikz/echocardiogram/CVI_mean_lml.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=midnightblue868137]
table{%
x  y
-0.965176862651772 5
-1 5
-1 4.9799859058673
-0.965176862651772 5
};
\addplot [draw=none, fill=teal882156]
table{%
x  y
-0.7 4.64651431294783
-0.661604515618406 4.7
-0.4 4.99808111091457
-0.398814414852452 5
-0.4 5
-0.7 5
-0.965176862651772 5
-1 4.9799859058673
-1 4.7
-1 4.43350699417605
-0.7 4.64651431294783
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 4.0840522386727
-0.683844546560555 4.1
-0.45625863378095 4.4
-0.4 4.47779383823009
-0.284551333453605 4.7
-0.1 4.9989392438043
-0.0994177888688242 5
-0.1 5
-0.398814414852452 5
-0.4 4.99808111091457
-0.661604515618406 4.7
-0.7 4.64651431294783
-1 4.43350699417605
-1 4.4
-1 4.1
-1 3.94161783758784
-0.7 4.0840522386727
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.7 3.68118046939443
-0.558389151780856 3.8
-0.4 3.95623038856431
-0.302299117977726 4.1
-0.142873898469358 4.4
-0.1 4.48184555936192
0.00483484948736258 4.7
0.167172769989289 5
-0.0994177888688242 5
-0.1 4.9989392438043
-0.284551333453605 4.7
-0.4 4.47779383823009
-0.45625863378095 4.4
-0.683844546560555 4.1
-0.7 4.0840522386727
-1 3.94161783758784
-1 3.8
-1 3.56075833823817
-0.7 3.68118046939443
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
-0.865838045614262 3.2
-0.7 3.27677137022905
-0.457621772036447 3.5
-0.4 3.54796712768506
-0.19737084955357 3.8
-0.1 3.94658159046342
-0.00994218157588041 4.1
0.134946482163237 4.4
0.2 4.53641519335707
0.282901635281974 4.7
0.4468623454466 5
0.2 5
0.167172769989289 5
0.00483484948736258 4.7
-0.1 4.48184555936192
-0.142873898469358 4.4
-0.302299117977726 4.1
-0.4 3.95623038856431
-0.558389151780856 3.8
-0.7 3.68118046939443
-1 3.56075833823817
-1 3.5
-1 3.2
-1 3.13918422394161
-0.865838045614262 3.2
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
-0.7 2.85400786496181
-0.641064005744569 2.9
-0.4 3.11827470011557
-0.336797662132565 3.2
-0.108562796678952 3.5
-0.1 3.51080495436832
0.0996284614464144 3.8
0.2 3.97638442185797
0.27324600729951 4.1
0.425953415003237 4.4
0.5 4.54825982858438
0.58750213534616 4.7
0.763072142064107 5
0.5 5
0.4468623454466 5
0.282901635281974 4.7
0.2 4.53641519335707
0.134946482163237 4.4
-0.00994218157588041 4.1
-0.1 3.94658159046342
-0.19737084955357 3.8
-0.4 3.54796712768506
-0.457621772036447 3.5
-0.7 3.27677137022905
-0.865838045614262 3.2
-1 3.13918422394161
-1 2.9
-1 2.73953269355362
-0.7 2.85400786496181
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
-0.7 2.46996967206763
-0.530298590178671 2.6
-0.4 2.70026762544519
-0.224172720741803 2.9
-0.1 3.06196630532303
-0.00401542727905356 3.2
0.198167336380329 3.5
0.2 3.50272521981886
0.404339343152064 3.8
0.5 3.96578574226325
0.586005186895158 4.1
0.759846139273216 4.4
0.8 4.47032526837776
0.952548848017844 4.7
1.1 4.92779093578274
1.15212887393327 5
1.1 5
0.8 5
0.763072142064107 5
0.58750213534616 4.7
0.5 4.54825982858438
0.425953415003237 4.4
0.27324600729951 4.1
0.2 3.97638442185797
0.0996284614464144 3.8
-0.1 3.51080495436832
-0.108562796678952 3.5
-0.336797662132565 3.2
-0.4 3.11827470011557
-0.641064005744569 2.9
-0.7 2.85400786496181
-1 2.73953269355362
-1 2.6
-1 2.35667560055035
-0.7 2.46996967206763
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
-0.857132272416404 2
-0.7 2.06026117107486
-0.4 2.29459629105761
-0.395123815500629 2.3
-0.121612467546804 2.6
-0.1 2.62477042137366
0.113199003239896 2.9
0.2 3.02720312873475
0.324189886715699 3.2
0.5 3.45447235645461
0.53513500291541 3.5
0.751036823978578 3.8
0.8 3.87820009322412
0.959432279445561 4.1
1.1 4.31115033984553
1.16791580543921 4.4
1.38738825139699 4.7
1.4 4.71752474178267
1.62175710834103 5
1.4 5
1.15212887393327 5
1.1 4.92779093578274
0.952548848017844 4.7
0.8 4.47032526837776
0.759846139273216 4.4
0.586005186895158 4.1
0.5 3.96578574226325
0.404339343152064 3.8
0.2 3.50272521981886
0.198167336380329 3.5
-0.00401542727905356 3.2
-0.1 3.06196630532303
-0.224172720741803 2.9
-0.4 2.70026762544519
-0.530298590178671 2.6
-0.7 2.46996967206763
-1 2.35667560055035
-1 2.3
-1 2
-1 1.94266677834174
-0.857132272416404 2
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
-0.7 1.6018097573662
-0.587951796883488 1.7
-0.4 1.8477615932449
-0.264870209531329 2
-0.1 2.18383556344031
-0.00575025364131102 2.3
0.2 2.55758936712225
0.235340688553063 2.6
0.468910428146778 2.9
0.5 2.94407080882945
0.703380242314739 3.2
0.8 3.32730802863878
0.947362498829797 3.5
1.1 3.69540776267712
1.19116264011306 3.8
1.4 4.05982957649237
1.43582941144356 4.1
1.68858175812974 4.4
1.7 4.41413629871771
1.95203619426201 4.7
2 4.75647909067455
2.22671768387992 5
2 5
1.7 5
1.62175710834103 5
1.4 4.71752474178267
1.38738825139699 4.7
1.16791580543921 4.4
1.1 4.31115033984553
0.959432279445561 4.1
0.8 3.87820009322412
0.751036823978578 3.8
0.53513500291541 3.5
0.5 3.45447235645461
0.324189886715699 3.2
0.2 3.02720312873475
0.113199003239896 2.9
-0.1 2.62477042137366
-0.121612467546804 2.6
-0.395123815500629 2.3
-0.4 2.29459629105761
-0.7 2.06026117107486
-0.857132272416404 2
-1 1.94266677834174
-1 1.7
-1 1.47061487646979
-0.7 1.6018097573662
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
-0.907346020206897 0.8
-0.7 0.945682140027573
-0.593075667080691 1.1
-0.4 1.30354675391036
-0.335047344159964 1.4
-0.1 1.6944777181404
-0.0959299737879746 1.7
0.144042790322979 2
0.2 2.07017436717603
0.39340298793235 2.3
0.5 2.43017059648522
0.654303283594219 2.6
0.8 2.77440082648581
0.918884820758215 2.9
1.1 3.10590438181471
1.19277143964126 3.2
1.4 3.42420372707997
1.47698864252986 3.5
1.7 3.73434793503732
1.7692000380693 3.8
2 4.03353472875555
2.07482200028238 4.1
2.3 4.31549625829081
2.40565046192547 4.4
2.6 4.56905162552453
2.79131029999639 4.7
2.9 4.78051983232811
3.2 4.9446311259962
3.31686089441833 5
3.2 5
2.9 5
2.6 5
2.3 5
2.22671768387992 5
2 4.75647909067455
1.95203619426201 4.7
1.7 4.41413629871771
1.68858175812974 4.4
1.43582941144356 4.1
1.4 4.05982957649237
1.19116264011306 3.8
1.1 3.69540776267712
0.947362498829797 3.5
0.8 3.32730802863878
0.703380242314739 3.2
0.5 2.94407080882945
0.468910428146778 2.9
0.235340688553063 2.6
0.2 2.55758936712225
-0.00575025364131102 2.3
-0.1 2.18383556344031
-0.264870209531329 2
-0.4 1.8477615932449
-0.587951796883488 1.7
-0.7 1.6018097573662
-1 1.47061487646979
-1 1.4
-1 1.1
-1 0.8
-1 0.694309397762023
-0.907346020206897 0.8
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
-0.7 -1
-0.4 -1
-0.1 -1
0.2 -1
0.268395607739889 -1
0.2 -0.906177363507018
0.0689963743774549 -0.7
-0.0747239951346661 -0.4
-0.1 -0.32983176993201
-0.186005073687891 -0.1
-0.243845426932723 0.2
-0.242439047774581 0.5
-0.175158616383199 0.8
-0.1 0.967282165178523
-0.0432249222786887 1.1
0.137165649537709 1.4
0.2 1.48773019474995
0.365969146691282 1.7
0.5 1.86352847931864
0.628672589800318 2
0.8 2.18464528112534
0.923371280417481 2.3
1.1 2.47360621029566
1.24505842155773 2.6
1.4 2.74516122552749
1.58671743211183 2.9
1.7 3.00189164015037
1.95425373659948 3.2
2 3.23884769296788
2.3 3.44569552155432
2.39135806079258 3.5
2.6 3.62655513929784
2.8931643931249 3.8
2.9 3.80392433949111
3.2 4.00826195610462
3.31746948768166 4.1
3.5 4.23359649298687
3.70794200368467 4.4
3.8 4.47052333898182
4.08567399811956 4.7
4.1 4.7112034575988
4.4 4.95321075279906
4.45588585707945 5
4.4 5
4.1 5
3.8 5
3.5 5
3.31686089441833 5
3.2 4.9446311259962
2.9 4.78051983232811
2.79131029999639 4.7
2.6 4.56905162552452
2.40565046192547 4.4
2.3 4.31549625829081
2.07482200028238 4.1
2 4.03353472875555
1.7692000380693 3.8
1.7 3.73434793503732
1.47698864252986 3.5
1.4 3.42420372707997
1.19277143964126 3.2
1.1 3.10590438181471
0.918884820758215 2.9
0.8 2.77440082648581
0.654303283594219 2.6
0.5 2.43017059648522
0.39340298793235 2.3
0.2 2.07017436717603
0.144042790322979 2
-0.0959299737879746 1.7
-0.1 1.6944777181404
-0.335047344159964 1.4
-0.4 1.30354675391036
-0.593075667080691 1.1
-0.7 0.945682140027573
-0.907346020206897 0.8
-1 0.694309397762023
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
2.9 -1
3.2 -1
3.5 -1
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.5
5 0.8
5 1.1
5 1.4
5 1.67149131170933
4.77196489614067 1.4
4.7 1.31426508296954
4.5194368379357 1.1
4.4 0.958114041470301
4.26598852127289 0.8
4.1 0.603802089867659
4.01114603183875 0.5
3.8 0.252626251919584
3.75418473674192 0.2
3.5 -0.0932011296803449
3.49390934201943 -0.1
3.23962436774244 -0.4
3.2 -0.446114938574731
2.97051454041684 -0.7
2.9 -0.774529811008731
2.66786576332552 -1
2.9 -1
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
0.2 -0.906177363507018
0.268395607739889 -1
0.5 -1
0.8 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.3 -1
2.6 -1
2.66786576332552 -1
2.9 -0.774529811008731
2.97051454041684 -0.7
3.2 -0.446114938574731
3.23962436774244 -0.4
3.49390934201943 -0.1
3.5 -0.0932011296803449
3.75418473674192 0.2
3.8 0.252626251919584
4.01114603183875 0.5
4.1 0.603802089867659
4.26598852127289 0.8
4.4 0.958114041470301
4.5194368379357 1.1
4.7 1.31426508296954
4.77196489614067 1.4
5 1.67149131170933
5 1.7
5 2
5 2.3
5 2.48288950145648
4.83489560484037 2.3
4.7 2.15058689633669
4.5636936575929 2
4.4 1.819184079394
4.29161635008209 1.7
4.1 1.48934122913492
4.01810297511227 1.4
3.8 1.16216105722075
3.74223872047861 1.1
3.5 0.839438043093628
3.46250703437472 0.8
3.2 0.523999773861243
3.17630163610119 0.5
2.9 0.220135099958207
2.87883417099557 0.2
2.6 -0.065903815241828
2.56026466207357 -0.1
2.3 -0.32523221046621
2.19645969950322 -0.4
2 -0.544948165524335
1.70908707471418 -0.7
1.7 -0.705051411070933
1.4 -0.789272567808442
1.1 -0.769037950221358
0.956942011932639 -0.7
0.8 -0.609098133104576
0.609069676713853 -0.4
0.5 -0.235754568918795
0.433885399128197 -0.1
0.347266291329367 0.2
0.329992272692239 0.5
0.389872613941067 0.8
0.5 1.05406773902187
0.526524124131536 1.1
0.761558691128087 1.4
0.8 1.44305540626704
1.08699717486163 1.7
1.1 1.71146700002849
1.4 1.92076955631912
1.52955422228205 2
1.7 2.10459402390023
2 2.28416847430162
2.02217965831132 2.3
2.3 2.48408552066446
2.44740650400265 2.6
2.6 2.71180353375187
2.82528905682054 2.9
2.9 2.95910242212003
3.18225738061835 3.2
3.2 3.21463891713398
3.5 3.46815803835583
3.5376876194921 3.5
3.8 3.71820112499239
3.8967366516131 3.8
4.1 3.96847366269511
4.25413111321935 4.1
4.4 4.22192842381034
4.60627798016336 4.4
4.7 4.47950525121164
4.95289884777972 4.7
5 4.74054788420939
5 5
4.7 5
4.45588585707945 5
4.4 4.95321075279906
4.1 4.7112034575988
4.08567399811956 4.7
3.8 4.47052333898182
3.70794200368467 4.4
3.5 4.23359649298687
3.31746948768166 4.1
3.2 4.00826195610462
2.9 3.80392433949111
2.8931643931249 3.8
2.6 3.62655513929784
2.39135806079258 3.5
2.3 3.44569552155432
2 3.23884769296788
1.95425373659948 3.2
1.7 3.00189164015037
1.58671743211183 2.9
1.4 2.74516122552749
1.24505842155773 2.6
1.1 2.47360621029566
0.923371280417481 2.3
0.8 2.18464528112534
0.628672589800318 2
0.5 1.86352847931864
0.365969146691282 1.7
0.2 1.48773019474995
0.137165649537709 1.4
-0.0432249222786887 1.1
-0.1 0.967282165178523
-0.175158616383199 0.8
-0.242439047774581 0.5
-0.243845426932723 0.2
-0.186005073687891 -0.1
-0.1 -0.32983176993201
-0.0747239951346661 -0.4
0.0689963743774549 -0.7
0.2 -0.906177363507018
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.1 -0.769037950221358
1.4 -0.789272567808442
1.7 -0.705051411070933
1.70908707471418 -0.7
2 -0.544948165524335
2.19645969950322 -0.4
2.3 -0.325232210466211
2.56026466207357 -0.1
2.6 -0.065903815241828
2.87883417099557 0.2
2.9 0.220135099958207
3.17630163610119 0.5
3.2 0.523999773861243
3.46250703437472 0.8
3.5 0.839438043093628
3.74223872047861 1.1
3.8 1.16216105722075
4.01810297511227 1.4
4.1 1.48934122913492
4.29161635008209 1.7
4.4 1.819184079394
4.5636936575929 2
4.7 2.15058689633669
4.83489560484037 2.3
5 2.48288950145648
5 2.6
5 2.9
5 3.2
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 4.74054788420939
4.95289884777972 4.7
4.7 4.47950525121164
4.60627798016336 4.4
4.4 4.22192842381034
4.25413111321935 4.1
4.1 3.96847366269511
3.8967366516131 3.8
3.8 3.71820112499239
3.5376876194921 3.5
3.5 3.46815803835583
3.2 3.21463891713398
3.18225738061835 3.2
2.9 2.95910242212003
2.82528905682054 2.9
2.6 2.71180353375187
2.44740650400265 2.6
2.3 2.48408552066446
2.02217965831132 2.3
2 2.28416847430162
1.7 2.10459402390023
1.52955422228205 2
1.4 1.92076955631912
1.1 1.71146700002849
1.08699717486163 1.7
0.8 1.44305540626704
0.761558691128087 1.4
0.526524124131536 1.1
0.5 1.05406773902187
0.389872613941067 0.8
0.329992272692239 0.5
0.347266291329367 0.2
0.433885399128197 -0.1
0.5 -0.235754568918795
0.609069676713853 -0.4
0.8 -0.609098133104576
0.956942011932639 -0.7
1.1 -0.769037950221358

1.50806690178828 0.5
1.64369055782157 0.8
1.7 0.855631866474338
1.9233144694474 1.1
2 1.16515509030378
2.24613268715144 1.4
2.3 1.44543079299295
2.58250997818986 1.7
2.6 1.71484665702472
2.9 1.95768179938965
2.95490446652596 2
3.2 2.18044241711861
3.36177470801188 2.3
3.5 2.39867390964995
3.777612100037 2.6
3.8 2.61581430137849
4.01752526981514 2.6
3.87658911982046 2.3
3.8 2.19587318863797
3.65465140263952 2
3.5 1.79700240778064
3.42496444872409 1.7
3.2 1.42118280742365
3.18244877908787 1.4
2.90907634007114 1.1
2.9 1.09059306849117
2.60648041753145 0.8
2.6 0.79384593594509
2.3 0.552205045241832
2.22340057947646 0.5
2 0.372524281433893
1.7 0.294984844072629
1.50806690178828 0.5
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
1.7 0.294984844072629
2 0.372524281433893
2.22340057947646 0.5
2.3 0.552205045241832
2.6 0.79384593594509
2.60648041753145 0.8
2.9 1.09059306849117
2.90907634007114 1.1
3.18244877908787 1.4
3.2 1.42118280742365
3.42496444872409 1.7
3.5 1.79700240778064
3.65465140263952 2
3.8 2.19587318863797
3.87658911982046 2.3
4.01752526981514 2.6
3.8 2.61581430137849
3.777612100037 2.6
3.5 2.39867390964995
3.36177470801188 2.3
3.2 2.18044241711861
2.95490446652596 2
2.9 1.95768179938965
2.6 1.71484665702472
2.58250997818986 1.7
2.3 1.44543079299295
2.24613268715144 1.4
2 1.16515509030378
1.9233144694474 1.1
1.7 0.855631866474338
1.64369055782157 0.8
1.50806690178828 0.5
1.7 0.294984844072629
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.3 1.1
};
\coordinate (CVI_mean_lml_t) at (axis cs:2.3,1.1);
\end{axis}



==> fig/tikz/echocardiogram/CVI_mean_lml_ep.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
-0.7 3.04472856709636
-0.694249777301187 3.2
-0.690851197804852 3.5
-0.685855692790104 3.8
-0.678938572726975 4.1
-0.678524766354408 4.4
-0.681554184854981 4.7
-0.685709903423596 5
-0.7 5
-0.761088990234973 5
-0.776521273448877 4.7
-0.789231483055611 4.4
-0.790721460054847 4.1
-0.771648747631824 3.8
-0.749683827232119 3.5
-0.73108879759604 3.2
-0.7 3.04472856709636
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
-0.7 -1
-0.4 -1
-0.1 -1
0.2 -1
0.268293315811215 -1
0.2 -0.906510069487696
0.0685033529112634 -0.7
-0.0768628795683596 -0.4
-0.1 -0.339617836447615
-0.19549178659847 -0.1
-0.27411406075025 0.2
-0.323188285836026 0.5
-0.352416118768839 0.8
-0.366896192034489 1.1
-0.367347195590322 1.4
-0.358257288002007 1.7
-0.349156994251774 2
-0.344468556977903 2.3
-0.343709068873184 2.6
-0.348244020201829 2.9
-0.348332596458776 3.2
-0.344126146459131 3.5
-0.351625063261929 3.8
-0.349511169515405 4.1
-0.342607922283778 4.4
-0.321246377758405 4.7
-0.301580567422848 5
-0.4 5
-0.685709903423596 5
-0.681554184854981 4.7
-0.678524766354408 4.4
-0.678938572726975 4.1
-0.685855692790104 3.8
-0.690851197804852 3.5
-0.694249777301187 3.2
-0.7 3.04472856709636
-0.73108879759604 3.2
-0.749683827232119 3.5
-0.771648747631824 3.8
-0.790721460054847 4.1
-0.789231483055611 4.4
-0.776521273448877 4.7
-0.761088990234973 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
2.9 -1
3.2 -1
3.5 -1
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.5
5 0.8
5 1.1
5 1.4
5 1.67148168466376
4.77197211269935 1.4
4.7 1.31425680404046
4.51944312023923 1.1
4.4 0.958107099086874
4.26599388247292 0.8
4.1 0.603796457738
4.01115049801081 0.5
3.8 0.252621874874822
3.75418835780717 0.2
3.5 -0.0932043592057104
3.49391220878338 -0.1
3.23962788021882 -0.4
3.2 -0.446118944921083
2.97051757194983 -0.7
2.9 -0.774532921548428
2.66786842001734 -1
2.9 -1
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
2.6 4.38754300678726
2.9 4.1560910867374
3.2 4.20819566776974
3.5 4.29697729921591
3.64200337616563 4.4
3.8 4.51212748893161
4.03382894132823 4.7
4.1 4.75224752361588
4.4 4.98633659713012
4.4165784013335 5
4.4 5
4.1 5
3.8 5
3.5 5
3.2 5
2.9 5
2.6 5
2.3 5
2.0166228554916 5
2.29804600560016 4.7
2.3 4.69854838052913
2.59221457233822 4.4
2.6 4.38754300678726
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
0.2 -0.906510069487696
0.268293315811215 -1
0.5 -1
0.8 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.3 -1
2.6 -1
2.66786842001734 -1
2.9 -0.774532921548428
2.97051757194983 -0.7
3.2 -0.446118944921083
3.23962788021882 -0.4
3.49391220878338 -0.1
3.5 -0.0932043592057104
3.75418835780717 0.2
3.8 0.252621874874822
4.01115049801081 0.5
4.1 0.603796457738
4.26599388247292 0.8
4.4 0.958107099086874
4.51944312023923 1.1
4.7 1.31425680404046
4.77197211269935 1.4
5 1.67148168466376
5 1.7
5 2
5 2.3
5 2.48273937124412
4.83502381001981 2.3
4.7 2.15045155169637
4.56381019860687 2
4.4 1.81906329133182
4.29172153604363 1.7
4.1 1.48923461515481
4.01819726987043 1.4
3.8 1.16206797616468
3.74232283989659 1.1
3.5 0.839357412469893
3.46258214404984 0.8
3.2 0.523929774781293
3.17636972282641 0.5
2.9 0.220072826910376
2.87889858654591 0.2
2.6 -0.0659623566171611
2.5603306342256 -0.1
2.3 -0.325290845793044
2.19653496639187 -0.4
2 -0.545007665905787
1.7091872645202 -0.7
1.7 -0.705107354542225
1.4 -0.789362495248651
1.1 -0.7692180900417
0.956365933768474 -0.7
0.8 -0.6099250205256
0.607021305913303 -0.4
0.5 -0.244428950680805
0.426879990086966 -0.1
0.321734253688921 0.2
0.255713244407407 0.5
0.219535378479618 0.8
0.205417229166258 1.1
0.211198552521702 1.4
0.240482478409022 1.7
0.288659351362879 2
0.335989529210535 2.3
0.373603973254495 2.6
0.399967060025626 2.9
0.414694879018706 3.2
0.430030606176207 3.5
0.439100786706575 3.8
0.435210988899999 4.1
0.43878796808782 4.4
0.461753847883229 4.7
0.464393395996721 5
0.2 5
-0.1 5
-0.301580567422848 5
-0.321246377758405 4.7
-0.342607922283778 4.4
-0.349511169515405 4.1
-0.351625063261929 3.8
-0.344126146459131 3.5
-0.348332596458776 3.2
-0.348244020201829 2.9
-0.343709068873184 2.6
-0.344468556977903 2.3
-0.349156994251774 2
-0.358257288002007 1.7
-0.367347195590322 1.4
-0.366896192034489 1.1
-0.352416118768839 0.8
-0.323188285836026 0.5
-0.27411406075025 0.2
-0.19549178659847 -0.1
-0.1 -0.339617836447615
-0.0768628795683596 -0.4
0.0685033529112634 -0.7
0.2 -0.906510069487696
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.1 2.83444345396014
1.39745914010686 2.9
1.4 2.90056633947562
1.40604492654922 2.9
1.7 2.86938083689707
2 2.74367678674568
2.3 2.69299764080089
2.6 2.81236823457615
2.71777531575429 2.9
2.9 3.02901831778416
3.11120299846648 3.2
3.2 3.26796083789855
3.49156153769966 3.5
3.5 3.50611696605296
3.8 3.74159685800089
3.87028019172195 3.8
4.1 3.98360167007488
4.23769088643773 4.1
4.4 4.23344981985688
4.5938803633525 4.4
4.7 4.48939411342708
4.94217529313736 4.7
5 4.7496233842659
5 5
4.7 5
4.4165784013335 5
4.4 4.98633659713012
4.1 4.75224752361588
4.03382894132823 4.7
3.8 4.51212748893161
3.64200337616563 4.4
3.5 4.29697729921591
3.2 4.20819566776974
2.9 4.1560910867374
2.6 4.38754300678726
2.59221457233822 4.4
2.3 4.69854838052913
2.29804600560016 4.7
2.0166228554916 5
2 5
1.7 5
1.4 5
1.1 5
0.8 5
0.566705395996062 5
0.571507037237621 4.7
0.644485913333756 4.4
0.686918766037016 4.1
0.737694863186255 3.8
0.8 3.60138110321543
0.816535174394114 3.5
0.892065642697614 3.2
1.0519708779359 2.9
1.1 2.83444345396014
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.1 -0.7692180900417
1.4 -0.789362495248651
1.7 -0.705107354542225
1.7091872645202 -0.7
2 -0.545007665905787
2.19653496639187 -0.4
2.3 -0.325290845793044
2.5603306342256 -0.1
2.6 -0.0659623566171611
2.87889858654591 0.2
2.9 0.220072826910376
3.17636972282641 0.5
3.2 0.523929774781293
3.46258214404984 0.8
3.5 0.839357412469893
3.74232283989659 1.1
3.8 1.16206797616468
4.01819726987043 1.4
4.1 1.48923461515481
4.29172153604363 1.7
4.4 1.81906329133182
4.56381019860687 2
4.7 2.15045155169637
4.83502381001981 2.3
5 2.48273937124412
5 2.6
5 2.9
5 3.2
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 4.7496233842659
4.94217529313736 4.7
4.7 4.48939411342708
4.5938803633525 4.4
4.4 4.23344981985688
4.23769088643773 4.1
4.1 3.98360167007488
3.87028019172195 3.8
3.8 3.74159685800089
3.5 3.50611696605296
3.49156153769966 3.5
3.2 3.26796083789855
3.11120299846648 3.2
2.9 3.02901831778416
2.71777531575429 2.9
2.6 2.81236823457615
2.3 2.69299764080089
2 2.74367678674568
1.7 2.86938083689707
1.40604492654922 2.9
1.4 2.90056633947562
1.39745914010686 2.9
1.1 2.83444345396014
1.0519708779359 2.9
0.892065642697614 3.2
0.816535174394114 3.5
0.8 3.60138110321543
0.737694863186255 3.8
0.686918766037016 4.1
0.644485913333755 4.4
0.571507037237621 4.7
0.566705395996062 5
0.5 5
0.464393395996721 5
0.461753847883229 4.7
0.43878796808782 4.4
0.435210988899999 4.1
0.439100786706575 3.8
0.430030606176207 3.5
0.414694879018706 3.2
0.399967060025626 2.9
0.373603973254495 2.6
0.335989529210535 2.3
0.288659351362879 2
0.240482478409023 1.7
0.211198552521702 1.4
0.205417229166258 1.1
0.219535378479618 0.8
0.255713244407407 0.5
0.321734253688921 0.2
0.426879990086966 -0.1
0.5 -0.244428950680805
0.607021305913303 -0.4
0.8 -0.6099250205256
0.956365933768474 -0.7
1.1 -0.7692180900417

1.45418883273977 0.5
1.57294490133436 0.8
1.7 0.928505246479521
1.85356392993428 1.1
2 1.21825863732594
2.19487099765071 1.4
2.3 1.48331316452727
2.54822543974618 1.7
2.6 1.74138967228703
2.9 1.98909500396889
2.91453658943567 2
3.2 2.20157220456237
3.33607333886538 2.3
3.5 2.41343146114979
3.76135459879511 2.6
3.8 2.62670768840921
4.09729041130077 2.6
3.88198411002012 2.3
3.8 2.18890865218268
3.65951989396601 2
3.5 1.79125805195532
3.42931321345837 1.7
3.2 1.41652489836532
3.18630515492982 1.4
2.91102542161836 1.1
2.9 1.088575142241
2.60855832096951 0.8
2.6 0.791872097107612
2.3 0.54808653860446
2.22985748610981 0.5
2 0.367714853000783
1.7 0.279134421605945
1.45418883273977 0.5
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
1.7 0.279134421605945
2 0.367714853000783
2.22985748610981 0.5
2.3 0.54808653860446
2.6 0.791872097107612
2.60855832096951 0.8
2.9 1.088575142241
2.91102542161836 1.1
3.18630515492982 1.4
3.2 1.41652489836532
3.42931321345837 1.7
3.5 1.79125805195532
3.65951989396601 2
3.8 2.18890865218268
3.88198411002012 2.3
4.09729041130077 2.6
3.8 2.62670768840921
3.76135459879511 2.6
3.5 2.41343146114979
3.33607333886538 2.3
3.2 2.20157220456237
2.91453658943567 2
2.9 1.98909500396889
2.6 1.74138967228703
2.54822543974618 1.7
2.3 1.48331316452727
2.19487099765071 1.4
2 1.21825863732594
1.85356392993428 1.1
1.7 0.928505246479521
1.57294490133436 0.8
1.45418883273977 0.5
1.7 0.279134421605945
};
\addplot [semithick, steelblue31119180, mark=mystar, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.3 1.1
};
\coordinate (CVI_mean_lml_ep_t) at (axis cs:2.3,1.1);
\end{axis}



==> fig/tikz/echocardiogram/CVI_nlpd.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
-0.7 -1
-0.4 -1
-0.1 -1
-0.0960640846782714 -1
-0.1 -0.991042838351951
-0.246798567458487 -0.7
-0.344821707827058 -0.4
-0.4 -0.158009648445284
-0.420551954827308 -0.1
-0.497295139914373 0.2
-0.541717810080686 0.5
-0.567139108039384 0.8
-0.57855917829852 1.1
-0.570591010421648 1.4
-0.542780262517072 1.7
-0.513833056519028 2
-0.496555109447484 2.3
-0.488673871844748 2.6
-0.492386632820635 2.9
-0.485637948105897 3.2
-0.470657956390004 3.5
-0.470714822223526 3.8
-0.47664937963605 4.1
-0.472114855455648 4.4
-0.46803203957881 4.7
-0.467077531768038 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
-0.1 -0.991042838351951
-0.0960640846782714 -1
0.2 -1
0.264173755190023 -1
0.2 -0.900474599309181
0.0901964040792849 -0.7
-0.0376315166470436 -0.4
-0.1 -0.211092002877031
-0.139141172020734 -0.1
-0.213235860192094 0.2
-0.258805583114065 0.5
-0.286253245249645 0.8
-0.301573408226686 1.1
-0.305245163814661 1.4
-0.298952559186939 1.7
-0.290634319651496 2
-0.284103734122101 2.3
-0.279572916910372 2.6
-0.278717957208294 2.9
-0.269824941943889 3.2
-0.259772181722104 3.5
-0.260173568095416 3.8
-0.266724650261333 4.1
-0.262833082315341 4.4
-0.255515706818434 4.7
-0.251359003457331 5
-0.4 5
-0.467077531768038 5
-0.46803203957881 4.7
-0.472114855455648 4.4
-0.47664937963605 4.1
-0.470714822223526 3.8
-0.470657956390004 3.5
-0.485637948105897 3.2
-0.492386632820635 2.9
-0.488673871844748 2.6
-0.496555109447484 2.3
-0.513833056519028 2
-0.542780262517072 1.7
-0.570591010421648 1.4
-0.57855917829852 1.1
-0.567139108039384 0.8
-0.541717810080686 0.5
-0.497295139914373 0.2
-0.420551954827308 -0.1
-0.4 -0.158009648445284
-0.344821707827058 -0.4
-0.246798567458487 -0.7
-0.1 -0.991042838351951
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
4.4 -1
4.7 -1
5 -1
5 -0.900589241679459
4.7 -0.932499092566007
4.4 -0.981035396435341
4.32395820675979 -1
4.4 -1
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
0.2 -0.900474599309181
0.264173755190023 -1
0.5 -1
0.653077614726839 -1
0.5 -0.852595046760952
0.396751519581127 -0.7
0.220246209843443 -0.4
0.2 -0.358982464203837
0.100272258940224 -0.1
0.019379771539017 0.2
-0.033529236310015 0.5
-0.0666352315002485 0.8
-0.087451576452196 1.1
-0.099685634551054 1.4
-0.1 1.42251931701655
-0.103399139324262 1.7
-0.102692234583129 2
-0.1 2.23404065316463
-0.0990383038537562 2.3
-0.0931732823465917 2.6
-0.0805849700739403 2.9
-0.0647679532483115 3.2
-0.0562610295651628 3.5
-0.0572820823188441 3.8
-0.0700404776133499 4.1
-0.0650653101652566 4.4
-0.0487941356490163 4.7
-0.039616165897567 5
-0.1 5
-0.251359003457331 5
-0.255515706818434 4.7
-0.262833082315341 4.4
-0.266724650261333 4.1
-0.260173568095416 3.8
-0.259772181722104 3.5
-0.269824941943889 3.2
-0.278717957208294 2.9
-0.279572916910372 2.6
-0.284103734122101 2.3
-0.290634319651496 2
-0.298952559186939 1.7
-0.305245163814661 1.4
-0.301573408226686 1.1
-0.286253245249645 0.8
-0.258805583114065 0.5
-0.213235860192094 0.2
-0.139141172020734 -0.1
-0.1 -0.211092002877032
-0.0376315166470436 -0.4
0.0901964040792849 -0.7
0.2 -0.900474599309181
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
2.3 -1
2.6 -1
2.9 -1
3.2 -1
3.5 -1
3.8 -1
4.1 -1
4.32395820675979 -1
4.4 -0.981035396435341
4.7 -0.932499092566007
5 -0.900589241679459
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.5
5 0.8
5 1.1
5 1.4
5 1.58862061267317
4.81073981655369 1.4
4.7 1.2896267864774
4.50922181631008 1.1
4.4 0.991428088762524
4.20649854315688 0.8
4.1 0.694636756413177
3.90161660704114 0.5
3.8 0.400317317252088
3.59284629992602 0.2
3.5 0.110297423827661
3.27696678387975 -0.1
3.2 -0.172345885554653
2.94767927624081 -0.4
2.9 -0.442625740797708
2.6 -0.694486043405224
2.59288549942659 -0.7
2.3 -0.927607973872394
2.186100206942 -1
2.3 -1
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
0.5 -0.852595046760952
0.653077614726839 -1
0.8 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.186100206942 -1
2.3 -0.927607973872394
2.59288549942659 -0.7
2.6 -0.694486043405224
2.9 -0.442625740797708
2.94767927624081 -0.4
3.2 -0.172345885554653
3.27696678387975 -0.1
3.5 0.110297423827661
3.59284629992602 0.2
3.8 0.400317317252088
3.90161660704114 0.5
4.1 0.694636756413177
4.20649854315688 0.8
4.4 0.991428088762524
4.50922181631008 1.1
4.7 1.2896267864774
4.81073981655369 1.4
5 1.58862061267317
5 1.7
5 2
5 2.16898556741552
4.83053963709092 2
4.7 1.8697855564035
4.5293614762248 1.7
4.4 1.57121326359655
4.22725639765252 1.4
4.1 1.27374534663523
3.92350726304195 1.1
3.8 0.978201138877553
3.6168437712715 0.8
3.5 0.68596751363116
3.30499050174841 0.5
3.2 0.399350481064787
2.98376128863404 0.2
2.9 0.122109429283298
2.64503546379759 -0.1
2.6 -0.139758370459814
2.3 -0.378748742620408
2.26881934618225 -0.4
2 -0.586000421030039
1.7779886986411 -0.7
1.7 -0.740567242134103
1.4 -0.824456572329459
1.1 -0.812407787891593
0.849783768912269 -0.7
0.8 -0.676366594211474
0.532451868677349 -0.4
0.5 -0.361200686773264
0.367852298170217 -0.1
0.25519395964755 0.2
0.2 0.422617865569531
0.185443451913083 0.5
0.151683918713466 0.8
0.132388904913179 1.1
0.123162394505602 1.4
0.122267235649904 1.7
0.127247883444105 2
0.139173881223846 2.3
0.152653261703993 2.6
0.169644609938675 2.9
0.2 3.19606024010452
0.200342435047642 3.2
0.223202013559864 3.5
0.226928295745223 3.8
0.220571340768798 4.1
0.22256593598869 4.4
0.226897671386788 4.7
0.227040000994463 5
0.2 5
-0.039616165897567 5
-0.0487941356490163 4.7
-0.0650653101652566 4.4
-0.0700404776133499 4.1
-0.0572820823188441 3.8
-0.0562610295651628 3.5
-0.0647679532483115 3.2
-0.0805849700739403 2.9
-0.0931732823465917 2.6
-0.0990383038537562 2.3
-0.1 2.23404065316463
-0.102692234583129 2
-0.103399139324262 1.7
-0.1 1.42251931701655
-0.099685634551054 1.4
-0.0874515764521961 1.1
-0.0666352315002485 0.8
-0.033529236310015 0.5
0.019379771539017 0.2
0.100272258940224 -0.1
0.2 -0.358982464203837
0.220246209843443 -0.4
0.396751519581127 -0.7
0.5 -0.852595046760952
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
1.1 -0.812407787891593
1.4 -0.824456572329459
1.7 -0.740567242134103
1.7779886986411 -0.7
2 -0.586000421030039
2.26881934618225 -0.4
2.3 -0.378748742620408
2.6 -0.139758370459814
2.64503546379759 -0.1
2.9 0.122109429283298
2.98376128863404 0.2
3.2 0.399350481064787
3.30499050174841 0.5
3.5 0.68596751363116
3.6168437712715 0.8
3.8 0.978201138877553
3.92350726304195 1.1
4.1 1.27374534663523
4.22725639765252 1.4
4.4 1.57121326359655
4.5293614762248 1.7
4.7 1.8697855564035
4.83053963709092 2
5 2.16898556741552
5 2.3
5 2.6
5 2.64805279768873
4.95183414331762 2.6
4.7 2.34888922103845
4.65090311447654 2.3
4.4 2.05038442835939
4.34922979921354 2
4.1 1.753040451615
4.04622870256029 1.7
3.8 1.45771874038069
3.74085261171886 1.4
3.5 1.16586586078092
3.43121217933579 1.1
3.2 0.879840198426633
3.11382782686308 0.8
2.9 0.603341605896553
2.78202272027186 0.5
2.6 0.341917136994091
2.42199158644405 0.2
2.3 0.103522123699517
2.00115521432348 -0.1
2 -0.100782711612921
1.7 -0.247673802178763
1.4 -0.326849101834872
1.1 -0.305969933903133
0.8 -0.142439805814336
0.764483928398994 -0.1
0.571466822293433 0.2
0.5 0.373780327052863
0.4683181276476 0.5
0.425699063863688 0.8
0.404127884408714 1.1
0.393964401139089 1.4
0.388535691693733 1.7
0.382846253562493 2
0.380963680188802 2.3
0.382836419840007 2.6
0.391142442111076 2.9
0.412467197373724 3.2
0.429292693740961 3.5
0.431761136118828 3.8
0.430037045434788 4.1
0.430591667670954 4.4
0.431652208531058 4.7
0.431696512745468 5
0.227040000994463 5
0.226897671386788 4.7
0.22256593598869 4.4
0.220571340768798 4.1
0.226928295745223 3.8
0.223202013559864 3.5
0.200342435047642 3.2
0.2 3.19606024010452
0.169644609938675 2.9
0.152653261703993 2.6
0.139173881223846 2.3
0.127247883444105 2
0.122267235649904 1.7
0.123162394505602 1.4
0.132388904913179 1.1
0.151683918713466 0.8
0.185443451913083 0.5
0.2 0.422617865569531
0.25519395964755 0.2
0.367852298170217 -0.1
0.5 -0.361200686773264
0.532451868677349 -0.4
0.8 -0.676366594211474
0.849783768912269 -0.7
1.1 -0.812407787891593
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
0.8 -0.142439805814336
1.1 -0.305969933903133
1.4 -0.326849101834872
1.7 -0.247673802178763
2 -0.100782711612921
2.00115521432348 -0.1
2.3 0.103522123699517
2.42199158644405 0.2
2.6 0.341917136994091
2.78202272027186 0.5
2.9 0.603341605896553
3.11382782686308 0.8
3.2 0.879840198426633
3.43121217933579 1.1
3.5 1.16586586078092
3.74085261171886 1.4
3.8 1.45771874038069
4.04622870256029 1.7
4.1 1.753040451615
4.34922979921354 2
4.4 2.05038442835939
4.65090311447654 2.3
4.7 2.34888922103845
4.95183414331762 2.6
5 2.64805279768873
5 2.9
5 3.2
5 3.21096141961589
4.98904757211163 3.2
4.7 2.9115279596125
4.68848436126867 2.9
4.4 2.61258677200566
4.38742491205732 2.6
4.1 2.31457634194313
4.08541446048232 2.3
3.8 2.01832543409149
3.78156347362882 2
3.5 1.72536666879801
3.47411557875155 1.7
3.2 1.43841198918997
3.15955834480493 1.4
2.9 1.16193048489211
2.83070322643501 1.1
2.6 0.902570961883835
2.47211006805144 0.8
2.3 0.668956764218275
2.04682503678103 0.5
2 0.470594301582375
1.7 0.342505756673426
1.4 0.291836653643006
1.1 0.380567273609099
0.989374229385994 0.5
0.842375239529694 0.8
0.8 1.04362962114236
0.794045955613396 1.1
0.787424542190501 1.4
0.790359310764733 1.7
0.79635114977393 2
0.8 2.0627595976291
0.821762840699565 2.3
0.889936806378718 2.6
0.979326297566991 2.9
1.05726773585402 3.2
1.1 3.39953954975219
1.13504100406128 3.5
1.18911294828195 3.8
1.25298047422168 4.1
1.4 4.38198876175403
1.40752390836937 4.4
1.7 4.66837922007786
1.71217822893114 4.7
1.80063071813257 5
1.7 5
1.4 5
1.1 5
0.8 5
0.5 5
0.431696512745468 5
0.431652208531057 4.7
0.430591667670954 4.4
0.430037045434788 4.1
0.431761136118828 3.8
0.429292693740961 3.5
0.412467197373724 3.2
0.391142442111076 2.9
0.382836419840007 2.6
0.380963680188802 2.3
0.382846253562493 2
0.388535691693733 1.7
0.393964401139089 1.4
0.404127884408714 1.1
0.425699063863688 0.8
0.4683181276476 0.5
0.5 0.373780327052863
0.571466822293433 0.2
0.764483928398994 -0.1
0.8 -0.142439805814336
};
\addplot [draw=none, fill=lavender231240249]
table{%
x  y
1.1 0.380567273609099
1.4 0.291836653643006
1.7 0.342505756673426
2 0.470594301582375
2.04682503678103 0.5
2.3 0.668956764218275
2.47211006805144 0.8
2.6 0.902570961883835
2.83070322643501 1.1
2.9 1.16193048489211
3.15955834480493 1.4
3.2 1.43841198918997
3.47411557875155 1.7
3.5 1.72536666879801
3.78156347362882 2
3.8 2.01832543409149
4.08541446048232 2.3
4.1 2.31457634194313
4.38742491205732 2.6
4.4 2.61258677200566
4.68848436126867 2.9
4.7 2.9115279596125
4.98904757211163 3.2
5 3.21096141961589
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 4.7655461716343
4.95406563688856 4.7
4.70576491021499 4.4
4.7 4.39366871522421
4.46997215769218 4.1
4.4 4.02028339947142
4.23601806263988 3.8
4.1 3.63931800964441
3.99872775866845 3.5
3.8 3.25861582361758
3.75704985579745 3.2
3.51210671565661 2.9
3.5 2.88649551139607
3.26080232743953 2.6
3.2 2.5328809306829
2.99531013568962 2.3
2.9 2.19941826733545
2.70781295519952 2
2.6 1.89633322069977
2.37832739112353 1.7
2.3 1.63592866115438
2 1.44135734447986
1.80504027400491 1.4
1.7 1.37729307644334
1.67029336499831 1.4
1.53753689842311 1.7
1.54822445766363 2
1.60752969350882 2.3
1.69757578711824 2.6
1.7 2.605971779573
1.79896801133233 2.9
1.88981904233676 3.2
1.97443549275229 3.5
2 3.59572815150662
2.06774894451493 3.8
2.17261660859927 4.1
2.3 4.34420965068084
2.32443005414539 4.4
2.4370304944343 4.7
2.6 4.96668215590438
2.61407638718954 5
2.6 5
2.3 5
2 5
1.80063071813257 5
1.71217822893114 4.7
1.7 4.66837922007786
1.40752390836937 4.4
1.4 4.38198876175403
1.25298047422168 4.1
1.18911294828195 3.8
1.13504100406128 3.5
1.1 3.39953954975219
1.05726773585402 3.2
0.979326297566991 2.9
0.889936806378718 2.6
0.821762840699565 2.3
0.8 2.0627595976291
0.79635114977393 2
0.790359310764733 1.7
0.787424542190501 1.4
0.794045955613396 1.1
0.8 1.04362962114236
0.842375239529694 0.8
0.989374229385994 0.5
1.1 0.380567273609099
};
\addplot [draw=none, fill=aliceblue242247253]
table{%
x  y
1.7 1.37729307644334
1.80504027400491 1.4
2 1.44135734447986
2.3 1.63592866115438
2.37832739112353 1.7
2.6 1.89633322069977
2.70781295519952 2
2.9 2.19941826733545
2.99531013568962 2.3
3.2 2.5328809306829
3.26080232743953 2.6
3.5 2.88649551139607
3.51210671565661 2.9
3.75704985579745 3.2
3.8 3.25861582361758
3.99872775866845 3.5
4.1 3.63931800964441
4.23601806263988 3.8
4.4 4.02028339947142
4.46997215769218 4.1
4.7 4.39366871522421
4.70576491021499 4.4
4.95406563688856 4.7
5 4.7655461716343
5 5
4.7 5
4.4 5
4.1 5
3.8 5
3.56450089163773 5
3.5 4.86264045547939
3.37847168726413 5
3.2 5
2.9 5
2.61407638718954 5
2.6 4.96668215590438
2.4370304944343 4.7
2.32443005414539 4.4
2.3 4.34420965068084
2.17261660859927 4.1
2.06774894451493 3.8
2 3.59572815150662
1.97443549275229 3.5
1.88981904233676 3.2
1.79896801133233 2.9
1.7 2.605971779573
1.69757578711824 2.6
1.60752969350882 2.3
1.54822445766363 2
1.53753689842311 1.7
1.67029336499831 1.4
1.7 1.37729307644334
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.3 1.1
};
\addplot [semithick, darkorange25512714, mark=mystar, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.3 1.1
};
\draw (axis cs:2.5,1.1) node[
  scale=0.5,
  anchor=base west,
  text=black,
  rotate=0.0
]{$-0.292$};
\draw (axis cs:2.5,1.1) node[
  scale=0.5,
  anchor=base west,
  text=black,
  rotate=0.0
]{$-0.292$};
\coordinate (CVI_mean_lml_b) at (axis cs:2.3,1.1);
\coordinate (CVI_mean_lml_ep_b) at (axis cs:2.3,1.1);
\end{axis}



==> fig/tikz/echocardiogram/EP_mean_lml.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
-0.7 -1
-0.4 -1
-0.1 -1
0.2 -1
0.268292939884207 -1
0.2 -0.906510594865882
0.0685030154336713 -0.7
-0.0768636512609822 -0.4
-0.1 -0.339622589666428
-0.195497119011841 -0.1
-0.274143244282072 0.2
-0.323311001633873 0.5
-0.352968120050937 0.8
-0.370252292866661 1.1
-0.380083527025108 1.4
-0.385592259427553 1.7
-0.38865171522344 2
-0.390342209926183 2.3
-0.391273465972884 2.6
-0.391785388831005 2.9
-0.392066875865516 3.2
-0.392221627068755 3.5
-0.392306384613658 3.8
-0.39235303765231 4.1
-0.392378479532656 4.4
-0.392392623654814 4.7
-0.392400269774 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
2.9 -1
3.2 -1
3.5 -1
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.5
5 0.8
5 1.1
5 1.4
5 1.67148109734247
4.77197257990226 1.4
4.7 1.31425625719337
4.51944356060274 1.1
4.4 0.958106591812919
4.26599429746891 0.8
4.1 0.603795988433022
4.0111508901448 0.5
3.8 0.252621440680748
3.75418873116582 0.2
3.5 -0.0932047634041315
3.49391257033031 -0.1
3.23962838683779 -0.4
3.2 -0.446119532693112
2.97051809176038 -0.7
2.9 -0.774533477444157
2.66786901061023 -1
2.9 -1
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
2.9 4.24437242128823
3.2 4.20200995709489
3.5 4.33515592647703
3.59349341454494 4.4
3.8 4.53152203340247
4.02922642691753 4.7
4.1 4.74926454005825
4.4 4.97853640508017
4.42612198684368 5
4.4 5
4.1 5
3.8 5
3.5 5
3.2 5
2.9 5
2.6 5
2.59917841022755 5
2.6 4.99531593454156
2.66543007010996 4.7
2.78391444008821 4.4
2.9 4.24437242128823
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
0.2 -0.906510594865883
0.268292939884207 -1
0.5 -1
0.8 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.3 -1
2.6 -1
2.66786901061023 -1
2.9 -0.774533477444157
2.97051809176038 -0.7
3.2 -0.446119532693112
3.23962838683779 -0.4
3.49391257033031 -0.1
3.5 -0.0932047634041315
3.75418873116582 0.2
3.8 0.252621440680748
4.0111508901448 0.5
4.1 0.603795988433022
4.26599429746891 0.8
4.4 0.958106591812919
4.51944356060274 1.1
4.7 1.31425625719337
4.77197257990226 1.4
5 1.67148109734247
5 1.7
5 2
5 2.3
5 2.48273875332464
4.83502435984861 2.3
4.7 2.15045094965629
4.5638107368472 2
4.4 1.81906270504577
4.29172206368825 1.7
4.1 1.48923404436727
4.01819778870687 1.4
3.8 1.16206742102425
3.74232335235987 1.1
3.5 0.839356870315865
3.46258265698267 0.8
3.2 0.523929244409933
3.17637024472926 0.5
2.9 0.220072305627016
2.87889913264853 0.2
2.6 -0.0659628717756402
2.56033123098339 -0.1
2.3 -0.325291355605386
2.19653566455678 -0.4
2 -0.545008175763969
1.70918820646876 -0.7
1.7 -0.705107877959708
1.4 -0.789363010018514
1.1 -0.769218621435184
0.956364825374661 -0.7
0.8 -0.609925951071492
0.607019688018436 -0.4
0.5 -0.244439820596952
0.426870634736545 -0.1
0.321670339943832 0.2
0.255389096111849 0.5
0.218203262574804 0.8
0.200102909212405 1.1
0.2 1.10435308358953
0.194675690100441 1.4
0.193068833527311 1.7
0.192820179076064 2
0.192934632419146 2.3
0.193086600420306 2.6
0.193199470648732 2.9
0.193270949365836 3.2
0.19331290045631 3.5
0.19333775684845 3.8
0.193353416621008 4.1
0.193358486066187 4.4
0.193360631302794 4.7
0.193364504052925 5
-0.1 5
-0.392400269774 5
-0.392392623654814 4.7
-0.392378479532656 4.4
-0.39235303765231 4.1
-0.392306384613658 3.8
-0.392221627068755 3.5
-0.392066875865516 3.2
-0.391785388831005 2.9
-0.391273465972884 2.6
-0.390342209926183 2.3
-0.38865171522344 2
-0.385592259427553 1.7
-0.380083527025108 1.4
-0.370252292866661 1.1
-0.352968120050937 0.8
-0.323311001633873 0.5
-0.274143244282072 0.2
-0.195497119011841 -0.1
-0.1 -0.339622589666428
-0.0768636512609822 -0.4
0.0685030154336713 -0.7
0.2 -0.906510594865883
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
2 2.8058781117997
2.3 2.72407630752604
2.6 2.84068901670802
2.68325062165099 2.9
2.9 3.03777115857955
3.11058135180595 3.2
3.2 3.26396118758386
3.49776749972444 3.5
3.5 3.50168831860793
3.8 3.7410031457538
3.87102275617888 3.8
4.1 3.98473277638828
4.23652124875547 4.1
4.4 4.23442729385256
4.59300397760213 4.4
4.7 4.48989122105909
4.94189266627535 4.7
5 4.74973789716725
5 5
4.7 5
4.42612198684368 5
4.4 4.97853640508017
4.1 4.74926454005825
4.02922642691753 4.7
3.8 4.53152203340247
3.59349341454494 4.4
3.5 4.33515592647703
3.2 4.20200995709489
2.9 4.24437242128823
2.78391444008821 4.4
2.66543007010996 4.7
2.6 4.99531593454156
2.59917841022755 5
2.3 5
2 5
1.7 5
1.63578724368796 5
1.63986814831756 4.7
1.64720001775666 4.4
1.6603130371856 4.1
1.683516633347 3.8
1.7 3.67166552745491
1.72315148294248 3.5
1.79317720742395 3.2
1.92516305789396 2.9
2 2.8058781117997
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.1 -0.769218621435184
1.4 -0.789363010018514
1.7 -0.705107877959708
1.70918820646876 -0.7
2 -0.545008175763969
2.19653566455678 -0.4
2.3 -0.325291355605386
2.56033123098339 -0.1
2.6 -0.0659628717756402
2.87889913264853 0.2
2.9 0.220072305627016
3.17637024472926 0.5
3.2 0.523929244409933
3.46258265698267 0.8
3.5 0.839356870315865
3.74232335235987 1.1
3.8 1.16206742102425
4.01819778870687 1.4
4.1 1.48923404436727
4.29172206368825 1.7
4.4 1.81906270504577
4.5638107368472 2
4.7 2.15045094965629
4.83502435984861 2.3
5 2.48273875332464
5 2.6
5 2.9
5 3.2
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 4.74973789716725
4.94189266627535 4.7
4.7 4.48989122105909
4.59300397760213 4.4
4.4 4.23442729385256
4.23652124875547 4.1
4.1 3.98473277638828
3.87102275617888 3.8
3.8 3.7410031457538
3.5 3.50168831860793
3.49776749972444 3.5
3.2 3.26396118758386
3.11058135180595 3.2
2.9 3.03777115857955
2.68325062165099 2.9
2.6 2.84068901670802
2.3 2.72407630752604
2 2.8058781117997
1.92516305789396 2.9
1.79317720742395 3.2
1.72315148294248 3.5
1.7 3.67166552745491
1.683516633347 3.8
1.6603130371856 4.1
1.64720001775666 4.4
1.63986814831756 4.7
1.63578724368796 5
1.4 5
1.1 5
0.8 5
0.5 5
0.2 5
0.193364504052925 5
0.193360631302794 4.7
0.193358486066187 4.4
0.193353416621008 4.1
0.19333775684845 3.8
0.19331290045631 3.5
0.193270949365836 3.2
0.193199470648732 2.9
0.193086600420306 2.6
0.192934632419146 2.3
0.192820179076064 2
0.193068833527311 1.7
0.194675690100441 1.4
0.2 1.10435308358953
0.200102909212405 1.1
0.218203262574804 0.8
0.255389096111849 0.5
0.321670339943832 0.2
0.426870634736545 -0.1
0.5 -0.244439820596952
0.607019688018436 -0.4
0.8 -0.609925951071492
0.956364825374661 -0.7
1.1 -0.769218621435184

1.45379016602848 0.5
1.57201099430827 0.8
1.7 0.929777579003553
1.85227264321027 1.1
2 1.21916940386603
2.19396707366563 1.4
2.3 1.48376991603112
2.5478279499435 1.7
2.6 1.7416613191625
2.9 1.98940760350944
2.91412364958238 2
3.2 2.20178044618718
3.33581362436753 2.3
3.5 2.41358332057376
3.76118686710319 2.6
3.8 2.62681841359479
4.09773200535539 2.6
3.88201733905981 2.3
3.8 2.18886721366457
3.65954716668607 2
3.5 1.79122867350045
3.42933453501412 1.7
3.2 1.41650584196978
3.18632075700368 1.4
2.91103249710958 1.1
2.9 1.08856782308592
2.60856518223404 0.8
2.6 0.791865580328002
2.3 0.54807197395681
2.22987900328984 0.5
2 0.367697103507165
1.7 0.279070475710721
1.45379016602848 0.5
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
1.7 0.279070475710721
2 0.367697103507165
2.22987900328984 0.5
2.3 0.54807197395681
2.6 0.791865580328002
2.60856518223404 0.8
2.9 1.08856782308592
2.91103249710958 1.1
3.18632075700368 1.4
3.2 1.41650584196978
3.42933453501412 1.7
3.5 1.79122867350045
3.65954716668607 2
3.8 2.18886721366457
3.88201733905981 2.3
4.09773200535539 2.6
3.8 2.62681841359479
3.76118686710319 2.6
3.5 2.41358332057376
3.33581362436753 2.3
3.2 2.20178044618718
2.91412364958238 2
2.9 1.98940760350944
2.6 1.7416613191625
2.5478279499435 1.7
2.3 1.48376991603112
2.19396707366563 1.4
2 1.21916940386603
1.85227264321027 1.1
1.7 0.929777579003554
1.57201099430827 0.8
1.45379016602848 0.5
1.7 0.279070475710721
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.3 1.1
};
\coordinate (EP_mean_lml_t) at (axis cs:2.3,1.1);
\end{axis}



==> fig/tikz/echocardiogram/EP_nlpd.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
-0.7 -1
-0.4 -1
-0.1 -1
-0.0960666445291083 -1
-0.1 -0.991049517927542
-0.246811896332477 -0.7
-0.344864469540773 -0.4
-0.4 -0.158585702546627
-0.420780972312434 -0.1
-0.497730818552558 0.2
-0.542328762564422 0.5
-0.567870241814071 0.8
-0.582293469728617 1.1
-0.59034597989735 1.4
-0.594808288597254 1.7
-0.597271187045396 2
-0.59862482666891 2.3
-0.599369168201818 2.6
-0.599776662296882 2.9
-0.600000072525989 3.2
-0.600127529152439 3.5
-0.60019477478938 3.8
-0.600232771124445 4.1
-0.600251134841291 4.4
-0.60026373900352 4.7
-0.600269293314614 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
-0.1 -0.991049517927542
-0.0960666445291083 -1
0.2 -1
0.264170495223897 -1
0.2 -0.900486297276987
0.0901832828150537 -0.7
-0.0376791112454593 -0.4
-0.1 -0.211437577789738
-0.139298760946809 -0.1
-0.213477810011345 0.2
-0.258930241730198 0.5
-0.28577070901396 0.8
-0.30108271242762 1.1
-0.309619126653858 1.4
-0.314324403289324 1.7
-0.316902294865363 2
-0.318315468485012 2.3
-0.319086787085061 2.6
-0.319508776238955 2.9
-0.319741831865047 3.2
-0.319885682297674 3.5
-0.319948630921234 3.8
-0.319986033060355 4.1
-0.320004129767474 4.4
-0.320024656948857 4.7
-0.320029607276049 5
-0.4 5
-0.600269293314614 5
-0.60026373900352 4.7
-0.600251134841291 4.4
-0.600232771124445 4.1
-0.60019477478938 3.8
-0.600127529152439 3.5
-0.600000072525989 3.2
-0.599776662296882 2.9
-0.599369168201818 2.6
-0.59862482666891 2.3
-0.597271187045396 2
-0.594808288597254 1.7
-0.59034597989735 1.4
-0.582293469728617 1.1
-0.567870241814071 0.8
-0.542328762564422 0.5
-0.497730818552558 0.2
-0.420780972312434 -0.1
-0.4 -0.158585702546627
-0.344864469540773 -0.4
-0.246811896332477 -0.7
-0.1 -0.991049517927542
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
4.4 -1
4.7 -1
5 -1
5 -0.900587866946047
4.7 -0.93249766101321
4.4 -0.981034822334875
4.32395544659234 -1
4.4 -1
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
0.2 -0.900486297276987
0.264170495223897 -1
0.5 -1
0.653075650103026 -1
0.5 -0.852602648468767
0.396741310329876 -0.7
0.22020573958669 -0.4
0.2 -0.359069408736662
0.10020380363719 -0.1
0.019375330779725 0.2
-0.0330032440061642 0.5
-0.0644567240487396 0.8
-0.0822405364853713 1.1
-0.091963578735321 1.4
-0.0972222688423913 1.7
-0.1 1.99461059438128
-0.100048079166575 2
-0.101487899764632 2.3
-0.102252370864973 2.6
-0.102671725751041 2.9
-0.102907609787934 3.2
-0.103069693879014 3.5
-0.103114587979247 3.8
-0.103143577350897 4.1
-0.103164341060822 4.4
-0.103200251495288 4.7
-0.103204369374876 5
-0.320029607276049 5
-0.320024656948857 4.7
-0.320004129767474 4.4
-0.319986033060355 4.1
-0.319948630921234 3.8
-0.319885682297674 3.5
-0.319741831865047 3.2
-0.319508776238955 2.9
-0.319086787085061 2.6
-0.318315468485012 2.3
-0.316902294865363 2
-0.314324403289324 1.7
-0.309619126653858 1.4
-0.30108271242762 1.1
-0.28577070901396 0.8
-0.258930241730198 0.5
-0.213477810011345 0.2
-0.139298760946809 -0.1
-0.1 -0.211437577789738
-0.0376791112454593 -0.4
0.0901832828150537 -0.7
0.2 -0.900486297276987
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
2.3 -1
2.6 -1
2.9 -1
3.2 -1
3.5 -1
3.8 -1
4.1 -1
4.32395544659234 -1
4.4 -0.981034822334875
4.7 -0.93249766101321
5 -0.900587866946047
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.5
5 0.8
5 1.1
5 1.4
5 1.58862141124152
4.81073902308484 1.4
4.7 1.28962731791234
4.509221550824 1.1
4.4 0.991428612540056
4.20649774742823 0.8
4.1 0.69463698721459
3.9016163738459 0.5
3.8 0.400317736418688
3.59284733533619 0.2
3.5 0.110296395926148
3.276965346151 -0.1
3.2 -0.172344279127631
2.94767966097986 -0.4
2.9 -0.442626116522417
2.6 -0.694485852066796
2.5928852992403 -0.7
2.3 -0.927607652330309
2.18609912032238 -1
2.3 -1
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
0.5 -0.852602648468767
0.653075650103026 -1
0.8 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.18609912032238 -1
2.3 -0.927607652330309
2.5928852992403 -0.7
2.6 -0.694485852066796
2.9 -0.442626116522417
2.94767966097986 -0.4
3.2 -0.172344279127631
3.276965346151 -0.1
3.5 0.110296395926148
3.59284733533619 0.2
3.8 0.400317736418688
3.9016163738459 0.5
4.1 0.69463698721459
4.20649774742823 0.8
4.4 0.991428612540056
4.509221550824 1.1
4.7 1.28962731791234
4.81073902308484 1.4
5 1.58862141124152
5 1.7
5 2
5 2.16899221157206
4.83053302579459 2
4.7 1.86979215596858
4.52935485560323 1.7
4.4 1.57121985449115
4.22724991537833 1.4
4.1 1.27375151047205
3.92349946286524 1.1
3.8 0.978209113945873
3.61683751146444 0.8
3.5 0.685973492749107
3.30498630223993 0.5
3.2 0.399354085320011
2.98375644089935 0.2
2.9 0.122114299598148
2.64503327630262 -0.1
2.6 -0.139756338599014
2.3 -0.378743933729713
2.26881262785342 -0.4
2 -0.585997389760476
1.77797890440458 -0.7
1.7 -0.74056123877494
1.4 -0.824453698886714
1.1 -0.812404041184555
0.849793236040761 -0.7
0.8 -0.676359410592132
0.532448005072069 -0.4
0.5 -0.361180429057389
0.367899448005423 -0.1
0.255626886161809 0.2
0.2 0.429236258579836
0.186933707894417 0.5
0.155911727957654 0.8
0.140780501284271 1.1
0.134331144929478 1.4
0.131966672927427 1.7
0.131251356406985 2
0.131084937741771 2.3
0.131093747326958 2.6
0.131111094726472 2.9
0.131147301450509 3.2
0.131140681286736 3.5
0.131206770525369 3.8
0.131222155629321 4.1
0.131170805819724 4.4
0.131171699657723 4.7
0.131088226216898 5
-0.1 5
-0.103204369374876 5
-0.103200251495288 4.7
-0.103164341060822 4.4
-0.103143577350897 4.1
-0.103114587979247 3.8
-0.103069693879014 3.5
-0.102907609787933 3.2
-0.102671725751041 2.9
-0.102252370864973 2.6
-0.101487899764632 2.3
-0.100048079166575 2
-0.1 1.99461059438128
-0.0972222688423913 1.7
-0.091963578735321 1.4
-0.0822405364853713 1.1
-0.0644567240487396 0.8
-0.0330032440061642 0.5
0.019375330779725 0.2
0.10020380363719 -0.1
0.2 -0.359069408736662
0.22020573958669 -0.4
0.396741310329876 -0.7
0.5 -0.852602648468767
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
1.1 -0.812404041184555
1.4 -0.824453698886714
1.7 -0.74056123877494
1.77797890440458 -0.7
2 -0.585997389760476
2.26881262785342 -0.4
2.3 -0.378743933729713
2.6 -0.139756338599014
2.64503327630262 -0.1
2.9 0.122114299598148
2.98375644089935 0.2
3.2 0.399354085320011
3.30498630223993 0.5
3.5 0.685973492749107
3.61683751146444 0.8
3.8 0.978209113945873
3.92349946286524 1.1
4.1 1.27375151047205
4.22724991537833 1.4
4.4 1.57121985449115
4.52935485560323 1.7
4.7 1.86979215596858
4.83053302579459 2
5 2.16899221157206
5 2.3
5 2.6
5 2.64811858258381
4.95176814500534 2.6
4.7 2.34895501950179
4.65083717009331 2.3
4.4 2.05045014138211
4.34916369917217 2
4.1 1.75310622939249
4.04616272645538 1.7
3.8 1.45778371151864
3.74078658350418 1.4
3.5 1.16592998188884
3.43114683949947 1.1
3.2 0.879903500072848
3.11376236036858 0.8
2.9 0.603400649016268
2.78195983728124 0.5
2.6 0.341975590271203
2.42192827433835 0.2
2.3 0.103572779541129
2.00109736348347 -0.1
2 -0.100743494522964
1.7 -0.247616812274428
1.4 -0.326779507789456
1.1 -0.305843505506703
0.8 -0.142133393998698
0.764764001515644 -0.1
0.572801140992269 0.2
0.5 0.382349726323804
0.471247163442713 0.5
0.433324269818113 0.8
0.419748657569644 1.1
0.419860069543983 1.4
0.425847375304936 1.7
0.432726031923646 2
0.438464093709868 2.3
0.44242921966752 2.6
0.444821174653225 2.9
0.446286451727076 3.2
0.447144156227302 3.5
0.447598876846611 3.8
0.447870371375095 4.1
0.447961639089379 4.4
0.44811478886484 4.7
0.447907548713282 5
0.2 5
0.131088226216898 5
0.131171699657723 4.7
0.131170805819724 4.4
0.131222155629321 4.1
0.131206770525369 3.8
0.131140681286736 3.5
0.131147301450509 3.2
0.131111094726472 2.9
0.131093747326958 2.6
0.131084937741771 2.3
0.131251356406985 2
0.131966672927427 1.7
0.134331144929478 1.4
0.140780501284271 1.1
0.155911727957654 0.8
0.186933707894417 0.5
0.2 0.429236258579836
0.255626886161809 0.2
0.367899448005423 -0.1
0.5 -0.361180429057389
0.532448005072069 -0.4
0.8 -0.676359410592132
0.849793236040761 -0.7
1.1 -0.812404041184555
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
0.8 -0.142133393998698
1.1 -0.305843505506703
1.4 -0.326779507789456
1.7 -0.247616812274428
2 -0.100743494522964
2.00109736348347 -0.1
2.3 0.103572779541129
2.42192827433835 0.2
2.6 0.341975590271203
2.78195983728124 0.5
2.9 0.603400649016268
3.11376236036858 0.8
3.2 0.879903500072848
3.43114683949947 1.1
3.5 1.16592998188884
3.74078658350418 1.4
3.8 1.45778371151864
4.04616272645538 1.7
4.1 1.75310622939249
4.34916369917217 2
4.4 2.05045014138211
4.65083717009331 2.3
4.7 2.34895501950179
4.95176814500534 2.6
5 2.64811858258381
5 2.9
5 3.2
5 3.2117332249615
4.98827578317723 3.2
4.7 2.91230026825601
4.68771264125672 2.9
4.4 2.61335520674974
4.38665713582557 2.6
4.1 2.31534028860573
4.08464942030028 2.3
3.8 2.01908278855325
3.78080150836173 2
3.5 1.72611776327374
3.47334746256756 1.7
3.2 1.43915965556748
3.15876912345325 1.4
2.9 1.16267408833295
2.82987318784106 1.1
2.6 0.903316881091446
2.47118513494919 0.8
2.3 0.669699630366487
2.04572016687086 0.5
2 0.471301780229352
1.7 0.343624864199941
1.4 0.293780252593494
1.1 0.385712390581395
0.996627724191489 0.5
0.860754914120293 0.8
0.826076912164099 1.1
0.841076927437848 1.4
0.878745083621843 1.7
0.92804190979635 2
0.983683227891248 2.3
1.0416050955813 2.6
1.09601619258307 2.9
1.1 2.92894387633454
1.14588381589032 3.2
1.19203652304196 3.5
1.2304075810798 3.8
1.26079803658659 4.1
1.27993221077035 4.4
1.29279571154659 4.7
1.29991780177125 5
1.1 5
0.8 5
0.5 5
0.447907548713282 5
0.44811478886484 4.7
0.447961639089379 4.4
0.447870371375095 4.1
0.447598876846611 3.8
0.447144156227302 3.5
0.446286451727076 3.2
0.444821174653225 2.9
0.44242921966752 2.6
0.438464093709868 2.3
0.432726031923646 2
0.425847375304936 1.7
0.419860069543983 1.4
0.419748657569644 1.1
0.433324269818113 0.8
0.471247163442713 0.5
0.5 0.382349726323804
0.572801140992269 0.2
0.764764001515644 -0.1
0.8 -0.142133393998698
};
\addplot [draw=none, fill=lavender231240249]
table{%
x  y
1.1 0.385712390581395
1.4 0.293780252593494
1.7 0.343624864199941
2 0.471301780229352
2.04572016687086 0.5
2.3 0.669699630366487
2.47118513494919 0.8
2.6 0.903316881091446
2.82987318784106 1.1
2.9 1.16267408833295
3.15876912345325 1.4
3.2 1.43915965556748
3.47334746256756 1.7
3.5 1.72611776327374
3.78080150836173 2
3.8 2.01908278855325
4.08464942030028 2.3
4.1 2.31534028860573
4.38665713582557 2.6
4.4 2.61335520674974
4.68771264125672 2.9
4.7 2.91230026825601
4.98827578317723 3.2
5 3.2117332249615
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 4.81163567371244
4.92220403342247 4.7
4.7 4.43031405595587
4.68006796960706 4.4
4.4450843140792 4.1
4.4 4.04850378964634
4.21553045664656 3.8
4.1 3.66347890881843
3.98110483376869 3.5
3.8 3.27951559922834
3.7416265648756 3.2
3.5 2.90337058293384
3.49742946075011 2.9
3.24638492447141 2.6
3.2 2.54881272644971
2.98029355879854 2.3
2.9 2.21539509950885
2.69034611270751 2
2.6 1.91348492570977
2.35532477353077 1.7
2.3 1.65523482240619
2 1.47203585461498
1.7 1.45052052397396
1.60947877065312 1.7
1.62270665197124 2
1.68214517508254 2.3
1.7 2.35945483139613
1.7786434212479 2.6
1.87645838403831 2.9
1.98266378023858 3.2
2 3.24373257899312
2.09825602051449 3.5
2.21074041703191 3.8
2.3 4.01644155484618
2.33332471745959 4.1
2.44844424308336 4.4
2.57206423669002 4.7
2.6 4.76373376861754
2.69253929619605 5
2.6 5
2.3 5
2 5
1.7 5
1.4 5
1.29991780177125 5
1.29279571154659 4.7
1.27993221077035 4.4
1.26079803658659 4.1
1.2304075810798 3.8
1.19203652304196 3.5
1.14588381589032 3.2
1.1 2.92894387633454
1.09601619258307 2.9
1.0416050955813 2.6
0.983683227891248 2.3
0.92804190979635 2
0.878745083621843 1.7
0.841076927437848 1.4
0.826076912164099 1.1
0.860754914120293 0.8
0.996627724191489 0.5
1.1 0.385712390581395
};
\addplot [draw=none, fill=aliceblue242247253]
table{%
x  y
1.7 1.45052052397396
2 1.47203585461498
2.3 1.65523482240619
2.35532477353077 1.7
2.6 1.91348492570977
2.69034611270751 2
2.9 2.21539509950885
2.98029355879854 2.3
3.2 2.54881272644971
3.24638492447141 2.6
3.49742946075011 2.9
3.5 2.90337058293384
3.7416265648756 3.2
3.8 3.27951559922834
3.98110483376869 3.5
4.1 3.66347890881843
4.21553045664656 3.8
4.4 4.04850378964634
4.4450843140792 4.1
4.68006796960706 4.4
4.7 4.43031405595587
4.92220403342247 4.7
5 4.81163567371244
5 5
4.7 5
4.4 5
4.1 5
3.8 5
3.5 5
3.2 5
2.9 5
2.69253929619605 5
2.6 4.76373376861754
2.57206423669002 4.7
2.44844424308336 4.4
2.33332471745959 4.1
2.3 4.01644155484618
2.21074041703191 3.8
2.09825602051449 3.5
2 3.24373257899312
1.98266378023858 3.2
1.87645838403831 2.9
1.7786434212479 2.6
1.7 2.35945483139613
1.68214517508254 2.3
1.62270665197124 2
1.60947877065312 1.7
1.7 1.45052052397396
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.3 1.1
};
\coordinate (MCMC_mean_lml_t) at (axis cs:2.3,1.1);
\end{axis}



==> fig/tikz/echocardiogram/LA_mean_lml.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=midnightblue854116]
table{%
x  y
-0.770846725437529 4.7
-0.7 4.74156337679119
-0.514274184116273 5
-0.7 5
-1 5
-1 4.7
-1 4.54539799950274
-0.770846725437529 4.7
};
\addplot [draw=none, fill=midnightblue868137]
table{%
x  y
-0.948520695138026 4.1
-0.7 4.24500042136663
-0.575432009489405 4.4
-0.4 4.64306015599291
-0.372871940869546 4.7
-0.240339744442836 5
-0.4 5
-0.514274184116273 5
-0.7 4.74156337679119
-0.770846725437529 4.7
-1 4.54539799950274
-1 4.4
-1 4.1
-1 4.07220493300203
-0.948520695138026 4.1
};
\addplot [draw=none, fill=teal882156]
table{%
x  y
-0.7 3.78559656340779
-0.686114072310305 3.8
-0.422791083688804 4.1
-0.4 4.1285299780812
-0.257635537530587 4.4
-0.117349405804961 4.7
-0.1 4.74027893313197
-0.0177751601506267 5
-0.1 5
-0.240339744442836 5
-0.372871940869546 4.7
-0.4 4.64306015599291
-0.575432009489405 4.4
-0.7 4.24500042136663
-0.948520695138026 4.1
-1 4.07220493300203
-1 3.8
-1 3.63751031822821
-0.7 3.78559656340779
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 3.37105046444097
-0.563663787244016 3.5
-0.4 3.66996107162561
-0.319376881533758 3.8
-0.153915303163309 4.1
-0.1 4.2030715527088
-0.0209996602254054 4.4
0.0804546564088628 4.7
0.170034712897189 5
-0.0177751601506267 5
-0.1 4.74027893313197
-0.117349405804961 4.7
-0.257635537530587 4.4
-0.4 4.1285299780812
-0.422791083688804 4.1
-0.686114072310305 3.8
-0.7 3.78559656340779
-1 3.63751031822821
-1 3.5
-1 3.23735242591643
-0.7 3.37105046444097
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.914140250806319 2.9
-0.7 2.98660877086956
-0.452473360275317 3.2
-0.4 3.24953947005438
-0.228112632741054 3.5
-0.1 3.71188155320469
-0.0582427464759061 3.8
0.0683302048358768 4.1
0.179232955176753 4.4
0.2 4.46399144576685
0.289649402006877 4.7
0.392420744648899 5
0.2 5
0.170034712897189 5
0.0804546564088628 4.7
-0.0209996602254054 4.4
-0.1 4.2030715527088
-0.153915303163309 4.1
-0.319376881533758 3.8
-0.4 3.66996107162561
-0.563663787244016 3.5
-0.7 3.37105046444097
-1 3.23735242591643
-1 3.2
-1 2.9
-1 2.86738341688191
-0.914140250806319 2.9
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
-0.769097930213732 2.6
-0.7 2.62563317464229
-0.4 2.86110095651982
-0.367477200182998 2.9
-0.141313022599581 3.2
-0.1 3.26146564587914
0.0258047316973586 3.5
0.162391455826884 3.8
0.2 3.89301460303404
0.293661658242819 4.1
0.415383421980025 4.4
0.5 4.63236897677146
0.523896862627831 4.7
0.618509894739973 5
0.5 5
0.392420744648899 5
0.289649402006877 4.7
0.2 4.46399144576685
0.179232955176753 4.4
0.0683302048358768 4.1
-0.0582427464759061 3.8
-0.1 3.71188155320469
-0.228112632741054 3.5
-0.4 3.24953947005438
-0.452473360275317 3.2
-0.7 2.98660877086956
-0.914140250806319 2.9
-1 2.86738341688191
-1 2.6
-1 2.51834732226055
-0.769097930213732 2.6
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
-0.7 2.27968551526295
-0.670463062906045 2.3
-0.4 2.49475847358315
-0.304008457393808 2.6
-0.1 2.84676241343666
-0.0651377430641524 2.9
0.109190343566746 3.2
0.2 3.38095722761593
0.264616825903318 3.5
0.411069612443622 3.8
0.5 4.00404723432533
0.542039347344209 4.1
0.658078804531894 4.4
0.757072710770934 4.7
0.8 4.84836429774993
0.842675247948128 5
0.8 5
0.618509894739973 5
0.523896862627831 4.7
0.5 4.63236897677146
0.415383421980025 4.4
0.293661658242819 4.1
0.2 3.89301460303404
0.162391455826884 3.8
0.0258047316973586 3.5
-0.1 3.26146564587914
-0.141313022599581 3.2
-0.367477200182998 2.9
-0.4 2.86110095651982
-0.7 2.62563317464229
-0.769097930213732 2.6
-1 2.51834732226055
-1 2.3
-1 2.17935551222585
-0.7 2.27968551526295
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
-0.7 1.93589683356074
-0.603937716721421 2
-0.4 2.13777077451777
-0.241359850368139 2.3
-0.1 2.45594378065479
0.00442476430510258 2.6
0.193661619360923 2.9
0.2 2.91128041190901
0.371673933863252 3.2
0.5 3.44474059487477
0.53015858529649 3.5
0.675363313700023 3.8
0.797818749587091 4.1
0.8 4.10599331717966
0.904398692164667 4.4
0.993416955428262 4.7
1.06948101436736 5
0.842675247948128 5
0.8 4.84836429774993
0.757072710770934 4.7
0.658078804531894 4.4
0.542039347344209 4.1
0.5 4.00404723432533
0.411069612443622 3.8
0.264616825903318 3.5
0.2 3.38095722761593
0.109190343566746 3.2
-0.0651377430641524 2.9
-0.1 2.84676241343666
-0.304008457393808 2.6
-0.4 2.49475847358315
-0.670463062906045 2.3
-0.7 2.27968551526295
-1 2.17935551222585
-1 2
-1 1.83853660865918
-0.7 1.93589683356074
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
-0.7 1.5754731435983
-0.516315748115764 1.7
-0.4 1.7760192099736
-0.17189871897624 2
-0.1 2.07364405295876
0.0791604638764046 2.3
0.2 2.47232708083832
0.290389829219392 2.6
0.480208505088533 2.9
0.5 2.9344318550563
0.661171113027904 3.2
0.8 3.46866889995903
0.8163234510151 3.5
0.952377654754447 3.8
1.06283822312366 4.1
1.1 4.21800445010167
1.1713855520266 4.4
1.27578515236901 4.7
1.36797060325905 5
1.1 5
1.06948101436736 5
0.993416955428262 4.7
0.904398692164667 4.4
0.8 4.10599331717966
0.797818749587091 4.1
0.675363313700023 3.8
0.53015858529649 3.5
0.5 3.44474059487477
0.371673933863252 3.2
0.2 2.91128041190901
0.193661619360923 2.9
0.00442476430510255 2.6
-0.1 2.45594378065479
-0.241359850368139 2.3
-0.4 2.13777077451777
-0.603937716721421 2
-0.7 1.93589683356074
-1 1.83853660865918
-1 1.7
-1 1.47702018261469
-0.7 1.5754731435983
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
-0.879442197122982 1.1
-0.7 1.16325323104118
-0.4 1.38374096211698
-0.384767545721264 1.4
-0.1 1.68093915674146
-0.0836718613708518 1.7
0.167400774348271 2
0.2 2.04227281235165
0.397219059525916 2.3
0.5 2.4500447972429
0.610223718344283 2.6
0.8 2.89502246208225
0.803294879277362 2.9
0.980078211684635 3.2
1.1 3.44995243942025
1.12794288171972 3.5
1.27366905655847 3.8
1.39665733534686 4.1
1.4 4.10915975981513
1.58651438554293 4.4
1.7 4.58027121828126
1.81637781398595 4.7
2 4.92228045262145
2.06787498909167 5
2 5
1.7 5
1.4 5
1.36797060325905 5
1.27578515236901 4.7
1.1713855520266 4.4
1.1 4.21800445010167
1.06283822312366 4.1
0.952377654754447 3.8
0.8163234510151 3.5
0.8 3.46866889995903
0.661171113027904 3.2
0.5 2.9344318550563
0.480208505088533 2.9
0.290389829219392 2.6
0.2 2.47232708083832
0.0791604638764046 2.3
-0.1 2.07364405295876
-0.17189871897624 2
-0.4 1.7760192099736
-0.516315748115764 1.7
-0.7 1.5754731435983
-1 1.47702018261469
-1 1.4
-1 1.1
-1 1.04712982826222
-0.879442197122982 1.1
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
-0.745790390267606 0.5
-0.7 0.525737306597864
-0.475345107119061 0.8
-0.4 0.866154041632287
-0.218582942805049 1.1
-0.1 1.22726039251075
0.0397010318259117 1.4
0.2 1.59060645469965
0.291686711697689 1.7
0.5 1.96292734107358
0.531522695956365 2
0.766780173274454 2.3
0.8 2.34688207600301
0.986148913596282 2.6
1.1 2.78216206313962
1.18549183134141 2.9
1.36887760937634 3.2
1.4 3.25996134406795
1.57339743925009 3.5
1.7 3.68506801552516
1.82216317012424 3.8
2 3.96406101848595
2.15066753317075 4.1
2.3 4.248710497119
2.46972274261838 4.4
2.6 4.51401800582155
2.85348531569859 4.7
2.9 4.73187668413727
3.2 4.89802081062103
3.3881614413704 5
3.2 5
2.9 5
2.6 5
2.3 5
2.06787498909167 5
2 4.92228045262145
1.81637781398595 4.7
1.7 4.58027121828126
1.58651438554293 4.4
1.4 4.10915975981513
1.39665733534686 4.1
1.27366905655847 3.8
1.12794288171972 3.5
1.1 3.44995243942025
0.980078211684635 3.2
0.803294879277362 2.9
0.8 2.89502246208225
0.610223718344283 2.6
0.5 2.4500447972429
0.397219059525916 2.3
0.2 2.04227281235165
0.167400774348271 2
-0.0836718613708518 1.7
-0.1 1.68093915674146
-0.384767545721264 1.4
-0.4 1.38374096211698
-0.7 1.16325323104118
-0.879442197122982 1.1
-1 1.04712982826222
-1 0.8
-1 0.5
-1 0.271072843262395
-0.745790390267606 0.5
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
-0.7 -1
-0.4 -1
-0.1 -1
0.2 -1
0.271120498104905 -1
0.2 -0.899955397232168
0.0761931253865913 -0.7
-0.0573217346331084 -0.4
-0.1 -0.244713835085297
-0.141210500017936 -0.1
-0.15691451675282 0.2
-0.1 0.465061569707551
-0.093326053341769 0.5
0.0434756149600258 0.8
0.2 1.04163359918746
0.240031872156106 1.1
0.477424855359738 1.4
0.5 1.42762936504854
0.741374745011006 1.7
0.8 1.77071662308879
1.00524387309712 2
1.1 2.12124152889475
1.26026775571816 2.3
1.4 2.48014464853401
1.51681977533571 2.6
1.7 2.81384386793372
1.79731217665157 2.9
2 3.09034410596653
2.14554188243657 3.2
2.3 3.32044939451558
2.55549086586376 3.5
2.6 3.53298107426745
2.9 3.74182216289594
2.97517760464434 3.8
3.2 3.96079591719266
3.37567897048816 4.1
3.5 4.19011296522787
3.75985556646054 4.4
3.8 4.43023146058122
4.1 4.67668059461738
4.12771824013601 4.7
4.4 4.9250765484049
4.48833210720707 5
4.4 5
4.1 5
3.8 5
3.5 5
3.3881614413704 5
3.2 4.89802081062103
2.9 4.73187668413727
2.85348531569859 4.7
2.6 4.51401800582155
2.46972274261838 4.4
2.3 4.248710497119
2.15066753317075 4.1
2 3.96406101848595
1.82216317012424 3.8
1.7 3.68506801552516
1.57339743925009 3.5
1.4 3.25996134406795
1.36887760937634 3.2
1.18549183134141 2.9
1.1 2.78216206313962
0.986148913596282 2.6
0.8 2.34688207600301
0.766780173274454 2.3
0.531522695956365 2
0.5 1.96292734107358
0.291686711697689 1.7
0.2 1.59060645469965
0.0397010318259117 1.4
-0.1 1.22726039251075
-0.218582942805049 1.1
-0.4 0.866154041632287
-0.475345107119061 0.8
-0.7 0.525737306597864
-0.745790390267606 0.5
-1 0.271072843262395
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
2.9 -1
3.2 -1
3.5 -1
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.5
5 0.8
5 1.1
5 1.4
5 1.67200579484359
4.77156390575556 1.4
4.7 1.31473124234568
4.51906867336313 1.1
4.4 0.95853231887067
4.26565234164692 0.8
4.1 0.604173249807123
4.01084052028012 0.5
3.8 0.252951616169658
3.75390782445521 0.2
3.5 -0.0929192740409071
3.49365772876124 -0.1
3.23928886420008 -0.4
3.2 -0.44573002537187
2.9701994116582 -0.7
2.9 -0.774204176990831
2.66756171075247 -1
2.9 -1
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
0.2 -0.899955397232168
0.271120498104905 -1
0.5 -1
0.8 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.3 -1
2.6 -1
2.66756171075247 -1
2.9 -0.774204176990831
2.9701994116582 -0.7
3.2 -0.44573002537187
3.23928886420008 -0.4
3.49365772876124 -0.1
3.5 -0.0929192740409071
3.75390782445521 0.2
3.8 0.252951616169658
4.01084052028012 0.5
4.1 0.604173249807123
4.26565234164692 0.8
4.4 0.95853231887067
4.51906867336313 1.1
4.7 1.31473124234568
4.77156390575556 1.4
5 1.67200579484359
5 1.7
5 2
5 2.3
5 2.48473151971359
4.83328654247109 2.3
4.7 2.15231994962017
4.56216770897631 2
4.4 1.82081096941691
4.29016867678511 1.7
4.1 1.49086627256681
4.01672638061466 1.4
3.8 1.16359080292771
3.74092246260816 1.1
3.5 0.840782384859678
3.46123445905785 0.8
3.2 0.525273922645391
3.17504494329108 0.5
2.9 0.221363155024441
2.87754260660189 0.2
2.6 -0.0646835793742387
2.55883822565615 -0.1
2.3 -0.323964283834997
2.19468315558327 -0.4
2 -0.543571124218279
1.70637257986645 -0.7
1.7 -0.703538925595516
1.4 -0.787178577876931
1.1 -0.76552583040695
0.96678182811295 -0.7
0.8 -0.598897492332308
0.627104711988193 -0.4
0.5 -0.175618814208185
0.468803901300451 -0.1
0.422499978739265 0.2
0.464670925577319 0.5
0.5 0.583030944694035
0.61351616873553 0.8
0.8 1.05507536419114
0.839623272295726 1.1
1.1 1.3670956465342
1.13664418126586 1.4
1.4 1.63588630581994
1.47811230686951 1.7
1.7 1.88475585456264
1.84258701508719 2
2 2.12474969690995
2.20970353534178 2.3
2.3 2.37137884196846
2.56017962375401 2.6
2.6 2.63281933151373
2.8959010955273 2.9
2.9 2.90353300747909
3.2 3.1725384000649
3.2312605483346 3.2
3.5 3.43518408449716
3.57521836614095 3.5
3.8 3.69213413510653
3.92596482206489 3.8
4.1 3.94693808274979
4.27797582140557 4.1
4.4 4.20319427168873
4.62688173287895 4.4
4.7 4.46247304717389
4.97159658981126 4.7
5 4.72456140432585
5 5
4.7 5
4.48833210720707 5
4.4 4.9250765484049
4.12771824013601 4.7
4.1 4.67668059461738
3.8 4.43023146058122
3.75985556646054 4.4
3.5 4.19011296522787
3.37567897048816 4.1
3.2 3.96079591719266
2.97517760464434 3.8
2.9 3.74182216289594
2.6 3.53298107426745
2.55549086586376 3.5
2.3 3.32044939451558
2.14554188243657 3.2
2 3.09034410596653
1.79731217665157 2.9
1.7 2.81384386793372
1.51681977533571 2.6
1.4 2.48014464853401
1.26026775571816 2.3
1.1 2.12124152889475
1.00524387309712 2
0.8 1.77071662308879
0.741374745011006 1.7
0.5 1.42762936504854
0.477424855359738 1.4
0.240031872156106 1.1
0.2 1.04163359918746
0.0434756149600258 0.8
-0.093326053341769 0.5
-0.1 0.465061569707551
-0.15691451675282 0.2
-0.141210500017936 -0.1
-0.1 -0.244713835085297
-0.0573217346331084 -0.4
0.0761931253865913 -0.7
0.2 -0.899955397232168
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.1 -0.76552583040695
1.4 -0.787178577876931
1.7 -0.703538925595516
1.70637257986645 -0.7
2 -0.543571124218279
2.19468315558327 -0.4
2.3 -0.323964283834997
2.55883822565615 -0.1
2.6 -0.0646835793742387
2.87754260660189 0.2
2.9 0.221363155024441
3.17504494329108 0.5
3.2 0.525273922645391
3.46123445905785 0.8
3.5 0.840782384859678
3.74092246260816 1.1
3.8 1.16359080292771
4.01672638061466 1.4
4.1 1.49086627256681
4.29016867678511 1.7
4.4 1.82081096941691
4.56216770897631 2
4.7 2.15231994962017
4.83328654247109 2.3
5 2.48473151971359
5 2.6
5 2.9
5 3.2
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 4.72456140432585
4.97159658981126 4.7
4.7 4.46247304717389
4.62688173287895 4.4
4.4 4.20319427168873
4.27797582140557 4.1
4.1 3.94693808274979
3.92596482206489 3.8
3.8 3.69213413510653
3.57521836614095 3.5
3.5 3.43518408449716
3.2312605483346 3.2
3.2 3.1725384000649
2.9 2.90353300747909
2.8959010955273 2.9
2.6 2.63281933151373
2.56017962375401 2.6
2.3 2.37137884196846
2.20970353534179 2.3
2 2.12474969690995
1.84258701508719 2
1.7 1.88475585456264
1.47811230686951 1.7
1.4 1.63588630581994
1.13664418126586 1.4
1.1 1.3670956465342
0.839623272295726 1.1
0.8 1.05507536419114
0.613516168735529 0.8
0.5 0.583030944694035
0.464670925577319 0.5
0.422499978739265 0.2
0.468803901300451 -0.1
0.5 -0.175618814208185
0.627104711988193 -0.4
0.8 -0.598897492332308
0.96678182811295 -0.7
1.1 -0.76552583040695

1.63142096763639 0.5
1.7 0.63987975572598
1.77994412264078 0.8
2 1.06650438977015
2.027271987784 1.1
2.3 1.37644962245172
2.32369237767356 1.4
2.6 1.6525888501728
2.65432931140693 1.7
2.9 1.90526324369543
3.01844858494706 2
3.2 2.14078072860505
3.40981071799698 2.3
3.5 2.36666272751214
3.8 2.5455231084479
3.85580129909709 2.3
3.8 2.2236522927102
3.63460036905763 2
3.5 1.82237921595706
3.40538208970559 1.7
3.2 1.44456795635142
3.16291568129725 1.4
2.9 1.10261929048313
2.89754600812685 1.1
2.6 0.809914396654287
2.5887905154058 0.8
2.3 0.57580483296097
2.18416232944373 0.5
2 0.398993624830202
1.7 0.388163690629359
1.63142096763639 0.5
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
1.7 0.388163690629359
2 0.398993624830202
2.18416232944373 0.5
2.3 0.57580483296097
2.5887905154058 0.8
2.6 0.809914396654287
2.89754600812685 1.1
2.9 1.10261929048313
3.16291568129725 1.4
3.2 1.44456795635142
3.40538208970559 1.7
3.5 1.82237921595706
3.63460036905763 2
3.8 2.2236522927102
3.85580129909709 2.3
3.8 2.5455231084479
3.5 2.36666272751214
3.40981071799698 2.3
3.2 2.14078072860505
3.01844858494706 2
2.9 1.90526324369543
2.65432931140692 1.7
2.6 1.6525888501728
2.32369237767356 1.4
2.3 1.37644962245172
2.027271987784 1.1
2 1.06650438977015
1.77994412264078 0.8
1.7 0.63987975572598
1.63142096763639 0.5
1.7 0.388163690629359
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.6 1.1
};
\coordinate (LA_mean_lml_t) at (axis cs:2.5999999999999996,1.1);
\end{axis}



==> fig/tikz/echocardiogram/LA_nlpd.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
-0.7 -1
-0.4 -1
-0.1 -1
-0.0909280536432816 -1
-0.1 -0.97844261861199
-0.236403358036593 -0.7
-0.330778596883959 -0.4
-0.390870267324148 -0.1
-0.4 -0.026399197546957
-0.445987950632673 0.2
-0.469217641955914 0.5
-0.463243380555057 0.8
-0.43298125106715 1.1
-0.4 1.29405481527416
-0.387554820236012 1.4
-0.340146470502198 1.7
-0.275912796548681 2
-0.191148232849348 2.3
-0.1 2.5551543477089
-0.0839713643511152 2.6
0.0319704791968145 2.9
0.180171934108393 3.2
0.2 3.23810398011469
0.350341363701064 3.5
0.5 3.72506952395062
0.54302190425031 3.8
0.72154762657555 4.1
0.8 4.22223509777509
0.898570544482484 4.4
1.08864895314517 4.7
1.1 4.71751891283711
1.25850931764208 5
1.1 5
0.8 5
0.5 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
-0.1 -0.97844261861199
-0.0909280536432816 -1
0.2 -1
0.274148911365241 -1
0.2 -0.879203537445671
0.105317666600165 -0.7
-0.0147591914175919 -0.4
-0.0972846817255847 -0.1
-0.1 -0.0834432471589206
-0.151601899504323 0.2
-0.167481351350185 0.5
-0.151161976140722 0.8
-0.106017506228233 1.1
-0.1 1.12743764215687
-0.0408906823436998 1.4
0.0478602994645863 1.7
0.164301346607063 2
0.2 2.0809804236218
0.310251575054423 2.3
0.488411902805043 2.6
0.5 2.61860254291985
0.672665341413231 2.9
0.8 3.09631234866078
0.85868551125316 3.2
1.03366558520834 3.5
1.1 3.60770522876717
1.20890355025532 3.8
1.39494144040013 4.1
1.4 4.10799602964276
1.55748174369637 4.4
1.7 4.64138359596756
1.72953485802466 4.7
1.88243135684862 5
1.7 5
1.4 5
1.25850931764208 5
1.1 4.71751891283711
1.08864895314517 4.7
0.898570544482485 4.4
0.8 4.22223509777509
0.72154762657555 4.1
0.54302190425031 3.8
0.5 3.72506952395062
0.350341363701064 3.5
0.2 3.23810398011469
0.180171934108393 3.2
0.0319704791968145 2.9
-0.0839713643511152 2.6
-0.1 2.5551543477089
-0.191148232849348 2.3
-0.275912796548681 2
-0.340146470502198 1.7
-0.387554820236012 1.4
-0.4 1.29405481527416
-0.43298125106715 1.1
-0.463243380555057 0.8
-0.469217641955914 0.5
-0.445987950632673 0.2
-0.4 -0.026399197546957
-0.390870267324148 -0.1
-0.330778596883959 -0.4
-0.236403358036593 -0.7
-0.1 -0.97844261861199
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
4.4 -1
4.7 -1
5 -1
5 -0.882090331488483
4.7 -0.91518049423135
4.4 -0.965493846952188
4.26176556407955 -1
4.4 -1
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
0.2 -0.879203537445671
0.274148911365241 -1
0.5 -1
0.671359426000825 -1
0.5 -0.825460238692615
0.4188251275522 -0.7
0.257636613805349 -0.4
0.2 -0.25503106704507
0.150104614932633 -0.1
0.096659475826528 0.2
0.0854127379432703 0.5
0.112368359157526 0.8
0.174116692049309 1.1
0.2 1.18760948515449
0.274225478073566 1.4
0.406955286718571 1.7
0.5 1.87641359281166
0.572509914826087 2
0.763606822604741 2.3
0.8 2.3553546519393
0.947849415857341 2.6
1.1 2.85008091192833
1.12833485270026 2.9
1.29947314342785 3.2
1.4 3.36693643243307
1.47299470383953 3.5
1.64158671822208 3.8
1.7 3.90054869815952
1.8015386401781 4.1
1.9612203697873 4.4
2 4.46997090126483
2.11472069320814 4.7
2.27483341396376 5
2 5
1.88243135684862 5
1.72953485802466 4.7
1.7 4.64138359596756
1.55748174369637 4.4
1.4 4.10799602964276
1.39494144040013 4.1
1.20890355025532 3.8
1.1 3.60770522876717
1.03366558520834 3.5
0.85868551125316 3.2
0.8 3.09631234866078
0.672665341413231 2.9
0.5 2.61860254291985
0.488411902805043 2.6
0.310251575054423 2.3
0.2 2.0809804236218
0.164301346607063 2
0.0478602994645863 1.7
-0.0408906823436998 1.4
-0.1 1.12743764215687
-0.106017506228233 1.1
-0.151161976140722 0.8
-0.167481351350185 0.5
-0.151601899504323 0.2
-0.1 -0.0834432471589206
-0.0972846817255847 -0.1
-0.0147591914175919 -0.4
0.105317666600165 -0.7
0.2 -0.879203537445671
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
2.3 -1
2.6 -1
2.9 -1
3.2 -1
3.5 -1
3.8 -1
4.1 -1
4.26176556407955 -1
4.4 -0.965493846952188
4.7 -0.91518049423135
5 -0.882090331488483
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.5
5 0.8
5 1.1
5 1.4
5 1.59775139191442
4.80157814922792 1.4
4.7 1.29875879354306
4.5000345228693 1.1
4.4 1.00056193323971
4.19726605413172 0.8
4.1 0.703772903932337
3.89230504361455 0.5
3.8 0.409455175448242
3.58339716883607 0.2
3.5 0.119432223199982
3.26727903512961 -0.1
3.2 -0.163231701401455
2.93757512979303 -0.4
2.9 -0.433584597398413
2.6 -0.687342777534821
2.58366177239335 -0.7
2.3 -0.920192613847395
2.17431654316262 -1
2.3 -1
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
0.5 -0.825460238692615
0.671359426000825 -1
0.8 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.17431654316262 -1
2.3 -0.920192613847395
2.58366177239335 -0.7
2.6 -0.687342777534821
2.9 -0.433584597398413
2.93757512979303 -0.4
3.2 -0.163231701401455
3.26727903512961 -0.1
3.5 0.119432223199982
3.58339716883607 0.2
3.8 0.409455175448242
3.89230504361455 0.5
4.1 0.703772903932337
4.19726605413172 0.8
4.4 1.00056193323971
4.5000345228693 1.1
4.7 1.29875879354306
4.80157814922792 1.4
5 1.59775139191442
5 1.7
5 2
5 2.18288695300145
4.81659549786411 2
4.7 1.88369713802383
4.51537342450445 1.7
4.4 1.58514301816416
4.21319043767593 1.4
4.1 1.28770723887701
3.90930391031348 1.1
3.8 0.992219361872359
3.60239929443036 0.8
3.5 0.700082950765152
3.29012457344101 0.5
3.2 0.413629760920811
2.96815856583608 0.2
2.9 0.136654501698285
2.62813190387701 -0.1
2.6 -0.124810863813201
2.3 -0.364102987499575
2.24708224380508 -0.4
2 -0.569979203267096
1.74481947421319 -0.7
1.7 -0.723071648069555
1.4 -0.803932171662837
1.1 -0.785972763344604
0.92350883037416 -0.7
0.8 -0.632728973725628
0.599007670582751 -0.4
0.5 -0.249610749663397
0.438495737759774 -0.1
0.369028882706883 0.2
0.357072038355169 0.5
0.396979863349331 0.8
0.480929700382086 1.1
0.5 1.14880251698331
0.615763818902064 1.4
0.78075130833773 1.7
0.8 1.73137297651022
0.964117501201518 2
1.1 2.21522829534034
1.15051638972186 2.3
1.32601822241122 2.6
1.4 2.72603372739313
1.49697304392701 2.9
1.66510443371522 3.2
1.7 3.26144648944032
1.82359757682562 3.5
1.98009694391667 3.8
2 3.8374021327508
2.13075878490025 4.1
2.28316337105314 4.4
2.3 4.43210163485487
2.43335694798848 4.7
2.58471849445837 5
2.3 5
2.27483341396376 5
2.11472069320814 4.7
2 4.46997090126483
1.9612203697873 4.4
1.8015386401781 4.1
1.7 3.90054869815952
1.64158671822208 3.8
1.47299470383953 3.5
1.4 3.36693643243307
1.29947314342785 3.2
1.12833485270026 2.9
1.1 2.85008091192833
0.947849415857341 2.6
0.8 2.3553546519393
0.763606822604741 2.3
0.572509914826087 2
0.5 1.87641359281166
0.406955286718571 1.7
0.274225478073566 1.4
0.2 1.18760948515449
0.174116692049309 1.1
0.112368359157525 0.8
0.0854127379432703 0.5
0.096659475826528 0.2
0.150104614932633 -0.1
0.2 -0.25503106704507
0.257636613805349 -0.4
0.4188251275522 -0.7
0.5 -0.825460238692615
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
1.1 -0.785972763344604
1.4 -0.803932171662837
1.7 -0.723071648069555
1.74481947421319 -0.7
2 -0.569979203267096
2.24708224380508 -0.4
2.3 -0.364102987499575
2.6 -0.124810863813201
2.62813190387701 -0.1
2.9 0.136654501698285
2.96815856583608 0.2
3.2 0.413629760920811
3.29012457344101 0.5
3.5 0.700082950765152
3.60239929443036 0.8
3.8 0.992219361872359
3.90930391031348 1.1
4.1 1.28770723887701
4.21319043767593 1.4
4.4 1.58514301816416
4.51537342450445 1.7
4.7 1.88369713802383
4.81659549786411 2
5 2.18288695300145
5 2.3
5 2.6
5 2.67695242915622
4.92285343187411 2.6
4.7 2.37780838253649
4.62183764109202 2.3
4.4 2.07933903009389
4.32001143032899 2
4.1 1.78205957040581
4.01673421898775 1.7
3.8 1.48685557678821
3.71085809829484 1.4
3.5 1.19521648183145
3.40030961081808 1.1
3.2 0.909574175362997
3.08126736700957 0.8
2.9 0.633744582670444
2.7464052987224 0.5
2.6 0.373429908962409
2.38060708681163 0.2
2.3 0.136726287044816
2 -0.0611252666024664
1.91968118367615 -0.1
1.7 -0.202569071207655
1.4 -0.266546694361001
1.1 -0.216837463643238
0.938780173840423 -0.1
0.8 0.066876211227495
0.746174157405758 0.2
0.711099439981218 0.5
0.750710690513455 0.8
0.8 0.954471114566277
0.854233763269353 1.1
0.998194615516009 1.4
1.1 1.5859878999656
1.16317703653244 1.7
1.33403778378232 2
1.4 2.11321630026324
1.50778041401835 2.3
1.6723991925679 2.6
1.7 2.64940979289704
1.83786457244751 2.9
1.99109950335442 3.2
2 3.21723971305875
2.14492018991709 3.5
2.29039060165541 3.8
2.3 3.8193837529745
2.44140810868502 4.1
2.5863982772035 4.4
2.6 4.42753990659462
2.74026922212379 4.7
2.88084936096731 5
2.6 5
2.58471849445837 5
2.43335694798848 4.7
2.3 4.43210163485487
2.28316337105314 4.4
2.13075878490025 4.1
2 3.8374021327508
1.98009694391667 3.8
1.82359757682562 3.5
1.7 3.26144648944032
1.66510443371522 3.2
1.49697304392701 2.9
1.4 2.72603372739313
1.32601822241122 2.6
1.15051638972186 2.3
1.1 2.21522829534034
0.964117501201518 2
0.8 1.73137297651022
0.78075130833773 1.7
0.615763818902064 1.4
0.5 1.14880251698331
0.480929700382086 1.1
0.396979863349331 0.8
0.357072038355169 0.5
0.369028882706883 0.2
0.438495737759774 -0.1
0.5 -0.249610749663397
0.599007670582751 -0.4
0.8 -0.632728973725628
0.92350883037416 -0.7
1.1 -0.785972763344604
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
1.1 -0.216837463643238
1.4 -0.266546694361001
1.7 -0.202569071207655
1.91968118367615 -0.1
2 -0.0611252666024664
2.3 0.136726287044816
2.38060708681163 0.2
2.6 0.373429908962409
2.7464052987224 0.5
2.9 0.633744582670444
3.08126736700957 0.8
3.2 0.909574175362997
3.40030961081808 1.1
3.5 1.19521648183145
3.71085809829484 1.4
3.8 1.48685557678821
4.01673421898775 1.7
4.1 1.78205957040581
4.32001143032899 2
4.4 2.07933903009389
4.62183764109202 2.3
4.7 2.37780838253649
4.92285343187411 2.6
5 2.67695242915622
5 2.9
5 3.2
5 3.29791608530615
4.90203066297329 3.2
4.7 2.99850715391113
4.60136231829664 2.9
4.4 2.69962414764382
4.30005601025348 2.6
4.1 2.40175159130473
3.99746995623952 2.3
3.8 2.10582201370471
3.69230642085448 2
3.5 1.8135837073613
3.38196872386225 1.7
3.2 1.52814752085739
3.06129859997743 1.4
2.9 1.25459422023081
2.7199222748721 1.1
2.6 1.00024914730906
2.33583710202843 0.8
2.3 0.773941778475423
2 0.617532784118473
1.7 0.531945571818001
1.4 0.69602175314925
1.36280618480276 0.8
1.38125769682687 1.1
1.4 1.15844128711623
1.49252177366716 1.4
1.62036395260018 1.7
1.7 1.87775502067842
1.76501043901024 2
1.91747977381044 2.3
2 2.47636780990776
2.07026535986409 2.6
2.22100200085476 2.9
2.3 3.07953728899643
2.36759128495094 3.2
2.51371912416729 3.5
2.6 3.7042471662612
2.65424989690011 3.8
2.80625209446979 4.1
2.9 4.31313760510649
2.95097153857783 4.4
3.0970925906816 4.7
3.2 4.98344671459788
3.20860361247589 5
3.2 5
2.9 5
2.88084936096731 5
2.74026922212379 4.7
2.6 4.42753990659462
2.5863982772035 4.4
2.44140810868502 4.1
2.3 3.8193837529745
2.29039060165541 3.8
2.14492018991709 3.5
2 3.21723971305875
1.99109950335442 3.2
1.83786457244751 2.9
1.7 2.64940979289704
1.6723991925679 2.6
1.50778041401835 2.3
1.4 2.11321630026324
1.33403778378232 2
1.16317703653244 1.7
1.1 1.5859878999656
0.99819461551601 1.4
0.854233763269353 1.1
0.8 0.954471114566277
0.750710690513455 0.8
0.711099439981218 0.5
0.746174157405758 0.2
0.8 0.066876211227495
0.938780173840423 -0.1
1.1 -0.216837463643238
};
\addplot [draw=none, fill=lavender231240249]
table{%
x  y
1.4 0.69602175314925
1.7 0.531945571818001
2 0.617532784118473
2.3 0.773941778475424
2.33583710202843 0.8
2.6 1.00024914730906
2.7199222748721 1.1
2.9 1.25459422023081
3.06129859997743 1.4
3.2 1.52814752085739
3.38196872386225 1.7
3.5 1.8135837073613
3.69230642085448 2
3.8 2.10582201370471
3.99746995623952 2.3
4.1 2.40175159130473
4.30005601025348 2.6
4.4 2.69962414764382
4.60136231829664 2.9
4.7 2.99850715391113
4.90203066297329 3.2
5 3.29791608530615
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.1 5
3.8 5
3.5 5
3.20860361247589 5
3.2 4.98344671459788
3.0970925906816 4.7
2.95097153857783 4.4
2.9 4.31313760510649
2.80625209446979 4.1
2.65424989690011 3.8
2.6 3.7042471662612
2.51371912416729 3.5
2.36759128495094 3.2
2.3 3.07953728899643
2.22100200085476 2.9
2.07026535986409 2.6
2 2.47636780990776
1.91747977381044 2.3
1.76501043901024 2
1.7 1.87775502067842
1.62036395260018 1.7
1.49252177366716 1.4
1.4 1.15844128711623
1.38125769682687 1.1
1.36280618480276 0.8
1.4 0.69602175314925
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.6 1.1
};
\coordinate (MCMC_mean_lml_t) at (axis cs:2.3,1.1);
\end{axis}



==> fig/tikz/echocardiogram/MCMC_mean_lml.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
3.2 4.91772315574936
3.5 4.88919420146702
3.8 4.92914387388733
3.97570817772518 5
3.8 5
3.5 5
3.2 5
3.06455126812895 5
3.2 4.91772315574936
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
2.9 4.87510780490077
3.2 4.72612110883283
3.5 4.71560126353787
3.8 4.76813351085414
4.1 4.87876057948272
4.37765594531042 5
4.1 5
3.97570817772518 5
3.8 4.92914387388733
3.5 4.88919420146702
3.2 4.91772315574936
3.06455126812895 5
2.9 5
2.7865245986378 5
2.9 4.87510780490077
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
3.2 4.3916001584582
3.22561236017764 4.4
3.5 4.45840213294571
3.8 4.54445147992283
4.09217246809941 4.7
4.1 4.70272051259192
4.4 4.79894521494665
4.7 4.93367388137257
4.93729891840107 5
4.7 5
4.4 5
4.37765594531042 5
4.1 4.87876057948272
3.8 4.76813351085414
3.5 4.71560126353787
3.2 4.72612110883283
2.9 4.87510780490077
2.7865245986378 5
2.6 5
2.52623424382574 5
2.6 4.88389506383018
2.75206889865113 4.7
2.9 4.52268135110161
3.17519873975904 4.4
3.2 4.3916001584582
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
-0.7 -1
-0.4 -1
-0.1 -1
0.2 -1
0.266759789121962 -1
0.2 -0.902947286382317
0.0773306123160817 -0.7
-0.0763601552133717 -0.4
-0.1 -0.33899262693692
-0.193306130362882 -0.1
-0.272078746996949 0.2
-0.321583498907524 0.5
-0.353183067732444 0.8
-0.384595198697933 1.1
-0.381833135352212 1.4
-0.384071598464404 1.7
-0.375397333746147 2
-0.4 2.29966557354184
-0.400034643071438 2.3
-0.414207628715078 2.6
-0.4 2.69996216712131
-0.375078351758091 2.9
-0.399622321991073 3.2
-0.39848705703767 3.5
-0.38831395222658 3.8
-0.385747259201743 4.1
-0.399002334647059 4.4
-0.4 4.42223451022915
-0.414821458094029 4.7
-0.4 4.80703518212581
-0.381194852923616 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
2.9 -1
3.2 -1
3.5 -1
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.5
5 0.8
5 1.1
5 1.4
5 1.66815746770342
4.7740033528416 1.4
4.7 1.31133492813727
4.52555511658744 1.1
4.4 0.954108915504737
4.26910527991133 0.8
4.1 0.598923786712073
4.01421574803925 0.5
3.8 0.248794671855185
3.7556135747852 0.2
3.5 -0.0931594540443076
3.49403404084006 -0.1
3.2431362101334 -0.4
3.2 -0.44834534322302
2.96322801672699 -0.7
2.9 -0.768244904075964
2.67550519348393 -1
2.9 -1
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
2.6 4.02717098349978
2.9 3.89785641916889
3.2 3.94481189352748
3.5 4.03381098871372
3.61320874043796 4.1
3.8 4.1923560916661
4.1 4.35580155079724
4.174225933897 4.4
4.4 4.51718188973637
4.7 4.65391152889212
4.79771953255564 4.7
5 4.76891928324504
5 5
4.93729891840107 5
4.7 4.93367388137257
4.4 4.79894521494665
4.1 4.70272051259192
4.09217246809941 4.7
3.8 4.54445147992283
3.5 4.45840213294571
3.22561236017764 4.4
3.2 4.3916001584582
3.17519873975904 4.4
2.9 4.52268135110161
2.75206889865113 4.7
2.6 4.88389506383018
2.52623424382574 5
2.3 5
2.14188616356761 5
2.26360812385338 4.7
2.3 4.58757176636508
2.37452398495957 4.4
2.54442581402706 4.1
2.6 4.02717098349978
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
0.2 -0.902947286382317
0.266759789121962 -1
0.5 -1
0.8 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.3 -1
2.6 -1
2.67550519348393 -1
2.9 -0.768244904075964
2.96322801672699 -0.7
3.2 -0.44834534322302
3.2431362101334 -0.4
3.49403404084006 -0.1
3.5 -0.0931594540443076
3.7556135747852 0.2
3.8 0.248794671855185
4.01421574803925 0.5
4.1 0.598923786712073
4.26910527991133 0.8
4.4 0.954108915504737
4.52555511658744 1.1
4.7 1.31133492813727
4.7740033528416 1.4
5 1.66815746770342
5 1.7
5 2
5 2.3
5 2.48577155246911
4.84241009051234 2.3
4.7 2.1475360330901
4.56796195774215 2
4.4 1.81914351421201
4.28918836548754 1.7
4.1 1.48024281744274
4.02892110638214 1.4
3.8 1.16131036223184
3.74208280588895 1.1
3.5 0.840589406221681
3.45964565994665 0.8
3.2 0.5268110656514
3.17398729279624 0.5
2.9 0.214808189505615
2.88446832022133 0.2
2.6 -0.0635446663760182
2.55804664244592 -0.1
2.3 -0.325477341890163
2.19328929646854 -0.4
2 -0.54481761316727
1.71148782064052 -0.7
1.7 -0.706242779798867
1.4 -0.789194332292585
1.1 -0.76495866089889
0.964423821852777 -0.7
0.8 -0.606430888862448
0.606124269071705 -0.4
0.5 -0.24973261577147
0.424209249207616 -0.1
0.320229056590322 0.2
0.254407721887344 0.5
0.200240238609763 0.8
0.2 0.821339299041248
0.197784465617757 1.1
0.197775852370963 1.4
0.179514819447238 1.7
0.190774845345903 2
0.183054005620865 2.3
0.196550179744192 2.6
0.175634292152275 2.9
0.187560052046637 3.2
0.160628757595659 3.5
0.2 3.6960823767791
0.22554086623571 3.8
0.2 3.91020123904279
0.167569187283226 4.1
0.162582612697315 4.4
0.173310943738844 4.7
0.165289085085439 5
-0.1 5
-0.381194852923616 5
-0.4 4.80703518212581
-0.414821458094029 4.7
-0.4 4.42223451022915
-0.399002334647059 4.4
-0.385747259201743 4.1
-0.38831395222658 3.8
-0.39848705703767 3.5
-0.399622321991073 3.2
-0.375078351758091 2.9
-0.4 2.69996216712131
-0.414207628715078 2.6
-0.400034643071438 2.3
-0.4 2.29966557354184
-0.375397333746147 2
-0.384071598464404 1.7
-0.381833135352212 1.4
-0.384595198697933 1.1
-0.353183067732444 0.8
-0.321583498907524 0.5
-0.272078746996949 0.2
-0.193306130362882 -0.1
-0.1 -0.33899262693692
-0.0763601552133717 -0.4
0.0773306123160817 -0.7
0.2 -0.902947286382317
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
2 2.88252486632849
2.3 2.74729496609349
2.6 2.86436638819567
2.65738690586667 2.9
2.9 3.02997029805087
3.13694351390101 3.2
3.2 3.23719802229956
3.5 3.46976198637041
3.54038752906044 3.5
3.8 3.68924634233184
3.97595144403008 3.8
4.1 3.86935709608467
4.4 4.06794175432599
4.44253618656643 4.1
4.7 4.26031804526757
5 4.39953501210795
5 4.4
5 4.7
5 4.76891928324504
4.79771953255564 4.7
4.7 4.65391152889212
4.4 4.51718188973637
4.174225933897 4.4
4.1 4.35580155079724
3.8 4.1923560916661
3.61320874043796 4.1
3.5 4.03381098871372
3.2 3.94481189352748
2.9 3.89785641916889
2.6 4.02717098349978
2.54442581402706 4.1
2.37452398495957 4.4
2.3 4.58757176636508
2.26360812385338 4.7
2.14188616356761 5
2 5
1.7 5
1.49333981043148 5
1.52130622985102 4.7
1.60323978318347 4.4
1.61850361847433 4.1
1.69967796613484 3.8
1.7 3.79308184781444
1.71427514640513 3.5
1.85117553717989 3.2
1.98480457082213 2.9
2 2.88252486632849
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.1 -0.76495866089889
1.4 -0.789194332292585
1.7 -0.706242779798867
1.71148782064052 -0.7
2 -0.54481761316727
2.19328929646854 -0.4
2.3 -0.325477341890163
2.55804664244592 -0.1
2.6 -0.0635446663760182
2.88446832022133 0.2
2.9 0.214808189505615
3.17398729279624 0.5
3.2 0.5268110656514
3.45964565994665 0.8
3.5 0.840589406221681
3.74208280588895 1.1
3.8 1.16131036223184
4.02892110638214 1.4
4.1 1.48024281744274
4.28918836548754 1.7
4.4 1.81914351421201
4.56796195774215 2
4.7 2.1475360330901
4.84241009051234 2.3
5 2.48577155246911
5 2.6
5 2.9
5 3.2
5 3.5
5 3.8
5 4.1
5 4.39953501210795
4.7 4.26031804526757
4.44253618656643 4.1
4.4 4.06794175432599
4.1 3.86935709608467
3.97595144403008 3.8
3.8 3.68924634233184
3.54038752906044 3.5
3.5 3.46976198637041
3.2 3.23719802229956
3.13694351390101 3.2
2.9 3.02997029805087
2.65738690586667 2.9
2.6 2.86436638819567
2.3 2.74729496609349
2 2.88252486632849
1.98480457082213 2.9
1.85117553717989 3.2
1.71427514640513 3.5
1.7 3.79308184781444
1.69967796613484 3.8
1.61850361847433 4.1
1.60323978318347 4.4
1.52130622985102 4.7
1.49333981043148 5
1.4 5
1.1 5
0.8 5
0.5 5
0.2 5
0.165289085085439 5
0.173310943738844 4.7
0.162582612697315 4.4
0.167569187283226 4.1
0.2 3.91020123904279
0.22554086623571 3.8
0.2 3.6960823767791
0.160628757595659 3.5
0.187560052046637 3.2
0.175634292152275 2.9
0.196550179744192 2.6
0.183054005620865 2.3
0.190774845345903 2
0.179514819447238 1.7
0.197775852370963 1.4
0.197784465617757 1.1
0.2 0.821339299041248
0.200240238609763 0.8
0.254407721887344 0.5
0.320229056590322 0.2
0.424209249207616 -0.1
0.5 -0.24973261577147
0.606124269071705 -0.4
0.8 -0.606430888862448
0.964423821852777 -0.7
1.1 -0.76495866089889

1.45871316329286 0.5
1.54154356647308 0.8
1.7 0.986369034006308
1.80460585262739 1.1
2 1.21151812656296
2.19179123752808 1.4
2.3 1.50578443302462
2.52304836897163 1.7
2.6 1.7579316894992
2.9 1.99708050513825
2.90394291492668 2
3.2 2.20151420323797
3.34492007840777 2.3
3.5 2.41176052609009
3.75939144909647 2.6
3.8 2.62585639069096
4.09866473295008 2.6
3.89877095744846 2.3
3.8 2.15887353245964
3.66090411724147 2
3.5 1.77187884564798
3.44827682831192 1.7
3.2 1.41528703811185
3.18843991707382 1.4
2.91118592135995 1.1
2.9 1.08814938475544
2.61259636289816 0.8
2.6 0.78823186077193
2.3 0.550925423907835
2.22737949647271 0.5
2 0.371579618846467
1.7 0.307133151794447
1.45871316329286 0.5
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
1.7 0.307133151794447
2 0.371579618846467
2.22737949647271 0.5
2.3 0.550925423907835
2.6 0.78823186077193
2.61259636289816 0.8
2.9 1.08814938475544
2.91118592135995 1.1
3.18843991707382 1.4
3.2 1.41528703811185
3.44827682831192 1.7
3.5 1.77187884564798
3.66090411724147 2
3.8 2.15887353245964
3.89877095744846 2.3
4.09866473295008 2.6
3.8 2.62585639069096
3.75939144909647 2.6
3.5 2.41176052609009
3.34492007840777 2.3
3.2 2.20151420323797
2.90394291492668 2
2.9 1.99708050513825
2.6 1.7579316894992
2.52304836897163 1.7
2.3 1.50578443302462
2.19179123752808 1.4
2 1.21151812656296
1.80460585262739 1.1
1.7 0.986369034006308
1.54154356647308 0.8
1.45871316329286 0.5
1.7 0.307133151794447
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.3 1.1
};
\coordinate (MCMC_mean_lml_t) at (axis cs:2.3,1.1);
\end{axis}



==> fig/tikz/echocardiogram/MCMC_nlpd.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
-0.7 -1
-0.4 -1
-0.1 -1
-0.0946239336597086 -1
-0.1 -0.987843004662823
-0.244942669247288 -0.7
-0.343978920927373 -0.4
-0.4 -0.154901566937889
-0.419223596756404 -0.1
-0.495461894783212 0.2
-0.541498472073756 0.5
-0.565355773779708 0.8
-0.581018723374253 1.1
-0.588475756293159 1.4
-0.593186633711579 1.7
-0.596433617260766 2
-0.596524267292175 2.3
-0.598160291288632 2.6
-0.598511828884898 2.9
-0.597733790287615 3.2
-0.5993751383829 3.5
-0.599899422950323 3.8
-0.599606997435496 4.1
-0.598009899341869 4.4
-0.599594132828508 4.7
-0.599549365224003 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
-0.1 -0.987843004662823
-0.0946239336597086 -1
0.2 -1
0.272816882948461 -1
0.2 -0.885359711612519
0.0993289072138745 -0.7
-0.0310145158872478 -0.4
-0.1 -0.194637459618441
-0.13332247978381 -0.1
-0.205885160690851 0.2
-0.25294259235996 0.5
-0.281314605054178 0.8
-0.297073660784284 1.1
-0.305334309418671 1.4
-0.310162632908927 1.7
-0.313087840552749 2
-0.313608618221665 2.3
-0.315185382798003 2.6
-0.314819441047424 2.9
-0.314974512777755 3.2
-0.316167748293179 3.5
-0.315758483234045 3.8
-0.316964118579501 4.1
-0.314982399099884 4.4
-0.31609084648631 4.7
-0.316750744336577 5
-0.4 5
-0.599549365224003 5
-0.599594132828508 4.7
-0.598009899341869 4.4
-0.599606997435497 4.1
-0.599899422950323 3.8
-0.5993751383829 3.5
-0.597733790287615 3.2
-0.598511828884898 2.9
-0.598160291288632 2.6
-0.596524267292175 2.3
-0.596433617260766 2
-0.593186633711579 1.7
-0.588475756293159 1.4
-0.581018723374253 1.1
-0.565355773779708 0.8
-0.541498472073756 0.5
-0.495461894783212 0.2
-0.419223596756404 -0.1
-0.4 -0.154901566937889
-0.343978920927373 -0.4
-0.244942669247288 -0.7
-0.1 -0.987843004662823
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
4.4 -1
4.7 -1
5 -1
5 -0.86756355721787
4.7 -0.9003230662054
4.4 -0.963330247367661
4.27162343941795 -1
4.4 -1
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
0.2 -0.885359711612519
0.272816882948461 -1
0.5 -1
0.681103136563752 -1
0.5 -0.825326284252711
0.416356511653707 -0.7
0.240439926490315 -0.4
0.2 -0.318284673024522
0.116744773891604 -0.1
0.0366975226811869 0.2
-0.0185380391893069 0.5
-0.0537492030107922 0.8
-0.0734941997436824 1.1
-0.0814275712929262 1.4
-0.0872212190060214 1.7
-0.0891539947388753 2
-0.0920882636393097 2.3
-0.0921239246764125 2.6
-0.091884681275061 2.9
-0.0933980271230276 3.2
-0.0922554964958181 3.5
-0.0946608751460168 3.8
-0.0934819619377508 4.1
-0.0933224524848282 4.4
-0.0928292543224212 4.7
-0.0935190771937688 5
-0.1 5
-0.316750744336577 5
-0.31609084648631 4.7
-0.314982399099884 4.4
-0.316964118579501 4.1
-0.315758483234045 3.8
-0.316167748293179 3.5
-0.314974512777755 3.2
-0.314819441047424 2.9
-0.315185382798003 2.6
-0.313608618221665 2.3
-0.313087840552749 2
-0.310162632908927 1.7
-0.305334309418671 1.4
-0.297073660784284 1.1
-0.281314605054178 0.8
-0.25294259235996 0.5
-0.205885160690851 0.2
-0.13332247978381 -0.1
-0.1 -0.194637459618441
-0.0310145158872478 -0.4
0.0993289072138745 -0.7
0.2 -0.885359711612519
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
2.3 -1
2.6 -1
2.9 -1
3.2 -1
3.5 -1
3.8 -1
4.1 -1
4.27162343941795 -1
4.4 -0.963330247367661
4.7 -0.9003230662054
5 -0.86756355721787
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.5
5 0.8
5 1.1
5 1.4
5 1.60791075721644
4.78620332894573 1.4
4.7 1.31492619247853
4.48613147887459 1.1
4.4 1.01355310938419
4.1805343610595 0.8
4.1 0.721650438942313
3.8841605250972 0.5
3.8 0.41642784758262
3.57084371326306 0.2
3.5 0.132742111115919
3.26209036219545 -0.1
3.2 -0.15643654963817
2.91396172689374 -0.4
2.9 -0.412940663151524
2.6 -0.678162860941578
2.57165357361352 -0.7
2.3 -0.91152006881819
2.16161069129241 -1
2.3 -1
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
0.5 -0.825326284252711
0.681103136563752 -1
0.8 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.16161069129241 -1
2.3 -0.91152006881819
2.57165357361352 -0.7
2.6 -0.678162860941578
2.9 -0.412940663151524
2.91396172689374 -0.4
3.2 -0.15643654963817
3.26209036219545 -0.1
3.5 0.132742111115919
3.57084371326306 0.2
3.8 0.41642784758262
3.8841605250972 0.5
4.1 0.721650438942313
4.1805343610595 0.8
4.4 1.01355310938419
4.48613147887459 1.1
4.7 1.31492619247853
4.78620332894573 1.4
5 1.60791075721644
5 1.7
5 2
5 2.20662821837755
4.79439424614699 2
4.7 1.90309596856351
4.49115017072904 1.7
4.4 1.61031003302273
4.19582101805868 1.4
4.1 1.30196236492272
3.8914608273738 1.1
3.8 1.01166122481176
3.58055678013004 0.8
3.5 0.720272681655889
3.2674520908817 0.5
3.2 0.435401123982867
2.94245453761031 0.2
2.9 0.160578556808407
2.60190742308587 -0.1
2.6 -0.101676997566426
2.3 -0.342048360695865
2.21393132934092 -0.4
2 -0.548058043042619
1.7 -0.699449861732663
1.69810246674164 -0.7
1.4 -0.783575116396992
1.1 -0.764504484690187
0.961485854369083 -0.7
0.8 -0.61716621499973
0.597450962694636 -0.4
0.5 -0.282099962814807
0.408535401241156 -0.1
0.296557617309591 0.2
0.21791311465643 0.5
0.2 0.619938961534664
0.179895384761638 0.8
0.163868307855527 1.1
0.155601826387836 1.4
0.153735800000263 1.7
0.152001808190364 2
0.155064162555397 2.3
0.152280089232774 2.6
0.154028539998024 2.9
0.151118512014191 3.2
0.154000783001966 3.5
0.151138062342658 3.8
0.150349085827647 4.1
0.155167081198613 4.4
0.150665623628191 4.7
0.151593280291427 5
-0.0935190771937688 5
-0.0928292543224212 4.7
-0.0933224524848282 4.4
-0.0934819619377508 4.1
-0.0946608751460168 3.8
-0.0922554964958181 3.5
-0.0933980271230276 3.2
-0.091884681275061 2.9
-0.0921239246764125 2.6
-0.0920882636393098 2.3
-0.0891539947388753 2
-0.0872212190060214 1.7
-0.0814275712929262 1.4
-0.0734941997436824 1.1
-0.0537492030107922 0.8
-0.0185380391893069 0.5
0.036697522681187 0.2
0.116744773891604 -0.1
0.2 -0.318284673024522
0.240439926490315 -0.4
0.416356511653707 -0.7
0.5 -0.825326284252711
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
1.1 -0.764504484690187
1.4 -0.783575116396992
1.69810246674164 -0.7
1.7 -0.699449861732663
2 -0.548058043042619
2.21393132934092 -0.4
2.3 -0.342048360695865
2.6 -0.101676997566426
2.60190742308587 -0.1
2.9 0.160578556808407
2.94245453761031 0.2
3.2 0.435401123982867
3.2674520908817 0.5
3.5 0.720272681655889
3.58055678013004 0.8
3.8 1.01166122481176
3.8914608273738 1.1
4.1 1.30196236492272
4.19582101805869 1.4
4.4 1.61031003302273
4.49115017072904 1.7
4.7 1.90309596856351
4.79439424614699 2
5 2.20662821837755
5 2.3
5 2.6
5 2.72411489774831
4.87655485902451 2.6
4.7 2.42238401952755
4.57808671114043 2.3
4.4 2.13362660305523
4.26847411406693 2
4.1 1.8261133753294
3.97482002997147 1.7
3.8 1.52641634519642
3.6672365491672 1.4
3.5 1.24157212028579
3.3525588742344 1.1
3.2 0.948818335537411
3.03159420261681 0.8
2.9 0.67980157405344
2.69905138659693 0.5
2.6 0.417279439391928
2.32873205284756 0.2
2.3 0.176539686778226
2 -0.0110978843906045
1.81782367119613 -0.1
1.7 -0.156692591994922
1.4 -0.226581490605269
1.1 -0.184023359436941
0.938362372799517 -0.1
0.8 0.00195005402399398
0.682369332821338 0.2
0.549228439739566 0.5
0.5 0.724847263194276
0.489680941097487 0.8
0.476241226433633 1.1
0.469161206467281 1.4
0.476711005231383 1.7
0.479731644862284 2
0.487054542334403 2.3
0.491598843485777 2.6
0.494660256147144 2.9
0.49636027696789 3.2
0.5 3.35649586998575
0.505504455546648 3.5
0.5 3.57543643796455
0.490281950132312 3.8
0.49669948338467 4.1
0.49690479636988 4.4
0.489539318005555 4.7
0.498506160451036 5
0.2 5
0.151593280291427 5
0.150665623628191 4.7
0.155167081198613 4.4
0.150349085827647 4.1
0.151138062342658 3.8
0.154000783001966 3.5
0.151118512014191 3.2
0.154028539998024 2.9
0.152280089232774 2.6
0.155064162555397 2.3
0.152001808190364 2
0.153735800000263 1.7
0.155601826387836 1.4
0.163868307855527 1.1
0.179895384761638 0.8
0.2 0.619938961534664
0.21791311465643 0.5
0.296557617309591 0.2
0.408535401241156 -0.1
0.5 -0.282099962814807
0.597450962694636 -0.4
0.8 -0.61716621499973
0.961485854369083 -0.7
1.1 -0.764504484690187
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
1.1 -0.184023359436941
1.4 -0.226581490605269
1.7 -0.156692591994922
1.81782367119613 -0.1
2 -0.0110978843906045
2.3 0.176539686778226
2.32873205284756 0.2
2.6 0.417279439391928
2.69905138659693 0.5
2.9 0.67980157405344
3.03159420261681 0.8
3.2 0.948818335537411
3.3525588742344 1.1
3.5 1.24157212028579
3.6672365491672 1.4
3.8 1.52641634519642
3.97482002997147 1.7
4.1 1.8261133753294
4.26847411406693 2
4.4 2.13362660305523
4.57808671114043 2.3
4.7 2.42238401952755
4.87655485902451 2.6
5 2.72411489774831
5 2.9
5 3.2
5 3.46883783042021
4.75707224507519 3.2
4.7 3.14289793655815
4.46859123643294 2.9
4.4 2.82826186556168
4.18721969239951 2.6
4.1 2.50759849135261
3.88756954515049 2.3
3.8 2.21460791322987
3.58328781352137 2
3.5 1.92166187237704
3.27741580417604 1.7
3.2 1.62308347780292
2.96096108012443 1.4
2.9 1.34632271797629
2.6194615920508 1.1
2.6 1.08439297933429
2.3 0.87905640215432
2.16846729554221 0.8
2 0.698335147405332
1.7 0.594679475000757
1.4 0.585605640900419
1.12832714225241 0.8
1.1 0.85004072603639
1.03735031837873 1.1
1.0173156073749 1.4
1.05527008741274 1.7
1.09049680704263 2
1.1 2.05432732895405
1.15799127798382 2.3
1.21028082333062 2.6
1.2707127737547 2.9
1.36667171786714 3.2
1.38973437419602 3.5
1.4 3.5605157980779
1.44823010360968 3.8
1.48034209563683 4.1
1.4928354519842 4.4
1.52467824393677 4.7
1.46557745868983 5
1.4 5
1.1 5
0.8 5
0.5 5
0.498506160451036 5
0.489539318005555 4.7
0.49690479636988 4.4
0.49669948338467 4.1
0.490281950132312 3.8
0.5 3.57543643796455
0.505504455546648 3.5
0.5 3.35649586998575
0.49636027696789 3.2
0.494660256147144 2.9
0.491598843485777 2.6
0.487054542334403 2.3
0.479731644862284 2
0.476711005231383 1.7
0.469161206467281 1.4
0.476241226433633 1.1
0.489680941097487 0.8
0.5 0.724847263194276
0.549228439739566 0.5
0.682369332821338 0.2
0.8 0.00195005402399401
0.938362372799517 -0.1
1.1 -0.184023359436941
};
\addplot [draw=none, fill=lavender231240249]
table{%
x  y
1.4 0.585605640900419
1.7 0.594679475000757
2 0.698335147405332
2.16846729554221 0.8
2.3 0.87905640215432
2.6 1.08439297933429
2.6194615920508 1.1
2.9 1.34632271797629
2.96096108012443 1.4
3.2 1.62308347780292
3.27741580417604 1.7
3.5 1.92166187237704
3.58328781352137 2
3.8 2.21460791322987
3.88756954515049 2.3
4.1 2.50759849135261
4.18721969239951 2.6
4.4 2.82826186556168
4.46859123643294 2.9
4.7 3.14289793655815
4.75707224507519 3.2
5 3.46883783042021
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.1 5
3.8 5
3.5 5
3.2 5
3.07153377678521 5
3.2 4.8229592080973
3.22464637283352 4.7
3.33127419426143 4.4
3.30365647260378 4.1
3.2 3.8421788192515
3.17499417034303 3.8
3.09777691045014 3.5
2.9 3.23634433541472
2.84103707105713 3.2
2.6 2.92291211710651
2.3 3.05071203410537
2.27950511047496 3.2
2.3 3.26198145050935
2.46446645550649 3.5
2.50839011362308 3.8
2.5948269807936 4.1
2.6 4.13150792322203
2.66588381333129 4.4
2.80844469428624 4.7
2.85461341557778 5
2.6 5
2.3 5
2 5
1.7 5
1.46557745868983 5
1.52467824393677 4.7
1.4928354519842 4.4
1.48034209563683 4.1
1.44823010360968 3.8
1.4 3.5605157980779
1.38973437419602 3.5
1.36667171786714 3.2
1.2707127737547 2.9
1.21028082333062 2.6
1.15799127798382 2.3
1.1 2.05432732895405
1.09049680704263 2
1.05527008741274 1.7
1.0173156073749 1.4
1.03735031837873 1.1
1.1 0.85004072603639
1.12832714225241 0.8
1.4 0.585605640900419
};
\addplot [draw=none, fill=aliceblue242247253]
table{%
x  y
2.3 3.05071203410537
2.6 2.92291211710651
2.84103707105713 3.2
2.9 3.23634433541472
3.09777691045014 3.5
3.17499417034303 3.8
3.2 3.8421788192515
3.30365647260378 4.1
3.33127419426143 4.4
3.22464637283352 4.7
3.2 4.8229592080973
3.07153377678521 5
2.9 5
2.85461341557778 5
2.80844469428624 4.7
2.66588381333129 4.4
2.6 4.13150792322203
2.5948269807936 4.1
2.50839011362308 3.8
2.46446645550649 3.5
2.3 3.26198145050935
2.27950511047496 3.2
2.3 3.05071203410537
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.3 1.1
};
\coordinate (CVI_mean_lml_b) at (axis cs:2.3,1.1);
\coordinate (CVI_mean_lml_ep_b) at (axis cs:2.3,1.1);
\end{axis}



==> fig/tikz/ionosphere/CVI_Z_mean_lml.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=black]
table{%
x  y
-0.887803536370183 2.3
-0.7 2.47818948030274
-0.619836284829823 2.6
-0.429266129003946 2.9
-0.4 2.95368923791362
-0.296020630545507 3.2
-0.174896990494099 3.5
-0.1 3.6844980636142
-0.055781372560884 3.8
0.0421805590940537 4.1
0.124094139322306 4.4
0.2 4.6682411330791
0.210431818487413 4.7
0.318010113820088 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2.19126598321229
-0.887803536370183 2.3
};
\addplot [draw=none, fill=midnightblue854116]
table{%
x  y
-0.909446355770153 2
-0.7 2.20270452217322
-0.637039238536336 2.3
-0.44246920336234 2.6
-0.4 2.66739635607674
-0.288035531188239 2.9
-0.165476329424148 3.2
-0.1 3.36552324573427
-0.0487960853713571 3.5
0.0634280330946776 3.8
0.157213913258208 4.1
0.2 4.25889439168267
0.244878516297484 4.4
0.34199762025272 4.7
0.445217176698017 5
0.318010113820088 5
0.210431818487413 4.7
0.2 4.6682411330791
0.124094139322306 4.4
0.0421805590940536 4.1
-0.055781372560884 3.8
-0.1 3.6844980636142
-0.174896990494099 3.5
-0.296020630545507 3.2
-0.4 2.95368923791362
-0.429266129003946 2.9
-0.619836284829823 2.6
-0.7 2.47818948030274
-0.887803536370183 2.3
-1 2.19126598321229
-1 2
-1 1.91034818876569
-0.909446355770153 2
};
\addplot [draw=none, fill=midnightblue868137]
table{%
x  y
-0.911612615541082 1.7
-0.7 1.90940202672529
-0.642654608677494 2
-0.451230327181388 2.3
-0.4 2.37981927645212
-0.291075697405879 2.6
-0.152548092906617 2.9
-0.1 3.0312828177877
-0.0343789430855926 3.2
0.0768614486752001 3.5
0.182637438750239 3.8
0.2 3.85647425456165
0.28741016486835 4.1
0.380748649058974 4.4
0.473563422018026 4.7
0.5 4.77825916121389
0.588310157793602 5
0.5 5
0.445217176698017 5
0.34199762025272 4.7
0.244878516297484 4.4
0.2 4.25889439168267
0.157213913258208 4.1
0.0634280330946776 3.8
-0.0487960853713571 3.5
-0.1 3.36552324573427
-0.165476329424148 3.2
-0.288035531188239 2.9
-0.4 2.66739635607674
-0.44246920336234 2.6
-0.637039238536336 2.3
-0.7 2.20270452217322
-0.909446355770153 2
-1 1.91034818876569
-1 1.7
-1 1.60262986792633
-0.911612615541082 1.7
};
\addplot [draw=none, fill=teal882156]
table{%
x  y
-0.866396441787389 1.4
-0.7 1.58421566770659
-0.634296303225982 1.7
-0.447635129721808 2
-0.4 2.07565743655085
-0.290693544179744 2.3
-0.147859318294695 2.6
-0.1 2.70593815468761
-0.0162761030295962 2.9
0.0972749995576437 3.2
0.2 3.49248552318655
0.203035120957713 3.5
0.323020298222182 3.8
0.426586147733769 4.1
0.5 4.34353040627111
0.520677355560144 4.4
0.629433945849478 4.7
0.743419494957307 5
0.588310157793602 5
0.5 4.77825916121389
0.473563422018026 4.7
0.380748649058974 4.4
0.28741016486835 4.1
0.2 3.85647425456165
0.182637438750239 3.8
0.0768614486752001 3.5
-0.0343789430855926 3.2
-0.1 3.0312828177877
-0.152548092906617 2.9
-0.291075697405879 2.6
-0.4 2.37981927645212
-0.451230327181388 2.3
-0.642654608677494 2
-0.7 1.90940202672529
-0.911612615541082 1.7
-1 1.60262986792633
-1 1.4
-1 1.22118687376234
-0.866396441787389 1.4
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 -1
-0.63023181870719 -1
-0.7 -0.842671506766909
-0.784568151738941 -0.7
-0.915499616444636 -0.4
-0.98973676037331 -0.1
-1 -0.000135601022570403
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.993110320219683 0.5
-0.905967038620477 0.8
-0.751916674413362 1.1
-0.7 1.17071846372481
-0.594358904607223 1.4
-0.429198977201722 1.7
-0.4 1.74755544704623
-0.280093238640615 2
-0.139777158153298 2.3
-0.1 2.38507811083795
-0.00408642508117368 2.6
0.120492957205753 2.9
0.2 3.11770831388228
0.235047557552763 3.2
0.354439817697037 3.5
0.467012748063868 3.8
0.5 3.89795748164492
0.583281658333042 4.1
0.689729159444706 4.4
0.791416316198089 4.7
0.8 4.72309958486296
0.907857072284553 5
0.8 5
0.743419494957307 5
0.629433945849478 4.7
0.520677355560144 4.4
0.5 4.34353040627111
0.426586147733769 4.1
0.323020298222182 3.8
0.203035120957713 3.5
0.2 3.49248552318655
0.0972749995576437 3.2
-0.0162761030295962 2.9
-0.1 2.70593815468761
-0.147859318294695 2.6
-0.290693544179744 2.3
-0.4 2.07565743655085
-0.447635129721808 2
-0.634296303225982 1.7
-0.7 1.58421566770659
-0.866396441787389 1.4
-1 1.22118687376234
-1 1.1
-1 0.8
-1 0.5
-1 0.408070540499119
-0.993110320219683 0.5
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.7 -0.842671506766909
-0.63023181870719 -1
-0.4 -1
-0.132291427040298 -1
-0.310431878482001 -0.7
-0.4 -0.494390936535004
-0.448671626690947 -0.4
-0.562400693593726 -0.1
-0.623639813109658 0.2
-0.635767686442034 0.5
-0.596686694308942 0.8
-0.507954661705399 1.1
-0.4 1.34891201838415
-0.382716070129897 1.4
-0.256211115050857 1.7
-0.121432198678606 2
-0.1 2.04649913707812
0.0127629667261701 2.3
0.139965780281142 2.6
0.2 2.74965464337609
0.270215716210392 2.9
0.394546964748395 3.2
0.5 3.48345044862309
0.507468257639685 3.5
0.642757284219381 3.8
0.759535173046664 4.1
0.8 4.21930673765459
0.863647299696693 4.4
0.967209197104609 4.7
1.07765142212448 5
0.907857072284553 5
0.8 4.72309958486296
0.791416316198089 4.7
0.689729159444706 4.4
0.583281658333042 4.1
0.5 3.89795748164492
0.467012748063868 3.8
0.354439817697037 3.5
0.235047557552763 3.2
0.2 3.11770831388228
0.120492957205753 2.9
-0.00408642508117368 2.6
-0.1 2.38507811083795
-0.139777158153298 2.3
-0.280093238640615 2
-0.4 1.74755544704623
-0.429198977201722 1.7
-0.594358904607223 1.4
-0.7 1.17071846372481
-0.751916674413362 1.1
-0.905967038620477 0.8
-0.993110320219683 0.5
-1 0.408070540499119
-1 0.2
-1 -0.000135601022570403
-0.98973676037331 -0.1
-0.915499616444636 -0.4
-0.784568151738941 -0.7
-0.7 -0.842671506766909
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.42682811095723
4.79507214898701 0.2
4.7 0.0952664273934251
4.52292525358075 -0.1
4.4 -0.234406231017718
4.24874108529173 -0.4
4.1 -0.560390214231539
3.97065675639507 -0.7
3.8 -0.879343268668054
3.685061154761 -1
3.8 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
-0.1 -1
0.184492798672959 -1
-0.01305187295772 -0.7
-0.1 -0.533474619903749
-0.170753974246655 -0.4
-0.28841860262527 -0.1
-0.359667325844168 0.2
-0.386082601145852 0.5
-0.366308291197467 0.8
-0.303184805642335 1.1
-0.206217471564188 1.4
-0.1 1.66943323069862
-0.088286156213178 1.7
0.040165151119247 2
0.165884234001464 2.3
0.2 2.38292383779893
0.303337065119393 2.6
0.437924399016145 2.9
0.5 3.05661987398538
0.568403392194062 3.2
0.700936730584654 3.5
0.8 3.73172472935393
0.830406414533106 3.8
0.947406956109716 4.1
1.04669450097912 4.4
1.1 4.56204365313521
1.14588185974249 4.7
1.25436515956689 5
1.1 5
1.07765142212448 5
0.967209197104609 4.7
0.863647299696693 4.4
0.8 4.21930673765459
0.759535173046664 4.1
0.642757284219381 3.8
0.507468257639685 3.5
0.5 3.48345044862309
0.394546964748395 3.2
0.270215716210392 2.9
0.2 2.74965464337609
0.139965780281142 2.6
0.0127629667261701 2.3
-0.1 2.04649913707812
-0.121432198678606 2
-0.256211115050857 1.7
-0.382716070129897 1.4
-0.4 1.34891201838415
-0.507954661705399 1.1
-0.596686694308942 0.8
-0.635767686442034 0.5
-0.623639813109658 0.2
-0.562400693593726 -0.1
-0.448671626690947 -0.4
-0.4 -0.494390936535004
-0.310431878482001 -0.7
-0.132291427040298 -1
-0.1 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
3.2 -1
3.5 -1
3.685061154761 -1
3.8 -0.879343268668054
3.97065675639507 -0.7
4.1 -0.560390214231539
4.24874108529173 -0.4
4.4 -0.234406231017718
4.52292525358075 -0.1
4.7 0.0952664273934251
4.79507214898701 0.2
5 0.42682811095723
5 0.5
5 0.8
5 1.09428510928327
4.71836234957136 0.8
4.7 0.780816384650542
4.43089473949017 0.5
4.4 0.467761846589516
4.14264421673528 0.2
4.1 0.155609367604578
3.85276474368825 -0.1
3.8 -0.154655398173025
3.55961635852971 -0.4
3.5 -0.461141719586737
3.26008438111652 -0.7
3.2 -0.760403116911697
2.9480939131654 -1
3.2 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
0.2 -1
0.479255325230415 -1
0.247784192472104 -0.7
0.2 -0.627556100427295
0.0695894990491935 -0.4
-0.058865877695452 -0.1
-0.1 0.0415499705682803
-0.145484626755543 0.2
-0.183594963890442 0.5
-0.172757311546239 0.8
-0.118026942188554 1.1
-0.1 1.15893972412165
-0.0278192127499779 1.4
0.083285818477204 1.7
0.2 1.99407508591922
0.202748932580916 2
0.346205164810557 2.3
0.480512606905033 2.6
0.5 2.64459926631278
0.634299000687848 2.9
0.770272641001781 3.2
0.8 3.26954754089552
0.902672376658098 3.5
1.03195126762173 3.8
1.1 3.98753582743597
1.13950528444993 4.1
1.23446426836409 4.4
1.33094606756315 4.7
1.4 4.90210656115945
1.43816244046763 5
1.4 5
1.25436515956689 5
1.14588185974249 4.7
1.1 4.56204365313521
1.04669450097912 4.4
0.947406956109716 4.1
0.830406414533106 3.8
0.8 3.73172472935393
0.700936730584654 3.5
0.568403392194062 3.2
0.5 3.05661987398538
0.437924399016145 2.9
0.303337065119393 2.6
0.2 2.38292383779893
0.165884234001464 2.3
0.040165151119247 2
-0.088286156213178 1.7
-0.1 1.66943323069862
-0.206217471564188 1.4
-0.303184805642335 1.1
-0.366308291197467 0.8
-0.386082601145852 0.5
-0.359667325844168 0.2
-0.28841860262527 -0.1
-0.170753974246655 -0.4
-0.1 -0.53347461990375
-0.01305187295772 -0.7
0.184492798672959 -1
0.2 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
2.6 -1
2.9 -1
2.9480939131654 -1
3.2 -0.760403116911697
3.26008438111652 -0.7
3.5 -0.461141719586737
3.55961635852971 -0.4
3.8 -0.154655398173025
3.85276474368825 -0.1
4.1 0.155609367604578
4.14264421673528 0.2
4.4 0.467761846589516
4.43089473949017 0.5
4.7 0.780816384650542
4.71836234957136 0.8
5 1.09428510928327
5 1.1
5 1.4
5 1.47533724051483
4.92695513125589 1.4
4.7 1.16648177320797
4.63558191456139 1.1
4.4 0.857762264042404
4.34401253823331 0.8
4.1 0.549564283484414
4.05180124816645 0.5
3.8 0.242766327842122
3.7579875310366 0.2
3.5 -0.0608765621536276
3.46064326037089 -0.1
3.2 -0.358243830418478
3.15596211224053 -0.4
2.9 -0.644301638648233
2.83611164061451 -0.7
2.6 -0.91132439731082
2.48332981395457 -1
2.6 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.5 -1
0.8 -1
0.851794670990709 -1
0.8 -0.970535633122456
0.518911950234126 -0.7
0.5 -0.679296397106257
0.311496769448637 -0.4
0.2 -0.192127890278311
0.157956712225812 -0.1
0.0643437686376515 0.2
0.0192686822014385 0.5
0.0231785743204161 0.8
0.0715661943776383 1.1
0.153450045961865 1.4
0.2 1.53362559126815
0.26828948278652 1.7
0.403317552088578 2
0.5 2.21762645374143
0.543886705034136 2.3
0.701884520848107 2.6
0.8 2.79798820047189
0.850762918965214 2.9
0.985281650177575 3.2
1.1 3.46839208382114
1.11327709480669 3.5
1.23450675729973 3.8
1.33461411337859 4.1
1.4 4.31735358838645
1.42905569074237 4.4
1.53929760744775 4.7
1.64931530844711 5
1.43816244046763 5
1.4 4.90210656115945
1.33094606756315 4.7
1.23446426836409 4.4
1.13950528444993 4.1
1.1 3.98753582743597
1.03195126762173 3.8
0.902672376658098 3.5
0.8 3.26954754089552
0.770272641001781 3.2
0.634299000687848 2.9
0.5 2.64459926631278
0.480512606905033 2.6
0.346205164810557 2.3
0.202748932580916 2
0.2 1.99407508591922
0.083285818477204 1.7
-0.0278192127499779 1.4
-0.1 1.15893972412165
-0.118026942188554 1.1
-0.172757311546239 0.8
-0.183594963890442 0.5
-0.145484626755543 0.2
-0.1 0.0415499705682803
-0.058865877695452 -0.1
0.0695894990491935 -0.4
0.2 -0.627556100427295
0.247784192472104 -0.7
0.479255325230415 -1
0.5 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
2.3 -1
2.48332981395457 -1
2.6 -0.91132439731082
2.83611164061451 -0.7
2.9 -0.644301638648233
3.15596211224053 -0.4
3.2 -0.358243830418478
3.46064326037089 -0.1
3.5 -0.0608765621536276
3.7579875310366 0.2
3.8 0.242766327842122
4.05180124816645 0.5
4.1 0.549564283484414
4.34401253823331 0.8
4.4 0.857762264042404
4.63558191456139 1.1
4.7 1.16648177320797
4.92695513125589 1.4
5 1.47533724051483
5 1.7
5 1.79864262907917
4.90455046336539 1.7
4.7 1.48947733796043
4.61366460134067 1.4
4.4 1.17999341138807
4.32302235702601 1.1
4.1 0.870466346039979
4.03221604029522 0.8
3.8 0.561773177019761
3.74019751186367 0.5
3.5 0.255902799821756
3.44474530765838 0.2
3.2 -0.0434461126404508
3.14144520769044 -0.1
2.9 -0.330343081806941
2.82127196294381 -0.4
2.6 -0.596208526424875
2.4638400039619 -0.7
2.3 -0.828914394497196
2.01609802089176 -1
2.3 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
0.8 -0.970535633122456
0.851794670990709 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.01609802089176 -1
2.3 -0.828914394497196
2.4638400039619 -0.7
2.6 -0.596208526424875
2.82127196294381 -0.4
2.9 -0.330343081806941
3.14144520769044 -0.1
3.2 -0.0434461126404508
3.44474530765838 0.2
3.5 0.255902799821756
3.74019751186367 0.5
3.8 0.561773177019761
4.03221604029522 0.8
4.1 0.87046634603998
4.32302235702601 1.1
4.4 1.17999341138807
4.61366460134067 1.4
4.7 1.48947733796043
4.90455046336539 1.7
5 1.79864262907917
5 2
5 2.10989261800648
4.8943949612319 2
4.7 1.7989778392269
4.6054769143076 1.7
4.4 1.48694607033075
4.31755809145606 1.4
4.1 1.1738749345094
4.03033469100125 1.1
3.8 0.860598571105965
3.742770024722 0.8
3.5 0.54936765382172
3.45257826911243 0.5
3.2 0.244546531968065
3.15525759608111 0.2
2.9 -0.0468929403683035
2.84167716467335 -0.1
2.6 -0.315235948266921
2.49085294260741 -0.4
2.3 -0.547945459935491
2.04512542945021 -0.7
2 -0.728023509531562
1.7 -0.843421819032086
1.4 -0.876807476093009
1.1 -0.813638660333255
0.903670295377008 -0.7
0.8 -0.630595760926061
0.589239322949432 -0.4
0.5 -0.279379708702474
0.402671562499095 -0.1
0.287964244110737 0.2
0.227636192594315 0.5
0.22565489540932 0.8
0.277183898600127 1.1
0.368336153788844 1.4
0.481870101614457 1.7
0.5 1.74224253935396
0.633047415969727 2
0.784418363224941 2.3
0.8 2.33073849034778
0.937751288710557 2.6
1.07853772938204 2.9
1.1 2.94992127392992
1.20443696553841 3.2
1.32680764200465 3.5
1.4 3.69482403492226
1.4440074567179 3.8
1.55391065672918 4.1
1.65707253051483 4.4
1.7 4.52144162922679
1.7817155393907 4.7
1.91352582600865 5
1.7 5
1.64931530844711 5
1.53929760744775 4.7
1.42905569074237 4.4
1.4 4.31735358838645
1.33461411337859 4.1
1.23450675729973 3.8
1.11327709480669 3.5
1.1 3.46839208382114
0.985281650177575 3.2
0.850762918965214 2.9
0.8 2.79798820047189
0.701884520848107 2.6
0.543886705034136 2.3
0.5 2.21762645374143
0.403317552088578 2
0.26828948278652 1.7
0.2 1.53362559126815
0.153450045961865 1.4
0.0715661943776383 1.1
0.0231785743204161 0.8
0.0192686822014385 0.5
0.0643437686376515 0.2
0.157956712225812 -0.1
0.2 -0.192127890278311
0.311496769448637 -0.4
0.5 -0.679296397106257
0.518911950234127 -0.7
0.8 -0.970535633122456
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.1 -0.813638660333255
1.4 -0.876807476093009
1.7 -0.843421819032085
2 -0.728023509531562
2.04512542945021 -0.7
2.3 -0.547945459935491
2.49085294260741 -0.4
2.6 -0.315235948266921
2.84167716467335 -0.1
2.9 -0.0468929403683035
3.15525759608111 0.2
3.2 0.244546531968065
3.45257826911243 0.5
3.5 0.54936765382172
3.742770024722 0.8
3.8 0.860598571105964
4.03033469100125 1.1
4.1 1.1738749345094
4.31755809145606 1.4
4.4 1.48694607033075
4.6054769143076 1.7
4.7 1.7989778392269
4.8943949612319 2
5 2.10989261800648
5 2.3
5 2.43964152761299
4.86754630963297 2.3
4.7 2.1250010981363
4.58277864155129 2
4.4 1.80785937585093
4.30019608448168 1.7
4.1 1.48804321752152
4.01948528199203 1.4
3.8 1.16643292633569
3.7394631714852 1.1
3.5 0.845764946425047
3.45770579412384 0.8
3.2 0.531342976561558
3.16973638515701 0.5
2.9 0.231473544988786
2.86672007000874 0.2
2.6 -0.0425311254433255
2.52819496447896 -0.1
2.3 -0.276976331062678
2.09390102755816 -0.4
2 -0.455884452422189
1.7 -0.556694997716268
1.4 -0.56579981625454
1.1 -0.467735858067864
1.00110454276309 -0.4
0.8 -0.220973823770508
0.710566493260102 -0.1
0.553646100096357 0.2
0.5 0.393182504321219
0.47828400775194 0.5
0.472045780396354 0.8
0.5 0.991974887942755
0.519890523883599 1.1
0.622986580811739 1.4
0.751735265863648 1.7
0.8 1.80016339814715
0.896019677804993 2
1.04052938898391 2.3
1.1 2.42324484504998
1.18129237025043 2.6
1.30878901766637 2.9
1.4 3.13193646071076
1.43075994985088 3.2
1.56488848742918 3.5
1.68182646983992 3.8
1.7 3.85147925286483
1.81496333742358 4.1
1.94731761295523 4.4
2 4.51966820850448
2.10348290542745 4.7
2.26533572554098 5
2 5
1.91352582600865 5
1.7817155393907 4.7
1.7 4.52144162922679
1.65707253051483 4.4
1.55391065672918 4.1
1.4440074567179 3.8
1.4 3.69482403492226
1.32680764200465 3.5
1.20443696553841 3.2
1.1 2.94992127392992
1.07853772938204 2.9
0.937751288710557 2.6
0.8 2.33073849034778
0.784418363224941 2.3
0.633047415969727 2
0.5 1.74224253935396
0.481870101614457 1.7
0.368336153788844 1.4
0.277183898600127 1.1
0.22565489540932 0.8
0.227636192594315 0.5
0.287964244110737 0.2
0.402671562499095 -0.1
0.5 -0.279379708702474
0.589239322949432 -0.4
0.8 -0.630595760926061
0.903670295377008 -0.7
1.1 -0.813638660333255
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.1 -0.467735858067864
1.4 -0.56579981625454
1.7 -0.556694997716268
2 -0.455884452422189
2.09390102755816 -0.4
2.3 -0.276976331062678
2.52819496447896 -0.1
2.6 -0.0425311254433254
2.86672007000874 0.2
2.9 0.231473544988786
3.16973638515701 0.5
3.2 0.531342976561558
3.45770579412385 0.8
3.5 0.845764946425047
3.7394631714852 1.1
3.8 1.16643292633569
4.01948528199203 1.4
4.1 1.48804321752152
4.30019608448168 1.7
4.4 1.80785937585093
4.58277864155129 2
4.7 2.1250010981363
4.86754630963297 2.3
5 2.43964152761299
5 2.6
5 2.82375092884554
4.79253028622682 2.6
4.7 2.50162540088679
4.51658338140634 2.3
4.4 2.17451632272406
4.24462389994033 2
4.1 1.84213914133324
3.97575939668927 1.7
3.8 1.50587578325077
3.70810114658658 1.4
3.5 1.16952551955643
3.43879777379268 1.1
3.2 0.839752107183495
3.1633543486585 0.8
2.9 0.526426404138827
2.87321711313195 0.5
2.6 0.242797849061096
2.54831060218158 0.2
2.3 0.00460775918817373
2.12546492719183 -0.1
2 -0.172072029463183
1.7 -0.255675114282336
1.4 -0.223767999328792
1.17318882513995 -0.1
1.1 -0.0373699573154024
0.921216135222994 0.2
0.809078964922939 0.5
0.8 0.624359345957525
0.789434712372087 0.8
0.8 0.872826549728106
0.83442129018677 1.1
0.925980227495733 1.4
1.04312936940351 1.7
1.1 1.82879695376347
1.1718272141191 2
1.30134172872221 2.3
1.4 2.5332539605055
1.43180122971074 2.6
1.5677094449419 2.9
1.69565918629487 3.2
1.7 3.21028781251731
1.85642802075039 3.5
1.99793196483044 3.8
2 3.80466090562326
2.177301107834 4.1
2.3 4.31766048472915
2.3613809735129 4.4
2.57523160573933 4.7
2.6 4.73667583864483
2.83387480527643 5
2.6 5
2.3 5
2.26533572554098 5
2.10348290542745 4.7
2 4.51966820850448
1.94731761295523 4.4
1.81496333742358 4.1
1.7 3.85147925286483
1.68182646983992 3.8
1.56488848742918 3.5
1.43075994985088 3.2
1.4 3.13193646071076
1.30878901766637 2.9
1.18129237025043 2.6
1.1 2.42324484504998
1.04052938898391 2.3
0.896019677804993 2
0.8 1.80016339814715
0.751735265863648 1.7
0.622986580811739 1.4
0.519890523883599 1.1
0.5 0.991974887942755
0.472045780396354 0.8
0.47828400775194 0.5
0.5 0.393182504321219
0.553646100096357 0.2
0.710566493260102 -0.1
0.8 -0.220973823770508
1.00110454276309 -0.4
1.1 -0.467735858067864
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.4 -0.223767999328792
1.7 -0.255675114282336
2 -0.172072029463183
2.12546492719183 -0.1
2.3 0.00460775918817373
2.54831060218158 0.2
2.6 0.242797849061096
2.87321711313195 0.5
2.9 0.526426404138827
3.1633543486585 0.8
3.2 0.839752107183495
3.43879777379268 1.1
3.5 1.16952551955643
3.70810114658658 1.4
3.8 1.50587578325077
3.97575939668927 1.7
4.1 1.84213914133324
4.24462389994033 2
4.4 2.17451632272406
4.51658338140634 2.3
4.7 2.50162540088679
4.79253028622682 2.6
5 2.82375092884554
5 2.9
5 3.2
5 3.37271257808246
4.8571665062046 3.2
4.7 3.01735869826754
4.60716458908571 2.9
4.4 2.65099780852878
4.36120155799867 2.6
4.11644018857642 2.3
4.1 2.28115001330592
3.86982128849106 2
3.8 1.91839359625049
3.62233266746056 1.7
3.5 1.55605234968775
3.37062538317583 1.4
3.2 1.20245838392017
3.11042090710894 1.1
2.9 0.868866863760362
2.83322260787167 0.8
2.6 0.570370963695039
2.51751094082461 0.5
2.3 0.325245037002366
2.08897997930215 0.2
2 0.150884903150571
1.7 0.0982416663779573
1.42296414768725 0.2
1.4 0.215293964815984
1.21916880552763 0.5
1.15917662218402 0.8
1.17910140908931 1.1
1.24796188274215 1.4
1.34422627810822 1.7
1.4 1.84948907742316
1.46410169409451 2
1.59877375172648 2.3
1.7 2.53320504934321
1.73742097821658 2.6
1.90101445193131 2.9
2 3.08912256498239
2.07613958975493 3.2
2.27267093204848 3.5
2.3 3.54424574252907
2.50457241406329 3.8
2.6 3.92513694815811
2.76675471105639 4.1
2.9 4.24252397719326
3.07798755977233 4.4
3.2 4.50701264152942
3.45621317145492 4.7
3.5 4.73217343031204
3.8 4.92488801070419
3.94227785564976 5
3.8 5
3.5 5
3.2 5
2.9 5
2.83387480527643 5
2.6 4.73667583864483
2.57523160573933 4.7
2.3613809735129 4.4
2.3 4.31766048472915
2.177301107834 4.1
2 3.80466090562326
1.99793196483044 3.8
1.85642802075039 3.5
1.7 3.21028781251731
1.69565918629487 3.2
1.5677094449419 2.9
1.43180122971075 2.6
1.4 2.5332539605055
1.30134172872221 2.3
1.1718272141191 2
1.1 1.82879695376347
1.04312936940351 1.7
0.925980227495733 1.4
0.83442129018677 1.1
0.8 0.872826549728106
0.789434712372087 0.8
0.8 0.624359345957525
0.809078964922939 0.5
0.921216135222994 0.2
1.1 -0.0373699573154024
1.17318882513995 -0.1
1.4 -0.223767999328792
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.7 0.0982416663779573
2 0.150884903150571
2.08897997930215 0.2
2.3 0.325245037002366
2.51751094082461 0.5
2.6 0.570370963695039
2.83322260787167 0.8
2.9 0.868866863760362
3.11042090710894 1.1
3.2 1.20245838392017
3.37062538317583 1.4
3.5 1.55605234968775
3.62233266746056 1.7
3.8 1.91839359625049
3.86982128849105 2
4.1 2.28115001330592
4.11644018857642 2.3
4.36120155799867 2.6
4.4 2.65099780852878
4.60716458908571 2.9
4.7 3.01735869826754
4.8571665062046 3.2
5 3.37271257808246
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.1 5
3.94227785564976 5
3.8 4.92488801070419
3.5 4.73217343031204
3.45621317145493 4.7
3.2 4.50701264152942
3.07798755977233 4.4
2.9 4.24252397719326
2.76675471105639 4.1
2.6 3.92513694815811
2.50457241406329 3.8
2.3 3.54424574252907
2.27267093204848 3.5
2.07613958975493 3.2
2 3.08912256498239
1.90101445193131 2.9
1.73742097821658 2.6
1.7 2.53320504934321
1.59877375172648 2.3
1.46410169409451 2
1.4 1.84948907742316
1.34422627810822 1.7
1.24796188274215 1.4
1.17910140908931 1.1
1.15917662218402 0.8
1.21916880552763 0.5
1.4 0.215293964815984
1.42296414768725 0.2
1.7 0.0982416663779573

1.62426969183373 0.8
1.58370078660496 1.1
1.62546997111104 1.4
1.7 1.66722811919781
1.71237970420816 1.7
1.85719091984473 2
2 2.28847289986088
2.00749261317666 2.3
2.21072160256115 2.6
2.3 2.73489998284801
2.43606880705134 2.9
2.6 3.10130942122487
2.69679963216052 3.2
2.9 3.41052537152328
3.00524165394418 3.5
3.2 3.67037314717018
3.39097238475481 3.8
3.5 3.87707315833577
3.8 4.002485466408
4.1 3.99181133748624
4.25471986543901 3.8
4.24420890807718 3.5
4.14517107244034 3.2
4.1 3.11592273737501
3.99376596122857 2.9
3.82675538145097 2.6
3.8 2.56077467011834
3.62961994984151 2.3
3.5 2.10951728758131
3.42475720004301 2
3.21102811702029 1.7
3.2 1.68612770739502
2.9652650974889 1.4
2.9 1.32288214303661
2.69367651262287 1.1
2.6 1.00261325623985
2.36654133219981 0.8
2.3 0.74565496412931
2 0.604796958566835
1.7 0.676483096217996
1.62426969183373 0.8
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.7 0.676483096217996
2 0.604796958566835
2.3 0.74565496412931
2.36654133219981 0.8
2.6 1.00261325623985
2.69367651262287 1.1
2.9 1.32288214303661
2.9652650974889 1.4
3.2 1.68612770739502
3.21102811702029 1.7
3.42475720004301 2
3.5 2.10951728758131
3.62961994984151 2.3
3.8 2.56077467011834
3.82675538145097 2.6
3.99376596122857 2.9
4.1 3.11592273737501
4.14517107244034 3.2
4.24420890807718 3.5
4.25471986543901 3.8
4.1 3.99181133748624
3.8 4.002485466408
3.5 3.87707315833577
3.39097238475481 3.8
3.2 3.67037314717018
3.00524165394418 3.5
2.9 3.41052537152328
2.69679963216052 3.2
2.6 3.10130942122487
2.43606880705134 2.9
2.3 2.73489998284801
2.21072160256115 2.6
2.00749261317666 2.3
2 2.28847289986088
1.85719091984473 2
1.71237970420816 1.7
1.7 1.66722811919781
1.62546997111104 1.4
1.58370078660496 1.1
1.62426969183373 0.8
1.7 0.676483096217996
};
\end{axis}



==> fig/tikz/ionosphere/CVI_Z_mean_lml_ep.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 -1
-0.630374306141722 -1
-0.7 -0.843727903324845
-0.785593009364752 -0.7
-0.919178533670886 -0.4
-1 -0.109620065259259
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.991814427340445 2.6
-0.982206258078465 2.9
-0.973594198172455 3.2
-0.962947610700397 3.5
-0.95860137839591 3.8
-0.95772014121668 4.1
-0.95553911758209 4.4
-0.952189688346234 4.7
-0.954747087003224 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.4597624765706
-0.991814427340445 2.6
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.7 -0.843727903324845
-0.630374306141722 -1
-0.4 -1
-0.132378827249292 -1
-0.310795970093145 -0.7
-0.4 -0.497424772666802
-0.450781050812477 -0.4
-0.569814348224621 -0.1
-0.646463009865711 0.2
-0.694884202463109 0.5
-0.7 0.550309613559817
-0.736740647889945 0.8
-0.758500395401488 1.1
-0.754796864060626 1.4
-0.723471408863638 1.7
-0.7 1.85800802161676
-0.686791129852197 2
-0.66492204816066 2.3
-0.651189492617596 2.6
-0.641879444980661 2.9
-0.637259071367033 3.2
-0.635380111881336 3.5
-0.633877164571546 3.8
-0.631102707040837 4.1
-0.631157341683875 4.4
-0.633420048876966 4.7
-0.634662928467753 5
-0.7 5
-0.954747087003224 5
-0.952189688346234 4.7
-0.95553911758209 4.4
-0.95772014121668 4.1
-0.95860137839591 3.8
-0.962947610700397 3.5
-0.973594198172455 3.2
-0.982206258078465 2.9
-0.991814427340445 2.6
-1 2.4597624765706
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.109620065259259
-0.919178533670886 -0.4
-0.785593009364752 -0.7
-0.7 -0.843727903324845
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.426827814382496
4.7950724005904 0.2
4.7 0.0952661574373754
4.52292548332033 -0.1
4.4 -0.234406473285072
4.24874129247816 -0.4
4.1 -0.560390427701388
3.97065694063432 -0.7
3.8 -0.87934345255221
3.68506131638209 -1
3.8 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
-0.1 -1
0.184428805667876 -1
-0.0133425619500507 -0.7
-0.1 -0.535216556743632
-0.172200398979209 -0.4
-0.293788538280436 -0.1
-0.376877457725241 0.2
-0.4 0.322849152487129
-0.43958256456326 0.5
-0.480706666526816 0.8
-0.502101124995642 1.1
-0.504551479820819 1.4
-0.489473449461786 1.7
-0.467075476682574 2
-0.448065281291103 2.3
-0.435959336002513 2.6
-0.42978829365325 2.9
-0.425885752123982 3.2
-0.42284307206708 3.5
-0.419907131301969 3.8
-0.416156531367368 4.1
-0.416214689809729 4.4
-0.421318330276144 4.7
-0.425037319366446 5
-0.634662928467753 5
-0.633420048876966 4.7
-0.631157341683875 4.4
-0.631102707040837 4.1
-0.633877164571546 3.8
-0.635380111881336 3.5
-0.637259071367033 3.2
-0.641879444980661 2.9
-0.651189492617596 2.6
-0.66492204816066 2.3
-0.686791129852197 2
-0.7 1.85800802161676
-0.723471408863638 1.7
-0.754796864060626 1.4
-0.758500395401488 1.1
-0.736740647889945 0.8
-0.7 0.550309613559817
-0.694884202463109 0.5
-0.646463009865711 0.2
-0.569814348224621 -0.1
-0.450781050812477 -0.4
-0.4 -0.497424772666802
-0.310795970093145 -0.7
-0.132378827249292 -1
-0.1 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
3.2 -1
3.5 -1
3.68506131638209 -1
3.8 -0.87934345255221
3.97065694063432 -0.7
4.1 -0.560390427701388
4.24874129247816 -0.4
4.4 -0.234406473285072
4.52292548332033 -0.1
4.7 0.0952661574373754
4.7950724005904 0.2
5 0.426827814382496
5 0.5
5 0.8
5 1.09428326042315
4.71836404306505 0.8
4.7 0.780814619545658
4.43089634690083 0.5
4.4 0.467760176346898
4.1426457241285 0.2
4.1 0.155607808405635
3.85276613267839 -0.1
3.8 -0.154656824514478
3.55961760752745 -0.4
3.5 -0.461142986734213
3.26008546890989 -0.7
3.2 -0.76040419767281
2.94809482490356 -1
3.2 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
0.2 -1
0.479199637837705 -1
0.247503281303958 -0.7
0.2 -0.628368827203212
0.0683857746688714 -0.4
-0.063637643351123 -0.1
-0.1 0.0104197484202614
-0.161819100483314 0.2
-0.226711494597569 0.5
-0.266571858880615 0.8
-0.288413363145018 1.1
-0.294414913617209 1.4
-0.287214340019897 1.7
-0.274589671992884 2
-0.264062950050659 2.3
-0.257899188622305 2.6
-0.254380353626097 2.9
-0.251552650299803 3.2
-0.247976305040504 3.5
-0.242833285648806 3.8
-0.237586611950344 4.1
-0.237055812911132 4.4
-0.240279428445201 4.7
-0.242843939570672 5
-0.4 5
-0.425037319366446 5
-0.421318330276145 4.7
-0.416214689809729 4.4
-0.416156531367368 4.1
-0.419907131301969 3.8
-0.42284307206708 3.5
-0.425885752123982 3.2
-0.42978829365325 2.9
-0.435959336002513 2.6
-0.448065281291103 2.3
-0.467075476682574 2
-0.489473449461786 1.7
-0.504551479820819 1.4
-0.502101124995642 1.1
-0.480706666526816 0.8
-0.43958256456326 0.5
-0.4 0.322849152487129
-0.376877457725241 0.2
-0.293788538280436 -0.1
-0.172200398979209 -0.4
-0.1 -0.535216556743632
-0.0133425619500507 -0.7
0.184428805667876 -1
0.2 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
2.6 -1
2.9 -1
2.94809482490356 -1
3.2 -0.76040419767281
3.26008546890989 -0.7
3.5 -0.461142986734214
3.55961760752745 -0.4
3.8 -0.154656824514478
3.85276613267839 -0.1
4.1 0.155607808405635
4.1426457241285 0.2
4.4 0.467760176346898
4.43089634690083 0.5
4.7 0.780814619545658
4.71836404306505 0.8
5 1.09428326042315
5 1.1
5 1.4
5 1.47532805864262
4.92696388080268 1.4
4.7 1.16647316305805
4.63559009684776 1.1
4.4 0.85775427475161
4.34402010577823 0.8
4.1 0.549556975606455
4.05180815335558 0.5
3.8 0.242759760814225
3.75799374354436 0.2
3.5 -0.0608823557093937
3.46064878824038 -0.1
3.2 -0.358248871806724
3.1559670067412 -0.4
2.9 -0.644305992969903
2.83611596042236 -0.7
2.6 -0.911328096415136
2.48333357938237 -1
2.6 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.5 -1
0.8 -1
0.851705815234448 -1
0.8 -0.970608276409583
0.518589232505654 -0.7
0.5 -0.679739006863561
0.310289994158632 -0.4
0.2 -0.199262447795258
0.153548446603023 -0.1
0.0496062274788138 0.2
-0.0209654907313481 0.5
-0.0659974466897385 0.8
-0.0919307086004041 1.1
-0.1 1.33595528167217
-0.102055645242867 1.4
-0.100307838046624 1.7
-0.1 1.71432244451367
-0.0933853236489037 2
-0.0875970342745543 2.3
-0.0843557617579154 2.6
-0.0808917363888052 2.9
-0.0768197011320476 3.2
-0.069730698675349 3.5
-0.0589426148008139 3.8
-0.0492323720864525 4.1
-0.0473196804218561 4.4
-0.0485459429633577 4.7
-0.0487248589848135 5
-0.1 5
-0.242843939570672 5
-0.240279428445201 4.7
-0.237055812911132 4.4
-0.237586611950344 4.1
-0.242833285648806 3.8
-0.247976305040504 3.5
-0.251552650299803 3.2
-0.254380353626097 2.9
-0.257899188622305 2.6
-0.264062950050659 2.3
-0.274589671992884 2
-0.287214340019897 1.7
-0.294414913617209 1.4
-0.288413363145018 1.1
-0.266571858880615 0.8
-0.226711494597569 0.5
-0.161819100483314 0.2
-0.1 0.0104197484202615
-0.063637643351123 -0.1
0.0683857746688714 -0.4
0.2 -0.628368827203212
0.247503281303958 -0.7
0.479199637837705 -1
0.5 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
2.3 -1
2.48333357938237 -1
2.6 -0.911328096415136
2.83611596042236 -0.7
2.9 -0.644305992969903
3.1559670067412 -0.4
3.2 -0.358248871806724
3.46064878824038 -0.1
3.5 -0.0608823557093937
3.75799374354436 0.2
3.8 0.242759760814225
4.05180815335558 0.5
4.1 0.549556975606455
4.34402010577823 0.8
4.4 0.85775427475161
4.63559009684776 1.1
4.7 1.16647316305805
4.92696388080268 1.4
5 1.47532805864262
5 1.7
5 1.79860493110323
4.90458635790486 1.7
4.7 1.48944154922141
4.6136985208135 1.4
4.4 1.1799597781737
4.3230540503225 1.1
4.1 0.870435188683754
4.03224524083691 0.8
3.8 0.561744845646815
3.74022401260888 0.5
3.5 0.255877564678861
3.44476906018404 0.2
3.2 -0.0434682080197323
3.14146637778613 -0.1
2.9 -0.330362242710339
2.82129081315828 -0.4
2.6 -0.596224864848557
2.46385661149616 -0.7
2.3 -0.828927495392599
2.0161124468465 -1
2.3 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
0.8 -0.970608276409583
0.851705815234448 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.0161124468465 -1
2.3 -0.828927495392599
2.46385661149616 -0.7
2.6 -0.596224864848558
2.82129081315828 -0.4
2.9 -0.330362242710339
3.14146637778613 -0.1
3.2 -0.0434682080197323
3.44476906018404 0.2
3.5 0.255877564678861
3.74022401260888 0.5
3.8 0.561744845646815
4.03224524083691 0.8
4.1 0.870435188683754
4.3230540503225 1.1
4.4 1.1799597781737
4.6136985208135 1.4
4.7 1.48944154922141
4.90458635790486 1.7
5 1.79860493110323
5 2
5 2.10975892767522
4.89452158363929 2
4.7 1.79885046407124
4.60559669990556 1.7
4.4 1.48682604749212
4.31767000878494 1.4
4.1 1.17376359113754
4.0304377468139 1.1
3.8 0.860497329866999
3.74286359272203 0.8
3.5 0.549277576932911
3.45266248802872 0.5
3.2 0.244467640586985
3.15533372015857 0.2
2.9 -0.0469621124710117
2.84174744298407 -0.1
2.6 -0.315297234136732
2.49091915887163 -0.4
2.3 -0.54799772353537
2.04518765423893 -0.7
2 -0.728062497200152
1.7 -0.843469938355707
1.4 -0.876875550996879
1.1 -0.813772394828865
0.903272033881048 -0.7
0.8 -0.631116963398705
0.587852299176417 -0.4
0.5 -0.283627586251941
0.398166779966601 -0.1
0.271981869492842 0.2
0.2 0.441703379574125
0.185848496995487 0.5
0.139635268776424 0.8
0.113022142860895 1.1
0.101175936045125 1.4
0.101020669340849 1.7
0.107964726422543 2
0.117070005666571 2.3
0.125714548845364 2.6
0.134440361396067 2.9
0.145836861031833 3.2
0.160910021384503 3.5
0.174668466162477 3.8
0.185219858749736 4.1
0.189626110630686 4.4
0.196478493271528 4.7
0.2 4.79371775245346
0.208979138972569 5
0.2 5
-0.0487248589848135 5
-0.0485459429633577 4.7
-0.0473196804218561 4.4
-0.0492323720864525 4.1
-0.0589426148008139 3.8
-0.069730698675349 3.5
-0.0768197011320476 3.2
-0.0808917363888052 2.9
-0.0843557617579155 2.6
-0.0875970342745543 2.3
-0.0933853236489037 2
-0.1 1.71432244451367
-0.100307838046624 1.7
-0.102055645242867 1.4
-0.1 1.33595528167217
-0.0919307086004041 1.1
-0.0659974466897385 0.8
-0.0209654907313481 0.5
0.0496062274788138 0.2
0.153548446603023 -0.1
0.2 -0.199262447795258
0.310289994158632 -0.4
0.5 -0.679739006863561
0.518589232505654 -0.7
0.8 -0.970608276409583
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.1 -0.813772394828865
1.4 -0.876875550996879
1.7 -0.843469938355707
2 -0.728062497200152
2.04518765423893 -0.7
2.3 -0.54799772353537
2.49091915887163 -0.4
2.6 -0.315297234136732
2.84174744298407 -0.1
2.9 -0.0469621124710117
3.15533372015857 0.2
3.2 0.244467640586985
3.45266248802872 0.5
3.5 0.549277576932911
3.74286359272203 0.8
3.8 0.860497329866999
4.0304377468139 1.1
4.1 1.17376359113754
4.31767000878494 1.4
4.4 1.48682604749212
4.60559669990556 1.7
4.7 1.79885046407124
4.8945215836393 2
5 2.10975892767522
5 2.3
5 2.43918719110633
4.86797035810383 2.3
4.7 2.12456811143156
4.58317798370976 2
4.4 1.80745198443363
4.30056676364717 1.7
4.1 1.48766653831497
4.01982419727302 1.4
3.8 1.16609204801458
3.73976921698291 1.1
3.5 0.845463319429932
3.45798081601056 0.8
3.2 0.531080133587768
3.16998652735658 0.5
2.9 0.23124260664295
2.86695790021022 0.2
2.6 -0.0427424831869032
2.5284383755196 -0.1
2.3 -0.277172628580335
2.09416475544301 -0.4
2 -0.456046179740096
1.7 -0.556908522040421
1.4 -0.566146748980064
1.1 -0.468510499964768
0.999586656175667 -0.4
0.8 -0.225300845612633
0.705562016667161 -0.1
0.535117528062293 0.2
0.5 0.290089452391455
0.439348594327413 0.5
0.383750917585162 0.8
0.351342614152106 1.1
0.336823079824352 1.4
0.336935671884925 1.7
0.346959216678859 2
0.361270597562067 2.3
0.375208218910249 2.6
0.391079072747805 2.9
0.41020037145768 3.2
0.427686792155666 3.5
0.441870188730686 3.8
0.45384862831052 4.1
0.463077171295378 4.4
0.475712382242172 4.7
0.492820433950919 5
0.208979138972569 5
0.2 4.79371775245346
0.196478493271528 4.7
0.189626110630686 4.4
0.185219858749736 4.1
0.174668466162477 3.8
0.160910021384503 3.5
0.145836861031833 3.2
0.134440361396067 2.9
0.125714548845364 2.6
0.117070005666571 2.3
0.107964726422543 2
0.101020669340849 1.7
0.101175936045125 1.4
0.113022142860895 1.1
0.139635268776424 0.8
0.185848496995487 0.5
0.2 0.441703379574125
0.271981869492842 0.2
0.398166779966601 -0.1
0.5 -0.283627586251941
0.587852299176417 -0.4
0.8 -0.631116963398705
0.903272033881048 -0.7
1.1 -0.813772394828865
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.1 -0.468510499964768
1.4 -0.566146748980064
1.7 -0.556908522040421
2 -0.456046179740096
2.09416475544301 -0.4
2.3 -0.277172628580335
2.5284383755196 -0.1
2.6 -0.0427424831869032
2.86695790021022 0.2
2.9 0.23124260664295
3.16998652735658 0.5
3.2 0.531080133587768
3.45798081601056 0.8
3.5 0.845463319429932
3.73976921698291 1.1
3.8 1.16609204801458
4.01982419727302 1.4
4.1 1.48766653831497
4.30056676364717 1.7
4.4 1.80745198443363
4.58317798370976 2
4.7 2.12456811143156
4.86797035810383 2.3
5 2.43918719110633
5 2.6
5 2.82220742575205
4.79392938708866 2.6
4.7 2.50015546861377
4.51788988225946 2.3
4.4 2.17313612733005
4.24582566518994 2
4.1 1.8408657997678
3.97685167611468 1.7
3.8 1.50472371495496
3.70908819734617 1.4
3.5 1.16850278342726
3.43969153760217 1.1
3.2 0.838856011822102
3.16417665894553 0.8
2.9 0.525634685699878
2.87401434128373 0.5
2.6 0.24206119811981
2.54917821794125 0.2
2.3 0.00388041992587775
2.12656555300688 -0.1
2 -0.17274169522257
1.7 -0.256658916197742
1.4 -0.225696083993047
1.16660349858221 -0.1
1.1 -0.0458887613400155
0.903372961754955 0.2
0.8 0.411446381450126
0.765656284144547 0.5
0.69293568622868 0.8
0.652503257354545 1.1
0.637935749801091 1.4
0.645048667970125 1.7
0.6661371587066 2
0.692322073517666 2.3
0.717657458320334 2.6
0.747648004198277 2.9
0.783257055158861 3.2
0.8 3.36101355492682
0.813934675045286 3.5
0.838247071482341 3.8
0.863535383845753 4.1
0.895425934665223 4.4
0.927918095755375 4.7
0.901307744019418 5
0.8 5
0.5 5
0.492820433950919 5
0.475712382242172 4.7
0.463077171295377 4.4
0.45384862831052 4.1
0.441870188730686 3.8
0.427686792155666 3.5
0.41020037145768 3.2
0.391079072747805 2.9
0.375208218910249 2.6
0.361270597562067 2.3
0.346959216678859 2
0.336935671884925 1.7
0.336823079824352 1.4
0.351342614152106 1.1
0.383750917585162 0.8
0.439348594327413 0.5
0.5 0.290089452391456
0.535117528062293 0.2
0.705562016667161 -0.1
0.8 -0.225300845612633
0.999586656175667 -0.4
1.1 -0.468510499964768
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.4 -0.225696083993047
1.7 -0.256658916197742
2 -0.17274169522257
2.12656555300688 -0.1
2.3 0.00388041992587775
2.54917821794125 0.2
2.6 0.24206119811981
2.87401434128373 0.5
2.9 0.525634685699878
3.16417665894553 0.8
3.2 0.838856011822102
3.43969153760217 1.1
3.5 1.16850278342726
3.70908819734617 1.4
3.8 1.50472371495496
3.97685167611468 1.7
4.1 1.8408657997678
4.24582566518994 2
4.4 2.17313612733005
4.51788988225946 2.3
4.7 2.50015546861377
4.79392938708866 2.6
5 2.82220742575205
5 2.9
5 3.2
5 3.36416239547044
4.86402877864307 3.2
4.7 3.00970557908262
4.6130798252606 2.9
4.4 2.64439535512441
4.36617422454984 2.6
4.12024050208794 2.3
4.1 2.27680981788541
3.87328613429644 2
3.8 1.91441715247167
3.62552906305976 1.7
3.5 1.55243025302097
3.3736298890464 1.4
3.2 1.19916843672157
3.11331832404184 1.1
2.9 0.865854105227136
2.83616626006059 0.8
2.6 0.567500131094599
2.52089327329214 0.5
2.3 0.322339626253324
2.09389318373127 0.2
2 0.148028940162396
1.7 0.0931981220859671
1.4 0.198038006120548
1.39767563068446 0.2
1.1788321812551 0.5
1.1 0.712043828637989
1.072384551468 0.8
1.02289625185053 1.1
1.00775851452689 1.4
1.02010180615749 1.7
1.04890895279984 2
1.08252146897138 2.3
1.1 2.45659270787973
1.11226810587956 2.6
1.13611524988078 2.9
1.15783804765819 3.2
1.17841593619748 3.5
1.19920726047565 3.8
1.22279816661409 4.1
1.24043937492037 4.4
1.25619755596146 4.7
1.26423316134893 5
1.1 5
0.901307744019418 5
0.927918095755375 4.7
0.895425934665223 4.4
0.863535383845753 4.1
0.838247071482341 3.8
0.813934675045286 3.5
0.8 3.36101355492682
0.783257055158861 3.2
0.747648004198277 2.9
0.717657458320334 2.6
0.692322073517666 2.3
0.6661371587066 2
0.645048667970125 1.7
0.637935749801091 1.4
0.652503257354545 1.1
0.69293568622868 0.8
0.765656284144547 0.5
0.8 0.411446381450126
0.903372961754955 0.2
1.1 -0.0458887613400155
1.16660349858221 -0.1
1.4 -0.225696083993047
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.4 0.198038006120548
1.7 0.0931981220859671
2 0.148028940162396
2.09389318373127 0.2
2.3 0.322339626253324
2.52089327329214 0.5
2.6 0.567500131094599
2.83616626006059 0.8
2.9 0.865854105227136
3.11331832404184 1.1
3.2 1.19916843672157
3.3736298890464 1.4
3.5 1.55243025302097
3.62552906305976 1.7
3.8 1.91441715247167
3.87328613429644 2
4.1 2.27680981788541
4.12024050208794 2.3
4.36617422454984 2.6
4.4 2.64439535512441
4.6130798252606 2.9
4.7 3.00970557908262
4.86402877864307 3.2
5 3.36416239547044
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.1 5
3.8 5
3.5 5
3.2 5
2.93442324356561 5
3.12697968559507 4.7
3.2 4.61182066376775
3.46170663539132 4.4
3.5 4.38120411705341
3.8 4.35222490388517
4.1 4.28230153668627
4.30709007041737 4.1
4.37144751821687 3.8
4.30297675898621 3.5
4.17960815910206 3.2
4.1 3.05642661518254
4.02119666435761 2.9
3.84481819297612 2.6
3.8 2.53487651716097
3.64604282369959 2.3
3.5 2.08748808697256
3.43983879933241 2
3.22164169850608 1.7
3.2 1.67285684895794
2.97644848453197 1.4
2.9 1.30987841481825
2.70623127130088 1.1
2.6 0.989593766593565
2.3825462625104 0.8
2.3 0.732281898374837
2 0.580807464034218
1.7 0.610129534219422
1.54457569164011 0.8
1.43441621363816 1.1
1.4 1.33573754068204
1.39368707609039 1.4
1.38597987485128 1.7
1.3893591085874 2
1.39761876063279 2.3
1.4 2.35440180068522
1.42066100033224 2.6
1.45011586701162 2.9
1.48096129753777 3.2
1.53146425657381 3.5
1.6056668489094 3.8
1.7 4.04653537754382
1.72442786891619 4.1
1.84090824994257 4.4
1.88989799497964 4.7
1.93177088047107 5
1.7 5
1.4 5
1.26423316134893 5
1.25619755596146 4.7
1.24043937492037 4.4
1.22279816661409 4.1
1.19920726047565 3.8
1.17841593619748 3.5
1.15783804765819 3.2
1.13611524988078 2.9
1.11226810587956 2.6
1.1 2.45659270787973
1.08252146897138 2.3
1.04890895279984 2
1.02010180615749 1.7
1.00775851452689 1.4
1.02289625185053 1.1
1.072384551468 0.8
1.1 0.712043828637989
1.1788321812551 0.5
1.39767563068446 0.2
1.4 0.198038006120548
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.7 0.610129534219422
2 0.580807464034218
2.3 0.732281898374837
2.3825462625104 0.8
2.6 0.989593766593565
2.70623127130088 1.1
2.9 1.30987841481825
2.97644848453197 1.4
3.2 1.67285684895794
3.22164169850608 1.7
3.43983879933241 2
3.5 2.08748808697256
3.64604282369959 2.3
3.8 2.53487651716097
3.84481819297612 2.6
4.02119666435761 2.9
4.1 3.05642661518254
4.17960815910206 3.2
4.30297675898621 3.5
4.37144751821687 3.8
4.30709007041737 4.1
4.1 4.28230153668627
3.8 4.35222490388517
3.5 4.38120411705341
3.46170663539132 4.4
3.2 4.61182066376775
3.12697968559507 4.7
2.93442324356561 5
2.9 5
2.6 5
2.3 5
2 5
1.93177088047107 5
1.88989799497964 4.7
1.84090824994257 4.4
1.72442786891619 4.1
1.7 4.04653537754382
1.6056668489094 3.8
1.53146425657381 3.5
1.48096129753777 3.2
1.45011586701162 2.9
1.42066100033224 2.6
1.4 2.35440180068522
1.39761876063279 2.3
1.3893591085874 2
1.38597987485128 1.7
1.39368707609039 1.4
1.4 1.33573754068204
1.43441621363816 1.1
1.54457569164011 0.8
1.7 0.610129534219422

2.29398784429908 1.7
2.2544655911244 2
2.3 2.1264305224387
2.44738480305428 2.3
2.6 2.43982420556941
2.7183601949031 2.3
2.63808097239987 2
2.6 1.93952469867833
2.306978936637 1.7
2.3 1.69487362718659
2.29398784429908 1.7
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
2.3 1.69487362718659
2.306978936637 1.7
2.6 1.93952469867833
2.63808097239987 2
2.7183601949031 2.3
2.6 2.43982420556941
2.44738480305428 2.3
2.3 2.1264305224387
2.2544655911244 2
2.29398784429908 1.7
2.3 1.69487362718659
};
\end{axis}



==> fig/tikz/ionosphere/CVI_mean_lml.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=black]
table{%
x  y
-0.887803536370183 2.3
-0.7 2.47818948030274
-0.619836284829823 2.6
-0.429266129003946 2.9
-0.4 2.95368923791362
-0.296020630545507 3.2
-0.174896990494099 3.5
-0.1 3.6844980636142
-0.055781372560884 3.8
0.0421805590940537 4.1
0.124094139322306 4.4
0.2 4.6682411330791
0.210431818487413 4.7
0.318010113820088 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2.19126598321229
-0.887803536370183 2.3
};
\addplot [draw=none, fill=midnightblue854116]
table{%
x  y
-0.909446355770153 2
-0.7 2.20270452217322
-0.637039238536336 2.3
-0.44246920336234 2.6
-0.4 2.66739635607674
-0.288035531188239 2.9
-0.165476329424148 3.2
-0.1 3.36552324573427
-0.0487960853713571 3.5
0.0634280330946776 3.8
0.157213913258208 4.1
0.2 4.25889439168267
0.244878516297484 4.4
0.34199762025272 4.7
0.445217176698017 5
0.318010113820088 5
0.210431818487413 4.7
0.2 4.6682411330791
0.124094139322306 4.4
0.0421805590940536 4.1
-0.055781372560884 3.8
-0.1 3.6844980636142
-0.174896990494099 3.5
-0.296020630545507 3.2
-0.4 2.95368923791362
-0.429266129003946 2.9
-0.619836284829823 2.6
-0.7 2.47818948030274
-0.887803536370183 2.3
-1 2.19126598321229
-1 2
-1 1.91034818876569
-0.909446355770153 2
};
\addplot [draw=none, fill=midnightblue868137]
table{%
x  y
-0.911612615541082 1.7
-0.7 1.90940202672529
-0.642654608677494 2
-0.451230327181388 2.3
-0.4 2.37981927645212
-0.291075697405879 2.6
-0.152548092906617 2.9
-0.1 3.0312828177877
-0.0343789430855926 3.2
0.0768614486752001 3.5
0.182637438750239 3.8
0.2 3.85647425456165
0.28741016486835 4.1
0.380748649058974 4.4
0.473563422018026 4.7
0.5 4.77825916121389
0.588310157793602 5
0.5 5
0.445217176698017 5
0.34199762025272 4.7
0.244878516297484 4.4
0.2 4.25889439168267
0.157213913258208 4.1
0.0634280330946776 3.8
-0.0487960853713571 3.5
-0.1 3.36552324573427
-0.165476329424148 3.2
-0.288035531188239 2.9
-0.4 2.66739635607674
-0.44246920336234 2.6
-0.637039238536336 2.3
-0.7 2.20270452217322
-0.909446355770153 2
-1 1.91034818876569
-1 1.7
-1 1.60262986792633
-0.911612615541082 1.7
};
\addplot [draw=none, fill=teal882156]
table{%
x  y
-0.866396441787389 1.4
-0.7 1.58421566770659
-0.634296303225982 1.7
-0.447635129721808 2
-0.4 2.07565743655085
-0.290693544179744 2.3
-0.147859318294695 2.6
-0.1 2.70593815468761
-0.0162761030295962 2.9
0.0972749995576437 3.2
0.2 3.49248552318655
0.203035120957713 3.5
0.323020298222182 3.8
0.426586147733769 4.1
0.5 4.34353040627111
0.520677355560144 4.4
0.629433945849478 4.7
0.743419494957307 5
0.588310157793602 5
0.5 4.77825916121389
0.473563422018026 4.7
0.380748649058974 4.4
0.28741016486835 4.1
0.2 3.85647425456165
0.182637438750239 3.8
0.0768614486752001 3.5
-0.0343789430855926 3.2
-0.1 3.0312828177877
-0.152548092906617 2.9
-0.291075697405879 2.6
-0.4 2.37981927645212
-0.451230327181388 2.3
-0.642654608677494 2
-0.7 1.90940202672529
-0.911612615541082 1.7
-1 1.60262986792633
-1 1.4
-1 1.22118687376234
-0.866396441787389 1.4
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 -1
-0.63023181870719 -1
-0.7 -0.842671506766909
-0.784568151738941 -0.7
-0.915499616444636 -0.4
-0.98973676037331 -0.1
-1 -0.000135601022570403
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.993110320219683 0.5
-0.905967038620477 0.8
-0.751916674413362 1.1
-0.7 1.17071846372481
-0.594358904607223 1.4
-0.429198977201722 1.7
-0.4 1.74755544704623
-0.280093238640615 2
-0.139777158153298 2.3
-0.1 2.38507811083795
-0.00408642508117368 2.6
0.120492957205753 2.9
0.2 3.11770831388228
0.235047557552763 3.2
0.354439817697037 3.5
0.467012748063868 3.8
0.5 3.89795748164492
0.583281658333042 4.1
0.689729159444706 4.4
0.791416316198089 4.7
0.8 4.72309958486296
0.907857072284553 5
0.8 5
0.743419494957307 5
0.629433945849478 4.7
0.520677355560144 4.4
0.5 4.34353040627111
0.426586147733769 4.1
0.323020298222182 3.8
0.203035120957713 3.5
0.2 3.49248552318655
0.0972749995576437 3.2
-0.0162761030295962 2.9
-0.1 2.70593815468761
-0.147859318294695 2.6
-0.290693544179744 2.3
-0.4 2.07565743655085
-0.447635129721808 2
-0.634296303225982 1.7
-0.7 1.58421566770659
-0.866396441787389 1.4
-1 1.22118687376234
-1 1.1
-1 0.8
-1 0.5
-1 0.408070540499119
-0.993110320219683 0.5
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.7 -0.842671506766909
-0.63023181870719 -1
-0.4 -1
-0.132291427040298 -1
-0.310431878482001 -0.7
-0.4 -0.494390936535004
-0.448671626690947 -0.4
-0.562400693593726 -0.1
-0.623639813109658 0.2
-0.635767686442034 0.5
-0.596686694308942 0.8
-0.507954661705399 1.1
-0.4 1.34891201838415
-0.382716070129897 1.4
-0.256211115050857 1.7
-0.121432198678606 2
-0.1 2.04649913707812
0.0127629667261701 2.3
0.139965780281142 2.6
0.2 2.74965464337609
0.270215716210392 2.9
0.394546964748395 3.2
0.5 3.48345044862309
0.507468257639685 3.5
0.642757284219381 3.8
0.759535173046664 4.1
0.8 4.21930673765459
0.863647299696693 4.4
0.967209197104609 4.7
1.07765142212448 5
0.907857072284553 5
0.8 4.72309958486296
0.791416316198089 4.7
0.689729159444706 4.4
0.583281658333042 4.1
0.5 3.89795748164492
0.467012748063868 3.8
0.354439817697037 3.5
0.235047557552763 3.2
0.2 3.11770831388228
0.120492957205753 2.9
-0.00408642508117368 2.6
-0.1 2.38507811083795
-0.139777158153298 2.3
-0.280093238640615 2
-0.4 1.74755544704623
-0.429198977201722 1.7
-0.594358904607223 1.4
-0.7 1.17071846372481
-0.751916674413362 1.1
-0.905967038620477 0.8
-0.993110320219683 0.5
-1 0.408070540499119
-1 0.2
-1 -0.000135601022570403
-0.98973676037331 -0.1
-0.915499616444636 -0.4
-0.784568151738941 -0.7
-0.7 -0.842671506766909
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.42682811095723
4.79507214898701 0.2
4.7 0.0952664273934251
4.52292525358075 -0.1
4.4 -0.234406231017718
4.24874108529173 -0.4
4.1 -0.560390214231539
3.97065675639507 -0.7
3.8 -0.879343268668054
3.685061154761 -1
3.8 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
-0.1 -1
0.184492798672959 -1
-0.01305187295772 -0.7
-0.1 -0.533474619903749
-0.170753974246655 -0.4
-0.28841860262527 -0.1
-0.359667325844168 0.2
-0.386082601145852 0.5
-0.366308291197467 0.8
-0.303184805642335 1.1
-0.206217471564188 1.4
-0.1 1.66943323069862
-0.088286156213178 1.7
0.040165151119247 2
0.165884234001464 2.3
0.2 2.38292383779893
0.303337065119393 2.6
0.437924399016145 2.9
0.5 3.05661987398538
0.568403392194062 3.2
0.700936730584654 3.5
0.8 3.73172472935393
0.830406414533106 3.8
0.947406956109716 4.1
1.04669450097912 4.4
1.1 4.56204365313521
1.14588185974249 4.7
1.25436515956689 5
1.1 5
1.07765142212448 5
0.967209197104609 4.7
0.863647299696693 4.4
0.8 4.21930673765459
0.759535173046664 4.1
0.642757284219381 3.8
0.507468257639685 3.5
0.5 3.48345044862309
0.394546964748395 3.2
0.270215716210392 2.9
0.2 2.74965464337609
0.139965780281142 2.6
0.0127629667261701 2.3
-0.1 2.04649913707812
-0.121432198678606 2
-0.256211115050857 1.7
-0.382716070129897 1.4
-0.4 1.34891201838415
-0.507954661705399 1.1
-0.596686694308942 0.8
-0.635767686442034 0.5
-0.623639813109658 0.2
-0.562400693593726 -0.1
-0.448671626690947 -0.4
-0.4 -0.494390936535004
-0.310431878482001 -0.7
-0.132291427040298 -1
-0.1 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
3.2 -1
3.5 -1
3.685061154761 -1
3.8 -0.879343268668054
3.97065675639507 -0.7
4.1 -0.560390214231539
4.24874108529173 -0.4
4.4 -0.234406231017718
4.52292525358075 -0.1
4.7 0.0952664273934251
4.79507214898701 0.2
5 0.42682811095723
5 0.5
5 0.8
5 1.09428510928327
4.71836234957136 0.8
4.7 0.780816384650542
4.43089473949017 0.5
4.4 0.467761846589516
4.14264421673528 0.2
4.1 0.155609367604578
3.85276474368825 -0.1
3.8 -0.154655398173025
3.55961635852971 -0.4
3.5 -0.461141719586737
3.26008438111652 -0.7
3.2 -0.760403116911697
2.9480939131654 -1
3.2 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
0.2 -1
0.479255325230415 -1
0.247784192472104 -0.7
0.2 -0.627556100427295
0.0695894990491935 -0.4
-0.058865877695452 -0.1
-0.1 0.0415499705682803
-0.145484626755543 0.2
-0.183594963890442 0.5
-0.172757311546239 0.8
-0.118026942188554 1.1
-0.1 1.15893972412165
-0.0278192127499779 1.4
0.083285818477204 1.7
0.2 1.99407508591922
0.202748932580916 2
0.346205164810557 2.3
0.480512606905033 2.6
0.5 2.64459926631278
0.634299000687848 2.9
0.770272641001781 3.2
0.8 3.26954754089552
0.902672376658098 3.5
1.03195126762173 3.8
1.1 3.98753582743597
1.13950528444993 4.1
1.23446426836409 4.4
1.33094606756315 4.7
1.4 4.90210656115945
1.43816244046763 5
1.4 5
1.25436515956689 5
1.14588185974249 4.7
1.1 4.56204365313521
1.04669450097912 4.4
0.947406956109716 4.1
0.830406414533106 3.8
0.8 3.73172472935393
0.700936730584654 3.5
0.568403392194062 3.2
0.5 3.05661987398538
0.437924399016145 2.9
0.303337065119393 2.6
0.2 2.38292383779893
0.165884234001464 2.3
0.040165151119247 2
-0.088286156213178 1.7
-0.1 1.66943323069862
-0.206217471564188 1.4
-0.303184805642335 1.1
-0.366308291197467 0.8
-0.386082601145852 0.5
-0.359667325844168 0.2
-0.28841860262527 -0.1
-0.170753974246655 -0.4
-0.1 -0.53347461990375
-0.01305187295772 -0.7
0.184492798672959 -1
0.2 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
2.6 -1
2.9 -1
2.9480939131654 -1
3.2 -0.760403116911697
3.26008438111652 -0.7
3.5 -0.461141719586737
3.55961635852971 -0.4
3.8 -0.154655398173025
3.85276474368825 -0.1
4.1 0.155609367604578
4.14264421673528 0.2
4.4 0.467761846589516
4.43089473949017 0.5
4.7 0.780816384650542
4.71836234957136 0.8
5 1.09428510928327
5 1.1
5 1.4
5 1.47533724051483
4.92695513125589 1.4
4.7 1.16648177320797
4.63558191456139 1.1
4.4 0.857762264042404
4.34401253823331 0.8
4.1 0.549564283484414
4.05180124816645 0.5
3.8 0.242766327842122
3.7579875310366 0.2
3.5 -0.0608765621536276
3.46064326037089 -0.1
3.2 -0.358243830418478
3.15596211224053 -0.4
2.9 -0.644301638648233
2.83611164061451 -0.7
2.6 -0.91132439731082
2.48332981395457 -1
2.6 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.5 -1
0.8 -1
0.851794670990709 -1
0.8 -0.970535633122456
0.518911950234126 -0.7
0.5 -0.679296397106257
0.311496769448637 -0.4
0.2 -0.192127890278311
0.157956712225812 -0.1
0.0643437686376515 0.2
0.0192686822014385 0.5
0.0231785743204161 0.8
0.0715661943776383 1.1
0.153450045961865 1.4
0.2 1.53362559126815
0.26828948278652 1.7
0.403317552088578 2
0.5 2.21762645374143
0.543886705034136 2.3
0.701884520848107 2.6
0.8 2.79798820047189
0.850762918965214 2.9
0.985281650177575 3.2
1.1 3.46839208382114
1.11327709480669 3.5
1.23450675729973 3.8
1.33461411337859 4.1
1.4 4.31735358838645
1.42905569074237 4.4
1.53929760744775 4.7
1.64931530844711 5
1.43816244046763 5
1.4 4.90210656115945
1.33094606756315 4.7
1.23446426836409 4.4
1.13950528444993 4.1
1.1 3.98753582743597
1.03195126762173 3.8
0.902672376658098 3.5
0.8 3.26954754089552
0.770272641001781 3.2
0.634299000687848 2.9
0.5 2.64459926631278
0.480512606905033 2.6
0.346205164810557 2.3
0.202748932580916 2
0.2 1.99407508591922
0.083285818477204 1.7
-0.0278192127499779 1.4
-0.1 1.15893972412165
-0.118026942188554 1.1
-0.172757311546239 0.8
-0.183594963890442 0.5
-0.145484626755543 0.2
-0.1 0.0415499705682803
-0.058865877695452 -0.1
0.0695894990491935 -0.4
0.2 -0.627556100427295
0.247784192472104 -0.7
0.479255325230415 -1
0.5 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
2.3 -1
2.48332981395457 -1
2.6 -0.91132439731082
2.83611164061451 -0.7
2.9 -0.644301638648233
3.15596211224053 -0.4
3.2 -0.358243830418478
3.46064326037089 -0.1
3.5 -0.0608765621536276
3.7579875310366 0.2
3.8 0.242766327842122
4.05180124816645 0.5
4.1 0.549564283484414
4.34401253823331 0.8
4.4 0.857762264042404
4.63558191456139 1.1
4.7 1.16648177320797
4.92695513125589 1.4
5 1.47533724051483
5 1.7
5 1.79864262907917
4.90455046336539 1.7
4.7 1.48947733796043
4.61366460134067 1.4
4.4 1.17999341138807
4.32302235702601 1.1
4.1 0.870466346039979
4.03221604029522 0.8
3.8 0.561773177019761
3.74019751186367 0.5
3.5 0.255902799821756
3.44474530765838 0.2
3.2 -0.0434461126404508
3.14144520769044 -0.1
2.9 -0.330343081806941
2.82127196294381 -0.4
2.6 -0.596208526424875
2.4638400039619 -0.7
2.3 -0.828914394497196
2.01609802089176 -1
2.3 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
0.8 -0.970535633122456
0.851794670990709 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.01609802089176 -1
2.3 -0.828914394497196
2.4638400039619 -0.7
2.6 -0.596208526424875
2.82127196294381 -0.4
2.9 -0.330343081806941
3.14144520769044 -0.1
3.2 -0.0434461126404508
3.44474530765838 0.2
3.5 0.255902799821756
3.74019751186367 0.5
3.8 0.561773177019761
4.03221604029522 0.8
4.1 0.87046634603998
4.32302235702601 1.1
4.4 1.17999341138807
4.61366460134067 1.4
4.7 1.48947733796043
4.90455046336539 1.7
5 1.79864262907917
5 2
5 2.10989261800648
4.8943949612319 2
4.7 1.7989778392269
4.6054769143076 1.7
4.4 1.48694607033075
4.31755809145606 1.4
4.1 1.1738749345094
4.03033469100125 1.1
3.8 0.860598571105965
3.742770024722 0.8
3.5 0.54936765382172
3.45257826911243 0.5
3.2 0.244546531968065
3.15525759608111 0.2
2.9 -0.0468929403683035
2.84167716467335 -0.1
2.6 -0.315235948266921
2.49085294260741 -0.4
2.3 -0.547945459935491
2.04512542945021 -0.7
2 -0.728023509531562
1.7 -0.843421819032086
1.4 -0.876807476093009
1.1 -0.813638660333255
0.903670295377008 -0.7
0.8 -0.630595760926061
0.589239322949432 -0.4
0.5 -0.279379708702474
0.402671562499095 -0.1
0.287964244110737 0.2
0.227636192594315 0.5
0.22565489540932 0.8
0.277183898600127 1.1
0.368336153788844 1.4
0.481870101614457 1.7
0.5 1.74224253935396
0.633047415969727 2
0.784418363224941 2.3
0.8 2.33073849034778
0.937751288710557 2.6
1.07853772938204 2.9
1.1 2.94992127392992
1.20443696553841 3.2
1.32680764200465 3.5
1.4 3.69482403492226
1.4440074567179 3.8
1.55391065672918 4.1
1.65707253051483 4.4
1.7 4.52144162922679
1.7817155393907 4.7
1.91352582600865 5
1.7 5
1.64931530844711 5
1.53929760744775 4.7
1.42905569074237 4.4
1.4 4.31735358838645
1.33461411337859 4.1
1.23450675729973 3.8
1.11327709480669 3.5
1.1 3.46839208382114
0.985281650177575 3.2
0.850762918965214 2.9
0.8 2.79798820047189
0.701884520848107 2.6
0.543886705034136 2.3
0.5 2.21762645374143
0.403317552088578 2
0.26828948278652 1.7
0.2 1.53362559126815
0.153450045961865 1.4
0.0715661943776383 1.1
0.0231785743204161 0.8
0.0192686822014385 0.5
0.0643437686376515 0.2
0.157956712225812 -0.1
0.2 -0.192127890278311
0.311496769448637 -0.4
0.5 -0.679296397106257
0.518911950234127 -0.7
0.8 -0.970535633122456
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.1 -0.813638660333255
1.4 -0.876807476093009
1.7 -0.843421819032085
2 -0.728023509531562
2.04512542945021 -0.7
2.3 -0.547945459935491
2.49085294260741 -0.4
2.6 -0.315235948266921
2.84167716467335 -0.1
2.9 -0.0468929403683035
3.15525759608111 0.2
3.2 0.244546531968065
3.45257826911243 0.5
3.5 0.54936765382172
3.742770024722 0.8
3.8 0.860598571105964
4.03033469100125 1.1
4.1 1.1738749345094
4.31755809145606 1.4
4.4 1.48694607033075
4.6054769143076 1.7
4.7 1.7989778392269
4.8943949612319 2
5 2.10989261800648
5 2.3
5 2.43964152761299
4.86754630963297 2.3
4.7 2.1250010981363
4.58277864155129 2
4.4 1.80785937585093
4.30019608448168 1.7
4.1 1.48804321752152
4.01948528199203 1.4
3.8 1.16643292633569
3.7394631714852 1.1
3.5 0.845764946425047
3.45770579412384 0.8
3.2 0.531342976561558
3.16973638515701 0.5
2.9 0.231473544988786
2.86672007000874 0.2
2.6 -0.0425311254433255
2.52819496447896 -0.1
2.3 -0.276976331062678
2.09390102755816 -0.4
2 -0.455884452422189
1.7 -0.556694997716268
1.4 -0.56579981625454
1.1 -0.467735858067864
1.00110454276309 -0.4
0.8 -0.220973823770508
0.710566493260102 -0.1
0.553646100096357 0.2
0.5 0.393182504321219
0.47828400775194 0.5
0.472045780396354 0.8
0.5 0.991974887942755
0.519890523883599 1.1
0.622986580811739 1.4
0.751735265863648 1.7
0.8 1.80016339814715
0.896019677804993 2
1.04052938898391 2.3
1.1 2.42324484504998
1.18129237025043 2.6
1.30878901766637 2.9
1.4 3.13193646071076
1.43075994985088 3.2
1.56488848742918 3.5
1.68182646983992 3.8
1.7 3.85147925286483
1.81496333742358 4.1
1.94731761295523 4.4
2 4.51966820850448
2.10348290542745 4.7
2.26533572554098 5
2 5
1.91352582600865 5
1.7817155393907 4.7
1.7 4.52144162922679
1.65707253051483 4.4
1.55391065672918 4.1
1.4440074567179 3.8
1.4 3.69482403492226
1.32680764200465 3.5
1.20443696553841 3.2
1.1 2.94992127392992
1.07853772938204 2.9
0.937751288710557 2.6
0.8 2.33073849034778
0.784418363224941 2.3
0.633047415969727 2
0.5 1.74224253935396
0.481870101614457 1.7
0.368336153788844 1.4
0.277183898600127 1.1
0.22565489540932 0.8
0.227636192594315 0.5
0.287964244110737 0.2
0.402671562499095 -0.1
0.5 -0.279379708702474
0.589239322949432 -0.4
0.8 -0.630595760926061
0.903670295377008 -0.7
1.1 -0.813638660333255
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.1 -0.467735858067864
1.4 -0.56579981625454
1.7 -0.556694997716268
2 -0.455884452422189
2.09390102755816 -0.4
2.3 -0.276976331062678
2.52819496447896 -0.1
2.6 -0.0425311254433254
2.86672007000874 0.2
2.9 0.231473544988786
3.16973638515701 0.5
3.2 0.531342976561558
3.45770579412385 0.8
3.5 0.845764946425047
3.7394631714852 1.1
3.8 1.16643292633569
4.01948528199203 1.4
4.1 1.48804321752152
4.30019608448168 1.7
4.4 1.80785937585093
4.58277864155129 2
4.7 2.1250010981363
4.86754630963297 2.3
5 2.43964152761299
5 2.6
5 2.82375092884554
4.79253028622682 2.6
4.7 2.50162540088679
4.51658338140634 2.3
4.4 2.17451632272406
4.24462389994033 2
4.1 1.84213914133324
3.97575939668927 1.7
3.8 1.50587578325077
3.70810114658658 1.4
3.5 1.16952551955643
3.43879777379268 1.1
3.2 0.839752107183495
3.1633543486585 0.8
2.9 0.526426404138827
2.87321711313195 0.5
2.6 0.242797849061096
2.54831060218158 0.2
2.3 0.00460775918817373
2.12546492719183 -0.1
2 -0.172072029463183
1.7 -0.255675114282336
1.4 -0.223767999328792
1.17318882513995 -0.1
1.1 -0.0373699573154024
0.921216135222994 0.2
0.809078964922939 0.5
0.8 0.624359345957525
0.789434712372087 0.8
0.8 0.872826549728106
0.83442129018677 1.1
0.925980227495733 1.4
1.04312936940351 1.7
1.1 1.82879695376347
1.1718272141191 2
1.30134172872221 2.3
1.4 2.5332539605055
1.43180122971074 2.6
1.5677094449419 2.9
1.69565918629487 3.2
1.7 3.21028781251731
1.85642802075039 3.5
1.99793196483044 3.8
2 3.80466090562326
2.177301107834 4.1
2.3 4.31766048472915
2.3613809735129 4.4
2.57523160573933 4.7
2.6 4.73667583864483
2.83387480527643 5
2.6 5
2.3 5
2.26533572554098 5
2.10348290542745 4.7
2 4.51966820850448
1.94731761295523 4.4
1.81496333742358 4.1
1.7 3.85147925286483
1.68182646983992 3.8
1.56488848742918 3.5
1.43075994985088 3.2
1.4 3.13193646071076
1.30878901766637 2.9
1.18129237025043 2.6
1.1 2.42324484504998
1.04052938898391 2.3
0.896019677804993 2
0.8 1.80016339814715
0.751735265863648 1.7
0.622986580811739 1.4
0.519890523883599 1.1
0.5 0.991974887942755
0.472045780396354 0.8
0.47828400775194 0.5
0.5 0.393182504321219
0.553646100096357 0.2
0.710566493260102 -0.1
0.8 -0.220973823770508
1.00110454276309 -0.4
1.1 -0.467735858067864
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.4 -0.223767999328792
1.7 -0.255675114282336
2 -0.172072029463183
2.12546492719183 -0.1
2.3 0.00460775918817373
2.54831060218158 0.2
2.6 0.242797849061096
2.87321711313195 0.5
2.9 0.526426404138827
3.1633543486585 0.8
3.2 0.839752107183495
3.43879777379268 1.1
3.5 1.16952551955643
3.70810114658658 1.4
3.8 1.50587578325077
3.97575939668927 1.7
4.1 1.84213914133324
4.24462389994033 2
4.4 2.17451632272406
4.51658338140634 2.3
4.7 2.50162540088679
4.79253028622682 2.6
5 2.82375092884554
5 2.9
5 3.2
5 3.37271257808246
4.8571665062046 3.2
4.7 3.01735869826754
4.60716458908571 2.9
4.4 2.65099780852878
4.36120155799867 2.6
4.11644018857642 2.3
4.1 2.28115001330592
3.86982128849106 2
3.8 1.91839359625049
3.62233266746056 1.7
3.5 1.55605234968775
3.37062538317583 1.4
3.2 1.20245838392017
3.11042090710894 1.1
2.9 0.868866863760362
2.83322260787167 0.8
2.6 0.570370963695039
2.51751094082461 0.5
2.3 0.325245037002366
2.08897997930215 0.2
2 0.150884903150571
1.7 0.0982416663779573
1.42296414768725 0.2
1.4 0.215293964815984
1.21916880552763 0.5
1.15917662218402 0.8
1.17910140908931 1.1
1.24796188274215 1.4
1.34422627810822 1.7
1.4 1.84948907742316
1.46410169409451 2
1.59877375172648 2.3
1.7 2.53320504934321
1.73742097821658 2.6
1.90101445193131 2.9
2 3.08912256498239
2.07613958975493 3.2
2.27267093204848 3.5
2.3 3.54424574252907
2.50457241406329 3.8
2.6 3.92513694815811
2.76675471105639 4.1
2.9 4.24252397719326
3.07798755977233 4.4
3.2 4.50701264152942
3.45621317145492 4.7
3.5 4.73217343031204
3.8 4.92488801070419
3.94227785564976 5
3.8 5
3.5 5
3.2 5
2.9 5
2.83387480527643 5
2.6 4.73667583864483
2.57523160573933 4.7
2.3613809735129 4.4
2.3 4.31766048472915
2.177301107834 4.1
2 3.80466090562326
1.99793196483044 3.8
1.85642802075039 3.5
1.7 3.21028781251731
1.69565918629487 3.2
1.5677094449419 2.9
1.43180122971075 2.6
1.4 2.5332539605055
1.30134172872221 2.3
1.1718272141191 2
1.1 1.82879695376347
1.04312936940351 1.7
0.925980227495733 1.4
0.83442129018677 1.1
0.8 0.872826549728106
0.789434712372087 0.8
0.8 0.624359345957525
0.809078964922939 0.5
0.921216135222994 0.2
1.1 -0.0373699573154024
1.17318882513995 -0.1
1.4 -0.223767999328792
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.7 0.0982416663779573
2 0.150884903150571
2.08897997930215 0.2
2.3 0.325245037002366
2.51751094082461 0.5
2.6 0.570370963695039
2.83322260787167 0.8
2.9 0.868866863760362
3.11042090710894 1.1
3.2 1.20245838392017
3.37062538317583 1.4
3.5 1.55605234968775
3.62233266746056 1.7
3.8 1.91839359625049
3.86982128849105 2
4.1 2.28115001330592
4.11644018857642 2.3
4.36120155799867 2.6
4.4 2.65099780852878
4.60716458908571 2.9
4.7 3.01735869826754
4.8571665062046 3.2
5 3.37271257808246
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.1 5
3.94227785564976 5
3.8 4.92488801070419
3.5 4.73217343031204
3.45621317145493 4.7
3.2 4.50701264152942
3.07798755977233 4.4
2.9 4.24252397719326
2.76675471105639 4.1
2.6 3.92513694815811
2.50457241406329 3.8
2.3 3.54424574252907
2.27267093204848 3.5
2.07613958975493 3.2
2 3.08912256498239
1.90101445193131 2.9
1.73742097821658 2.6
1.7 2.53320504934321
1.59877375172648 2.3
1.46410169409451 2
1.4 1.84948907742316
1.34422627810822 1.7
1.24796188274215 1.4
1.17910140908931 1.1
1.15917662218402 0.8
1.21916880552763 0.5
1.4 0.215293964815984
1.42296414768725 0.2
1.7 0.0982416663779573

1.62426969183373 0.8
1.58370078660496 1.1
1.62546997111104 1.4
1.7 1.66722811919781
1.71237970420816 1.7
1.85719091984473 2
2 2.28847289986088
2.00749261317666 2.3
2.21072160256115 2.6
2.3 2.73489998284801
2.43606880705134 2.9
2.6 3.10130942122487
2.69679963216052 3.2
2.9 3.41052537152328
3.00524165394418 3.5
3.2 3.67037314717018
3.39097238475481 3.8
3.5 3.87707315833577
3.8 4.002485466408
4.1 3.99181133748624
4.25471986543901 3.8
4.24420890807718 3.5
4.14517107244034 3.2
4.1 3.11592273737501
3.99376596122857 2.9
3.82675538145097 2.6
3.8 2.56077467011834
3.62961994984151 2.3
3.5 2.10951728758131
3.42475720004301 2
3.21102811702029 1.7
3.2 1.68612770739502
2.9652650974889 1.4
2.9 1.32288214303661
2.69367651262287 1.1
2.6 1.00261325623985
2.36654133219981 0.8
2.3 0.74565496412931
2 0.604796958566835
1.7 0.676483096217996
1.62426969183373 0.8
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.7 0.676483096217996
2 0.604796958566835
2.3 0.74565496412931
2.36654133219981 0.8
2.6 1.00261325623985
2.69367651262287 1.1
2.9 1.32288214303661
2.9652650974889 1.4
3.2 1.68612770739502
3.21102811702029 1.7
3.42475720004301 2
3.5 2.10951728758131
3.62961994984151 2.3
3.8 2.56077467011834
3.82675538145097 2.6
3.99376596122857 2.9
4.1 3.11592273737501
4.14517107244034 3.2
4.24420890807718 3.5
4.25471986543901 3.8
4.1 3.99181133748624
3.8 4.002485466408
3.5 3.87707315833577
3.39097238475481 3.8
3.2 3.67037314717018
3.00524165394418 3.5
2.9 3.41052537152328
2.69679963216052 3.2
2.6 3.10130942122487
2.43606880705134 2.9
2.3 2.73489998284801
2.21072160256115 2.6
2.00749261317666 2.3
2 2.28847289986088
1.85719091984473 2
1.71237970420816 1.7
1.7 1.66722811919781
1.62546997111104 1.4
1.58370078660496 1.1
1.62426969183373 0.8
1.7 0.676483096217996
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.6 2
};
\coordinate (CVI_mean_lml_t) at (axis cs:2.5999999999999996,2.0);
\end{axis}



==> fig/tikz/ionosphere/CVI_mean_lml_ep.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 -1
-0.630374306141722 -1
-0.7 -0.843727903324845
-0.785593009364752 -0.7
-0.919178533670886 -0.4
-1 -0.109620065259259
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.991814427340445 2.6
-0.982206258078465 2.9
-0.973594198172455 3.2
-0.962947610700397 3.5
-0.95860137839591 3.8
-0.95772014121668 4.1
-0.95553911758209 4.4
-0.952189688346234 4.7
-0.954747087003224 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.4597624765706
-0.991814427340445 2.6
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.7 -0.843727903324845
-0.630374306141722 -1
-0.4 -1
-0.132378827249292 -1
-0.310795970093145 -0.7
-0.4 -0.497424772666802
-0.450781050812477 -0.4
-0.569814348224621 -0.1
-0.646463009865711 0.2
-0.694884202463109 0.5
-0.7 0.550309613559817
-0.736740647889945 0.8
-0.758500395401488 1.1
-0.754796864060626 1.4
-0.723471408863638 1.7
-0.7 1.85800802161676
-0.686791129852197 2
-0.66492204816066 2.3
-0.651189492617596 2.6
-0.641879444980661 2.9
-0.637259071367033 3.2
-0.635380111881336 3.5
-0.633877164571546 3.8
-0.631102707040837 4.1
-0.631157341683875 4.4
-0.633420048876966 4.7
-0.634662928467753 5
-0.7 5
-0.954747087003224 5
-0.952189688346234 4.7
-0.95553911758209 4.4
-0.95772014121668 4.1
-0.95860137839591 3.8
-0.962947610700397 3.5
-0.973594198172455 3.2
-0.982206258078465 2.9
-0.991814427340445 2.6
-1 2.4597624765706
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.109620065259259
-0.919178533670886 -0.4
-0.785593009364752 -0.7
-0.7 -0.843727903324845
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.426827814382496
4.7950724005904 0.2
4.7 0.0952661574373754
4.52292548332033 -0.1
4.4 -0.234406473285072
4.24874129247816 -0.4
4.1 -0.560390427701388
3.97065694063432 -0.7
3.8 -0.87934345255221
3.68506131638209 -1
3.8 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
-0.1 -1
0.184428805667876 -1
-0.0133425619500507 -0.7
-0.1 -0.535216556743632
-0.172200398979209 -0.4
-0.293788538280436 -0.1
-0.376877457725241 0.2
-0.4 0.322849152487129
-0.43958256456326 0.5
-0.480706666526816 0.8
-0.502101124995642 1.1
-0.504551479820819 1.4
-0.489473449461786 1.7
-0.467075476682574 2
-0.448065281291103 2.3
-0.435959336002513 2.6
-0.42978829365325 2.9
-0.425885752123982 3.2
-0.42284307206708 3.5
-0.419907131301969 3.8
-0.416156531367368 4.1
-0.416214689809729 4.4
-0.421318330276144 4.7
-0.425037319366446 5
-0.634662928467753 5
-0.633420048876966 4.7
-0.631157341683875 4.4
-0.631102707040837 4.1
-0.633877164571546 3.8
-0.635380111881336 3.5
-0.637259071367033 3.2
-0.641879444980661 2.9
-0.651189492617596 2.6
-0.66492204816066 2.3
-0.686791129852197 2
-0.7 1.85800802161676
-0.723471408863638 1.7
-0.754796864060626 1.4
-0.758500395401488 1.1
-0.736740647889945 0.8
-0.7 0.550309613559817
-0.694884202463109 0.5
-0.646463009865711 0.2
-0.569814348224621 -0.1
-0.450781050812477 -0.4
-0.4 -0.497424772666802
-0.310795970093145 -0.7
-0.132378827249292 -1
-0.1 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
3.2 -1
3.5 -1
3.68506131638209 -1
3.8 -0.87934345255221
3.97065694063432 -0.7
4.1 -0.560390427701388
4.24874129247816 -0.4
4.4 -0.234406473285072
4.52292548332033 -0.1
4.7 0.0952661574373754
4.7950724005904 0.2
5 0.426827814382496
5 0.5
5 0.8
5 1.09428326042315
4.71836404306505 0.8
4.7 0.780814619545658
4.43089634690083 0.5
4.4 0.467760176346898
4.1426457241285 0.2
4.1 0.155607808405635
3.85276613267839 -0.1
3.8 -0.154656824514478
3.55961760752745 -0.4
3.5 -0.461142986734213
3.26008546890989 -0.7
3.2 -0.76040419767281
2.94809482490356 -1
3.2 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
0.2 -1
0.479199637837705 -1
0.247503281303958 -0.7
0.2 -0.628368827203212
0.0683857746688714 -0.4
-0.063637643351123 -0.1
-0.1 0.0104197484202614
-0.161819100483314 0.2
-0.226711494597569 0.5
-0.266571858880615 0.8
-0.288413363145018 1.1
-0.294414913617209 1.4
-0.287214340019897 1.7
-0.274589671992884 2
-0.264062950050659 2.3
-0.257899188622305 2.6
-0.254380353626097 2.9
-0.251552650299803 3.2
-0.247976305040504 3.5
-0.242833285648806 3.8
-0.237586611950344 4.1
-0.237055812911132 4.4
-0.240279428445201 4.7
-0.242843939570672 5
-0.4 5
-0.425037319366446 5
-0.421318330276145 4.7
-0.416214689809729 4.4
-0.416156531367368 4.1
-0.419907131301969 3.8
-0.42284307206708 3.5
-0.425885752123982 3.2
-0.42978829365325 2.9
-0.435959336002513 2.6
-0.448065281291103 2.3
-0.467075476682574 2
-0.489473449461786 1.7
-0.504551479820819 1.4
-0.502101124995642 1.1
-0.480706666526816 0.8
-0.43958256456326 0.5
-0.4 0.322849152487129
-0.376877457725241 0.2
-0.293788538280436 -0.1
-0.172200398979209 -0.4
-0.1 -0.535216556743632
-0.0133425619500507 -0.7
0.184428805667876 -1
0.2 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
2.6 -1
2.9 -1
2.94809482490356 -1
3.2 -0.76040419767281
3.26008546890989 -0.7
3.5 -0.461142986734214
3.55961760752745 -0.4
3.8 -0.154656824514478
3.85276613267839 -0.1
4.1 0.155607808405635
4.1426457241285 0.2
4.4 0.467760176346898
4.43089634690083 0.5
4.7 0.780814619545658
4.71836404306505 0.8
5 1.09428326042315
5 1.1
5 1.4
5 1.47532805864262
4.92696388080268 1.4
4.7 1.16647316305805
4.63559009684776 1.1
4.4 0.85775427475161
4.34402010577823 0.8
4.1 0.549556975606455
4.05180815335558 0.5
3.8 0.242759760814225
3.75799374354436 0.2
3.5 -0.0608823557093937
3.46064878824038 -0.1
3.2 -0.358248871806724
3.1559670067412 -0.4
2.9 -0.644305992969903
2.83611596042236 -0.7
2.6 -0.911328096415136
2.48333357938237 -1
2.6 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.5 -1
0.8 -1
0.851705815234448 -1
0.8 -0.970608276409583
0.518589232505654 -0.7
0.5 -0.679739006863561
0.310289994158632 -0.4
0.2 -0.199262447795258
0.153548446603023 -0.1
0.0496062274788138 0.2
-0.0209654907313481 0.5
-0.0659974466897385 0.8
-0.0919307086004041 1.1
-0.1 1.33595528167217
-0.102055645242867 1.4
-0.100307838046624 1.7
-0.1 1.71432244451367
-0.0933853236489037 2
-0.0875970342745543 2.3
-0.0843557617579154 2.6
-0.0808917363888052 2.9
-0.0768197011320476 3.2
-0.069730698675349 3.5
-0.0589426148008139 3.8
-0.0492323720864525 4.1
-0.0473196804218561 4.4
-0.0485459429633577 4.7
-0.0487248589848135 5
-0.1 5
-0.242843939570672 5
-0.240279428445201 4.7
-0.237055812911132 4.4
-0.237586611950344 4.1
-0.242833285648806 3.8
-0.247976305040504 3.5
-0.251552650299803 3.2
-0.254380353626097 2.9
-0.257899188622305 2.6
-0.264062950050659 2.3
-0.274589671992884 2
-0.287214340019897 1.7
-0.294414913617209 1.4
-0.288413363145018 1.1
-0.266571858880615 0.8
-0.226711494597569 0.5
-0.161819100483314 0.2
-0.1 0.0104197484202615
-0.063637643351123 -0.1
0.0683857746688714 -0.4
0.2 -0.628368827203212
0.247503281303958 -0.7
0.479199637837705 -1
0.5 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
2.3 -1
2.48333357938237 -1
2.6 -0.911328096415136
2.83611596042236 -0.7
2.9 -0.644305992969903
3.1559670067412 -0.4
3.2 -0.358248871806724
3.46064878824038 -0.1
3.5 -0.0608823557093937
3.75799374354436 0.2
3.8 0.242759760814225
4.05180815335558 0.5
4.1 0.549556975606455
4.34402010577823 0.8
4.4 0.85775427475161
4.63559009684776 1.1
4.7 1.16647316305805
4.92696388080268 1.4
5 1.47532805864262
5 1.7
5 1.79860493110323
4.90458635790486 1.7
4.7 1.48944154922141
4.6136985208135 1.4
4.4 1.1799597781737
4.3230540503225 1.1
4.1 0.870435188683754
4.03224524083691 0.8
3.8 0.561744845646815
3.74022401260888 0.5
3.5 0.255877564678861
3.44476906018404 0.2
3.2 -0.0434682080197323
3.14146637778613 -0.1
2.9 -0.330362242710339
2.82129081315828 -0.4
2.6 -0.596224864848557
2.46385661149616 -0.7
2.3 -0.828927495392599
2.0161124468465 -1
2.3 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
0.8 -0.970608276409583
0.851705815234448 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.0161124468465 -1
2.3 -0.828927495392599
2.46385661149616 -0.7
2.6 -0.596224864848558
2.82129081315828 -0.4
2.9 -0.330362242710339
3.14146637778613 -0.1
3.2 -0.0434682080197323
3.44476906018404 0.2
3.5 0.255877564678861
3.74022401260888 0.5
3.8 0.561744845646815
4.03224524083691 0.8
4.1 0.870435188683754
4.3230540503225 1.1
4.4 1.1799597781737
4.6136985208135 1.4
4.7 1.48944154922141
4.90458635790486 1.7
5 1.79860493110323
5 2
5 2.10975892767522
4.89452158363929 2
4.7 1.79885046407124
4.60559669990556 1.7
4.4 1.48682604749212
4.31767000878494 1.4
4.1 1.17376359113754
4.0304377468139 1.1
3.8 0.860497329866999
3.74286359272203 0.8
3.5 0.549277576932911
3.45266248802872 0.5
3.2 0.244467640586985
3.15533372015857 0.2
2.9 -0.0469621124710117
2.84174744298407 -0.1
2.6 -0.315297234136732
2.49091915887163 -0.4
2.3 -0.54799772353537
2.04518765423893 -0.7
2 -0.728062497200152
1.7 -0.843469938355707
1.4 -0.876875550996879
1.1 -0.813772394828865
0.903272033881048 -0.7
0.8 -0.631116963398705
0.587852299176417 -0.4
0.5 -0.283627586251941
0.398166779966601 -0.1
0.271981869492842 0.2
0.2 0.441703379574125
0.185848496995487 0.5
0.139635268776424 0.8
0.113022142860895 1.1
0.101175936045125 1.4
0.101020669340849 1.7
0.107964726422543 2
0.117070005666571 2.3
0.125714548845364 2.6
0.134440361396067 2.9
0.145836861031833 3.2
0.160910021384503 3.5
0.174668466162477 3.8
0.185219858749736 4.1
0.189626110630686 4.4
0.196478493271528 4.7
0.2 4.79371775245346
0.208979138972569 5
0.2 5
-0.0487248589848135 5
-0.0485459429633577 4.7
-0.0473196804218561 4.4
-0.0492323720864525 4.1
-0.0589426148008139 3.8
-0.069730698675349 3.5
-0.0768197011320476 3.2
-0.0808917363888052 2.9
-0.0843557617579155 2.6
-0.0875970342745543 2.3
-0.0933853236489037 2
-0.1 1.71432244451367
-0.100307838046624 1.7
-0.102055645242867 1.4
-0.1 1.33595528167217
-0.0919307086004041 1.1
-0.0659974466897385 0.8
-0.0209654907313481 0.5
0.0496062274788138 0.2
0.153548446603023 -0.1
0.2 -0.199262447795258
0.310289994158632 -0.4
0.5 -0.679739006863561
0.518589232505654 -0.7
0.8 -0.970608276409583
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.1 -0.813772394828865
1.4 -0.876875550996879
1.7 -0.843469938355707
2 -0.728062497200152
2.04518765423893 -0.7
2.3 -0.54799772353537
2.49091915887163 -0.4
2.6 -0.315297234136732
2.84174744298407 -0.1
2.9 -0.0469621124710117
3.15533372015857 0.2
3.2 0.244467640586985
3.45266248802872 0.5
3.5 0.549277576932911
3.74286359272203 0.8
3.8 0.860497329866999
4.0304377468139 1.1
4.1 1.17376359113754
4.31767000878494 1.4
4.4 1.48682604749212
4.60559669990556 1.7
4.7 1.79885046407124
4.8945215836393 2
5 2.10975892767522
5 2.3
5 2.43918719110633
4.86797035810383 2.3
4.7 2.12456811143156
4.58317798370976 2
4.4 1.80745198443363
4.30056676364717 1.7
4.1 1.48766653831497
4.01982419727302 1.4
3.8 1.16609204801458
3.73976921698291 1.1
3.5 0.845463319429932
3.45798081601056 0.8
3.2 0.531080133587768
3.16998652735658 0.5
2.9 0.23124260664295
2.86695790021022 0.2
2.6 -0.0427424831869032
2.5284383755196 -0.1
2.3 -0.277172628580335
2.09416475544301 -0.4
2 -0.456046179740096
1.7 -0.556908522040421
1.4 -0.566146748980064
1.1 -0.468510499964768
0.999586656175667 -0.4
0.8 -0.225300845612633
0.705562016667161 -0.1
0.535117528062293 0.2
0.5 0.290089452391455
0.439348594327413 0.5
0.383750917585162 0.8
0.351342614152106 1.1
0.336823079824352 1.4
0.336935671884925 1.7
0.346959216678859 2
0.361270597562067 2.3
0.375208218910249 2.6
0.391079072747805 2.9
0.41020037145768 3.2
0.427686792155666 3.5
0.441870188730686 3.8
0.45384862831052 4.1
0.463077171295378 4.4
0.475712382242172 4.7
0.492820433950919 5
0.208979138972569 5
0.2 4.79371775245346
0.196478493271528 4.7
0.189626110630686 4.4
0.185219858749736 4.1
0.174668466162477 3.8
0.160910021384503 3.5
0.145836861031833 3.2
0.134440361396067 2.9
0.125714548845364 2.6
0.117070005666571 2.3
0.107964726422543 2
0.101020669340849 1.7
0.101175936045125 1.4
0.113022142860895 1.1
0.139635268776424 0.8
0.185848496995487 0.5
0.2 0.441703379574125
0.271981869492842 0.2
0.398166779966601 -0.1
0.5 -0.283627586251941
0.587852299176417 -0.4
0.8 -0.631116963398705
0.903272033881048 -0.7
1.1 -0.813772394828865
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.1 -0.468510499964768
1.4 -0.566146748980064
1.7 -0.556908522040421
2 -0.456046179740096
2.09416475544301 -0.4
2.3 -0.277172628580335
2.5284383755196 -0.1
2.6 -0.0427424831869032
2.86695790021022 0.2
2.9 0.23124260664295
3.16998652735658 0.5
3.2 0.531080133587768
3.45798081601056 0.8
3.5 0.845463319429932
3.73976921698291 1.1
3.8 1.16609204801458
4.01982419727302 1.4
4.1 1.48766653831497
4.30056676364717 1.7
4.4 1.80745198443363
4.58317798370976 2
4.7 2.12456811143156
4.86797035810383 2.3
5 2.43918719110633
5 2.6
5 2.82220742575205
4.79392938708866 2.6
4.7 2.50015546861377
4.51788988225946 2.3
4.4 2.17313612733005
4.24582566518994 2
4.1 1.8408657997678
3.97685167611468 1.7
3.8 1.50472371495496
3.70908819734617 1.4
3.5 1.16850278342726
3.43969153760217 1.1
3.2 0.838856011822102
3.16417665894553 0.8
2.9 0.525634685699878
2.87401434128373 0.5
2.6 0.24206119811981
2.54917821794125 0.2
2.3 0.00388041992587775
2.12656555300688 -0.1
2 -0.17274169522257
1.7 -0.256658916197742
1.4 -0.225696083993047
1.16660349858221 -0.1
1.1 -0.0458887613400155
0.903372961754955 0.2
0.8 0.411446381450126
0.765656284144547 0.5
0.69293568622868 0.8
0.652503257354545 1.1
0.637935749801091 1.4
0.645048667970125 1.7
0.6661371587066 2
0.692322073517666 2.3
0.717657458320334 2.6
0.747648004198277 2.9
0.783257055158861 3.2
0.8 3.36101355492682
0.813934675045286 3.5
0.838247071482341 3.8
0.863535383845753 4.1
0.895425934665223 4.4
0.927918095755375 4.7
0.901307744019418 5
0.8 5
0.5 5
0.492820433950919 5
0.475712382242172 4.7
0.463077171295377 4.4
0.45384862831052 4.1
0.441870188730686 3.8
0.427686792155666 3.5
0.41020037145768 3.2
0.391079072747805 2.9
0.375208218910249 2.6
0.361270597562067 2.3
0.346959216678859 2
0.336935671884925 1.7
0.336823079824352 1.4
0.351342614152106 1.1
0.383750917585162 0.8
0.439348594327413 0.5
0.5 0.290089452391456
0.535117528062293 0.2
0.705562016667161 -0.1
0.8 -0.225300845612633
0.999586656175667 -0.4
1.1 -0.468510499964768
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.4 -0.225696083993047
1.7 -0.256658916197742
2 -0.17274169522257
2.12656555300688 -0.1
2.3 0.00388041992587775
2.54917821794125 0.2
2.6 0.24206119811981
2.87401434128373 0.5
2.9 0.525634685699878
3.16417665894553 0.8
3.2 0.838856011822102
3.43969153760217 1.1
3.5 1.16850278342726
3.70908819734617 1.4
3.8 1.50472371495496
3.97685167611468 1.7
4.1 1.8408657997678
4.24582566518994 2
4.4 2.17313612733005
4.51788988225946 2.3
4.7 2.50015546861377
4.79392938708866 2.6
5 2.82220742575205
5 2.9
5 3.2
5 3.36416239547044
4.86402877864307 3.2
4.7 3.00970557908262
4.6130798252606 2.9
4.4 2.64439535512441
4.36617422454984 2.6
4.12024050208794 2.3
4.1 2.27680981788541
3.87328613429644 2
3.8 1.91441715247167
3.62552906305976 1.7
3.5 1.55243025302097
3.3736298890464 1.4
3.2 1.19916843672157
3.11331832404184 1.1
2.9 0.865854105227136
2.83616626006059 0.8
2.6 0.567500131094599
2.52089327329214 0.5
2.3 0.322339626253324
2.09389318373127 0.2
2 0.148028940162396
1.7 0.0931981220859671
1.4 0.198038006120548
1.39767563068446 0.2
1.1788321812551 0.5
1.1 0.712043828637989
1.072384551468 0.8
1.02289625185053 1.1
1.00775851452689 1.4
1.02010180615749 1.7
1.04890895279984 2
1.08252146897138 2.3
1.1 2.45659270787973
1.11226810587956 2.6
1.13611524988078 2.9
1.15783804765819 3.2
1.17841593619748 3.5
1.19920726047565 3.8
1.22279816661409 4.1
1.24043937492037 4.4
1.25619755596146 4.7
1.26423316134893 5
1.1 5
0.901307744019418 5
0.927918095755375 4.7
0.895425934665223 4.4
0.863535383845753 4.1
0.838247071482341 3.8
0.813934675045286 3.5
0.8 3.36101355492682
0.783257055158861 3.2
0.747648004198277 2.9
0.717657458320334 2.6
0.692322073517666 2.3
0.6661371587066 2
0.645048667970125 1.7
0.637935749801091 1.4
0.652503257354545 1.1
0.69293568622868 0.8
0.765656284144547 0.5
0.8 0.411446381450126
0.903372961754955 0.2
1.1 -0.0458887613400155
1.16660349858221 -0.1
1.4 -0.225696083993047
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.4 0.198038006120548
1.7 0.0931981220859671
2 0.148028940162396
2.09389318373127 0.2
2.3 0.322339626253324
2.52089327329214 0.5
2.6 0.567500131094599
2.83616626006059 0.8
2.9 0.865854105227136
3.11331832404184 1.1
3.2 1.19916843672157
3.3736298890464 1.4
3.5 1.55243025302097
3.62552906305976 1.7
3.8 1.91441715247167
3.87328613429644 2
4.1 2.27680981788541
4.12024050208794 2.3
4.36617422454984 2.6
4.4 2.64439535512441
4.6130798252606 2.9
4.7 3.00970557908262
4.86402877864307 3.2
5 3.36416239547044
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.1 5
3.8 5
3.5 5
3.2 5
2.93442324356561 5
3.12697968559507 4.7
3.2 4.61182066376775
3.46170663539132 4.4
3.5 4.38120411705341
3.8 4.35222490388517
4.1 4.28230153668627
4.30709007041737 4.1
4.37144751821687 3.8
4.30297675898621 3.5
4.17960815910206 3.2
4.1 3.05642661518254
4.02119666435761 2.9
3.84481819297612 2.6
3.8 2.53487651716097
3.64604282369959 2.3
3.5 2.08748808697256
3.43983879933241 2
3.22164169850608 1.7
3.2 1.67285684895794
2.97644848453197 1.4
2.9 1.30987841481825
2.70623127130088 1.1
2.6 0.989593766593565
2.3825462625104 0.8
2.3 0.732281898374837
2 0.580807464034218
1.7 0.610129534219422
1.54457569164011 0.8
1.43441621363816 1.1
1.4 1.33573754068204
1.39368707609039 1.4
1.38597987485128 1.7
1.3893591085874 2
1.39761876063279 2.3
1.4 2.35440180068522
1.42066100033224 2.6
1.45011586701162 2.9
1.48096129753777 3.2
1.53146425657381 3.5
1.6056668489094 3.8
1.7 4.04653537754382
1.72442786891619 4.1
1.84090824994257 4.4
1.88989799497964 4.7
1.93177088047107 5
1.7 5
1.4 5
1.26423316134893 5
1.25619755596146 4.7
1.24043937492037 4.4
1.22279816661409 4.1
1.19920726047565 3.8
1.17841593619748 3.5
1.15783804765819 3.2
1.13611524988078 2.9
1.11226810587956 2.6
1.1 2.45659270787973
1.08252146897138 2.3
1.04890895279984 2
1.02010180615749 1.7
1.00775851452689 1.4
1.02289625185053 1.1
1.072384551468 0.8
1.1 0.712043828637989
1.1788321812551 0.5
1.39767563068446 0.2
1.4 0.198038006120548
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.7 0.610129534219422
2 0.580807464034218
2.3 0.732281898374837
2.3825462625104 0.8
2.6 0.989593766593565
2.70623127130088 1.1
2.9 1.30987841481825
2.97644848453197 1.4
3.2 1.67285684895794
3.22164169850608 1.7
3.43983879933241 2
3.5 2.08748808697256
3.64604282369959 2.3
3.8 2.53487651716097
3.84481819297612 2.6
4.02119666435761 2.9
4.1 3.05642661518254
4.17960815910206 3.2
4.30297675898621 3.5
4.37144751821687 3.8
4.30709007041737 4.1
4.1 4.28230153668627
3.8 4.35222490388517
3.5 4.38120411705341
3.46170663539132 4.4
3.2 4.61182066376775
3.12697968559507 4.7
2.93442324356561 5
2.9 5
2.6 5
2.3 5
2 5
1.93177088047107 5
1.88989799497964 4.7
1.84090824994257 4.4
1.72442786891619 4.1
1.7 4.04653537754382
1.6056668489094 3.8
1.53146425657381 3.5
1.48096129753777 3.2
1.45011586701162 2.9
1.42066100033224 2.6
1.4 2.35440180068522
1.39761876063279 2.3
1.3893591085874 2
1.38597987485128 1.7
1.39368707609039 1.4
1.4 1.33573754068204
1.43441621363816 1.1
1.54457569164011 0.8
1.7 0.610129534219422

2.29398784429908 1.7
2.2544655911244 2
2.3 2.1264305224387
2.44738480305428 2.3
2.6 2.43982420556941
2.7183601949031 2.3
2.63808097239987 2
2.6 1.93952469867833
2.306978936637 1.7
2.3 1.69487362718659
2.29398784429908 1.7
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
2.3 1.69487362718659
2.306978936637 1.7
2.6 1.93952469867833
2.63808097239987 2
2.7183601949031 2.3
2.6 2.43982420556941
2.44738480305428 2.3
2.3 2.1264305224387
2.2544655911244 2
2.29398784429908 1.7
2.3 1.69487362718659
};
\addplot [semithick, steelblue31119180, mark=mystar, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.6 2.3
};
\coordinate (CVI_mean_lml_ep_t) at (axis cs:2.5999999999999996,2.3);
\end{axis}



==> fig/tikz/ionosphere/EP_mean_lml.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 -1
-0.630374544276068 -1
-0.7 -0.843728432300117
-0.785593318332215 -0.7
-0.919178937508608 -0.4
-1 -0.109627768100631
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.7 -0.843728432300117
-0.630374544276068 -1
-0.4 -1
-0.132379190179163 -1
-0.310796245617727 -0.7
-0.4 -0.497425894591842
-0.450781723536628 -0.4
-0.569817564633205 -0.1
-0.646479686118241 0.2
-0.694953083545844 0.5
-0.7 0.549110207640592
-0.73729191753767 0.8
-0.763092475978174 1.1
-0.777629218436182 1.4
-0.785735607562296 1.7
-0.790222709426886 2
-0.792698516120397 2.3
-0.794061766744929 2.6
-0.794810382661111 2.9
-0.795222179624226 3.2
-0.795448542231857 3.5
-0.795572819671237 3.8
-0.795640534724803 4.1
-0.795677323842163 4.4
-0.795697781273079 4.7
-0.795702449312108 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.109627768100631
-0.919178937508608 -0.4
-0.785593318332215 -0.7
-0.7 -0.843728432300117
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.426827238482618
4.79507290425082 0.2
4.7 0.0952656097687691
4.5229259668264 -0.1
4.4 -0.234406995030365
4.24874175977513 -0.4
4.1 -0.56039092815883
3.97065739937761 -0.7
3.8 -0.879343940035325
3.68506178131539 -1
3.8 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
-0.1 -1
0.184428417382373 -1
-0.0133428881864432 -0.7
-0.1 -0.535217643254775
-0.172201134399025 -0.4
-0.293792420360517 -0.1
-0.37689884740682 0.2
-0.4 0.322560735696051
-0.439697740386097 0.5
-0.48122584639067 0.8
-0.505411279782844 1.1
-0.519187650962993 1.4
-0.526918007662885 1.7
-0.53121370972616 2
-0.533588236537153 2.3
-0.534891528340367 2.6
-0.53560497341615 2.9
-0.536010076924284 3.2
-0.53622808782812 3.5
-0.536343840616874 3.8
-0.536412667234086 4.1
-0.536445776675347 4.4
-0.536461378049058 4.7
-0.536476127565304 5
-0.7 5
-0.795702449312108 5
-0.795697781273079 4.7
-0.795677323842163 4.4
-0.795640534724803 4.1
-0.795572819671237 3.8
-0.795448542231857 3.5
-0.795222179624226 3.2
-0.794810382661111 2.9
-0.794061766744929 2.6
-0.792698516120398 2.3
-0.790222709426886 2
-0.785735607562296 1.7
-0.777629218436182 1.4
-0.763092475978174 1.1
-0.73729191753767 0.8
-0.7 0.549110207640592
-0.694953083545844 0.5
-0.646479686118241 0.2
-0.569817564633205 -0.1
-0.450781723536628 -0.4
-0.4 -0.497425894591842
-0.310796245617727 -0.7
-0.132379190179163 -1
-0.1 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
3.2 -1
3.5 -1
3.68506178131539 -1
3.8 -0.879343940035325
3.97065739937761 -0.7
4.1 -0.56039092815883
4.24874175977513 -0.4
4.4 -0.234406995030365
4.5229259668264 -0.1
4.7 0.0952656097687691
4.79507290425082 0.2
5 0.426827238482618
5 0.5
5 0.8
5 1.09428267699756
4.71836459469848 0.8
4.7 0.780814043708929
4.4308968924863 0.5
4.4 0.467759607811532
4.14264626483322 0.2
4.1 0.155607246587923
3.85276667077306 -0.1
3.8 -0.154657380707196
3.55961814751762 -0.4
3.5 -0.461143539438702
3.26008601932133 -0.7
3.2 -0.760404750505741
2.94809540227575 -1
3.2 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
0.2 -1
0.479199202481931 -1
0.247502875016608 -0.7
0.2 -0.628369663921204
0.0683849512924204 -0.4
-0.0636424847392376 -0.1
-0.1 0.0103756471075001
-0.161848042560175 0.2
-0.226837395463425 0.5
-0.267086224872554 0.8
-0.291049919388357 1.1
-0.304886148043596 1.4
-0.312711683416437 1.7
-0.317080803422331 2
-0.319501889551532 2.3
-0.320831810794547 2.6
-0.321560005308259 2.9
-0.321966803128818 3.2
-0.322191204921119 3.5
-0.322308531987494 3.8
-0.322378140559442 4.1
-0.322417490457115 4.4
-0.322430085404546 4.7
-0.322445378548834 5
-0.4 5
-0.536476127565304 5
-0.536461378049058 4.7
-0.536445776675347 4.4
-0.536412667234086 4.1
-0.536343840616874 3.8
-0.53622808782812 3.5
-0.536010076924284 3.2
-0.53560497341615 2.9
-0.534891528340367 2.6
-0.533588236537153 2.3
-0.53121370972616 2
-0.526918007662885 1.7
-0.519187650962993 1.4
-0.505411279782844 1.1
-0.48122584639067 0.8
-0.439697740386097 0.5
-0.4 0.322560735696051
-0.37689884740682 0.2
-0.293792420360517 -0.1
-0.172201134399025 -0.4
-0.1 -0.535217643254775
-0.0133428881864432 -0.7
0.184428417382373 -1
0.2 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
2.6 -1
2.9 -1
2.94809540227575 -1
3.2 -0.760404750505741
3.26008601932133 -0.7
3.5 -0.461143539438702
3.55961814751762 -0.4
3.8 -0.154657380707196
3.85276667077306 -0.1
4.1 0.155607246587923
4.14264626483322 0.2
4.4 0.467759607811532
4.4308968924863 0.5
4.7 0.780814043708929
4.71836459469848 0.8
5 1.09428267699756
5 1.1
5 1.4
5 1.47532757621586
4.92696434844735 1.4
4.7 1.16647268279125
4.63559056209395 1.1
4.4 0.857753796971313
4.3440205693216 0.8
4.1 0.549556500145947
4.05180861616025 0.5
3.8 0.242759288100864
3.75799420849592 0.2
3.5 -0.0608828258763909
3.46064926186942 -0.1
3.2 -0.358249340299958
3.15596750156097 -0.4
2.9 -0.644306462696972
2.83611649980847 -0.7
2.6 -0.911328574550102
2.48333420758498 -1
2.6 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.5 -1
0.8 -1
0.851704894553099 -1
0.8 -0.970608801511826
0.51858866021418 -0.7
0.5 -0.679739695616698
0.310288963410192 -0.4
0.2 -0.199271579713494
0.153542680312456 -0.1
0.0495720145137534 0.2
-0.0211219485052116 0.5
-0.0665969574468901 0.8
-0.0943582997359591 1.1
-0.1 1.20392706846327
-0.110104865332004 1.4
-0.118845221400728 1.7
-0.123715355340529 2
-0.126411431698308 2.3
-0.127897344550025 2.6
-0.128713614925711 2.9
-0.129135922989436 3.2
-0.129388542178392 3.5
-0.129521861119369 3.8
-0.129592059606898 4.1
-0.129651801450066 4.4
-0.129663640310008 4.7
-0.129675902995443 5
-0.322445378548834 5
-0.322430085404546 4.7
-0.322417490457115 4.4
-0.322378140559442 4.1
-0.322308531987494 3.8
-0.322191204921119 3.5
-0.321966803128818 3.2
-0.321560005308259 2.9
-0.320831810794547 2.6
-0.319501889551532 2.3
-0.317080803422331 2
-0.312711683416437 1.7
-0.304886148043596 1.4
-0.291049919388357 1.1
-0.267086224872554 0.8
-0.226837395463425 0.5
-0.161848042560175 0.2
-0.1 0.0103756471075001
-0.0636424847392376 -0.1
0.0683849512924204 -0.4
0.2 -0.628369663921204
0.247502875016608 -0.7
0.479199202481931 -1
0.5 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
2.3 -1
2.48333420758498 -1
2.6 -0.911328574550102
2.83611649980847 -0.7
2.9 -0.644306462696972
3.15596750156097 -0.4
3.2 -0.358249340299958
3.46064926186942 -0.1
3.5 -0.0608828258763909
3.75799420849592 0.2
3.8 0.242759288100864
4.05180861616026 0.5
4.1 0.549556500145947
4.3440205693216 0.8
4.4 0.857753796971313
4.63559056209395 1.1
4.7 1.16647268279125
4.92696434844735 1.4
5 1.47532757621586
5 1.7
5 1.79860441787934
4.90458685456997 1.7
4.7 1.48944103810372
4.61369901425825 1.4
4.4 1.17995927020628
4.32305453962478 1.1
4.1 0.870434683161155
4.03224572773145 0.8
3.8 0.561744343850852
3.74022449903477 0.5
3.5 0.255877067122317
3.4447695525772 0.2
3.2 -0.0434687013171448
3.1414668892108 -0.1
2.9 -0.330362732858763
2.82129136812974 -0.4
2.6 -0.596225355841743
2.46385725622611 -0.7
2.3 -0.828927998362426
2.01611327343486 -1
2.3 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
0.8 -0.970608801511826
0.851704894553099 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.01611327343486 -1
2.3 -0.828927998362426
2.46385725622611 -0.7
2.6 -0.596225355841743
2.82129136812974 -0.4
2.9 -0.330362732858763
3.1414668892108 -0.1
3.2 -0.0434687013171448
3.4447695525772 0.2
3.5 0.255877067122317
3.74022449903477 0.5
3.8 0.561744343850852
4.03224572773145 0.8
4.1 0.870434683161155
4.32305453962478 1.1
4.4 1.17995927020628
4.61369901425825 1.4
4.7 1.48944103810372
4.90458685456997 1.7
5 1.79860441787934
5 2
5 2.10975825070246
4.89452223036283 2
4.7 1.79884980089441
4.60559732911209 1.7
4.4 1.48682540079121
4.31767061744929 1.4
4.1 1.17376296400611
4.03043833288393 1.1
3.8 0.860496725408788
3.74286415722105 0.8
3.5 0.549276996677436
3.45266303811418 0.5
3.2 0.244467083000101
3.15533427178094 0.2
2.9 -0.046962651074745
2.84174802398825 -0.1
2.6 -0.315297756270018
2.49091981872151 -0.4
2.3 -0.547998233825746
2.04518849243425 -0.7
2 -0.728063015706875
1.7 -0.84347044320404
1.4 -0.876876062208286
1.1 -0.813772923282861
0.903271102800505 -0.7
0.8 -0.631117771504194
0.587850889633072 -0.4
0.5 -0.283633927303007
0.398159552004331 -0.1
0.271935494111753 0.2
0.2 0.441070556670682
0.185668150294046 0.5
0.138977337818399 0.8
0.110812553965399 1.1
0.0944223808698643 1.4
0.0851106689774662 1.7
0.0798981238322578 2
0.0770072774649889 2.3
0.0754109687187379 2.6
0.0745312845295598 2.9
0.0740623073289441 3.2
0.0738518375733257 3.5
0.0737101063014443 3.8
0.0736199695477504 4.1
0.0735570261261334 4.4
0.0735683656540531 4.7
0.0735220027235311 5
-0.1 5
-0.129675902995443 5
-0.129663640310008 4.7
-0.129651801450066 4.4
-0.129592059606898 4.1
-0.129521861119369 3.8
-0.129388542178392 3.5
-0.129135922989436 3.2
-0.128713614925711 2.9
-0.127897344550025 2.6
-0.126411431698308 2.3
-0.123715355340529 2
-0.118845221400728 1.7
-0.110104865332004 1.4
-0.1 1.20392706846327
-0.0943582997359591 1.1
-0.0665969574468901 0.8
-0.0211219485052116 0.5
0.0495720145137534 0.2
0.153542680312456 -0.1
0.2 -0.199271579713494
0.310288963410192 -0.4
0.5 -0.679739695616698
0.51858866021418 -0.7
0.8 -0.970608801511826
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.1 -0.813772923282861
1.4 -0.876876062208287
1.7 -0.84347044320404
2 -0.728063015706875
2.04518849243425 -0.7
2.3 -0.547998233825746
2.49091981872151 -0.4
2.6 -0.315297756270018
2.84174802398825 -0.1
2.9 -0.046962651074745
3.15533427178094 0.2
3.2 0.244467083000101
3.45266303811418 0.5
3.5 0.549276996677436
3.74286415722105 0.8
3.8 0.860496725408788
4.03043833288393 1.1
4.1 1.17376296400611
4.31767061744929 1.4
4.4 1.48682540079121
4.60559732911209 1.7
4.7 1.79884980089441
4.89452223036283 2
5 2.10975825070246
5 2.3
5 2.43918523337247
4.86797216510435 2.3
4.7 2.12456627581719
4.58317966001014 2
4.4 1.80745028722645
4.30056828132303 1.7
4.1 1.48766501255591
4.01982553583923 1.4
3.8 1.16609072085129
3.73977037227382 1.1
3.5 0.845462198301538
3.4579818018482 0.8
3.2 0.531079196668367
3.16998738719934 0.5
2.9 0.231241798862957
2.86695869979742 0.2
2.6 -0.0427432083849245
2.52843918686387 -0.1
2.3 -0.277173267437393
2.09416569043076 -0.4
2 -0.456046734766185
1.7 -0.556909102424021
1.4 -0.566147413858327
1.1 -0.468511492605041
0.999584902777726 -0.4
0.8 -0.225308185561794
0.705552974497791 -0.1
0.535053915889397 0.2
0.5 0.289732619593579
0.439117880706818 0.5
0.382871767742134 0.8
0.348411959323356 1.1
0.328189961436426 1.4
0.316649458884579 1.7
0.310173451536976 2
0.306577801542003 2.3
0.304595252232248 2.6
0.303497575407559 2.9
0.302897860540387 3.2
0.30267437192289 3.5
0.30253515896352 3.8
0.302394656010642 4.1
0.302332339057013 4.4
0.302357616854435 4.7
0.302272169606694 5
0.2 5
0.0735220027235311 5
0.0735683656540531 4.7
0.0735570261261334 4.4
0.0736199695477504 4.1
0.0737101063014443 3.8
0.0738518375733257 3.5
0.0740623073289441 3.2
0.0745312845295598 2.9
0.0754109687187379 2.6
0.0770072774649889 2.3
0.0798981238322578 2
0.0851106689774662 1.7
0.0944223808698643 1.4
0.110812553965399 1.1
0.138977337818399 0.8
0.185668150294046 0.5
0.2 0.441070556670682
0.271935494111753 0.2
0.398159552004331 -0.1
0.5 -0.283633927303007
0.587850889633072 -0.4
0.8 -0.631117771504194
0.903271102800505 -0.7
1.1 -0.813772923282861
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.1 -0.468511492605041
1.4 -0.566147413858327
1.7 -0.556909102424021
2 -0.456046734766185
2.09416569043076 -0.4
2.3 -0.277173267437393
2.52843918686387 -0.1
2.6 -0.0427432083849245
2.86695869979742 0.2
2.9 0.231241798862957
3.16998738719934 0.5
3.2 0.531079196668367
3.4579818018482 0.8
3.5 0.845462198301538
3.73977037227382 1.1
3.8 1.16609072085129
4.01982553583923 1.4
4.1 1.48766501255591
4.30056828132303 1.7
4.4 1.80745028722645
4.58317966001014 2
4.7 2.12456627581719
4.86797216510435 2.3
5 2.43918523337247
5 2.6
5 2.822195555668
4.79393993014427 2.6
4.7 2.5001444815168
4.51789937251052 2.3
4.4 2.17312623647465
4.24583395709031 2
4.1 1.84085723723849
3.97685866568074 1.7
3.8 1.50471668519324
3.70909384565925 1.4
3.5 1.16849738532341
3.43969591931967 1.1
3.2 0.838852130674039
3.16417995652777 0.8
2.9 0.525631921574634
2.87401689511687 0.5
2.6 0.242059032544974
2.54918036276977 0.2
2.3 0.00387869130840411
2.12656746349215 -0.1
2 -0.172742819870995
1.7 -0.256660310628476
1.4 -0.225698651653853
1.16659311713766 -0.1
1.1 -0.0459065282426709
0.903313020290944 0.2
0.8 0.4109363092748
0.765391233336146 0.5
0.691823733359029 0.8
0.648099433267094 1.1
0.623081729193137 1.4
0.609060344885945 1.7
0.601284960359536 2
0.596996325520034 2.3
0.594648593538073 2.6
0.593347436434988 2.9
0.592639207747028 3.2
0.592326390937602 3.5
0.592216848361809 3.8
0.592034820514654 4.1
0.591987846855438 4.4
0.592004888010516 4.7
0.591922353365951 5
0.5 5
0.302272169606694 5
0.302357616854435 4.7
0.302332339057013 4.4
0.302394656010642 4.1
0.30253515896352 3.8
0.30267437192289 3.5
0.302897860540387 3.2
0.303497575407559 2.9
0.304595252232248 2.6
0.306577801542003 2.3
0.310173451536976 2
0.316649458884579 1.7
0.328189961436426 1.4
0.348411959323356 1.1
0.382871767742134 0.8
0.439117880706818 0.5
0.5 0.289732619593579
0.535053915889397 0.2
0.705552974497791 -0.1
0.8 -0.225308185561794
0.999584902777726 -0.4
1.1 -0.468511492605041
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.4 -0.225698651653853
1.7 -0.256660310628476
2 -0.172742819870995
2.12656746349215 -0.1
2.3 0.00387869130840408
2.54918036276977 0.2
2.6 0.242059032544974
2.87401689511687 0.5
2.9 0.525631921574634
3.16417995652777 0.8
3.2 0.838852130674039
3.43969591931967 1.1
3.5 1.16849738532341
3.70909384565925 1.4
3.8 1.50471668519324
3.97685866568074 1.7
4.1 1.84085723723849
4.24583395709031 2
4.4 2.17312623647465
4.51789937251052 2.3
4.7 2.5001444815168
4.79393993014427 2.6
5 2.822195555668
5 2.9
5 3.2
5 3.36398410870191
4.86416696881337 3.2
4.7 3.00955871186771
4.61318927582226 2.9
4.4 2.64428598755867
4.36625462018729 2.6
4.12029382459848 2.3
4.1 2.27674916752766
3.87333126497212 2
3.8 1.91436633869338
3.62556655673402 1.7
3.5 1.55238974858146
3.37366019205101 1.4
3.2 1.19913813475713
3.11334197746485 1.1
2.9 0.865832567996902
2.83618440157503 0.8
2.6 0.567484519349088
2.52090768863342 0.5
2.3 0.322328055872802
2.09390514555991 0.2
2 0.148022120169449
1.7 0.093187468812536
1.4 0.19800963392432
1.39764165852953 0.2
1.17862116774814 0.5
1.1 0.709925599604263
1.07148756674104 0.8
1.01846733377682 1.1
0.990443983625179 1.4
0.975783502814695 1.7
0.968099189528386 2
0.964035159530904 2.3
0.961865378994784 2.6
0.960690307999244 2.9
0.96005064071163 3.2
0.959735676798127 3.5
0.9595495320601 3.8
0.959438036209288 4.1
0.959422381227558 4.4
0.959414964350159 4.7
0.959354706393768 5
0.8 5
0.591922353365951 5
0.592004888010516 4.7
0.591987846855438 4.4
0.592034820514654 4.1
0.592216848361809 3.8
0.592326390937602 3.5
0.592639207747028 3.2
0.593347436434988 2.9
0.594648593538073 2.6
0.596996325520034 2.3
0.601284960359536 2
0.609060344885946 1.7
0.623081729193137 1.4
0.648099433267094 1.1
0.691823733359029 0.8
0.765391233336146 0.5
0.8 0.4109363092748
0.903313020290944 0.2
1.1 -0.0459065282426709
1.16659311713766 -0.1
1.4 -0.225698651653853
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.4 0.19800963392432
1.7 0.093187468812536
2 0.148022120169449
2.09390514555991 0.2
2.3 0.322328055872802
2.52090768863342 0.5
2.6 0.567484519349088
2.83618440157503 0.8
2.9 0.865832567996902
3.11334197746485 1.1
3.2 1.19913813475713
3.37366019205101 1.4
3.5 1.55238974858146
3.62556655673402 1.7
3.8 1.91436633869338
3.87333126497212 2
4.1 2.27674916752766
4.12029382459848 2.3
4.36625462018729 2.6
4.4 2.64428598755867
4.61318927582226 2.9
4.7 3.00955871186771
4.86416696881337 3.2
5 3.36398410870191
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.1 5
3.8 5
3.5 5
3.22448356487704 5
3.35855193069072 4.7
3.5 4.55495073247683
3.8 4.44104005316282
3.92660820118737 4.4
4.1 4.32324093824975
4.32851314080946 4.1
4.37778410295361 3.8
4.30590621832074 3.5
4.1811576217969 3.2
4.1 3.05399406486709
4.02225820237411 2.9
3.84541508811821 2.6
3.8 2.53404560194576
3.64652680481759 2.3
3.5 2.0869155912921
3.4402094835399 2
3.22185295339158 1.7
3.2 1.67259554427751
2.97663494919125 1.4
2.9 1.30966900625813
2.70639338375798 1.1
2.6 0.989432881824791
2.38268661308732 0.8
2.3 0.732167178461006
2 0.580653008462253
1.7 0.609777718429224
1.5438858096377 0.8
1.43201523891514 1.1
1.4 1.29931187045626
1.38867430382139 1.4
1.37405033476595 1.7
1.36836978762148 2
1.36641112902869 2.3
1.36583019424259 2.6
1.3656969712779 2.9
1.36568885093531 3.2
1.36570712251373 3.5
1.36572063298586 3.8
1.36573118293138 4.1
1.36574349677644 4.4
1.36574889249246 4.7
1.36568427020987 5
1.1 5
0.959354706393768 5
0.959414964350159 4.7
0.959422381227558 4.4
0.959438036209288 4.1
0.9595495320601 3.8
0.959735676798127 3.5
0.96005064071163 3.2
0.960690307999244 2.9
0.961865378994784 2.6
0.964035159530904 2.3
0.968099189528386 2
0.975783502814695 1.7
0.990443983625179 1.4
1.01846733377682 1.1
1.07148756674104 0.8
1.1 0.709925599604263
1.17862116774814 0.5
1.39764165852953 0.2
1.4 0.19800963392432
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.7 0.609777718429224
2 0.580653008462253
2.3 0.732167178461006
2.38268661308732 0.8
2.6 0.989432881824791
2.70639338375798 1.1
2.9 1.30966900625813
2.97663494919125 1.4
3.2 1.67259554427751
3.22185295339158 1.7
3.4402094835399 2
3.5 2.0869155912921
3.64652680481759 2.3
3.8 2.53404560194576
3.84541508811821 2.6
4.02225820237411 2.9
4.1 3.05399406486709
4.1811576217969 3.2
4.30590621832074 3.5
4.37778410295361 3.8
4.32851314080946 4.1
4.1 4.32324093824975
3.92660820118737 4.4
3.8 4.44104005316282
3.5 4.55495073247683
3.35855193069072 4.7
3.22448356487704 5
3.2 5
2.9 5
2.6 5
2.3 5
2 5
1.7 5
1.4 5
1.36568427020987 5
1.36574889249246 4.7
1.36574349677644 4.4
1.36573118293138 4.1
1.36572063298586 3.8
1.36570712251373 3.5
1.36568885093531 3.2
1.3656969712779 2.9
1.36583019424259 2.6
1.36641112902869 2.3
1.36836978762148 2
1.37405033476595 1.7
1.38867430382139 1.4
1.4 1.29931187045626
1.43201523891514 1.1
1.5438858096377 0.8
1.7 0.609777718429224

2.26863298283404 1.7
2.21079010239148 2
2.28199097320245 2.3
2.3 2.34009611831683
2.6 2.58766341313403
2.77146904463203 2.3
2.65292587020905 2
2.6 1.91740648935923
2.33317051682758 1.7
2.3 1.67553623514475
2.26863298283404 1.7
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
2.3 1.67553623514475
2.33317051682758 1.7
2.6 1.91740648935923
2.65292587020905 2
2.77146904463203 2.3
2.6 2.58766341313403
2.3 2.34009611831683
2.28199097320245 2.3
2.21079010239148 2
2.26863298283404 1.7
2.3 1.67553623514475
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.6 2.3
};
\coordinate (EP_mean_lml_t) at (axis cs:2.5999999999999996,2.3);
\end{axis}



==> fig/tikz/ionosphere/EP_nlpd.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.993046079078129 -0.7
-1 -0.682456059536561
-1 -0.7
-1 -1
-0.849950118890908 -1
-0.993046079078129 -0.7
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.24687971172109
4.85320131676648 -0.4
4.7 -0.564179877493954
4.57400800820614 -0.7
4.4 -0.896589166387531
4.30937018348592 -1
4.4 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.7 -1
-0.4 -1
-0.357937770746485 -1
-0.4 -0.920454737259672
-0.536478658983322 -0.7
-0.668882385722362 -0.4
-0.7 -0.307190537287978
-0.793642587061063 -0.1
-0.883283955161926 0.2
-0.93755948177925 0.5
-0.969701315703878 0.8
-0.988285271423967 1.1
-0.998807839551515 1.4
-1 1.45981242394716
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.682456059536561
-0.993046079078129 -0.7
-0.849950118890908 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
3.8 -1
4.1 -1
4.30937018348592 -1
4.4 -0.896589166387531
4.57400800820614 -0.7
4.7 -0.564179877493954
4.85320131676648 -0.4
5 -0.24687971172109
5 -0.1
5 0.2
5 0.5
5 0.509109080195882
4.99090977543248 0.5
4.7 0.208089488016905
4.69193305761424 0.2
4.4 -0.0936073795393936
4.39362729509308 -0.1
4.1 -0.39638395564762
4.09639160331966 -0.4
3.80130108788315 -0.7
3.8 -0.701366710250752
3.51195801435298 -1
3.8 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
-0.4 -0.920454737259672
-0.357937770746485 -1
-0.1 -1
-0.0824055721056321 -1
-0.1 -0.971420065557444
-0.268896990869209 -0.7
-0.4 -0.419047132875951
-0.410237711507883 -0.4
-0.540450355437839 -0.1
-0.62531488153994 0.2
-0.679766916308785 0.5
-0.7 0.676654458601436
-0.719466766498174 0.8
-0.747704236298657 1.1
-0.763608410569283 1.4
-0.772535129587902 1.7
-0.777428886332772 2
-0.780190355359319 2.3
-0.78165340431827 2.6
-0.782472362631639 2.9
-0.782928435718369 3.2
-0.78315853779024 3.5
-0.783325628990979 3.8
-0.783377518707213 4.1
-0.783424312519485 4.4
-0.783438195606944 4.7
-0.783394177349718 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.45981242394716
-0.998807839551515 1.4
-0.988285271423967 1.1
-0.969701315703878 0.8
-0.93755948177925 0.5
-0.883283955161926 0.2
-0.793642587061063 -0.1
-0.7 -0.307190537287978
-0.668882385722362 -0.4
-0.536478658983322 -0.7
-0.4 -0.920454737259672
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
3.2 -1
3.5 -1
3.51195801435298 -1
3.8 -0.701366710250752
3.80130108788315 -0.7
4.09639160331966 -0.4
4.1 -0.39638395564762
4.39362729509308 -0.1
4.4 -0.0936073795393936
4.69193305761424 0.2
4.7 0.208089488016905
4.99090977543248 0.5
5 0.509109080195882
5 0.8
5 0.858779853419721
4.94133912778899 0.8
4.7 0.558291782569271
4.64184520524559 0.5
4.4 0.257657277863762
4.34243340741268 0.2
4.1 -0.0429898474741598
4.04286453020555 -0.1
3.8 -0.343241633812952
3.74253488893468 -0.4
3.5 -0.642229456715975
3.44023596924593 -0.7
3.2 -0.938535492804216
3.13396689201265 -1
3.2 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
-0.1 -0.971420065557444
-0.0824055721056321 -1
0.139742943908956 -1
-0.0508494033851291 -0.7
-0.1 -0.611361128063785
-0.214278985563612 -0.4
-0.337055175836026 -0.1
-0.4 0.108357305753898
-0.430514109622992 0.2
-0.498167527661812 0.5
-0.539319310126744 0.8
-0.563583144490135 1.1
-0.577508389544066 1.4
-0.585389895432187 1.7
-0.589760253789016 2
-0.592204803099541 2.3
-0.593495215086206 2.6
-0.594175424972845 2.9
-0.594649588038568 3.2
-0.594883104188035 3.5
-0.595025285652373 3.8
-0.59507301131138 4.1
-0.595084912647465 4.4
-0.595094202084801 4.7
-0.595088424196251 5
-0.7 5
-0.783394177349718 5
-0.783438195606944 4.7
-0.783424312519485 4.4
-0.783377518707213 4.1
-0.783325628990979 3.8
-0.78315853779024 3.5
-0.782928435718369 3.2
-0.782472362631639 2.9
-0.78165340431827 2.6
-0.780190355359319 2.3
-0.777428886332772 2
-0.772535129587902 1.7
-0.763608410569283 1.4
-0.747704236298657 1.1
-0.719466766498174 0.8
-0.7 0.676654458601436
-0.679766916308785 0.5
-0.62531488153994 0.2
-0.540450355437839 -0.1
-0.410237711507883 -0.4
-0.4 -0.419047132875951
-0.268896990869209 -0.7
-0.1 -0.971420065557444
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
2.9 -1
3.13396689201265 -1
3.2 -0.938535492804216
3.44023596924593 -0.7
3.5 -0.642229456715976
3.74253488893468 -0.4
3.8 -0.343241633812952
4.04286453020555 -0.1
4.1 -0.0429898474741598
4.34243340741268 0.2
4.4 0.257657277863762
4.64184520524559 0.5
4.7 0.558291782569271
4.94133912778899 0.8
5 0.858779853419721
5 1.1
5 1.12642507698041
4.97367524355801 1.1
4.7 0.825869303308933
4.6742602462231 0.8
4.4 0.525211052995519
4.37492062503265 0.5
4.1 0.224726243207143
4.07532622276323 0.2
3.8 -0.0748360969905174
3.77461393404871 -0.1
3.5 -0.371886272216511
3.47089459464273 -0.4
3.2 -0.663623571536255
3.16040236203237 -0.7
2.9 -0.945894839270928
2.8360181773609 -1
2.9 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.2 -1
0.366572749902599 -1
0.2 -0.779972914481214
0.14746951165139 -0.7
-0.022676448951135 -0.4
-0.1 -0.236449489236339
-0.160313441719449 -0.1
-0.257888581354024 0.2
-0.324332189624473 0.5
-0.367337059182322 0.8
-0.393733183253564 1.1
-0.4 1.2208968984157
-0.409609410327006 1.4
-0.418709921435284 1.7
-0.423783092273418 2
-0.426565334247583 2.3
-0.428037449007648 2.6
-0.428746124534195 2.9
-0.429382395982182 3.2
-0.4296927277858 3.5
-0.429841738310072 3.8
-0.429898852079318 4.1
-0.429875553535031 4.4
-0.429876678969414 4.7
-0.429861888769289 5
-0.595088424196251 5
-0.595094202084801 4.7
-0.595084912647465 4.4
-0.59507301131138 4.1
-0.595025285652373 3.8
-0.594883104188035 3.5
-0.594649588038568 3.2
-0.594175424972845 2.9
-0.593495215086206 2.6
-0.592204803099541 2.3
-0.589760253789016 2
-0.585389895432187 1.7
-0.577508389544066 1.4
-0.563583144490136 1.1
-0.539319310126744 0.8
-0.498167527661812 0.5
-0.430514109622992 0.2
-0.4 0.108357305753898
-0.337055175836026 -0.1
-0.214278985563612 -0.4
-0.1 -0.611361128063785
-0.0508494033851291 -0.7
0.139742943908956 -1
0.2 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
2.6 -1
2.8360181773609 -1
2.9 -0.945894839270928
3.16040236203237 -0.7
3.2 -0.663623571536255
3.47089459464273 -0.4
3.5 -0.371886272216511
3.77461393404871 -0.1
3.8 -0.0748360969905174
4.07532622276323 0.2
4.1 0.224726243207143
4.37492062503265 0.5
4.4 0.525211052995519
4.6742602462231 0.8
4.7 0.825869303308933
4.97367524355801 1.1
5 1.12642507698041
5 1.35119532891518
4.74975831260738 1.1
4.7 1.05015887910102
4.45109387847556 0.8
4.4 0.748807626121454
4.15249190300204 0.5
4.1 0.447440671870792
3.85308436603527 0.2
3.8 0.147010132831059
3.55080910460021 -0.1
3.5 -0.150304432265112
3.24149672463198 -0.4
3.2 -0.440382920039311
2.91739327975142 -0.7
2.9 -0.716424266260446
2.6 -0.973637713325355
2.56338068847013 -1
2.6 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
0.2 -0.779972914481214
0.366572749902599 -1
0.5 -1
0.629990289721692 -1
0.5 -0.875078333332229
0.367261982063186 -0.7
0.2 -0.458460791605014
0.166364896784398 -0.4
0.0241993832909909 -0.1
-0.0878921264711029 0.2
-0.1 0.244471795285214
-0.159632182430639 0.5
-0.204344217437112 0.8
-0.231519957724939 1.1
-0.247387832171849 1.4
-0.256455803834689 1.7
-0.261538512817302 2
-0.26436363197156 2.3
-0.265879939526243 2.6
-0.266646220747686 2.9
-0.267141908958684 3.2
-0.267477563584968 3.5
-0.267575731860339 3.8
-0.267630430797114 4.1
-0.267719246510437 4.4
-0.26769890214087 4.7
-0.267665572560852 5
-0.4 5
-0.429861888769289 5
-0.429876678969414 4.7
-0.429875553535031 4.4
-0.429898852079318 4.1
-0.429841738310072 3.8
-0.4296927277858 3.5
-0.429382395982182 3.2
-0.428746124534195 2.9
-0.428037449007648 2.6
-0.426565334247583 2.3
-0.423783092273418 2
-0.418709921435284 1.7
-0.409609410327006 1.4
-0.4 1.2208968984157
-0.393733183253564 1.1
-0.367337059182322 0.8
-0.324332189624473 0.5
-0.257888581354024 0.2
-0.160313441719449 -0.1
-0.1 -0.236449489236339
-0.022676448951135 -0.4
0.14746951165139 -0.7
0.2 -0.779972914481214
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
2.3 -1
2.56338068847013 -1
2.6 -0.973637713325355
2.9 -0.716424266260446
2.91739327975142 -0.7
3.2 -0.440382920039311
3.24149672463198 -0.4
3.5 -0.150304432265112
3.55080910460021 -0.1
3.8 0.147010132831059
3.85308436603527 0.2
4.1 0.447440671870792
4.15249190300204 0.5
4.4 0.748807626121454
4.45109387847556 0.8
4.7 1.05015887910102
4.74975831260738 1.1
5 1.35119532891518
5 1.4
5 1.56133179449268
4.83982007691019 1.4
4.7 1.25969319705762
4.54193160934562 1.1
4.4 0.957418150765352
4.24459278032004 0.8
4.1 0.654719633906387
3.94718300774705 0.5
3.8 0.352535376728952
3.64801323224508 0.2
3.5 0.0531435657888305
3.34345388562429 -0.1
3.2 -0.23912144005127
3.0263498600475 -0.4
2.9 -0.517289012350681
2.68244783241513 -0.7
2.6 -0.771221138177949
2.3 -0.987745069744542
2.27729139289291 -1
2.3 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
0.5 -0.875078333332229
0.629990289721692 -1
0.8 -1
1.05545398714696 -1
0.8 -0.854540475370865
0.638771266685746 -0.7
0.5 -0.553063817519783
0.39634590892488 -0.4
0.21733783382211 -0.1
0.2 -0.0641805615290039
0.104255476878184 0.2
0.0253402917276357 0.5
-0.0280817230927953 0.8
-0.061766473177585 1.1
-0.0818046161018843 1.4
-0.0933903756762468 1.7
-0.0998966107425815 2
-0.1 2.00845331718299
-0.102818596863842 2.3
-0.104395771352929 2.6
-0.105246529332984 2.9
-0.105555886955312 3.2
-0.105914382403055 3.5
-0.105953018805659 3.8
-0.106004242239955 4.1
-0.106236914629795 4.4
-0.106192153519174 4.7
-0.106137732734427 5
-0.267665572560852 5
-0.26769890214087 4.7
-0.267719246510437 4.4
-0.267630430797114 4.1
-0.267575731860339 3.8
-0.267477563584968 3.5
-0.267141908958684 3.2
-0.266646220747686 2.9
-0.265879939526243 2.6
-0.26436363197156 2.3
-0.261538512817302 2
-0.256455803834689 1.7
-0.247387832171849 1.4
-0.231519957724939 1.1
-0.204344217437112 0.8
-0.159632182430639 0.5
-0.1 0.244471795285214
-0.0878921264711029 0.2
0.0241993832909909 -0.1
0.166364896784398 -0.4
0.2 -0.458460791605014
0.367261982063186 -0.7
0.5 -0.875078333332229
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
2 -1
2.27729139289291 -1
2.3 -0.987745069744542
2.6 -0.771221138177949
2.68244783241513 -0.7
2.9 -0.517289012350681
3.0263498600475 -0.4
3.2 -0.23912144005127
3.34345388562429 -0.1
3.5 0.0531435657888305
3.64801323224508 0.2
3.8 0.352535376728952
3.94718300774705 0.5
4.1 0.654719633906387
4.24459278032004 0.8
4.4 0.957418150765352
4.54193160934562 1.1
4.7 1.25969319705762
4.8398200769102 1.4
5 1.56133179449268
5 1.7
5 1.76793456418427
4.93290164124145 1.7
4.7 1.46541924972923
4.63576425038947 1.4
4.4 1.16181665788069
4.3396741216021 1.1
4.1 0.857248649180256
4.04432055223204 0.8
3.8 0.552683710269904
3.74848380049002 0.5
3.5 0.25064030286078
3.44930010595965 0.2
3.2 -0.0440540982500887
3.14081443446033 -0.1
2.9 -0.323808055198171
2.81043760080094 -0.4
2.6 -0.578275896693289
2.42851890431244 -0.7
2.3 -0.79407670646572
2 -0.954737321217756
1.85185215694523 -1
2 -1
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
0.8 -0.854540475370865
1.05545398714696 -1
1.1 -1
1.4 -1
1.7 -1
1.85185215694523 -1
2 -0.954737321217756
2.3 -0.79407670646572
2.42851890431244 -0.7
2.6 -0.578275896693289
2.81043760080094 -0.4
2.9 -0.323808055198171
3.14081443446033 -0.1
3.2 -0.0440540982500887
3.44930010595965 0.2
3.5 0.25064030286078
3.74848380049002 0.5
3.8 0.552683710269904
4.04432055223204 0.8
4.1 0.857248649180256
4.3396741216021 1.1
4.4 1.16181665788069
4.63576425038947 1.4
4.7 1.46541924972923
4.93290164124145 1.7
5 1.76793456418427
5 1.97561738612771
4.72777518371461 1.7
4.7 1.67202457054423
4.43289662792351 1.4
4.4 1.36676583167154
4.13966753179712 1.1
4.1 1.05982316796211
3.8472986574076 0.8
3.8 0.752121389901928
3.55346581027833 0.5
3.5 0.446345724622624
3.25336438705756 0.2
3.2 0.147758556652563
2.93789446886879 -0.1
2.9 -0.135218351421903
2.6 -0.390193974536719
2.5862366421956 -0.4
2.3 -0.601695240989293
2.10560703476903 -0.7
2 -0.755625469598971
1.7 -0.831514612525769
1.4 -0.819574054929143
1.1 -0.717300123504848
1.07046957139096 -0.7
0.8 -0.50365725368589
0.70253029744019 -0.4
0.5 -0.14560277858027
0.473962237522076 -0.1
0.337557427665275 0.2
0.231837189546066 0.5
0.2 0.632099489302464
0.171789364504152 0.8
0.140296850573636 1.1
0.121480334631978 1.4
0.110618581253024 1.7
0.10447332407532 2
0.101131159178147 2.3
0.0993685051275202 2.6
0.0982617817495881 2.9
0.0977668586843641 3.2
0.0975881004118903 3.5
0.0975566044602504 3.8
0.0975292805116182 4.1
0.0973719704274078 4.4
0.0973847026853033 4.7
0.0973331713354009 5
-0.1 5
-0.106137732734427 5
-0.106192153519174 4.7
-0.106236914629795 4.4
-0.106004242239955 4.1
-0.105953018805659 3.8
-0.105914382403055 3.5
-0.105555886955312 3.2
-0.105246529332984 2.9
-0.104395771352929 2.6
-0.102818596863842 2.3
-0.1 2.00845331718299
-0.0998966107425815 2
-0.0933903756762468 1.7
-0.0818046161018843 1.4
-0.061766473177585 1.1
-0.0280817230927953 0.8
0.0253402917276357 0.5
0.104255476878184 0.2
0.2 -0.0641805615290039
0.21733783382211 -0.1
0.39634590892488 -0.4
0.5 -0.553063817519783
0.638771266685746 -0.7
0.8 -0.854540475370865
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.1 -0.717300123504848
1.4 -0.819574054929143
1.7 -0.831514612525769
2 -0.755625469598971
2.10560703476903 -0.7
2.3 -0.601695240989293
2.5862366421956 -0.4
2.6 -0.390193974536719
2.9 -0.135218351421903
2.93789446886879 -0.1
3.2 0.147758556652563
3.25336438705756 0.2
3.5 0.446345724622624
3.55346581027833 0.5
3.8 0.752121389901928
3.8472986574076 0.8
4.1 1.05982316796211
4.13966753179712 1.1
4.4 1.36676583167154
4.43289662792351 1.4
4.7 1.67202457054423
4.72777518371461 1.7
5 1.97561738612771
5 2
5 2.19944327441909
4.804587589948 2
4.7 1.89400416226158
4.51178565946804 1.7
4.4 1.58600129679774
4.2215019061107 1.4
4.1 1.27529462689647
3.93311107214859 1.1
3.8 0.962918754229442
3.64458189756714 0.8
3.5 0.651978067790234
3.35178492880512 0.5
3.2 0.348400988118726
3.04699621027399 0.2
2.9 0.0613250389957688
2.71440988430729 -0.1
2.6 -0.196904386000443
2.31494285687438 -0.4
2.3 -0.410529410543765
2 -0.552440834580388
1.7 -0.607577434481008
1.4 -0.550835334708847
1.13532473026318 -0.4
1.1 -0.370633471393881
0.837668679764822 -0.1
0.8 -0.0406410278354222
0.653212400878943 0.2
0.523787202640514 0.5
0.5 0.584968949593239
0.451997769224608 0.8
0.408662733428489 1.1
0.3823319980857 1.4
0.366990589724622 1.7
0.35827936013098 2
0.353531054173327 2.3
0.351246260295598 2.6
0.349637397199726 2.9
0.348893314331963 3.2
0.348571153147261 3.5
0.348840643381239 3.8
0.348588920653255 4.1
0.348364875494424 4.4
0.348585915178597 4.7
0.34816792119646 5
0.2 5
0.0973331713354009 5
0.0973847026853033 4.7
0.0973719704274078 4.4
0.0975292805116182 4.1
0.0975566044602504 3.8
0.0975881004118903 3.5
0.0977668586843641 3.2
0.0982617817495881 2.9
0.0993685051275202 2.6
0.101131159178147 2.3
0.10447332407532 2
0.110618581253024 1.7
0.121480334631978 1.4
0.140296850573636 1.1
0.171789364504152 0.8
0.2 0.632099489302464
0.231837189546066 0.5
0.337557427665275 0.2
0.473962237522076 -0.1
0.5 -0.14560277858027
0.70253029744019 -0.4
0.8 -0.50365725368589
1.07046957139096 -0.7
1.1 -0.717300123504848
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.4 -0.550835334708847
1.7 -0.607577434481008
2 -0.552440834580388
2.3 -0.410529410543765
2.31494285687438 -0.4
2.6 -0.196904386000443
2.71440988430729 -0.1
2.9 0.0613250389957688
3.04699621027399 0.2
3.2 0.348400988118726
3.35178492880512 0.5
3.5 0.651978067790234
3.64458189756714 0.8
3.8 0.962918754229442
3.93311107214859 1.1
4.1 1.27529462689647
4.2215019061107 1.4
4.4 1.58600129679774
4.51178565946804 1.7
4.7 1.89400416226158
4.804587589948 2
5 2.19944327441909
5 2.3
5 2.44636158565678
4.85848708705163 2.3
4.7 2.13773624406678
4.56892058546589 2
4.4 1.82512336774664
4.2829418928299 1.7
4.1 1.50832541244215
3.99995230821653 1.4
3.8 1.18871607699375
3.71807646942649 1.1
3.5 0.870168904790018
3.43370998869079 0.8
3.2 0.559698870448264
3.14020848507106 0.5
2.9 0.267770960737543
2.82387370420785 0.2
2.6 0.00811937327108038
2.44959969158175 -0.1
2.3 -0.203267698363978
2 -0.340880196835296
1.7 -0.374019738910392
1.4 -0.256458234804257
1.21975663010257 -0.1
1.1 0.0640601854715124
1.00723761527305 0.2
0.876357947863023 0.5
0.8 0.794484022584544
0.798334140843649 0.8
0.739619115694817 1.1
0.704469933150752 1.4
0.684186760262167 1.7
0.672756573758448 2
0.666600181227111 2.3
0.663380526605021 2.6
0.661420409849163 2.9
0.660333958330392 3.2
0.659665636686648 3.5
0.659793562946923 3.8
0.659258978252257 4.1
0.658929955583364 4.4
0.659302026101016 4.7
0.658983529003759 5
0.5 5
0.34816792119646 5
0.348585915178597 4.7
0.348364875494424 4.4
0.348588920653255 4.1
0.348840643381239 3.8
0.348571153147261 3.5
0.348893314331963 3.2
0.349637397199726 2.9
0.351246260295598 2.6
0.353531054173327 2.3
0.35827936013098 2
0.366990589724622 1.7
0.3823319980857 1.4
0.408662733428489 1.1
0.451997769224608 0.8
0.5 0.584968949593239
0.523787202640514 0.5
0.653212400878943 0.2
0.8 -0.0406410278354222
0.837668679764823 -0.1
1.1 -0.370633471393881
1.13532473026318 -0.4
1.4 -0.550835334708847
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.4 -0.256458234804257
1.7 -0.374019738910392
2 -0.340880196835296
2.3 -0.203267698363978
2.44959969158175 -0.1
2.6 0.00811937327108038
2.82387370420785 0.2
2.9 0.267770960737543
3.14020848507106 0.5
3.2 0.559698870448264
3.43370998869079 0.8
3.5 0.870168904790018
3.71807646942649 1.1
3.8 1.18871607699375
3.99995230821653 1.4
4.1 1.50832541244215
4.2829418928299 1.7
4.4 1.82512336774664
4.56892058546589 2
4.7 2.13773624406678
4.85848708705163 2.3
5 2.44636158565678
5 2.6
5 2.73853888808747
4.86926255651825 2.6
4.7 2.42355703376729
4.58627005430564 2.3
4.4 2.10216316840005
4.30830222030347 2
4.1 1.7743813955664
4.03437893238666 1.7
3.8 1.44248338367175
3.7625036632485 1.4
3.5 1.11170253308973
3.48938493367785 1.1
3.20750490775865 0.8
3.2 0.792283437170621
2.90726297891657 0.5
2.9 0.492978288774939
2.6 0.230083634848384
2.55836356257174 0.2
2.3 0.0241604911285129
2.02263590401721 -0.1
2 -0.109516372423506
1.7 -0.110734837134658
1.67756298388837 -0.1
1.4 0.0959175408865534
1.31921692397477 0.2
1.17233870617443 0.5
1.1 0.747576818049967
1.08371998796512 0.8
1.02426492781079 1.1
0.988862447207624 1.4
0.968224636454071 1.7
0.956469277568601 2
0.949992209987533 2.3
0.946481130021191 2.6
0.944482768613946 2.9
0.943304814758561 3.2
0.942745530250826 3.5
0.942357065587006 3.8
0.942087505346352 4.1
0.941609121201042 4.4
0.941546963991914 4.7
0.941444288896334 5
0.8 5
0.658983529003759 5
0.659302026101016 4.7
0.658929955583364 4.4
0.659258978252257 4.1
0.659793562946923 3.8
0.659665636686648 3.5
0.660333958330392 3.2
0.661420409849163 2.9
0.663380526605021 2.6
0.666600181227111 2.3
0.672756573758448 2
0.684186760262167 1.7
0.704469933150751 1.4
0.739619115694817 1.1
0.798334140843649 0.8
0.8 0.794484022584544
0.876357947863023 0.5
1.00723761527305 0.2
1.1 0.0640601854715124
1.21975663010257 -0.1
1.4 -0.256458234804257
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
1.7 -0.110734837134658
2 -0.109516372423506
2.02263590401721 -0.1
2.3 0.0241604911285129
2.55836356257174 0.2
2.6 0.230083634848384
2.9 0.492978288774938
2.90726297891657 0.5
3.2 0.792283437170621
3.20750490775865 0.8
3.48938493367785 1.1
3.5 1.11170253308973
3.7625036632485 1.4
3.8 1.44248338367175
4.03437893238666 1.7
4.1 1.7743813955664
4.30830222030347 2
4.4 2.10216316840005
4.58627005430564 2.3
4.7 2.42355703376729
4.86926255651825 2.6
5 2.73853888808747
5 2.9
5 3.13382969038957
4.78966029061125 2.9
4.7 2.80321242644039
4.52406910265262 2.6
4.4 2.46194568980428
4.26453728135678 2.3
4.1 2.11144265305537
4.00847673373854 2
3.8 1.75638039628226
3.75345225060271 1.7
3.5 1.4042420922237
3.4963650754636 1.4
3.22490571632994 1.1
3.2 1.07337332988174
2.93525860908636 0.8
2.9 0.764805592806116
2.60960792916 0.5
2.6 0.491616695619393
2.3 0.289331647207929
2.07713012603599 0.2
2 0.171910323306799
1.78683009709281 0.2
1.7 0.217560867244063
1.4566715290214 0.5
1.4 0.61092303221788
1.33562074773269 0.8
1.27269146896813 1.1
1.23469718681288 1.4
1.2120965125271 1.7
1.19900579946449 2
1.1915515788169 2.3
1.18755269110716 2.6
1.18526550048697 2.9
1.18399298407842 3.2
1.18342572760026 3.5
1.18293633954783 3.8
1.18281521051986 4.1
1.18237741589526 4.4
1.18204493686969 4.7
1.18137968051848 5
1.1 5
0.941444288896334 5
0.941546963991914 4.7
0.941609121201042 4.4
0.942087505346352 4.1
0.942357065587006 3.8
0.942745530250826 3.5
0.943304814758561 3.2
0.944482768613946 2.9
0.946481130021191 2.6
0.949992209987533 2.3
0.956469277568601 2
0.968224636454071 1.7
0.988862447207624 1.4
1.02426492781079 1.1
1.08371998796512 0.8
1.1 0.747576818049967
1.17233870617443 0.5
1.31921692397477 0.2
1.4 0.0959175408865534
1.67756298388837 -0.1
1.7 -0.110734837134658
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
2 0.171910323306799
2.07713012603599 0.2
2.3 0.289331647207929
2.6 0.491616695619393
2.60960792916 0.5
2.9 0.764805592806116
2.93525860908636 0.8
3.2 1.07337332988174
3.22490571632994 1.1
3.4963650754636 1.4
3.5 1.4042420922237
3.75345225060271 1.7
3.8 1.75638039628226
4.00847673373854 2
4.1 2.11144265305537
4.26453728135678 2.3
4.4 2.46194568980428
4.52406910265262 2.6
4.7 2.80321242644039
4.78966029061125 2.9
5 3.13382969038957
5 3.2
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.505255374827 5
4.50603353968448 4.7
4.54639259407966 4.4
4.64517825771178 4.1
4.7 3.86206165153993
4.71687112029294 3.8
4.7 3.75567513038573
4.6321226827839 3.5
4.47311820367621 3.2
4.4 3.0930197664394
4.28698432164876 2.9
4.1 2.61694847284583
4.08990695133634 2.6
3.87281492371227 2.3
3.8 2.20604311270138
3.6466617881235 2
3.5 1.81232591215152
3.4118394266757 1.7
3.2 1.44161353162266
3.16392146029599 1.4
2.9 1.10887922551414
2.8908431194666 1.1
2.6 0.83284786921299
2.5532548214612 0.8
2.3 0.635305913651329
2 0.547711562257116
1.7 0.716528847770479
1.65374309447749 0.8
1.55101651992251 1.1
1.49054680290274 1.4
1.45495832752082 1.7
1.43441182524898 2
1.42275575334912 2.3
1.41624607749528 2.6
1.41269036265828 2.9
1.41064426051652 3.2
1.40978717544081 3.5
1.40912803360263 3.8
1.40892994530028 4.1
1.40917322604842 4.4
1.40866957628493 4.7
1.40633117353011 5
1.4 5
1.18137968051848 5
1.18204493686969 4.7
1.18237741589526 4.4
1.18281521051986 4.1
1.18293633954783 3.8
1.18342572760026 3.5
1.18399298407842 3.2
1.18526550048697 2.9
1.18755269110716 2.6
1.1915515788169 2.3
1.19900579946449 2
1.2120965125271 1.7
1.23469718681288 1.4
1.27269146896813 1.1
1.33562074773269 0.8
1.4 0.61092303221788
1.4566715290214 0.5
1.7 0.217560867244063
1.78683009709281 0.2
2 0.171910323306799
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
1.7 0.716528847770479
2 0.547711562257116
2.3 0.635305913651329
2.5532548214612 0.8
2.6 0.83284786921299
2.8908431194666 1.1
2.9 1.10887922551414
3.16392146029599 1.4
3.2 1.44161353162266
3.4118394266757 1.7
3.5 1.81232591215152
3.6466617881235 2
3.8 2.20604311270138
3.87281492371227 2.3
4.08990695133634 2.6
4.1 2.61694847284583
4.28698432164876 2.9
4.4 3.0930197664394
4.47311820367621 3.2
4.6321226827839 3.5
4.7 3.75567513038573
4.71687112029294 3.8
4.7 3.86206165153993
4.64517825771178 4.1
4.54639259407966 4.4
4.50603353968448 4.7
4.505255374827 5
4.4 5
4.1 5
3.95391354402175 5
3.93256537312184 4.7
3.9078194369511 4.4
3.87959881448346 4.1
3.84416880756817 3.8
3.8 3.52907519501967
3.79505338161763 3.5
3.73189737074098 3.2
3.64067221243657 2.9
3.51606543286772 2.6
3.5 2.57058423979862
3.3522359616821 2.3
3.2 2.052288950481
3.16474988834593 2
2.937081189354 1.7
2.9 1.65535953720146
2.64956032620939 1.4
2.6 1.35240622244255
2.3 1.16870878209477
2 1.21074464032854
1.89681784964567 1.4
1.80839307455314 1.7
1.76167682089118 2
1.73703264915858 2.3
1.72411896652108 2.6
1.71793967091603 2.9
1.71369628797411 3.2
1.71227828942232 3.5
1.71046867506278 3.8
1.7110905924772 4.1
1.71105188975203 4.4
1.71015728447808 4.7
1.7110805040372 5
1.7 5
1.40633117353011 5
1.40866957628493 4.7
1.40917322604842 4.4
1.40892994530028 4.1
1.40912803360263 3.8
1.40978717544081 3.5
1.41064426051652 3.2
1.41269036265828 2.9
1.41624607749528 2.6
1.42275575334912 2.3
1.43441182524898 2
1.45495832752082 1.7
1.49054680290274 1.4
1.55101651992251 1.1
1.65374309447749 0.8
1.7 0.716528847770479
};
\addplot [draw=none, fill=lavender231240249]
table{%
x  y
2 1.21074464032854
2.3 1.16870878209477
2.6 1.35240622244255
2.64956032620939 1.4
2.9 1.65535953720146
2.937081189354 1.7
3.16474988834593 2
3.2 2.052288950481
3.3522359616821 2.3
3.5 2.57058423979862
3.51606543286772 2.6
3.64067221243657 2.9
3.73189737074098 3.2
3.79505338161763 3.5
3.8 3.52907519501967
3.84416880756817 3.8
3.87959881448346 4.1
3.9078194369511 4.4
3.93256537312183 4.7
3.95391354402175 5
3.8 5
3.5 5
3.2 5
2.9 5
2.6 5
2.3 5
2 5
1.7110805040372 5
1.71015728447808 4.7
1.71105188975203 4.4
1.7110905924772 4.1
1.71046867506278 3.8
1.71227828942232 3.5
1.71369628797411 3.2
1.71793967091603 2.9
1.72411896652108 2.6
1.73703264915858 2.3
1.76167682089118 2
1.80839307455314 1.7
1.89681784964567 1.4
2 1.21074464032854
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.6 2.3
};
\coordinate (MCMC_mean_lml_t) at (axis cs:2.5999999999999996,2.3);
\end{axis}



==> fig/tikz/ionosphere/LA_mean_lml.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=black]
table{%
x  y
-0.98969493285119 1.7
-0.7 1.93693563293899
-0.652825288184789 2
-0.437576679648867 2.3
-0.4 2.35640348206868
-0.277416713887113 2.6
-0.144547272436322 2.9
-0.1 3.01282375519994
-0.0281011272545283 3.2
0.0736613366237861 3.5
0.162416549525102 3.8
0.2 3.94225437591525
0.247811884759637 4.1
0.328888969255092 4.4
0.404341536628608 4.7
0.470007344680966 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.69130526173602
-0.98969493285119 1.7
};
\addplot [draw=none, fill=midnightblue854116]
table{%
x  y
-0.7 1.69522539761921
-0.69650109110355 1.7
-0.472293788152735 2
-0.4 2.10179585665403
-0.293718578941505 2.3
-0.148573212141849 2.6
-0.1 2.71164183812745
-0.0207032836296829 2.9
0.0909767474335347 3.2
0.187932735948772 3.5
0.2 3.54144431056564
0.286412110418002 3.8
0.374183169179918 4.1
0.451007887873279 4.4
0.5 4.59778741921424
0.529495024471819 4.7
0.602583322814291 5
0.5 5
0.470007344680966 5
0.404341536628608 4.7
0.328888969255092 4.4
0.247811884759637 4.1
0.2 3.94225437591525
0.162416549525102 3.8
0.0736613366237861 3.5
-0.0281011272545283 3.2
-0.1 3.01282375519994
-0.144547272436322 2.9
-0.277416713887114 2.6
-0.4 2.35640348206868
-0.437576679648867 2.3
-0.652825288184789 2
-0.7 1.93693563293899
-0.98969493285119 1.7
-1 1.69130526173602
-1 1.44233700257652
-0.7 1.69522539761921
};
\addplot [draw=none, fill=midnightblue868137]
table{%
x  y
-0.740141378782518 1.4
-0.7 1.43354846338111
-0.504739834315994 1.7
-0.4 1.84301533946911
-0.313148042980968 2
-0.157408887798162 2.3
-0.1 2.42100461315329
-0.0182577713764361 2.6
0.103967139622306 2.9
0.2 3.1703635372307
0.212060055153895 3.2
0.322183695776578 3.5
0.417575962384454 3.8
0.5 4.09791993621942
0.500681686365564 4.1
0.589961759871852 4.4
0.671760610589368 4.7
0.740268727246731 5
0.602583322814291 5
0.529495024471819 4.7
0.5 4.59778741921424
0.451007887873279 4.4
0.374183169179918 4.1
0.286412110418002 3.8
0.2 3.54144431056565
0.187932735948772 3.5
0.0909767474335347 3.2
-0.0207032836296828 2.9
-0.1 2.71164183812745
-0.148573212141849 2.6
-0.293718578941505 2.3
-0.4 2.10179585665403
-0.472293788152735 2
-0.69650109110355 1.7
-0.7 1.69522539761921
-1 1.44233700257652
-1 1.4
-1 1.15938314998198
-0.740141378782518 1.4
};
\addplot [draw=none, fill=teal882156]
table{%
x  y
-0.735058309420949 1.1
-0.7 1.13230886576121
-0.522109152425132 1.4
-0.4 1.57061670579714
-0.329910933072817 1.7
-0.168286203155239 2
-0.1 2.13465377986889
-0.0196477329836999 2.3
0.112948370128177 2.6
0.2 2.82284649152457
0.234467389513829 2.9
0.354888469685945 3.2
0.458793646574459 3.5
0.5 3.63441250520525
0.559915988473361 3.8
0.656051913121065 4.1
0.74019439492917 4.4
0.8 4.64044939779095
0.81376584779496 4.7
0.87680841692896 5
0.8 5
0.740268727246731 5
0.671760610589368 4.7
0.589961759871852 4.4
0.500681686365564 4.1
0.5 4.09791993621942
0.417575962384454 3.8
0.322183695776578 3.5
0.212060055153895 3.2
0.2 3.1703635372307
0.103967139622306 2.9
-0.0182577713764362 2.6
-0.1 2.42100461315329
-0.157408887798162 2.3
-0.313148042980968 2
-0.4 1.84301533946911
-0.504739834315994 1.7
-0.7 1.43354846338111
-0.740141378782518 1.4
-1 1.15938314998198
-1 1.1
-1 0.801222372208951
-0.735058309420949 1.1
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 -1
-0.626499312919086 -1
-0.7 -0.824555413895271
-0.769747595534814 -0.7
-0.885649303759669 -0.4
-0.931451477072777 -0.1
-0.911133324584917 0.2
-0.817018909455515 0.5
-0.7 0.697447941452113
-0.663755600125929 0.8
-0.505576319090628 1.1
-0.4 1.26424989954538
-0.333801787654514 1.4
-0.17546198039779 1.7
-0.1 1.84409805942968
-0.0219911238794309 2
0.119169518999681 2.3
0.2 2.49012026355942
0.253327461216008 2.6
0.384517310240055 2.9
0.497716884217994 3.2
0.5 3.20671310685083
0.617326434994538 3.5
0.721156074165182 3.8
0.8 4.0607916837466
0.810987818244 4.1
0.886785369611373 4.4
0.953390754380593 4.7
1.01247021856641 5
0.87680841692896 5
0.81376584779496 4.7
0.8 4.64044939779095
0.74019439492917 4.4
0.656051913121065 4.1
0.559915988473361 3.8
0.5 3.63441250520525
0.458793646574459 3.5
0.354888469685945 3.2
0.234467389513829 2.9
0.2 2.82284649152457
0.112948370128177 2.6
-0.0196477329836999 2.3
-0.1 2.13465377986889
-0.168286203155239 2
-0.329910933072817 1.7
-0.4 1.57061670579714
-0.522109152425132 1.4
-0.7 1.13230886576121
-0.735058309420949 1.1
-1 0.801222372208951
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.7 -0.824555413895271
-0.626499312919086 -1
-0.4 -1
-0.130056904132333 -1
-0.305282657827144 -0.7
-0.4 -0.46643921750387
-0.431879627577105 -0.4
-0.527985567147406 -0.1
-0.558596436736948 0.2
-0.525745875271354 0.5
-0.431927188458507 0.8
-0.4 0.863383763397351
-0.309684271313024 1.1
-0.168955944720212 1.4
-0.1 1.53497835415742
-0.0194910684725497 1.7
0.12558204441416 2
0.2 2.16408215151962
0.270295876016042 2.3
0.411791232270228 2.6
0.5 2.81218599732525
0.542627136653626 2.9
0.673041572787812 3.2
0.78532805079673 3.5
0.8 3.54378668788598
0.879526324890694 3.8
0.960450163353344 4.1
1.03096786419389 4.4
1.09301566096623 4.7
1.1 4.73707025903489
1.14182926123576 5
1.1 5
1.01247021856641 5
0.953390754380593 4.7
0.886785369611373 4.4
0.810987818244 4.1
0.8 4.0607916837466
0.721156074165182 3.8
0.617326434994538 3.5
0.5 3.20671310685083
0.497716884217994 3.2
0.384517310240055 2.9
0.253327461216008 2.6
0.2 2.49012026355942
0.119169518999681 2.3
-0.0219911238794309 2
-0.1 1.84409805942968
-0.17546198039779 1.7
-0.333801787654514 1.4
-0.4 1.26424989954538
-0.505576319090628 1.1
-0.663755600125929 0.8
-0.7 0.697447941452113
-0.817018909455515 0.5
-0.911133324584917 0.2
-0.931451477072777 -0.1
-0.885649303759669 -0.4
-0.769747595534814 -0.7
-0.7 -0.824555413895271
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.426895774477043
4.7950134617249 0.2
4.7 0.0953299397500597
4.52286988362783 -0.1
4.4 -0.234347135137896
4.2486891584975 -0.4
4.1 -0.560335904402993
3.97060838543732 -0.7
3.8 -0.879294222639098
3.6850163779104 -1
3.8 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
-0.1 -1
0.186111473320534 -1
-0.0089891479165638 -0.7
-0.1 -0.517405625210117
-0.159362956873369 -0.4
-0.263710878325414 -0.1
-0.311023592864711 0.2
-0.301827573495484 0.5
-0.239069726389733 0.8
-0.134012146867178 1.1
-0.1 1.17491682544684
-0.00225000921010395 1.4
0.137933881451548 1.7
0.2 1.8328990822477
0.289067585849476 2
0.438580472120932 2.3
0.5 2.43545576752768
0.586826146125383 2.6
0.727663608967588 2.9
0.8 3.07531272588885
0.847678004127566 3.2
0.948649173602943 3.5
1.03515046395719 3.8
1.1 4.05880908946123
1.108804138486 4.1
1.16625397519579 4.4
1.216101153236 4.7
1.25972651375857 5
1.14182926123576 5
1.1 4.73707025903489
1.09301566096623 4.7
1.03096786419389 4.4
0.960450163353344 4.1
0.879526324890694 3.8
0.8 3.54378668788598
0.785328050796729 3.5
0.673041572787812 3.2
0.542627136653626 2.9
0.5 2.81218599732525
0.411791232270228 2.6
0.270295876016042 2.3
0.2 2.16408215151962
0.12558204441416 2
-0.0194910684725497 1.7
-0.1 1.53497835415742
-0.168955944720212 1.4
-0.309684271313024 1.1
-0.4 0.863383763397351
-0.431927188458507 0.8
-0.525745875271354 0.5
-0.558596436736948 0.2
-0.527985567147406 -0.1
-0.431879627577105 -0.4
-0.4 -0.46643921750387
-0.305282657827144 -0.7
-0.130056904132333 -1
-0.1 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
3.2 -1
3.5 -1
3.6850163779104 -1
3.8 -0.879294222639098
3.97060838543732 -0.7
4.1 -0.560335904402993
4.2486891584975 -0.4
4.4 -0.234347135137896
4.52286988362783 -0.1
4.7 0.0953299397500597
4.7950134617249 0.2
5 0.426895774477043
5 0.5
5 0.8
5 1.09442908735092
4.7182285967573 0.8
4.7 0.780955875276663
4.43076536394755 0.5
4.4 0.467896418475461
4.14251966204327 0.2
4.1 0.155738394663562
3.85264554641771 -0.1
3.8 -0.154532767439813
3.55950306900957 -0.4
3.5 -0.461026555981702
3.25997742483603 -0.7
3.2 -0.760296687267487
2.94799339998669 -1
3.2 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
0.2 -1
0.480674863529688 -1
0.251707627293815 -0.7
0.2 -0.618820628338011
0.0790549293993027 -0.4
-0.0369928056616922 -0.1
-0.0992526558403742 0.2
-0.1 0.248492106983091
-0.103736809148078 0.5
-0.1 0.520675716115847
-0.0518951100977248 0.8
0.0441634393721431 1.1
0.165793548335491 1.4
0.2 1.47545684245246
0.316639459074454 1.7
0.468740166237941 2
0.5 2.0645168661017
0.63245588285236 2.3
0.782666981511763 2.6
0.8 2.63806283871114
0.910722273704785 2.9
1.01915658533374 3.2
1.1 3.46085639277653
1.11041188590372 3.5
1.18127492868321 3.8
1.2415543086107 4.1
1.29336798469986 4.4
1.33831574394726 4.7
1.37762376628137 5
1.25972651375857 5
1.216101153236 4.7
1.16625397519579 4.4
1.108804138486 4.1
1.1 4.05880908946123
1.03515046395719 3.8
0.948649173602943 3.5
0.847678004127566 3.2
0.8 3.07531272588885
0.727663608967588 2.9
0.586826146125383 2.6
0.5 2.43545576752768
0.438580472120932 2.3
0.289067585849476 2
0.2 1.8328990822477
0.137933881451548 1.7
-0.00225000921010393 1.4
-0.1 1.17491682544684
-0.134012146867178 1.1
-0.239069726389733 0.8
-0.301827573495484 0.5
-0.311023592864711 0.2
-0.263710878325414 -0.1
-0.159362956873369 -0.4
-0.1 -0.517405625210117
-0.0089891479165638 -0.7
0.186111473320534 -1
0.2 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
2.6 -1
2.9 -1
2.94799339998669 -1
3.2 -0.760296687267487
3.25997742483603 -0.7
3.5 -0.461026555981702
3.55950306900957 -0.4
3.8 -0.154532767439813
3.85264554641771 -0.1
4.1 0.155738394663562
4.14251966204327 0.2
4.4 0.467896418475461
4.43076536394755 0.5
4.7 0.780955875276663
4.7182285967573 0.8
5 1.09442908735092
5 1.1
5 1.4
5 1.47561702862979
4.9266859867362 1.4
4.7 1.16675228909616
4.63532186683052 1.1
4.4 0.858022580652404
4.34376228519303 0.8
4.1 0.549813178643565
4.05156134558614 0.5
3.8 0.243002416802163
3.75775795644895 0.2
3.5 -0.0606544463364168
3.46042275251366 -0.1
3.2 -0.358035981476285
3.1557474121798 -0.4
2.9 -0.644106839298839
2.83589694861749 -0.7
2.6 -0.91114017732721
2.4831065124231 -1
2.6 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.5 -1
0.8 -1
0.854161869868211 -1
0.8 -0.968893620710238
0.523493602513966 -0.7
0.5 -0.673511036018172
0.32107081466164 -0.4
0.2 -0.152265629070902
0.178332052465827 -0.1
0.106224960753034 0.2
0.0937170927144302 0.5
0.136862470358069 0.8
0.2 1.01682253069062
0.22828027888714 1.1
0.364455646519051 1.4
0.5 1.67965431977119
0.51151038194038 1.7
0.684677118252525 2
0.8 2.21716436249138
0.841187571011962 2.3
0.977050811687362 2.6
1.09251148538895 2.9
1.1 2.9216904623485
1.18281791649955 3.2
1.25758730201074 3.5
1.32061280935361 3.8
1.37430447873539 4.1
1.4 4.26371553273251
1.4220571831043 4.4
1.46571103984253 4.7
1.50454291157247 5
1.4 5
1.37762376628137 5
1.33831574394726 4.7
1.29336798469986 4.4
1.2415543086107 4.1
1.18127492868321 3.8
1.11041188590372 3.5
1.1 3.46085639277653
1.01915658533374 3.2
0.910722273704785 2.9
0.8 2.63806283871114
0.782666981511763 2.6
0.63245588285236 2.3
0.5 2.0645168661017
0.468740166237941 2
0.316639459074454 1.7
0.2 1.47545684245246
0.165793548335491 1.4
0.0441634393721431 1.1
-0.0518951100977248 0.8
-0.1 0.520675716115847
-0.103736809148078 0.5
-0.1 0.248492106983091
-0.0992526558403742 0.2
-0.0369928056616922 -0.1
0.0790549293993027 -0.4
0.2 -0.618820628338011
0.251707627293815 -0.7
0.480674863529688 -1
0.5 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
2.3 -1
2.4831065124231 -1
2.6 -0.91114017732721
2.83589694861749 -0.7
2.9 -0.644106839298839
3.1557474121798 -0.4
3.2 -0.358035981476285
3.46042275251366 -0.1
3.5 -0.0606544463364168
3.75775795644895 0.2
3.8 0.243002416802163
4.05156134558614 0.5
4.1 0.549813178643565
4.34376228519303 0.8
4.4 0.858022580652404
4.63532186683052 1.1
4.7 1.16675228909616
4.9266859867362 1.4
5 1.47561702862979
5 1.7
5 1.79922447523375
4.90399122857764 1.7
4.7 1.49004414391141
4.61312118057744 1.4
4.4 1.18054313671189
4.32249647359374 1.1
4.1 0.87099635501488
4.031708886264 0.8
3.8 0.562280540895242
3.73970865091196 0.5
3.5 0.256385023662788
3.4442711830774 0.2
3.2 -0.0429898244400704
3.14097727371862 -0.1
2.9 -0.329910296175334
2.82079461146782 -0.4
2.6 -0.595793736146751
2.46332889514465 -0.7
2.3 -0.828514172098357
2.01551280578107 -1
2.3 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
0.8 -0.968893620710238
0.854161869868211 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.01551280578107 -1
2.3 -0.828514172098357
2.46332889514465 -0.7
2.6 -0.595793736146751
2.82079461146782 -0.4
2.9 -0.329910296175334
3.14097727371862 -0.1
3.2 -0.0429898244400704
3.4442711830774 0.2
3.5 0.256385023662788
3.73970865091196 0.5
3.8 0.562280540895242
4.031708886264 0.8
4.1 0.87099635501488
4.32249647359374 1.1
4.4 1.18054313671189
4.61312118057744 1.4
4.7 1.49004414391141
4.90399122857764 1.7
5 1.79922447523375
5 2
5 2.11096685928938
4.89336771761192 2
4.7 1.80002975939396
4.60447635156941 1.7
4.4 1.48797218605786
4.31658733007334 1.4
4.1 1.17487152339411
4.0293942754882 1.1
3.8 0.861562699253724
3.74185525500041 0.8
3.5 0.550298258738172
3.45167653146071 0.5
3.2 0.245445259517233
3.15434461615604 0.2
2.9 -0.0460195547355659
2.84070881419173 -0.1
2.6 -0.314373017095695
2.48975331456501 -0.4
2.3 -0.547080167672456
2.04376441051217 -0.7
2 -0.727172792781982
1.7 -0.842412276326301
1.4 -0.875439224877849
1.1 -0.81133140477354
0.909650401169936 -0.7
0.8 -0.624611641282002
0.6005334086893 -0.4
0.5 -0.25267833604883
0.423874920335993 -0.1
0.333805109589373 0.2
0.311407291604276 0.5
0.354772239403486 0.8
0.448673996512769 1.1
0.5 1.22119763433289
0.589588445533397 1.4
0.752529638116467 1.7
0.8 1.78674669333951
0.910174519376601 2
1.05052444013745 2.3
1.1 2.41751086646264
1.16712280936495 2.6
1.26142955890722 2.9
1.33950653265098 3.2
1.4 3.47679868523706
1.40504348140025 3.5
1.46369494813881 3.8
1.51443313998046 4.1
1.55894702668284 4.4
1.59838580341143 4.7
1.633575476336 5
1.50454291157247 5
1.46571103984253 4.7
1.4220571831043 4.4
1.4 4.26371553273251
1.37430447873539 4.1
1.32061280935361 3.8
1.25758730201074 3.5
1.18281791649955 3.2
1.1 2.9216904623485
1.09251148538895 2.9
0.977050811687362 2.6
0.841187571011962 2.3
0.8 2.21716436249138
0.684677118252525 2
0.511510381940381 1.7
0.5 1.67965431977119
0.364455646519051 1.4
0.22828027888714 1.1
0.2 1.01682253069062
0.136862470358069 0.8
0.0937170927144302 0.5
0.106224960753034 0.2
0.178332052465827 -0.1
0.2 -0.152265629070902
0.32107081466164 -0.4
0.5 -0.673511036018172
0.523493602513966 -0.7
0.8 -0.968893620710238
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.1 -0.81133140477354
1.4 -0.875439224877849
1.7 -0.842412276326301
2 -0.727172792781982
2.04376441051217 -0.7
2.3 -0.547080167672456
2.48975331456501 -0.4
2.6 -0.314373017095695
2.84070881419173 -0.1
2.9 -0.0460195547355659
3.15434461615604 0.2
3.2 0.245445259517233
3.45167653146071 0.5
3.5 0.550298258738172
3.74185525500041 0.8
3.8 0.861562699253724
4.0293942754882 1.1
4.1 1.17487152339411
4.31658733007334 1.4
4.4 1.48797218605786
4.60447635156941 1.7
4.7 1.80002975939396
4.89336771761192 2
5 2.11096685928938
5 2.3
5 2.44140653196377
4.86588003766196 2.3
4.7 2.12673418988102
4.58115897135297 2
4.4 1.8095556714348
4.29862699519331 1.7
4.1 1.48970150357551
4.01796074749628 1.4
3.8 1.16806027992501
3.7379611354267 1.1
3.5 0.847379465339559
3.45618443024314 0.8
3.2 0.532969886497801
3.16812877343466 0.5
2.9 0.233136987680117
2.86490912354403 0.2
2.6 -0.0408002674528504
2.52594704078789 -0.1
2.3 -0.275132353506875
2.09074509111521 -0.4
2 -0.453955031779027
1.7 -0.554187283918514
1.4 -0.561939072641315
1.1 -0.460351243444775
1.01424334873029 -0.4
0.8 -0.19504495875276
0.734941470559886 -0.1
0.607859719544259 0.2
0.569844478355088 0.5
0.613515228317331 0.8
0.716174910319499 1.1
0.8 1.28192122924354
0.852944975886672 1.4
1.00008984331973 1.7
1.1 1.91225328835798
1.13684759328359 2
1.25332253635193 2.3
1.35000278354841 2.6
1.4 2.78211603790869
1.43189971741865 2.9
1.50206640596442 3.2
1.56089492071617 3.5
1.61173526393034 3.8
1.65633280489051 4.1
1.69583687026137 4.4
1.7 4.43449107888542
1.74869891704145 4.7
1.79943519913956 5
1.7 5
1.633575476336 5
1.59838580341143 4.7
1.55894702668284 4.4
1.51443313998046 4.1
1.46369494813881 3.8
1.40504348140025 3.5
1.4 3.47679868523706
1.33950653265098 3.2
1.26142955890722 2.9
1.16712280936495 2.6
1.1 2.41751086646264
1.05052444013745 2.3
0.910174519376601 2
0.8 1.78674669333951
0.752529638116467 1.7
0.589588445533397 1.4
0.5 1.22119763433289
0.448673996512769 1.1
0.354772239403486 0.8
0.311407291604276 0.5
0.333805109589373 0.2
0.423874920335993 -0.1
0.5 -0.25267833604883
0.6005334086893 -0.4
0.8 -0.624611641282002
0.909650401169936 -0.7
1.1 -0.81133140477354
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.1 -0.460351243444775
1.4 -0.561939072641315
1.7 -0.554187283918513
2 -0.453955031779027
2.09074509111521 -0.4
2.3 -0.275132353506875
2.52594704078789 -0.1
2.6 -0.0408002674528504
2.86490912354403 0.2
2.9 0.233136987680117
3.16812877343466 0.5
3.2 0.532969886497801
3.45618443024314 0.8
3.5 0.847379465339559
3.7379611354267 1.1
3.8 1.16806027992501
4.01796074749628 1.4
4.1 1.48970150357551
4.29862699519331 1.7
4.4 1.8095556714348
4.58115897135297 2
4.7 2.12673418988102
4.86588003766196 2.3
5 2.44140653196377
5 2.6
5 2.82586010005206
4.79056181619954 2.6
4.7 2.50372708892605
4.51464847806178 2.3
4.4 2.17661591793979
4.24271246550135 2
4.1 1.84425888026722
3.97383756758341 1.7
3.8 1.50806319838673
3.70610578544106 1.4
3.5 1.17185647920642
3.43663013589241 1.1
3.2 0.842327700576725
3.16085724557158 0.8
2.9 0.529357661213566
2.87009929817806 0.5
2.6 0.246180950339213
2.54389963437853 0.2
2.3 0.00855804273848933
2.11806001876116 -0.1
2 -0.16755982685301
1.7 -0.249037261447716
1.4 -0.211760821663375
1.20673795019905 -0.1
1.1 0.00592800125382328
0.975227386346859 0.2
0.904269401007911 0.5
0.928290571404999 0.8
1.01264385407269 1.1
1.1 1.32333206876729
1.12740868454039 1.4
1.24821785970298 1.7
1.35913208069621 2
1.4 2.12167830886043
1.45995946517305 2.3
1.54454167231291 2.6
1.61216024207596 2.9
1.66831848941372 3.2
1.7 3.39183310254181
1.72522625957844 3.5
1.79142413333922 3.8
1.85127627865164 4.1
1.90594455823056 4.4
1.95671563832759 4.7
2 4.97213111940465
2.01072158374703 5
2 5
1.79943519913956 5
1.74869891704145 4.7
1.7 4.43449107888542
1.69583687026137 4.4
1.65633280489051 4.1
1.61173526393034 3.8
1.56089492071617 3.5
1.50206640596442 3.2
1.43189971741865 2.9
1.4 2.78211603790869
1.35000278354841 2.6
1.25332253635193 2.3
1.13684759328359 2
1.1 1.91225328835798
1.00008984331973 1.7
0.852944975886672 1.4
0.8 1.28192122924354
0.716174910319499 1.1
0.613515228317331 0.8
0.569844478355088 0.5
0.607859719544259 0.2
0.734941470559886 -0.1
0.8 -0.19504495875276
1.01424334873029 -0.4
1.1 -0.460351243444775
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.4 -0.211760821663375
1.7 -0.249037261447716
2 -0.16755982685301
2.11806001876116 -0.1
2.3 0.00855804273848933
2.54389963437853 0.2
2.6 0.246180950339213
2.87009929817806 0.5
2.9 0.529357661213566
3.16085724557158 0.8
3.2 0.842327700576725
3.43663013589241 1.1
3.5 1.17185647920642
3.70610578544106 1.4
3.8 1.50806319838673
3.97383756758341 1.7
4.1 1.84425888026722
4.24271246550135 2
4.4 2.17661591793979
4.51464847806178 2.3
4.7 2.50372708892605
4.79056181619954 2.6
5 2.82586010005206
5 2.9
5 3.2
5 3.37082539983578
4.85861242130293 3.2
4.7 3.01586615197074
4.60825604021245 2.9
4.4 2.65004667343415
4.36187750152779 2.6
4.11657521101582 2.3
4.1 2.28101971561426
3.8694103595145 2
3.8 1.91900798387346
3.6212776342188 1.7
3.5 1.55759615897124
3.36876632475643 1.4
3.2 1.20515381454443
3.1074248626943 1.1
2.9 0.873039698723924
2.82832428513847 0.8
2.6 0.576481556471614
2.50868503550875 0.5
2.3 0.333800497669126
2.06985248674226 0.2
2 0.16199004258685
1.7 0.118117968478554
1.50445890998905 0.2
1.4 0.291517554279681
1.29751652259458 0.5
1.27348222162803 0.8
1.32166373783713 1.1
1.4 1.38349774447733
1.40483371037944 1.4
1.51040921485388 1.7
1.60491360375799 2
1.68249192558212 2.3
1.7 2.37942132403077
1.75786158368456 2.6
1.82907959667086 2.9
1.89663361758659 3.2
1.95999661303566 3.5
2 3.70512193380177
2.03658118222658 3.8
2.15377039571137 4.1
2.27527596907159 4.4
2.3 4.46188945504113
2.53705505414279 4.7
2.6 4.76760927794761
2.9 4.93778746755134
3.17097159126119 5
2.9 5
2.6 5
2.3 5
2.01072158374703 5
2 4.97213111940465
1.95671563832759 4.7
1.90594455823056 4.4
1.85127627865164 4.1
1.79142413333922 3.8
1.72522625957844 3.5
1.7 3.39183310254181
1.66831848941372 3.2
1.61216024207596 2.9
1.54454167231291 2.6
1.45995946517305 2.3
1.4 2.12167830886043
1.35913208069621 2
1.24821785970298 1.7
1.12740868454039 1.4
1.1 1.32333206876729
1.01264385407269 1.1
0.928290571404999 0.8
0.904269401007911 0.5
0.975227386346859 0.2
1.1 0.00592800125382328
1.20673795019905 -0.1
1.4 -0.211760821663375
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.7 0.118117968478554
2 0.16199004258685
2.06985248674226 0.2
2.3 0.333800497669126
2.50868503550875 0.5
2.6 0.576481556471614
2.82832428513847 0.8
2.9 0.873039698723924
3.1074248626943 1.1
3.2 1.20515381454443
3.36876632475643 1.4
3.5 1.55759615897124
3.6212776342188 1.7
3.8 1.91900798387346
3.8694103595145 2
4.1 2.28101971561426
4.11657521101582 2.3
4.36187750152779 2.6
4.4 2.65004667343415
4.60825604021245 2.9
4.7 3.01586615197074
4.85861242130293 3.2
5 3.37082539983578
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.1 5
3.8 5
3.5 5
3.2 5
3.17097159126119 5
2.9 4.93778746755134
2.6 4.76760927794761
2.53705505414279 4.7
2.3 4.46188945504113
2.27527596907159 4.4
2.15377039571137 4.1
2.03658118222658 3.8
2 3.70512193380177
1.95999661303566 3.5
1.89663361758659 3.2
1.82907959667086 2.9
1.75786158368456 2.6
1.7 2.37942132403077
1.68249192558212 2.3
1.60491360375799 2
1.51040921485388 1.7
1.40483371037944 1.4
1.4 1.38349774447733
1.32166373783713 1.1
1.27348222162803 0.8
1.29751652259458 0.5
1.4 0.291517554279681
1.50445890998905 0.2
1.7 0.118117968478554

1.73935540876649 0.8
1.7 1.0116570767537
1.69461387666087 1.1
1.7 1.1341974756223
1.75241150353498 1.4
1.83114930857613 1.7
1.90482087722052 2
1.96713520787773 2.3
2 2.47093623732075
2.04511226945642 2.6
2.16121459498396 2.9
2.26927572911146 3.2
2.3 3.28379504050042
2.47168244912057 3.5
2.6 3.64394625786988
2.80739156449697 3.8
2.9 3.86573274693935
3.2 4.02498421804217
3.36705601410348 4.1
3.5 4.15533040674902
3.8 4.23635449228786
4.1 4.1483097588653
4.15302569559584 4.1
4.27727821395309 3.8
4.25238203825616 3.5
4.15117838248067 3.2
4.1 3.10446483961365
4.00101865641307 2.9
3.83214378419052 2.6
3.8 2.55296916542618
3.63535181785287 2.3
3.5 2.10227873950019
3.42976681230868 2
3.21313238506604 1.7
3.2 1.68359704334459
2.96493087454872 1.4
2.9 1.32403668326993
2.68785196467163 1.1
2.6 1.01004372433949
2.3462493820132 0.8
2.3 0.763210179115927
2 0.651727075772223
1.73935540876649 0.8
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
2 0.651727075772223
2.3 0.763210179115927
2.3462493820132 0.8
2.6 1.01004372433949
2.68785196467163 1.1
2.9 1.32403668326993
2.96493087454872 1.4
3.2 1.68359704334459
3.21313238506604 1.7
3.42976681230868 2
3.5 2.10227873950019
3.63535181785287 2.3
3.8 2.55296916542618
3.83214378419052 2.6
4.00101865641307 2.9
4.1 3.10446483961365
4.15117838248067 3.2
4.25238203825616 3.5
4.27727821395309 3.8
4.15302569559584 4.1
4.1 4.1483097588653
3.8 4.23635449228786
3.5 4.15533040674902
3.36705601410348 4.1
3.2 4.02498421804217
2.9 3.86573274693935
2.80739156449697 3.8
2.6 3.64394625786988
2.47168244912057 3.5
2.3 3.28379504050042
2.26927572911146 3.2
2.16121459498396 2.9
2.04511226945642 2.6
2 2.47093623732075
1.96713520787773 2.3
1.90482087722052 2
1.83114930857613 1.7
1.75241150353498 1.4
1.7 1.1341974756223
1.69461387666087 1.1
1.7 1.0116570767537
1.73935540876649 0.8
2 0.651727075772223
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.6 2
};
\coordinate (LA_mean_lml_t) at (axis cs:2.5999999999999996,2.0);
\end{axis}



==> fig/tikz/ionosphere/LA_nlpd.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.984077465721504 -0.7
-1 -0.656642501404779
-1 -0.7
-1 -1
-0.842675463503891 -1
-0.984077465721504 -0.7
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.248612659817514
4.85484175658747 -0.4
4.7 -0.565890711622873
4.57556230336927 -0.7
4.4 -0.898244548280145
4.31077856488127 -1
4.4 -1
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.933812830981764 2.6
-0.836639305599365 2.9
-0.710156748355352 3.2
-0.7 3.22301421587641
-0.598276602420841 3.5
-0.45733727478394 3.8
-0.4 3.9102330948533
-0.296156558887705 4.1
-0.1 4.39876882435735
-0.0989693183626628 4.4
0.156958165698123 4.7
0.2 4.74805596226539
0.5 4.99123811788958
0.509943855100262 5
0.5 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.34045768267708
-0.933812830981764 2.6
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.7 -1
-0.4 -1
-0.350777004685354 -1
-0.4 -0.902737135340693
-0.521680658521269 -0.7
-0.648661292732866 -0.4
-0.7 -0.219595678194078
-0.747476284115334 -0.1
-0.818936662493266 0.2
-0.846178648185329 0.5
-0.839385797067413 0.8
-0.803626049056942 1.1
-0.740183567371608 1.4
-0.7 1.54021123656844
-0.664390300004621 1.7
-0.579149462903975 2
-0.466588799569338 2.3
-0.4 2.45066502794538
-0.332814548724353 2.6
-0.174060609066928 2.9
-0.1 3.02369402420448
0.0314396924769751 3.2
0.2 3.40551303035356
0.304059519777284 3.5
0.5 3.67581545010529
0.633593308533212 3.8
0.8 3.95543151067036
0.917554614925884 4.1
1.1 4.31447587188985
1.1611825190826 4.4
1.39152518365767 4.7
1.4 4.71090460602014
1.58568304126048 5
1.4 5
1.1 5
0.8 5
0.509943855100262 5
0.5 4.99123811788958
0.2 4.74805596226539
0.156958165698123 4.7
-0.0989693183626628 4.4
-0.1 4.39876882435735
-0.296156558887705 4.1
-0.4 3.9102330948533
-0.45733727478394 3.8
-0.598276602420841 3.5
-0.7 3.22301421587641
-0.710156748355352 3.2
-0.836639305599365 2.9
-0.933812830981764 2.6
-1 2.34045768267708
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.656642501404779
-0.984077465721504 -0.7
-0.842675463503891 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
3.8 -1
4.1 -1
4.31077856488127 -1
4.4 -0.898244548280145
4.57556230336927 -0.7
4.7 -0.565890711622873
4.85484175658747 -0.4
5 -0.248612659817514
5 -0.1
5 0.2
5 0.5
5 0.509391606379587
4.99062818506038 0.5
4.7 0.208367557111386
4.6916562955904 0.2
4.4 -0.0933363791887899
4.3933578531233 -0.1
4.1 -0.396123769208984
4.09613264356514 -0.4
3.80094089434982 -0.7
3.8 -0.700988278852773
3.51161143624176 -1
3.8 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
-0.4 -0.902737135340693
-0.350777004685354 -1
-0.1 -1
-0.0731929716639243 -1
-0.1 -0.954249108598043
-0.252514764416078 -0.7
-0.383086493271764 -0.4
-0.4 -0.347821568356449
-0.493864407345397 -0.1
-0.557628556235795 0.2
-0.580580380506146 0.5
-0.569402307055913 0.8
-0.52776230115859 1.1
-0.456512577135763 1.4
-0.4 1.57473868439532
-0.360195731578295 1.7
-0.241897215640972 2
-0.1 2.27877954907155
-0.0869213810956298 2.3
0.116121042636436 2.6
0.2 2.70988989526871
0.389693490789137 2.9
0.5 3.00580483079416
0.700355000517879 3.2
0.8 3.29518911692957
0.965786134501774 3.5
1.1 3.65884126694775
1.20036453869502 3.8
1.4 4.06146011608924
1.42538766743995 4.1
1.62630054767896 4.4
1.7 4.50381742738924
1.80944673529777 4.7
1.9959593202508 5
1.7 5
1.58568304126048 5
1.4 4.71090460602014
1.39152518365767 4.7
1.1611825190826 4.4
1.1 4.31447587188985
0.917554614925884 4.1
0.8 3.95543151067036
0.633593308533212 3.8
0.5 3.67581545010529
0.304059519777284 3.5
0.2 3.40551303035356
0.0314396924769751 3.2
-0.1 3.02369402420448
-0.174060609066928 2.9
-0.332814548724353 2.6
-0.4 2.45066502794538
-0.466588799569338 2.3
-0.579149462903975 2
-0.664390300004621 1.7
-0.7 1.54021123656844
-0.740183567371608 1.4
-0.803626049056942 1.1
-0.839385797067413 0.8
-0.846178648185329 0.5
-0.818936662493266 0.2
-0.747476284115334 -0.1
-0.7 -0.219595678194078
-0.648661292732867 -0.4
-0.521680658521269 -0.7
-0.4 -0.902737135340693
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
3.2 -1
3.5 -1
3.51161143624176 -1
3.8 -0.700988278852773
3.80094089434982 -0.7
4.09613264356514 -0.4
4.1 -0.396123769208984
4.3933578531233 -0.1
4.4 -0.0933363791887899
4.6916562955904 0.2
4.7 0.208367557111386
4.99062818506038 0.5
5 0.509391606379587
5 0.8
5 0.860179229786565
4.93994625813735 0.8
4.7 0.55967914263808
4.64046737762829 0.5
4.4 0.259025281485254
4.34107801007421 0.2
4.1 -0.0416519189845057
4.0415407134537 -0.1
3.8 -0.341947793414507
3.74125201617465 -0.4
3.5 -0.640995086585285
3.43900097736257 -0.7
3.2 -0.93737177943557
3.1327801652246 -1
3.2 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
-0.1 -0.954249108598043
-0.0731929716639243 -1
0.152057961700366 -1
-0.0314172698493838 -0.7
-0.1 -0.563102527140904
-0.181379711703076 -0.4
-0.286654099211886 -0.1
-0.347900297285224 0.2
-0.368575776421735 0.5
-0.351535096659348 0.8
-0.299862129756888 1.1
-0.2148133899421 1.4
-0.1 1.68728832946689
-0.0939724871365724 1.7
0.0727585965988975 2
0.2 2.18877999181227
0.295727985699126 2.3
0.5 2.51615020848497
0.579724896027425 2.6
0.8 2.8208489447425
0.862866672550731 2.9
1.1 3.1851036034869
1.11047514082572 3.2
1.32450700330536 3.5
1.4 3.59975938612534
1.53289208625931 3.8
1.7 4.03602372796581
1.7370459442087 4.1
1.91266794727093 4.4
2 4.54019574205203
2.08119925039138 4.7
2.24409777766034 5
2 5
1.9959593202508 5
1.80944673529777 4.7
1.7 4.50381742738924
1.62630054767896 4.4
1.42538766743995 4.1
1.4 4.06146011608924
1.20036453869502 3.8
1.1 3.65884126694775
0.965786134501774 3.5
0.8 3.29518911692957
0.700355000517879 3.2
0.5 3.00580483079416
0.389693490789137 2.9
0.2 2.70988989526871
0.116121042636436 2.6
-0.0869213810956298 2.3
-0.1 2.27877954907155
-0.241897215640972 2
-0.360195731578295 1.7
-0.4 1.57473868439532
-0.456512577135763 1.4
-0.52776230115859 1.1
-0.569402307055913 0.8
-0.580580380506145 0.5
-0.557628556235795 0.2
-0.493864407345397 -0.1
-0.4 -0.347821568356449
-0.383086493271764 -0.4
-0.252514764416078 -0.7
-0.1 -0.954249108598043
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
2.9 -1
3.1327801652246 -1
3.2 -0.93737177943557
3.43900097736257 -0.7
3.5 -0.640995086585284
3.74125201617465 -0.4
3.8 -0.341947793414507
4.0415407134537 -0.1
4.1 -0.0416519189845057
4.34107801007421 0.2
4.4 0.259025281485254
4.64046737762829 0.5
4.7 0.55967914263808
4.93994625813735 0.8
5 0.860179229786565
5 1.1
5 1.12917139881396
4.97094217211506 1.1
4.7 0.828591086217189
4.67155686870777 0.8
4.4 0.527893596273515
4.37225992629762 0.5
4.1 0.227349105355702
4.07272152636806 0.2
3.8 -0.0722985718786533
3.77207436033148 -0.1
3.5 -0.369460893117791
3.46841843869965 -0.4
3.2 -0.661330274471783
3.15797150391821 -0.7
2.9 -0.943735417835994
2.83359742154338 -1
2.9 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.2 -1
0.381620963432472 -1
0.2 -0.746024128538071
0.17111040720426 -0.7
0.0161072264180137 -0.4
-0.0982262075256112 -0.1
-0.1 -0.0922310594728944
-0.163047083739727 0.2
-0.180584587428509 0.5
-0.154799271542983 0.8
-0.1 1.05012023738435
-0.0872621563016148 1.1
0.02675098318111 1.4
0.183722867926384 1.7
0.2 1.72666698698505
0.411272989188918 2
0.5 2.10086556748846
0.677346721903365 2.3
0.8 2.42813349412045
0.93323037188578 2.6
1.1 2.80385074055692
1.166843703312 2.9
1.38617646052815 3.2
1.4 3.21848112621947
1.58803232237596 3.5
1.7 3.65892226877872
1.78345303048317 3.8
1.96625724845309 4.1
2 4.15425745313785
2.12712739736164 4.4
2.29496253666528 4.7
2.3 4.7088696414934
2.44061878889558 5
2.3 5
2.24409777766034 5
2.08119925039138 4.7
2 4.54019574205203
1.91266794727093 4.4
1.7370459442087 4.1
1.7 4.03602372796581
1.53289208625931 3.8
1.4 3.59975938612534
1.32450700330536 3.5
1.11047514082572 3.2
1.1 3.1851036034869
0.862866672550731 2.9
0.8 2.8208489447425
0.579724896027425 2.6
0.5 2.51615020848497
0.295727985699126 2.3
0.2 2.18877999181227
0.0727585965988975 2
-0.0939724871365724 1.7
-0.1 1.68728832946689
-0.2148133899421 1.4
-0.299862129756888 1.1
-0.351535096659348 0.8
-0.368575776421735 0.5
-0.347900297285224 0.2
-0.286654099211886 -0.1
-0.181379711703076 -0.4
-0.1 -0.563102527140904
-0.0314172698493838 -0.7
0.152057961700366 -1
0.2 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
2.6 -1
2.83359742154338 -1
2.9 -0.943735417835993
3.15797150391821 -0.7
3.2 -0.661330274471783
3.46841843869965 -0.4
3.5 -0.369460893117791
3.77207436033148 -0.1
3.8 -0.0722985718786533
4.07272152636806 0.2
4.1 0.227349105355701
4.37225992629762 0.5
4.4 0.527893596273515
4.67155686870777 0.8
4.7 0.828591086217189
4.97094217211506 1.1
5 1.12917139881396
5 1.35648250003652
4.74451604501068 1.1
4.7 1.05540726890931
4.44591442845533 0.8
4.4 0.753992656987136
4.14740528415203 0.5
4.1 0.452526641321469
3.84812553328314 0.2
3.8 0.151949102960754
3.54601165567103 -0.1
3.5 -0.145569681082181
3.23688468544405 -0.4
3.2 -0.435910666262702
2.91297242541526 -0.7
2.9 -0.712256545707225
2.6 -0.970268747032543
2.55885723244644 -1
2.6 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
0.2 -0.746024128538071
0.381620963432472 -1
0.5 -1
0.652181704282138 -1
0.5 -0.843652328977002
0.397130740153801 -0.7
0.213268299294523 -0.4
0.2 -0.371440121596556
0.0974010585649551 -0.1
0.0323651699005199 0.2
0.0187181476178897 0.5
0.0562340950049464 0.8
0.142051033481551 1.1
0.2 1.23626191096314
0.288278825117619 1.4
0.495576291495498 1.7
0.5 1.70554852989767
0.739292942480849 2
0.8 2.0673291942542
0.97251569332565 2.3
1.1 2.46039892322947
1.19502585423197 2.6
1.4 2.88484425233494
1.41018618846175 2.9
1.61215862486945 3.2
1.7 3.32571746137699
1.80545646040451 3.5
1.99015696629834 3.8
2 3.81586583102626
2.15039321188275 4.1
2.3 4.3702681891685
2.31478626334415 4.4
2.46215893364476 4.7
2.6 4.96119979944558
2.61914564818091 5
2.6 5
2.44061878889558 5
2.3 4.7088696414934
2.29496253666528 4.7
2.12712739736164 4.4
2 4.15425745313785
1.96625724845309 4.1
1.78345303048317 3.8
1.7 3.65892226877872
1.58803232237596 3.5
1.4 3.21848112621947
1.38617646052815 3.2
1.166843703312 2.9
1.1 2.80385074055692
0.93323037188578 2.6
0.8 2.42813349412045
0.677346721903365 2.3
0.5 2.10086556748846
0.411272989188918 2
0.2 1.72666698698505
0.183722867926384 1.7
0.02675098318111 1.4
-0.0872621563016148 1.1
-0.1 1.05012023738435
-0.154799271542982 0.8
-0.180584587428509 0.5
-0.163047083739727 0.2
-0.1 -0.0922310594728944
-0.0982262075256112 -0.1
0.0161072264180137 -0.4
0.17111040720426 -0.7
0.2 -0.746024128538071
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
2.3 -1
2.55885723244644 -1
2.6 -0.970268747032543
2.9 -0.712256545707225
2.91297242541526 -0.7
3.2 -0.435910666262702
3.23688468544405 -0.4
3.5 -0.145569681082181
3.54601165567103 -0.1
3.8 0.151949102960754
3.84812553328314 0.2
4.1 0.452526641321469
4.14740528415203 0.5
4.4 0.753992656987136
4.44591442845533 0.8
4.7 1.05540726890931
4.74451604501068 1.1
5 1.35648250003652
5 1.4
5 1.56985625545671
4.83138201442704 1.4
4.7 1.2681451898728
4.53361009290656 1.1
4.4 0.965752258038529
4.2364344245572 0.8
4.1 0.662876327902386
3.93923987202545 0.5
3.8 0.360433207180807
3.64032168014839 0.2
3.5 0.0606919489150481
3.33601574686586 -0.1
3.2 -0.232008700248167
3.0191148382574 -0.4
2.9 -0.510672740315544
2.67530148510254 -0.7
2.6 -0.765112174449431
2.3 -0.982576975112515
2.26791107264657 -1
2.3 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
0.5 -0.843652328977002
0.652181704282138 -1
0.8 -1
1.09125023079345 -1
0.8 -0.820714384917647
0.682688031470972 -0.7
0.5 -0.477504188377527
0.453715348770736 -0.4
0.321328994982619 -0.1
0.244137570407051 0.2
0.234717648098492 0.5
0.292194460189775 0.8
0.408315396954102 1.1
0.5 1.2642812170125
0.579343387651308 1.4
0.795063693494037 1.7
0.8 1.70598465662687
1.00168130370805 2
1.1 2.1301374274159
1.21105543152092 2.3
1.4 2.57190813674409
1.4187276996615 2.6
1.62071005905013 2.9
1.7 3.01490203719251
1.81444231767853 3.2
1.99888327311237 3.5
2 3.50180765713463
2.16209117001907 3.8
2.3 4.05269950860764
2.32401493746244 4.1
2.47322744687751 4.4
2.6 4.64743071114978
2.62616841469697 4.7
2.77443015740221 5
2.61914564818091 5
2.6 4.96119979944558
2.46215893364476 4.7
2.31478626334415 4.4
2.3 4.3702681891685
2.15039321188275 4.1
2 3.81586583102626
1.99015696629834 3.8
1.80545646040451 3.5
1.7 3.32571746137699
1.61215862486945 3.2
1.41018618846175 2.9
1.4 2.88484425233494
1.19502585423197 2.6
1.1 2.46039892322947
0.972515693325649 2.3
0.8 2.0673291942542
0.739292942480849 2
0.5 1.70554852989767
0.495576291495498 1.7
0.288278825117619 1.4
0.2 1.23626191096314
0.142051033481551 1.1
0.0562340950049464 0.8
0.0187181476178896 0.5
0.0323651699005199 0.2
0.0974010585649551 -0.1
0.2 -0.371440121596556
0.213268299294523 -0.4
0.397130740153801 -0.7
0.5 -0.843652328977002
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
2 -1
2.26791107264657 -1
2.3 -0.982576975112515
2.6 -0.765112174449431
2.67530148510254 -0.7
2.9 -0.510672740315544
3.0191148382574 -0.4
3.2 -0.232008700248167
3.33601574686586 -0.1
3.5 0.0606919489150481
3.64032168014839 0.2
3.8 0.360433207180807
3.93923987202545 0.5
4.1 0.662876327902386
4.2364344245572 0.8
4.4 0.965752258038529
4.53361009290656 1.1
4.7 1.2681451898728
4.83138201442704 1.4
5 1.56985625545671
5 1.7
5 1.78150561580843
4.91951423914337 1.7
4.7 1.47885042601447
4.62260280622243 1.4
4.4 1.17502513497764
4.32682613393674 1.1
4.1 0.870128833043896
4.03185670128455 0.8
3.8 0.565101224568563
3.73643536988802 0.5
3.5 0.262459960759686
3.43761024196691 0.2
3.2 -0.0329379475676969
3.12930020274008 -0.1
2.9 -0.313438833364405
2.79874502770904 -0.4
2.6 -0.568626451134216
2.41604990092365 -0.7
2.3 -0.7850605615674
2 -0.946094570734656
1.82449359225173 -1
2 -1
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
0.8 -0.820714384917647
1.09125023079345 -1
1.1 -1
1.4 -1
1.7 -1
1.82449359225173 -1
2 -0.946094570734656
2.3 -0.7850605615674
2.41604990092365 -0.7
2.6 -0.568626451134216
2.79874502770904 -0.4
2.9 -0.313438833364405
3.12930020274008 -0.1
3.2 -0.0329379475676969
3.43761024196691 0.2
3.5 0.262459960759686
3.73643536988802 0.5
3.8 0.565101224568563
4.03185670128455 0.8
4.1 0.870128833043896
4.32682613393674 1.1
4.4 1.17502513497764
4.62260280622243 1.4
4.7 1.47885042601447
4.91951423914337 1.7
5 1.78150561580843
5 1.99572040567386
4.70797985371417 1.7
4.7 1.69196069805657
4.41342020753607 1.4
4.4 1.38643678653367
4.12063113169136 1.1
4.1 1.07909190517333
3.82880993112509 0.8
3.8 0.770812068385105
3.53557995151643 0.5
3.5 0.464253812433464
3.23604319925081 0.2
3.2 0.164665543085355
2.92097781742202 -0.1
2.9 -0.119526720096983
2.6 -0.375003337897337
2.5652128190428 -0.4
2.3 -0.587128180705482
2.07887555224964 -0.7
2 -0.741542163881027
1.7 -0.815138607499403
1.4 -0.797035639341261
1.14146871952961 -0.7
1.1 -0.678138197966008
0.8 -0.422603892293716
0.781663058945688 -0.4
0.606292831404546 -0.1
0.514048273030343 0.2
0.508266527042215 0.5
0.575044052988075 0.8
0.698886143189104 1.1
0.8 1.27480912864027
0.860526565643633 1.4
1.04013641826296 1.7
1.1 1.78651792926789
1.22928423794441 2
1.4 2.26003770785538
1.42589397663039 2.3
1.6253659798664 2.6
1.7 2.71005489686499
1.81973595880995 2.9
2 3.19489263992569
2.00292535789498 3.2
2.17069150232268 3.5
2.3 3.73964143227784
2.33138745305083 3.8
2.48234987796425 4.1
2.6 4.33640739191742
2.63213125167171 4.4
2.78010496715362 4.7
2.9 4.94083084110241
2.93010803491904 5
2.9 5
2.77443015740221 5
2.62616841469697 4.7
2.6 4.64743071114978
2.47322744687751 4.4
2.32401493746244 4.1
2.3 4.05269950860764
2.16209117001907 3.8
2 3.50180765713463
1.99888327311237 3.5
1.81444231767853 3.2
1.7 3.01490203719251
1.62071005905013 2.9
1.4187276996615 2.6
1.4 2.57190813674409
1.21105543152092 2.3
1.1 2.1301374274159
1.00168130370805 2
0.8 1.70598465662687
0.795063693494037 1.7
0.579343387651308 1.4
0.5 1.2642812170125
0.408315396954102 1.1
0.292194460189775 0.8
0.234717648098492 0.5
0.244137570407051 0.2
0.321328994982619 -0.1
0.453715348770736 -0.4
0.5 -0.477504188377527
0.682688031470972 -0.7
0.8 -0.820714384917647
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.4 -0.797035639341261
1.7 -0.815138607499404
2 -0.741542163881027
2.07887555224964 -0.7
2.3 -0.587128180705482
2.5652128190428 -0.4
2.6 -0.375003337897337
2.9 -0.119526720096983
2.92097781742202 -0.1
3.2 0.164665543085355
3.23604319925081 0.2
3.5 0.464253812433464
3.53557995151643 0.5
3.8 0.770812068385104
3.82880993112509 0.8
4.1 1.07909190517333
4.12063113169136 1.1
4.4 1.38643678653367
4.41342020753607 1.4
4.7 1.69196069805657
4.70797985371417 1.7
5 1.99572040567386
5 2
5 2.23181833530156
4.77291505319258 2
4.7 1.92607165760233
4.48075010416483 1.7
4.4 1.6175956690209
4.19129413862253 1.4
4.1 1.30620259923539
3.90384900132663 1.1
3.8 0.992895885498266
3.61622707764298 0.8
3.5 0.680772370866209
3.32408334705793 0.5
3.2 0.375768555896362
3.01943975408796 0.2
2.9 0.0870282517116709
2.68612075970986 -0.1
2.6 -0.17310871337369
2.3 -0.387522132740081
2.27417880585455 -0.4
2 -0.528307352412701
1.7 -0.578621203387148
1.4 -0.507808636667542
1.22820619537417 -0.4
1.1 -0.268594837804478
0.970517661145236 -0.1
0.856211155039364 0.2
0.832375784135709 0.5
0.874662499094641 0.8
0.969853678348691 1.1
1.1 1.38145844090228
1.10759195253807 1.4
1.26512821593694 1.7
1.4 1.92619836700787
1.44474589925979 2
1.63681488972512 2.3
1.7 2.395771198956
1.83034725136391 2.6
2 2.87933478271112
2.01198338161434 2.9
2.18290242424289 3.2
2.3 3.41749318013545
2.34422081725975 3.5
2.49684192340736 3.8
2.6 4.01244550669262
2.64516347895747 4.1
2.79288697357147 4.4
2.9 4.62524419277767
2.93877209614131 4.7
3.08744822941827 5
2.93010803491904 5
2.9 4.94083084110241
2.78010496715362 4.7
2.63213125167171 4.4
2.6 4.33640739191742
2.48234987796425 4.1
2.33138745305083 3.8
2.3 3.73964143227784
2.17069150232268 3.5
2.00292535789498 3.2
2 3.19489263992569
1.81973595880995 2.9
1.7 2.71005489686499
1.6253659798664 2.6
1.42589397663039 2.3
1.4 2.26003770785538
1.22928423794441 2
1.1 1.78651792926789
1.04013641826296 1.7
0.860526565643632 1.4
0.8 1.27480912864027
0.698886143189103 1.1
0.575044052988075 0.8
0.508266527042215 0.5
0.514048273030343 0.2
0.606292831404546 -0.1
0.781663058945688 -0.4
0.8 -0.422603892293716
1.1 -0.678138197966008
1.14146871952961 -0.7
1.4 -0.797035639341261
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.4 -0.507808636667542
1.7 -0.578621203387148
2 -0.528307352412701
2.27417880585455 -0.4
2.3 -0.387522132740081
2.6 -0.17310871337369
2.68612075970985 -0.1
2.9 0.0870282517116709
3.01943975408796 0.2
3.2 0.375768555896362
3.32408334705793 0.5
3.5 0.680772370866209
3.61622707764298 0.8
3.8 0.992895885498266
3.90384900132663 1.1
4.1 1.30620259923539
4.19129413862253 1.4
4.4 1.6175956690209
4.48075010416483 1.7
4.7 1.92607165760233
4.77291505319258 2
5 2.23181833530156
5 2.3
5 2.50003082073566
4.8066437002053 2.3
4.7 2.19074079720283
4.51853061786387 2
4.4 1.87716160873874
4.23431236437492 1.7
4.1 1.5590613006372
3.95313248062565 1.4
3.8 1.23784993040455
3.67271862083165 1.1
3.5 0.917482046257561
3.38901656026121 0.8
3.2 0.60503836754711
3.09487720829333 0.5
2.9 0.310993756778633
2.77574247536566 0.2
2.6 0.0490455377221992
2.39428465983452 -0.1
2.3 -0.165043773905077
2 -0.296987390446643
1.7 -0.31819508024419
1.4 -0.163983070553052
1.33719787879389 -0.1
1.17708923966084 0.2
1.12489052259581 0.5
1.14431648350285 0.8
1.2188296444388 1.1
1.33589005577068 1.4
1.4 1.52681759578049
1.49200516162626 1.7
1.66719591566241 2
1.7 2.05217619301718
1.85667172841281 2.3
2 2.53752224224769
2.03668281238676 2.6
2.20680100450509 2.9
2.3 3.07337906584297
2.37000433293188 3.2
2.52338526057619 3.5
2.6 3.65953297906184
2.6738657656885 3.8
2.82092822421618 4.1
2.9 4.27224109058894
2.96718935858004 4.4
3.11410042695146 4.7
3.2 4.88975154516125
3.25842920285461 5
3.2 5
3.08744822941827 5
2.93877209614131 4.7
2.9 4.62524419277767
2.79288697357147 4.4
2.64516347895747 4.1
2.6 4.01244550669262
2.49684192340736 3.8
2.34422081725975 3.5
2.3 3.41749318013545
2.18290242424289 3.2
2.01198338161434 2.9
2 2.87933478271112
1.83034725136391 2.6
1.7 2.395771198956
1.63681488972512 2.3
1.44474589925979 2
1.4 1.92619836700787
1.26512821593694 1.7
1.10759195253807 1.4
1.1 1.38145844090228
0.969853678348691 1.1
0.874662499094641 0.8
0.832375784135709 0.5
0.856211155039364 0.2
0.970517661145236 -0.1
1.1 -0.268594837804478
1.22820619537417 -0.4
1.4 -0.507808636667542
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.4 -0.163983070553052
1.7 -0.31819508024419
2 -0.296987390446643
2.3 -0.165043773905077
2.39428465983452 -0.1
2.6 0.0490455377221992
2.77574247536566 0.2
2.9 0.310993756778633
3.09487720829333 0.5
3.2 0.60503836754711
3.38901656026121 0.8
3.5 0.917482046257561
3.67271862083165 1.1
3.8 1.23784993040455
3.95313248062565 1.4
4.1 1.5590613006372
4.23431236437492 1.7
4.4 1.87716160873874
4.51853061786387 2
4.7 2.19074079720283
4.8066437002053 2.3
5 2.50003082073566
5 2.6
5 2.83308974322457
4.78012687092552 2.6
4.7 2.51636749020805
4.50092556259009 2.3
4.4 2.19261408099824
4.2271130710689 2
4.1 1.86198581507066
3.95694070702316 1.7
3.8 1.52705721572238
3.68753260153407 1.4
3.5 1.1933935251799
3.41479921584319 1.1
3.2 0.869760492059111
3.13185492329307 0.8
2.9 0.568374008908132
2.82431964378239 0.5
2.6 0.30488100888781
2.45404066575272 0.2
2.3 0.0963521019549079
2 -0.0229081206621052
1.7 0.0136015384710033
1.51232984552625 0.2
1.4 0.487620642584583
1.39689387263961 0.5
1.3977203977788 0.8
1.4 0.810624997982781
1.47036474186985 1.1
1.58822161432426 1.4
1.7 1.62873691918346
1.73850656578969 1.7
1.91418417308967 2
2 2.1462235914891
2.09014226363358 2.3
2.2543205142431 2.6
2.3 2.6860787452218
2.4199477823298 2.9
2.5703745069639 3.2
2.6 3.26158596412631
2.72787539584628 3.5
2.87004760545585 3.8
2.9 3.86517181752535
3.0268642634255 4.1
3.16854154171766 4.4
3.2 4.47034483427768
3.32367967819349 4.7
3.46368898512586 5
3.25842920285461 5
3.2 4.88975154516125
3.11410042695146 4.7
2.96718935858004 4.4
2.9 4.27224109058894
2.82092822421618 4.1
2.6738657656885 3.8
2.6 3.65953297906184
2.52338526057619 3.5
2.37000433293188 3.2
2.3 3.07337906584297
2.20680100450509 2.9
2.03668281238676 2.6
2 2.53752224224769
1.85667172841281 2.3
1.7 2.05217619301718
1.66719591566241 2
1.49200516162626 1.7
1.4 1.52681759578049
1.33589005577068 1.4
1.2188296444388 1.1
1.14431648350285 0.8
1.12489052259581 0.5
1.17708923966084 0.2
1.33719787879389 -0.1
1.4 -0.163983070553052
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
1.7 0.0136015384710033
2 -0.0229081206621052
2.3 0.096352101954908
2.45404066575272 0.2
2.6 0.30488100888781
2.82431964378239 0.5
2.9 0.568374008908132
3.13185492329307 0.8
3.2 0.869760492059111
3.41479921584319 1.1
3.5 1.1933935251799
3.68753260153407 1.4
3.8 1.52705721572238
3.95694070702316 1.7
4.1 1.86198581507066
4.2271130710689 2
4.4 2.19261408099824
4.50092556259009 2.3
4.7 2.51636749020805
4.78012687092552 2.6
5 2.83308974322457
5 2.9
5 3.2
5 3.37428031563749
4.85747524190292 3.2
4.7 3.01662098909934
4.60948527657441 2.9
4.4 2.64404728617685
4.36696099499039 2.6
4.12344343158229 2.3
4.1 2.27302981837257
3.87435935931576 2
3.8 1.91273269341048
3.62219927136181 1.7
3.5 1.5568796111065
3.36278753257251 1.4
3.2 1.2163046084776
3.08870113601218 1.1
2.9 0.905264701287266
2.78230715788127 0.8
2.6 0.64136227103316
2.39145848047982 0.5
2.3 0.442112656590829
2 0.382876275680384
1.82383980966362 0.5
1.72685450936771 0.8
1.78493548008428 1.1
1.89668456814258 1.4
2 1.62722247061001
2.03694441616355 1.7
2.19854354783379 2
2.3 2.20180882182675
2.35535900919094 2.3
2.51425549501245 2.6
2.6 2.77790091591877
2.67038780736823 2.9
2.82513445182968 3.2
2.9 3.36573595799036
2.97853928751328 3.5
3.13097408891898 3.8
3.2 3.95119305989405
3.28780608274691 4.1
3.4373038531676 4.4
3.5 4.53489689785157
3.60053410546258 4.7
3.74721251492769 5
3.5 5
3.46368898512586 5
3.32367967819349 4.7
3.2 4.47034483427768
3.16854154171766 4.4
3.0268642634255 4.1
2.9 3.86517181752535
2.87004760545585 3.8
2.72787539584628 3.5
2.6 3.26158596412631
2.5703745069639 3.2
2.4199477823298 2.9
2.3 2.6860787452218
2.2543205142431 2.6
2.09014226363358 2.3
2 2.1462235914891
1.91418417308967 2
1.73850656578969 1.7
1.7 1.62873691918346
1.58822161432426 1.4
1.47036474186985 1.1
1.4 0.810624997982781
1.3977203977788 0.8
1.39689387263961 0.5
1.4 0.487620642584583
1.51232984552625 0.2
1.7 0.0136015384710033
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
2 0.382876275680384
2.3 0.442112656590829
2.39145848047982 0.5
2.6 0.64136227103316
2.78230715788127 0.8
2.9 0.905264701287266
3.08870113601218 1.1
3.2 1.2163046084776
3.36278753257251 1.4
3.5 1.5568796111065
3.62219927136181 1.7
3.8 1.91273269341049
3.87435935931576 2
4.1 2.27302981837257
4.12344343158229 2.3
4.36696099499039 2.6
4.4 2.64404728617685
4.60948527657441 2.9
4.7 3.01662098909934
4.85747524190292 3.2
5 3.37428031563749
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.1 5
3.8 5
3.74721251492769 5
3.60053410546258 4.7
3.5 4.53489689785157
3.43730385316761 4.4
3.28780608274691 4.1
3.2 3.95119305989405
3.13097408891898 3.8
2.97853928751328 3.5
2.9 3.36573595799036
2.82513445182968 3.2
2.67038780736823 2.9
2.6 2.77790091591877
2.51425549501245 2.6
2.35535900919094 2.3
2.3 2.20180882182675
2.19854354783379 2
2.03694441616355 1.7
2 1.62722247061001
1.89668456814258 1.4
1.78493548008428 1.1
1.72685450936771 0.8
1.82383980966363 0.5
2 0.382876275680384

2.49478070400118 1.4
2.52064703996763 1.7
2.6 1.98045562815734
2.60953782826967 2
2.78078599047628 2.3
2.8967061464742 2.6
2.9 2.60759989915647
3.09647588601585 2.9
3.2 3.13676438019662
3.26496872515982 3.2
3.46609239182623 3.5
3.5 3.57175141698763
3.8 3.66219564206396
3.8421556185035 3.5
3.86751448890131 3.2
3.82740368567913 2.9
3.8 2.83217190340143
3.69979653183857 2.6
3.54144807679694 2.3
3.5 2.2370304649307
3.32390856989033 2
3.2 1.82973703595812
3.07693506459563 1.7
2.9 1.50361141742085
2.73696884106438 1.4
2.6 1.30667919989855
2.49478070400118 1.4
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
2.6 1.30667919989855
2.73696884106438 1.4
2.9 1.50361141742085
3.07693506459563 1.7
3.2 1.82973703595812
3.32390856989033 2
3.5 2.2370304649307
3.54144807679694 2.3
3.69979653183857 2.6
3.8 2.83217190340143
3.82740368567913 2.9
3.86751448890131 3.2
3.8421556185035 3.5
3.8 3.66219564206396
3.5 3.57175141698763
3.46609239182623 3.5
3.26496872515982 3.2
3.2 3.13676438019662
3.09647588601585 2.9
2.9 2.60759989915647
2.8967061464742 2.6
2.78078599047628 2.3
2.60953782826967 2
2.6 1.98045562815734
2.52064703996763 1.7
2.49478070400118 1.4
2.6 1.30667919989855
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.6 2
};
\coordinate (MCMC_mean_lml_t) at (axis cs:2.5999999999999996,2.3);
\end{axis}



==> fig/tikz/ionosphere/MCMC_Z_mean_lml.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 -1
-0.628083036480438 -1
-0.7 -0.839491766705347
-0.785137758572593 -0.7
-0.916338537615211 -0.4
-1 -0.104483605449326
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.7 -0.839491766705347
-0.628083036480438 -1
-0.4 -1
-0.132297169985446 -1
-0.309357652311431 -0.7
-0.4 -0.488442999484471
-0.446004515297071 -0.4
-0.570932821607788 -0.1
-0.647874239629687 0.2
-0.692706420635705 0.5
-0.7 0.572713340782343
-0.734641410976332 0.8
-0.764147359107519 1.1
-0.783748620766099 1.4
-0.797329712452957 1.7
-0.793868846686783 2
-0.798587691375314 2.3
-0.799125547173093 2.6
-0.795941388473745 2.9
-0.791926837208806 3.2
-0.787332075319462 3.5
-0.792425202224076 3.8
-0.794587122886033 4.1
-0.790770933369016 4.4
-0.769495150926387 4.7
-0.759023556459586 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.104483605449326
-0.916338537615211 -0.4
-0.785137758572593 -0.7
-0.7 -0.839491766705347
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.435555969381053
4.79515158353724 0.2
4.7 0.0964531441658846
4.5219498415051 -0.1
4.4 -0.235370839952745
4.24744542593169 -0.4
4.1 -0.553876562643017
3.96572883758809 -0.7
3.8 -0.881876882751663
3.68684054653596 -1
3.8 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
-0.1 -1
0.185833182501877 -1
-0.0129442924595993 -0.7
-0.1 -0.534660858806054
-0.171766793765333 -0.4
-0.293861730457134 -0.1
-0.377852380564369 0.2
-0.4 0.314854394283738
-0.442150726711821 0.5
-0.484176412556751 0.8
-0.507175514438292 1.1
-0.521414748971389 1.4
-0.529650627541356 1.7
-0.534230939492277 2
-0.540546545863572 2.3
-0.53612607595211 2.6
-0.531216443855774 2.9
-0.535313281753017 3.2
-0.54198432329154 3.5
-0.535336631772919 3.8
-0.533531274996734 4.1
-0.533493667936806 4.4
-0.520068318471907 4.7
-0.513911115851788 5
-0.7 5
-0.759023556459586 5
-0.769495150926387 4.7
-0.790770933369016 4.4
-0.794587122886033 4.1
-0.792425202224076 3.8
-0.787332075319462 3.5
-0.791926837208806 3.2
-0.795941388473745 2.9
-0.799125547173093 2.6
-0.798587691375314 2.3
-0.793868846686783 2
-0.797329712452957 1.7
-0.783748620766099 1.4
-0.764147359107519 1.1
-0.734641410976332 0.8
-0.7 0.572713340782343
-0.692706420635705 0.5
-0.647874239629687 0.2
-0.570932821607788 -0.1
-0.446004515297071 -0.4
-0.4 -0.488442999484471
-0.309357652311431 -0.7
-0.132297169985446 -1
-0.1 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
3.2 -1
3.5 -1
3.68684054653596 -1
3.8 -0.881876882751663
3.96572883758809 -0.7
4.1 -0.553876562643017
4.24744542593169 -0.4
4.4 -0.235370839952745
4.5219498415051 -0.1
4.7 0.0964531441658846
4.79515158353724 0.2
5 0.435555969381053
5 0.5
5 0.8
5 1.09247036702448
4.71482434756247 0.8
4.7 0.784520958183638
4.43090047447988 0.5
4.4 0.467537481713072
4.1419052826224 0.2
4.1 0.156492798135398
3.85355861896472 -0.1
3.8 -0.155469724515125
3.56226270250559 -0.4
3.5 -0.463886853193504
3.25595926491395 -0.7
3.2 -0.755762865909364
2.94669419786125 -1
3.2 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
0.2 -1
0.477186108458128 -1
0.245296639450667 -0.7
0.2 -0.631523695723888
0.0678251166408557 -0.4
-0.0627200252983941 -0.1
-0.1 0.00734446872388141
-0.165629573086297 0.2
-0.228546882303718 0.5
-0.269642818242884 0.8
-0.292313118903478 1.1
-0.306621326539261 1.4
-0.315283186143941 1.7
-0.317271216669356 2
-0.326080516420742 2.3
-0.323338722334885 2.6
-0.3195291255029 2.9
-0.323988813316381 3.2
-0.332515300228122 3.5
-0.32058468907546 3.8
-0.318305756194783 4.1
-0.315933438865933 4.4
-0.311632191807604 4.7
-0.298758606343128 5
-0.4 5
-0.513911115851788 5
-0.520068318471907 4.7
-0.533493667936806 4.4
-0.533531274996734 4.1
-0.535336631772919 3.8
-0.54198432329154 3.5
-0.535313281753017 3.2
-0.531216443855774 2.9
-0.536126075952111 2.6
-0.540546545863572 2.3
-0.534230939492277 2
-0.529650627541356 1.7
-0.521414748971389 1.4
-0.507175514438292 1.1
-0.484176412556751 0.8
-0.442150726711821 0.5
-0.4 0.314854394283738
-0.377852380564369 0.2
-0.293861730457134 -0.1
-0.171766793765333 -0.4
-0.1 -0.534660858806054
-0.0129442924595993 -0.7
0.185833182501877 -1
0.2 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
2.6 -1
2.9 -1
2.94669419786125 -1
3.2 -0.755762865909364
3.25595926491395 -0.7
3.5 -0.463886853193504
3.56226270250559 -0.4
3.8 -0.155469724515125
3.85355861896472 -0.1
4.1 0.156492798135398
4.1419052826224 0.2
4.4 0.467537481713072
4.43090047447988 0.5
4.7 0.784520958183638
4.71482434756247 0.8
5 1.09247036702448
5 1.1
5 1.4
5 1.47506023440983
4.92828345889908 1.4
4.7 1.1654784021854
4.63595003261734 1.1
4.4 0.85701475167215
4.34473248351165 0.8
4.1 0.550865329307997
4.05030627585474 0.5
3.8 0.240767823813469
3.76010823511598 0.2
3.5 -0.0617081263749525
3.46189328739709 -0.1
3.2 -0.361653133329009
3.15928860919309 -0.4
2.9 -0.643139174647718
2.83439597951242 -0.7
2.6 -0.910270648300375
2.48210360904021 -1
2.6 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.5 -1
0.8 -1
0.846786836074247 -1
0.8 -0.973911149314422
0.518307425327254 -0.7
0.5 -0.679893874365984
0.310734358582563 -0.4
0.2 -0.199704847912966
0.153636449548891 -0.1
0.0465123845816379 0.2
-0.0232773394511494 0.5
-0.0675823414070297 0.8
-0.0945565357943983 1.1
-0.1 1.17680665036013
-0.115130456578019 1.4
-0.126385338736128 1.7
-0.120305138235134 2
-0.134599687483608 2.3
-0.135384372923433 2.6
-0.134734468252884 2.9
-0.133009115263765 3.2
-0.139167789981155 3.5
-0.12741991236581 3.8
-0.131133100521231 4.1
-0.120679666830558 4.4
-0.124402815226487 4.7
-0.102705336678426 5
-0.298758606343128 5
-0.311632191807604 4.7
-0.315933438865933 4.4
-0.318305756194783 4.1
-0.32058468907546 3.8
-0.332515300228122 3.5
-0.323988813316381 3.2
-0.3195291255029 2.9
-0.323338722334885 2.6
-0.326080516420742 2.3
-0.317271216669356 2
-0.315283186143941 1.7
-0.306621326539261 1.4
-0.292313118903478 1.1
-0.269642818242884 0.8
-0.228546882303718 0.5
-0.165629573086297 0.2
-0.1 0.00734446872388141
-0.0627200252983941 -0.1
0.0678251166408558 -0.4
0.2 -0.631523695723888
0.245296639450667 -0.7
0.477186108458128 -1
0.5 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
2.3 -1
2.48210360904021 -1
2.6 -0.910270648300375
2.83439597951242 -0.7
2.9 -0.643139174647718
3.15928860919309 -0.4
3.2 -0.361653133329009
3.46189328739709 -0.1
3.5 -0.0617081263749525
3.76010823511598 0.2
3.8 0.240767823813469
4.05030627585474 0.5
4.1 0.550865329307997
4.34473248351165 0.8
4.4 0.85701475167215
4.63595003261734 1.1
4.7 1.1654784021854
4.92828345889908 1.4
5 1.47506023440983
5 1.7
5 1.80091074609064
4.90450144266554 1.7
4.7 1.48671426349617
4.61491551461527 1.4
4.4 1.18057769161808
4.32213687407443 1.1
4.1 0.87134292815941
4.03238787283315 0.8
3.8 0.562621815903959
3.73903207494647 0.5
3.5 0.256276984146024
3.44487546736161 0.2
3.2 -0.0459379273452271
3.14371573539578 -0.1
2.9 -0.331162318915532
2.8226710715054 -0.4
2.6 -0.596468633601444
2.46172671563609 -0.7
2.3 -0.827122949018584
2.02031671885892 -1
2.3 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
0.8 -0.973911149314422
0.846786836074247 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.02031671885892 -1
2.3 -0.827122949018584
2.46172671563609 -0.7
2.6 -0.596468633601444
2.8226710715054 -0.4
2.9 -0.331162318915532
3.14371573539578 -0.1
3.2 -0.0459379273452271
3.44487546736161 0.2
3.5 0.256276984146024
3.73903207494647 0.5
3.8 0.562621815903959
4.03238787283315 0.8
4.1 0.87134292815941
4.32213687407443 1.1
4.4 1.18057769161808
4.61491551461527 1.4
4.7 1.48671426349617
4.90450144266554 1.7
5 1.80091074609064
5 2
5 2.11528852833246
4.89272534309702 2
4.7 1.79619023895179
4.60833235434149 1.7
4.4 1.48768270684089
4.31607423488311 1.4
4.1 1.17649114824839
4.02781032099185 1.1
3.8 0.859777103407666
3.7439892521333 0.8
3.5 0.549516466042729
3.45210396245757 0.5
3.2 0.242754242144457
3.15738801927862 0.2
2.9 -0.0477214205926212
2.84217838951949 -0.1
2.6 -0.316812858699128
2.49304526542951 -0.4
2.3 -0.547263838746386
2.0420748844928 -0.7
2 -0.726632825270835
1.7 -0.845401059187088
1.4 -0.878508423686653
1.1 -0.81548227942587
0.901813343607192 -0.7
0.8 -0.630507086221147
0.589706150762685 -0.4
0.5 -0.283503385685433
0.396117046223836 -0.1
0.270101183287389 0.2
0.2 0.423053362293101
0.180566211913731 0.5
0.135012092037866 0.8
0.105638744629899 1.1
0.0909762385565749 1.4
0.0775119052046285 1.7
0.0705184954621692 2
0.0697735678784609 2.3
0.0622958811510286 2.6
0.0630507190860281 2.9
0.0677148303066955 3.2
0.0671051327014628 3.5
0.0672702123317382 3.8
0.0738426860172136 4.1
0.0758230959450331 4.4
0.0737046741534509 4.7
0.090600827806713 5
-0.1 5
-0.102705336678426 5
-0.124402815226487 4.7
-0.120679666830558 4.4
-0.131133100521231 4.1
-0.12741991236581 3.8
-0.139167789981155 3.5
-0.133009115263765 3.2
-0.134734468252884 2.9
-0.135384372923433 2.6
-0.134599687483608 2.3
-0.120305138235134 2
-0.126385338736128 1.7
-0.115130456578019 1.4
-0.1 1.17680665036013
-0.0945565357943983 1.1
-0.0675823414070297 0.8
-0.0232773394511494 0.5
0.0465123845816379 0.2
0.153636449548891 -0.1
0.2 -0.199704847912966
0.310734358582563 -0.4
0.5 -0.679893874365984
0.518307425327254 -0.7
0.8 -0.973911149314422
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.1 -0.81548227942587
1.4 -0.878508423686653
1.7 -0.845401059187088
2 -0.726632825270835
2.0420748844928 -0.7
2.3 -0.547263838746386
2.49304526542951 -0.4
2.6 -0.316812858699128
2.84217838951949 -0.1
2.9 -0.0477214205926212
3.15738801927862 0.2
3.2 0.242754242144457
3.45210396245757 0.5
3.5 0.549516466042729
3.7439892521333 0.8
3.8 0.859777103407666
4.02781032099185 1.1
4.1 1.17649114824839
4.31607423488311 1.4
4.4 1.48768270684089
4.60833235434149 1.7
4.7 1.79619023895179
4.89272534309702 2
5 2.11528852833246
5 2.3
5 2.44783211381545
4.8621448020589 2.3
4.7 2.12456112666832
4.58534254191561 2
4.4 1.80476842473268
4.30135210961867 1.7
4.1 1.48873218948655
4.01968212166557 1.4
3.8 1.16631358542057
3.7401108338103 1.1
3.5 0.843118580937249
3.45953688790842 0.8
3.2 0.531249807636862
3.1700256115719 0.5
2.9 0.22905200412994
2.86921296418964 0.2
2.6 -0.0428928694991999
2.52836510438033 -0.1
2.3 -0.277425659490179
2.09633396645935 -0.4
2 -0.456884132452843
1.7 -0.556948235845993
1.4 -0.565819964770676
1.1 -0.469278125979672
0.999713821385611 -0.4
0.8 -0.226768476072142
0.703103158805833 -0.1
0.532146737015545 0.2
0.5 0.282256499161079
0.435467953401978 0.5
0.376591420200521 0.8
0.339597817269598 1.1
0.321876197664118 1.4
0.307793009386699 1.7
0.291425006196929 2
0.300361048581582 2.3
0.282612290614768 2.6
0.286616491138662 2.9
0.290260915382805 3.2
0.296310458543871 3.5
0.28741668711093 3.8
0.304938912035858 4.1
0.295770797725385 4.4
0.295558220783525 4.7
0.306647585747655 5
0.2 5
0.090600827806713 5
0.0737046741534509 4.7
0.0758230959450331 4.4
0.0738426860172136 4.1
0.0672702123317382 3.8
0.0671051327014628 3.5
0.0677148303066955 3.2
0.0630507190860281 2.9
0.0622958811510286 2.6
0.0697735678784608 2.3
0.0705184954621692 2
0.0775119052046285 1.7
0.0909762385565749 1.4
0.105638744629899 1.1
0.135012092037866 0.8
0.180566211913731 0.5
0.2 0.423053362293101
0.270101183287389 0.2
0.396117046223836 -0.1
0.5 -0.283503385685433
0.589706150762685 -0.4
0.8 -0.630507086221147
0.901813343607192 -0.7
1.1 -0.81548227942587
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
4.4 4.90683091956904
4.7 4.86099004925851
5 4.83660711885688
5 5
4.7 5
4.4 5
4.11079656911044 5
4.4 4.90683091956904
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.1 -0.469278125979672
1.4 -0.565819964770676
1.7 -0.556948235845993
2 -0.456884132452843
2.09633396645935 -0.4
2.3 -0.277425659490179
2.52836510438033 -0.1
2.6 -0.0428928694991999
2.86921296418964 0.2
2.9 0.22905200412994
3.1700256115719 0.5
3.2 0.531249807636862
3.45953688790842 0.8
3.5 0.843118580937249
3.7401108338103 1.1
3.8 1.16631358542057
4.01968212166557 1.4
4.1 1.48873218948655
4.30135210961867 1.7
4.4 1.80476842473268
4.58534254191561 2
4.7 2.12456112666832
4.8621448020589 2.3
5 2.44783211381545
5 2.6
5 2.84462181930561
4.78329044867749 2.6
4.7 2.50948845431576
4.51545435002488 2.3
4.4 2.17307922945315
4.24513209239501 2
4.1 1.8446400130659
3.97562687960408 1.7
3.8 1.50408202914529
3.7093005453969 1.4
3.5 1.16560348496872
3.44292641764274 1.1
3.2 0.839893608620309
3.16233965539869 0.8
2.9 0.525429431514895
2.87445218457802 0.5
2.6 0.242166776670078
2.54933127821564 0.2
2.3 0.00427126414605693
2.12493775601356 -0.1
2 -0.172339272790196
1.7 -0.257466374583586
1.4 -0.224027840270749
1.16762739502117 -0.1
1.1 -0.0469962828607122
0.896753931183421 0.2
0.8 0.393806929870573
0.758621736496967 0.5
0.683879758185339 0.8
0.63497149505541 1.1
0.607213497921803 1.4
0.593833523858204 1.7
0.593020079308868 2
0.588285755030223 2.3
0.569565767218626 2.6
0.578737512445986 2.9
0.570844902772524 3.2
0.577614281659197 3.5
0.576453682415611 3.8
0.587440405665896 4.1
0.578073874177438 4.4
0.581677520396131 4.7
0.578926984838491 5
0.5 5
0.306647585747655 5
0.295558220783525 4.7
0.295770797725385 4.4
0.304938912035858 4.1
0.28741668711093 3.8
0.296310458543871 3.5
0.290260915382805 3.2
0.286616491138662 2.9
0.282612290614768 2.6
0.300361048581582 2.3
0.291425006196929 2
0.307793009386699 1.7
0.321876197664118 1.4
0.339597817269598 1.1
0.376591420200521 0.8
0.435467953401978 0.5
0.5 0.282256499161079
0.532146737015545 0.2
0.703103158805833 -0.1
0.8 -0.226768476072142
0.999713821385611 -0.4
1.1 -0.469278125979672
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
4.7 4.63481801377176
5 4.61270697044927
5 4.7
5 4.83660711885688
4.7 4.86099004925851
4.4 4.90683091956904
4.11079656911044 5
4.1 5
3.8 5
3.69295752383939 5
3.8 4.9389433245669
4.1 4.78002576868718
4.4 4.72712909377555
4.5326406942861 4.7
4.7 4.63481801377176
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.4 -0.224027840270749
1.7 -0.257466374583586
2 -0.172339272790196
2.12493775601356 -0.1
2.3 0.00427126414605693
2.54933127821564 0.2
2.6 0.242166776670078
2.87445218457802 0.5
2.9 0.525429431514895
3.16233965539869 0.8
3.2 0.839893608620309
3.44292641764274 1.1
3.5 1.16560348496872
3.7093005453969 1.4
3.8 1.50408202914529
3.97562687960408 1.7
4.1 1.8446400130659
4.24513209239501 2
4.4 2.17307922945315
4.51545435002488 2.3
4.7 2.50948845431576
4.78329044867749 2.6
5 2.84462181930561
5 2.9
5 3.2
5 3.48810774195149
4.82025160928708 3.2
4.7 3.05204077939909
4.59008834736932 2.9
4.4 2.65649453934318
4.35700611238691 2.6
4.11416521062691 2.3
4.1 2.28388396088237
3.87339104397902 2
3.8 1.91272890383829
3.62542052321095 1.7
3.5 1.55304977783749
3.37575264349036 1.4
3.2 1.19452789773935
3.11766759420825 1.1
2.9 0.867762937411036
2.83204423079175 0.8
2.6 0.569181139771532
2.52207504866375 0.5
2.3 0.319188122043924
2.09336351614093 0.2
2 0.148785609885607
1.7 0.0910614843143679
1.4 0.194580065586144
1.39338791388719 0.2
1.16902026032054 0.5
1.1 0.674156702002918
1.05892088625324 0.8
1.00769936191124 1.1
0.978682023074552 1.4
0.953481352250301 1.7
0.94873384676 2
0.946259956175011 2.3
0.948971906997313 2.6
0.949182851973337 2.9
0.942834294455432 3.2
0.936190467270986 3.5
0.941070876209939 3.8
0.938059523526077 4.1
0.942632160980046 4.4
0.952524570176085 4.7
0.947199130059276 5
0.8 5
0.578926984838491 5
0.581677520396131 4.7
0.578073874177438 4.4
0.587440405665896 4.1
0.576453682415611 3.8
0.577614281659197 3.5
0.570844902772524 3.2
0.578737512445986 2.9
0.569565767218626 2.6
0.588285755030223 2.3
0.593020079308868 2
0.593833523858204 1.7
0.607213497921803 1.4
0.63497149505541 1.1
0.683879758185339 0.8
0.758621736496967 0.5
0.8 0.393806929870573
0.896753931183421 0.2
1.1 -0.0469962828607122
1.16762739502117 -0.1
1.4 -0.224027840270749
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
4.4 4.37251042880526
4.7 4.23052088121462
5 4.13342690595152
5 4.4
5 4.61270697044927
4.7 4.63481801377176
4.5326406942861 4.7
4.4 4.72712909377555
4.1 4.78002576868718
3.8 4.9389433245669
3.69295752383939 5
3.5 5
3.23230249178809 5
3.5 4.7031239342004
3.50632281691084 4.7
3.8 4.56054936900192
4.1 4.47853144952654
4.34773153987551 4.4
4.4 4.37251042880526
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.4 0.194580065586144
1.7 0.0910614843143679
2 0.148785609885607
2.09336351614093 0.2
2.3 0.319188122043924
2.52207504866375 0.5
2.6 0.569181139771532
2.83204423079175 0.8
2.9 0.867762937411036
3.11766759420825 1.1
3.2 1.19452789773935
3.37575264349036 1.4
3.5 1.55304977783749
3.62542052321095 1.7
3.8 1.91272890383829
3.87339104397902 2
4.1 2.28388396088237
4.11416521062691 2.3
4.35700611238691 2.6
4.4 2.65649453934318
4.59008834736932 2.9
4.7 3.05204077939909
4.82025160928708 3.2
5 3.48810774195149
5 3.5
5 3.8
5 4.1
5 4.13342690595152
4.7 4.23052088121462
4.4 4.37251042880526
4.34773153987551 4.4
4.1 4.47853144952654
3.8 4.56054936900192
3.50632281691084 4.7
3.5 4.7031239342004
3.23230249178809 5
3.2 5
2.9 5
2.7684776006974 5
2.9 4.75720887535102
2.93385766260408 4.7
3.10200673375586 4.4
3.2 4.27897947699511
3.5 4.16314281585631
3.60906358531919 4.1
3.8 3.98672370526821
4.09133069174093 3.8
4.1 3.77072296226599
4.16738615455446 3.5
4.13945301894238 3.2
4.1 3.11085792357118
4.01137642613525 2.9
3.83728878963627 2.6
3.8 2.54287416158196
3.64850224916085 2.3
3.5 2.0823543126475
3.44425822317755 2
3.22562671485119 1.7
3.2 1.66702872834225
2.9796880037232 1.4
2.9 1.30522396500098
2.71131125293451 1.1
2.6 0.989086777351215
2.38701890138875 0.8
2.3 0.724961667298567
2 0.574637545350544
1.7 0.606433487318516
1.53320514774366 0.8
1.41880325165348 1.1
1.4 1.20662197272315
1.3763472497271 1.4
1.36197589028979 1.7
1.34804056155834 2
1.34422706700631 2.3
1.34576851747578 2.6
1.33289049230596 2.9
1.34660392779546 3.2
1.33957626540385 3.5
1.3417284561438 3.8
1.35517840052126 4.1
1.34537902903759 4.4
1.37860787479585 4.7
1.34722675059007 5
1.1 5
0.947199130059276 5
0.952524570176085 4.7
0.942632160980046 4.4
0.938059523526077 4.1
0.941070876209939 3.8
0.936190467270986 3.5
0.942834294455432 3.2
0.949182851973337 2.9
0.948971906997313 2.6
0.946259956175011 2.3
0.94873384676 2
0.953481352250301 1.7
0.978682023074552 1.4
1.00769936191124 1.1
1.05892088625324 0.8
1.1 0.674156702002918
1.16902026032054 0.5
1.39338791388719 0.2
1.4 0.194580065586144
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.7 0.606433487318516
2 0.574637545350544
2.3 0.724961667298567
2.38701890138875 0.8
2.6 0.989086777351215
2.71131125293451 1.1
2.9 1.30522396500098
2.9796880037232 1.4
3.2 1.66702872834225
3.22562671485119 1.7
3.44425822317755 2
3.5 2.0823543126475
3.64850224916085 2.3
3.8 2.54287416158196
3.83728878963627 2.6
4.01137642613525 2.9
4.1 3.11085792357118
4.13945301894238 3.2
4.16738615455446 3.5
4.1 3.77072296226599
4.09133069174093 3.8
3.8 3.98672370526821
3.60906358531919 4.1
3.5 4.16314281585631
3.2 4.27897947699511
3.10200673375586 4.4
2.93385766260408 4.7
2.9 4.75720887535102
2.7684776006974 5
2.6 5
2.3 5
2 5
1.7 5
1.4 5
1.34722675059007 5
1.37860787479585 4.7
1.34537902903759 4.4
1.35517840052126 4.1
1.3417284561438 3.8
1.33957626540385 3.5
1.34660392779546 3.2
1.33289049230596 2.9
1.34576851747578 2.6
1.34422706700631 2.3
1.34804056155834 2
1.36197589028979 1.7
1.3763472497271 1.4
1.4 1.20662197272315
1.41880325165348 1.1
1.53320514774366 0.8
1.7 0.606433487318516

2.17910753775819 1.7
2.12006172560509 2
2.19569054936812 2.3
2.3 2.56523275124001
2.34641441560179 2.6
2.6 2.74327818248192
2.86870483867345 2.6
2.84943220850641 2.3
2.69533776899785 2
2.6 1.86429065624951
2.39319272704027 1.7
2.3 1.62638865892298
2.17910753775819 1.7
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
2.3 1.62638865892298
2.39319272704027 1.7
2.6 1.86429065624951
2.69533776899785 2
2.84943220850641 2.3
2.86870483867345 2.6
2.6 2.74327818248192
2.34641441560179 2.6
2.3 2.56523275124001
2.19569054936812 2.3
2.12006172560509 2
2.17910753775819 1.7
2.3 1.62638865892298
};
\end{axis}



==> fig/tikz/ionosphere/MCMC_mean_lml.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 -1
-0.628083036480438 -1
-0.7 -0.839491766705347
-0.785137758572593 -0.7
-0.916338537615211 -0.4
-1 -0.104483605449326
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.7 -0.839491766705347
-0.628083036480438 -1
-0.4 -1
-0.132297169985446 -1
-0.309357652311431 -0.7
-0.4 -0.488442999484471
-0.446004515297071 -0.4
-0.570932821607788 -0.1
-0.647874239629687 0.2
-0.692706420635705 0.5
-0.7 0.572713340782343
-0.734641410976332 0.8
-0.764147359107519 1.1
-0.783748620766099 1.4
-0.797329712452957 1.7
-0.793868846686783 2
-0.798587691375314 2.3
-0.799125547173093 2.6
-0.795941388473745 2.9
-0.791926837208806 3.2
-0.787332075319462 3.5
-0.792425202224076 3.8
-0.794587122886033 4.1
-0.790770933369016 4.4
-0.769495150926387 4.7
-0.759023556459586 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.104483605449326
-0.916338537615211 -0.4
-0.785137758572593 -0.7
-0.7 -0.839491766705347
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.435555969381053
4.79515158353724 0.2
4.7 0.0964531441658846
4.5219498415051 -0.1
4.4 -0.235370839952745
4.24744542593169 -0.4
4.1 -0.553876562643017
3.96572883758809 -0.7
3.8 -0.881876882751663
3.68684054653596 -1
3.8 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
-0.1 -1
0.185833182501877 -1
-0.0129442924595993 -0.7
-0.1 -0.534660858806054
-0.171766793765333 -0.4
-0.293861730457134 -0.1
-0.377852380564369 0.2
-0.4 0.314854394283738
-0.442150726711821 0.5
-0.484176412556751 0.8
-0.507175514438292 1.1
-0.521414748971389 1.4
-0.529650627541356 1.7
-0.534230939492277 2
-0.540546545863572 2.3
-0.53612607595211 2.6
-0.531216443855774 2.9
-0.535313281753017 3.2
-0.54198432329154 3.5
-0.535336631772919 3.8
-0.533531274996734 4.1
-0.533493667936806 4.4
-0.520068318471907 4.7
-0.513911115851788 5
-0.7 5
-0.759023556459586 5
-0.769495150926387 4.7
-0.790770933369016 4.4
-0.794587122886033 4.1
-0.792425202224076 3.8
-0.787332075319462 3.5
-0.791926837208806 3.2
-0.795941388473745 2.9
-0.799125547173093 2.6
-0.798587691375314 2.3
-0.793868846686783 2
-0.797329712452957 1.7
-0.783748620766099 1.4
-0.764147359107519 1.1
-0.734641410976332 0.8
-0.7 0.572713340782343
-0.692706420635705 0.5
-0.647874239629687 0.2
-0.570932821607788 -0.1
-0.446004515297071 -0.4
-0.4 -0.488442999484471
-0.309357652311431 -0.7
-0.132297169985446 -1
-0.1 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
3.2 -1
3.5 -1
3.68684054653596 -1
3.8 -0.881876882751663
3.96572883758809 -0.7
4.1 -0.553876562643017
4.24744542593169 -0.4
4.4 -0.235370839952745
4.5219498415051 -0.1
4.7 0.0964531441658846
4.79515158353724 0.2
5 0.435555969381053
5 0.5
5 0.8
5 1.09247036702448
4.71482434756247 0.8
4.7 0.784520958183638
4.43090047447988 0.5
4.4 0.467537481713072
4.1419052826224 0.2
4.1 0.156492798135398
3.85355861896472 -0.1
3.8 -0.155469724515125
3.56226270250559 -0.4
3.5 -0.463886853193504
3.25595926491395 -0.7
3.2 -0.755762865909364
2.94669419786125 -1
3.2 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
0.2 -1
0.477186108458128 -1
0.245296639450667 -0.7
0.2 -0.631523695723888
0.0678251166408557 -0.4
-0.0627200252983941 -0.1
-0.1 0.00734446872388141
-0.165629573086297 0.2
-0.228546882303718 0.5
-0.269642818242884 0.8
-0.292313118903478 1.1
-0.306621326539261 1.4
-0.315283186143941 1.7
-0.317271216669356 2
-0.326080516420742 2.3
-0.323338722334885 2.6
-0.3195291255029 2.9
-0.323988813316381 3.2
-0.332515300228122 3.5
-0.32058468907546 3.8
-0.318305756194783 4.1
-0.315933438865933 4.4
-0.311632191807604 4.7
-0.298758606343128 5
-0.4 5
-0.513911115851788 5
-0.520068318471907 4.7
-0.533493667936806 4.4
-0.533531274996734 4.1
-0.535336631772919 3.8
-0.54198432329154 3.5
-0.535313281753017 3.2
-0.531216443855774 2.9
-0.536126075952111 2.6
-0.540546545863572 2.3
-0.534230939492277 2
-0.529650627541356 1.7
-0.521414748971389 1.4
-0.507175514438292 1.1
-0.484176412556751 0.8
-0.442150726711821 0.5
-0.4 0.314854394283738
-0.377852380564369 0.2
-0.293861730457134 -0.1
-0.171766793765333 -0.4
-0.1 -0.534660858806054
-0.0129442924595993 -0.7
0.185833182501877 -1
0.2 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
2.6 -1
2.9 -1
2.94669419786125 -1
3.2 -0.755762865909364
3.25595926491395 -0.7
3.5 -0.463886853193504
3.56226270250559 -0.4
3.8 -0.155469724515125
3.85355861896472 -0.1
4.1 0.156492798135398
4.1419052826224 0.2
4.4 0.467537481713072
4.43090047447988 0.5
4.7 0.784520958183638
4.71482434756247 0.8
5 1.09247036702448
5 1.1
5 1.4
5 1.47506023440983
4.92828345889908 1.4
4.7 1.1654784021854
4.63595003261734 1.1
4.4 0.85701475167215
4.34473248351165 0.8
4.1 0.550865329307997
4.05030627585474 0.5
3.8 0.240767823813469
3.76010823511598 0.2
3.5 -0.0617081263749525
3.46189328739709 -0.1
3.2 -0.361653133329009
3.15928860919309 -0.4
2.9 -0.643139174647718
2.83439597951242 -0.7
2.6 -0.910270648300375
2.48210360904021 -1
2.6 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.5 -1
0.8 -1
0.846786836074247 -1
0.8 -0.973911149314422
0.518307425327254 -0.7
0.5 -0.679893874365984
0.310734358582563 -0.4
0.2 -0.199704847912966
0.153636449548891 -0.1
0.0465123845816379 0.2
-0.0232773394511494 0.5
-0.0675823414070297 0.8
-0.0945565357943983 1.1
-0.1 1.17680665036013
-0.115130456578019 1.4
-0.126385338736128 1.7
-0.120305138235134 2
-0.134599687483608 2.3
-0.135384372923433 2.6
-0.134734468252884 2.9
-0.133009115263765 3.2
-0.139167789981155 3.5
-0.12741991236581 3.8
-0.131133100521231 4.1
-0.120679666830558 4.4
-0.124402815226487 4.7
-0.102705336678426 5
-0.298758606343128 5
-0.311632191807604 4.7
-0.315933438865933 4.4
-0.318305756194783 4.1
-0.32058468907546 3.8
-0.332515300228122 3.5
-0.323988813316381 3.2
-0.3195291255029 2.9
-0.323338722334885 2.6
-0.326080516420742 2.3
-0.317271216669356 2
-0.315283186143941 1.7
-0.306621326539261 1.4
-0.292313118903478 1.1
-0.269642818242884 0.8
-0.228546882303718 0.5
-0.165629573086297 0.2
-0.1 0.00734446872388141
-0.0627200252983941 -0.1
0.0678251166408558 -0.4
0.2 -0.631523695723888
0.245296639450667 -0.7
0.477186108458128 -1
0.5 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
2.3 -1
2.48210360904021 -1
2.6 -0.910270648300375
2.83439597951242 -0.7
2.9 -0.643139174647718
3.15928860919309 -0.4
3.2 -0.361653133329009
3.46189328739709 -0.1
3.5 -0.0617081263749525
3.76010823511598 0.2
3.8 0.240767823813469
4.05030627585474 0.5
4.1 0.550865329307997
4.34473248351165 0.8
4.4 0.85701475167215
4.63595003261734 1.1
4.7 1.1654784021854
4.92828345889908 1.4
5 1.47506023440983
5 1.7
5 1.80091074609064
4.90450144266554 1.7
4.7 1.48671426349617
4.61491551461527 1.4
4.4 1.18057769161808
4.32213687407443 1.1
4.1 0.87134292815941
4.03238787283315 0.8
3.8 0.562621815903959
3.73903207494647 0.5
3.5 0.256276984146024
3.44487546736161 0.2
3.2 -0.0459379273452271
3.14371573539578 -0.1
2.9 -0.331162318915532
2.8226710715054 -0.4
2.6 -0.596468633601444
2.46172671563609 -0.7
2.3 -0.827122949018584
2.02031671885892 -1
2.3 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
0.8 -0.973911149314422
0.846786836074247 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.02031671885892 -1
2.3 -0.827122949018584
2.46172671563609 -0.7
2.6 -0.596468633601444
2.8226710715054 -0.4
2.9 -0.331162318915532
3.14371573539578 -0.1
3.2 -0.0459379273452271
3.44487546736161 0.2
3.5 0.256276984146024
3.73903207494647 0.5
3.8 0.562621815903959
4.03238787283315 0.8
4.1 0.87134292815941
4.32213687407443 1.1
4.4 1.18057769161808
4.61491551461527 1.4
4.7 1.48671426349617
4.90450144266554 1.7
5 1.80091074609064
5 2
5 2.11528852833246
4.89272534309702 2
4.7 1.79619023895179
4.60833235434149 1.7
4.4 1.48768270684089
4.31607423488311 1.4
4.1 1.17649114824839
4.02781032099185 1.1
3.8 0.859777103407666
3.7439892521333 0.8
3.5 0.549516466042729
3.45210396245757 0.5
3.2 0.242754242144457
3.15738801927862 0.2
2.9 -0.0477214205926212
2.84217838951949 -0.1
2.6 -0.316812858699128
2.49304526542951 -0.4
2.3 -0.547263838746386
2.0420748844928 -0.7
2 -0.726632825270835
1.7 -0.845401059187088
1.4 -0.878508423686653
1.1 -0.81548227942587
0.901813343607192 -0.7
0.8 -0.630507086221147
0.589706150762685 -0.4
0.5 -0.283503385685433
0.396117046223836 -0.1
0.270101183287389 0.2
0.2 0.423053362293101
0.180566211913731 0.5
0.135012092037866 0.8
0.105638744629899 1.1
0.0909762385565749 1.4
0.0775119052046285 1.7
0.0705184954621692 2
0.0697735678784609 2.3
0.0622958811510286 2.6
0.0630507190860281 2.9
0.0677148303066955 3.2
0.0671051327014628 3.5
0.0672702123317382 3.8
0.0738426860172136 4.1
0.0758230959450331 4.4
0.0737046741534509 4.7
0.090600827806713 5
-0.1 5
-0.102705336678426 5
-0.124402815226487 4.7
-0.120679666830558 4.4
-0.131133100521231 4.1
-0.12741991236581 3.8
-0.139167789981155 3.5
-0.133009115263765 3.2
-0.134734468252884 2.9
-0.135384372923433 2.6
-0.134599687483608 2.3
-0.120305138235134 2
-0.126385338736128 1.7
-0.115130456578019 1.4
-0.1 1.17680665036013
-0.0945565357943983 1.1
-0.0675823414070297 0.8
-0.0232773394511494 0.5
0.0465123845816379 0.2
0.153636449548891 -0.1
0.2 -0.199704847912966
0.310734358582563 -0.4
0.5 -0.679893874365984
0.518307425327254 -0.7
0.8 -0.973911149314422
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.1 -0.81548227942587
1.4 -0.878508423686653
1.7 -0.845401059187088
2 -0.726632825270835
2.0420748844928 -0.7
2.3 -0.547263838746386
2.49304526542951 -0.4
2.6 -0.316812858699128
2.84217838951949 -0.1
2.9 -0.0477214205926212
3.15738801927862 0.2
3.2 0.242754242144457
3.45210396245757 0.5
3.5 0.549516466042729
3.7439892521333 0.8
3.8 0.859777103407666
4.02781032099185 1.1
4.1 1.17649114824839
4.31607423488311 1.4
4.4 1.48768270684089
4.60833235434149 1.7
4.7 1.79619023895179
4.89272534309702 2
5 2.11528852833246
5 2.3
5 2.44783211381545
4.8621448020589 2.3
4.7 2.12456112666832
4.58534254191561 2
4.4 1.80476842473268
4.30135210961867 1.7
4.1 1.48873218948655
4.01968212166557 1.4
3.8 1.16631358542057
3.7401108338103 1.1
3.5 0.843118580937249
3.45953688790842 0.8
3.2 0.531249807636862
3.1700256115719 0.5
2.9 0.22905200412994
2.86921296418964 0.2
2.6 -0.0428928694991999
2.52836510438033 -0.1
2.3 -0.277425659490179
2.09633396645935 -0.4
2 -0.456884132452843
1.7 -0.556948235845993
1.4 -0.565819964770676
1.1 -0.469278125979672
0.999713821385611 -0.4
0.8 -0.226768476072142
0.703103158805833 -0.1
0.532146737015545 0.2
0.5 0.282256499161079
0.435467953401978 0.5
0.376591420200521 0.8
0.339597817269598 1.1
0.321876197664118 1.4
0.307793009386699 1.7
0.291425006196929 2
0.300361048581582 2.3
0.282612290614768 2.6
0.286616491138662 2.9
0.290260915382805 3.2
0.296310458543871 3.5
0.28741668711093 3.8
0.304938912035858 4.1
0.295770797725385 4.4
0.295558220783525 4.7
0.306647585747655 5
0.2 5
0.090600827806713 5
0.0737046741534509 4.7
0.0758230959450331 4.4
0.0738426860172136 4.1
0.0672702123317382 3.8
0.0671051327014628 3.5
0.0677148303066955 3.2
0.0630507190860281 2.9
0.0622958811510286 2.6
0.0697735678784608 2.3
0.0705184954621692 2
0.0775119052046285 1.7
0.0909762385565749 1.4
0.105638744629899 1.1
0.135012092037866 0.8
0.180566211913731 0.5
0.2 0.423053362293101
0.270101183287389 0.2
0.396117046223836 -0.1
0.5 -0.283503385685433
0.589706150762685 -0.4
0.8 -0.630507086221147
0.901813343607192 -0.7
1.1 -0.81548227942587
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
4.4 4.90683091956904
4.7 4.86099004925851
5 4.83660711885688
5 5
4.7 5
4.4 5
4.11079656911044 5
4.4 4.90683091956904
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.1 -0.469278125979672
1.4 -0.565819964770676
1.7 -0.556948235845993
2 -0.456884132452843
2.09633396645935 -0.4
2.3 -0.277425659490179
2.52836510438033 -0.1
2.6 -0.0428928694991999
2.86921296418964 0.2
2.9 0.22905200412994
3.1700256115719 0.5
3.2 0.531249807636862
3.45953688790842 0.8
3.5 0.843118580937249
3.7401108338103 1.1
3.8 1.16631358542057
4.01968212166557 1.4
4.1 1.48873218948655
4.30135210961867 1.7
4.4 1.80476842473268
4.58534254191561 2
4.7 2.12456112666832
4.8621448020589 2.3
5 2.44783211381545
5 2.6
5 2.84462181930561
4.78329044867749 2.6
4.7 2.50948845431576
4.51545435002488 2.3
4.4 2.17307922945315
4.24513209239501 2
4.1 1.8446400130659
3.97562687960408 1.7
3.8 1.50408202914529
3.7093005453969 1.4
3.5 1.16560348496872
3.44292641764274 1.1
3.2 0.839893608620309
3.16233965539869 0.8
2.9 0.525429431514895
2.87445218457802 0.5
2.6 0.242166776670078
2.54933127821564 0.2
2.3 0.00427126414605693
2.12493775601356 -0.1
2 -0.172339272790196
1.7 -0.257466374583586
1.4 -0.224027840270749
1.16762739502117 -0.1
1.1 -0.0469962828607122
0.896753931183421 0.2
0.8 0.393806929870573
0.758621736496967 0.5
0.683879758185339 0.8
0.63497149505541 1.1
0.607213497921803 1.4
0.593833523858204 1.7
0.593020079308868 2
0.588285755030223 2.3
0.569565767218626 2.6
0.578737512445986 2.9
0.570844902772524 3.2
0.577614281659197 3.5
0.576453682415611 3.8
0.587440405665896 4.1
0.578073874177438 4.4
0.581677520396131 4.7
0.578926984838491 5
0.5 5
0.306647585747655 5
0.295558220783525 4.7
0.295770797725385 4.4
0.304938912035858 4.1
0.28741668711093 3.8
0.296310458543871 3.5
0.290260915382805 3.2
0.286616491138662 2.9
0.282612290614768 2.6
0.300361048581582 2.3
0.291425006196929 2
0.307793009386699 1.7
0.321876197664118 1.4
0.339597817269598 1.1
0.376591420200521 0.8
0.435467953401978 0.5
0.5 0.282256499161079
0.532146737015545 0.2
0.703103158805833 -0.1
0.8 -0.226768476072142
0.999713821385611 -0.4
1.1 -0.469278125979672
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
4.7 4.63481801377176
5 4.61270697044927
5 4.7
5 4.83660711885688
4.7 4.86099004925851
4.4 4.90683091956904
4.11079656911044 5
4.1 5
3.8 5
3.69295752383939 5
3.8 4.9389433245669
4.1 4.78002576868718
4.4 4.72712909377555
4.5326406942861 4.7
4.7 4.63481801377176
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.4 -0.224027840270749
1.7 -0.257466374583586
2 -0.172339272790196
2.12493775601356 -0.1
2.3 0.00427126414605693
2.54933127821564 0.2
2.6 0.242166776670078
2.87445218457802 0.5
2.9 0.525429431514895
3.16233965539869 0.8
3.2 0.839893608620309
3.44292641764274 1.1
3.5 1.16560348496872
3.7093005453969 1.4
3.8 1.50408202914529
3.97562687960408 1.7
4.1 1.8446400130659
4.24513209239501 2
4.4 2.17307922945315
4.51545435002488 2.3
4.7 2.50948845431576
4.78329044867749 2.6
5 2.84462181930561
5 2.9
5 3.2
5 3.48810774195149
4.82025160928708 3.2
4.7 3.05204077939909
4.59008834736932 2.9
4.4 2.65649453934318
4.35700611238691 2.6
4.11416521062691 2.3
4.1 2.28388396088237
3.87339104397902 2
3.8 1.91272890383829
3.62542052321095 1.7
3.5 1.55304977783749
3.37575264349036 1.4
3.2 1.19452789773935
3.11766759420825 1.1
2.9 0.867762937411036
2.83204423079175 0.8
2.6 0.569181139771532
2.52207504866375 0.5
2.3 0.319188122043924
2.09336351614093 0.2
2 0.148785609885607
1.7 0.0910614843143679
1.4 0.194580065586144
1.39338791388719 0.2
1.16902026032054 0.5
1.1 0.674156702002918
1.05892088625324 0.8
1.00769936191124 1.1
0.978682023074552 1.4
0.953481352250301 1.7
0.94873384676 2
0.946259956175011 2.3
0.948971906997313 2.6
0.949182851973337 2.9
0.942834294455432 3.2
0.936190467270986 3.5
0.941070876209939 3.8
0.938059523526077 4.1
0.942632160980046 4.4
0.952524570176085 4.7
0.947199130059276 5
0.8 5
0.578926984838491 5
0.581677520396131 4.7
0.578073874177438 4.4
0.587440405665896 4.1
0.576453682415611 3.8
0.577614281659197 3.5
0.570844902772524 3.2
0.578737512445986 2.9
0.569565767218626 2.6
0.588285755030223 2.3
0.593020079308868 2
0.593833523858204 1.7
0.607213497921803 1.4
0.63497149505541 1.1
0.683879758185339 0.8
0.758621736496967 0.5
0.8 0.393806929870573
0.896753931183421 0.2
1.1 -0.0469962828607122
1.16762739502117 -0.1
1.4 -0.224027840270749
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
4.4 4.37251042880526
4.7 4.23052088121462
5 4.13342690595152
5 4.4
5 4.61270697044927
4.7 4.63481801377176
4.5326406942861 4.7
4.4 4.72712909377555
4.1 4.78002576868718
3.8 4.9389433245669
3.69295752383939 5
3.5 5
3.23230249178809 5
3.5 4.7031239342004
3.50632281691084 4.7
3.8 4.56054936900192
4.1 4.47853144952654
4.34773153987551 4.4
4.4 4.37251042880526
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.4 0.194580065586144
1.7 0.0910614843143679
2 0.148785609885607
2.09336351614093 0.2
2.3 0.319188122043924
2.52207504866375 0.5
2.6 0.569181139771532
2.83204423079175 0.8
2.9 0.867762937411036
3.11766759420825 1.1
3.2 1.19452789773935
3.37575264349036 1.4
3.5 1.55304977783749
3.62542052321095 1.7
3.8 1.91272890383829
3.87339104397902 2
4.1 2.28388396088237
4.11416521062691 2.3
4.35700611238691 2.6
4.4 2.65649453934318
4.59008834736932 2.9
4.7 3.05204077939909
4.82025160928708 3.2
5 3.48810774195149
5 3.5
5 3.8
5 4.1
5 4.13342690595152
4.7 4.23052088121462
4.4 4.37251042880526
4.34773153987551 4.4
4.1 4.47853144952654
3.8 4.56054936900192
3.50632281691084 4.7
3.5 4.7031239342004
3.23230249178809 5
3.2 5
2.9 5
2.7684776006974 5
2.9 4.75720887535102
2.93385766260408 4.7
3.10200673375586 4.4
3.2 4.27897947699511
3.5 4.16314281585631
3.60906358531919 4.1
3.8 3.98672370526821
4.09133069174093 3.8
4.1 3.77072296226599
4.16738615455446 3.5
4.13945301894238 3.2
4.1 3.11085792357118
4.01137642613525 2.9
3.83728878963627 2.6
3.8 2.54287416158196
3.64850224916085 2.3
3.5 2.0823543126475
3.44425822317755 2
3.22562671485119 1.7
3.2 1.66702872834225
2.9796880037232 1.4
2.9 1.30522396500098
2.71131125293451 1.1
2.6 0.989086777351215
2.38701890138875 0.8
2.3 0.724961667298567
2 0.574637545350544
1.7 0.606433487318516
1.53320514774366 0.8
1.41880325165348 1.1
1.4 1.20662197272315
1.3763472497271 1.4
1.36197589028979 1.7
1.34804056155834 2
1.34422706700631 2.3
1.34576851747578 2.6
1.33289049230596 2.9
1.34660392779546 3.2
1.33957626540385 3.5
1.3417284561438 3.8
1.35517840052126 4.1
1.34537902903759 4.4
1.37860787479585 4.7
1.34722675059007 5
1.1 5
0.947199130059276 5
0.952524570176085 4.7
0.942632160980046 4.4
0.938059523526077 4.1
0.941070876209939 3.8
0.936190467270986 3.5
0.942834294455432 3.2
0.949182851973337 2.9
0.948971906997313 2.6
0.946259956175011 2.3
0.94873384676 2
0.953481352250301 1.7
0.978682023074552 1.4
1.00769936191124 1.1
1.05892088625324 0.8
1.1 0.674156702002918
1.16902026032054 0.5
1.39338791388719 0.2
1.4 0.194580065586144
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.7 0.606433487318516
2 0.574637545350544
2.3 0.724961667298567
2.38701890138875 0.8
2.6 0.989086777351215
2.71131125293451 1.1
2.9 1.30522396500098
2.9796880037232 1.4
3.2 1.66702872834225
3.22562671485119 1.7
3.44425822317755 2
3.5 2.0823543126475
3.64850224916085 2.3
3.8 2.54287416158196
3.83728878963627 2.6
4.01137642613525 2.9
4.1 3.11085792357118
4.13945301894238 3.2
4.16738615455446 3.5
4.1 3.77072296226599
4.09133069174093 3.8
3.8 3.98672370526821
3.60906358531919 4.1
3.5 4.16314281585631
3.2 4.27897947699511
3.10200673375586 4.4
2.93385766260408 4.7
2.9 4.75720887535102
2.7684776006974 5
2.6 5
2.3 5
2 5
1.7 5
1.4 5
1.34722675059007 5
1.37860787479585 4.7
1.34537902903759 4.4
1.35517840052126 4.1
1.3417284561438 3.8
1.33957626540385 3.5
1.34660392779546 3.2
1.33289049230596 2.9
1.34576851747578 2.6
1.34422706700631 2.3
1.34804056155834 2
1.36197589028979 1.7
1.3763472497271 1.4
1.4 1.20662197272315
1.41880325165348 1.1
1.53320514774366 0.8
1.7 0.606433487318516

2.17910753775819 1.7
2.12006172560509 2
2.19569054936812 2.3
2.3 2.56523275124001
2.34641441560179 2.6
2.6 2.74327818248192
2.86870483867345 2.6
2.84943220850641 2.3
2.69533776899785 2
2.6 1.86429065624951
2.39319272704027 1.7
2.3 1.62638865892298
2.17910753775819 1.7
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
2.3 1.62638865892298
2.39319272704027 1.7
2.6 1.86429065624951
2.69533776899785 2
2.84943220850641 2.3
2.86870483867345 2.6
2.6 2.74327818248192
2.34641441560179 2.6
2.3 2.56523275124001
2.19569054936812 2.3
2.12006172560509 2
2.17910753775819 1.7
2.3 1.62638865892298
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.6 2.3
};
\coordinate (MCMC_mean_lml_t) at (axis cs:2.5999999999999996,2.3);
\end{axis}



==> fig/tikz/ionosphere/MCMC_nlpd.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.987631342381908 -0.7
-1 -0.669037888522156
-1 -0.7
-1 -1
-0.846599560839285 -1
-0.987631342381908 -0.7
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.262310923591289
4.87036766054405 -0.4
4.7 -0.57957514013496
4.58125616380785 -0.7
4.4 -0.901749861485052
4.31841895456113 -1
4.4 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.7 -1
-0.4 -1
-0.351561214780702 -1
-0.4 -0.905791077095116
-0.52513300757469 -0.7
-0.659645262945515 -0.4
-0.7 -0.276649708969893
-0.778089726761848 -0.1
-0.870076272769718 0.2
-0.925125931202963 0.5
-0.957981277539397 0.8
-0.976962056864845 1.1
-0.987701744189795 1.4
-0.994021210029531 1.7
-0.997102760039764 2
-0.999381739833486 2.3
-1 2.53612361431302
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.669037888522156
-0.987631342381908 -0.7
-0.846599560839285 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
3.8 -1
4.1 -1
4.31841895456113 -1
4.4 -0.901749861485052
4.58125616380785 -0.7
4.7 -0.57957514013496
4.87036766054405 -0.4
5 -0.262310923591289
5 -0.1
5 0.2
5 0.5
5 0.501394654711274
4.99859764119557 0.5
4.7 0.205740312443439
4.6942802685507 0.2
4.4 -0.0988377278342563
4.39885097038163 -0.1
4.1 -0.398913010160201
4.09890901870467 -0.4
3.80470727833624 -0.7
3.8 -0.704914995413712
3.51641297019941 -1
3.8 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.999918823017921 2.9
-0.999891738010709 3.2
-0.999660750304313 3.5
-1 3.54926143521982
-1 3.5
-1 3.2
-1 2.9
-1 2.80240027301694
-0.999918823017921 2.9
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.999572168416651 5
-1 5
-1 4.93589216170494
-0.999572168416651 5
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
-0.4 -0.905791077095116
-0.351561214780702 -1
-0.1 -1
-0.073023963762896 -1
-0.1 -0.955497392039094
-0.255527046396092 -0.7
-0.394886428668062 -0.4
-0.4 -0.386525454943208
-0.522664643264931 -0.1
-0.608647833376481 0.2
-0.663994884001796 0.5
-0.697612417175645 0.8
-0.7 0.833043881482367
-0.726318642678539 1.1
-0.741662898904655 1.4
-0.750109090656691 1.7
-0.755438210608192 2
-0.760014662249923 2.3
-0.759702028471696 2.6
-0.758990625513164 2.9
-0.762372974412664 3.2
-0.761387783812923 3.5
-0.761160702628202 3.8
-0.761032953528364 4.1
-0.762890492257896 4.4
-0.760885358944909 4.7
-0.764696273727522 5
-0.999572168416651 5
-1 4.93589216170494
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.54926143521982
-0.999660750304313 3.5
-0.999891738010709 3.2
-0.999918823017921 2.9
-1 2.80240027301694
-1 2.6
-1 2.53612361431302
-0.999381739833486 2.3
-0.997102760039764 2
-0.994021210029531 1.7
-0.987701744189795 1.4
-0.976962056864845 1.1
-0.957981277539397 0.8
-0.925125931202962 0.5
-0.870076272769718 0.2
-0.778089726761848 -0.1
-0.7 -0.276649708969893
-0.659645262945515 -0.4
-0.52513300757469 -0.7
-0.4 -0.905791077095116
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
3.2 -1
3.5 -1
3.51641297019941 -1
3.8 -0.704914995413712
3.80470727833624 -0.7
4.09890901870467 -0.4
4.1 -0.398913010160201
4.39885097038163 -0.1
4.4 -0.0988377278342563
4.6942802685507 0.2
4.7 0.205740312443439
4.99859764119557 0.5
5 0.501394654711274
5 0.8
5 0.856634002831547
4.94327505837646 0.8
4.7 0.557704754773376
4.64241816821156 0.5
4.4 0.256936130804654
4.34407251302747 0.2
4.1 -0.0461108198443381
4.04520745310153 -0.1
3.8 -0.344540827301652
3.74437748199919 -0.4
3.5 -0.645281952677741
3.44280359697204 -0.7
3.2 -0.939440779510592
3.13526743002636 -1
3.2 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
-0.1 -0.955497392039094
-0.073023963762896 -1
0.155701098157631 -1
-0.0337139547093719 -0.7
-0.1 -0.577675756459087
-0.194144565327138 -0.4
-0.314761199784428 -0.1
-0.4 0.187920274980392
-0.403936445818905 0.2
-0.472910871515824 0.5
-0.513916256579416 0.8
-0.539130241285211 1.1
-0.552484385825435 1.4
-0.560603924500407 1.7
-0.564886173163135 2
-0.568128977238872 2.3
-0.568326074898116 2.6
-0.568818103566034 2.9
-0.569695285781795 3.2
-0.570481056912603 3.5
-0.569949410418453 3.8
-0.570543789617279 4.1
-0.572009020335824 4.4
-0.569118526476488 4.7
-0.57206339994642 5
-0.7 5
-0.764696273727522 5
-0.760885358944909 4.7
-0.762890492257896 4.4
-0.761032953528364 4.1
-0.761160702628202 3.8
-0.761387783812923 3.5
-0.762372974412664 3.2
-0.758990625513164 2.9
-0.759702028471696 2.6
-0.760014662249923 2.3
-0.755438210608192 2
-0.750109090656691 1.7
-0.741662898904655 1.4
-0.726318642678539 1.1
-0.7 0.833043881482367
-0.697612417175645 0.8
-0.663994884001796 0.5
-0.608647833376481 0.2
-0.522664643264931 -0.1
-0.4 -0.386525454943208
-0.394886428668062 -0.4
-0.255527046396092 -0.7
-0.1 -0.955497392039094
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
2.9 -1
3.13526743002636 -1
3.2 -0.939440779510592
3.44280359697204 -0.7
3.5 -0.645281952677741
3.74437748199919 -0.4
3.8 -0.344540827301652
4.04520745310153 -0.1
4.1 -0.0461108198443381
4.34407251302747 0.2
4.4 0.256936130804654
4.64241816821156 0.5
4.7 0.557704754773376
4.94327505837646 0.8
5 0.856634002831547
5 1.1
5 1.12690661655916
4.97337711356961 1.1
4.7 0.826979035233722
4.67280214803942 0.8
4.4 0.526718763475895
4.37338984423971 0.5
4.1 0.222512090546306
4.0775452620109 0.2
3.8 -0.0737673555336447
3.77373472951212 -0.1
3.5 -0.373080960423171
3.47209751166025 -0.4
3.2 -0.662569984754921
3.15902777686745 -0.7
2.9 -0.945448656018762
2.83546901341327 -1
2.9 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.2 -1
0.387275500110552 -1
0.2 -0.743956033650646
0.171582022818641 -0.7
0.00466424386987806 -0.4
-0.1 -0.167705146817837
-0.128783936892982 -0.1
-0.226363888469943 0.2
-0.291617411537234 0.5
-0.333959114157248 0.8
-0.360696728990026 1.1
-0.375437762066745 1.4
-0.385263181948958 1.7
-0.389660857093527 2
-0.392234175732849 2.3
-0.393236661921815 2.6
-0.395103266124212 2.9
-0.393102068757472 3.2
-0.396001234089912 3.5
-0.395579536019951 3.8
-0.396768444918463 4.1
-0.398196974117945 4.4
-0.394012463325571 4.7
-0.395566412138908 5
-0.4 5
-0.57206339994642 5
-0.569118526476488 4.7
-0.572009020335824 4.4
-0.570543789617279 4.1
-0.569949410418453 3.8
-0.570481056912603 3.5
-0.569695285781795 3.2
-0.568818103566034 2.9
-0.568326074898116 2.6
-0.568128977238872 2.3
-0.564886173163135 2
-0.560603924500407 1.7
-0.552484385825435 1.4
-0.539130241285211 1.1
-0.513916256579416 0.8
-0.472910871515824 0.5
-0.403936445818905 0.2
-0.4 0.187920274980393
-0.314761199784428 -0.1
-0.194144565327138 -0.4
-0.1 -0.577675756459087
-0.0337139547093719 -0.7
0.155701098157631 -1
0.2 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
2.6 -1
2.83546901341327 -1
2.9 -0.945448656018762
3.15902777686745 -0.7
3.2 -0.662569984754921
3.47209751166025 -0.4
3.5 -0.373080960423171
3.77373472951212 -0.1
3.8 -0.0737673555336447
4.0775452620109 0.2
4.1 0.222512090546306
4.37338984423971 0.5
4.4 0.526718763475895
4.67280214803942 0.8
4.7 0.826979035233722
4.97337711356962 1.1
5 1.12690661655916
5 1.35394877362422
4.74872911484549 1.1
4.7 1.05133436821538
4.44662715400651 0.8
4.4 0.753290960521842
4.14773862876401 0.5
4.1 0.451545777668693
3.8490950687944 0.2
3.8 0.151573206272001
3.54811390751279 -0.1
3.5 -0.147998995584964
3.2387924978814 -0.4
3.2 -0.437434173929681
2.91258612794311 -0.7
2.9 -0.711926320124721
2.6 -0.969320736005583
2.55766067333659 -1
2.6 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
0.2 -0.743956033650646
0.387275500110552 -1
0.5 -1
0.663633982963679 -1
0.5 -0.835887656902012
0.400720818897634 -0.7
0.202204822188324 -0.4
0.2 -0.396064836120831
0.0669027079044743 -0.1
-0.0413631922646411 0.2
-0.1 0.426207590811361
-0.116364560364288 0.5
-0.16010594908605 0.8
-0.186751270950059 1.1
-0.201675372933607 1.4
-0.210974108873333 1.7
-0.216185420632461 2
-0.218534305390007 2.3
-0.219951276915138 2.6
-0.221419141590499 2.9
-0.21930711841102 3.2
-0.221030108557116 3.5
-0.22166405406782 3.8
-0.221349854469805 4.1
-0.221297993157454 4.4
-0.221274620922568 4.7
-0.221991083105276 5
-0.395566412138908 5
-0.394012463325571 4.7
-0.398196974117945 4.4
-0.396768444918463 4.1
-0.395579536019951 3.8
-0.396001234089912 3.5
-0.393102068757472 3.2
-0.395103266124212 2.9
-0.393236661921815 2.6
-0.392234175732849 2.3
-0.389660857093527 2
-0.385263181948958 1.7
-0.375437762066745 1.4
-0.360696728990026 1.1
-0.333959114157248 0.8
-0.291617411537234 0.5
-0.226363888469943 0.2
-0.128783936892982 -0.1
-0.1 -0.167705146817837
0.00466424386987804 -0.4
0.171582022818641 -0.7
0.2 -0.743956033650646
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
2.3 -1
2.55766067333659 -1
2.6 -0.969320736005583
2.9 -0.711926320124721
2.91258612794311 -0.7
3.2 -0.437434173929681
3.2387924978814 -0.4
3.5 -0.147998995584964
3.54811390751279 -0.1
3.8 0.151573206272001
3.8490950687944 0.2
4.1 0.451545777668693
4.14773862876401 0.5
4.4 0.753290960521842
4.44662715400651 0.8
4.7 1.05133436821538
4.74872911484549 1.1
5 1.35394877362422
5 1.4
5 1.57207603981011
4.83082183062565 1.4
4.7 1.26786183538985
4.53548753018861 1.1
4.4 0.965525536998066
4.23815227463903 0.8
4.1 0.661338472321402
3.93900235192865 0.5
3.8 0.360680393268935
3.63829095672107 0.2
3.5 0.0618658829315944
3.33574868173095 -0.1
3.2 -0.231451282525465
3.01907262353394 -0.4
2.9 -0.509913152244595
2.67128099743499 -0.7
2.6 -0.761469278481725
2.3 -0.979850013992502
2.26263082653635 -1
2.3 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
0.5 -0.835887656902013
0.663633982963679 -1
0.8 -1
1.1 -1
1.15216418468496 -1
1.1 -0.986376271725275
0.8 -0.806207434964198
0.694121939012011 -0.7
0.5 -0.480383738449133
0.448308151161296 -0.4
0.286633168284685 -0.1
0.2 0.0939468996775037
0.163486626283783 0.2
0.0890150524139158 0.5
0.040730061101028 0.8
0.00877410642053182 1.1
-0.00895936926686972 1.4
-0.0196956757687846 1.7
-0.0266220457650931 2
-0.0295960048524443 2.3
-0.0317965809466283 2.6
-0.0321983425090186 2.9
-0.0306276030247306 3.2
-0.031914036876084 3.5
-0.0337773291199139 3.8
-0.0318803237653005 4.1
-0.0306192638967867 4.4
-0.0322654648577952 4.7
-0.0335087293773884 5
-0.1 5
-0.221991083105276 5
-0.221274620922568 4.7
-0.221297993157454 4.4
-0.221349854469805 4.1
-0.22166405406782 3.8
-0.221030108557116 3.5
-0.219307118411021 3.2
-0.221419141590499 2.9
-0.219951276915138 2.6
-0.218534305390007 2.3
-0.216185420632461 2
-0.210974108873333 1.7
-0.201675372933607 1.4
-0.186751270950059 1.1
-0.16010594908605 0.8
-0.116364560364288 0.5
-0.1 0.426207590811361
-0.0413631922646411 0.2
0.0669027079044743 -0.1
0.2 -0.396064836120831
0.202204822188324 -0.4
0.400720818897634 -0.7
0.5 -0.835887656902013
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
2 -1
2.26263082653635 -1
2.3 -0.979850013992502
2.6 -0.761469278481725
2.67128099743499 -0.7
2.9 -0.509913152244595
3.01907262353394 -0.4
3.2 -0.231451282525465
3.33574868173095 -0.1
3.5 0.0618658829315944
3.63829095672107 0.2
3.8 0.360680393268935
3.93900235192865 0.5
4.1 0.661338472321402
4.23815227463903 0.8
4.4 0.965525536998066
4.53548753018861 1.1
4.7 1.26786183538985
4.83082183062565 1.4
5 1.57207603981011
5 1.7
5 1.78834018877653
4.91359127257387 1.7
4.7 1.48275205437669
4.61895408969483 1.4
4.4 1.17656187159192
4.32558364283282 1.1
4.1 0.869143499236021
4.03304976833587 0.8
3.8 0.566448454980606
3.73508803341613 0.5
3.5 0.26638817335847
3.43346499702977 0.2
3.2 -0.0301751072542921
3.12644987875048 -0.1
2.9 -0.311405419528096
2.79727868557449 -0.4
2.6 -0.565513455609739
2.41092525226952 -0.7
2.3 -0.781820476197308
2 -0.941971827539133
1.80050388808936 -1
2 -1
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
0.8 -0.806207434964198
1.1 -0.986376271725275
1.15216418468496 -1
1.4 -1
1.7 -1
1.80050388808936 -1
2 -0.941971827539133
2.3 -0.781820476197308
2.41092525226952 -0.7
2.6 -0.565513455609739
2.79727868557449 -0.4
2.9 -0.311405419528096
3.12644987875048 -0.1
3.2 -0.0301751072542921
3.43346499702977 0.2
3.5 0.26638817335847
3.73508803341613 0.5
3.8 0.566448454980606
4.03304976833586 0.8
4.1 0.869143499236021
4.32558364283282 1.1
4.4 1.17656187159192
4.61895408969483 1.4
4.7 1.48275205437669
4.91359127257387 1.7
5 1.78834018877653
5 2
5 2.00572718592155
4.99449626887664 2
4.70147894811677 1.7
4.7 1.69849573235751
4.40765851635537 1.4
4.4 1.39218464216306
4.11600332857767 1.1
4.1 1.08362260494767
3.82537405083283 0.8
3.8 0.77457131660021
3.53177759914443 0.5
3.5 0.468421944432743
3.23098439124582 0.2
3.2 0.169452227661753
2.91617222402833 -0.1
2.9 -0.115097803647663
2.6 -0.372778911776431
2.56175262963931 -0.4
2.3 -0.582541025879104
2.07277144172778 -0.7
2 -0.738280724347386
1.7 -0.80608823956104
1.4 -0.783023082121682
1.1839682860658 -0.7
1.1 -0.655736508237924
0.8 -0.409583019407673
0.791631031549263 -0.4
0.575076023195487 -0.1
0.5 0.0379944513843503
0.434064113450461 0.2
0.342302943491253 0.5
0.281113499336725 0.8
0.238148696182393 1.1
0.215351431781829 1.4
0.20197199865182 1.7
0.2 1.77073979235495
0.195568024414028 2
0.192085126106771 2.3
0.18979999490968 2.6
0.193116406680711 2.9
0.19064330938776 3.2
0.188939745064054 3.5
0.186640527168483 3.8
0.189124613202038 4.1
0.190121086228375 4.4
0.195087528601484 4.7
0.190227102531704 5
-0.0335087293773884 5
-0.0322654648577952 4.7
-0.0306192638967867 4.4
-0.0318803237653005 4.1
-0.0337773291199139 3.8
-0.031914036876084 3.5
-0.0306276030247306 3.2
-0.0321983425090186 2.9
-0.0317965809466283 2.6
-0.0295960048524443 2.3
-0.0266220457650931 2
-0.0196956757687846 1.7
-0.00895936926686972 1.4
0.00877410642053182 1.1
0.040730061101028 0.8
0.0890150524139158 0.5
0.163486626283783 0.2
0.2 0.0939468996775037
0.286633168284685 -0.1
0.448308151161296 -0.4
0.5 -0.480383738449133
0.694121939012011 -0.7
0.8 -0.806207434964198
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.4 -0.783023082121682
1.7 -0.80608823956104
2 -0.738280724347386
2.07277144172778 -0.7
2.3 -0.582541025879104
2.56175262963931 -0.4
2.6 -0.372778911776431
2.9 -0.115097803647663
2.91617222402833 -0.1
3.2 0.169452227661753
3.23098439124582 0.2
3.5 0.468421944432743
3.53177759914443 0.5
3.8 0.77457131660021
3.82537405083283 0.8
4.1 1.08362260494767
4.11600332857767 1.1
4.4 1.39218464216306
4.40765851635537 1.4
4.7 1.69849573235751
4.70147894811677 1.7
4.99449626887664 2
5 2.00572718592155
5 2.24485187479287
4.7647013904611 2
4.7 1.93372887400089
4.47225831191394 1.7
4.4 1.62608765283183
4.18524174102221 1.4
4.1 1.31214043202534
3.89720373350682 1.1
3.8 0.999423327178447
3.608709598306 0.8
3.5 0.688527661141932
3.31523887034918 0.5
3.2 0.385036124087583
3.01326724037992 0.2
2.9 0.092732953021084
2.67994685167931 -0.1
2.6 -0.168506060290718
2.3 -0.380441201541144
2.26055691097686 -0.4
2 -0.525178149310969
1.7 -0.570261521490292
1.4 -0.497222313910125
1.2451779219263 -0.4
1.1 -0.261736117135857
0.958627312426981 -0.1
0.8 0.190147107343721
0.794671156945757 0.2
0.681673251024444 0.5
0.609894900124583 0.8
0.566707788034168 1.1
0.540844643955083 1.4
0.525323676359062 1.7
0.523078113719696 2
0.514621263534683 2.3
0.51268120269884 2.6
0.513018349580179 2.9
0.511869831852482 3.2
0.507933319153224 3.5
0.509935651420885 3.8
0.515761780208158 4.1
0.508186332987005 4.4
0.512928628512075 4.7
0.512924910738791 5
0.5 5
0.2 5
0.190227102531704 5
0.195087528601484 4.7
0.190121086228375 4.4
0.189124613202038 4.1
0.186640527168483 3.8
0.188939745064054 3.5
0.19064330938776 3.2
0.193116406680711 2.9
0.18979999490968 2.6
0.192085126106771 2.3
0.195568024414028 2
0.2 1.77073979235495
0.201971998651819 1.7
0.215351431781829 1.4
0.238148696182393 1.1
0.281113499336725 0.8
0.342302943491253 0.5
0.434064113450461 0.2
0.5 0.0379944513843503
0.575076023195487 -0.1
0.791631031549263 -0.4
0.8 -0.409583019407673
1.1 -0.655736508237924
1.1839682860658 -0.7
1.4 -0.783023082121682
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.4 -0.497222313910125
1.7 -0.570261521490292
2 -0.525178149310969
2.26055691097686 -0.4
2.3 -0.380441201541144
2.6 -0.168506060290718
2.67994685167931 -0.1
2.9 0.092732953021084
3.01326724037992 0.2
3.2 0.385036124087583
3.31523887034918 0.5
3.5 0.688527661141932
3.608709598306 0.8
3.8 0.999423327178447
3.89720373350682 1.1
4.1 1.31214043202534
4.18524174102221 1.4
4.4 1.62608765283183
4.47225831191394 1.7
4.7 1.93372887400089
4.7647013904611 2
5 2.24485187479287
5 2.3
5 2.51998130993191
4.79282251870878 2.3
4.7 2.20273024351134
4.50828105316642 2
4.4 1.88839236295958
4.22676711928172 1.7
4.1 1.56558804459155
3.94536508649151 1.4
3.8 1.24694536931368
3.6652155802059 1.1
3.5 0.92695167651993
3.37886186729126 0.8
3.2 0.617104757053384
3.08578473345359 0.5
2.9 0.316059504684432
2.76930960956742 0.2
2.6 0.0540208327288016
2.38484476099606 -0.1
2.3 -0.158237985907612
2 -0.295170088992457
1.7 -0.314939859570399
1.4 -0.170803957182072
1.32648485537225 -0.1
1.1288591906247 0.2
1.1 0.276721972984926
1.01296122764107 0.5
0.941349538465119 0.8
0.899763927831817 1.1
0.875924368711358 1.4
0.865079662057272 1.7
0.856905413414872 2
0.853383923202872 2.3
0.852217828630405 2.6
0.850593679603196 2.9
0.845288018976932 3.2
0.848694694600721 3.5
0.845456048415513 3.8
0.843632654788657 4.1
0.84673413852565 4.4
0.847903343138327 4.7
0.847312699527684 5
0.8 5
0.512924910738791 5
0.512928628512075 4.7
0.508186332987005 4.4
0.515761780208158 4.1
0.509935651420885 3.8
0.507933319153224 3.5
0.511869831852482 3.2
0.51301834958018 2.9
0.51268120269884 2.6
0.514621263534683 2.3
0.523078113719696 2
0.525323676359062 1.7
0.540844643955083 1.4
0.566707788034168 1.1
0.609894900124583 0.8
0.681673251024444 0.5
0.794671156945757 0.2
0.8 0.190147107343721
0.958627312426981 -0.1
1.1 -0.261736117135857
1.2451779219263 -0.4
1.4 -0.497222313910125
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.4 -0.170803957182072
1.7 -0.314939859570399
2 -0.295170088992457
2.3 -0.158237985907612
2.38484476099606 -0.1
2.6 0.0540208327288016
2.76930960956742 0.2
2.9 0.316059504684432
3.08578473345359 0.5
3.2 0.617104757053384
3.37886186729126 0.8
3.5 0.92695167651993
3.6652155802059 1.1
3.8 1.24694536931368
3.94536508649151 1.4
4.1 1.56558804459155
4.22676711928172 1.7
4.4 1.88839236295958
4.50828105316642 2
4.7 2.20273024351134
4.79282251870878 2.3
5 2.51998130993191
5 2.6
5 2.87271801248454
4.76014627238759 2.6
4.7 2.53518781111153
4.48944266147315 2.3
4.4 2.20429844301056
4.21617031715745 2
4.1 1.87114765919253
3.95056779900382 1.7
3.8 1.53649384503228
3.68142042797869 1.4
3.5 1.19915571837448
3.40971163318568 1.1
3.2 0.878323292454459
3.12335574743424 0.8
2.9 0.569697362851342
2.8241013145974 0.5
2.6 0.306008422022024
2.45654650338829 0.2
2.3 0.09388836726598
2 -0.0326942427550576
1.7 -0.0161173047475997
1.44046508124381 0.2
1.4 0.25720071118729
1.29258023753406 0.5
1.21458386087976 0.8
1.17026930074109 1.1
1.14262070970199 1.4
1.12937761385952 1.7
1.11979854918084 2
1.11883992135672 2.3
1.11282928790356 2.6
1.11211112158333 2.9
1.10839375815252 3.2
1.1118389278038 3.5
1.11199206972638 3.8
1.10976486636975 4.1
1.10932966291453 4.4
1.11129154727769 4.7
1.1103776693395 5
1.1 5
0.847312699527684 5
0.847903343138327 4.7
0.84673413852565 4.4
0.843632654788657 4.1
0.845456048415513 3.8
0.848694694600721 3.5
0.845288018976932 3.2
0.850593679603196 2.9
0.852217828630405 2.6
0.853383923202872 2.3
0.856905413414872 2
0.865079662057272 1.7
0.875924368711358 1.4
0.899763927831817 1.1
0.941349538465119 0.8
1.01296122764107 0.5
1.1 0.276721972984926
1.1288591906247 0.2
1.32648485537225 -0.1
1.4 -0.170803957182072
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
1.7 -0.0161173047475997
2 -0.0326942427550576
2.3 0.09388836726598
2.45654650338829 0.2
2.6 0.306008422022024
2.8241013145974 0.5
2.9 0.569697362851342
3.12335574743424 0.8
3.2 0.878323292454459
3.40971163318568 1.1
3.5 1.19915571837448
3.68142042797869 1.4
3.8 1.53649384503228
3.95056779900383 1.7
4.1 1.87114765919253
4.21617031715745 2
4.4 2.20429844301056
4.48944266147315 2.3
4.7 2.53518781111153
4.76014627238759 2.6
5 2.87271801248454
5 2.9
5 3.2
5 3.44204586310426
4.84113271953168 3.2
4.7 3.03158590401784
4.60017708606217 2.9
4.4 2.64825314732256
4.36365356084746 2.6
4.12821219461009 2.3
4.1 2.26786849919679
3.88140778313116 2
3.8 1.90442322576462
3.62751456959494 1.7
3.5 1.5480120736534
3.3720036900207 1.4
3.2 1.20626167764627
3.10059348810825 1.1
2.9 0.893756616001639
2.79953122117375 0.8
2.6 0.620495355383438
2.43925571993056 0.5
2.3 0.40421079078977
2 0.299406619138124
1.7 0.39298906689898
1.61985706449107 0.5
1.4883831548433 0.8
1.41652882308105 1.1
1.4 1.22494125856545
1.38301403459373 1.4
1.36498420128647 1.7
1.35470623134027 2
1.35117651854284 2.3
1.34799898887268 2.6
1.34676449798603 2.9
1.34368756646834 3.2
1.3448024151224 3.5
1.34276879081648 3.8
1.34559852154025 4.1
1.34500448167276 4.4
1.3423652188131 4.7
1.34855307562312 5
1.1103776693395 5
1.11129154727769 4.7
1.10932966291453 4.4
1.10976486636975 4.1
1.11199206972638 3.8
1.1118389278038 3.5
1.10839375815252 3.2
1.11211112158333 2.9
1.11282928790356 2.6
1.11883992135672 2.3
1.11979854918084 2
1.12937761385952 1.7
1.14262070970199 1.4
1.17026930074109 1.1
1.21458386087976 0.8
1.29258023753406 0.5
1.4 0.25720071118729
1.44046508124381 0.2
1.7 -0.0161173047475997
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
1.7 0.39298906689898
2 0.299406619138124
2.3 0.40421079078977
2.43925571993056 0.5
2.6 0.620495355383438
2.79953122117375 0.8
2.9 0.893756616001639
3.10059348810825 1.1
3.2 1.20626167764627
3.3720036900207 1.4
3.5 1.5480120736534
3.62751456959494 1.7
3.8 1.90442322576462
3.88140778313116 2
4.1 2.26786849919679
4.12821219461009 2.3
4.36365356084746 2.6
4.4 2.64825314732256
4.60017708606217 2.9
4.7 3.03158590401784
4.84113271953168 3.2
5 3.44204586310426
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.26781032199141 5
4.38513729249552 4.7
4.38944398041989 4.4
4.4 4.31054769775231
4.42525954233083 4.1
4.40207389659378 3.8
4.4 3.79460322199615
4.28850529706392 3.5
4.19363453847936 3.2
4.1 3.0109947772772
4.04336385413301 2.9
3.85661721291655 2.6
3.8 2.51372865048462
3.65858977068221 2.3
3.5 2.07434998208515
3.44547420243501 2
3.21199492935994 1.7
3.2 1.68550733087126
2.94703380368862 1.4
2.9 1.34867935766636
2.63590915844605 1.1
2.6 1.06728070069056
2.3 0.869719014358149
2 0.818629019352863
1.79250249971712 1.1
1.7 1.39751895097904
1.69963670976635 1.4
1.66959631561994 1.7
1.65834133149817 2
1.6559277065894 2.3
1.64833708751511 2.6
1.65219728170077 2.9
1.64671426137855 3.2
1.64574700512202 3.5
1.64320853377532 3.8
1.64716370355855 4.1
1.64618548258624 4.4
1.64293434812291 4.7
1.63976275924946 5
1.4 5
1.34855307562312 5
1.3423652188131 4.7
1.34500448167276 4.4
1.34559852154025 4.1
1.34276879081648 3.8
1.3448024151224 3.5
1.34368756646834 3.2
1.34676449798603 2.9
1.34799898887268 2.6
1.35117651854284 2.3
1.35470623134027 2
1.36498420128647 1.7
1.38301403459373 1.4
1.4 1.22494125856545
1.41652882308105 1.1
1.4883831548433 0.8
1.61985706449107 0.5
1.7 0.39298906689898
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
2 0.818629019352863
2.3 0.869719014358149
2.6 1.06728070069056
2.63590915844605 1.1
2.9 1.34867935766637
2.94703380368862 1.4
3.2 1.68550733087126
3.21199492935994 1.7
3.44547420243501 2
3.5 2.07434998208515
3.65858977068221 2.3
3.8 2.51372865048462
3.85661721291655 2.6
4.04336385413301 2.9
4.1 3.0109947772772
4.19363453847936 3.2
4.28850529706392 3.5
4.4 3.79460322199615
4.40207389659378 3.8
4.42525954233083 4.1
4.4 4.31054769775231
4.38944398041989 4.4
4.38513729249552 4.7
4.26781032199141 5
4.1 5
3.8 5
3.5 5
3.2 5
2.9 5
2.6 5
2.3 5
2 5
1.7 5
1.63976275924946 5
1.64293434812291 4.7
1.64618548258624 4.4
1.64716370355855 4.1
1.64320853377532 3.8
1.64574700512202 3.5
1.64671426137855 3.2
1.65219728170077 2.9
1.64833708751511 2.6
1.6559277065894 2.3
1.65834133149817 2
1.66959631561994 1.7
1.69963670976635 1.4
1.7 1.39751895097904
1.79250249971712 1.1
2 0.818629019352863

2.54941500428936 2.3
2.4496331897529 2.6
2.50859751467823 2.9
2.47865165011729 3.2
2.52054470896683 3.5
2.57792555713494 3.8
2.6 3.91542411815578
2.69371089856396 4.1
2.78333392756837 4.4
2.86675928781121 4.7
2.9 4.839116430356
2.91180267981874 4.7
2.9823778202882 4.4
3.2 4.17382029005782
3.22691278909861 4.1
3.22323036952995 3.8
3.21548457033851 3.5
3.20553296474001 3.2
3.2 3.18109326064541
3.0465437076516 2.9
2.94256417209332 2.6
2.9 2.51825297137327
2.65492852481193 2.3
2.6 2.24740008945206
2.54941500428936 2.3
};
\addplot [draw=none, fill=lavender231240249]
table{%
x  y
2.6 2.24740008945206
2.65492852481193 2.3
2.9 2.51825297137327
2.94256417209332 2.6
3.0465437076516 2.9
3.2 3.18109326064541
3.20553296474001 3.2
3.21548457033851 3.5
3.22323036952995 3.8
3.22691278909861 4.1
3.2 4.17382029005782
2.9823778202882 4.4
2.91180267981874 4.7
2.9 4.839116430356
2.86675928781121 4.7
2.78333392756837 4.4
2.69371089856396 4.1
2.6 3.91542411815578
2.57792555713494 3.8
2.52054470896683 3.5
2.47865165011729 3.2
2.50859751467823 2.9
2.4496331897529 2.6
2.54941500428936 2.3
2.6 2.24740008945206
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.6 2.3
};
\coordinate (CVI_mean_lml_b) at (axis cs:2.5999999999999996,2.0);
\coordinate (CVI_mean_lml_ep_b) at (axis cs:2.5999999999999996,2.3);
\end{axis}



==> fig/tikz/ionosphere/cvi_Z_0.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{pink}{RGB}{255,192,203}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
axis background/.style={fill=pink},
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=black]
table{%
x  y
-0.7 -0.274910200162423
-0.4 -0.122514768983477
-0.374860056963016 -0.1
-0.1 0.0563790170625844
0.0715616288956246 0.2
0.2 0.268693899796434
0.5 0.437187097443227
0.617985010469972 0.5
0.8 0.560532032788399
1.1 0.703895934946012
1.21667297980405 0.8
1.4 0.934497002226144
1.55932653193647 1.1
1.7 1.24513617406479
1.84006047389303 1.4
2 1.57830794779882
2.10868282218159 1.7
2.3 1.92004811073895
2.37037805902862 2
2.6 2.27590752490414
2.62105509003649 2.3
2.87792907531765 2.6
2.9 2.62676015538143
3.14280324221269 2.9
3.2 2.96979703432035
3.4094231854909 3.2
3.5 3.30688284527983
3.68027266189265 3.5
3.8 3.63554457029331
3.95239953825642 3.8
4.1 3.97091511117955
4.21491382268577 4.1
4.4 4.33330332118378
4.45779780111041 4.4
4.69126366725857 4.7
4.7 4.71174155022035
4.94961013703058 5
4.7 5
4.4 5
4.1 5
3.8 5
3.5 5
3.2 5
2.9 5
2.6 5
2.3 5
2 5
1.7 5
1.4 5
1.1 5
0.8 5
0.5 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.330684344742375
-0.7 -0.274910200162423
};
\addplot [draw=none, fill=midnightblue854116]
table{%
x  y
-0.7 -0.423165877752524
-0.665651473916218 -0.4
-0.4 -0.284691539023569
-0.193773821358193 -0.1
-0.1 -0.0466482755907682
0.194632295777341 0.2
0.2 0.20287085964138
0.5 0.362252259243771
0.758739334974199 0.5
0.8 0.513721902435958
1.1 0.64450807974143
1.28877147040378 0.8
1.4 0.881602285231736
1.61024725198285 1.1
1.7 1.19260005200929
1.88757469554655 1.4
2 1.52533690580242
2.15599110759493 1.7
2.3 1.86563533428986
2.41827518351485 2
2.6 2.21835563325513
2.67135130309134 2.3
2.9 2.58346716327711
2.91460217491655 2.6
3.17516227175328 2.9
3.2 2.930309406301
3.44534637537195 3.2
3.5 3.26449260704035
3.71984346593007 3.5
3.8 3.59074604963629
3.99391397091989 3.8
4.1 3.92284314859613
4.25770839790636 4.1
4.4 4.27936025167696
4.50454361901285 4.4
4.7 4.65817338973618
4.73638091125191 4.7
4.98112734510324 5
4.94961013703058 5
4.7 4.71174155022035
4.69126366725857 4.7
4.45779780111041 4.4
4.4 4.33330332118378
4.21491382268577 4.1
4.1 3.97091511117955
3.95239953825642 3.8
3.8 3.63554457029331
3.68027266189265 3.5
3.5 3.30688284527983
3.4094231854909 3.2
3.2 2.96979703432035
3.14280324221269 2.9
2.9 2.62676015538143
2.87792907531765 2.6
2.62105509003649 2.3
2.6 2.27590752490414
2.37037805902862 2
2.3 1.92004811073895
2.10868282218159 1.7
2 1.57830794779882
1.84006047389303 1.4
1.7 1.24513617406479
1.55932653193647 1.1
1.4 0.934497002226144
1.21667297980405 0.8
1.1 0.703895934946012
0.8 0.560532032788399
0.617985010469972 0.5
0.5 0.437187097443227
0.2 0.268693899796434
0.0715616288956246 0.2
-0.1 0.0563790170625844
-0.374860056963016 -0.1
-0.4 -0.122514768983477
-0.7 -0.274910200162423
-1 -0.330684344742375
-1 -0.4
-1 -0.501762830879718
-0.7 -0.423165877752524
};
\addplot [draw=none, fill=midnightblue868137]
table{%
x  y
-0.833037989695701 -0.7
-0.7 -0.675154165258568
-0.4 -0.492123219792619
-0.331828307278501 -0.4
-0.1 -0.198740286251025
-0.0249011540422955 -0.1
0.2 0.0804680193814682
0.335233558574848 0.2
0.5 0.287317421044315
0.8 0.439874011466784
0.899085456324761 0.5
1.1 0.585120224536848
1.3608699610035 0.8
1.4 0.828707568237329
1.66116797202924 1.1
1.7 1.14006392995379
1.93508891720006 1.4
2 1.47236586380603
2.20329939300827 1.7
2.3 1.81122255784077
2.46617230800108 2
2.6 2.16080374160611
2.72164751614619 2.3
2.9 2.52111244605808
2.96967526993137 2.6
3.2 2.88420470731722
3.21434961290087 2.9
3.481269565253 3.2
3.5 3.22210236880086
3.75941426996748 3.5
3.8 3.54594752897927
4.03542840358337 3.8
4.1 3.8747711860127
4.30050297312695 4.1
4.4 4.22541718217014
4.55128943691529 4.4
4.7 4.59642802126619
4.79008721822622 4.7
5 4.97207280670204
5 5
4.98112734510324 5
4.73638091125191 4.7
4.7 4.65817338973618
4.50454361901285 4.4
4.4 4.27936025167696
4.25770839790636 4.1
4.1 3.92284314859613
3.99391397091989 3.8
3.8 3.59074604963629
3.71984346593006 3.5
3.5 3.26449260704035
3.44534637537195 3.2
3.2 2.930309406301
3.17516227175328 2.9
2.91460217491655 2.6
2.9 2.58346716327711
2.67135130309134 2.3
2.6 2.21835563325513
2.41827518351485 2
2.3 1.86563533428986
2.15599110759493 1.7
2 1.52533690580242
1.88757469554655 1.4
1.7 1.19260005200929
1.61024725198285 1.1
1.4 0.881602285231736
1.28877147040378 0.8
1.1 0.64450807974143
0.8 0.513721902435958
0.758739334974199 0.5
0.5 0.362252259243771
0.2 0.20287085964138
0.194632295777341 0.2
-0.1 -0.0466482755907682
-0.193773821358193 -0.1
-0.4 -0.284691539023569
-0.665651473916218 -0.4
-0.7 -0.423165877752524
-1 -0.501762830879718
-1 -0.7
-1 -0.750599133981164
-0.833037989695701 -0.7
};
\addplot [draw=none, fill=teal882156]
table{%
x  y
-0.7 -1
-0.488069190428003 -1
-0.4 -0.929613390606909
-0.291817330003266 -0.7
-0.1 -0.408151151123477
-0.0967026485327831 -0.4
0.130854100580871 -0.1
0.2 -0.0445150756577544
0.476634283438534 0.2
0.5 0.21238258284486
0.8 0.354813386040932
1.03926229318349 0.5
1.1 0.525732369332266
1.4 0.759080076919363
1.43763111869926 0.8
1.7 1.07920894466994
1.71788142866448 1.1
1.98260313885357 1.4
2 1.41939482180963
2.2506076784216 1.7
2.3 1.75680978139168
2.51406943248731 2
2.6 2.1032518499571
2.77194372920104 2.3
2.9 2.45875772883905
3.0247483649462 2.6
3.2 2.81624833613172
3.27608621001518 2.9
3.5 3.16502773534157
3.5326917950897 3.2
3.79898507400489 3.5
3.8 3.50114900832225
4.07694283624684 3.8
4.1 3.82669922342928
4.34329754834755 4.1
4.4 4.17147411266332
4.59803525481773 4.4
4.7 4.53468265279619
4.84379352520052 4.7
5 4.90246282129463
5 4.97207280670204
4.79008721822622 4.7
4.7 4.59642802126619
4.55128943691529 4.4
4.4 4.22541718217014
4.30050297312695 4.1
4.1 3.8747711860127
4.03542840358337 3.8
3.8 3.54594752897927
3.75941426996748 3.5
3.5 3.22210236880086
3.481269565253 3.2
3.21434961290087 2.9
3.2 2.88420470731722
2.96967526993137 2.6
2.9 2.52111244605808
2.72164751614619 2.3
2.6 2.16080374160611
2.46617230800108 2
2.3 1.81122255784077
2.20329939300827 1.7
2 1.47236586380603
1.93508891720006 1.4
1.7 1.14006392995379
1.66116797202924 1.1
1.4 0.828707568237329
1.3608699610035 0.8
1.1 0.585120224536848
0.899085456324761 0.5
0.8 0.439874011466784
0.5 0.287317421044315
0.335233558574848 0.2
0.2 0.0804680193814682
-0.0249011540422955 -0.1
-0.1 -0.198740286251025
-0.331828307278501 -0.4
-0.4 -0.492123219792619
-0.7 -0.675154165258568
-0.833037989695701 -0.7
-1 -0.750599133981164
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.4 -1
-0.1 -1
-0.0429567933321329 -1
-0.0100217549872096 -0.7
0.0946985521912709 -0.4
0.2 -0.250799981925627
0.294345382790627 -0.1
0.5 0.0776532488382486
0.651334261693725 0.2
0.8 0.26975276061508
1.1 0.439676080093953
1.16905833915205 0.5
1.4 0.669592565492461
1.51992636539292 0.8
1.7 0.991631603688134
1.79320266419247 1.1
2 1.34373022553258
2.04833819577644 1.4
2.29791596383494 1.7
2.3 1.70239700494259
2.56196655697353 2
2.6 2.04569995830809
2.82223994225589 2.3
2.9 2.39640301162002
3.07982145996102 2.6
3.2 2.74829196494623
3.33782280712949 2.9
3.5 3.09195536886512
3.60099926259 3.2
3.8 3.42481197690014
3.87005529870403 3.5
4.1 3.76338483778665
4.1329392556581 3.8
4.38609212356814 4.1
4.4 4.11753104315649
4.64478107272017 4.4
4.7 4.4729372843262
4.89749983217483 4.7
5 4.83285283588723
5 4.90246282129463
4.84379352520052 4.7
4.7 4.53468265279619
4.59803525481773 4.4
4.4 4.17147411266332
4.34329754834755 4.1
4.1 3.82669922342928
4.07694283624684 3.8
3.8 3.50114900832225
3.79898507400489 3.5
3.5326917950897 3.2
3.5 3.16502773534157
3.27608621001518 2.9
3.2 2.81624833613172
3.0247483649462 2.6
2.9 2.45875772883905
2.77194372920104 2.3
2.6 2.1032518499571
2.51406943248731 2
2.3 1.75680978139168
2.2506076784216 1.7
2 1.41939482180963
1.98260313885357 1.4
1.71788142866448 1.1
1.7 1.07920894466994
1.43763111869926 0.8
1.4 0.759080076919363
1.1 0.525732369332266
1.03926229318349 0.5
0.8 0.354813386040932
0.5 0.21238258284486
0.476634283438534 0.2
0.2 -0.0445150756577544
0.130854100580871 -0.1
-0.0967026485327831 -0.4
-0.1 -0.408151151123477
-0.291817330003266 -0.7
-0.4 -0.929613390606909
-0.488069190428003 -1
-0.4 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
0.2 -1
0.24830920465528 -1
0.224044643249559 -0.7
0.288759144843966 -0.4
0.464012840589566 -0.1
0.5 -0.0689127534675543
0.8 0.169598337684932
0.837713179084443 0.2
1.1 0.333229593647595
1.29091742214939 0.5
1.4 0.580105054065559
1.60222161208659 0.8
1.7 0.904054262706325
1.86852389972047 1.1
2 1.25495702325246
2.12459825674402 1.4
2.3 1.61192114041275
2.37566118770168 1.7
2.6 1.97967991777447
2.6174966502833 2
2.87253615531074 2.3
2.9 2.33404829440098
3.13489455497585 2.6
3.2 2.68033559376074
3.3995594042438 2.9
3.5 3.01888300238868
3.6693067300903 3.2
3.8 3.34764474121224
3.94195469868029 3.5
4.1 3.68102933364598
4.2070268423779 3.8
4.4 4.03825522956857
4.45404642046506 4.1
4.69152689062261 4.4
4.7 4.4111919158562
4.95120613914914 4.7
5 4.76324285047982
5 4.83285283588723
4.89749983217483 4.7
4.7 4.4729372843262
4.64478107272017 4.4
4.4 4.11753104315649
4.38609212356814 4.1
4.1329392556581 3.8
4.1 3.76338483778665
3.87005529870403 3.5
3.8 3.42481197690014
3.60099926259 3.2
3.5 3.09195536886512
3.33782280712949 2.9
3.2 2.74829196494623
3.07982145996103 2.6
2.9 2.39640301162002
2.82223994225589 2.3
2.6 2.04569995830809
2.56196655697353 2
2.3 1.70239700494259
2.29791596383494 1.7
2.04833819577644 1.4
2 1.34373022553258
1.79320266419247 1.1
1.7 0.991631603688134
1.51992636539292 0.8
1.4 0.669592565492461
1.16905833915205 0.5
1.1 0.439676080093953
0.8 0.26975276061508
0.651334261693725 0.2
0.5 0.0776532488382486
0.294345382790627 -0.1
0.2 -0.250799981925627
0.0946985521912709 -0.4
-0.0100217549872096 -0.7
-0.0429567933321329 -1
0.2 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.440611099194882
4.7807548925822 0.2
4.7 0.111354909269737
4.50601001038444 -0.1
4.4 -0.215286437574118
4.22848895111091 -0.4
4.1 -0.537473280352706
3.94618022502158 -0.7
3.8 -0.851934610990629
3.65522671695479 -1
3.8 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
0.5 -1
0.517922658219617 -1
0.5 -0.934927104749343
0.451721987807538 -0.7
0.486072218611819 -0.4
0.5 -0.375333043854897
0.670811761675477 -0.1
0.8 0.000666586426869537
1.04727255522047 0.2
1.1 0.226783107201237
1.4 0.482842151162919
1.41417532327234 0.5
1.68451685878025 0.8
1.7 0.816476921724516
1.94384513524847 1.1
2 1.16618382097234
2.2008583177116 1.4
2.3 1.51978340684068
2.45480901485195 1.7
2.6 1.88100747869613
2.70245876510116 2
2.9 2.25099425402405
2.94294769242816 2.3
3.18996764999068 2.6
3.2 2.61237922257525
3.46129600135812 2.9
3.5 2.94581063591223
3.7376141975906 3.2
3.8 3.27047750552433
4.01385409865654 3.5
4.1 3.59867382950532
4.28111442909769 3.8
4.4 3.94678263721625
4.53411419224167 4.1
4.7 4.31502601971353
4.77435995805406 4.4
5 4.68934709234574
5 4.7
5 4.76324285047982
4.95120613914914 4.7
4.7 4.4111919158562
4.69152689062261 4.4
4.45404642046506 4.1
4.4 4.03825522956857
4.2070268423779 3.8
4.1 3.68102933364598
3.94195469868029 3.5
3.8 3.34764474121224
3.6693067300903 3.2
3.5 3.01888300238868
3.3995594042438 2.9
3.2 2.68033559376074
3.13489455497585 2.6
2.9 2.33404829440098
2.87253615531074 2.3
2.6174966502833 2
2.6 1.97967991777447
2.37566118770168 1.7
2.3 1.61192114041275
2.12459825674402 1.4
2 1.25495702325246
1.86852389972047 1.1
1.7 0.904054262706325
1.60222161208659 0.8
1.4 0.580105054065559
1.29091742214939 0.5
1.1 0.333229593647595
0.837713179084443 0.2
0.8 0.169598337684932
0.5 -0.0689127534675543
0.464012840589566 -0.1
0.288759144843966 -0.4
0.224044643249559 -0.7
0.24830920465528 -1
0.5 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
2.9 -1
3.2 -1
3.5 -1
3.65522671695479 -1
3.8 -0.851934610990629
3.94618022502158 -0.7
4.1 -0.537473280352706
4.22848895111091 -0.4
4.4 -0.215286437574118
4.50601001038444 -0.1
4.7 0.111354909269737
4.7807548925822 0.2
5 0.440611099194882
5 0.5
5 0.8
5 1.1
5 1.10820399755333
4.99196086400583 1.1
4.7 0.800828229204842
4.69918330816689 0.8
4.406702071206 0.5
4.4 0.493072257045866
4.1119672783541 0.2
4.1 0.18770212430148
3.81341136253676 -0.1
3.8 -0.113658109830582
3.50888847481422 -0.4
3.5 -0.408924543878771
3.2 -0.696134655486769
3.19565813361179 -0.7
2.9 -0.97472080957973
2.86934502364861 -1
2.9 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
0.5 -0.934927104749343
0.517922658219617 -1
0.8 -1
0.834873375090284 -1
0.8 -0.94085389882002
0.715722123544581 -0.7
0.729031315468549 -0.4
0.8 -0.275164389666924
0.915294917283265 -0.1
1.1 0.0391443316356602
1.25203392016275 0.2
1.4 0.319194917316124
1.54937598067579 0.5
1.7 0.6735380809105
1.79895543998713 0.8
2 1.05990389557373
2.03211162887195 1.1
2.27711837867919 1.4
2.3 1.42764567326861
2.53395684200221 1.7
2.6 1.78233503961778
2.78742087991902 2
2.9 2.14304209588383
3.03755488577724 2.3
3.2 2.50321027587634
3.28768659289668 2.6
3.5 2.85243942233596
3.54444182886033 2.9
3.8 3.18834815402504
3.81089117127718 3.2
4.0857534986328 3.5
4.1 3.51631832536466
4.35520201581748 3.8
4.4 3.85531004486394
4.61418196401827 4.1
4.7 4.21123983990039
4.86518230098161 4.4
5 4.57288203313249
5 4.68934709234574
4.77435995805406 4.4
4.7 4.31502601971353
4.53411419224167 4.1
4.4 3.94678263721625
4.28111442909769 3.8
4.1 3.59867382950532
4.01385409865654 3.5
3.8 3.27047750552433
3.7376141975906 3.2
3.5 2.94581063591223
3.46129600135812 2.9
3.2 2.61237922257525
3.18996764999068 2.6
2.94294769242816 2.3
2.9 2.25099425402405
2.70245876510116 2
2.6 1.88100747869613
2.45480901485195 1.7
2.3 1.51978340684068
2.2008583177116 1.4
2 1.16618382097234
1.94384513524847 1.1
1.7 0.816476921724516
1.68451685878025 0.8
1.41417532327234 0.5
1.4 0.482842151162919
1.1 0.226783107201237
1.04727255522047 0.2
0.8 0.000666586426869523
0.670811761675477 -0.1
0.5 -0.375333043854897
0.486072218611819 -0.4
0.451721987807538 -0.7
0.5 -0.934927104749343
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
2.6 -1
2.86934502364861 -1
2.9 -0.97472080957973
3.19565813361179 -0.7
3.2 -0.696134655486769
3.5 -0.408924543878771
3.50888847481422 -0.4
3.8 -0.113658109830582
3.81341136253676 -0.1
4.1 0.18770212430148
4.1119672783541 0.2
4.4 0.493072257045866
4.406702071206 0.5
4.69918330816689 0.8
4.7 0.800828229204842
4.99196086400583 1.1
5 1.10820399755333
5 1.4
5 1.49403577443948
4.9072601248572 1.4
4.7 1.18914780585568
4.61151511631144 1.1
4.4 0.88595882449398
4.3138785439641 0.8
4.1 0.585266009811783
4.01336448251647 0.5
3.8 0.288316282873046
3.70830258868943 0.2
3.5 -0.00294533102645982
3.39567982220657 -0.1
3.2 -0.285365924950609
3.06967634857038 -0.4
2.9 -0.55391555495196
2.71883666100136 -0.7
2.6 -0.801021786094604
2.32081618064799 -1
2.6 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.8 -0.94085389882002
0.834873375090284 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.3 -1
2.32081618064799 -1
2.6 -0.801021786094604
2.71883666100136 -0.7
2.9 -0.55391555495196
3.06967634857038 -0.4
3.2 -0.285365924950609
3.39567982220657 -0.1
3.5 -0.00294533102645982
3.70830258868943 0.2
3.8 0.288316282873046
4.01336448251647 0.5
4.1 0.585266009811783
4.3138785439641 0.8
4.4 0.88595882449398
4.61151511631144 1.1
4.7 1.18914780585568
4.9072601248572 1.4
5 1.49403577443948
5 1.7
5 1.82656271178155
4.87470172789747 1.7
4.7 1.52298294555551
4.57744105975843 1.4
4.4 1.22129769877259
4.27799701149146 1.1
4.1 0.922321761767055
3.97528460594237 0.8
3.8 0.627339010481248
3.66744178986508 0.5
3.5 0.338385061802531
3.35096434655434 0.2
3.2 0.0589089666713741
3.01866053310205 -0.1
2.9 -0.205316601428963
2.65536731248623 -0.4
2.6 -0.445368764794064
2.3 -0.650175712551641
2.2026055855132 -0.7
2 -0.811010787226785
1.7 -0.908564666945236
1.4 -0.913323272030174
1.1 -0.720120299451536
1.08730931285246 -0.7
1.05369658503582 -0.4
1.1 -0.319213530829277
1.21720342428191 -0.1
1.4 0.100815586467676
1.46249608828111 0.2
1.68457663807925 0.5
1.7 0.517769680034594
1.92084296751911 0.8
2 0.902331647782581
2.15830597153916 1.1
2.3 1.28479892940057
2.39460663809838 1.4
2.6 1.67052456324849
2.62467222813025 1.7
2.87238299473688 2
2.9 2.03508993774361
3.13216207912631 2.3
3.2 2.38486166347062
3.39490444778641 2.6
3.5 2.72495800831818
3.66356374585366 2.9
3.8 3.05394202364865
3.93652278276424 3.2
4.1 3.38561800356561
4.20378532848817 3.5
4.4 3.7379476701955
4.45482104147952 3.8
4.69424973579487 4.1
4.7 4.10745366008725
4.95600464390916 4.4
5 4.45641697391924
5 4.57288203313249
4.86518230098161 4.4
4.7 4.21123983990039
4.61418196401827 4.1
4.4 3.85531004486394
4.35520201581748 3.8
4.1 3.51631832536466
4.0857534986328 3.5
3.81089117127718 3.2
3.8 3.18834815402504
3.54444182886033 2.9
3.5 2.85243942233596
3.28768659289668 2.6
3.2 2.50321027587634
3.03755488577724 2.3
2.9 2.14304209588383
2.78742087991902 2
2.6 1.78233503961778
2.53395684200221 1.7
2.3 1.42764567326861
2.27711837867919 1.4
2.03211162887195 1.1
2 1.05990389557373
1.79895543998713 0.8
1.7 0.6735380809105
1.54937598067579 0.5
1.4 0.319194917316124
1.25203392016275 0.2
1.1 0.0391443316356602
0.915294917283265 -0.1
0.8 -0.275164389666924
0.729031315468549 -0.4
0.715722123544581 -0.7
0.8 -0.94085389882002
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
1.1 -0.720120299451536
1.4 -0.913323272030174
1.7 -0.908564666945236
2 -0.811010787226785
2.2026055855132 -0.7
2.3 -0.650175712551641
2.6 -0.445368764794064
2.65536731248623 -0.4
2.9 -0.205316601428963
3.01866053310205 -0.1
3.2 0.0589089666713741
3.35096434655434 0.2
3.5 0.338385061802531
3.66744178986508 0.5
3.8 0.627339010481248
3.97528460594237 0.8
4.1 0.922321761767055
4.27799701149146 1.1
4.4 1.22129769877259
4.57744105975843 1.4
4.7 1.52298294555551
4.87470172789747 1.7
5 1.82656271178155
5 2
5 2.15548364744485
4.84548868900192 2
4.7 1.85296073321033
4.54692388487427 1.7
4.4 1.55253860557145
4.24592815486115 1.4
4.1 1.25496413788152
3.94139966836902 1.1
3.8 0.961467114996799
3.63140120114782 0.8
3.5 0.674045381465227
3.31212721428094 0.5
3.2 0.396257822400498
2.97525839187981 0.2
2.9 0.134401677707064
2.60189704344876 -0.1
2.6 -0.101498394381859
2.3 -0.284648499690097
2.02830113474519 -0.4
2 -0.412380949455997
1.7 -0.41112561726886
1.68160316432433 -0.4
1.58985398061728 -0.1
1.69256985657153 0.2
1.7 0.210551300569869
1.88262043978631 0.5
2 0.685682806264617
2.07769800882513 0.8
2.28450031420637 1.1
2.3 1.12021486277031
2.5297681009861 1.4
2.6 1.49250276460224
2.77368425008548 1.7
2.9 1.86701709748468
3.01443763474864 2
3.2 2.23837228451241
3.25518437341768 2.3
3.5 2.59534273372558
3.5043178970363 2.6
3.78268566284699 2.9
3.8 2.91953589327226
4.0621543942513 3.2
4.1 3.24297128310346
4.33321685794583 3.5
4.4 3.58098728264144
4.59348999950016 3.8
4.7 3.93584298008621
4.84450846920686 4.1
5 4.29785707900253
5 4.4
5 4.45641697391924
4.95600464390916 4.4
4.7 4.10745366008725
4.69424973579487 4.1
4.45482104147952 3.8
4.4 3.7379476701955
4.20378532848817 3.5
4.1 3.38561800356561
3.93652278276424 3.2
3.8 3.05394202364865
3.66356374585366 2.9
3.5 2.72495800831818
3.39490444778641 2.6
3.2 2.38486166347062
3.13216207912631 2.3
2.9 2.03508993774361
2.87238299473688 2
2.62467222813025 1.7
2.6 1.67052456324849
2.39460663809838 1.4
2.3 1.28479892940057
2.15830597153916 1.1
2 0.902331647782581
1.92084296751911 0.8
1.7 0.517769680034594
1.68457663807925 0.5
1.46249608828111 0.2
1.4 0.100815586467676
1.21720342428191 -0.1
1.1 -0.319213530829277
1.05369658503582 -0.4
1.08730931285246 -0.7
1.1 -0.720120299451536
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.7 -0.41112561726886
2 -0.412380949455997
2.02830113474519 -0.4
2.3 -0.284648499690097
2.6 -0.101498394381859
2.60189704344876 -0.1
2.9 0.134401677707064
2.97525839187981 0.2
3.2 0.396257822400498
3.31212721428094 0.5
3.5 0.674045381465227
3.63140120114782 0.8
3.8 0.961467114996799
3.94139966836902 1.1
4.1 1.25496413788152
4.24592815486115 1.4
4.4 1.55253860557145
4.54692388487427 1.7
4.7 1.85296073321033
4.84548868900192 2
5 2.15548364744485
5 2.3
5 2.52518379582168
4.77462265746059 2.3
4.7 2.22482590085005
4.47317679845034 2
4.4 1.9268882073068
4.16895133941228 1.7
4.1 1.63185891610916
3.86075924747471 1.4
3.8 1.340885727771
3.54622736540182 1.1
3.5 1.05607769913685
3.2204481495892 0.8
3.2 0.781319577731751
2.9 0.533114933184428
2.85075833991717 0.5
2.6 0.332644654596243
2.31902622566227 0.2
2.3 0.191177328088121
2.27616519524273 0.2
2.19309640923186 0.5
2.29932937954835 0.8
2.3 0.801031298802555
2.51927594289593 1.1
2.6 1.22059739206651
2.73878822430142 1.4
2.9 1.63567113725478
2.95221255829508 1.7
3.183987637155 2
3.2 2.02056938381139
3.45021539977723 2.3
3.5 2.3600595645486
3.72245627243049 2.6
3.8 2.68812596667054
3.99731908511644 2.9
4.1 3.01667936724312
4.26660640954582 3.2
4.4 3.36084346295252
4.52329102047632 3.5
4.7 3.72483837479737
4.76618691729238 3.8
5 4.09953460279969
5 4.1
5 4.29785707900253
4.84450846920686 4.1
4.7 3.93584298008621
4.59348999950016 3.8
4.4 3.58098728264144
4.33321685794583 3.5
4.1 3.24297128310346
4.0621543942513 3.2
3.8 2.91953589327226
3.78268566284699 2.9
3.5043178970363 2.6
3.5 2.59534273372558
3.25518437341768 2.3
3.2 2.23837228451241
3.01443763474864 2
2.9 1.86701709748468
2.77368425008548 1.7
2.6 1.49250276460224
2.5297681009861 1.4
2.3 1.12021486277031
2.28450031420637 1.1
2.07769800882513 0.8
2 0.685682806264617
1.88262043978631 0.5
1.7 0.210551300569869
1.69256985657153 0.2
1.58985398061728 -0.1
1.68160316432433 -0.4
1.7 -0.41112561726886
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
2.3 0.191177328088121
2.31902622566226 0.2
2.6 0.332644654596243
2.85075833991717 0.5
2.9 0.533114933184428
3.2 0.781319577731751
3.2204481495892 0.8
3.5 1.05607769913685
3.54622736540182 1.1
3.8 1.340885727771
3.86075924747471 1.4
4.1 1.63185891610916
4.16895133941228 1.7
4.4 1.9268882073068
4.47317679845034 2
4.7 2.22482590085005
4.77462265746059 2.3
5 2.52518379582168
5 2.6
5 2.9
5 3.10706906982321
4.77216220173296 2.9
4.7 2.83044585947817
4.44051928647572 2.6
4.4 2.56177401800098
4.26986325557845 2.6
4.39320113283587 2.9
4.4 2.90851903821906
4.65236892939843 3.2
4.7 3.2640558241322
4.90212261485594 3.5
5 3.63521241232135
5 3.8
5 4.09953460279969
4.76618691729238 3.8
4.7 3.72483837479737
4.52329102047632 3.5
4.4 3.36084346295252
4.26660640954582 3.2
4.1 3.01667936724312
3.99731908511644 2.9
3.8 2.68812596667054
3.72245627243049 2.6
3.5 2.3600595645486
3.45021539977723 2.3
3.2 2.02056938381139
3.183987637155 2
2.95221255829508 1.7
2.9 1.63567113725478
2.73878822430142 1.4
2.6 1.22059739206651
2.51927594289593 1.1
2.3 0.801031298802555
2.29932937954835 0.8
2.19309640923186 0.5
2.27616519524273 0.2
2.3 0.191177328088121

4.09314636697896 2.3
4.1 2.31406090617872
4.10278574288269 2.3
4.1 2.29742338426291
4.09314636697896 2.3
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
4.1 2.29742338426291
4.10278574288269 2.3
4.1 2.31406090617872
4.09314636697896 2.3
4.1 2.29742338426291
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
4.4 2.56177401800098
4.44051928647572 2.6
4.7 2.83044585947817
4.77216220173296 2.9
5 3.10706906982321
5 3.2
5 3.5
5 3.63521241232135
4.90212261485594 3.5
4.7 3.2640558241322
4.65236892939843 3.2
4.4 2.90851903821906
4.39320113283587 2.9
4.26986325557845 2.6
4.4 2.56177401800098
};
\end{axis}



==> fig/tikz/ionosphere/cvi_Z_1.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{pink}{RGB}{255,192,203}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
axis background/.style={fill=pink},
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=black]
table{%
x  y
-0.7 -0.143108051704595
-0.639079799268924 -0.1
-0.4 0.0104445026156063
-0.198110480067553 0.2
-0.1 0.263260004551004
0.169283254471634 0.5
0.2 0.518332147441299
0.5 0.673030357428858
0.737108075907782 0.8
0.8 0.822996966098302
1.1 1.02614166158903
1.16448496753834 1.1
1.39847742161505 1.4
1.4 1.40211151754437
1.61406310021124 1.7
1.7 1.85352060119555
1.80277623204633 2
1.98097334829862 2.3
2 2.33456926978106
2.18480299829649 2.6
2.3 2.80807235779569
2.36281220109538 2.9
2.54474369620578 3.2
2.6 3.30655600432777
2.72549203464635 3.5
2.88433494839782 3.8
2.9 3.83155950902389
3.06714416638555 4.1
3.2 4.36727792786737
3.22041193354554 4.4
3.39793306767193 4.7
3.5 4.90967509108081
3.55544529852534 5
3.5 5
3.2 5
2.9 5
2.6 5
2.3 5
2 5
1.7 5
1.4 5
1.1 5
0.8 5
0.5 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.231564820572039
-0.7 -0.143108051704595
};
\addplot [draw=none, fill=midnightblue854116]
table{%
x  y
-0.7 -0.315047771207418
-0.4 -0.103474196634036
-0.397431681083405 -0.1
-0.1 0.173631446040884
-0.0797124373562194 0.2
0.2 0.437579967204379
0.277572033700933 0.5
0.5 0.612590940637838
0.8 0.768252701263929
0.841336631979831 0.8
1.1 0.966167914367962
1.21684743907385 1.1
1.4 1.33577384880998
1.44602803705855 1.4
1.64622114807678 1.7
1.7 1.79607237053179
1.84308437594601 2
2 2.27694110015362
2.01627073926639 2.3
2.22041426343845 2.6
2.3 2.74375019842867
2.40676216339368 2.9
2.57710514127498 3.2
2.6 3.24415034118954
2.76597617380744 3.5
2.9 3.7611485337458
2.92494940247489 3.8
3.10586527342775 4.1
3.2 4.28937922388571
3.26900491880981 4.4
3.43565036020977 4.7
3.5 4.83219282951176
3.60300722994071 5
3.55544529852534 5
3.5 4.90967509108081
3.39793306767193 4.7
3.22041193354554 4.4
3.2 4.36727792786737
3.06714416638555 4.1
2.9 3.83155950902389
2.88433494839782 3.8
2.72549203464635 3.5
2.6 3.30655600432777
2.54474369620578 3.2
2.36281220109538 2.9
2.3 2.80807235779569
2.18480299829649 2.6
2 2.33456926978106
1.98097334829862 2.3
1.80277623204633 2
1.7 1.85352060119555
1.61406310021124 1.7
1.4 1.40211151754437
1.39847742161505 1.4
1.16448496753834 1.1
1.1 1.02614166158903
0.8 0.822996966098302
0.737108075907782 0.8
0.5 0.673030357428858
0.2 0.518332147441299
0.169283254471634 0.5
-0.1 0.263260004551004
-0.198110480067553 0.2
-0.4 0.0104445026156063
-0.639079799268924 -0.1
-0.7 -0.143108051704595
-1 -0.231564820572039
-1 -0.384851863219847
-0.7 -0.315047771207418
};
\addplot [draw=none, fill=midnightblue868137]
table{%
x  y
-0.7 -0.561672510092
-0.527055567525559 -0.4
-0.4 -0.31965149653175
-0.237621426468989 -0.1
-0.1 0.0266090747083495
0.0334043294210058 0.2
0.2 0.341501730586772
0.396972551051352 0.5
0.5 0.552151523846818
0.8 0.696552457134422
0.934694074106961 0.8
1.1 0.906194167146889
1.26920991060935 1.1
1.4 1.26836719402612
1.49433540013258 1.4
1.67837919594232 1.7
1.7 1.73862413986803
1.8833925198457 2
2 2.20580107325045
2.06646831316874 2.3
2.25602552858042 2.6
2.3 2.67942803906165
2.45071212569198 2.9
2.6 3.1762128028749
2.61592415730647 3.2
2.80646031296853 3.5
2.9 3.68226424964328
2.97560684073322 3.8
3.14458638046994 4.1
3.2 4.21148051990405
3.31759790407408 4.4
3.47336765274762 4.7
3.5 4.75471056794271
3.65056916135609 5
3.60300722994071 5
3.5 4.83219282951176
3.43565036020977 4.7
3.26900491880981 4.4
3.2 4.28937922388571
3.10586527342775 4.1
2.92494940247489 3.8
2.9 3.7611485337458
2.76597617380744 3.5
2.6 3.24415034118954
2.57710514127498 3.2
2.40676216339368 2.9
2.3 2.74375019842867
2.22041426343845 2.6
2.01627073926639 2.3
2 2.27694110015362
1.84308437594601 2
1.7 1.79607237053179
1.64622114807678 1.7
1.44602803705855 1.4
1.4 1.33577384880998
1.21684743907385 1.1
1.1 0.966167914367962
0.841336631979831 0.8
0.8 0.768252701263929
0.5 0.612590940637838
0.277572033700933 0.5
0.2 0.437579967204379
-0.0797124373562194 0.2
-0.1 0.173631446040884
-0.397431681083405 -0.1
-0.4 -0.103474196634036
-0.7 -0.315047771207418
-1 -0.384851863219847
-1 -0.4
-1 -0.64930584527524
-0.7 -0.561672510092
};
\addplot [draw=none, fill=teal882156]
table{%
x  y
-0.7 -1
-0.649139813441775 -1
-0.419597729739991 -0.7
-0.4 -0.682197470629254
-0.268024759015415 -0.4
-0.1 -0.144369088758649
-0.0805239897072255 -0.1
0.146521096198231 0.2
0.2 0.245423493969164
0.5 0.484604367494485
0.521900239871475 0.5
0.8 0.624852213004915
1.02805151623409 0.8
1.1 0.846220419925816
1.32157238214485 1.1
1.4 1.20096053924227
1.54264276320661 1.4
1.7 1.67258054502975
1.71907891648243 1.7
1.92370066374538 2
2 2.13466104634727
2.1166658870711 2.3
2.29163679372238 2.6
2.3 2.61510587969463
2.49466208799027 2.9
2.6 3.09489647139837
2.67036075390115 3.2
2.84694445212962 3.5
2.9 3.60337996554077
3.02626427899155 3.8
3.18330748751214 4.1
3.2 4.13358181592238
3.36619088933835 4.4
3.5 4.67106915962613
3.51836024974354 4.7
3.69813109277147 5
3.65056916135609 5
3.5 4.75471056794271
3.47336765274762 4.7
3.31759790407408 4.4
3.2 4.21148051990405
3.14458638046994 4.1
2.97560684073322 3.8
2.9 3.68226424964328
2.80646031296853 3.5
2.61592415730647 3.2
2.6 3.1762128028749
2.45071212569198 2.9
2.3 2.67942803906165
2.25602552858042 2.6
2.06646831316874 2.3
2 2.20580107325045
1.8833925198457 2
1.7 1.73862413986803
1.67837919594232 1.7
1.49433540013258 1.4
1.4 1.26836719402612
1.26920991060935 1.1
1.1 0.906194167146889
0.934694074106961 0.8
0.8 0.696552457134422
0.5 0.552151523846818
0.396972551051352 0.5
0.2 0.341501730586772
0.0334043294210058 0.2
-0.1 0.0266090747083495
-0.237621426468989 -0.1
-0.4 -0.31965149653175
-0.527055567525559 -0.4
-0.7 -0.561672510092
-1 -0.64930584527524
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.4 -1
-0.140998707952808 -1
-0.131453393279904 -0.7
-0.1 -0.592028529291196
-0.0657907750454092 -0.4
0.0597477787413893 -0.1
0.2 0.0964254007385054
0.276699566448813 0.2
0.5 0.372331796404725
0.681607626818533 0.5
0.8 0.553151968875409
1.1 0.776799790737491
1.11939384834134 0.8
1.37393485368036 1.1
1.4 1.13355388445841
1.59095012628065 1.4
1.7 1.58890058455256
1.77730483595928 1.7
1.96400880764507 2
2 2.0635210194441
2.16686346097346 2.3
2.3 2.53283033362676
2.34688317400441 2.6
2.53861205028857 2.9
2.6 3.01358013992183
2.72479735049584 3.2
2.88742859129072 3.5
2.9 3.52449568143825
3.07692171724988 3.8
3.2 4.04308157633809
3.23669330807297 4.1
3.41478387460262 4.4
3.5 4.57262997552141
3.5808322685773 4.7
3.74569302418684 5
3.69813109277147 5
3.51836024974354 4.7
3.5 4.67106915962613
3.36619088933835 4.4
3.2 4.13358181592238
3.18330748751214 4.1
3.02626427899155 3.8
2.9 3.60337996554077
2.84694445212962 3.5
2.67036075390115 3.2
2.6 3.09489647139837
2.49466208799027 2.9
2.3 2.61510587969463
2.29163679372238 2.6
2.1166658870711 2.3
2 2.13466104634727
1.92370066374538 2
1.71907891648243 1.7
1.7 1.67258054502975
1.54264276320661 1.4
1.4 1.20096053924227
1.32157238214485 1.1
1.1 0.846220419925816
1.02805151623409 0.8
0.8 0.624852213004915
0.521900239871475 0.5
0.5 0.484604367494485
0.2 0.245423493969164
0.146521096198231 0.2
-0.0805239897072255 -0.1
-0.1 -0.144369088758649
-0.268024759015415 -0.4
-0.4 -0.682197470629254
-0.419597729739991 -0.7
-0.649139813441775 -1
-0.4 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.1 -1
0.139160076386304 -1
0.0866127820678382 -0.7
0.105212188126611 -0.4
0.2 -0.100075401031482
0.200023423716574 -0.1
0.422177733120803 0.2
0.5 0.260059225314964
0.8 0.46560588762562
0.838906516266475 0.5
1.1 0.675631291223516
1.20396405692413 0.8
1.4 1.04657726010546
1.43670340451282 1.1
1.63925748935468 1.4
1.7 1.50522062407537
1.83553075543614 1.7
2 1.98904088924184
2.00771412087261 2
2.21706103487581 2.3
2.3 2.44504438121734
2.40815613104255 2.6
2.58256201258686 2.9
2.6 2.9322638084453
2.77923394709053 3.2
2.9 3.4288700541686
2.94718420739849 3.5
3.12757915550821 3.8
3.2 3.94303232581284
3.30119154494965 4.1
3.4633768598669 4.4
3.5 4.47419079141669
3.64330428741107 4.7
3.79325495560222 5
3.74569302418684 5
3.5808322685773 4.7
3.5 4.57262997552141
3.41478387460262 4.4
3.23669330807297 4.1
3.2 4.04308157633809
3.07692171724988 3.8
2.9 3.52449568143825
2.88742859129072 3.5
2.72479735049584 3.2
2.6 3.01358013992183
2.53861205028857 2.9
2.34688317400441 2.6
2.3 2.53283033362676
2.16686346097346 2.3
2 2.0635210194441
1.96400880764507 2
1.77730483595928 1.7
1.7 1.58890058455256
1.59095012628065 1.4
1.4 1.13355388445841
1.37393485368036 1.1
1.11939384834134 0.8
1.1 0.776799790737491
0.8 0.553151968875409
0.681607626818533 0.5
0.5 0.372331796404725
0.276699566448813 0.2
0.2 0.0964254007385055
0.0597477787413893 -0.1
-0.0657907750454092 -0.4
-0.1 -0.592028529291197
-0.131453393279904 -0.7
-0.140998707952808 -1
-0.1 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.42823519455197
4.79347674085844 0.2
4.7 0.0971011461777639
4.52077962953888 -0.1
4.4 -0.231887177698999
4.24575565579729 -0.4
4.1 -0.556819085168929
3.96641995550988 -0.7
3.8 -0.874246729190063
3.67897859125494 -1
3.8 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
0.2 -1
0.392471285668093 -1
0.298611296768336 -0.7
0.284380769631626 -0.4
0.368113371521897 -0.1
0.5 0.0883571456244582
0.595377931441404 0.2
0.8 0.332651948778081
0.989303611215696 0.5
1.1 0.57446279170954
1.28853426550693 0.8
1.4 0.940203449304739
1.50978615944257 1.1
1.68756485242871 1.4
1.7 1.42154066359819
1.893756674913 1.7
2 1.88671372414089
2.07974223862414 2
2.26725860877817 2.3
2.3 2.35725842880792
2.46942908808068 2.6
2.6 2.83381277039305
2.64558056231281 2.9
2.83367054368521 3.2
2.9 3.32570441687879
3.01561936181035 3.5
3.17823659376654 3.8
3.2 3.84298307528758
3.36568978182633 4.1
3.5 4.36826635572959
3.52089011027465 4.4
3.70577630624483 4.7
3.8 4.89120561938821
3.87143335658595 5
3.8 5
3.79325495560222 5
3.64330428741107 4.7
3.5 4.47419079141669
3.4633768598669 4.4
3.30119154494965 4.1
3.2 3.94303232581284
3.12757915550821 3.8
2.94718420739849 3.5
2.9 3.4288700541686
2.77923394709053 3.2
2.6 2.9322638084453
2.58256201258686 2.9
2.40815613104255 2.6
2.3 2.44504438121734
2.21706103487581 2.3
2.00771412087261 2
2 1.98904088924184
1.83553075543614 1.7
1.7 1.50522062407537
1.63925748935468 1.4
1.43670340451282 1.1
1.4 1.04657726010546
1.20396405692413 0.8
1.1 0.675631291223516
0.838906516266475 0.5
0.8 0.46560588762562
0.5 0.260059225314964
0.422177733120803 0.2
0.200023423716574 -0.1
0.2 -0.100075401031482
0.105212188126611 -0.4
0.0866127820678382 -0.7
0.139160076386304 -1
0.2 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
3.2 -1
3.5 -1
3.67897859125494 -1
3.8 -0.874246729190063
3.96641995550988 -0.7
4.1 -0.556819085168929
4.24575565579729 -0.4
4.4 -0.231887177698999
4.52077962953888 -0.1
4.7 0.0971011461777639
4.79347674085844 0.2
5 0.42823519455197
5 0.5
5 0.8
5 1.09534673866786
4.71679160220002 0.8
4.7 0.78247799199656
4.42839874318774 0.5
4.4 0.470425851710325
4.13865204965182 0.2
4.1 0.159898576653119
3.84642199492435 -0.1
3.8 -0.14783274302415
3.54969072812311 -0.4
3.5 -0.450562065142332
3.24484824799023 -0.7
3.2 -0.744595239575609
2.92517351135883 -1
3.2 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
0.5 -1
0.675412426084248 -1
0.516855668493644 -0.7
0.5 -0.610493449019668
0.473704826540016 -0.4
0.5 -0.282386647441525
0.551924433149644 -0.1
0.8 0.199339251409744
0.800514039814682 0.2
1.1 0.450109504539973
1.13574385653145 0.5
1.37310447408972 0.8
1.4 0.833829638504022
1.58286891437232 1.1
1.7 1.30501227668172
1.76342693379741 1.4
1.95198259438985 1.7
2 1.78438655903994
2.15177035637566 2
2.3 2.25663413842665
2.33057065051526 2.3
2.53070204511882 2.6
2.6 2.72409154975768
2.7211412854902 2.9
2.8881071402799 3.2
2.9 3.22253877958899
3.08405451622221 3.5
3.2 3.72444017554782
3.25048854540047 3.8
3.43018801870301 4.1
3.5 4.2394399180008
3.60569595442897 4.4
3.76824832507859 4.7
3.8 4.76443282393212
3.95467116953446 5
3.87143335658595 5
3.8 4.89120561938821
3.70577630624483 4.7
3.52089011027465 4.4
3.5 4.36826635572959
3.36568978182633 4.1
3.2 3.84298307528758
3.17823659376654 3.8
3.01561936181035 3.5
2.9 3.32570441687879
2.83367054368522 3.2
2.64558056231281 2.9
2.6 2.83381277039305
2.46942908808068 2.6
2.3 2.35725842880792
2.26725860877817 2.3
2.07974223862414 2
2 1.88671372414089
1.893756674913 1.7
1.7 1.42154066359819
1.68756485242871 1.4
1.50978615944257 1.1
1.4 0.940203449304739
1.28853426550693 0.8
1.1 0.57446279170954
0.989303611215696 0.5
0.8 0.332651948778081
0.595377931441404 0.2
0.5 0.0883571456244583
0.368113371521897 -0.1
0.284380769631626 -0.4
0.298611296768336 -0.7
0.392471285668093 -1
0.5 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
2.6 -1
2.9 -1
2.92517351135883 -1
3.2 -0.744595239575609
3.24484824799023 -0.7
3.5 -0.450562065142332
3.54969072812311 -0.4
3.8 -0.14783274302415
3.84642199492435 -0.1
4.1 0.159898576653119
4.13865204965182 0.2
4.4 0.470425851710325
4.42839874318774 0.5
4.7 0.78247799199656
4.71679160220002 0.8
5 1.09534673866786
5 1.1
5 1.4
5 1.47633254778675
4.92578471682232 1.4
4.7 1.16811996891551
4.63368673784062 1.1
4.4 0.860468460713345
4.34094470803994 0.8
4.1 0.553987798688955
4.04687713979121 0.5
3.8 0.249840011671075
3.75017327653796 0.2
3.5 -0.0499045364879898
3.44834169503598 -0.1
3.2 -0.341818284428371
3.13655623959673 -0.4
2.9 -0.620590696759601
2.80496438090744 -0.7
2.6 -0.878241208084895
2.43187026274449 -1
2.6 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.8 -1
1.1 -1
1.12212189738183 -1
1.1 -0.992423034446277
0.803749657992207 -0.7
0.8 -0.691357459687112
0.729022608824551 -0.4
0.793006616224012 -0.1
0.8 -0.0915614653595127
1.02682485264756 0.2
1.1 0.261110710624412
1.2711513266727 0.5
1.4 0.674755050709316
1.476096066888 0.8
1.65595166930208 1.1
1.7 1.1770969423874
1.84884089211257 1.4
2 1.67295812944776
2.01855050515993 1.7
2.22379847412718 2
2.3 2.13192983846556
2.41848062009844 2.3
2.59197500215696 2.6
2.6 2.6143703291223
2.79670200866758 2.9
2.9 3.09087920591381
2.97486831918092 3.2
3.15248967063407 3.5
3.2 3.59196758955838
3.33900579938481 3.8
3.49468625557969 4.1
3.5 4.11061348027201
3.6905017985833 4.4
3.8 4.61725674562546
3.85670919624636 4.7
4.03790898248297 5
3.95467116953446 5
3.8 4.76443282393212
3.76824832507859 4.7
3.60569595442897 4.4
3.5 4.2394399180008
3.43018801870301 4.1
3.25048854540047 3.8
3.2 3.72444017554782
3.08405451622221 3.5
2.9 3.22253877958899
2.8881071402799 3.2
2.7211412854902 2.9
2.6 2.72409154975768
2.53070204511882 2.6
2.33057065051526 2.3
2.3 2.25663413842665
2.15177035637566 2
2 1.78438655903994
1.95198259438985 1.7
1.76342693379741 1.4
1.7 1.30501227668172
1.58286891437232 1.1
1.4 0.833829638504022
1.37310447408972 0.8
1.13574385653145 0.5
1.1 0.450109504539973
0.800514039814682 0.2
0.8 0.199339251409744
0.551924433149644 -0.1
0.5 -0.282386647441525
0.473704826540016 -0.4
0.5 -0.610493449019668
0.516855668493644 -0.7
0.675412426084248 -1
0.8 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
2 -1
2.3 -1
2.43187026274449 -1
2.6 -0.878241208084895
2.80496438090744 -0.7
2.9 -0.620590696759601
3.13655623959673 -0.4
3.2 -0.341818284428371
3.44834169503598 -0.1
3.5 -0.0499045364879898
3.75017327653796 0.2
3.8 0.249840011671075
4.04687713979121 0.5
4.1 0.553987798688955
4.34094470803994 0.8
4.4 0.860468460713345
4.63368673784062 1.1
4.7 1.16811996891551
4.92578471682232 1.4
5 1.47633254778675
5 1.7
5 1.79995960737287
4.90291784565926 1.7
4.7 1.49168819242044
4.61098594977347 1.4
4.4 1.18367463976807
4.31868330679825 1.1
4.1 0.876477872937585
4.02531725108214 0.8
3.8 0.571311017315045
3.72943627301572 0.5
3.5 0.270507901985844
3.428161245684 0.2
3.2 -0.0219120831243947
3.11578693068864 -0.1
2.9 -0.299683191732182
2.78037721638682 -0.4
2.6 -0.553709183466978
2.39460776515619 -0.7
2.3 -0.770891065946207
2 -0.939246324603768
1.82313677857434 -1
2 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
1.1 -0.992423034446277
1.12212189738183 -1
1.4 -1
1.7 -1
1.82313677857434 -1
2 -0.939246324603768
2.3 -0.770891065946207
2.39460776515619 -0.7
2.6 -0.553709183466978
2.78037721638682 -0.4
2.9 -0.299683191732182
3.11578693068864 -0.1
3.2 -0.0219120831243947
3.428161245684 0.2
3.5 0.270507901985844
3.72943627301572 0.5
3.8 0.571311017315045
4.02531725108214 0.8
4.1 0.876477872937585
4.31868330679825 1.1
4.4 1.18367463976807
4.61098594977347 1.4
4.7 1.49168819242044
4.90291784565926 1.7
5 1.79995960737287
5 2
5 2.11180843251395
4.89197502527348 2
4.7 1.80221218329437
4.6015241646703 1.7
4.4 1.49231673752609
4.31124582323596 1.4
4.1 1.18255877503405
4.02052351310262 1.1
3.8 0.874155459117952
3.72790030551529 0.8
3.5 0.569697948224116
3.43037353499925 0.5
3.2 0.273834654775865
3.12190355416508 0.2
2.9 -0.00612488283192081
2.78954025703241 -0.1
2.6 -0.259810380790265
2.40162993792741 -0.4
2.3 -0.473145048028228
2 -0.626841392724243
1.72079726792005 -0.7
1.7 -0.705971472670489
1.61574841756031 -0.7
1.4 -0.677191920166118
1.1 -0.407277500676471
1.09623720127046 -0.4
1.1 -0.306127173367352
1.10703059182877 -0.1
1.24569523283708 0.2
1.4 0.481006996897587
1.4083938573814 0.5
1.58767813289761 0.8
1.7 1.0151054505999
1.75090233569733 1.1
1.93425485042774 1.4
2 1.51872042180133
2.12435632898501 1.7
2.2958265918787 2
2.3 2.00722553850447
2.50639058968162 2.3
2.6 2.46518754001415
2.69483010570656 2.6
2.87226273184497 2.9
2.9 2.9512543143517
3.07066565125328 3.2
3.2 3.44460324433895
3.238544519783 3.5
3.42752305336916 3.8
3.5 3.94146293859685
3.60886727466117 4.1
3.77530764273762 4.4
3.8 4.44899241367656
3.97203140702814 4.7
4.1 4.94411157816079
4.14075516017102 5
4.1 5
4.03790898248297 5
3.85670919624636 4.7
3.8 4.61725674562546
3.6905017985833 4.4
3.5 4.11061348027201
3.49468625557969 4.1
3.33900579938481 3.8
3.2 3.59196758955838
3.15248967063407 3.5
2.97486831918092 3.2
2.9 3.09087920591381
2.79670200866758 2.9
2.6 2.6143703291223
2.59197500215696 2.6
2.41848062009844 2.3
2.3 2.13192983846556
2.22379847412718 2
2.01855050515993 1.7
2 1.67295812944776
1.84884089211257 1.4
1.7 1.1770969423874
1.65595166930208 1.1
1.476096066888 0.8
1.4 0.674755050709316
1.2711513266727 0.5
1.1 0.261110710624412
1.02682485264756 0.2
0.8 -0.0915614653595127
0.793006616224012 -0.1
0.729022608824551 -0.4
0.8 -0.691357459687112
0.803749657992207 -0.7
1.1 -0.992423034446277
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.7 -0.705971472670489
1.72079726792005 -0.7
2 -0.626841392724243
2.3 -0.473145048028228
2.40162993792741 -0.4
2.6 -0.259810380790265
2.78954025703241 -0.1
2.9 -0.00612488283192081
3.12190355416508 0.2
3.2 0.273834654775866
3.43037353499925 0.5
3.5 0.569697948224116
3.72790030551529 0.8
3.8 0.874155459117952
4.02052351310262 1.1
4.1 1.18255877503405
4.31124582323596 1.4
4.4 1.49231673752609
4.6015241646703 1.7
4.7 1.80221218329437
4.89197502527348 2
5 2.11180843251395
5 2.3
5 2.44278124016346
4.86342072581702 2.3
4.7 2.13028166489413
4.57615776478022 2
4.4 1.81652793970842
4.28991568989047 1.7
4.1 1.5018006403214
4.00408037963623 1.4
3.8 1.18738852983548
3.71706199420987 1.1
3.5 0.876320349530265
3.4256157835466 0.8
3.2 0.574138264577999
3.12329610659517 0.5
2.9 0.28956719280777
2.79605236890509 0.2
2.6 0.0348636234897159
2.40709934651543 -0.1
2.3 -0.174162788563357
2 -0.306573411561038
1.7 -0.320988349741622
1.47226562812242 -0.1
1.47909859526614 0.2
1.581686463477 0.5
1.69926019890722 0.8
1.7 0.801416778865258
1.87902896550122 1.1
2 1.34117744257085
2.03729311043469 1.4
2.23016215281009 1.7
2.3 1.82359723044587
2.42348608820069 2
2.59430055926479 2.3
2.6 2.3100574994683
2.80395205292694 2.6
2.9 2.77451335114315
2.98888934303585 2.9
3.16646298332565 3.2
3.2 3.26342679391429
3.36460531872827 3.5
3.5 3.75669136776093
3.53127034965912 3.8
3.72750894881915 4.1
3.8 4.23888184416985
3.91639444166609 4.4
4.08735361780993 4.7
4.1 4.72412410922671
4.30117522996329 5
4.14075516017102 5
4.1 4.94411157816079
3.97203140702814 4.7
3.8 4.44899241367656
3.77530764273762 4.4
3.60886727466117 4.1
3.5 3.94146293859685
3.42752305336916 3.8
3.238544519783 3.5
3.2 3.44460324433895
3.07066565125328 3.2
2.9 2.9512543143517
2.87226273184497 2.9
2.69483010570656 2.6
2.6 2.46518754001415
2.50639058968162 2.3
2.3 2.00722553850447
2.2958265918787 2
2.12435632898501 1.7
2 1.51872042180133
1.93425485042774 1.4
1.75090233569733 1.1
1.7 1.0151054505999
1.58767813289761 0.8
1.4083938573814 0.5
1.4 0.481006996897587
1.24569523283708 0.2
1.10703059182877 -0.1
1.1 -0.306127173367352
1.09623720127046 -0.4
1.1 -0.407277500676471
1.4 -0.677191920166118
1.61574841756031 -0.7
1.7 -0.705971472670489
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.7 -0.320988349741622
2 -0.306573411561038
2.3 -0.174162788563357
2.40709934651543 -0.1
2.6 0.0348636234897159
2.79605236890509 0.2
2.9 0.28956719280777
3.12329610659517 0.5
3.2 0.574138264577999
3.4256157835466 0.8
3.5 0.876320349530265
3.71706199420987 1.1
3.8 1.18738852983548
4.00408037963623 1.4
4.1 1.5018006403214
4.28991568989047 1.7
4.4 1.81652793970842
4.57615776478022 2
4.7 2.13028166489413
4.86342072581702 2.3
5 2.44278124016346
5 2.6
5 2.82979590006601
4.78387789312603 2.6
4.7 2.51165277457201
4.5031443052399 2.3
4.4 2.19060672322507
4.22466696923754 2
4.1 1.86689883734278
3.94737906616986 1.7
3.8 1.54225235752643
3.66898601917386 1.4
3.5 1.2206528803186
3.38542790318278 1.1
3.2 0.909058282855618
3.08908016866812 0.8
2.9 0.618162833314826
2.76281370007048 0.5
2.6 0.363027349398987
2.35677038232348 0.2
2.3 0.162817616849908
2 0.0879115277404764
1.83892143324013 0.2
1.80659334401027 0.5
1.89859077867616 0.8
2 1.07024656030547
2.01492377429526 1.1
2.19924253105024 1.4
2.3 1.59399929790346
2.37076512746283 1.7
2.55456719590956 2
2.6 2.08112248918462
2.75543112200708 2.3
2.9 2.56367988327449
2.92640198534381 2.6
3.12933388096002 2.9
3.2 3.03090891032322
3.32287946386448 3.2
3.49066611767354 3.5
3.5 3.51769587252907
3.70383346967638 3.8
3.8 3.97667695416542
3.89493450889978 4.1
4.08059933795013 4.4
4.1 4.43514641599351
4.30628862824788 4.7
4.4 4.8538991350488
4.52534036194298 5
4.4 5
4.30117522996329 5
4.1 4.72412410922671
4.08735361780993 4.7
3.91639444166609 4.4
3.8 4.23888184416985
3.72750894881915 4.1
3.53127034965912 3.8
3.5 3.75669136776093
3.36460531872827 3.5
3.2 3.26342679391429
3.16646298332564 3.2
2.98888934303585 2.9
2.9 2.77451335114315
2.80395205292694 2.6
2.6 2.3100574994683
2.59430055926479 2.3
2.42348608820069 2
2.3 1.82359723044587
2.23016215281009 1.7
2.03729311043469 1.4
2 1.34117744257085
1.87902896550122 1.1
1.7 0.801416778865258
1.69926019890722 0.8
1.581686463477 0.5
1.47909859526614 0.2
1.47226562812242 -0.1
1.7 -0.320988349741622
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
2 0.0879115277404764
2.3 0.162817616849908
2.35677038232348 0.2
2.6 0.363027349398987
2.76281370007048 0.5
2.9 0.618162833314826
3.08908016866812 0.8
3.2 0.909058282855618
3.38542790318278 1.1
3.5 1.2206528803186
3.66898601917386 1.4
3.8 1.54225235752643
3.94737906616986 1.7
4.1 1.86689883734278
4.22466696923754 2
4.4 2.19060672322507
4.5031443052399 2.3
4.7 2.51165277457201
4.78387789312603 2.6
5 2.82979590006601
5 2.9
5 3.2
5 3.39613801302053
4.82987952083014 3.2
4.7 3.05329823914389
4.57032541861749 2.9
4.4 2.70334087422841
4.31407676018073 2.6
4.1 2.34777692619528
4.06018951149549 2.3
3.80615834962873 2
3.8 1.99313233104834
3.53902700727141 1.7
3.5 1.65682551361885
3.2610362257439 1.4
3.2 1.33488843335737
2.9603694016543 1.1
2.9 1.04093175195052
2.60665808044346 0.8
2.6 0.794550043229876
2.3 0.726213138882332
2.25635088348389 0.8
2.28214583240162 1.1
2.3 1.14507756555666
2.44199740503213 1.4
2.5789325950198 1.7
2.6 1.74023469127794
2.78099712730463 2
2.9 2.23023064876256
2.95119095686011 2.3
3.14676576220901 2.6
3.2 2.69814589624037
3.35358128447781 2.9
3.5 3.16468476426641
3.52918097057887 3.2
3.74662470951493 3.5
3.8 3.59348178522237
3.97261366921727 3.8
4.1 4.00148404726132
4.19314823547687 4.1
4.4 4.37861280850701
4.42333107033599 4.4
4.69795384957641 4.7
4.7 4.70261582613103
5 4.97631389974387
5 5
4.7 5
4.52534036194298 5
4.4 4.8538991350488
4.30628862824788 4.7
4.1 4.43514641599351
4.08059933795013 4.4
3.89493450889978 4.1
3.8 3.97667695416542
3.70383346967638 3.8
3.5 3.51769587252907
3.49066611767354 3.5
3.32287946386448 3.2
3.2 3.03090891032322
3.12933388096002 2.9
2.92640198534381 2.6
2.9 2.56367988327449
2.75543112200709 2.3
2.6 2.08112248918462
2.55456719590956 2
2.37076512746283 1.7
2.3 1.59399929790346
2.19924253105024 1.4
2.01492377429526 1.1
2 1.07024656030547
1.89859077867616 0.8
1.80659334401027 0.5
1.83892143324013 0.2
2 0.0879115277404764
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
2.3 0.726213138882332
2.6 0.794550043229876
2.60665808044346 0.8
2.9 1.04093175195052
2.9603694016543 1.1
3.2 1.33488843335737
3.2610362257439 1.4
3.5 1.65682551361885
3.53902700727141 1.7
3.8 1.99313233104834
3.80615834962873 2
4.06018951149549 2.3
4.1 2.34777692619528
4.31407676018073 2.6
4.4 2.70334087422841
4.57032541861749 2.9
4.7 3.05329823914389
4.82987952083014 3.2
5 3.39613801302053
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 4.97631389974387
4.7 4.70261582613103
4.69795384957641 4.7
4.42333107033599 4.4
4.4 4.37861280850701
4.19314823547687 4.1
4.1 4.00148404726132
3.97261366921727 3.8
3.8 3.59348178522237
3.74662470951493 3.5
3.52918097057887 3.2
3.5 3.16468476426641
3.35358128447781 2.9
3.2 2.69814589624037
3.14676576220901 2.6
2.95119095686011 2.3
2.9 2.23023064876256
2.78099712730463 2
2.6 1.74023469127794
2.5789325950198 1.7
2.44199740503213 1.4
2.3 1.14507756555666
2.28214583240162 1.1
2.25635088348389 0.8
2.3 0.726213138882332
};
\end{axis}



==> fig/tikz/ionosphere/cvi_Z_2.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{pink}{RGB}{255,192,203}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
axis background/.style={fill=pink},
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=black]
table{%
x  y
-0.7 0.149587686592467
-0.638105876024053 0.2
-0.4 0.325303915962609
-0.211231190208758 0.5
-0.1 0.571350012872375
0.190638350607604 0.8
0.2 0.805054035713951
0.5 0.94163864436891
0.762304165085369 1.1
0.8 1.11718609594725
1.09501984543751 1.4
1.1 1.40519993789155
1.31010714335863 1.7
1.4 1.88753145879692
1.46649836776572 2
1.61241436062542 2.3
1.7 2.56735271471361
1.71748107300304 2.6
1.86237878563504 2.9
1.96809674584288 3.2
2 3.30618864385518
2.09356993680697 3.5
2.21352697168406 3.8
2.3 4.07039852324278
2.31390409072888 4.1
2.44590503804833 4.4
2.55630011596609 4.7
2.6 4.83596526129323
2.67376040364843 5
2.6 5
2.3 5
2 5
1.7 5
1.4 5
1.1 5
0.8 5
0.5 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 0.0268005416815821
-0.7 0.149587686592467
};
\addplot [draw=none, fill=midnightblue854116]
table{%
x  y
-0.976321954986477 -0.1
-0.7 -0.00245563781399598
-0.451433459417152 0.2
-0.4 0.227067008946146
-0.105080762640492 0.5
-0.1 0.503259090180733
0.2 0.725601231973949
0.306708976085226 0.8
0.5 0.887484228759184
0.8 1.06037412172893
0.841709664028243 1.1
1.1 1.34076627054214
1.14375179472605 1.4
1.34185341815469 1.7
1.4 1.82130344640185
1.50565647080083 2
1.64069696421516 2.3
1.7 2.48102085822573
1.7637076879425 2.6
1.89912509558497 2.9
1.99814857307554 3.2
2 3.20616239689334
2.14186148067432 3.5
2.25469301921667 3.8
2.3 3.94167354763663
2.37436741675078 4.1
2.49912785452928 4.4
2.6 4.68796369457835
2.60580460525211 4.7
2.74015901916464 5
2.67376040364843 5
2.6 4.83596526129323
2.55630011596609 4.7
2.44590503804833 4.4
2.31390409072888 4.1
2.3 4.07039852324278
2.21352697168406 3.8
2.09356993680697 3.5
2 3.30618864385518
1.96809674584288 3.2
1.86237878563504 2.9
1.71748107300304 2.6
1.7 2.56735271471361
1.61241436062542 2.3
1.46649836776572 2
1.4 1.88753145879692
1.31010714335863 1.7
1.1 1.40519993789155
1.09501984543751 1.4
0.8 1.11718609594725
0.762304165085369 1.1
0.5 0.94163864436891
0.2 0.805054035713951
0.190638350607604 0.8
-0.1 0.571350012872375
-0.211231190208758 0.5
-0.4 0.325303915962609
-0.638105876024053 0.2
-0.7 0.149587686592467
-1 0.0268005416815821
-1 -0.1
-1 -0.113635025487589
-0.976321954986477 -0.1
};
\addplot [draw=none, fill=midnightblue868137]
table{%
x  y
-0.7 -0.206255222501128
-0.610959554160728 -0.1
-0.4 0.0618927778795594
-0.298472603786578 0.2
-0.1 0.379394150254796
0.00752632915171929 0.5
0.2 0.642179234561339
0.426359827343502 0.8
0.5 0.833329813149458
0.8 0.992024660466224
0.913653383389549 1.1
1.1 1.27370367242215
1.19328622474753 1.4
1.37359969295075 1.7
1.4 1.75507543400679
1.54481457383595 2
1.6689795678049 2.3
1.7 2.39468900173785
1.80993430288197 2.6
1.93587140553489 2.9
2 3.09509557282292
2.05378096132746 3.2
2.19015302454167 3.5
2.29585906674928 3.8
2.3 3.81294857203048
2.43483074277267 4.1
2.55235067101024 4.4
2.6 4.53602641994022
2.6790775799283 4.7
2.80655763468084 5
2.74015901916464 5
2.60580460525211 4.7
2.6 4.68796369457835
2.49912785452928 4.4
2.37436741675078 4.1
2.3 3.94167354763663
2.25469301921667 3.8
2.14186148067432 3.5
2 3.20616239689334
1.99814857307554 3.2
1.89912509558497 2.9
1.7637076879425 2.6
1.7 2.48102085822573
1.64069696421516 2.3
1.50565647080083 2
1.4 1.82130344640185
1.34185341815469 1.7
1.14375179472605 1.4
1.1 1.34076627054214
0.841709664028243 1.1
0.8 1.06037412172893
0.5 0.887484228759184
0.306708976085226 0.8
0.2 0.725601231973949
-0.1 0.503259090180733
-0.105080762640492 0.5
-0.4 0.227067008946146
-0.451433459417152 0.2
-0.7 -0.00245563781399598
-0.976321954986477 -0.1
-1 -0.113635025487589
-1 -0.361657301531692
-0.7 -0.206255222501128
};
\addplot [draw=none, fill=teal882156]
table{%
x  y
-0.821615652949895 -0.7
-0.7 -0.613962183026814
-0.585531195547181 -0.4
-0.4 -0.163500146742961
-0.373163179237936 -0.1
-0.158332774281871 0.2
-0.1 0.252725455678275
0.12045799685298 0.5
0.2 0.558757237148729
0.5 0.762622511360658
0.552580952966625 0.8
0.8 0.923675199203517
0.985597102750855 1.1
1.1 1.20664107430216
1.24282065476901 1.4
1.4 1.68488147352238
1.40933206870046 1.7
1.58397267687107 2
1.69726217139464 2.3
1.7 2.30835714524996
1.85616091782143 2.6
1.97261771548482 2.9
2 2.98330390720781
2.1110927774916 3.2
2.23844456840902 3.5
2.3 3.6758906167434
2.36224497145959 3.8
2.49529406879456 4.1
2.6 4.38289306412794
2.60863878451022 4.4
2.75235055460449 4.7
2.87295625019704 5
2.80655763468084 5
2.6790775799283 4.7
2.6 4.53602641994022
2.55235067101024 4.4
2.43483074277267 4.1
2.3 3.81294857203048
2.29585906674928 3.8
2.19015302454167 3.5
2.05378096132746 3.2
2 3.09509557282292
1.93587140553489 2.9
1.80993430288197 2.6
1.7 2.39468900173785
1.6689795678049 2.3
1.54481457383595 2
1.4 1.75507543400679
1.37359969295075 1.7
1.19328622474753 1.4
1.1 1.27370367242215
0.913653383389549 1.1
0.8 0.992024660466224
0.5 0.833329813149458
0.426359827343502 0.8
0.2 0.642179234561339
0.00752632915171929 0.5
-0.1 0.379394150254796
-0.298472603786578 0.2
-0.4 0.0618927778795594
-0.610959554160728 -0.1
-0.7 -0.206255222501128
-1 -0.361657301531692
-1 -0.4
-1 -0.7
-1 -0.88264584737124
-0.821615652949895 -0.7
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 -1
-0.4 -1
-0.328678087919341 -1
-0.343038936823249 -0.7
-0.301779177685628 -0.4
-0.195147632461982 -0.1
-0.1 0.0433919827344686
-0.0186028091711405 0.2
0.2 0.452399703490239
0.244404133089037 0.5
0.5 0.665422285902104
0.689317814356559 0.8
0.8 0.855325737940809
1.05754082211216 1.1
1.1 1.13957847618216
1.29235508479049 1.4
1.4 1.59510223825535
1.46474924130828 1.7
1.62313077990618 2
1.7 2.20546543398474
1.75359960412878 2.3
1.9023875327609 2.6
2 2.86769459065665
2.01759045059568 2.9
2.16840459365575 3.2
2.28673611227637 3.5
2.3 3.53790069100038
2.43145149528725 3.8
2.55575739481646 4.1
2.6 4.21953407033665
2.69113299362658 4.4
2.82562352928068 4.7
2.9 4.88940441896669
2.95739527210191 5
2.9 5
2.87295625019704 5
2.75235055460449 4.7
2.60863878451022 4.4
2.6 4.38289306412795
2.49529406879456 4.1
2.36224497145959 3.8
2.3 3.6758906167434
2.23844456840902 3.5
2.1110927774916 3.2
2 2.98330390720781
1.97261771548482 2.9
1.85616091782143 2.6
1.7 2.30835714524996
1.69726217139464 2.3
1.58397267687107 2
1.40933206870046 1.7
1.4 1.68488147352238
1.24282065476901 1.4
1.1 1.20664107430216
0.985597102750855 1.1
0.8 0.923675199203517
0.552580952966625 0.8
0.5 0.762622511360658
0.2 0.558757237148729
0.12045799685298 0.5
-0.1 0.252725455678275
-0.158332774281871 0.2
-0.373163179237936 -0.1
-0.4 -0.163500146742961
-0.585531195547181 -0.4
-0.7 -0.613962183026814
-0.821615652949895 -0.7
-1 -0.88264584737124
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.1 -1
0.0168472440431322 -1
-0.0642309558146708 -0.7
-0.0807302436264612 -0.4
-0.0228800044743461 -0.1
0.120834900863119 0.2
0.2 0.291404349398278
0.394589313728619 0.5
0.5 0.56822206044355
0.8 0.776986586648075
0.822121325868151 0.8
1.1 1.0561429195894
1.13155307708078 1.1
1.34188951481198 1.4
1.4 1.50532300298832
1.5201664139161 1.7
1.6622888829413 2
1.7 2.10079887662525
1.81294388714041 2.3
1.94861414770036 2.6
2 2.74092169869244
2.08661889933833 2.9
2.2257164098199 3.2
2.3 3.39235485837292
2.35796761160525 3.5
2.50065801911492 3.8
2.6 4.05276084366013
2.62498991233846 4.1
2.77362720274294 4.4
2.89889650395688 4.7
2.9 4.70281012294423
3.05423124233517 5
2.95739527210191 5
2.9 4.88940441896669
2.82562352928068 4.7
2.69113299362658 4.4
2.6 4.21953407033665
2.55575739481646 4.1
2.43145149528725 3.8
2.3 3.53790069100038
2.28673611227637 3.5
2.16840459365575 3.2
2.01759045059568 2.9
2 2.86769459065665
1.9023875327609 2.6
1.75359960412878 2.3
1.7 2.20546543398474
1.62313077990618 2
1.46474924130828 1.7
1.4 1.59510223825535
1.29235508479049 1.4
1.1 1.13957847618216
1.05754082211216 1.1
0.8 0.855325737940809
0.689317814356559 0.8
0.5 0.665422285902104
0.244404133089037 0.5
0.2 0.452399703490239
-0.0186028091711405 0.2
-0.1 0.0433919827344686
-0.195147632461982 -0.1
-0.301779177685628 -0.4
-0.343038936823249 -0.7
-0.328678087919341 -1
-0.1 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.427868175880811
4.79403076155439 0.2
4.7 0.0964566321876548
4.52173453770737 -0.1
4.4 -0.23305550542443
4.24734772692115 -0.4
4.1 -0.558813310890865
3.96895586096222 -0.7
3.8 -0.87740650684667
3.68286584618631 -1
3.8 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
0.2 -1
0.29836262484583 -1
0.2 -0.784190609433404
0.167335750091515 -0.7
0.11368486202405 -0.4
0.142787953800111 -0.1
0.2 0.0332342802272498
0.276215711843166 0.2
0.5 0.442935103018024
0.556197030143712 0.5
0.8 0.656210494777689
0.93821567677951 0.8
1.1 0.949129504172849
1.20854412422079 1.1
1.39142394483346 1.4
1.4 1.41554376772128
1.57558358652393 1.7
1.7 1.99514218851835
1.70287997055929 2
1.87228817015205 2.3
1.99484076263983 2.6
2 2.61414880672824
2.15564734808098 2.9
2.28302822598404 3.2
2.3 3.24394783799843
2.43788576105934 3.5
2.56986454294259 3.8
2.6 3.87667517279252
2.71814071815264 4.1
2.8561214118593 4.4
2.9 4.50519884387567
3.00568841474515 4.7
3.15106721256844 5
3.05423124233517 5
2.9 4.70281012294423
2.89889650395688 4.7
2.77362720274294 4.4
2.62498991233846 4.1
2.6 4.05276084366013
2.50065801911492 3.8
2.35796761160525 3.5
2.3 3.39235485837292
2.2257164098199 3.2
2.08661889933833 2.9
2 2.74092169869244
1.94861414770036 2.6
1.81294388714041 2.3
1.7 2.10079887662525
1.6622888829413 2
1.5201664139161 1.7
1.4 1.50532300298832
1.34188951481198 1.4
1.13155307708078 1.1
1.1 1.0561429195894
0.822121325868151 0.8
0.8 0.776986586648075
0.5 0.56822206044355
0.394589313728619 0.5
0.2 0.291404349398278
0.120834900863119 0.2
-0.0228800044743461 -0.1
-0.0807302436264611 -0.4
-0.0642309558146708 -0.7
0.0168472440431322 -1
0.2 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
3.2 -1
3.5 -1
3.68286584618631 -1
3.8 -0.87740650684667
3.96895586096222 -0.7
4.1 -0.558813310890865
4.24734772692115 -0.4
4.4 -0.23305550542443
4.52173453770737 -0.1
4.7 0.0964566321876548
4.79403076155439 0.2
5 0.427868175880811
5 0.5
5 0.8
5 1.09489535301403
4.71763699565325 0.8
4.7 0.78157997686298
4.4299271370301 0.5
4.4 0.46878690704914
4.14126195691096 0.2
4.1 0.157085399103983
3.85069214663895 -0.1
3.8 -0.152430190518982
3.55643174638383 -0.4
3.5 -0.457735608165141
3.25515402071558 -0.7
3.2 -0.755244392602074
2.94045998112604 -1
3.2 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
0.2 -0.784190609433404
0.29836262484583 -1
0.5 -1
0.586036487256506 -1
0.5 -0.882182581550041
0.404655463418508 -0.7
0.320021240631429 -0.4
0.329074864039415 -0.1
0.452536998905648 0.2
0.5 0.251524748030211
0.744696336336559 0.5
0.8 0.535434402907304
1.05431002769087 0.8
1.1 0.8421160887563
1.2855351713608 1.1
1.4 1.29278160497128
1.46590935688437 1.4
1.63100075913175 1.7
1.7 1.86368087125318
1.78081727315729 2
1.93163245316368 2.3
2 2.46938234028007
2.07571635964678 2.6
2.22467579682363 2.9
2.3 3.08236653485918
2.36670958356833 3.2
2.51780391051344 3.5
2.6 3.69368437720151
2.65975378570037 3.8
2.81129152396682 4.1
2.9 4.30113406337014
2.9560344323954 4.4
3.11299284154531 4.7
3.2 4.88632557185811
3.26666548491238 5
3.2 5
3.15106721256844 5
3.00568841474515 4.7
2.9 4.50519884387567
2.8561214118593 4.4
2.71814071815264 4.1
2.6 3.87667517279252
2.56986454294259 3.8
2.43788576105934 3.5
2.3 3.24394783799843
2.28302822598404 3.2
2.15564734808098 2.9
2 2.61414880672824
1.99484076263983 2.6
1.87228817015205 2.3
1.70287997055929 2
1.7 1.99514218851835
1.57558358652393 1.7
1.4 1.41554376772128
1.39142394483346 1.4
1.20854412422079 1.1
1.1 0.949129504172849
0.93821567677951 0.8
0.8 0.656210494777689
0.556197030143712 0.5
0.5 0.442935103018024
0.276215711843166 0.2
0.2 0.0332342802272498
0.142787953800111 -0.1
0.11368486202405 -0.4
0.167335750091515 -0.7
0.2 -0.784190609433404
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
2.6 -1
2.9 -1
2.94045998112604 -1
3.2 -0.755244392602074
3.25515402071558 -0.7
3.5 -0.457735608165141
3.55643174638383 -0.4
3.8 -0.152430190518982
3.85069214663895 -0.1
4.1 0.157085399103983
4.14126195691096 0.2
4.4 0.46878690704914
4.4299271370301 0.5
4.7 0.78157997686298
4.71763699565325 0.8
5 1.09489535301403
5 1.1
5 1.4
5 1.47579353743648
4.92645666213449 1.4
4.7 1.16710968937187
4.6348865143515 1.1
4.4 0.858687916339615
4.342986241976 0.8
4.1 0.550992639737573
4.05022898634048 0.5
3.8 0.245008272549614
3.75553039844082 0.2
3.5 -0.0573777741055841
3.4567547148229 -0.1
3.2 -0.35288882021447
3.14970059974017 -0.4
2.9 -0.63630801633762
2.8256990302483 -0.7
2.6 -0.899686535502806
2.46514091073115 -1
2.6 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.5 -0.882182581550041
0.586036487256506 -1
0.8 -1
0.993173479193655 -1
0.8 -0.851551909266143
0.686725783867816 -0.7
0.548887656249961 -0.4
0.536077800481293 -0.1
0.672267488436933 0.2
0.8 0.33020885304621
0.924859367945439 0.5
1.1 0.686121931710753
1.17157744556655 0.8
1.36252621850081 1.1
1.4 1.16311332334694
1.54561912168613 1.4
1.68641793173957 1.7
1.7 1.73221955398801
1.85875457575529 2
1.99097673617531 2.3
2 2.32235536616883
2.16094485993882 2.6
2.29370424556628 2.9
2.3 2.91524257638298
2.46148507675722 3.2
2.59772205996754 3.5
2.6 3.50536766893956
2.76559557953165 3.8
2.9 4.08914129727101
2.90649906245991 4.1
3.07574029408945 4.4
3.2 4.65375906421404
3.22847344793801 4.7
3.40142932595578 5
3.26666548491238 5
3.2 4.88632557185811
3.11299284154531 4.7
2.9560344323954 4.4
2.9 4.30113406337014
2.81129152396682 4.1
2.65975378570037 3.8
2.6 3.69368437720151
2.51780391051344 3.5
2.36670958356833 3.2
2.3 3.08236653485918
2.22467579682363 2.9
2.07571635964678 2.6
2 2.46938234028007
1.93163245316368 2.3
1.78081727315729 2
1.7 1.86368087125318
1.63100075913175 1.7
1.46590935688437 1.4
1.4 1.29278160497128
1.2855351713608 1.1
1.1 0.8421160887563
1.05431002769087 0.8
0.8 0.535434402907304
0.744696336336559 0.5
0.5 0.251524748030211
0.452536998905648 0.2
0.329074864039415 -0.1
0.320021240631429 -0.4
0.404655463418508 -0.7
0.5 -0.882182581550041
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
2 -1
2.3 -1
2.46514091073115 -1
2.6 -0.899686535502806
2.8256990302483 -0.7
2.9 -0.63630801633762
3.14970059974017 -0.4
3.2 -0.35288882021447
3.4567547148229 -0.1
3.5 -0.0573777741055841
3.75553039844082 0.2
3.8 0.245008272549614
4.05022898634048 0.5
4.1 0.550992639737573
4.342986241976 0.8
4.4 0.858687916339615
4.6348865143515 1.1
4.7 1.16710968937187
4.92645666213449 1.4
5 1.47579353743648
5 1.7
5 1.79915461355839
4.90395508668252 1.7
4.7 1.4902367021926
4.61277543043856 1.4
4.4 1.18117622224217
4.32165072032469 1.1
4.1 0.872347641533607
4.03007494795145 0.8
3.8 0.564755997498912
3.73685449933096 0.5
3.5 0.260542503422094
3.43952184616346 0.2
3.2 -0.0364198232439162
3.13316965861326 -0.1
2.9 -0.319986228908746
2.80763324516651 -0.4
2.6 -0.58125777954559
2.43962370091713 -0.7
2.3 -0.807549758829626
2 -0.982316421992883
1.95143722198782 -1
2 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
0.8 -0.851551909266143
0.993173479193655 -1
1.1 -1
1.4 -1
1.7 -1
1.95143722198782 -1
2 -0.982316421992883
2.3 -0.807549758829626
2.43962370091713 -0.7
2.6 -0.58125777954559
2.80763324516651 -0.4
2.9 -0.319986228908746
3.13316965861326 -0.1
3.2 -0.0364198232439163
3.43952184616346 0.2
3.5 0.260542503422094
3.73685449933096 0.5
3.8 0.564755997498912
4.03007494795146 0.8
4.1 0.872347641533607
4.32165072032469 1.1
4.4 1.18117622224217
4.61277543043856 1.4
4.7 1.4902367021926
4.90395508668252 1.7
5 1.79915461355839
5 2
5 2.11054772434689
4.89360440314468 2
4.7 1.80000332189722
4.60425251683755 1.7
4.4 1.48859250637939
4.31564641771284 1.4
4.1 1.1765191835496
4.02737317324861 1.1
3.8 0.864770157763998
3.73824063621424 0.8
3.5 0.555764933746262
3.4456920039951 0.5
3.2 0.254052962763181
3.14465019442473 0.2
2.9 -0.0331615990754136
2.82456710982759 -0.1
2.6 -0.295792975411965
2.46041431173062 -0.4
2.3 -0.52055794349456
2 -0.689219397838695
1.96526350232502 -0.7
1.7 -0.788518912893744
1.4 -0.795757025826645
1.13064893846519 -0.7
1.1 -0.683918052372564
0.862263455301072 -0.4
0.808979197176202 -0.1
0.915747076651849 0.2
1.1 0.496409060392084
1.10157019576748 0.5
1.28960614275726 0.8
1.4 0.993702256538403
1.45970059393379 1.1
1.62532888648788 1.4
1.7 1.56612655293769
1.77995119754959 1.7
1.93669187835329 2
2 2.14677863471262
2.0923206058009 2.3
2.24617336023087 2.6
2.3 2.72300246481967
2.40503767769329 2.9
2.55626056994611 3.2
2.6 3.29661653068173
2.72079142626089 3.5
2.87143737336294 3.8
2.9 3.86144615549496
3.04277730721477 4.1
3.1954461557835 4.4
3.2 4.40929971013923
3.37900242346363 4.7
3.5 4.92486808462959
3.55097158046927 5
3.5 5
3.40142932595578 5
3.22847344793801 4.7
3.2 4.65375906421404
3.07574029408945 4.4
2.90649906245991 4.1
2.9 4.08914129727101
2.76559557953165 3.8
2.6 3.50536766893956
2.59772205996754 3.5
2.46148507675722 3.2
2.3 2.91524257638298
2.29370424556628 2.9
2.16094485993882 2.6
2 2.32235536616883
1.99097673617531 2.3
1.85875457575529 2
1.7 1.73221955398801
1.68641793173957 1.7
1.54561912168613 1.4
1.4 1.16311332334694
1.36252621850081 1.1
1.17157744556655 0.8
1.1 0.686121931710753
0.924859367945439 0.5
0.8 0.33020885304621
0.672267488436933 0.2
0.536077800481293 -0.1
0.548887656249961 -0.4
0.686725783867817 -0.7
0.8 -0.851551909266143
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.4 -0.795757025826645
1.7 -0.788518912893744
1.96526350232502 -0.7
2 -0.689219397838695
2.3 -0.52055794349456
2.46041431173062 -0.4
2.6 -0.295792975411965
2.82456710982759 -0.1
2.9 -0.0331615990754136
3.14465019442473 0.2
3.2 0.254052962763181
3.4456920039951 0.5
3.5 0.555764933746262
3.73824063621424 0.8
3.8 0.864770157763998
4.02737317324861 1.1
4.1 1.1765191835496
4.31564641771284 1.4
4.4 1.48859250637939
4.60425251683755 1.7
4.7 1.80000332189722
4.89360440314468 2
5 2.11054772434689
5 2.3
5 2.44060235130092
4.86632466487456 2.3
4.7 2.12655646015842
4.58086295229619 2
4.4 1.81038479699748
4.29723671252278 1.7
4.1 1.49207692345473
4.01502236356696 1.4
3.8 1.17269283611067
3.73287795941005 1.1
3.5 0.855156587544217
3.44807131182379 0.8
3.2 0.544983928396696
3.15542347055309 0.5
2.9 0.250770510190608
2.84429189235777 0.2
2.6 -0.0156940003341733
2.48863491059147 -0.1
2.3 -0.239771003173965
2.00599830960146 -0.4
2 -0.403307071020074
1.7 -0.473386636864232
1.4 -0.41812124233256
1.37146042068492 -0.4
1.15654484000173 -0.1
1.17170370862548 0.2
1.27929852386724 0.5
1.4 0.773910537155201
1.41111469676114 0.8
1.57601459408808 1.1
1.7 1.3832055436715
1.70943630747579 1.4
1.88585912783741 1.7
2 1.95550062581111
2.02716772636927 2
2.2011955897932 2.3
2.3 2.51337179457529
2.35374934070532 2.6
2.52061677134727 2.9
2.6 3.06815878446863
2.68196428885888 3.2
2.84512683607756 3.5
2.9 3.61301996475516
3.01805089499911 3.8
3.17905555196963 4.1
3.2 4.14132728502981
3.36805634511244 4.4
3.5 4.63814038225687
3.54456265715794 4.7
3.74076226577316 5
3.55097158046927 5
3.5 4.92486808462959
3.37900242346363 4.7
3.2 4.40929971013923
3.1954461557835 4.4
3.04277730721477 4.1
2.9 3.86144615549496
2.87143737336294 3.8
2.72079142626089 3.5
2.6 3.29661653068173
2.55626056994611 3.2
2.40503767769329 2.9
2.3 2.72300246481967
2.24617336023087 2.6
2.0923206058009 2.3
2 2.14677863471262
1.93669187835329 2
1.77995119754959 1.7
1.7 1.56612655293769
1.62532888648788 1.4
1.45970059393379 1.1
1.4 0.993702256538402
1.28960614275726 0.8
1.10157019576748 0.5
1.1 0.496409060392084
0.915747076651849 0.2
0.808979197176202 -0.1
0.862263455301072 -0.4
1.1 -0.683918052372564
1.13064893846519 -0.7
1.4 -0.795757025826645
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.4 -0.41812124233256
1.7 -0.473386636864232
2 -0.403307071020074
2.00599830960146 -0.4
2.3 -0.239771003173965
2.48863491059147 -0.1
2.6 -0.0156940003341733
2.84429189235777 0.2
2.9 0.250770510190608
3.15542347055309 0.5
3.2 0.544983928396696
3.44807131182379 0.8
3.5 0.855156587544217
3.73287795941005 1.1
3.8 1.17269283611067
4.01502236356696 1.4
4.1 1.49207692345473
4.29723671252278 1.7
4.4 1.81038479699748
4.58086295229619 2
4.7 2.12655646015842
4.86632466487456 2.3
5 2.44060235130092
5 2.6
5 2.82540896904459
4.79020775909165 2.6
4.7 2.50434134611541
4.51299165739907 2.3
4.4 2.1788898225363
4.23926404305045 2
4.1 1.84897034858928
3.96804367441076 1.7
3.8 1.51616584338751
3.69726472715451 1.4
3.5 1.18449963301572
3.42365210965462 1.1
3.2 0.860943620424
3.14171381672196 0.8
2.9 0.555842893921685
2.84027496465344 0.5
2.6 0.283229883915723
2.49059364601898 0.2
2.3 0.0602550022006703
2 -0.0927031919802147
1.89471860243888 -0.1
1.7 -0.113246003636299
1.67484476517317 -0.1
1.45605628540484 0.2
1.48298793508482 0.5
1.58293927819678 0.8
1.69232859424238 1.1
1.7 1.11752290620282
1.85871551063049 1.4
1.99176705812523 1.7
2 1.71842917231501
2.17190442201822 2
2.3 2.27161290045591
2.31803600351024 2.3
2.49963164270009 2.6
2.6 2.80615972184803
2.6610101862487 2.9
2.83417442074013 3.2
2.9 3.33090018644796
3.01248419199326 3.5
3.17973377725238 3.8
3.2 3.8387005554256
3.37984597422818 4.1
3.5 4.30936991133788
3.5700391863193 4.4
3.7717097398656 4.7
3.8 4.74599048265881
4.0079928192014 5
3.8 5
3.74076226577316 5
3.54456265715794 4.7
3.5 4.63814038225687
3.36805634511244 4.4
3.2 4.1413272850298
3.17905555196963 4.1
3.01805089499911 3.8
2.9 3.61301996475516
2.84512683607756 3.5
2.68196428885888 3.2
2.6 3.06815878446863
2.52061677134728 2.9
2.35374934070532 2.6
2.3 2.51337179457529
2.2011955897932 2.3
2.02716772636927 2
2 1.95550062581111
1.88585912783741 1.7
1.70943630747579 1.4
1.7 1.3832055436715
1.57601459408808 1.1
1.41111469676114 0.8
1.4 0.773910537155201
1.27929852386724 0.5
1.17170370862548 0.2
1.15654484000173 -0.1
1.37146042068492 -0.4
1.4 -0.41812124233256
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.7 -0.113246003636299
1.89471860243888 -0.1
2 -0.0927031919802147
2.3 0.0602550022006703
2.49059364601898 0.2
2.6 0.283229883915723
2.84027496465344 0.5
2.9 0.555842893921685
3.14171381672196 0.8
3.2 0.860943620424
3.42365210965462 1.1
3.5 1.18449963301572
3.69726472715451 1.4
3.8 1.51616584338751
3.96804367441076 1.7
4.1 1.84897034858928
4.23926404305045 2
4.4 2.1788898225363
4.51299165739907 2.3
4.7 2.50434134611541
4.79020775909165 2.6
5 2.82540896904459
5 2.9
5 3.2
5 3.37828896894242
4.85088366579314 3.2
4.7 3.02590030765925
4.59878638491649 2.9
4.4 2.66350537868974
4.35060733877826 2.6
4.10474542922032 2.3
4.1 2.29461155416832
3.85398559179285 2
3.8 1.93776413591041
3.60121786980827 1.7
3.5 1.58316264189462
3.34220105452406 1.4
3.2 1.23979387840445
3.07073098332466 1.1
2.9 0.919947835025573
2.77321099427183 0.8
2.6 0.640382774066456
2.40955148870689 0.5
2.3 0.422092004166336
2 0.328343504720431
1.80329501921971 0.5
1.81180840393734 0.8
1.90610123400115 1.1
2 1.3664651340641
2.01677901485133 1.4
2.18787257405507 1.7
2.3 1.94816323152004
2.33250231518657 2
2.51302683871878 2.3
2.6 2.47652533483634
2.68339345018974 2.6
2.85582531306054 2.9
2.9 2.98564357449268
3.05084276784031 3.2
3.2 3.46728997406315
3.22596689782693 3.5
3.43899823148534 3.8
3.5 3.9018101978495
3.66686801039959 4.1
3.8 4.29151553876977
3.9093510649839 4.4
4.1 4.62342379951903
4.19576998247082 4.7
4.4 4.8852079092601
4.57781606710707 5
4.4 5
4.1 5
4.0079928192014 5
3.8 4.74599048265881
3.7717097398656 4.7
3.5700391863193 4.4
3.5 4.30936991133788
3.37984597422818 4.1
3.2 3.8387005554256
3.17973377725238 3.8
3.01248419199326 3.5
2.9 3.33090018644796
2.83417442074013 3.2
2.6610101862487 2.9
2.6 2.80615972184803
2.49963164270009 2.6
2.31803600351024 2.3
2.3 2.27161290045591
2.17190442201822 2
2 1.71842917231501
1.99176705812523 1.7
1.85871551063049 1.4
1.7 1.11752290620282
1.69232859424238 1.1
1.58293927819678 0.8
1.48298793508482 0.5
1.45605628540484 0.2
1.67484476517317 -0.1
1.7 -0.113246003636299
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
2 0.328343504720431
2.3 0.422092004166336
2.40955148870689 0.5
2.6 0.640382774066456
2.77321099427183 0.8
2.9 0.919947835025573
3.07073098332466 1.1
3.2 1.23979387840445
3.34220105452406 1.4
3.5 1.58316264189462
3.60121786980827 1.7
3.8 1.93776413591041
3.85398559179285 2
4.1 2.29461155416832
4.10474542922032 2.3
4.35060733877826 2.6
4.4 2.66350537868974
4.59878638491649 2.9
4.7 3.02590030765925
4.85088366579314 3.2
5 3.37828896894242
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.57781606710707 5
4.4 4.8852079092601
4.19576998247082 4.7
4.1 4.62342379951903
3.9093510649839 4.4
3.8 4.29151553876977
3.66686801039959 4.1
3.5 3.9018101978495
3.43899823148534 3.8
3.22596689782693 3.5
3.2 3.46728997406315
3.05084276784031 3.2
2.9 2.98564357449268
2.85582531306054 2.9
2.68339345018974 2.6
2.6 2.47652533483634
2.51302683871878 2.3
2.33250231518657 2
2.3 1.94816323152004
2.18787257405507 1.7
2.01677901485133 1.4
2 1.3664651340641
1.90610123400115 1.1
1.81180840393734 0.8
1.80329501921971 0.5
2 0.328343504720431

2.40927049070689 1.4
2.51225246923272 1.7
2.6 1.93270995931648
2.64340248853572 2
2.82797210152017 2.3
2.9 2.44399083597382
3.02498762322818 2.6
3.19711976591534 2.9
3.2 2.90503856612676
3.46023133871775 3.2
3.5 3.25877185543214
3.77772063829841 3.5
3.8 3.52464238085655
4.1 3.51156354440793
4.10580668998281 3.5
4.1 3.46539986734474
4.05140864292541 3.2
3.9182153334058 2.9
3.8 2.67421580173713
3.75767141552739 2.6
3.56391723099392 2.3
3.5 2.20885980784159
3.3407359320668 2
3.2 1.80922393015354
3.10101071993819 1.7
2.9 1.46152146339619
2.8195260454505 1.4
2.6 1.21374309330245
2.40927049070689 1.4
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
2.6 1.21374309330245
2.8195260454505 1.4
2.9 1.46152146339619
3.10101071993819 1.7
3.2 1.80922393015354
3.3407359320668 2
3.5 2.20885980784159
3.56391723099392 2.3
3.75767141552739 2.6
3.8 2.67421580173713
3.9182153334058 2.9
4.05140864292541 3.2
4.1 3.46539986734474
4.10580668998281 3.5
4.1 3.51156354440793
3.8 3.52464238085655
3.77772063829841 3.5
3.5 3.25877185543214
3.46023133871775 3.2
3.2 2.90503856612676
3.19711976591534 2.9
3.02498762322818 2.6
2.9 2.44399083597382
2.82797210152017 2.3
2.64340248853572 2
2.6 1.93270995931648
2.51225246923272 1.7
2.40927049070689 1.4
2.6 1.21374309330245
};
\end{axis}



==> fig/tikz/ionosphere/cvi_Z_3.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{pink}{RGB}{255,192,203}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
axis background/.style={fill=pink},
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=black]
table{%
x  y
-0.836932524283127 0.5
-0.7 0.545469188622682
-0.4 0.736935546910175
-0.334640438727835 0.8
-0.1 0.956195928041712
0.0904312414369314 1.1
0.2 1.15647205338154
0.5 1.30984874626077
0.622005642860097 1.4
0.8 1.51078741247726
0.97313973591425 1.7
1.1 1.86143906079865
1.19055760170119 2
1.34244234103615 2.3
1.4 2.47562477810805
1.46077337050556 2.6
1.57850643028679 2.9
1.65606216685844 3.2
1.7 3.44162959816277
1.72269203808822 3.5
1.82944467369835 3.8
1.90739961913945 4.1
1.96806242810525 4.4
2 4.57744134582785
2.04183963015934 4.7
2.13423690111923 5
2 5
1.7 5
1.4 5
1.1 5
0.8 5
0.5 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.411353746759602
-0.836932524283127 0.5
};
\addplot [draw=none, fill=midnightblue854116]
table{%
x  y
-0.7 0.415377085699868
-0.611537438390037 0.5
-0.4 0.62901133754094
-0.222788537547129 0.8
-0.1 0.881738125273898
0.189031313205787 1.1
0.2 1.10565329272953
0.5 1.2494818839475
0.703702763404658 1.4
0.8 1.45993741510987
1.01967022963403 1.7
1.1 1.8022255690189
1.22925704928602 2
1.36777666495021 2.3
1.4 2.39832255463301
1.49854549743478 2.6
1.6071046568654 2.9
1.67808574814276 3.2
1.7 3.32051417859506
1.7697767869917 3.5
1.86894979951299 3.8
1.94166618708693 4.1
1.998349054691 4.4
2 4.40917245551672
2.09928402839867 4.7
2.18493490432779 5
2.13423690111923 5
2.04183963015934 4.7
2 4.57744134582785
1.96806242810525 4.4
1.90739961913945 4.1
1.82944467369835 3.8
1.72269203808822 3.5
1.7 3.44162959816277
1.65606216685844 3.2
1.57850643028679 2.9
1.46077337050556 2.6
1.4 2.47562477810805
1.34244234103615 2.3
1.19055760170119 2
1.1 1.86143906079865
0.973139735914251 1.7
0.8 1.51078741247726
0.622005642860097 1.4
0.5 1.30984874626077
0.2 1.15647205338154
0.0904312414369314 1.1
-0.1 0.956195928041712
-0.334640438727835 0.8
-0.4 0.736935546910175
-0.7 0.545469188622682
-0.836932524283127 0.5
-1 0.411353746759602
-1 0.262506456859429
-0.7 0.415377085699868
};
\addplot [draw=none, fill=midnightblue868137]
table{%
x  y
-0.795841717806527 0.2
-0.7 0.246096674388144
-0.434576163316107 0.5
-0.4 0.521087128171706
-0.110936636366422 0.8
-0.1 0.807280322506085
0.2 1.02121817668762
0.312739533224854 1.1
0.5 1.18911502163423
0.785399883949219 1.4
0.8 1.40908741774248
1.06620072335381 1.7
1.1 1.74301207723914
1.26795649687085 2
1.39311098886426 2.3
1.4 2.32102033115797
1.53631762436401 2.6
1.63570288344401 2.9
1.7 3.19933906289938
1.70027792938382 3.2
1.81686153589518 3.5
1.90845492532763 3.8
1.97593275503441 4.1
2 4.2278678133563
2.06078489766677 4.4
2.15672842663799 4.7
2.23563290753635 5
2.18493490432779 5
2.09928402839867 4.7
2 4.40917245551672
1.998349054691 4.4
1.94166618708693 4.1
1.86894979951299 3.8
1.7697767869917 3.5
1.7 3.32051417859506
1.67808574814276 3.2
1.6071046568654 2.9
1.49854549743478 2.6
1.4 2.39832255463301
1.36777666495021 2.3
1.22925704928602 2
1.1 1.8022255690189
1.01967022963403 1.7
0.8 1.45993741510987
0.703702763404658 1.4
0.5 1.2494818839475
0.2 1.10565329272953
0.189031313205787 1.1
-0.1 0.881738125273898
-0.222788537547129 0.8
-0.4 0.62901133754094
-0.611537438390037 0.5
-0.7 0.415377085699868
-1 0.262506456859429
-1 0.2
-1 0.0369925316052205
-0.795841717806527 0.2
};
\addplot [draw=none, fill=teal882156]
table{%
x  y
-0.767393468966219 -0.1
-0.7 -0.0491575370712178
-0.53902600301117 0.2
-0.4 0.331563742684298
-0.28602255005143 0.5
-0.1 0.677826506663736
0.0128795937293204 0.8
0.2 0.932575352716157
0.439590501863254 1.1
0.5 1.12874815932096
0.8 1.33287211646182
0.86148367886894 1.4
1.1 1.67627434646315
1.11609273930651 1.7
1.30665594445568 2
1.4 2.23044084913742
1.43718068906624 2.3
1.57408975129323 2.6
1.66430111002263 2.9
1.7 3.0661983125335
1.75626468920693 3.2
1.86394628479867 3.5
1.94796005114227 3.8
2 4.04470766846925
2.02125452781022 4.1
2.12507425330997 4.4
2.21417282487731 4.7
2.28633091074491 5
2.23563290753635 5
2.15672842663799 4.7
2.06078489766677 4.4
2 4.2278678133563
1.97593275503441 4.1
1.90845492532763 3.8
1.81686153589518 3.5
1.70027792938382 3.2
1.7 3.19933906289938
1.63570288344401 2.9
1.53631762436401 2.6
1.4 2.32102033115797
1.39311098886426 2.3
1.26795649687085 2
1.1 1.74301207723914
1.06620072335381 1.7
0.8 1.40908741774248
0.785399883949219 1.4
0.5 1.18911502163423
0.312739533224854 1.1
0.2 1.02121817668762
-0.1 0.807280322506085
-0.110936636366422 0.8
-0.4 0.521087128171706
-0.434576163316107 0.5
-0.7 0.246096674388144
-0.795841717806527 0.2
-1 0.0369925316052205
-1 -0.1
-1 -0.385537993890404
-0.767393468966219 -0.1
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 -1
-0.463272481548232 -1
-0.531997906780678 -0.7
-0.534032980708759 -0.4
-0.466887263021206 -0.1
-0.4 0.0190179630381567
-0.336492657051155 0.2
-0.144367326246291 0.5
-0.1 0.542412528127407
0.137992451396251 0.8
0.2 0.843932528744698
0.5 1.04529936210897
0.56621979306133 1.1
0.8 1.25113739768122
0.936346030206018 1.4
1.1 1.58956100503532
1.17490904107145 1.7
1.34535539204051 2
1.4 2.13490253648757
1.48824773419974 2.3
1.61186187822245 2.6
1.69289933660124 2.9
1.7 2.93305756216762
1.81225144903005 3.2
1.91103103370215 3.5
1.98746517695691 3.8
2 3.85894255065343
2.09266316176501 4.1
2.18936360895317 4.4
2.27161722311664 4.7
2.3 4.82105398827575
2.36718804829126 5
2.3 5
2.28633091074491 5
2.21417282487731 4.7
2.12507425330997 4.4
2.02125452781022 4.1
2 4.04470766846925
1.94796005114227 3.8
1.86394628479867 3.5
1.75626468920693 3.2
1.7 3.0661983125335
1.66430111002263 2.9
1.57408975129323 2.6
1.43718068906624 2.3
1.4 2.23044084913742
1.30665594445568 2
1.11609273930651 1.7
1.1 1.67627434646315
0.86148367886894 1.4
0.8 1.33287211646182
0.5 1.12874815932096
0.439590501863254 1.1
0.2 0.932575352716157
0.0128795937293204 0.8
-0.1 0.677826506663736
-0.28602255005143 0.5
-0.4 0.331563742684298
-0.53902600301117 0.2
-0.7 -0.0491575370712178
-0.767393468966219 -0.1
-1 -0.385537993890404
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.4 -1
-0.1 -1
-0.0573861828274515 -1
-0.1 -0.899878404221397
-0.18578225769567 -0.7
-0.251586781733601 -0.4
-0.247110535671339 -0.1
-0.165556411533151 0.2
-0.1 0.307496356155361
0.00266015693430968 0.5
0.2 0.717068201478016
0.28165101503614 0.8
0.5 0.940864152454138
0.692647532083978 1.1
0.8 1.16940267890062
1.0112083815431 1.4
1.1 1.5028476636075
1.23372534283639 1.7
1.38405483962534 2
1.4 2.03936422383773
1.53931477933324 2.3
1.64963400515167 2.6
1.7 2.79184690497077
1.75085644640593 2.9
1.86823820885316 3.2
1.95811578260563 3.5
2 3.66973400091075
2.05550689528629 3.8
2.16407179571979 4.1
2.25365296459636 4.4
2.3 4.57628796791045
2.35109451630367 4.7
2.45917832086926 5
2.36718804829126 5
2.3 4.82105398827575
2.27161722311664 4.7
2.18936360895317 4.4
2.09266316176501 4.1
2 3.85894255065343
1.98746517695691 3.8
1.91103103370215 3.5
1.81225144903005 3.2
1.7 2.93305756216762
1.69289933660124 2.9
1.61186187822245 2.6
1.48824773419974 2.3
1.4 2.13490253648757
1.34535539204051 2
1.17490904107145 1.7
1.1 1.58956100503532
0.936346030206018 1.4
0.8 1.25113739768122
0.56621979306133 1.1
0.5 1.04529936210897
0.2 0.843932528744698
0.137992451396251 0.8
-0.1 0.542412528127407
-0.144367326246291 0.5
-0.336492657051155 0.2
-0.4 0.0190179630381567
-0.466887263021206 -0.1
-0.534032980708759 -0.4
-0.531997906780678 -0.7
-0.463272481548232 -1
-0.4 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.427274561502933
4.79464956616827 0.2
4.7 0.0957428445502204
4.52247532402799 -0.1
4.4 -0.233907415150985
4.24825287708376 -0.4
4.1 -0.559854393298119
3.97009987993415 -0.7
3.8 -0.878727471183331
3.68437637266473 -1
3.8 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
-0.1 -0.899878404221397
-0.0573861828274515 -1
0.2 -1
0.238651940305817 -1
0.2 -0.936512379005937
0.075469651877805 -0.7
-0.020425549851012 -0.4
-0.0481258128874495 -0.1
0.0051039265622931 0.2
0.152137613753684 0.5
0.2 0.552647260378511
0.443532669277765 0.8
0.5 0.836428942799307
0.8 1.07920776261958
0.817472520400451 1.1
1.08607073288017 1.4
1.1 1.41613432217968
1.29254164460134 1.7
1.4 1.92695942081881
1.44159789867446 2
1.59038182446673 2.3
1.68740613208089 2.6
1.7 2.64797075068541
1.81851082030552 2.9
1.92422496867628 3.2
2 3.477365104014
2.01049577315506 3.5
2.13681139158501 3.8
2.23548042967458 4.1
2.3 4.32920247289178
2.33130519816104 4.4
2.45209004254918 4.7
2.55116859344727 5
2.45917832086926 5
2.35109451630367 4.7
2.3 4.57628796791045
2.25365296459636 4.4
2.16407179571979 4.1
2.05550689528629 3.8
2 3.66973400091075
1.95811578260563 3.5
1.86823820885316 3.2
1.75085644640593 2.9
1.7 2.79184690497077
1.64963400515167 2.6
1.53931477933324 2.3
1.4 2.03936422383773
1.38405483962534 2
1.23372534283639 1.7
1.1 1.5028476636075
1.0112083815431 1.4
0.8 1.16940267890062
0.692647532083978 1.1
0.5 0.940864152454138
0.28165101503614 0.8
0.2 0.717068201478016
0.00266015693430968 0.5
-0.1 0.307496356155361
-0.165556411533151 0.2
-0.247110535671339 -0.1
-0.251586781733601 -0.4
-0.18578225769567 -0.7
-0.1 -0.899878404221397
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
3.2 -1
3.5 -1
3.68437637266473 -1
3.8 -0.878727471183331
3.97009987993415 -0.7
4.1 -0.559854393298119
4.24825287708375 -0.4
4.4 -0.233907415150985
4.52247532402799 -0.1
4.7 0.0957428445502204
4.79464956616827 0.2
5 0.427274561502933
5 0.5
5 0.8
5 1.09451720331793
4.71811020195125 0.8
4.7 0.781080965112653
4.43058364046437 0.5
4.4 0.468089773030919
4.14222200081593 0.2
4.1 0.156058286659064
3.8521469507926 -0.1
3.8 -0.153993217576236
3.55867441858784 -0.4
3.5 -0.460133182285482
3.25862715794234 -0.7
3.2 -0.758873883857357
2.94583450250542 -1
3.2 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
0.2 -0.936512379005937
0.238651940305817 -1
0.5 -1
0.527506439842161 -1
0.5 -0.968931360456081
0.32503854878001 -0.7
0.2 -0.420028202002165
0.192491742876154 -0.4
0.141967874097875 -0.1
0.175592623653434 0.2
0.2 0.252187480071104
0.329682859009638 0.5
0.5 0.673474269222392
0.616472898162942 0.8
0.8 0.941400255374447
0.93327749307467 1.1
1.1 1.29164958849986
1.17196089237918 1.4
1.35135794636628 1.7
1.4 1.80273535528428
1.5123456959806 2
1.64144886960023 2.3
1.7 2.48970778561996
1.75641385716902 2.6
1.8861651942051 2.9
1.98021172849939 3.2
2 3.2724325135489
2.10552276081744 3.5
2.21811588788372 3.8
2.3 4.07377485225681
2.31222555522834 4.1
2.44347525148662 4.4
2.5530855687947 4.7
2.6 4.84925331222578
2.6695084668576 5
2.6 5
2.55116859344727 5
2.45209004254918 4.7
2.33130519816104 4.4
2.3 4.32920247289178
2.23548042967458 4.1
2.13681139158501 3.8
2.01049577315506 3.5
2 3.477365104014
1.92422496867628 3.2
1.81851082030552 2.9
1.7 2.64797075068541
1.68740613208089 2.6
1.59038182446673 2.3
1.44159789867446 2
1.4 1.92695942081881
1.29254164460134 1.7
1.1 1.41613432217968
1.08607073288017 1.4
0.817472520400451 1.1
0.8 1.07920776261958
0.5 0.836428942799307
0.443532669277765 0.8
0.2 0.552647260378511
0.152137613753684 0.5
0.00510392656229311 0.2
-0.0481258128874495 -0.1
-0.020425549851012 -0.4
0.075469651877805 -0.7
0.2 -0.936512379005937
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
2.6 -1
2.9 -1
2.94583450250542 -1
3.2 -0.758873883857357
3.25862715794234 -0.7
3.5 -0.460133182285482
3.55867441858784 -0.4
3.8 -0.153993217576236
3.8521469507926 -0.1
4.1 0.156058286659064
4.14222200081593 0.2
4.4 0.468089773030919
4.43058364046437 0.5
4.7 0.781080965112653
4.71811020195125 0.8
5 1.09451720331793
5 1.1
5 1.4
5 1.47549559157617
4.92678680231116 1.4
4.7 1.16668255765374
4.63536311241363 1.1
4.4 0.858043134222664
4.34370333562605 0.8
4.1 0.549987266325777
4.05133707320506 0.5
3.8 0.24342556431852
3.75726713302428 0.2
3.5 -0.0598475403445489
3.45950495259205 -0.1
3.2 -0.356665365061377
3.15412924299272 -0.4
2.9 -0.641938178691898
2.83305862206142 -0.7
2.6 -0.90786416572354
2.47794882610577 -1
2.6 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.5 -0.968931360456081
0.527506439842161 -1
0.8 -1
0.917284010794772 -1
0.8 -0.92251056234191
0.601722874927915 -0.7
0.5 -0.548579104902745
0.428042665089899 -0.4
0.355905452712856 -0.1
0.380781337292395 0.2
0.5 0.452164022234173
0.524696140149885 0.5
0.795336877928132 0.8
0.8 0.803592748129318
1.04908246574889 1.1
1.1 1.15853033682503
1.26037200232091 1.4
1.4 1.67038439756273
1.41712977017872 1.7
1.58309349328674 2
1.69251591473373 2.3
1.7 2.32424870764342
1.84104525970957 2.6
1.95381956810469 2.9
2 3.05406715443328
2.07220671722335 3.2
2.20054974847982 3.5
2.29942038418243 3.8
2.3 3.80193791238274
2.43894962763687 4.1
2.55564530481219 4.4
2.6 4.52743218550575
2.6868639762045 4.7
2.81766117339455 5
2.6695084668576 5
2.6 4.84925331222578
2.5530855687947 4.7
2.44347525148662 4.4
2.31222555522834 4.1
2.3 4.07377485225681
2.21811588788372 3.8
2.10552276081744 3.5
2 3.2724325135489
1.98021172849939 3.2
1.8861651942051 2.9
1.75641385716902 2.6
1.7 2.48970778561996
1.64144886960023 2.3
1.5123456959806 2
1.4 1.80273535528428
1.35135794636628 1.7
1.17196089237918 1.4
1.1 1.29164958849986
0.93327749307467 1.1
0.8 0.941400255374447
0.616472898162942 0.8
0.5 0.673474269222392
0.329682859009638 0.5
0.2 0.252187480071105
0.175592623653434 0.2
0.141967874097875 -0.1
0.192491742876154 -0.4
0.2 -0.420028202002165
0.32503854878001 -0.7
0.5 -0.968931360456081
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
2.3 -1
2.47794882610577 -1
2.6 -0.90786416572354
2.83305862206142 -0.7
2.9 -0.641938178691898
3.15412924299272 -0.4
3.2 -0.356665365061377
3.45950495259205 -0.1
3.5 -0.0598475403445489
3.75726713302428 0.2
3.8 0.24342556431852
4.05133707320506 0.5
4.1 0.549987266325777
4.34370333562605 0.8
4.4 0.858043134222664
4.63536311241363 1.1
4.7 1.16668255765374
4.92678680231116 1.4
5 1.47549559157617
5 1.7
5 1.79881407777866
4.90435633155322 1.7
4.7 1.4897157717793
4.6133888702296 1.4
4.4 1.18035218614326
4.3226079242226 1.1
4.1 0.871029045277058
4.03157635836932 0.8
3.8 0.562661934008452
3.73920341099797 0.5
3.5 0.257284917480005
3.44319629012801 0.2
3.2 -0.0413514008078016
3.13899650659901 -0.1
2.9 -0.327248494165587
2.81723664222854 -0.4
2.6 -0.591713532492732
2.45661656038144 -0.7
2.3 -0.822399551728807
2.00147022411007 -1
2.3 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
0.8 -0.92251056234191
0.917284010794772 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.00147022411007 -1
2.3 -0.822399551728808
2.45661656038144 -0.7
2.6 -0.591713532492732
2.81723664222854 -0.4
2.9 -0.327248494165587
3.13899650659901 -0.1
3.2 -0.0413514008078016
3.44319629012801 0.2
3.5 0.257284917480005
3.73920341099797 0.5
3.8 0.562661934008452
4.03157635836932 0.8
4.1 0.871029045277058
4.3226079242226 1.1
4.4 1.18035218614326
4.6133888702296 1.4
4.7 1.4897157717793
4.90435633155322 1.7
5 1.79881407777866
5 2
5 2.11011411222453
4.89413405817975 2
4.7 1.79930636826338
4.60508836462019 1.7
4.4 1.48745950178678
4.31696320792221 1.4
4.1 1.17469044703212
4.02942178081617 1.1
3.8 0.861879994677756
3.74138177586592 0.8
3.5 0.551329174135008
3.45047855946054 0.5
3.2 0.247457961125625
3.15204013275488 0.2
2.9 -0.0426845212062221
2.83650483076803 -0.1
2.6 -0.309241874829976
2.48161503801582 -0.4
2.3 -0.539376263980941
2.0252854904174 -0.7
2 -0.715454563183798
1.7 -0.824825610974109
1.4 -0.847486649090978
1.1 -0.764483645981105
1.004721075127 -0.7
0.8 -0.517164187788256
0.719915028678844 -0.4
0.607402995656922 -0.1
0.61840324751021 0.2
0.755088356552235 0.5
0.8 0.55003202850369
0.965343386347848 0.8
1.1 0.975806295054487
1.17276349266571 1.1
1.34878311226263 1.4
1.4 1.49917958837835
1.51615524301967 1.7
1.65384129059289 2
1.7 2.12997800219697
1.79207556066461 2.3
1.92567666225012 2.6
2 2.82035680195075
2.04206759164411 2.9
2.18388597020159 3.2
2.2955767361422 3.5
2.3 3.51343466055541
2.44298500816067 3.8
2.56567370004541 4.1
2.6 4.19282339533938
2.71024394757186 4.4
2.8490809761012 4.7
2.9 4.82421224641266
3.00085928474016 5
2.9 5
2.81766117339455 5
2.6868639762045 4.7
2.6 4.52743218550575
2.55564530481219 4.4
2.43894962763687 4.1
2.3 3.80193791238274
2.29942038418243 3.8
2.20054974847982 3.5
2.07220671722335 3.2
2 3.05406715443328
1.95381956810469 2.9
1.84104525970957 2.6
1.7 2.32424870764342
1.69251591473373 2.3
1.58309349328674 2
1.41712977017872 1.7
1.4 1.67038439756273
1.26037200232091 1.4
1.1 1.15853033682503
1.04908246574889 1.1
0.8 0.803592748129318
0.795336877928132 0.8
0.524696140149886 0.5
0.5 0.452164022234173
0.380781337292395 0.2
0.355905452712856 -0.1
0.428042665089899 -0.4
0.5 -0.548579104902745
0.601722874927915 -0.7
0.8 -0.92251056234191
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.1 -0.764483645981105
1.4 -0.847486649090978
1.7 -0.824825610974109
2 -0.715454563183798
2.0252854904174 -0.7
2.3 -0.539376263980941
2.48161503801582 -0.4
2.6 -0.309241874829976
2.83650483076803 -0.1
2.9 -0.0426845212062221
3.15204013275488 0.2
3.2 0.247457961125625
3.45047855946054 0.5
3.5 0.551329174135008
3.74138177586592 0.8
3.8 0.861879994677756
4.02942178081617 1.1
4.1 1.17469044703212
4.31696320792221 1.4
4.4 1.48745950178678
4.60508836462019 1.7
4.7 1.79930636826338
4.89413405817975 2
5 2.11011411222453
5 2.3
5 2.43997549263181
4.86713234089063 2.3
4.7 2.12551711415746
4.58214899433482 2
4.4 1.80867877955414
4.29923792430302 1.7
4.1 1.48934002255764
4.01805188434507 1.4
3.8 1.1684378403587
3.73736120491673 1.1
3.5 0.84876555045057
3.45465183902709 0.8
3.2 0.535691115428242
3.1652365563473 0.5
2.9 0.237619735231539
2.85972257678181 0.2
2.6 -0.0339435551410591
2.51588501696469 -0.1
2.3 -0.264897827945303
2.06625001661122 -0.4
2 -0.438373239744192
1.7 -0.527862326619188
1.4 -0.513049420105828
1.16548509027274 -0.4
1.1 -0.347021070893225
0.937316303614642 -0.1
0.902152038188406 0.2
0.988804050625156 0.5
1.1 0.708882804855028
1.13824397698751 0.8
1.30262490320386 1.1
1.4 1.29217845519374
1.45853280375187 1.4
1.61518071586061 1.7
1.7 1.91340590880733
1.74861965597943 2
1.89996237758747 2.3
2 2.56516847345907
2.01964014358966 2.6
2.17460294884954 2.9
2.29556522317984 3.2
2.3 3.2119949989057
2.4564310525808 3.5
2.58699666847507 3.8
2.6 3.83305765674979
2.74930153999338 4.1
2.89259304691357 4.4
2.9 4.41676822322059
3.07233398242633 4.7
3.2 4.94158706175084
3.2411267731549 5
3.2 5
3.00085928474016 5
2.9 4.82421224641266
2.8490809761012 4.7
2.71024394757186 4.4
2.6 4.19282339533938
2.56567370004541 4.1
2.44298500816067 3.8
2.3 3.51343466055541
2.2955767361422 3.5
2.18388597020159 3.2
2.04206759164411 2.9
2 2.82035680195075
1.92567666225012 2.6
1.79207556066461 2.3
1.7 2.12997800219697
1.65384129059289 2
1.51615524301967 1.7
1.4 1.49917958837835
1.34878311226263 1.4
1.17276349266571 1.1
1.1 0.975806295054487
0.965343386347848 0.8
0.8 0.55003202850369
0.755088356552235 0.5
0.61840324751021 0.2
0.607402995656922 -0.1
0.719915028678844 -0.4
0.8 -0.517164187788256
1.004721075127 -0.7
1.1 -0.764483645981105
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.4 -0.513049420105828
1.7 -0.527862326619188
2 -0.438373239744192
2.06625001661122 -0.4
2.3 -0.264897827945303
2.51588501696469 -0.1
2.6 -0.0339435551410591
2.85972257678181 0.2
2.9 0.237619735231539
3.1652365563473 0.5
3.2 0.535691115428242
3.45465183902709 0.8
3.5 0.84876555045057
3.73736120491673 1.1
3.8 1.1684378403587
4.01805188434507 1.4
4.1 1.48934002255764
4.29923792430302 1.7
4.4 1.80867877955414
4.58214899433482 2
4.7 2.12551711415746
4.86713234089063 2.3
5 2.43997549263181
5 2.6
5 2.82433951998709
4.79172850648337 2.6
4.7 2.50255631328102
4.51536558915733 2.3
4.4 2.17599261279669
4.24282107953188 2
4.1 1.84443258845803
3.97317490647132 1.7
3.8 1.50932525988278
3.70448582352229 1.4
3.5 1.1745412892654
3.43377640609463 1.1
3.2 0.846841121786535
3.15625056061233 0.8
2.9 0.536256349040808
2.86254225677242 0.5
2.6 0.256347842989217
2.52985694690364 0.2
2.3 0.0234826184482284
2.08226288574858 -0.1
2 -0.145026726321633
1.7 -0.205799093773526
1.4 -0.113837336065261
1.38392353105655 -0.1
1.22513033267761 0.2
1.23479163357933 0.5
1.32315257705529 0.8
1.4 0.987273755178107
1.44893363263872 1.1
1.59766597662133 1.4
1.7 1.65103596120577
1.72686190126745 1.7
1.88850827569771 2
2 2.27490542871985
2.01471617210747 2.3
2.18088989626817 2.6
2.3 2.87961221672415
2.31233992359101 2.9
2.48394377296421 3.2
2.6 3.44871150252853
2.63271739155031 3.5
2.80800372627502 3.8
2.9 3.98112870535235
2.98080203386856 4.1
3.16524519320757 4.4
3.2 4.46107840902184
3.37779712126838 4.7
3.5 4.87964094831359
3.60549257764284 5
3.5 5
3.2411267731549 5
3.2 4.94158706175084
3.07233398242633 4.7
2.9 4.41676822322059
2.89259304691357 4.4
2.74930153999338 4.1
2.6 3.83305765674979
2.58699666847507 3.8
2.4564310525808 3.5
2.3 3.2119949989057
2.29556522317984 3.2
2.17460294884954 2.9
2.01964014358966 2.6
2 2.56516847345907
1.89996237758747 2.3
1.74861965597943 2
1.7 1.91340590880733
1.61518071586061 1.7
1.45853280375187 1.4
1.4 1.29217845519374
1.30262490320386 1.1
1.13824397698751 0.8
1.1 0.708882804855028
0.988804050625156 0.5
0.902152038188407 0.2
0.937316303614642 -0.1
1.1 -0.347021070893225
1.16548509027274 -0.4
1.4 -0.513049420105828
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.4 -0.113837336065261
1.7 -0.205799093773526
2 -0.145026726321633
2.08226288574858 -0.1
2.3 0.0234826184482284
2.52985694690364 0.2
2.6 0.256347842989217
2.86254225677242 0.5
2.9 0.536256349040808
3.15625056061233 0.8
3.2 0.846841121786535
3.43377640609463 1.1
3.5 1.1745412892654
3.70448582352229 1.4
3.8 1.50932525988278
3.97317490647132 1.7
4.1 1.84443258845803
4.24282107953188 2
4.4 2.17599261279669
4.51536558915733 2.3
4.7 2.50255631328102
4.79172850648337 2.6
5 2.82433951998709
5 2.9
5 3.2
5 3.37466727413837
4.85499443093195 3.2
4.7 3.02031063543764
4.60429544935196 2.9
4.4 2.65530086921113
4.35759843399134 2.6
4.1124119948477 2.3
4.1 2.28581486150692
3.86435661417285 2
3.8 1.92512931058503
3.61503640645642 1.7
3.5 1.56551829337701
3.36082312516618 1.4
3.2 1.21553426892888
3.09685556034175 1.1
2.9 0.886778676275226
2.81310162137567 0.8
2.6 0.59495754584789
2.48255474362963 0.5
2.3 0.359480767399114
2.00074422866831 0.2
2 0.199626920100318
1.97024043920893 0.2
1.7 0.20703906241046
1.54134487542508 0.5
1.56133334822485 0.8
1.64454186962378 1.1
1.7 1.25520825145143
1.76873063638432 1.4
1.91410511831163 1.7
2 1.90797021225669
2.05375260302618 2
2.21698927973336 2.3
2.3 2.483285645228
2.37380415220411 2.6
2.54145256858372 2.9
2.6 3.018003036589
2.72261137111919 3.2
2.89457715854097 3.5
2.9 3.51004699919405
3.10892776071107 3.8
3.2 3.94361479633385
3.33134774356779 4.1
3.5 4.32354714201414
3.57732164312963 4.4
3.8 4.64241789236328
3.87267471438548 4.7
4.1 4.89549387000778
4.26899021269229 5
4.1 5
3.8 5
3.60549257764284 5
3.5 4.87964094831359
3.37779712126838 4.7
3.2 4.46107840902184
3.16524519320757 4.4
2.98080203386856 4.1
2.9 3.98112870535235
2.80800372627502 3.8
2.63271739155031 3.5
2.6 3.44871150252853
2.48394377296421 3.2
2.31233992359101 2.9
2.3 2.87961221672415
2.18088989626817 2.6
2.01471617210747 2.3
2 2.27490542871985
1.88850827569771 2
1.72686190126745 1.7
1.7 1.65103596120577
1.59766597662133 1.4
1.44893363263872 1.1
1.4 0.987273755178107
1.32315257705529 0.8
1.23479163357933 0.5
1.22513033267761 0.2
1.38392353105655 -0.1
1.4 -0.113837336065261
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
2 0.199626920100318
2.00074422866831 0.2
2.3 0.359480767399114
2.48255474362963 0.5
2.6 0.59495754584789
2.81310162137567 0.8
2.9 0.886778676275226
3.09685556034175 1.1
3.2 1.21553426892888
3.36082312516618 1.4
3.5 1.56551829337701
3.61503640645642 1.7
3.8 1.92512931058503
3.86435661417285 2
4.1 2.28581486150692
4.1124119948477 2.3
4.35759843399134 2.6
4.4 2.65530086921113
4.60429544935196 2.9
4.7 3.02031063543764
4.85499443093195 3.2
5 3.37466727413837
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.26899021269229 5
4.1 4.89549387000778
3.87267471438548 4.7
3.8 4.64241789236328
3.57732164312963 4.4
3.5 4.32354714201414
3.33134774356779 4.1
3.2 3.94361479633385
3.10892776071107 3.8
2.9 3.51004699919405
2.89457715854097 3.5
2.72261137111919 3.2
2.6 3.018003036589
2.54145256858372 2.9
2.37380415220411 2.6
2.3 2.483285645228
2.21698927973336 2.3
2.05375260302618 2
2 1.90797021225669
1.91410511831163 1.7
1.76873063638432 1.4
1.7 1.25520825145143
1.64454186962378 1.1
1.56133334822485 0.8
1.54134487542508 0.5
1.7 0.20703906241046
1.97024043920893 0.2
2 0.199626920100318

1.97377878027458 1.1
2 1.21523161076605
2.06575077316421 1.4
2.20130981480333 1.7
2.3 1.93734507678501
2.33878820784206 2
2.51966129865352 2.3
2.6 2.45599538377004
2.70686456459347 2.6
2.89011647238397 2.9
2.9 2.91671603751236
3.13458207574225 3.2
3.2 3.29374052069301
3.4121997381554 3.5
3.5 3.60007864579351
3.78014373234942 3.8
3.8 3.81627330747669
4.1 3.84749505043442
4.15787749776576 3.8
4.20571384336655 3.5
4.12222442846929 3.2
4.1 3.15863764574446
3.97014598680576 2.9
3.80866997866096 2.6
3.8 2.58738712044126
3.60762904758687 2.3
3.5 2.14351850272182
3.39748969163157 2
3.2 1.72354265301462
3.18107408228187 1.7
2.93154704455748 1.4
2.9 1.36353409833047
2.64099901857787 1.1
2.6 1.05907535327651
2.3 0.842654323957203
2 0.865687221265062
1.97377878027458 1.1
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
2 0.865687221265062
2.3 0.842654323957203
2.6 1.05907535327651
2.64099901857787 1.1
2.9 1.36353409833047
2.93154704455748 1.4
3.18107408228187 1.7
3.2 1.72354265301462
3.39748969163157 2
3.5 2.14351850272182
3.60762904758687 2.3
3.8 2.58738712044126
3.80866997866096 2.6
3.97014598680576 2.9
4.1 3.15863764574446
4.12222442846929 3.2
4.20571384336655 3.5
4.15787749776576 3.8
4.1 3.84749505043442
3.8 3.81627330747669
3.78014373234942 3.8
3.5 3.60007864579351
3.4121997381554 3.5
3.2 3.29374052069301
3.13458207574225 3.2
2.9 2.91671603751236
2.89011647238397 2.9
2.70686456459347 2.6
2.6 2.45599538377004
2.51966129865352 2.3
2.33878820784206 2
2.3 1.93734507678501
2.20130981480333 1.7
2.06575077316421 1.4
2 1.21523161076605
1.97377878027458 1.1
2 0.865687221265062
};
\end{axis}



==> fig/tikz/ionosphere/epcvi_Z_0.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=black]
table{%
x  y
-0.7 1.80667270970637
-0.4 1.76757668570865
-0.1 1.95220216390316
-0.0759552979986963 2
0.0466045770962084 2.3
0.120287984136679 2.6
0.17455465597499 2.9
0.2 3.18685125881169
0.5 2.92276745118519
0.8 3.09054484008162
0.862800803665858 3.2
1.04505975328637 3.5
1.1 3.65192620333567
1.4 3.51260757527248
1.7 3.51850778147981
1.87719666111012 3.8
1.96706665607896 4.1
2 4.22808607276294
2.08129202100572 4.4
2.19068175041941 4.7
2.2388737120188 5
2 5
1.7 5
1.4 5
1.1 5
0.8 5
0.5 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.85084700183156
-0.7 1.80667270970637
};
\addplot [draw=none, fill=midnightblue854116]
table{%
x  y
-0.4 1.6973810021123
-0.396129465683735 1.7
-0.1 1.85052098329546
-0.024804578918042 2
0.0796877338348194 2.3
0.142967414617826 2.6
0.191353924522275 2.9
0.2 2.99746921213282
0.5 2.92000964589601
0.8 3.06356481103421
0.878280818572134 3.2
1.04846607728117 3.5
1.1 3.64250669936875
1.4 3.5102715844122
1.7 3.51628862177115
1.87859360093642 3.8
1.96755642913216 4.1
2 4.22618122195036
2.08219275764037 4.4
2.19102793210854 4.7
2.23903083369333 5
2.2388737120188 5
2.19068175041941 4.7
2.08129202100572 4.4
2 4.22808607276294
1.96706665607896 4.1
1.87719666111012 3.8
1.7 3.51850778147981
1.4 3.51260757527248
1.1 3.65192620333567
1.04505975328637 3.5
0.862800803665858 3.2
0.8 3.09054484008162
0.5 2.92276745118519
0.2 3.18685125881169
0.17455465597499 2.9
0.120287984136679 2.6
0.0466045770962084 2.3
-0.0759552979986963 2
-0.1 1.95220216390316
-0.4 1.76757668570865
-0.7 1.80667270970637
-1 1.85084700183156
-1 1.72705628962401
-0.7 1.70058409256025
-0.633543804993009 1.7
-0.4 1.6973810021123
};
\addplot [draw=none, fill=midnightblue868137]
table{%
x  y
-0.7 1.51515412540278
-0.4 1.56202130238904
-0.196085637745511 1.7
-0.1 1.74883980268776
0.0263461401626122 2
0.11277089057343 2.3
0.165646845098973 2.6
0.2 2.8272025620108
0.22159912293721 2.9
0.5 2.91725184060683
0.8 3.0365847819868
0.893760833478411 3.2
1.05187240127598 3.5
1.1 3.63308719540184
1.4 3.50793559355192
1.7 3.5140694620625
1.87999054076272 3.8
1.96804620218536 4.1
2 4.22427637113778
2.08309349427502 4.4
2.19137411379767 4.7
2.23918795536786 5
2.23903083369333 5
2.19102793210854 4.7
2.08219275764037 4.4
2 4.22618122195036
1.96755642913216 4.1
1.87859360093642 3.8
1.7 3.51628862177115
1.4 3.5102715844122
1.1 3.64250669936875
1.04846607728117 3.5
0.878280818572134 3.2
0.8 3.06356481103421
0.5 2.92000964589601
0.2 2.99746921213282
0.191353924522275 2.9
0.142967414617826 2.6
0.0796877338348194 2.3
-0.024804578918042 2
-0.1 1.85052098329546
-0.396129465683735 1.7
-0.4 1.6973810021123
-0.633543804993009 1.7
-0.7 1.70058409256025
-1 1.72705628962401
-1 1.7
-1 1.52406247781672
-0.7 1.51515412540278
};
\addplot [draw=none, fill=teal882156]
table{%
x  y
-0.7 1.26608355272809
-0.502334661421004 1.4
-0.4 1.42666160266578
-0.1 1.61717326482254
-0.0584021239598037 1.7
0.0774968592432662 2
0.145854047312041 2.3
0.18832627558012 2.6
0.2 2.67720688548246
0.266103093775666 2.9
0.5 2.91449403531765
0.8 3.00960475293939
0.909240848384688 3.2
1.05527872527079 3.5
1.1 3.62366769143493
1.4 3.50559960269164
1.7 3.51185030235384
1.88138748058902 3.8
1.96853597523855 4.1
2 4.2223715203252
2.08399423090967 4.4
2.1917202954868 4.7
2.2393450770424 5
2.23918795536786 5
2.19137411379767 4.7
2.08309349427502 4.4
2 4.22427637113778
1.96804620218536 4.1
1.87999054076272 3.8
1.7 3.5140694620625
1.4 3.50793559355192
1.1 3.63308719540184
1.05187240127598 3.5
0.893760833478411 3.2
0.8 3.0365847819868
0.5 2.91725184060683
0.22159912293721 2.9
0.2 2.8272025620108
0.165646845098973 2.6
0.11277089057343 2.3
0.0263461401626122 2
-0.1 1.74883980268776
-0.196085637745511 1.7
-0.4 1.56202130238904
-0.7 1.51515412540278
-1 1.52406247781672
-1 1.4
-1 1.20227650593779
-0.7 1.26608355272809
};
\addplot [draw=none, fill=teal882156]
table{%
x  y
1.1 2.20086908254393
1.18043802473607 2.3
1.1 2.42163671839743
0.944046477332684 2.3
1.1 2.20086908254393
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 -1
-0.4 -1
-0.389476327452745 -1
-0.4 -0.970168223632014
-0.532081859718046 -0.7
-0.625189794486681 -0.4
-0.682190667122587 -0.1
-0.7 0.0761579599352704
-0.72438649670081 0.2
-0.71965097662781 0.5
-0.7 0.549780159378334
-0.657323206407427 0.8
-0.504825790110109 1.1
-0.4 1.17831069723333
-0.193323356202982 1.4
-0.1 1.45779210274373
0.0216435015147724 1.7
0.12864757832392 2
0.178937204050652 2.3
0.2 2.47024043050852
0.240493525567873 2.6
0.310607064614122 2.9
0.5 2.91173623002847
0.8 2.98262472389198
0.924720863290964 3.2
1.0586850492656 3.5
1.1 3.61424818746801
1.4 3.50326361183136
1.7 3.50963114264518
1.88278442041531 3.8
1.96902574829175 4.1
2 4.22046666951262
2.08489496754432 4.4
2.19206647717593 4.7
2.23950219871693 5
2.2393450770424 5
2.1917202954868 4.7
2.08399423090967 4.4
2 4.2223715203252
1.96853597523855 4.1
1.88138748058902 3.8
1.7 3.51185030235384
1.4 3.50559960269164
1.1 3.62366769143493
1.05527872527079 3.5
0.909240848384688 3.2
0.8 3.00960475293939
0.5 2.91449403531765
0.266103093775666 2.9
0.2 2.67720688548246
0.18832627558012 2.6
0.145854047312041 2.3
0.0774968592432662 2
-0.0584021239598037 1.7
-0.1 1.61717326482254
-0.4 1.42666160266578
-0.502334661421004 1.4
-0.7 1.26608355272809
-1 1.20227650593779
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
0.8 2.25584918770536
1.1 2.05387205343634
1.29971615679539 2.3
1.10104975551324 2.6
1.1 2.60062571384586
0.8 2.66285437397566
0.737906523817897 2.6
0.772678209479611 2.3
0.8 2.25584918770536

0.944046477332684 2.3
1.1 2.42163671839743
1.18043802473607 2.3
1.1 2.20086908254393
0.944046477332684 2.3
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.4 -0.970168223632014
-0.389476327452745 -1
-0.1 -1
0.030187815495779 -1
-0.1 -0.708063652618292
-0.104052846660734 -0.7
-0.229436985555903 -0.4
-0.310924285683658 -0.1
-0.358370611112497 0.2
-0.371722786480517 0.5
-0.338581976336117 0.8
-0.21697898400694 1.1
-0.1 1.22540984049921
-0.0250652042687275 1.4
0.101689126989349 1.7
0.179798297404575 2
0.2 2.15625232671605
0.234857712255975 2.3
0.323938430687153 2.6
0.355111035452578 2.9
0.5 2.90897842473929
0.8 2.95564469484457
0.940200878197241 3.2
1.0620913732604 3.5
1.1 3.6048286835011
1.4 3.50092762097109
1.7 3.50741198293653
1.88418136024161 3.8
1.96951552134494 4.1
2 4.21856181870004
2.08579570417897 4.4
2.19241265886506 4.7
2.23965932039146 5
2.23950219871693 5
2.19206647717593 4.7
2.08489496754432 4.4
2 4.22046666951262
1.96902574829175 4.1
1.88278442041531 3.8
1.7 3.50963114264518
1.4 3.50326361183136
1.1 3.61424818746801
1.0586850492656 3.5
0.924720863290964 3.2
0.8 2.98262472389198
0.5 2.91173623002847
0.310607064614122 2.9
0.240493525567873 2.6
0.2 2.47024043050852
0.178937204050652 2.3
0.12864757832392 2
0.0216435015147724 1.7
-0.1 1.45779210274373
-0.193323356202982 1.4
-0.4 1.17831069723333
-0.504825790110109 1.1
-0.657323206407427 0.8
-0.7 0.549780159378334
-0.71965097662781 0.5
-0.72438649670081 0.2
-0.7 0.0761579599352704
-0.682190667122587 -0.1
-0.625189794486681 -0.4
-0.532081859718046 -0.7
-0.4 -0.970168223632014
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.430718312970896
4.79002175560691 0.2
4.7 0.10120428529988
4.51571501453951 -0.1
4.4 -0.225881882999694
4.23883000130923 -0.4
4.1 -0.548680550189895
3.9574006527064 -0.7
3.8 -0.86390491379288
3.6676685590488 -1
3.8 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
1.1 1.92542025211175
1.23212317191695 2
1.4 2.25045283760322
1.4112338489048 2.3
1.4 2.32052571333984
1.19540844451623 2.6
1.1 2.65686884611986
0.8 2.74029119406074
0.6614071326151 2.6
0.700228675627696 2.3
0.8 2.13877392620144
0.995508569646014 2
1.1 1.92542025211175

0.772678209479611 2.3
0.737906523817897 2.6
0.8 2.66285437397566
1.1 2.60062571384586
1.10104975551324 2.6
1.29971615679539 2.3
1.1 2.05387205343634
0.8 2.25584918770536
0.772678209479611 2.3
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
-0.1 -0.708063652618292
0.030187815495779 -1
0.2 -1
0.340859318464211 -1
0.2 -0.756045903182467
0.169815612617396 -0.7
0.0391350227393599 -0.4
-0.0515178837682759 -0.1
-0.1 0.157538878697872
-0.108962312439336 0.2
-0.131530150582937 0.5
-0.1 0.770671421099367
-0.0973721076378267 0.8
-0.0153089807296693 1.1
0.0924985855917102 1.4
0.181734752463925 1.7
0.2 1.78215588563328
0.261938736719008 2
0.330795195192749 2.3
0.407383335806432 2.6
0.399615006291035 2.9
0.5 2.90622061945011
0.8 2.92866466579716
0.955680893103517 3.2
1.06549769725521 3.5
1.1 3.59540917953419
1.38314633310922 3.5
1.4 3.49099880331952
1.46145991797193 3.5
1.7 3.50519282322787
1.88557830006791 3.8
1.97000529439814 4.1
2 4.21665696788745
2.08669644081362 4.4
2.19275884055419 4.7
2.239816442066 5
2.23965932039146 5
2.19241265886506 4.7
2.08579570417897 4.4
2 4.21856181870004
1.96951552134494 4.1
1.88418136024161 3.8
1.7 3.50741198293653
1.4 3.50092762097109
1.1 3.6048286835011
1.0620913732604 3.5
0.940200878197241 3.2
0.8 2.95564469484457
0.5 2.90897842473929
0.355111035452578 2.9
0.323938430687153 2.6
0.234857712255975 2.3
0.2 2.15625232671605
0.179798297404575 2
0.101689126989349 1.7
-0.0250652042687275 1.4
-0.1 1.22540984049921
-0.21697898400694 1.1
-0.338581976336117 0.8
-0.371722786480517 0.5
-0.358370611112497 0.2
-0.310924285683658 -0.1
-0.229436985555903 -0.4
-0.104052846660734 -0.7
-0.1 -0.708063652618292
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
2.9 -1
3.2 -1
3.5 -1
3.6676685590488 -1
3.8 -0.86390491379288
3.9574006527064 -0.7
4.1 -0.548680550189895
4.23883000130923 -0.4
4.4 -0.225881882999694
4.51571501453951 -0.1
4.7 0.10120428529988
4.79002175560691 0.2
5 0.430718312970896
5 0.5
5 0.8
5 1.09903101313281
4.7113185302518 0.8
4.7 0.788238049953423
4.42039163377194 0.5
4.4 0.478877759380667
4.12744342945122 0.2
4.1 0.17171647301158
3.83132027130774 -0.1
3.8 -0.132020923841732
3.53009505066946 -0.4
3.5 -0.430368591543748
3.22035150601635 -0.7
3.2 -0.72008115224909
2.9 -0.996990536624111
2.89641398244436 -1
2.9 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
1.1 1.80769671669986
1.4 1.96883248709575
1.41866488689562 2
1.48177887027681 2.3
1.4 2.44942070725561
1.28976713351922 2.6
1.1 2.71311197839386
0.8 2.81772801414582
0.584907741412303 2.6
0.627779141775781 2.3
0.8 2.02169866469752
0.830569682752099 2
1.1 1.80769671669986

0.995508569646014 2
0.8 2.13877392620144
0.700228675627696 2.3
0.6614071326151 2.6
0.8 2.74029119406074
1.1 2.65686884611986
1.19540844451623 2.6
1.4 2.32052571333984
1.4112338489048 2.3
1.4 2.25045283760322
1.23212317191695 2
1.1 1.92542025211175
0.995508569646014 2
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
0.2 -0.756045903182467
0.340859318464211 -1
0.5 -1
0.652073983852195 -1
0.5 -0.809182022760108
0.431963540399577 -0.7
0.280922477379295 -0.4
0.2 -0.184574797843576
0.170926295776475 -0.1
0.103062783911911 0.2
0.0741386210057196 0.5
0.0873813602763293 0.8
0.140903850172815 1.1
0.2 1.34464874751662
0.212364406437111 1.4
0.291488821995375 1.7
0.364307447648375 2
0.426732678129524 2.3
0.490828240925711 2.6
0.444118977129491 2.9
0.5 2.90346281416093
0.8 2.90168463674975
0.971160908009794 3.2
1.06890402125002 3.5
1.1 3.58598967556727
1.35519202073634 3.5
1.4 3.47606898031028
1.56340032990325 3.5
1.7 3.50297366351922
1.88697523989421 3.8
1.97049506745134 4.1
2 4.21475211707487
2.08759717744827 4.4
2.19310502224331 4.7
2.23997356374053 5
2.239816442066 5
2.19275884055419 4.7
2.08669644081362 4.4
2 4.21665696788745
1.97000529439814 4.1
1.88557830006791 3.8
1.7 3.50519282322787
1.46145991797193 3.5
1.4 3.49099880331952
1.38314633310922 3.5
1.1 3.59540917953419
1.06549769725521 3.5
0.955680893103517 3.2
0.8 2.92866466579716
0.5 2.90622061945011
0.399615006291035 2.9
0.407383335806432 2.6
0.330795195192749 2.3
0.261938736719008 2
0.2 1.78215588563328
0.181734752463925 1.7
0.0924985855917102 1.4
-0.0153089807296693 1.1
-0.0973721076378267 0.8
-0.1 0.770671421099367
-0.131530150582937 0.5
-0.108962312439336 0.2
-0.1 0.157538878697872
-0.0515178837682759 -0.1
0.0391350227393599 -0.4
0.169815612617396 -0.7
0.2 -0.756045903182467
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
2.6 -1
2.89641398244436 -1
2.9 -0.996990536624111
3.2 -0.72008115224909
3.22035150601635 -0.7
3.5 -0.430368591543748
3.53009505066946 -0.4
3.8 -0.132020923841732
3.83132027130774 -0.1
4.1 0.17171647301158
4.12744342945122 0.2
4.4 0.478877759380667
4.42039163377194 0.5
4.7 0.788238049953423
4.7113185302518 0.8
5 1.09903101313281
5 1.1
5 1.4
5 1.48026536703885
4.92126262673868 1.4
4.7 1.17419554432057
4.62689045813906 1.1
4.4 0.86939363801584
4.33114785917977 0.8
4.1 0.566541118102313
4.0332447480132 0.5
3.8 0.266743871609415
3.73181261241491 0.2
3.5 -0.0282019880039165
3.4243450645548 -0.1
3.2 -0.315307461555757
3.10595251630708 -0.4
2.9 -0.589775449908307
2.76686419383323 -0.7
2.6 -0.844369357739477
2.3872333927542 -1
2.6 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
1.1 1.68624536916603
1.13329002054475 1.7
1.4 1.80903934082623
1.51435814965223 2
1.55232389164882 2.3
1.4 2.57831570117139
1.38412582252221 2.6
1.1 2.76935511066786
0.8 2.8951648342309
0.508408350209505 2.6
0.555329607923865 2.3
0.685805290485953 2
0.8 1.87801928719953
1.07994511466254 1.7
1.1 1.68624536916603

0.830569682752099 2
0.8 2.02169866469752
0.627779141775781 2.3
0.584907741412303 2.6
0.8 2.81772801414582
1.1 2.71311197839386
1.28976713351922 2.6
1.4 2.44942070725561
1.48177887027681 2.3
1.41866488689562 2
1.4 1.96883248709575
1.1 1.80769671669986
0.830569682752099 2
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.5 -0.809182022760108
0.652073983852195 -1
0.8 -1
1.08875657906782 -1
0.8 -0.784060028927105
0.731999922079539 -0.7
0.53009262517786 -0.4
0.5 -0.342803560190149
0.402423004598841 -0.1
0.321587086430466 0.2
0.280068362799638 0.5
0.277366733178355 0.8
0.307697571546617 1.1
0.356823981319225 1.4
0.410026134729881 1.7
0.466676158577741 2
0.5 2.17382207331364
0.545630699167083 2
0.8 1.7282873369336
0.844483392254557 1.7
1.1 1.52475409096836
1.4 1.63803963480096
1.44740099510957 1.7
1.61005141240883 2
1.62286891302083 2.3
1.4496070286419 2.6
1.4 2.63489414163016
1.1 2.82559824294186
0.924431764220838 2.9
0.98664092291607 3.2
1.07231034524483 3.5
1.1 3.57657017160036
1.32723770836345 3.5
1.4 3.46113915730104
1.66534074183456 3.5
1.7 3.50075450381056
1.88837217972051 3.8
1.97098484050453 4.1
2 4.21284726626229
2.08849791408292 4.4
2.19345120393244 4.7
2.24013068541506 5
2.23997356374053 5
2.19310502224331 4.7
2.08759717744827 4.4
2 4.21475211707487
1.97049506745134 4.1
1.88697523989421 3.8
1.7 3.50297366351922
1.56340032990325 3.5
1.4 3.47606898031028
1.35519202073634 3.5
1.1 3.58598967556727
1.06890402125002 3.5
0.971160908009794 3.2
0.8 2.90168463674975
0.5 2.90346281416093
0.444118977129491 2.9
0.490828240925711 2.6
0.426732678129524 2.3
0.364307447648375 2
0.291488821995375 1.7
0.212364406437111 1.4
0.2 1.34464874751662
0.140903850172815 1.1
0.0873813602763293 0.8
0.0741386210057196 0.5
0.103062783911911 0.2
0.170926295776475 -0.1
0.2 -0.184574797843576
0.280922477379295 -0.4
0.431963540399577 -0.7
0.5 -0.809182022760108

1.07994511466254 1.7
0.8 1.87801928719953
0.685805290485953 2
0.555329607923865 2.3
0.508408350209505 2.6
0.8 2.8951648342309
1.1 2.76935511066786
1.38412582252221 2.6
1.4 2.57831570117139
1.55232389164882 2.3
1.51435814965223 2
1.4 1.80903934082623
1.13329002054475 1.7
1.1 1.68624536916603
1.07994511466254 1.7

0.488622947967947 2.9
0.5 2.90070500887175
0.564274480746582 2.9
0.5 2.83306227254248
0.488622947967947 2.9
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
2 -1
2.3 -1
2.3872333927542 -1
2.6 -0.844369357739477
2.76686419383323 -0.7
2.9 -0.589775449908307
3.10595251630708 -0.4
3.2 -0.315307461555757
3.4243450645548 -0.1
3.5 -0.0282019880039165
3.73181261241491 0.2
3.8 0.266743871609415
4.0332447480132 0.5
4.1 0.566541118102313
4.33114785917977 0.8
4.4 0.86939363801584
4.62689045813906 1.1
4.7 1.17419554432057
4.92126262673867 1.4
5 1.48026536703885
5 1.7
5 1.80518948052222
4.89669747375315 1.7
4.7 1.49973374455307
4.60168849646531 1.4
4.4 1.19551520622838
4.30530645826889 1.1
4.1 0.893190778063021
4.00674213867083 0.8
3.8 0.593872386447785
3.70453755184329 0.5
3.5 0.29945020454268
3.39588536572125 0.2
3.2 0.013242132594238
3.07502859032184 -0.1
2.9 -0.259230600129423
2.72991773981795 -0.4
2.6 -0.509692033712093
2.33511540613358 -0.7
2.3 -0.726530970211593
2 -0.904909985593338
1.76344201374988 -1
2 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
0.8 -0.784060028927105
1.08875657906782 -1
1.1 -1
1.4 -1
1.7 -1
1.76344201374988 -1
2 -0.904909985593338
2.3 -0.726530970211593
2.33511540613358 -0.7
2.6 -0.509692033712093
2.72991773981795 -0.4
2.9 -0.259230600129423
3.07502859032184 -0.1
3.2 0.013242132594238
3.39588536572125 0.2
3.5 0.29945020454268
3.70453755184329 0.5
3.8 0.593872386447785
4.00674213867083 0.8
4.1 0.893190778063021
4.30530645826889 1.1
4.4 1.19551520622838
4.60168849646531 1.4
4.7 1.49973374455307
4.89669747375315 1.7
5 1.80518948052222
5 2
5 2.11913093664886
4.88319271561081 2
4.7 1.8133698035942
4.58856649915414 1.7
4.4 1.50863788676697
4.29281188801616 1.4
4.1 1.20548043993703
3.99520856986345 1.1
3.8 0.904933907455805
3.69436420969014 0.8
3.5 0.608894519104543
3.38746018165394 0.5
3.2 0.320910553312139
3.06844427930818 0.2
2.9 0.0471431918343839
2.72403224323199 -0.1
2.6 -0.203153085258535
2.32412592710352 -0.4
2.3 -0.41751060188327
2 -0.581682354918844
1.7 -0.686804227900297
1.54946714050034 -0.7
1.4 -0.71344532432835
1.35040913589678 -0.7
1.1 -0.618124529134646
0.85613934309435 -0.4
0.8 -0.334707086512652
0.675513935618629 -0.1
0.562907456506167 0.2
0.5 0.471159686154618
0.495241021550103 0.5
0.475520282780566 0.8
0.480929835523756 1.1
0.5 1.37759454218152
0.506598256298428 1.4
0.8 1.49826814732593
0.990382196359561 1.4
1.1 1.33910085747317
1.25242748335252 1.4
1.4 1.44296378555799
1.59663816222854 1.7
1.7 1.97607114569345
1.70850828460732 2
1.7 2.11740939632512
1.69341393439284 2.3
1.50924751180246 2.6
1.4 2.67684592796508
1.1 2.88184137521586
1.05715050499363 2.9
1.00212093782235 3.2
1.07571666923963 3.5
1.1 3.56715066763345
1.29928339599057 3.5
1.4 3.44620933429181
1.7 3.49202596459321
1.70336427546839 3.5
1.8897691195468 3.8
1.97147461355773 4.1
2 4.21094241544971
2.08939865071757 4.4
2.19379738562157 4.7
2.2402878070896 5
2.24013068541506 5
2.19345120393244 4.7
2.08849791408292 4.4
2 4.21284726626229
1.97098484050453 4.1
1.8883721797205 3.8
1.7 3.50075450381056
1.66534074183456 3.5
1.4 3.46113915730104
1.32723770836345 3.5
1.1 3.57657017160036
1.07231034524483 3.5
0.98664092291607 3.2
0.924431764220838 2.9
1.1 2.82559824294186
1.4 2.63489414163016
1.4496070286419 2.6
1.62286891302083 2.3
1.61005141240883 2
1.44740099510957 1.7
1.4 1.63803963480096
1.1 1.52475409096836
0.844483392254557 1.7
0.8 1.7282873369336
0.545630699167083 2
0.5 2.17382207331364
0.466676158577741 2
0.410026134729881 1.7
0.356823981319225 1.4
0.307697571546617 1.1
0.277366733178355 0.8
0.280068362799638 0.5
0.321587086430466 0.2
0.402423004598841 -0.1
0.5 -0.342803560190149
0.53009262517786 -0.4
0.731999922079539 -0.7
0.8 -0.784060028927105
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
0.5 2.83306227254248
0.564274480746582 2.9
0.5 2.90070500887175
0.488622947967947 2.9
0.5 2.83306227254248
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.4 -0.71344532432835
1.54946714050034 -0.7
1.7 -0.686804227900297
2 -0.581682354918844
2.3 -0.41751060188327
2.32412592710352 -0.4
2.6 -0.203153085258535
2.72403224323199 -0.1
2.9 0.0471431918343839
3.06844427930818 0.2
3.2 0.320910553312139
3.38746018165394 0.5
3.5 0.608894519104543
3.69436420969014 0.8
3.8 0.904933907455805
3.99520856986345 1.1
4.1 1.20548043993703
4.29281188801616 1.4
4.4 1.50863788676697
4.58856649915414 1.7
4.7 1.8133698035942
4.88319271561081 2
5 2.11913093664886
5 2.3
5 2.45417958714986
4.84945227476474 2.3
4.7 2.1472471853956
4.55619145837582 2
4.4 1.84080603534634
4.2623967189796 1.7
4.1 1.53518719864705
3.96741728960342 1.4
3.8 1.2313811576454
3.66979488604908 1.1
3.5 0.931425637588966
3.36652283930991 0.8
3.2 0.639256821465614
3.05112573875608 0.5
2.9 0.36184467808694
2.70905773217863 0.2
2.6 0.10969068307966
2.3052003048664 -0.1
2.3 -0.103649431144238
2 -0.249510518819473
1.7 -0.321992535899067
1.4 -0.291692097900202
1.1 -0.118943469394644
1.08367285503452 -0.1
0.906611163510795 0.2
0.8 0.490754255931259
0.797904928180214 0.5
0.774751930257917 0.8
0.8 0.972681170313325
1.1 1.03924665558161
1.18959092114989 1.1
1.4 1.17303789889103
1.58159517526936 1.4
1.7 1.58696105378509
1.75853331272898 1.7
1.85023701444648 2
1.80397078384647 2.3
1.7 2.38759772874288
1.56888799496302 2.6
1.4 2.7187977143
1.1406573910072 2.9
1.1 2.93385662675312
1.01760095272862 3.2
1.07912299323444 3.5
1.1 3.55773116366653
1.27132908361768 3.5
1.4 3.43127951128257
1.7 3.47994417929935
1.70846162603244 3.5
1.8911660593731 3.8
1.97196438661092 4.1
2 4.20903756463713
2.09029938735222 4.4
2.1941435673107 4.7
2.24044492876413 5
2.2402878070896 5
2.19379738562157 4.7
2.08939865071757 4.4
2 4.21094241544971
1.97147461355773 4.1
1.8897691195468 3.8
1.70336427546839 3.5
1.7 3.49202596459321
1.4 3.44620933429181
1.29928339599057 3.5
1.1 3.56715066763345
1.07571666923963 3.5
1.00212093782235 3.2
1.05715050499363 2.9
1.1 2.88184137521586
1.4 2.67684592796508
1.50924751180246 2.6
1.69341393439284 2.3
1.7 2.11740939632512
1.70850828460732 2
1.7 1.97607114569345
1.59663816222854 1.7
1.4 1.44296378555799
1.25242748335252 1.4
1.1 1.33910085747317
0.990382196359561 1.4
0.8 1.49826814732593
0.506598256298429 1.4
0.5 1.37759454218152
0.480929835523756 1.1
0.475520282780566 0.8
0.495241021550103 0.5
0.5 0.471159686154618
0.562907456506167 0.2
0.675513935618629 -0.1
0.8 -0.334707086512652
0.85613934309435 -0.4
1.1 -0.618124529134646
1.35040913589678 -0.7
1.4 -0.71344532432835
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.1 -0.118943469394644
1.4 -0.291692097900202
1.7 -0.321992535899067
2 -0.249510518819473
2.3 -0.103649431144238
2.3052003048664 -0.1
2.6 0.10969068307966
2.70905773217863 0.2
2.9 0.36184467808694
3.05112573875608 0.5
3.2 0.639256821465614
3.36652283930991 0.8
3.5 0.931425637588966
3.66979488604908 1.1
3.8 1.2313811576454
3.96741728960342 1.4
4.1 1.53518719864705
4.2623967189796 1.7
4.4 1.84080603534634
4.55619145837582 2
4.7 2.1472471853956
4.84945227476474 2.3
5 2.45417958714986
5 2.6
5 2.84985750572038
4.75788257065643 2.6
4.7 2.54045778396981
4.4679276083581 2.3
4.4 2.23015277436087
4.17893617042875 2
4.1 1.91891147134113
3.88988811815007 1.7
3.8 1.60806438210188
3.59844565094062 1.4
3.5 1.30053270623623
3.30051634378077 1.1
3.2 1.0012468010558
2.98828067465553 0.8
2.9 0.718191718426055
2.64445256324177 0.5
2.6 0.46317896127855
2.3 0.2643970904243
2.1444826757748 0.2
2 0.142985417181377
1.7 0.154790569901582
1.61614629524509 0.2
1.43816313337148 0.5
1.50240928104081 0.8
1.66060131022672 1.1
1.7 1.15617188923581
1.83064772369506 1.4
1.94894820234403 1.7
1.99196574428565 2
1.91864778381939 2.3
1.7 2.48421568587504
1.62852847812358 2.6
1.4 2.76074950063492
1.20070015303957 2.9
1.1 2.98385603234697
1.0330809676349 3.2
1.08252931722925 3.5
1.1 3.54831165969962
1.2433747712448 3.5
1.4 3.41634968827333
1.7 3.46786239400549
1.71355897659649 3.5
1.8925629991994 3.8
1.97245415966412 4.1
2 4.20713271382455
2.09120012398687 4.4
2.19448974899983 4.7
2.24060205043866 5
2.24044492876413 5
2.1941435673107 4.7
2.09029938735222 4.4
2 4.20903756463713
1.97196438661092 4.1
1.8911660593731 3.8
1.70846162603244 3.5
1.7 3.47994417929935
1.4 3.43127951128257
1.27132908361768 3.5
1.1 3.55773116366653
1.07912299323444 3.5
1.01760095272862 3.2
1.1 2.93385662675312
1.1406573910072 2.9
1.4 2.7187977143
1.56888799496302 2.6
1.7 2.38759772874288
1.80397078384647 2.3
1.85023701444648 2
1.75853331272898 1.7
1.7 1.58696105378509
1.58159517526936 1.4
1.4 1.17303789889103
1.18959092114989 1.1
1.1 1.03924665558161
0.8 0.972681170313325
0.774751930257917 0.8
0.797904928180214 0.5
0.8 0.490754255931259
0.906611163510795 0.2
1.08367285503452 -0.1
1.1 -0.118943469394644
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.7 0.154790569901582
2 0.142985417181377
2.1444826757748 0.2
2.3 0.2643970904243
2.6 0.46317896127855
2.64445256324177 0.5
2.9 0.718191718426055
2.98828067465553 0.8
3.2 1.0012468010558
3.30051634378077 1.1
3.5 1.30053270623623
3.59844565094062 1.4
3.8 1.60806438210188
3.88988811815007 1.7
4.1 1.91891147134113
4.17893617042875 2
4.4 2.23015277436087
4.4679276083581 2.3
4.7 2.54045778396981
4.75788257065643 2.6
5 2.84985750572038
5 2.9
5 3.2
5 3.44955115369285
4.76857651799359 3.2
4.7 3.12700905600015
4.49523867171222 2.9
4.4 2.79711627747586
4.22699081722801 2.6
4.1 2.46057741985633
3.95975502362411 2.3
3.8 2.12366568626401
3.6888261692735 2
3.5 1.79488611682397
3.40899604357549 1.7
3.2 1.48340999369206
3.11082223505134 1.4
2.9 1.20161626577283
2.76920628667415 1.1
2.6 0.968246981608933
2.3 0.812128819304523
2.10802142847657 1.1
2.17355529627643 1.4
2.24748783474718 1.7
2.26748114655306 2
2.09104429058279 2.3
2 2.32820408233051
1.7 2.5808336430072
1.68816896128413 2.6
1.4 2.80270128696984
1.26074291507195 2.9
1.1 3.03385543794082
1.04856098254118 3.2
1.08593564122406 3.5
1.1 3.53889215573271
1.21542045887191 3.5
1.4 3.40141986526409
1.7 3.45578060871163
1.71865632716053 3.5
1.8939599390257 3.8
1.97294393271732 4.1
2 4.20522786301197
2.09210086062152 4.4
2.19483593068896 4.7
2.2407591721132 5
2.24060205043866 5
2.19448974899983 4.7
2.09120012398687 4.4
2 4.20713271382455
1.97245415966412 4.1
1.8925629991994 3.8
1.71355897659649 3.5
1.7 3.46786239400549
1.4 3.41634968827333
1.2433747712448 3.5
1.1 3.54831165969962
1.08252931722925 3.5
1.0330809676349 3.2
1.1 2.98385603234697
1.20070015303957 2.9
1.4 2.76074950063492
1.62852847812358 2.6
1.7 2.48421568587504
1.91864778381939 2.3
1.99196574428565 2
1.94894820234403 1.7
1.83064772369506 1.4
1.7 1.15617188923581
1.66060131022672 1.1
1.50240928104081 0.8
1.43816313337148 0.5
1.61614629524509 0.2
1.7 0.154790569901582
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
2.3 0.812128819304523
2.6 0.968246981608933
2.76920628667415 1.1
2.9 1.20161626577283
3.11082223505134 1.4
3.2 1.48340999369206
3.40899604357549 1.7
3.5 1.79488611682397
3.6888261692735 2
3.8 2.12366568626401
3.95975502362411 2.3
4.1 2.46057741985633
4.22699081722801 2.6
4.4 2.79711627747586
4.49523867171222 2.9
4.7 3.12700905600015
4.76857651799359 3.2
5 3.44955115369285
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 4.76152778978305
4.95588259706151 4.7
4.70937234657086 4.4
4.7 4.38778878749724
4.54590704299425 4.1
4.4 3.90275588817715
4.34224786404277 3.8
4.12209115299895 3.5
4.1 3.46937062844092
3.90572405790523 3.2
3.8 3.06392396905811
3.64510284887959 2.9
3.5 2.73573448954039
3.3224318958476 2.6
3.2 2.48972883836721
2.9 2.35530642077432
2.6 2.3312965355765
2.3 2.34341298922766
2 2.42525976223558
1.7924229628467 2.6
1.7 2.62668121617475
1.4 2.84465307330477
1.32078567710432 2.9
1.1 3.08385484353467
1.06404099744745 3.2
1.08934196521886 3.5
1.1 3.52947265176579
1.18746614649903 3.5
1.4 3.38649004225486
1.7 3.44369882341777
1.72375367772458 3.5
1.89535687885199 3.8
1.97343370577051 4.1
2 4.20332301219939
2.09300159725617 4.4
2.19518211237809 4.7
2.24091629378773 5
2.2407591721132 5
2.19483593068896 4.7
2.09210086062152 4.4
2 4.20522786301197
1.97294393271732 4.1
1.8939599390257 3.8
1.71865632716053 3.5
1.7 3.45578060871163
1.4 3.4014198652641
1.21542045887191 3.5
1.1 3.53889215573271
1.08593564122406 3.5
1.04856098254118 3.2
1.1 3.03385543794082
1.26074291507195 2.9
1.4 2.80270128696984
1.68816896128413 2.6
1.7 2.5808336430072
2 2.32820408233051
2.09104429058279 2.3
2.26748114655306 2
2.24748783474718 1.7
2.17355529627643 1.4
2.10802142847657 1.1
2.3 0.812128819304523
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
2 2.42525976223558
2.3 2.34341298922766
2.6 2.3312965355765
2.9 2.35530642077432
3.2 2.48972883836721
3.3224318958476 2.6
3.5 2.73573448954039
3.64510284887959 2.9
3.8 3.06392396905811
3.90572405790523 3.2
4.1 3.46937062844092
4.12209115299895 3.5
4.34224786404277 3.8
4.4 3.90275588817715
4.54590704299425 4.1
4.7 4.38778878749724
4.70937234657086 4.4
4.95588259706151 4.7
5 4.76152778978305
5 5
4.94760649204131 5
4.7 4.71872180016013
4.68713156276973 4.7
4.48342176395384 4.4
4.4 4.29524565497129
4.27992344710325 4.1
4.1 3.87645330314255
4.04228274791067 3.8
3.8 3.52768805322644
3.77383550276807 3.5
3.5 3.22524488136553
3.47306820687712 3.2
3.2 2.94507904103759
3.13925110445225 2.9
2.9 2.70630146060337
2.64088675053818 2.6
2.6 2.57755797080331
2.3 2.47376231331063
2 2.52231544214065
1.90771713167319 2.6
1.7 2.65996502949774
1.4 2.88660485963969
1.38082843913669 2.9
1.1 3.13385424912852
1.07952101235373 3.2
1.09274828921367 3.5
1.1 3.52005314779888
1.15951183412615 3.5
1.4 3.37156021924562
1.7 3.43161703812391
1.72885102828863 3.5
1.89675381867829 3.8
1.97392347882371 4.1
2 4.20141816138681
2.09390233389082 4.4
2.19552829406722 4.7
2.24107341546226 5
2.24091629378773 5
2.19518211237809 4.7
2.09300159725617 4.4
2 4.20332301219939
1.97343370577051 4.1
1.89535687885199 3.8
1.72375367772458 3.5
1.7 3.44369882341777
1.4 3.38649004225486
1.18746614649903 3.5
1.1 3.52947265176579
1.08934196521886 3.5
1.06404099744745 3.2
1.1 3.08385484353467
1.32078567710432 2.9
1.4 2.84465307330477
1.7 2.62668121617475
1.7924229628467 2.6
2 2.42525976223558
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
2 2.52231544214065
2.3 2.47376231331063
2.6 2.57755797080331
2.64088675053818 2.6
2.9 2.70630146060337
3.13925110445225 2.9
3.2 2.94507904103759
3.47306820687712 3.2
3.5 3.22524488136553
3.77383550276807 3.5
3.8 3.52768805322644
4.04228274791067 3.8
4.1 3.87645330314255
4.27992344710325 4.1
4.4 4.29524565497129
4.48342176395384 4.4
4.68713156276973 4.7
4.7 4.71872180016013
4.94760649204131 5
4.82287467299723 5
4.7 4.86041574862744
4.58973816757452 4.7
4.4 4.47241203253226
4.35268041730329 4.4
4.11045301535021 4.1
4.1 4.08701260401932
3.88332422357066 3.8
3.8 3.70634833998874
3.6050061329233 3.5
3.5 3.39464122724392
3.29235246981701 3.2
3.2 3.11378498274282
2.91190155585853 2.9
2.9 2.89036445833083
2.6 2.67364885694615
2.3 2.60141428896215
2 2.60704079489638
1.7 2.69324884282074
1.42962807658428 2.9
1.4 2.91827908460285
1.1 3.18385365472237
1.09500102726001 3.2
1.09615461320848 3.5
1.1 3.51063364383197
1.13155752175326 3.5
1.4 3.35663039623638
1.7 3.41953525283005
1.73394837885267 3.5
1.89815075850459 3.8
1.9744132518769 4.1
2 4.19951331057423
2.09480307052547 4.4
2.19587447575635 4.7
2.2412305371368 5
2.24107341546226 5
2.19552829406722 4.7
2.09390233389082 4.4
2 4.20141816138681
1.97392347882371 4.1
1.89675381867829 3.8
1.72885102828863 3.5
1.7 3.43161703812391
1.4 3.37156021924562
1.15951183412615 3.5
1.1 3.52005314779888
1.09274828921367 3.5
1.07952101235373 3.2
1.1 3.13385424912852
1.38082843913669 2.9
1.4 2.88660485963969
1.7 2.65996502949774
1.90771713167319 2.6
2 2.52231544214065
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
1.7 2.69324884282074
2 2.60704079489638
2.3 2.60141428896215
2.6 2.67364885694615
2.9 2.89036445833083
2.91190155585853 2.9
3.2 3.11378498274282
3.29235246981701 3.2
3.5 3.39464122724392
3.6050061329233 3.5
3.8 3.70634833998874
3.88332422357066 3.8
4.1 4.08701260401932
4.11045301535021 4.1
4.35268041730329 4.4
4.4 4.47241203253226
4.58973816757452 4.7
4.7 4.86041574862744
4.82287467299723 5
4.7 5
4.69931930341273 5
4.49234477237932 4.7
4.4 4.58923388835921
4.27634004576182 4.4
4.1 4.18666109028295
4.03320888755639 4.1
3.8 3.83804399797351
3.76608431589027 3.8
3.5 3.52758702957535
3.47322586023434 3.5
3.2 3.23374686398312
3.16241309468706 3.2
2.9 2.96518521112175
2.79627870695943 2.9
2.6 2.75468237202898
2.3 2.64625083280749
2 2.64231748842646
1.7 2.72653265614374
1.47315387227763 2.9
1.4 2.94513238706486
1.11997612328179 3.2
1.4 3.34170057322715
1.7 3.40745346753619
1.73904572941672 3.5
1.89954769833089 3.8
1.9749030249301 4.1
2 4.19760845976165
2.09570380716013 4.4
2.19622065744548 4.7
2.24138765881133 5
2.2412305371368 5
2.19587447575635 4.7
2.09480307052547 4.4
2 4.19951331057423
1.9744132518769 4.1
1.89815075850459 3.8
1.73394837885267 3.5
1.7 3.41953525283005
1.4 3.35663039623638
1.13155752175326 3.5
1.1 3.51063364383197
1.09615461320848 3.5
1.09500102726001 3.2
1.1 3.18385365472237
1.4 2.91827908460285
1.42962807658428 2.9
1.7 2.69324884282074

1.09956093720328 3.5
1.1 3.50121413986505
1.10360320938038 3.5
1.1 3.45202163753907
1.09956093720328 3.5
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
1.7 2.72653265614374
2 2.64231748842646
2.3 2.64625083280749
2.6 2.75468237202898
2.79627870695943 2.9
2.9 2.96518521112175
3.16241309468706 3.2
3.2 3.23374686398312
3.47322586023434 3.5
3.5 3.52758702957535
3.76608431589027 3.8
3.8 3.83804399797351
4.03320888755639 4.1
4.1 4.18666109028295
4.27634004576182 4.4
4.4 4.58923388835921
4.49234477237931 4.7
4.69931930341273 5
4.65360156156293 5
4.4 4.70277752460084
4.39808548899427 4.7
4.19999967422034 4.4
4.1 4.27901885032374
3.96202725903332 4.1
3.8 3.91800001946574
3.69480465780888 3.8
3.5 3.60056203121661
3.40240116749219 3.5
3.2 3.30276411049798
3.08554240498349 3.2
2.9 3.03397131646148
2.68682774919946 2.9
2.6 2.83571588711181
2.3 2.69108737665284
2 2.67759418195654
1.7 2.75981646946673
1.51667966797098 2.9
1.4 2.97198568952687
1.14947993418777 3.2
1.4 3.32677075021791
1.7 3.39537168224233
1.74414307998077 3.5
1.90094463815719 3.8
1.9753927979833 4.1
2 4.19570360894907
2.09660454379478 4.4
2.19656683913461 4.7
2.24154478048586 5
2.24138765881133 5
2.19622065744548 4.7
2.09570380716013 4.4
2 4.19760845976165
1.9749030249301 4.1
1.89954769833089 3.8
1.73904572941672 3.5
1.7 3.40745346753619
1.4 3.34170057322715
1.11997612328179 3.2
1.4 2.94513238706486
1.47315387227763 2.9
1.7 2.72653265614374
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
1.1 3.45202163753907
1.10360320938038 3.5
1.1 3.50121413986505
1.09956093720328 3.5
1.1 3.45202163753907
};
\addplot [draw=none, fill=lavender231240249]
table{%
x  y
1.7 2.75981646946673
2 2.67759418195654
2.3 2.69108737665284
2.6 2.83571588711181
2.68682774919946 2.9
2.9 3.03397131646148
3.08554240498349 3.2
3.2 3.30276411049798
3.40240116749219 3.5
3.5 3.60056203121661
3.69480465780888 3.8
3.8 3.91800001946574
3.96202725903332 4.1
4.1 4.27901885032374
4.19999967422034 4.4
4.39808548899427 4.7
4.4 4.70277752460084
4.65360156156293 5
4.60788381971312 5
4.4 4.7563589785892
4.36115250077418 4.7
4.12365930267887 4.4
4.1 4.37137661036454
3.89084563051024 4.1
3.8 3.99795604095798
3.62352499972749 3.8
3.5 3.67353703285787
3.33157647475004 3.5
3.2 3.37178135701285
3.00867171527993 3.2
2.9 3.1027574218012
2.6 2.90685201788372
2.58396089860653 2.9
2.3 2.73592392049818
2 2.71287087548662
1.7 2.79310028278973
1.56020546366433 2.9
1.4 2.99883899198887
1.17898374509376 3.2
1.4 3.31184092720867
1.7 3.38328989694847
1.74924043054482 3.5
1.90234157798348 3.8
1.97588257103649 4.1
2 4.19379875813649
2.09750528042943 4.4
2.19691302082374 4.7
2.2417019021604 5
2.24154478048586 5
2.19656683913461 4.7
2.09660454379478 4.4
2 4.19570360894907
1.9753927979833 4.1
1.90094463815719 3.8
1.74414307998077 3.5
1.7 3.39537168224233
1.4 3.32677075021791
1.14947993418777 3.2
1.4 2.97198568952687
1.51667966797098 2.9
1.7 2.75981646946673
};
\addplot [draw=none, fill=aliceblue242247253]
table{%
x  y
1.7 2.79310028278973
2 2.71287087548662
2.3 2.73592392049818
2.58396089860653 2.9
2.6 2.90685201788372
2.9 3.1027574218012
3.00867171527993 3.2
3.2 3.37178135701285
3.33157647475004 3.5
3.5 3.67353703285787
3.62352499972749 3.8
3.8 3.99795604095798
3.89084563051024 4.1
4.1 4.37137661036454
4.12365930267887 4.4
4.36115250077418 4.7
4.4 4.7563589785892
4.60788381971312 5
4.56216607786332 5
4.4 4.80994043257755
4.3242195125541 4.7
4.1 4.43062009586644
4.07672182832891 4.4
3.81966400198717 4.1
3.8 4.07791206245021
3.55224534164609 3.8
3.5 3.74651203449913
3.26075178200789 3.5
3.2 3.44079860352771
2.93180102557637 3.2
2.9 3.17154352714093
2.6 2.94000204246824
2.50636381486713 2.9
2.3 2.78076046434352
2 2.74814756901669
1.7 2.82638409611272
1.60373125935768 2.9
1.4 3.02569229445088
1.20848755599974 3.2
1.4 3.29691110419944
1.7 3.37120811165461
1.75433778110886 3.5
1.90373851780978 3.8
1.97637234408969 4.1
2 4.19189390732391
2.09840601706408 4.4
2.19725920251287 4.7
2.24185902383493 5
2.2417019021604 5
2.19691302082374 4.7
2.09750528042943 4.4
2 4.19379875813649
1.97588257103649 4.1
1.90234157798348 3.8
1.74924043054482 3.5
1.7 3.38328989694847
1.4 3.31184092720867
1.17898374509376 3.2
1.4 2.99883899198887
1.56020546366433 2.9
1.7 2.79310028278973
};
\addplot [draw=none, fill=white]
table{%
x  y
1.7 2.82638409611272
2 2.74814756901669
2.3 2.78076046434352
2.50636381486713 2.9
2.6 2.94000204246824
2.9 3.17154352714093
2.93180102557637 3.2
3.2 3.44079860352771
3.26075178200789 3.5
3.5 3.74651203449913
3.55224534164609 3.8
3.8 4.07791206245021
3.81966400198717 4.1
4.07672182832891 4.4
4.1 4.43062009586643
4.3242195125541 4.7
4.4 4.80994043257755
4.56216607786332 5
4.4 5
4.1 5
3.8 5
3.5 5
3.2 5
2.9 5
2.6 5
2.3 5
2.24185902383493 5
2.19725920251287 4.7
2.09840601706408 4.4
2 4.19189390732391
1.97637234408969 4.1
1.90373851780978 3.8
1.75433778110886 3.5
1.7 3.37120811165461
1.4 3.29691110419944
1.20848755599974 3.2
1.4 3.02569229445088
1.60373125935768 2.9
1.7 2.82638409611272
};
\end{axis}



==> fig/tikz/ionosphere/epcvi_Z_1.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=black]
table{%
x  y
-0.7 1.76418255628028
-0.4 1.70051179099733
-0.1 1.92729106872595
-0.0513764617486618 2
0.145121725654417 2.3
0.2 2.38286607490331
0.5 2.35846460635274
0.614913640832791 2.3
0.8 2.17281487565585
1.1 2.26951912854613
1.12155204867612 2.3
1.4 2.48590903489574
1.4774445173367 2.6
1.67825552633863 2.9
1.7 2.93746814026509
1.93351958051193 3.2
2 3.48654998279001
2.01398961239969 3.5
2.26434110560528 3.8
2.29715636766392 4.1
2.3 4.11642094541032
2.5444937063305 4.4
2.58009185708787 4.7
2.59400962409832 5
2.3 5
2 5
1.7 5
1.4 5
1.1 5
0.8 5
0.5 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.88615124440577
-0.7 1.76418255628028
};
\addplot [draw=none, fill=midnightblue854116]
table{%
x  y
-0.7 1.66911186342935
-0.4 1.59979005656838
-0.283447119121194 1.7
-0.1 1.83846946032842
0.00802230533243431 2
0.188053684717284 2.3
0.2 2.31803891009404
0.5 2.32246813388973
0.544161677107852 2.3
0.8 2.12419650451041
1.1 2.2067563185111
1.16592962295157 2.3
1.4 2.45627982783805
1.49755671147543 2.6
1.68067473009942 2.9
1.7 2.93329958381941
1.93722747163615 3.2
2 3.47056789143117
2.0306128820919 3.5
2.26593292545861 3.8
2.2975845974234 4.1
2.3 4.11394807386003
2.54662574507182 4.4
2.58065719884807 4.7
2.59421264279783 5
2.59400962409832 5
2.58009185708787 4.7
2.5444937063305 4.4
2.3 4.11642094541032
2.29715636766392 4.1
2.26434110560528 3.8
2.01398961239969 3.5
2 3.48654998279001
1.93351958051193 3.2
1.7 2.93746814026509
1.67825552633863 2.9
1.4774445173367 2.6
1.4 2.48590903489574
1.12155204867612 2.3
1.1 2.26951912854613
0.8 2.17281487565585
0.614913640832791 2.3
0.5 2.35846460635274
0.2 2.38286607490331
0.145121725654417 2.3
-0.0513764617486619 2
-0.1 1.92729106872595
-0.4 1.70051179099733
-0.7 1.76418255628028
-1 1.88615124440577
-1 1.76340668405334
-0.782960326779908 1.7
-0.7 1.66911186342935
};
\addplot [draw=none, fill=midnightblue868137]
table{%
x  y
-0.7 1.51267914419595
-0.4 1.49861735803137
-0.165774470310466 1.7
-0.1 1.74964785193089
0.0674210724135305 2
0.2 2.22669613651645
0.5 2.27348536779441
0.8 2.07557813336497
1.1 2.14399350847607
1.21030719722703 2.3
1.4 2.42665062078036
1.51766890561416 2.6
1.68309393386021 2.9
1.7 2.92913102737372
1.94093536276037 3.2
2 3.45458580007232
2.04723615178411 3.5
2.26752474531194 3.8
2.29801282718287 4.1
2.3 4.11147520230973
2.54875778381313 4.4
2.58122254060828 4.7
2.59441566149734 5
2.59421264279783 5
2.58065719884807 4.7
2.54662574507182 4.4
2.3 4.11394807386003
2.2975845974234 4.1
2.26593292545861 3.8
2.0306128820919 3.5
2 3.47056789143117
1.93722747163615 3.2
1.7 2.93329958381941
1.68067473009942 2.9
1.49755671147543 2.6
1.4 2.45627982783805
1.16592962295157 2.3
1.1 2.2067563185111
0.8 2.12419650451041
0.544161677107852 2.3
0.5 2.32246813388973
0.2 2.31803891009404
0.188053684717284 2.3
0.00802230533243434 2
-0.1 1.83846946032842
-0.283447119121194 1.7
-0.4 1.59979005656838
-0.7 1.66911186342935
-0.782960326779908 1.7
-1 1.76340668405334
-1 1.7
-1 1.58502040369332
-0.7 1.51267914419595
};
\addplot [draw=none, fill=teal882156]
table{%
x  y
-0.7 1.31008130395418
-0.4 1.39469034533131
-0.395595595842696 1.4
-0.1 1.63806050095035
-0.0644434619724808 1.7
0.126819839494626 2
0.2 2.1251304408493
0.5 2.20293470683296
0.8 2.02695976221954
1.1 2.08123069844105
1.25468477150249 2.3
1.4 2.39702141372268
1.53778109975289 2.6
1.685513137621 2.9
1.7 2.92496247092804
1.94464325388459 3.2
2 3.43860370871348
2.06385942147633 3.5
2.26911656516527 3.8
2.29844105694234 4.1
2.3 4.10900233075943
2.55088982255445 4.4
2.58178788236849 4.7
2.59461868019685 5
2.59441566149734 5
2.58122254060828 4.7
2.54875778381313 4.4
2.3 4.11147520230973
2.29801282718287 4.1
2.26752474531194 3.8
2.04723615178411 3.5
2 3.45458580007232
1.94093536276037 3.2
1.7 2.92913102737372
1.68309393386021 2.9
1.51766890561416 2.6
1.4 2.42665062078036
1.21030719722703 2.3
1.1 2.14399350847607
0.8 2.07557813336497
0.5 2.27348536779441
0.2 2.22669613651645
0.0674210724135305 2
-0.1 1.74964785193089
-0.165774470310466 1.7
-0.4 1.49861735803137
-0.7 1.51267914419595
-1 1.58502040369332
-1 1.4
-1 1.29008641824905
-0.7 1.31008130395418
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 -1
-0.438432188555942 -1
-0.578010907751698 -0.7
-0.664511964806299 -0.4
-0.7 -0.218022750583121
-0.741276791317675 -0.1
-0.803762424257419 0.2
-0.814005066446362 0.5
-0.736159809613695 0.8
-0.7 0.837239558768808
-0.561077336801606 1.1
-0.4 1.18446705417145
-0.221213570019612 1.4
-0.1 1.49762040979868
0.0161765546282249 1.7
0.186218606575723 2
0.2 2.02356474518214
0.5 2.13238404587151
0.742442240418554 2
0.8 1.96460795183122
0.980666506680193 2
1.1 2.01846788840602
1.29906234577795 2.3
1.4 2.36739220666499
1.55789329389162 2.6
1.68793234138179 2.9
1.7 2.92079391448236
1.94835114500881 3.2
2 3.42262161735464
2.08048269116854 3.5
2.2707083850186 3.8
2.29886928670182 4.1
2.3 4.10652945920914
2.55302186129577 4.4
2.58235322412869 4.7
2.59482169889636 5
2.59461868019685 5
2.58178788236849 4.7
2.55088982255445 4.4
2.3 4.10900233075943
2.29844105694234 4.1
2.26911656516527 3.8
2.06385942147633 3.5
2 3.43860370871348
1.94464325388459 3.2
1.7 2.92496247092804
1.685513137621 2.9
1.53778109975289 2.6
1.4 2.39702141372268
1.25468477150249 2.3
1.1 2.08123069844105
0.8 2.02695976221954
0.5 2.20293470683296
0.2 2.1251304408493
0.126819839494626 2
-0.0644434619724808 1.7
-0.1 1.63806050095035
-0.395595595842696 1.4
-0.4 1.39469034533131
-0.7 1.31008130395418
-1 1.29008641824905
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.4 -1
-0.1 -1
-0.0232281421316345 -1
-0.1 -0.833741072297996
-0.169162344752899 -0.7
-0.287555353138361 -0.4
-0.365253350536488 -0.1
-0.4 0.120718721045168
-0.417655945567124 0.2
-0.439877741227798 0.5
-0.4 0.756307667585479
-0.395637990323785 0.8
-0.281045296092595 1.1
-0.1 1.32473816131904
-0.0669230180647825 1.4
0.0967965712289307 1.7
0.2 1.88750803761585
0.340107091088721 2
0.5 2.06183338491005
0.613238904820955 2
0.8 1.88516131057399
1.1 1.93084092442962
1.16090846039056 2
1.34343992005341 2.3
1.4 2.3377629996073
1.57800548803035 2.6
1.69035154514258 2.9
1.7 2.91662535803668
1.95205903613303 3.2
2 3.4066395259958
2.09710596086075 3.5
2.27230020487193 3.8
2.29929751646129 4.1
2.3 4.10405658765884
2.55515390003708 4.4
2.5829185658889 4.7
2.59502471759587 5
2.59482169889636 5
2.58235322412869 4.7
2.55302186129577 4.4
2.3 4.10652945920914
2.29886928670182 4.1
2.2707083850186 3.8
2.08048269116854 3.5
2 3.42262161735464
1.94835114500881 3.2
1.7 2.92079391448236
1.68793234138179 2.9
1.55789329389162 2.6
1.4 2.36739220666499
1.29906234577795 2.3
1.1 2.01846788840602
0.980666506680193 2
0.8 1.96460795183122
0.742442240418554 2
0.5 2.13238404587151
0.2 2.02356474518214
0.186218606575723 2
0.0161765546282249 1.7
-0.1 1.49762040979868
-0.221213570019612 1.4
-0.4 1.18446705417145
-0.561077336801606 1.1
-0.7 0.837239558768808
-0.736159809613695 0.8
-0.814005066446362 0.5
-0.803762424257419 0.2
-0.741276791317675 -0.1
-0.7 -0.218022750583121
-0.664511964806299 -0.4
-0.578010907751698 -0.7
-0.438432188555942 -1
-0.4 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.427650207779054
4.79414269439625 0.2
4.7 0.0963425942742112
4.52168077538323 -0.1
4.4 -0.232934479081172
4.24702624778779 -0.4
4.1 -0.558327560585782
3.96825464333407 -0.7
3.8 -0.876444643413551
3.68166085407058 -1
3.8 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
-0.1 -0.833741072297996
-0.0232281421316345 -1
0.2 -1
0.264874874538866 -1
0.2 -0.895710551189304
0.09094669354407 -0.7
-0.0359159652866374 -0.4
-0.1 -0.190935605642161
-0.130939736549275 -0.1
-0.197140493255724 0.2
-0.221833978668212 0.5
-0.194492289834357 0.8
-0.1 1.05196681938043
-0.0878122944121932 1.1
0.0415629447267126 1.4
0.177416587829636 1.7
0.2 1.74103130437776
0.5 1.98318766707351
0.8 1.80571466931676
1.1 1.83284734497198
1.24721149442765 2
1.38781749432887 2.3
1.4 2.30813379254961
1.59811768216908 2.6
1.69277074890336 2.9
1.7 2.912456801591
1.95576692725725 3.2
2 3.39065743463696
2.11372923055296 3.5
2.27389202472526 3.8
2.29972574622076 4.1
2.3 4.10158371610854
2.5572859387784 4.4
2.58348390764911 4.7
2.59522773629538 5
2.59502471759587 5
2.5829185658889 4.7
2.55515390003708 4.4
2.3 4.10405658765884
2.29929751646129 4.1
2.27230020487193 3.8
2.09710596086075 3.5
2 3.4066395259958
1.95205903613303 3.2
1.7 2.91662535803668
1.69035154514258 2.9
1.57800548803035 2.6
1.4 2.3377629996073
1.34343992005341 2.3
1.16090846039056 2
1.1 1.93084092442961
0.8 1.88516131057399
0.613238904820955 2
0.5 2.06183338491005
0.340107091088721 2
0.2 1.88750803761585
0.0967965712289307 1.7
-0.0669230180647825 1.4
-0.1 1.32473816131904
-0.281045296092595 1.1
-0.395637990323785 0.8
-0.4 0.756307667585479
-0.439877741227798 0.5
-0.417655945567124 0.2
-0.4 0.120718721045168
-0.365253350536488 -0.1
-0.287555353138361 -0.4
-0.169162344752899 -0.7
-0.1 -0.833741072297996
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
3.2 -1
3.5 -1
3.68166085407058 -1
3.8 -0.876444643413551
3.96825464333407 -0.7
4.1 -0.558327560585782
4.24702624778779 -0.4
4.4 -0.232934479081172
4.52168077538323 -0.1
4.7 0.0963425942742112
4.79414269439625 0.2
5 0.427650207779054
5 0.5
5 0.8
5 1.09496918906705
4.71742122202701 0.8
4.7 0.781811170455064
4.42948154788899 0.5
4.4 0.469269234479108
4.14047620710207 0.2
4.1 0.157939182531764
3.84942008608694 -0.1
3.8 -0.151051813900129
3.55448349213952 -0.4
3.5 -0.455651259919661
3.2522964195144 -0.7
3.2 -0.752277578947777
2.93645331103511 -1
3.2 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
0.2 -0.895710551189304
0.264874874538866 -1
0.5 -1
0.542778822852785 -1
0.5 -0.953278570046052
0.332041776298762 -0.7
0.2 -0.452920026894077
0.175182291541177 -0.4
0.0673007811939628 -0.1
-0.00106688868188498 0.2
-0.0310795417841411 0.5
-0.016511534713533 0.8
0.0482815065622026 1.1
0.150048907518208 1.4
0.2 1.51702918066834
0.319903982148411 1.7
0.5 1.84712208956119
0.8 1.72626802805952
1.1 1.73485376551435
1.33351452846473 2
1.4 2.15450162248645
1.45332208982949 2.3
1.6182298763078 2.6
1.69518995266415 2.9
1.7 2.90828824514531
1.95947481838147 3.2
2 3.37467534327812
2.13035250024517 3.5
2.27548384457859 3.8
2.3 4.09315590036418
2.30790660805254 4.1
2.55941797751972 4.4
2.58404924940931 4.7
2.5954307549949 5
2.59522773629538 5
2.58348390764911 4.7
2.5572859387784 4.4
2.3 4.10158371610854
2.29972574622076 4.1
2.27389202472526 3.8
2.11372923055296 3.5
2 3.39065743463696
1.95576692725725 3.2
1.7 2.912456801591
1.69277074890336 2.9
1.59811768216908 2.6
1.4 2.30813379254961
1.38781749432887 2.3
1.24721149442765 2
1.1 1.83284734497198
0.8 1.80571466931676
0.5 1.98318766707351
0.2 1.74103130437776
0.177416587829636 1.7
0.0415629447267126 1.4
-0.0878122944121932 1.1
-0.1 1.05196681938043
-0.194492289834357 0.8
-0.221833978668212 0.5
-0.197140493255724 0.2
-0.130939736549275 -0.1
-0.1 -0.190935605642161
-0.0359159652866374 -0.4
0.09094669354407 -0.7
0.2 -0.895710551189304
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
2.6 -1
2.9 -1
2.93645331103511 -1
3.2 -0.752277578947777
3.2522964195144 -0.7
3.5 -0.455651259919661
3.55448349213952 -0.4
3.8 -0.151051813900129
3.84942008608694 -0.1
4.1 0.157939182531764
4.14047620710207 0.2
4.4 0.469269234479108
4.42948154788899 0.5
4.7 0.781811170455064
4.71742122202701 0.8
5 1.09496918906705
5 1.1
5 1.4
5 1.47596271175951
4.92625004830775 1.4
4.7 1.16742640510358
4.63452152197352 1.1
4.4 0.859230804588626
4.34238416471385 0.8
4.1 0.551866826853851
4.04928323933756 0.5
3.8 0.246347589252107
3.75409493634782 0.2
3.5 -0.0554166293060709
3.45462382018089 -0.1
3.2 -0.350146331127376
3.14657630862738 -0.4
2.9 -0.6326726331646
2.82118016150534 -0.7
2.6 -0.895210599176612
2.45899601340835 -1
2.6 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.5 -0.953278570046052
0.542778822852785 -1
0.8 -1
0.929064773421502 -1
0.8 -0.921712749820649
0.596252574840905 -0.7
0.5 -0.5794336474854
0.398809359818802 -0.4
0.267980033592353 -0.1
0.2 0.121201251107268
0.179913650614282 0.2
0.139867471424222 0.5
0.140945650478088 0.8
0.184375307536598 1.1
0.2 1.15263456478789
0.295886767518987 1.4
0.486465432911747 1.7
0.5 1.71105651204887
0.532476575131271 1.7
0.8 1.60193475617572
1.1 1.60520102111036
1.19854801408933 1.7
1.4 1.95546283681631
1.42402429818967 2
1.52682107910055 2.3
1.63834207044653 2.6
1.69760915642494 2.9
1.7 2.90411968869963
1.96318270950569 3.2
2 3.35869325191928
2.14697576993738 3.5
2.27707566443192 3.8
2.3 4.07412145657398
2.32989604341371 4.1
2.56155001626104 4.4
2.58461459116952 4.7
2.59563377369441 5
2.5954307549949 5
2.58404924940931 4.7
2.55941797751972 4.4
2.30790660805254 4.1
2.3 4.09315590036418
2.27548384457859 3.8
2.13035250024517 3.5
2 3.37467534327812
1.95947481838147 3.2
1.7 2.90828824514531
1.69518995266415 2.9
1.6182298763078 2.6
1.45332208982949 2.3
1.4 2.15450162248645
1.33351452846473 2
1.1 1.73485376551435
0.8 1.72626802805952
0.5 1.84712208956119
0.319903982148411 1.7
0.2 1.51702918066834
0.150048907518208 1.4
0.0482815065622026 1.1
-0.016511534713533 0.8
-0.0310795417841411 0.5
-0.00106688868188501 0.2
0.0673007811939628 -0.1
0.175182291541177 -0.4
0.2 -0.452920026894077
0.332041776298762 -0.7
0.5 -0.953278570046052
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
2 -1
2.3 -1
2.45899601340835 -1
2.6 -0.895210599176612
2.82118016150534 -0.7
2.9 -0.6326726331646
3.14657630862738 -0.4
3.2 -0.350146331127376
3.45462382018089 -0.1
3.5 -0.055416629306071
3.75409493634782 0.2
3.8 0.246347589252107
4.04928323933756 0.5
4.1 0.551866826853851
4.34238416471385 0.8
4.4 0.859230804588626
4.63452152197352 1.1
4.7 1.16742640510358
4.92625004830775 1.4
5 1.47596271175951
5 1.7
5 1.79939478894329
4.90365972456672 1.7
4.7 1.49065325595007
4.61228722041136 1.4
4.4 1.18185722003797
4.32088323883714 1.1
4.1 0.873407726773052
4.02891724844201 0.8
3.8 0.566331627277074
3.73516503257666 0.5
3.5 0.262778798678003
3.43711010830382 0.2
3.2 -0.0333886775865087
3.12975371454942 -0.1
2.9 -0.316073796589874
2.80279158032664 -0.4
2.6 -0.576522891090572
2.43302946285484 -0.7
2.3 -0.80243931176732
2 -0.978838185577959
1.944553026009 -1
2 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
0.8 -0.921712749820649
0.929064773421502 -1
1.1 -1
1.4 -1
1.7 -1
1.944553026009 -1
2 -0.978838185577959
2.3 -0.80243931176732
2.43302946285484 -0.7
2.6 -0.576522891090572
2.80279158032664 -0.4
2.9 -0.316073796589874
3.12975371454942 -0.1
3.2 -0.0333886775865087
3.43711010830383 0.2
3.5 0.262778798678003
3.73516503257666 0.5
3.8 0.566331627277074
4.02891724844201 0.8
4.1 0.873407726773053
4.32088323883714 1.1
4.4 1.18185722003797
4.61228722041136 1.4
4.7 1.49065325595007
4.90365972456672 1.7
5 1.79939478894329
5 2
5 2.11080038010894
4.89327902462079 2
4.7 1.8004736827109
4.60369475222599 1.7
4.4 1.48938025760345
4.31476759258856 1.4
4.1 1.17774453503416
4.02607193332264 1.1
3.8 0.866557260366155
3.7364043418624 0.8
3.5 0.558217404771401
3.44318378675278 0.5
3.2 0.257234539245991
3.14126987405738 0.2
2.9 -0.0292482756930255
2.81999482418905 -0.1
2.6 -0.291298464004867
2.45440736242929 -0.4
2.3 -0.516064986278838
2 -0.686700343927284
1.96069263618483 -0.7
1.7 -0.79431545161167
1.4 -0.823184433720367
1.1 -0.759047101208345
1.00327857360329 -0.7
0.8 -0.55685846645802
0.674573487290526 -0.4
0.5 -0.130947941514419
0.486174626140577 -0.1
0.391068454260696 0.2
0.337242047117545 0.5
0.328161056780403 0.8
0.370852448821876 1.1
0.473599099300429 1.4
0.5 1.44175759656311
0.8 1.45542935151343
1.1 1.4580721227156
1.35149545004045 1.7
1.4 1.76150899865867
1.52864714593847 2
1.60032006837161 2.3
1.65845426458526 2.6
1.7 2.89830709260282
1.7007105810261 2.9
1.96689060062991 3.2
2 3.34271116056044
2.1635990396296 3.5
2.27866748428525 3.8
2.3 4.05508701278379
2.35188547877487 4.1
2.56368205500235 4.4
2.58517993292973 4.7
2.59583679239392 5
2.59563377369441 5
2.58461459116952 4.7
2.56155001626103 4.4
2.32989604341371 4.1
2.3 4.07412145657398
2.27707566443192 3.8
2.14697576993738 3.5
2 3.35869325191928
1.96318270950569 3.2
1.7 2.90411968869963
1.69760915642494 2.9
1.63834207044653 2.6
1.52682107910055 2.3
1.42402429818967 2
1.4 1.95546283681631
1.19854801408933 1.7
1.1 1.60520102111036
0.8 1.60193475617572
0.532476575131271 1.7
0.5 1.71105651204887
0.486465432911747 1.7
0.295886767518987 1.4
0.2 1.15263456478789
0.184375307536598 1.1
0.140945650478088 0.8
0.139867471424222 0.5
0.179913650614282 0.2
0.2 0.121201251107268
0.267980033592353 -0.1
0.398809359818803 -0.4
0.5 -0.5794336474854
0.596252574840905 -0.7
0.8 -0.921712749820649
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.1 -0.759047101208345
1.4 -0.823184433720367
1.7 -0.79431545161167
1.96069263618483 -0.7
2 -0.686700343927284
2.3 -0.516064986278838
2.45440736242929 -0.4
2.6 -0.291298464004867
2.81999482418905 -0.1
2.9 -0.0292482756930255
3.14126987405738 0.2
3.2 0.257234539245991
3.44318378675278 0.5
3.5 0.558217404771401
3.7364043418624 0.8
3.8 0.866557260366155
4.02607193332264 1.1
4.1 1.17774453503416
4.31476759258856 1.4
4.4 1.48938025760345
4.60369475222599 1.7
4.7 1.8004736827109
4.89327902462079 2
5 2.11080038010894
5 2.3
5 2.440676163264
4.86612790668729 2.3
4.7 2.12691320814114
4.58037304792948 2
4.4 1.81113468654835
4.29637406898901 1.7
4.1 1.49333346954555
4.01371789513495 1.4
3.8 1.17453916892145
3.73107833259665 1.1
3.5 0.857608118826382
3.44572954379575 0.8
3.2 0.547971131002995
3.15248238510874 0.5
2.9 0.25413463426075
2.84069546986163 0.2
2.6 -0.0123014875201433
2.4847138321172 -0.1
2.3 -0.237281713407923
2.0075533317432 -0.4
2 -0.404246379006801
1.7 -0.489621929218694
1.4 -0.484247813291773
1.15334213722251 -0.4
1.1 -0.374960248504133
0.800987850123024 -0.1
0.8 -0.0986479012688937
0.661955691573642 0.2
0.578677595833173 0.5
0.559281385407535 0.8
0.650498798177562 1.1
0.8 1.20375884417856
1.1 1.24686633637272
1.25583099037541 1.4
1.4 1.53517108590083
1.50204763544177 1.7
1.63326999368726 2
1.67381905764268 2.3
1.67856645872399 2.6
1.7 2.75389732107041
1.76132514494433 2.9
1.97059849175413 3.2
2 3.3267290692016
2.18022230932181 3.5
2.28025930413858 3.8
2.3 4.03605256899359
2.37387491413604 4.1
2.56581409374367 4.4
2.58574527468993 4.7
2.59603981109343 5
2.59583679239392 5
2.58517993292973 4.7
2.56368205500235 4.4
2.35188547877487 4.1
2.3 4.05508701278379
2.27866748428525 3.8
2.1635990396296 3.5
2 3.34271116056044
1.96689060062991 3.2
1.7007105810261 2.9
1.7 2.89830709260282
1.65845426458526 2.6
1.60032006837161 2.3
1.52864714593847 2
1.4 1.76150899865867
1.35149545004045 1.7
1.1 1.4580721227156
0.8 1.45542935151343
0.5 1.44175759656311
0.473599099300429 1.4
0.370852448821876 1.1
0.328161056780403 0.8
0.337242047117545 0.5
0.391068454260696 0.2
0.486174626140577 -0.1
0.5 -0.130947941514419
0.674573487290526 -0.4
0.8 -0.55685846645802
1.00327857360329 -0.7
1.1 -0.759047101208345
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.4 -0.484247813291773
1.7 -0.489621929218694
2 -0.404246379006801
2.0075533317432 -0.4
2.3 -0.237281713407923
2.4847138321172 -0.1
2.6 -0.0123014875201433
2.84069546986163 0.2
2.9 0.25413463426075
3.15248238510874 0.5
3.2 0.547971131002995
3.44572954379575 0.8
3.5 0.857608118826382
3.73107833259665 1.1
3.8 1.17453916892145
4.01371789513495 1.4
4.1 1.49333346954555
4.29637406898901 1.7
4.4 1.81113468654835
4.58037304792948 2
4.7 2.12691320814114
4.86612790668729 2.3
5 2.440676163264
5 2.6
5 2.82459743929917
4.79071188311493 2.6
4.7 2.50392235437445
4.5131019242183 2.3
4.4 2.17896729785815
4.23895408186587 2
4.1 1.84960740311131
3.96734309758018 1.7
3.8 1.51733246373604
3.69625282528228 1.4
3.5 1.1860293452056
3.42244789385135 1.1
3.2 0.86251592537153
3.14052161459968 0.8
2.9 0.55696807454509
2.83962970982684 0.5
2.6 0.283087954525548
2.49265028904649 0.2
2.3 0.0570803170097792
2.00858477252396 -0.1
2 -0.104497822356076
1.7 -0.158595895935631
1.43442337682212 -0.1
1.4 -0.0876536728651526
1.1 0.189332361741858
1.09212246452768 0.2
0.98295564042865 0.5
1.0197309947661 0.8
1.1 0.868833383076249
1.25635751644895 1.1
1.4 1.24007027977027
1.49350889229173 1.4
1.65148743727714 1.7
1.7 1.84179785587742
1.76842603805294 2
1.82084609815222 2.3
1.7 2.57222001043378
1.69867865286272 2.6
1.7 2.609487549538
1.82193970886256 2.9
1.97430638287835 3.2
2 3.31074697784276
2.19684557901402 3.5
2.28185112399191 3.8
2.3 4.01701812520339
2.39586434949721 4.1
2.56794613248499 4.4
2.58631061645014 4.7
2.59624282979294 5
2.59603981109343 5
2.58574527468993 4.7
2.56581409374367 4.4
2.37387491413604 4.1
2.3 4.03605256899359
2.28025930413858 3.8
2.18022230932181 3.5
2 3.3267290692016
1.97059849175413 3.2
1.76132514494433 2.9
1.7 2.75389732107041
1.67856645872399 2.6
1.67381905764268 2.3
1.63326999368726 2
1.50204763544177 1.7
1.4 1.53517108590083
1.25583099037541 1.4
1.1 1.24686633637272
0.8 1.20375884417856
0.650498798177562 1.1
0.559281385407535 0.8
0.578677595833173 0.5
0.661955691573642 0.2
0.8 -0.0986479012688937
0.800987850123024 -0.1
1.1 -0.374960248504133
1.15334213722251 -0.4
1.4 -0.484247813291773
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.7 -0.158595895935631
2 -0.104497822356076
2.00858477252396 -0.1
2.3 0.0570803170097792
2.49265028904649 0.2
2.6 0.283087954525548
2.83962970982684 0.5
2.9 0.55696807454509
3.14052161459968 0.8
3.2 0.86251592537153
3.42244789385135 1.1
3.5 1.1860293452056
3.69625282528228 1.4
3.8 1.51733246373604
3.96734309758018 1.7
4.1 1.84960740311131
4.23895408186587 2
4.4 2.17896729785815
4.5131019242183 2.3
4.7 2.50392235437445
4.79071188311493 2.6
5 2.82459743929917
5 2.9
5 3.2
5 3.37100987462944
4.85663889923982 3.2
4.7 3.01983966433805
4.60350812440196 2.9
4.4 2.65877221747196
4.35430664825907 2.6
4.10708687305396 2.3
4.1 2.29197272543022
3.85633925153363 2
3.8 1.93520071817105
3.6040433215455 1.7
3.5 1.58007056549724
3.34610603429117 1.4
3.2 1.23528185695766
3.0767544383216 1.1
2.9 0.912692894582719
2.78393213870162 0.8
2.6 0.628194552147323
2.43451343267391 0.5
2.3 0.40078786773267
2 0.263909379394088
1.7 0.287245340643122
1.51266114945217 0.5
1.49101109535171 0.8
1.58565940466175 1.1
1.7 1.37908556099992
1.70895872208696 1.4
1.85783506116197 1.7
1.95735161581271 2
2 2.24960135676621
2.01518034620009 2.3
2 2.34306175551584
1.93236101177034 2.6
1.88255427278078 2.9
1.97801427400257 3.2
2 3.29476488648392
2.21346884870623 3.5
2.28344294384524 3.8
2.3 3.9979836814132
2.41785378485837 4.1
2.5700781712263 4.4
2.58687595821035 4.7
2.59644584849245 5
2.59624282979294 5
2.58631061645014 4.7
2.56794613248499 4.4
2.39586434949721 4.1
2.3 4.01701812520339
2.28185112399191 3.8
2.19684557901402 3.5
2 3.31074697784276
1.97430638287835 3.2
1.82193970886256 2.9
1.7 2.609487549538
1.69867865286272 2.6
1.7 2.57222001043378
1.82084609815222 2.3
1.76842603805294 2
1.7 1.84179785587742
1.65148743727714 1.7
1.49350889229173 1.4
1.4 1.24007027977027
1.25635751644895 1.1
1.1 0.868833383076249
1.0197309947661 0.8
0.98295564042865 0.5
1.09212246452768 0.2
1.1 0.189332361741858
1.4 -0.0876536728651526
1.43442337682212 -0.1
1.7 -0.158595895935631
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.7 0.287245340643122
2 0.263909379394088
2.3 0.40078786773267
2.43451343267391 0.5
2.6 0.628194552147323
2.78393213870162 0.8
2.9 0.912692894582719
3.0767544383216 1.1
3.2 1.23528185695766
3.34610603429117 1.4
3.5 1.58007056549724
3.6040433215455 1.7
3.8 1.93520071817105
3.85633925153363 2
4.1 2.29197272543022
4.10708687305396 2.3
4.35430664825907 2.6
4.4 2.65877221747196
4.60350812440196 2.9
4.7 3.01983966433805
4.85663889923983 3.2
5 3.37100987462944
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.1 5
3.93363425928545 5
3.8 4.74199605022459
3.78632668295913 4.7
3.77395383358761 4.4
3.8 4.26913911649214
4.08482777866121 4.1
4.1 4.09091082672841
4.26204081255275 3.8
4.23393467081053 3.5
4.12945274366587 3.2
4.1 3.14769462716675
3.97114213904785 2.9
3.80284787551637 2.6
3.8 2.5959572629351
3.59789075811523 2.3
3.5 2.16168183799639
3.38188180430561 2
3.2 1.75380457960993
3.15549666442387 1.7
2.90686057376664 1.4
2.9 1.39228365462069
2.60343984565387 1.1
2.6 1.09668937616658
2.3 0.91602256370281
2 1.03245373935426
1.98587143715 1.1
2 1.18440873780638
2.05291046551846 1.4
2.16856781551944 1.7
2.26553077019054 2
2.3 2.12292107802235
2.38027751907505 2.3
2.44050805184095 2.6
2.3 2.77548498727718
2 2.73112834317938
1.94316883669901 2.9
1.98172216512679 3.2
2 3.27878279512508
2.23009211839844 3.5
2.28503476369857 3.8
2.3 3.978949237623
2.43984322021954 4.1
2.57221020996762 4.4
2.58744129997056 4.7
2.59664886719197 5
2.59644584849245 5
2.58687595821035 4.7
2.5700781712263 4.4
2.41785378485837 4.1
2.3 3.9979836814132
2.28344294384524 3.8
2.21346884870623 3.5
2 3.29476488648392
1.97801427400257 3.2
1.88255427278078 2.9
1.93236101177034 2.6
2 2.34306175551584
2.01518034620009 2.3
2 2.24960135676621
1.95735161581271 2
1.85783506116197 1.7
1.70895872208696 1.4
1.7 1.37908556099992
1.58565940466175 1.1
1.49101109535171 0.8
1.51266114945217 0.5
1.7 0.287245340643122
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
2 1.03245373935426
2.3 0.91602256370281
2.6 1.09668937616658
2.60343984565387 1.1
2.9 1.39228365462069
2.90686057376664 1.4
3.15549666442387 1.7
3.2 1.75380457960993
3.38188180430561 2
3.5 2.16168183799639
3.59789075811523 2.3
3.8 2.5959572629351
3.80284787551637 2.6
3.97114213904785 2.9
4.1 3.14769462716675
4.12945274366587 3.2
4.23393467081053 3.5
4.26204081255275 3.8
4.1 4.09091082672841
4.08482777866121 4.1
3.8 4.26913911649214
3.77395383358761 4.4
3.78632668295913 4.7
3.8 4.74199605022459
3.93363425928545 5
3.8 5
3.70198926938805 5
3.53627089102306 4.7
3.5 4.63748534302217
3.37525179896783 4.4
3.2 4.15597299306176
3.16958167646142 4.1
2.97582268448817 3.8
2.9 3.70486342257082
2.73808540842588 3.5
2.6 3.37878715021883
2.45980493493789 3.2
2.3 3.0786262811969
2 2.90469084788944
1.98543005625101 3.2
2 3.26280070376624
2.24671538809065 3.5
2.2866265835519 3.8
2.3 3.9599147938328
2.46183265558071 4.1
2.57434224870894 4.4
2.58800664173076 4.7
2.59685188589148 5
2.59664886719197 5
2.58744129997056 4.7
2.57221020996762 4.4
2.43984322021954 4.1
2.3 3.978949237623
2.28503476369857 3.8
2.23009211839844 3.5
2 3.27878279512508
1.98172216512679 3.2
1.94316883669901 2.9
2 2.73112834317938
2.3 2.77548498727718
2.44050805184095 2.6
2.38027751907505 2.3
2.3 2.12292107802235
2.26553077019054 2
2.16856781551944 1.7
2.05291046551846 1.4
2 1.18440873780638
1.98587143715 1.1
2 1.03245373935426
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
2 2.90469084788944
2.3 3.0786262811969
2.45980493493789 3.2
2.6 3.37878715021883
2.73808540842588 3.5
2.9 3.70486342257082
2.97582268448817 3.8
3.16958167646142 4.1
3.2 4.15597299306176
3.37525179896783 4.4
3.5 4.63748534302217
3.53627089102306 4.7
3.70198926938805 5
3.55439726078757 5
3.5 4.90962953042447
3.40548773172412 4.7
3.2 4.43250623997585
3.18141631009706 4.4
2.99826873214388 4.1
2.9 3.97590285382531
2.78110475858915 3.8
2.6 3.60395548480232
2.53116314142509 3.5
2.3 3.24826834809527
2.26333865778287 3.5
2.28821840340523 3.8
2.3 3.94088035004261
2.48382209094188 4.1
2.57647428745025 4.4
2.58857198349097 4.7
2.59705490459099 5
2.59685188589148 5
2.58800664173076 4.7
2.57434224870894 4.4
2.46183265558071 4.1
2.3 3.9599147938328
2.2866265835519 3.8
2.24671538809065 3.5
2 3.26280070376624
1.98543005625101 3.2
2 2.90469084788944

1.98913794737523 3.2
2 3.2468186124074
2.26215642951177 3.2
2 2.97984379308096
1.98913794737523 3.2
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
2 2.97984379308096
2.26215642951177 3.2
2 3.2468186124074
1.98913794737523 3.2
2 2.97984379308096

1.99284583849945 3.2
2 3.23083652104855
2.17266620775323 3.2
2 3.05499673827248
1.99284583849945 3.2
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
2.3 3.24826834809527
2.53116314142509 3.5
2.6 3.60395548480232
2.78110475858916 3.8
2.9 3.97590285382531
2.99826873214388 4.1
3.18141631009706 4.4
3.2 4.43250623997585
3.40548773172412 4.7
3.5 4.90962953042447
3.55439726078757 5
3.5 5
3.46269809476813 5
3.29494044802696 4.7
3.2 4.57641122315173
3.09914639561862 4.4
2.9 4.14492887314355
2.87284055603094 4.1
2.63487754370904 3.8
2.6 3.76224532584902
2.42634735972105 3.5
2.3 3.36241046310279
2.27996192747508 3.5
2.28981022325856 3.8
2.3 3.92184590625241
2.50581152630304 4.1
2.57860632619157 4.4
2.58913732525118 4.7
2.5972579232905 5
2.59705490459099 5
2.58857198349097 4.7
2.57647428745025 4.4
2.48382209094188 4.1
2.3 3.94088035004261
2.28821840340523 3.8
2.26333865778287 3.5
2.3 3.24826834809527
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
2 3.05499673827248
2.17266620775323 3.2
2 3.23083652104856
1.99284583849945 3.2
2 3.05499673827248

1.99655372962367 3.2
2 3.21485442968971
2.0831759859947 3.2
2 3.130149683464
1.99655372962367 3.2
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
2.3 3.36241046310279
2.42634735972105 3.5
2.6 3.76224532584902
2.63487754370904 3.8
2.87284055603094 4.1
2.9 4.14492887314355
3.09914639561862 4.4
3.2 4.57641122315173
3.29494044802696 4.7
3.46269809476813 5
3.40362327298902 5
3.2 4.71180401399151
3.19343367122303 4.7
3.01687648114017 4.4
2.9 4.25030200694903
2.80914263700477 4.1
2.6 3.85647824155238
2.52780096166421 4.1
2.58073836493289 4.4
2.58970266701138 4.7
2.59746094199001 5
2.5972579232905 5
2.58913732525118 4.7
2.57860632619157 4.4
2.50581152630304 4.1
2.3 3.92184590625241
2.28981022325856 3.8
2.27996192747508 3.5
2.3 3.36241046310279

2.29658519716729 3.5
2.29140204311189 3.8
2.3 3.90281146246221
2.56293172509084 3.8
2.32153157801701 3.5
2.3 3.47655257811032
2.29658519716729 3.5
};
\addplot [draw=none, fill=lavender231240249]
table{%
x  y
2 3.130149683464
2.0831759859947 3.2
2 3.21485442968971
1.99655372962367 3.2
2 3.130149683464
};
\addplot [draw=none, fill=lavender231240249]
table{%
x  y
2.3 3.47655257811032
2.32153157801701 3.5
2.56293172509084 3.8
2.3 3.90281146246221
2.29140204311189 3.8
2.29658519716729 3.5
2.3 3.47655257811032

2.29299386296522 3.8
2.3 3.88377701867202
2.51425272547307 3.8
2.3 3.5458770190118
2.29299386296522 3.8
};
\addplot [draw=none, fill=lavender231240249]
table{%
x  y
2.6 3.85647824155238
2.80914263700477 4.1
2.9 4.25030200694903
3.01687648114017 4.4
3.19343367122303 4.7
3.2 4.71180401399151
3.40362327298902 5
3.34454845120992 5
3.2 4.7954149208441
3.14692265351925 4.7
2.93460656666173 4.4
2.9 4.35567514075451
2.7454447179786 4.1
2.6 3.93064690210318
2.54979039702538 4.1
2.5828704036742 4.4
2.59026800877159 4.7
2.59766396068952 5
2.59746094199001 5
2.58970266701138 4.7
2.58073836493289 4.4
2.52780096166421 4.1
2.6 3.85647824155238
};
\addplot [draw=none, fill=aliceblue242247253]
table{%
x  y
2.3 3.5458770190118
2.51425272547307 3.8
2.3 3.88377701867202
2.29299386296522 3.8
2.3 3.5458770190118

2.29458568281855 3.8
2.3 3.86474257488182
2.46557372585529 3.8
2.3 3.60361468590532
2.29458568281855 3.8
};
\addplot [draw=none, fill=aliceblue242247253]
table{%
x  y
2.6 3.93064690210318
2.7454447179786 4.1
2.9 4.35567514075451
2.93460656666173 4.4
3.14692265351925 4.7
3.2 4.7954149208441
3.34454845120992 5
3.28547362943082 5
3.2 4.87902582769669
3.10041163581547 4.7
2.9 4.43555579989751
2.87717202218616 4.4
2.68174679895243 4.1
2.6 4.00481556265398
2.57177983238654 4.1
2.58500244241552 4.4
2.5908333505318 4.7
2.59786697938903 5
2.59766396068952 5
2.59026800877159 4.7
2.58287040367421 4.4
2.54979039702538 4.1
2.6 3.93064690210318
};
\addplot [draw=none, fill=white]
table{%
x  y
2.3 3.60361468590532
2.46557372585529 3.8
2.3 3.86474257488182
2.29458568281855 3.8
2.3 3.60361468590532
};
\addplot [draw=none, fill=white]
table{%
x  y
2.6 4.00481556265398
2.68174679895243 4.1
2.87717202218616 4.4
2.9 4.43555579989751
3.10041163581547 4.7
3.2 4.87902582769669
3.28547362943082 5
3.2 5
2.9 5
2.6 5
2.59786697938903 5
2.5908333505318 4.7
2.58500244241552 4.4
2.57177983238654 4.1
2.6 4.00481556265398
};
\end{axis}



==> fig/tikz/ionosphere/epcvi_Z_2.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=black]
table{%
x  y
-0.4 1.92644084732426
-0.324349008381272 2
-0.1 2.26984666742348
-0.0827350376026435 2.3
0.103196779931219 2.6
0.2 2.63492995565039
0.386103802860905 2.6
0.5 2.52502873166884
0.8 2.33977642989771
1.1 2.46890912658319
1.19735965805778 2.6
1.35162424412567 2.9
1.4 3.05664456591048
1.46114103264829 3.2
1.5439660228546 3.5
1.61283705179227 3.8
1.6660466314657 4.1
1.69999973257785 4.4
1.7 4.50043071870572
1.73901202109268 4.7
1.99999999975129 5
1.7 5
1.4 5
1.1 5
0.8 5
0.5 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2.20305724097009
-0.7 2.00054785047147
-0.696607586845095 2
-0.4 1.92644084732426
};
\addplot [draw=none, fill=midnightblue854116]
table{%
x  y
-0.7 1.89284257007716
-0.4 1.84338130049253
-0.238927455078163 2
-0.1 2.1671017448972
-0.0239061430042111 2.3
0.144217186297553 2.6
0.2 2.62012837183821
0.307242235918708 2.6
0.5 2.47311873076672
0.8 2.30295062704891
1.1 2.4155572473727
1.2369834745851 2.6
1.37542237124707 2.9
1.4 2.9795843272633
1.4940071921834 3.2
1.57007525704023 3.5
1.63471718882191 3.8
1.68050773608995 4.1
1.7 4.31418377390753
1.72369149027536 4.4
1.78169670616749 4.7
1.99999999979646 5
1.99999999975129 5
1.73901202109268 4.7
1.7 4.50043071870572
1.69999973257785 4.4
1.6660466314657 4.1
1.61283705179227 3.8
1.5439660228546 3.5
1.46114103264829 3.2
1.4 3.05664456591048
1.35162424412567 2.9
1.19735965805778 2.6
1.1 2.46890912658319
0.8 2.33977642989771
0.5 2.52502873166884
0.386103802860905 2.6
0.2 2.63492995565039
0.103196779931219 2.6
-0.0827350376026435 2.3
-0.1 2.26984666742348
-0.324349008381272 2
-0.4 1.92644084732426
-0.696607586845095 2
-0.7 2.00054785047147
-1 2.20305724097009
-1 2.09492216815876
-0.858999904400612 2
-0.7 1.89284257007716
};
\addplot [draw=none, fill=midnightblue868137]
table{%
x  y
-0.7 1.7845886180168
-0.4 1.76032175366079
-0.153505901775055 2
-0.1 2.06435682237092
0.0349227515942213 2.3
0.185237592663887 2.6
0.2 2.60532678802603
0.22838066897651 2.6
0.5 2.4212087298646
0.715215002390359 2.3
0.8 2.24526455319107
0.932304156557288 2.3
1.1 2.3622053681622
1.27660729111242 2.6
1.39922049836846 2.9
1.4 2.90252408861612
1.52687335171852 3.2
1.59618449122586 3.5
1.65659732585155 3.8
1.69496884071419 4.1
1.7 4.15528309528007
1.76755957972497 4.4
1.8243813912423 4.7
1.99999999984163 5
1.99999999979646 5
1.78169670616749 4.7
1.72369149027536 4.4
1.7 4.31418377390753
1.68050773608995 4.1
1.63471718882191 3.8
1.57007525704023 3.5
1.4940071921834 3.2
1.4 2.9795843272633
1.37542237124707 2.9
1.2369834745851 2.6
1.1 2.4155572473727
0.8 2.30295062704891
0.5 2.47311873076672
0.307242235918708 2.6
0.2 2.62012837183821
0.144217186297553 2.6
-0.0239061430042111 2.3
-0.1 2.1671017448972
-0.238927455078163 2
-0.4 1.84338130049253
-0.7 1.89284257007716
-0.858999904400612 2
-1 2.09492216815876
-1 2
-1 1.97245088537635
-0.7 1.7845886180168
};
\addplot [draw=none, fill=teal882156]
table{%
x  y
-0.7 1.64978993213216
-0.4 1.6571880340414
-0.362799118908943 1.7
-0.1 1.9514247687824
-0.0718244079208755 2
0.0937516461926536 2.3
0.2 2.52149543284939
0.5 2.36929872896247
0.623044983112751 2.3
0.8 2.18576148861855
1.07613239273343 2.3
1.1 2.30885348895171
1.31623110763974 2.6
1.4 2.80582907142115
1.44419192467452 2.9
1.55973951125363 3.2
1.62229372541149 3.5
1.67847746288118 3.8
1.7 3.98040502880621
1.73459773513846 4.1
1.81142766917457 4.4
1.86706607631711 4.7
1.9999999998868 5
1.99999999984163 5
1.8243813912423 4.7
1.76755957972497 4.4
1.7 4.15528309528007
1.69496884071419 4.1
1.65659732585155 3.8
1.59618449122586 3.5
1.52687335171852 3.2
1.4 2.90252408861612
1.39922049836846 2.9
1.27660729111242 2.6
1.1 2.3622053681622
0.932304156557288 2.3
0.8 2.24526455319107
0.715215002390359 2.3
0.5 2.4212087298646
0.22838066897651 2.6
0.2 2.60532678802603
0.185237592663887 2.6
0.0349227515942213 2.3
-0.1 2.06435682237092
-0.153505901775055 2
-0.4 1.76032175366079
-0.7 1.7845886180168
-1 1.97245088537635
-1 1.74698755282003
-0.853584783159644 1.7
-0.7 1.64978993213216
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 -1
-0.59647122917149 -1
-0.7 -0.750651190354067
-0.72930210711376 -0.7
-0.872608389477208 -0.4
-0.960165968496895 -0.1
-1 0.113450556486823
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.79856735459872 1.4
-0.7 1.42011059315021
-0.4 1.50079895684448
-0.226906937027633 1.7
-0.1 1.82141420957393
0.00358695689234252 2
0.152580540791086 2.3
0.2 2.39885511884737
0.5 2.31738872806035
0.530874963835143 2.3
0.8 2.12625842404602
1.1 2.23483484812282
1.1553785063278 2.3
1.35585492416706 2.6
1.4 2.70846914302547
1.48988036257047 2.9
1.59260567078875 3.2
1.64840295959711 3.5
1.7 3.79753928665749
1.70095451743336 3.8
1.78765440192099 4.1
1.85529575862417 4.4
1.90975076139192 4.7
1.99999999993196 5
1.9999999998868 5
1.86706607631711 4.7
1.81142766917457 4.4
1.73459773513846 4.1
1.7 3.98040502880621
1.67847746288118 3.8
1.62229372541149 3.5
1.55973951125363 3.2
1.44419192467452 2.9
1.4 2.80582907142115
1.31623110763974 2.6
1.1 2.30885348895171
1.07613239273343 2.3
0.8 2.18576148861855
0.623044983112751 2.3
0.5 2.36929872896247
0.2 2.52149543284939
0.0937516461926536 2.3
-0.0718244079208755 2
-0.1 1.9514247687824
-0.362799118908943 1.7
-0.4 1.6571880340414
-0.7 1.64978993213216
-0.853584783159644 1.7
-1 1.74698755282003
-1 1.7
-1 1.4
-1 1.18086407565795
-0.79856735459872 1.4
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.7 -0.750651190354067
-0.59647122917149 -1
-0.4 -1
-0.1 -1
-0.0998397950129974 -1
-0.1 -0.999715551296465
-0.277183587179175 -0.7
-0.398450585361596 -0.4
-0.4 -0.395173232854723
-0.517843170979797 -0.1
-0.592048490775595 0.2
-0.632567128172627 0.5
-0.639160370580398 0.8
-0.577837747141335 1.1
-0.4 1.28030499481473
-0.336126449773367 1.4
-0.1 1.6856278665277
-0.0928237339854743 1.7
0.0789983217055606 2
0.2 2.26764921349323
0.5 2.23564195249353
0.8 2.0667553594735
1.1 2.15670430696244
1.22177523131665 2.3
1.39547874069438 2.6
1.4 2.6111092146298
1.53556880046642 2.9
1.62547183032387 3.2
1.67451219378274 3.5
1.7 3.64697788131124
1.759357698215 3.8
1.84071106870353 4.1
1.89916384807377 4.4
1.95243544646672 4.7
1.99999999997713 5
1.99999999993196 5
1.90975076139192 4.7
1.85529575862417 4.4
1.78765440192099 4.1
1.70095451743336 3.8
1.7 3.79753928665749
1.64840295959711 3.5
1.59260567078875 3.2
1.48988036257047 2.9
1.4 2.70846914302547
1.35585492416706 2.6
1.1553785063278 2.3
1.1 2.23483484812282
0.8 2.12625842404602
0.530874963835143 2.3
0.5 2.31738872806035
0.2 2.39885511884737
0.152580540791086 2.3
0.00358695689234252 2
-0.1 1.82141420957393
-0.226906937027633 1.7
-0.4 1.50079895684448
-0.7 1.42011059315021
-0.79856735459872 1.4
-1 1.18086407565795
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 0.113450556486823
-0.960165968496895 -0.1
-0.872608389477208 -0.4
-0.72930210711376 -0.7
-0.7 -0.750651190354067
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.427421317076998
4.79450314535937 0.2
4.7 0.0958949142585274
4.52228760720803 -0.1
4.4 -0.2336839213476
4.24798564389403 -0.4
4.1 -0.559514565995753
3.96972454952689 -0.7
3.8 -0.878258823528987
3.68387615330652 -1
3.8 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
-0.1 -0.999715551296465
-0.0998397950129974 -1
0.2 -1
0.206482520397573 -1
0.2 -0.990926472203802
0.0151087288138017 -0.7
-0.1 -0.461671877638938
-0.131110231292802 -0.4
-0.248074069088806 -0.1
-0.323496268141078 0.2
-0.364415940460755 0.5
-0.36688409754387 0.8
-0.307724704776282 1.1
-0.156433987985149 1.4
-0.1 1.46826477763639
0.015709585067667 1.7
0.154409686518778 2
0.2 2.10084332480469
0.5 2.13886607984736
0.8 2.00725229490098
1.1 2.07857376580205
1.28817195630549 2.3
1.4 2.49659354702545
1.45501810345972 2.6
1.58125723836236 2.9
1.65833798985898 3.2
1.7 3.49447098323229
1.70176007255307 3.5
1.81776087899664 3.8
1.89376773548607 4.1
1.94303193752337 4.4
1.99512013154153 4.7
2 4.75640343984717
2.04430760588377 5
2 5
1.99999999997713 5
1.95243544646672 4.7
1.89916384807377 4.4
1.84071106870353 4.1
1.759357698215 3.8
1.7 3.64697788131124
1.67451219378274 3.5
1.62547183032387 3.2
1.53556880046642 2.9
1.4 2.6111092146298
1.39547874069438 2.6
1.22177523131665 2.3
1.1 2.15670430696244
0.8 2.0667553594735
0.5 2.23564195249353
0.2 2.26764921349323
0.0789983217055606 2
-0.0928237339854743 1.7
-0.1 1.6856278665277
-0.336126449773367 1.4
-0.4 1.28030499481473
-0.577837747141335 1.1
-0.639160370580398 0.8
-0.632567128172627 0.5
-0.592048490775595 0.2
-0.517843170979797 -0.1
-0.4 -0.395173232854723
-0.398450585361596 -0.4
-0.277183587179175 -0.7
-0.1 -0.999715551296465
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
3.2 -1
3.5 -1
3.68387615330652 -1
3.8 -0.878258823528987
3.96972454952689 -0.7
4.1 -0.559514565995753
4.24798564389403 -0.4
4.4 -0.2336839213476
4.52228760720803 -0.1
4.7 0.0958949142585274
4.79450314535937 0.2
5 0.427421317076998
5 0.5
5 0.8
5 1.09461137759801
4.71798614819758 0.8
4.7 0.781211952694352
4.43041107566689 0.5
4.4 0.468274668520038
4.14199010116668 0.2
4.1 0.156308299398841
3.85184554085044 -0.1
3.8 -0.153669388815468
3.5582889145246 -0.4
3.5 -0.459724185356203
3.25813172823883 -0.7
3.2 -0.758361293586508
2.94518609169235 -1
3.2 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
0.2 -0.990926472203802
0.206482520397573 -1
0.494232940710735 -1
0.271882455940537 -0.7
0.2 -0.583951061138574
0.100252964167846 -0.4
-0.0222060766645366 -0.1
-0.1 0.177775522417886
-0.106439345987975 0.2
-0.156844031125307 0.5
-0.163382075006605 0.8
-0.109088872537673 1.1
-0.1 1.11876039468863
-0.00419411335216972 1.4
0.124242904120809 1.7
0.2 1.89150558855811
0.342868319640846 2
0.5 2.04209020720118
0.599370182466088 2
0.8 1.90574714034893
1.09807436340017 2
1.1 2.00044322464167
1.35456868129433 2.3
1.4 2.37986819580597
1.51712261691156 2.6
1.62694567625831 2.9
1.6912041493941 3.2
1.7 3.26216989452783
1.77570934553498 3.5
1.87616405977828 3.8
1.94682440226861 4.1
1.98690002697297 4.4
2 4.47564528037524
2.07217032742841 4.7
2.13404566863439 5
2.04430760588377 5
2 4.75640343984717
1.99512013154153 4.7
1.94303193752337 4.4
1.89376773548607 4.1
1.81776087899664 3.8
1.70176007255307 3.5
1.7 3.49447098323229
1.65833798985898 3.2
1.58125723836236 2.9
1.45501810345972 2.6
1.4 2.49659354702545
1.28817195630549 2.3
1.1 2.07857376580205
0.8 2.00725229490098
0.5 2.13886607984736
0.2 2.10084332480469
0.154409686518778 2
0.015709585067667 1.7
-0.1 1.46826477763639
-0.156433987985149 1.4
-0.307724704776283 1.1
-0.36688409754387 0.8
-0.364415940460755 0.5
-0.323496268141078 0.2
-0.248074069088806 -0.1
-0.131110231292802 -0.4
-0.1 -0.461671877638938
0.0151087288138017 -0.7
0.2 -0.990926472203802
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
2.6 -1
2.9 -1
2.94518609169235 -1
3.2 -0.758361293586508
3.25813172823883 -0.7
3.5 -0.459724185356203
3.5582889145246 -0.4
3.8 -0.153669388815468
3.85184554085044 -0.1
4.1 0.156308299398841
4.14199010116668 0.2
4.4 0.468274668520038
4.43041107566689 0.5
4.7 0.781211952694352
4.71798614819758 0.8
5 1.09461137759801
5 1.1
5 1.4
5 1.47559820450213
4.92668113907479 1.4
4.7 1.16681209832839
4.63523090688416 1.1
4.4 0.858206901310713
4.34353753940705 0.8
4.1 0.550191808783052
4.05113046188574 0.5
3.8 0.243678940750822
3.75700908276042 0.2
3.5 -0.0595329063871397
3.45917618741695 -0.1
3.2 -0.356270788696874
3.15369441603302 -0.4
2.9 -0.641442778264059
2.83246331463017 -0.7
2.6 -0.907268459540468
2.47718131873072 -1
2.6 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.5 -1
0.8 -1
0.87167555128642 -1
0.8 -0.958810621623269
0.540050586507949 -0.7
0.5 -0.654588572483722
0.336999309684982 -0.4
0.2 -0.128648953656484
0.187598589323427 -0.1
0.0940625947714358 0.2
0.0400249475916946 0.5
0.0263883151322445 0.8
0.058994042494162 1.1
0.135476572925003 1.4
0.2 1.58141052529089
0.265704133388217 1.7
0.5 1.89675571800413
0.8 1.79841218568287
1.1 1.87795282030614
1.21076734918953 2
1.4 2.25297574628656
1.42815351778083 2.3
1.5792271303634 2.6
1.67263411415426 2.9
1.7 3.03496934145306
1.763270708962 3.2
1.84965861851688 3.5
1.93456724055991 3.8
1.99988106905114 4.1
2 4.1009557365769
2.07310161404236 4.4
2.1536564441127 4.7
2.223783731385 5
2.13404566863439 5
2.07217032742841 4.7
2 4.47564528037524
1.98690002697297 4.4
1.94682440226861 4.1
1.87616405977828 3.8
1.77570934553498 3.5
1.7 3.26216989452783
1.6912041493941 3.2
1.62694567625831 2.9
1.51712261691156 2.6
1.4 2.37986819580597
1.35456868129433 2.3
1.1 2.00044322464167
1.09807436340017 2
0.8 1.90574714034893
0.599370182466088 2
0.5 2.04209020720118
0.342868319640846 2
0.2 1.89150558855811
0.124242904120809 1.7
-0.00419411335216971 1.4
-0.1 1.11876039468863
-0.109088872537673 1.1
-0.163382075006605 0.8
-0.156844031125307 0.5
-0.106439345987975 0.2
-0.1 0.177775522417886
-0.0222060766645366 -0.1
0.100252964167846 -0.4
0.2 -0.583951061138574
0.271882455940537 -0.7
0.494232940710735 -1
0.5 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
2.3 -1
2.47718131873072 -1
2.6 -0.907268459540468
2.83246331463017 -0.7
2.9 -0.641442778264059
3.15369441603302 -0.4
3.2 -0.356270788696874
3.45917618741695 -0.1
3.5 -0.0595329063871397
3.75700908276042 0.2
3.8 0.243678940750822
4.05113046188574 0.5
4.1 0.550191808783051
4.34353753940705 0.8
4.4 0.858206901310713
4.63523090688416 1.1
4.7 1.16681209832839
4.92668113907479 1.4
5 1.47559820450213
5 1.7
5 1.79891388729162
4.9042540041083 1.7
4.7 1.48983879727282
4.61326470855168 1.4
4.4 1.18050246147881
4.32245846000972 1.1
4.1 0.871210723173061
4.03139728013036 0.8
3.8 0.562880916887528
3.73898697988202 0.5
3.5 0.257550811777379
3.44292760272945 0.2
3.2 -0.0410254124537604
3.13865033578117 -0.1
2.9 -0.326854753837886
2.81678697897855 -0.4
2.6 -0.591282935616191
2.45614828521243 -0.7
2.3 -0.822095012455535
2.00202631127204 -1
2.3 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
0.8 -0.958810621623269
0.87167555128642 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.00202631127204 -1
2.3 -0.822095012455535
2.45614828521243 -0.7
2.6 -0.591282935616191
2.81678697897855 -0.4
2.9 -0.326854753837886
3.13865033578117 -0.1
3.2 -0.0410254124537604
3.44292760272945 0.2
3.5 0.257550811777379
3.73898697988202 0.5
3.8 0.562880916887528
4.03139728013036 0.8
4.1 0.871210723173061
4.32245846000972 1.1
4.4 1.18050246147881
4.61326470855168 1.4
4.7 1.48983879727282
4.9042540041083 1.7
5 1.79891388729162
5 2
5 2.11013131628779
4.89411548331124 2
4.7 1.79934099979278
4.60505663967082 1.7
4.4 1.48750996142264
4.31692131067666 1.4
4.1 1.17475344320153
4.02937345542996 1.1
3.8 0.861951755289998
3.74132965563244 0.8
3.5 0.551407130780717
3.45042311646713 0.5
3.2 0.247538590077212
3.15198537623576 0.2
2.9 -0.0426231661866669
2.83649340176847 -0.1
2.6 -0.309292537316767
2.48192502651909 -0.4
2.3 -0.539824169732172
2.02778439624961 -0.7
2 -0.717075552898462
1.7 -0.83026887938118
1.4 -0.86226945668585
1.1 -0.79937437816858
0.929401600435103 -0.7
0.8 -0.613211399842793
0.611789117409079 -0.4
0.5 -0.245431655866674
0.424907183077849 -0.1
0.311576584686548 0.2
0.240107730419595 0.5
0.212466533318124 0.8
0.233841983235793 1.1
0.313327139915945 1.4
0.483273059322341 1.7
0.5 1.71404685994098
0.644141953867116 1.7
0.8 1.68245217750055
0.846796569883737 1.7
1.1 1.75520933238706
1.322166652485 2
1.4 2.10405154231713
1.51731474615459 2.3
1.64133164381525 2.6
1.7 2.81059714649204
1.7420312572207 2.9
1.8496620062553 3.2
1.92360789149879 3.5
1.99297042134155 3.8
2 3.83229424276145
2.11609794831923 4.1
2.17732730337861 4.4
2.23514256079699 4.7
2.3 4.95224637100484
2.32508951127611 5
2.3 5
2.223783731385 5
2.1536564441127 4.7
2.07310161404236 4.4
2 4.1009557365769
1.99988106905114 4.1
1.93456724055991 3.8
1.84965861851688 3.5
1.763270708962 3.2
1.7 3.03496934145306
1.67263411415426 2.9
1.5792271303634 2.6
1.42815351778083 2.3
1.4 2.25297574628656
1.21076734918953 2
1.1 1.87795282030614
0.8 1.79841218568287
0.5 1.89675571800413
0.265704133388217 1.7
0.2 1.58141052529089
0.135476572925003 1.4
0.058994042494162 1.1
0.0263883151322445 0.8
0.0400249475916946 0.5
0.0940625947714358 0.2
0.187598589323427 -0.1
0.2 -0.128648953656484
0.336999309684982 -0.4
0.5 -0.654588572483722
0.540050586507949 -0.7
0.8 -0.958810621623269
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.1 -0.79937437816858
1.4 -0.86226945668585
1.7 -0.83026887938118
2 -0.717075552898462
2.02778439624961 -0.7
2.3 -0.539824169732172
2.48192502651909 -0.4
2.6 -0.309292537316767
2.83649340176847 -0.1
2.9 -0.0426231661866669
3.15198537623576 0.2
3.2 0.247538590077212
3.45042311646713 0.5
3.5 0.551407130780717
3.74132965563244 0.8
3.8 0.861951755289998
4.02937345542996 1.1
4.1 1.17475344320153
4.31692131067666 1.4
4.4 1.48750996142264
4.60505663967082 1.7
4.7 1.79934099979278
4.89411548331124 2
5 2.11013131628779
5 2.3
5 2.43966356012422
4.8674356965954 2.3
4.7 2.12521224413641
4.58245452147818 2
4.4 1.80836643847555
4.29956160519466 1.7
4.1 1.48899866551343
4.01841376606644 1.4
3.8 1.16804014393129
3.7377842892721 1.1
3.5 0.848280511277725
3.4551659565234 0.8
3.2 0.535079027542775
3.1659013542285 0.5
2.9 0.236800347010135
2.86071682701778 0.2
2.6 -0.0351809820453805
2.51789183454623 -0.1
2.3 -0.26707460020954
2.07287859479009 -0.4
2 -0.442686720424545
1.7 -0.539282416733847
1.4 -0.544392835174251
1.1 -0.445331327258253
1.03366543236642 -0.4
0.8 -0.19531786188205
0.731248457552916 -0.1
0.570171738772389 0.2
0.5 0.399201908713815
0.475489926863453 0.5
0.442512921133457 0.8
0.454000316149584 1.1
0.5 1.2942466829518
0.575528311019098 1.4
0.8 1.47136358650214
1.1 1.58056754140413
1.20146125093124 1.7
1.4 1.93439997295554
1.44061049812669 2
1.60647597452835 2.3
1.7 2.58496859022668
1.70752843330053 2.6
1.84683884515687 2.9
1.93605330354859 3.2
1.99755716448069 3.5
2 3.51085843720357
2.12770179277759 3.8
2.23245672455141 4.1
2.28155299271487 4.4
2.3 4.53934154827034
2.34554378082007 4.7
2.49159730711275 5
2.32508951127611 5
2.3 4.95224637100484
2.23514256079699 4.7
2.17732730337861 4.4
2.11609794831923 4.1
2 3.83229424276145
1.99297042134155 3.8
1.92360789149879 3.5
1.8496620062553 3.2
1.7420312572207 2.9
1.7 2.81059714649204
1.64133164381525 2.6
1.51731474615459 2.3
1.4 2.10405154231713
1.322166652485 2
1.1 1.75520933238706
0.846796569883737 1.7
0.8 1.68245217750055
0.644141953867116 1.7
0.5 1.71404685994098
0.483273059322341 1.7
0.313327139915945 1.4
0.233841983235793 1.1
0.212466533318124 0.8
0.240107730419595 0.5
0.311576584686548 0.2
0.424907183077849 -0.1
0.5 -0.245431655866674
0.611789117409079 -0.4
0.8 -0.613211399842793
0.929401600435103 -0.7
1.1 -0.79937437816858
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.1 -0.445331327258253
1.4 -0.544392835174251
1.7 -0.539282416733847
2 -0.442686720424545
2.07287859479009 -0.4
2.3 -0.26707460020954
2.51789183454623 -0.1
2.6 -0.0351809820453805
2.86071682701778 0.2
2.9 0.236800347010135
3.1659013542285 0.5
3.2 0.535079027542775
3.4551659565234 0.8
3.5 0.848280511277725
3.7377842892721 1.1
3.8 1.16804014393129
4.01841376606644 1.4
4.1 1.48899866551343
4.29956160519466 1.7
4.4 1.80836643847555
4.58245452147818 2
4.7 2.12521224413641
4.8674356965954 2.3
5 2.43966356012422
5 2.6
5 2.82286546394278
4.79313443577765 2.6
4.7 2.50107024299672
4.51679953465721 2.3
4.4 2.17445118905452
4.24432582605103 2
4.1 1.84277444018936
3.97480494498137 1.7
3.8 1.50747231091338
3.7063097231068 1.4
3.5 1.17239947475217
3.43589140758654 1.1
3.2 0.844286425728175
3.15883941901585 0.8
2.9 0.533073271677709
2.86608438138346 0.5
2.6 0.252064980863123
2.53599475634991 0.2
2.3 0.0170747655838139
2.09909172713572 -0.1
2 -0.155589925188752
1.7 -0.231874689547786
1.4 -0.191248460565978
1.23130134321579 -0.1
1.1 0.010847705735343
0.950514839854611 0.2
0.813800950994889 0.5
0.8 0.583189011404739
0.770852189296661 0.8
0.8 0.971874548051642
0.830958432156067 1.1
1.1 1.32700605776436
1.14561709025503 1.4
1.38586731523792 1.7
1.4 1.71668541250289
1.57538935642537 2
1.69563720290211 2.3
1.7 2.31329348402361
1.84359603755772 2.6
1.95164643309303 2.9
2 3.09192302498958
2.05049384783486 3.2
2.16710615225756 3.5
2.27287734172674 3.8
2.3 3.89243468333303
2.38849944981601 4.1
2.47638301406209 4.4
2.5687236363634 4.7
2.6 4.78595718897204
2.72094433074872 5
2.6 5
2.49159730711275 5
2.34554378082007 4.7
2.3 4.53934154827034
2.28155299271487 4.4
2.23245672455141 4.1
2.12770179277759 3.8
2 3.51085843720357
1.99755716448069 3.5
1.93605330354859 3.2
1.84683884515687 2.9
1.70752843330053 2.6
1.7 2.58496859022668
1.60647597452835 2.3
1.44061049812669 2
1.4 1.93439997295554
1.20146125093124 1.7
1.1 1.58056754140413
0.8 1.47136358650214
0.575528311019098 1.4
0.5 1.2942466829518
0.454000316149584 1.1
0.442512921133457 0.8
0.475489926863453 0.5
0.5 0.399201908713815
0.570171738772389 0.2
0.731248457552916 -0.1
0.8 -0.19531786188205
1.03366543236642 -0.4
1.1 -0.445331327258253
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.4 -0.191248460565978
1.7 -0.231874689547786
2 -0.155589925188752
2.09909172713572 -0.1
2.3 0.0170747655838139
2.53599475634991 0.2
2.6 0.252064980863123
2.86608438138346 0.5
2.9 0.533073271677709
3.15883941901585 0.8
3.2 0.844286425728175
3.43589140758654 1.1
3.5 1.17239947475217
3.7063097231068 1.4
3.8 1.50747231091338
3.97480494498137 1.7
4.1 1.84277444018936
4.24432582605103 2
4.4 2.17445118905452
4.51679953465721 2.3
4.7 2.50107024299672
4.79313443577765 2.6
5 2.82286546394278
5 2.9
5 3.2
5 3.36564560170044
4.86251668132533 3.2
4.7 3.01175500473688
4.61119931495068 2.9
4.4 2.6472236835433
4.36388008437534 2.6
4.11766344073217 2.3
4.1 2.27980979911038
3.8699321761659 2
3.8 1.91860277018188
3.62117906802333 1.7
3.5 1.55819134268919
3.36789230223747 1.4
3.2 1.20702835832545
3.10547044539372 1.1
2.9 0.876489814082272
2.82471082241366 0.8
2.6 0.581725614046515
2.50190580447461 0.5
2.3 0.341050878894599
2.05229188931263 0.2
2 0.172141522752009
1.7 0.132276481307763
1.52928402075615 0.2
1.4 0.294452799917417
1.26735189754254 0.5
1.20924203609357 0.8
1.26922791947584 1.1
1.4 1.3566385502112
1.41802312613609 1.4
1.58334599320434 1.7
1.7 1.96585912045405
1.7186346076235 2
1.87208432949862 2.3
1.97966364181491 2.6
2 2.66516085571355
2.12727074787354 2.9
2.24484923203237 3.2
2.3 3.36537328737048
2.37305723303764 3.5
2.50270497133495 3.8
2.59945063361035 4.1
2.6 4.10183481545187
2.78776536416871 4.4
2.9 4.61837688632043
2.96442554439847 4.7
3.16954170901878 5
2.9 5
2.72094433074872 5
2.6 4.78595718897204
2.5687236363634 4.7
2.47638301406209 4.4
2.38849944981601 4.1
2.3 3.89243468333303
2.27287734172674 3.8
2.16710615225756 3.5
2.05049384783486 3.2
2 3.09192302498958
1.95164643309303 2.9
1.84359603755772 2.6
1.7 2.31329348402361
1.69563720290211 2.3
1.57538935642537 2
1.4 1.71668541250289
1.38586731523792 1.7
1.14561709025503 1.4
1.1 1.32700605776436
0.830958432156067 1.1
0.8 0.971874548051642
0.770852189296661 0.8
0.8 0.583189011404739
0.813800950994889 0.5
0.950514839854611 0.2
1.1 0.010847705735343
1.23130134321579 -0.1
1.4 -0.191248460565978
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.7 0.132276481307763
2 0.172141522752009
2.05229188931263 0.2
2.3 0.341050878894599
2.50190580447461 0.5
2.6 0.581725614046515
2.82471082241366 0.8
2.9 0.876489814082272
3.10547044539372 1.1
3.2 1.20702835832545
3.36789230223747 1.4
3.5 1.55819134268919
3.62117906802333 1.7
3.8 1.91860277018188
3.8699321761659 2
4.1 2.27980979911038
4.11766344073217 2.3
4.36388008437534 2.6
4.4 2.6472236835433
4.61119931495068 2.9
4.7 3.01175500473688
4.86251668132533 3.2
5 3.36564560170044
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.1 5
3.8 5
3.5 5
3.2 5
3.16954170901878 5
2.96442554439847 4.7
2.9 4.61837688632043
2.78776536416871 4.4
2.6 4.10183481545187
2.59945063361035 4.1
2.50270497133495 3.8
2.37305723303764 3.5
2.3 3.36537328737048
2.24484923203237 3.2
2.12727074787354 2.9
2 2.66516085571355
1.97966364181491 2.6
1.87208432949862 2.3
1.7186346076235 2
1.7 1.96585912045405
1.58334599320434 1.7
1.41802312613609 1.4
1.4 1.3566385502112
1.26922791947584 1.1
1.20924203609357 0.8
1.26735189754254 0.5
1.4 0.294452799917417
1.52928402075615 0.2
1.7 0.132276481307763

1.68032231192512 0.8
1.65077632817416 1.1
1.7 1.34876529263829
1.71291581667847 1.4
1.8448393888398 1.7
1.96563481449369 2
2 2.09657990597183
2.11294972037761 2.3
2.25362085460842 2.6
2.3 2.70992017417101
2.42383870871251 2.9
2.574367371572 3.2
2.6 3.25746528076095
2.77352969918907 3.5
2.9 3.69969554702532
3.00821863092109 3.8
3.2 3.9894639670063
3.39881406964381 4.1
3.5 4.15517314200111
3.8 4.28101314087038
4.1 4.235956074388
4.27045072270051 4.1
4.35516477413061 3.8
4.29229782441509 3.5
4.17144572317675 3.2
4.1 3.07158636783121
4.01288651013903 2.9
3.83746620850692 2.6
3.8 2.5458309532975
3.63736663150683 2.3
3.5 2.10145473872206
3.42924317848824 2
3.21139645333337 1.7
3.2 1.68581981632197
2.96239189565169 1.4
2.9 1.32731010212061
2.6852974513046 1.1
2.6 1.0129999023553
2.34618032994911 0.8
2.3 0.76335838526983
2 0.642241796364894
1.7 0.764349060288057
1.68032231192512 0.8
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.7 0.764349060288057
2 0.642241796364894
2.3 0.76335838526983
2.34618032994911 0.8
2.6 1.0129999023553
2.6852974513046 1.1
2.9 1.32731010212061
2.96239189565169 1.4
3.2 1.68581981632197
3.21139645333337 1.7
3.42924317848824 2
3.5 2.10145473872206
3.63736663150683 2.3
3.8 2.5458309532975
3.83746620850692 2.6
4.01288651013903 2.9
4.1 3.07158636783121
4.17144572317675 3.2
4.29229782441509 3.5
4.35516477413061 3.8
4.27045072270051 4.1
4.1 4.235956074388
3.8 4.28101314087038
3.5 4.15517314200111
3.39881406964381 4.1
3.2 3.9894639670063
3.00821863092109 3.8
2.9 3.69969554702532
2.77352969918907 3.5
2.6 3.25746528076095
2.574367371572 3.2
2.42383870871251 2.9
2.3 2.70992017417101
2.25362085460842 2.6
2.11294972037761 2.3
2 2.09657990597183
1.96563481449369 2
1.8448393888398 1.7
1.71291581667847 1.4
1.7 1.34876529263829
1.65077632817416 1.1
1.68032231192512 0.8
1.7 0.764349060288057
};
\end{axis}



==> fig/tikz/ionosphere/epcvi_Z_3.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=black]
table{%
x  y
-0.7 2.39902781208479
-0.4 2.39809062478824
-0.265119192580467 2.6
-0.130456072767915 2.9
-0.1 2.90154389686911
-0.0822550453015546 2.9
0.2 2.68984487292395
0.49796018841738 2.9
0.5 2.90097474328463
0.515461636719854 2.9
0.8 2.80436180277707
0.947126694023023 2.9
1.1 2.9991377295482
1.22379754600779 3.2
1.33802980517156 3.5
1.39844960439297 3.8
1.4 3.81357216620267
1.47559392102352 4.1
1.53839405519987 4.4
1.58805834957141 4.7
1.6196252547942 5
1.4 5
1.1 5
0.8 5
0.5 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.67617008137247
-0.927268474476483 2.6
-0.7 2.39902781208479
};
\addplot [draw=none, fill=midnightblue854116]
table{%
x  y
-0.7 2.32412963773587
-0.4 2.31779479359664
-0.211479451819613 2.6
-0.1 2.89103598772043
0.2 2.6757291520609
0.5 2.84871884773406
0.8 2.7533727110768
1.0255666553662 2.9
1.1 2.9482697272916
1.25514904788777 3.2
1.35768847708543 3.5
1.4 3.71321150400329
1.43089064771312 3.8
1.50450511300462 4.1
1.56220270467022 4.4
1.60796619056488 4.7
1.63647816946868 5
1.6196252547942 5
1.58805834957141 4.7
1.53839405519987 4.4
1.47559392102352 4.1
1.4 3.81357216620267
1.39844960439297 3.8
1.33802980517156 3.5
1.22379754600779 3.2
1.1 2.9991377295482
0.947126694023023 2.9
0.8 2.80436180277707
0.515461636719854 2.9
0.5 2.90097474328463
0.49796018841738 2.9
0.2 2.68984487292395
-0.0822550453015546 2.9
-0.1 2.90154389686911
-0.130456072767915 2.9
-0.265119192580467 2.6
-0.4 2.39809062478824
-0.7 2.39902781208479
-0.927268474476483 2.6
-1 2.67617008137247
-1 2.6
-1 2.57567258115114
-0.7 2.32412963773587
};
\addplot [draw=none, fill=midnightblue868137]
table{%
x  y
-0.7 2.19938068642292
-0.4 2.20477854344126
-0.336671781840247 2.3
-0.157839711058759 2.6
-0.1 2.75100036071839
0.2 2.66161343119785
0.5 2.79161783530149
0.8 2.70238361937653
1.1 2.89616541701189
1.10264790909053 2.9
1.28650054976774 3.2
1.3773471489993 3.5
1.4 3.61414971854296
1.46614972993761 3.8
1.53341630498571 4.1
1.58601135414058 4.4
1.62787403155835 4.7
1.65333108414317 5
1.63647816946868 5
1.60796619056488 4.7
1.56220270467022 4.4
1.50450511300462 4.1
1.43089064771312 3.8
1.4 3.71321150400329
1.35768847708543 3.5
1.25514904788777 3.2
1.1 2.9482697272916
1.0255666553662 2.9
0.8 2.7533727110768
0.5 2.84871884773406
0.2 2.6757291520609
-0.1 2.89103598772043
-0.211479451819613 2.6
-0.4 2.31779479359664
-0.7 2.32412963773587
-1 2.57567258115114
-1 2.40348770991421
-0.859008881527219 2.3
-0.7 2.19938068642292
};
\addplot [draw=none, fill=teal882156]
table{%
x  y
-0.7 2.0509382968263
-0.4 2.0824463983142
-0.255313261874965 2.3
-0.104199970297905 2.6
-0.1 2.61096473371635
0.2 2.6474977103348
0.5 2.73451682286892
0.8 2.65139452767626
1.1 2.82109346399717
1.15448762867623 2.9
1.31785205164772 3.2
1.39700582091317 3.5
1.4 3.51508793308262
1.50140881216211 3.8
1.56232749696681 4.1
1.60982000361093 4.4
1.64778187255182 4.7
1.67018399881766 5
1.65333108414317 5
1.62787403155835 4.7
1.58601135414058 4.4
1.53341630498571 4.1
1.46614972993761 3.8
1.4 3.61414971854296
1.3773471489993 3.5
1.28650054976774 3.2
1.10264790909053 2.9
1.1 2.89616541701189
0.8 2.70238361937653
0.5 2.79161783530149
0.2 2.66161343119785
-0.1 2.75100036071839
-0.157839711058759 2.6
-0.336671781840247 2.3
-0.4 2.20477854344126
-0.7 2.19938068642292
-0.859008881527219 2.3
-1 2.40348770991421
-1 2.3
-1 2.16189224305916
-0.7 2.0509382968263
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 -1
-0.620082857069415 -1
-0.7 -0.81594025393569
-0.767990190054375 -0.7
-0.903592207190763 -0.4
-0.987276340319323 -0.1
-1 -0.035509434178804
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.958114354962515 1.7
-0.7 1.81168531903844
-0.4 1.93329155367691
-0.359407814709817 2
-0.173954741909682 2.3
-0.1 2.44895922707397
-0.0158669300081982 2.6
0.2 2.63338198947174
0.5 2.67741581043635
0.8 2.60040543597599
1.1 2.74602151098245
1.20632734826193 2.9
1.3492035535277 3.2
1.4 3.39695452777353
1.4387524200178 3.5
1.5366678943866 3.8
1.59123868894791 4.1
1.63362865308128 4.4
1.66768971354528 4.7
1.68703691349214 5
1.67018399881766 5
1.64778187255182 4.7
1.60982000361093 4.4
1.56232749696681 4.1
1.50140881216211 3.8
1.4 3.51508793308262
1.39700582091317 3.5
1.31785205164772 3.2
1.15448762867623 2.9
1.1 2.82109346399717
0.8 2.65139452767626
0.5 2.73451682286892
0.2 2.6474977103348
-0.1 2.61096473371635
-0.104199970297905 2.6
-0.255313261874965 2.3
-0.4 2.0824463983142
-0.7 2.0509382968263
-1 2.16189224305916
-1 2
-1 1.7
-1 1.61327806830657
-0.958114354962515 1.7
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.7 -0.81594025393569
-0.620082857069415 -1
-0.4 -1
-0.123459220609086 -1
-0.301248370436914 -0.7
-0.4 -0.469569160327106
-0.435660399705966 -0.4
-0.554641947907192 -0.1
-0.630573123126127 0.2
-0.677384421654401 0.5
-0.7 0.767779204715573
-0.704002733599896 0.8
-0.706617156987906 1.1
-0.7 1.13089789617092
-0.656648861707678 1.4
-0.456044543705043 1.7
-0.4 1.72869246781585
-0.234908977437414 2
-0.1 2.2767579267612
-0.0897740816829539 2.3
0.0754133494412596 2.6
0.2 2.61926626860869
0.5 2.62031479800378
0.579187873769834 2.6
0.8 2.51356393904459
0.95363638589274 2.6
1.1 2.67094955796773
1.25816706784763 2.9
1.38055505540767 3.2
1.4 3.27539444480339
1.48446764933234 3.5
1.57192697661109 3.8
1.62014988092901 4.1
1.65743730255163 4.4
1.68759755453875 4.7
1.7 4.91890038976082
1.71416941286662 5
1.7 5
1.68703691349214 5
1.66768971354528 4.7
1.63362865308128 4.4
1.59123868894791 4.1
1.5366678943866 3.8
1.4387524200178 3.5
1.4 3.39695452777353
1.3492035535277 3.2
1.20632734826193 2.9
1.1 2.74602151098245
0.8 2.60040543597599
0.5 2.67741581043635
0.2 2.63338198947174
-0.0158669300081982 2.6
-0.1 2.44895922707397
-0.173954741909682 2.3
-0.359407814709817 2
-0.4 1.93329155367691
-0.7 1.81168531903844
-0.958114354962515 1.7
-1 1.61327806830657
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.035509434178804
-0.987276340319323 -0.1
-0.903592207190763 -0.4
-0.767990190054375 -0.7
-0.7 -0.81594025393569
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.427575471329604
4.79438050433936 0.2
4.7 0.096033238100319
4.52221404651555 -0.1
4.4 -0.233618044452185
4.24800859571853 -0.4
4.1 -0.559586338181979
3.96990232077303 -0.7
3.8 -0.878536577833272
3.68428355906994 -1
3.8 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
-0.1 -1
0.190176482896133 -1
-0.00559863684216425 -0.7
-0.1 -0.515856376028279
-0.160792933535497 -0.4
-0.2807873040771 -0.1
-0.361561877356838 0.2
-0.4 0.422766029602564
-0.416196651851139 0.5
-0.448777368074948 0.8
-0.444196519238098 1.1
-0.4 1.28193701132329
-0.378768570941123 1.4
-0.256439777637472 1.7
-0.11041014016501 2
-0.1 2.02135579754652
0.0225963288443374 2.3
0.166693628890717 2.6
0.2 2.60515054774564
0.308475777932465 2.6
0.5 2.52898862549509
0.8 2.42643507943253
1.1 2.5941123212672
1.10471780744551 2.6
1.31000678743333 2.9
1.4 3.1461505212806
1.42347144305085 3.2
1.53018287864688 3.5
1.60718605883558 3.8
1.6490610729101 4.1
1.68124595202198 4.4
1.7 4.60289214019143
1.72483815641318 4.7
1.77555924701854 5
1.71416941286662 5
1.7 4.91890038976082
1.68759755453875 4.7
1.65743730255163 4.4
1.62014988092901 4.1
1.57192697661109 3.8
1.48446764933234 3.5
1.4 3.27539444480339
1.38055505540767 3.2
1.25816706784763 2.9
1.1 2.67094955796773
0.95363638589274 2.6
0.8 2.51356393904459
0.579187873769834 2.6
0.5 2.62031479800378
0.2 2.61926626860869
0.0754133494412596 2.6
-0.0897740816829539 2.3
-0.1 2.2767579267612
-0.234908977437414 2
-0.4 1.72869246781585
-0.456044543705043 1.7
-0.656648861707678 1.4
-0.7 1.13089789617092
-0.706617156987906 1.1
-0.704002733599896 0.8
-0.7 0.767779204715573
-0.677384421654401 0.5
-0.630573123126127 0.2
-0.554641947907192 -0.1
-0.435660399705966 -0.4
-0.4 -0.469569160327106
-0.301248370436914 -0.7
-0.123459220609086 -1
-0.1 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
3.2 -1
3.5 -1
3.68428355906994 -1
3.8 -0.878536577833272
3.96990232077303 -0.7
4.1 -0.559586338181979
4.24800859571853 -0.4
4.4 -0.233618044452185
4.52221404651555 -0.1
4.7 0.096033238100319
4.79438050433936 0.2
5 0.427575471329604
5 0.5
5 0.8
5 1.09464446470368
4.71800930677869 0.8
4.7 0.781185957134813
4.43053387341261 0.5
4.4 0.468139552927304
4.14227430237279 0.2
4.1 0.155995859881211
3.85238027101622 -0.1
3.8 -0.154255217418805
3.5592056244994 -0.4
3.5 -0.460717388386171
3.25962653944846 -0.7
3.2 -0.759938023917337
2.94755441887409 -1
3.2 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
0.2 -1
0.482616343090616 -1
0.253614103309373 -0.7
0.2 -0.617670585206511
0.0767959158640885 -0.4
-0.0521331374141795 -0.1
-0.1 0.0521743495082384
-0.146655573378493 0.2
-0.207531738483219 0.5
-0.237890542007259 0.8
-0.235462816338636 1.1
-0.186075950886899 1.4
-0.1 1.6628659806454
-0.0901683530994571 1.7
0.0200828130519659 2
0.134966739371629 2.3
0.2 2.44303300919835
0.5 2.41876197017268
0.8 2.33930621982047
1.1 2.48689320806803
1.19063267364461 2.6
1.36184650701903 2.9
1.4 3.00435789453548
1.48527478159422 3.2
1.57589810796142 3.5
1.64244514106008 3.8
1.6779722648912 4.1
1.7 4.33462371719439
1.71764444239989 4.4
1.79072063606691 4.7
1.83694908117045 5
1.77555924701854 5
1.72483815641318 4.7
1.7 4.60289214019143
1.68124595202198 4.4
1.6490610729101 4.1
1.60718605883558 3.8
1.53018287864688 3.5
1.42347144305085 3.2
1.4 3.1461505212806
1.31000678743333 2.9
1.10471780744551 2.6
1.1 2.5941123212672
0.8 2.42643507943253
0.5 2.52898862549509
0.308475777932465 2.6
0.2 2.60515054774564
0.166693628890717 2.6
0.0225963288443374 2.3
-0.1 2.02135579754652
-0.11041014016501 2
-0.256439777637472 1.7
-0.378768570941123 1.4
-0.4 1.28193701132329
-0.444196519238098 1.1
-0.448777368074948 0.8
-0.416196651851139 0.5
-0.4 0.422766029602564
-0.361561877356838 0.2
-0.2807873040771 -0.1
-0.160792933535497 -0.4
-0.1 -0.515856376028279
-0.00559863684216425 -0.7
0.190176482896133 -1
0.2 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
2.6 -1
2.9 -1
2.94755441887409 -1
3.2 -0.759938023917337
3.25962653944846 -0.7
3.5 -0.460717388386171
3.5592056244994 -0.4
3.8 -0.154255217418805
3.85238027101622 -0.1
4.1 0.155995859881211
4.14227430237279 0.2
4.4 0.468139552927304
4.43053387341261 0.5
4.7 0.781185957134813
4.71800930677869 0.8
5 1.09464446470368
5 1.1
5 1.4
5 1.47557509778039
4.92672384683156 1.4
4.7 1.16672329025503
4.63534700627913 1.1
4.4 0.858006900027043
4.34377374487571 0.8
4.1 0.549814346653994
4.05155522120122 0.5
3.8 0.243027624357409
3.75772648033338 0.2
3.5 -0.0605939855459721
3.46035244042033 -0.1
3.2 -0.357924828739216
3.15561456116943 -0.4
2.9 -0.643925071745268
2.83565646182652 -0.7
2.6 -0.910862845640366
2.48266783690915 -1
2.6 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.5 -1
0.8 -1
0.854821166767958 -1
0.8 -0.96866897957557
0.523151676246289 -0.7
0.5 -0.674503394604429
0.316689489161038 -0.4
0.2 -0.182950407007892
0.162051802850994 -0.1
0.0613146929633707 0.2
-0.00408922573748556 0.5
-0.038259676274224 0.8
-0.0399108245386069 1.1
-0.00339321021683228 1.4
0.0656332602870151 1.7
0.151122705525244 2
0.2 2.1408849756272
0.453417809200823 2.3
0.5 2.30853531485027
0.537090873646865 2.3
0.8 2.22212738193045
0.927450288942925 2.3
1.1 2.37967409486887
1.27654753984372 2.6
1.4 2.85343530466673
1.42219851550342 2.9
1.54707812013759 3.2
1.62161333727596 3.5
1.67770422328457 3.8
1.7 4.01794076466541
1.72213480222584 4.1
1.8007549200184 4.4
1.85660311572064 4.7
1.89833891532237 5
1.83694908117045 5
1.79072063606691 4.7
1.71764444239989 4.4
1.7 4.33462371719439
1.6779722648912 4.1
1.64244514106008 3.8
1.57589810796142 3.5
1.48527478159422 3.2
1.4 3.00435789453548
1.36184650701903 2.9
1.19063267364461 2.6
1.1 2.48689320806803
0.8 2.33930621982047
0.5 2.41876197017268
0.2 2.44303300919835
0.134966739371629 2.3
0.0200828130519658 2
-0.0901683530994571 1.7
-0.1 1.6628659806454
-0.186075950886899 1.4
-0.235462816338636 1.1
-0.237890542007259 0.8
-0.207531738483219 0.5
-0.146655573378493 0.2
-0.1 0.0521743495082384
-0.0521331374141795 -0.1
0.0767959158640885 -0.4
0.2 -0.617670585206511
0.253614103309373 -0.7
0.482616343090616 -1
0.5 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
2.3 -1
2.48266783690915 -1
2.6 -0.910862845640366
2.83565646182652 -0.7
2.9 -0.643925071745268
3.15561456116943 -0.4
3.2 -0.357924828739216
3.46035244042033 -0.1
3.5 -0.0605939855459721
3.75772648033338 0.2
3.8 0.243027624357409
4.05155522120122 0.5
4.1 0.549814346653994
4.34377374487571 0.8
4.4 0.858006900027043
4.63534700627913 1.1
4.7 1.16672329025503
4.92672384683156 1.4
5 1.47557509778039
5 1.7
5 1.7988411365632
4.90435689045632 1.7
4.7 1.48967931157847
4.61346734692834 1.4
4.4 1.18020025030932
4.32281945507813 1.1
4.1 0.870682308448654
4.03200254435591 0.8
3.8 0.562005696555877
3.73996445880754 0.5
3.5 0.256162791508133
3.44447743885226 0.2
3.2 -0.0431437680276684
3.1411154604646 -0.1
2.9 -0.329978301103447
2.8208271456952 -0.4
2.6 -0.595753223128231
2.46316281193073 -0.7
2.3 -0.828328633987503
2.01493031119422 -1
2.3 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
0.8 -0.96866897957557
0.854821166767958 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.01493031119422 -1
2.3 -0.828328633987503
2.46316281193073 -0.7
2.6 -0.595753223128231
2.8208271456952 -0.4
2.9 -0.329978301103447
3.1411154604646 -0.1
3.2 -0.0431437680276684
3.44447743885226 0.2
3.5 0.256162791508133
3.73996445880754 0.5
3.8 0.562005696555877
4.03200254435591 0.8
4.1 0.870682308448654
4.32281945507813 1.1
4.4 1.18020025030932
4.61346734692834 1.4
4.7 1.48967931157847
4.90435689045632 1.7
5 1.7988411365632
5 2
5 2.10999497317809
4.89429265240676 2
4.7 1.79908925506867
4.60536516263595 1.7
4.4 1.48707052951531
4.31743294949454 1.4
4.1 1.17401927619143
4.03018969064206 1.1
3.8 0.860772394913711
3.74259556058721 0.8
3.5 0.549582868313769
3.45235979275098 0.5
3.2 0.244816954271096
3.15497060116703 0.2
2.9 -0.0465506384886087
2.84127231608834 -0.1
2.6 -0.314797566705791
2.4902074452399 -0.4
2.3 -0.547368721611563
2.04388952361887 -0.7
2 -0.727237047100282
1.7 -0.842468547875184
1.4 -0.875711866289619
1.1 -0.812375872060567
0.906689318599808 -0.7
0.8 -0.628458071075692
0.592423610682954 -0.4
0.5 -0.276197777078057
0.404083371461603 -0.1
0.281327575456297 0.2
0.2 0.488720945157343
0.197426350627825 0.5
0.159100582981724 0.8
0.149947766641217 1.1
0.17120814981188 1.4
0.2 1.56354930895246
0.236286339857405 1.7
0.399169701754782 2
0.5 2.07679658476117
0.8 2.08024996911982
1.1 2.25247250922896
1.13675620846676 2.3
1.36246240604282 2.6
1.4 2.67706085037876
1.50628047995948 2.9
1.60888145868096 3.2
1.6673285665905 3.5
1.7 3.69809260044837
1.73690929307842 3.8
1.81510313608586 4.1
1.88386539763691 4.4
1.92248559537437 4.7
1.95972874947429 5
1.89833891532237 5
1.85660311572064 4.7
1.8007549200184 4.4
1.72213480222584 4.1
1.7 4.01794076466541
1.67770422328457 3.8
1.62161333727596 3.5
1.54707812013759 3.2
1.42219851550342 2.9
1.4 2.85343530466673
1.27654753984372 2.6
1.1 2.37967409486887
0.927450288942925 2.3
0.8 2.22212738193045
0.537090873646865 2.3
0.5 2.30853531485027
0.453417809200823 2.3
0.2 2.1408849756272
0.151122705525244 2
0.0656332602870151 1.7
-0.00339321021683228 1.4
-0.0399108245386069 1.1
-0.0382596762742241 0.8
-0.00408922573748555 0.5
0.0613146929633707 0.2
0.162051802850994 -0.1
0.2 -0.182950407007892
0.316689489161038 -0.4
0.5 -0.674503394604429
0.523151676246289 -0.7
0.8 -0.96866897957557
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.1 -0.812375872060567
1.4 -0.875711866289619
1.7 -0.842468547875184
2 -0.727237047100282
2.04388952361887 -0.7
2.3 -0.547368721611563
2.4902074452399 -0.4
2.6 -0.314797566705791
2.84127231608834 -0.1
2.9 -0.0465506384886087
3.15497060116703 0.2
3.2 0.244816954271096
3.45235979275098 0.5
3.5 0.549582868313769
3.74259556058721 0.8
3.8 0.860772394913711
4.03018969064206 1.1
4.1 1.17401927619143
4.31743294949454 1.4
4.4 1.48707052951531
4.60536516263595 1.7
4.7 1.79908925506867
4.89429265240676 2
5 2.10999497317809
5 2.3
5 2.43943335684748
4.86773215873856 2.3
4.7 2.12482065207582
4.58293425106925 2
4.4 1.80771573416583
4.30031358216558 1.7
4.1 1.48794871763717
4.01955554319457 1.4
3.8 1.16640206205373
3.73947597360324 1.1
3.5 0.845812347437079
3.45764847962026 0.8
3.2 0.531481165621904
3.1695900349921 0.5
2.9 0.231712036601257
2.86644700274506 0.2
2.6 -0.0421803002299643
2.52768519860179 -0.1
2.3 -0.276475863640708
2.09273243068732 -0.4
2 -0.455134881248826
1.7 -0.555650585775197
1.4 -0.564462454957503
1.1 -0.466379850683005
1.00316896499216 -0.4
0.8 -0.221235841892356
0.709645835304679 -0.1
0.541603710641463 0.2
0.5 0.309810550105422
0.44747738960254 0.5
0.399515045283918 0.8
0.385099986265514 1.1
0.412656772092163 1.4
0.5 1.69987608183132
0.500071454329858 1.7
0.8 1.87339905267401
0.963076669257213 2
1.1 2.06747152821866
1.27982992252685 2.3
1.4 2.47959727571912
1.46524774193493 2.6
1.59036244441554 2.9
1.67068479722433 3.2
1.7 3.3873200913312
1.736697170062 3.5
1.83729941337531 3.8
1.90807146994588 4.1
1.96697587525543 4.4
1.9883680750281 4.7
2 4.80174877783435
2.06519232031015 5
2 5
1.95972874947429 5
1.92248559537437 4.7
1.88386539763691 4.4
1.81510313608586 4.1
1.73690929307842 3.8
1.7 3.69809260044837
1.6673285665905 3.5
1.60888145868096 3.2
1.50628047995948 2.9
1.4 2.67706085037876
1.36246240604282 2.6
1.13675620846676 2.3
1.1 2.25247250922896
0.8 2.08024996911982
0.5 2.07679658476117
0.399169701754782 2
0.236286339857405 1.7
0.2 1.56354930895246
0.17120814981188 1.4
0.149947766641217 1.1
0.159100582981724 0.8
0.197426350627825 0.5
0.2 0.488720945157343
0.281327575456297 0.2
0.404083371461603 -0.1
0.5 -0.276197777078057
0.592423610682954 -0.4
0.8 -0.628458071075692
0.906689318599808 -0.7
1.1 -0.812375872060567
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.1 -0.466379850683005
1.4 -0.564462454957503
1.7 -0.555650585775197
2 -0.455134881248826
2.09273243068732 -0.4
2.3 -0.276475863640708
2.52768519860179 -0.1
2.6 -0.0421803002299643
2.86644700274506 0.2
2.9 0.231712036601257
3.1695900349921 0.5
3.2 0.531481165621904
3.45764847962026 0.8
3.5 0.845812347437079
3.73947597360324 1.1
3.8 1.16640206205373
4.01955554319457 1.4
4.1 1.48794871763717
4.30031358216558 1.7
4.4 1.80771573416583
4.58293425106925 2
4.7 2.12482065207582
4.86773215873856 2.3
5 2.43943335684748
5 2.6
5 2.82247784136345
4.79366711359787 2.6
4.7 2.50043822393827
4.51761690279968 2.3
4.4 2.17343814828187
4.24553737035061 2
4.1 1.84119627735261
3.976541752794 1.7
3.8 1.50509363538501
3.70874696372777 1.4
3.5 1.16892448458387
3.43930314512206 1.1
3.2 0.839343327121651
3.16371391566575 0.8
2.9 0.526204544848483
2.87342291622652 0.5
2.6 0.242739050341515
2.54831590079012 0.2
2.3 0.00471278929335286
2.12487600077155 -0.1
2 -0.171659273376072
1.7 -0.254956265715488
1.4 -0.222993403463381
1.17244902189986 -0.1
1.1 -0.0405712797430118
0.90910041661963 0.2
0.8 0.429359523046549
0.773502636143046 0.5
0.710280587698416 0.8
0.69628700459342 1.1
0.756611571973504 1.4
0.8 1.46456697620506
0.960825023517949 1.7
1.1 1.80667235089064
1.2332152141408 2
1.4 2.249736634878
1.4279376354931 2.3
1.58112345708687 2.6
1.6744444088716 2.9
1.7 3.00990876340276
1.7804925512933 3.2
1.86531153637011 3.5
1.9376895336722 3.8
2 4.0946897933495
2.0025347278549 4.1
2.11977847386142 4.4
2.18035938677011 4.7
2.2547005658751 5
2.06519232031015 5
2 4.80174877783435
1.9883680750281 4.7
1.96697587525543 4.4
1.90807146994588 4.1
1.83729941337531 3.8
1.736697170062 3.5
1.7 3.3873200913312
1.67068479722433 3.2
1.59036244441554 2.9
1.46524774193493 2.6
1.4 2.47959727571912
1.27982992252685 2.3
1.1 2.06747152821866
0.963076669257213 2
0.8 1.87339905267401
0.500071454329858 1.7
0.5 1.69987608183132
0.412656772092163 1.4
0.385099986265514 1.1
0.399515045283918 0.8
0.44747738960254 0.5
0.5 0.309810550105422
0.541603710641463 0.2
0.709645835304679 -0.1
0.8 -0.221235841892356
1.00316896499216 -0.4
1.1 -0.466379850683005
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.4 -0.222993403463381
1.7 -0.254956265715488
2 -0.171659273376072
2.12487600077155 -0.1
2.3 0.00471278929335286
2.54831590079012 0.2
2.6 0.242739050341515
2.87342291622652 0.5
2.9 0.526204544848483
3.16371391566575 0.8
3.2 0.839343327121651
3.43930314512206 1.1
3.5 1.16892448458387
3.70874696372777 1.4
3.8 1.50509363538501
3.976541752794 1.7
4.1 1.84119627735261
4.24553737035061 2
4.4 2.17343814828187
4.51761690279968 2.3
4.7 2.50043822393827
4.79366711359787 2.6
5 2.82247784136345
5 2.9
5 3.2
5 3.36460387866135
4.86364713978543 3.2
4.7 3.01016702916008
4.61269966409699 2.9
4.4 2.64488725040398
4.36579169954064 2.6
4.11988165757251 2.3
4.1 2.27722415432974
3.87289649676808 2
3.8 1.91488811616354
3.62509495799514 1.7
3.5 1.5529756488177
3.37312807192067 1.4
3.2 1.19980927938346
3.1127112908778 1.1
2.9 0.866614338295181
2.83538075121806 0.8
2.6 0.568412944763621
2.51972852123419 0.5
2.3 0.323466481726627
2.09146390146506 0.2
2 0.149496788388093
1.7 0.0959289355431222
1.40846591865726 0.2
1.4 0.205112484661205
1.19007489360661 0.5
1.1 0.784062572411478
1.09565725091656 0.8
1.08134100424083 1.1
1.1 1.17656082919531
1.14749155706174 1.4
1.28374973029432 1.7
1.4 1.90026811458504
1.4506651424494 2
1.60245757501803 2.3
1.6969991722388 2.6
1.7 2.61076109789687
1.84157869455917 2.9
1.93361640036147 3.2
1.99392590267822 3.5
2 3.53321618317452
2.1116369874339 3.8
2.22916346696913 4.1
2.3 4.33106958939927
2.34117189304587 4.4
2.47675226956991 4.7
2.56916676173535 5
2.3 5
2.2547005658751 5
2.18035938677011 4.7
2.11977847386142 4.4
2.0025347278549 4.1
2 4.0946897933495
1.9376895336722 3.8
1.86531153637011 3.5
1.7804925512933 3.2
1.7 3.00990876340276
1.6744444088716 2.9
1.58112345708687 2.6
1.4279376354931 2.3
1.4 2.249736634878
1.2332152141408 2
1.1 1.80667235089064
0.960825023517949 1.7
0.8 1.46456697620506
0.756611571973504 1.4
0.69628700459342 1.1
0.710280587698416 0.8
0.773502636143046 0.5
0.8 0.429359523046549
0.90910041661963 0.2
1.1 -0.0405712797430118
1.17244902189986 -0.1
1.4 -0.222993403463381
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.7 0.0959289355431222
2 0.149496788388093
2.09146390146506 0.2
2.3 0.323466481726627
2.51972852123419 0.5
2.6 0.568412944763621
2.83538075121806 0.8
2.9 0.866614338295181
3.1127112908778 1.1
3.2 1.19980927938346
3.37312807192067 1.4
3.5 1.5529756488177
3.62509495799514 1.7
3.8 1.91488811616354
3.87289649676808 2
4.1 2.27722415432974
4.11988165757251 2.3
4.36579169954064 2.6
4.4 2.64488725040398
4.61269966409699 2.9
4.7 3.01016702916008
4.86364713978543 3.2
5 3.36460387866135
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.1 5
3.8 5
3.5 5
3.2 5
2.9 5
2.6 5
2.56916676173535 5
2.47675226956991 4.7
2.34117189304587 4.4
2.3 4.33106958939927
2.22916346696913 4.1
2.1116369874339 3.8
2 3.53321618317452
1.99392590267822 3.5
1.93361640036147 3.2
1.84157869455917 2.9
1.7 2.61076109789687
1.6969991722388 2.6
1.60245757501803 2.3
1.4506651424494 2
1.4 1.90026811458504
1.28374973029432 1.7
1.14749155706174 1.4
1.1 1.17656082919531
1.08134100424083 1.1
1.09565725091656 0.8
1.1 0.784062572411478
1.19007489360661 0.5
1.4 0.205112484661205
1.40846591865726 0.2
1.7 0.0959289355431222

1.56699032136722 0.8
1.49189915381004 1.1
1.51559385226691 1.4
1.59898579120127 1.7
1.69827253169097 2
1.7 2.00467125289676
1.85083211084817 2.3
1.96593122053771 2.6
2 2.70822611818884
2.10635595069808 2.9
2.2334174660442 3.2
2.3 3.3749040013979
2.37509923529026 3.5
2.52508923016466 3.8
2.6 3.96174779549541
2.73874281917323 4.1
2.9 4.25559453387072
3.2 4.33786810953451
3.5 4.37895049912713
3.8 4.36158293026951
4.1 4.2826029260611
4.30429498722269 4.1
4.37013406369054 3.8
4.3020026469923 3.5
4.17882664095433 3.2
4.1 3.05786985090744
4.02040041368056 2.9
3.84414045676212 2.6
3.8 2.53587908355772
3.64526676742677 2.3
3.5 2.08868590977095
3.43893700057339 2
3.22082664337118 1.7
3.2 1.67388884545725
2.97538455110951 1.4
2.9 1.31117931168764
2.70474805956034 1.1
2.6 0.991231218957548
2.38015654218098 0.8
2.3 0.734364103115407
2 0.585196525786507
1.7 0.623773591985308
1.56699032136722 0.8
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.7 0.623773591985308
2 0.585196525786507
2.3 0.734364103115407
2.38015654218098 0.8
2.6 0.991231218957548
2.70474805956034 1.1
2.9 1.31117931168764
2.97538455110951 1.4
3.2 1.67388884545725
3.22082664337118 1.7
3.43893700057339 2
3.5 2.08868590977095
3.64526676742677 2.3
3.8 2.53587908355772
3.84414045676212 2.6
4.02040041368056 2.9
4.1 3.05786985090744
4.17882664095433 3.2
4.3020026469923 3.5
4.37013406369054 3.8
4.30429498722269 4.1
4.1 4.2826029260611
3.8 4.36158293026951
3.5 4.37895049912713
3.2 4.33786810953451
2.9 4.25559453387072
2.73874281917323 4.1
2.6 3.96174779549541
2.52508923016466 3.8
2.37509923529026 3.5
2.3 3.3749040013979
2.2334174660442 3.2
2.10635595069808 2.9
2 2.70822611818884
1.96593122053771 2.6
1.85083211084817 2.3
1.7 2.00467125289676
1.69827253169097 2
1.59898579120127 1.7
1.51559385226691 1.4
1.49189915381004 1.1
1.56699032136722 0.8
1.7 0.623773591985308

2.58870934663548 2
2.6 2.04127561789875
2.60331264899851 2
2.6 1.99467965262418
2.58870934663548 2
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
2.6 1.99467965262418
2.60331264899851 2
2.6 2.04127561789875
2.58870934663548 2
2.6 1.99467965262418
};
\end{axis}



==> fig/tikz/monks-2/CVI_mean_lml.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=black]
table{%
x  y
-0.920107799967142 2.6
-0.7 2.82714254983733
-0.655665014603796 2.9
-0.493390181969532 3.2
-0.4 3.37191777238415
-0.334869954460264 3.5
-0.195320161847708 3.8
-0.1 4.03802210357154
-0.0695970550703829 4.1
0.0662723741844487 4.4
0.191031336141143 4.7
0.2 4.72270913865676
0.331409159960633 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.51967486955673
-0.920107799967142 2.6
};
\addplot [draw=none, fill=midnightblue854116]
table{%
x  y
-0.737552747950222 2.6
-0.7 2.63875295161773
-0.54102677146991 2.9
-0.4 3.16313595275238
-0.380720201429242 3.2
-0.229245824253607 3.5
-0.1 3.79072870763159
-0.0950846334380037 3.8
0.0519046886535025 4.1
0.184642434354555 4.4
0.2 4.43701295206299
0.331110711801016 4.7
0.469121300512775 5
0.331409159960633 5
0.2 4.72270913865676
0.191031336141143 4.7
0.0662723741844487 4.4
-0.0695970550703829 4.1
-0.1 4.03802210357154
-0.195320161847708 3.8
-0.334869954460264 3.5
-0.4 3.37191777238415
-0.493390181969532 3.2
-0.655665014603796 2.9
-0.7 2.82714254983733
-0.920107799967142 2.6
-1 2.51967486955673
-1 2.3361305641013
-0.737552747950222 2.6
};
\addplot [draw=none, fill=midnightblue868137]
table{%
x  y
-0.848560695446037 2.3
-0.7 2.44939234949786
-0.602917911122479 2.6
-0.426388528336024 2.9
-0.4 2.94923725100602
-0.268851749858652 3.2
-0.123621694046949 3.5
-0.1 3.55313521440246
0.0308804494823886 3.8
0.173406432377388 4.1
0.2 4.16028854968378
0.327551082824567 4.4
0.473336067252805 4.7
0.5 4.75838876770947
0.619618416465338 5
0.5 5
0.469121300512775 5
0.331110711801016 4.7
0.2 4.43701295206299
0.184642434354555 4.4
0.0519046886535025 4.1
-0.0950846334380037 3.8
-0.1 3.79072870763159
-0.229245824253607 3.5
-0.380720201429242 3.2
-0.4 3.16313595275238
-0.54102677146991 2.9
-0.7 2.63875295161773
-0.737552747950222 2.6
-1 2.3361305641013
-1 2.3
-1 2.1422721570422
-0.848560695446037 2.3
};
\addplot [draw=none, fill=teal882156]
table{%
x  y
-0.945848725784808 2
-0.7 2.25650753503059
-0.672350061109555 2.3
-0.480693468559175 2.6
-0.4 2.73850331048995
-0.310134337821421 2.9
-0.156983298288062 3.2
-0.1 3.31885256127566
0.00292887734297503 3.5
0.15684553240278 3.8
0.2 3.89146185063008
0.318678581119018 4.1
0.474118054320355 4.4
0.5 4.45355955292162
0.627875115223979 4.7
0.77381084925321 5
0.619618416465338 5
0.5 4.75838876770947
0.473336067252805 4.7
0.327551082824567 4.4
0.2 4.16028854968378
0.173406432377388 4.1
0.0308804494823886 3.8
-0.1 3.55313521440246
-0.123621694046949 3.5
-0.268851749858652 3.2
-0.4 2.94923725100602
-0.426388528336024 2.9
-0.602917911122479 2.6
-0.7 2.44939234949786
-0.848560695446037 2.3
-1 2.1422721570422
-1 2
-1 1.94248951293318
-0.945848725784808 2
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.749327817790461 2
-0.7 2.05146643290291
-0.541997045987355 2.3
-0.4 2.52867090258293
-0.357777843712225 2.6
-0.19339694491525 2.9
-0.1 3.0859621317568
-0.0308332676403845 3.2
0.135507537827228 3.5
0.2 3.62758076634404
0.304381603544435 3.8
0.470611271651926 4.1
0.5 4.15706846450748
0.633084546129453 4.4
0.785255348960459 4.7
0.8 4.73042344482334
0.929936007770934 5
0.8 5
0.77381084925321 5
0.627875115223979 4.7
0.5 4.45355955292162
0.474118054320355 4.4
0.318678581119018 4.1
0.2 3.89146185063008
0.15684553240278 3.8
0.00292887734297505 3.5
-0.1 3.31885256127566
-0.156983298288062 3.2
-0.310134337821421 2.9
-0.4 2.73850331048995
-0.480693468559175 2.6
-0.672350061109555 2.3
-0.7 2.25650753503059
-0.945848725784808 2
-1 1.94248951293318
-1 1.73377765339955
-0.749327817790461 2
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.826066076823109 1.7
-0.7 1.83435284652301
-0.596775758245168 2
-0.411644030865155 2.3
-0.4 2.31875145380049
-0.233519271891089 2.6
-0.1 2.85293568837018
-0.0696377450055647 2.9
0.110144297083494 3.2
0.2 3.36613774642162
0.286107786080632 3.5
0.463158800097386 3.8
0.5 3.86702229683942
0.634944554894372 4.1
0.794710222116807 4.4
0.8 4.41045596242035
0.9454262885797 4.7
1.08645659712984 5
0.929936007770934 5
0.8 4.73042344482334
0.785255348960459 4.7
0.633084546129453 4.4
0.5 4.15706846450748
0.470611271651926 4.1
0.304381603544435 3.8
0.2 3.62758076634404
0.135507537827228 3.5
-0.0308332676403844 3.2
-0.1 3.0859621317568
-0.19339694491525 2.9
-0.357777843712225 2.6
-0.4 2.52867090258293
-0.541997045987355 2.3
-0.7 2.05146643290291
-0.749327817790461 2
-1 1.73377765339955
-1 1.7
-1 1.49578187178308
-0.826066076823109 1.7
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
-0.867020474858366 1.4
-0.7 1.59802809720837
-0.641732064143264 1.7
-0.458958679409548 2
-0.4 2.09588596857943
-0.276671065426125 2.3
-0.109260700069953 2.6
-0.1 2.61754324685723
0.082219258432474 2.9
0.2 3.10442396543776
0.265338748367193 3.2
0.453778403899661 3.5
0.5 3.57924269730822
0.635048555477963 3.8
0.8 4.09575640496149
0.802343400299924 4.1
0.960128912427992 4.4
1.1 4.68751777828749
1.10609782562298 4.7
1.24607977243319 5
1.1 5
1.08645659712984 5
0.9454262885797 4.7
0.8 4.41045596242035
0.794710222116807 4.4
0.634944554894372 4.1
0.5 3.86702229683942
0.463158800097386 3.8
0.286107786080632 3.5
0.2 3.36613774642162
0.110144297083494 3.2
-0.0696377450055647 2.9
-0.1 2.85293568837018
-0.233519271891089 2.6
-0.4 2.31875145380049
-0.411644030865155 2.3
-0.596775758245168 2
-0.7 1.83435284652301
-0.826066076823109 1.7
-1 1.49578187178308
-1 1.4
-1 1.21186405744285
-0.867020474858366 1.4
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
-0.850638926752099 1.1
-0.7 1.31916455234397
-0.661809134236656 1.4
-0.493281224856727 1.7
-0.4 1.85701775728745
-0.31476440214737 2
-0.141244934252241 2.3
-0.1 2.37428036612395
0.0536580434096807 2.6
0.2 2.83912208092427
0.244468523499283 2.9
0.445521889224258 3.2
0.5 3.28834749528219
0.636706633845201 3.5
0.8 3.77994424034276
0.811634598665077 3.8
0.976458615538759 4.1
1.1 4.34618626980149
1.12743671625155 4.4
1.27234001737871 4.7
1.4 4.98603217292057
1.40660055716337 5
1.4 5
1.24607977243319 5
1.10609782562298 4.7
1.1 4.68751777828749
0.960128912427992 4.4
0.802343400299924 4.1
0.8 4.09575640496149
0.635048555477963 3.8
0.5 3.57924269730822
0.453778403899661 3.5
0.265338748367193 3.2
0.2 3.10442396543776
0.082219258432474 2.9
-0.1 2.61754324685723
-0.109260700069953 2.6
-0.276671065426125 2.3
-0.4 2.09588596857943
-0.458958679409548 2
-0.641732064143264 1.7
-0.7 1.59802809720837
-0.867020474858366 1.4
-1 1.21186405744285
-1 1.1
-1 0.808276559704439
-0.850638926752099 1.1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
-0.7 -1
-0.4 -1
-0.300999604925293 -1
-0.4 -0.848657633980007
-0.496075527658535 -0.7
-0.644310174959835 -0.4
-0.7 -0.238029212663569
-0.757190950585458 -0.1
-0.82337277442722 0.2
-0.821090072085807 0.5
-0.751450475454198 0.8
-0.7 0.909150280775696
-0.6379176583879 1.1
-0.50117951761402 1.4
-0.4 1.58867951964136
-0.3381610048284 1.7
-0.16580219654403 2
-0.1 2.11653490286381
0.0299201994138521 2.3
0.2 2.56542520280611
0.226924577497664 2.6
0.442637464434633 2.9
0.5 2.98797242942374
0.645487045857324 3.2
0.8 3.45382126357678
0.828304984792481 3.5
0.999336131269362 3.8
1.1 3.99460227425111
1.1563299734391 4.1
1.30433642705614 4.4
1.4 4.60991248167223
1.44440939971264 4.7
1.58261694615689 5
1.40660055716337 5
1.4 4.98603217292057
1.27234001737871 4.7
1.12743671625155 4.4
1.1 4.34618626980149
0.976458615538759 4.1
0.811634598665077 3.8
0.8 3.77994424034276
0.636706633845201 3.5
0.5 3.28834749528219
0.445521889224258 3.2
0.244468523499283 2.9
0.2 2.83912208092427
0.0536580434096807 2.6
-0.1 2.37428036612395
-0.141244934252241 2.3
-0.31476440214737 2
-0.4 1.85701775728745
-0.493281224856727 1.7
-0.661809134236656 1.4
-0.7 1.31916455234397
-0.850638926752099 1.1
-1 0.808276559704439
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
4.7 3.97322817530533
4.92905012807 4.1
5 4.13327393102003
5 4.4
5 4.7
5 5
4.7 5
4.52998956392185 5
4.47360185386588 4.7
4.42392120244298 4.4
4.44395508323177 4.1
4.7 3.97322817530533
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
-0.4 -0.848657633980007
-0.300999604925293 -1
-0.1 -1
0.2 -1
0.22576750268943 -1
0.2 -0.987397355405176
-0.0907556747013801 -0.7
-0.1 -0.692091201372
-0.300849843389206 -0.4
-0.4 -0.229170367020434
-0.461546046679889 -0.1
-0.552070395989178 0.2
-0.580086158296601 0.5
-0.547996400078823 0.8
-0.463225861340356 1.1
-0.4 1.24832412443486
-0.330032165030882 1.4
-0.171764142556691 1.7
-0.1 1.83075185366585
0.0216598943514213 2
0.2 2.27039836394777
0.224574737815275 2.3
0.453959999208749 2.6
0.5 2.66660972427091
0.671391168025435 2.9
0.8 3.10189850396946
0.864061862666973 3.2
1.03828105757377 3.5
1.1 3.61638834699867
1.20328598809053 3.8
1.35026239459339 4.1
1.4 4.20750549204639
1.49971403485297 4.4
1.63575966472882 4.7
1.7 4.85058495261462
1.77511112497288 5
1.7 5
1.58261694615689 5
1.44440939971264 4.7
1.4 4.60991248167223
1.30433642705614 4.4
1.1563299734391 4.1
1.1 3.99460227425111
0.999336131269362 3.8
0.828304984792481 3.5
0.8 3.45382126357678
0.645487045857324 3.2
0.5 2.98797242942374
0.442637464434633 2.9
0.226924577497664 2.6
0.2 2.56542520280611
0.0299201994138521 2.3
-0.1 2.11653490286381
-0.16580219654403 2
-0.3381610048284 1.7
-0.4 1.58867951964136
-0.50117951761402 1.4
-0.6379176583879 1.1
-0.7 0.909150280775696
-0.751450475454198 0.8
-0.821090072085807 0.5
-0.82337277442722 0.2
-0.757190950585458 -0.1
-0.7 -0.238029212663569
-0.644310174959835 -0.4
-0.496075527658535 -0.7
-0.4 -0.848657633980007
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
2.3 -1
2.6 -1
2.9 -1
3.2 -1
3.5 -1
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.5
5 0.8
5 1.1
5 1.4
5 1.7
5 2
5 2.3
5 2.6
5 2.9
5 3.2
5 3.5
5 3.8
5 4.1
5 4.13327393102003
4.92905012807 4.1
4.7 3.97322817530533
4.44395508323177 4.1
4.42392120244298 4.4
4.47360185386588 4.7
4.52998956392185 5
4.4 5
4.1 5
3.8 5
3.74488760718315 5
3.6606152167265 4.7
3.57039196689039 4.4
3.5 4.17401159595335
3.47918455391182 4.1
3.39461618968347 3.8
3.3045177681672 3.5
3.21022541824669 3.2
3.2 3.16687795753629
3.12376199454335 2.9
3.03452686778239 2.6
2.94053432134424 2.3
2.9 2.1739827551387
2.84926128296473 2
2.76489220683419 1.7
2.6761197711155 1.4
2.6 1.16710888220797
2.58131970560119 1.1
2.51539551071449 0.8
2.45454321169478 0.5
2.39923124041508 0.2
2.3625846419215 -0.1
2.37636529211644 -0.4
2.39611896527755 -0.7
2.3 -0.766973976577944
2.08872918442603 -1
2.3 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
0.2 -0.987397355405176
0.22576750268943 -1
0.5 -1
0.8 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.08872918442603 -1
2.3 -0.766973976577944
2.39611896527755 -0.7
2.37636529211644 -0.4
2.3625846419215 -0.1
2.39923124041508 0.2
2.45454321169478 0.5
2.51539551071449 0.8
2.58131970560119 1.1
2.6 1.16710888220797
2.6761197711155 1.4
2.76489220683419 1.7
2.84926128296473 2
2.9 2.1739827551387
2.94053432134424 2.3
3.03452686778239 2.6
3.12376199454335 2.9
3.2 3.16687795753629
3.21022541824669 3.2
3.3045177681672 3.5
3.39461618968347 3.8
3.47918455391182 4.1
3.5 4.17401159595335
3.57039196689039 4.4
3.6606152167265 4.7
3.74488760718315 5
3.5 5
3.2 5
3.17160473814333 5
3.0854092915777 4.7
2.99436977888813 4.4
2.9 4.11288843229755
2.89576950454465 4.1
2.79557655129515 3.8
2.69223680858442 3.5
2.6 3.25159212755468
2.58106327899355 3.2
2.47239324734398 2.9
2.35743296557936 2.6
2.3 2.45696873333558
2.23858120624334 2.3
2.11934757847342 2
2 1.72335452090336
1.99001943838739 1.7
1.86269109380701 1.4
1.72204204762059 1.1
1.7 1.05479797609606
1.57702890589088 0.8
1.41176945618838 0.5
1.4 0.480099521695426
1.2299325182083 0.2
1.1 0.0223229217337417
0.99950112316184 -0.1
0.8 -0.294004558933668
0.615220806708365 -0.4
0.5 -0.451176915452167
0.2 -0.430207634895825
0.163956997557916 -0.4
-0.1 -0.195277798900189
-0.158351461130445 -0.1
-0.296118030160182 0.2
-0.361343719643415 0.5
-0.344916256191656 0.8
-0.26198189723331 1.1
-0.140984430974521 1.4
-0.1 1.48279733990885
0.0509157162483437 1.7
0.2 1.926701891817
0.265030767439189 2
0.498881945599403 2.3
0.5 2.30152601300789
0.737361300539822 2.6
0.8 2.69319802046219
0.945743306542202 2.9
1.1 3.17451806215197
1.1163614657832 3.2
1.29128131495003 3.5
1.4 3.73234576778532
1.43926161311286 3.8
1.59388223820957 4.1
1.7 4.3519529606909
1.72719581407692 4.4
1.87999805107457 4.7
2 4.99822723649565
2.0010399098099 5
2 5
1.77511112497288 5
1.7 4.85058495261462
1.63575966472882 4.7
1.49971403485297 4.4
1.4 4.20750549204638
1.35026239459339 4.1
1.20328598809053 3.8
1.1 3.61638834699867
1.03828105757377 3.5
0.864061862666973 3.2
0.8 3.10189850396946
0.671391168025435 2.9
0.5 2.66660972427091
0.453959999208749 2.6
0.224574737815275 2.3
0.2 2.27039836394777
0.0216598943514213 2
-0.1 1.83075185366585
-0.171764142556691 1.7
-0.330032165030882 1.4
-0.4 1.24832412443486
-0.463225861340356 1.1
-0.547996400078823 0.8
-0.580086158296601 0.5
-0.552070395989178 0.2
-0.461546046679889 -0.1
-0.4 -0.229170367020434
-0.300849843389206 -0.4
-0.1 -0.692091201372
-0.0907556747013801 -0.7
0.2 -0.987397355405176
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
0.2 -0.430207634895825
0.5 -0.451176915452167
0.615220806708365 -0.4
0.8 -0.294004558933668
0.99950112316184 -0.1
1.1 0.0223229217337417
1.2299325182083 0.2
1.4 0.480099521695426
1.41176945618838 0.5
1.57702890589088 0.8
1.7 1.05479797609606
1.72204204762059 1.1
1.86269109380701 1.4
1.99001943838739 1.7
2 1.72335452090336
2.11934757847342 2
2.23858120624334 2.3
2.3 2.45696873333558
2.35743296557936 2.6
2.47239324734398 2.9
2.58106327899355 3.2
2.6 3.25159212755468
2.69223680858442 3.5
2.79557655129515 3.8
2.89576950454465 4.1
2.9 4.11288843229755
2.99436977888813 4.4
3.0854092915777 4.7
3.17160473814333 5
2.9 5
2.6 5
2.3 5
2.0010399098099 5
2 4.99822723649565
1.87999805107457 4.7
1.72719581407692 4.4
1.7 4.3519529606909
1.59388223820957 4.1
1.43926161311286 3.8
1.4 3.73234576778532
1.29128131495003 3.5
1.1163614657832 3.2
1.1 3.17451806215197
0.945743306542202 2.9
0.8 2.69319802046219
0.737361300539822 2.6
0.5 2.30152601300789
0.498881945599403 2.3
0.265030767439189 2
0.2 1.926701891817
0.0509157162483437 1.7
-0.1 1.48279733990885
-0.140984430974521 1.4
-0.26198189723331 1.1
-0.344916256191656 0.8
-0.361343719643415 0.5
-0.296118030160182 0.2
-0.158351461130445 -0.1
-0.1 -0.195277798900189
0.163956997557916 -0.4
0.2 -0.430207634895825

0.172771508228072 0.2
-0.069633870343601 0.5
-0.0982279072883391 0.8
0.0136956222242727 1.1
0.165761233897707 1.4
0.2 1.45615191771887
0.430707670699826 1.7
0.5 1.7830722311442
0.723093765305484 2
0.8 2.09497744423645
0.989316328093617 2.3
1.1 2.47594970436328
1.20893947879339 2.6
1.37018256431798 2.9
1.4 2.96423739952787
1.57672855044161 3.2
1.68965487710129 3.5
1.7 3.52614426795332
1.908525266759 3.8
2 4.0909372563737
2.13920845451018 3.8
2.07478720514274 3.5
2 3.21424270563354
1.99073251592057 3.2
1.84248581580715 2.9
1.7421548551895 2.6
1.7 2.48786548454142
1.59710687146309 2.3
1.47341002853799 2
1.4 1.82336621703259
1.33458378557529 1.7
1.19351109220695 1.4
1.1 1.20330223272426
1.04582323329427 1.1
0.882905886591578 0.8
0.8 0.665753672718882
0.680450615717748 0.5
0.5 0.297465165226767
0.27087788239829 0.2
0.2 0.178124312097543
0.172771508228072 0.2

2.27803308195184 4.4
2.3 4.47014232984446
2.31783387633143 4.4
2.3 4.19386330308158
2.27803308195184 4.4
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
0.2 0.178124312097543
0.27087788239829 0.2
0.5 0.297465165226767
0.680450615717748 0.5
0.8 0.665753672718883
0.882905886591578 0.8
1.04582323329427 1.1
1.1 1.20330223272426
1.19351109220695 1.4
1.33458378557529 1.7
1.4 1.82336621703259
1.47341002853799 2
1.59710687146309 2.3
1.7 2.48786548454142
1.7421548551895 2.6
1.84248581580715 2.9
1.99073251592057 3.2
2 3.21424270563354
2.07478720514274 3.5
2.13920845451018 3.8
2 4.0909372563737
1.908525266759 3.8
1.7 3.52614426795332
1.68965487710129 3.5
1.57672855044161 3.2
1.4 2.96423739952787
1.37018256431798 2.9
1.20893947879339 2.6
1.1 2.47594970436328
0.989316328093617 2.3
0.8 2.09497744423645
0.723093765305484 2
0.5 1.7830722311442
0.430707670699826 1.7
0.2 1.45615191771887
0.165761233897707 1.4
0.0136956222242726 1.1
-0.0982279072883391 0.8
-0.0696338703436009 0.5
0.172771508228072 0.2
0.2 0.178124312097543
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
2.3 4.19386330308158
2.31783387633143 4.4
2.3 4.47014232984446
2.27803308195184 4.4
2.3 4.19386330308158
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
0.5 1.1
};
\coordinate (CVI_mean_lml_t) at (axis cs:0.5,1.1);
\end{axis}



==> fig/tikz/monks-2/CVI_mean_lml_ep.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
-0.97525226931139 2
-0.932222577809493 2.3
-0.91207964947791 2.6
-0.901938618771274 2.9
-0.896614312919123 3.2
-0.893463511902922 3.5
-0.892350555504677 3.8
-0.889737660918043 4.1
-0.888238491116599 4.4
-0.889162149211957 4.7
-0.890608844845943 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.88932358528935
-0.97525226931139 2
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
-0.7 -1
-0.4 -1
-0.3011288580888 -1
-0.4 -0.84930619825004
-0.496790049525929 -0.7
-0.646944825021479 -0.4
-0.7 -0.257743928700262
-0.770892638487678 -0.1
-0.861711979770339 0.2
-0.914028938419039 0.5
-0.943521856217833 0.8
-0.952951537143442 1.1
-0.928245805992006 1.4
-0.876429830730517 1.7
-0.831428182018604 2
-0.80422392063189 2.3
-0.788689272406753 2.6
-0.780960529477013 2.9
-0.775435595074854 3.2
-0.769016228516305 3.5
-0.766937271532894 3.8
-0.766115937502952 4.1
-0.764421369572577 4.4
-0.765362325609484 4.7
-0.765799098029738 5
-0.890608844845943 5
-0.889162149211957 4.7
-0.888238491116599 4.4
-0.889737660918043 4.1
-0.892350555504677 3.8
-0.893463511902922 3.5
-0.896614312919123 3.2
-0.901938618771274 2.9
-0.91207964947791 2.6
-0.932222577809493 2.3
-0.97525226931139 2
-1 1.88932358528935
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
4.7 3.97324597276211
4.92902240765937 4.1
5 4.13328607734118
5 4.4
5 4.7
5 5
4.7 5
4.53005178095103 5
4.47365337996902 4.7
4.42397212253614 4.4
4.44402830070764 4.1
4.7 3.97324597276211
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
-0.4 -0.84930619825004
-0.3011288580888 -1
-0.1 -1
0.2 -1
0.225569024611727 -1
0.2 -0.987512904203333
-0.0914549511029986 -0.7
-0.1 -0.692746086348342
-0.303073283706847 -0.4
-0.4 -0.240164447674899
-0.469868948072664 -0.1
-0.577610124461439 0.2
-0.645875986135609 0.5
-0.687598230029835 0.8
-0.7 0.967071365202493
-0.711617142131497 1.1
-0.714186150439763 1.4
-0.701316239575394 1.7
-0.7 1.72406445937573
-0.686270080116989 2
-0.671790870598363 2.3
-0.658195326720599 2.6
-0.649983075209307 2.9
-0.642351464267436 3.2
-0.632413018563346 3.5
-0.627375811645272 3.8
-0.623760989328005 4.1
-0.623646699357831 4.4
-0.625826069785111 4.7
-0.625705460611982 5
-0.7 5
-0.765799098029738 5
-0.765362325609484 4.7
-0.764421369572577 4.4
-0.766115937502952 4.1
-0.766937271532894 3.8
-0.769016228516305 3.5
-0.775435595074854 3.2
-0.780960529477013 2.9
-0.788689272406753 2.6
-0.80422392063189 2.3
-0.831428182018604 2
-0.876429830730517 1.7
-0.928245805992006 1.4
-0.952951537143442 1.1
-0.943521856217833 0.8
-0.91402893841904 0.5
-0.861711979770339 0.2
-0.770892638487678 -0.1
-0.7 -0.257743928700262
-0.646944825021479 -0.4
-0.496790049525929 -0.7
-0.4 -0.84930619825004
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
2.3 -1
2.6 -1
2.9 -1
3.2 -1
3.5 -1
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.5
5 0.8
5 1.1
5 1.4
5 1.7
5 2
5 2.3
5 2.6
5 2.9
5 3.2
5 3.5
5 3.8
5 4.1
5 4.13328607734118
4.92902240765937 4.1
4.7 3.97324597276211
4.44402830070764 4.1
4.42397212253613 4.4
4.47365337996902 4.7
4.53005178095103 5
4.4 5
4.1 5
3.8 5
3.74547102629578 5
3.66114475279069 4.7
3.57084147763053 4.4
3.5 4.17281547866344
3.47951578629619 4.1
3.39493348469236 3.8
3.3047869975814 3.5
3.21043732514236 3.2
3.2 3.16621077350362
3.12393330238167 2.9
3.0346707693314 2.6
2.94064654266202 2.3
2.9 2.17367800091953
2.84934167419289 2
2.7649612745509 1.7
2.67617675474316 1.4
2.6 1.16698301585867
2.58135231980063 1.1
2.51542540657076 0.8
2.45456998472544 0.5
2.39925679942786 0.2
2.36261047085138 -0.1
2.37639043651404 -0.4
2.39614343649514 -0.7
2.3 -0.766992119597533
2.08874453011251 -1
2.3 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
0.2 -0.987512904203332
0.225569024611727 -1
0.5 -1
0.8 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.08874453011251 -1
2.3 -0.766992119597533
2.39614343649514 -0.7
2.37639043651404 -0.4
2.36261047085138 -0.1
2.39925679942786 0.2
2.45456998472544 0.5
2.51542540657076 0.8
2.58135231980063 1.1
2.6 1.16698301585867
2.67617675474316 1.4
2.7649612745509 1.7
2.84934167419289 2
2.9 2.17367800091953
2.94064654266202 2.3
3.0346707693314 2.6
3.12393330238166 2.9
3.2 3.16621077350362
3.21043732514236 3.2
3.3047869975814 3.5
3.39493348469236 3.8
3.47951578629619 4.1
3.5 4.17281547866344
3.57084147763053 4.4
3.66114475279069 4.7
3.74547102629578 5
3.5 5
3.2 5
3.17691944210985 5
3.09029325753857 4.7
2.99814799033303 4.4
2.9 4.10461122686218
2.8984942561579 4.1
2.79851471738287 3.8
2.69467085314811 3.5
2.6 3.24646324423536
2.58300829085673 3.2
2.47442738721158 2.9
2.35911767002208 2.6
2.3 2.45324784499644
2.24014635367978 2.3
2.12079734885936 2
2 1.72087602260921
1.99109456006501 1.7
1.86387321540813 1.4
1.72297408138959 1.1
1.7 1.05295007533724
1.57796289572424 0.8
1.41251521811832 0.5
1.4 0.478854106403645
1.23071185313772 0.2
1.1 0.0213572292448348
1.00032055769184 -0.1
0.8 -0.294839049704366
0.61694835468439 -0.4
0.5 -0.452069007293833
0.2 -0.431842443377406
0.16164713679439 -0.4
-0.1 -0.203323713369142
-0.16551462155828 -0.1
-0.323022260001164 0.2
-0.4 0.396931339488241
-0.4289679915501 0.5
-0.482614159024565 0.8
-0.512630484034288 1.1
-0.52642747173246 1.4
-0.529844239274343 1.7
-0.526968024147752 2
-0.519918286159152 2.3
-0.509546041656968 2.6
-0.49877565473724 2.9
-0.489633957837323 3.2
-0.480674678894873 3.5
-0.471618987992666 3.8
-0.459867952458055 4.1
-0.464479661445022 4.4
-0.468688618801034 4.7
-0.468569708988599 5
-0.625705460611982 5
-0.625826069785111 4.7
-0.623646699357831 4.4
-0.623760989328005 4.1
-0.627375811645272 3.8
-0.632413018563346 3.5
-0.642351464267436 3.2
-0.649983075209307 2.9
-0.658195326720599 2.6
-0.671790870598363 2.3
-0.686270080116989 2
-0.7 1.72406445937573
-0.701316239575394 1.7
-0.714186150439763 1.4
-0.711617142131497 1.1
-0.7 0.967071365202493
-0.687598230029835 0.8
-0.645875986135609 0.5
-0.577610124461439 0.2
-0.469868948072664 -0.1
-0.4 -0.240164447674899
-0.303073283706847 -0.4
-0.1 -0.692746086348342
-0.0914549511029986 -0.7
0.2 -0.987512904203332
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
0.2 -0.431842443377406
0.5 -0.452069007293833
0.61694835468439 -0.4
0.8 -0.294839049704366
1.00032055769184 -0.1
1.1 0.0213572292448348
1.23071185313772 0.2
1.4 0.478854106403645
1.41251521811832 0.5
1.57796289572424 0.8
1.7 1.05295007533724
1.72297408138959 1.1
1.86387321540813 1.4
1.99109456006501 1.7
2 1.72087602260921
2.12079734885936 2
2.24014635367978 2.3
2.3 2.45324784499644
2.35911767002208 2.6
2.47442738721158 2.9
2.58300829085673 3.2
2.6 3.24646324423536
2.69467085314811 3.5
2.79851471738287 3.8
2.8984942561579 4.1
2.9 4.10461122686218
2.99814799033303 4.4
3.09029325753857 4.7
3.17691944210985 5
2.9 5
2.61455775170223 5
2.6 4.93524469884942
2.52023291603366 4.7
2.43257133142084 4.4
2.35075329888756 4.1
2.3 3.9302630286436
2.24544703019644 3.8
2.13202366378759 3.5
2.02957525025705 3.2
2 3.11968626841226
1.89697189003585 2.9
1.77515508425829 2.6
1.7 2.41350799553003
1.64289605957389 2.3
1.50411947256562 2
1.4 1.76452902418816
1.36736469544382 1.7
1.21787401783922 1.4
1.1 1.16270942579464
1.06733527098461 1.1
0.899860400023334 0.8
0.8 0.641104688085241
0.698335162881309 0.5
0.5 0.278087584793829
0.329125117758456 0.2
0.2 0.156303417888548
0.136902389742971 0.2
-0.1 0.390780779545637
-0.144083743316103 0.5
-0.225621038469594 0.8
-0.275082087082615 1.1
-0.304760768798108 1.4
-0.324836565257004 1.7
-0.33402927693619 2
-0.327202874041706 2.3
-0.301715861091076 2.6
-0.259723063798931 2.9
-0.217039293676519 3.2
-0.158277370522084 3.5
-0.1 3.69413479724631
0.117945585651844 3.8
0.2 3.84128742932451
0.368590211288512 4.1
0.5 4.28927979503243
0.795665007409399 4.1
0.8 4.09713110452154
0.822439402449223 4.1
1.1 4.13790277829795
1.36542359269808 4.4
1.4 4.44000987685849
1.55166561667691 4.7
1.69410365379653 5
1.4 5
1.1 5
0.8 5
0.5 5
0.2 5
-0.1 5
-0.4 5
-0.468569708988599 5
-0.468688618801034 4.7
-0.464479661445022 4.4
-0.459867952458055 4.1
-0.471618987992666 3.8
-0.480674678894873 3.5
-0.489633957837323 3.2
-0.49877565473724 2.9
-0.509546041656968 2.6
-0.519918286159152 2.3
-0.526968024147752 2
-0.529844239274343 1.7
-0.52642747173246 1.4
-0.512630484034288 1.1
-0.482614159024565 0.8
-0.4289679915501 0.5
-0.4 0.396931339488241
-0.323022260001164 0.2
-0.16551462155828 -0.1
-0.1 -0.203323713369142
0.16164713679439 -0.4
0.2 -0.431842443377406
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
0.2 0.156303417888548
0.329125117758456 0.2
0.5 0.278087584793829
0.698335162881309 0.5
0.8 0.641104688085241
0.899860400023334 0.8
1.06733527098461 1.1
1.1 1.16270942579464
1.21787401783922 1.4
1.36736469544382 1.7
1.4 1.76452902418816
1.50411947256562 2
1.64289605957389 2.3
1.7 2.41350799553003
1.77515508425829 2.6
1.89697189003585 2.9
2 3.11968626841225
2.02957525025705 3.2
2.13202366378759 3.5
2.24544703019644 3.8
2.3 3.9302630286436
2.35075329888756 4.1
2.43257133142084 4.4
2.52023291603366 4.7
2.6 4.93524469884942
2.61455775170223 5
2.6 5
2.3 5
2 5
1.7 5
1.69410365379653 5
1.55166561667691 4.7
1.4 4.44000987685849
1.36542359269808 4.4
1.1 4.13790277829795
0.822439402449223 4.1
0.8 4.09713110452154
0.795665007409399 4.1
0.5 4.28927979503243
0.368590211288512 4.1
0.2 3.84128742932451
0.117945585651844 3.8
-0.1 3.69413479724631
-0.158277370522084 3.5
-0.217039293676519 3.2
-0.259723063798931 2.9
-0.301715861091076 2.6
-0.327202874041706 2.3
-0.334029276936191 2
-0.324836565257004 1.7
-0.304760768798108 1.4
-0.275082087082615 1.1
-0.225621038469594 0.8
-0.144083743316103 0.5
-0.1 0.390780779545637
0.136902389742971 0.2
0.2 0.156303417888548

0.196416719462205 1.7
0.2 1.75487525248871
0.208429396547629 1.7
0.2 1.65969683452467
0.196416719462205 1.7
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
0.2 1.65969683452467
0.208429396547629 1.7
0.2 1.75487525248871
0.196416719462205 1.7
0.2 1.65969683452467
};
\addplot [semithick, steelblue31119180, mark=mystar, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
0.2 1.7
};
\coordinate (CVI_mean_lml_ep_t) at (axis cs:0.19999999999999996,1.6999999999999997);
\end{axis}



==> fig/tikz/monks-2/EP_mean_lml.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
-0.7 -1
-0.4 -1
-0.301129187761653 -1
-0.4 -0.849306756573533
-0.496790417224104 -0.7
-0.646945454606407 -0.4
-0.7 -0.257750119111283
-0.770896862364333 -0.1
-0.861730599939512 0.2
-0.914096157662696 0.5
-0.944148118735225 0.8
-0.961208446699022 1.1
-0.970784970259666 1.4
-0.976114079346522 1.7
-0.979062599401558 2
-0.980688274841379 2.3
-0.981582775459348 2.6
-0.982074393087576 2.9
-0.982344412282142 3.2
-0.982492666990132 3.5
-0.982574050326342 3.8
-0.982618720295619 4.1
-0.982643237284906 4.4
-0.98265667035997 4.7
-0.982664061876877 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
4.7 3.9732454868231
4.9290234444048 4.1
5 4.1332855624664
5 4.4
5 4.7
5 5
4.7 5
4.53005190676344 5
4.47365348667205 4.7
4.42397219830206 4.4
4.44402802336383 4.1
4.7 3.9732454868231
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
-0.4 -0.849306756573533
-0.301129187761653 -1
-0.1 -1
0.2 -1
0.225568031249843 -1
0.2 -0.987513406145137
-0.0914556959859441 -0.7
-0.1 -0.692746770948018
-0.303074746358663 -0.4
-0.4 -0.240175935903742
-0.469877305162018 -0.1
-0.577650559554616 0.2
-0.646022055315696 0.5
-0.688185718182388 0.8
-0.7 0.938751962751864
-0.716417492321437 1.1
-0.733865997234772 1.4
-0.743521556865514 1.7
-0.748846476345805 2
-0.751776969134168 2.3
-0.753387759805958 2.6
-0.754272544371908 2.9
-0.754758352665147 3.2
-0.755025044640356 3.5
-0.755171427964971 3.8
-0.755251770651913 4.1
-0.755295863001119 4.4
-0.755320061795957 4.7
-0.755333344057494 5
-0.982664061876877 5
-0.98265667035997 4.7
-0.982643237284906 4.4
-0.982618720295619 4.1
-0.982574050326342 3.8
-0.982492666990132 3.5
-0.982344412282142 3.2
-0.982074393087576 2.9
-0.981582775459348 2.6
-0.980688274841379 2.3
-0.979062599401558 2
-0.976114079346522 1.7
-0.970784970259666 1.4
-0.961208446699022 1.1
-0.944148118735225 0.8
-0.914096157662696 0.5
-0.861730599939512 0.2
-0.770896862364333 -0.1
-0.7 -0.257750119111283
-0.646945454606407 -0.4
-0.496790417224104 -0.7
-0.4 -0.849306756573533
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
2.3 -1
2.6 -1
2.9 -1
3.2 -1
3.5 -1
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.5
5 0.8
5 1.1
5 1.4
5 1.7
5 2
5 2.3
5 2.6
5 2.9
5 3.2
5 3.5
5 3.8
5 4.1
5 4.1332855624664
4.9290234444048 4.1
4.7 3.9732454868231
4.44402802336383 4.1
4.42397219830206 4.4
4.47365348667205 4.7
4.53005190676344 5
4.4 5
4.1 5
3.8 5
3.745472980996 5
3.66114635668975 4.7
3.5708426388244 4.4
3.5 4.17281270793013
3.47951657537183 4.1
3.39493423488628 3.8
3.30478755468014 3.5
3.2104377197 3.2
3.2 3.16620953152581
3.12393364829683 2.9
3.03467105151717 2.6
2.94064677643784 2.3
2.9 2.17367732510046
2.84934186309321 2
2.76496144842226 1.7
2.67617692999021 1.4
2.6 1.1669825487076
2.58135244297534 1.1
2.515425515162 0.8
2.45457008561515 0.5
2.39925688492026 0.2
2.36261050131375 -0.1
2.37639036012176 -0.4
2.39614361726619 -0.7
2.3 -0.766992484497325
2.08874571067732 -1
2.3 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
0.2 -0.987513406145137
0.225568031249843 -1
0.5 -1
0.8 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.08874571067732 -1
2.3 -0.766992484497325
2.39614361726619 -0.7
2.37639036012176 -0.4
2.36261050131375 -0.1
2.39925688492026 0.2
2.45457008561515 0.5
2.515425515162 0.8
2.58135244297534 1.1
2.6 1.1669825487076
2.67617692999021 1.4
2.76496144842226 1.7
2.84934186309321 2
2.9 2.17367732510046
2.94064677643784 2.3
3.03467105151717 2.6
3.12393364829683 2.9
3.2 3.16620953152581
3.2104377197 3.2
3.30478755468014 3.5
3.39493423488628 3.8
3.47951657537183 4.1
3.5 4.17281270793013
3.5708426388244 4.4
3.66114635668975 4.7
3.745472980996 5
3.5 5
3.2 5
3.176985431703 5
3.0903542869531 4.7
2.9981844927007 4.4
2.9 4.10455295808962
2.89851361910304 4.1
2.79854124922443 3.8
2.69468796033843 3.5
2.6 3.24643439628645
2.58302048877392 3.2
2.47444071034972 2.9
2.35912594341028 2.6
2.3 2.45323105517994
2.24015480285802 2.3
2.12080375399036 2
2 1.72086775369791
1.99109832266677 1.7
1.8638775660348 1.4
1.72297652408129 1.1
1.7 1.0529453107052
1.5779655329325 0.8
1.41251673093404 0.5
1.4 0.478851589201338
1.23071343603649 0.2
1.1 0.0213553665171038
1.00032202618617 -0.1
0.8 -0.294840560174458
0.616950958179982 -0.4
0.5 -0.452070348934349
0.2 -0.431844691887662
0.161644102953842 -0.4
-0.1 -0.203340867716977
-0.165529298322137 -0.1
-0.323111073546014 0.2
-0.4 0.396165914220634
-0.429247749101146 0.5
-0.48347000828796 0.8
-0.515250772884952 1.1
-0.533439711684728 1.4
-0.543675825941442 1.7
-0.54937534412754 2
-0.552528927559883 2.3
-0.554267652139304 2.6
-0.555224186588334 2.9
-0.555749943860613 3.2
-0.556038697058157 3.5
-0.556197205675324 3.8
-0.556284247326562 4.1
-0.556331991757354 4.4
-0.556358137529699 4.7
-0.556372625886749 5
-0.7 5
-0.755333344057494 5
-0.755320061795957 4.7
-0.755295863001119 4.4
-0.755251770651913 4.1
-0.755171427964971 3.8
-0.755025044640356 3.5
-0.754758352665147 3.2
-0.754272544371908 2.9
-0.753387759805958 2.6
-0.751776969134168 2.3
-0.748846476345805 2
-0.743521556865514 1.7
-0.733865997234772 1.4
-0.716417492321437 1.1
-0.7 0.938751962751864
-0.688185718182388 0.8
-0.646022055315696 0.5
-0.577650559554616 0.2
-0.469877305162018 -0.1
-0.4 -0.240175935903742
-0.303074746358663 -0.4
-0.1 -0.692746770948018
-0.0914556959859441 -0.7
0.2 -0.987513406145137
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
0.2 -0.431844691887662
0.5 -0.452070348934349
0.616950958179982 -0.4
0.8 -0.294840560174458
1.00032202618617 -0.1
1.1 0.0213553665171038
1.23071343603649 0.2
1.4 0.478851589201338
1.41251673093404 0.5
1.5779655329325 0.8
1.7 1.0529453107052
1.72297652408129 1.1
1.8638775660348 1.4
1.99109832266677 1.7
2 1.72086775369791
2.12080375399036 2
2.24015480285802 2.3
2.3 2.45323105517994
2.35912594341028 2.6
2.47444071034972 2.9
2.58302048877392 3.2
2.6 3.24643439628645
2.69468796033843 3.5
2.79854124922443 3.8
2.89851361910304 4.1
2.9 4.10455295808962
2.9981844927007 4.4
3.0903542869531 4.7
3.176985431703 5
2.9 5
2.61892196397443 5
2.6 4.91813296188899
2.52729362520901 4.7
2.43652117085491 4.4
2.35257153175899 4.1
2.3 3.92573433465028
2.24792112444102 3.8
2.13370297759111 3.5
2.03036329770598 3.2
2 3.11776168658483
1.89831807812482 2.9
1.77589358625951 2.6
1.7 2.41214520857429
1.6437905698357 2.3
1.50471727472231 2
1.4 1.76364873758174
1.36786616869036 1.7
1.21825312223788 1.4
1.1 1.16221928471544
1.0675938870705 1.1
0.900041761484729 0.8
0.8 0.640868160973054
0.698483643942616 0.5
0.5 0.277947503394804
0.329431550770419 0.2
0.2 0.156176335038154
0.136667940111999 0.2
-0.1 0.389835271474425
-0.144604918137706 0.5
-0.227345584620891 0.8
-0.279025687506569 1.1
-0.309668853325422 1.4
-0.327254864305549 1.7
-0.337153864058677 2
-0.342664219396754 2.3
-0.345712600349279 2.6
-0.347392632850572 2.9
-0.348317071564422 3.2
-0.34882455763794 3.5
-0.349103069186907 3.8
-0.349256890688297 4.1
-0.349340784792028 4.4
-0.349386671060326 4.7
-0.349412068401548 5
-0.4 5
-0.556372625886749 5
-0.556358137529699 4.7
-0.556331991757354 4.4
-0.556284247326562 4.1
-0.556197205675324 3.8
-0.556038697058157 3.5
-0.555749943860613 3.2
-0.555224186588334 2.9
-0.554267652139304 2.6
-0.552528927559883 2.3
-0.54937534412754 2
-0.543675825941442 1.7
-0.533439711684728 1.4
-0.515250772884952 1.1
-0.48347000828796 0.8
-0.429247749101146 0.5
-0.4 0.396165914220634
-0.323111073546014 0.2
-0.165529298322137 -0.1
-0.1 -0.203340867716977
0.161644102953842 -0.4
0.2 -0.431844691887662
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
0.2 0.156176335038154
0.329431550770419 0.2
0.5 0.277947503394804
0.698483643942616 0.5
0.8 0.640868160973054
0.900041761484729 0.8
1.0675938870705 1.1
1.1 1.16221928471544
1.21825312223788 1.4
1.36786616869036 1.7
1.4 1.76364873758174
1.50471727472231 2
1.6437905698357 2.3
1.7 2.41214520857429
1.77589358625951 2.6
1.89831807812482 2.9
2 3.11776168658483
2.03036329770598 3.2
2.13370297759111 3.5
2.24792112444102 3.8
2.3 3.92573433465028
2.35257153175899 4.1
2.43652117085491 4.4
2.52729362520901 4.7
2.6 4.91813296188899
2.61892196397443 5
2.6 5
2.3 5
2 5
1.7 5
1.4 5
1.1 5
0.8 5
0.504443496663082 5
0.504356802569745 4.7
0.504196201032246 4.4
0.503903002095767 4.1
0.503365357368379 3.8
0.502380996778014 3.5
0.500547636899416 3.2
0.5 3.15187287456212
0.495320770435094 2.9
0.484799453752751 2.6
0.464643691440085 2.3
0.425911382614737 2
0.353659555485811 1.7
0.229738285518987 1.4
0.2 1.35611674378397
0.183585166770394 1.4
0.119141815320184 1.7
0.0828944238912264 2
0.0627239532477024 2.3
0.0515658798084649 2.6
0.0454135738333662 2.9
0.0420281245121197 3.2
0.0401731364917775 3.5
0.039155956521024 3.8
0.038587965636053 4.1
0.0383145191194321 4.4
0.0381395323713309 4.7
0.0380312629848861 5
-0.1 5
-0.349412068401548 5
-0.349386671060326 4.7
-0.349340784792028 4.4
-0.349256890688297 4.1
-0.349103069186907 3.8
-0.34882455763794 3.5
-0.348317071564422 3.2
-0.347392632850572 2.9
-0.345712600349279 2.6
-0.342664219396754 2.3
-0.337153864058677 2
-0.327254864305549 1.7
-0.309668853325422 1.4
-0.279025687506569 1.1
-0.227345584620891 0.8
-0.144604918137706 0.5
-0.1 0.389835271474425
0.136667940111999 0.2
0.2 0.156176335038154
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
0.2 1.35611674378397
0.229738285518987 1.4
0.353659555485811 1.7
0.425911382614737 2
0.464643691440085 2.3
0.484799453752751 2.6
0.495320770435094 2.9
0.5 3.15187287456212
0.500547636899416 3.2
0.502380996778014 3.5
0.503365357368379 3.8
0.503903002095767 4.1
0.504196201032246 4.4
0.504356802569745 4.7
0.504443496663082 5
0.5 5
0.2 5
0.0380312629848861 5
0.0381395323713309 4.7
0.0383145191194321 4.4
0.038587965636053 4.1
0.039155956521024 3.8
0.0401731364917775 3.5
0.0420281245121197 3.2
0.0454135738333662 2.9
0.0515658798084649 2.6
0.0627239532477023 2.3
0.0828944238912264 2
0.119141815320184 1.7
0.183585166770394 1.4
0.2 1.35611674378397
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
0.2 5
};
\coordinate (EP_mean_lml_t) at (axis cs:0.19999999999999996,5.0);
\end{axis}



==> fig/tikz/monks-2/EP_nlpd.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
3.5 -1
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.5
5 0.8
5 0.866695855702396
4.93395294535289 0.8
4.7 0.561402380348049
4.63968865299602 0.5
4.4 0.251483291236795
4.35019387569185 0.2
4.1 -0.0675342543831391
4.06947648652586 -0.1
3.8068878928401 -0.4
3.8 -0.409985089487919
3.59735640323214 -0.7
3.5 -0.919499741828612
3.46360714415965 -1
3.5 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
-0.7 -1
-0.401391977962482 -1
-0.610937176149326 -0.7
-0.7 -0.525980913600416
-0.767727671836684 -0.4
-0.886115553004937 -0.1
-0.955130211553321 0.2
-0.995587597917725 0.5
-1 0.552066060450769
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
1.1 -1
1.4 -1
1.7 -1
2 -1
2.3 -1
2.6 -1
2.9 -1
3.2 -1
3.46360714415965 -1
3.5 -0.919499741828612
3.59735640323215 -0.7
3.8 -0.409985089487919
3.8068878928401 -0.4
4.06947648652586 -0.1
4.1 -0.0675342543831391
4.35019387569185 0.2
4.4 0.251483291236795
4.63968865299602 0.5
4.7 0.561402380348049
4.93395294535289 0.8
5 0.866695855702396
5 1.1
5 1.4
5 1.7
5 2
5 2.3
5 2.6
5 2.9
5 3.2
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.58229072995892 5
4.42227503933907 4.7
4.4 4.65942604006138
4.2757819183725 4.4
4.11339742855596 4.1
4.1 4.07580500484418
3.96686152195469 3.8
3.80107625504408 3.5
3.8 3.49807721466367
3.65456217410415 3.2
3.5 2.92431387727759
3.48804415381498 2.9
3.33742094988032 2.6
3.2 2.35922960550778
3.17005102972374 2.3
3.01302991573085 2
2.9 1.80658966838433
2.84408480915337 1.7
2.67691656371397 1.4
2.6 1.27246576023734
2.5050526038892 1.1
2.31969131697275 0.8
2.3 0.768758261723015
2.14190094975039 0.5
2 0.289066095262475
1.94135156210471 0.2
1.72831567786959 -0.1
1.7 -0.138502472104023
1.5028599505206 -0.4
1.4 -0.526634878800062
1.24794535631729 -0.7
1.1 -0.867612760484385
0.969611209672371 -1
1.1 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
-0.4 -1
-0.1 -1
0.2 -1
0.5 -1
0.8 -1
0.969611209672371 -1
1.1 -0.867612760484385
1.24794535631729 -0.7
1.4 -0.526634878800062
1.5028599505206 -0.4
1.7 -0.138502472104023
1.72831567786959 -0.1
1.94135156210471 0.2
2 0.289066095262475
2.14190094975039 0.5
2.3 0.768758261723015
2.31969131697275 0.8
2.5050526038892 1.1
2.6 1.27246576023734
2.67691656371397 1.4
2.84408480915337 1.7
2.9 1.80658966838433
3.01302991573085 2
3.17005102972374 2.3
3.2 2.35922960550778
3.33742094988032 2.6
3.48804415381498 2.9
3.5 2.92431387727759
3.65456217410415 3.2
3.8 3.49807721466367
3.80107625504408 3.5
3.96686152195469 3.8
4.1 4.07580500484418
4.11339742855596 4.1
4.2757819183725 4.4
4.4 4.65942604006138
4.42227503933906 4.7
4.58229072995892 5
4.4 5
4.16590976643694 5
4.1 4.88199455279574
4.01398782787212 4.7
3.85687684570484 4.4
3.8 4.2989566731482
3.70477082070808 4.1
3.54341533710813 3.8
3.5 3.72370324149068
3.3908260308337 3.5
3.22319028592046 3.2
3.2 3.15985811926406
3.06950908667521 2.9
2.9 2.61055324189177
2.89437913324224 2.6
2.73648239413026 2.3
2.6 2.07439497562884
2.55829350690867 2
2.38441571406276 1.7
2.3 1.56648273366174
2.19985561646031 1.4
2.00033519992665 1.1
2 1.09950066038192
1.80212534001477 0.8
1.7 0.658587516471111
1.58233625729877 0.5
1.4 0.269746217600833
1.34166915345233 0.2
1.1 -0.0747517802502148
1.07614328774938 -0.1
0.8 -0.380339825377062
0.777781413265321 -0.4
0.5 -0.642071576982605
0.393584384858448 -0.7
0.2 -0.810747570770368
-0.1 -0.769542261641756
-0.169783916468867 -0.7
-0.4 -0.480234832407009
-0.451323260408195 -0.4
-0.606296532242399 -0.1
-0.7 0.17432661999965
-0.70913635268031 0.2
-0.784291521533466 0.5
-0.827032284969609 0.8
-0.851121233366765 1.1
-0.864575752402227 1.4
-0.872039244368761 1.7
-0.8761611321905 2
-0.878431296480694 2.3
-0.879679464844899 2.6
-0.880365538623723 2.9
-0.88074208302343 3.2
-0.880948906625268 3.5
-0.881062404885734 3.8
-0.881124737447592 4.1
-0.881158727111001 4.4
-0.88117677955617 4.7
-0.881188043412037 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.552066060450769
-0.995587597917724 0.5
-0.955130211553321 0.2
-0.886115553004937 -0.1
-0.767727671836684 -0.4
-0.7 -0.525980913600416
-0.610937176149326 -0.7
-0.401391977962482 -1
-0.4 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
-0.1 -0.769542261641756
0.2 -0.810747570770368
0.393584384858448 -0.7
0.5 -0.642071576982605
0.777781413265321 -0.4
0.8 -0.380339825377062
1.07614328774938 -0.1
1.1 -0.0747517802502148
1.34166915345233 0.2
1.4 0.269746217600833
1.58233625729877 0.5
1.7 0.658587516471111
1.80212534001477 0.8
2 1.09950066038192
2.00033519992665 1.1
2.19985561646031 1.4
2.3 1.56648273366174
2.38441571406276 1.7
2.55829350690867 2
2.6 2.07439497562884
2.73648239413026 2.3
2.89437913324224 2.6
2.9 2.61055324189177
3.06950908667521 2.9
3.2 3.15985811926406
3.22319028592046 3.2
3.3908260308337 3.5
3.5 3.72370324149068
3.54341533710813 3.8
3.70477082070808 4.1
3.8 4.2989566731482
3.85687684570484 4.4
4.01398782787212 4.7
4.1 4.88199455279574
4.16590976643694 5
4.1 5
3.87725712646523 5
3.8 4.85585282699044
3.72016755023465 4.7
3.56756126903886 4.4
3.5 4.27593636254089
3.4087889700287 4.1
3.25178413214033 3.8
3.2 3.70691887470685
3.09051775041823 3.5
2.92654846854907 3.2
2.9 3.15361770518572
2.76153356766481 2.9
2.6 2.62099458759811
2.58784405563027 2.6
2.41556360834958 2.3
2.3 2.11122960683151
2.23153176774377 2
2.04184138527796 1.7
2 1.63622319845401
1.84217451350105 1.4
1.7 1.19821894319496
1.62754949487585 1.1
1.4 0.804122436768172
1.39663157317597 0.8
1.14866120551009 0.5
1.1 0.443461713253617
0.876878361918104 0.2
0.8 0.119372214554357
0.566291251180974 -0.1
0.5 -0.159887440865248
0.2 -0.349015336996383
-0.1 -0.351729421548556
-0.351476171162338 -0.1
-0.4 -0.0421644025442943
-0.506347502019382 0.2
-0.591465851143454 0.5
-0.64293531057503 0.8
-0.673005738779683 1.1
-0.690133715844078 1.4
-0.699734676830833 1.7
-0.7 1.71481559444235
-0.705604571331571 2
-0.70885099940781 2.3
-0.71063502178848 2.6
-0.711615716362173 2.9
-0.712153687938192 3.2
-0.712449256296104 3.5
-0.712611413047232 3.8
-0.712700515804931 4.1
-0.712748879222884 4.4
-0.712776201885908 4.7
-0.712790499051213 5
-0.881188043412037 5
-0.88117677955617 4.7
-0.881158727111001 4.4
-0.881124737447592 4.1
-0.881062404885734 3.8
-0.880948906625268 3.5
-0.880742083023431 3.2
-0.880365538623723 2.9
-0.879679464844899 2.6
-0.878431296480694 2.3
-0.8761611321905 2
-0.872039244368761 1.7
-0.864575752402227 1.4
-0.851121233366765 1.1
-0.827032284969609 0.8
-0.784291521533466 0.5
-0.70913635268031 0.2
-0.7 0.17432661999965
-0.606296532242399 -0.1
-0.451323260408195 -0.4
-0.4 -0.480234832407009
-0.169783916468867 -0.7
-0.1 -0.769542261641756
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
-0.1 -0.351729421548556
0.2 -0.349015336996383
0.5 -0.159887440865248
0.566291251180974 -0.1
0.8 0.119372214554357
0.876878361918104 0.2
1.1 0.443461713253617
1.14866120551009 0.5
1.39663157317597 0.8
1.4 0.804122436768172
1.62754949487585 1.1
1.7 1.19821894319496
1.84217451350105 1.4
2 1.63622319845401
2.04184138527796 1.7
2.23153176774377 2
2.3 2.11122960683151
2.41556360834958 2.3
2.58784405563027 2.6
2.6 2.62099458759811
2.76153356766481 2.9
2.9 3.15361770518572
2.92654846854907 3.2
3.09051775041823 3.5
3.2 3.70691887470685
3.25178413214033 3.8
3.4087889700287 4.1
3.5 4.27593636254089
3.56756126903886 4.4
3.72016755023465 4.7
3.8 4.85585282699044
3.87725712646523 5
3.8 5
3.60828859119554 5
3.5 4.78215793028003
3.45742970891797 4.7
3.3009437562903 4.4
3.2 4.20355777223773
3.14536127400571 4.1
2.98533422060631 3.8
2.9 3.64057374423691
2.82345128365175 3.5
2.65734389615335 3.2
2.6 3.09811674599215
2.48680515020251 2.9
2.31047855133863 2.6
2.3 2.58249484612146
2.12745642131764 2.3
2 2.09912815651356
1.93546182050215 2
1.73196243769277 1.7
1.7 1.65395755021367
1.51478587811397 1.4
1.4 1.24844831920064
1.27961973535779 1.1
1.1 0.883477429272549
1.02479559665569 0.8
0.8 0.55168187970103
0.747759238225471 0.5
0.5 0.257093634972729
0.420173601638067 0.2
0.2 0.0485780740891342
-0.1 0.0400745312193923
-0.236703703794805 0.2
-0.4 0.465936805176833
-0.41089878538715 0.5
-0.474406230760791 0.8
-0.511425829145336 1.1
-0.53250051970359 1.4
-0.544314321381836 1.7
-0.550869554539853 2
-0.55449653407888 2.3
-0.556496497720404 2.6
-0.557590774327048 2.9
-0.558197629239758 3.2
-0.558528834027955 3.5
-0.558709376198053 3.8
-0.558807728220768 4.1
-0.558860394342356 4.4
-0.558891405420354 4.7
-0.558909585979953 5
-0.7 5
-0.712790499051213 5
-0.712776201885908 4.7
-0.712748879222884 4.4
-0.712700515804931 4.1
-0.712611413047232 3.8
-0.712449256296104 3.5
-0.712153687938192 3.2
-0.711615716362173 2.9
-0.71063502178848 2.6
-0.70885099940781 2.3
-0.705604571331571 2
-0.7 1.71481559444235
-0.699734676830833 1.7
-0.690133715844078 1.4
-0.673005738779683 1.1
-0.64293531057503 0.8
-0.591465851143454 0.5
-0.506347502019382 0.2
-0.4 -0.0421644025442943
-0.351476171162338 -0.1
-0.1 -0.351729421548556
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
-0.1 0.0400745312193923
0.2 0.0485780740891342
0.420173601638067 0.2
0.5 0.257093634972729
0.747759238225471 0.5
0.8 0.55168187970103
1.02479559665569 0.8
1.1 0.883477429272549
1.27961973535779 1.1
1.4 1.24844831920064
1.51478587811397 1.4
1.7 1.65395755021367
1.73196243769277 1.7
1.93546182050215 2
2 2.09912815651356
2.12745642131764 2.3
2.3 2.58249484612146
2.31047855133863 2.6
2.48680515020251 2.9
2.6 3.09811674599215
2.65734389615335 3.2
2.82345128365175 3.5
2.9 3.64057374423691
2.98533422060631 3.8
3.14536127400571 4.1
3.2 4.20355777223773
3.3009437562903 4.4
3.45742970891797 4.7
3.5 4.78215793028003
3.60828859119554 5
3.5 5
3.3294354085471 5
3.2 4.74410734860012
3.1805876551398 4.7
3.03230658980621 4.4
2.9 4.14885135166634
2.87710110182875 4.1
2.72197194188663 3.8
2.6 3.57907071806333
2.55983833244518 3.5
2.39359532744002 3.2
2.3 3.03983455013933
2.22160473486647 2.9
2.03907147593327 2.6
2 2.53769169162984
1.85016629698948 2.3
1.7 2.07668239680687
1.64505904337514 2
1.42738508011584 1.7
1.4 1.66323622890431
1.18514203100803 1.4
1.1 1.29586753825358
0.917187988837428 1.1
0.8 0.969722030071103
0.621320258419941 0.8
0.5 0.680058089092687
0.246586549593501 0.5
0.2 0.467410463959087
-0.1 0.492721385561129
-0.104731192934055 0.5
-0.238368395721025 0.8
-0.315430364765524 1.1
-0.358245610190718 1.4
-0.381729894750654 1.7
-0.394558355976554 2
-0.4 2.23149131893679
-0.400980520915839 2.3
-0.403358701841026 2.6
-0.404654329478439 2.9
-0.405378382528222 3.2
-0.405771501080121 3.5
-0.405984722412913 3.8
-0.406100095503909 4.1
-0.406161232030761 4.4
-0.40619830241714 4.7
-0.406221902677733 5
-0.558909585979953 5
-0.558891405420354 4.7
-0.558860394342356 4.4
-0.558807728220768 4.1
-0.558709376198053 3.8
-0.558528834027955 3.5
-0.558197629239758 3.2
-0.557590774327048 2.9
-0.556496497720404 2.6
-0.55449653407888 2.3
-0.550869554539853 2
-0.544314321381836 1.7
-0.53250051970359 1.4
-0.511425829145336 1.1
-0.474406230760792 0.8
-0.41089878538715 0.5
-0.4 0.465936805176833
-0.236703703794805 0.2
-0.1 0.0400745312193923
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
-0.1 0.492721385561129
0.2 0.467410463959087
0.246586549593501 0.5
0.5 0.680058089092687
0.621320258419941 0.8
0.8 0.969722030071103
0.917187988837428 1.1
1.1 1.29586753825358
1.18514203100803 1.4
1.4 1.66323622890431
1.42738508011584 1.7
1.64505904337514 2
1.7 2.07668239680687
1.85016629698948 2.3
2 2.53769169162984
2.03907147593327 2.6
2.22160473486647 2.9
2.3 3.03983455013933
2.39359532744002 3.2
2.55983833244518 3.5
2.6 3.57907071806333
2.72197194188663 3.8
2.87710110182875 4.1
2.9 4.14885135166634
3.03230658980621 4.4
3.1805876551398 4.7
3.2 4.74410734860012
3.3294354085471 5
3.2 5
3.08297179121435 5
2.93145139588048 4.7
2.9 4.6407274452292
2.79169888769969 4.4
2.63550792202337 4.1
2.6 4.03552980892614
2.48372375629649 3.8
2.31750447321878 3.5
2.3 3.4697412777676
2.15149230294774 3.2
2 2.94673640932859
1.9696165880895 2.9
1.78170362505671 2.6
1.7 2.47510471078174
1.56890506177677 2.3
1.4 2.06379598031203
1.33943268707942 2
1.1 1.71270310366153
1.08430682632647 1.7
0.8 1.42456706926124
0.762599251853928 1.4
0.5 1.19509537463087
0.29473168071768 1.1
0.2 1.05283458362296
0.127759721469511 1.1
-0.0885978980913069 1.4
-0.1 1.4360050361426
-0.126053905034402 1.7
-0.142420621522615 2
-0.151452988140635 2.3
-0.156413700391069 2.6
-0.159118699611584 2.9
-0.160622559240481 3.2
-0.161381387827057 3.5
-0.161909544518214 3.8
-0.16210630212632 4.1
-0.162331852175974 4.4
-0.162393183082575 4.7
-0.162454329812011 5
-0.4 5
-0.406221902677733 5
-0.40619830241714 4.7
-0.406161232030761 4.4
-0.406100095503909 4.1
-0.405984722412913 3.8
-0.405771501080121 3.5
-0.405378382528222 3.2
-0.404654329478439 2.9
-0.403358701841026 2.6
-0.400980520915839 2.3
-0.4 2.23149131893679
-0.394558355976554 2
-0.381729894750654 1.7
-0.358245610190718 1.4
-0.315430364765524 1.1
-0.238368395721025 0.8
-0.104731192934055 0.5
-0.1 0.492721385561129
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
0.2 1.05283458362296
0.29473168071768 1.1
0.5 1.19509537463087
0.762599251853928 1.4
0.8 1.42456706926124
1.08430682632647 1.7
1.1 1.71270310366153
1.33943268707942 2
1.4 2.06379598031203
1.56890506177677 2.3
1.7 2.47510471078174
1.78170362505671 2.6
1.9696165880895 2.9
2 2.94673640932859
2.15149230294774 3.2
2.3 3.4697412777676
2.31750447321878 3.5
2.48372375629649 3.8
2.6 4.03552980892614
2.63550792202337 4.1
2.79169888769969 4.4
2.9 4.6407274452292
2.93145139588048 4.7
3.08297179121435 5
2.9 5
2.87306592394544 5
2.73395288609068 4.7
2.6 4.43479128106582
2.5809065652518 4.4
2.42839474956455 4.1
2.3 3.85758112230731
2.26444316536287 3.8
2.09523538163962 3.5
2 3.33288966331035
1.90573105969674 3.2
1.71895915899042 2.9
1.7 2.86995667365119
1.47683303724157 2.6
1.4 2.49287963727507
1.17604043058355 2.3
1.1 2.2182870478591
0.8 2.1075604988149
0.551647280493328 2.3
0.5 2.45154916179919
0.464133870082648 2.6
0.428967765157999 2.9
0.410745602185158 3.2
0.401494805508508 3.5
0.396381092330729 3.8
0.393481912323637 4.1
0.392158278603429 4.4
0.390776469588562 4.7
0.390793284464668 5
0.2 5
-0.1 5
-0.162454329812011 5
-0.162393183082575 4.7
-0.162331852175974 4.4
-0.16210630212632 4.1
-0.161909544518214 3.8
-0.161381387827057 3.5
-0.160622559240481 3.2
-0.159118699611584 2.9
-0.156413700391069 2.6
-0.151452988140635 2.3
-0.142420621522615 2
-0.126053905034402 1.7
-0.1 1.4360050361426
-0.0885978980913069 1.4
0.127759721469511 1.1
0.2 1.05283458362296
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
0.8 2.1075604988149
1.1 2.2182870478591
1.17604043058355 2.3
1.4 2.49287963727507
1.47683303724157 2.6
1.7 2.86995667365119
1.71895915899042 2.9
1.90573105969674 3.2
2 3.33288966331035
2.09523538163962 3.5
2.26444316536287 3.8
2.3 3.85758112230731
2.42839474956455 4.1
2.5809065652518 4.4
2.6 4.43479128106582
2.73395288609068 4.7
2.87306592394544 5
2.68509827573808 5
2.6 4.81838888709149
2.52894488617241 4.7
2.3744211399081 4.4
2.3 4.25028020834985
2.19681528343381 4.1
2.02989585675962 3.8
2 3.74505637701426
1.801420532074 3.5
1.7 3.33913802993372
1.51241212677174 3.2
1.4 3.08369877239733
1.16082177429872 3.2
1.1 3.31495612995831
1.06332131000288 3.5
1.03406382111051 3.8
1.01939504699369 4.1
1.01135597400831 4.4
1.00708136229247 4.7
1.0050612490916 5
0.8 5
0.5 5
0.390793284464668 5
0.390776469588562 4.7
0.392158278603428 4.4
0.393481912323637 4.1
0.396381092330729 3.8
0.401494805508508 3.5
0.410745602185158 3.2
0.428967765157999 2.9
0.464133870082648 2.6
0.5 2.45154916179919
0.551647280493328 2.3
0.8 2.1075604988149
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
1.4 3.08369877239733
1.51241212677174 3.2
1.7 3.33913802993372
1.801420532074 3.5
2 3.74505637701426
2.02989585675962 3.8
2.19681528343381 4.1
2.3 4.25028020834985
2.3744211399081 4.4
2.52894488617241 4.7
2.6 4.8183888870915
2.68509827573808 5
2.6 5
2.42565845179801 5
2.3 4.73320008045716
2.26692274324232 4.7
2.04313120797871 4.4
2 4.32280455063568
1.7 4.16592085406217
1.59778766115197 4.4
1.54558998471053 4.7
1.52269100815489 5
1.4 5
1.1 5
1.0050612490916 5
1.00708136229247 4.7
1.01135597400831 4.4
1.01939504699369 4.1
1.03406382111051 3.8
1.06332131000288 3.5
1.1 3.31495612995831
1.16082177429872 3.2
1.4 3.08369877239733
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
1.7 4.16592085406217
2 4.32280455063568
2.04313120797871 4.4
2.26692274324232 4.7
2.3 4.73320008045716
2.42565845179801 5
2.3 5
2 5
1.7 5
1.52269100815489 5
1.54558998471053 4.7
1.59778766115197 4.4
1.7 4.16592085406217
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
0.2 5
};
\coordinate (MCMC_mean_lml_t) at (axis cs:0.19999999999999996,2.3);
\end{axis}



==> fig/tikz/monks-2/LA_mean_lml.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=black]
table{%
x  y
-0.97546288542887 2
-0.7 2.24554600409092
-0.662931313180758 2.3
-0.474474985269566 2.6
-0.4 2.73273815830952
-0.323578106085472 2.9
-0.205711864122868 3.2
-0.107107039934028 3.5
-0.1 3.52446567598157
-0.00563293647796663 3.8
0.0837590097650391 4.1
0.162013727770183 4.4
0.2 4.5628070378083
0.252949625257827 4.7
0.359560569809569 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.97853357552316
-0.97546288542887 2
};
\addplot [draw=none, fill=midnightblue854116]
table{%
x  y
-0.788458527631973 2
-0.7 2.07885141388097
-0.549456636882046 2.3
-0.4 2.54407540986686
-0.37167012224738 2.6
-0.236716790066982 2.9
-0.124492609177707 3.2
-0.1 3.27485598644421
-0.0145991811392592 3.5
0.0844711853345052 3.8
0.170510481312675 4.1
0.2 4.21493883638251
0.277107926273043 4.4
0.391756353130871 4.7
0.496424374158348 5
0.359560569809569 5
0.252949625257827 4.7
0.2 4.5628070378083
0.162013727770183 4.4
0.0837590097650391 4.1
-0.00563293647796663 3.8
-0.1 3.52446567598157
-0.107107039934028 3.5
-0.205711864122868 3.2
-0.323578106085472 2.9
-0.4 2.73273815830952
-0.474474985269566 2.6
-0.662931313180758 2.3
-0.7 2.24554600409092
-0.97546288542887 2
-1 1.97853357552316
-1 1.81493182390517
-0.788458527631973 2
};
\addplot [draw=none, fill=midnightblue868137]
table{%
x  y
-0.94116410814297 1.7
-0.7 1.90947396566789
-0.635773450249176 2
-0.435981960583334 2.3
-0.4 2.35876160443863
-0.277795183849867 2.6
-0.149855474048493 2.9
-0.1 3.0353263645785
-0.0306853425174449 3.2
0.0795577115011112 3.5
0.174575307146977 3.8
0.2 3.88984029977563
0.294554380513879 4.1
0.417991285066011 4.4
0.5 4.6176663180643
0.534547831585783 4.7
0.651360439460759 5
0.5 5
0.496424374158348 5
0.391756353130871 4.7
0.277107926273043 4.4
0.2 4.21493883638251
0.170510481312675 4.1
0.0844711853345052 3.8
-0.0145991811392592 3.5
-0.1 3.27485598644421
-0.124492609177707 3.2
-0.236716790066982 2.9
-0.37167012224738 2.6
-0.4 2.54407540986686
-0.549456636882046 2.3
-0.7 2.07885141388097
-0.788458527631973 2
-1 1.81493182390517
-1 1.7
-1 1.64740587871035
-0.94116410814297 1.7
};
\addplot [draw=none, fill=teal882156]
table{%
x  y
-0.743389929750605 1.7
-0.7 1.7376882809175
-0.513894679026054 2
-0.4 2.1733322704383
-0.329797840686371 2.3
-0.183920245452354 2.6
-0.1 2.80317355542089
-0.0548774936432514 2.9
0.0685569934491584 3.2
0.173714604141481 3.5
0.2 3.58400213776503
0.304927565746442 3.8
0.437803627895722 4.1
0.5 4.25286707868987
0.566464740476894 4.4
0.691451890339456 4.7
0.8 4.98220179015663
0.807022278735933 5
0.8 5
0.651360439460759 5
0.534547831585783 4.7
0.5 4.6176663180643
0.417991285066011 4.4
0.294554380513879 4.1
0.2 3.88984029977563
0.174575307146977 3.8
0.0795577115011112 3.5
-0.0306853425174449 3.2
-0.1 3.0353263645785
-0.149855474048493 2.9
-0.277795183849867 2.6
-0.4 2.35876160443863
-0.435981960583334 2.3
-0.635773450249176 2
-0.7 1.90947396566789
-0.94116410814297 1.7
-1 1.64740587871035
-1 1.47061312860462
-0.743389929750605 1.7
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.873497730392246 1.4
-0.7 1.5540294986898
-0.596769671260843 1.7
-0.4 1.98734905408715
-0.392504038459938 2
-0.226998923006889 2.3
-0.1 2.57628495545454
-0.0878148740049705 2.6
0.0510355210471758 2.9
0.167799329415762 3.2
0.2 3.29312120785362
0.308231065060395 3.5
0.451100874905233 3.8
0.5 3.91146667717486
0.591786706267204 4.1
0.725510728120007 4.4
0.8 4.58093777943435
0.85013185425923 4.7
0.96796577026017 5
0.807022278735933 5
0.8 4.98220179015663
0.691451890339456 4.7
0.566464740476894 4.4
0.5 4.25286707868987
0.437803627895722 4.1
0.304927565746442 3.8
0.2 3.58400213776503
0.173714604141481 3.5
0.0685569934491584 3.2
-0.0548774936432514 2.9
-0.1 2.80317355542089
-0.183920245452354 2.6
-0.329797840686371 2.3
-0.4 2.1733322704383
-0.513894679026054 2
-0.7 1.7376882809175
-0.743389929750605 1.7
-1 1.47061312860462
-1 1.4
-1 1.27643014960617
-0.873497730392246 1.4
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.967725164136459 1.1
-0.7 1.3610631733784
-0.674439640088914 1.4
-0.464526300378266 1.7
-0.4 1.79422982342059
-0.278076679771111 2
-0.124200005327407 2.3
-0.1 2.35264688263159
0.0270935373795888 2.6
0.156948535737603 2.9
0.2 3.0127007521949
0.305264209887922 3.2
0.458378052476907 3.5
0.5 3.58821916072713
0.61108630472881 3.8
0.754006449211656 4.1
0.8 4.20434298628183
0.887973062875789 4.4
1.01279832143935 4.7
1.1 4.92470715934158
1.12962234704621 5
1.1 5
0.96796577026017 5
0.85013185425923 4.7
0.8 4.58093777943435
0.725510728120007 4.4
0.591786706267204 4.1
0.5 3.91146667717486
0.451100874905233 3.8
0.308231065060395 3.5
0.2 3.29312120785362
0.167799329415762 3.2
0.0510355210471758 2.9
-0.0878148740049705 2.6
-0.1 2.57628495545454
-0.226998923006889 2.3
-0.392504038459938 2
-0.4 1.98734905408715
-0.596769671260843 1.7
-0.7 1.5540294986898
-0.873497730392246 1.4
-1 1.27643014960617
-1 1.1
-1 1.0620781860859
-0.967725164136459 1.1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
-0.996232449964928 0.8
-0.741226067864428 1.1
-0.7 1.14020021105343
-0.529452559787839 1.4
-0.4 1.59065625075887
-0.333484653299482 1.7
-0.163649321082285 2
-0.1 2.12633912977418
-0.0024299444969553 2.3
0.142001948764148 2.6
0.2 2.73787333340811
0.297596738428466 2.9
0.461087697019017 3.2
0.5 3.27703358840727
0.626008131095895 3.5
0.778015001388394 3.8
0.8 3.84658331082777
0.921849617617276 4.1
1.05344498955594 4.4
1.1 4.51325295102967
1.17820980886408 4.7
1.29453572312319 5
1.12962234704621 5
1.1 4.92470715934158
1.01279832143935 4.7
0.887973062875789 4.4
0.8 4.20434298628182
0.754006449211656 4.1
0.61108630472881 3.8
0.5 3.58821916072713
0.458378052476907 3.5
0.305264209887922 3.2
0.2 3.0127007521949
0.156948535737603 2.9
0.0270935373795888 2.6
-0.1 2.35264688263159
-0.124200005327407 2.3
-0.278076679771111 2
-0.4 1.79422982342059
-0.464526300378266 1.7
-0.674439640088914 1.4
-0.7 1.3610631733784
-0.967725164136459 1.1
-1 1.0620781860859
-1 0.8
-1 0.793901337298764
-0.996232449964928 0.8
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
-0.925767848368051 0.5
-0.748688587401753 0.8
-0.7 0.858152769534889
-0.568778574241418 1.1
-0.4 1.37227230732534
-0.383873491970355 1.4
-0.203588105832329 1.7
-0.1 1.8927451063922
-0.0350853137445076 2
0.12518118654149 2.3
0.2 2.46262553859048
0.288192284113451 2.6
0.462033738797179 2.9
0.5 2.97059550738873
0.639736528124761 3.2
0.8 3.49931484794129
0.800376309098867 3.5
0.954492609995084 3.8
1.09191811320393 4.1
1.1 4.11860726162125
1.22575799401479 4.4
1.3467932441256 4.7
1.4 4.84004374438006
1.46614249109149 5
1.4 5
1.29453572312319 5
1.17820980886408 4.7
1.1 4.51325295102967
1.05344498955594 4.4
0.921849617617276 4.1
0.8 3.84658331082777
0.778015001388394 3.8
0.626008131095895 3.5
0.5 3.27703358840727
0.461087697019017 3.2
0.297596738428466 2.9
0.2 2.73787333340811
0.142001948764148 2.6
-0.0024299444969553 2.3
-0.1 2.12633912977418
-0.163649321082285 2
-0.333484653299482 1.7
-0.4 1.59065625075887
-0.529452559787839 1.4
-0.7 1.14020021105343
-0.741226067864428 1.1
-0.996232449964928 0.8
-1 0.793901337298764
-1 0.5
-1 0.297367768936973
-0.925767848368051 0.5
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
-0.7 -1
-0.4 -1
-0.297542915105962 -1
-0.4 -0.837530122459197
-0.485650790700146 -0.7
-0.622941587051075 -0.4
-0.695269334380669 -0.1
-0.7 -0.0101789557859276
-0.713321800011933 0.2
-0.7 0.252882364546936
-0.661933598365895 0.5
-0.556347803503527 0.8
-0.408358384636386 1.1
-0.4 1.11348368227833
-0.233361262598495 1.4
-0.1 1.64418419883121
-0.0646020552179901 1.7
0.111198718456314 2
0.2 2.17841313113389
0.282845786625283 2.3
0.466262414707811 2.6
0.5 2.65929493926795
0.658250996816068 2.9
0.8 3.14947981854741
0.829720837695138 3.2
0.991422452454639 3.5
1.1 3.72717079887062
1.13706782186659 3.8
1.27692399423108 4.1
1.4 4.3980739033938
1.40089568751031 4.4
1.53209447751875 4.7
1.64962351359299 5
1.46614249109149 5
1.4 4.84004374438006
1.3467932441256 4.7
1.22575799401479 4.4
1.1 4.11860726162125
1.09191811320393 4.1
0.954492609995084 3.8
0.800376309098867 3.5
0.8 3.49931484794129
0.639736528124761 3.2
0.5 2.97059550738873
0.462033738797179 2.9
0.288192284113451 2.6
0.2 2.46262553859048
0.12518118654149 2.3
-0.0350853137445076 2
-0.1 1.8927451063922
-0.203588105832329 1.7
-0.383873491970355 1.4
-0.4 1.37227230732534
-0.568778574241418 1.1
-0.7 0.858152769534889
-0.748688587401753 0.8
-0.925767848368051 0.5
-1 0.297367768936973
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
4.7 3.97171602757072
4.93153762957275 4.1
5 4.13215117759946
5 4.4
5 4.7
5 5
4.7 5
4.52783003537738 5
4.47144536491432 4.7
4.42130362876527 4.4
4.4392307678279 4.1
4.7 3.97171602757072
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
-0.4 -0.837530122459197
-0.297542915105962 -1
-0.1 -1
0.2 -1
0.231753593955092 -1
0.2 -0.984102868611781
-0.0800867443085926 -0.7
-0.1 -0.681921487252495
-0.282366150143603 -0.4
-0.4 -0.155806714532372
-0.422064887385549 -0.1
-0.47925893891135 0.2
-0.460883942750378 0.5
-0.4 0.712005542645901
-0.373655454915479 0.8
-0.231954374444271 1.1
-0.1 1.36016952030205
-0.0749805208344122 1.4
0.110173436179029 1.7
0.2 1.87001324183174
0.293454801958562 2
0.483103040287513 2.3
0.5 2.32828526843105
0.693245473793749 2.6
0.8 2.77701661861546
0.877990317839277 2.9
1.04276394786298 3.2
1.1 3.31508586109358
1.20046221490478 3.5
1.34051059799173 3.8
1.4 3.939282526073
1.47965974292919 4.1
1.61009512172716 4.4
1.7 4.63029738175933
1.73352592016301 4.7
1.86573032233717 5
1.7 5
1.64962351359299 5
1.53209447751875 4.7
1.40089568751031 4.4
1.4 4.3980739033938
1.27692399423108 4.1
1.13706782186659 3.8
1.1 3.72717079887062
0.991422452454639 3.5
0.829720837695138 3.2
0.8 3.14947981854741
0.658250996816068 2.9
0.5 2.65929493926795
0.466262414707811 2.6
0.282845786625283 2.3
0.2 2.17841313113389
0.111198718456314 2
-0.0646020552179901 1.7
-0.1 1.64418419883121
-0.233361262598495 1.4
-0.4 1.11348368227833
-0.408358384636386 1.1
-0.556347803503527 0.8
-0.661933598365895 0.5
-0.7 0.252882364546936
-0.713321800011933 0.2
-0.7 -0.0101789557859276
-0.695269334380669 -0.1
-0.622941587051075 -0.4
-0.485650790700146 -0.7
-0.4 -0.837530122459197
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
2.3 -1
2.6 -1
2.9 -1
3.2 -1
3.5 -1
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.5
5 0.8
5 1.1
5 1.4
5 1.7
5 2
5 2.3
5 2.6
5 2.9
5 3.2
5 3.5
5 3.8
5 4.1
5 4.13215117759946
4.93153762957275 4.1
4.7 3.97171602757072
4.4392307678279 4.1
4.42130362876527 4.4
4.47144536491432 4.7
4.52783003537738 5
4.4 5
4.1 5
3.8 5
3.73826225442764 5
3.65416682396262 4.7
3.56419225879855 4.4
3.5 4.19233544502192
3.47413774284548 4.1
3.38961381471096 3.8
3.29975682653205 3.5
3.20582314257899 3.2
3.2 3.18100145786671
3.12013866755114 2.9
3.0311315912687 2.6
2.93739035082428 2.3
2.9 2.18303948370563
2.84685001456056 2
2.76257851533066 1.7
2.67381844302562 1.4
2.6 1.17294539827733
2.5797798310533 1.1
2.51380967654968 0.8
2.45281133848482 0.5
2.39716296228311 0.2
2.35992288888664 -0.1
2.37293201305806 -0.4
2.39157469251876 -0.7
2.3 -0.763671041040373
2.085860987573 -1
2.3 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
0.2 -0.984102868611781
0.231753593955092 -1
0.5 -1
0.8 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.085860987573 -1
2.3 -0.763671041040373
2.39157469251876 -0.7
2.37293201305806 -0.4
2.35992288888664 -0.1
2.39716296228311 0.2
2.45281133848482 0.5
2.51380967654968 0.8
2.5797798310533 1.1
2.6 1.17294539827733
2.67381844302562 1.4
2.76257851533066 1.7
2.84685001456056 2
2.9 2.18303948370563
2.93739035082428 2.3
3.0311315912687 2.6
3.12013866755114 2.9
3.2 3.18100145786671
3.20582314257899 3.2
3.29975682653205 3.5
3.38961381471096 3.8
3.47413774284548 4.1
3.5 4.19233544502192
3.56419225879855 4.4
3.65416682396262 4.7
3.73826225442764 5
3.5 5
3.2 5
3.14584841766882 5
3.06262247806609 4.7
2.97520915684209 4.4
2.9 4.16387577676846
2.87896761380612 4.1
2.77928771759864 3.8
2.67734866468334 3.5
2.6 3.28822090591008
2.56745394529444 3.2
2.45874052335052 2.9
2.3443375299753 2.6
2.3 2.48820573694076
2.22616132094643 2.3
2.10690618913077 2
2 1.74904337554282
1.97896506858309 1.7
1.85102246771491 1.4
1.71096476446894 1.1
1.7 1.07731853203915
1.56608779369092 0.8
1.40117490053216 0.5
1.4 0.498002072625222
1.21885615735715 0.2
1.1 0.0369395337042822
0.986971447865012 -0.1
0.8 -0.281190682507417
0.588444489747861 -0.4
0.5 -0.438260117788626
0.2 -0.412022478919361
0.186612940802493 -0.4
-0.1 -0.142303025714794
-0.122413120355282 -0.1
-0.219784639071904 0.2
-0.229991743037001 0.5
-0.164059370049661 0.8
-0.1 0.963347847676843
-0.0256279964406165 1.1
0.144583637658594 1.4
0.2 1.502537671653
0.348447989135668 1.7
0.5 1.93714054154365
0.553190182193391 2
0.770552374276731 2.3
0.8 2.34586277637928
0.975922401150145 2.6
1.1 2.8318675135477
1.14318056715348 2.9
1.30710170994007 3.2
1.4 3.40909552531201
1.45218774899664 3.5
1.5993155893375 3.8
1.7 4.05281871216662
1.72654514765132 4.1
1.87494661564853 4.4
1.99127543913985 4.7
2 4.72276229333113
2.147194269243 5
2 5
1.86573032233717 5
1.73352592016301 4.7
1.7 4.63029738175933
1.61009512172716 4.4
1.47965974292919 4.1
1.4 3.939282526073
1.34051059799173 3.8
1.20046221490478 3.5
1.1 3.31508586109358
1.04276394786298 3.2
0.877990317839277 2.9
0.8 2.77701661861546
0.693245473793749 2.6
0.5 2.32828526843105
0.483103040287513 2.3
0.293454801958562 2
0.2 1.87001324183174
0.110173436179029 1.7
-0.0749805208344122 1.4
-0.1 1.36016952030205
-0.231954374444271 1.1
-0.373655454915479 0.8
-0.4 0.712005542645901
-0.460883942750378 0.5
-0.47925893891135 0.2
-0.422064887385549 -0.1
-0.4 -0.155806714532372
-0.282366150143603 -0.4
-0.1 -0.681921487252495
-0.0800867443085926 -0.7
0.2 -0.984102868611781
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
0.2 -0.412022478919362
0.5 -0.438260117788626
0.588444489747861 -0.4
0.8 -0.281190682507417
0.986971447865012 -0.1
1.1 0.0369395337042822
1.21885615735715 0.2
1.4 0.498002072625222
1.40117490053216 0.5
1.56608779369092 0.8
1.7 1.07731853203915
1.71096476446894 1.1
1.85102246771491 1.4
1.97896506858309 1.7
2 1.74904337554282
2.10690618913077 2
2.22616132094643 2.3
2.3 2.48820573694076
2.3443375299753 2.6
2.45874052335052 2.9
2.56745394529444 3.2
2.6 3.28822090591008
2.67734866468334 3.5
2.77928771759864 3.8
2.87896761380612 4.1
2.9 4.16387577676846
2.97520915684209 4.4
3.06262247806609 4.7
3.14584841766882 5
2.9 5
2.6 5
2.3 5
2.147194269243 5
2 4.72276229333113
1.99127543913985 4.7
1.87494661564853 4.4
1.72654514765132 4.1
1.7 4.05281871216662
1.5993155893375 3.8
1.45218774899664 3.5
1.4 3.40909552531201
1.30710170994007 3.2
1.14318056715348 2.9
1.1 2.8318675135477
0.975922401150145 2.6
0.8 2.34586277637928
0.770552374276731 2.3
0.553190182193391 2
0.5 1.93714054154365
0.348447989135668 1.7
0.2 1.502537671653
0.144583637658594 1.4
-0.0256279964406165 1.1
-0.1 0.963347847676843
-0.164059370049661 0.8
-0.229991743037001 0.5
-0.219784639071904 0.2
-0.122413120355282 -0.1
-0.1 -0.142303025714794
0.186612940802493 -0.4
0.2 -0.412022478919362

0.155087736713085 0.5
0.178320331666288 0.8
0.2 0.858283691967649
0.370701949062108 1.1
0.5 1.31621509630539
0.604329611631135 1.4
0.8 1.61909748791253
0.934530381406671 1.7
1.1 1.9252157925875
1.17907069014416 1.7
1.10114082730878 1.4
1.1 1.39740843037537
0.940365364540273 1.1
0.80613402558826 0.8
0.8 0.789765234989715
0.581455465354679 0.5
0.5 0.410358951286572
0.2 0.376473242015802
0.155087736713085 0.5
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
0.2 0.376473242015802
0.5 0.410358951286572
0.581455465354679 0.5
0.8 0.789765234989715
0.80613402558826 0.8
0.940365364540273 1.1
1.1 1.39740843037537
1.10114082730878 1.4
1.17907069014416 1.7
1.1 1.9252157925875
0.934530381406671 1.7
0.8 1.61909748791253
0.604329611631135 1.4
0.5 1.31621509630539
0.370701949062108 1.1
0.2 0.858283691967649
0.178320331666288 0.8
0.155087736713085 0.5
0.2 0.376473242015802
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
0.5 0.8
};
\coordinate (LA_mean_lml_t) at (axis cs:0.5,0.7999999999999998);
\end{axis}



==> fig/tikz/monks-2/LA_nlpd.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
3.5 -1
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.5
5 0.8
5 0.851599548156451
4.94889208139839 0.8
4.7 0.546249803525021
4.65455658561958 0.5
4.4 0.236228761321347
4.36492898321648 0.2
4.1 -0.0829669890696125
4.08396668407002 -0.1
3.82629971941419 -0.4
3.8 -0.437878268000465
3.61561105080754 -0.7
3.5 -0.956077750108102
3.47977994503357 -1
3.5 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
-0.7 -1
-0.4 -1
-0.392300916762359 -1
-0.4 -0.992008920731128
-0.599602995895498 -0.7
-0.7 -0.489885828157559
-0.746258552869895 -0.4
-0.859523381572987 -0.1
-0.920061576136476 0.2
-0.947389623896293 0.5
-0.951860208699694 0.8
-0.939044151676924 1.1
-0.911471505050337 1.4
-0.869389401561962 1.7
-0.811189321816397 2
-0.733601890370294 2.3
-0.7 2.41259169633374
-0.653962106454848 2.6
-0.566074577333592 2.9
-0.453273164243968 3.2
-0.4 3.32574240994128
-0.327683752807229 3.5
-0.183658461757355 3.8
-0.1 3.95379839250094
-0.0321191277336206 4.1
0.124107311519617 4.4
0.2 4.53183946698896
0.262178254680495 4.7
0.388282992144327 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
1.1 -1
1.4 -1
1.7 -1
2 -1
2.3 -1
2.6 -1
2.9 -1
3.2 -1
3.47977994503357 -1
3.5 -0.956077750108102
3.61561105080754 -0.7
3.8 -0.437878268000465
3.82629971941419 -0.4
4.08396668407002 -0.1
4.1 -0.0829669890696126
4.36492898321647 0.2
4.4 0.236228761321347
4.65455658561958 0.5
4.7 0.546249803525021
4.94889208139839 0.8
5 0.851599548156451
5 1.1
5 1.4
5 1.7
5 2
5 2.3
5 2.6
5 2.9
5 3.2
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.59273165486808 5
4.43394820792119 4.7
4.4 4.63823025660319
4.28600830246006 4.4
4.12518850433175 4.1
4.1 4.05456521089833
3.97722051481825 3.8
3.81304251488608 3.5
3.8 3.47672320484406
3.66506632664847 3.2
3.5 2.90596006920323
3.4970672222259 2.9
3.34814356312024 2.6
3.2 2.34080284238191
3.17935090611741 2.3
3.02410787195001 2
2.9 1.78797549842946
2.85379567503124 1.7
2.68860119624816 1.4
2.6 1.2533898027229
2.51540763668018 1.1
2.33245908778745 0.8
2.3 0.748636471305286
2.15336435287045 0.5
2 0.272520526954174
1.95211445477997 0.2
1.7417981975918 -0.1
1.7 -0.156659367325554
1.51581839218659 -0.4
1.4 -0.542019311226122
1.26046788471262 -0.7
1.1 -0.880337994437494
0.980162690971935 -1
1.1 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
-0.4 -0.992008920731128
-0.392300916762359 -1
-0.1 -1
0.2 -1
0.5 -1
0.8 -1
0.980162690971935 -1
1.1 -0.880337994437494
1.26046788471262 -0.7
1.4 -0.542019311226122
1.51581839218659 -0.4
1.7 -0.156659367325554
1.7417981975918 -0.1
1.95211445477997 0.2
2 0.272520526954174
2.15336435287045 0.5
2.3 0.748636471305286
2.33245908778745 0.8
2.51540763668018 1.1
2.6 1.2533898027229
2.68860119624816 1.4
2.85379567503124 1.7
2.9 1.78797549842946
3.02410787195001 2
3.17935090611741 2.3
3.2 2.34080284238191
3.34814356312024 2.6
3.4970672222259 2.9
3.5 2.90596006920323
3.66506632664847 3.2
3.8 3.47672320484406
3.81304251488608 3.5
3.97722051481825 3.8
4.1 4.05456521089833
4.12518850433175 4.1
4.28600830246006 4.4
4.4 4.63823025660319
4.43394820792119 4.7
4.59273165486808 5
4.4 5
4.17532319143744 5
4.1 4.86477724834338
4.02185203357677 4.7
3.86641333798051 4.4
3.8 4.28177262399305
3.71259717990505 4.1
3.55298318079481 3.8
3.5 3.70671591078442
3.39866306768015 3.5
3.2329062276144 3.2
3.2 3.14295301800381
3.07744169771574 2.9
2.90256729067051 2.6
2.9 2.59564469254449
2.74467940797936 2.3
2.6 2.06040384916855
2.56599605943689 2
2.3931777009861 1.7
2.3 1.55244613220779
2.20791894298433 1.4
2.01017652017667 1.1
2 1.08483599929242
1.81106840519189 0.8
1.7 0.646207447475757
1.59107217776995 0.5
1.4 0.258978770075939
1.35038203871 0.2
1.1 -0.0837680141579553
1.08449358501722 -0.1
0.8 -0.386482147701161
0.784365714278067 -0.4
0.5 -0.642655485911381
0.388267868097576 -0.7
0.2 -0.802040082952758
-0.1 -0.75120915639601
-0.149638401458545 -0.7
-0.4 -0.440647447729874
-0.424784716843762 -0.4
-0.569973513025463 -0.1
-0.654865049096544 0.2
-0.695114996361553 0.5
-0.7 0.725072847937589
-0.702030448889506 0.8
-0.7 0.825665382172634
-0.682688938547355 1.1
-0.643572415905429 1.4
-0.585795003208615 1.7
-0.507834514617485 2
-0.405635229956212 2.3
-0.4 2.315152617303
-0.291767206983258 2.6
-0.153723001755547 2.9
-0.1 3.00587805254748
-0.0116451975853078 3.2
0.142097544209446 3.5
0.2 3.60449189113191
0.272719282645466 3.8
0.397378896371436 4.1
0.5 4.31420009999352
0.530839781421605 4.4
0.64465866992768 4.7
0.783569886304317 5
0.5 5
0.388282992144327 5
0.262178254680495 4.7
0.2 4.53183946698896
0.124107311519617 4.4
-0.0321191277336206 4.1
-0.1 3.95379839250094
-0.183658461757355 3.8
-0.327683752807229 3.5
-0.4 3.32574240994128
-0.453273164243968 3.2
-0.566074577333592 2.9
-0.653962106454848 2.6
-0.7 2.41259169633374
-0.733601890370294 2.3
-0.811189321816397 2
-0.869389401561962 1.7
-0.911471505050337 1.4
-0.939044151676924 1.1
-0.951860208699694 0.8
-0.947389623896293 0.5
-0.920061576136476 0.2
-0.859523381572987 -0.1
-0.746258552869895 -0.4
-0.7 -0.489885828157559
-0.599602995895498 -0.7
-0.4 -0.992008920731128
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
-0.1 -0.75120915639601
0.2 -0.802040082952758
0.388267868097576 -0.7
0.5 -0.642655485911381
0.784365714278067 -0.4
0.8 -0.386482147701161
1.08449358501722 -0.1
1.1 -0.0837680141579553
1.35038203871 0.2
1.4 0.258978770075939
1.59107217776995 0.5
1.7 0.646207447475757
1.81106840519189 0.8
2 1.08483599929242
2.01017652017667 1.1
2.20791894298433 1.4
2.3 1.55244613220779
2.3931777009861 1.7
2.56599605943689 2
2.6 2.06040384916855
2.74467940797936 2.3
2.9 2.59564469254449
2.90256729067051 2.6
3.07744169771574 2.9
3.2 3.14295301800381
3.2329062276144 3.2
3.39866306768015 3.5
3.5 3.70671591078442
3.55298318079481 3.8
3.71259717990505 4.1
3.8 4.28177262399305
3.86641333798051 4.4
4.02185203357677 4.7
4.1 4.86477724834338
4.17532319143744 5
4.1 5
3.88320376032751 5
3.8 4.84461143466823
3.72583357525156 4.7
3.57329722691769 4.4
3.5 4.26526722424986
3.41418054273795 4.1
3.25725554774353 3.8
3.2 3.69695361869449
3.09558701974822 3.5
2.9318245510843 3.2
2.9 3.14432579787137
2.76631019274071 2.9
2.6 2.61292150893463
2.59251843696442 2.6
2.42012963486239 2.3
2.3 2.10384977939211
2.2360703994504 2
2.04636345845787 1.7
2 1.62934419606862
1.84662829527674 1.4
1.7 1.19225742830565
1.63185937088865 1.1
1.40047454540576 0.8
1.4 0.799393068050833
1.15115140002336 0.5
1.1 0.440796235513629
0.875655564593796 0.2
0.8 0.121343500178599
0.557280852993159 -0.1
0.5 -0.150654637914632
0.2 -0.328264918732764
-0.1 -0.30909347539858
-0.281750123436077 -0.1
-0.4 0.0925070850115513
-0.438344768894358 0.2
-0.495021432536706 0.5
-0.50663171819104 0.8
-0.483418476312649 1.1
-0.430864156146349 1.4
-0.4 1.52183377011922
-0.349844860105122 1.7
-0.247911845073008 2
-0.123009067334112 2.3
-0.1 2.34993121135606
0.00991381546205082 2.6
0.156797314737205 2.9
0.2 2.98214602118029
0.281245713137404 3.2
0.402337311536032 3.5
0.5 3.71460106620656
0.530457715688714 3.8
0.641819604152673 4.1
0.772474289202791 4.4
0.8 4.4595706070956
0.886770051197415 4.7
1.00788890243188 5
0.8 5
0.783569886304317 5
0.64465866992768 4.7
0.530839781421605 4.4
0.5 4.31420009999352
0.397378896371436 4.1
0.272719282645466 3.8
0.2 3.60449189113191
0.142097544209446 3.5
-0.0116451975853078 3.2
-0.1 3.00587805254748
-0.153723001755547 2.9
-0.291767206983258 2.6
-0.4 2.315152617303
-0.405635229956212 2.3
-0.507834514617485 2
-0.585795003208615 1.7
-0.643572415905429 1.4
-0.682688938547355 1.1
-0.7 0.825665382172634
-0.702030448889506 0.8
-0.7 0.725072847937589
-0.695114996361553 0.5
-0.654865049096544 0.2
-0.569973513025463 -0.1
-0.424784716843762 -0.4
-0.4 -0.440647447729874
-0.149638401458545 -0.7
-0.1 -0.75120915639601
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
-0.1 -0.30909347539858
0.2 -0.328264918732764
0.5 -0.150654637914632
0.557280852993159 -0.1
0.8 0.121343500178599
0.875655564593796 0.2
1.1 0.440796235513629
1.15115140002336 0.5
1.4 0.799393068050833
1.40047454540576 0.8
1.63185937088865 1.1
1.7 1.19225742830565
1.84662829527674 1.4
2 1.62934419606862
2.04636345845787 1.7
2.2360703994504 2
2.3 2.10384977939211
2.42012963486239 2.3
2.59251843696442 2.6
2.6 2.61292150893463
2.76631019274071 2.9
2.9 3.14432579787137
2.9318245510843 3.2
3.09558701974822 3.5
3.2 3.69695361869449
3.25725554774353 3.8
3.41418054273795 4.1
3.5 4.26526722424986
3.57329722691769 4.4
3.72583357525156 4.7
3.8 4.84461143466823
3.88320376032751 5
3.8 5
3.61276727939495 5
3.5 4.77424052734533
3.46173605102294 4.7
3.30458439293028 4.4
3.2 4.19731184317899
3.14895276829245 4.1
2.98820566870463 3.8
2.9 3.63579726926024
2.82648102296949 3.5
2.6595610957931 3.2
2.6 3.09450681587098
2.48947357376647 2.9
2.31215151875957 2.6
2.3 2.57975352189497
2.12989989932332 2.3
2 2.09616669979895
1.93796092134965 2
1.7340923592628 1.7
1.7 1.65104266622325
1.51727250823475 1.4
1.4 1.24582958778893
1.28036987214186 1.1
1.1 0.884789102006002
1.01966590760179 0.8
0.8 0.563956153845935
0.728542876077477 0.5
0.5 0.287088182862544
0.358739773378366 0.2
0.2 0.102614815430907
-0.1 0.152264931109265
-0.131629008717313 0.2
-0.250050767624797 0.5
-0.284424598421292 0.8
-0.262285364343356 1.1
-0.202653796447228 1.4
-0.113477401050257 1.7
-0.1 1.7361727486913
0.00469628275829408 2
0.132398662784728 2.3
0.2 2.44300310549095
0.257637843300451 2.6
0.369764840804929 2.9
0.493075329202903 3.2
0.5 3.21584405477143
0.60027825720613 3.5
0.715455744406846 3.8
0.8 3.99669359157893
0.837619779932917 4.1
0.949369771217062 4.4
1.07549735402795 4.7
1.1 4.7550431446898
1.1903913686334 5
1.1 5
1.00788890243188 5
0.886770051197415 4.7
0.8 4.4595706070956
0.772474289202791 4.4
0.641819604152673 4.1
0.530457715688714 3.8
0.5 3.71460106620656
0.402337311536032 3.5
0.281245713137404 3.2
0.2 2.98214602118029
0.156797314737205 2.9
0.00991381546205082 2.6
-0.1 2.34993121135606
-0.123009067334112 2.3
-0.247911845073008 2
-0.349844860105122 1.7
-0.4 1.52183377011922
-0.430864156146349 1.4
-0.483418476312649 1.1
-0.50663171819104 0.8
-0.495021432536706 0.5
-0.438344768894358 0.2
-0.4 0.0925070850115513
-0.281750123436077 -0.1
-0.1 -0.30909347539858
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
-0.1 0.152264931109265
0.2 0.102614815430907
0.358739773378366 0.2
0.5 0.287088182862544
0.728542876077477 0.5
0.8 0.563956153845935
1.01966590760179 0.8
1.1 0.884789102006002
1.28036987214186 1.1
1.4 1.24582958778893
1.51727250823475 1.4
1.7 1.65104266622325
1.7340923592628 1.7
1.93796092134964 2
2 2.09616669979895
2.12989989932332 2.3
2.3 2.57975352189497
2.31215151875957 2.6
2.48947357376647 2.9
2.6 3.09450681587098
2.6595610957931 3.2
2.82648102296949 3.5
2.9 3.63579726926024
2.98820566870463 3.8
3.14895276829245 4.1
3.2 4.19731184317899
3.30458439293028 4.4
3.46173605102294 4.7
3.5 4.77424052734533
3.61276727939495 5
3.5 5
3.33972423382106 5
3.2 4.73054921768055
3.18676884251458 4.7
3.0408472031665 4.4
2.9 4.13844826117538
2.88229464918475 4.1
2.72937752663343 3.8
2.6 3.56993010107869
2.56515934332191 3.5
2.40036462937574 3.2
2.3 3.03061096329715
2.22817509256247 2.9
2.04535259630352 2.6
2 2.52831576497078
1.85836763275126 2.3
1.7 2.06637490461355
1.65282724835792 2
1.43488794552028 1.7
1.4 1.65342858631757
1.18976921965976 1.4
1.1 1.29183587097795
0.905629655303309 1.1
0.8 0.988374715464995
0.557366511413082 0.8
0.5 0.749498128755901
0.2 0.643190060977751
0.0685598235913436 0.8
0.0284154986464954 1.1
0.0740707806100883 1.4
0.153475192271546 1.7
0.2 1.83069146257214
0.254656717335563 2
0.353081995989714 2.3
0.454157198376137 2.6
0.5 2.72127139022933
0.559144985953358 2.9
0.660761087045669 3.2
0.771320708909909 3.5
0.8 3.57078090850776
0.883179018593206 3.8
0.994353410752075 4.1
1.1 4.35908819327187
1.11536096631171 4.4
1.22749354548932 4.7
1.34683660727176 5
1.1903913686334 5
1.1 4.7550431446898
1.07549735402795 4.7
0.949369771217062 4.4
0.837619779932917 4.1
0.8 3.99669359157893
0.715455744406846 3.8
0.60027825720613 3.5
0.5 3.21584405477143
0.493075329202903 3.2
0.369764840804929 2.9
0.257637843300451 2.6
0.2 2.44300310549095
0.132398662784728 2.3
0.0046962827582941 2
-0.1 1.7361727486913
-0.113477401050257 1.7
-0.202653796447228 1.4
-0.262285364343356 1.1
-0.284424598421292 0.8
-0.250050767624797 0.5
-0.131629008717313 0.2
-0.1 0.152264931109265
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
0.2 0.643190060977751
0.5 0.749498128755901
0.557366511413082 0.8
0.8 0.988374715464995
0.905629655303309 1.1
1.1 1.29183587097795
1.18976921965976 1.4
1.4 1.65342858631757
1.43488794552028 1.7
1.65282724835792 2
1.7 2.06637490461355
1.85836763275126 2.3
2 2.52831576497078
2.04535259630352 2.6
2.22817509256247 2.9
2.3 3.03061096329715
2.40036462937574 3.2
2.56515934332191 3.5
2.6 3.56993010107869
2.72937752663343 3.8
2.88229464918475 4.1
2.9 4.13844826117537
3.0408472031665 4.4
3.18676884251458 4.7
3.2 4.73054921768055
3.33972423382106 5
3.2 5
3.10571643431048 5
2.95634779295494 4.7
2.9 4.59633617693938
2.81229471768142 4.4
2.65793857300684 4.1
2.6 3.99694861466205
2.50392531224484 3.8
2.33882870196757 3.5
2.3 3.4340020828755
2.17321481793325 3.2
2 2.91392269545753
1.9910789140015 2.9
1.80632557484129 2.6
1.7 2.43899912981276
1.5966604008077 2.3
1.4 2.0276729519917
1.37244851134632 2
1.11216079816873 1.7
1.1 1.68537629533856
0.8 1.4453981807389
0.5 1.48502186400191
0.46832134669212 1.7
0.498415217007412 2
0.5 2.00643365132782
0.572561429604415 2.3
0.64839912649847 2.6
0.731179819307895 2.9
0.8 3.11345649363724
0.829141716985742 3.2
0.932652710463017 3.5
1.03636345350047 3.8
1.1 3.96810348643718
1.14934528029991 4.1
1.25968019992136 4.4
1.3740093819586 4.7
1.4 4.76353779416604
1.49119533750626 5
1.4 5
1.34683660727176 5
1.22749354548932 4.7
1.11536096631171 4.4
1.1 4.35908819327187
0.994353410752075 4.1
0.883179018593206 3.8
0.8 3.57078090850776
0.771320708909909 3.5
0.660761087045669 3.2
0.559144985953358 2.9
0.5 2.72127139022933
0.454157198376137 2.6
0.353081995989714 2.3
0.254656717335563 2
0.2 1.83069146257214
0.153475192271546 1.7
0.0740707806100883 1.4
0.0284154986464954 1.1
0.0685598235913436 0.8
0.2 0.643190060977751
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
0.5 1.48502186400191
0.8 1.4453981807389
1.1 1.68537629533856
1.11216079816873 1.7
1.37244851134632 2
1.4 2.0276729519917
1.5966604008077 2.3
1.7 2.43899912981276
1.80632557484129 2.6
1.9910789140015 2.9
2 2.91392269545753
2.17321481793325 3.2
2.3 3.4340020828755
2.33882870196757 3.5
2.50392531224484 3.8
2.6 3.99694861466205
2.65793857300684 4.1
2.81229471768142 4.4
2.9 4.59633617693938
2.95634779295494 4.7
3.10571643431048 5
2.91467666084913 5
2.9 4.97230802096003
2.77386540037251 4.7
2.62293051553859 4.4
2.6 4.35789799850593
2.46908723291904 4.1
2.30926387430429 3.8
2.3 3.78370276652119
2.13975654974071 3.5
2 3.25686111514972
1.95987749231486 3.2
1.77050088456927 2.9
1.7 2.78904242755579
1.54356439326928 2.6
1.4 2.40048557984288
1.26856313910604 2.3
1.1 2.1303637405558
0.853552128262069 2.3
0.873767243174348 2.6
0.935743534965914 2.9
1.00881793721762 3.2
1.09202852598256 3.5
1.1 3.52364517616169
1.20070624264214 3.8
1.30073523570395 4.1
1.4 4.38783479296733
1.40470219525236 4.4
1.5207764013548 4.7
1.62933264724498 5
1.49119533750626 5
1.4 4.76353779416604
1.3740093819586 4.7
1.25968019992136 4.4
1.14934528029991 4.1
1.1 3.96810348643718
1.03636345350047 3.8
0.932652710463017 3.5
0.829141716985742 3.2
0.8 3.11345649363724
0.731179819307895 2.9
0.64839912649847 2.6
0.572561429604415 2.3
0.5 2.00643365132782
0.498415217007412 2
0.46832134669212 1.7
0.5 1.48502186400191
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
1.1 2.1303637405558
1.26856313910604 2.3
1.4 2.40048557984288
1.54356439326928 2.6
1.7 2.78904242755579
1.77050088456927 2.9
1.95987749231486 3.2
2 3.25686111514972
2.13975654974071 3.5
2.3 3.78370276652119
2.30926387430429 3.8
2.46908723291904 4.1
2.6 4.35789799850593
2.62293051553859 4.4
2.77386540037251 4.7
2.9 4.97230802096003
2.91467666084913 5
2.9 5
2.74874357329156 5
2.60690082810652 4.7
2.6 4.6865259696707
2.44199520193185 4.4
2.3 4.11512840487134
2.28923255853127 4.1
2.10630246637553 3.8
2 3.60403122448762
1.91257821226659 3.5
1.72242713712496 3.2
1.7 3.16343081481381
1.42941116732429 2.9
1.4 2.86136289953468
1.33624148355171 2.9
1.26738333377515 3.2
1.30881951369675 3.5
1.37297863392991 3.8
1.4 3.89389308112034
1.47631843586745 4.1
1.57438052840647 4.4
1.66759758700431 4.7
1.7 4.7933663282071
1.78369538907714 5
1.7 5
1.62933264724498 5
1.5207764013548 4.7
1.40470219525236 4.4
1.4 4.38783479296733
1.30073523570395 4.1
1.20070624264214 3.8
1.1 3.52364517616169
1.09202852598256 3.5
1.00881793721762 3.2
0.935743534965914 2.9
0.873767243174348 2.6
0.853552128262069 2.3
1.1 2.1303637405558
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
1.4 2.86136289953468
1.42941116732429 2.9
1.7 3.16343081481381
1.72242713712496 3.2
1.91257821226659 3.5
2 3.60403122448762
2.10630246637553 3.8
2.28923255853127 4.1
2.3 4.11512840487134
2.44199520193185 4.4
2.6 4.6865259696707
2.60690082810652 4.7
2.74874357329156 5
2.6 5
2.5698816735322 5
2.39375460078861 4.7
2.3 4.4976007799915
2.206874203423 4.4
2.03253497342231 4.1
2 4.03705327110283
1.7 3.96280337128787
1.69797411437697 4.1
1.7 4.11020062139277
1.80722560047393 4.4
1.88104744711372 4.7
1.95505248490938 5
1.78369538907714 5
1.7 4.7933663282071
1.66759758700431 4.7
1.57438052840647 4.4
1.47631843586745 4.1
1.4 3.89389308112034
1.37297863392991 3.8
1.30881951369675 3.5
1.26738333377515 3.2
1.33624148355171 2.9
1.4 2.86136289953468
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
1.7 3.96280337128787
2 4.03705327110283
2.03253497342231 4.1
2.206874203423 4.4
2.3 4.4976007799915
2.39375460078861 4.7
2.5698816735322 5
2.3 5
2 5
1.95505248490938 5
1.88104744711372 4.7
1.80722560047393 4.4
1.7 4.11020062139277
1.69797411437697 4.1
1.7 3.96280337128787
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
0.5 0.8
};
\coordinate (MCMC_mean_lml_t) at (axis cs:0.19999999999999996,2.3);
\end{axis}



==> fig/tikz/monks-2/MCMC_mean_lml.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=black]
table{%
x  y
2 4.45821435832248
2.3 4.41455508649962
2.6 4.43129501458274
2.9 4.48730883639203
3.2 4.5850742248947
3.42878198906596 4.7
3.5 4.72564570658419
3.8 4.85499741581759
4.09224084498225 5
3.8 5
3.5 5
3.2 5
2.9 5
2.6 5
2.3 5
2 5
1.7 5
1.49029348725925 5
1.7 4.72583468075358
1.72954072193245 4.7
2 4.45821435832248
};
\addplot [draw=none, fill=midnightblue854116]
table{%
x  y
2.3 4.36446648737086
2.6 4.38059359031325
2.6588775597003 4.4
2.9 4.44384945034461
3.2 4.52759751907682
3.5 4.66731164753469
3.56248667474086 4.7
3.8 4.79134699576773
4.1 4.92237498526361
4.27709243715944 5
4.1 5
4.09224084498225 5
3.8 4.85499741581759
3.5 4.72564570658419
3.42878198906596 4.7
3.2 4.5850742248947
2.9 4.48730883639203
2.6 4.43129501458274
2.3 4.41455508649962
2 4.45821435832248
1.72954072193245 4.7
1.7 4.72583468075358
1.49029348725925 5
1.46031489036019 5
1.68051434174964 4.7
1.7 4.67221822944061
2 4.4181499687997
2.139345123598 4.4
2.3 4.36446648737086
};
\addplot [draw=none, fill=midnightblue868137]
table{%
x  y
2 4.3614414902253
2.3 4.29643363951405
2.6 4.30182511171636
2.89785508701995 4.4
2.9 4.40039006429719
3.2 4.47012081325894
3.5 4.58073503220741
3.7279855265983 4.7
3.8 4.72769657571786
4.1 4.83975254905836
4.4 4.96183228200547
4.48725214278479 5
4.4 5
4.27709243715944 5
4.1 4.92237498526361
3.8 4.79134699576773
3.56248667474086 4.7
3.5 4.66731164753469
3.2 4.52759751907682
2.9 4.44384945034461
2.6588775597003 4.4
2.6 4.38059359031325
2.3 4.36446648737086
2.139345123598 4.4
2 4.4181499687997
1.7 4.67221822944061
1.68051434174964 4.7
1.46031489036019 5
1.43033629346113 5
1.62334473480377 4.7
1.7 4.59070838857539
1.94315471908862 4.4
2 4.3614414902253
};
\addplot [draw=none, fill=teal882156]
table{%
x  y
2 4.29094803869615
2.3 4.22840079165724
2.6 4.22305663311947
2.9 4.31223553899208
3.1455034035328 4.4
3.2 4.41264410744106
3.5 4.49415841688013
3.8 4.63704386350437
3.93488497380785 4.7
4.1 4.75713011285312
4.4 4.85213851196691
4.7 4.97477773914347
5 4.98710187914525
5 5
4.7 5
4.48725214278479 5
4.4 4.96183228200547
4.1 4.83975254905836
3.8 4.72769657571786
3.7279855265983 4.7
3.5 4.58073503220741
3.2 4.47012081325894
2.9 4.40039006429719
2.89785508701995 4.4
2.6 4.30182511171636
2.3 4.29643363951405
2 4.3614414902253
1.94315471908862 4.4
1.7 4.59070838857539
1.62334473480377 4.7
1.43033629346113 5
1.40035769656207 5
1.5661751278579 4.7
1.7 4.50919854771018
1.83922902076674 4.4
2 4.29094803869615
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
2 4.220454587167
2.3 4.16036794380042
2.6 4.14428815452258
2.9 4.22367622490986
3.2 4.31327661422003
3.46971830438975 4.4
3.5 4.40758180155286
3.8 4.52559028720082
4.1 4.6492478512214
4.23309109456548 4.7
4.4 4.74244474192835
4.7 4.80839827272133
5 4.86375758185438
5 4.98710187914525
4.7 4.97477773914347
4.4 4.85213851196691
4.1 4.75713011285312
3.93488497380785 4.7
3.8 4.63704386350437
3.5 4.49415841688013
3.2 4.41264410744106
3.1455034035328 4.4
2.9 4.31223553899208
2.6 4.22305663311947
2.3 4.22840079165724
2 4.29094803869615
1.83922902076674 4.4
1.7 4.50919854771018
1.5661751278579 4.7
1.40035769656207 5
1.4 5
1.34118267384842 5
1.4 4.8976014524394
1.50900552091204 4.7
1.7 4.42768870684497
1.73530332244485 4.4
2 4.220454587167
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
2.3 4.08737205089824
2.6 4.05445894475889
2.75740889250523 4.1
2.9 4.13511691082764
3.2 4.20209469051999
3.5 4.27441808984739
3.76338585927878 4.4
3.8 4.41413671089727
4.1 4.48475652115247
4.4 4.58600692471206
4.7 4.63926061033112
4.85462368297155 4.7
5 4.74041328456351
5 4.86375758185438
4.7 4.80839827272133
4.4 4.74244474192835
4.23309109456548 4.7
4.1 4.6492478512214
3.8 4.52559028720082
3.5 4.40758180155286
3.46971830438975 4.4
3.2 4.31327661422003
2.9 4.22367622490986
2.6 4.14428815452258
2.3 4.16036794380042
2 4.220454587167
1.73530332244485 4.4
1.7 4.42768870684497
1.50900552091204 4.7
1.4 4.8976014524394
1.34118267384842 5
1.28165508044921 5
1.4 4.79396635879117
1.45183591396617 4.7
1.65029887643394 4.4
1.7 4.32792880144599
2 4.14996113563785
2.25885139998116 4.1
2.3 4.08737205089824
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
2 4.0599807815703
2.3 3.97528775947553
2.6 3.95042281019971
2.9 4.01760860850423
3.2 4.08437940657086
3.27026095233096 4.1
3.5 4.13678301979842
3.8 4.22076310133234
4.1 4.28151935922751
4.39977967822564 4.4
4.4 4.40006624217714
4.7 4.46496638492998
5 4.53019182150138
5 4.7
5 4.74041328456351
4.85462368297155 4.7
4.7 4.63926061033112
4.4 4.58600692471206
4.1 4.48475652115247
3.8 4.41413671089727
3.76338585927878 4.4
3.5 4.27441808984739
3.2 4.20209469051999
2.9 4.13511691082764
2.75740889250523 4.1
2.6 4.05445894475889
2.3 4.08737205089824
2.25885139998116 4.1
2 4.14996113563785
1.7 4.32792880144599
1.65029887643394 4.4
1.45183591396617 4.7
1.4 4.79396635879117
1.28165508044921 5
1.22212748704999 5
1.39083893448867 4.7
1.4 4.68842784258903
1.5750286178926 4.4
1.7 4.21878000642261
1.93665866947417 4.1
2 4.0599807815703
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
2 3.92258308860939
2.3 3.86320346805281
2.6 3.84638667564053
2.9 3.88107797603272
3.2 3.8932620892998
3.5 3.92997349507122
3.8 3.95043736640723
4.1 3.9903552025673
4.4 4.07582378041666
4.47279839868686 4.1
4.7 4.15306645343656
5 4.21937848861097
5 4.4
5 4.53019182150138
4.7 4.46496638492998
4.4 4.40006624217714
4.39977967822564 4.4
4.1 4.28151935922751
3.8 4.22076310133234
3.5 4.13678301979842
3.27026095233096 4.1
3.2 4.08437940657086
2.9 4.01760860850423
2.6 3.95042281019971
2.3 3.97528775947553
2 4.0599807815703
1.93665866947417 4.1
1.7 4.21878000642261
1.5750286178926 4.4
1.4 4.68842784258903
1.39083893448867 4.7
1.22212748704999 5
1.16259989365078 5
1.29264533457924 4.7
1.4 4.56439076486086
1.49975835935126 4.4
1.7 4.10963121139922
1.71918933786764 4.1
2 3.92258308860939
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
-0.7 -1
-0.4 -1
-0.301486328428696 -1
-0.4 -0.849707151760544
-0.497536424680621 -0.7
-0.650642704639478 -0.4
-0.7 -0.267410388512019
-0.774305560304957 -0.1
-0.863609095258383 0.2
-0.914537768871143 0.5
-0.942313470163013 0.8
-0.966026187747765 1.1
-0.969612000708607 1.4
-0.97092396410361 1.7
-0.977467946765416 2
-0.974528589836557 2.3
-0.979992828421931 2.6
-0.986645855547835 2.9
-0.971786848876576 3.2
-0.967700814360241 3.5
-0.977803211379025 3.8
-0.966154622709294 4.1
-0.930296428224959 4.4
-0.922341411178175 4.7
-0.896723825576484 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
3.8 3.34407396233544
4.1 3.26306882648709
4.4 3.35203634120508
4.69885665864401 3.5
4.7 3.50044327716883
5 3.6508796291292
5 3.8
5 4.1
5 4.21937848861097
4.7 4.15306645343656
4.47279839868686 4.1
4.4 4.07582378041666
4.1 3.9903552025673
3.8 3.95043736640723
3.5 3.92997349507122
3.2 3.8932620892998
2.9 3.88107797603272
2.6 3.84638667564053
2.3 3.86320346805281
2 3.92258308860939
1.71918933786764 4.1
1.7 4.10963121139922
1.49975835935126 4.4
1.4 4.56439076486086
1.29264533457924 4.7
1.16259989365078 5
1.10307230025156 5
1.19445173466982 4.7
1.4 4.4403536871327
1.42448810080992 4.4
1.57733353659516 4.1
1.7 3.95911398858194
1.97156441826447 3.8
2 3.77879366634898
2.3 3.7028606190983
2.6 3.65598837783612
2.9 3.64731242583096
3.2 3.58739230418944
3.5 3.54958749353472
3.61167594635806 3.5
3.8 3.34407396233544
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
-0.4 -0.849707151760544
-0.301486328428696 -1
-0.1 -1
0.2 -1
0.230671797721758 -1
0.2 -0.984819896364115
-0.0936548697730123 -0.7
-0.1 -0.694639070918025
-0.304633595615592 -0.4
-0.4 -0.244213855425091
-0.472158007203864 -0.1
-0.579866848716083 0.2
-0.651710084271046 0.5
-0.690464535202377 0.8
-0.7 0.925005808497229
-0.716350215042926 1.1
-0.737525097007352 1.4
-0.745358935757723 1.7
-0.743235284422173 2
-0.742934554627079 2.3
-0.75552075839787 2.6
-0.757710215907628 2.9
-0.748103405059813 3.2
-0.748540468773214 3.5
-0.736785733158356 3.8
-0.746210312723054 4.1
-0.708924662537897 4.4
-0.7 4.61709124219682
-0.697182857814246 4.7
-0.673515821747843 5
-0.7 5
-0.896723825576484 5
-0.922341411178175 4.7
-0.930296428224959 4.4
-0.966154622709294 4.1
-0.977803211379025 3.8
-0.967700814360241 3.5
-0.971786848876577 3.2
-0.986645855547834 2.9
-0.979992828421931 2.6
-0.974528589836557 2.3
-0.977467946765416 2
-0.97092396410361 1.7
-0.969612000708607 1.4
-0.966026187747765 1.1
-0.942313470163013 0.8
-0.914537768871143 0.5
-0.863609095258383 0.2
-0.774305560304957 -0.1
-0.7 -0.267410388512019
-0.650642704639478 -0.4
-0.497536424680621 -0.7
-0.4 -0.849707151760544
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
2.3 -1
2.6 -1
2.9 -1
3.2 -1
3.5 -1
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.5
5 0.8
5 1.1
5 1.4
5 1.7
5 2
5 2.3
5 2.6
5 2.9
5 3.2
5 3.5
5 3.6508796291292
4.7 3.50044327716883
4.69885665864401 3.5
4.4 3.35203634120508
4.1 3.26306882648709
3.8 3.34407396233544
3.61167594635806 3.5
3.5 3.54958749353472
3.2 3.58739230418944
2.9 3.64731242583096
2.6 3.65598837783612
2.3 3.7028606190983
2 3.77879366634898
1.97156441826447 3.8
1.7 3.95911398858194
1.57733353659516 4.1
1.42448810080992 4.4
1.4 4.4403536871327
1.19445173466982 4.7
1.10307230025156 5
1.1 5
0.970676323615426 5
1.09298396864885 4.7
1.1 4.68936927690564
1.28177203110036 4.4
1.4 4.19612400532359
1.44279553654702 4.1
1.7 3.8045931710347
1.70783929704198 3.8
2 3.58211603320559
2.24716187926409 3.5
2.3 3.46271545572612
2.6 3.31284404117762
2.80320230479843 3.2
2.9 2.94462888407888
2.91819333728202 2.9
2.95637364608628 2.6
2.91147017306824 2.3
2.9 2.26533232303958
2.82539057481502 2
2.75303700822583 1.7
2.66680705194947 1.4
2.6 1.12325454478519
2.59500205102171 1.1
2.52180429266252 0.8
2.45977554906756 0.5
2.39132721051452 0.2
2.31877119033417 -0.1
2.40705680033232 -0.4
2.39548344172734 -0.7
2.3 -0.810400064899295
2.07416379181452 -1
2.3 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
0.2 -0.984819896364115
0.230671797721758 -1
0.5 -1
0.8 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.07416379181452 -1
2.3 -0.810400064899295
2.39548344172734 -0.7
2.40705680033232 -0.4
2.31877119033417 -0.1
2.39132721051452 0.2
2.45977554906756 0.5
2.52180429266252 0.8
2.59500205102171 1.1
2.6 1.12325454478519
2.66680705194947 1.4
2.75303700822583 1.7
2.82539057481502 2
2.9 2.26533232303958
2.91147017306824 2.3
2.95637364608628 2.6
2.91819333728202 2.9
2.9 2.94462888407889
2.80320230479843 3.2
2.6 3.31284404117762
2.3 3.46271545572612
2.24716187926409 3.5
2 3.58211603320559
1.70783929704198 3.8
1.7 3.8045931710347
1.44279553654702 4.1
1.4 4.19612400532359
1.28177203110036 4.4
1.1 4.68936927690564
1.09298396864885 4.7
0.970676323615426 5
0.834314845435185 5
0.908870075888777 4.7
1.1 4.41039905659215
1.10653233701413 4.4
1.21876699169053 4.1
1.4 3.80411776546676
1.40290581242444 3.8
1.7 3.50074278853719
1.70123526611942 3.5
2 3.26439539880634
2.09006744147143 3.2
2.25801398228885 2.9
2.23943796835259 2.6
2.19146167943782 2.3
2.09904764723096 2
2 1.73379883928602
1.98766586591193 1.7
1.86158961346987 1.4
1.72272929630301 1.1
1.7 1.05146223536078
1.5807449445597 0.8
1.41945281775099 0.5
1.4 0.468127602932281
1.22627341678267 0.2
1.1 0.0248744781563919
1.004026720791 -0.1
0.8 -0.298823054367381
0.625405832953192 -0.4
0.5 -0.457352136624025
0.2 -0.434441460094791
0.158445354561305 -0.4
-0.1 -0.206486998825056
-0.168404312811361 -0.1
-0.322903815099418 0.2
-0.4 0.3919448000202
-0.431680344468073 0.5
-0.486624920869417 0.8
-0.516108136999376 1.1
-0.533240039199033 1.4
-0.547707801599335 1.7
-0.546912079483277 2
-0.553520209036411 2.3
-0.551201527474215 2.6
-0.555379139739154 2.9
-0.551226943153677 3.2
-0.550533611185282 3.5
-0.540353560391608 3.8
-0.543918377757781 4.1
-0.529505192526277 4.4
-0.514212352228398 4.7
-0.492295115079372 5
-0.673515821747843 5
-0.697182857814246 4.7
-0.7 4.61709124219682
-0.708924662537897 4.4
-0.746210312723054 4.1
-0.736785733158356 3.8
-0.748540468773214 3.5
-0.748103405059813 3.2
-0.757710215907628 2.9
-0.75552075839787 2.6
-0.742934554627079 2.3
-0.743235284422173 2
-0.745358935757723 1.7
-0.737525097007352 1.4
-0.716350215042926 1.1
-0.7 0.925005808497229
-0.690464535202377 0.8
-0.651710084271046 0.5
-0.579866848716083 0.2
-0.472158007203864 -0.1
-0.4 -0.244213855425091
-0.304633595615592 -0.4
-0.1 -0.694639070918025
-0.0936548697730123 -0.7
0.2 -0.984819896364115
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
0.2 -0.434441460094791
0.5 -0.457352136624025
0.625405832953192 -0.4
0.8 -0.298823054367381
1.004026720791 -0.1
1.1 0.0248744781563919
1.22627341678267 0.2
1.4 0.468127602932281
1.41945281775099 0.5
1.5807449445597 0.8
1.7 1.05146223536078
1.72272929630301 1.1
1.86158961346987 1.4
1.98766586591193 1.7
2 1.73379883928602
2.09904764723096 2
2.19146167943782 2.3
2.23943796835259 2.6
2.25801398228885 2.9
2.09006744147143 3.2
2 3.26439539880634
1.70123526611942 3.5
1.7 3.50074278853719
1.40290581242444 3.8
1.4 3.80411776546676
1.21876699169053 4.1
1.10653233701413 4.4
1.1 4.41039905659215
0.908870075888777 4.7
0.834314845435185 5
0.8 5
0.547167683544275 5
0.658240626786555 4.7
0.8 4.4432295502918
0.820010594702054 4.4
0.90106395939268 4.1
1.0104861956007 3.8
1.1 3.60859151463014
1.15553969527407 3.5
1.32565348024788 3.2
1.4 3.0825588295968
1.53632937987169 2.9
1.64036334401752 2.6
1.58755031187129 2.3
1.48204079538251 2
1.4 1.77809878380887
1.36405664022627 1.7
1.23682570194575 1.4
1.1 1.12929489268957
1.08308767414583 1.1
0.906816075301588 0.8
0.8 0.629240761988058
0.7042659300184 0.5
0.5 0.27658766170714
0.336582501638463 0.2
0.2 0.151723460345106
0.130617283674486 0.2
-0.1 0.386417028057984
-0.146928490915596 0.5
-0.229235795282095 0.8
-0.283525188480095 1.1
-0.308542523586132 1.4
-0.336731322938169 1.7
-0.340020840859529 2
-0.359032752499086 2.3
-0.336635395867947 2.6
-0.34392514324559 2.9
-0.343398478234119 3.2
-0.341190234507101 3.5
-0.331898357546166 3.8
-0.325275505748864 4.1
-0.323311154964585 4.4
-0.29796183726483 4.7
-0.239144621681755 5
-0.4 5
-0.492295115079372 5
-0.514212352228398 4.7
-0.529505192526277 4.4
-0.543918377757781 4.1
-0.540353560391608 3.8
-0.550533611185282 3.5
-0.551226943153677 3.2
-0.555379139739154 2.9
-0.551201527474215 2.6
-0.553520209036411 2.3
-0.546912079483277 2
-0.547707801599335 1.7
-0.533240039199033 1.4
-0.516108136999376 1.1
-0.486624920869417 0.8
-0.431680344468073 0.5
-0.4 0.3919448000202
-0.322903815099418 0.2
-0.168404312811361 -0.1
-0.1 -0.206486998825056
0.158445354561305 -0.4
0.2 -0.434441460094791
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
0.2 0.151723460345106
0.336582501638463 0.2
0.5 0.27658766170714
0.7042659300184 0.5
0.8 0.629240761988058
0.906816075301588 0.8
1.08308767414583 1.1
1.1 1.12929489268957
1.23682570194575 1.4
1.36405664022627 1.7
1.4 1.77809878380887
1.48204079538251 2
1.58755031187129 2.3
1.64036334401752 2.6
1.53632937987169 2.9
1.4 3.0825588295968
1.32565348024788 3.2
1.15553969527407 3.5
1.1 3.60859151463014
1.0104861956007 3.8
0.90106395939268 4.1
0.820010594702054 4.4
0.8 4.4432295502918
0.658240626786555 4.7
0.547167683544275 5
0.5 5
0.2 5
-0.1 5
-0.239144621681755 5
-0.29796183726483 4.7
-0.323311154964585 4.4
-0.325275505748864 4.1
-0.331898357546166 3.8
-0.341190234507101 3.5
-0.343398478234119 3.2
-0.34392514324559 2.9
-0.336635395867947 2.6
-0.359032752499086 2.3
-0.340020840859529 2
-0.336731322938169 1.7
-0.308542523586132 1.4
-0.283525188480095 1.1
-0.229235795282095 0.8
-0.146928490915596 0.5
-0.1 0.386417028057984
0.130617283674486 0.2
0.2 0.151723460345106

0.119588831211478 1.4
0.0690778068193293 1.7
0.0193479069205601 2
-0.0201802152852135 2.3
0.0244646708312302 2.6
0.0377602921136549 2.9
0.0454109075991477 3.2
0.0509254718301785 3.5
0.0284586589686856 3.8
0.126170096778087 4.1
0.2 4.31361042024933
0.274935818296477 4.1
0.405328092560044 3.8
0.463835995982904 3.5
0.437192181554081 3.2
0.5 2.94864209496468
0.506306910197257 2.9
0.537059220922952 2.6
0.542622848210235 2.3
0.516439258804833 2
0.5 1.90655981098815
0.43389382306295 1.7
0.346084459569719 1.4
0.2 1.18464681714952
0.119588831211478 1.4
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
0.2 1.18464681714952
0.346084459569719 1.4
0.43389382306295 1.7
0.5 1.90655981098815
0.516439258804833 2
0.542622848210235 2.3
0.537059220922952 2.6
0.506306910197257 2.9
0.5 2.94864209496468
0.437192181554081 3.2
0.463835995982904 3.5
0.405328092560044 3.8
0.274935818296477 4.1
0.2 4.31361042024933
0.126170096778087 4.1
0.0284586589686856 3.8
0.0509254718301785 3.5
0.0454109075991477 3.2
0.0377602921136549 2.9
0.0244646708312302 2.6
-0.0201802152852135 2.3
0.0193479069205601 2
0.0690778068193293 1.7
0.119588831211478 1.4
0.2 1.18464681714952
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
0.2 2.3
};
\coordinate (MCMC_mean_lml_t) at (axis cs:0.19999999999999996,2.3);
\end{axis}



==> fig/tikz/monks-2/MCMC_nlpd.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
3.5 -1
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.5
5 0.8
5 0.839463020512593
4.95623301726304 0.8
4.7 0.547184884359738
4.65233637615277 0.5
4.4 0.235788581029688
4.36296615546957 0.2
4.12516747512841 -0.1
4.1 -0.124548017163562
3.85770065596012 -0.4
3.8 -0.485748522651224
3.64158537887167 -0.7
3.5 -0.969768850996085
3.48181573936642 -1
3.5 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
-0.7 -1
-0.4 -1
-0.392270066547457 -1
-0.4 -0.992269030695477
-0.606337837366515 -0.7
-0.7 -0.51978414234985
-0.76469755546591 -0.4
-0.884899997748735 -0.1
-0.954685848291287 0.2
-0.994221360945818 0.5
-1 0.565647755353666
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
1.1 -1
1.4 -1
1.7 -1
2 -1
2.3 -1
2.6 -1
2.9 -1
3.2 -1
3.48181573936642 -1
3.5 -0.969768850996085
3.64158537887167 -0.7
3.8 -0.485748522651224
3.85770065596012 -0.4
4.1 -0.124548017163562
4.12516747512841 -0.1
4.36296615546957 0.2
4.4 0.235788581029688
4.65233637615277 0.5
4.7 0.547184884359738
4.95623301726304 0.8
5 0.839463020512593
5 1.1
5 1.4
5 1.7
5 2
5 2.3
5 2.6
5 2.9
5 3.2
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.1 5
3.86047742666099 5
3.8 4.73359063330178
3.79435706554489 4.7
3.76163591534845 4.4
3.71951143268572 4.1
3.6871938286065 3.8
3.63756478775292 3.5
3.55161319798525 3.2
3.5 3.0966570873162
3.42751800844769 2.9
3.32641104844156 2.6
3.2 2.37328668673136
3.1666787591016 2.3
3.01960646453548 2
2.9 1.7680551121273
2.86451021299694 1.7
2.68750782902191 1.4
2.6 1.25280692335502
2.52130381957972 1.1
2.34633673719158 0.8
2.3 0.730969981540032
2.15854973675903 0.5
2 0.259038958554671
1.95870752520729 0.2
1.75818609257466 -0.1
1.7 -0.180166058610541
1.52833161471267 -0.4
1.4 -0.556645750794917
1.26789230827452 -0.7
1.1 -0.892654595958203
0.993332032175121 -1
1.1 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
-0.4 -0.992269030695477
-0.392270066547457 -1
-0.1 -1
0.2 -1
0.5 -1
0.8 -1
0.993332032175121 -1
1.1 -0.892654595958203
1.26789230827452 -0.7
1.4 -0.556645750794917
1.52833161471267 -0.4
1.7 -0.180166058610541
1.75818609257466 -0.1
1.95870752520729 0.2
2 0.259038958554671
2.15854973675903 0.5
2.3 0.730969981540032
2.34633673719158 0.8
2.52130381957972 1.1
2.6 1.25280692335502
2.68750782902191 1.4
2.86451021299694 1.7
2.9 1.7680551121273
3.01960646453548 2
3.1666787591016 2.3
3.2 2.37328668673136
3.32641104844156 2.6
3.42751800844769 2.9
3.5 3.0966570873162
3.55161319798525 3.2
3.63756478775292 3.5
3.6871938286065 3.8
3.71951143268572 4.1
3.76163591534845 4.4
3.79435706554489 4.7
3.8 4.73359063330178
3.86047742666099 5
3.8 5
3.5 5
3.29317447925092 5
3.33167999434032 4.7
3.30608544437768 4.4
3.29444124313541 4.1
3.24258006704706 3.8
3.2 3.51812725612064
3.19814941735652 3.5
3.12786387453488 3.2
3.0200212484885 2.9
2.9 2.65859397736122
2.87370304532448 2.6
2.7329138979422 2.3
2.6 2.07345839835288
2.56195288197755 2
2.38307443447101 1.7
2.3 1.56241467526072
2.20894352491781 1.4
2.00746734571725 1.1
2 1.08894968128902
1.81711184831527 0.8
1.7 0.637077448526531
1.59272231925657 0.5
1.4 0.261151709973423
1.34757310499822 0.2
1.1 -0.0820597781973982
1.08301137456669 -0.1
0.8 -0.380416426499089
0.777898369307415 -0.4
0.5 -0.639024145592912
0.375586868360552 -0.7
0.2 -0.792435879561636
-0.1 -0.744907530548922
-0.144902237736758 -0.7
-0.4 -0.459411767846626
-0.43797979201061 -0.4
-0.597402701016802 -0.1
-0.7 0.187788587447961
-0.704340305031977 0.2
-0.77819221737514 0.5
-0.822581739346635 0.8
-0.847249950063258 1.1
-0.861230259307191 1.4
-0.868667335214878 1.7
-0.872671545915202 2
-0.874326027200269 2.3
-0.876610426521112 2.6
-0.876721237990005 2.9
-0.877438855195298 3.2
-0.878117532324565 3.5
-0.878457569681616 3.8
-0.877723520712146 4.1
-0.879752175022339 4.4
-0.875007359219885 4.7
-0.872672513689424 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.565647755353666
-0.994221360945818 0.5
-0.954685848291287 0.2
-0.884899997748735 -0.1
-0.76469755546591 -0.4
-0.7 -0.51978414234985
-0.606337837366515 -0.7
-0.4 -0.992269030695477
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
-0.1 -0.744907530548922
0.2 -0.792435879561636
0.375586868360552 -0.7
0.5 -0.639024145592912
0.777898369307415 -0.4
0.8 -0.380416426499089
1.08301137456669 -0.1
1.1 -0.0820597781973982
1.34757310499822 0.2
1.4 0.261151709973423
1.59272231925657 0.5
1.7 0.637077448526531
1.81711184831527 0.8
2 1.08894968128902
2.00746734571725 1.1
2.20894352491781 1.4
2.3 1.56241467526072
2.38307443447101 1.7
2.56195288197755 2
2.6 2.07345839835288
2.7329138979422 2.3
2.87370304532448 2.6
2.9 2.65859397736122
3.0200212484885 2.9
3.12786387453488 3.2
3.19814941735652 3.5
3.2 3.51812725612064
3.24258006704706 3.8
3.29444124313541 4.1
3.30608544437768 4.4
3.33167999434032 4.7
3.29317447925092 5
3.2 5
2.94712519418572 5
3.01845787189829 4.7
3.01532046998603 4.4
3.00143242153737 4.1
2.95402390602298 3.8
2.92240887193356 3.5
2.9 3.43618027034913
2.82369901062869 3.2
2.70096522064466 2.9
2.6 2.69480973714244
2.55764257200533 2.6
2.40157077418265 2.3
2.3 2.12559195979964
2.22777838977224 2
2.04119285376862 1.7
2 1.63302000101389
1.85341875073936 1.4
1.7 1.18967175589532
1.6301143018808 1.1
1.40639976271477 0.8
1.4 0.792187304046701
1.16366622261655 0.5
1.1 0.428440556070552
0.866639001851193 0.2
0.8 0.130319989263015
0.541860040167315 -0.1
0.5 -0.137682078888297
0.2 -0.317509876249371
-0.1 -0.313661787025814
-0.313118593564381 -0.1
-0.4 0.00270151890554357
-0.488445344142924 0.2
-0.577713090506096 0.5
-0.632097774509576 0.8
-0.664137489549118 1.1
-0.68373702600561 1.4
-0.694180770589057 1.7
-0.698119187240342 2
-0.699639802059148 2.3
-0.7 2.3226247989201
-0.704682153085391 2.6
-0.70462241637641 2.9
-0.705220599789411 3.2
-0.705126962606621 3.5
-0.708476358165609 3.8
-0.705970243523936 4.1
-0.709963423334291 4.4
-0.7 4.68879393332609
-0.699638749372967 4.7
-0.693903130744155 5
-0.7 5
-0.872672513689424 5
-0.875007359219885 4.7
-0.879752175022339 4.4
-0.877723520712146 4.1
-0.878457569681616 3.8
-0.878117532324565 3.5
-0.877438855195298 3.2
-0.876721237990005 2.9
-0.876610426521112 2.6
-0.874326027200269 2.3
-0.872671545915202 2
-0.868667335214878 1.7
-0.861230259307191 1.4
-0.847249950063258 1.1
-0.822581739346635 0.8
-0.77819221737514 0.5
-0.704340305031977 0.2
-0.7 0.187788587447961
-0.597402701016802 -0.1
-0.43797979201061 -0.4
-0.4 -0.459411767846626
-0.144902237736758 -0.7
-0.1 -0.744907530548922
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
-0.1 -0.313661787025814
0.2 -0.317509876249372
0.5 -0.137682078888297
0.541860040167315 -0.1
0.8 0.130319989263015
0.866639001851193 0.2
1.1 0.428440556070552
1.16366622261655 0.5
1.4 0.792187304046701
1.40639976271477 0.8
1.6301143018808 1.1
1.7 1.18967175589532
1.85341875073936 1.4
2 1.63302000101389
2.04119285376862 1.7
2.22777838977224 2
2.3 2.12559195979964
2.40157077418265 2.3
2.55764257200533 2.6
2.6 2.69480973714244
2.70096522064466 2.9
2.82369901062869 3.2
2.9 3.43618027034913
2.92240887193356 3.5
2.95402390602298 3.8
3.00143242153737 4.1
3.01532046998603 4.4
3.01845787189829 4.7
2.94712519418572 5
2.9 5
2.67445474710099 5
2.74397744099569 4.7
2.74285527371822 4.4
2.73091389815342 4.1
2.69605676868422 3.8
2.67288478566236 3.5
2.6 3.28588188279039
2.56977816568156 3.2
2.43608485543472 2.9
2.3 2.6252681369126
2.28631082075366 2.6
2.11779087884989 2.3
2 2.10529697507047
1.93568130032712 2
1.73411148685695 1.7
1.7 1.64846418847713
1.5198417560576 1.4
1.4 1.24902835657736
1.27228011342194 1.1
1.1 0.896755073078871
1.0073979220398 0.8
0.8 0.573581581092328
0.719262950309377 0.5
0.5 0.302173799232668
0.34110946701546 0.2
0.2 0.111603369665418
-0.1 0.110610066462849
-0.176535004661799 0.2
-0.374574435729857 0.5
-0.4 0.561530052959511
-0.45105273046732 0.8
-0.490960345822375 1.1
-0.516650184501635 1.4
-0.528149399814139 1.7
-0.533557281760609 2
-0.537486491201191 2.3
-0.540943942297374 2.6
-0.538713222651003 2.9
-0.540177867726786 3.2
-0.542657688158546 3.5
-0.541251795845367 3.8
-0.543487034840789 4.1
-0.542189200675777 4.4
-0.540987387215325 4.7
-0.534731600227071 5
-0.693903130744155 5
-0.699638749372967 4.7
-0.7 4.68879393332609
-0.709963423334291 4.4
-0.705970243523936 4.1
-0.708476358165609 3.8
-0.705126962606621 3.5
-0.705220599789411 3.2
-0.70462241637641 2.9
-0.704682153085391 2.6
-0.7 2.3226247989201
-0.699639802059148 2.3
-0.698119187240342 2
-0.694180770589057 1.7
-0.68373702600561 1.4
-0.664137489549118 1.1
-0.632097774509576 0.8
-0.577713090506096 0.5
-0.488445344142924 0.2
-0.4 0.00270151890554357
-0.313118593564381 -0.1
-0.1 -0.313661787025814
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
-0.1 0.110610066462849
0.2 0.111603369665418
0.34110946701546 0.2
0.5 0.302173799232668
0.719262950309377 0.5
0.8 0.573581581092328
1.0073979220398 0.8
1.1 0.896755073078871
1.27228011342194 1.1
1.4 1.24902835657736
1.5198417560576 1.4
1.7 1.64846418847713
1.73411148685695 1.7
1.93568130032712 2
2 2.10529697507047
2.11779087884989 2.3
2.28631082075366 2.6
2.3 2.6252681369126
2.43608485543472 2.9
2.56977816568156 3.2
2.6 3.28588188279039
2.67288478566236 3.5
2.69605676868422 3.8
2.73091389815342 4.1
2.74285527371822 4.4
2.74397744099569 4.7
2.67445474710099 5
2.6 5
2.46884114180582 5
2.50245176426341 4.7
2.47624504305126 4.4
2.49388793846851 4.1
2.46873174228345 3.8
2.42180894646551 3.5
2.31421799766062 3.2
2.3 3.1670072427142
2.18166082539285 2.9
2.01557564172576 2.6
2 2.57259925501357
1.83447263494849 2.3
1.7 2.07410849373336
1.65159455914893 2
1.41582061613968 1.7
1.4 1.67850580906245
1.17424705523498 1.4
1.1 1.31366244901816
0.880880374532825 1.1
0.8 1.01536161408876
0.541696694296143 0.8
0.5 0.762279140751031
0.2 0.585417089235091
-0.1 0.646596807641488
-0.171388778178224 0.8
-0.250964738090342 1.1
-0.308587020914697 1.4
-0.333949204037346 1.7
-0.346435490925812 2
-0.358099218986924 2.3
-0.360428074213172 2.6
-0.35610094350418 2.9
-0.35948532125601 3.2
-0.36546292478763 3.5
-0.359341764837401 3.8
-0.367651680278551 4.1
-0.361114063901115 4.4
-0.366119494924356 4.7
-0.357181287803877 5
-0.4 5
-0.534731600227071 5
-0.540987387215325 4.7
-0.542189200675777 4.4
-0.543487034840789 4.1
-0.541251795845367 3.8
-0.542657688158546 3.5
-0.540177867726786 3.2
-0.538713222651003 2.9
-0.540943942297374 2.6
-0.537486491201192 2.3
-0.533557281760609 2
-0.528149399814139 1.7
-0.516650184501635 1.4
-0.490960345822375 1.1
-0.45105273046732 0.8
-0.4 0.561530052959511
-0.374574435729857 0.5
-0.176535004661799 0.2
-0.1 0.110610066462849
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
-0.1 0.646596807641488
0.2 0.585417089235091
0.5 0.762279140751031
0.541696694296143 0.8
0.8 1.01536161408876
0.880880374532825 1.1
1.1 1.31366244901816
1.17424705523498 1.4
1.4 1.67850580906245
1.41582061613968 1.7
1.65159455914893 2
1.7 2.07410849373336
1.83447263494849 2.3
2 2.57259925501357
2.01557564172576 2.6
2.18166082539285 2.9
2.3 3.1670072427142
2.31421799766062 3.2
2.42180894646551 3.5
2.46873174228345 3.8
2.49388793846851 4.1
2.47624504305126 4.4
2.50245176426341 4.7
2.46884114180582 5
2.3 5
2.28251005348956 5
2.27166757476312 4.7
2.23780805959679 4.4
2.29017609203592 4.1
2.24645684726277 3.8
2.1605477361205 3.5
2.0550056094617 3.2
2 3.07787895009102
1.91823823228526 2.9
1.74890532162047 2.6
1.7 2.52336527246963
1.53605786250305 2.3
1.4 2.09542820824267
1.31702768059823 2
1.1 1.75159338690687
1.01953086708018 1.7
0.8 1.52987632654157
0.58264317254363 1.4
0.5 1.34385182097658
0.2 1.34772566437838
0.163585931803705 1.4
0.0426976493245724 1.7
-0.0181563827425974 2
-0.0564011236258905 2.3
-0.0443928849312791 2.6
-0.0718884143468232 2.9
-0.0748446043298512 3.2
-0.0595714258076439 3.5
-0.0921631376178882 3.8
-0.0707894387802219 4.1
-0.1 4.31222428217228
-0.105052858139728 4.4
-0.1 4.44076799055792
-0.0309133172993642 4.7
-0.0517932862800002 5
-0.1 5
-0.357181287803877 5
-0.366119494924356 4.7
-0.361114063901115 4.4
-0.367651680278551 4.1
-0.359341764837401 3.8
-0.36546292478763 3.5
-0.35948532125601 3.2
-0.35610094350418 2.9
-0.360428074213172 2.6
-0.358099218986924 2.3
-0.346435490925812 2
-0.333949204037346 1.7
-0.308587020914697 1.4
-0.250964738090342 1.1
-0.171388778178224 0.8
-0.1 0.646596807641488
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
0.2 1.34772566437838
0.5 1.34385182097658
0.58264317254363 1.4
0.8 1.52987632654157
1.01953086708018 1.7
1.1 1.75159338690687
1.31702768059823 2
1.4 2.09542820824267
1.53605786250305 2.3
1.7 2.52336527246963
1.74890532162047 2.6
1.91823823228526 2.9
2 3.07787895009102
2.0550056094617 3.2
2.1605477361205 3.5
2.24645684726277 3.8
2.29017609203592 4.1
2.23780805959679 4.4
2.27166757476312 4.7
2.28251005348956 5
2.0548900192735 5
2.0191552777867 4.7
2.02343341879284 4.4
2.09508089546078 4.1
2 3.84006902057176
1.98239754632533 3.8
1.89052170391422 3.5
1.80919700951205 3.2
1.7 2.98409954573041
1.63419150635701 2.9
1.42790252394273 2.6
1.4 2.56073648505258
1.166277661422 2.3
1.1 2.22320281911039
0.8 2.27221241683098
0.771881213774825 2.3
0.661181347278363 2.6
0.600165729539065 2.9
0.549553570263162 3.2
0.588236773412099 3.5
0.571329469169261 3.8
0.521729627420455 4.1
0.596423496542708 4.4
0.563020491715601 4.7
0.797304728395435 5
0.5 5
0.2 5
-0.0517932862800002 5
-0.0309133172993642 4.7
-0.1 4.44076799055792
-0.105052858139728 4.4
-0.1 4.31222428217228
-0.0707894387802219 4.1
-0.0921631376178882 3.8
-0.0595714258076439 3.5
-0.0748446043298512 3.2
-0.0718884143468232 2.9
-0.0443928849312791 2.6
-0.0564011236258905 2.3
-0.0181563827425974 2
0.0426976493245724 1.7
0.163585931803705 1.4
0.2 1.34772566437838
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
0.8 2.27221241683098
1.1 2.22320281911039
1.166277661422 2.3
1.4 2.56073648505258
1.42790252394273 2.6
1.63419150635701 2.9
1.7 2.98409954573041
1.80919700951205 3.2
1.89052170391422 3.5
1.98239754632533 3.8
2 3.84006902057176
2.09508089546078 4.1
2.02343341879284 4.4
2.0191552777867 4.7
2.0548900192735 5
2 5
1.74525511812747 5
1.78708389474256 4.7
1.74965446748262 4.4
1.8386272349285 4.1
1.74809563036473 3.8
1.7 3.67750989728814
1.5047272707331 3.5
1.44230743073998 3.2
1.4 3.14184692520835
1.27593897181409 3.2
1.1 3.4311449458121
1.08176747358723 3.5
1.1 3.59039588731655
1.19807867468256 3.8
1.1 3.91898377330247
1.03902716187813 4.1
1.1 4.31455730682668
1.12743555753286 4.4
1.1 4.45942566886983
1.02913322042707 4.7
1.1 4.95105201523807
1.13724522221372 5
1.1 5
0.8 5
0.797304728395435 5
0.563020491715601 4.7
0.596423496542708 4.4
0.521729627420455 4.1
0.571329469169261 3.8
0.588236773412099 3.5
0.549553570263162 3.2
0.600165729539065 2.9
0.661181347278363 2.6
0.771881213774825 2.3
0.8 2.27221241683098
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
1.4 3.14184692520835
1.44230743073998 3.2
1.5047272707331 3.5
1.7 3.67750989728814
1.74809563036473 3.8
1.8386272349285 4.1
1.74965446748262 4.4
1.78708389474256 4.7
1.74525511812747 5
1.7 5
1.4 5
1.13724522221372 5
1.1 4.95105201523807
1.02913322042707 4.7
1.1 4.45942566886983
1.12743555753286 4.4
1.1 4.31455730682668
1.03902716187813 4.1
1.1 3.91898377330247
1.19807867468256 3.8
1.1 3.59039588731655
1.08176747358723 3.5
1.1 3.4311449458121
1.27593897181409 3.2
1.4 3.14184692520835
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
0.2 2.3
};
\coordinate (CVI_mean_lml_b) at (axis cs:0.5,1.1);
\coordinate (CVI_mean_lml_ep_b) at (axis cs:0.19999999999999996,1.6999999999999997);
\end{axis}



==> fig/tikz/parkinsons/CVI_mean_lml.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=black]
table{%
x  y
-0.7 2.2414170717495
-0.643952244938434 2.3
-0.4 2.54558585754713
-0.370296010482878 2.6
-0.215612128883443 2.9
-0.1 3.16366234574019
-0.0890222859063814 3.2
0.00574496792424713 3.5
0.0920851650388677 3.8
0.158590342962005 4.1
0.2 4.30473283984208
0.218838158243989 4.4
0.285135101296094 4.7
0.353800511655173 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2.08241300587579
-0.7 2.2414170717495
};
\addplot [draw=none, fill=midnightblue854116]
table{%
x  y
-0.7 1.96473446946498
-0.666986931754244 2
-0.4 2.27960620203503
-0.389283947781193 2.3
-0.225972755133375 2.6
-0.1 2.85568821998779
-0.0854580593748024 2.9
0.0048274098644713 3.2
0.0962018770973644 3.5
0.177282266980043 3.8
0.2 3.90474442320307
0.240406856739082 4.1
0.299333435396895 4.4
0.364099759436204 4.7
0.430038459760615 5
0.353800511655173 5
0.285135101296094 4.7
0.218838158243989 4.4
0.2 4.30473283984208
0.158590342962005 4.1
0.0920851650388677 3.8
0.00574496792424713 3.5
-0.0890222859063814 3.2
-0.1 3.16366234574019
-0.215612128883443 2.9
-0.370296010482878 2.6
-0.4 2.54558585754713
-0.643952244938434 2.3
-0.7 2.2414170717495
-1 2.08241300587579
-1 2
-1 1.80210149163812
-0.7 1.96473446946498
};
\addplot [draw=none, fill=midnightblue868137]
table{%
x  y
-0.7 1.66739535990689
-0.672628938952518 1.7
-0.4 1.99222489596112
-0.396033361678869 2
-0.238561070187928 2.3
-0.1 2.56354889202482
-0.0871494969876712 2.6
0.0106751805096471 2.9
0.0986771056353243 3.2
0.186658786270482 3.5
0.2 3.55023181814831
0.261043814231102 3.8
0.32169783713098 4.1
0.3798287125498 4.4
0.443064417576315 4.7
0.5 4.96925638317346
0.507683992937541 5
0.5 5
0.430038459760615 5
0.364099759436204 4.7
0.299333435396895 4.4
0.240406856739082 4.1
0.2 3.90474442320307
0.177282266980043 3.8
0.0962018770973644 3.5
0.0048274098644713 3.2
-0.0854580593748024 2.9
-0.1 2.85568821998779
-0.225972755133375 2.6
-0.389283947781193 2.3
-0.4 2.27960620203503
-0.666986931754244 2
-0.7 1.96473446946498
-1 1.80210149163812
-1 1.7
-1 1.48615535483905
-0.7 1.66739535990689
};
\addplot [draw=none, fill=teal882156]
table{%
x  y
-0.982452498317352 1.1
-0.7 1.30361434718251
-0.633689079873498 1.4
-0.4 1.68112062104692
-0.391390419390565 1.7
-0.238783785270578 2
-0.1 2.27486975855229
-0.0913504758629681 2.3
0.013917308046221 2.6
0.106808420394096 2.9
0.192526801406177 3.2
0.2 3.22562787547754
0.274479017354025 3.5
0.344283388409309 3.8
0.402988817522879 4.1
0.460323989702706 4.4
0.5 4.59157255672323
0.527021977956248 4.7
0.601019522959869 5
0.507683992937541 5
0.5 4.96925638317346
0.443064417576315 4.7
0.3798287125498 4.4
0.32169783713098 4.1
0.261043814231102 3.8
0.2 3.55023181814831
0.186658786270482 3.5
0.0986771056353243 3.2
0.0106751805096471 2.9
-0.0871494969876713 2.6
-0.1 2.56354889202482
-0.238561070187928 2.3
-0.396033361678869 2
-0.4 1.99222489596112
-0.672628938952518 1.7
-0.7 1.66739535990689
-1 1.48615535483905
-1 1.4
-1 1.1
-1 1.08241728031725
-0.982452498317352 1.1
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 -1
-0.4 -1
-0.343093276589475 -1
-0.4 -0.90045400412193
-0.543016517063655 -0.7
-0.684613676301647 -0.4
-0.7 -0.351627390160387
-0.81313246309775 -0.1
-0.856793260059638 0.2
-0.804841873534874 0.5
-0.7 0.689662614559513
-0.671450754499558 0.8
-0.527901160010461 1.1
-0.4 1.29121353268964
-0.360325982886771 1.4
-0.225572460969655 1.7
-0.1 1.95972549787508
-0.0867605516366383 2
0.0158442135689558 2.3
0.114984113080113 2.6
0.2 2.88946993978282
0.202954597879158 2.9
0.284970352006802 3.2
0.361843096343931 3.5
0.427522962587516 3.8
0.484279797914777 4.1
0.5 4.18282076838653
0.550965403421436 4.4
0.623884019698364 4.7
0.694355052982196 5
0.601019522959869 5
0.527021977956248 4.7
0.5 4.59157255672323
0.460323989702706 4.4
0.402988817522879 4.1
0.344283388409309 3.8
0.274479017354025 3.5
0.2 3.22562787547754
0.192526801406177 3.2
0.106808420394096 2.9
0.013917308046221 2.6
-0.0913504758629681 2.3
-0.1 2.27486975855229
-0.238783785270578 2
-0.391390419390565 1.7
-0.4 1.68112062104692
-0.633689079873498 1.4
-0.7 1.30361434718251
-0.982452498317352 1.1
-1 1.08241728031725
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.4 -0.90045400412193
-0.343093276589475 -1
-0.1 -1
0.2 -1
0.242492683082818 -1
0.2 -0.937106774122799
0.03095217552599 -0.7
-0.1 -0.444640290563668
-0.128840888057076 -0.4
-0.280088761708127 -0.1
-0.358275997585822 0.2
-0.381794127271694 0.5
-0.356835603985354 0.8
-0.288392877856446 1.1
-0.185446439097509 1.4
-0.1 1.60043536125713
-0.0710164056898968 1.7
0.025982933410485 2
0.123038903000879 2.3
0.2 2.54565916222921
0.216110445855727 2.6
0.299510637592736 2.9
0.377292244489161 3.2
0.449207175333836 3.5
0.5 3.74542084754483
0.513868783451888 3.8
0.583697999402375 4.1
0.651468783066386 4.4
0.72074606144048 4.7
0.787690583004524 5
0.694355052982196 5
0.623884019698364 4.7
0.550965403421436 4.4
0.5 4.18282076838653
0.484279797914777 4.1
0.427522962587516 3.8
0.361843096343931 3.5
0.284970352006802 3.2
0.202954597879158 2.9
0.2 2.88946993978282
0.114984113080113 2.6
0.0158442135689557 2.3
-0.0867605516366383 2
-0.1 1.95972549787508
-0.225572460969655 1.7
-0.360325982886771 1.4
-0.4 1.29121353268964
-0.527901160010461 1.1
-0.671450754499558 0.8
-0.7 0.689662614559513
-0.804841873534874 0.5
-0.856793260059639 0.2
-0.81313246309775 -0.1
-0.7 -0.351627390160387
-0.684613676301647 -0.4
-0.543016517063655 -0.7
-0.4 -0.90045400412193
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
0.2 -0.937106774122799
0.242492683082818 -1
0.5 -1
0.555470324540704 -1
0.5 -0.938913734556099
0.321383589018569 -0.7
0.2 -0.508751767317023
0.130553216599694 -0.4
-0.0151745590196048 -0.1
-0.1 0.188606935664053
-0.104267754744926 0.2
-0.16172239816197 0.5
-0.157306182149834 0.8
-0.102764829620459 1.1
-0.1 1.10849021363609
-0.035181472120885 1.4
0.0484006903969931 1.7
0.138726418457608 2
0.2 2.19750343263978
0.230479510506707 2.3
0.317552075471233 2.6
0.396066677306314 2.9
0.46961413697152 3.2
0.5 3.33205025990262
0.546847818754863 3.5
0.621132679876523 3.8
0.687462093774378 4.1
0.751972162711336 4.4
0.8 4.61732747185571
0.824418328364311 4.7
0.911637412798082 5
0.8 5
0.787690583004524 5
0.72074606144048 4.7
0.651468783066386 4.4
0.583697999402375 4.1
0.513868783451888 3.8
0.5 3.74542084754483
0.449207175333836 3.5
0.377292244489161 3.2
0.299510637592736 2.9
0.216110445855727 2.6
0.2 2.54565916222921
0.123038903000879 2.3
0.025982933410485 2
-0.0710164056898968 1.7
-0.1 1.60043536125713
-0.185446439097509 1.4
-0.288392877856446 1.1
-0.356835603985354 0.8
-0.381794127271694 0.5
-0.358275997585822 0.2
-0.280088761708127 -0.1
-0.128840888057076 -0.4
-0.1 -0.444640290563668
0.0309521755259899 -0.7
0.2 -0.937106774122799
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
0.5 -0.938913734556099
0.555470324540704 -1
0.8 -1
0.871386803682708 -1
0.8 -0.946459938196365
0.574024782449055 -0.7
0.5 -0.617860488121408
0.349243965820273 -0.4
0.2 -0.129902199742833
0.184125886057689 -0.1
0.0688348884385142 0.2
0.0115472465134416 0.5
0.00240103055130071 0.8
0.0326594987056121 1.1
0.0915661637088311 1.4
0.167817786483883 1.7
0.2 1.81135872182782
0.252739285901961 2
0.338546114568573 2.3
0.41899370508674 2.6
0.492622717019892 2.9
0.5 2.93067312521003
0.579384184484578 3.2
0.658761304192731 3.5
0.728396576301158 3.8
0.791226188146381 4.1
0.8 4.14181200488551
0.873850322994585 4.4
0.958743367056405 4.7
1.0402346847711 5
0.911637412798082 5
0.824418328364311 4.7
0.8 4.61732747185571
0.751972162711336 4.4
0.687462093774378 4.1
0.621132679876523 3.8
0.546847818754863 3.5
0.5 3.33205025990262
0.46961413697152 3.2
0.396066677306314 2.9
0.317552075471233 2.6
0.230479510506707 2.3
0.2 2.19750343263978
0.138726418457608 2
0.0484006903969931 1.7
-0.035181472120885 1.4
-0.1 1.10849021363609
-0.102764829620459 1.1
-0.157306182149834 0.8
-0.16172239816197 0.5
-0.104267754744926 0.2
-0.1 0.188606935664053
-0.0151745590196048 -0.1
0.130553216599694 -0.4
0.2 -0.508751767317023
0.321383589018569 -0.7
0.5 -0.938913734556099
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
3.5 -1
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.5
5 0.589475123811497
4.92151616580008 0.5
4.7 0.251479287946024
4.65349816564598 0.2
4.4 -0.0727872031202808
4.37411688805644 -0.1
4.1 -0.374498224817066
4.07347599166483 -0.4
3.8 -0.642799607867404
3.73074235447198 -0.7
3.5 -0.868950089862986
3.29580952499083 -1
3.5 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.8 -0.946459938196365
0.871386803682708 -1
1.1 -1
1.38254798154345 -1
1.1 -0.873221775310734
0.866775611243382 -0.7
0.8 -0.652900207406123
0.571193498624294 -0.4
0.5 -0.315298717355334
0.370968533377132 -0.1
0.240691375462821 0.2
0.2 0.35682470482901
0.166574080354256 0.5
0.14606263231496 0.8
0.167324763875543 1.1
0.2 1.28802985254005
0.219196624605384 1.4
0.29036829758966 1.7
0.368263320077331 2
0.446612718630439 2.3
0.5 2.51310242912817
0.526911246881903 2.6
0.61599034667883 2.9
0.6977143100901 3.2
0.7706747896306 3.5
0.8 3.63223161657298
0.85120723955841 3.8
0.93534211558196 4.1
1.01529158716358 4.4
1.0930684057485 4.7
1.1 4.72637949285264
1.19759142942564 5
1.1 5
1.0402346847711 5
0.958743367056405 4.7
0.873850322994585 4.4
0.8 4.14181200488551
0.791226188146381 4.1
0.728396576301158 3.8
0.658761304192731 3.5
0.579384184484578 3.2
0.5 2.93067312521003
0.492622717019892 2.9
0.41899370508674 2.6
0.338546114568573 2.3
0.252739285901961 2
0.2 1.81135872182782
0.167817786483883 1.7
0.0915661637088311 1.4
0.0326594987056121 1.1
0.00240103055130071 0.8
0.0115472465134416 0.5
0.0688348884385142 0.2
0.184125886057689 -0.1
0.2 -0.129902199742833
0.349243965820273 -0.4
0.5 -0.617860488121408
0.574024782449055 -0.7
0.8 -0.946459938196365
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
2.3 -1
2.6 -1
2.9 -1
3.2 -1
3.29580952499083 -1
3.5 -0.868950089862986
3.73074235447198 -0.7
3.8 -0.642799607867404
4.07347599166483 -0.4
4.1 -0.374498224817066
4.37411688805644 -0.1
4.4 -0.0727872031202808
4.65349816564598 0.2
4.7 0.251479287946024
4.92151616580008 0.5
5 0.589475123811497
5 0.8
5 1.1
5 1.35821149400892
4.76116643749644 1.1
4.7 1.03405699501617
4.48133897998084 0.8
4.4 0.713372082718719
4.19712968202838 0.5
4.1 0.39875181733083
3.90508179638076 0.2
3.8 0.0945099350631382
3.59847831740216 -0.1
3.5 -0.192571434797028
3.2630177901154 -0.4
3.2 -0.45285835980644
2.9 -0.677217732238221
2.86439960233878 -0.7
2.6 -0.859480416434124
2.3 -0.985923573299535
2.24451570014029 -1
2.3 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
1.1 -0.873221775310734
1.38254798154345 -1
1.4 -1
1.7 -1
2 -1
2.24451570014029 -1
2.3 -0.985923573299535
2.6 -0.859480416434124
2.86439960233878 -0.7
2.9 -0.677217732238221
3.2 -0.45285835980644
3.2630177901154 -0.4
3.5 -0.192571434797028
3.59847831740216 -0.1
3.8 0.0945099350631382
3.90508179638076 0.2
4.1 0.39875181733083
4.19712968202838 0.5
4.4 0.713372082718719
4.48133897998084 0.8
4.7 1.03405699501617
4.76116643749644 1.1
5 1.35821149400892
5 1.4
5 1.7
5 1.87365384718484
4.83779228387123 1.7
4.7 1.55270669820526
4.55651674628675 1.4
4.4 1.23386730200292
4.27291459554955 1.1
4.1 0.918717622984194
3.98524127251307 0.8
3.8 0.609955985189029
3.69026867598457 0.5
3.5 0.312085634157688
3.3815960960534 0.2
3.2 0.0322909551170692
3.04509706256604 -0.1
2.9 -0.219064345411314
2.6444840816742 -0.4
2.6 -0.429727945762779
2.3 -0.58479948896004
2 -0.683309308868948
1.85616123958559 -0.7
1.7 -0.715990458647444
1.56936198220251 -0.7
1.4 -0.679813469468208
1.1 -0.567549029271743
0.855005852207048 -0.4
0.8 -0.362597488604624
0.578962060704853 -0.1
0.5 0.0130555207989881
0.412989079858663 0.2
0.327048931881001 0.5
0.295112957665973 0.8
0.307940784248948 1.1
0.352054188079399 1.4
0.414074770945865 1.7
0.483787354252701 2
0.5 2.06514131832492
0.57264954054524 2.3
0.660499503617691 2.6
0.741575956195512 2.9
0.8 3.13229542183011
0.823317769030552 3.2
0.919636427966355 3.5
1.00523458749684 3.8
1.0831851546953 4.1
1.1 4.16627368564227
1.18235311025726 4.4
1.28400269856568 4.7
1.37991940883698 5
1.19759142942564 5
1.1 4.72637949285264
1.0930684057485 4.7
1.01529158716358 4.4
0.93534211558196 4.1
0.85120723955841 3.8
0.8 3.63223161657298
0.7706747896306 3.5
0.6977143100901 3.2
0.61599034667883 2.9
0.526911246881903 2.6
0.5 2.51310242912817
0.446612718630439 2.3
0.368263320077331 2
0.29036829758966 1.7
0.219196624605384 1.4
0.2 1.28802985254005
0.167324763875543 1.1
0.14606263231496 0.8
0.166574080354256 0.5
0.2 0.35682470482901
0.240691375462821 0.2
0.370968533377132 -0.1
0.5 -0.315298717355334
0.571193498624294 -0.4
0.8 -0.652900207406124
0.866775611243382 -0.7
1.1 -0.873221775310734
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.7 -0.715990458647444
1.85616123958559 -0.7
2 -0.683309308868948
2.3 -0.58479948896004
2.6 -0.429727945762779
2.6444840816742 -0.4
2.9 -0.219064345411314
3.04509706256604 -0.1
3.2 0.0322909551170692
3.3815960960534 0.2
3.5 0.312085634157688
3.69026867598457 0.5
3.8 0.609955985189029
3.98524127251307 0.8
4.1 0.918717622984194
4.27291459554955 1.1
4.4 1.23386730200292
4.55651674628675 1.4
4.7 1.55270669820526
4.83779228387123 1.7
5 1.87365384718484
5 2
5 2.3
5 2.4099067454351
4.89919521966923 2.3
4.7 2.08316805617825
4.62335693955243 2
4.4 1.75832055813952
4.34581018533348 1.7
4.1 1.4367901319386
4.06532446437989 1.4
3.8 1.12100465114017
3.77970859985319 1.1
3.5 0.815001801738431
3.48487411859094 0.8
3.2 0.525216218688345
3.17258353505708 0.5
2.9 0.261008617769037
2.82402265156757 0.2
2.6 0.0334588430006852
2.38717414815213 -0.1
2.3 -0.149000987291711
2 -0.269200455313326
1.7 -0.33298067199545
1.4 -0.330799764938192
1.1 -0.248127267256356
0.873592121564212 -0.1
0.8 -0.0473924947249847
0.626136764244435 0.2
0.5 0.463867962605774
0.489021346173649 0.5
0.447402692842758 0.8
0.450463288356224 1.1
0.484911751553414 1.4
0.5 1.48131732584846
0.552028895686338 1.7
0.633919713367205 2
0.716231954276998 2.3
0.794087760353479 2.6
0.8 2.62292942765191
0.898309478542714 2.9
0.995289821558311 3.2
1.08175301931 3.5
1.1 3.5678989018979
1.18768217042161 3.8
1.29115253286428 4.1
1.38766850952658 4.4
1.4 4.43898546584583
1.51287024778853 4.7
1.63385456289276 5
1.4 5
1.37991940883698 5
1.28400269856568 4.7
1.18235311025726 4.4
1.1 4.16627368564227
1.0831851546953 4.1
1.00523458749684 3.8
0.919636427966355 3.5
0.823317769030552 3.2
0.8 3.13229542183011
0.741575956195512 2.9
0.66049950361769 2.6
0.57264954054524 2.3
0.5 2.06514131832492
0.483787354252701 2
0.414074770945865 1.7
0.352054188079399 1.4
0.307940784248948 1.1
0.295112957665973 0.8
0.327048931881001 0.5
0.412989079858663 0.2
0.5 0.0130555207989881
0.578962060704853 -0.1
0.8 -0.362597488604624
0.855005852207048 -0.4
1.1 -0.567549029271743
1.4 -0.679813469468208
1.56936198220251 -0.7
1.7 -0.715990458647444
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.1 -0.248127267256356
1.4 -0.330799764938192
1.7 -0.33298067199545
2 -0.269200455313326
2.3 -0.149000987291711
2.38717414815213 -0.1
2.6 0.0334588430006852
2.82402265156757 0.2
2.9 0.261008617769037
3.17258353505709 0.5
3.2 0.525216218688345
3.48487411859094 0.8
3.5 0.815001801738431
3.77970859985319 1.1
3.8 1.12100465114017
4.06532446437989 1.4
4.1 1.4367901319386
4.34581018533348 1.7
4.4 1.75832055813952
4.62335693955243 2
4.7 2.08316805617825
4.89919521966923 2.3
5 2.4099067454351
5 2.6
5 2.9
5 3.2
5 3.20535722996318
4.99570475733337 3.2
4.7376485107908 2.9
4.7 2.85657915229964
4.47739863122583 2.6
4.4 2.5112825719026
4.2156113211387 2.3
4.1 2.16887084883184
3.95122959515939 2
3.8 1.83148623080117
3.68241429425835 1.7
3.5 1.50258449930557
3.40595005226405 1.4
3.2 1.18737360105779
3.11623868163562 1.1
2.9 0.89304069682768
2.80286844996045 0.8
2.6 0.628373306077486
2.44209692387462 0.5
2.3 0.401921340126978
2 0.221800460194425
1.95367018270089 0.2
1.7 0.10508687800165
1.4 0.0573397825991788
1.1 0.110094133959248
0.971850584365856 0.2
0.8 0.355129754024001
0.727570628849687 0.5
0.648564128493775 0.8
0.635049785707014 1.1
0.666273803565866 1.4
0.722386207015598 1.7
0.789701902989838 2
0.8 2.04108572066204
0.890775567422282 2.3
0.990081403820024 2.6
1.08213866199208 2.9
1.1 2.95969646356865
1.20075229317473 3.2
1.3139852239761 3.5
1.4 3.75176168753755
1.42292892663486 3.8
1.55710088443502 4.1
1.6805197709442 4.4
1.7 4.44912760165051
1.83738919418612 4.7
1.98748482614855 5
1.7 5
1.63385456289276 5
1.51287024778853 4.7
1.4 4.43898546584583
1.38766850952658 4.4
1.29115253286428 4.1
1.18768217042161 3.8
1.1 3.5678989018979
1.08175301931 3.5
0.995289821558311 3.2
0.898309478542714 2.9
0.8 2.62292942765191
0.794087760353479 2.6
0.716231954276998 2.3
0.633919713367205 2
0.552028895686338 1.7
0.5 1.48131732584846
0.484911751553414 1.4
0.450463288356224 1.1
0.447402692842758 0.8
0.489021346173649 0.5
0.5 0.463867962605774
0.626136764244435 0.2
0.8 -0.0473924947249847
0.873592121564212 -0.1
1.1 -0.248127267256356
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
4.4 4.69600090578702
4.7 4.69978038945049
4.70041654970692 4.7
5 4.84151092177993
5 5
4.7 5
4.4 5
4.28919714875555 5
4.39729902249434 4.7
4.4 4.69600090578702
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.1 0.110094133959248
1.4 0.0573397825991788
1.7 0.10508687800165
1.95367018270089 0.2
2 0.221800460194425
2.3 0.401921340126978
2.44209692387462 0.5
2.6 0.628373306077486
2.80286844996045 0.8
2.9 0.89304069682768
3.11623868163562 1.1
3.2 1.18737360105779
3.40595005226405 1.4
3.5 1.50258449930557
3.68241429425835 1.7
3.8 1.83148623080117
3.95122959515939 2
4.1 2.16887084883184
4.2156113211387 2.3
4.4 2.5112825719026
4.47739863122583 2.6
4.7 2.85657915229964
4.7376485107908 2.9
4.99570475733337 3.2
5 3.20535722996318
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 4.84151092177993
4.70041654970692 4.7
4.7 4.69978038945049
4.4 4.69600090578702
4.39729902249434 4.7
4.28919714875555 5
4.1 5
3.8 5
3.5 5
3.31001029929812 5
3.41431777022834 4.7
3.42054118529671 4.4
3.39560259660744 4.1
3.35769862904152 3.8
3.30978351877491 3.5
3.24639990259624 3.2
3.2 3.03171369520293
3.1704342672739 2.9
3.0936489630298 2.6
2.984411411696 2.3
2.9 2.13292621271514
2.84618387116297 2
2.68451538316967 1.7
2.6 1.58095689185099
2.48756813842357 1.4
2.3 1.16764416292583
2.24620237931616 1.1
2 0.85260276516941
1.93853347945483 0.8
1.7 0.634980736305313
1.4 0.520879752449725
1.1 0.585740539827341
0.952781005829848 0.8
0.878573145063733 1.1
0.89334028938859 1.4
0.951485702444988 1.7
1.02750584240127 2
1.1 2.26458567104817
1.11441806332547 2.3
1.24076554959813 2.6
1.35456183306196 2.9
1.4 3.02470792956746
1.49117509386034 3.2
1.632953134852 3.5
1.7 3.65462200098953
1.79020124216031 3.8
1.95864380795763 4.1
2 4.17768833942882
2.17143999689698 4.4
2.3 4.5820767570017
2.42721216712075 4.7
2.6 4.8784443367022
2.79883608965826 5
2.6 5
2.3 5
2 5
1.98748482614855 5
1.83738919418612 4.7
1.7 4.44912760165051
1.6805197709442 4.4
1.55710088443502 4.1
1.42292892663486 3.8
1.4 3.75176168753755
1.3139852239761 3.5
1.20075229317473 3.2
1.1 2.95969646356865
1.08213866199208 2.9
0.990081403820024 2.6
0.890775567422282 2.3
0.8 2.04108572066204
0.789701902989838 2
0.722386207015598 1.7
0.666273803565866 1.4
0.635049785707014 1.1
0.648564128493775 0.8
0.727570628849687 0.5
0.8 0.355129754024001
0.971850584365856 0.2
1.1 0.110094133959248
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.1 0.585740539827341
1.4 0.520879752449725
1.7 0.634980736305313
1.93853347945483 0.8
2 0.85260276516941
2.24620237931616 1.1
2.3 1.16764416292583
2.48756813842357 1.4
2.6 1.58095689185099
2.68451538316967 1.7
2.84618387116297 2
2.9 2.13292621271514
2.984411411696 2.3
3.0936489630298 2.6
3.1704342672739 2.9
3.2 3.03171369520293
3.24639990259624 3.2
3.30978351877491 3.5
3.35769862904152 3.8
3.39560259660744 4.1
3.42054118529671 4.4
3.41431777022834 4.7
3.31001029929812 5
3.2 5
2.9 5
2.79883608965826 5
2.6 4.87844433670221
2.42721216712075 4.7
2.3 4.5820767570017
2.17143999689698 4.4
2 4.17768833942882
1.95864380795763 4.1
1.79020124216031 3.8
1.7 3.65462200098953
1.632953134852 3.5
1.49117509386034 3.2
1.4 3.02470792956746
1.35456183306196 2.9
1.24076554959813 2.6
1.11441806332547 2.3
1.1 2.26458567104817
1.02750584240127 2
0.951485702444988 1.7
0.89334028938859 1.4
0.878573145063733 1.1
0.952781005829848 0.8
1.1 0.585740539827341

1.38682013162037 1.4
1.36184649840956 1.7
1.4 1.94416911281371
1.41843565688973 2
1.5584149946821 2.3
1.67767975765503 2.6
1.7 2.65187810905808
1.88795268833869 2.9
2 3.08823135853021
2.18268329455353 3.2
2.3 3.29783413406861
2.37717484210599 3.2
2.40593391273591 2.9
2.35614299749467 2.6
2.3 2.41094940946004
2.2530625064107 2.3
2.11141594680976 2
2 1.78648556386859
1.92827669006095 1.7
1.7 1.42538684118354
1.55428939049711 1.4
1.4 1.37498903223188
1.38682013162037 1.4
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.4 1.37498903223188
1.55428939049711 1.4
1.7 1.42538684118354
1.92827669006095 1.7
2 1.78648556386859
2.11141594680976 2
2.2530625064107 2.3
2.3 2.41094940946004
2.35614299749467 2.6
2.40593391273591 2.9
2.37717484210599 3.2
2.3 3.29783413406861
2.18268329455353 3.2
2 3.08823135853021
1.88795268833869 2.9
1.7 2.65187810905808
1.67767975765503 2.6
1.5584149946821 2.3
1.41843565688973 2
1.4 1.94416911281371
1.36184649840956 1.7
1.38682013162037 1.4
1.4 1.37498903223188
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
1.7 2
};
\coordinate (CVI_mean_lml_t) at (axis cs:1.6999999999999997,2.0);
\end{axis}



==> fig/tikz/parkinsons/CVI_mean_lml_ep.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 -1
-0.4 -1
-0.343297793594463 -1
-0.4 -0.901329457265568
-0.544393025744032 -0.7
-0.689121718904544 -0.4
-0.7 -0.370370013599173
-0.840274064312877 -0.1
-0.931053238780318 0.2
-0.982066472191937 0.5
-1 0.683630361780575
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.991708490645045 1.4
-0.8899418325346 1.7
-0.7 1.98819596836463
-0.697176299271114 2
-0.644931835356631 2.3
-0.610978984028315 2.6
-0.588927913761947 2.9
-0.570931092934582 3.2
-0.552980059575664 3.5
-0.542240187292291 3.8
-0.540471237227902 4.1
-0.540047287748294 4.4
-0.537018460104706 4.7
-0.521730367577003 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.31359912087186
-0.991708490645045 1.4
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.4 -0.901329457265569
-0.343297793594463 -1
-0.1 -1
0.2 -1
0.242427156973383 -1
0.2 -0.937293196379489
0.0305753651532684 -0.7
-0.1 -0.447812835187258
-0.131190319213515 -0.4
-0.287543313106442 -0.1
-0.379497204443621 0.2
-0.4 0.30353380271446
-0.45936730594736 0.5
-0.512732591125764 0.8
-0.535838339838692 1.1
-0.521017623035221 1.4
-0.467504765093605 1.7
-0.402973957437485 2
-0.4 2.01650964398851
-0.372185901791976 2.3
-0.349568998488401 2.6
-0.332833845979787 2.9
-0.320361570514069 3.2
-0.310558127502583 3.5
-0.302297803932611 3.8
-0.29746807653786 4.1
-0.296174652152796 4.4
-0.295834533715577 4.7
-0.291917725523593 5
-0.4 5
-0.521730367577003 5
-0.537018460104706 4.7
-0.540047287748294 4.4
-0.540471237227902 4.1
-0.542240187292291 3.8
-0.552980059575664 3.5
-0.570931092934582 3.2
-0.588927913761947 2.9
-0.610978984028315 2.6
-0.644931835356631 2.3
-0.697176299271114 2
-0.7 1.98819596836463
-0.8899418325346 1.7
-0.991708490645045 1.4
-1 1.31359912087186
-1 1.1
-1 0.8
-1 0.683630361780575
-0.982066472191937 0.5
-0.931053238780318 0.2
-0.840274064312877 -0.1
-0.7 -0.370370013599173
-0.689121718904545 -0.4
-0.544393025744032 -0.7
-0.4 -0.901329457265569
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
0.2 -0.937293196379489
0.242427156973383 -1
0.5 -1
0.555413827797106 -1
0.5 -0.939032060802479
0.321120553107418 -0.7
0.2 -0.510220548992679
0.129216635517459 -0.4
-0.0197688311631893 -0.1
-0.1 0.141296447203821
-0.124906289433245 0.2
-0.212052096377954 0.5
-0.261701728229274 0.8
-0.286403098410361 1.1
-0.286742276861089 1.4
-0.265484964672528 1.7
-0.236806389203088 2
-0.211944114842798 2.3
-0.19197835692626 2.6
-0.175934435176178 2.9
-0.164106697669355 3.2
-0.156161551357944 3.5
-0.148965697253938 3.8
-0.143847893010681 4.1
-0.142501290709935 4.4
-0.144509957603634 4.7
-0.144235377703372 5
-0.291917725523593 5
-0.295834533715577 4.7
-0.296174652152796 4.4
-0.29746807653786 4.1
-0.302297803932611 3.8
-0.310558127502583 3.5
-0.320361570514069 3.2
-0.332833845979787 2.9
-0.349568998488401 2.6
-0.372185901791976 2.3
-0.4 2.01650964398851
-0.402973957437485 2
-0.467504765093605 1.7
-0.521017623035221 1.4
-0.535838339838692 1.1
-0.512732591125764 0.8
-0.45936730594736 0.5
-0.4 0.30353380271446
-0.379497204443621 0.2
-0.287543313106442 -0.1
-0.131190319213515 -0.4
-0.1 -0.447812835187258
0.0305753651532684 -0.7
0.2 -0.937293196379489
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
0.5 -0.939032060802479
0.555413827797106 -1
0.8 -1
0.87132832702707 -1
0.8 -0.946539171349402
0.573769413562108 -0.7
0.5 -0.618451633772237
0.348214990611947 -0.4
0.2 -0.1373270211964
0.179753012376363 -0.1
0.0556456941995673 0.2
-0.0221483675958121 0.5
-0.0693231540133634 0.8
-0.0952150131474265 1.1
-0.1 1.2892959776153
-0.103571049514232 1.4
-0.1 1.49319681296813
-0.0942267400887723 1.7
-0.0780493341196982 2
-0.0618068799956686 2.3
-0.0475200902838808 2.6
-0.035853880749725 2.9
-0.02755632791368 3.2
-0.0213419867878708 3.5
-0.0148525653368496 3.8
-0.0110526333121953 4.1
-0.011140590705833 4.4
-0.0131021081319563 4.7
-0.013301136749282 5
-0.1 5
-0.144235377703372 5
-0.144509957603634 4.7
-0.142501290709935 4.4
-0.143847893010681 4.1
-0.148965697253938 3.8
-0.156161551357944 3.5
-0.164106697669355 3.2
-0.175934435176178 2.9
-0.19197835692626 2.6
-0.211944114842798 2.3
-0.236806389203088 2
-0.265484964672528 1.7
-0.286742276861089 1.4
-0.286403098410361 1.1
-0.261701728229275 0.8
-0.212052096377954 0.5
-0.124906289433245 0.2
-0.1 0.141296447203821
-0.0197688311631893 -0.1
0.129216635517459 -0.4
0.2 -0.510220548992679
0.321120553107418 -0.7
0.5 -0.939032060802479
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
3.5 -1
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.5
5 0.589472078926016
4.92151868005754 0.5
4.7 0.251476839542626
4.65350028580877 0.2
4.4 -0.0727891786247329
4.37411871738195 -0.1
4.1 -0.374499903913896
4.07347768979503 -0.4
3.8 -0.642801154677325
3.73074411606113 -0.7
3.5 -0.868951519886687
3.29581151382926 -1
3.5 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.8 -0.946539171349402
0.87132832702707 -1
1.1 -1
1.38249967712715 -1
1.1 -0.873305766347414
0.866485583980235 -0.7
0.8 -0.653234616511699
0.570081468240903 -0.4
0.5 -0.3178290270885
0.367342200340397 -0.1
0.228398998312448 0.2
0.2 0.285110011728479
0.135152638668638 0.5
0.0794065449763839 0.8
0.048322080303202 1.1
0.0361157710369146 1.4
0.0392256410334022 1.7
0.050945660588854 2
0.0649100720176348 2.3
0.0785286014692426 2.6
0.0884528115911574 2.9
0.0952857875021769 3.2
0.102285283146277 3.5
0.110243580129387 3.8
0.113424233577871 4.1
0.111689937070037 4.4
0.110006384278475 4.7
0.110471378421995 5
-0.013301136749282 5
-0.0131021081319563 4.7
-0.011140590705833 4.4
-0.0110526333121953 4.1
-0.0148525653368496 3.8
-0.0213419867878707 3.5
-0.02755632791368 3.2
-0.035853880749725 2.9
-0.0475200902838808 2.6
-0.0618068799956686 2.3
-0.0780493341196981 2
-0.0942267400887723 1.7
-0.1 1.49319681296813
-0.103571049514232 1.4
-0.1 1.2892959776153
-0.0952150131474265 1.1
-0.0693231540133634 0.8
-0.0221483675958121 0.5
0.0556456941995673 0.2
0.179753012376363 -0.1
0.2 -0.1373270211964
0.348214990611947 -0.4
0.5 -0.618451633772237
0.573769413562108 -0.7
0.8 -0.946539171349402
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
2.3 -1
2.6 -1
2.9 -1
3.2 -1
3.29581151382926 -1
3.5 -0.868951519886687
3.73074411606113 -0.7
3.8 -0.642801154677325
4.07347768979503 -0.4
4.1 -0.374499903913896
4.37411871738195 -0.1
4.4 -0.0727891786247329
4.65350028580877 0.2
4.7 0.251476839542625
4.92151868005754 0.5
5 0.589472078926016
5 0.8
5 1.1
5 1.35819427342782
4.76118191242418 1.1
4.7 1.03404050184891
4.48135405952045 0.8
4.4 0.713356271798296
4.19714445284628 0.5
4.1 0.398736704779651
3.90509625150511 0.2
3.8 0.0944956929423012
3.59849222295027 -0.1
3.5 -0.192584336475283
3.26303057717242 -0.4
3.2 -0.452869058869501
2.9 -0.67722550273437
2.86441090025872 -0.7
2.6 -0.859487612183848
2.3 -0.985929180638597
2.24453787322502 -1
2.3 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
1.1 -0.873305766347414
1.38249967712715 -1
1.4 -1
1.7 -1
2 -1
2.24453787322502 -1
2.3 -0.985929180638597
2.6 -0.859487612183848
2.86441090025872 -0.7
2.9 -0.67722550273437
3.2 -0.452869058869501
3.26303057717242 -0.4
3.5 -0.192584336475283
3.59849222295027 -0.1
3.8 0.0944956929423012
3.90509625150511 0.2
4.1 0.398736704779651
4.19714445284628 0.5
4.4 0.713356271798296
4.48135405952045 0.8
4.7 1.03404050184891
4.76118191242418 1.1
5 1.35819427342782
5 1.4
5 1.7
5 1.87360970722164
4.83783405304263 1.7
4.7 1.55266242638218
4.55655968486814 1.4
4.4 1.2338218388617
4.2729600992466 1.1
4.1 0.918669571460478
3.98529113287076 0.8
3.8 0.609903932402564
3.69032458341533 0.5
3.5 0.312029270808362
3.3816580522046 0.2
3.2 0.0322330971298574
3.04516094113706 -0.1
2.9 -0.219116760542623
2.64454308710858 -0.4
2.6 -0.429767452858512
2.3 -0.584840867105772
2 -0.683350338339288
1.85659010358191 -0.7
1.7 -0.716045658895343
1.5687261689943 -0.7
1.4 -0.679934193894691
1.1 -0.567911959397337
0.853624198157092 -0.4
0.8 -0.363929400718101
0.574751587656935 -0.1
0.5 0.00163439420726803
0.402330299291429 0.2
0.29775088233646 0.5
0.230537646987567 0.8
0.2 1.03080421367597
0.19185917375383 1.1
0.174937976799599 1.4
0.172678022155576 1.7
0.179940655297406 2
0.191627024030938 2.3
0.2 2.49360174069719
0.205138599799582 2.6
0.214647141062556 2.9
0.221755056013096 3.2
0.232170505373876 3.5
0.244290989395717 3.8
0.24885428157949 4.1
0.24662860190858 4.4
0.246373428723507 4.7
0.248684241668323 5
0.2 5
0.110471378421995 5
0.110006384278475 4.7
0.111689937070037 4.4
0.113424233577871 4.1
0.110243580129387 3.8
0.102285283146277 3.5
0.095285787502177 3.2
0.0884528115911574 2.9
0.0785286014692426 2.6
0.0649100720176348 2.3
0.050945660588854 2
0.0392256410334022 1.7
0.0361157710369146 1.4
0.048322080303202 1.1
0.0794065449763839 0.8
0.135152638668638 0.5
0.2 0.285110011728479
0.228398998312448 0.2
0.367342200340397 -0.1
0.5 -0.3178290270885
0.570081468240903 -0.4
0.8 -0.653234616511699
0.866485583980235 -0.7
1.1 -0.873305766347414
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.7 -0.716045658895343
1.85659010358191 -0.7
2 -0.683350338339288
2.3 -0.584840867105772
2.6 -0.429767452858512
2.64454308710858 -0.4
2.9 -0.219116760542623
3.04516094113706 -0.1
3.2 0.0322330971298574
3.3816580522046 0.2
3.5 0.312029270808362
3.69032458341533 0.5
3.8 0.609903932402564
3.98529113287076 0.8
4.1 0.918669571460478
4.2729600992466 1.1
4.4 1.2338218388617
4.55655968486814 1.4
4.7 1.55266242638218
4.83783405304263 1.7
5 1.87360970722164
5 2
5 2.3
5 2.40970208825892
4.89938435526501 2.3
4.7 2.08296759088353
4.62354599173212 2
4.4 1.75811802968869
4.3460049504647 1.7
4.1 1.43657642622608
4.06553310039329 1.4
3.8 1.12076775413799
3.77994322842077 1.1
3.5 0.814730093561251
3.4851521929015 0.8
3.2 0.524908977086795
3.17292017016114 0.5
2.9 0.260687750652317
2.82440892407637 0.2
2.6 0.0331614547417042
2.38759364198873 -0.1
2.3 -0.149242278184581
2 -0.269500031379237
1.7 -0.333374718016264
1.4 -0.331463505346882
1.1 -0.24965546914809
0.868043620837991 -0.1
0.8 -0.0531842035484198
0.613593635354149 0.2
0.5 0.400965377826553
0.464064629792185 0.5
0.391961291514648 0.8
0.349297338345772 1.1
0.327509335696395 1.4
0.320717819360945 1.7
0.324365585213791 2
0.334285787457432 2.3
0.346644452869105 2.6
0.357343727656702 2.9
0.36917625049559 3.2
0.385654098419695 3.5
0.401072966587308 3.8
0.409304184883073 4.1
0.412542236254125 4.4
0.418772165149005 4.7
0.424650535456794 5
0.248684241668323 5
0.246373428723507 4.7
0.246628601908581 4.4
0.24885428157949 4.1
0.244290989395717 3.8
0.232170505373876 3.5
0.221755056013096 3.2
0.214647141062556 2.9
0.205138599799582 2.6
0.2 2.49360174069719
0.191627024030938 2.3
0.179940655297406 2
0.172678022155576 1.7
0.174937976799599 1.4
0.19185917375383 1.1
0.2 1.03080421367597
0.230537646987566 0.8
0.29775088233646 0.5
0.402330299291429 0.2
0.5 0.00163439420726805
0.574751587656935 -0.1
0.8 -0.363929400718101
0.853624198157092 -0.4
1.1 -0.567911959397337
1.4 -0.679934193894691
1.5687261689943 -0.7
1.7 -0.716045658895343
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.1 -0.24965546914809
1.4 -0.331463505346882
1.7 -0.333374718016264
2 -0.269500031379237
2.3 -0.149242278184581
2.38759364198873 -0.1
2.6 0.0331614547417042
2.82440892407637 0.2
2.9 0.260687750652317
3.17292017016114 0.5
3.2 0.524908977086795
3.4851521929015 0.8
3.5 0.814730093561251
3.77994322842077 1.1
3.8 1.12076775413799
4.06553310039329 1.4
4.1 1.43657642622608
4.3460049504647 1.7
4.4 1.75811802968869
4.62354599173212 2
4.7 2.08296759088353
4.89938435526501 2.3
5 2.40970208825892
5 2.6
5 2.9
5 3.2
5 3.20149980035012
4.99879627432426 3.2
4.7397828613351 2.9
4.7 2.85413520713493
4.47954389390549 2.6
4.4 2.50884770530444
4.21781744294966 2.3
4.1 2.16637870124081
3.95354409211756 2
3.8 1.82887560868663
3.68487187874698 1.7
3.5 1.4998333195169
3.40856462941091 1.4
3.2 1.18454356118826
3.11899718787807 1.1
2.9 0.890287732071384
2.80572816788054 0.8
2.6 0.625880379526888
2.44507411261568 0.5
2.3 0.399795147750668
2 0.21972963574455
1.95818337602791 0.2
1.7 0.102824901571377
1.4 0.0540245486715281
1.1 0.103618170934725
0.956072112676059 0.2
0.8 0.324932845919967
0.699815256938265 0.5
0.58206209625196 0.8
0.511546766670432 1.1
0.5 1.19176678969189
0.483109712190314 1.4
0.472512968913268 1.7
0.471631774066583 2
0.478072452855176 2.3
0.488150305938628 2.6
0.5 2.89899127961576
0.500061590792163 2.9
0.524570086925668 3.2
0.556405729978096 3.5
0.583728660659113 3.8
0.602620788390415 4.1
0.618607213540644 4.4
0.63505355880534 4.7
0.645017706316257 5
0.5 5
0.424650535456794 5
0.418772165149005 4.7
0.412542236254125 4.4
0.409304184883073 4.1
0.401072966587308 3.8
0.385654098419695 3.5
0.36917625049559 3.2
0.357343727656702 2.9
0.346644452869105 2.6
0.334285787457432 2.3
0.324365585213791 2
0.320717819360945 1.7
0.327509335696395 1.4
0.349297338345772 1.1
0.391961291514648 0.8
0.464064629792185 0.5
0.5 0.400965377826553
0.613593635354149 0.2
0.8 -0.0531842035484198
0.868043620837991 -0.1
1.1 -0.24965546914809
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
4.4 4.85316008514366
4.7 4.75796172579074
5 4.88501091661423
5 5
4.7 5
4.4 5
4.36128249235818 5
4.4 4.85316008514366
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.1 0.103618170934725
1.4 0.0540245486715281
1.7 0.102824901571377
1.95818337602791 0.2
2 0.21972963574455
2.3 0.399795147750668
2.44507411261568 0.5
2.6 0.625880379526888
2.80572816788054 0.8
2.9 0.890287732071384
3.11899718787807 1.1
3.2 1.18454356118826
3.40856462941091 1.4
3.5 1.4998333195169
3.68487187874698 1.7
3.8 1.82887560868663
3.95354409211756 2
4.1 2.16637870124081
4.21781744294966 2.3
4.4 2.50884770530444
4.47954389390549 2.6
4.7 2.85413520713493
4.7397828613351 2.9
4.99879627432426 3.2
5 3.20149980035012
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 4.88501091661423
4.7 4.75796172579074
4.4 4.85316008514366
4.36128249235818 5
4.1 5
3.8 5
3.63367167881869 5
3.59150137651786 4.7
3.54036035591807 4.4
3.5 4.2009073986955
3.4806385757475 4.1
3.42459177719462 3.8
3.36693803550371 3.5
3.29929869484354 3.2
3.20728620182807 2.9
3.2 2.87954705873198
3.12538907724686 2.6
3.01442739608678 2.3
2.9 2.08025804221991
2.86662315106489 2
2.70569319304019 1.7
2.6 1.55228967262865
2.50476399903878 1.4
2.3 1.14803030053033
2.26164497539668 1.1
2 0.837372635667205
1.95660215914417 0.8
1.7 0.620556553019328
1.4 0.502229439579436
1.1 0.541765364813181
0.864377320182252 0.8
0.8 0.915274867596882
0.752925186119584 1.1
0.71112306599836 1.4
0.693038970379523 1.7
0.689503111614847 2
0.694602650958041 2.3
0.704219116088984 2.6
0.718068762514211 2.9
0.742805578466908 3.2
0.777608202102408 3.5
0.8 3.70510761117118
0.822076451046621 3.8
0.877438467711822 4.1
0.92264392520916 4.4
0.949170367057986 4.7
0.965108864356723 5
0.8 5
0.645017706316257 5
0.63505355880534 4.7
0.618607213540644 4.4
0.602620788390415 4.1
0.583728660659113 3.8
0.556405729978096 3.5
0.524570086925668 3.2
0.500061590792163 2.9
0.5 2.89899127961576
0.488150305938628 2.6
0.478072452855176 2.3
0.471631774066583 2
0.472512968913268 1.7
0.483109712190314 1.4
0.5 1.19176678969189
0.511546766670432 1.1
0.58206209625196 0.8
0.699815256938265 0.5
0.8 0.324932845919967
0.956072112676059 0.2
1.1 0.103618170934725
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.1 0.541765364813181
1.4 0.502229439579436
1.7 0.620556553019328
1.95660215914417 0.8
2 0.837372635667205
2.26164497539668 1.1
2.3 1.14803030053033
2.50476399903878 1.4
2.6 1.55228967262865
2.70569319304019 1.7
2.86662315106489 2
2.9 2.08025804221991
3.01442739608678 2.3
3.12538907724686 2.6
3.2 2.87954705873198
3.20728620182807 2.9
3.29929869484354 3.2
3.36693803550371 3.5
3.42459177719462 3.8
3.4806385757475 4.1
3.5 4.2009073986955
3.54036035591807 4.4
3.59150137651786 4.7
3.63367167881869 5
3.5 5
3.2 5
2.9 5
2.7271703701219 5
2.81201280248423 4.7
2.83814854986688 4.4
2.83033183185714 4.1
2.79573028796983 3.8
2.74171174903851 3.5
2.67497170497212 3.2
2.6 2.93464500578151
2.58872315600473 2.9
2.47780573317423 2.6
2.36167271667298 2.3
2.3 2.1657208009767
2.21236800234856 2
2.03696850414839 1.7
2 1.64592794271965
1.79138972898015 1.4
1.7 1.30532926879116
1.4 1.14693115715242
1.1 1.33983607321095
1.07907737976832 1.4
1.02937137520425 1.7
1.01697304698815 2
1.0282170894212 2.3
1.05887755424769 2.6
1.1 2.8691237332636
1.10594731709112 2.9
1.16720762308746 3.2
1.22346365898116 3.5
1.26980198261393 3.8
1.3004373514198 4.1
1.33516227619351 4.4
1.38343365828378 4.7
1.4 4.80104863070432
1.52351648539904 5
1.4 5
1.1 5
0.965108864356723 5
0.949170367057986 4.7
0.92264392520916 4.4
0.877438467711822 4.1
0.822076451046621 3.8
0.8 3.70510761117118
0.777608202102409 3.5
0.742805578466908 3.2
0.718068762514211 2.9
0.704219116088984 2.6
0.694602650958041 2.3
0.689503111614847 2
0.693038970379523 1.7
0.71112306599836 1.4
0.752925186119584 1.1
0.8 0.915274867596882
0.864377320182252 0.8
1.1 0.541765364813181
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.1 1.33983607321095
1.4 1.14693115715242
1.7 1.30532926879116
1.79138972898015 1.4
2 1.64592794271965
2.03696850414839 1.7
2.21236800234856 2
2.3 2.1657208009767
2.36167271667298 2.3
2.47780573317423 2.6
2.58872315600473 2.9
2.6 2.93464500578151
2.67497170497212 3.2
2.74171174903851 3.5
2.79573028796983 3.8
2.83033183185714 4.1
2.83814854986688 4.4
2.81201280248423 4.7
2.7271703701219 5
2.6 5
2.3 5
2 5
1.7 5
1.52351648539904 5
1.4 4.80104863070432
1.38343365828378 4.7
1.33516227619351 4.4
1.3004373514198 4.1
1.26980198261393 3.8
1.22346365898116 3.5
1.16720762308746 3.2
1.10594731709112 2.9
1.1 2.8691237332636
1.05887755424769 2.6
1.0282170894212 2.3
1.01697304698815 2
1.02937137520425 1.7
1.07907737976832 1.4
1.1 1.33983607321095
};
\addplot [semithick, steelblue31119180, mark=mystar, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2 3.2
};
\coordinate (CVI_mean_lml_ep_t) at (axis cs:2.0,3.2);
\end{axis}



==> fig/tikz/parkinsons/CVI_nlpd.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 -1
-0.462973412428671 -1
-0.61919254269507 -0.7
-0.7 -0.436603835335294
-0.71897563327871 -0.4
-0.843974248657507 -0.1
-0.913360251059671 0.2
-0.951806525353232 0.5
-0.972921586060407 0.8
-0.981891795975942 1.1
-0.973460611108265 1.4
-0.938296618541962 1.7
-0.881818978637884 2
-0.836405598520415 2.3
-0.81250255309572 2.6
-0.816571875775801 2.9
-0.821632405078472 3.2
-0.792868681040872 3.5
-0.767289119847191 3.8
-0.850879722467759 4.1
-0.876975157508525 4.4
-0.876092745884248 4.7
-0.772247772925056 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.4 -1
-0.1 -1
-0.0267349815600369 -1
-0.1 -0.83291135254353
-0.179062405911325 -0.7
-0.313639695001234 -0.4
-0.396030024886528 -0.1
-0.4 -0.0804869761686454
-0.49577719198752 0.2
-0.554565217936678 0.5
-0.587597536199282 0.8
-0.603337969888707 1.1
-0.598340822462933 1.4
-0.568921761879785 1.7
-0.529122239058379 2
-0.499595832375791 2.3
-0.483602987213582 2.6
-0.489144477259532 2.9
-0.49391996406581 3.2
-0.489508875646292 3.5
-0.486081053664454 3.8
-0.491064245617322 4.1
-0.492102011441577 4.4
-0.488941005774994 4.7
-0.482079434277046 5
-0.7 5
-0.772247772925056 5
-0.876092745884248 4.7
-0.876975157508525 4.4
-0.850879722467759 4.1
-0.767289119847191 3.8
-0.792868681040872 3.5
-0.821632405078472 3.2
-0.816571875775801 2.9
-0.81250255309572 2.6
-0.836405598520415 2.3
-0.881818978637884 2
-0.938296618541962 1.7
-0.973460611108265 1.4
-0.981891795975942 1.1
-0.972921586060407 0.8
-0.951806525353232 0.5
-0.913360251059671 0.2
-0.843974248657507 -0.1
-0.71897563327871 -0.4
-0.7 -0.436603835335294
-0.61919254269507 -0.7
-0.462973412428671 -1
-0.4 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
-0.1 -0.83291135254353
-0.0267349815600369 -1
0.2 -1
0.203106708887918 -1
0.2 -0.994654436861639
0.0265081591405983 -0.7
-0.0937880244794738 -0.4
-0.1 -0.381510141036895
-0.221386334046548 -0.1
-0.300661349863307 0.2
-0.348736541925316 0.5
-0.377504433815935 0.8
-0.392503067146323 1.1
-0.391801316929547 1.4
-0.375445594785626 1.7
-0.355572174990689 2
-0.342661419366718 2.3
-0.337293306665317 2.6
-0.341753946196422 2.9
-0.345078151228884 3.2
-0.344468617653053 3.5
-0.345338920107995 3.8
-0.346562463221161 4.1
-0.345934978374766 4.4
-0.34458371280959 4.7
-0.343499380244378 5
-0.4 5
-0.482079434277046 5
-0.488941005774994 4.7
-0.492102011441577 4.4
-0.491064245617322 4.1
-0.486081053664454 3.8
-0.489508875646292 3.5
-0.49391996406581 3.2
-0.489144477259532 2.9
-0.483602987213582 2.6
-0.499595832375791 2.3
-0.529122239058379 2
-0.568921761879785 1.7
-0.598340822462933 1.4
-0.603337969888707 1.1
-0.587597536199282 0.8
-0.554565217936678 0.5
-0.49577719198752 0.2
-0.4 -0.0804869761686454
-0.396030024886528 -0.1
-0.313639695001234 -0.4
-0.179062405911325 -0.7
-0.1 -0.83291135254353
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
0.2 -0.994654436861639
0.203106708887918 -1
0.370102437444876 -1
0.2 -0.707312995148428
0.195694125620472 -0.7
0.042285391335532 -0.4
-0.0638017614831722 -0.1
-0.1 0.037594834816024
-0.153109217599093 0.2
-0.216243307673302 0.5
-0.253666594395479 0.8
-0.274168832001588 1.1
-0.278135585511742 1.4
-0.267108352038083 1.7
-0.252806981658225 2
-0.243907651908738 2.3
-0.241728901861528 2.6
-0.247821630607284 2.9
-0.251551536029681 3.2
-0.25174797053658 3.5
-0.255577439492088 3.8
-0.257682490000803 4.1
-0.257305030418719 4.4
-0.256399446515742 4.7
-0.254281850929429 5
-0.343499380244378 5
-0.34458371280959 4.7
-0.345934978374766 4.4
-0.346562463221161 4.1
-0.345338920107995 3.8
-0.344468617653053 3.5
-0.345078151228884 3.2
-0.341753946196422 2.9
-0.337293306665317 2.6
-0.342661419366718 2.3
-0.355572174990689 2
-0.375445594785626 1.7
-0.391801316929547 1.4
-0.392503067146323 1.1
-0.377504433815935 0.8
-0.348736541925316 0.5
-0.300661349863307 0.2
-0.221386334046548 -0.1
-0.1 -0.381510141036895
-0.0937880244794738 -0.4
0.0265081591405983 -0.7
0.2 -0.994654436861639
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.2 -0.707312995148428
0.370102437444876 -1
0.5 -1
0.541721918527781 -1
0.5 -0.950365733197156
0.339545430502933 -0.7
0.2 -0.442089440038142
0.178358807150538 -0.4
0.0549009747604763 -0.1
-0.0297904758077604 0.2
-0.0871419794282473 0.5
-0.1 0.601217265724453
-0.129828754975023 0.8
-0.155834596856853 1.1
-0.164469854093937 1.4
-0.15877110929054 1.7
-0.150041788325761 2
-0.145153884450757 2.3
-0.146164497057738 2.6
-0.153889315018146 2.9
-0.158024920830478 3.2
-0.159027323420108 3.5
-0.165815958876181 3.8
-0.168802516780446 4.1
-0.168675082462672 4.4
-0.168215180221894 4.7
-0.16506432161448 5
-0.254281850929429 5
-0.256399446515742 4.7
-0.257305030418719 4.4
-0.257682490000803 4.1
-0.255577439492088 3.8
-0.25174797053658 3.5
-0.251551536029681 3.2
-0.247821630607284 2.9
-0.241728901861528 2.6
-0.243907651908738 2.3
-0.252806981658225 2
-0.267108352038083 1.7
-0.278135585511742 1.4
-0.274168832001588 1.1
-0.253666594395479 0.8
-0.216243307673302 0.5
-0.153109217599093 0.2
-0.1 0.037594834816024
-0.0638017614831722 -0.1
0.042285391335532 -0.4
0.195694125620472 -0.7
0.2 -0.707312995148428
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.289688047242736
4.90896640558331 0.2
4.7 -0.00521186567527747
4.60262313648993 -0.1
4.4 -0.295854690119946
4.29059038799054 -0.4
4.1 -0.578544338003129
3.96681999314687 -0.7
3.8 -0.846598629154208
3.6168258133465 -1
3.8 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
0.5 -0.950365733197156
0.541721918527781 -1
0.729531261474717 -1
0.5 -0.726939309752893
0.482735115969146 -0.7
0.311669930465164 -0.4
0.2 -0.162738527122395
0.173603711004124 -0.1
0.0799008126976204 0.2
0.0176954623520883 0.5
-0.0226852723762792 0.8
-0.047480293769359 1.1
-0.058051689922415 1.4
-0.0567612524260783 1.7
-0.0520993811950412 2
-0.0494308075418666 2.3
-0.0514640796903973 2.6
-0.058826082290169 2.9
-0.0626996295840397 3.2
-0.0642108075941522 3.5
-0.0727411978748024 3.8
-0.077557637455519 4.1
-0.0779630017834254 4.4
-0.077791756636181 4.7
-0.0737754753944908 5
-0.1 5
-0.16506432161448 5
-0.168215180221894 4.7
-0.168675082462672 4.4
-0.168802516780446 4.1
-0.165815958876181 3.8
-0.159027323420108 3.5
-0.158024920830478 3.2
-0.153889315018146 2.9
-0.146164497057738 2.6
-0.145153884450757 2.3
-0.150041788325761 2
-0.15877110929054 1.7
-0.164469854093937 1.4
-0.155834596856853 1.1
-0.129828754975023 0.8
-0.1 0.601217265724453
-0.0871419794282473 0.5
-0.0297904758077604 0.2
0.0549009747604763 -0.1
0.178358807150538 -0.4
0.2 -0.442089440038142
0.339545430502933 -0.7
0.5 -0.950365733197156
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
3.2 -1
3.5 -1
3.6168258133465 -1
3.8 -0.846598629154208
3.96681999314687 -0.7
4.1 -0.578544338003129
4.29059038799054 -0.4
4.4 -0.295854690119945
4.60262313648993 -0.1
4.7 -0.00521186567527746
4.90896640558331 0.2
5 0.289688047242736
5 0.5
5 0.8
5 0.923134943945064
4.87602521036433 0.8
4.7 0.625219940184137
4.5732596732044 0.5
4.4 0.328916709803235
4.26829761436712 0.2
4.1 0.0354537581654869
3.95931162273134 -0.1
3.8 -0.252988400437954
3.6426741977422 -0.4
3.5 -0.532494225874431
3.31045584206093 -0.7
3.2 -0.796096541579519
2.94269114714841 -1
3.2 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
0.5 -0.726939309752893
0.729531261474717 -1
0.8 -1
0.981427434921187 -1
0.8 -0.863083643985299
0.662493598074891 -0.7
0.5 -0.496694954780719
0.444458654553784 -0.4
0.300419530171041 -0.1
0.2 0.167375676609564
0.189592101203001 0.2
0.122532904132424 0.5
0.0791611489646303 0.8
0.0519583499905063 1.1
0.0388687352449256 1.4
0.0377461534436827 1.7
0.0412655361810348 2
0.0437391397111039 2.3
0.0424289364633042 2.6
0.0377591230443872 2.9
0.0355654660040305 3.2
0.0342774599792909 3.5
0.0294403484355674 3.8
0.0217914303870503 4.1
0.0199147817421502 4.4
0.0202807159675672 4.7
0.0230931195258128 5
-0.0737754753944908 5
-0.077791756636181 4.7
-0.0779630017834254 4.4
-0.077557637455519 4.1
-0.0727411978748024 3.8
-0.0642108075941522 3.5
-0.0626996295840397 3.2
-0.058826082290169 2.9
-0.0514640796903973 2.6
-0.0494308075418666 2.3
-0.0520993811950412 2
-0.0567612524260783 1.7
-0.058051689922415 1.4
-0.0474802937693589 1.1
-0.0226852723762792 0.8
0.0176954623520883 0.5
0.0799008126976204 0.2
0.173603711004124 -0.1
0.2 -0.162738527122395
0.311669930465164 -0.4
0.482735115969146 -0.7
0.5 -0.726939309752893
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
2.6 -1
2.9 -1
2.94269114714841 -1
3.2 -0.796096541579519
3.31045584206093 -0.7
3.5 -0.532494225874431
3.6426741977422 -0.4
3.8 -0.252988400437954
3.95931162273134 -0.1
4.1 0.0354537581654869
4.26829761436712 0.2
4.4 0.328916709803235
4.5732596732044 0.5
4.7 0.625219940184137
4.87602521036433 0.8
5 0.923134943945064
5 1.1
5 1.33154634793451
4.76722346986633 1.1
4.7 1.03315430857844
4.46464703523205 0.8
4.4 0.735996100930168
4.16006712101184 0.5
4.1 0.440985910225643
3.8519010413039 0.2
3.8 0.149697852960429
3.5371528014742 -0.1
3.5 -0.135139720877302
3.20968697054315 -0.4
3.2 -0.408758664940909
2.9 -0.666167296150191
2.85678220441783 -0.7
2.6 -0.894601825758243
2.43042747809424 -1
2.6 -1
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
0.8 -0.863083643985299
0.981427434921187 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.3 -1
2.43042747809424 -1
2.6 -0.894601825758243
2.85678220441783 -0.7
2.9 -0.666167296150191
3.2 -0.408758664940909
3.20968697054315 -0.4
3.5 -0.135139720877302
3.5371528014742 -0.1
3.8 0.149697852960429
3.8519010413039 0.2
4.1 0.440985910225643
4.16006712101184 0.5
4.4 0.735996100930168
4.46464703523205 0.8
4.7 1.03315430857844
4.76722346986633 1.1
5 1.33154634793451
5 1.4
5 1.68428372574002
4.71447378219196 1.4
4.7 1.38559635989364
4.41219476995073 1.1
4.4 1.08790963848643
4.1081712761223 0.8
4.1 0.791951476144403
3.80107346200311 0.5
3.8 0.498954665081251
3.5 0.210945103771168
3.48838272773469 0.2
3.2 -0.0685054880412507
3.16495865304224 -0.1
2.9 -0.333275331713594
2.81879096677023 -0.4
2.6 -0.573440932424446
2.41561330679806 -0.7
2.3 -0.774896831895921
2 -0.918645120479062
1.7 -0.990889651230554
1.4 -0.975417878210897
1.1 -0.862823333607061
0.88009839615437 -0.7
0.8 -0.639358021793045
0.609663065336627 -0.4
0.5 -0.24517975329092
0.42955539618057 -0.1
0.316063362759587 0.2
0.233419590516514 0.5
0.2 0.675000181607667
0.18100757030554 0.8
0.151396993750372 1.1
0.135789160412266 1.4
0.132253559313444 1.7
0.134630453557111 2
0.136909086964074 2.3
0.136321952617006 2.6
0.134344328378943 2.9
0.133830561592101 3.2
0.132765727552734 3.5
0.131621894745937 3.8
0.12114049822962 4.1
0.117792565267726 4.4
0.118353188571316 4.7
0.119961714446116 5
0.0230931195258128 5
0.0202807159675672 4.7
0.0199147817421502 4.4
0.0217914303870504 4.1
0.0294403484355674 3.8
0.0342774599792909 3.5
0.0355654660040306 3.2
0.0377591230443872 2.9
0.0424289364633042 2.6
0.0437391397111039 2.3
0.0412655361810348 2
0.0377461534436827 1.7
0.0388687352449256 1.4
0.0519583499905063 1.1
0.0791611489646303 0.8
0.122532904132424 0.5
0.189592101203001 0.2
0.2 0.167375676609564
0.300419530171041 -0.1
0.444458654553784 -0.4
0.5 -0.496694954780719
0.662493598074891 -0.7
0.8 -0.863083643985299
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.1 -0.862823333607061
1.4 -0.975417878210897
1.7 -0.990889651230554
2 -0.918645120479062
2.3 -0.774896831895921
2.41561330679806 -0.7
2.6 -0.573440932424446
2.81879096677023 -0.4
2.9 -0.333275331713594
3.16495865304224 -0.1
3.2 -0.0685054880412507
3.48838272773469 0.2
3.5 0.210945103771168
3.8 0.498954665081251
3.80107346200311 0.5
4.1 0.791951476144403
4.1081712761223 0.8
4.4 1.08790963848643
4.41219476995073 1.1
4.7 1.38559635989364
4.71447378219196 1.4
5 1.68428372574002
5 1.7
5 2
5 2.03220722952608
4.96770348272118 2
4.7 1.73330716820139
4.66652866194888 1.7
4.4 1.43524503223021
4.36444718693214 1.4
4.1 1.1386289631717
4.06077371697762 1.1
3.8 0.84448682757774
3.75428925206688 0.8
3.5 0.554561130475585
3.4427362677175 0.5
3.2 0.271835403554159
3.12162423117098 0.2
2.9 0.00140142925116503
2.78100613341484 -0.1
2.6 -0.248448706211929
2.39457920829593 -0.4
2.3 -0.465482803073336
2 -0.629170001091195
1.77983189208023 -0.7
1.7 -0.72259073107037
1.4 -0.725727472750696
1.32286642669031 -0.7
1.1 -0.624947444108682
0.8 -0.402295584820718
0.798174556362214 -0.4
0.587847312913066 -0.1
0.5 0.0533864234363622
0.444293672449464 0.2
0.361427632002915 0.5
0.303842402632213 0.8
0.264671161455444 1.1
0.241370355763102 1.4
0.232478414037315 1.7
0.231665434951785 2
0.231667279662029 2.3
0.230176301200929 2.6
0.22921967750064 2.9
0.229350643493149 3.2
0.228563838958192 3.5
0.229544041227791 3.8
0.218864209403011 4.1
0.214819066453352 4.4
0.215736999422217 4.7
0.216994339254729 5
0.2 5
0.119961714446116 5
0.118353188571316 4.7
0.117792565267726 4.4
0.12114049822962 4.1
0.131621894745937 3.8
0.132765727552734 3.5
0.133830561592101 3.2
0.134344328378943 2.9
0.136321952617006 2.6
0.136909086964074 2.3
0.134630453557111 2
0.132253559313444 1.7
0.135789160412266 1.4
0.151396993750372 1.1
0.18100757030554 0.8
0.2 0.675000181607667
0.233419590516514 0.5
0.316063362759587 0.2
0.42955539618057 -0.1
0.5 -0.24517975329092
0.609663065336627 -0.4
0.8 -0.639358021793045
0.88009839615437 -0.7
1.1 -0.862823333607061
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.4 -0.725727472750696
1.7 -0.72259073107037
1.77983189208023 -0.7
2 -0.629170001091195
2.3 -0.465482803073336
2.39457920829593 -0.4
2.6 -0.248448706211929
2.78100613341484 -0.1
2.9 0.00140142925116504
3.12162423117098 0.2
3.2 0.271835403554159
3.4427362677175 0.5
3.5 0.554561130475585
3.75428925206688 0.8
3.8 0.84448682757774
4.06077371697762 1.1
4.1 1.1386289631717
4.36444718693214 1.4
4.4 1.43524503223021
4.66652866194888 1.7
4.7 1.73330716820139
4.96770348272118 2
5 2.03220722952608
5 2.3
5 2.40769155493629
4.89212324607957 2.3
4.7 2.1084615606003
4.59120013247639 2
4.4 1.80983108186212
4.28954465615569 1.7
4.1 1.51225587359706
3.98657135671727 1.4
3.8 1.216535506006
3.68120199457599 1.1
3.5 0.924075711947814
3.37140239511574 0.8
3.2 0.637325570239639
3.05318266039451 0.5
2.9 0.360435113906408
2.71809514849485 0.2
2.6 0.100143647608089
2.34507998219939 -0.1
2.3 -0.133085177576289
2 -0.316415908215985
1.79504525145987 -0.4
1.7 -0.433551433713132
1.4 -0.456595592880402
1.20216168919354 -0.4
1.1 -0.36891896443937
0.8 -0.126915432228316
0.781133986368736 -0.1
0.610966139827656 0.2
0.5 0.461798473194046
0.489435673489316 0.5
0.431488360073371 0.8
0.391173215928739 1.1
0.363953152176882 1.4
0.347177216431675 1.7
0.337270062409898 2
0.329756824508001 2.3
0.323949157880652 2.6
0.32046542912919 2.9
0.319211516951367 3.2
0.318574828045564 3.5
0.318850210143686 3.8
0.310332306539534 4.1
0.307379697840978 4.4
0.309697688629883 4.7
0.31480702524665 5
0.216994339254729 5
0.215736999422217 4.7
0.214819066453352 4.4
0.218864209403011 4.1
0.229544041227791 3.8
0.228563838958192 3.5
0.229350643493149 3.2
0.22921967750064 2.9
0.230176301200929 2.6
0.231667279662029 2.3
0.231665434951785 2
0.232478414037315 1.7
0.241370355763102 1.4
0.264671161455444 1.1
0.303842402632213 0.8
0.361427632002915 0.5
0.444293672449464 0.2
0.5 0.0533864234363622
0.587847312913066 -0.1
0.798174556362214 -0.4
0.8 -0.402295584820718
1.1 -0.624947444108682
1.32286642669031 -0.7
1.4 -0.725727472750696
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.4 -0.456595592880402
1.7 -0.433551433713132
1.79504525145987 -0.4
2 -0.316415908215985
2.3 -0.133085177576289
2.34507998219939 -0.1
2.6 0.100143647608089
2.71809514849485 0.2
2.9 0.360435113906408
3.05318266039451 0.5
3.2 0.637325570239639
3.37140239511574 0.8
3.5 0.924075711947814
3.68120199457599 1.1
3.8 1.216535506006
3.98657135671727 1.4
4.1 1.51225587359706
4.28954465615569 1.7
4.4 1.80983108186212
4.59120013247639 2
4.7 2.1084615606003
4.89212324607957 2.3
5 2.40769155493629
5 2.6
5 2.84601712709268
4.75397796931874 2.6
4.7 2.5461300567514
4.45381431960235 2.3
4.4 2.24638034354299
4.15340320563898 2
4.1 1.94694671799834
3.85239339412828 1.7
3.8 1.64823124075184
3.55000880078155 1.4
3.5 1.35108006037241
3.24462974928136 1.1
3.2 1.05714085692929
2.9329011202428 0.8
2.9 0.769451854607594
2.60752137040383 0.5
2.6 0.49343394006201
2.3 0.243809352185563
2.24312951111185 0.2
2 0.0345129881983331
1.73175653234501 -0.1
1.7 -0.113647062059893
1.4 -0.15849842083692
1.17870267675984 -0.1
1.1 -0.0760830979193156
0.813305417901699 0.2
0.8 0.217083780461941
0.680799402224583 0.5
0.591264814062583 0.8
0.527535595850996 1.1
0.5 1.26796372787322
0.486535948590661 1.4
0.461876018826034 1.7
0.442874689868011 2
0.427846369353972 2.3
0.417722014560375 2.6
0.411711180757739 2.9
0.409072390409585 3.2
0.408585817132937 3.5
0.408156379059581 3.8
0.401800403676058 4.1
0.399940329228604 4.4
0.40365837783755 4.7
0.412619711238572 5
0.31480702524665 5
0.309697688629883 4.7
0.307379697840978 4.4
0.310332306539534 4.1
0.318850210143686 3.8
0.318574828045564 3.5
0.319211516951367 3.2
0.32046542912919 2.9
0.323949157880652 2.6
0.329756824508001 2.3
0.337270062409898 2
0.347177216431675 1.7
0.363953152176882 1.4
0.391173215928738 1.1
0.431488360073371 0.8
0.489435673489316 0.5
0.5 0.461798473194046
0.610966139827656 0.2
0.781133986368736 -0.1
0.8 -0.126915432228316
1.1 -0.36891896443937
1.20216168919354 -0.4
1.4 -0.456595592880402
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
1.4 -0.15849842083692
1.7 -0.113647062059893
1.73175653234501 -0.1
2 0.0345129881983331
2.24312951111185 0.2
2.3 0.243809352185563
2.6 0.49343394006201
2.60752137040383 0.5
2.9 0.769451854607594
2.9329011202428 0.8
3.2 1.05714085692929
3.24462974928136 1.1
3.5 1.35108006037241
3.55000880078155 1.4
3.8 1.64823124075184
3.85239339412828 1.7
4.1 1.94694671799834
4.15340320563898 2
4.4 2.24638034354299
4.45381431960235 2.3
4.7 2.5461300567514
4.75397796931874 2.6
5 2.84601712709268
5 2.9
5 3.2
5 3.5
5 3.56176602277033
4.94077687879755 3.5
4.7 3.25407966115297
4.64955918850704 3.2
4.4 2.94172300608622
4.36264525914529 2.9
4.1 2.62304797178837
4.08047255972783 2.6
3.80183885682163 2.3
3.8 2.29812845705091
3.52385300076358 2
3.5 1.97559711443156
3.25147649442118 1.7
3.2 1.64722704433559
2.98097994493541 1.4
2.9 1.31760606693522
2.70508121187226 1.1
2.6 0.996246220953655
2.41203661439937 0.8
2.3 0.697499181745943
2.07648249992369 0.5
2 0.441154814873747
1.7 0.259637639377227
1.45937979592938 0.2
1.4 0.187642029077031
1.35794060853084 0.2
1.1 0.296755913195722
0.94069721300464 0.5
0.8 0.760702497842676
0.788266911344679 0.8
0.724608080009246 1.1
0.676950175723418 1.4
0.637704214570928 1.7
0.60119235682289 2
0.5624914730991 2.3
0.530544424535088 2.6
0.508178112653806 2.9
0.5 3.11956829724351
0.498933263867803 3.2
0.49859680622031 3.5
0.497462547975476 3.8
0.493268500812581 4.1
0.492500960616229 4.4
0.497619067045216 4.7
0.5 4.75759166034915
0.521188967864805 5
0.5 5
0.412619711238572 5
0.40365837783755 4.7
0.399940329228604 4.4
0.401800403676058 4.1
0.408156379059581 3.8
0.408585817132937 3.5
0.409072390409585 3.2
0.411711180757739 2.9
0.417722014560375 2.6
0.427846369353972 2.3
0.442874689868011 2
0.461876018826034 1.7
0.486535948590661 1.4
0.5 1.26796372787322
0.527535595850996 1.1
0.591264814062583 0.8
0.680799402224583 0.5
0.8 0.217083780461941
0.813305417901699 0.2
1.1 -0.0760830979193156
1.17870267675984 -0.1
1.4 -0.15849842083692
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
1.4 0.187642029077031
1.45937979592938 0.2
1.7 0.259637639377227
2 0.441154814873747
2.07648249992369 0.5
2.3 0.697499181745943
2.41203661439937 0.8
2.6 0.996246220953655
2.70508121187226 1.1
2.9 1.31760606693522
2.98097994493541 1.4
3.2 1.64722704433559
3.25147649442118 1.7
3.5 1.97559711443156
3.52385300076358 2
3.8 2.29812845705091
3.80183885682163 2.3
4.08047255972783 2.6
4.1 2.62304797178837
4.36264525914529 2.9
4.4 2.94172300608622
4.64955918850704 3.2
4.7 3.25407966115297
4.94077687879755 3.5
5 3.56176602277033
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.13308104360676 5
4.1 4.91453526280494
4.02821743087959 4.7
3.92261807208254 4.4
3.8 4.11145212685522
3.79560032536564 4.1
3.68577895801083 3.8
3.5618177918503 3.5
3.5 3.37115767875257
3.4325540818257 3.2
3.30556442988016 2.9
3.2 2.70248629232815
3.15388391723195 2.6
3.00360088135288 2.3
2.9 2.1351339594942
2.82549530085139 2
2.63158811455604 1.7
2.6 1.65860954027485
2.41587829872791 1.4
2.3 1.25978061724214
2.15905631758052 1.1
2 0.93842126001527
1.81997964623142 0.8
1.7 0.71702039816483
1.4 0.650821291840224
1.1614548553654 0.8
1.1 0.86029868447558
1.00732129596269 1.1
0.925663262058472 1.4
0.868653129903074 1.7
0.830387790337713 2
0.8 2.28563535077439
0.798834025198466 2.3
0.779719720583812 2.6
0.76054033759329 2.9
0.733621778541242 3.2
0.718638299150874 3.5
0.711512783835667 3.8
0.703556506614518 4.1
0.704197696613521 4.4
0.710519438436228 4.7
0.71985374399077 5
0.521188967864805 5
0.5 4.75759166034915
0.497619067045216 4.7
0.492500960616229 4.4
0.493268500812581 4.1
0.497462547975476 3.8
0.49859680622031 3.5
0.498933263867803 3.2
0.5 3.11956829724351
0.508178112653806 2.9
0.530544424535088 2.6
0.5624914730991 2.3
0.60119235682289 2
0.637704214570928 1.7
0.676950175723418 1.4
0.724608080009246 1.1
0.788266911344678 0.8
0.8 0.760702497842676
0.94069721300464 0.5
1.1 0.296755913195722
1.35794060853084 0.2
1.4 0.187642029077031
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
1.4 0.650821291840224
1.7 0.71702039816483
1.81997964623142 0.8
2 0.93842126001527
2.15905631758052 1.1
2.3 1.25978061724214
2.41587829872791 1.4
2.6 1.65860954027485
2.63158811455604 1.7
2.82549530085139 2
2.9 2.1351339594942
3.00360088135288 2.3
3.15388391723195 2.6
3.2 2.70248629232815
3.30556442988016 2.9
3.4325540818257 3.2
3.5 3.37115767875257
3.5618177918503 3.5
3.68577895801083 3.8
3.79560032536564 4.1
3.8 4.11145212685522
3.92261807208254 4.4
4.02821743087959 4.7
4.1 4.91453526280494
4.13308104360676 5
4.1 5
3.8 5
3.68762449054956 5
3.5890657549784 4.7
3.5 4.44322026857283
3.48182734040949 4.4
3.35588984946052 4.1
3.23757275471237 3.8
3.2 3.70949311871752
3.0995197961646 3.5
2.96608775557696 3.2
2.9 3.05383349973355
2.81739132169606 2.9
2.66716339502556 2.6
2.6 2.46998289804514
2.49399094314619 2.3
2.31732257252637 2
2.3 1.97302685785593
2.07902062675943 1.7
2 1.60201492605324
1.72841779969054 1.4
1.7 1.37898913682111
1.57508067123171 1.4
1.4 1.4524727170014
1.28560646766643 1.7
1.18212302914159 2
1.1 2.27079942852522
1.09584419305482 2.3
1.06114564385989 2.6
1.02998332234917 2.9
0.992116660394823 3.2
0.972771567585894 3.5
0.958203414090533 3.8
0.925815619307152 4.1
0.921535637633397 4.4
0.92119403661125 4.7
0.925750733726676 5
0.8 5
0.71985374399077 5
0.710519438436228 4.7
0.704197696613521 4.4
0.703556506614518 4.1
0.711512783835667 3.8
0.718638299150874 3.5
0.733621778541242 3.2
0.76054033759329 2.9
0.779719720583811 2.6
0.798834025198466 2.3
0.8 2.28563535077439
0.830387790337713 2
0.868653129903074 1.7
0.925663262058472 1.4
1.00732129596269 1.1
1.1 0.86029868447558
1.1614548553654 0.8
1.4 0.650821291840224
};
\addplot [draw=none, fill=lavender231240249]
table{%
x  y
1.7 1.37898913682111
1.72841779969054 1.4
2 1.60201492605324
2.07902062675943 1.7
2.3 1.97302685785593
2.31732257252637 2
2.49399094314619 2.3
2.6 2.46998289804514
2.66716339502556 2.6
2.81739132169606 2.9
2.9 3.05383349973355
2.96608775557696 3.2
3.0995197961646 3.5
3.2 3.70949311871752
3.23757275471237 3.8
3.35588984946052 4.1
3.48182734040949 4.4
3.5 4.44322026857283
3.5890657549784 4.7
3.68762449054956 5
3.5 5
3.2 5
2.9 5
2.88135118445627 5
2.79294308012176 4.7
2.68537039798095 4.4
2.6 4.11263276306503
2.5914944986448 4.1
2.42520877718537 3.8
2.3 3.54420675568063
2 3.56993966826576
1.94943492887191 3.8
1.84125730840841 4.1
1.7 4.27067197543831
1.4 4.2264411112437
1.26636751894285 4.4
1.21246190915719 4.7
1.22537611150965 5
1.1 5
0.925750733726676 5
0.92119403661125 4.7
0.921535637633397 4.4
0.925815619307152 4.1
0.958203414090533 3.8
0.972771567585894 3.5
0.992116660394823 3.2
1.02998332234917 2.9
1.06114564385989 2.6
1.09584419305482 2.3
1.1 2.27079942852522
1.18212302914159 2
1.28560646766643 1.7
1.4 1.4524727170014
1.57508067123171 1.4
1.7 1.37898913682111
};
\addplot [draw=none, fill=aliceblue242247253]
table{%
x  y
2 3.56993966826576
2.3 3.54420675568063
2.42520877718537 3.8
2.5914944986448 4.1
2.6 4.11263276306503
2.68537039798095 4.4
2.79294308012176 4.7
2.88135118445627 5
2.6 5
2.3 5
2 5
1.7 5
1.4 5
1.22537611150965 5
1.21246190915719 4.7
1.26636751894285 4.4
1.4 4.2264411112437
1.7 4.27067197543831
1.84125730840841 4.1
1.94943492887191 3.8
2 3.56993966826576
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
1.7 2
};
\addplot [semithick, darkorange25512714, mark=mystar, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2 3.2
};
\draw (axis cs:1.9,2) node[
  scale=0.5,
  anchor=base west,
  text=black,
  rotate=0.0
]{$-0.131$};
\draw (axis cs:2.2,3.2) node[
  scale=0.5,
  anchor=base west,
  text=black,
  rotate=0.0
]{$-0.113$};
\coordinate (CVI_mean_lml_b) at (axis cs:1.6999999999999997,2.0);
\coordinate (CVI_mean_lml_ep_b) at (axis cs:2.0,3.2);
\end{axis}



==> fig/tikz/parkinsons/EP_mean_lml.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 -1
-0.4 -1
-0.34329807719284 -1
-0.4 -0.901329948403741
-0.544393373104068 -0.7
-0.689122140289584 -0.4
-0.7 -0.370371882429084
-0.840277459657959 -0.1
-0.931069408865609 0.2
-0.982131816906032 0.5
-1 0.679211890270218
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.4 -0.901329948403741
-0.34329807719284 -1
-0.1 -1
0.2 -1
0.242426840925684 -1
0.2 -0.937293674575226
0.0305750213000737 -0.7
-0.1 -0.447814173431007
-0.131191243697406 -0.4
-0.287547436276765 -0.1
-0.379517121391696 0.2
-0.4 0.303298863701692
-0.459503217205528 0.5
-0.513551054259658 0.8
-0.543748527256206 1.1
-0.560524192187796 1.4
-0.569801019095525 1.7
-0.574915122339996 2
-0.577729733014973 2.3
-0.579275568285505 2.6
-0.580124757648604 2.9
-0.580591386785393 3.2
-0.58084731916834 3.5
-0.580988108204185 3.8
-0.581065302346975 4.1
-0.581106710262608 4.4
-0.581130827683772 4.7
-0.58114432692538 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.679211890270218
-0.982131816906032 0.5
-0.931069408865609 0.2
-0.840277459657959 -0.1
-0.7 -0.370371882429084
-0.689122140289584 -0.4
-0.544393373104068 -0.7
-0.4 -0.901329948403741
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
0.2 -0.937293674575226
0.242426840925684 -1
0.5 -1
0.555413394470513 -1
0.5 -0.939032555236686
0.321120164913259 -0.7
0.2 -0.510221753263321
0.12921571572247 -0.4
-0.0197734673179264 -0.1
-0.1 0.141222755037454
-0.124942381204387 0.2
-0.212189490672091 0.5
-0.262310761647908 0.8
-0.290777314205623 1.1
-0.30675919153809 1.4
-0.315653321008694 1.7
-0.320574454703634 2
-0.323288196098341 2.3
-0.324781365245956 2.6
-0.325602091280028 2.9
-0.326052368512024 3.2
-0.32629912002411 3.5
-0.326434559207628 3.8
-0.326509001836367 4.1
-0.32654995530981 4.4
-0.326572782885025 4.7
-0.326585354048396 5
-0.4 5
-0.58114432692538 5
-0.581130827683772 4.7
-0.581106710262608 4.4
-0.581065302346975 4.1
-0.580988108204185 3.8
-0.58084731916834 3.5
-0.580591386785393 3.2
-0.580124757648604 2.9
-0.579275568285505 2.6
-0.577729733014973 2.3
-0.574915122339996 2
-0.569801019095525 1.7
-0.560524192187796 1.4
-0.543748527256206 1.1
-0.513551054259658 0.8
-0.459503217205528 0.5
-0.4 0.303298863701692
-0.379517121391696 0.2
-0.287547436276765 -0.1
-0.131191243697406 -0.4
-0.1 -0.447814173431007
0.0305750213000737 -0.7
0.2 -0.937293674575226
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
0.5 -0.939032555236686
0.555413394470513 -1
0.8 -1
0.871327679236925 -1
0.8 -0.946539677342019
0.57376889268283 -0.7
0.5 -0.618452505772925
0.348213973522339 -0.4
0.2 -0.137338024463413
0.179746503224973 -0.1
0.0556117635704417 0.2
-0.0222854467443626 0.5
-0.0698444524677641 0.8
-0.0979268443695853 1.1
-0.1 1.1379208256587
-0.118734204686359 1.4
-0.130679205046216 1.7
-0.137277625136431 2
-0.140912033205852 2.3
-0.142913351112343 2.6
-0.144012937673045 2.9
-0.144614640145352 3.2
-0.144942946842813 3.5
-0.145123415993708 3.8
-0.145222531000965 4.1
-0.145279357907837 4.4
-0.145308816407426 4.7
-0.145325875592773 5
-0.326585354048396 5
-0.326572782885025 4.7
-0.32654995530981 4.4
-0.326509001836367 4.1
-0.326434559207628 3.8
-0.32629912002411 3.5
-0.326052368512024 3.2
-0.325602091280028 2.9
-0.324781365245956 2.6
-0.323288196098341 2.3
-0.320574454703634 2
-0.315653321008694 1.7
-0.30675919153809 1.4
-0.290777314205623 1.1
-0.262310761647908 0.8
-0.212189490672091 0.5
-0.124942381204387 0.2
-0.1 0.141222755037454
-0.0197734673179264 -0.1
0.12921571572247 -0.4
0.2 -0.510221753263321
0.321120164913259 -0.7
0.5 -0.939032555236686
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
3.5 -1
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.5
5 0.589471618781631
4.92151907803033 0.5
4.7 0.251476403601128
4.65350067791099 0.2
4.4 -0.0727896044252133
4.37411912306116 -0.1
4.1 -0.37450033925469
4.07347814588621 -0.4
3.8 -0.642801619368743
3.73074469817407 -0.7
3.5 -0.868952020142315
3.29581239756963 -1
3.5 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.8 -0.946539677342019
0.871327679236925 -1
1.1 -1
1.38249862456712 -1
1.1 -0.873306294989918
0.866484765721406 -0.7
0.8 -0.653235359537488
0.570079996352487 -0.4
0.5 -0.317833864850796
0.367334997669448 -0.1
0.228356110384231 0.2
0.2 0.284842202393179
0.134978619964381 0.5
0.078803200407906 0.8
0.0458758219731935 1.1
0.0270395961638236 1.4
0.0164449880969554 1.7
0.0105481744403242 2
0.00728653275952433 2.3
0.0054870581481901 2.6
0.0044968526926757 2.9
0.0039542437407951 3.2
0.00365738558360686 3.5
0.00349490297078496 3.8
0.00340570794084553 4.1
0.00335439716735357 4.4
0.00332747031697954 4.7
0.00331038713869476 5
-0.1 5
-0.145325875592773 5
-0.145308816407426 4.7
-0.145279357907837 4.4
-0.145222531000965 4.1
-0.145123415993708 3.8
-0.144942946842813 3.5
-0.144614640145351 3.2
-0.144012937673045 2.9
-0.142913351112343 2.6
-0.140912033205852 2.3
-0.137277625136431 2
-0.130679205046216 1.7
-0.118734204686359 1.4
-0.1 1.1379208256587
-0.0979268443695853 1.1
-0.0698444524677641 0.8
-0.0222854467443626 0.5
0.0556117635704417 0.2
0.179746503224973 -0.1
0.2 -0.137338024463413
0.348213973522339 -0.4
0.5 -0.618452505772925
0.57376889268283 -0.7
0.8 -0.946539677342019
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
2.3 -1
2.6 -1
2.9 -1
3.2 -1
3.29581239756963 -1
3.5 -0.868952020142315
3.73074469817407 -0.7
3.8 -0.642801619368743
4.07347814588621 -0.4
4.1 -0.37450033925469
4.37411912306116 -0.1
4.4 -0.0727896044252133
4.65350067791099 0.2
4.7 0.251476403601128
4.92151907803033 0.5
5 0.589471618781631
5 0.8
5 1.1
5 1.35819372439162
4.76118241447812 1.1
4.7 1.03403996211827
4.48135455964079 0.8
4.4 0.713355740157767
4.19714495664974 0.5
4.1 0.398736179763041
3.90509676367222 0.2
3.8 0.094495176475591
3.59849276162794 -0.1
3.5 -0.192584849482227
3.26303119625551 -0.4
3.2 -0.452869586516999
2.9 -0.677225989027872
2.86441166619797 -0.7
2.6 -0.859488111125581
2.3 -0.985929679057267
2.24453986661817 -1
2.3 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
1.1 -0.873306294989918
1.38249862456712 -1
1.4 -1
1.7 -1
2 -1
2.24453986661817 -1
2.3 -0.985929679057267
2.6 -0.859488111125581
2.86441166619797 -0.7
2.9 -0.677225989027872
3.2 -0.452869586516999
3.26303119625551 -0.4
3.5 -0.192584849482227
3.59849276162794 -0.1
3.8 0.094495176475591
3.90509676367222 0.2
4.1 0.398736179763041
4.19714495664974 0.5
4.4 0.713355740157767
4.48135455964079 0.8
4.7 1.03403996211827
4.76118241447812 1.1
5 1.35819372439162
5 1.4
5 1.7
5 1.87360908356253
4.83783464184914 1.7
4.7 1.552661799543
4.55656028247203 1.4
4.4 1.2338212076871
4.27296071621835 1.1
4.1 0.918668924413318
3.98529177979893 0.8
3.8 0.609903267231548
3.69032526597367 0.5
3.5 0.312028591500527
3.38165876375631 0.2
3.2 0.0322324306331707
3.045161671477 -0.1
2.9 -0.219117369999003
2.64454388675202 -0.4
2.6 -0.429767991073804
2.3 -0.584841407134458
2 -0.683350877868963
1.85659488203611 -0.7
1.7 -0.71604616796347
1.56872177185467 -0.7
1.4 -0.6799347789923
1.1 -0.567912845351504
0.853621803281215 -0.4
0.8 -0.363932252440836
0.574740836088327 -0.1
0.5 0.00158949299395905
0.402282360578034 0.2
0.297536943474683 0.5
0.229794167308889 0.8
0.2 1.01603438708835
0.189678488315972 1.1
0.168137759293689 1.4
0.156043297617256 1.7
0.149318481869032 2
0.145600791067011 2.3
0.143551671203109 2.6
0.142424000246787 2.9
0.141805406754276 3.2
0.141465919814555 3.5
0.141281027737406 3.8
0.141179580133892 4.1
0.141121457665797 4.4
0.141090159748641 4.7
0.141068722807189 5
0.00331038713869476 5
0.00332747031697954 4.7
0.00335439716735356 4.4
0.00340570794084553 4.1
0.00349490297078495 3.8
0.00365738558360686 3.5
0.0039542437407951 3.2
0.00449685269267568 2.9
0.0054870581481901 2.6
0.00728653275952433 2.3
0.0105481744403243 2
0.0164449880969554 1.7
0.0270395961638236 1.4
0.0458758219731935 1.1
0.078803200407906 0.8
0.134978619964381 0.5
0.2 0.284842202393179
0.228356110384231 0.2
0.367334997669448 -0.1
0.5 -0.317833864850796
0.570079996352487 -0.4
0.8 -0.653235359537488
0.866484765721406 -0.7
1.1 -0.873306294989918
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.7 -0.71604616796347
1.85659488203611 -0.7
2 -0.683350877868963
2.3 -0.584841407134458
2.6 -0.429767991073804
2.64454388675202 -0.4
2.9 -0.219117369999003
3.045161671477 -0.1
3.2 0.0322324306331707
3.38165876375631 0.2
3.5 0.312028591500527
3.69032526597367 0.5
3.8 0.609903267231548
3.98529177979893 0.8
4.1 0.918668924413318
4.27296071621835 1.1
4.4 1.2338212076871
4.55656028247203 1.4
4.7 1.552661799543
4.83783464184914 1.7
5 1.87360908356253
5 2
5 2.3
5 2.40969948158608
4.89938684523714 2.3
4.7 2.08296502426404
4.62354852639302 2
4.4 1.75811539057996
4.34600762482958 1.7
4.1 1.43657364945195
4.06553595233489 1.4
3.8 1.12076464013691
3.77994638146135 1.1
3.5 0.814726593280346
3.48515573927847 0.8
3.2 0.524905237342599
3.17292399698311 0.5
2.9 0.260684310586918
2.82441221370224 0.2
2.6 0.0331590563399267
2.38759585290831 -0.1
2.3 -0.149243517090544
2 -0.269501253793168
1.7 -0.333375986851175
1.4 -0.331465389426253
1.1 -0.249660090302975
0.868026082072399 -0.1
0.8 -0.0532087289240011
0.61352263630901 0.2
0.5 0.400474230281563
0.463827160492382 0.5
0.39113097509771 0.8
0.346804209647155 1.1
0.320925056623472 1.4
0.306221472764139 1.7
0.297996907695571 2
0.293436133220256 2.3
0.290918728902691 2.6
0.289532144146239 2.9
0.288771023021899 3.2
0.288352267409588 3.5
0.288125829925869 3.8
0.288000184234593 4.1
0.287927333084614 4.4
0.287892715208283 4.7
0.287866316743882 5
0.2 5
0.141068722807189 5
0.141090159748641 4.7
0.141121457665797 4.4
0.141179580133892 4.1
0.141281027737406 3.8
0.141465919814555 3.5
0.141805406754276 3.2
0.142424000246787 2.9
0.143551671203109 2.6
0.145600791067011 2.3
0.149318481869032 2
0.156043297617256 1.7
0.168137759293689 1.4
0.189678488315972 1.1
0.2 1.01603438708835
0.229794167308889 0.8
0.297536943474683 0.5
0.402282360578034 0.2
0.5 0.00158949299395908
0.574740836088327 -0.1
0.8 -0.363932252440836
0.853621803281215 -0.4
1.1 -0.567912845351504
1.4 -0.6799347789923
1.56872177185467 -0.7
1.7 -0.71604616796347
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.1 -0.249660090302975
1.4 -0.331465389426253
1.7 -0.333375986851175
2 -0.269501253793168
2.3 -0.149243517090544
2.38759585290831 -0.1
2.6 0.0331590563399267
2.82441221370224 0.2
2.9 0.260684310586918
3.17292399698311 0.5
3.2 0.524905237342599
3.48515573927847 0.8
3.5 0.814726593280346
3.77994638146135 1.1
3.8 1.12076464013691
4.06553595233489 1.4
4.1 1.43657364945195
4.34600762482958 1.7
4.4 1.75811539057996
4.62354852639302 2
4.7 2.08296502426404
4.89938684523714 2.3
5 2.40969948158608
5 2.6
5 2.9
5 3.2
5 3.20134804241159
4.99891809444487 3.2
4.73987158608921 2.9
4.7 2.8540339875342
4.47964009434104 2.6
4.4 2.50873923846982
4.21792533944032 2.3
4.1 2.16625820425968
3.95366413658403 2
3.8 1.82874262837158
3.68499934695851 1.7
3.5 1.49969510338664
3.40869011104257 1.4
3.2 1.18441603257764
3.11910619924845 1.1
2.9 0.890190429744583
2.80580778190203 0.8
2.6 0.625820262659103
2.44512055126484 0.5
2.3 0.399765405066787
2 0.219713425893975
1.95821377990761 0.2
1.7 0.102811437433233
1.4 0.0540056434541372
1.1 0.103577356395635
0.955963319767001 0.2
0.8 0.324641592797179
0.69948227542238 0.5
0.580743210635291 0.8
0.50757714174497 1.1
0.5 1.15290778743306
0.477121873452546 1.4
0.461262134212912 1.7
0.452375928186049 2
0.447443662999615 2.3
0.444719643015739 2.6
0.443218974944147 2.9
0.442395373168327 3.2
0.441941423138208 3.5
0.441698030426062 3.8
0.44156061482218 4.1
0.441479339110577 4.4
0.441448825791651 4.7
0.441421679458475 5
0.287866316743882 5
0.287892715208283 4.7
0.287927333084614 4.4
0.288000184234593 4.1
0.288125829925869 3.8
0.288352267409588 3.5
0.288771023021899 3.2
0.289532144146239 2.9
0.290918728902691 2.6
0.293436133220256 2.3
0.297996907695571 2
0.306221472764139 1.7
0.320925056623472 1.4
0.346804209647155 1.1
0.39113097509771 0.8
0.463827160492382 0.5
0.5 0.400474230281563
0.61352263630901 0.2
0.8 -0.0532087289240011
0.868026082072399 -0.1
1.1 -0.249660090302975
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
4.4 4.90409372987003
4.7 4.76897972572884
5 4.891150477443
5 5
4.7 5
4.4 5
4.37707080341979 5
4.4 4.90409372987003
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.1 0.103577356395635
1.4 0.0540056434541372
1.7 0.102811437433233
1.95821377990761 0.2
2 0.219713425893975
2.3 0.399765405066787
2.44512055126484 0.5
2.6 0.625820262659103
2.80580778190203 0.8
2.9 0.890190429744583
3.11910619924845 1.1
3.2 1.18441603257764
3.40869011104257 1.4
3.5 1.49969510338664
3.68499934695851 1.7
3.8 1.82874262837158
3.95366413658403 2
4.1 2.16625820425968
4.21792533944032 2.3
4.4 2.50873923846982
4.47964009434104 2.6
4.7 2.8540339875342
4.73987158608921 2.9
4.99891809444487 3.2
5 3.20134804241159
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 4.891150477443
4.7 4.76897972572884
4.4 4.90409372987003
4.37707080341979 5
4.1 5
3.8 5
3.67270770900557 5
3.62183327902492 4.7
3.56513632411119 4.4
3.5 4.10781979995267
3.49836162430043 4.1
3.43765874700452 3.8
3.37650698791409 3.5
3.30676431212138 3.2
3.21398889711215 2.9
3.2 2.86113836990173
3.12984291104183 2.6
3.01934109321786 2.3
2.9 2.07219653504709
2.86966126436518 2
2.70763095996602 1.7
2.6 1.55010138235191
2.50568501641721 1.4
2.3 1.14722762393689
2.26224694840304 1.1
2 0.836978626421816
1.95699511615503 0.8
1.7 0.620308136632781
1.4 0.502005999346113
1.1 0.54114510689435
0.862033110586477 0.8
0.8 0.907166659508274
0.749176953194605 1.1
0.701774966816214 1.4
0.67472729544217 1.7
0.659601883799886 2
0.651225594517795 2.3
0.646607313724235 2.6
0.644067680695232 2.9
0.64267238673761 3.2
0.641904513008744 3.5
0.641488758748172 3.8
0.641277566493062 4.1
0.641149813637217 4.4
0.641072807663562 4.7
0.641040780836066 5
0.5 5
0.441421679458475 5
0.441448825791651 4.7
0.441479339110577 4.4
0.44156061482218 4.1
0.441698030426062 3.8
0.441941423138208 3.5
0.442395373168326 3.2
0.443218974944147 2.9
0.444719643015739 2.6
0.447443662999615 2.3
0.452375928186049 2
0.461262134212912 1.7
0.477121873452546 1.4
0.5 1.15290778743306
0.50757714174497 1.1
0.580743210635291 0.8
0.69948227542238 0.5
0.8 0.324641592797179
0.955963319767001 0.2
1.1 0.103577356395635
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.1 0.54114510689435
1.4 0.502005999346113
1.7 0.620308136632781
1.95699511615503 0.8
2 0.836978626421816
2.26224694840304 1.1
2.3 1.14722762393689
2.50568501641721 1.4
2.6 1.55010138235191
2.70763095996602 1.7
2.86966126436518 2
2.9 2.07219653504709
3.01934109321786 2.3
3.12984291104183 2.6
3.2 2.86113836990173
3.21398889711215 2.9
3.30676431212138 3.2
3.37650698791409 3.5
3.43765874700452 3.8
3.49836162430043 4.1
3.5 4.10781979995267
3.56513632411119 4.4
3.62183327902492 4.7
3.67270770900557 5
3.5 5
3.2 5
3.01889537438775 5
2.99348420551071 4.7
2.95900553907814 4.4
2.91513657011169 4.1
2.9 4.02045914978919
2.85269995195936 3.8
2.77906237882258 3.5
2.69896925774185 3.2
2.60856912043295 2.9
2.6 2.87605649498908
2.49411745890114 2.6
2.37113193313386 2.3
2.3 2.15061208185546
2.21893650196528 2
2.0427836541897 1.7
2 1.63755564492979
1.7961027583091 1.4
1.7 1.30104347018171
1.4 1.14116949621178
1.1 1.3100245013302
1.06563296512483 1.4
0.99894055607306 1.7
0.962764604527992 2
0.943176730036651 2.3
0.932536232132951 2.6
0.926738194872232 2.9
0.923572066245933 3.2
0.921831306948891 3.5
0.920886335368333 3.8
0.920410527475587 4.1
0.920130786573023 4.4
0.919931814982588 4.7
0.919918571755725 5
0.8 5
0.641040780836066 5
0.641072807663562 4.7
0.641149813637217 4.4
0.641277566493062 4.1
0.641488758748172 3.8
0.641904513008744 3.5
0.64267238673761 3.2
0.644067680695232 2.9
0.646607313724235 2.6
0.651225594517795 2.3
0.659601883799886 2
0.67472729544217 1.7
0.701774966816214 1.4
0.749176953194605 1.1
0.8 0.907166659508274
0.862033110586477 0.8
1.1 0.54114510689435
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.1 1.3100245013302
1.4 1.14116949621178
1.7 1.30104347018171
1.7961027583091 1.4
2 1.63755564492979
2.0427836541897 1.7
2.21893650196528 2
2.3 2.15061208185546
2.37113193313386 2.3
2.49411745890114 2.6
2.6 2.87605649498908
2.60856912043295 2.9
2.69896925774185 3.2
2.77906237882258 3.5
2.85269995195936 3.8
2.9 4.02045914978919
2.91513657011169 4.1
2.95900553907814 4.4
2.99348420551071 4.7
3.01889537438775 5
2.9 5
2.6 5
2.3 5
2 5
1.7 5
1.4 5
1.1 5
0.919918571755725 5
0.919931814982588 4.7
0.920130786573023 4.4
0.920410527475587 4.1
0.920886335368333 3.8
0.921831306948891 3.5
0.923572066245933 3.2
0.926738194872232 2.9
0.932536232132951 2.6
0.943176730036651 2.3
0.962764604527992 2
0.99894055607306 1.7
1.06563296512483 1.4
1.1 1.3100245013302
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
1.7 5
};
\coordinate (EP_mean_lml_t) at (axis cs:1.6999999999999997,5.0);
\end{axis}



==> fig/tikz/parkinsons/EP_nlpd.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 -1
-0.462977445185488 -1
-0.619204346305965 -0.7
-0.7 -0.43675509978454
-0.71905949141394 -0.4
-0.844176696433607 -0.1
-0.91376937736936 0.2
-0.952470460166789 0.5
-0.973928955222299 0.8
-0.985781431874338 1.1
-0.992312896438304 1.4
-0.995902481970698 1.7
-0.997878655424666 2
-0.998963893815676 2.3
-0.999555763807554 2.6
-0.999883734410392 2.9
-1 3.08741190626057
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.4 -1
-0.1 -1
-0.0267376431262537 -1
-0.1 -0.832932278235846
-0.179079492729512 -0.7
-0.313688210234026 -0.4
-0.396159683282895 -0.1
-0.4 -0.0811958983198747
-0.496304231792295 0.2
-0.555358455188459 0.5
-0.588633673856492 0.8
-0.607257174305914 1.1
-0.617597849176599 1.4
-0.623320434366396 1.7
-0.626479949145692 2
-0.628218109509337 2.3
-0.629161347752053 2.6
-0.629681025691614 2.9
-0.629998984936503 3.2
-0.630126843481917 3.5
-0.630226567557312 3.8
-0.630271153126006 4.1
-0.630291317456911 4.4
-0.630312220861989 4.7
-0.630285919450859 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 3.08741190626057
-0.999883734410392 2.9
-0.999555763807554 2.6
-0.998963893815676 2.3
-0.997878655424666 2
-0.995902481970698 1.7
-0.992312896438304 1.4
-0.985781431874338 1.1
-0.973928955222299 0.8
-0.952470460166789 0.5
-0.91376937736936 0.2
-0.844176696433607 -0.1
-0.71905949141394 -0.4
-0.7 -0.43675509978454
-0.619204346305965 -0.7
-0.462977445185488 -1
-0.4 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
-0.1 -0.832932278235846
-0.0267376431262537 -1
0.2 -1
0.203103728128659 -1
0.2 -0.994659964887947
0.026495070402654 -0.7
-0.0938332088651013 -0.4
-0.1 -0.381665198931812
-0.221559575158676 -0.1
-0.300987768602906 0.2
-0.349208823298014 0.5
-0.37804860692142 0.8
-0.394897665435407 1.1
-0.4 1.25764847151692
-0.408044876937971 1.4
-0.417581184062925 1.7
-0.422829119008205 2
-0.425694492883283 2.3
-0.427293156010895 2.6
-0.428146024784639 2.9
-0.428640075435279 3.2
-0.428883875577184 3.5
-0.429039406029432 3.8
-0.429108607341045 4.1
-0.429166814480387 4.4
-0.429165635900314 4.7
-0.429184444467578 5
-0.630285919450859 5
-0.630312220861989 4.7
-0.630291317456911 4.4
-0.630271153126006 4.1
-0.630226567557312 3.8
-0.630126843481917 3.5
-0.629998984936503 3.2
-0.629681025691614 2.9
-0.629161347752053 2.6
-0.628218109509337 2.3
-0.626479949145692 2
-0.623320434366396 1.7
-0.617597849176599 1.4
-0.607257174305914 1.1
-0.588633673856492 0.8
-0.555358455188459 0.5
-0.496304231792295 0.2
-0.4 -0.0811958983198747
-0.396159683282895 -0.1
-0.313688210234026 -0.4
-0.179079492729512 -0.7
-0.1 -0.832932278235846
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
0.2 -0.994659964887947
0.203103728128659 -1
0.370099439546107 -1
0.2 -0.707340030420407
0.195677962352913 -0.7
0.0422396668341959 -0.4
-0.0639299152525823 -0.1
-0.1 0.0368299274098587
-0.153448037982617 0.2
-0.216540999737023 0.5
-0.253549710222118 0.8
-0.274888138835766 1.1
-0.286969685075757 1.4
-0.293735989626585 1.7
-0.29748071389181 2
-0.299555866367914 2.3
-0.300705205353416 2.6
-0.301340266564244 2.9
-0.301674612216768 3.2
-0.301855688893427 3.5
-0.30196382922024 3.8
-0.302011212071202 4.1
-0.302044414071524 4.4
-0.302051981437025 4.7
-0.302078417878437 5
-0.4 5
-0.429184444467578 5
-0.429165635900315 4.7
-0.429166814480387 4.4
-0.429108607341045 4.1
-0.429039406029432 3.8
-0.428883875577184 3.5
-0.428640075435279 3.2
-0.428146024784639 2.9
-0.427293156010895 2.6
-0.425694492883283 2.3
-0.422829119008205 2
-0.417581184062925 1.7
-0.408044876937971 1.4
-0.4 1.25764847151692
-0.394897665435407 1.1
-0.37804860692142 0.8
-0.349208823298014 0.5
-0.300987768602906 0.2
-0.221559575158676 -0.1
-0.1 -0.381665198931812
-0.0938332088651013 -0.4
0.026495070402654 -0.7
0.2 -0.994659964887947
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.2 -0.707340030420407
0.370099439546107 -1
0.5 -1
0.541718770011135 -1
0.5 -0.95037099052468
0.339534663286232 -0.7
0.2 -0.442170485961017
0.178312542533493 -0.4
0.0548064613415225 -0.1
-0.0299305673118086 0.2
-0.0871871988287335 0.5
-0.1 0.602753985830592
-0.129050813522815 0.8
-0.154878612236124 1.1
-0.169426822045351 1.4
-0.177542842740621 1.7
-0.182018153612705 2
-0.184516506439669 2.3
-0.185886608520439 2.6
-0.186665216788137 2.9
-0.187045000643792 3.2
-0.187264388931613 3.5
-0.187390050031929 3.8
-0.187444383689269 4.1
-0.187473971156541 4.4
-0.18749330766976 4.7
-0.187533776557727 5
-0.302078417878437 5
-0.302051981437025 4.7
-0.302044414071524 4.4
-0.302011212071202 4.1
-0.30196382922024 3.8
-0.301855688893427 3.5
-0.301674612216768 3.2
-0.301340266564244 2.9
-0.300705205353416 2.6
-0.299555866367914 2.3
-0.29748071389181 2
-0.293735989626585 1.7
-0.286969685075758 1.4
-0.274888138835766 1.1
-0.253549710222118 0.8
-0.216540999737023 0.5
-0.153448037982617 0.2
-0.1 0.0368299274098587
-0.0639299152525822 -0.1
0.0422396668341959 -0.4
0.195677962352913 -0.7
0.2 -0.707340030420407
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.289687158413563
4.90896763284922 0.2
4.7 -0.0052121765293414
4.60262327254439 -0.1
4.4 -0.295855091972646
4.29059065233739 -0.4
4.1 -0.578543908243871
3.96681913580492 -0.7
3.8 -0.846598447114944
3.61682558985325 -1
3.8 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
0.5 -0.95037099052468
0.541718770011135 -1
0.729529184485935 -1
0.5 -0.726950097793526
0.4827274058075 -0.7
0.311642547510009 -0.4
0.2 -0.162858947798061
0.173542837935627 -0.1
0.0799412495694319 0.2
0.0182177131158802 0.5
-0.0209200918325735 0.8
-0.04464382918693 1.1
-0.0584917636693226 1.4
-0.0663765683808375 1.7
-0.0707729975419627 2
-0.0732493063398115 2.3
-0.074608355718263 2.6
-0.0753902908458025 2.9
-0.0757624672483075 3.2
-0.0759795778643714 3.5
-0.076100967272202 3.8
-0.07615540385633 4.1
-0.0761808408617825 4.4
-0.0762061578343341 4.7
-0.07625377601654 5
-0.1 5
-0.187533776557727 5
-0.18749330766976 4.7
-0.187473971156541 4.4
-0.187444383689269 4.1
-0.187390050031929 3.8
-0.187264388931614 3.5
-0.187045000643792 3.2
-0.186665216788137 2.9
-0.185886608520439 2.6
-0.184516506439669 2.3
-0.182018153612705 2
-0.177542842740621 1.7
-0.169426822045351 1.4
-0.154878612236124 1.1
-0.129050813522815 0.8
-0.1 0.602753985830592
-0.0871871988287335 0.5
-0.0299305673118086 0.2
0.0548064613415225 -0.1
0.178312542533493 -0.4
0.2 -0.442170485961017
0.339534663286232 -0.7
0.5 -0.95037099052468
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
3.2 -1
3.5 -1
3.61682558985325 -1
3.8 -0.846598447114944
3.96681913580492 -0.7
4.1 -0.578543908243871
4.29059065233739 -0.4
4.4 -0.295855091972646
4.60262327254439 -0.1
4.7 -0.00521217652934142
4.90896763284922 0.2
5 0.289687158413563
5 0.5
5 0.8
5 0.92313740798343
4.87602278768383 0.8
4.7 0.625222399454868
4.57325917648142 0.5
4.4 0.328916235351615
4.26829612215651 0.2
4.1 0.0354555117506015
3.95930921797121 -0.1
3.8 -0.252985679294881
3.64267133308535 -0.4
3.5 -0.532490775081275
3.3104542904374 -0.7
3.2 -0.79609522798472
2.9426883790154 -1
3.2 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
0.5 -0.726950097793526
0.729529184485935 -1
0.8 -1
0.981426647837354 -1
0.8 -0.863083319756415
0.662490643366555 -0.7
0.5 -0.496695553351211
0.444452504625046 -0.4
0.300443167688201 -0.1
0.2 0.16802488021787
0.189813066450673 0.2
0.123622625060494 0.5
0.0822287718247756 0.8
0.057354859432228 1.1
0.0429088677576482 1.4
0.0347044558264794 1.7
0.030129511112171 2
0.0275729407497837 2.3
0.0261601409442277 2.6
0.0253643128480255 2.9
0.0249581472982045 3.2
0.0247464571825936 3.5
0.0246284978728007 3.8
0.0245655962298932 4.1
0.0245323308255222 4.4
0.0245052455328499 4.7
0.0244465433836109 5
-0.07625377601654 5
-0.0762061578343341 4.7
-0.0761808408617824 4.4
-0.07615540385633 4.1
-0.076100967272202 3.8
-0.0759795778643714 3.5
-0.0757624672483075 3.2
-0.0753902908458025 2.9
-0.074608355718263 2.6
-0.0732493063398114 2.3
-0.0707729975419627 2
-0.0663765683808375 1.7
-0.0584917636693226 1.4
-0.0446438291869301 1.1
-0.0209200918325735 0.8
0.0182177131158802 0.5
0.0799412495694319 0.2
0.173542837935627 -0.1
0.2 -0.162858947798061
0.311642547510009 -0.4
0.4827274058075 -0.7
0.5 -0.726950097793526
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
2.6 -1
2.9 -1
2.9426883790154 -1
3.2 -0.79609522798472
3.3104542904374 -0.7
3.5 -0.532490775081275
3.64267133308535 -0.4
3.8 -0.25298567929488
3.95930921797121 -0.1
4.1 0.0354555117506015
4.26829612215651 0.2
4.4 0.328916235351615
4.57325917648142 0.5
4.7 0.625222399454868
4.87602278768383 0.8
5 0.92313740798343
5 1.1
5 1.33155838549471
4.76721188965617 1.1
4.7 1.03316580521861
4.4646356162636 0.8
4.4 0.736006594623566
4.16005723043474 0.5
4.1 0.440996386668106
3.85188945215533 0.2
3.8 0.149709276873277
3.53714081720049 -0.1
3.5 -0.135128373079285
3.20968312834873 -0.4
3.2 -0.4087552807266
2.9 -0.666165544434876
2.85678048577662 -0.7
2.6 -0.894600044699672
2.43042571511517 -1
2.6 -1
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
0.8 -0.863083319756415
0.981426647837354 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.3 -1
2.43042571511517 -1
2.6 -0.894600044699671
2.85678048577662 -0.7
2.9 -0.666165544434876
3.2 -0.4087552807266
3.20968312834873 -0.4
3.5 -0.135128373079285
3.53714081720049 -0.1
3.8 0.149709276873277
3.85188945215534 0.2
4.1 0.440996386668106
4.16005723043474 0.5
4.4 0.736006594623566
4.4646356162636 0.8
4.7 1.03316580521861
4.76721188965617 1.1
5 1.33155838549471
5 1.4
5 1.68431328253693
4.71444474713589 1.4
4.7 1.38562522629023
4.41216826686338 1.1
4.4 1.0879359075702
4.10814198611025 0.8
4.1 0.791980304294838
3.80104612738665 0.5
3.8 0.498981287054021
3.5 0.210967673187943
3.48835922463386 0.2
3.2 -0.0684895316417944
3.16494279380518 -0.1
2.9 -0.333265580198973
2.81878172502425 -0.4
2.6 -0.573435036921117
2.41560798509715 -0.7
2.3 -0.774893442139838
2 -0.918642080576515
1.7 -0.99088774472876
1.4 -0.97541537997319
1.1 -0.862817497772067
0.880106046952056 -0.7
0.8 -0.639338104015451
0.609690393887284 -0.4
0.5 -0.24497906206995
0.42968416573645 -0.1
0.316653718636402 0.2
0.235479749099939 0.5
0.2 0.698051326992424
0.185377635482125 0.8
0.159353548051386 1.1
0.144309499184619 1.4
0.135785480033796 1.7
0.131032019766305 2
0.128395187839379 2.3
0.126928637606718 2.6
0.126118916541854 2.9
0.125678761844716 3.2
0.125472492229559 3.5
0.125357963017803 3.8
0.125286596316116 4.1
0.125245502512827 4.4
0.125216648900034 4.7
0.125146862783762 5
0.0244465433836109 5
0.0245052455328499 4.7
0.0245323308255222 4.4
0.0245655962298932 4.1
0.0246284978728007 3.8
0.0247464571825936 3.5
0.0249581472982044 3.2
0.0253643128480255 2.9
0.0261601409442277 2.6
0.0275729407497837 2.3
0.0301295111121711 2
0.0347044558264793 1.7
0.0429088677576482 1.4
0.057354859432228 1.1
0.0822287718247756 0.8
0.123622625060494 0.5
0.189813066450673 0.2
0.2 0.16802488021787
0.300443167688201 -0.1
0.444452504625046 -0.4
0.5 -0.49669555335121
0.662490643366555 -0.7
0.8 -0.863083319756415
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.1 -0.862817497772067
1.4 -0.97541537997319
1.7 -0.99088774472876
2 -0.918642080576514
2.3 -0.774893442139838
2.41560798509715 -0.7
2.6 -0.573435036921117
2.81878172502426 -0.4
2.9 -0.333265580198973
3.16494279380518 -0.1
3.2 -0.0684895316417944
3.48835922463386 0.2
3.5 0.210967673187943
3.8 0.498981287054021
3.80104612738665 0.5
4.1 0.791980304294838
4.10814198611025 0.8
4.4 1.0879359075702
4.41216826686338 1.1
4.7 1.38562522629023
4.71444474713589 1.4
5 1.68431328253693
5 1.7
5 2
5 2.03226982371445
4.96764061380945 2
4.7 1.73337169421081
4.6664639488351 1.7
4.4 1.43531238959514
4.36437678150728 1.4
4.1 1.13869980418457
4.06070267990497 1.1
3.8 0.844559057050787
3.7542160971527 0.8
3.5 0.554627613044648
3.44266915460839 0.5
3.2 0.27189040624882
3.12156997701519 0.2
2.9 0.00144059182277606
2.7809711453693 -0.1
2.6 -0.248423644473177
2.39455287691139 -0.4
2.3 -0.465464864298334
2 -0.629153711987658
1.77979406360806 -0.7
1.7 -0.72257962181301
1.4 -0.725714472671277
1.32290807744577 -0.7
1.1 -0.624909956038429
0.8 -0.402210656310366
0.798242197441118 -0.4
0.588181177087876 -0.1
0.5 0.0550926783426439
0.44522843913699 0.2
0.364313960181572 0.5
0.310916701159924 0.8
0.277941054757254 1.1
0.258518000519843 1.4
0.247401709250475 1.7
0.241161824796056 2
0.237706049963283 2.3
0.235776056641138 2.6
0.234729396101363 2.9
0.234125369053197 3.2
0.233864045022491 3.5
0.233722740855359 3.8
0.233627713066835 4.1
0.23354766547288 4.4
0.233534713296517 4.7
0.233421215823805 5
0.2 5
0.125146862783762 5
0.125216648900034 4.7
0.125245502512827 4.4
0.125286596316116 4.1
0.125357963017803 3.8
0.125472492229559 3.5
0.125678761844716 3.2
0.126118916541854 2.9
0.126928637606718 2.6
0.128395187839379 2.3
0.131032019766305 2
0.135785480033796 1.7
0.144309499184619 1.4
0.159353548051386 1.1
0.185377635482125 0.8
0.2 0.698051326992424
0.235479749099939 0.5
0.316653718636402 0.2
0.42968416573645 -0.1
0.5 -0.24497906206995
0.609690393887284 -0.4
0.8 -0.639338104015451
0.880106046952056 -0.7
1.1 -0.862817497772067
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.4 -0.725714472671277
1.7 -0.72257962181301
1.77979406360806 -0.7
2 -0.629153711987658
2.3 -0.465464864298334
2.39455287691139 -0.4
2.6 -0.248423644473177
2.7809711453693 -0.1
2.9 0.00144059182277603
3.12156997701519 0.2
3.2 0.27189040624882
3.44266915460839 0.5
3.5 0.554627613044648
3.7542160971527 0.8
3.8 0.844559057050787
4.06070267990497 1.1
4.1 1.13869980418457
4.36437678150728 1.4
4.4 1.43531238959514
4.6664639488351 1.7
4.7 1.73337169421081
4.96764061380945 2
5 2.03226982371445
5 2.3
5 2.40785077937003
4.89197128371109 2.3
4.7 2.10861375179069
4.59104413555941 2
4.4 1.80998551741057
4.28937269423049 1.7
4.1 1.51244075634275
3.98638169633572 1.4
3.8 1.21671792566012
3.68102937310018 1.1
3.5 0.924239430377538
3.37122391811051 0.8
3.2 0.637488710639907
3.05302557146337 0.5
2.9 0.360569660823058
2.71796338361638 0.2
2.6 0.10024822452413
2.34497453672107 -0.1
2.3 -0.133007699677224
2 -0.316332601601697
1.79487119567055 -0.4
1.7 -0.433486461179458
1.4 -0.456514811883581
1.20254735067582 -0.4
1.1 -0.368737800723599
0.8 -0.126298591612985
0.781589605744055 -0.1
0.612758380029763 0.2
0.5 0.47456128180874
0.493148171263207 0.5
0.440154068462146 0.8
0.407518814367291 1.1
0.388330847763193 1.4
0.37736828511237 1.7
0.37121952685518 2
0.36782043869769 2.3
0.365937517000138 2.6
0.364937366997296 2.9
0.364322692343248 3.2
0.36406185918833 3.5
0.363933876594177 3.8
0.363859543733027 4.1
0.363704227646663 4.4
0.363792397244436 4.7
0.363629881675718 5
0.233421215823805 5
0.233534713296517 4.7
0.23354766547288 4.4
0.233627713066835 4.1
0.233722740855359 3.8
0.233864045022491 3.5
0.234125369053197 3.2
0.234729396101363 2.9
0.235776056641138 2.6
0.237706049963283 2.3
0.241161824796056 2
0.247401709250475 1.7
0.258518000519843 1.4
0.277941054757254 1.1
0.310916701159924 0.8
0.364313960181572 0.5
0.44522843913699 0.2
0.5 0.0550926783426439
0.588181177087876 -0.1
0.798242197441118 -0.4
0.8 -0.402210656310366
1.1 -0.624909956038429
1.32290807744577 -0.7
1.4 -0.725714472671277
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.4 -0.456514811883581
1.7 -0.433486461179458
1.79487119567055 -0.4
2 -0.316332601601697
2.3 -0.133007699677224
2.34497453672107 -0.1
2.6 0.10024822452413
2.71796338361638 0.2
2.9 0.360569660823058
3.05302557146337 0.5
3.2 0.637488710639907
3.37122391811051 0.8
3.5 0.924239430377538
3.68102937310018 1.1
3.8 1.21671792566012
3.98638169633572 1.4
4.1 1.51244075634275
4.28937269423049 1.7
4.4 1.80998551741057
4.59104413555941 2
4.7 2.10861375179069
4.89197128371109 2.3
5 2.40785077937003
5 2.6
5 2.84645775542229
4.75351645627975 2.6
4.7 2.54658636242834
4.45339759486712 2.3
4.4 2.24679754500039
4.15297964861885 2
4.1 1.94737679080191
3.85188262070094 1.7
3.8 1.64873771315799
3.5495799964856 1.4
3.5 1.351493555089
3.2441593280119 1.1
3.2 1.05759665782289
2.93248390343859 0.8
2.9 0.769835804679738
2.60715004489403 0.5
2.6 0.493757529947416
2.3 0.244205805171589
2.2426150686435 0.2
2 0.0349062954814148
1.73100554746268 -0.1
1.7 -0.113318699167674
1.4 -0.158060991409965
1.18116213662651 -0.1
1.1 -0.0750964899631812
0.817020791799995 0.2
0.8 0.222647131800148
0.686839602920919 0.5
0.605862296265673 0.8
0.556341751834511 1.1
0.527477816743436 1.4
0.511090850644273 1.7
0.501930088097536 2
0.5 2.11466960147239
0.497934827432096 2.3
0.496098977359138 2.6
0.495145337893227 2.9
0.4945200156333 3.2
0.494259673354169 3.5
0.494145012332995 3.8
0.49409137439922 4.1
0.493860789820447 4.4
0.494050081192354 4.7
0.493838547527631 5
0.363629881675718 5
0.363792397244436 4.7
0.363704227646663 4.4
0.363859543733027 4.1
0.363933876594177 3.8
0.36406185918833 3.5
0.364322692343248 3.2
0.364937366997296 2.9
0.365937517000138 2.6
0.36782043869769 2.3
0.37121952685518 2
0.37736828511237 1.7
0.388330847763193 1.4
0.407518814367291 1.1
0.440154068462146 0.8
0.493148171263207 0.5
0.5 0.47456128180874
0.612758380029763 0.2
0.781589605744055 -0.1
0.8 -0.126298591612985
1.1 -0.368737800723599
1.20254735067582 -0.4
1.4 -0.456514811883581
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
1.4 -0.158060991409965
1.7 -0.113318699167674
1.73100554746268 -0.1
2 0.0349062954814148
2.2426150686435 0.2
2.3 0.244205805171589
2.6 0.493757529947416
2.60715004489403 0.5
2.9 0.769835804679738
2.93248390343859 0.8
3.2 1.05759665782289
3.2441593280119 1.1
3.5 1.351493555089
3.5495799964856 1.4
3.8 1.64873771315799
3.85188262070094 1.7
4.1 1.94737679080191
4.15297964861885 2
4.4 2.24679754500039
4.45339759486712 2.3
4.7 2.54658636242834
4.75351645627975 2.6
5 2.84645775542229
5 2.9
5 3.2
5 3.5
5 3.56676035034804
4.93598556527765 3.5
4.7 3.25873138549407
4.64522848417877 3.2
4.4 2.94643818910698
4.35840659160175 2.9
4.1 2.62749652512196
4.07673382838115 2.6
3.8 2.30081060032573
3.79935575356604 2.3
3.52170471288019 2
3.5 1.97780198477251
3.2493431392816 1.7
3.2 1.64938848415701
2.97908228129857 1.4
2.9 1.31955346265432
2.70325316695858 1.1
2.6 0.998052222749989
2.41023501066828 0.8
2.3 0.699198261130518
2.07446092850599 0.5
2 0.442743266656254
1.7 0.261519754760501
1.45021327178377 0.2
1.4 0.189650445146263
1.36533418432541 0.2
1.1 0.303252245544786
0.950785710270327 0.5
0.805192538120151 0.8
0.8 0.81815833898391
0.753142620283511 1.1
0.724073583273361 1.4
0.707609896702471 1.7
0.698467153557125 2
0.693465911628691 2.3
0.690618847336176 2.6
0.689345930866454 2.9
0.688419704138026 3.2
0.687948967161019 3.5
0.687669301413851 3.8
0.68751917777333 4.1
0.687626792175488 4.4
0.687315226454934 4.7
0.687156066878178 5
0.5 5
0.493838547527631 5
0.494050081192354 4.7
0.493860789820447 4.4
0.49409137439922 4.1
0.494145012332995 3.8
0.494259673354169 3.5
0.4945200156333 3.2
0.495145337893227 2.9
0.496098977359138 2.6
0.497934827432096 2.3
0.5 2.11466960147239
0.501930088097536 2
0.511090850644273 1.7
0.527477816743436 1.4
0.556341751834511 1.1
0.605862296265673 0.8
0.686839602920919 0.5
0.8 0.222647131800148
0.817020791799995 0.2
1.1 -0.0750964899631812
1.18116213662651 -0.1
1.4 -0.158060991409965
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
1.4 0.189650445146263
1.45021327178377 0.2
1.7 0.261519754760501
2 0.442743266656254
2.07446092850599 0.5
2.3 0.699198261130518
2.41023501066828 0.8
2.6 0.998052222749989
2.70325316695858 1.1
2.9 1.31955346265432
2.97908228129857 1.4
3.2 1.64938848415701
3.2493431392816 1.7
3.5 1.97780198477251
3.52170471288019 2
3.79935575356604 2.3
3.8 2.30081060032573
4.07673382838115 2.6
4.1 2.62749652512196
4.35840659160175 2.9
4.4 2.94643818910698
4.64522848417877 3.2
4.7 3.25873138549407
4.93598556527765 3.5
5 3.56676035034804
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.11770144017766 5
4.1 4.95473373890912
4.01220979556807 4.7
3.90467230936323 4.4
3.8 4.15286212093802
3.77949671815168 4.1
3.66955143439975 3.8
3.54455045051803 3.5
3.5 3.40558606710574
3.42007134073308 3.2
3.29220531412152 2.9
3.2 2.72569842854231
3.14381824356978 2.6
2.99322393180767 2.3
2.9 2.15069161842178
2.81718109076699 2
2.62341110370431 1.7
2.6 1.66925666065445
2.40818237869302 1.4
2.3 1.26891610322785
2.15068296536427 1.1
2 0.947086034889244
1.80742565213699 0.8
1.7 0.726227286485678
1.4 0.666933769178102
1.20770960052633 0.8
1.1 0.934550224432722
1.04827931799563 1.1
0.995021919056638 1.4
0.966082030870646 1.7
0.950513070259199 2
0.942147205115834 2.3
0.937478842563093 2.6
0.935365817114842 2.9
0.93407003363625 3.2
0.933241213759339 3.5
0.933014243637521 3.8
0.932763601910273 4.1
0.932809084868851 4.4
0.932062703388684 4.7
0.930975798597903 5
0.8 5
0.687156066878178 5
0.687315226454934 4.7
0.687626792175488 4.4
0.68751917777333 4.1
0.687669301413851 3.8
0.687948967161019 3.5
0.688419704138026 3.2
0.689345930866454 2.9
0.690618847336176 2.6
0.693465911628691 2.3
0.698467153557125 2
0.707609896702471 1.7
0.724073583273361 1.4
0.753142620283511 1.1
0.8 0.81815833898391
0.805192538120151 0.8
0.950785710270327 0.5
1.1 0.303252245544786
1.36533418432541 0.2
1.4 0.189650445146263
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
1.4 0.666933769178102
1.7 0.726227286485678
1.80742565213699 0.8
2 0.947086034889244
2.15068296536427 1.1
2.3 1.26891610322785
2.40818237869302 1.4
2.6 1.66925666065445
2.62341110370431 1.7
2.81718109076699 2
2.9 2.15069161842178
2.99322393180767 2.3
3.14381824356978 2.6
3.2 2.72569842854231
3.29220531412152 2.9
3.42007134073308 3.2
3.5 3.40558606710574
3.54455045051803 3.5
3.66955143439975 3.8
3.77949671815168 4.1
3.8 4.15286212093802
3.90467230936323 4.4
4.01220979556807 4.7
4.1 4.95473373890912
4.11770144017766 5
4.1 5
3.8 5
3.6165861167538 5
3.52910410757483 4.7
3.5 4.6103192420603
3.4140589354633 4.4
3.29978002150301 4.1
3.2 3.81934255056711
3.19100705772001 3.8
3.05050461736539 3.5
2.92921596556896 3.2
2.9 3.13285522994601
2.77672801656671 2.9
2.63569229169964 2.6
2.6 2.52945676516988
2.45546205737174 2.3
2.3 2.0272244645154
2.27669491970272 2
2.03437988018354 1.7
2 1.657289845662
1.7 1.47214904574396
1.44652345808205 1.7
1.4 1.82409812203469
1.37633161265924 2
1.35577847919037 2.3
1.34545966182491 2.6
1.33999868508035 2.9
1.33727889795318 3.2
1.33580618313814 3.5
1.33516063192043 3.8
1.33438055265011 4.1
1.33491754823083 4.4
1.33511820573293 4.7
1.33374369339377 5
1.1 5
0.930975798597903 5
0.932062703388684 4.7
0.932809084868851 4.4
0.932763601910273 4.1
0.933014243637521 3.8
0.933241213759339 3.5
0.93407003363625 3.2
0.935365817114842 2.9
0.937478842563093 2.6
0.942147205115834 2.3
0.950513070259199 2
0.966082030870646 1.7
0.995021919056638 1.4
1.04827931799563 1.1
1.1 0.934550224432722
1.20770960052633 0.8
1.4 0.666933769178102
};
\addplot [draw=none, fill=lavender231240249]
table{%
x  y
1.7 1.47214904574396
2 1.657289845662
2.03437988018354 1.7
2.27669491970272 2
2.3 2.0272244645154
2.45546205737174 2.3
2.6 2.52945676516988
2.63569229169964 2.6
2.77672801656671 2.9
2.9 3.13285522994601
2.92921596556896 3.2
3.05050461736538 3.5
3.19100705772001 3.8
3.2 3.81934255056711
3.29978002150301 4.1
3.4140589354633 4.4
3.5 4.6103192420603
3.52910410757483 4.7
3.6165861167538 5
3.5 5
3.2 5
2.9 5
2.6 5
2.3 5
2 5
1.7 5
1.4 5
1.33374369339377 5
1.33511820573293 4.7
1.33491754823083 4.4
1.33438055265011 4.1
1.33516063192043 3.8
1.33580618313814 3.5
1.33727889795318 3.2
1.33999868508035 2.9
1.34545966182491 2.6
1.35577847919037 2.3
1.37633161265924 2
1.4 1.82409812203469
1.44652345808205 1.7
1.7 1.47214904574396
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
1.7 5
};
\coordinate (MCMC_mean_lml_t) at (axis cs:1.6999999999999997,4.7);
\end{axis}



==> fig/tikz/parkinsons/LA_mean_lml.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=black]
table{%
x  y
-0.772459884962436 1.7
-0.7 1.7311815580608
-0.4 1.99254702494831
-0.39537960154668 2
-0.21387530043062 2.3
-0.1 2.506133312273
-0.0661412451193169 2.6
0.0323442915485077 2.9
0.118332352927821 3.2
0.193548510468204 3.5
0.2 3.52836957273263
0.254828647504395 3.8
0.307718656171473 4.1
0.355644944031644 4.4
0.397218701723194 4.7
0.434285597476358 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.59657930595309
-0.772459884962436 1.7
};
\addplot [draw=none, fill=midnightblue854116]
table{%
x  y
-0.894780052667948 1.4
-0.7 1.48584431981862
-0.460890545153886 1.7
-0.4 1.75274880028399
-0.246719054763248 2
-0.1 2.25107042422871
-0.0812872756719281 2.3
0.0259203300134342 2.6
0.11996652497444 2.9
0.2 3.19168041134574
0.202041679395627 3.2
0.268741061209295 3.5
0.32640460235753 3.8
0.376561156386708 4.1
0.422781864902654 4.4
0.46230987449056 4.7
0.497559772676115 5
0.434285597476358 5
0.397218701723194 4.7
0.355644944031644 4.4
0.307718656171473 4.1
0.254828647504395 3.8
0.2 3.52836957273263
0.193548510468204 3.5
0.118332352927821 3.2
0.0323442915485077 2.9
-0.0661412451193169 2.6
-0.1 2.506133312273
-0.21387530043062 2.3
-0.39537960154668 2
-0.4 1.99254702494831
-0.7 1.7311815580608
-0.772459884962436 1.7
-1 1.59657930595309
-1 1.4
-1 1.34749867189479
-0.894780052667948 1.4
};
\addplot [draw=none, fill=midnightblue868137]
table{%
x  y
-0.929002183510206 1.1
-0.7 1.21053019388643
-0.508115720417348 1.4
-0.4 1.49622661128542
-0.277139992196704 1.7
-0.1 1.99655625898311
-0.0986493163006022 2
0.0160032009927434 2.3
0.117981905146186 2.6
0.2 2.87341997577781
0.207157538262323 2.9
0.280409108623257 3.2
0.343459976643842 3.5
0.397980557210665 3.8
0.445403656601943 4.1
0.489918785773665 4.4
0.5 4.47887564695998
0.53240938109724 4.7
0.571597598525436 5
0.5 5
0.497559772676115 5
0.46230987449056 4.7
0.422781864902654 4.4
0.376561156386708 4.1
0.32640460235753 3.8
0.268741061209295 3.5
0.202041679395627 3.2
0.2 3.19168041134574
0.11996652497444 2.9
0.0259203300134342 2.6
-0.0812872756719281 2.3
-0.1 2.25107042422871
-0.246719054763248 2
-0.4 1.75274880028399
-0.460890545153886 1.7
-0.7 1.48584431981862
-0.894780052667948 1.4
-1 1.34749867189479
-1 1.1
-1 1.05738546505945
-0.929002183510206 1.1
};
\addplot [draw=none, fill=teal882156]
table{%
x  y
-0.813233712250118 0.8
-0.7 0.865654379772521
-0.505783877512551 1.1
-0.4 1.20436139222724
-0.294058225757821 1.4
-0.11963289560404 1.7
-0.1 1.73286811747668
0.00477288435564172 2
0.113293677657415 2.3
0.2 2.56728143891274
0.209567438386022 2.6
0.289800765953635 2.9
0.358776537850887 3.2
0.41817889207839 3.5
0.4695565120638 3.8
0.5 4.00181163492201
0.517374757994295 4.1
0.567843857331041 4.4
0.609397848159339 4.7
0.646067185839152 5
0.571597598525436 5
0.53240938109724 4.7
0.5 4.47887564695998
0.489918785773665 4.4
0.445403656601943 4.1
0.397980557210665 3.8
0.343459976643842 3.5
0.280409108623257 3.2
0.207157538262323 2.9
0.2 2.87341997577781
0.117981905146186 2.6
0.0160032009927434 2.3
-0.0986493163006022 2
-0.1 1.99655625898311
-0.277139992196704 1.7
-0.4 1.49622661128542
-0.508115720417348 1.4
-0.7 1.21053019388643
-0.929002183510206 1.1
-1 1.05738546505945
-1 0.8
-1 0.647912648695088
-0.813233712250118 0.8
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 -1
-0.4 -1
-0.337696777644427 -1
-0.4 -0.883800331564835
-0.52298565079611 -0.7
-0.647860383812798 -0.4
-0.692181854950971 -0.1
-0.669771874851978 0.2
-0.579235322006379 0.5
-0.417639047160486 0.8
-0.4 0.821677607397284
-0.280766193764738 1.1
-0.126336523417773 1.4
-0.1 1.44563015338239
-0.00323728869485466 1.7
0.108195085011886 2
0.2 2.26724730718544
0.21019501316749 2.3
0.297265469680009 2.6
0.372443993644948 2.9
0.437143967078517 3.2
0.492897807512937 3.5
0.5 3.54257839329321
0.550318337109634 3.8
0.601335772625249 4.1
0.647675095064793 4.4
0.686386315221438 4.7
0.720536773152868 5
0.646067185839152 5
0.609397848159339 4.7
0.567843857331041 4.4
0.517374757994295 4.1
0.5 4.00181163492201
0.4695565120638 3.8
0.41817889207839 3.5
0.358776537850887 3.2
0.289800765953635 2.9
0.209567438386022 2.6
0.2 2.56728143891274
0.113293677657415 2.3
0.00477288435564174 2
-0.1 1.73286811747668
-0.11963289560404 1.7
-0.294058225757821 1.4
-0.4 1.20436139222724
-0.505783877512551 1.1
-0.7 0.865654379772521
-0.813233712250118 0.8
-1 0.647912648695088
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.4 -0.883800331564835
-0.337696777644427 -1
-0.1 -1
0.2 -1
0.2441935381235 -1
0.2 -0.933483259775818
0.0363441633049308 -0.7
-0.1 -0.416468270269399
-0.109972390467757 -0.4
-0.245278282320638 -0.1
-0.297524401836472 0.2
-0.28425886371783 0.5
-0.21484963904584 0.8
-0.100940385619632 1.1
-0.1 1.1018495869388
5.48705900608876e-05 1.4
0.107304158557957 1.7
0.2 1.96456098891184
0.211332888353739 2
0.30390847014137 2.3
0.384963500973996 2.6
0.455087221336261 2.9
0.5 3.11990738770221
0.519134148424911 3.2
0.583025707715436 3.5
0.637878925987447 3.8
0.685296787256203 4.1
0.727506332798544 4.4
0.763374782283537 4.7
0.795006360466583 5
0.720536773152868 5
0.686386315221438 4.7
0.647675095064793 4.4
0.601335772625249 4.1
0.550318337109634 3.8
0.5 3.54257839329321
0.492897807512937 3.5
0.437143967078517 3.2
0.372443993644948 2.9
0.297265469680009 2.6
0.21019501316749 2.3
0.2 2.26724730718544
0.108195085011886 2
-0.00323728869485468 1.7
-0.1 1.44563015338239
-0.126336523417773 1.4
-0.280766193764738 1.1
-0.4 0.821677607397284
-0.417639047160486 0.8
-0.579235322006379 0.5
-0.669771874851978 0.2
-0.692181854950971 -0.1
-0.647860383812798 -0.4
-0.52298565079611 -0.7
-0.4 -0.883800331564835
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
0.2 -0.933483259775818
0.2441935381235 -1
0.5 -1
0.556937214193981 -1
0.5 -0.936607868620544
0.32512133729214 -0.7
0.2 -0.495561241702584
0.141193568174964 -0.4
0.00613447495549785 -0.1
-0.063152084927334 0.2
-0.0770033576263265 0.5
-0.0429536344519094 0.8
0.0272630807090672 1.1
0.118747461643071 1.4
0.2 1.64275249913837
0.217663683232832 1.7
0.312223258687888 2
0.39762192711525 2.3
0.472661532267983 2.6
0.5 2.72172671290119
0.546814459732253 2.9
0.615804621728844 3.2
0.674772106583379 3.5
0.72543951486526 3.8
0.769257801887157 4.1
0.8 4.33980278381937
0.810528387319905 4.4
0.8579477295622 4.7
0.899768794169388 5
0.8 5
0.795006360466583 5
0.763374782283537 4.7
0.727506332798544 4.4
0.685296787256203 4.1
0.637878925987447 3.8
0.583025707715436 3.5
0.519134148424911 3.2
0.5 3.11990738770221
0.455087221336261 2.9
0.384963500973996 2.6
0.30390847014137 2.3
0.211332888353739 2
0.2 1.96456098891184
0.107304158557957 1.7
5.48705900608737e-05 1.4
-0.1 1.1018495869388
-0.100940385619632 1.1
-0.21484963904584 0.8
-0.28425886371783 0.5
-0.297524401836472 0.2
-0.245278282320638 -0.1
-0.109972390467757 -0.4
-0.1 -0.416468270269399
0.0363441633049308 -0.7
0.2 -0.933483259775818
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
0.5 -0.936607868620544
0.556937214193981 -1
0.8 -1
0.872965268102551 -1
0.8 -0.944809553456646
0.577688105026448 -0.7
0.5 -0.611574316158006
0.357460838945897 -0.4
0.204094231818636 -0.1
0.2 -0.0883386261260229
0.106570320363601 0.2
0.074599200672895 0.5
0.0955993411751715 0.8
0.155195172728946 1.1
0.2 1.25783876127685
0.237657317853371 1.4
0.327078243269465 1.7
0.413113629022038 2
0.49133538408913 2.3
0.5 2.33552800358125
0.575462825098307 2.6
0.649354931807498 2.9
0.712475095032778 3.2
0.766518505451323 3.5
0.8 3.71324405173898
0.81845715044658 3.8
0.875487888888053 4.1
0.925075046515754 4.4
0.96847666221874 4.7
1.00670855053048 5
0.899768794169388 5
0.8579477295622 4.7
0.810528387319905 4.4
0.8 4.33980278381937
0.769257801887157 4.1
0.72543951486526 3.8
0.674772106583379 3.5
0.615804621728844 3.2
0.546814459732253 2.9
0.5 2.72172671290119
0.472661532267983 2.6
0.39762192711525 2.3
0.312223258687888 2
0.217663683232832 1.7
0.2 1.64275249913837
0.118747461643071 1.4
0.0272630807090672 1.1
-0.0429536344519094 0.8
-0.0770033576263265 0.5
-0.0631520849273341 0.2
0.00613447495549782 -0.1
0.141193568174964 -0.4
0.2 -0.495561241702584
0.32512133729214 -0.7
0.5 -0.936607868620544
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
3.5 -1
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.5
5 0.589603943489993
4.92140286908942 0.5
4.7 0.251604488602233
4.65338464158573 0.2
4.4 -0.0726672083157395
4.37400233302927 -0.1
4.1 -0.374385172807172
4.07335776555334 -0.4
3.8 -0.642694282695919
3.73061269150594 -0.7
3.5 -0.868852008930525
3.29564924190242 -1
3.5 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.8 -0.944809553456646
0.872965268102551 -1
1.1 -1
1.3840784943225 -1
1.1 -0.871594425932914
0.871151411714666 -0.7
0.8 -0.648760207787633
0.580227012511391 -0.4
0.5 -0.298759994706989
0.387993437215595 -0.1
0.27574281418879 0.2
0.226870720674374 0.5
0.235220900587806 0.8
0.2849114600903 1.1
0.357038683697208 1.4
0.436492803306098 1.7
0.5 1.94210314505208
0.517936916219335 2
0.607419993532091 2.3
0.685104790786305 2.6
0.751895403882744 2.9
0.8 3.14965408186636
0.81303001988082 3.2
0.882827466906642 3.5
0.942773001615848 3.8
0.994581851476129 4.1
1.0396217057116 4.4
1.07900559487528 4.7
1.1 4.87943534863876
1.12161160466686 5
1.1 5
1.00670855053048 5
0.96847666221874 4.7
0.925075046515754 4.4
0.875487888888053 4.1
0.81845715044658 3.8
0.8 3.71324405173898
0.766518505451323 3.5
0.712475095032778 3.2
0.649354931807499 2.9
0.575462825098307 2.6
0.5 2.33552800358125
0.49133538408913 2.3
0.413113629022038 2
0.327078243269465 1.7
0.237657317853371 1.4
0.2 1.25783876127685
0.155195172728946 1.1
0.0955993411751715 0.8
0.074599200672895 0.5
0.106570320363601 0.2
0.2 -0.0883386261260229
0.204094231818636 -0.1
0.357460838945897 -0.4
0.5 -0.611574316158006
0.577688105026448 -0.7
0.8 -0.944809553456646
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
2.3 -1
2.6 -1
2.9 -1
3.2 -1
3.29564924190242 -1
3.5 -0.868852008930525
3.73061269150594 -0.7
3.8 -0.642694282695919
4.07335776555334 -0.4
4.1 -0.374385172807172
4.37400233302927 -0.1
4.4 -0.0726672083157395
4.65338464158573 0.2
4.7 0.251604488602233
4.92140286908942 0.5
5 0.589603943489993
5 0.8
5 1.1
5 1.35806197345755
4.7612812657916 1.1
4.7 1.03393791206495
4.48142229467689 0.8
4.4 0.713289897123053
4.19717176793322 0.5
4.1 0.398715969881764
3.90506822189354 0.2
3.8 0.094532023698685
3.59839107737397 -0.1
3.5 -0.192482206475605
3.26283996485765 -0.4
3.2 -0.452705030842276
2.9 -0.677040779454552
2.86410987802061 -0.7
2.6 -0.8592690888479
2.3 -0.985696188304485
2.24356468711583 -1
2.3 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
1.1 -0.871594425932914
1.3840784943225 -1
1.4 -1
1.7 -1
2 -1
2.24356468711583 -1
2.3 -0.985696188304485
2.6 -0.8592690888479
2.86410987802061 -0.7
2.9 -0.677040779454552
3.2 -0.452705030842276
3.26283996485765 -0.4
3.5 -0.192482206475605
3.59839107737397 -0.1
3.8 0.094532023698685
3.90506822189354 0.2
4.1 0.398715969881764
4.19717176793322 0.5
4.4 0.713289897123053
4.48142229467689 0.8
4.7 1.03393791206495
4.7612812657916 1.1
5 1.35806197345755
5 1.4
5 1.7
5 1.87297671148061
4.83843320543848 1.7
4.7 1.55203522724538
4.55716158170118 1.4
4.4 1.23320382220737
4.27355638915074 1.1
4.1 0.918081742444561
3.98584354344191 0.8
3.8 0.609406116503203
3.69073466666389 0.5
3.5 0.311735245436953
3.38176469974129 0.2
3.2 0.0322630960323436
3.04483260871058 -0.1
2.9 -0.218761400094902
2.64376360845783 -0.4
2.6 -0.429230119431574
2.3 -0.584137949577895
2 -0.68246939051007
1.84699990902459 -0.7
1.7 -0.714853080614815
1.58128958052776 -0.7
1.4 -0.677786294813093
1.1 -0.563425196227594
0.866930132616892 -0.4
0.8 -0.352174112987115
0.599166934985939 -0.1
0.5 0.0624731177272731
0.444241874844144 0.2
0.382343870469929 0.5
0.378109027591365 0.8
0.415589412247604 1.1
0.476420049541045 1.4
0.5 1.49602375813105
0.559943599270071 1.7
0.64716158083072 2
0.725783733898005 2.3
0.794746756474303 2.6
0.8 2.62483446740155
0.877882156848327 2.9
0.950759917320029 3.2
1.01325112253299 3.5
1.06708885278511 3.8
1.1 4.00924041502383
1.12117046144473 4.1
1.18455925223864 4.4
1.24083973949196 4.7
1.29094687504187 5
1.12161160466686 5
1.1 4.87943534863876
1.07900559487528 4.7
1.0396217057116 4.4
0.994581851476129 4.1
0.942773001615848 3.8
0.882827466906642 3.5
0.81303001988082 3.2
0.8 3.14965408186636
0.751895403882744 2.9
0.685104790786305 2.6
0.607419993532091 2.3
0.517936916219335 2
0.5 1.94210314505208
0.436492803306098 1.7
0.357038683697208 1.4
0.2849114600903 1.1
0.235220900587806 0.8
0.226870720674374 0.5
0.27574281418879 0.2
0.387993437215595 -0.1
0.5 -0.298759994706989
0.580227012511391 -0.4
0.8 -0.648760207787633
0.871151411714666 -0.7
1.1 -0.871594425932914
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.7 -0.714853080614815
1.84699990902459 -0.7
2 -0.68246939051007
2.3 -0.584137949577895
2.6 -0.429230119431574
2.64376360845783 -0.4
2.9 -0.218761400094902
3.04483260871058 -0.1
3.2 0.0322630960323436
3.38176469974129 0.2
3.5 0.311735245436953
3.69073466666389 0.5
3.8 0.609406116503203
3.98584354344191 0.8
4.1 0.918081742444561
4.27355638915074 1.1
4.4 1.23320382220737
4.55716158170118 1.4
4.7 1.55203522724538
4.83843320543848 1.7
5 1.87297671148061
5 2
5 2.3
5 2.40823882115354
4.9007848312331 2.3
4.7 2.08138971678273
4.62507755763012 2
4.4 1.75635479363743
4.34772973713397 1.7
4.1 1.43455946748216
4.06750279707156 1.4
3.8 1.11853001946892
3.78212045863925 1.1
3.5 0.812656468702458
3.48718515762088 0.8
3.2 0.523850001348982
3.17381386427297 0.5
2.9 0.261179978599984
2.82319847040735 0.2
2.6 0.034776922199653
2.38416404300033 -0.1
2.3 -0.147164508326973
2 -0.266559159474679
1.7 -0.329228885520862
1.4 -0.324995411866916
1.1 -0.237627749806718
0.90198193694063 -0.1
0.8 -0.01836302637132
0.663699402163638 0.2
0.555288826051729 0.5
0.530020581348224 0.8
0.563992764687012 1.1
0.628355926872602 1.4
0.702811803052148 1.7
0.776386245442105 2
0.8 2.09864801719704
0.864495513365567 2.3
0.950494635148531 2.6
1.02458822134941 2.9
1.08848981475924 3.2
1.1 3.25991601724196
1.16657127096896 3.5
1.24031580197559 3.8
1.30553053912884 4.1
1.36337173558725 4.4
1.4 4.61233420826537
1.42380083187117 4.7
1.49777783274946 5
1.4 5
1.29094687504187 5
1.24083973949196 4.7
1.18455925223864 4.4
1.12117046144473 4.1
1.1 4.00924041502383
1.06708885278511 3.8
1.01325112253299 3.5
0.95075991732003 3.2
0.877882156848327 2.9
0.8 2.62483446740155
0.794746756474303 2.6
0.725783733898005 2.3
0.64716158083072 2
0.559943599270071 1.7
0.5 1.49602375813105
0.476420049541045 1.4
0.415589412247604 1.1
0.378109027591365 0.8
0.382343870469929 0.5
0.444241874844144 0.2
0.5 0.0624731177272731
0.599166934985939 -0.1
0.8 -0.352174112987115
0.866930132616892 -0.4
1.1 -0.563425196227594
1.4 -0.677786294813093
1.58128958052776 -0.7
1.7 -0.714853080614815
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.1 -0.237627749806718
1.4 -0.324995411866916
1.7 -0.329228885520862
2 -0.266559159474679
2.3 -0.147164508326973
2.38416404300033 -0.1
2.6 0.034776922199653
2.82319847040735 0.2
2.9 0.261179978599984
3.17381386427297 0.5
3.2 0.523850001348982
3.48718515762088 0.8
3.5 0.812656468702458
3.78212045863925 1.1
3.8 1.11853001946892
4.06750279707156 1.4
4.1 1.43455946748216
4.34772973713397 1.7
4.4 1.75635479363743
4.62507755763012 2
4.7 2.08138971678273
4.9007848312331 2.3
5 2.40823882115354
5 2.6
5 2.9
5 3.1959523546639
4.74469484613678 2.9
4.7 2.84841328631667
4.48533356343283 2.6
4.4 2.50200158325352
4.22487858810536 2.3
4.1 2.15784998694717
3.96224386184336 2
3.8 1.81824447765594
3.69512327867661 1.7
3.5 1.48798372659679
3.41869715318512 1.4
3.2 1.17588190580447
3.12468479451514 1.1
2.9 0.889849607774607
2.80288926970009 0.8
2.6 0.631980965170255
2.43455321329086 0.5
2.3 0.408321097573832
2 0.230658172214139
1.93240963021519 0.2
1.7 0.115991799063942
1.4 0.0734648979416278
1.1 0.137865687040976
1.02201324550762 0.2
0.8 0.455772342806742
0.782591978823036 0.5
0.734314197467165 0.8
0.74473449375978 1.1
0.788304564402034 1.4
0.8 1.4558373198844
0.870584244252085 1.7
0.95769608849652 2
1.03741435699253 2.3
1.1 2.56094433369485
1.11321669179933 2.6
1.20855738776443 2.9
1.29167278652428 3.2
1.36536949926876 3.5
1.4 3.65486854398797
1.45097623105201 3.8
1.54701807486551 4.1
1.63019902441883 4.4
1.7 4.67854553270892
1.70872509889745 4.7
1.82764482438438 5
1.7 5
1.49777783274946 5
1.42380083187117 4.7
1.4 4.61233420826537
1.36337173558725 4.4
1.30553053912884 4.1
1.24031580197559 3.8
1.16657127096896 3.5
1.1 3.25991601724196
1.08848981475924 3.2
1.02458822134941 2.9
0.950494635148531 2.6
0.864495513365567 2.3
0.8 2.09864801719704
0.776386245442105 2
0.702811803052148 1.7
0.628355926872602 1.4
0.563992764687012 1.1
0.530020581348224 0.8
0.555288826051729 0.5
0.663699402163638 0.2
0.8 -0.01836302637132
0.90198193694063 -0.1
1.1 -0.237627749806718
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
4.4 4.7083436614896
4.7 4.71431332036197
5 4.85477336509839
5 5
4.7 5
4.4 5
4.27570671475516 5
4.4 4.7083436614896
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.1 0.137865687040976
1.4 0.0734648979416278
1.7 0.115991799063942
1.93240963021519 0.2
2 0.230658172214139
2.3 0.408321097573832
2.43455321329086 0.5
2.6 0.631980965170255
2.80288926970009 0.8
2.9 0.889849607774607
3.12468479451514 1.1
3.2 1.17588190580447
3.41869715318512 1.4
3.5 1.48798372659679
3.69512327867662 1.7
3.8 1.81824447765594
3.96224386184336 2
4.1 2.15784998694717
4.22487858810536 2.3
4.4 2.50200158325352
4.48533356343283 2.6
4.7 2.84841328631667
4.74469484613678 2.9
5 3.1959523546639
5 3.2
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 4.85477336509839
4.7 4.71431332036197
4.4 4.7083436614896
4.27570671475516 5
4.1 5
3.8 5
3.5 5
3.40252217131995 5
3.45343564971624 4.7
3.45332067557052 4.4
3.43134623940275 4.1
3.39785838499487 3.8
3.35624079310121 3.5
3.30368698957537 3.2
3.2296877499671 2.9
3.2 2.80728870063055
3.15006382411932 2.6
3.04125222504554 2.3
2.9 2.04939795766798
2.87531176428428 2
2.69164827776869 1.7
2.6 1.58179524857312
2.47796221718545 1.4
2.3 1.1888122043216
2.22594061324934 1.1
2 0.879984285714497
1.89937788744153 0.8
1.7 0.669677644892016
1.4 0.578094135312274
1.1 0.718964783073244
1.06153724131718 0.8
1.01848350257405 1.1
1.04097114088593 1.4
1.09134262172359 1.7
1.1 1.73899282102904
1.18473395540795 2
1.27528547691459 2.3
1.35719666885572 2.6
1.4 2.76528503308784
1.45493488985671 2.9
1.56880411186108 3.2
1.67070462199257 3.5
1.7 3.59184995460553
1.80001861211045 3.8
1.93038264121725 4.1
2 4.27010000421775
2.08391062834727 4.4
2.27408184126154 4.7
2.3 4.74083635642235
2.49724726447817 5
2.3 5
2 5
1.82764482438438 5
1.70872509889745 4.7
1.7 4.67854553270892
1.63019902441883 4.4
1.54701807486551 4.1
1.45097623105201 3.8
1.4 3.65486854398797
1.36536949926876 3.5
1.29167278652428 3.2
1.20855738776443 2.9
1.11321669179933 2.6
1.1 2.56094433369485
1.03741435699253 2.3
0.95769608849652 2
0.870584244252085 1.7
0.8 1.4558373198844
0.788304564402034 1.4
0.74473449375978 1.1
0.734314197467165 0.8
0.782591978823036 0.5
0.8 0.455772342806742
1.02201324550762 0.2
1.1 0.137865687040976
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.1 0.718964783073244
1.4 0.578094135312274
1.7 0.669677644892016
1.89937788744153 0.8
2 0.879984285714497
2.22594061324934 1.1
2.3 1.1888122043216
2.47796221718545 1.4
2.6 1.58179524857312
2.69164827776869 1.7
2.87531176428428 2
2.9 2.04939795766798
3.04125222504554 2.3
3.15006382411932 2.6
3.2 2.80728870063055
3.2296877499671 2.9
3.30368698957537 3.2
3.35624079310121 3.5
3.39785838499487 3.8
3.43134623940275 4.1
3.45332067557052 4.4
3.45343564971624 4.7
3.40252217131995 5
3.2 5
2.9 5
2.6 5
2.49724726447817 5
2.3 4.74083635642235
2.27408184126154 4.7
2.08391062834727 4.4
2 4.27010000421775
1.93038264121725 4.1
1.80001861211045 3.8
1.7 3.59184995460553
1.67070462199257 3.5
1.56880411186108 3.2
1.45493488985671 2.9
1.4 2.76528503308784
1.35719666885572 2.6
1.27528547691459 2.3
1.18473395540795 2
1.1 1.73899282102904
1.09134262172359 1.7
1.04097114088593 1.4
1.01848350257405 1.1
1.06153724131718 0.8
1.1 0.718964783073244

1.66520108871867 1.7
1.645965220111 2
1.69442064729974 2.3
1.7 2.32035195862854
1.85812136321933 2.6
1.97748441382511 2.9
2 2.95253609619867
2.24051828104952 3.2
2.3 3.28756001743155
2.49396539679901 3.2
2.42557237926231 2.9
2.34489447184889 2.6
2.3 2.48053119580333
2.20100957016369 2.3
2.05492064173572 2
2 1.90377617524186
1.75671603481736 1.7
1.7 1.64814715687143
1.66520108871867 1.7

2.57682500522606 3.5
2.6 3.53788383172416
2.60671008353094 3.5
2.6 3.41873007057282
2.57682500522606 3.5
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.7 1.64814715687143
1.75671603481736 1.7
2 1.90377617524186
2.05492064173572 2
2.20100957016369 2.3
2.3 2.48053119580333
2.34489447184889 2.6
2.42557237926231 2.9
2.49396539679901 3.2
2.3 3.28756001743155
2.24051828104952 3.2
2 2.95253609619867
1.97748441382511 2.9
1.85812136321933 2.6
1.7 2.32035195862854
1.69442064729974 2.3
1.645965220111 2
1.66520108871867 1.7
1.7 1.64814715687143
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
2.6 3.41873007057282
2.60671008353094 3.5
2.6 3.53788383172416
2.57682500522606 3.5
2.6 3.41873007057282
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2 2.3
};
\coordinate (LA_mean_lml_t) at (axis cs:2.0,2.3);
\end{axis}



==> fig/tikz/parkinsons/LA_nlpd.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 -1
-0.455694782976736 -1
-0.61112244168742 -0.7
-0.698132582660652 -0.4
-0.7 -0.391224249679828
-0.815269219547046 -0.1
-0.876452051818132 0.2
-0.902050364641805 0.5
-0.904033012988572 0.8
-0.888138879029881 1.1
-0.856414768918915 1.4
-0.808466368809077 1.7
-0.742020664160229 2
-0.7 2.15627256073835
-0.680114280421231 2.3
-0.630587700461568 2.6
-0.565929004563796 2.9
-0.481605123002026 3.2
-0.4 3.43539119747744
-0.38497772958158 3.5
-0.309147134569726 3.8
-0.210119623515117 4.1
-0.1 4.3640361928344
-0.0851517499908406 4.4
0.0452496841878621 4.7
0.2 4.97741887542292
0.216348350884391 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.4 -1
-0.1 -1
-0.0212732948109916 -1
-0.1 -0.813662566383539
-0.166004115026487 -0.7
-0.297557936476125 -0.4
-0.374877067814499 -0.1
-0.4 0.0623466157846053
-0.437675744095722 0.2
-0.475474252098531 0.5
-0.477318611047455 0.8
-0.451231479042152 1.1
-0.4 1.399754456032
-0.399974747750666 1.4
-0.358286163497074 1.7
-0.300857329507489 2
-0.224447022281811 2.3
-0.124143639754818 2.6
-0.1 2.66569907729652
-0.0169961358575289 2.9
0.115012995722929 3.2
0.2 3.3659201467006
0.287145065552571 3.5
0.5 3.78796342584856
0.510576865824403 3.8
0.781733705818006 4.1
0.8 4.11969797430092
1.04235946076651 4.4
1.1 4.46450730657905
1.2652805006217 4.7
1.4 4.87669640584839
1.47498256026639 5
1.4 5
1.1 5
0.8 5
0.5 5
0.216348350884391 5
0.2 4.97741887542292
0.0452496841878621 4.7
-0.0851517499908407 4.4
-0.1 4.3640361928344
-0.210119623515117 4.1
-0.309147134569726 3.8
-0.38497772958158 3.5
-0.4 3.43539119747744
-0.481605123002026 3.2
-0.565929004563796 2.9
-0.630587700461568 2.6
-0.680114280421231 2.3
-0.7 2.15627256073835
-0.742020664160229 2
-0.808466368809077 1.7
-0.856414768918915 1.4
-0.888138879029881 1.1
-0.904033012988572 0.8
-0.902050364641805 0.5
-0.876452051818132 0.2
-0.815269219547046 -0.1
-0.7 -0.391224249679828
-0.698132582660652 -0.4
-0.61112244168742 -0.7
-0.455694782976736 -1
-0.4 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
-0.1 -0.813662566383539
-0.0212732948109916 -1
0.2 -1
0.209936400597169 -1
0.2 -0.982156747342992
0.0386312732522342 -0.7
-0.0769422164151812 -0.4
-0.1 -0.320545524347628
-0.185072070826102 -0.1
-0.250769770989332 0.2
-0.278000994504965 0.5
-0.276268697359673 0.8
-0.25035615628742 1.1
-0.201922097121707 1.4
-0.129964158449655 1.7
-0.1 1.80174979797539
-0.0455234187211962 2
0.057635272927661 2.3
0.192217373035997 2.6
0.2 2.61629914030158
0.370105204466033 2.9
0.5 3.08560018786762
0.595562103554131 3.2
0.8 3.43060031408318
0.859210871332377 3.5
1.1 3.77203265895309
1.11994085347524 3.8
1.33653500333124 4.1
1.4 4.18353447756902
1.5331719706287 4.4
1.7 4.64474855988664
1.73123539799353 4.7
1.90495603023311 5
1.7 5
1.47498256026639 5
1.4 4.87669640584839
1.2652805006217 4.7
1.1 4.46450730657905
1.04235946076651 4.4
0.8 4.11969797430092
0.781733705818006 4.1
0.510576865824403 3.8
0.5 3.78796342584856
0.287145065552571 3.5
0.2 3.3659201467006
0.115012995722929 3.2
-0.0169961358575289 2.9
-0.1 2.66569907729652
-0.124143639754818 2.6
-0.224447022281811 2.3
-0.300857329507489 2
-0.358286163497074 1.7
-0.399974747750666 1.4
-0.4 1.399754456032
-0.451231479042152 1.1
-0.477318611047455 0.8
-0.475474252098531 0.5
-0.437675744095722 0.2
-0.4 0.0623466157846053
-0.374877067814499 -0.1
-0.297557936476125 -0.4
-0.166004115026487 -0.7
-0.1 -0.813662566383539
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
0.2 -0.982156747342992
0.209936400597169 -1
0.379583165558855 -1
0.210836334403503 -0.7
0.2 -0.678145955915305
0.0658544532726656 -0.4
-0.0293334220090769 -0.1
-0.0873094704611413 0.2
-0.1 0.349615335949565
-0.116709855382628 0.5
-0.111343640867446 0.8
-0.1 0.893615604298219
-0.0785144708432933 1.1
-0.0232026753461205 1.4
0.0576363794497322 1.7
0.167523592995601 2
0.2 2.07689831316581
0.316989715017489 2.3
0.5 2.58602621160662
0.510731033436611 2.6
0.754529244244202 2.9
0.8 2.95254883595025
1.00873178547404 3.2
1.1 3.30390841847545
1.24105263032515 3.5
1.4 3.70962731048575
1.45664654283477 3.8
1.65234840454269 4.1
1.7 4.17012182182163
1.83196468873358 4.4
2 4.66617256543503
2.01773068767378 4.7
2.17513075374836 5
2 5
1.90495603023311 5
1.73123539799353 4.7
1.7 4.64474855988664
1.5331719706287 4.4
1.4 4.18353447756902
1.33653500333124 4.1
1.11994085347524 3.8
1.1 3.77203265895309
0.859210871332377 3.5
0.8 3.43060031408318
0.595562103554131 3.2
0.5 3.08560018786762
0.370105204466033 2.9
0.2 2.61629914030158
0.192217373035997 2.6
0.057635272927661 2.3
-0.0455234187211962 2
-0.1 1.80174979797539
-0.129964158449655 1.7
-0.201922097121707 1.4
-0.25035615628742 1.1
-0.276268697359673 0.8
-0.278000994504965 0.5
-0.250769770989332 0.2
-0.185072070826102 -0.1
-0.1 -0.320545524347628
-0.0769422164151812 -0.4
0.0386312732522342 -0.7
0.2 -0.982156747342992
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.5 -1
0.555078582567625 -1
0.5 -0.930895611351041
0.357649550640895 -0.7
0.208349772045638 -0.4
0.2 -0.378650450738691
0.098733940512264 -0.1
0.0358151770189627 0.2
0.0115592782560456 0.5
0.0216805474062808 0.8
0.0631795792590218 1.1
0.135018755343615 1.4
0.2 1.59678700381744
0.241832543122736 1.7
0.389852811507469 2
0.5 2.1844245811227
0.58324608016236 2.3
0.8 2.57008229969934
0.824143919417946 2.6
1.07654940295485 2.9
1.1 2.92702178946936
1.29827413386791 3.2
1.4 3.33425245944486
1.50535595624657 3.5
1.7 3.78917288976769
1.70641011664755 3.8
1.88174791304702 4.1
2 4.28778073034951
2.06014144777069 4.4
2.22474110166687 4.7
2.3 4.82947515196365
2.38939512903686 5
2.3 5
2.17513075374836 5
2.01773068767379 4.7
2 4.66617256543502
1.83196468873358 4.4
1.7 4.17012182182163
1.65234840454269 4.1
1.45664654283477 3.8
1.4 3.70962731048575
1.24105263032515 3.5
1.1 3.30390841847545
1.00873178547404 3.2
0.8 2.95254883595025
0.754529244244202 2.9
0.510731033436611 2.6
0.5 2.58602621160662
0.316989715017489 2.3
0.2 2.07689831316581
0.167523592995601 2
0.0576363794497322 1.7
-0.0232026753461205 1.4
-0.0785144708432933 1.1
-0.1 0.893615604298219
-0.111343640867446 0.8
-0.116709855382628 0.5
-0.1 0.349615335949565
-0.0873094704611413 0.2
-0.0293334220090769 -0.1
0.0658544532726656 -0.4
0.2 -0.678145955915305
0.210836334403503 -0.7
0.379583165558855 -1
0.5 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.293716493872058
4.90487055808837 0.2
4.7 -0.00112938670289524
4.5984140909186 -0.1
4.4 -0.291686384994102
4.28617810124306 -0.4
4.1 -0.57426002068481
3.96204668153677 -0.7
3.8 -0.842215660231345
3.61141712986693 -1
3.8 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
0.5 -0.930895611351041
0.555078582567625 -1
0.744879852902016 -1
0.505686966175866 -0.7
0.5 -0.692046171298314
0.346172300544193 -0.4
0.22848665602982 -0.1
0.2 0.0156727705609066
0.158939824499066 0.2
0.136011922499938 0.5
0.15234851314515 0.8
0.2 1.07414340351693
0.205437702104645 1.1
0.301862347094348 1.4
0.436034488943695 1.7
0.5 1.8179651299316
0.619957193299287 2
0.8 2.23827333247225
0.847850574143051 2.3
1.09578650908233 2.6
1.1 2.60494602875514
1.31619101813403 2.9
1.4 3.01075680452861
1.52238399764984 3.2
1.7 3.46510864196106
1.72108682537527 3.5
1.90031304195998 3.8
2 3.95924602442046
2.07748821650672 4.1
2.24459606966333 4.4
2.3 4.49618746773107
2.408966327764 4.7
2.5760962609923 5
2.38939512903686 5
2.3 4.82947515196365
2.22474110166687 4.7
2.06014144777069 4.4
2 4.28778073034951
1.88174791304702 4.1
1.70641011664755 3.8
1.7 3.78917288976769
1.50535595624657 3.5
1.4 3.33425245944486
1.29827413386791 3.2
1.1 2.92702178946936
1.07654940295485 2.9
0.824143919417946 2.6
0.8 2.57008229969934
0.58324608016236 2.3
0.5 2.1844245811227
0.389852811507469 2
0.241832543122736 1.7
0.2 1.59678700381744
0.135018755343615 1.4
0.0631795792590218 1.1
0.0216805474062808 0.8
0.0115592782560456 0.5
0.0358151770189627 0.2
0.098733940512264 -0.1
0.2 -0.378650450738691
0.208349772045638 -0.4
0.357649550640895 -0.7
0.5 -0.930895611351041
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
3.2 -1
3.5 -1
3.61141712986693 -1
3.8 -0.842215660231345
3.96204668153677 -0.7
4.1 -0.57426002068481
4.28617810124306 -0.4
4.4 -0.291686384994102
4.5984140909186 -0.1
4.7 -0.00112938670289524
4.90487055808837 0.2
5 0.293716493872058
5 0.5
5 0.8
5 0.929498224501656
4.86963814782579 0.8
4.7 0.631553190237892
4.56688322744444 0.5
4.4 0.335201329975082
4.26193426451525 0.2
4.1 0.0416622504196441
3.9529565581794 -0.1
3.8 -0.246893323730931
3.63629220471929 -0.4
3.5 -0.526556921108368
3.3039124424845 -0.7
3.2 -0.79036480766649
2.93557322484563 -1
3.2 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
0.8 -1
1.00598282391283 -1
0.8 -0.834044021168576
0.692773098542395 -0.7
0.5 -0.430386262783465
0.483994829042749 -0.4
0.364607310321048 -0.1
0.291965222025707 0.2
0.268970502175687 0.5
0.294211628783333 0.8
0.363531389033222 1.1
0.474714922537704 1.4
0.5 1.45372026938002
0.642632418965567 1.7
0.8 1.92718569528069
0.853072397557459 2
1.08997970735932 2.3
1.1 2.31210210853272
1.31188342848019 2.6
1.4 2.71689834119719
1.52081404200286 2.9
1.7 3.16877627438489
1.71933164431156 3.2
1.90120932142959 3.5
2 3.65907396305656
2.07996284645248 3.8
2.24801382632169 4.1
2.3 4.19104852126257
2.41491999104141 4.4
2.58017623384166 4.7
2.6 4.73516653973403
2.73992250513973 5
2.6 5
2.5760962609923 5
2.408966327764 4.7
2.3 4.49618746773107
2.24459606966333 4.4
2.07748821650672 4.1
2 3.95924602442046
1.90031304195998 3.8
1.72108682537527 3.5
1.7 3.46510864196106
1.52238399764984 3.2
1.4 3.01075680452861
1.31619101813403 2.9
1.1 2.60494602875514
1.09578650908233 2.6
0.847850574143051 2.3
0.8 2.23827333247225
0.619957193299287 2
0.5 1.8179651299316
0.436034488943695 1.7
0.301862347094348 1.4
0.205437702104645 1.1
0.2 1.07414340351693
0.15234851314515 0.8
0.136011922499938 0.5
0.158939824499066 0.2
0.2 0.0156727705609066
0.22848665602982 -0.1
0.346172300544193 -0.4
0.5 -0.692046171298314
0.505686966175866 -0.7
0.744879852902016 -1
0.8 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
2.6 -1
2.9 -1
2.93557322484563 -1
3.2 -0.79036480766649
3.3039124424845 -0.7
3.5 -0.526556921108368
3.63629220471929 -0.4
3.8 -0.246893323730931
3.9529565581794 -0.1
4.1 0.0416622504196441
4.26193426451525 0.2
4.4 0.335201329975082
4.56688322744444 0.5
4.7 0.631553190237892
4.86963814782579 0.8
5 0.929498224501656
5 1.1
5 1.34205029770283
4.75667774672349 1.1
4.7 1.04363457071733
4.45409975319719 0.8
4.4 0.746428718478555
4.14953267807437 0.5
4.1 0.451321622099335
3.84141657674954 0.2
3.8 0.159842324334873
3.52677603592264 -0.1
3.5 -0.125338460558759
3.2 -0.399517358977896
3.19945080463954 -0.4
2.9 -0.658007709956063
2.84642184032821 -0.7
2.6 -0.886594332984976
2.41730790889433 -1
2.6 -1
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
0.8 -0.834044021168576
1.00598282391283 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.3 -1
2.41730790889433 -1
2.6 -0.886594332984976
2.84642184032821 -0.7
2.9 -0.658007709956063
3.19945080463954 -0.4
3.2 -0.399517358977896
3.5 -0.125338460558759
3.52677603592264 -0.1
3.8 0.159842324334873
3.84141657674954 0.2
4.1 0.451321622099335
4.14953267807437 0.5
4.4 0.746428718478555
4.45409975319719 0.8
4.7 1.04363457071733
4.75667774672349 1.1
5 1.34205029770283
5 1.4
5 1.69993772617664
4.7 1.40129342525664
4.69869763091744 1.4
4.4 1.10366081489425
4.39629544812573 1.1
4.1 0.80774287792531
4.0920992500715 0.8
3.8 0.514696447406888
3.78479475629421 0.5
3.5 0.226466316016418
3.47194570103264 0.2
3.2 -0.0534957484076629
3.14838512075766 -0.1
2.9 -0.318953468583279
2.80149699917411 -0.4
2.6 -0.559650747880089
2.39515746171235 -0.7
2.3 -0.761382610404774
2 -0.904081525803997
1.7 -0.974573610827958
1.4 -0.954940919188282
1.1 -0.833486762432242
0.932171167879391 -0.7
0.8 -0.585386039828671
0.668430570181298 -0.4
0.501037164588505 -0.1
0.5 -0.0968730040435268
0.42994436536582 0.2
0.410930691966831 0.5
0.442500764236336 0.8
0.5 1.021767357983
0.526177096227076 1.1
0.669322645723743 1.4
0.8 1.61509094064979
0.85612928903867 1.7
1.07687082976231 2
1.1 2.02919539911228
1.29816541310154 2.3
1.4 2.43643492399283
1.51020297122499 2.6
1.7 2.88624779865033
1.70874919420485 2.9
1.89428936690357 3.2
2 3.37169144404435
2.07530506696999 3.5
2.24453187113398 3.8
2.3 3.89796163425571
2.41550288457381 4.1
2.57917733239982 4.4
2.6 4.43761744598487
2.74189383193363 4.7
2.9 4.99926177598583
2.90041578646477 5
2.9 5
2.73992250513973 5
2.6 4.73516653973403
2.58017623384166 4.7
2.41491999104141 4.4
2.3 4.19104852126257
2.24801382632169 4.1
2.07996284645248 3.8
2 3.65907396305656
1.90120932142959 3.5
1.71933164431156 3.2
1.7 3.16877627438489
1.52081404200286 2.9
1.4 2.71689834119719
1.31188342848019 2.6
1.1 2.31210210853272
1.08997970735932 2.3
0.853072397557459 2
0.8 1.92718569528069
0.642632418965567 1.7
0.5 1.45372026938002
0.474714922537704 1.4
0.363531389033222 1.1
0.294211628783333 0.8
0.268970502175687 0.5
0.291965222025707 0.2
0.364607310321048 -0.1
0.483994829042749 -0.4
0.5 -0.430386262783465
0.692773098542395 -0.7
0.8 -0.834044021168576
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.1 -0.833486762432242
1.4 -0.954940919188282
1.7 -0.974573610827958
2 -0.904081525803997
2.3 -0.761382610404774
2.39515746171235 -0.7
2.6 -0.559650747880089
2.80149699917411 -0.4
2.9 -0.318953468583279
3.14838512075766 -0.1
3.2 -0.0534957484076629
3.47194570103264 0.2
3.5 0.226466316016418
3.78479475629421 0.5
3.8 0.514696447406888
4.0920992500715 0.8
4.1 0.80774287792531
4.39629544812573 1.1
4.4 1.10366081489425
4.69869763091744 1.4
4.7 1.40129342525664
5 1.69993772617664
5 1.7
5 2
5 2.05835580557515
4.9414492394566 2
4.7 1.75956699854027
4.6400849456843 1.7
4.4 1.4616749586208
4.3377025689984 1.4
4.1 1.16528827654555
4.03359168222994 1.1
3.8 0.871369746306168
3.72657949862817 0.8
3.5 0.581444403164131
3.41458696796937 0.5
3.2 0.298172822522168
3.09315763455079 0.2
2.9 0.0266967990731534
2.75145350195731 -0.1
2.6 -0.224094820069593
2.36065319339773 -0.4
2.3 -0.441730335152246
2 -0.602711248233517
1.7 -0.694843780307137
1.4 -0.691103604249349
1.1 -0.570829843108835
0.901468367815022 -0.4
0.8 -0.290884139410471
0.694974507165547 -0.1
0.595605921248189 0.2
0.571530287338116 0.5
0.616351682966629 0.8
0.717549078592974 1.1
0.8 1.26743170699694
0.874355775044196 1.4
1.07193229222448 1.7
1.1 1.73800331219856
1.28699244298906 2
1.4 2.15493276586118
1.49933522347294 2.3
1.69680492793264 2.6
1.7 2.60481873900616
1.88779525636674 2.9
2 3.08387189888068
2.07067975434228 3.2
2.24208034690096 3.5
2.3 3.60313133643697
2.41762337788732 3.8
2.58166024510511 4.1
2.6 4.13366460121655
2.74787610269351 4.4
2.9 4.69515081166959
2.90275841890534 4.7
3.07149250281028 5
2.90041578646477 5
2.9 4.99926177598583
2.74189383193363 4.7
2.6 4.43761744598487
2.57917733239982 4.4
2.41550288457381 4.1
2.3 3.89796163425571
2.24453187113398 3.8
2.07530506696999 3.5
2 3.37169144404435
1.89428936690357 3.2
1.70874919420485 2.9
1.7 2.88624779865033
1.51020297122499 2.6
1.4 2.43643492399283
1.29816541310154 2.3
1.1 2.02919539911228
1.07687082976231 2
0.85612928903867 1.7
0.8 1.61509094064979
0.669322645723743 1.4
0.526177096227076 1.1
0.5 1.021767357983
0.442500764236336 0.8
0.410930691966831 0.5
0.42994436536582 0.2
0.5 -0.0968730040435268
0.501037164588505 -0.1
0.668430570181298 -0.4
0.8 -0.585386039828671
0.932171167879391 -0.7
1.1 -0.833486762432242
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.1 -0.570829843108835
1.4 -0.691103604249349
1.7 -0.694843780307137
2 -0.602711248233517
2.3 -0.441730335152246
2.36065319339773 -0.4
2.6 -0.224094820069593
2.75145350195731 -0.1
2.9 0.0266967990731534
3.09315763455079 0.2
3.2 0.298172822522168
3.41458696796937 0.5
3.5 0.581444403164131
3.72657949862817 0.8
3.8 0.871369746306168
4.03359168222994 1.1
4.1 1.16528827654555
4.3377025689984 1.4
4.4 1.4616749586208
4.6400849456843 1.7
4.7 1.75956699854027
4.9414492394566 2
5 2.05835580557515
5 2.3
5 2.45478320029319
4.84480768275685 2.3
4.7 2.15573412549517
4.54354643673133 2
4.4 1.85738961798811
4.24135678599095 1.7
4.1 1.56022585769225
3.93761738339976 1.4
3.8 1.26497551411338
3.63137319753569 1.1
3.5 0.972704850571255
3.32099982823923 0.8
3.2 0.685192312827117
3.00249384637639 0.5
2.9 0.406537420732816
2.66567680082897 0.2
2.6 0.144604046036164
2.3 -0.088205658698573
2.28215525833188 -0.1
2 -0.266118325903965
1.7 -0.380073502262649
1.4 -0.392184193646478
1.1 -0.259396370579486
0.951895811323225 -0.1
0.8 0.169216215999936
0.789818843451294 0.2
0.763519016374629 0.5
0.8 0.754886168684135
0.808520991128163 0.8
0.931214339270998 1.1
1.09232520474273 1.4
1.1 1.4116700449456
1.29362281654837 1.7
1.4 1.85317813209472
1.50065582712434 2
1.69511596620158 2.3
1.7 2.30742583379179
1.89131448766822 2.6
2 2.77979299725834
2.07603444592374 2.9
2.24925720710114 3.2
2.3 3.29099028301757
2.43003020589509 3.5
2.59504781087638 3.8
2.6 3.80912603374375
2.76766146461302 4.1
2.9 4.36205242347335
2.92194434466542 4.4
3.08965714589107 4.7
3.2 4.91104909045494
3.24931759577261 5
3.2 5
3.07149250281028 5
2.90275841890534 4.7
2.9 4.69515081166959
2.74787610269351 4.4
2.6 4.13366460121655
2.58166024510511 4.1
2.41762337788732 3.8
2.3 3.60313133643697
2.24208034690096 3.5
2.07067975434228 3.2
2 3.08387189888068
1.88779525636674 2.9
1.7 2.60481873900616
1.69680492793264 2.6
1.49933522347294 2.3
1.4 2.15493276586118
1.28699244298906 2
1.1 1.73800331219856
1.07193229222448 1.7
0.874355775044196 1.4
0.8 1.26743170699694
0.717549078592974 1.1
0.616351682966629 0.8
0.571530287338116 0.5
0.595605921248189 0.2
0.694974507165547 -0.1
0.8 -0.290884139410471
0.901468367815022 -0.4
1.1 -0.570829843108835
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.1 -0.259396370579486
1.4 -0.392184193646478
1.7 -0.380073502262649
2 -0.266118325903965
2.28215525833188 -0.1
2.3 -0.088205658698573
2.6 0.144604046036164
2.66567680082897 0.2
2.9 0.406537420732816
3.00249384637639 0.5
3.2 0.685192312827117
3.32099982823923 0.8
3.5 0.972704850571255
3.63137319753569 1.1
3.8 1.26497551411338
3.93761738339976 1.4
4.1 1.56022585769225
4.24135678599095 1.7
4.4 1.85738961798811
4.54354643673133 2
4.7 2.15573412549517
4.84480768275685 2.3
5 2.45478320029319
5 2.6
5 2.9
5 2.9514257720986
4.94860078958469 2.9
4.7 2.65194200703162
4.64810811243612 2.6
4.4 2.35282641104458
4.34726834808096 2.3
4.1 2.05430812355616
4.04587616506277 2
3.8 1.75668212671509
3.74371809041953 1.7
3.5 1.46014177242276
3.44073944069793 1.4
3.2 1.1648340485884
3.13613216936165 1.1
2.9 0.874044052412695
2.82433221146298 0.8
2.6 0.597180362053592
2.49089660251751 0.5
2.3 0.346098168096088
2.09981039858317 0.2
2 0.135998911163926
1.7 0.0053550940053898
1.4 -0.00888706710589414
1.1 0.196046094317276
1.09767984510576 0.2
1.02994179044168 0.5
1.06187971626885 0.8
1.1 0.907900140726078
1.18221447579755 1.1
1.34396468668181 1.4
1.4 1.48939628586763
1.53930748024056 1.7
1.7 1.95997010123981
1.72709492132497 2
1.92194476936591 2.3
2 2.43112641555527
2.11105198883928 2.6
2.27970589392901 2.9
2.3 2.93665571361371
2.47097162722732 3.2
2.6 3.43589571968152
2.64272772662822 3.5
2.81689121548281 3.8
2.9 3.96671327465241
2.98041948920469 4.1
3.13775212800186 4.4
3.2 4.52396251709783
3.30302932362994 4.7
3.44751461489005 5
3.24931759577261 5
3.2 4.91104909045494
3.08965714589107 4.7
2.92194434466542 4.4
2.9 4.36205242347335
2.76766146461302 4.1
2.6 3.80912603374375
2.59504781087637 3.8
2.43003020589509 3.5
2.3 3.29099028301757
2.24925720710114 3.2
2.07603444592374 2.9
2 2.77979299725834
1.89131448766822 2.6
1.7 2.30742583379179
1.69511596620158 2.3
1.50065582712434 2
1.4 1.85317813209472
1.29362281654837 1.7
1.1 1.4116700449456
1.09232520474273 1.4
0.931214339270998 1.1
0.808520991128163 0.8
0.8 0.754886168684135
0.763519016374629 0.5
0.789818843451294 0.2
0.8 0.169216215999936
0.951895811323225 -0.1
1.1 -0.259396370579486
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
1.1 0.196046094317276
1.4 -0.00888706710589414
1.7 0.00535509400538978
2 0.135998911163926
2.09981039858317 0.2
2.3 0.346098168096088
2.49089660251751 0.5
2.6 0.597180362053592
2.82433221146298 0.8
2.9 0.874044052412695
3.13613216936165 1.1
3.2 1.1648340485884
3.44073944069793 1.4
3.5 1.46014177242276
3.74371809041953 1.7
3.8 1.75668212671509
4.04587616506277 2
4.1 2.05430812355616
4.34726834808096 2.3
4.4 2.35282641104458
4.64810811243612 2.6
4.7 2.65194200703162
4.94860078958469 2.9
5 2.9514257720986
5 3.2
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.32178433072806 5
4.23647597274745 4.7
4.12812280471197 4.4
4.1 4.33142094009158
4.02077104766664 4.1
3.93163694110467 3.8
3.81572292213262 3.5
3.8 3.4603562109591
3.73133499642604 3.2
3.62675796983053 2.9
3.5 2.66393453265014
3.47549717384692 2.6
3.31633378528108 2.3
3.2 2.13424506004375
3.12938899391381 2
2.92273518171223 1.7
2.9 1.67347633217508
2.69492306199024 1.4
2.6 1.29378136568317
2.43022872498035 1.1
2.3 0.970729281984772
2.10757831619385 0.8
2 0.716162692546386
1.7 0.585568816714095
1.49359913053829 0.8
1.55752094992034 1.1
1.67774347822932 1.4
1.7 1.44066371369561
1.87017921694662 1.7
2 1.9463707224573
2.03777973758052 2
2.22782393430103 2.3
2.3 2.43672367099695
2.42125200649011 2.6
2.58428173102769 2.9
2.6 2.92930953156499
2.80330829198491 3.2
2.9 3.39599132888229
2.97912503361917 3.5
3.14095823076946 3.8
3.2 3.93541915572051
3.32136923020607 4.1
3.45838275799539 4.4
3.5 4.50371357515265
3.64747314735293 4.7
3.77449403172787 5
3.5 5
3.44751461489005 5
3.30302932362994 4.7
3.2 4.52396251709783
3.13775212800186 4.4
2.98041948920469 4.1
2.9 3.96671327465241
2.81689121548281 3.8
2.64272772662822 3.5
2.6 3.43589571968152
2.47097162722732 3.2
2.3 2.93665571361371
2.27970589392901 2.9
2.11105198883928 2.6
2 2.43112641555527
1.92194476936591 2.3
1.72709492132497 2
1.7 1.95997010123981
1.53930748024056 1.7
1.4 1.48939628586763
1.34396468668181 1.4
1.18221447579755 1.1
1.1 0.907900140726078
1.06187971626885 0.8
1.02994179044168 0.5
1.09767984510576 0.2
1.1 0.196046094317276
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
1.7 0.585568816714095
2 0.716162692546386
2.10757831619385 0.8
2.3 0.970729281984772
2.43022872498035 1.1
2.6 1.29378136568317
2.69492306199024 1.4
2.9 1.67347633217508
2.92273518171223 1.7
3.12938899391381 2
3.2 2.13424506004375
3.31633378528108 2.3
3.47549717384692 2.6
3.5 2.66393453265014
3.62675796983053 2.9
3.73133499642604 3.2
3.8 3.4603562109591
3.81572292213262 3.5
3.93163694110467 3.8
4.02077104766664 4.1
4.1 4.33142094009158
4.12812280471197 4.4
4.23647597274745 4.7
4.32178433072806 5
4.1 5
3.8 5
3.77449403172787 5
3.64747314735293 4.7
3.5 4.50371357515265
3.45838275799539 4.4
3.32136923020607 4.1
3.2 3.93541915572051
3.14095823076946 3.8
2.97912503361917 3.5
2.9 3.39599132888229
2.80330829198492 3.2
2.6 2.92930953156499
2.58428173102769 2.9
2.42125200649011 2.6
2.3 2.43672367099695
2.22782393430103 2.3
2.03777973758052 2
2 1.9463707224573
1.87017921694662 1.7
1.7 1.44066371369561
1.67774347822932 1.4
1.55752094992034 1.1
1.49359913053829 0.8
1.7 0.585568816714095
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2 2.3
};
\coordinate (MCMC_mean_lml_t) at (axis cs:1.6999999999999997,4.7);
\end{axis}



==> fig/tikz/parkinsons/MCMC_mean_lml.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 -1
-0.4 -1
-0.342842514570438 -1
-0.4 -0.908109145150121
-0.553914411826153 -0.7
-0.691691439843195 -0.4
-0.7 -0.380298003116879
-0.846846870447652 -0.1
-0.934649619636087 0.2
-0.983033203007205 0.5
-1 0.656301835723364
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.4 -0.908109145150121
-0.342842514570438 -1
-0.1 -1
0.2 -1
0.243956420614923 -1
0.2 -0.933362089992242
0.0341441444890167 -0.7
-0.1 -0.446830526394375
-0.130587699766179 -0.4
-0.289504908942738 -0.1
-0.387308900407179 0.2
-0.4 0.271782856734428
-0.459473490228503 0.5
-0.52580824398059 0.8
-0.54540372273763 1.1
-0.566352270787885 1.4
-0.595282683923046 1.7
-0.587423753625179 2
-0.576327314572094 2.3
-0.594282817718339 2.6
-0.578755639717174 2.9
-0.577581662242138 3.2
-0.573010559151926 3.5
-0.591707870531491 3.8
-0.586595224537128 4.1
-0.59588317483363 4.4
-0.572656156745429 4.7
-0.553739329682415 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.656301835723364
-0.983033203007205 0.5
-0.934649619636087 0.2
-0.846846870447652 -0.1
-0.7 -0.380298003116879
-0.691691439843195 -0.4
-0.553914411826153 -0.7
-0.4 -0.908109145150121
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
0.2 -0.933362089992242
0.243956420614923 -1
0.5 -1
0.557615763898899 -1
0.5 -0.936364888948977
0.325270839800495 -0.7
0.2 -0.508249736443694
0.128391963692363 -0.4
-0.0220318235755189 -0.1
-0.1 0.141939267949234
-0.124424645030818 0.2
-0.212806245352751 0.5
-0.266377386046556 0.8
-0.295080376859082 1.1
-0.309032344900388 1.4
-0.332098798894811 1.7
-0.32843256047624 2
-0.323267242494939 2.3
-0.329614713227928 2.6
-0.334230542275878 2.9
-0.328990832296511 3.2
-0.320126788901375 3.5
-0.340527130758928 3.8
-0.328053592314202 4.1
-0.336933916933497 4.4
-0.328974087839307 4.7
-0.308048555467763 5
-0.4 5
-0.553739329682415 5
-0.572656156745429 4.7
-0.59588317483363 4.4
-0.586595224537128 4.1
-0.591707870531491 3.8
-0.573010559151926 3.5
-0.577581662242138 3.2
-0.578755639717174 2.9
-0.594282817718339 2.6
-0.576327314572094 2.3
-0.587423753625179 2
-0.595282683923046 1.7
-0.566352270787885 1.4
-0.54540372273763 1.1
-0.52580824398059 0.8
-0.459473490228503 0.5
-0.4 0.271782856734428
-0.387308900407179 0.2
-0.289504908942738 -0.1
-0.130587699766179 -0.4
-0.1 -0.446830526394375
0.0341441444890167 -0.7
0.2 -0.933362089992242
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
0.5 -0.936364888948977
0.557615763898899 -1
0.8 -1
0.874004828027978 -1
0.8 -0.944811460554839
0.576240067621728 -0.7
0.5 -0.61571578212343
0.348806401787612 -0.4
0.2 -0.137888343646623
0.179354436729703 -0.1
0.0567446707810254 0.2
-0.022553300786603 0.5
-0.0717176237939854 0.8
-0.0986056037691966 1.1
-0.1 1.12333961379817
-0.121966849679458 1.4
-0.13794644746113 1.7
-0.140921299103641 2
-0.141530187464708 2.3
-0.146867163613317 2.6
-0.147267843979927 2.9
-0.153405072767634 3.2
-0.146281036930058 3.5
-0.156898817572413 3.8
-0.147949677584104 4.1
-0.147995814185149 4.4
-0.150175875616256 4.7
-0.151201045494762 5
-0.308048555467763 5
-0.328974087839307 4.7
-0.336933916933497 4.4
-0.328053592314202 4.1
-0.340527130758928 3.8
-0.320126788901375 3.5
-0.328990832296511 3.2
-0.334230542275878 2.9
-0.329614713227928 2.6
-0.323267242494939 2.3
-0.32843256047624 2
-0.332098798894811 1.7
-0.309032344900388 1.4
-0.295080376859082 1.1
-0.266377386046556 0.8
-0.212806245352751 0.5
-0.124424645030818 0.2
-0.1 0.141939267949234
-0.022031823575519 -0.1
0.128391963692363 -0.4
0.2 -0.508249736443694
0.325270839800495 -0.7
0.5 -0.936364888948977
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
3.5 -1
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.5
5 0.586410544982543
4.92380599510234 0.5
4.7 0.257506907097127
4.6476741682604 0.2
4.4 -0.0740497362511419
4.375117848717 -0.1
4.1 -0.377394274205721
4.07706132602339 -0.4
3.8 -0.642765061442584
3.7296474875059 -0.7
3.5 -0.870614722525815
3.29862533567971 -1
3.5 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.8 -0.944811460554839
0.874004828027978 -1
1.1 -1
1.38074169557023 -1
1.1 -0.872271110534154
0.868994415596657 -0.7
0.8 -0.650403240117008
0.572495874704994 -0.4
0.5 -0.314854547473202
0.368011701036236 -0.1
0.229537066775476 0.2
0.2 0.288634540384542
0.135541713606528 0.5
0.0740445292700868 0.8
0.042149912291611 1.1
0.0233426682156818 1.4
0.0124500607691805 1.7
0.00776746854157116 2
0.0054334065642255 2.3
0.000187686025402339 2.6
0.00120550152862764 2.9
-0.00176906296617664 3.2
-0.00103767857957225 3.5
-0.00404481866516807 3.8
-0.00305828380498006 4.1
0.000930773157021933 4.4
-0.00167568190612685 4.7
-0.00643487823127392 5
-0.1 5
-0.151201045494762 5
-0.150175875616256 4.7
-0.147995814185149 4.4
-0.147949677584104 4.1
-0.156898817572413 3.8
-0.146281036930058 3.5
-0.153405072767634 3.2
-0.147267843979927 2.9
-0.146867163613317 2.6
-0.141530187464708 2.3
-0.140921299103641 2
-0.13794644746113 1.7
-0.121966849679458 1.4
-0.1 1.12333961379817
-0.0986056037691966 1.1
-0.0717176237939854 0.8
-0.022553300786603 0.5
0.0567446707810254 0.2
0.179354436729703 -0.1
0.2 -0.137888343646623
0.348806401787612 -0.4
0.5 -0.61571578212343
0.576240067621728 -0.7
0.8 -0.944811460554839
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
2.3 -1
2.6 -1
2.9 -1
3.2 -1
3.29862533567971 -1
3.5 -0.870614722525815
3.7296474875059 -0.7
3.8 -0.642765061442584
4.07706132602339 -0.4
4.1 -0.377394274205721
4.375117848717 -0.1
4.4 -0.0740497362511419
4.6476741682604 0.2
4.7 0.257506907097127
4.92380599510234 0.5
5 0.586410544982543
5 0.8
5 1.1
5 1.35651761240092
4.76404216363878 1.1
4.7 1.02937465482492
4.4804287138315 0.8
4.4 0.716608093561754
4.19653710298391 0.5
4.1 0.398848863093832
3.89867318642701 0.2
3.8 0.0995780552977577
3.60049908045675 -0.1
3.5 -0.195326624362132
3.262839610469 -0.4
3.2 -0.452014825235213
2.9 -0.676140790525404
2.86329671707881 -0.7
2.6 -0.862907396159775
2.3 -0.988515026842146
2.25531651268904 -1
2.3 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
1.1 -0.872271110534154
1.38074169557023 -1
1.4 -1
1.7 -1
2 -1
2.25531651268904 -1
2.3 -0.988515026842146
2.6 -0.862907396159775
2.86329671707881 -0.7
2.9 -0.676140790525404
3.2 -0.452014825235213
3.262839610469 -0.4
3.5 -0.195326624362132
3.60049908045675 -0.1
3.8 0.0995780552977577
3.89867318642701 0.2
4.1 0.398848863093832
4.19653710298391 0.5
4.4 0.716608093561754
4.4804287138315 0.8
4.7 1.02937465482492
4.76404216363878 1.1
5 1.35651761240092
5 1.4
5 1.7
5 1.87196898645321
4.84404532779013 1.7
4.7 1.5451338715497
4.55649247852757 1.4
4.4 1.23444104905176
4.27540839059137 1.1
4.1 0.917554700454934
3.98671696289627 0.8
3.8 0.612371299950996
3.68658730637742 0.5
3.5 0.310740766628519
3.38436045581303 0.2
3.2 0.0299833237745886
3.04562232455593 -0.1
2.9 -0.21755571576911
2.64488648949911 -0.4
2.6 -0.430452261959068
2.3 -0.583906997225269
2 -0.677640069271607
1.83331432970401 -0.7
1.7 -0.715901079653994
1.56775479596915 -0.7
1.4 -0.680476074785181
1.1 -0.569788774592031
0.855242207325241 -0.4
0.8 -0.362965499977796
0.575657788114759 -0.1
0.5 0.00282767333718516
0.402294922480387 0.2
0.298064435795522 0.5
0.222062949071385 0.8
0.2 0.958414157440032
0.182905428352418 1.1
0.163096433220625 1.4
0.152217144867571 1.7
0.145618748727357 2
0.142096874934152 2.3
0.134931593233069 2.6
0.136655398669303 2.9
0.139398531892919 3.2
0.133828606181045 3.5
0.134992175087852 3.8
0.129056909505766 4.1
0.136232030030403 4.4
0.135005183618643 4.7
0.132476125011699 5
-0.00643487823127392 5
-0.00167568190612688 4.7
0.000930773157021905 4.4
-0.00305828380498006 4.1
-0.00404481866516807 3.8
-0.00103767857957225 3.5
-0.00176906296617663 3.2
0.00120550152862767 2.9
0.000187686025402325 2.6
0.0054334065642255 2.3
0.00776746854157116 2
0.0124500607691805 1.7
0.0233426682156818 1.4
0.042149912291611 1.1
0.0740445292700868 0.8
0.135541713606528 0.5
0.2 0.288634540384542
0.229537066775476 0.2
0.368011701036236 -0.1
0.5 -0.314854547473202
0.572495874704994 -0.4
0.8 -0.650403240117008
0.868994415596657 -0.7
1.1 -0.872271110534154
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
4.1 4.87932185149433
4.4 4.8470598180883
4.7 4.89696473280566
5 4.96529918136096
5 5
4.7 5
4.4 5
4.1 5
3.97304917443437 5
4.1 4.87932185149433
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.7 -0.715901079653994
1.83331432970401 -0.7
2 -0.677640069271607
2.3 -0.583906997225269
2.6 -0.430452261959068
2.64488648949911 -0.4
2.9 -0.21755571576911
3.04562232455593 -0.1
3.2 0.0299833237745886
3.38436045581303 0.2
3.5 0.310740766628519
3.68658730637742 0.5
3.8 0.612371299950996
3.98671696289627 0.8
4.1 0.917554700454934
4.27540839059137 1.1
4.4 1.23444104905176
4.55649247852757 1.4
4.7 1.5451338715497
4.84404532779013 1.7
5 1.87196898645321
5 2
5 2.3
5 2.4072024481562
4.90129788486486 2.3
4.7 2.07877613823775
4.62761629212258 2
4.4 1.75924135155014
4.34568504797384 1.7
4.1 1.43857223991614
4.06252452661124 1.4
3.8 1.11359212495003
3.7874080422826 1.1
3.5 0.815319787883316
3.48432343355334 0.8
3.2 0.517333809778703
3.18142386061821 0.5
2.9 0.256000751807743
2.82570847886291 0.2
2.6 0.0368683990201208
2.39234035270431 -0.1
2.3 -0.151088710946475
2 -0.266741844767693
1.7 -0.332795155256774
1.4 -0.333046966676322
1.1 -0.250689831176393
0.864438977084732 -0.1
0.8 -0.0562590711588729
0.611470275028098 0.2
0.5 0.399261890473464
0.463635133530751 0.5
0.384429513311265 0.8
0.339015504983037 1.1
0.314889173225621 1.4
0.301740563392304 1.7
0.291629966053022 2
0.287689226108791 2.3
0.279911417232008 2.6
0.280680442208296 2.9
0.283192443115968 3.2
0.278637958600904 3.5
0.280775030435291 3.8
0.269574595186345 4.1
0.278265980425368 4.4
0.27843424454162 4.7
0.278199798395334 5
0.2 5
0.132476125011699 5
0.135005183618643 4.7
0.136232030030403 4.4
0.129056909505766 4.1
0.134992175087852 3.8
0.133828606181045 3.5
0.139398531892919 3.2
0.136655398669303 2.9
0.134931593233069 2.6
0.142096874934152 2.3
0.145618748727357 2
0.152217144867571 1.7
0.163096433220625 1.4
0.182905428352418 1.1
0.2 0.958414157440032
0.222062949071385 0.8
0.298064435795522 0.5
0.402294922480387 0.2
0.5 0.00282767333718516
0.575657788114759 -0.1
0.8 -0.362965499977796
0.855242207325241 -0.4
1.1 -0.569788774592031
1.4 -0.680476074785181
1.56775479596915 -0.7
1.7 -0.715901079653994
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
4.1 4.56338854736657
4.4 4.5745872387017
4.7 4.64556181145203
4.87164863186618 4.7
5 4.72360326863621
5 4.96529918136096
4.7 4.89696473280566
4.4 4.8470598180883
4.1 4.87932185149433
3.97304917443437 5
3.8 5
3.6462687497639 5
3.8 4.798080257717
3.90422838640067 4.7
4.1 4.56338854736657
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.1 -0.250689831176393
1.4 -0.333046966676322
1.7 -0.332795155256774
2 -0.266741844767693
2.3 -0.151088710946475
2.39234035270431 -0.1
2.6 0.0368683990201208
2.82570847886291 0.2
2.9 0.256000751807743
3.18142386061821 0.5
3.2 0.517333809778703
3.48432343355334 0.8
3.5 0.815319787883316
3.7874080422826 1.1
3.8 1.11359212495003
4.06252452661124 1.4
4.1 1.43857223991614
4.34568504797384 1.7
4.4 1.75924135155014
4.62761629212258 2
4.7 2.07877613823775
4.90129788486486 2.3
5 2.4072024481562
5 2.6
5 2.9
5 3.2
5 3.26163816786973
4.96072194217837 3.2
4.73650396230026 2.9
4.7 2.85337616185184
4.49406842191844 2.6
4.4 2.49426369411961
4.20923180510732 2.3
4.1 2.17525753775333
3.95852187614465 2
3.8 1.8239053087161
3.68433045081485 1.7
3.5 1.49554202552617
3.41476582133355 1.4
3.2 1.18402911795443
3.12033315275869 1.1
2.9 0.886887522891272
2.80924172200665 0.8
2.6 0.624023500313785
2.44687613166623 0.5
2.3 0.39831874883326
2 0.221165297466083
1.95653972509657 0.2
1.7 0.0961711258820301
1.4 0.0457245191791079
1.1 0.0987379639427957
0.947037126052679 0.2
0.8 0.322452513899104
0.700963896133878 0.5
0.57277647547749 0.8
0.5 1.08292776735593
0.497248156667755 1.1
0.471001604641374 1.4
0.456332084566349 1.7
0.442957433986847 2
0.439845924212995 2.3
0.434450337228736 2.6
0.432238763627256 2.9
0.428961857367221 3.2
0.433025121492969 3.5
0.432481683068015 3.8
0.419836898905609 4.1
0.426301754822581 4.4
0.427981618944734 4.7
0.430367461026911 5
0.278199798395334 5
0.27843424454162 4.7
0.278265980425368 4.4
0.269574595186345 4.1
0.280775030435291 3.8
0.278637958600904 3.5
0.283192443115968 3.2
0.280680442208296 2.9
0.279911417232008 2.6
0.287689226108791 2.3
0.291629966053022 2
0.301740563392304 1.7
0.314889173225621 1.4
0.339015504983037 1.1
0.384429513311265 0.8
0.463635133530751 0.5
0.5 0.399261890473464
0.611470275028097 0.2
0.8 -0.0562590711588729
0.864438977084732 -0.1
1.1 -0.250689831176393
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
4.1 4.04915951667973
4.4 4.06923830125536
4.7 4.06966006198822
5 4.05096925491667
5 4.1
5 4.4
5 4.7
5 4.72360326863621
4.87164863186618 4.7
4.7 4.64556181145203
4.4 4.5745872387017
4.1 4.56338854736658
3.90422838640067 4.7
3.8 4.798080257717
3.6462687497639 5
3.5 5
3.37713644795855 5
3.5 4.75122616327609
3.53716866447839 4.7
3.72574739996625 4.4
3.8 4.24434860429973
4.03926019542729 4.1
4.1 4.04915951667973
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.1 0.0987379639427957
1.4 0.0457245191791079
1.7 0.0961711258820301
1.95653972509657 0.2
2 0.221165297466083
2.3 0.39831874883326
2.44687613166623 0.5
2.6 0.624023500313785
2.80924172200665 0.8
2.9 0.886887522891272
3.12033315275869 1.1
3.2 1.18402911795443
3.41476582133355 1.4
3.5 1.49554202552617
3.68433045081485 1.7
3.8 1.8239053087161
3.95852187614465 2
4.1 2.17525753775333
4.20923180510732 2.3
4.4 2.49426369411961
4.49406842191844 2.6
4.7 2.85337616185184
4.73650396230026 2.9
4.96072194217837 3.2
5 3.26163816786973
5 3.5
5 3.8
5 4.05096925491667
4.7 4.06966006198822
4.4 4.06923830125536
4.1 4.04915951667973
4.03926019542729 4.1
3.8 4.24434860429973
3.72574739996625 4.4
3.53716866447839 4.7
3.5 4.75122616327609
3.37713644795855 5
3.2 5
3.12245151745904 5
3.2 4.7621526036933
3.22072185454335 4.7
3.29896818647863 4.4
3.35684267313523 4.1
3.3615574760488 3.8
3.35364112438645 3.5
3.28914961921301 3.2
3.21754033266213 2.9
3.2 2.84539479203441
3.14203953433135 2.6
3.03036422980795 2.3
2.9 2.04057773517843
2.88260117862291 2
2.72275278391771 1.7
2.6 1.54179009377587
2.51080968720789 1.4
2.3 1.12659695273473
2.27905171608178 1.1
2 0.832285433688785
1.96149044398706 0.8
1.7 0.610648638247046
1.41803069504482 0.5
1.4 0.494171924630935
1.35145854907979 0.5
1.1 0.536147765587526
0.853761317407356 0.8
0.8 0.889903393774783
0.74229507806027 1.1
0.685546329657279 1.4
0.660958308403082 1.7
0.643539225765824 2
0.64076822292806 2.3
0.62822400624071 2.6
0.624538526791193 2.9
0.619763456767675 3.2
0.624456341898923 3.5
0.62364228628177 3.8
0.607721289128392 4.1
0.614045608198894 4.4
0.62371063116472 4.7
0.621551512772645 5
0.5 5
0.430367461026911 5
0.427981618944734 4.7
0.426301754822581 4.4
0.419836898905609 4.1
0.432481683068015 3.8
0.433025121492969 3.5
0.428961857367221 3.2
0.432238763627256 2.9
0.434450337228736 2.6
0.439845924212995 2.3
0.442957433986847 2
0.456332084566349 1.7
0.471001604641374 1.4
0.497248156667755 1.1
0.5 1.08292776735593
0.57277647547749 0.8
0.700963896133878 0.5
0.8 0.322452513899104
0.947037126052679 0.2
1.1 0.0987379639427957
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.4 0.494171924630935
1.41803069504482 0.5
1.7 0.610648638247046
1.96149044398706 0.8
2 0.832285433688785
2.27905171608178 1.1
2.3 1.12659695273473
2.51080968720789 1.4
2.6 1.54179009377587
2.72275278391771 1.7
2.88260117862291 2
2.9 2.04057773517843
3.03036422980795 2.3
3.14203953433135 2.6
3.2 2.84539479203441
3.21754033266213 2.9
3.28914961921301 3.2
3.35364112438645 3.5
3.3615574760488 3.8
3.35684267313523 4.1
3.29896818647863 4.4
3.22072185454335 4.7
3.2 4.7621526036933
3.12245151745904 5
2.9 5
2.75400967262578 5
2.79083320905532 4.7
2.86340188516321 4.4
2.85468760466654 4.1
2.82850486427798 3.8
2.78066487609084 3.5
2.72061375079994 3.2
2.62314310298322 2.9
2.6 2.840602231866
2.51329333431771 2.6
2.39129306167425 2.3
2.3 2.11878722644892
2.23767606332254 2
2.06892880171066 1.7
2 1.59917581581181
1.81943538044639 1.4
1.7 1.26788128213802
1.4 1.11528376877497
1.1 1.24315601091453
1.03499206280385 1.4
0.963799857408822 1.7
0.931128765183407 2
0.920978651997985 2.3
0.891910496088836 2.6
0.885421973954241 2.9
0.894359273738887 3.2
0.881073572495806 3.5
0.878584535357217 3.8
0.870138916283507 4.1
0.872957885498438 4.4
0.891677530377061 4.7
0.881362782920378 5
0.8 5
0.621551512772645 5
0.62371063116472 4.7
0.614045608198894 4.4
0.607721289128392 4.1
0.62364228628177 3.8
0.624456341898923 3.5
0.619763456767675 3.2
0.624538526791193 2.9
0.62822400624071 2.6
0.64076822292806 2.3
0.643539225765824 2
0.660958308403082 1.7
0.685546329657279 1.4
0.74229507806027 1.1
0.8 0.889903393774783
0.853761317407357 0.8
1.1 0.536147765587526
1.35145854907979 0.5
1.4 0.494171924630935
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.1 1.24315601091453
1.4 1.11528376877497
1.7 1.26788128213802
1.81943538044639 1.4
2 1.59917581581181
2.06892880171066 1.7
2.23767606332254 2
2.3 2.11878722644892
2.39129306167425 2.3
2.51329333431771 2.6
2.6 2.840602231866
2.62314310298322 2.9
2.72061375079994 3.2
2.78066487609084 3.5
2.82850486427798 3.8
2.85468760466654 4.1
2.86340188516321 4.4
2.79083320905532 4.7
2.75400967262578 5
2.6 5
2.3 5
2 5
1.90048161485988 5
1.96099307301577 4.7
1.77066590280575 4.4
2 4.13174773157662
2.00477182718837 4.1
2 4.06222766202447
1.86119054978039 3.8
1.89397959492727 3.5
1.78147411988338 3.2
1.7 3.07463485476987
1.62492088525605 3.2
1.54264424795277 3.5
1.609371493857 3.8
1.59714292952566 4.1
1.66156940136214 4.4
1.56079395622978 4.7
1.59875467729156 5
1.4 5
1.1 5
0.881362782920378 5
0.891677530377061 4.7
0.872957885498438 4.4
0.870138916283507 4.1
0.878584535357217 3.8
0.881073572495806 3.5
0.894359273738887 3.2
0.885421973954241 2.9
0.891910496088836 2.6
0.920978651997985 2.3
0.931128765183407 2
0.963799857408822 1.7
1.03499206280385 1.4
1.1 1.24315601091453
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
1.7 3.07463485476987
1.78147411988338 3.2
1.89397959492727 3.5
1.86119054978039 3.8
2 4.06222766202447
2.00477182718837 4.1
2 4.13174773157662
1.77066590280575 4.4
1.96099307301577 4.7
1.90048161485988 5
1.7 5
1.59875467729156 5
1.56079395622978 4.7
1.66156940136214 4.4
1.59714292952566 4.1
1.609371493857 3.8
1.54264424795277 3.5
1.62492088525605 3.2
1.7 3.07463485476987
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
1.7 4.7
};
\coordinate (MCMC_mean_lml_t) at (axis cs:1.6999999999999997,4.7);
\end{axis}



==> fig/tikz/parkinsons/MCMC_nlpd.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 -1
-0.464363943291081 -1
-0.616902899870422 -0.7
-0.7 -0.425228539563463
-0.713131207721178 -0.4
-0.842545202685727 -0.1
-0.912473726724063 0.2
-0.951494195991543 0.5
-0.972937011189697 0.8
-0.984347823583732 1.1
-0.991626157910889 1.4
-0.995218493609741 1.7
-0.997717185912925 2
-0.99722892131606 2.3
-0.99786624784592 2.6
-0.999145264733647 2.9
-0.999322448924934 3.2
-0.998640697198187 3.5
-0.998832464531764 3.8
-0.999456995354154 4.1
-0.997906203395754 4.4
-1 4.61961723665558
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.999269807502097 5
-1 5
-1 4.85464556918161
-0.999269807502097 5
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.4 -1
-0.1 -1
-0.0227227208493405 -1
-0.1 -0.822603707783186
-0.172416232068812 -0.7
-0.308277046715498 -0.4
-0.39303935622388 -0.1
-0.4 -0.0653597604249011
-0.489413483783014 0.2
-0.549866582341149 0.5
-0.58350444848245 0.8
-0.602176823116456 1.1
-0.613196869195445 1.4
-0.618912865494469 1.7
-0.6218361487348 2
-0.62443673524919 2.3
-0.624505258692322 2.6
-0.625083607903919 2.9
-0.626278959533143 3.2
-0.625711331015946 3.5
-0.626125936417008 3.8
-0.626273993657568 4.1
-0.626181224702574 4.4
-0.625427809630169 4.7
-0.625654642998792 5
-0.7 5
-0.999269807502097 5
-1 4.85464556918161
-1 4.7
-1 4.61961723665558
-0.997906203395754 4.4
-0.999456995354154 4.1
-0.998832464531764 3.8
-0.998640697198187 3.5
-0.999322448924934 3.2
-0.999145264733647 2.9
-0.99786624784592 2.6
-0.99722892131606 2.3
-0.997717185912925 2
-0.995218493609741 1.7
-0.991626157910889 1.4
-0.984347823583732 1.1
-0.972937011189697 0.8
-0.951494195991543 0.5
-0.912473726724063 0.2
-0.842545202685727 -0.1
-0.713131207721178 -0.4
-0.7 -0.425228539563463
-0.616902899870422 -0.7
-0.464363943291081 -1
-0.4 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
-0.1 -0.822603707783186
-0.0227227208493405 -1
0.2 -1
0.210261065618459 -1
0.2 -0.981954385807553
0.0345366981590175 -0.7
-0.0872578412039393 -0.4
-0.1 -0.362486592415634
-0.213619580356616 -0.1
-0.293052178171922 0.2
-0.342598952742861 0.5
-0.372049494959654 0.8
-0.389379414122643 1.1
-0.399606962198215 1.4
-0.4 1.42508067798055
-0.407478337183648 1.7
-0.412402758485576 2
-0.417554905815056 2.3
-0.418029120529442 2.6
-0.418012589414539 2.9
-0.419579784446712 3.2
-0.419001906917473 3.5
-0.419514753751627 3.8
-0.419729719556123 4.1
-0.418888601000523 4.4
-0.419104463449392 4.7
-0.420231173643196 5
-0.625654642998792 5
-0.625427809630169 4.7
-0.626181224702574 4.4
-0.626273993657567 4.1
-0.626125936417008 3.8
-0.625711331015946 3.5
-0.626278959533143 3.2
-0.625083607903919 2.9
-0.624505258692322 2.6
-0.62443673524919 2.3
-0.6218361487348 2
-0.618912865494469 1.7
-0.613196869195445 1.4
-0.602176823116456 1.1
-0.58350444848245 0.8
-0.549866582341149 0.5
-0.489413483783014 0.2
-0.4 -0.0653597604249011
-0.39303935622388 -0.1
-0.308277046715498 -0.4
-0.172416232068812 -0.7
-0.1 -0.822603707783186
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
0.2 -0.981954385807553
0.210261065618459 -1
0.378502927590058 -1
0.20692790952507 -0.7
0.2 -0.687016113800317
0.0535350577350898 -0.4
-0.0544946967355646 -0.1
-0.1 0.0731569982765369
-0.140880571809285 0.2
-0.205433091888063 0.5
-0.243599340981967 0.8
-0.264993501922456 1.1
-0.277800260712784 1.4
-0.284152724889535 1.7
-0.287827540347146 2
-0.290629599284392 2.3
-0.291339303018508 2.6
-0.292133659620998 2.9
-0.292374031325198 3.2
-0.292052508117179 3.5
-0.292615787599776 3.8
-0.293044938926881 4.1
-0.292890748823439 4.4
-0.292808305592122 4.7
-0.292658891003849 5
-0.4 5
-0.420231173643196 5
-0.419104463449392 4.7
-0.418888601000523 4.4
-0.419729719556123 4.1
-0.419514753751627 3.8
-0.419001906917473 3.5
-0.419579784446712 3.2
-0.418012589414539 2.9
-0.418029120529442 2.6
-0.417554905815056 2.3
-0.412402758485576 2
-0.407478337183648 1.7
-0.4 1.42508067798055
-0.399606962198215 1.4
-0.389379414122643 1.1
-0.372049494959654 0.8
-0.342598952742861 0.5
-0.293052178171922 0.2
-0.213619580356616 -0.1
-0.1 -0.362486592415634
-0.0872578412039393 -0.4
0.0345366981590175 -0.7
0.2 -0.981954385807553
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
0.5 -1
0.55393914388637 -1
0.5 -0.93429667429426
0.354142499355675 -0.7
0.2 -0.411115068271811
0.194327956674119 -0.4
0.0695862615217053 -0.1
-0.0163264729592773 0.2
-0.0744440048847364 0.5
-0.1 0.698702907052728
-0.115149187004279 0.8
-0.140607589722269 1.1
-0.155993559227352 1.4
-0.164057748445294 1.7
-0.168594006416887 2
-0.171118078400475 2.3
-0.17228280976868 2.6
-0.173990326513326 2.9
-0.173486304794533 3.2
-0.173177333509994 3.5
-0.174031059647389 3.8
-0.174794219626188 4.1
-0.175043171150825 4.4
-0.17467839930082 4.7
-0.173591394542169 5
-0.292658891003849 5
-0.292808305592122 4.7
-0.292890748823439 4.4
-0.293044938926881 4.1
-0.292615787599776 3.8
-0.292052508117179 3.5
-0.292374031325198 3.2
-0.292133659620998 2.9
-0.291339303018508 2.6
-0.290629599284392 2.3
-0.287827540347146 2
-0.284152724889535 1.7
-0.277800260712784 1.4
-0.264993501922456 1.1
-0.243599340981967 0.8
-0.205433091888063 0.5
-0.140880571809285 0.2
-0.1 0.0731569982765369
-0.0544946967355645 -0.1
0.0535350577350898 -0.4
0.2 -0.687016113800317
0.20692790952507 -0.7
0.378502927590058 -1
0.5 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.299618114420471
4.90177234899725 0.2
4.7 0.00349443092525191
4.59404624675683 -0.1
4.4 -0.290800901341395
4.28531122921967 -0.4
4.1 -0.572916989290201
3.95775826878518 -0.7
3.8 -0.835217994105079
3.60417515949748 -1
3.8 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
0.5 -0.93429667429426
0.55393914388637 -1
0.748074620496593 -1
0.50178505126356 -0.7
0.5 -0.697728690571002
0.332796235923762 -0.4
0.2 -0.115148384790396
0.193667219778975 -0.1
0.0980828779009689 0.2
0.036022562771581 0.5
-0.00391657696935958 0.8
-0.0272106613258917 1.1
-0.0420309922759901 1.4
-0.050166295483441 1.7
-0.0547296031487563 2
-0.0568021423980881 2.3
-0.0580347697511861 2.6
-0.0601429450713846 2.9
-0.059337011658848 3.2
-0.0592892348438951 3.5
-0.0599323770410931 3.8
-0.0607121417000669 4.1
-0.0611032355688399 4.4
-0.0605353695282196 4.7
-0.0596557655167595 5
-0.1 5
-0.173591394542169 5
-0.17467839930082 4.7
-0.175043171150825 4.4
-0.174794219626188 4.1
-0.174031059647389 3.8
-0.173177333509994 3.5
-0.173486304794533 3.2
-0.173990326513326 2.9
-0.17228280976868 2.6
-0.171118078400475 2.3
-0.168594006416887 2
-0.164057748445294 1.7
-0.155993559227352 1.4
-0.140607589722269 1.1
-0.115149187004279 0.8
-0.1 0.698702907052728
-0.0744440048847364 0.5
-0.0163264729592773 0.2
0.0695862615217053 -0.1
0.194327956674119 -0.4
0.2 -0.411115068271811
0.354142499355675 -0.7
0.5 -0.93429667429426
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
3.2 -1
3.5 -1
3.60417515949748 -1
3.8 -0.835217994105079
3.95775826878518 -0.7
4.1 -0.572916989290201
4.28531122921967 -0.4
4.4 -0.290800901341395
4.59404624675683 -0.1
4.7 0.00349443092525194
4.90177234899725 0.2
5 0.299618114420471
5 0.5
5 0.8
5 0.931638546501722
4.86548658588809 0.8
4.7 0.635554656009718
4.56198964203617 0.5
4.4 0.339843679698447
4.25867764830268 0.2
4.1 0.0457948293020004
3.94780939420578 -0.1
3.8 -0.240924136821279
3.63227149427042 -0.4
3.5 -0.524186524831028
3.29827061589975 -0.7
3.2 -0.783952677727631
2.93182997027423 -1
3.2 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
0.8 -1
1.01860074870314 -1
0.8 -0.827312902377491
0.695424196168953 -0.7
0.5 -0.451341135980785
0.471166933319481 -0.4
0.329131594305392 -0.1
0.215041085271098 0.2
0.2 0.255183365349538
0.146489130427899 0.5
0.10501391861843 0.8
0.0808598755580827 1.1
0.065257816265565 1.4
0.0566337334215902 1.7
0.0518620193258747 2
0.0498784613365575 2.3
0.0487824141864278 2.6
0.0465054052976981 2.9
0.0471426987325825 3.2
0.0466129084549834 3.5
0.0467122237077035 3.8
0.046195168795452 4.1
0.0459859601470549 4.4
0.0467555720833924 4.7
0.0459752537180146 5
-0.0596557655167595 5
-0.0605353695282196 4.7
-0.0611032355688399 4.4
-0.0607121417000669 4.1
-0.059932377041093 3.8
-0.0592892348438951 3.5
-0.059337011658848 3.2
-0.0601429450713846 2.9
-0.0580347697511861 2.6
-0.0568021423980881 2.3
-0.0547296031487563 2
-0.050166295483441 1.7
-0.0420309922759901 1.4
-0.0272106613258917 1.1
-0.00391657696935957 0.8
0.036022562771581 0.5
0.0980828779009689 0.2
0.193667219778975 -0.1
0.2 -0.115148384790396
0.332796235923762 -0.4
0.5 -0.697728690571002
0.50178505126356 -0.7
0.748074620496593 -1
0.8 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
2.6 -1
2.9 -1
2.93182997027423 -1
3.2 -0.783952677727631
3.29827061589975 -0.7
3.5 -0.524186524831028
3.63227149427042 -0.4
3.8 -0.240924136821279
3.94780939420578 -0.1
4.1 0.0457948293020004
4.25867764830268 0.2
4.4 0.339843679698447
4.56198964203617 0.5
4.7 0.635554656009718
4.86548658588809 0.8
5 0.931638546501722
5 1.1
5 1.34483794445732
4.75209432966119 1.1
4.7 1.0488280278521
4.45033960010443 0.8
4.4 0.750383101846543
4.14680322499502 0.5
4.1 0.453590373683857
3.83603471828802 0.2
3.8 0.165210743179445
3.52057744806575 -0.1
3.5 -0.119692948480786
3.2 -0.395295307538776
3.19477767039613 -0.4
2.9 -0.651595953275982
2.83853009780449 -0.7
2.6 -0.881728508904743
2.40379350295047 -1
2.6 -1
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
0.8 -0.827312902377491
1.01860074870314 -1
1.1 -1
1.4 -1
1.7 -1
2 -1
2.3 -1
2.40379350295047 -1
2.6 -0.881728508904743
2.83853009780449 -0.7
2.9 -0.651595953275982
3.19477767039613 -0.4
3.2 -0.395295307538776
3.5 -0.119692948480786
3.52057744806575 -0.1
3.8 0.165210743179445
3.83603471828802 0.2
4.1 0.453590373683857
4.14680322499502 0.5
4.4 0.750383101846543
4.45033960010443 0.8
4.7 1.0488280278521
4.75209432966119 1.1
5 1.34483794445732
5 1.4
5 1.7
5 1.70711983192157
4.99282539662408 1.7
4.7 1.40117608546941
4.69883942628297 1.4
4.4 1.10699119512243
4.39279840958095 1.1
4.1 0.808699830353362
4.09132378488612 0.8
3.8 0.521174896187459
3.77764801108086 0.5
3.5 0.235004003728757
3.46253535412041 0.2
3.2 -0.04137087261315
3.13494638520348 -0.1
2.9 -0.312402070526964
2.79268644962091 -0.4
2.6 -0.552192192725802
2.37402980712387 -0.7
2.3 -0.745681806071373
2 -0.892010275797454
1.7 -0.96087763706174
1.4 -0.937354033810608
1.1 -0.820423297714492
0.945610106093436 -0.7
0.8 -0.583286854086759
0.656868728060864 -0.4
0.5 -0.173239029624236
0.465208196337994 -0.1
0.352793990296552 0.2
0.272153323339938 0.5
0.217858239294393 0.8
0.2 0.966652450411479
0.188930412442057 1.1
0.17254662480712 1.4
0.163433762326621 1.7
0.158453641800506 2
0.156559065071203 2.3
0.155599598124042 2.6
0.153153755666781 2.9
0.153622409124013 3.2
0.152515051753862 3.5
0.1533568244565 3.8
0.153102479290971 4.1
0.15307515586295 4.4
0.154046513695004 4.7
0.151606272952789 5
0.0459752537180146 5
0.0467555720833924 4.7
0.0459859601470549 4.4
0.046195168795452 4.1
0.0467122237077035 3.8
0.0466129084549833 3.5
0.0471426987325825 3.2
0.0465054052976981 2.9
0.0487824141864278 2.6
0.0498784613365574 2.3
0.0518620193258747 2
0.0566337334215902 1.7
0.065257816265565 1.4
0.0808598755580827 1.1
0.10501391861843 0.8
0.146489130427899 0.5
0.2 0.255183365349538
0.215041085271098 0.2
0.329131594305392 -0.1
0.471166933319481 -0.4
0.5 -0.451341135980785
0.695424196168953 -0.7
0.8 -0.827312902377491
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.1 -0.820423297714492
1.4 -0.937354033810608
1.7 -0.96087763706174
2 -0.892010275797454
2.3 -0.745681806071373
2.37402980712387 -0.7
2.6 -0.552192192725802
2.79268644962091 -0.4
2.9 -0.312402070526964
3.13494638520348 -0.1
3.2 -0.04137087261315
3.46253535412041 0.2
3.5 0.235004003728757
3.77764801108086 0.5
3.8 0.521174896187459
4.09132378488612 0.8
4.1 0.808699830353362
4.39279840958095 1.1
4.4 1.10699119512243
4.69883942628297 1.4
4.7 1.40117608546941
4.99282539662408 1.7
5 1.70711983192157
5 2
5 2.06923070157202
4.93318273807948 2
4.7 1.76868321738852
4.63025039167162 1.7
4.4 1.4665192998539
4.33414815571507 1.4
4.1 1.17297512708496
4.02477171311939 1.1
3.8 0.874585624643712
3.72242063969519 0.8
3.5 0.590225058230116
3.40478107679186 0.5
3.2 0.309377835844187
3.0808128365303 0.2
2.9 0.0378545781329951
2.73705461642043 -0.1
2.6 -0.211761190030712
2.33592489020162 -0.4
2.3 -0.423890089434068
2 -0.586287041986845
1.7 -0.67234666304857
1.4 -0.668065387847965
1.1 -0.558095316909107
0.898187972934483 -0.4
0.8 -0.316462225059086
0.65253578132894 -0.1
0.5 0.174675930686682
0.490546895322006 0.2
0.41209594966986 0.5
0.357362619176909 0.8
0.326674668928176 1.1
0.305816259566484 1.4
0.294046439856383 1.7
0.287573430587584 2
0.285145496859461 2.3
0.283596424924948 2.6
0.280507114634917 2.9
0.280638100898364 3.2
0.278858865801483 3.5
0.280518844793654 3.8
0.280455122505136 4.1
0.280501424796154 4.4
0.281417084141899 4.7
0.27797487454588 5
0.2 5
0.151606272952789 5
0.154046513695004 4.7
0.15307515586295 4.4
0.153102479290971 4.1
0.1533568244565 3.8
0.152515051753862 3.5
0.153622409124013 3.2
0.153153755666781 2.9
0.155599598124042 2.6
0.156559065071203 2.3
0.158453641800506 2
0.163433762326621 1.7
0.17254662480712 1.4
0.188930412442057 1.1
0.2 0.966652450411479
0.217858239294393 0.8
0.272153323339938 0.5
0.352793990296552 0.2
0.465208196337994 -0.1
0.5 -0.173239029624236
0.656868728060864 -0.4
0.8 -0.583286854086759
0.945610106093436 -0.7
1.1 -0.820423297714492
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.1 -0.558095316909107
1.4 -0.668065387847965
1.7 -0.67234666304857
2 -0.586287041986845
2.3 -0.423890089434068
2.33592489020162 -0.4
2.6 -0.211761190030712
2.73705461642043 -0.1
2.9 0.0378545781329951
3.0808128365303 0.2
3.2 0.309377835844187
3.40478107679186 0.5
3.5 0.590225058230116
3.72242063969519 0.8
3.8 0.874585624643712
4.02477171311939 1.1
4.1 1.17297512708496
4.33414815571507 1.4
4.4 1.4665192998539
4.63025039167162 1.7
4.7 1.76868321738852
4.93318273807948 2
5 2.06923070157202
5 2.3
5 2.47557738212513
4.82469488390853 2.3
4.7 2.17013723478699
4.53218873993874 2
4.4 1.87015779870175
4.22720881890822 1.7
4.1 1.57129760419598
3.93010471325548 1.4
3.8 1.27439816117138
3.62347379326433 1.1
3.5 0.981691445612048
3.30974353791258 0.8
3.2 0.696535438685732
2.98713459478928 0.5
2.9 0.420713922362942
2.64590620572835 0.2
2.6 0.161698235439875
2.3 -0.0663034969546733
2.24922169346528 -0.1
2 -0.243551420856727
1.7 -0.355255589056547
1.4 -0.367687315490992
1.1 -0.261456405218877
0.907768006355786 -0.1
0.8 0.0138406579356853
0.701024333689034 0.2
0.582957216849879 0.5
0.5 0.782913579429241
0.496866999059426 0.8
0.46780524111108 1.1
0.448020039730475 1.4
0.437056838682047 1.7
0.431082633848183 2
0.428779598393745 2.3
0.426659466670909 2.6
0.424079833689986 2.9
0.423500311073272 3.2
0.421818877814315 3.5
0.423630446333005 3.8
0.423785748944826 4.1
0.423789478422166 4.4
0.423831137303865 4.7
0.421876955832227 5
0.27797487454588 5
0.281417084141899 4.7
0.280501424796154 4.4
0.280455122505136 4.1
0.280518844793654 3.8
0.278858865801483 3.5
0.280638100898364 3.2
0.280507114634917 2.9
0.283596424924948 2.6
0.285145496859461 2.3
0.287573430587584 2
0.294046439856383 1.7
0.305816259566484 1.4
0.326674668928176 1.1
0.357362619176909 0.8
0.41209594966986 0.5
0.490546895322006 0.2
0.5 0.174675930686682
0.65253578132894 -0.1
0.8 -0.316462225059086
0.898187972934483 -0.4
1.1 -0.558095316909107
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.1 -0.261456405218877
1.4 -0.367687315490992
1.7 -0.355255589056547
2 -0.243551420856727
2.24922169346528 -0.1
2.3 -0.0663034969546733
2.6 0.161698235439875
2.64590620572835 0.2
2.9 0.420713922362942
2.98713459478928 0.5
3.2 0.696535438685732
3.30974353791258 0.8
3.5 0.981691445612048
3.62347379326433 1.1
3.8 1.27439816117138
3.93010471325548 1.4
4.1 1.57129760419598
4.22720881890822 1.7
4.4 1.87015779870175
4.53218873993874 2
4.7 2.17013723478699
4.82469488390853 2.3
5 2.47557738212513
5 2.6
5 2.9
5 3.00852342616264
4.89552281470241 2.9
4.7 2.68796897962821
4.61573785789259 2.6
4.4 2.37918317118655
4.32500389991704 2.3
4.1 2.07317252959768
4.02632917310276 2
3.8 1.78427569536578
3.71769016998044 1.7
3.5 1.48233291975787
3.41413532401567 1.4
3.2 1.19877859110409
3.10181005421994 1.1
2.9 0.899031440999263
2.79761937995992 0.8
2.6 0.628836480518914
2.45242385747019 0.5
2.3 0.382060807437429
2.05770008938669 0.2
2 0.162017592079876
1.7 0.0295043466655127
1.4 -0.00359153984248853
1.1 0.111508276801587
1.01641805642033 0.2
0.810476324391026 0.5
0.8 0.520902146227397
0.718943130029958 0.8
0.672752098448708 1.1
0.646422245731174 1.4
0.628859290099853 1.7
0.620685640372761 2
0.614690038491022 2.3
0.61176954805241 2.6
0.609177037955735 2.9
0.607911385789179 3.2
0.605014625646999 3.5
0.608386343885374 3.8
0.607338140938079 4.1
0.608946733468905 4.4
0.609209228293832 4.7
0.606542599115207 5
0.5 5
0.421876955832227 5
0.423831137303865 4.7
0.423789478422166 4.4
0.423785748944826 4.1
0.423630446333005 3.8
0.421818877814315 3.5
0.423500311073272 3.2
0.424079833689986 2.9
0.426659466670909 2.6
0.428779598393745 2.3
0.431082633848183 2
0.437056838682047 1.7
0.448020039730475 1.4
0.46780524111108 1.1
0.496866999059426 0.8
0.5 0.782913579429241
0.582957216849879 0.5
0.701024333689034 0.2
0.8 0.0138406579356853
0.907768006355786 -0.1
1.1 -0.261456405218877
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
1.1 0.111508276801587
1.4 -0.00359153984248853
1.7 0.0295043466655127
2 0.162017592079876
2.05770008938669 0.2
2.3 0.382060807437429
2.45242385747019 0.5
2.6 0.628836480518914
2.79761937995992 0.8
2.9 0.899031440999263
3.10181005421994 1.1
3.2 1.19877859110409
3.41413532401567 1.4
3.5 1.48233291975787
3.71769016998043 1.7
3.8 1.78427569536578
4.02632917310276 2
4.1 2.07317252959768
4.32500389991704 2.3
4.4 2.37918317118655
4.61573785789259 2.6
4.7 2.68796897962821
4.89552281470241 2.9
5 3.00852342616264
5 3.2
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.1 5
3.84845398692897 5
3.89633532245727 4.7
3.9230730807588 4.4
3.91564142401963 4.1
3.87217199039526 3.8
3.8 3.62697748503488
3.76501403858078 3.5
3.73316183109079 3.2
3.66303109342247 2.9
3.5 2.61422894998258
3.49463221656965 2.6
3.33953776013555 2.3
3.2 2.13042906753937
3.11701093189469 2
2.90603518946809 1.7
2.9 1.69323597178435
2.68807077565547 1.4
2.6 1.31229571528266
2.40268181597842 1.1
2.3 0.994301715290334
2.10409200332991 0.8
2 0.713316219013126
1.7 0.541920941050087
1.48471548947478 0.5
1.4 0.486047911807822
1.37218344991421 0.5
1.1 0.717232704941113
1.06090357219946 0.8
0.973769028405711 1.1
0.927138482945144 1.4
0.899809098816056 1.7
0.888793642266197 2
0.875340175150486 2.3
0.871629483957066 2.6
0.870265549354729 2.9
0.870680502720189 3.2
0.86611902713886 3.5
0.870292496810171 3.8
0.86271838968263 4.1
0.871294500451066 4.4
0.874094501229564 4.7
0.86797683475466 5
0.8 5
0.606542599115207 5
0.609209228293832 4.7
0.608946733468905 4.4
0.607338140938079 4.1
0.608386343885374 3.8
0.605014625646999 3.5
0.607911385789179 3.2
0.609177037955735 2.9
0.61176954805241 2.6
0.614690038491022 2.3
0.620685640372761 2
0.628859290099853 1.7
0.646422245731174 1.4
0.672752098448708 1.1
0.718943130029958 0.8
0.8 0.520902146227397
0.810476324391026 0.5
1.01641805642033 0.2
1.1 0.111508276801587
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
1.4 0.486047911807822
1.48471548947478 0.5
1.7 0.541920941050087
2 0.713316219013126
2.10409200332991 0.8
2.3 0.994301715290334
2.40268181597842 1.1
2.6 1.31229571528266
2.68807077565547 1.4
2.9 1.69323597178435
2.90603518946809 1.7
3.11701093189469 2
3.2 2.13042906753937
3.33953776013555 2.3
3.49463221656965 2.6
3.5 2.61422894998258
3.66303109342247 2.9
3.73316183109079 3.2
3.76501403858078 3.5
3.8 3.62697748503488
3.87217199039526 3.8
3.91564142401963 4.1
3.9230730807588 4.4
3.89633532245727 4.7
3.84845398692897 5
3.8 5
3.5 5
3.23240775099194 5
3.27586800931827 4.7
3.22476009144267 4.4
3.20509800959199 4.1
3.2 4.0708463971735
3.13747765018091 3.8
3.02824170068408 3.5
2.92102572542285 3.2
2.9 3.15002633775272
2.76354004156317 2.9
2.65087028247294 2.6
2.6 2.49373190137104
2.48021923021842 2.3
2.3 2.02092883179715
2.27953722625003 2
2.04848119598444 1.7
2 1.64495399677673
1.7 1.49250799230782
1.50163703156589 1.7
1.42614370101364 2
1.44567102695707 2.3
1.4030708420485 2.6
1.4 2.65869204585387
1.39329564934742 2.9
1.38033131548872 3.2
1.39562153839263 3.5
1.4 3.55453742600314
1.43849775811476 3.8
1.41504433934054 4.1
1.4 4.35515869149099
1.39838139014789 4.4
1.39924766278661 4.7
1.4 4.7098789096789
1.43521618449869 5
1.4 5
1.1 5
0.86797683475466 5
0.874094501229564 4.7
0.871294500451066 4.4
0.86271838968263 4.1
0.870292496810171 3.8
0.86611902713886 3.5
0.870680502720189 3.2
0.870265549354729 2.9
0.871629483957066 2.6
0.875340175150486 2.3
0.888793642266197 2
0.899809098816056 1.7
0.927138482945144 1.4
0.97376902840571 1.1
1.06090357219946 0.8
1.1 0.717232704941113
1.37218344991421 0.5
1.4 0.486047911807822
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
1.7 1.49250799230782
2 1.64495399677673
2.04848119598444 1.7
2.27953722625003 2
2.3 2.02092883179715
2.48021923021842 2.3
2.6 2.49373190137104
2.65087028247294 2.6
2.76354004156317 2.9
2.9 3.15002633775272
2.92102572542285 3.2
3.02824170068408 3.5
3.13747765018091 3.8
3.2 4.0708463971735
3.20509800959199 4.1
3.22476009144267 4.4
3.27586800931827 4.7
3.23240775099194 5
3.2 5
2.9 5
2.6 5
2.3 5
2 5
1.7 5
1.43521618449869 5
1.4 4.7098789096789
1.39924766278661 4.7
1.39838139014789 4.4
1.4 4.35515869149099
1.41504433934054 4.1
1.43849775811476 3.8
1.4 3.55453742600314
1.39562153839263 3.5
1.38033131548872 3.2
1.39329564934742 2.9
1.4 2.65869204585387
1.4030708420485 2.6
1.44567102695707 2.3
1.42614370101364 2
1.50163703156588 1.7
1.7 1.49250799230782
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
1.7 4.7
};
\coordinate (CVI_mean_lml_b) at (axis cs:1.6999999999999997,2.0);
\coordinate (CVI_mean_lml_ep_b) at (axis cs:2.0,3.2);
\end{axis}



==> fig/tikz/sonar/CVI_mean_lml.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=black]
table{%
x  y
-0.7 3.16565030043721
-0.4 3.17091381378001
-0.1 3.19824266991304
-0.0942486001410637 3.2
0.2 3.29231335815144
0.471922358501923 3.5
0.5 3.51859334396373
0.720345346548896 3.8
0.8 3.92611704123903
0.876790940550142 4.1
0.980845643324678 4.4
1.08867329877863 4.7
1.1 4.72659559822169
1.207920710135 5
1.1 5
0.8 5
0.5 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 3.1650936820637
-0.7 3.16565030043721
};
\addplot [draw=none, fill=midnightblue854116]
table{%
x  y
-0.7 2.89088668793358
-0.4 2.89526627009248
-0.337507012616309 2.9
-0.1 2.92073964743905
0.2 3.01014565510554
0.451210430741572 3.2
0.5 3.23729836678296
0.687021430583823 3.5
0.8 3.64613015274548
0.882531080047619 3.8
1.01204690245944 4.1
1.1 4.35589055337977
1.11464317466006 4.4
1.21829470676944 4.7
1.33309362557923 5
1.207920710135 5
1.1 4.72659559822169
1.08867329877863 4.7
0.980845643324678 4.4
0.876790940550142 4.1
0.8 3.92611704123903
0.720345346548896 3.8
0.5 3.51859334396373
0.471922358501923 3.5
0.2 3.29231335815144
-0.0942486001410637 3.2
-0.1 3.19824266991304
-0.4 3.17091381378001
-0.7 3.16565030043721
-1 3.1650936820637
-1 2.9
-1 2.89042375724064
-0.7 2.89088668793358
};
\addplot [draw=none, fill=midnightblue868137]
table{%
x  y
-0.7 2.65030469799627
-0.4 2.65454471840788
-0.1 2.67651731127687
0.2 2.75124681698491
0.433240090120479 2.9
0.5 2.95005507175558
0.676893218482383 3.2
0.8 3.3734039187431
0.865349349892973 3.5
1.02283871127817 3.8
1.1 3.98338135025371
1.14596762453748 4.1
1.24527926216291 4.4
1.34741885770819 4.7
1.4 4.83998377291159
1.46600514976405 5
1.4 5
1.33309362557923 5
1.21829470676944 4.7
1.11464317466006 4.4
1.1 4.35589055337977
1.01204690245944 4.1
0.882531080047619 3.8
0.8 3.64613015274548
0.687021430583823 3.5
0.5 3.23729836678296
0.451210430741572 3.2
0.2 3.01014565510554
-0.1 2.92073964743905
-0.337507012616309 2.9
-0.4 2.89526627009248
-0.7 2.89088668793358
-1 2.89042375724064
-1 2.64985601315158
-0.7 2.65030469799627
};
\addplot [draw=none, fill=teal882156]
table{%
x  y
-0.7 2.3972058660483
-0.4 2.40165619306707
-0.1 2.4246213170148
0.2 2.50151717143843
0.354935041400296 2.6
0.5 2.69064901686043
0.672673066932451 2.9
0.8 3.08190561523297
0.860128068054557 3.2
1.01340885892549 3.5
1.1 3.66953583142273
1.16070904593964 3.8
1.27740565385081 4.1
1.37591534966576 4.4
1.4 4.47116939066614
1.48777408798931 4.7
1.60780277298269 5
1.46600514976405 5
1.4 4.83998377291159
1.34741885770819 4.7
1.24527926216291 4.4
1.14596762453748 4.1
1.1 3.98338135025371
1.02283871127817 3.8
0.865349349892973 3.5
0.8 3.3734039187431
0.676893218482383 3.2
0.5 2.95005507175558
0.433240090120479 2.9
0.2 2.75124681698491
-0.1 2.67651731127687
-0.4 2.65454471840788
-0.7 2.65030469799627
-1 2.64985601315158
-1 2.6
-1 2.3967345649283
-0.7 2.3972058660483
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 2.13212552271346
-0.4 2.1367063539902
-0.1 2.16039322260866
0.2 2.24017715720227
0.290922953338158 2.3
0.5 2.43161351696665
0.641891734097447 2.6
0.8 2.79403115718323
0.860910751477746 2.9
1.01218389866737 3.2
1.1 3.37453428696385
1.15903940501393 3.5
1.29560114089953 3.8
1.4 4.07600504684418
1.41029531648255 4.1
1.5239416994846 4.4
1.63584449685344 4.7
1.7 4.86599080717611
1.76234390357608 5
1.7 5
1.60780277298269 5
1.48777408798931 4.7
1.4 4.47116939066614
1.37591534966576 4.4
1.27740565385081 4.1
1.16070904593964 3.8
1.1 3.66953583142273
1.01340885892549 3.5
0.860128068054557 3.2
0.8 3.08190561523297
0.672673066932451 2.9
0.5 2.69064901686043
0.354935041400296 2.6
0.2 2.50151717143843
-0.1 2.4246213170148
-0.4 2.40165619306707
-0.7 2.3972058660483
-1 2.3967345649283
-1 2.3
-1 2.13164056126656
-0.7 2.13212552271346
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.7 1.85313652533113
-0.4 1.85784932548721
-0.1 1.88218567897288
0.2 1.96406258346848
0.253359434105338 2
0.5 2.16019382454557
0.614297206336496 2.3
0.8 2.52199868536289
0.846627843238075 2.6
1.01673393528742 2.9
1.1 3.06754026937235
1.16271529019778 3.2
1.30124824527315 3.5
1.4 3.7263235702844
1.43562073127217 3.8
1.56330804709567 4.1
1.67589890559435 4.4
1.7 4.46559981075372
1.80614400678066 4.7
1.94057266839029 5
1.76234390357608 5
1.7 4.86599080717611
1.63584449685344 4.7
1.5239416994846 4.4
1.41029531648255 4.1
1.4 4.07600504684418
1.29560114089953 3.8
1.15903940501393 3.5
1.1 3.37453428696385
1.01218389866737 3.2
0.860910751477746 2.9
0.8 2.79403115718323
0.641891734097447 2.6
0.5 2.43161351696665
0.290922953338158 2.3
0.2 2.24017715720227
-0.1 2.16039322260866
-0.4 2.1367063539902
-0.7 2.13212552271346
-1 2.13164056126656
-1 2
-1 1.85263738453046
-0.7 1.85313652533113
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
-0.7 1.54428187718062
-0.4 1.54956647370199
-0.1 1.57683453526659
0.2 1.66847365474418
0.241975865858479 1.7
0.5 1.87130956074727
0.602638257784757 2
0.8 2.24365194324072
0.833007271980905 2.3
1.01066010224549 2.6
1.1 2.76173096195678
1.17136904486693 2.9
1.31116276421426 3.2
1.4 3.39859179759942
1.45071679183306 3.5
1.59319518770105 3.8
1.7 4.0592094865101
1.72068762913174 4.1
1.86081848339749 4.4
1.99343834201339 4.7
2 4.71498028141542
2.15483769397642 5
2 5
1.94057266839029 5
1.80614400678066 4.7
1.7 4.46559981075372
1.67589890559435 4.4
1.56330804709567 4.1
1.43562073127217 3.8
1.4 3.7263235702844
1.30124824527315 3.5
1.16271529019778 3.2
1.1 3.06754026937235
1.01673393528742 2.9
0.846627843238075 2.6
0.8 2.52199868536289
0.614297206336496 2.3
0.5 2.16019382454557
0.253359434105338 2
0.2 1.96406258346848
-0.1 1.88218567897288
-0.4 1.85784932548721
-0.7 1.85313652533113
-1 1.85263738453046
-1 1.7
-1 1.54372201205149
-0.7 1.54428187718062
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
-0.7 1.16313811512378
-0.4 1.16938709018504
-0.1 1.20168318499783
0.2 1.31094746831912
0.298100394251755 1.4
0.5 1.54996803725865
0.607541705838146 1.7
0.8 1.94444025213364
0.831610797717693 2
1.00584722013473 2.3
1.1 2.46340698002118
1.17350464030511 2.6
1.32464072840415 2.9
1.4 3.06513275130281
1.46971901691573 3.2
1.61668227386878 3.5
1.7 3.68272644847351
1.76474202748528 3.8
1.91464104727391 4.1
2 4.28545935408717
2.06640431781542 4.4
2.23159481101734 4.7
2.3 4.82953344438569
2.41121151331232 5
2.3 5
2.15483769397642 5
2 4.71498028141542
1.99343834201339 4.7
1.86081848339749 4.4
1.72068762913174 4.1
1.7 4.0592094865101
1.59319518770105 3.8
1.45071679183306 3.5
1.4 3.39859179759942
1.31116276421426 3.2
1.17136904486693 2.9
1.1 2.76173096195678
1.01066010224549 2.6
0.833007271980905 2.3
0.8 2.24365194324072
0.602638257784757 2
0.5 1.87130956074727
0.241975865858479 1.7
0.2 1.66847365474418
-0.1 1.57683453526659
-0.4 1.54956647370199
-0.7 1.54428187718062
-1 1.54372201205149
-1 1.4
-1 1.16247618453207
-0.7 1.16313811512378
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
-0.7 0.438163017198231
-0.4 0.461607707922988
-0.308171447021435 0.5
-0.1 0.543588956628419
0.2 0.775943700284208
0.211702129295929 0.8
0.45221936868635 1.1
0.5 1.14315670516344
0.650913349315266 1.4
0.8 1.61228116234583
0.844875301553291 1.7
1.01303695810234 2
1.1 2.15386317524843
1.17816769863482 2.3
1.33492853954362 2.6
1.4 2.73268347467073
1.49200897876112 2.9
1.64334039906806 3.2
1.7 3.31876675233928
1.80514930153258 3.5
1.96568276606892 3.8
2 3.87011917208201
2.14076731763387 4.1
2.3 4.38057884192098
2.31367107868454 4.4
2.51656105028311 4.7
2.6 4.82938284890714
2.73548204641565 5
2.6 5
2.41121151331232 5
2.3 4.82953344438569
2.23159481101734 4.7
2.06640431781542 4.4
2 4.28545935408717
1.91464104727391 4.1
1.76474202748528 3.8
1.7 3.68272644847351
1.61668227386878 3.5
1.46971901691573 3.2
1.4 3.06513275130281
1.32464072840415 2.9
1.17350464030511 2.6
1.1 2.46340698002118
1.00584722013473 2.3
0.831610797717693 2
0.8 1.94444025213364
0.607541705838146 1.7
0.5 1.54996803725865
0.298100394251755 1.4
0.2 1.31094746831912
-0.1 1.20168318499783
-0.4 1.16938709018504
-0.7 1.16313811512378
-1 1.16247618453207
-1 1.1
-1 0.8
-1 0.5
-1 0.435718225846365
-0.7 0.438163017198231
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
-0.7 -1
-0.4 -1
-0.1 -1
0.2 -1
0.5 -1
0.8 -1
1.1 -1
1.2131293391408 -1
1.1 -0.900167807023832
0.942885305110445 -0.7
0.8 -0.450764187603198
0.771055657208888 -0.4
0.641286886626531 -0.1
0.581357867451718 0.2
0.580288024760002 0.5
0.63789165427519 0.8
0.752513873251945 1.1
0.8 1.18428095315865
0.888917521490762 1.4
1.0371128319915 1.7
1.1 1.81575785502356
1.19522776283371 2
1.34986660804023 2.3
1.4 2.3985462390628
1.51485060111972 2.6
1.6730118603799 2.9
1.7 2.95436679892524
1.84874567401374 3.2
2 3.46961609737443
2.02103788093293 3.5
2.21621479569943 3.8
2.3 3.94011777901665
2.4181329106218 4.1
2.6 4.3620161970505
2.63249896332277 4.4
2.878235337858 4.7
2.9 4.72762166940641
3.16691876531098 5
2.9 5
2.73548204641565 5
2.6 4.82938284890714
2.51656105028311 4.7
2.31367107868454 4.4
2.3 4.38057884192098
2.14076731763387 4.1
2 3.87011917208201
1.96568276606892 3.8
1.80514930153258 3.5
1.7 3.31876675233928
1.64334039906806 3.2
1.49200897876112 2.9
1.4 2.73268347467073
1.33492853954362 2.6
1.17816769863482 2.3
1.1 2.15386317524843
1.01303695810234 2
0.844875301553291 1.7
0.8 1.61228116234583
0.650913349315266 1.4
0.5 1.14315670516344
0.45221936868635 1.1
0.211702129295929 0.8
0.2 0.775943700284208
-0.1 0.543588956628419
-0.308171447021435 0.5
-0.4 0.461607707922988
-0.7 0.438163017198231
-1 0.435718225846365
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
2.9 -1
3.2 -1
3.5 -1
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.5
5 0.8
5 1.1
5 1.15667498979421
4.94712574863099 1.1
4.7 0.834642207964992
4.66732540609385 0.8
4.4 0.515671067350475
4.384943343264 0.5
4.1 0.20169820388912
4.098317192437 0.2
3.80560822302211 -0.1
3.8 -0.105885491558224
3.5 -0.39786666170763
3.49757834027223 -0.4
3.2 -0.67231399622598
3.16384725869458 -0.7
2.9 -0.917055423321227
2.76309505079241 -1
2.9 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.1 -0.900167807023832
1.2131293391408 -1
1.4 -1
1.7 -1
2 -1
2.3 -1
2.6 -1
2.76309505079241 -1
2.9 -0.917055423321227
3.16384725869458 -0.7
3.2 -0.67231399622598
3.49757834027224 -0.4
3.5 -0.39786666170763
3.8 -0.105885491558224
3.80560822302211 -0.1
4.098317192437 0.2
4.1 0.20169820388912
4.384943343264 0.5
4.4 0.515671067350475
4.66732540609385 0.8
4.7 0.834642207964992
4.94712574863099 1.1
5 1.15667498979421
5 1.4
5 1.7
5 1.71034934933941
4.99027231726601 1.7
4.70745751846803 1.4
4.7 1.39208649534584
4.42247022939667 1.1
4.4 1.0763823254895
4.13325538351133 0.8
4.1 0.765599391203105
3.83675090668296 0.5
3.8 0.462967333588238
3.52732572734617 0.2
3.5 0.173609992505097
3.2 -0.0949411139956128
3.19381793259053 -0.1
2.9 -0.337793998333101
2.80611956976964 -0.4
2.6 -0.539022465563873
2.3 -0.6758840497638
2.18669979232651 -0.7
2 -0.744550550587058
1.7 -0.714195521106328
1.67190417676363 -0.7
1.4 -0.565623870323472
1.23851729003426 -0.4
1.1 -0.217400953989837
1.03364651713125 -0.1
0.925577163842954 0.2
0.886766601022368 0.5
0.908213299093222 0.8
0.981302652094586 1.1
1.093288544425 1.4
1.1 1.41396028444942
1.23244200611762 1.7
1.37812250153874 2
1.4 2.04335903114193
1.5464707691359 2.3
1.7 2.58547537967538
1.70950710183498 2.6
1.89869155915179 2.9
2 3.07381207684743
2.09078286648391 3.2
2.29355891632677 3.5
2.3 3.51009610362941
2.5274429552544 3.8
2.6 3.89961315606966
2.7805936082846 4.1
2.9 4.24060406006906
3.07123119146831 4.4
3.2 4.52587462844697
3.43666688535206 4.7
3.5 4.7487642131677
3.8 4.90086911755811
4.1 4.97276018064431
4.4 4.94518873993666
4.7 4.88179818920552
5 4.91796868771343
5 5
4.7 5
4.4 5
4.1 5
3.8 5
3.5 5
3.2 5
3.16691876531098 5
2.9 4.72762166940641
2.878235337858 4.7
2.63249896332277 4.4
2.6 4.3620161970505
2.4181329106218 4.1
2.3 3.94011777901665
2.21621479569943 3.8
2.02103788093293 3.5
2 3.46961609737443
1.84874567401374 3.2
1.7 2.95436679892524
1.6730118603799 2.9
1.51485060111972 2.6
1.4 2.3985462390628
1.34986660804023 2.3
1.19522776283371 2
1.1 1.81575785502356
1.0371128319915 1.7
0.888917521490762 1.4
0.8 1.18428095315865
0.752513873251945 1.1
0.63789165427519 0.8
0.580288024760002 0.5
0.581357867451718 0.2
0.641286886626531 -0.1
0.771055657208888 -0.4
0.8 -0.450764187603198
0.942885305110445 -0.7
1.1 -0.900167807023832
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.7 -0.714195521106328
2 -0.744550550587058
2.18669979232651 -0.7
2.3 -0.6758840497638
2.6 -0.539022465563873
2.80611956976964 -0.4
2.9 -0.337793998333101
3.19381793259053 -0.1
3.2 -0.0949411139956128
3.5 0.173609992505097
3.52732572734617 0.2
3.8 0.462967333588238
3.83675090668296 0.5
4.1 0.765599391203105
4.13325538351133 0.8
4.4 1.0763823254895
4.42247022939667 1.1
4.7 1.39208649534584
4.70745751846803 1.4
4.99027231726601 1.7
5 1.71034934933941
5 2
5 2.23123701727786
4.78551004410833 2
4.7 1.90854283606952
4.50604064476904 1.7
4.4 1.58745481975873
4.22460242936169 1.4
4.1 1.26950213529561
3.93928957680448 1.1
3.8 0.957407581098489
3.64652596754113 0.8
3.5 0.655698000749445
3.33943150277515 0.5
3.2 0.371359461883217
3.00330822728244 0.2
2.9 0.114562193172056
2.6 -0.0997601058587612
2.59956095536763 -0.1
2.3 -0.253902485501411
2 -0.326649998149026
1.7 -0.28906966546191
1.41598316362667 -0.1
1.4 -0.0858736826294364
1.23235589953205 0.2
1.15058600948813 0.5
1.1479338780053 0.8
1.20664692463604 1.1
1.306560632164 1.4
1.4 1.62388975752689
1.43712338748063 1.7
1.59825056891319 2
1.7 2.19099834310359
1.77146652408461 2.3
1.96129162890873 2.6
2 2.66406714684089
2.1765638779536 2.9
2.3 3.07724811218651
2.4060028459608 3.2
2.6 3.43923088217092
2.66175005250593 3.5
2.9 3.75032106085655
2.96199237962638 3.8
3.2 4.00413523169426
3.36111338783374 4.1
3.5 4.18866227194038
3.8 4.27718123534228
4.1 4.24516825574532
4.4 4.15585524335524
4.7 4.17341728740406
5 4.30723579481908
5 4.4
5 4.7
5 4.91796868771343
4.7 4.88179818920552
4.4 4.94518873993666
4.1 4.97276018064431
3.8 4.90086911755811
3.5 4.7487642131677
3.43666688535206 4.7
3.2 4.52587462844697
3.07123119146831 4.4
2.9 4.24060406006906
2.7805936082846 4.1
2.6 3.89961315606966
2.5274429552544 3.8
2.3 3.51009610362941
2.29355891632677 3.5
2.09078286648391 3.2
2 3.07381207684743
1.89869155915179 2.9
1.70950710183498 2.6
1.7 2.58547537967538
1.5464707691359 2.3
1.4 2.04335903114193
1.37812250153874 2
1.23244200611762 1.7
1.1 1.41396028444942
1.093288544425 1.4
0.981302652094586 1.1
0.908213299093222 0.8
0.886766601022368 0.5
0.925577163842954 0.2
1.03364651713125 -0.1
1.1 -0.217400953989837
1.23851729003426 -0.4
1.4 -0.565623870323472
1.67190417676363 -0.7
1.7 -0.714195521106328
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.7 -0.28906966546191
2 -0.326649998149026
2.3 -0.253902485501411
2.59956095536763 -0.1
2.6 -0.0997601058587612
2.9 0.114562193172056
3.00330822728244 0.2
3.2 0.371359461883217
3.33943150277515 0.5
3.5 0.655698000749445
3.64652596754113 0.8
3.8 0.957407581098489
3.93928957680448 1.1
4.1 1.26950213529561
4.22460242936169 1.4
4.4 1.58745481975873
4.50604064476904 1.7
4.7 1.90854283606952
4.78551004410833 2
5 2.23123701727786
5 2.3
5 2.6
5 2.9
5 3.2
5 3.5
5 3.8
5 4.1
5 4.30723579481908
4.7 4.17341728740406
4.4 4.15585524335524
4.1 4.24516825574532
3.8 4.27718123534228
3.5 4.18866227194038
3.36111338783374 4.1
3.2 4.00413523169426
2.96199237962638 3.8
2.9 3.75032106085655
2.66175005250593 3.5
2.6 3.43923088217092
2.4060028459608 3.2
2.3 3.07724811218651
2.1765638779536 2.9
2 2.66406714684089
1.96129162890873 2.6
1.77146652408461 2.3
1.7 2.19099834310359
1.59825056891319 2
1.43712338748063 1.7
1.4 1.62388975752689
1.306560632164 1.4
1.20664692463604 1.1
1.1479338780053 0.8
1.15058600948813 0.5
1.23235589953205 0.2
1.4 -0.0858736826294364
1.41598316362667 -0.1
1.7 -0.28906966546191

1.65640678283951 0.2
1.45841070607948 0.5
1.40800095289737 0.8
1.45598041772459 1.1
1.55868243761597 1.4
1.68673101915187 1.7
1.7 1.72652154461201
1.8721897291322 2
2 2.20962784893182
2.07082179784428 2.3
2.2936913503519 2.6
2.3 2.60876221330457
2.56495160956995 2.9
2.6 2.94146356293913
2.88380976033025 3.2
2.9 3.21588883023736
3.2 3.40852296555317
3.5 3.49904155185025
3.8 3.39950955591518
4.1 3.20757721777964
4.13813164579534 3.2
4.4 3.11353999095216
4.7 3.02730025030332
4.72913443362536 2.9
4.7 2.85672406151205
4.55310284308308 2.6
4.4 2.37476145089384
4.35811104091694 2.3
4.13430465873339 2
4.1 1.95988621329979
3.89706607525963 1.7
3.8 1.58772472176675
3.65230163236658 1.4
3.5 1.22868987832621
3.39396131143162 1.1
3.2 0.894195470126802
3.11373258239129 0.8
2.9 0.596685280926324
2.7919903342488 0.5
2.6 0.349720507420937
2.35763902276695 0.2
2.3 0.168379271221777
2 0.0929066580955489
1.7 0.160757600723371
1.65640678283951 0.2
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.7 0.160757600723371
2 0.0929066580955489
2.3 0.168379271221777
2.35763902276695 0.2
2.6 0.349720507420937
2.7919903342488 0.5
2.9 0.596685280926324
3.11373258239129 0.8
3.2 0.894195470126802
3.39396131143162 1.1
3.5 1.22868987832621
3.65230163236658 1.4
3.8 1.58772472176675
3.89706607525963 1.7
4.1 1.95988621329979
4.13430465873339 2
4.35811104091694 2.3
4.4 2.37476145089384
4.55310284308308 2.6
4.7 2.85672406151205
4.72913443362536 2.9
4.7 3.02730025030332
4.4 3.11353999095216
4.13813164579534 3.2
4.1 3.20757721777964
3.8 3.39950955591518
3.5 3.49904155185024
3.2 3.40852296555317
2.9 3.21588883023736
2.88380976033025 3.2
2.6 2.94146356293913
2.56495160956995 2.9
2.3 2.60876221330457
2.2936913503519 2.6
2.07082179784428 2.3
2 2.20962784893182
1.8721897291322 2
1.7 1.72652154461201
1.68673101915187 1.7
1.55868243761597 1.4
1.45598041772459 1.1
1.40800095289737 0.8
1.45841070607948 0.5
1.65640678283951 0.2
1.7 0.160757600723371

1.8968231021778 0.8
1.85050684873016 1.1
1.92891556421659 1.4
2 1.55937787965493
2.09371291978104 1.7
2.29697102829639 2
2.3 2.00413945932581
2.6 2.29485828233551
2.61152081860939 2.3
2.9 2.44095114629279
3.17490187342644 2.3
3.19892858082429 2
3.10483741415373 1.7
2.95555308899522 1.4
2.9 1.32217098390495
2.73143195526586 1.1
2.6 0.959932590584673
2.4036757175606 0.8
2.3 0.731092095611878
2 0.693540535064607
1.8968231021778 0.8
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
2 0.693540535064607
2.3 0.731092095611878
2.4036757175606 0.8
2.6 0.959932590584673
2.73143195526586 1.1
2.9 1.32217098390495
2.95555308899522 1.4
3.10483741415373 1.7
3.19892858082429 2
3.17490187342644 2.3
2.9 2.44095114629279
2.61152081860939 2.3
2.6 2.29485828233551
2.3 2.00413945932581
2.29697102829639 2
2.09371291978104 1.7
2 1.55937787965493
1.92891556421659 1.4
1.85050684873016 1.1
1.8968231021778 0.8
2 0.693540535064607
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.3 1.4
};
\coordinate (CVI_mean_lml_t) at (axis cs:2.3,1.4);
\end{axis}



==> fig/tikz/sonar/CVI_mean_lml_ep.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
-0.7 -1
-0.4 -1
-0.1 -1
0.2 -1
0.5 -1
0.8 -1
1.1 -1
1.21295824196119 -1
1.1 -0.900557660997067
0.94219469441135 -0.7
0.8 -0.455950677282548
0.767580604364458 -0.4
0.630198648619474 -0.1
0.54970977188049 0.2
0.502497191689195 0.5
0.5 0.525596097192026
0.456819506180673 0.8
0.437703258641597 1.1
0.460317829182174 1.4
0.5 1.55375947945086
0.519520958404101 1.7
0.567172395141058 2
0.601909859005566 2.3
0.623729785521208 2.6
0.638253970377723 2.9
0.648285061057222 3.2
0.656946057927524 3.5
0.667167230180885 3.8
0.675347061725806 4.1
0.678684419381215 4.4
0.67704193751093 4.7
0.673454691676556 5
0.5 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
2.9 -1
3.2 -1
3.5 -1
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.5
5 0.8
5 1.1
5 1.15666076539897
4.94713864227741 1.1
4.7 0.834630011646976
4.66733666717823 0.8
4.4 0.515660740512926
4.38495314567039 0.5
4.1 0.201689475309697
4.09832582718239 0.2
3.80561835342575 -0.1
3.8 -0.105896109471668
3.5 -0.39787365135669
3.49758624847359 -0.4
3.2 -0.672321082277539
3.16385612956399 -0.7
2.9 -0.917063113853185
2.76310661983596 -1
2.9 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.1 -0.900557660997067
1.21295824196119 -1
1.4 -1
1.7 -1
2 -1
2.3 -1
2.6 -1
2.76310661983596 -1
2.9 -0.917063113853185
3.16385612956399 -0.7
3.2 -0.672321082277539
3.49758624847359 -0.4
3.5 -0.39787365135669
3.8 -0.105896109471669
3.80561835342575 -0.1
4.09832582718239 0.2
4.1 0.201689475309697
4.38495314567039 0.5
4.4 0.515660740512926
4.66733666717823 0.8
4.7 0.834630011646976
4.94713864227741 1.1
5 1.15666076539897
5 1.4
5 1.7
5 1.71025066316714
4.9903647493885 1.7
4.70754560837212 1.4
4.7 1.39199313212583
4.4225547793237 1.1
4.4 1.076293766744
4.13333678239064 0.8
4.1 0.765515576703005
3.8368296752597 0.5
3.8 0.462888271151609
3.52740258603426 0.2
3.5 0.173535869078466
3.2 -0.0950042663639224
3.19389484483189 -0.1
2.9 -0.33786622187703
2.80622473061675 -0.4
2.6 -0.53910363982718
2.3 -0.675967841089494
2.18714240211246 -0.7
2 -0.744689817663412
1.7 -0.714476460020128
1.67129953105533 -0.7
1.4 -0.566746055878361
1.23630780652892 -0.4
1.1 -0.226505900033944
1.02590055239924 -0.1
0.902286268317637 0.2
0.827905513604234 0.5
0.8 0.687068479433827
0.780532390408277 0.8
0.753770953836983 1.1
0.755417026856847 1.4
0.784538882264389 1.7
0.8 1.81429314039651
0.819069108785462 2
0.844911858220069 2.3
0.864149212252196 2.6
0.878078300507822 2.9
0.887663413204969 3.2
0.896966204632867 3.5
0.906110566006993 3.8
0.913192256349447 4.1
0.916183723295225 4.4
0.916582830690603 4.7
0.912984635210765 5
0.8 5
0.673454691676556 5
0.67704193751093 4.7
0.678684419381215 4.4
0.675347061725806 4.1
0.667167230180885 3.8
0.656946057927524 3.5
0.648285061057222 3.2
0.638253970377723 2.9
0.623729785521208 2.6
0.601909859005566 2.3
0.567172395141058 2
0.519520958404101 1.7
0.5 1.55375947945086
0.460317829182174 1.4
0.437703258641597 1.1
0.456819506180673 0.8
0.5 0.525596097192026
0.502497191689195 0.5
0.54970977188049 0.2
0.630198648619474 -0.1
0.767580604364458 -0.4
0.8 -0.455950677282548
0.94219469441135 -0.7
1.1 -0.900557660997067
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.7 -0.714476460020128
2 -0.744689817663412
2.18714240211246 -0.7
2.3 -0.675967841089494
2.6 -0.53910363982718
2.80622473061675 -0.4
2.9 -0.33786622187703
3.19389484483189 -0.1
3.2 -0.0950042663639224
3.5 0.173535869078466
3.52740258603426 0.2
3.8 0.462888271151609
3.8368296752597 0.5
4.1 0.765515576703005
4.13333678239064 0.8
4.4 1.076293766744
4.4225547793237 1.1
4.7 1.39199313212583
4.70754560837212 1.4
4.9903647493885 1.7
5 1.71025066316714
5 2
5 2.23057919224633
4.78610103755152 2
4.7 1.90792006280571
4.50660548288716 1.7
4.4 1.5868656657135
4.22514437585977 1.4
4.1 1.26894440317701
3.9398138532781 1.1
3.8 0.956877953025448
3.6470412841372 0.8
3.5 0.655191787461548
3.33995293526862 0.5
3.2 0.370871392909845
3.00386340826984 0.2
2.9 0.114090426139545
2.60030541602561 -0.1
2.6 -0.100210014385939
2.3 -0.254564591539806
2 -0.327667491673999
1.7 -0.291463549704914
1.4053854319494 -0.1
1.4 -0.095633369646424
1.21010105300554 0.2
1.1 0.474700875092839
1.09191002517998 0.5
1.03003866305471 0.8
0.997081922825104 1.1
0.988352259374929 1.4
1.00005649978758 1.7
1.02023621856976 2
1.03928941798055 2.3
1.05754692990798 2.6
1.07228897037141 2.9
1.0820017495192 3.2
1.09369888679759 3.5
1.1 3.72179423149186
1.10249625391905 3.8
1.10946038879408 4.1
1.11208160943657 4.4
1.11238089164188 4.7
1.10627159142114 5
1.1 5
0.912984635210765 5
0.916582830690603 4.7
0.916183723295225 4.4
0.913192256349447 4.1
0.906110566006993 3.8
0.896966204632867 3.5
0.887663413204969 3.2
0.878078300507822 2.9
0.864149212252196 2.6
0.844911858220069 2.3
0.819069108785462 2
0.8 1.81429314039651
0.784538882264389 1.7
0.755417026856847 1.4
0.753770953836983 1.1
0.780532390408277 0.8
0.8 0.687068479433827
0.827905513604234 0.5
0.902286268317638 0.2
1.02590055239924 -0.1
1.1 -0.226505900033944
1.23630780652892 -0.4
1.4 -0.566746055878361
1.67129953105533 -0.7
1.7 -0.714476460020128
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
4.7 4.30405839673397
5 4.38367837208333
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.26477319438192 5
4.34593311191188 4.7
4.4 4.55603480411107
4.53912336739425 4.4
4.7 4.30405839673397
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.7 -0.291463549704914
2 -0.327667491673999
2.3 -0.254564591539806
2.6 -0.100210014385939
2.60030541602561 -0.1
2.9 0.114090426139545
3.00386340826984 0.2
3.2 0.370871392909845
3.33995293526862 0.5
3.5 0.655191787461548
3.6470412841372 0.8
3.8 0.956877953025448
3.9398138532781 1.1
4.1 1.26894440317701
4.22514437585977 1.4
4.4 1.5868656657135
4.50660548288716 1.7
4.7 1.90792006280571
4.78610103755152 2
5 2.23057919224633
5 2.3
5 2.6
5 2.9
5 3.2
5 3.5
5 3.8
5 4.1
5 4.38367837208333
4.7 4.30405839673397
4.53912336739425 4.4
4.4 4.55603480411107
4.34593311191188 4.7
4.26477319438192 5
4.1 5
3.8 5
3.78036493047596 5
3.8 4.84220817467759
3.81364493863215 4.7
3.84314509688166 4.4
3.88975100275971 4.1
3.96121260470699 3.8
4.06760329218514 3.5
4.1 3.42579408990918
4.4 3.21790897670276
4.7 3.20509116644694
4.71879537986505 3.2
4.75085588254628 2.9
4.7 2.82574451428269
4.56827947804742 2.6
4.4 2.35610378973323
4.36803027974883 2.3
4.14013863034766 2
4.1 1.95313776248712
3.90211688715918 1.7
3.8 1.58204402579417
3.65667153671691 1.4
3.5 1.22395608613735
3.39783893556414 1.1
3.2 0.890172406769838
3.11743563416258 0.8
2.9 0.593036585033442
2.79614601575597 0.5
2.6 0.346106961783132
2.36399082249044 0.2
2.3 0.164715504968296
2 0.0862805191134525
1.7 0.144953781026729
1.63385976869788 0.2
1.4 0.478222419417511
1.39002082769652 0.5
1.30038371083266 0.8
1.25055912156767 1.1
1.22941400531587 1.4
1.22923534786882 1.7
1.23986635905758 2
1.25517354153817 2.3
1.27247607716694 2.6
1.28742897978283 2.9
1.29850602713858 3.2
1.30869483897856 3.5
1.32353044029199 3.8
1.34056383445612 4.1
1.34319084008117 4.4
1.34059203936101 4.7
1.33823411801729 5
1.10627159142114 5
1.11238089164188 4.7
1.11208160943657 4.4
1.10946038879408 4.1
1.10249625391905 3.8
1.1 3.72179423149186
1.09369888679759 3.5
1.0820017495192 3.2
1.07228897037141 2.9
1.05754692990798 2.6
1.03928941798055 2.3
1.02023621856976 2
1.00005649978758 1.7
0.988352259374929 1.4
0.997081922825104 1.1
1.03003866305471 0.8
1.09191002517998 0.5
1.1 0.474700875092839
1.21010105300554 0.2
1.4 -0.095633369646424
1.4053854319494 -0.1
1.7 -0.291463549704914
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.7 0.144953781026729
2 0.0862805191134524
2.3 0.164715504968296
2.36399082249044 0.2
2.6 0.346106961783132
2.79614601575597 0.5
2.9 0.593036585033442
3.11743563416258 0.8
3.2 0.890172406769838
3.39783893556414 1.1
3.5 1.22395608613735
3.65667153671691 1.4
3.8 1.58204402579417
3.90211688715918 1.7
4.1 1.95313776248712
4.14013863034766 2
4.36803027974883 2.3
4.4 2.35610378973323
4.56827947804742 2.6
4.7 2.82574451428269
4.75085588254628 2.9
4.71879537986505 3.2
4.7 3.20509116644694
4.4 3.21790897670276
4.1 3.42579408990918
4.06760329218514 3.5
3.96121260470699 3.8
3.88975100275971 4.1
3.84314509688166 4.4
3.81364493863215 4.7
3.8 4.84220817467759
3.78036493047596 5
3.5 5
3.2 5
3.02723140574978 5
3.16348811830552 4.7
3.2 4.58088542173194
3.22972691472713 4.4
3.2764545295654 4.1
3.32199824742544 3.8
3.3527339848198 3.5
3.37675690223211 3.2
3.39140192058597 2.9
3.39029859846506 2.6
3.36168613598698 2.3
3.28938926011656 2
3.2 1.7863290589273
3.16601729266619 1.7
2.99666867752635 1.4
2.9 1.26813830305868
2.77084812346828 1.1
2.6 0.918634899386146
2.45722860188643 0.8
2.3 0.691455578444042
2 0.611065078320588
1.7 0.778338495897648
1.68775860760649 0.8
1.58498513468872 1.1
1.53283634972871 1.4
1.51200709117208 1.7
1.51088968472872 2
1.52490623974236 2.3
1.54680226831163 2.6
1.5702917196614 2.9
1.59330689375931 3.2
1.6211853533581 3.5
1.6480266638657 3.8
1.6714365690762 4.1
1.67856551892882 4.4
1.68579042126681 4.7
1.6949078179837 5
1.4 5
1.33823411801729 5
1.34059203936101 4.7
1.34319084008117 4.4
1.34056383445612 4.1
1.32353044029199 3.8
1.30869483897856 3.5
1.29850602713858 3.2
1.28742897978283 2.9
1.27247607716694 2.6
1.25517354153817 2.3
1.23986635905758 2
1.22923534786882 1.7
1.22941400531587 1.4
1.25055912156767 1.1
1.30038371083266 0.8
1.39002082769652 0.5
1.4 0.478222419417511
1.63385976869788 0.2
1.7 0.144953781026729
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.7 0.778338495897648
2 0.611065078320588
2.3 0.691455578444042
2.45722860188643 0.8
2.6 0.918634899386146
2.77084812346828 1.1
2.9 1.26813830305868
2.99666867752635 1.4
3.16601729266619 1.7
3.2 1.7863290589273
3.28938926011656 2
3.36168613598698 2.3
3.39029859846507 2.6
3.39140192058597 2.9
3.37675690223211 3.2
3.3527339848198 3.5
3.32199824742544 3.8
3.2764545295654 4.1
3.22972691472713 4.4
3.2 4.58088542173194
3.16348811830552 4.7
3.02723140574978 5
2.9 5
2.6 5
2.3 5
2 5
1.7 5
1.6949078179837 5
1.68579042126681 4.7
1.67856551892882 4.4
1.6714365690762 4.1
1.6480266638657 3.8
1.6211853533581 3.5
1.59330689375931 3.2
1.5702917196614 2.9
1.54680226831163 2.6
1.52490623974236 2.3
1.51088968472872 2
1.51200709117208 1.7
1.53283634972871 1.4
1.58498513468872 1.1
1.68775860760649 0.8
1.7 0.778338495897648
};
\addplot [semithick, steelblue31119180, mark=mystar, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.3 2.3
};
\coordinate (CVI_mean_lml_ep_t) at (axis cs:2.3,2.3);
\end{axis}



==> fig/tikz/sonar/CVI_nlpd.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
-0.7 -1
-0.4 -1
-0.1 -1
0.2 -1
0.5 -1
0.8 -1
0.851754565890981 -1
0.8 -0.916544504721435
0.663788010784339 -0.7
0.535655376047085 -0.4
0.5 -0.284131635618716
0.422223065185197 -0.1
0.339709350460476 0.2
0.292383566302578 0.5
0.265519743613348 0.8
0.253475000296209 1.1
0.261842783329571 1.4
0.294833664598799 1.7
0.338142711097179 2
0.37421436558364 2.3
0.399992055514138 2.6
0.408752015113104 2.9
0.418628617445052 3.2
0.433183615004942 3.5
0.425436104202174 3.8
0.409497007416244 4.1
0.404375064854492 4.4
0.405717502571241 4.7
0.421719467290972 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.286190108870508
4.9119688287745 0.2
4.7 -0.00900560776676811
4.60564011641675 -0.1
4.4 -0.300728114912045
4.29441480618319 -0.4
4.1 -0.586598928658204
3.97424124737324 -0.7
3.8 -0.862639531003357
3.63689165102444 -1
3.8 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
0.8 -0.916544504721435
0.851754565890981 -1
1.1 -1
1.31150999789376 -1
1.1 -0.774289330698911
1.04544495549878 -0.7
0.863877382158607 -0.4
0.8 -0.254887093050948
0.728344054708188 -0.1
0.633678766530461 0.2
0.576838087802923 0.5
0.543106779423274 0.8
0.525421393228357 1.1
0.525602235392635 1.4
0.543608485035052 1.7
0.566432060528645 2
0.583097677966866 2.3
0.591149502924966 2.6
0.589395822782406 2.9
0.588686981956009 3.2
0.590237943484404 3.5
0.585021329307306 3.8
0.57721383471722 4.1
0.574361702732874 4.4
0.57497894395621 4.7
0.582196145428018 5
0.5 5
0.421719467290972 5
0.405717502571241 4.7
0.404375064854492 4.4
0.409497007416244 4.1
0.425436104202174 3.8
0.433183615004942 3.5
0.418628617445052 3.2
0.408752015113104 2.9
0.399992055514138 2.6
0.37421436558364 2.3
0.338142711097179 2
0.294833664598799 1.7
0.261842783329571 1.4
0.253475000296209 1.1
0.265519743613348 0.8
0.292383566302578 0.5
0.339709350460476 0.2
0.422223065185197 -0.1
0.5 -0.284131635618716
0.535655376047085 -0.4
0.663788010784339 -0.7
0.8 -0.916544504721435
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
3.2 -1
3.5 -1
3.63689165102444 -1
3.8 -0.862639531003357
3.97424124737324 -0.7
4.1 -0.586598928658204
4.29441480618319 -0.4
4.4 -0.300728114912045
4.60564011641675 -0.1
4.7 -0.00900560776676812
4.9119688287745 0.2
5 0.286190108870508
5 0.5
5 0.8
5 0.825006268131743
4.97456718450442 0.8
4.7 0.529517658947304
4.66960753191868 0.5
4.4 0.237241035459002
4.36085164983148 0.2
4.1 -0.0497231328847067
4.04528011860334 -0.1
3.8 -0.328033462366687
3.71699563056252 -0.4
3.5 -0.592361694695171
3.3631703033812 -0.7
3.2 -0.833901772428891
2.95091147026207 -1
3.2 -1
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.1 -0.774289330698911
1.31150999789376 -1
1.4 -1
1.7 -1
2 -1
2.3 -1
2.6 -1
2.9 -1
2.95091147026207 -1
3.2 -0.833901772428891
3.3631703033812 -0.7
3.5 -0.592361694695171
3.71699563056252 -0.4
3.8 -0.328033462366687
4.04528011860334 -0.1
4.1 -0.0497231328847067
4.36085164983148 0.2
4.4 0.237241035459002
4.66960753191868 0.5
4.7 0.529517658947304
4.97456718450442 0.8
5 0.825006268131743
5 1.1
5 1.18522301867327
4.91359323934918 1.1
4.7 0.889552272245707
4.60827529022793 0.8
4.4 0.596970504999669
4.29893406348032 0.5
4.1 0.309500907974326
3.98243837940091 0.2
3.8 0.0303507509409883
3.65277925206921 -0.1
3.5 -0.235424634632003
3.29718611701312 -0.4
3.2 -0.479683414384573
2.9 -0.689782839988762
2.88201714384888 -0.7
2.6 -0.863529531670269
2.3 -0.967745192890664
2 -0.993892770017432
1.7 -0.925213714878321
1.4 -0.729423428026406
1.37196187759371 -0.7
1.12349272853914 -0.4
1.1 -0.364403460507611
0.958354633260611 -0.1
0.851812109049335 0.2
0.8 0.422830459847938
0.780769641834721 0.5
0.732782747572173 0.8
0.705779853951447 1.1
0.697176335192932 1.4
0.704777212662279 1.7
0.716828420138849 2
0.724252764979481 2.3
0.72410377692128 2.6
0.715118570994107 2.9
0.708824908866298 3.2
0.705650535819083 3.5
0.699978717044208 3.8
0.694568622653409 4.1
0.69296328054805 4.4
0.693249336006367 4.7
0.696673105325699 5
0.582196145428018 5
0.57497894395621 4.7
0.574361702732874 4.4
0.57721383471722 4.1
0.585021329307306 3.8
0.590237943484404 3.5
0.588686981956009 3.2
0.589395822782406 2.9
0.591149502924966 2.6
0.583097677966866 2.3
0.566432060528645 2
0.543608485035052 1.7
0.525602235392635 1.4
0.525421393228357 1.1
0.543106779423274 0.8
0.576838087802923 0.5
0.633678766530461 0.2
0.728344054708188 -0.1
0.8 -0.254887093050948
0.863877382158607 -0.4
1.04544495549878 -0.7
1.1 -0.774289330698911
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.4 -0.729423428026406
1.7 -0.925213714878321
2 -0.993892770017432
2.3 -0.967745192890664
2.6 -0.863529531670269
2.88201714384888 -0.7
2.9 -0.689782839988762
3.2 -0.479683414384573
3.29718611701312 -0.4
3.5 -0.235424634632003
3.65277925206921 -0.1
3.8 0.0303507509409883
3.98243837940091 0.2
4.1 0.309500907974326
4.29893406348032 0.5
4.4 0.596970504999669
4.60827529022793 0.8
4.7 0.889552272245707
4.91359323934918 1.1
5 1.18522301867327
5 1.4
5 1.51135194068176
4.88756575297895 1.4
4.7 1.21497516314298
4.58303951025354 1.1
4.4 0.921224171708128
4.27504584402448 0.8
4.1 0.631871594720384
3.96084304739607 0.5
3.8 0.349777485377789
3.63516318832734 0.2
3.5 0.0794959323431471
3.28691452501702 -0.1
3.2 -0.171735281104697
2.9 -0.392179600915051
2.88728727423298 -0.4
2.6 -0.570054823116865
2.3 -0.683680820420351
2.13850068355949 -0.7
2 -0.714374845782423
1.9453608811708 -0.7
1.7 -0.63545060425525
1.4 -0.413914518887529
1.38823754695097 -0.4
1.17903067972079 -0.1
1.1 0.0585018010151374
1.04209497433154 0.2
0.959550356130231 0.5
0.908180336152494 0.8
0.877299019863653 1.1
0.863316915340185 1.4
0.863667198875009 1.7
0.869050075915465 2
0.871062831557088 2.3
0.865028830704318 2.6
0.849824079751907 2.9
0.83796749163673 3.2
0.829137814121023 3.5
0.820823021159373 3.8
0.816213796497512 4.1
0.815838584392782 4.4
0.816276435697988 4.7
0.816295540073061 5
0.8 5
0.696673105325699 5
0.693249336006367 4.7
0.69296328054805 4.4
0.694568622653409 4.1
0.699978717044208 3.8
0.705650535819083 3.5
0.708824908866298 3.2
0.715118570994108 2.9
0.72410377692128 2.6
0.724252764979481 2.3
0.716828420138849 2
0.704777212662279 1.7
0.697176335192932 1.4
0.705779853951447 1.1
0.732782747572173 0.8
0.780769641834721 0.5
0.8 0.422830459847938
0.851812109049335 0.2
0.958354633260611 -0.1
1.1 -0.364403460507611
1.12349272853914 -0.4
1.37196187759371 -0.7
1.4 -0.729423428026406
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
2 -0.714374845782423
2.13850068355949 -0.7
2.3 -0.683680820420351
2.6 -0.570054823116865
2.88728727423298 -0.4
2.9 -0.392179600915051
3.2 -0.171735281104697
3.28691452501702 -0.1
3.5 0.0794959323431471
3.63516318832734 0.2
3.8 0.349777485377789
3.96084304739607 0.5
4.1 0.631871594720384
4.27504584402448 0.8
4.4 0.921224171708128
4.58303951025354 1.1
4.7 1.21497516314298
4.88756575297895 1.4
5 1.51135194068176
5 1.7
5 1.84935620956353
4.85013545727525 1.7
4.7 1.55144120070682
4.54751314654606 1.4
4.4 1.25519755904484
4.2425801881605 1.1
4.1 0.961973395750988
3.93315384754191 0.8
3.8 0.674178777647799
3.61478744632156 0.5
3.5 0.395995828568722
3.27793637817055 0.2
3.2 0.134351088629698
2.9 -0.0997671232897449
2.89965370183206 -0.1
2.6 -0.285960241938177
2.32905605589814 -0.4
2.3 -0.411544807142824
2 -0.444129384022591
1.84721326680479 -0.4
1.7 -0.352709476987095
1.41582416397562 -0.1
1.4 -0.0815374410668533
1.24791933014398 0.2
1.14067427934948 0.5
1.1 0.675011664624098
1.07574056143801 0.8
1.03914955398065 1.1
1.02133108285336 1.4
1.01926679134769 1.7
1.02353001749743 2
1.02442179177819 2.3
1.01655628101292 2.6
1.00319866106655 2.9
0.995456757204702 3.2
0.988794567767691 3.5
0.981089714005505 3.8
0.975796210883707 4.1
0.978268684299217 4.4
0.983382848430537 4.7
0.98360073964653 5
0.816295540073061 5
0.816276435697988 4.7
0.815838584392782 4.4
0.816213796497512 4.1
0.820823021159373 3.8
0.829137814121023 3.5
0.83796749163673 3.2
0.849824079751907 2.9
0.865028830704318 2.6
0.871062831557088 2.3
0.869050075915465 2
0.863667198875009 1.7
0.863316915340185 1.4
0.877299019863653 1.1
0.908180336152494 0.8
0.959550356130231 0.5
1.04209497433154 0.2
1.1 0.0585018010151374
1.17903067972079 -0.1
1.38823754695097 -0.4
1.4 -0.413914518887529
1.7 -0.63545060425525
1.9453608811708 -0.7
2 -0.714374845782423
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
2 -0.444129384022591
2.3 -0.411544807142824
2.32905605589814 -0.4
2.6 -0.285960241938177
2.89965370183206 -0.1
2.9 -0.0997671232897449
3.2 0.134351088629698
3.27793637817055 0.2
3.5 0.395995828568722
3.61478744632156 0.5
3.8 0.674178777647799
3.93315384754191 0.8
4.1 0.961973395750988
4.2425801881605 1.1
4.4 1.25519755904484
4.54751314654606 1.4
4.7 1.55144120070682
4.85013545727525 1.7
5 1.84935620956353
5 2
5 2.24520731312465
4.75671586304905 2
4.7 1.94351043117092
4.45916373359255 1.7
4.4 1.6413078601003
4.16177779491913 1.4
4.1 1.33921839203487
3.86287530624216 1.1
3.8 1.03917317571715
3.55827615109865 0.8
3.5 0.745485622400823
3.23882533323793 0.5
3.2 0.465956385170324
2.9 0.214169106618472
2.88090181133377 0.2
2.6 0.0122051732004319
2.36141534548152 -0.1
2.3 -0.126130420236021
2 -0.15891335892344
1.83064065402537 -0.1
1.7 -0.0437365792698784
1.48826948627167 0.2
1.4 0.347981276208309
1.34131198150369 0.5
1.26486785655878 0.8
1.21649237374565 1.1
1.18941441001923 1.4
1.17949491709026 1.7
1.17771604140848 2
1.17560269334914 2.3
1.16930886778411 2.6
1.15901319496836 2.9
1.15333711845359 3.2
1.14793937820155 3.5
1.14009028980045 3.8
1.1327788680233 4.1
1.13523583757704 4.4
1.14312374282323 4.7
1.14774395865236 5
1.1 5
0.98360073964653 5
0.983382848430537 4.7
0.978268684299217 4.4
0.975796210883707 4.1
0.981089714005505 3.8
0.988794567767691 3.5
0.995456757204702 3.2
1.00319866106655 2.9
1.01655628101292 2.6
1.02442179177819 2.3
1.02353001749743 2
1.01926679134769 1.7
1.02133108285336 1.4
1.03914955398065 1.1
1.07574056143801 0.8
1.1 0.675011664624098
1.14067427934948 0.5
1.24791933014398 0.2
1.4 -0.0815374410668533
1.41582416397562 -0.1
1.7 -0.352709476987095
1.84721326680479 -0.4
2 -0.444129384022591
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
2 -0.15891335892344
2.3 -0.126130420236021
2.36141534548152 -0.1
2.6 0.0122051732004319
2.88090181133377 0.2
2.9 0.214169106618472
3.2 0.465956385170324
3.23882533323793 0.5
3.5 0.745485622400823
3.55827615109865 0.8
3.8 1.03917317571715
3.86287530624216 1.1
4.1 1.33921839203487
4.16177779491913 1.4
4.4 1.6413078601003
4.45916373359255 1.7
4.7 1.94351043117092
4.75671586304905 2
5 2.24520731312465
5 2.3
5 2.6
5 2.82744878059042
4.78866928435687 2.6
4.7 2.50783749804657
4.51344697232665 2.3
4.4 2.18001496950889
4.24433989735074 2
4.1 1.84464185809405
3.97847590239264 1.7
3.8 1.50595467164565
3.71130395165539 1.4
3.5 1.17248072062024
3.43678031622683 1.1
3.2 0.856804008655454
3.14467951014136 0.8
2.9 0.575216524216051
2.80842464584656 0.5
2.6 0.347155496189846
2.3163187603486 0.2
2.3 0.192482823716539
2 0.166302521400163
1.92768911691906 0.2
1.7 0.347142615332899
1.60471302624847 0.5
1.48210877907416 0.8
1.40449694583521 1.1
1.4 1.12551489021138
1.36748106804352 1.4
1.34471428620755 1.7
1.33161394980946 2
1.32466721309104 2.3
1.32356298716404 2.6
1.31900268274287 2.9
1.31198970788101 3.2
1.30590917700317 3.5
1.29545045405773 3.8
1.28063455376851 4.1
1.27586314941529 4.4
1.285852192414 4.7
1.30465713328685 5
1.14774395865236 5
1.14312374282323 4.7
1.13523583757704 4.4
1.1327788680233 4.1
1.14009028980045 3.8
1.14793937820155 3.5
1.15333711845359 3.2
1.15901319496836 2.9
1.16930886778411 2.6
1.17560269334914 2.3
1.17771604140848 2
1.17949491709026 1.7
1.18941441001923 1.4
1.21649237374565 1.1
1.26486785655878 0.8
1.34131198150369 0.5
1.4 0.347981276208309
1.48826948627167 0.2
1.7 -0.0437365792698784
1.83064065402537 -0.1
2 -0.15891335892344
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
2 0.166302521400163
2.3 0.192482823716539
2.3163187603486 0.2
2.6 0.347155496189846
2.80842464584656 0.5
2.9 0.575216524216051
3.14467951014136 0.8
3.2 0.856804008655454
3.43678031622683 1.1
3.5 1.17248072062024
3.71130395165539 1.4
3.8 1.50595467164565
3.97847590239264 1.7
4.1 1.84464185809405
4.24433989735074 2
4.4 2.18001496950889
4.51344697232665 2.3
4.7 2.50783749804657
4.78866928435687 2.6
5 2.82744878059042
5 2.9
5 3.2
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.1 5
4.0739780931267 5
4.1 4.93615411121294
4.31721106665857 4.7
4.4 4.5998222370402
4.7 4.42429386972823
4.83910378925582 4.4
4.98376537427595 4.1
4.83291070008791 3.8
4.7 3.58931935316576
4.65643561388784 3.5
4.47095201214013 3.2
4.4 3.09991909060441
4.28185695644017 2.9
4.1 2.62525027482742
4.0856807121486 2.6
3.8924278130797 2.3
3.8 2.17276637382617
3.68846135411503 2
3.5 1.73937186576666
3.47307620926052 1.7
3.24333097599465 1.4
3.2 1.34992040379073
2.98223391626805 1.1
2.9 1.0154206203858
2.66137610962758 0.8
2.6 0.750312094749203
2.3 0.594330417327251
2 0.60296154573949
1.81113688165343 0.8
1.7 0.992376495396443
1.66940128806252 1.1
1.61263919816691 1.4
1.57357789369552 1.7
1.54583747992667 2
1.52981807247973 2.3
1.52724942632655 2.6
1.51961807229324 2.9
1.51011644836304 3.2
1.50454033765379 3.5
1.49042042930734 3.8
1.45936817779069 4.1
1.43956990344341 4.4
1.4633471902283 4.7
1.50872411019967 5
1.4 5
1.30465713328685 5
1.285852192414 4.7
1.27586314941529 4.4
1.28063455376851 4.1
1.29545045405773 3.8
1.30590917700317 3.5
1.31198970788101 3.2
1.31900268274287 2.9
1.32356298716404 2.6
1.32466721309104 2.3
1.33161394980946 2
1.34471428620755 1.7
1.36748106804352 1.4
1.4 1.12551489021138
1.40449694583521 1.1
1.48210877907416 0.8
1.60471302624847 0.5
1.7 0.347142615332899
1.92768911691906 0.2
2 0.166302521400163
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
2 0.60296154573949
2.3 0.594330417327251
2.6 0.750312094749203
2.66137610962758 0.8
2.9 1.0154206203858
2.98223391626805 1.1
3.2 1.34992040379073
3.24333097599465 1.4
3.47307620926052 1.7
3.5 1.73937186576666
3.68846135411503 2
3.8 2.17276637382617
3.8924278130797 2.3
4.0856807121486 2.6
4.1 2.62525027482742
4.28185695644017 2.9
4.4 3.09991909060441
4.47095201214013 3.2
4.65643561388784 3.5
4.7 3.58931935316576
4.83291070008791 3.8
4.98376537427595 4.1
4.83910378925582 4.4
4.7 4.42429386972823
4.4 4.5998222370402
4.31721106665857 4.7
4.1 4.93615411121294
4.0739780931267 5
3.8 5
3.5 5
3.42257255129008 5
3.5 4.79113796529771
3.5685918099441 4.7
3.8 4.41471887857621
3.80759559632339 4.4
3.85829087807663 4.1
3.82410435724376 3.8
3.8 3.66947261211104
3.77140480436367 3.5
3.70825458500355 3.2
3.60775180782944 2.9
3.5 2.64744582693384
3.47892944160593 2.6
3.32203539592906 2.3
3.2 2.08135974481858
3.14823728502996 2
2.94349304639014 1.7
2.9 1.64254233776094
2.66645881098659 1.4
2.6 1.33545160683181
2.3 1.20145575221824
2 1.39884213119886
1.99953000072104 1.4
1.91424891509759 1.7
1.85557094072957 2
1.81784079865024 2.3
1.79285470567461 2.6
1.76808616463614 2.9
1.75587260131332 3.2
1.75124518474101 3.5
1.74652723332804 3.8
1.74190065443972 4.1
1.74240553241903 4.4
1.74274057525188 4.7
1.75024579729925 5
1.7 5
1.50872411019967 5
1.4633471902283 4.7
1.43956990344341 4.4
1.45936817779069 4.1
1.49042042930734 3.8
1.50454033765379 3.5
1.51011644836304 3.2
1.51961807229324 2.9
1.52724942632655 2.6
1.52981807247973 2.3
1.54583747992667 2
1.57357789369552 1.7
1.61263919816691 1.4
1.66940128806252 1.1
1.7 0.992376495396443
1.81113688165343 0.8
2 0.60296154573949
};
\addplot [draw=none, fill=lavender231240249]
table{%
x  y
2 1.39884213119886
2.3 1.20145575221824
2.6 1.33545160683181
2.66645881098659 1.4
2.9 1.64254233776094
2.94349304639014 1.7
3.14823728502996 2
3.2 2.08135974481858
3.32203539592906 2.3
3.47892944160593 2.6
3.5 2.64744582693384
3.60775180782944 2.9
3.70825458500355 3.2
3.77140480436367 3.5
3.8 3.66947261211104
3.82410435724376 3.8
3.85829087807663 4.1
3.80759559632339 4.4
3.8 4.41471887857621
3.5685918099441 4.7
3.5 4.79113796529771
3.42257255129008 5
3.2 5
2.99331576537855 5
3.2 4.77731964997039
3.25091078601664 4.7
3.27627757794581 4.4
3.2414263135777 4.1
3.2 3.81815755430972
2.9 3.96328829661638
2.8071222555818 4.1
2.71779305850078 4.4
2.6941698443655 4.7
2.71663162028952 5
2.6 5
2.39292827507559 5
2.41399883822717 4.7
2.3526305283774 4.4
2.3 4.2576239281542
2.27942903869468 4.1
2.21867107610452 3.8
2.15045617791556 3.5
2.03193492156979 3.2
2 3.16981369635125
1.99650394320808 3.2
1.96131938487478 3.5
1.93882734099825 3.8
1.93323786342379 4.1
1.92820932809319 4.4
1.91239722068362 4.7
1.91249302581319 5
1.75024579729925 5
1.74274057525188 4.7
1.74240553241903 4.4
1.74190065443972 4.1
1.74652723332804 3.8
1.751245184741 3.5
1.75587260131332 3.2
1.76808616463614 2.9
1.79285470567461 2.6
1.81784079865024 2.3
1.85557094072957 2
1.91424891509759 1.7
1.99953000072104 1.4
2 1.39884213119886
};
\addplot [draw=none, fill=aliceblue242247253]
table{%
x  y
2 3.16981369635125
2.03193492156979 3.2
2.15045617791556 3.5
2.21867107610452 3.8
2.27942903869468 4.1
2.3 4.2576239281542
2.3526305283774 4.4
2.41399883822717 4.7
2.39292827507559 5
2.3 5
2 5
1.91249302581319 5
1.91239722068362 4.7
1.92820932809319 4.4
1.93323786342379 4.1
1.93882734099825 3.8
1.96131938487478 3.5
1.99650394320808 3.2
2 3.16981369635125
};
\addplot [draw=none, fill=aliceblue242247253]
table{%
x  y
2.9 3.96328829661638
3.2 3.81815755430972
3.2414263135777 4.1
3.27627757794581 4.4
3.25091078601664 4.7
3.2 4.77731964997039
2.99331576537855 5
2.9 5
2.71663162028952 5
2.6941698443655 4.7
2.71779305850078 4.4
2.8071222555818 4.1
2.9 3.96328829661638
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.3 1.4
};
\addplot [semithick, darkorange25512714, mark=mystar, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.3 2.3
};
\draw (axis cs:2.5,1.4) node[
  scale=0.5,
  anchor=base west,
  text=black,
  rotate=0.0
]{$-0.319$};
\draw (axis cs:2.5,2.3) node[
  scale=0.5,
  anchor=base west,
  text=black,
  rotate=0.0
]{$-0.297$};
\coordinate (CVI_mean_lml_b) at (axis cs:2.3,1.4);
\coordinate (CVI_mean_lml_ep_b) at (axis cs:2.3,2.3);
\end{axis}



==> fig/tikz/sonar/EP_mean_lml.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
-0.7 -1
-0.4 -1
-0.1 -1
0.2 -1
0.5 -1
0.8 -1
1.1 -1
1.21295767440994 -1
1.1 -0.90055816385219
0.942194301953048 -0.7
0.8 -0.455951859306061
0.767579880726946 -0.4
0.630195892574996 -0.1
0.54969806240402 0.2
0.502454593918102 0.5
0.5 0.524807819905138
0.456120685649725 0.8
0.429236092371708 1.1
0.414334131276586 1.4
0.406105846461488 1.7
0.40157398879048 2
0.39908182589744 2.3
0.397712557525182 2.6
0.396960607139439 2.9
0.396547788347639 3.2
0.396321186480547 3.5
0.396196810316166 3.8
0.396128547982054 4.1
0.396091111481308 4.4
0.396070527291873 4.7
0.396061720297732 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
2.9 -1
3.2 -1
3.5 -1
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.5
5 0.8
5 1.1
5 1.15666030146446
4.94713907359017 1.1
4.7 0.834629557018556
4.6673370951209 0.8
4.4 0.515660294469146
4.38495357389055 0.5
4.1 0.201689036685242
4.09832626180489 0.2
3.80561891764915 -0.1
3.8 -0.105896701205389
3.5 -0.397874083282001
3.49758673878833 -0.4
3.2 -0.672321520910411
3.16385670305221 -0.7
2.9 -0.917063576698737
2.76310738864044 -1
2.9 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.1 -0.90055816385219
1.21295767440994 -1
1.4 -1
1.7 -1
2 -1
2.3 -1
2.6 -1
2.76310738864044 -1
2.9 -0.917063576698737
3.16385670305221 -0.7
3.2 -0.672321520910411
3.49758673878833 -0.4
3.5 -0.397874083282001
3.8 -0.105896701205389
3.80561891764915 -0.1
4.09832626180489 0.2
4.1 0.201689036685242
4.38495357389055 0.5
4.4 0.515660294469146
4.6673370951209 0.8
4.7 0.834629557018556
4.94713907359017 1.1
5 1.15666030146446
5 1.4
5 1.7
5 1.7102500960749
4.99036528184632 1.7
4.70754614889557 1.4
4.7 1.39199255872563
4.42255531920274 1.1
4.4 1.07629319976019
4.13333732538405 0.8
4.1 0.765515015590104
3.83683022792334 0.5
3.8 0.462887714773066
3.52740316078953 0.2
3.5 0.173535314277176
3.2 -0.0950047703254983
3.19389546008013 -0.1
2.9 -0.337866731800756
2.80622549632083 -0.4
2.6 -0.539104162018941
2.3 -0.675968333069659
2.18714471609617 -0.7
2 -0.744690377966083
1.7 -0.714477060481763
1.6712983365712 -0.7
1.4 -0.566747004102404
1.23630653742544 -0.4
1.1 -0.226512802826754
1.02589493009648 -0.1
0.902260389010049 0.2
0.827810487580758 0.5
0.8 0.68473347892906
0.779953355550952 0.8
0.748927839089474 1.1
0.731612206695752 1.4
0.722012001229762 1.7
0.71671197987234 2
0.713793581101467 2.3
0.71218903225448 2.6
0.711307333826163 2.9
0.710823241298549 3.2
0.710557719896731 3.5
0.710411652369756 3.8
0.710331521959189 4.1
0.710287610244334 4.4
0.710263446067328 4.7
0.710250901122478 5
0.5 5
0.396061720297732 5
0.396070527291873 4.7
0.396091111481308 4.4
0.396128547982054 4.1
0.396196810316166 3.8
0.396321186480547 3.5
0.396547788347639 3.2
0.396960607139439 2.9
0.397712557525182 2.6
0.39908182589744 2.3
0.40157398879048 2
0.406105846461488 1.7
0.414334131276586 1.4
0.429236092371708 1.1
0.456120685649725 0.8
0.5 0.524807819905138
0.502454593918102 0.5
0.54969806240402 0.2
0.630195892574996 -0.1
0.767579880726946 -0.4
0.8 -0.455951859306061
0.942194301953048 -0.7
1.1 -0.90055816385219
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.7 -0.714477060481763
2 -0.744690377966083
2.18714471609617 -0.7
2.3 -0.675968333069659
2.6 -0.539104162018942
2.80622549632083 -0.4
2.9 -0.337866731800756
3.19389546008013 -0.1
3.2 -0.0950047703254983
3.5 0.173535314277176
3.52740316078953 0.2
3.8 0.462887714773066
3.83683022792334 0.5
4.1 0.765515015590104
4.13333732538405 0.8
4.4 1.07629319976019
4.42255531920274 1.1
4.7 1.39199255872563
4.70754614889557 1.4
4.99036528184632 1.7
5 1.7102500960749
5 2
5 2.23057706032832
4.78610294225811 2
4.7 1.90791805736043
4.50660728540306 1.7
4.4 1.58686378787345
4.22514607676315 1.4
4.1 1.2689426554255
3.9398154525266 1.1
3.8 0.956876339986117
3.64704278179581 0.8
3.5 0.655190317808656
3.33995433548622 0.5
3.2 0.370870084005221
3.00386472925385 0.2
2.9 0.114089309231044
2.60030672879115 -0.1
2.6 -0.100210917157206
2.3 -0.254565775075074
2 -0.327669032011941
1.7 -0.291466810672756
1.4053717144656 -0.1
1.4 -0.0956454953654419
1.2100564659049 0.2
1.1 0.47423059814629
1.0917506460749 0.5
1.02945062324232 0.8
0.993767018958129 1.1
0.973647438785118 1.4
0.962427026317176 1.7
0.956212305827147 2
0.952784544206949 2.3
0.950897196804607 2.6
0.949859974962952 2.9
0.949291038467734 3.2
0.948977278722192 3.5
0.948805590672872 3.8
0.948711110854049 4.1
0.948659613963268 4.4
0.948630875626112 4.7
0.948615306893053 5
0.8 5
0.710250901122478 5
0.710263446067328 4.7
0.710287610244334 4.4
0.710331521959189 4.1
0.710411652369756 3.8
0.710557719896731 3.5
0.710823241298549 3.2
0.711307333826163 2.9
0.71218903225448 2.6
0.713793581101467 2.3
0.71671197987234 2
0.722012001229762 1.7
0.731612206695752 1.4
0.748927839089474 1.1
0.779953355550952 0.8
0.8 0.68473347892906
0.827810487580758 0.5
0.902260389010049 0.2
1.02589493009648 -0.1
1.1 -0.226512802826754
1.23630653742544 -0.4
1.4 -0.566747004102403
1.6712983365712 -0.7
1.7 -0.714477060481763
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
4.7 4.3160861868128
5 4.38860763800602
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.34143970482555 5
4.38923306877608 4.7
4.4 4.65947633990798
4.57615331644963 4.4
4.7 4.3160861868128
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.7 -0.291466810672756
2 -0.327669032011941
2.3 -0.254565775075074
2.6 -0.100210917157206
2.60030672879115 -0.1
2.9 0.114089309231044
3.00386472925385 0.2
3.2 0.370870084005221
3.33995433548622 0.5
3.5 0.655190317808656
3.64704278179581 0.8
3.8 0.956876339986117
3.9398154525266 1.1
4.1 1.2689426554255
4.22514607676315 1.4
4.4 1.58686378787345
4.50660728540306 1.7
4.7 1.90791805736043
4.78610294225811 2
5 2.23057706032832
5 2.3
5 2.6
5 2.9
5 3.2
5 3.5
5 3.8
5 4.1
5 4.38860763800602
4.7 4.3160861868128
4.57615331644963 4.4
4.4 4.65947633990798
4.38923306877608 4.7
4.34143970482555 5
4.1 5
3.88324439788041 5
3.89147103450656 4.7
3.90660702913955 4.4
3.93449866548898 4.1
3.98559957303565 3.8
4.07661311750497 3.5
4.1 3.44201082167293
4.4 3.22030795334155
4.7 3.20607029242272
4.72213158285792 3.2
4.75112202313758 2.9
4.7 2.82537884739319
4.56844580635973 2.6
4.4 2.35592921071023
4.36811969527411 2.3
4.14018511178162 2
4.1 1.95308442223169
3.90215479814387 1.7
3.8 1.58200241020973
3.65670148661978 1.4
3.5 1.22392516236348
3.39786210017014 1.1
3.2 0.890149912322441
3.11745393605348 0.8
2.9 0.593019425594487
2.79616216191381 0.5
2.6 0.346093051629892
2.36400832390855 0.2
2.3 0.164705360008539
2 0.0862615506843688
1.7 0.144908295093625
1.63379105521112 0.2
1.4 0.477760632482092
1.38979730456669 0.5
1.29959646844543 0.8
1.2473831889597 1.1
1.2178263208676 1.4
1.20132291861156 1.7
1.1921798089711 2
1.18713697084782 2.3
1.18436113094419 2.6
1.18283576165394 2.9
1.18199879039979 3.2
1.18153622447879 3.5
1.18128405266719 3.8
1.18114492015929 4.1
1.18107125863871 4.4
1.18102762682734 4.7
1.18100481988659 5
1.1 5
0.948615306893053 5
0.948630875626112 4.7
0.948659613963268 4.4
0.948711110854049 4.1
0.948805590672872 3.8
0.948977278722192 3.5
0.949291038467734 3.2
0.949859974962952 2.9
0.950897196804607 2.6
0.952784544206949 2.3
0.956212305827147 2
0.962427026317176 1.7
0.973647438785118 1.4
0.993767018958129 1.1
1.02945062324232 0.8
1.0917506460749 0.5
1.1 0.47423059814629
1.2100564659049 0.2
1.4 -0.0956454953654419
1.4053717144656 -0.1
1.7 -0.291466810672756
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.7 0.144908295093625
2 0.0862615506843688
2.3 0.164705360008539
2.36400832390855 0.2
2.6 0.346093051629892
2.79616216191381 0.5
2.9 0.593019425594487
3.11745393605348 0.8
3.2 0.890149912322441
3.39786210017014 1.1
3.5 1.22392516236348
3.65670148661978 1.4
3.8 1.58200241020973
3.90215479814387 1.7
4.1 1.95308442223169
4.14018511178162 2
4.36811969527411 2.3
4.4 2.35592921071023
4.56844580635973 2.6
4.7 2.82537884739319
4.75112202313758 2.9
4.72213158285792 3.2
4.7 3.20607029242272
4.4 3.22030795334155
4.1 3.44201082167293
4.07661311750497 3.5
3.98559957303565 3.8
3.93449866548898 4.1
3.90660702913955 4.4
3.89147103450656 4.7
3.88324439788041 5
3.8 5
3.5 5
3.38282777866259 5
3.38351523200191 4.7
3.38474451122496 4.4
3.38683796535359 4.1
3.3902410115962 3.8
3.39525489195891 3.5
3.4012603556904 3.2
3.40498730099834 2.9
3.3980738893448 2.6
3.36589702752026 2.3
3.29149133101012 2
3.2 1.78303366628358
3.16705039876429 1.7
2.99726871481532 1.4
2.9 1.26741544972046
2.77127519184164 1.1
2.6 0.918226998113257
2.45765101685623 0.8
2.3 0.691138923740589
2 0.610514601640501
1.7 0.776518712624626
1.68665651739959 0.8
1.5814508481808 1.1
1.52311980816449 1.4
1.49108809873681 1.7
1.47354067841451 2
1.46392763184652 2.3
1.45866202543518 2.6
1.45577378421677 2.9
1.45418770997856 3.2
1.45331778933054 3.5
1.45283987401805 3.8
1.45257680440285 4.1
1.45244280384335 4.4
1.45235746458169 4.7
1.45231429965564 5
1.4 5
1.18100481988659 5
1.18102762682734 4.7
1.18107125863871 4.4
1.18114492015929 4.1
1.18128405266719 3.8
1.18153622447879 3.5
1.18199879039979 3.2
1.18283576165394 2.9
1.18436113094419 2.6
1.18713697084782 2.3
1.1921798089711 2
1.20132291861156 1.7
1.2178263208676 1.4
1.2473831889597 1.1
1.29959646844543 0.8
1.38979730456669 0.5
1.4 0.477760632482092
1.63379105521112 0.2
1.7 0.144908295093625
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.7 0.776518712624626
2 0.610514601640501
2.3 0.691138923740589
2.45765101685623 0.8
2.6 0.918226998113257
2.77127519184164 1.1
2.9 1.26741544972046
2.99726871481532 1.4
3.16705039876429 1.7
3.2 1.78303366628358
3.29149133101012 2
3.36589702752026 2.3
3.3980738893448 2.6
3.40498730099834 2.9
3.4012603556904 3.2
3.39525489195891 3.5
3.3902410115962 3.8
3.38683796535359 4.1
3.38474451122496 4.4
3.38351523200191 4.7
3.38282777866259 5
3.2 5
2.9 5
2.61785358999958 5
2.61747918763803 4.7
2.61679941946423 4.4
2.61555346667957 4.1
2.61330105467049 3.8
2.60920419012369 3.5
2.60180067341418 3.2
2.6 3.15959400314202
2.57446714527971 2.9
2.52481695440584 2.6
2.44656011137927 2.3
2.33403400345391 2
2.3 1.93829687447
2.20790943636469 2
2.01507286312659 2.3
2 2.35254447522765
1.98614836560742 2.6
1.97700825204144 2.9
1.97202437932158 3.2
1.96929853020166 3.5
1.96780383162443 3.8
1.96703779737409 4.1
1.96654421968963 4.4
1.96627882369869 4.7
1.96615219466318 5
1.7 5
1.45231429965564 5
1.45235746458169 4.7
1.45244280384335 4.4
1.45257680440285 4.1
1.45283987401805 3.8
1.45331778933054 3.5
1.45418770997856 3.2
1.45577378421677 2.9
1.45866202543518 2.6
1.46392763184652 2.3
1.47354067841451 2
1.49108809873681 1.7
1.52311980816449 1.4
1.5814508481808 1.1
1.68665651739959 0.8
1.7 0.776518712624626
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
2.3 1.93829687447
2.33403400345391 2
2.44656011137927 2.3
2.52481695440584 2.6
2.57446714527971 2.9
2.6 3.15959400314202
2.60180067341418 3.2
2.60920419012369 3.5
2.61330105467049 3.8
2.61555346667957 4.1
2.61679941946423 4.4
2.61747918763803 4.7
2.61785358999958 5
2.6 5
2.3 5
2 5
1.96615219466318 5
1.96627882369869 4.7
1.96654421968963 4.4
1.96703779737409 4.1
1.96780383162443 3.8
1.96929853020166 3.5
1.97202437932158 3.2
1.97700825204144 2.9
1.98614836560742 2.6
2 2.35254447522765
2.01507286312659 2.3
2.20790943636469 2
2.3 1.93829687447
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.3 5
};
\coordinate (EP_mean_lml_t) at (axis cs:2.3,5.0);
\end{axis}



==> fig/tikz/sonar/EP_nlpd.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
-0.7 -1
-0.4 -1
-0.1 -1
0.2 -1
0.5 -1
0.8 -1
0.85175123376382 -1
0.8 -0.916557371075154
0.663771631992592 -0.7
0.535604993600457 -0.4
0.5 -0.284479480003464
0.421985226980955 -0.1
0.339231033498293 0.2
0.291620141631917 0.5
0.264393870298186 0.8
0.24899192397917 1.1
0.240369882702465 1.4
0.235580623425132 1.7
0.232933540905145 2
0.23147508586484 2.3
0.230672921209164 2.6
0.230232022166655 2.9
0.229989940783376 3.2
0.229857040713624 3.5
0.229784053645617 3.8
0.229744044716629 4.1
0.2297296944526 4.4
0.22971351220926 4.7
0.229719025144089 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.286189868418361
4.91196907887571 0.2
4.7 -0.00900585201547864
4.60564036716419 -0.1
4.4 -0.300728353289095
4.29441504843626 -0.4
4.1 -0.586599166815803
3.97424151708905 -0.7
3.8 -0.862639778112704
3.63689194070762 -1
3.8 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
0.8 -0.916557371075154
0.85175123376382 -1
1.1 -1
1.31150580503317 -1
1.1 -0.774309761141788
1.04542687430489 -0.7
0.863817889712365 -0.4
0.8 -0.255193878539204
0.728132990238156 -0.1
0.633272408326946 0.2
0.576261463194884 0.5
0.542497648585855 0.8
0.522928340161816 1.1
0.511805870029344 1.4
0.505572245178367 1.7
0.502108498239864 2
0.500194942837381 2.3
0.5 2.35538823982072
0.49867909002544 2.6
0.497787778616558 2.9
0.49729882787617 3.2
0.497030457805442 3.5
0.496882953588828 3.8
0.496802336434836 4.1
0.496758993181168 4.4
0.496733575219414 4.7
0.496837349210428 5
0.229719025144089 5
0.22971351220926 4.7
0.2297296944526 4.4
0.229744044716629 4.1
0.229784053645617 3.8
0.229857040713624 3.5
0.229989940783376 3.2
0.230232022166655 2.9
0.230672921209164 2.6
0.23147508586484 2.3
0.232933540905145 2
0.235580623425132 1.7
0.240369882702465 1.4
0.24899192397917 1.1
0.264393870298186 0.8
0.291620141631917 0.5
0.339231033498293 0.2
0.421985226980955 -0.1
0.5 -0.284479480003464
0.535604993600457 -0.4
0.663771631992592 -0.7
0.8 -0.916557371075154
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
3.2 -1
3.5 -1
3.63689194070762 -1
3.8 -0.862639778112704
3.97424151708905 -0.7
4.1 -0.586599166815803
4.29441504843626 -0.4
4.4 -0.300728353289095
4.60564036716419 -0.1
4.7 -0.00900585201547864
4.91196907887571 0.2
5 0.286189868418361
5 0.5
5 0.8
5 0.825006088173497
4.97456731713693 0.8
4.7 0.529517533512805
4.66960766394273 0.5
4.4 0.237240826048367
4.36085190158962 0.2
4.1 -0.0497233825141191
4.04528041749889 -0.1
3.8 -0.328033725645464
3.71699590399306 -0.4
3.5 -0.592361939329257
3.36317056768861 -0.7
3.2 -0.833901978173596
2.95091187066464 -1
3.2 -1
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.1 -0.774309761141788
1.31150580503317 -1
1.4 -1
1.7 -1
2 -1
2.3 -1
2.6 -1
2.9 -1
2.95091187066464 -1
3.2 -0.833901978173596
3.36317056768861 -0.7
3.5 -0.592361939329257
3.71699590399306 -0.4
3.8 -0.328033725645464
4.04528041749889 -0.1
4.1 -0.0497233825141191
4.36085190158962 0.2
4.4 0.237240826048367
4.66960766394273 0.5
4.7 0.529517533512805
4.97456731713693 0.8
5 0.825006088173497
5 1.1
5 1.18522318743356
4.91359310242627 1.1
4.7 0.88955279490408
4.60827501524469 0.8
4.4 0.596970768532048
4.2989336022066 0.5
4.1 0.309501254278159
3.98243807702795 0.2
3.8 0.0303510204276115
3.65277913744687 -0.1
3.5 -0.235424435207148
3.29718630516991 -0.4
3.2 -0.479683539887879
2.9 -0.689783233311925
2.88201789899721 -0.7
2.6 -0.863530094656111
2.3 -0.967745974851855
2 -0.993894068387488
1.7 -0.925217348800428
1.4 -0.729438062748287
1.37194648620639 -0.7
1.12343168857686 -0.4
1.1 -0.36451524418739
0.958203991334638 -0.1
0.851518298550655 0.2
0.8 0.421479387560875
0.780425299680413 0.5
0.733103907343023 0.8
0.706013044478105 1.1
0.690731788869416 1.4
0.682206008779465 1.7
0.677478780769649 2
0.674873108449297 2.3
0.673439093356673 2.6
0.672646565065209 2.9
0.672213807831263 3.2
0.671980785983445 3.5
0.671843424329178 3.8
0.671771121581256 4.1
0.671732899171629 4.4
0.671710267021819 4.7
0.671733024153411 5
0.5 5
0.496837349210428 5
0.496733575219414 4.7
0.496758993181168 4.4
0.496802336434836 4.1
0.496882953588828 3.8
0.497030457805442 3.5
0.49729882787617 3.2
0.497787778616558 2.9
0.49867909002544 2.6
0.5 2.35538823982072
0.500194942837381 2.3
0.502108498239864 2
0.505572245178367 1.7
0.511805870029344 1.4
0.522928340161815 1.1
0.542497648585855 0.8
0.576261463194883 0.5
0.633272408326946 0.2
0.728132990238156 -0.1
0.8 -0.255193878539204
0.863817889712365 -0.4
1.04542687430489 -0.7
1.1 -0.774309761141788
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.4 -0.729438062748287
1.7 -0.925217348800428
2 -0.993894068387488
2.3 -0.967745974851855
2.6 -0.863530094656111
2.88201789899721 -0.7
2.9 -0.689783233311925
3.2 -0.479683539887879
3.29718630516991 -0.4
3.5 -0.235424435207148
3.65277913744687 -0.1
3.8 0.0303510204276115
3.98243807702795 0.2
4.1 0.309501254278159
4.2989336022066 0.5
4.4 0.596970768532048
4.60827501524469 0.8
4.7 0.88955279490408
4.91359310242627 1.1
5 1.18522318743356
5 1.4
5 1.51135772476789
4.88756004442121 1.4
4.7 1.21498078869789
4.58303407387129 1.1
4.4 0.921229102638829
4.27504146537387 0.8
4.1 0.631876259170099
3.96083827602985 0.5
3.8 0.349782052370775
3.63515877773836 0.2
3.5 0.0794999334876496
3.2869118564554 -0.1
3.2 -0.171733107476084
2.9 -0.39217940379075
2.88728710581034 -0.4
2.6 -0.57005435174808
2.3 -0.683682404801741
2.138526282962 -0.7
2 -0.714378271620628
1.94534445789571 -0.7
1.7 -0.635460063645514
1.4 -0.413956909594079
1.38819954020057 -0.4
1.1789304820429 -0.1
1.1 0.0583612927988197
1.0420185582422 0.2
0.959898958828356 0.5
0.90979872084526 0.8
0.880215911910496 1.1
0.863221221708568 1.4
0.853641155805526 1.7
0.848299587245396 2
0.845348921214866 2.3
0.843718676539932 2.6
0.842817322161564 2.9
0.842325884198186 3.2
0.842060078964461 3.5
0.841902402082435 3.8
0.841820658112015 4.1
0.841778613804425 4.4
0.841751153372062 4.7
0.84174092334964 5
0.8 5
0.671733024153411 5
0.671710267021819 4.7
0.671732899171629 4.4
0.671771121581256 4.1
0.671843424329178 3.8
0.671980785983445 3.5
0.672213807831263 3.2
0.672646565065209 2.9
0.673439093356673 2.6
0.674873108449297 2.3
0.677478780769649 2
0.682206008779465 1.7
0.690731788869416 1.4
0.706013044478105 1.1
0.733103907343023 0.8
0.780425299680413 0.5
0.8 0.421479387560875
0.851518298550655 0.2
0.958203991334638 -0.1
1.1 -0.36451524418739
1.12343168857686 -0.4
1.37194648620639 -0.7
1.4 -0.729438062748287
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
2 -0.714378271620628
2.138526282962 -0.7
2.3 -0.683682404801741
2.6 -0.57005435174808
2.88728710581034 -0.4
2.9 -0.39217940379075
3.2 -0.171733107476084
3.2869118564554 -0.1
3.5 0.0794999334876496
3.63515877773836 0.2
3.8 0.349782052370775
3.96083827602985 0.5
4.1 0.631876259170099
4.27504146537387 0.8
4.4 0.921229102638829
4.58303407387129 1.1
4.7 1.21498078869789
4.88756004442121 1.4
5 1.51135772476789
5 1.7
5 1.84938782460853
4.85010391563703 1.7
4.7 1.55147235348711
4.54748218023257 1.4
4.4 1.25522779867953
4.24255039445556 1.1
4.1 0.962001776209395
3.93312635637259 0.8
3.8 0.67420517055776
3.61476331793759 0.5
3.5 0.396017883060912
3.2779179700835 0.2
3.2 0.134366361720738
2.9 -0.0997595949245761
2.89964254280266 -0.1
2.6 -0.28595240526499
2.32905895724457 -0.4
2.3 -0.411546298360034
2 -0.444134149251469
1.84717866021249 -0.4
1.7 -0.35271222867935
1.41582238448464 -0.1
1.4 -0.081495846706697
1.24812319373042 0.2
1.14184002363597 0.5
1.1 0.687718633199729
1.0789709405292 0.8
1.04504955487364 1.1
1.02561409331402 1.4
1.01466895809819 1.7
1.0085732370035 2
1.00521295136082 2.3
1.00334424438605 2.6
1.00231855557273 2.9
1.00175888144019 3.2
1.00144338067227 3.5
1.0012707926227 3.8
1.00118095094313 4.1
1.00113770779399 4.4
1.00110033492359 4.7
1.00109049413818 5
0.84174092334964 5
0.841751153372062 4.7
0.841778613804425 4.4
0.841820658112015 4.1
0.841902402082435 3.8
0.842060078964461 3.5
0.842325884198186 3.2
0.842817322161564 2.9
0.843718676539932 2.6
0.845348921214866 2.3
0.848299587245396 2
0.853641155805526 1.7
0.863221221708568 1.4
0.880215911910496 1.1
0.90979872084526 0.8
0.959898958828356 0.5
1.0420185582422 0.2
1.1 0.0583612927988197
1.1789304820429 -0.1
1.38819954020057 -0.4
1.4 -0.413956909594079
1.7 -0.635460063645514
1.94534445789571 -0.7
2 -0.714378271620628
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
2 -0.444134149251469
2.3 -0.411546298360034
2.32905895724457 -0.4
2.6 -0.28595240526499
2.89964254280266 -0.1
2.9 -0.0997595949245761
3.2 0.134366361720738
3.2779179700835 0.2
3.5 0.396017883060912
3.61476331793759 0.5
3.8 0.67420517055776
3.93312635637259 0.8
4.1 0.962001776209395
4.24255039445556 1.1
4.4 1.25522779867953
4.54748218023257 1.4
4.7 1.55147235348711
4.85010391563703 1.7
5 1.84938782460853
5 2
5 2.24534814213346
4.75657559627892 2
4.7 1.94365010683896
4.45902526071287 1.7
4.4 1.64144515284217
4.16164269727526 1.4
4.1 1.33935114379795
3.86274579469659 1.1
3.8 1.0392982061815
3.55815701689795 0.8
3.5 0.745596601599647
3.23872482350537 0.5
3.2 0.466044285357531
2.9 0.21423977226989
2.88081222682275 0.2
2.6 0.0122664672478637
2.36134294118354 -0.1
2.3 -0.126099209944502
2 -0.158867306896595
1.83082400700639 -0.1
1.7 -0.0435163089388764
1.48891315770487 0.2
1.4 0.351171009658952
1.343166747717 0.5
1.26993638928534 0.8
1.22635293984955 1.1
1.20123746919531 1.4
1.18706044005777 1.7
1.17915881597298 2
1.1747945857593 2.3
1.1723726132021 2.6
1.17103593471721 2.9
1.1703236518478 3.2
1.16990450859671 3.5
1.16968659928853 3.8
1.16957476131022 4.1
1.16950184093978 4.4
1.16946769787813 4.7
1.1694696603259 5
1.1 5
1.00109049413818 5
1.00110033492359 4.7
1.00113770779399 4.4
1.00118095094313 4.1
1.0012707926227 3.8
1.00144338067227 3.5
1.00175888144019 3.2
1.00231855557273 2.9
1.00334424438605 2.6
1.00521295136082 2.3
1.0085732370035 2
1.01466895809819 1.7
1.02561409331402 1.4
1.04504955487364 1.1
1.0789709405292 0.8
1.1 0.687718633199729
1.14184002363597 0.5
1.24812319373042 0.2
1.4 -0.081495846706697
1.41582238448464 -0.1
1.7 -0.35271222867935
1.84717866021249 -0.4
2 -0.444134149251469
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
2 -0.158867306896595
2.3 -0.126099209944502
2.36134294118354 -0.1
2.6 0.0122664672478637
2.88081222682275 0.2
2.9 0.21423977226989
3.2 0.466044285357531
3.23872482350537 0.5
3.5 0.745596601599647
3.55815701689795 0.8
3.8 1.0392982061815
3.86274579469659 1.1
4.1 1.33935114379795
4.16164269727526 1.4
4.4 1.64144515284217
4.45902526071287 1.7
4.7 1.94365010683896
4.75657559627892 2
5 2.24534814213346
5 2.3
5 2.6
5 2.8286368888116
4.78757005169376 2.6
4.7 2.50897369922007
4.51242433109066 2.3
4.4 2.18108941991995
4.24341144529514 2
4.1 1.84562726951993
3.97764601872064 1.7
3.8 1.50683271806568
3.71057368028831 1.4
3.5 1.17322431744
3.43614894686696 1.1
3.2 0.857408958491147
3.14412098352474 0.8
2.9 0.57570273790569
2.80789659845925 0.5
2.6 0.34754885610724
2.31572507496053 0.2
2.3 0.192758129392047
2 0.166777778813658
1.92893569379234 0.2
1.7 0.349877756590416
1.60753083931162 0.5
1.49026582027566 0.8
1.42206007300931 1.1
1.4 1.27013215801376
1.38804363109099 1.4
1.37226191046083 1.7
1.36343835195915 2
1.35853027287525 2.3
1.35583384755197 2.6
1.35431574511678 2.9
1.3535491195496 3.2
1.35307431086848 3.5
1.35283288509833 3.8
1.35271362078584 4.1
1.35258177370048 4.4
1.35258944055915 4.7
1.35262566072362 5
1.1694696603259 5
1.16946769787813 4.7
1.16950184093978 4.4
1.16957476131022 4.1
1.16968659928853 3.8
1.16990450859671 3.5
1.1703236518478 3.2
1.17103593471721 2.9
1.1723726132021 2.6
1.1747945857593 2.3
1.17915881597298 2
1.18706044005777 1.7
1.20123746919531 1.4
1.22635293984955 1.1
1.26993638928534 0.8
1.343166747717 0.5
1.4 0.351171009658952
1.48891315770487 0.2
1.7 -0.0435163089388764
1.83082400700639 -0.1
2 -0.158867306896595
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
2 0.166777778813658
2.3 0.192758129392047
2.31572507496053 0.2
2.6 0.347548856107239
2.80789659845925 0.5
2.9 0.57570273790569
3.14412098352474 0.8
3.2 0.857408958491147
3.43614894686696 1.1
3.5 1.17322431744
3.71057368028831 1.4
3.8 1.50683271806568
3.97764601872064 1.7
4.1 1.84562726951993
4.24341144529514 2
4.4 2.18108941991995
4.51242433109066 2.3
4.7 2.50897369922007
4.78757005169376 2.6
5 2.8286368888116
5 2.9
5 3.2
5 3.5
5 3.8
5 4.1
5 4.1245482456077
4.99920418229785 4.1
4.83566566079458 3.8
4.7 3.59027156994091
4.65431245958465 3.5
4.46679646333315 3.2
4.4 3.10612988346239
4.27716456659768 2.9
4.1 2.63304533402494
4.08111104770374 2.6
3.8877779464906 2.3
3.8 2.17898907047089
3.68436569932029 2
3.5 1.74449614030419
3.46958316404155 1.7
3.24034125137871 1.4
3.2 1.35333350672374
2.97950552407279 1.1
2.9 1.01816932622466
2.65866396099234 0.8
2.6 0.75250893177336
2.3 0.597292619886785
2 0.609145867328913
1.82397204670725 0.8
1.7 1.04167153580843
1.68515595443357 1.1
1.63982417938353 1.4
1.61423580207149 1.7
1.60000065880779 2
1.59208687979173 2.3
1.58774520778606 2.6
1.58529916659512 2.9
1.58400634480386 3.2
1.58335510734165 3.5
1.58287300080076 3.8
1.582646537395 4.1
1.58251303589843 4.4
1.58242953182988 4.7
1.58243605047107 5
1.4 5
1.35262566072362 5
1.35258944055915 4.7
1.35258177370048 4.4
1.35271362078584 4.1
1.35283288509833 3.8
1.35307431086848 3.5
1.3535491195496 3.2
1.35431574511678 2.9
1.35583384755197 2.6
1.35853027287525 2.3
1.36343835195915 2
1.37226191046083 1.7
1.38804363109099 1.4
1.4 1.27013215801376
1.42206007300931 1.1
1.49026582027566 0.8
1.60753083931162 0.5
1.7 0.349877756590416
1.92893569379234 0.2
2 0.166777778813658
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
4.7 4.5334197657555
5 4.40916207848949
5 4.7
5 5
4.7 5
4.44582721388638 5
4.58752643054022 4.7
4.7 4.5334197657555
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
2 0.609145867328913
2.3 0.597292619886785
2.6 0.75250893177336
2.65866396099234 0.8
2.9 1.01816932622466
2.97950552407279 1.1
3.2 1.35333350672374
3.24034125137871 1.4
3.46958316404155 1.7
3.5 1.74449614030419
3.68436569932029 2
3.8 2.17898907047089
3.8877779464906 2.3
4.08111104770374 2.6
4.1 2.63304533402494
4.27716456659768 2.9
4.4 3.10612988346239
4.46679646333315 3.2
4.65431245958465 3.5
4.7 3.59027156994091
4.83566566079458 3.8
4.99920418229785 4.1
5 4.1245482456077
5 4.4
5 4.40916207848949
4.7 4.5334197657555
4.58752643054022 4.7
4.44582721388638 5
4.4 5
4.1 5
3.82806761644402 5
3.83141817324806 4.7
3.83508451408783 4.4
3.83535562968846 4.1
3.82187023414471 3.8
3.8 3.64365400094681
3.77957216597602 3.5
3.70117504940218 3.2
3.59467196298947 2.9
3.5 2.68047944237142
3.46342679270703 2.6
3.30696166247405 2.3
3.2 2.10883171139053
3.12982614508176 2
2.92804945507068 1.7
2.9 1.66273796609349
2.64598369636844 1.4
2.6 1.35527797807633
2.3 1.23776497299511
2.10263863400719 1.4
2 1.58574853254512
1.97779967975766 1.7
1.9451794822899 2
1.92737452171822 2.3
1.91757690126985 2.6
1.91226167814291 2.9
1.90932013041649 3.2
1.90772780925878 3.5
1.9068632884806 3.8
1.90672461175671 4.1
1.90595684498462 4.4
1.90549875359533 4.7
1.90560189604378 5
1.7 5
1.58243605047107 5
1.58242953182988 4.7
1.58251303589843 4.4
1.582646537395 4.1
1.58287300080076 3.8
1.58335510734165 3.5
1.58400634480386 3.2
1.58529916659512 2.9
1.58774520778606 2.6
1.59208687979173 2.3
1.60000065880779 2
1.61423580207149 1.7
1.63982417938353 1.4
1.68515595443357 1.1
1.7 1.04167153580843
1.82397204670725 0.8
2 0.609145867328913
};
\addplot [draw=none, fill=lavender231240249]
table{%
x  y
2.3 1.23776497299511
2.6 1.35527797807633
2.64598369636844 1.4
2.9 1.66273796609349
2.92804945507068 1.7
3.12982614508176 2
3.2 2.10883171139053
3.30696166247405 2.3
3.46342679270703 2.6
3.5 2.68047944237142
3.59467196298947 2.9
3.70117504940218 3.2
3.77957216597602 3.5
3.8 3.64365400094681
3.82187023414471 3.8
3.83535562968846 4.1
3.83508451408783 4.4
3.83141817324806 4.7
3.82806761644402 5
3.8 5
3.5 5
3.2 5
2.9 5
2.6 5
2.3 5
2 5
1.90560189604378 5
1.90549875359533 4.7
1.90595684498462 4.4
1.90672461175671 4.1
1.9068632884806 3.8
1.90772780925878 3.5
1.90932013041649 3.2
1.91226167814291 2.9
1.91757690126985 2.6
1.92737452171822 2.3
1.9451794822899 2
1.97779967975766 1.7
2 1.58574853254512
2.10263863400719 1.4
2.3 1.23776497299511
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.3 5
};
\coordinate (MCMC_mean_lml_t) at (axis cs:2.3,4.3999999999999995);
\end{axis}



==> fig/tikz/sonar/LA_mean_lml.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=black]
table{%
x  y
-0.7 2.5419421610295
-0.4 2.54590893508679
-0.1 2.56666240669374
0.0424092226140856 2.6
0.2 2.63848968894809
0.5 2.82527635850863
0.562263197606425 2.9
0.78979626839934 3.2
0.8 3.21474422799801
0.934953052193053 3.5
1.0599099339701 3.8
1.1 3.90682929944879
1.163921621219 4.1
1.25405797402585 4.4
1.33374650523851 4.7
1.4 4.97801310047305
1.40555649720428 5
1.4 5
1.1 5
0.8 5
0.5 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.5415203164776
-0.7 2.5419421610295
};
\addplot [draw=none, fill=midnightblue854116]
table{%
x  y
-0.7 2.31953744771536
-0.4 2.32340565771285
-0.1 2.34360136333392
0.2 2.41218417632197
0.5 2.5874922885006
0.511218077275012 2.6
0.760745441253001 2.9
0.8 2.95183746285302
0.928793199043521 3.2
1.06608431985975 3.5
1.1 3.58229771080106
1.17925517809806 3.8
1.27585391627384 4.1
1.36370182876201 4.4
1.4 4.53982227421945
1.44413749829955 4.7
1.51874075335972 5
1.40555649720428 5
1.4 4.97801310047305
1.33374650523851 4.7
1.25405797402585 4.4
1.163921621219 4.1
1.1 3.90682929944879
1.0599099339701 3.8
0.934953052193053 3.5
0.8 3.21474422799801
0.78979626839934 3.2
0.562263197606425 2.9
0.5 2.82527635850863
0.2 2.63848968894809
0.0424092226140856 2.6
-0.1 2.56666240669374
-0.4 2.54590893508679
-0.7 2.5419421610295
-1 2.5415203164776
-1 2.31912617437663
-0.7 2.31953744771536
};
\addplot [draw=none, fill=midnightblue868137]
table{%
x  y
-0.7 2.09918130578114
-0.4 2.10291058137983
-0.1 2.12234862961794
0.2 2.18826805001136
0.400892347962246 2.3
0.5 2.35701866327328
0.717928228670548 2.6
0.8 2.69932037679758
0.913745569986524 2.9
1.06482235640694 3.2
1.1 3.27758386097522
1.18920779870272 3.5
1.29509506752694 3.8
1.38778621132868 4.1
1.4 4.14207283797893
1.4802435343806 4.4
1.56051834240038 4.7
1.63192500951517 5
1.51874075335972 5
1.44413749829955 4.7
1.4 4.53982227421945
1.36370182876201 4.4
1.27585391627384 4.1
1.17925517809806 3.8
1.1 3.58229771080106
1.06608431985975 3.5
0.928793199043521 3.2
0.8 2.95183746285302
0.760745441253001 2.9
0.511218077275012 2.6
0.5 2.5874922885006
0.2 2.41218417632197
-0.1 2.34360136333392
-0.4 2.32340565771285
-0.7 2.31953744771536
-1 2.31912617437663
-1 2.3
-1 2.09878510125521
-0.7 2.09918130578114
};
\addplot [draw=none, fill=teal882156]
table{%
x  y
-0.7 1.87600206803703
-0.4 1.8797193815808
-0.1 1.8990659870282
0.2 1.96458245796871
0.2649357991981 2
0.5 2.12813802955171
0.662778570193863 2.3
0.8 2.4538157485332
0.889593153696283 2.6
1.05553294791658 2.9
1.1 2.98917923453642
1.19308096702852 3.2
1.3095375938239 3.5
1.4 3.76653312395777
1.41223668207108 3.8
1.51155454950732 4.1
1.60019892926574 4.4
1.6768991865012 4.7
1.7 4.79973860228521
1.75932442361183 5
1.7 5
1.63192500951517 5
1.56051834240038 4.7
1.4802435343806 4.4
1.4 4.14207283797893
1.38778621132868 4.1
1.29509506752694 3.8
1.18920779870272 3.5
1.1 3.27758386097521
1.06482235640694 3.2
0.913745569986524 2.9
0.8 2.69932037679758
0.717928228670548 2.6
0.5 2.35701866327328
0.400892347962246 2.3
0.2 2.18826805001136
-0.1 2.12234862961794
-0.4 2.10291058137983
-0.7 2.09918130578114
-1 2.09878510125521
-1 2
-1 1.87560748115753
-0.7 1.87600206803703
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 1.64651334447519
-0.4 1.65039952877993
-0.1 1.67059682085392
0.0298339521476609 1.7
0.2 1.73609783800867
0.5 1.89709413789804
0.599775273267261 2
0.8 2.21200255996515
0.857261803650324 2.3
1.03818152875975 2.6
1.1 2.71321588785154
1.19038975566022 2.9
1.31862916197473 3.2
1.4 3.41692430553875
1.43344567580596 3.5
1.54186644685367 3.8
1.63677259782164 4.1
1.7 4.32509951810601
1.72599513066029 4.4
1.82098205556579 4.7
1.90817612089693 5
1.75932442361183 5
1.7 4.79973860228521
1.6768991865012 4.7
1.60019892926574 4.4
1.51155454950732 4.1
1.41223668207108 3.8
1.4 3.76653312395777
1.3095375938239 3.5
1.19308096702852 3.2
1.1 2.98917923453642
1.05553294791658 2.9
0.889593153696283 2.6
0.8 2.4538157485332
0.662778570193863 2.3
0.5 2.12813802955171
0.2649357991981 2
0.2 1.96458245796871
-0.1 1.8990659870282
-0.4 1.8797193815808
-0.7 1.87600206803703
-1 1.87560748115753
-1 1.7
-1 1.6461011929407
-0.7 1.64651334447519
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.7 1.40343714025018
-0.4 1.40719492287684
-0.1 1.42667272433701
0.2 1.49243735734176
0.5 1.65954477926643
0.538268585281586 1.7
0.8 1.97041660451584
0.819823794809938 2
1.01390291153605 2.3
1.1 2.44545926862778
1.18118130464237 2.6
1.32207988652762 2.9
1.4 3.08812397044502
1.44953855113651 3.2
1.56819168004561 3.5
1.67149621163627 3.8
1.7 3.89226666343827
1.7786606690154 4.1
1.88071409519129 4.4
1.97192533524665 4.7
2 4.79804454265709
2.06876716960773 5
2 5
1.90817612089693 5
1.82098205556579 4.7
1.72599513066029 4.4
1.7 4.32509951810601
1.63677259782164 4.1
1.54186644685367 3.8
1.43344567580596 3.5
1.4 3.41692430553875
1.31862916197473 3.2
1.19038975566022 2.9
1.1 2.71321588785154
1.03818152875975 2.6
0.857261803650324 2.3
0.8 2.21200255996515
0.599775273267261 2
0.5 1.89709413789804
0.2 1.73609783800867
0.0298339521476609 1.7
-0.1 1.67059682085392
-0.4 1.65039952877993
-0.7 1.64651334447519
-1 1.6461011929407
-1 1.40303878561636
-0.7 1.40343714025018
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
-0.7 1.12342854076245
-0.4 1.12756059962255
-0.1 1.14896335817529
0.2 1.22139715595257
0.489397198623783 1.4
0.5 1.40581024843363
0.778288571725537 1.7
0.8 1.72243189156138
0.985998028198479 2
1.1 2.18110952414929
1.1666009927509 2.3
1.32019953113386 2.6
1.4 2.7753052496609
1.460456500785 2.9
1.59032279240676 3.2
1.7 3.49183302325806
1.70368784326597 3.5
1.8276402101955 3.8
1.93755134151465 4.1
2 4.28955024674938
2.04378877392727 4.4
2.15150501102855 4.7
2.24826044569505 5
2.06876716960773 5
2 4.79804454265709
1.97192533524665 4.7
1.88071409519129 4.4
1.7786606690154 4.1
1.7 3.89226666343827
1.67149621163627 3.8
1.56819168004561 3.5
1.44953855113651 3.2
1.4 3.08812397044502
1.32207988652762 2.9
1.18118130464237 2.6
1.1 2.44545926862778
1.01390291153605 2.3
0.819823794809938 2
0.8 1.97041660451584
0.538268585281586 1.7
0.5 1.65954477926643
0.2 1.49243735734176
-0.1 1.42667272433701
-0.4 1.40719492287684
-0.7 1.40343714025018
-1 1.40303878561636
-1 1.4
-1 1.12299077991299
-0.7 1.12342854076245
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
-0.7 0.763615961735051
-0.4 0.770412295162155
-0.15010469067348 0.8
-0.1 0.804182960071555
0.2 0.889448312931198
0.482751216039434 1.1
0.5 1.11039955021058
0.748767193289071 1.4
0.8 1.45434881114903
0.961384414368374 1.7
1.1 1.91399753176735
1.14984583921328 2
1.31448671540043 2.3
1.4 2.4727444086919
1.46690966629506 2.6
1.60852274449983 2.9
1.7 3.12097149837591
1.73886937244809 3.2
1.87284221660856 3.5
1.99125762097738 3.8
2 3.82427238806016
2.11953361509439 4.1
2.2349930846249 4.4
2.3 4.58813115340713
2.34987330036822 4.7
2.47429409804437 5
2.3 5
2.24826044569505 5
2.15150501102855 4.7
2.04378877392727 4.4
2 4.28955024674938
1.93755134151465 4.1
1.8276402101955 3.8
1.70368784326597 3.5
1.7 3.49183302325806
1.59032279240676 3.2
1.460456500785 2.9
1.4 2.7753052496609
1.32019953113386 2.6
1.1666009927509 2.3
1.1 2.18110952414929
0.985998028198479 2
0.8 1.72243189156138
0.778288571725537 1.7
0.5 1.40581024843363
0.489397198623783 1.4
0.2 1.22139715595257
-0.1 1.14896335817529
-0.4 1.12756059962255
-0.7 1.12342854076245
-1 1.12299077991299
-1 1.1
-1 0.8
-1 0.76289787958112
-0.7 0.763615961735051
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
-0.7 0.00906386395044136
-0.4 0.022683204008186
-0.1 0.0996035069779093
-0.000332795113220055 0.2
0.2 0.310929908346478
0.317160151091967 0.5
0.5 0.685607918818782
0.556028650311917 0.8
0.762395114789271 1.1
0.8 1.14427236649531
0.952342632992034 1.4
1.1 1.63390240513185
1.13768877197285 1.7
1.30861016851228 2
1.4 2.17314097187033
1.47108712244242 2.3
1.62398523815856 2.6
1.7 2.76762169629433
1.77054072222395 2.9
1.91478441357911 3.2
2 3.39834387851833
2.05252882806727 3.5
2.19269233297105 3.8
2.3 4.05892463507926
2.32112440434463 4.1
2.46440599197716 4.4
2.59656684580436 4.7
2.6 4.70834025354309
2.7689716590386 5
2.6 5
2.47429409804437 5
2.34987330036822 4.7
2.3 4.58813115340713
2.2349930846249 4.4
2.11953361509439 4.1
2 3.82427238806016
1.99125762097738 3.8
1.87284221660856 3.5
1.73886937244809 3.2
1.7 3.12097149837591
1.60852274449983 2.9
1.46690966629506 2.6
1.4 2.4727444086919
1.31448671540043 2.3
1.14984583921328 2
1.1 1.91399753176735
0.961384414368374 1.7
0.8 1.45434881114903
0.748767193289071 1.4
0.5 1.11039955021058
0.482751216039434 1.1
0.2 0.889448312931198
-0.1 0.804182960071555
-0.15010469067348 0.8
-0.4 0.770412295162155
-0.7 0.763615961735051
-1 0.76289787958112
-1 0.5
-1 0.2
-1 0.00764489719220519
-0.7 0.00906386395044136
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
-0.7 -1
-0.4 -1
-0.1 -1
0.2 -1
0.5 -1
0.8 -1
1.1 -1
1.21773696417642 -1
1.1 -0.892984288028696
0.952905987962947 -0.7
0.8 -0.401745724968177
0.799109365951306 -0.4
0.693183320234792 -0.1
0.671990300512717 0.2
0.725883717058675 0.5
0.8 0.670998628285098
0.838665178528701 0.8
0.977978274999737 1.1
1.1 1.31704618579108
1.14271310504614 1.4
1.30995734826826 1.7
1.4 1.86557241790589
1.47791606781298 2
1.63963545568305 2.3
1.7 2.42290365070994
1.80126414686504 2.6
1.95511196299276 2.9
2 2.99615395763843
2.11435660630542 3.2
2.2641050775789 3.5
2.3 3.57921325659775
2.42206443446815 3.8
2.57373886246611 4.1
2.6 4.15573019530305
2.76181948736905 4.4
2.9 4.6246070521497
2.96611839589592 4.7
3.2 4.97230516525015
3.24402186943071 5
3.2 5
2.9 5
2.7689716590386 5
2.6 4.70834025354308
2.59656684580436 4.7
2.46440599197716 4.4
2.32112440434463 4.1
2.3 4.05892463507926
2.19269233297105 3.8
2.05252882806727 3.5
2 3.39834387851833
1.91478441357911 3.2
1.77054072222395 2.9
1.7 2.76762169629433
1.62398523815856 2.6
1.47108712244242 2.3
1.4 2.17314097187033
1.30861016851228 2
1.13768877197285 1.7
1.1 1.63390240513185
0.952342632992034 1.4
0.8 1.14427236649531
0.762395114789271 1.1
0.556028650311917 0.8
0.5 0.685607918818782
0.317160151091967 0.5
0.2 0.310929908346478
-0.000332795113220027 0.2
-0.1 0.0996035069779093
-0.4 0.022683204008186
-0.7 0.00906386395044137
-1 0.00764489719220519
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
2.9 -1
3.2 -1
3.5 -1
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.5
5 0.8
5 1.1
5 1.15719019704031
4.94665113650242 1.1
4.7 0.835120547259927
4.66687770113738 0.8
4.4 0.516115651810093
4.38451762218435 0.5
4.1 0.202114082651208
4.09790524622663 0.2
3.80508915410967 -0.1
3.8 -0.105341214014355
3.5 -0.397478541053309
3.49713788886405 -0.4
3.2 -0.671912639719125
3.16332377781646 -0.7
2.9 -0.91661095608708
2.76235503772267 -1
2.9 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.1 -0.892984288028696
1.21773696417642 -1
1.4 -1
1.7 -1
2 -1
2.3 -1
2.6 -1
2.76235503772267 -1
2.9 -0.91661095608708
3.16332377781646 -0.7
3.2 -0.671912639719125
3.49713788886405 -0.4
3.5 -0.397478541053309
3.8 -0.105341214014355
3.80508915410967 -0.1
4.09790524622663 0.2
4.1 0.202114082651208
4.38451762218435 0.5
4.4 0.516115651810093
4.66687770113738 0.8
4.7 0.835120547259927
4.94665113650242 1.1
5 1.15719019704031
5 1.4
5 1.7
5 1.71187738096889
4.98883810537126 1.7
4.70602705938078 1.4
4.7 1.39360343366967
4.42105868382771 1.1
4.4 1.07786288272637
4.13184451925888 0.8
4.1 0.767055099708655
3.83531212526263 0.5
3.8 0.464414534668897
3.52581323710529 0.2
3.5 0.175070455433189
3.2 -0.0935844819312744
3.19215475487074 -0.1
2.9 -0.336289449268051
2.80376451695378 -0.4
2.6 -0.537267750178346
2.3 -0.6739883842891
2.17651808654829 -0.7
2 -0.741617485666705
1.7 -0.709271773151285
1.68203719088193 -0.7
1.4 -0.553856259570135
1.25681745678855 -0.4
1.1 -0.161256096991832
1.06998236721084 -0.1
0.991688805544917 0.2
0.994665107546722 0.5
1.06467905579612 0.8
1.1 0.882907865991574
1.18607016028433 1.1
1.33187921374221 1.4
1.4 1.52900677596376
1.49733985640536 1.7
1.66152103185433 2
1.7 2.07384325319326
1.8365242703256 2.3
1.99748873151658 2.6
2 2.6049888223972
2.17840205911352 2.9
2.3 3.12796071133657
2.34597774778083 3.2
2.52181502501677 3.5
2.6 3.64552240355281
2.71625773260013 3.8
2.9 4.06370362846383
2.93441348623933 4.1
3.2 4.39337698353501
3.2104823157282 4.4
3.5 4.58553898813559
3.76227443999853 4.7
3.8 4.7169397544184
4.1 4.77633855609594
4.4 4.75847731824587
4.7 4.74224909942231
5 4.82105410285723
5 5
4.7 5
4.4 5
4.1 5
3.8 5
3.5 5
3.24402186943071 5
3.2 4.97230516525015
2.96611839589592 4.7
2.9 4.6246070521497
2.76181948736905 4.4
2.6 4.15573019530305
2.57373886246611 4.1
2.42206443446815 3.8
2.3 3.57921325659775
2.2641050775789 3.5
2.11435660630542 3.2
2 2.99615395763843
1.95511196299276 2.9
1.80126414686504 2.6
1.7 2.42290365070994
1.63963545568305 2.3
1.47791606781298 2
1.4 1.86557241790589
1.30995734826826 1.7
1.14271310504614 1.4
1.1 1.31704618579108
0.977978274999737 1.1
0.838665178528701 0.8
0.8 0.670998628285098
0.725883717058675 0.5
0.671990300512717 0.2
0.693183320234792 -0.1
0.799109365951306 -0.4
0.8 -0.401745724968177
0.952905987962947 -0.7
1.1 -0.892984288028696
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.7 -0.709271773151285
2 -0.741617485666705
2.17651808654829 -0.7
2.3 -0.6739883842891
2.6 -0.537267750178346
2.80376451695378 -0.4
2.9 -0.336289449268051
3.19215475487074 -0.1
3.2 -0.0935844819312744
3.5 0.175070455433189
3.52581323710529 0.2
3.8 0.464414534668897
3.83531212526263 0.5
4.1 0.767055099708655
4.13184451925888 0.8
4.4 1.07786288272637
4.42105868382771 1.1
4.7 1.39360343366967
4.70602705938078 1.4
4.98883810537126 1.7
5 1.71187738096889
5 2
5 2.23597278619964
4.78119357980543 2
4.7 1.91312386822083
4.50182137738616 1.7
4.4 1.59189880435983
4.22044020486996 1.4
4.1 1.2738407356907
3.93511048026839 1.1
3.8 0.961695682502989
3.64219418412128 0.8
3.5 0.660022206552038
3.33470424504705 0.5
3.2 0.375833844951955
2.99773887379784 0.2
2.9 0.119301226017904
2.6 -0.0945383899926945
2.58990743306943 -0.1
2.3 -0.247241862431271
2 -0.317235823715968
1.7 -0.271445992794565
1.46681624946175 -0.1
1.4 -0.0245726121914776
1.29593921674075 0.2
1.25705360265018 0.5
1.29979505089869 0.8
1.39640298858195 1.1
1.4 1.10780902600871
1.54844768888741 1.4
1.7 1.69716033373434
1.70171424477429 1.7
1.88738063128887 2
2 2.20172580310856
2.06653402974739 2.3
2.25274618786729 2.6
2.3 2.68279859391323
2.44867238602946 2.9
2.6 3.14965388983094
2.64314896874897 3.2
2.87989483526686 3.5
2.9 3.52722954194487
3.174678181769 3.8
3.2 3.82679510070101
3.5 3.99749314646821
3.8 4.0778193868118
4.1 4.05847173590817
4.4 4.01909460709493
4.7 4.08129112066227
4.73235952638708 4.1
5 4.23493547853752
5 4.4
5 4.7
5 4.82105410285723
4.7 4.74224909942231
4.4 4.75847731824587
4.1 4.77633855609594
3.8 4.7169397544184
3.76227443999853 4.7
3.5 4.58553898813559
3.2104823157282 4.4
3.2 4.39337698353501
2.93441348623932 4.1
2.9 4.06370362846383
2.71625773260013 3.8
2.6 3.64552240355281
2.52181502501677 3.5
2.34597774778083 3.2
2.3 3.12796071133657
2.17840205911352 2.9
2 2.6049888223972
1.99748873151658 2.6
1.8365242703256 2.3
1.7 2.07384325319326
1.66152103185433 2
1.49733985640536 1.7
1.4 1.52900677596376
1.33187921374221 1.4
1.18607016028433 1.1
1.1 0.882907865991574
1.06467905579612 0.8
0.994665107546722 0.5
0.991688805544917 0.2
1.06998236721084 -0.1
1.1 -0.161256096991832
1.25681745678855 -0.4
1.4 -0.553856259570135
1.68203719088193 -0.7
1.7 -0.709271773151285
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.7 -0.271445992794565
2 -0.317235823715968
2.3 -0.247241862431271
2.58990743306943 -0.1
2.6 -0.0945383899926945
2.9 0.119301226017904
2.99773887379784 0.2
3.2 0.375833844951955
3.33470424504705 0.5
3.5 0.660022206552038
3.64219418412128 0.8
3.8 0.961695682502989
3.93511048026839 1.1
4.1 1.2738407356907
4.22044020486995 1.4
4.4 1.59189880435983
4.50182137738616 1.7
4.7 1.91312386822083
4.78119357980543 2
5 2.23597278619964
5 2.3
5 2.6
5 2.9
5 3.2
5 3.5
5 3.8
5 4.1
5 4.23493547853752
4.73235952638708 4.1
4.7 4.08129112066227
4.4 4.01909460709493
4.1 4.05847173590817
3.8 4.0778193868118
3.5 3.99749314646821
3.2 3.82679510070101
3.174678181769 3.8
2.9 3.52722954194486
2.87989483526686 3.5
2.64314896874897 3.2
2.6 3.14965388983094
2.44867238602946 2.9
2.3 2.68279859391323
2.25274618786729 2.6
2.06653402974739 2.3
2 2.20172580310856
1.88738063128887 2
1.70171424477429 1.7
1.7 1.69716033373434
1.54844768888741 1.4
1.4 1.10780902600871
1.39640298858195 1.1
1.29979505089869 0.8
1.25705360265018 0.5
1.29593921674075 0.2
1.4 -0.0245726121914775
1.46681624946175 -0.1
1.7 -0.271445992794565

1.7754696411695 0.2
1.7 0.246584193613995
1.58685226171352 0.5
1.58755874177715 0.8
1.66649746448138 1.1
1.7 1.17882178157543
1.81606161989662 1.4
1.97631552968635 1.7
2 1.74233566665997
2.1782437403804 2
2.3 2.19684722349277
2.38032959072012 2.3
2.58539842022966 2.6
2.6 2.62280142848537
2.8560147930286 2.9
2.9 2.95275286716952
3.2 3.19226669769613
3.22685186539382 3.2
3.5 3.28262760676088
3.8 3.21458328306168
3.83934893940408 3.2
4.1 3.06158923358511
4.4 3.00096184264522
4.63565762716813 2.9
4.51066130732037 2.6
4.4 2.43427501108499
4.32612348154794 2.3
4.11431984850099 2
4.1 1.9832181340341
3.8788217783665 1.7
3.8 1.60870411577546
3.63548343557671 1.4
3.5 1.24764274628287
3.37768367035547 1.1
3.2 0.912027727880328
3.0962754339774 0.8
2.9 0.614594579199633
2.76996130861712 0.5
2.6 0.36870424757768
2.32048957652716 0.2
2.3 0.189042502011088
2 0.126046548352351
1.7754696411695 0.2
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
2 0.126046548352351
2.3 0.189042502011088
2.32048957652716 0.2
2.6 0.36870424757768
2.76996130861712 0.5
2.9 0.614594579199633
3.0962754339774 0.8
3.2 0.912027727880328
3.37768367035547 1.1
3.5 1.24764274628287
3.63548343557671 1.4
3.8 1.60870411577546
3.8788217783665 1.7
4.1 1.9832181340341
4.11431984850099 2
4.32612348154794 2.3
4.4 2.43427501108499
4.51066130732037 2.6
4.63565762716813 2.9
4.4 3.00096184264522
4.1 3.06158923358511
3.83934893940408 3.2
3.8 3.21458328306168
3.5 3.28262760676088
3.22685186539382 3.2
3.2 3.19226669769613
2.9 2.95275286716952
2.8560147930286 2.9
2.6 2.62280142848537
2.58539842022966 2.6
2.38032959072013 2.3
2.3 2.19684722349277
2.1782437403804 2
2 1.74233566665997
1.97631552968635 1.7
1.81606161989662 1.4
1.7 1.17882178157543
1.66649746448138 1.1
1.58755874177715 0.8
1.58685226171352 0.5
1.7 0.246584193613995
1.7754696411695 0.2
2 0.126046548352351

2.20298295806207 1.1
2.27920351111664 1.4
2.3 1.43964078841077
2.51272948353604 1.7
2.6 1.82522837228171
2.87490813795415 2
2.9 2.01846452642803
2.92403157820986 2
2.96689566178279 1.7
2.9 1.5293249276099
2.83004144610202 1.4
2.61749892794739 1.1
2.6 1.08197978881467
2.3 0.929958501274746
2.20298295806207 1.1
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
2.3 0.929958501274746
2.6 1.08197978881467
2.61749892794739 1.1
2.83004144610202 1.4
2.9 1.5293249276099
2.96689566178279 1.7
2.92403157820986 2
2.9 2.01846452642803
2.87490813795415 2
2.6 1.82522837228171
2.51272948353604 1.7
2.3 1.43964078841077
2.27920351111664 1.4
2.20298295806207 1.1
2.3 0.929958501274746
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.6 1.4
};
\coordinate (LA_mean_lml_t) at (axis cs:2.5999999999999996,1.4);
\end{axis}



==> fig/tikz/sonar/LA_nlpd.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
-0.7 -1
-0.4 -1
-0.1 -1
0.2 -1
0.5 -1
0.8 -1
0.858450849754058 -1
0.8 -0.90211174558615
0.675915292392639 -0.7
0.550807025344361 -0.4
0.5 -0.210297250008607
0.457895605368133 -0.1
0.386878072784125 0.2
0.357332275261367 0.5
0.356662956964188 0.8
0.378789911713104 1.1
0.421639848186834 1.4
0.486003411153453 1.7
0.5 1.75456710508547
0.545474537893888 2
0.617159280656287 2.3
0.711169661274424 2.6
0.8 2.82954376306057
0.82668565334845 2.9
0.951961390864461 3.2
1.1 3.47817184761857
1.11221209842927 3.5
1.28722442353139 3.8
1.4 3.96751789481104
1.49296180786847 4.1
1.7 4.36800118257464
1.72288756636034 4.4
1.94437918168139 4.7
2 4.77132719707694
2.15322306821516 5
2 5
1.7 5
1.4 5
1.1 5
0.8 5
0.5 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.287533860959105
4.91059765442421 0.2
4.7 -0.00765053490141188
4.6042372308721 -0.1
4.4 -0.299353787242402
4.29295732581158 -0.4
4.1 -0.585192570414855
3.97268972517353 -0.7
3.8 -0.861181321738935
3.63517704904432 -1
3.8 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
0.8 -0.90211174558615
0.858450849754058 -1
1.1 -1
1.32380325835952 -1
1.1 -0.751326992389011
1.06329295399059 -0.7
0.887774238705091 -0.4
0.8 -0.168472288070813
0.771683034008006 -0.1
0.693528664944386 0.2
0.66200871294816 0.5
0.665242184222116 0.8
0.697259190531989 1.1
0.756103803426912 1.4
0.8 1.56220392180396
0.835056748697184 1.7
0.930794098954081 2
1.05660131317697 2.3
1.1 2.39149015306937
1.20391096968409 2.6
1.38391090941112 2.9
1.4 2.92548385071163
1.58179791026229 3.2
1.7 3.35984076045778
1.7984359264743 3.5
2 3.76487184323181
2.0234641508319 3.8
2.22910744005815 4.1
2.3 4.1968689305856
2.42562962023464 4.4
2.6 4.65422444601798
2.62643673101975 4.7
2.80442953433356 5
2.6 5
2.3 5
2.15322306821516 5
2 4.77132719707694
1.94437918168139 4.7
1.72288756636034 4.4
1.7 4.36800118257464
1.49296180786847 4.1
1.4 3.96751789481104
1.28722442353139 3.8
1.11221209842927 3.5
1.1 3.47817184761857
0.951961390864461 3.2
0.82668565334845 2.9
0.8 2.82954376306057
0.711169661274424 2.6
0.617159280656287 2.3
0.545474537893888 2
0.5 1.75456710508547
0.486003411153453 1.7
0.421639848186834 1.4
0.378789911713104 1.1
0.356662956964188 0.8
0.357332275261367 0.5
0.386878072784125 0.2
0.457895605368133 -0.1
0.5 -0.210297250008607
0.550807025344361 -0.4
0.675915292392639 -0.7
0.8 -0.90211174558615
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
3.2 -1
3.5 -1
3.63517704904432 -1
3.8 -0.861181321738935
3.97268972517353 -0.7
4.1 -0.585192570414855
4.29295732581158 -0.4
4.4 -0.299353787242402
4.6042372308721 -0.1
4.7 -0.00765053490141188
4.91059765442421 0.2
5 0.287533860959105
5 0.5
5 0.8
5 0.8280507331679
4.97147123527642 0.8
4.7 0.532578556629122
4.66645675476555 0.5
4.4 0.240330106850089
4.35760598393492 0.2
4.1 -0.0465863805264019
4.04186938130045 -0.1
3.8 -0.324817781878379
3.7132932878362 -0.4
3.5 -0.589018595421012
3.35893394510637 -0.7
3.2 -0.830359212490653
2.94562412024698 -1
3.2 -1
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.1 -0.751326992389011
1.32380325835952 -1
1.4 -1
1.7 -1
2 -1
2.3 -1
2.6 -1
2.9 -1
2.94562412024698 -1
3.2 -0.830359212490653
3.35893394510637 -0.7
3.5 -0.589018595421012
3.7132932878362 -0.4
3.8 -0.324817781878379
4.04186938130045 -0.1
4.1 -0.0465863805264019
4.35760598393492 0.2
4.4 0.240330106850089
4.66645675476555 0.5
4.7 0.532578556629122
4.97147123527642 0.8
5 0.8280507331679
5 1.1
5 1.19184572447153
4.90687785020918 1.1
4.7 0.89618365615246
4.60148153958075 0.8
4.4 0.603618063303677
4.29200259725414 0.5
4.1 0.316178491767025
3.97526241793472 0.2
3.8 0.0370836001765468
3.6451600463051 -0.1
3.5 -0.228592544747069
3.28873141146874 -0.4
3.2 -0.472679842349154
2.9 -0.68326139854711
2.87047490185629 -0.7
2.6 -0.8560873001587
2.3 -0.960021591391963
2 -0.984790914487716
1.7 -0.911462731673425
1.4 -0.704470591676837
1.39586641566079 -0.7
1.15894658312674 -0.4
1.1 -0.294525277462301
1.0082036313025 -0.1
0.924790212019816 0.2
0.891420728242819 0.5
0.898608098207334 0.8
0.940299156107995 1.1
1.01393170854295 1.4
1.1 1.64756309396143
1.11916921717541 1.7
1.24880815033481 2
1.4 2.27756741566215
1.41302189013927 2.3
1.5998421163878 2.6
1.7 2.74310434040593
1.80724218919349 2.9
2 3.16044392761455
2.02630122647683 3.2
2.23052799564378 3.5
2.3 3.59638404238173
2.4271411802492 3.8
2.6 4.05531288240384
2.62617910040847 4.1
2.80457523361823 4.4
2.9 4.5482365443923
2.98429431327004 4.7
3.16243921670402 5
2.9 5
2.80442953433356 5
2.62643673101975 4.7
2.6 4.65422444601798
2.42562962023464 4.4
2.3 4.1968689305856
2.22910744005815 4.1
2.0234641508319 3.8
2 3.76487184323181
1.7984359264743 3.5
1.7 3.35984076045778
1.58179791026229 3.2
1.4 2.92548385071163
1.38391090941112 2.9
1.20391096968409 2.6
1.1 2.39149015306937
1.05660131317697 2.3
0.930794098954081 2
0.835056748697184 1.7
0.8 1.56220392180396
0.756103803426912 1.4
0.697259190531989 1.1
0.665242184222116 0.8
0.66200871294816 0.5
0.693528664944386 0.2
0.771683034008006 -0.1
0.8 -0.168472288070813
0.887774238705091 -0.4
1.06329295399059 -0.7
1.1 -0.751326992389011
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.4 -0.704470591676837
1.7 -0.911462731673425
2 -0.984790914487716
2.3 -0.960021591391963
2.6 -0.8560873001587
2.87047490185629 -0.7
2.9 -0.68326139854711
3.2 -0.472679842349154
3.28873141146874 -0.4
3.5 -0.228592544747069
3.6451600463051 -0.1
3.8 0.0370836001765469
3.97526241793472 0.2
4.1 0.316178491767025
4.29200259725414 0.5
4.4 0.603618063303677
4.60148153958075 0.8
4.7 0.89618365615246
4.90687785020918 1.1
5 1.19184572447153
5 1.4
5 1.52436750739704
4.8744128818768 1.4
4.7 1.22797264568348
4.56979852569215 1.1
4.4 0.934195154061715
4.26164237708675 0.8
4.1 0.644807566927222
3.94713389038181 0.5
3.8 0.362675386340662
3.62086360074135 0.2
3.5 0.0923682212563318
3.27143324661511 -0.1
3.2 -0.158846768915778
2.9 -0.379128639566615
2.8658787887668 -0.4
2.6 -0.555914437818297
2.3 -0.668353149606771
2 -0.695236175611101
1.7 -0.606365719595095
1.44371156104062 -0.4
1.4 -0.353962602602168
1.24526351852578 -0.1
1.1385379630426 0.2
1.1 0.482151149535622
1.09776090175814 0.5
1.1 0.556035440744115
1.110181483251 0.8
1.1649937070323 1.1
1.25573366323058 1.4
1.38208341345117 1.7
1.4 1.73620014462783
1.54050416140996 2
1.7 2.25350281024685
1.72980796796619 2.3
1.93298436905691 2.6
2 2.69266995245416
2.1371567916999 2.9
2.3 3.13212501188761
2.34289403995944 3.2
2.53553611845737 3.5
2.6 3.59615516619865
2.72066906600692 3.8
2.9 4.08505191219658
2.90859160810642 4.1
3.07854172940324 4.4
3.2 4.60071682680012
3.25392082851301 4.7
3.41821357312896 5
3.2 5
3.16243921670402 5
2.98429431327004 4.7
2.9 4.5482365443923
2.80457523361823 4.4
2.62617910040847 4.1
2.6 4.05531288240384
2.4271411802492 3.8
2.3 3.59638404238173
2.23052799564378 3.5
2.02630122647683 3.2
2 3.16044392761455
1.80724218919349 2.9
1.7 2.74310434040593
1.5998421163878 2.6
1.41302189013927 2.3
1.4 2.27756741566215
1.24880815033481 2
1.11916921717541 1.7
1.1 1.64756309396143
1.01393170854295 1.4
0.940299156107995 1.1
0.898608098207334 0.8
0.891420728242819 0.5
0.924790212019816 0.2
1.0082036313025 -0.1
1.1 -0.294525277462301
1.15894658312674 -0.4
1.39586641566079 -0.7
1.4 -0.704470591676837
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.7 -0.606365719595095
2 -0.695236175611101
2.3 -0.668353149606771
2.6 -0.555914437818297
2.8658787887668 -0.4
2.9 -0.379128639566615
3.2 -0.158846768915778
3.27143324661511 -0.1
3.5 0.0923682212563318
3.62086360074135 0.2
3.8 0.362675386340662
3.94713389038181 0.5
4.1 0.644807566927222
4.26164237708675 0.8
4.4 0.934195154061715
4.56979852569215 1.1
4.7 1.22797264568348
4.8744128818768 1.4
5 1.52436750739704
5 1.7
5 1.87521601796271
4.82413759905145 1.7
4.7 1.57719591971941
4.52149554196447 1.4
4.4 1.28078763700607
4.21648258358248 1.1
4.1 0.987319841725494
3.9068163782932 0.8
3.8 0.699191213647369
3.58782285474697 0.5
3.5 0.420593409169734
3.2494479380085 0.2
3.2 0.158492462609989
2.9 -0.073836835329406
2.86060007541799 -0.1
2.6 -0.258934497992782
2.3 -0.381818875288457
2.0947477203556 -0.4
2 -0.407777917492372
1.97655333546479 -0.4
1.7 -0.288489620152778
1.51995360075315 -0.1
1.4 0.106076763681022
1.36319903432995 0.2
1.31412459024189 0.5
1.32568667880174 0.8
1.38714325612807 1.1
1.4 1.13854992039393
1.49697262134466 1.4
1.64142847462614 1.7
1.7 1.80239540104479
1.81866375358602 2
2 2.27418817880065
2.01655773290037 2.3
2.21344481076339 2.6
2.3 2.72616751224559
2.41048559763635 2.9
2.6 3.19206628925516
2.60483594888864 3.2
2.78484256672637 3.5
2.9 3.68619533759035
2.96686157135894 3.8
3.14120168423702 4.1
3.2 4.19846186301998
3.31241541794585 4.4
3.47980013133056 4.7
3.5 4.73542180585003
3.64687705015033 5
3.5 5
3.41821357312896 5
3.25392082851301 4.7
3.2 4.60071682680012
3.07854172940324 4.4
2.90859160810642 4.1
2.9 4.08505191219658
2.72066906600692 3.8
2.6 3.59615516619865
2.53553611845737 3.5
2.34289403995944 3.2
2.3 3.13212501188761
2.1371567916999 2.9
2 2.69266995245416
1.93298436905691 2.6
1.72980796796619 2.3
1.7 2.25350281024685
1.54050416140996 2
1.4 1.73620014462783
1.38208341345117 1.7
1.25573366323058 1.4
1.1649937070323 1.1
1.110181483251 0.8
1.1 0.556035440744115
1.09776090175814 0.5
1.1 0.482151149535622
1.1385379630426 0.2
1.24526351852578 -0.1
1.4 -0.353962602602168
1.44371156104062 -0.4
1.7 -0.606365719595095
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
2 -0.407777917492372
2.0947477203556 -0.4
2.3 -0.381818875288457
2.6 -0.258934497992782
2.86060007541799 -0.1
2.9 -0.073836835329406
3.2 0.158492462609989
3.2494479380085 0.2
3.5 0.420593409169734
3.58782285474697 0.5
3.8 0.699191213647369
3.9068163782932 0.8
4.1 0.987319841725494
4.21648258358248 1.1
4.4 1.28078763700607
4.52149554196447 1.4
4.7 1.57719591971941
4.82413759905145 1.7
5 1.87521601796271
5 2
5 2.29900524689475
4.70316756199839 2
4.7 1.99684641853641
4.40611544337162 1.7
4.4 1.69393776599872
4.10932407407346 1.4
4.1 1.39083776078022
3.8109216818543 1.1
3.8 1.08945631280869
3.50627693902584 0.8
3.5 0.794148775085332
3.2 0.515241510023114
3.1832113060879 0.5
2.9 0.267270665914772
2.80700024533669 0.2
2.6 0.0657506701631916
2.3 -0.0660533305060849
2 -0.0811431543093389
1.7 0.12207367003366
1.65141147408939 0.2
1.56535204655364 0.5
1.56728301845635 0.8
1.63177717124316 1.1
1.7 1.28262999128147
1.75043247161047 1.4
1.90872078750318 1.7
2 1.85115163248032
2.09135750892257 2
2.28037423660466 2.3
2.3 2.32959145574231
2.4723893237314 2.6
2.6 2.80223671203714
2.66070067174132 2.9
2.84009168311132 3.2
2.9 3.29909548522657
3.02111222642103 3.5
3.19300737615607 3.8
3.2 3.81192099760861
3.36599283931168 4.1
3.5 4.34459954718084
3.53322667165111 4.4
3.70291210620997 4.7
3.8 4.87679320067581
3.87597838937129 5
3.8 5
3.64687705015033 5
3.5 4.73542180585003
3.47980013133056 4.7
3.31241541794585 4.4
3.2 4.19846186301998
3.14120168423702 4.1
2.96686157135894 3.8
2.9 3.68619533759035
2.78484256672637 3.5
2.60483594888864 3.2
2.6 3.19206628925516
2.41048559763635 2.9
2.3 2.72616751224559
2.21344481076339 2.6
2.01655773290037 2.3
2 2.27418817880065
1.81866375358602 2
1.7 1.80239540104479
1.64142847462614 1.7
1.49697262134466 1.4
1.4 1.13854992039393
1.38714325612807 1.1
1.32568667880174 0.8
1.31412459024189 0.5
1.36319903432995 0.2
1.4 0.106076763681022
1.51995360075315 -0.1
1.7 -0.288489620152778
1.97655333546479 -0.4
2 -0.407777917492372
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
1.7 0.12207367003366
2 -0.0811431543093389
2.3 -0.0660533305060849
2.6 0.0657506701631916
2.80700024533669 0.2
2.9 0.267270665914772
3.1832113060879 0.5
3.2 0.515241510023114
3.5 0.794148775085332
3.50627693902584 0.8
3.8 1.08945631280869
3.8109216818543 1.1
4.1 1.39083776078022
4.10932407407346 1.4
4.4 1.69393776599872
4.40611544337162 1.7
4.7 1.99684641853641
4.70316756199839 2
5 2.29900524689475
5 2.3
5 2.6
5 2.9
5 3.02649174039704
4.88994895049604 2.9
4.7 2.6919949300203
4.62421674140529 2.6
4.4 2.34528233212659
4.36455846730313 2.3
4.10853006554039 2
4.1 1.990826863581
3.85331258363998 1.7
3.8 1.64219010537523
3.59396679862019 1.4
3.5 1.29939922672518
3.32201712803414 1.1
3.2 0.976090414293064
3.02309516294653 0.8
2.9 0.689539000521915
2.65751352517244 0.5
2.6 0.459934691700749
2.3 0.340884103170795
2 0.407783571133775
1.93417690669514 0.5
1.87879166841019 0.8
1.92789483708047 1.1
2 1.29783773305421
2.04449991210219 1.4
2.20319420690014 1.7
2.3 1.87067806659302
2.37946660195087 2
2.55628761670101 2.3
2.6 2.37234576590047
2.74402523182686 2.6
2.9 2.8787570178213
2.91366920533015 2.9
3.09723293760685 3.2
3.2 3.38617508058873
3.27162026049118 3.5
3.43817840974955 3.8
3.5 3.91639795865583
3.61573760283082 4.1
3.77641340964895 4.4
3.8 4.44399914889875
3.96869797971838 4.7
4.1 4.94222695183689
4.14467594483898 5
4.1 5
3.87597838937129 5
3.8 4.87679320067581
3.70291210620997 4.7
3.53322667165111 4.4
3.5 4.34459954718084
3.36599283931168 4.1
3.2 3.81192099760861
3.19300737615607 3.8
3.02111222642103 3.5
2.9 3.29909548522657
2.84009168311132 3.2
2.66070067174132 2.9
2.6 2.80223671203714
2.4723893237314 2.6
2.3 2.32959145574231
2.28037423660466 2.3
2.09135750892257 2
2 1.85115163248032
1.90872078750318 1.7
1.75043247161047 1.4
1.7 1.28262999128147
1.63177717124316 1.1
1.56728301845635 0.8
1.56535204655364 0.5
1.65141147408939 0.2
1.7 0.12207367003366
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
2 0.407783571133775
2.3 0.340884103170795
2.6 0.459934691700749
2.65751352517244 0.5
2.9 0.689539000521915
3.02309516294653 0.8
3.2 0.976090414293064
3.32201712803414 1.1
3.5 1.29939922672518
3.59396679862019 1.4
3.8 1.64219010537523
3.85331258363998 1.7
4.1 1.990826863581
4.10853006554039 2
4.36455846730313 2.3
4.4 2.34528233212659
4.62421674140529 2.6
4.7 2.6919949300203
4.88994895049604 2.9
5 3.02649174039704
5 3.2
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.14467594483898 5
4.1 4.94222695183689
3.96869797971838 4.7
3.8 4.44399914889875
3.77641340964895 4.4
3.61573760283082 4.1
3.5 3.91639795865583
3.43817840974955 3.8
3.27162026049118 3.5
3.2 3.38617508058873
3.09723293760685 3.2
2.91366920533015 2.9
2.9 2.8787570178213
2.74402523182686 2.6
2.6 2.37234576590047
2.55628761670101 2.3
2.37946660195087 2
2.3 1.87067806659302
2.20319420690014 1.7
2.04449991210219 1.4
2 1.29783773305421
1.92789483708047 1.1
1.87879166841019 0.8
1.93417690669514 0.5
2 0.407783571133775

2.54488126102858 1.4
2.6 1.62284700793523
2.6352305636627 1.7
2.80198556741409 2
2.9 2.22630992759991
2.95166303741022 2.3
3.12720065136265 2.6
3.2 2.753549025635
3.3076679482487 2.9
3.46114157881062 3.2
3.5 3.28177742818393
3.65917124077265 3.5
3.79732406197255 3.8
3.8 3.80538806923098
4.03605131121543 4.1
4.1 4.21656522555584
4.32304160013619 4.4
4.4 4.492421151607
4.7 4.43347078480221
4.73834173823934 4.4
4.73826807860714 4.1
4.7 4.03343841071939
4.58788358565849 3.8
4.41478986582891 3.5
4.4 3.47918311838495
4.2103544388664 3.2
4.1 3.03159806265247
4.00883295700515 2.9
3.82244780435384 2.6
3.8 2.56645791527565
3.61274871052393 2.3
3.5 2.12571460575505
3.40192127709451 2
3.20093782815789 1.7
3.2 1.69878470973878
2.92796688399737 1.4
2.9 1.36913110679325
2.6 1.21935490399292
2.54488126102858 1.4
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
2.6 1.21935490399292
2.9 1.36913110679325
2.92796688399737 1.4
3.2 1.69878470973878
3.20093782815789 1.7
3.40192127709451 2
3.5 2.12571460575505
3.61274871052393 2.3
3.8 2.56645791527565
3.82244780435384 2.6
4.00883295700515 2.9
4.1 3.03159806265247
4.2103544388664 3.2
4.4 3.47918311838495
4.41478986582891 3.5
4.58788358565849 3.8
4.7 4.03343841071939
4.73826807860714 4.1
4.73834173823934 4.4
4.7 4.43347078480221
4.4 4.492421151607
4.32304160013619 4.4
4.1 4.21656522555584
4.03605131121543 4.1
3.8 3.80538806923098
3.79732406197255 3.8
3.65917124077265 3.5
3.5 3.28177742818393
3.46114157881062 3.2
3.3076679482487 2.9
3.2 2.753549025635
3.12720065136265 2.6
2.95166303741022 2.3
2.9 2.22630992759991
2.80198556741409 2
2.6352305636627 1.7
2.6 1.62284700793523
2.54488126102858 1.4
2.6 1.21935490399292
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.6 1.4
};
\coordinate (MCMC_mean_lml_t) at (axis cs:2.3,4.3999999999999995);
\end{axis}



==> fig/tikz/sonar/MCMC_mean_lml.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=teal1996167]
table{%
x  y
5 4.96754019818762
5 5
4.88475565344959 5
5 4.96754019818762
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
4.7 4.95379475357842
5 4.88377179582971
5 4.96754019818762
4.88475565344959 5
4.7 5
4.63622091029571 5
4.7 4.95379475357842
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
4.7 4.83181114483125
5 4.8000033934718
5 4.88377179582971
4.7 4.95379475357842
4.63622091029571 5
4.4678416865653 5
4.7 4.83181114483125
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
4.4 4.90006076766884
4.7 4.70982753608408
5 4.71623499111389
5 4.8000033934718
4.7 4.83181114483125
4.4678416865653 5
4.4 5
4.32867602203369 5
4.4 4.90006076766884
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
4.7 4.56896731186938
5 4.57843047493753
5 4.7
5 4.71623499111389
4.7 4.70982753608408
4.4 4.90006076766884
4.32867602203369 5
4.20922336403183 5
4.4 4.73268357866432
4.45255267036249 4.7
4.7 4.56896731186938
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
-0.7 -1
-0.4 -1
-0.1 -1
0.2 -1
0.5 -1
0.8 -1
1.1 -1
1.21465999189911 -1
1.1 -0.891272299081315
0.944452502199756 -0.7
0.8 -0.461715314288046
0.764526650399561 -0.4
0.630200745421904 -0.1
0.548548419061736 0.2
0.5 0.470078229327864
0.49192044169805 0.5
0.450371054034429 0.8
0.424933547467442 1.1
0.405335128807508 1.4
0.398664407963261 1.7
0.397013869552354 2
0.404977509992142 2.3
0.403112345197508 2.6
0.393697229816709 2.9
0.39362983965272 3.2
0.40084024706367 3.5
0.396805559124207 3.8
0.410090861233702 4.1
0.377600947028817 4.4
0.400321206212393 4.7
0.418344428107199 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
2.9 -1
3.2 -1
3.5 -1
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.5
5 0.8
5 1.1
5 1.15518807716301
4.94895014266088 1.1
4.7 0.829037462545853
4.67258846001352 0.8
4.4 0.509618657838923
4.39054823917529 0.5
4.1068747810249 0.2
4.1 0.192364860876072
3.80040414017353 -0.1
3.8 -0.100406711348457
3.50319913985983 -0.4
3.5 -0.403258291997257
3.2 -0.669870370998292
3.16103683173013 -0.7
2.9 -0.918959080527966
2.76960713471105 -1
2.9 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
4.4 4.536693046742
4.7 4.42645304775075
5 4.42763570976425
5 4.57843047493753
4.7 4.56896731186938
4.45255267036249 4.7
4.4 4.73268357866432
4.20922336403183 5
4.1 5
4.0836798758582 5
4.1 4.95866822249854
4.21992529998199 4.7
4.4 4.536693046742
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.1 -0.891272299081315
1.21465999189911 -1
1.4 -1
1.7 -1
2 -1
2.3 -1
2.6 -1
2.76960713471105 -1
2.9 -0.918959080527966
3.16103683173013 -0.7
3.2 -0.669870370998292
3.5 -0.403258291997257
3.50319913985983 -0.4
3.8 -0.100406711348457
3.80040414017353 -0.1
4.1 0.192364860876072
4.1068747810249 0.2
4.39054823917529 0.5
4.4 0.509618657838923
4.67258846001352 0.8
4.7 0.829037462545852
4.94895014266088 1.1
5 1.15518807716301
5 1.4
5 1.7
5 1.71732882558806
4.98406150011194 1.7
4.70412079470105 1.4
4.7 1.39558710022178
4.41580497367759 1.1
4.4 1.08337136837647
4.13373884356069 0.8
4.1 0.765764895576151
3.83498793284055 0.5
3.8 0.464077764207702
3.53805622298748 0.2
3.5 0.163967839960798
3.2 -0.0972466460467314
3.19674790770186 -0.1
2.9 -0.340278710601036
2.81043107257186 -0.4
2.6 -0.541654069841394
2.3 -0.676452523101304
2.18924782320821 -0.7
2 -0.745595292481217
1.7 -0.719327048817343
1.66078273871457 -0.7
1.4 -0.567870318953034
1.23777058769805 -0.4
1.1 -0.229239313305597
1.02524605063604 -0.1
0.902277717393231 0.2
0.825491223623312 0.5
0.8 0.678020179467556
0.779652142882663 0.8
0.750318662772026 1.1
0.731818170701485 1.4
0.723813353354203 1.7
0.708967468168276 2
0.709185895529595 2.3
0.713300701284686 2.6
0.705737375767297 2.9
0.714221092039486 3.2
0.69351438304545 3.5
0.705811271042395 3.8
0.707115813842384 4.1
0.69661061075143 4.4
0.723340868368687 4.7
0.712886339004541 5
0.5 5
0.418344428107199 5
0.400321206212393 4.7
0.377600947028817 4.4
0.410090861233702 4.1
0.396805559124207 3.8
0.40084024706367 3.5
0.39362983965272 3.2
0.393697229816709 2.9
0.403112345197508 2.6
0.404977509992142 2.3
0.397013869552354 2
0.398664407963261 1.7
0.405335128807508 1.4
0.424933547467442 1.1
0.450371054034429 0.8
0.49192044169805 0.5
0.5 0.470078229327864
0.548548419061736 0.2
0.630200745421904 -0.1
0.764526650399561 -0.4
0.8 -0.461715314288046
0.944452502199756 -0.7
1.1 -0.891272299081315
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
4.4 4.28655500559064
4.7 4.18931004580822
5 4.20237513586021
5 4.4
5 4.42763570976425
4.7 4.42645304775075
4.4 4.536693046742
4.21992529998199 4.7
4.1 4.95866822249854
4.0836798758582 5
3.89310150228015 5
4.01290237753385 4.7
4.1 4.53994422619633
4.26625484797304 4.4
4.4 4.28655500559064
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.7 -0.719327048817343
2 -0.745595292481217
2.18924782320821 -0.7
2.3 -0.676452523101304
2.6 -0.541654069841394
2.81043107257186 -0.4
2.9 -0.340278710601036
3.19674790770186 -0.1
3.2 -0.0972466460467314
3.5 0.163967839960798
3.53805622298748 0.2
3.8 0.464077764207702
3.83498793284055 0.5
4.1 0.765764895576151
4.13373884356069 0.8
4.4 1.08337136837647
4.41580497367759 1.1
4.7 1.39558710022178
4.70412079470105 1.4
4.98406150011194 1.7
5 1.71732882558806
5 2
5 2.24631093926525
4.77933484104206 2
4.7 1.91300912918879
4.51058298618101 1.7
4.4 1.57794257692425
4.23049166292922 1.4
4.1 1.26348429665013
3.94234417913593 1.1
3.8 0.959245436779199
3.64872386525702 0.8
3.5 0.652785616623921
3.34159547606758 0.5
3.2 0.371586354548625
2.99996740711003 0.2
2.9 0.114698138409573
2.60184468286694 -0.1
2.6 -0.101260994056586
2.3 -0.255179552535022
2 -0.328869189953262
1.7 -0.290772362964497
1.4 -0.105522492811581
1.39529797363967 -0.1
1.20947041463957 0.2
1.1 0.47018958742105
1.09041170600163 0.5
1.02988210977992 0.8
0.991297734133349 1.1
0.972237792919081 1.4
0.960975659227452 1.7
0.950798666179695 2
0.949533809757573 2.3
0.945938850174752 2.6
0.95062215494287 2.9
0.946891025442809 3.2
0.927656724200458 3.5
0.956994716254905 3.8
0.941015079109196 4.1
0.945156491021445 4.4
0.94861752590844 4.7
0.94405143967128 5
0.8 5
0.712886339004541 5
0.723340868368687 4.7
0.69661061075143 4.4
0.707115813842384 4.1
0.705811271042395 3.8
0.69351438304545 3.5
0.714221092039486 3.2
0.705737375767297 2.9
0.713300701284686 2.6
0.709185895529595 2.3
0.708967468168276 2
0.723813353354203 1.7
0.731818170701485 1.4
0.750318662772026 1.1
0.779652142882663 0.8
0.8 0.678020179467556
0.825491223623312 0.5
0.902277717393231 0.2
1.02524605063604 -0.1
1.1 -0.229239313305597
1.23777058769805 -0.4
1.4 -0.567870318953034
1.66078273871457 -0.7
1.7 -0.719327048817343
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
4.1 4.09562225933384
4.4 3.85398129639858
4.7 3.82576177240952
5 3.89916951831899
5 4.1
5 4.20237513586021
4.7 4.18931004580822
4.4 4.28655500559064
4.26625484797304 4.4
4.1 4.53994422619633
4.01290237753385 4.7
3.89310150228015 5
3.8 5
3.67532800382773 5
3.8 4.76241750333714
3.8252199145296 4.7
3.93828931776542 4.4
4.09732421909513 4.1
4.1 4.09562225933384
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.4 -0.105522492811581
1.7 -0.290772362964497
2 -0.328869189953262
2.3 -0.255179552535022
2.6 -0.101260994056586
2.60184468286694 -0.1
2.9 0.114698138409573
2.99996740711003 0.2
3.2 0.371586354548625
3.34159547606758 0.5
3.5 0.652785616623921
3.64872386525702 0.8
3.8 0.959245436779199
3.94234417913593 1.1
4.1 1.26348429665013
4.23049166292922 1.4
4.4 1.57794257692425
4.51058298618101 1.7
4.7 1.91300912918879
4.77933484104206 2
5 2.24631093926525
5 2.3
5 2.6
5 2.9
5 3.2
5 3.5
5 3.8
5 3.89916951831899
4.7 3.82576177240952
4.4 3.85398129639858
4.1 4.09562225933384
4.09732421909513 4.1
3.93828931776542 4.4
3.8252199145296 4.7
3.8 4.76241750333714
3.67532800382773 5
3.5 5
3.42527292961058 5
3.5 4.79569947077527
3.53956028284708 4.7
3.63280727508924 4.4
3.70662382996202 4.1
3.8 3.80454765518774
3.80215469492774 3.8
3.94472656863582 3.5
4.1 3.22501919193917
4.1502572909197 3.2
4.4 3.05715364018668
4.67814885488081 2.9
4.54758023939278 2.6
4.4 2.39435455908619
4.34633887399646 2.3
4.1284732974314 2
4.1 1.96779909262179
3.90542406665801 1.7
3.8 1.57500233351409
3.65747213867777 1.4
3.5 1.22487953692002
3.39873446145546 1.1
3.2 0.889110455143887
3.11830995439399 0.8
2.9 0.591008932174623
2.80057195005417 0.5
2.6 0.34107697165884
2.36331891176296 0.2
2.3 0.165902477421105
2 0.0830066183723321
1.7 0.142828840569799
1.63161910171956 0.2
1.4 0.47743019018194
1.38951493792536 0.5
1.2955867762498 0.8
1.24182963290073 1.1
1.21614583401549 1.4
1.19566669891827 1.7
1.19009313574837 2
1.18498215623709 2.3
1.17325139281029 2.6
1.1860989736092 2.9
1.17438663391022 3.2
1.16364504496345 3.5
1.19653809376397 3.8
1.16988660996745 4.1
1.18231086993907 4.4
1.16973715285556 4.7
1.17089514778742 5
1.1 5
0.94405143967128 5
0.94861752590844 4.7
0.945156491021445 4.4
0.941015079109196 4.1
0.956994716254905 3.8
0.927656724200458 3.5
0.946891025442809 3.2
0.95062215494287 2.9
0.945938850174752 2.6
0.949533809757573 2.3
0.950798666179695 2
0.960975659227452 1.7
0.972237792919081 1.4
0.991297734133349 1.1
1.02988210977992 0.8
1.09041170600163 0.5
1.1 0.47018958742105
1.20947041463957 0.2
1.39529797363967 -0.1
1.4 -0.105522492811581
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.7 0.142828840569799
2 0.0830066183723321
2.3 0.165902477421105
2.36331891176296 0.2
2.6 0.34107697165884
2.80057195005417 0.5
2.9 0.591008932174623
3.11830995439399 0.8
3.2 0.889110455143887
3.39873446145546 1.1
3.5 1.22487953692002
3.65747213867777 1.4
3.8 1.57500233351409
3.90542406665801 1.7
4.1 1.96779909262179
4.1284732974314 2
4.34633887399646 2.3
4.4 2.39435455908619
4.54758023939278 2.6
4.67814885488081 2.9
4.4 3.05715364018668
4.1502572909197 3.2
4.1 3.22501919193917
3.94472656863582 3.5
3.80215469492774 3.8
3.8 3.80454765518774
3.70662382996202 4.1
3.63280727508924 4.4
3.53956028284708 4.7
3.5 4.79569947077527
3.42527292961058 5
3.2 5
3.12313195100522 5
3.2 4.79266388338639
3.22200183135529 4.7
3.24244940973363 4.4
3.29817034540495 4.1
3.3315638817274 3.8
3.36065650296659 3.5
3.39809192677493 3.2
3.40079247236628 2.9
3.38784687672582 2.6
3.35452380407668 2.3
3.30038232213378 2
3.2 1.77146689744119
3.17117764119836 1.7
3.00079196135661 1.4
2.9 1.26689550197381
2.77111324140129 1.1
2.6 0.911577396678885
2.45111233750666 0.8
2.3 0.697284011771814
2 0.608168388461951
1.7 0.756627881508767
1.67422061979418 0.8
1.57736472583616 1.1
1.52376265749396 1.4
1.48115688446947 1.7
1.46876899657637 2
1.44746777960495 2.3
1.44207169211649 2.6
1.44851515176513 2.9
1.44340338635248 3.2
1.44179314780372 3.5
1.453586153699 3.8
1.42845737623721 4.1
1.45182882219746 4.4
1.45026841352205 4.7
1.45013483964012 5
1.4 5
1.17089514778742 5
1.16973715285556 4.7
1.18231086993907 4.4
1.16988660996745 4.1
1.19653809376397 3.8
1.16364504496345 3.5
1.17438663391022 3.2
1.1860989736092 2.9
1.17325139281029 2.6
1.18498215623709 2.3
1.19009313574837 2
1.19566669891827 1.7
1.21614583401549 1.4
1.24182963290073 1.1
1.2955867762498 0.8
1.38951493792536 0.5
1.4 0.47743019018194
1.63161910171956 0.2
1.7 0.142828840569799
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
1.7 0.756627881508767
2 0.608168388461951
2.3 0.697284011771814
2.45111233750666 0.8
2.6 0.911577396678885
2.77111324140129 1.1
2.9 1.26689550197381
3.00079196135661 1.4
3.17117764119836 1.7
3.2 1.77146689744119
3.30038232213378 2
3.35452380407668 2.3
3.38784687672582 2.6
3.40079247236628 2.9
3.39809192677493 3.2
3.36065650296659 3.5
3.3315638817274 3.8
3.29817034540495 4.1
3.24244940973363 4.4
3.22200183135529 4.7
3.2 4.79266388338639
3.12313195100522 5
2.9 5
2.62932955684343 5
2.6 4.83582916011025
2.50177571887652 4.7
2.55037859040551 4.4
2.6 4.18249693676247
2.61481366967971 4.1
2.6 3.88806099537805
2.5897271491413 3.8
2.55887093882847 3.5
2.6 3.43937718210992
2.67453684713279 3.2
2.60600076172106 2.9
2.6 2.86845624864742
2.51999028513195 2.6
2.57048812946171 2.3
2.38836158460222 2
2.3 1.82916624104418
2 1.9344918943446
1.97942319302205 2
1.98413096128117 2.3
1.97303846127936 2.6
1.96218142217195 2.9
1.94704950616493 3.2
1.94369382261925 3.5
1.97060362293718 3.8
1.9299876081082 4.1
1.91665531318873 4.4
1.93346443154491 4.7
1.96515296725738 5
1.7 5
1.45013483964012 5
1.45026841352205 4.7
1.45182882219746 4.4
1.42845737623721 4.1
1.453586153699 3.8
1.44179314780372 3.5
1.44340338635248 3.2
1.44851515176513 2.9
1.44207169211649 2.6
1.44746777960495 2.3
1.46876899657637 2
1.48115688446947 1.7
1.52376265749396 1.4
1.57736472583616 1.1
1.67422061979418 0.8
1.7 0.756627881508767
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
2 1.9344918943446
2.3 1.82916624104418
2.38836158460222 2
2.57048812946171 2.3
2.51999028513195 2.6
2.6 2.86845624864742
2.60600076172106 2.9
2.67453684713279 3.2
2.6 3.43937718210992
2.55887093882847 3.5
2.5897271491413 3.8
2.6 3.88806099537805
2.61481366967971 4.1
2.6 4.18249693676247
2.55037859040551 4.4
2.50177571887652 4.7
2.6 4.83582916011025
2.62932955684343 5
2.6 5
2.3 5
2 5
1.96515296725738 5
1.93346443154491 4.7
1.91665531318873 4.4
1.9299876081082 4.1
1.97060362293718 3.8
1.94369382261925 3.5
1.94704950616493 3.2
1.96218142217195 2.9
1.97303846127936 2.6
1.98413096128117 2.3
1.97942319302205 2
2 1.9344918943446
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.3 4.4
};
\coordinate (MCMC_mean_lml_t) at (axis cs:2.3,4.3999999999999995);
\end{axis}



==> fig/tikz/sonar/MCMC_nlpd.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
-0.7 -1
-0.4 -1
-0.1 -1
0.2 -1
0.5 -1
0.8 -1
0.855784590984756 -1
0.8 -0.910030925043458
0.66876248777036 -0.7
0.537649923904841 -0.4
0.5 -0.278378904218252
0.425313818027684 -0.1
0.341943830925648 0.2
0.29376389567299 0.5
0.265974515889218 0.8
0.251381087338949 1.1
0.241261543550524 1.4
0.237072265419835 1.7
0.234032233398144 2
0.232665105182383 2.3
0.232499636414297 2.6
0.231620378912247 2.9
0.230914412525237 3.2
0.231402463072887 3.5
0.230858626029423 3.8
0.231282302499613 4.1
0.23085853689323 4.4
0.230256289678857 4.7
0.22905861847892 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
3.8 -1
4.1 -1
4.4 -1
4.7 -1
5 -1
5 -0.7
5 -0.4
5 -0.1
5 0.2
5 0.290721533866956
4.90729556061076 0.2
4.7 -0.00351077283749773
4.59842967741124 -0.1
4.4 -0.294486473433217
4.29096902781277 -0.4
4.1 -0.580814999567983
3.96532848731861 -0.7
3.8 -0.859034426426311
3.63448352822695 -1
3.8 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
0.8 -0.910030925043458
0.855784590984756 -1
1.1 -1
1.32210356509856 -1
1.1 -0.761275456511763
1.0549549344029 -0.7
0.872167561251771 -0.4
0.8 -0.237892929628755
0.735688612066866 -0.1
0.639259206061423 0.2
0.581249576005907 0.5
0.546536799010119 0.8
0.527554041344369 1.1
0.515071992060272 1.4
0.508693577266261 1.7
0.505342625829199 2
0.503833269785337 2.3
0.502051757456063 2.6
0.501705128849181 2.9
0.50194001324051 3.2
0.501651645268985 3.5
0.500574945727238 3.8
0.501672450457658 4.1
0.501728467946873 4.4
0.501842807891978 4.7
0.500833441943481 5
0.5 5
0.22905861847892 5
0.230256289678857 4.7
0.23085853689323 4.4
0.231282302499613 4.1
0.230858626029422 3.8
0.231402463072887 3.5
0.230914412525237 3.2
0.231620378912247 2.9
0.232499636414297 2.6
0.232665105182383 2.3
0.234032233398144 2
0.237072265419835 1.7
0.241261543550524 1.4
0.251381087338949 1.1
0.265974515889218 0.8
0.29376389567299 0.5
0.341943830925648 0.2
0.425313818027684 -0.1
0.5 -0.278378904218252
0.537649923904841 -0.4
0.66876248777036 -0.7
0.8 -0.910030925043458
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
3.2 -1
3.5 -1
3.63448352822695 -1
3.8 -0.859034426426311
3.96532848731861 -0.7
4.1 -0.580814999567983
4.29096902781277 -0.4
4.4 -0.294486473433217
4.59842967741124 -0.1
4.7 -0.00351077283749773
4.90729556061076 0.2
5 0.290721533866956
5 0.5
5 0.8
5 0.835199929821241
4.9646522376468 0.8
4.7 0.540428475085999
4.65758177012618 0.5
4.4 0.249474615642887
4.34888488325409 0.2
4.1 -0.0415410777620083
4.03602437865895 -0.1
3.8 -0.319160585480253
3.70597885593229 -0.4
3.5 -0.583674423372801
3.35069652158069 -0.7
3.2 -0.822265790490041
2.93063637035373 -1
3.2 -1
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.1 -0.761275456511763
1.32210356509856 -1
1.4 -1
1.7 -1
2 -1
2.3 -1
2.6 -1
2.9 -1
2.93063637035373 -1
3.2 -0.822265790490041
3.35069652158069 -0.7
3.5 -0.583674423372801
3.70597885593229 -0.4
3.8 -0.319160585480253
4.03602437865895 -0.1
4.1 -0.0415410777620083
4.34888488325409 0.2
4.4 0.249474615642887
4.65758177012618 0.5
4.7 0.540428475085999
4.9646522376468 0.8
5 0.835199929821241
5 1.1
5 1.20407258867829
4.89442686989917 1.1
4.7 0.906304280980076
4.59233455815873 0.8
4.4 0.615660683394016
4.27767367186422 0.5
4.1 0.327413695941566
3.96468463502125 0.2
3.8 0.0477236490218834
3.63517917164311 -0.1
3.5 -0.219152717472595
3.27815241985998 -0.4
3.2 -0.464010739098961
2.9 -0.672223406615456
2.85146746772765 -0.7
2.6 -0.847939357636323
2.3 -0.953019415116844
2 -0.981427327186255
1.7 -0.90906605570829
1.4 -0.709691873861355
1.3908237991115 -0.7
1.1390887847504 -0.4
1.1 -0.340906421548591
0.97086441045775 -0.1
0.862336208469875 0.2
0.8 0.465429088012617
0.791470785444502 0.5
0.743415362457904 0.8
0.715589023546238 1.1
0.698814131390003 1.4
0.690989839863762 1.7
0.685850737384195 2
0.685097745522224 2.3
0.682092818032055 2.6
0.681211942921311 2.9
0.680700502925132 3.2
0.681265591447665 3.5
0.680289006370286 3.8
0.679756938582125 4.1
0.680288254418103 4.4
0.679922845058657 4.7
0.679691920069292 5
0.500833441943481 5
0.501842807891978 4.7
0.501728467946873 4.4
0.501672450457658 4.1
0.500574945727238 3.8
0.501651645268985 3.5
0.50194001324051 3.2
0.501705128849181 2.9
0.502051757456063 2.6
0.503833269785337 2.3
0.505342625829199 2
0.508693577266261 1.7
0.515071992060272 1.4
0.527554041344369 1.1
0.546536799010119 0.8
0.581249576005907 0.5
0.639259206061423 0.2
0.735688612066866 -0.1
0.8 -0.237892929628755
0.872167561251771 -0.4
1.0549549344029 -0.7
1.1 -0.761275456511763
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.4 -0.709691873861355
1.7 -0.90906605570829
2 -0.981427327186255
2.3 -0.953019415116844
2.6 -0.847939357636323
2.85146746772765 -0.7
2.9 -0.672223406615456
3.2 -0.464010739098961
3.27815241985998 -0.4
3.5 -0.219152717472595
3.63517917164311 -0.1
3.8 0.0477236490218834
3.96468463502125 0.2
4.1 0.327413695941566
4.27767367186422 0.5
4.4 0.615660683394016
4.59233455815873 0.8
4.7 0.906304280980076
4.89442686989917 1.1
5 1.20407258867829
5 1.4
5 1.54412800635529
4.85714860646807 1.4
4.7 1.24504014944518
4.55190048890399 1.1
4.4 0.949977386049007
4.24423519298826 0.8
4.1 0.663544203795119
3.92872496404729 0.5
3.8 0.378437543974489
3.60043913939449 0.2
3.5 0.109723288508321
3.25865004727353 -0.1
3.2 -0.148433491037811
2.9 -0.366037685374953
2.84409747834825 -0.4
2.6 -0.543916934841222
2.3 -0.659074184877798
2 -0.688137639074059
1.7 -0.608249379681067
1.4191586126476 -0.4
1.4 -0.383100497618135
1.2021270489526 -0.1
1.1 0.107173448780093
1.0624468553171 0.2
0.977894018473946 0.5
0.926519818906574 0.8
0.895228216312221 1.1
0.877050649852704 1.4
0.868102744891991 1.7
0.861814668475347 2
0.861192012356647 2.3
0.858043934928377 2.6
0.856874306608001 2.9
0.856179035672803 3.2
0.85682746476786 3.5
0.856136233402732 3.8
0.854394049040227 4.1
0.855382064957515 4.4
0.854918649827902 4.7
0.855052548309907 5
0.8 5
0.679691920069292 5
0.679922845058657 4.7
0.680288254418103 4.4
0.679756938582125 4.1
0.680289006370286 3.8
0.681265591447665 3.5
0.680700502925132 3.2
0.681211942921311 2.9
0.682092818032055 2.6
0.685097745522223 2.3
0.685850737384195 2
0.690989839863762 1.7
0.698814131390003 1.4
0.715589023546238 1.1
0.743415362457904 0.8
0.791470785444502 0.5
0.8 0.465429088012617
0.862336208469875 0.2
0.97086441045775 -0.1
1.1 -0.340906421548591
1.1390887847504 -0.4
1.3908237991115 -0.7
1.4 -0.709691873861355
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
1.7 -0.608249379681067
2 -0.688137639074059
2.3 -0.659074184877798
2.6 -0.543916934841222
2.84409747834825 -0.4
2.9 -0.366037685374953
3.2 -0.148433491037811
3.25865004727353 -0.1
3.5 0.109723288508321
3.60043913939449 0.2
3.8 0.378437543974489
3.92872496404729 0.5
4.1 0.663544203795119
4.24423519298826 0.8
4.4 0.949977386049007
4.55190048890399 1.1
4.7 1.24504014944518
4.85714860646807 1.4
5 1.54412800635529
5 1.7
5 1.89657764227212
4.80005437937654 1.7
4.7 1.59896821782855
4.50011496060656 1.4
4.4 1.30215608365097
4.19624396569181 1.1
4.1 1.00752690190738
3.88574193455454 0.8
3.8 0.718342023752044
3.56704186002539 0.5
3.5 0.440167914568084
3.22099727728505 0.2
3.2 0.181802583129959
2.9 -0.0591882002231574
2.83853443241584 -0.1
2.6 -0.244563332356626
2.3 -0.369848558210648
2.05609210010696 -0.4
2 -0.406459373040782
1.97800950970666 -0.4
1.7 -0.305784054415443
1.46882230584835 -0.1
1.4 -0.0196300728214189
1.28358138658326 0.2
1.17367205136409 0.5
1.10471116397461 0.8
1.1 0.833062337821632
1.06802829125732 1.1
1.04853915238868 1.4
1.03750561186807 1.7
1.02996178451571 2
1.02833436878568 2.3
1.02623384739837 2.6
1.02501552173312 2.9
1.02507281773242 3.2
1.0244865107503 3.5
1.02426881322184 3.8
1.02186461351097 4.1
1.02342520698405 4.4
1.02352949858715 4.7
1.02322587097197 5
0.855052548309907 5
0.854918649827902 4.7
0.855382064957515 4.4
0.854394049040227 4.1
0.856136233402732 3.8
0.85682746476786 3.5
0.856179035672803 3.2
0.856874306608001 2.9
0.858043934928377 2.6
0.861192012356647 2.3
0.861814668475346 2
0.868102744891991 1.7
0.877050649852704 1.4
0.895228216312221 1.1
0.926519818906574 0.8
0.977894018473946 0.5
1.0624468553171 0.2
1.1 0.107173448780093
1.2021270489526 -0.1
1.4 -0.383100497618135
1.4191586126476 -0.4
1.7 -0.608249379681067
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
2 -0.406459373040782
2.05609210010696 -0.4
2.3 -0.369848558210648
2.6 -0.244563332356626
2.83853443241584 -0.1
2.9 -0.0591882002231573
3.2 0.181802583129959
3.22099727728505 0.2
3.5 0.440167914568084
3.56704186002539 0.5
3.8 0.718342023752044
3.88574193455454 0.8
4.1 1.00752690190738
4.1962439656918 1.1
4.4 1.30215608365097
4.50011496060656 1.4
4.7 1.59896821782855
4.80005437937654 1.7
5 1.89657764227212
5 2
5 2.3
5 2.32977629134852
4.97274090508582 2.3
4.7 2.03205671686577
4.66847044665058 2
4.4 1.71946154001019
4.38119896815021 1.7
4.1 1.41774189271489
4.08387134698406 1.4
3.8 1.10168940050062
3.79841925719311 1.1
3.5 0.811175994798851
3.48871330093197 0.8
3.2 0.534769569789416
3.1605040840115 0.5
2.9 0.284760712635653
2.78763441314499 0.2
2.6 0.0756506511919061
2.3 -0.0625030218754735
2 -0.0971813193264847
1.7 0.0353701411461059
1.55624958273418 0.2
1.4 0.472477878292825
1.38943340596759 0.5
1.31029198324408 0.8
1.26531869368691 1.1
1.24017974799947 1.4
1.2261479258105 1.7
1.21492721180423 2
1.21303913841 2.3
1.20958372782171 2.6
1.20978174792215 2.9
1.20931122586039 3.2
1.20783347267016 3.5
1.20748734685311 3.8
1.20624122939292 4.1
1.20690032988594 4.4
1.20754502718016 4.7
1.20737615329191 5
1.1 5
1.02322587097197 5
1.02352949858715 4.7
1.02342520698405 4.4
1.02186461351097 4.1
1.02426881322184 3.8
1.0244865107503 3.5
1.02507281773242 3.2
1.02501552173312 2.9
1.02623384739837 2.6
1.02833436878568 2.3
1.02996178451571 2
1.03750561186807 1.7
1.04853915238868 1.4
1.06802829125732 1.1
1.1 0.833062337821632
1.10471116397461 0.8
1.17367205136409 0.5
1.28358138658326 0.2
1.4 -0.0196300728214189
1.46882230584835 -0.1
1.7 -0.305784054415443
1.97800950970666 -0.4
2 -0.406459373040782
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
1.7 0.0353701411461059
2 -0.0971813193264847
2.3 -0.0625030218754735
2.6 0.0756506511919061
2.78763441314499 0.2
2.9 0.284760712635653
3.1605040840115 0.5
3.2 0.534769569789416
3.48871330093197 0.8
3.5 0.811175994798851
3.79841925719311 1.1
3.8 1.10168940050062
4.08387134698406 1.4
4.1 1.41774189271489
4.38119896815021 1.7
4.4 1.71946154001019
4.66847044665058 2
4.7 2.03205671686577
4.97274090508582 2.3
5 2.32977629134852
5 2.6
5 2.9
5 2.99383859105106
4.92114962865154 2.9
4.7 2.65512022193623
4.65693623964671 2.6
4.4 2.32776306532457
4.3775769026254 2.3
4.11921512348326 2
4.1 1.97996433411412
3.86144039756994 1.7
3.8 1.63121036717135
3.59808256160097 1.4
3.5 1.29394801998631
3.32966197560031 1.1
3.2 0.971779744130386
3.02927336633198 0.8
2.9 0.68712939579492
2.66800430755603 0.5
2.6 0.449404736454397
2.3 0.304058698356257
2 0.277411917888296
1.7 0.484854988156856
1.6909887320139 0.5
1.56946374082115 0.8
1.49581045488363 1.1
1.45632346571578 1.4
1.43534981772255 1.7
1.41647073264983 2
1.41484449837393 2.3
1.40673983698232 2.6
1.41070246865865 2.9
1.40783884548878 3.2
1.40554839431406 3.5
1.4042333515628 3.8
1.40725154736284 4.1
1.40453763886087 4.4
1.40596687166943 4.7
1.40657277354598 5
1.4 5
1.20737615329191 5
1.20754502718016 4.7
1.20690032988594 4.4
1.20624122939292 4.1
1.20748734685311 3.8
1.20783347267016 3.5
1.20931122586039 3.2
1.20978174792215 2.9
1.20958372782171 2.6
1.21303913841 2.3
1.21492721180423 2
1.2261479258105 1.7
1.24017974799947 1.4
1.26531869368691 1.1
1.31029198324408 0.8
1.38943340596759 0.5
1.4 0.472477878292825
1.55624958273418 0.2
1.7 0.0353701411461059
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
1.7 0.484854988156856
2 0.277411917888296
2.3 0.304058698356257
2.6 0.449404736454397
2.66800430755603 0.5
2.9 0.68712939579492
3.02927336633198 0.8
3.2 0.971779744130386
3.32966197560031 1.1
3.5 1.29394801998631
3.59808256160097 1.4
3.8 1.63121036717135
3.86144039756994 1.7
4.1 1.97996433411412
4.11921512348326 2
4.3775769026254 2.3
4.4 2.32776306532457
4.65693623964671 2.6
4.7 2.65512022193623
4.92114962865154 2.9
5 2.99383859105106
5 3.2
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.80413184073506 5
4.92295458138159 4.7
4.84944504274529 4.4
4.80153668996229 4.1
4.7 3.9247681986575
4.6262841332919 3.8
4.51673223202724 3.5
4.4 3.3171284764621
4.33012555486539 3.2
4.11356511718633 2.9
4.1 2.88019341349077
3.92417659756912 2.6
3.8 2.42114261086234
3.72643472598688 2.3
3.52130540085646 2
3.5 1.9725300785483
3.29507322267721 1.7
3.2 1.57404968498509
3.06513077674458 1.4
2.9 1.22406787386697
2.76316383026881 1.1
2.6 0.951543494676247
2.33011018847228 0.8
2.3 0.78589399404953
2.20385463846214 0.8
2 0.849699682521031
1.85050657254204 1.1
1.75965991842763 1.4
1.71136965008732 1.7
1.7 1.81506042708377
1.68912274313401 2
1.68369209959074 2.3
1.68213972370822 2.6
1.67812967352139 2.9
1.67406001512416 3.2
1.67522621603955 3.5
1.67391612759254 3.8
1.67448513448776 4.1
1.67502387573805 4.4
1.67620027594299 4.7
1.66907952903416 5
1.40657277354598 5
1.40596687166943 4.7
1.40453763886087 4.4
1.40725154736284 4.1
1.4042333515628 3.8
1.40554839431406 3.5
1.40783884548878 3.2
1.41070246865865 2.9
1.40673983698232 2.6
1.41484449837393 2.3
1.41647073264983 2
1.43534981772255 1.7
1.45632346571578 1.4
1.49581045488363 1.1
1.56946374082115 0.8
1.6909887320139 0.5
1.7 0.484854988156856
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
2.3 0.78589399404953
2.33011018847228 0.8
2.6 0.951543494676247
2.76316383026881 1.1
2.9 1.22406787386697
3.06513077674458 1.4
3.2 1.57404968498509
3.29507322267721 1.7
3.5 1.9725300785483
3.52130540085646 2
3.72643472598688 2.3
3.8 2.42114261086234
3.92417659756912 2.6
4.1 2.88019341349077
4.11356511718633 2.9
4.33012555486539 3.2
4.4 3.3171284764621
4.51673223202724 3.5
4.6262841332919 3.8
4.7 3.9247681986575
4.80153668996229 4.1
4.84944504274529 4.4
4.92295458138159 4.7
4.80413184073506 5
4.7 5
4.4 5
4.1 5
3.8 5
3.5943623939703 5
3.57590955531601 4.7
3.64876290679388 4.4
3.67374501841264 4.1
3.62855819102244 3.8
3.54738736905446 3.5
3.5 3.20085718655481
3.4996608285366 3.2
3.28288868569787 2.9
3.2 2.71371474215291
3.13166529050397 2.6
2.97051112490385 2.3
2.9 2.17904236348771
2.70131146930918 2
2.6 1.90658952055931
2.30672094367428 2
2.3 2.00482748792678
2.22993131765632 2.3
2.19924806669824 2.6
2.2005206903558 2.9
2.18937815160528 3.2
2.18187011281536 3.5
2.17271035824495 3.8
2.17727668956901 4.1
2.1614925405776 4.4
2.17424066975738 4.7
2.1656825327969 5
2 5
1.7 5
1.66907952903416 5
1.67620027594299 4.7
1.67502387573805 4.4
1.67448513448776 4.1
1.67391612759254 3.8
1.67522621603955 3.5
1.67406001512416 3.2
1.67812967352139 2.9
1.68213972370822 2.6
1.68369209959074 2.3
1.68912274313401 2
1.7 1.81506042708377
1.71136965008732 1.7
1.75965991842763 1.4
1.85050657254204 1.1
2 0.849699682521031
2.20385463846214 0.8
2.3 0.78589399404953
};
\addplot [draw=none, fill=lavender231240249]
table{%
x  y
2.6 1.90658952055931
2.70131146930918 2
2.9 2.17904236348771
2.97051112490385 2.3
3.13166529050397 2.6
3.2 2.71371474215291
3.28288868569787 2.9
3.4996608285366 3.2
3.5 3.20085718655481
3.54738736905446 3.5
3.62855819102244 3.8
3.67374501841264 4.1
3.64876290679388 4.4
3.57590955531601 4.7
3.5943623939703 5
3.5 5
3.2 5
2.9 5
2.6 5
2.3 5
2.1656825327969 5
2.17424066975738 4.7
2.1614925405776 4.4
2.17727668956901 4.1
2.17271035824495 3.8
2.18187011281536 3.5
2.18937815160528 3.2
2.2005206903558 2.9
2.19924806669824 2.6
2.22993131765632 2.3
2.3 2.00482748792678
2.30672094367428 2
2.6 1.90658952055931
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
2.3 4.4
};
\coordinate (CVI_mean_lml_b) at (axis cs:2.3,1.4);
\coordinate (CVI_mean_lml_ep_b) at (axis cs:2.3,2.3);
\end{axis}



==> fig/tikz/usps/CVI_mean_lml.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=black]
table{%
x  y
-0.7 2.43575217843821
-0.4 2.43575279875926
-0.1 2.43578203857492
0.2 2.43650212207671
0.5 2.4478048052457
0.8 2.55492029077843
0.827612790707195 2.6
1.0093507742594 2.9
1.1 3.07915134728688
1.12936548837269 3.2
1.20179802331553 3.5
1.27411187149183 3.8
1.3318329907232 4.1
1.38157306883822 4.4
1.4 4.50145416230472
1.43090961131613 4.7
1.48469104248718 5
1.4 5
1.1 5
0.8 5
0.5 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.43575217387621
-0.7 2.43575217843821
};
\addplot [draw=none, fill=midnightblue854116]
table{%
x  y
-0.7 2.13256430510958
-0.4 2.13256494249716
-0.1 2.13259498670467
0.2 2.13333491710662
0.5 2.14496199671774
0.8 2.25612744813654
0.826064857306796 2.3
1.00901128201571 2.6
1.1 2.75441448253252
1.14019649747856 2.9
1.21195704868945 3.2
1.28198589973627 3.5
1.3506286682357 3.8
1.4 4.06740189804121
1.40500903149482 4.1
1.44736910439497 4.4
1.49408840282174 4.7
1.54790208152653 5
1.48469104248718 5
1.43090961131613 4.7
1.4 4.50145416230472
1.38157306883822 4.4
1.3318329907232 4.1
1.27411187149183 3.8
1.20179802331553 3.5
1.12936548837269 3.2
1.1 3.07915134728687
1.0093507742594 2.9
0.827612790707195 2.6
0.8 2.55492029077843
0.5 2.4478048052457
0.2 2.43650212207671
-0.1 2.43578203857492
-0.4 2.43575279875926
-0.7 2.43575217843821
-1 2.43575217387621
-1 2.3
-1 2.13256430042206
-0.7 2.13256430510958
};
\addplot [draw=none, fill=midnightblue868137]
table{%
x  y
-0.7 1.81089526128912
-0.4 1.8108959144547
-0.1 1.81092670197628
0.2 1.81168486958257
0.5 1.82359236562566
0.8 1.93729696674359
0.83631042423276 2
1.01330618674802 2.3
1.1 2.44447710178747
1.14440292891804 2.6
1.22519361408293 2.9
1.2945486090062 3.2
1.36217377615701 3.5
1.4 3.6712263801221
1.42320087876205 3.8
1.46868973794042 4.1
1.51052748867311 4.4
1.55726719432736 4.7
1.61111312056588 5
1.54790208152653 5
1.49408840282174 4.7
1.44736910439497 4.4
1.40500903149482 4.1
1.4 4.06740189804121
1.3506286682357 3.8
1.28198589973627 3.5
1.21195704868945 3.2
1.14019649747856 2.9
1.1 2.75441448253252
1.00901128201571 2.6
0.826064857306796 2.3
0.8 2.25612744813654
0.5 2.14496199671774
0.2 2.13333491710662
-0.1 2.13259498670467
-0.4 2.13256494249716
-0.7 2.13256430510958
-1 2.13256430042206
-1 2
-1 1.81089525648555
-0.7 1.81089526128912
};
\addplot [draw=none, fill=teal882156]
table{%
x  y
-0.7 1.44563016073505
-0.4 1.44563088781964
-0.1 1.44566515906739
0.2 1.44650906862559
0.5 1.45976535845048
0.8 1.58653974437543
0.85875931670189 1.7
1.03014686111924 2
1.1 2.12047647374883
1.15014546205755 2.3
1.23349312369738 2.6
1.31019073068731 2.9
1.37714016932296 3.2
1.4 3.3031405470588
1.43608786808309 3.5
1.48859879793018 3.8
1.53237044438602 4.1
1.57368587295124 4.4
1.62044598583297 4.7
1.67432415960522 5
1.61111312056588 5
1.55726719432736 4.7
1.51052748867311 4.4
1.46868973794042 4.1
1.42320087876205 3.8
1.4 3.6712263801221
1.36217377615701 3.5
1.2945486090062 3.2
1.22519361408293 2.9
1.14440292891804 2.6
1.1 2.44447710178747
1.01330618674802 2.3
0.83631042423276 2
0.8 1.93729696674359
0.5 1.82359236562566
0.2 1.81168486958257
-0.1 1.81092670197628
-0.4 1.8108959144547
-0.7 1.81089526128912
-1 1.81089525648555
-1 1.7
-1 1.44563015538785
-0.7 1.44563016073505
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 0.927444337444335
-0.4 0.927445500130728
-0.1 0.927500303446659
0.2 0.928850163554711
0.5 0.950155597412596
0.714710298782487 1.1
0.8 1.14311845855859
0.909467988550456 1.4
1.06062848949602 1.7
1.1 1.7701006506726
1.16243614918314 2
1.24352721167163 2.3
1.32258331847672 2.6
1.39518784729168 2.9
1.4 2.92177982598863
1.45142053909928 3.2
1.50439987505267 3.5
1.5539967170983 3.8
1.59605115083163 4.1
1.63684425722938 4.4
1.68362477733859 4.7
1.7 4.79115700136455
1.74383225979131 5
1.7 5
1.67432415960522 5
1.62044598583297 4.7
1.57368587295124 4.4
1.53237044438602 4.1
1.48859879793018 3.8
1.43608786808309 3.5
1.4 3.3031405470588
1.37714016932296 3.2
1.31019073068731 2.9
1.23349312369738 2.6
1.15014546205755 2.3
1.1 2.12047647374883
1.03014686111924 2
0.85875931670189 1.7
0.8 1.58653974437543
0.5 1.45976535845048
0.2 1.44650906862559
-0.1 1.44566515906739
-0.4 1.44563088781964
-0.7 1.44563016073505
-1 1.44563015538785
-1 1.4
-1 1.1
-1 0.927444328893513
-0.7 0.927444337444335
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.7 -1
-0.4 -1
-0.1 -1
0.2 -1
0.5 -1
0.8 -1
1.09596232707405 -1
0.969736059340869 -0.7
0.898909877100176 -0.4
0.861315015722151 -0.1
0.849342548746477 0.2
0.86500198897695 0.5
0.914226062872122 0.8
1.0002157792929 1.1
1.1 1.34933148280288
1.10989147300574 1.4
1.18234669535297 1.7
1.26004930260978 2
1.3369089612857 2.3
1.4 2.55126903859946
1.41021136292242 2.6
1.46987868131414 2.9
1.52252014699871 3.2
1.57271188202226 3.5
1.61939463626643 3.8
1.65973185727723 4.1
1.7 4.39998015917878
1.70000315235812 4.4
1.75518213895943 4.7
1.81764784582531 5
1.74383225979131 5
1.7 4.79115700136455
1.68362477733859 4.7
1.63684425722938 4.4
1.59605115083163 4.1
1.5539967170983 3.8
1.50439987505267 3.5
1.45142053909928 3.2
1.4 2.92177982598863
1.39518784729168 2.9
1.32258331847672 2.6
1.24352721167163 2.3
1.16243614918314 2
1.1 1.7701006506726
1.06062848949602 1.7
0.909467988550456 1.4
0.8 1.14311845855859
0.714710298782487 1.1
0.5 0.950155597412596
0.2 0.928850163554711
-0.1 0.927500303446659
-0.4 0.927445500130728
-0.7 0.927444337444335
-1 0.927444328893513
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
1.1 -1
1.4 -1
1.40687851555708 -1
1.4 -0.979674894216474
1.28180062571429 -0.7
1.19979113936145 -0.4
1.14710066770115 -0.1
1.11678639309876 0.2
1.10839611191285 0.5
1.12334642906106 0.8
1.16095833078655 1.1
1.21692399950885 1.4
1.28464514715193 1.7
1.35766245603642 2
1.4 2.17163679738198
1.42665369114626 2.3
1.48814268417641 2.6
1.54395100279722 2.9
1.59361975489813 3.2
1.64102388899185 3.5
1.68479255543456 3.8
1.7 3.91623124425074
1.72820261870275 4.1
1.77537596307047 4.4
1.82967092129473 4.7
1.8914634318593 5
1.81764784582531 5
1.75518213895943 4.7
1.70000315235812 4.4
1.7 4.39998015917878
1.65973185727723 4.1
1.61939463626643 3.8
1.57271188202226 3.5
1.52252014699871 3.2
1.46987868131414 2.9
1.41021136292242 2.6
1.4 2.55126903859946
1.3369089612857 2.3
1.26004930260978 2
1.18234669535297 1.7
1.10989147300574 1.4
1.1 1.34933148280288
1.0002157792929 1.1
0.914226062872122 0.8
0.86500198897695 0.5
0.849342548746477 0.2
0.861315015722151 -0.1
0.898909877100176 -0.4
0.969736059340869 -0.7
1.09596232707405 -1
1.1 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
5 -1
5 -0.944105589218123
4.940755988288 -1
5 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
1.4 -0.979674894216474
1.40687851555708 -1
1.58809144631712 -1
1.47047863382651 -0.7
1.4 -0.464612746738297
1.37679098862429 -0.4
1.29597770701927 -0.1
1.24954946471337 0.2
1.23161337524566 0.5
1.24023078530009 0.8
1.27275964498299 1.1
1.32395652601197 1.4
1.38694359895089 1.7
1.4 1.75517942156949
1.44905636311945 2
1.50882305062897 2.3
1.5660740054304 2.6
1.6180233242803 2.9
1.66471936279756 3.2
1.7 3.43521730469482
1.71131367858709 3.5
1.76070435328163 3.8
1.80491197457973 4.1
1.85074877378281 4.4
1.90415970363004 4.7
1.9652790178933 5
1.8914634318593 5
1.82967092129473 4.7
1.77537596307047 4.4
1.72820261870275 4.1
1.7 3.91623124425074
1.68479255543456 3.8
1.64102388899185 3.5
1.59361975489813 3.2
1.54395100279722 2.9
1.48814268417641 2.6
1.42665369114626 2.3
1.4 2.17163679738198
1.35766245603642 2
1.28464514715193 1.7
1.21692399950885 1.4
1.16095833078655 1.1
1.12334642906106 0.8
1.10839611191285 0.5
1.11678639309876 0.2
1.14710066770115 -0.1
1.19979113936145 -0.4
1.28180062571429 -0.7
1.4 -0.979674894216474
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
4.7 -1
4.940755988288 -1
5 -0.944105589218123
5 -0.7
5 -0.580083786247486
4.87320128606774 -0.7
4.7 -0.866017115239386
4.55231807766689 -1
4.7 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
1.7 -1
1.76428797211272 -1
1.7 -0.87769584949114
1.61801836731498 -0.7
1.51169296868456 -0.4
1.43555186381662 -0.1
1.4 0.108017169396518
1.38231253632799 0.2
1.35483063857848 0.5
1.35711514153912 0.8
1.38456095917944 1.1
1.4 1.19687991598014
1.42785150152282 1.4
1.47977884033685 1.7
1.53568672950072 2
1.59099241011168 2.3
1.6440053266844 2.6
1.69209564576339 2.9
1.7 2.95243823977674
1.74381708551584 3.2
1.79409738715513 3.5
1.83980179996831 3.8
1.88162133045671 4.1
1.92612158449515 4.4
1.97864848596535 4.7
2 4.8053482567088
2.05329703381077 5
2 5
1.9652790178933 5
1.90415970363004 4.7
1.85074877378281 4.4
1.80491197457973 4.1
1.76070435328163 3.8
1.71131367858709 3.5
1.7 3.43521730469482
1.66471936279756 3.2
1.6180233242803 2.9
1.5660740054304 2.6
1.50882305062897 2.3
1.44905636311945 2
1.4 1.75517942156949
1.38694359895089 1.7
1.32395652601197 1.4
1.27275964498299 1.1
1.24023078530009 0.8
1.23161337524566 0.5
1.24954946471337 0.2
1.29597770701927 -0.1
1.37679098862429 -0.4
1.4 -0.464612746738297
1.47047863382651 -0.7
1.58809144631712 -1
1.7 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
4.4 -1
4.55231807766689 -1
4.7 -0.866017115239386
4.87320128606774 -0.7
5 -0.580083786247486
5 -0.4
5 -0.305813558934924
4.90079113546 -0.4
4.7 -0.591921809464302
4.58166366753734 -0.7
4.4 -0.867966188768813
4.24584621133185 -1
4.4 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
1.7 -0.877695849491139
1.76428797211272 -1
1.93238430787804 -1
1.76672109112001 -0.7
1.7 -0.55338622454653
1.64024183994693 -0.4
1.55355177819463 -0.1
1.4970951055888 0.2
1.46845213088625 0.5
1.46618392860571 0.8
1.48673612043579 1.1
1.52404729755247 1.4
1.57122958339129 1.7
1.62231709588198 2
1.67316176959439 2.3
1.7 2.46113305321414
1.72706121862593 2.6
1.78143648286635 2.9
1.83079271711136 3.2
1.87688109572317 3.5
1.918899246655 3.8
1.95833068633369 4.1
2 4.38943583808908
2.00215205828549 4.4
2.07424147221408 4.7
2.15392861437192 5
2.05329703381077 5
2 4.8053482567088
1.97864848596535 4.7
1.92612158449515 4.4
1.88162133045671 4.1
1.83980179996831 3.8
1.79409738715513 3.5
1.74381708551584 3.2
1.7 2.95243823977674
1.69209564576339 2.9
1.6440053266844 2.6
1.59099241011168 2.3
1.53568672950072 2
1.47977884033685 1.7
1.42785150152282 1.4
1.4 1.19687991598014
1.38456095917944 1.1
1.35711514153912 0.8
1.35483063857848 0.5
1.38231253632799 0.2
1.4 0.108017169396518
1.43555186381662 -0.1
1.51169296868456 -0.4
1.61801836731498 -0.7
1.7 -0.877695849491139
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
4.1 -1
4.24584621133185 -1
4.4 -0.867966188768814
4.58166366753734 -0.7
4.7 -0.591921809464302
4.90079113546 -0.4
5 -0.305813558934924
5 -0.1
5 -0.0692551929490948
4.96775790819687 -0.1
4.7 -0.355469887032312
4.65159617040324 -0.4
4.4 -0.631919621589155
4.32142224709315 -0.7
4.1 -0.892944764692555
3.96332788389228 -1
4.1 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
2 -1
2.13258508017327 -1
2 -0.844242666074332
1.91687815609386 -0.7
1.77583495360705 -0.4
1.7 -0.193177490821799
1.67155169257264 -0.1
1.60911401808627 0.2
1.57652017667036 0.5
1.57072336631434 0.8
1.58736899171723 1.1
1.62024309358211 1.4
1.66268032644574 1.7
1.7 1.93940772193869
1.71119634867098 2
1.76874038721409 2.3
1.82319789949827 2.6
1.8726012804316 2.9
1.91776834870688 3.2
1.95966480429122 3.5
1.99799669334168 3.8
2 3.81575991977667
2.05168923729569 4.1
2.1106954215011 4.4
2.17831450872619 4.7
2.25456019493307 5
2.15392861437192 5
2.07424147221408 4.7
2.00215205828549 4.4
2 4.38943583808908
1.95833068633369 4.1
1.918899246655 3.8
1.87688109572317 3.5
1.83079271711136 3.2
1.78143648286635 2.9
1.72706121862593 2.6
1.7 2.46113305321414
1.67316176959439 2.3
1.62231709588198 2
1.57122958339129 1.7
1.52404729755247 1.4
1.48673612043579 1.1
1.46618392860571 0.8
1.46845213088625 0.5
1.4970951055888 0.2
1.55355177819463 -0.1
1.64024183994693 -0.4
1.7 -0.55338622454653
1.76672109112001 -0.7
1.93238430787804 -1
2 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
3.8 -1
3.96332788389228 -1
4.1 -0.892944764692555
4.32142224709315 -0.7
4.4 -0.631919621589155
4.65159617040324 -0.4
4.7 -0.355469887032312
4.96775790819687 -0.1
5 -0.0692551929490948
5 0.147956590955561
4.7399678210521 -0.1
4.7 -0.138133606577178
4.41535360142576 -0.4
4.4 -0.414152844325836
4.1 -0.674475375656343
4.06794812613031 -0.7
3.8 -0.911585247501649
3.66896775061558 -1
3.8 -1
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
2 -0.844242666074333
2.13258508017327 -1
2.3 -1
2.40356320291551 -1
2.3 -0.93942975376855
2.09460029989718 -0.7
2 -0.569751240567441
1.91754736676643 -0.4
1.805016699062 -0.1
1.72585548605112 0.2
1.7 0.37084870747823
1.68458822245447 0.5
1.67526280402296 0.8
1.68800186299867 1.1
1.7 1.22328846834191
1.72080430004269 1.4
1.76810051779101 1.7
1.81960069383186 2
1.87082313307862 2.3
1.91933458037061 2.6
1.96376607799685 2.9
2 3.16379828972787
2.00713276454428 3.2
2.06355326495861 3.5
2.1150863084903 3.8
2.16484686635578 4.1
2.21923878471671 4.4
2.28238754523829 4.7
2.3 4.77074060069749
2.37873384208205 5
2.3 5
2.25456019493307 5
2.17831450872619 4.7
2.1106954215011 4.4
2.05168923729569 4.1
2 3.81575991977667
1.99799669334168 3.8
1.95966480429122 3.5
1.91776834870688 3.2
1.8726012804316 2.9
1.82319789949827 2.6
1.76874038721409 2.3
1.71119634867098 2
1.7 1.93940772193869
1.66268032644574 1.7
1.62024309358211 1.4
1.58736899171723 1.1
1.57072336631434 0.8
1.57652017667036 0.5
1.60911401808627 0.2
1.67155169257264 -0.1
1.7 -0.193177490821799
1.77583495360705 -0.4
1.91687815609386 -0.7
2 -0.844242666074333
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
3.5 -1
3.66896775061558 -1
3.8 -0.911585247501649
4.06794812613031 -0.7
4.1 -0.674475375656343
4.4 -0.414152844325836
4.41535360142576 -0.4
4.7 -0.138133606577178
4.7399678210521 -0.1
5 0.147956590955561
5 0.2
5 0.366312632311544
4.82636722520565 0.2
4.7 0.0795147073263887
4.50625245444153 -0.1
4.4 -0.19779111269381
4.1691678088586 -0.4
4.1 -0.460070167538259
3.8 -0.698926698960819
3.79844180066402 -0.7
3.5 -0.899062589088601
3.3024179324688 -1
3.5 -1
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
2.3 -0.939429753768551
2.40356320291551 -1
2.6 -1
2.9 -1
3.2 -1
3.3024179324688 -1
3.5 -0.899062589088601
3.79844180066402 -0.7
3.8 -0.698926698960819
4.1 -0.460070167538259
4.1691678088586 -0.4
4.4 -0.19779111269381
4.50625245444153 -0.1
4.7 0.0795147073263887
4.82636722520565 0.2
5 0.366312632311544
5 0.5
5 0.593662191805729
4.90266354302644 0.5
4.7 0.306666881770494
4.58567220852131 0.2
4.4 0.0290907997072321
4.25414143003244 -0.1
4.1 -0.23372626783411
3.89427367744358 -0.4
3.8 -0.474146139400195
3.5 -0.67915682258319
3.45995785828116 -0.7
3.2 -0.826633698447913
2.9 -0.901481769243244
2.6 -0.869347089402767
2.31271549527254 -0.7
2.3 -0.691081195639139
2.08836702950336 -0.4
2 -0.248348977345599
1.94339457880688 -0.1
1.86290715610054 0.2
1.81619708893765 0.5
1.80116977901948 0.8
1.8125553279178 1.1
1.84254526008995 1.4
1.88315168917714 1.7
1.92800503899274 2
1.97290587894315 2.3
2 2.48676034467729
2.02364100341266 2.6
2.08340211956098 2.9
2.13790411301452 3.2
2.18749576872371 3.5
2.2331631577402 3.8
2.27800449541586 4.1
2.3 4.22949019795072
2.34312636088015 4.4
2.4291161030431 4.7
2.52228985022672 5
2.37873384208205 5
2.3 4.77074060069749
2.28238754523829 4.7
2.21923878471671 4.4
2.16484686635578 4.1
2.1150863084903 3.8
2.06355326495861 3.5
2.00713276454428 3.2
2 3.16379828972787
1.96376607799685 2.9
1.91933458037061 2.6
1.87082313307862 2.3
1.81960069383186 2
1.76810051779101 1.7
1.72080430004269 1.4
1.7 1.22328846834191
1.68800186299867 1.1
1.67526280402296 0.8
1.68458822245447 0.5
1.7 0.37084870747823
1.72585548605112 0.2
1.805016699062 -0.1
1.91754736676643 -0.4
2 -0.569751240567441
2.09460029989718 -0.7
2.3 -0.939429753768551
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
2.6 -0.869347089402767
2.9 -0.901481769243244
3.2 -0.826633698447913
3.45995785828116 -0.7
3.5 -0.67915682258319
3.8 -0.474146139400195
3.89427367744358 -0.4
4.1 -0.23372626783411
4.25414143003244 -0.1
4.4 0.0290907997072321
4.58567220852131 0.2
4.7 0.306666881770494
4.90266354302644 0.5
5 0.593662191805729
5 0.8
5 0.84094771397525
4.95766674629575 0.8
4.7 0.553712956923832
4.64285181684097 0.5
4.4 0.27599529450705
4.31499841788381 0.2
4.1 0.013198305185269
3.96180519608464 -0.1
3.8 -0.227158059220213
3.55326667475716 -0.4
3.5 -0.435282498036119
3.2 -0.581549654608866
2.9 -0.655801614810442
2.6 -0.61016948113367
2.3 -0.400432125531047
2.29968581958872 -0.4
2.12685170979648 -0.1
2 0.199847560581636
1.99995882614996 0.2
1.95172156629908 0.5
1.93370028921963 0.8
1.94034682995577 1.1
1.9642862201372 1.4
1.99820286056328 1.7
2 1.7133322346278
2.0562173145732 2
2.11498859547071 2.3
2.17054354515722 2.6
2.22181857967537 2.9
2.26867546148476 3.2
2.3 3.4165638775781
2.31874438857161 3.5
2.38333114149211 3.8
2.44577428197846 4.1
2.51161874183589 4.4
2.58453380477797 4.7
2.6 4.75348371131275
2.69619690908574 5
2.6 5
2.52228985022672 5
2.4291161030431 4.7
2.34312636088015 4.4
2.3 4.22949019795072
2.27800449541586 4.1
2.2331631577402 3.8
2.18749576872371 3.5
2.13790411301452 3.2
2.08340211956098 2.9
2.02364100341266 2.6
2 2.48676034467729
1.97290587894315 2.3
1.92800503899274 2
1.88315168917714 1.7
1.84254526008995 1.4
1.8125553279178 1.1
1.80116977901948 0.8
1.81619708893765 0.5
1.86290715610054 0.2
1.94339457880688 -0.1
2 -0.248348977345599
2.08836702950336 -0.4
2.3 -0.691081195639139
2.31271549527254 -0.7
2.6 -0.869347089402767
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
2.3 -0.400432125531047
2.6 -0.61016948113367
2.9 -0.655801614810442
3.2 -0.581549654608866
3.5 -0.435282498036119
3.55326667475716 -0.4
3.8 -0.227158059220213
3.96180519608464 -0.1
4.1 0.013198305185269
4.31499841788381 0.2
4.4 0.27599529450705
4.64285181684097 0.5
4.7 0.553712956923832
4.95766674629575 0.8
5 0.84094771397525
5 1.1
5 1.13282198997296
4.96629838483167 1.1
4.7 0.844462263012505
4.65311870641709 0.8
4.4 0.565454441811999
4.32760655932547 0.5
4.1 0.301349402064105
3.97786146892987 0.2
3.8 0.0598764986680609
3.57476926041141 -0.1
3.5 -0.149325300007273
3.2 -0.294969246855156
2.9 -0.363397819396982
2.6 -0.293468023927622
2.38214502312699 -0.1
2.3 0.00132099940350652
2.21749615813533 0.2
2.13969249269956 0.5
2.10586158198284 0.8
2.10810682770971 1.1
2.13521169738027 1.4
2.17640421898083 1.7
2.22359727209454 2
2.27152369127838 2.3
2.3 2.48150742329869
2.32898143073349 2.6
2.39950858817131 2.9
2.4636658809834 3.2
2.5218542946685 3.5
2.57535841099829 3.8
2.6 3.93948400641088
2.64314294086352 4.1
2.72731914021732 4.4
2.8149346733837 4.7
2.9 4.97796984101568
2.90903287665362 5
2.9 5
2.69619690908574 5
2.6 4.75348371131275
2.58453380477797 4.7
2.51161874183589 4.4
2.44577428197846 4.1
2.38333114149211 3.8
2.31874438857161 3.5
2.3 3.4165638775781
2.26867546148476 3.2
2.22181857967537 2.9
2.17054354515722 2.6
2.11498859547071 2.3
2.0562173145732 2
2 1.7133322346278
1.99820286056328 1.7
1.9642862201372 1.4
1.94034682995577 1.1
1.93370028921963 0.8
1.95172156629908 0.5
1.99995882614996 0.2
2 0.199847560581636
2.12685170979648 -0.1
2.29968581958872 -0.4
2.3 -0.400432125531047
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
2.6 -0.293468023927622
2.9 -0.363397819396982
3.2 -0.294969246855156
3.5 -0.149325300007273
3.57476926041141 -0.1
3.8 0.0598764986680609
3.97786146892987 0.2
4.1 0.301349402064105
4.32760655932547 0.5
4.4 0.565454441811999
4.65311870641709 0.8
4.7 0.844462263012505
4.96629838483167 1.1
5 1.13282198997296
5 1.4
5 1.51831415842629
4.87976387906779 1.4
4.7 1.22627732137533
4.5685393151972 1.1
4.4 0.942515504258384
4.24460600443901 0.8
4.1 0.672703472352486
3.89468364587457 0.5
3.8 0.424960416682148
3.5 0.2122787432703
3.47577170333608 0.2
3.2 0.0773973664914754
2.9 0.0326407165447734
2.6 0.154191987226353
2.56283373764256 0.2
2.40742158387844 0.5
2.33254010337352 0.8
2.3194097847078 1.1
2.34635303518929 1.4
2.39526618057078 1.7
2.45376428987153 2
2.51435915007036 2.3
2.57301585874658 2.6
2.6 2.74189461708434
2.64626412673152 2.9
2.72899078495349 3.2
2.80377540626931 3.5
2.87191847027918 3.8
2.9 3.92809188901041
2.95525655374473 4.1
3.04994563835993 4.4
3.1415920546115 4.7
3.2 4.88993545921907
3.24623933091769 5
3.2 5
2.90903287665362 5
2.9 4.97796984101568
2.8149346733837 4.7
2.72731914021732 4.4
2.64314294086352 4.1
2.6 3.93948400641088
2.57535841099829 3.8
2.5218542946685 3.5
2.4636658809834 3.2
2.39950858817131 2.9
2.32898143073349 2.6
2.3 2.48150742329869
2.27152369127838 2.3
2.22359727209454 2
2.17640421898083 1.7
2.13521169738027 1.4
2.10810682770971 1.1
2.10586158198284 0.8
2.13969249269956 0.5
2.21749615813533 0.2
2.3 0.00132099940350651
2.38214502312699 -0.1
2.6 -0.293468023927622
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
2.6 0.154191987226353
2.9 0.0326407165447734
3.2 0.0773973664914754
3.47577170333608 0.2
3.5 0.212278743270299
3.8 0.424960416682148
3.89468364587457 0.5
4.1 0.672703472352486
4.24460600443901 0.8
4.4 0.942515504258384
4.5685393151972 1.1
4.7 1.22627732137533
4.87976387906779 1.4
5 1.51831415842629
5 1.7
5 2
5 2.12825625584788
4.87568385494953 2
4.7 1.82404728097741
4.57739562146594 1.7
4.4 1.52742384869477
4.26753545490147 1.4
4.1 1.24678868884651
3.93056680816985 1.1
3.8 0.994202575626654
3.52556828588769 0.8
3.5 0.783528078672908
3.2 0.681846671035695
2.9 0.748504400933031
2.86079567983618 0.8
2.7603821767471 1.1
2.7479681009238 1.4
2.78034904585052 1.7
2.83388315217612 2
2.89581836262044 2.3
2.9 2.31822381221807
2.99630889801903 2.6
3.09341355670104 2.9
3.18391217321687 3.2
3.2 3.25476853744932
3.30196691303656 3.5
3.41627009584025 3.8
3.5 4.03839264298875
3.52982122769672 4.1
3.66875801770604 4.4
3.7955437392981 4.7
3.8 4.71087652597704
3.96158788516389 5
3.8 5
3.5 5
3.24623933091769 5
3.2 4.88993545921907
3.1415920546115 4.7
3.04994563835993 4.4
2.95525655374473 4.1
2.9 3.92809188901041
2.87191847027918 3.8
2.80377540626931 3.5
2.72899078495349 3.2
2.64626412673152 2.9
2.6 2.74189461708434
2.57301585874658 2.6
2.51435915007036 2.3
2.45376428987153 2
2.39526618057078 1.7
2.34635303518929 1.4
2.3194097847078 1.1
2.33254010337352 0.8
2.40742158387844 0.5
2.56283373764256 0.2
2.6 0.154191987226353
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
2.9 0.748504400933031
3.2 0.681846671035695
3.5 0.783528078672908
3.52556828588769 0.8
3.8 0.994202575626654
3.93056680816985 1.1
4.1 1.24678868884651
4.26753545490147 1.4
4.4 1.52742384869477
4.57739562146594 1.7
4.7 1.82404728097741
4.87568385494953 2
5 2.12825625584788
5 2.3
5 2.6
5 2.9
5 3.2
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.1 5
3.96158788516389 5
3.8 4.71087652597704
3.7955437392981 4.7
3.66875801770604 4.4
3.52982122769672 4.1
3.5 4.03839264298875
3.41627009584025 3.8
3.30196691303656 3.5
3.2 3.25476853744932
3.18391217321687 3.2
3.09341355670104 2.9
2.99630889801903 2.6
2.9 2.31822381221807
2.89581836262044 2.3
2.83388315217612 2
2.78034904585052 1.7
2.7479681009238 1.4
2.7603821767471 1.1
2.86079567983618 0.8
2.9 0.748504400933031
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
4.1 2.6
};
\coordinate (CVI_mean_lml_t) at (axis cs:4.1,2.5999999999999996);
\end{axis}



==> fig/tikz/usps/CVI_mean_lml_ep.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.7 -1
-0.4 -1
-0.1 -1
0.2 -1
0.5 -1
0.8 -1
1.09577202829887 -1
0.96907649387897 -0.7
0.896661780149741 -0.4
0.854085933459407 -0.1
0.828488714066202 0.2
0.813050294721689 0.5
0.804059387128294 0.8
0.801636454070267 1.1
0.813021947534641 1.4
0.842298708654784 1.7
0.876603851902134 2
0.899913594318754 2.3
0.911397146239435 2.6
0.918297322038359 2.9
0.923283701756049 3.2
0.926519990408518 3.5
0.928376989351724 3.8
0.93082980985643 4.1
0.931620107709309 4.4
0.931399430559217 4.7
0.930582776060257 5
0.8 5
0.5 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
1.1 -1
1.4 -1
1.40684232454936 -1
1.4 -0.979814086978441
1.2815598868487 -0.7
1.19887993135095 -0.4
1.14388259427558 -0.1
1.1068186871949 0.2
1.1 0.279763797549154
1.06438131683377 0.5
1.03605332227485 0.8
1.02323021799576 1.1
1.02946519940342 1.4
1.05628249407747 1.7
1.08988635884254 2
1.1 2.12220338536228
1.10749812776536 2.3
1.11482361830999 2.6
1.11930386790978 2.9
1.12271723548911 3.2
1.12591273305288 3.5
1.1282571309491 3.8
1.12903793022618 4.1
1.12886712047471 4.4
1.12885773776228 4.7
1.12923554583508 5
1.1 5
0.930582776060257 5
0.931399430559217 4.7
0.931620107709309 4.4
0.93082980985643 4.1
0.928376989351724 3.8
0.926519990408517 3.5
0.923283701756049 3.2
0.918297322038359 2.9
0.911397146239435 2.6
0.899913594318754 2.3
0.876603851902134 2
0.842298708654784 1.7
0.813021947534641 1.4
0.801636454070267 1.1
0.804059387128294 0.8
0.813050294721689 0.5
0.828488714066202 0.2
0.854085933459407 -0.1
0.896661780149741 -0.4
0.96907649387897 -0.7
1.09577202829887 -1
1.1 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
5 -1
5 -0.944105594076901
4.94075599334152 -1
5 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
1.4 -0.979814086978441
1.40684232454936 -1
1.58805477720789 -1
1.47031751564252 -0.7
1.4 -0.466786549581591
1.37584663629875 -0.4
1.29271981606041 -0.1
1.23966573053337 0.2
1.20628739824358 0.5
1.18607147309355 0.8
1.17577713628119 1.1
1.17663865175134 1.4
1.18852466969098 1.7
1.20411597006683 2
1.21618079361722 2.3
1.22382498374807 2.6
1.22878573295126 2.9
1.23249404209883 3.2
1.23555823143053 3.5
1.23752346783185 3.8
1.23784469771992 4.1
1.23705463255743 4.4
1.23601114947875 4.7
1.23568049407572 5
1.12923554583508 5
1.12885773776228 4.7
1.12886712047471 4.4
1.12903793022618 4.1
1.1282571309491 3.8
1.12591273305288 3.5
1.12271723548911 3.2
1.11930386790978 2.9
1.11482361830999 2.6
1.10749812776536 2.3
1.1 2.12220338536228
1.08988635884254 2
1.05628249407747 1.7
1.02946519940342 1.4
1.02323021799576 1.1
1.03605332227485 0.8
1.06438131683377 0.5
1.1 0.279763797549154
1.1068186871949 0.2
1.14388259427558 -0.1
1.19887993135095 -0.4
1.2815598868487 -0.7
1.4 -0.979814086978441
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
4.7 -1
4.94075599334152 -1
5 -0.944105594076901
5 -0.7
5 -0.580083807230669
4.87320130771449 -0.7
4.7 -0.866017136240416
4.55231809990177 -1
4.7 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
1.7 -1
1.76425476507256 -1
1.7 -0.87787488025199
1.61785856722326 -0.7
1.51102149769456 -0.4
1.4329818372633 -0.1
1.4 0.0723100694735326
1.37251277387184 0.2
1.33012510066124 0.5
1.30489554706674 0.8
1.29172299431716 1.1
1.2903258224345 1.4
1.299778900296 1.7
1.31341477932488 2
1.32486345946909 2.3
1.33282634918615 2.6
1.33826759799274 2.9
1.34227084870855 3.2
1.34520372980819 3.5
1.34678980471461 3.8
1.34665146521366 4.1
1.34524214464016 4.4
1.34316456119521 4.7
1.34212544231637 5
1.23568049407572 5
1.23601114947875 4.7
1.23705463255743 4.4
1.23784469771992 4.1
1.23752346783185 3.8
1.23555823143053 3.5
1.23249404209883 3.2
1.22878573295126 2.9
1.22382498374807 2.6
1.21618079361722 2.3
1.20411597006683 2
1.18852466969098 1.7
1.17663865175134 1.4
1.17577713628119 1.1
1.18607147309355 0.8
1.20628739824358 0.5
1.23966573053337 0.2
1.29271981606041 -0.1
1.37584663629875 -0.4
1.4 -0.466786549581591
1.47031751564252 -0.7
1.58805477720789 -1
1.7 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
4.4 -1
4.55231809990177 -1
4.7 -0.866017136240416
4.87320130771449 -0.7
5 -0.580083807230669
5 -0.4
5 -0.305813621572904
4.9007912005623 -0.4
4.7 -0.591921872952037
4.58166373539622 -0.7
4.4 -0.86796625338301
4.24584628358593 -1
4.4 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
1.7 -0.87787488025199
1.76425476507256 -1
1.93235393110316 -1
1.76656621588236 -0.7
1.7 -0.554368468888623
1.63959082590314 -0.4
1.55110683563086 -0.1
1.48924637376458 0.2
1.44775877323889 0.5
1.42157633317805 0.8
1.40708335087601 1.1
1.40372461890144 1.4
1.41021872806536 1.7
1.42094566884668 2
1.43075900372915 2.3
1.43824961210043 2.6
1.44374378299979 2.9
1.44779607179187 3.2
1.4505762228937 3.5
1.45197159832698 3.8
1.45161469481296 4.1
1.44994549955464 4.4
1.4472200484953 4.7
1.4458480338532 5
1.4 5
1.34212544231637 5
1.34316456119521 4.7
1.34524214464016 4.4
1.34665146521366 4.1
1.34678980471461 3.8
1.34520372980819 3.5
1.34227084870855 3.2
1.33826759799274 2.9
1.33282634918615 2.6
1.32486345946909 2.3
1.31341477932488 2
1.299778900296 1.7
1.2903258224345 1.4
1.29172299431716 1.1
1.30489554706674 0.8
1.33012510066124 0.5
1.37251277387184 0.2
1.4 0.0723100694735326
1.4329818372633 -0.1
1.51102149769456 -0.4
1.61785856722326 -0.7
1.7 -0.87787488025199
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
4.1 -1
4.24584628358593 -1
4.4 -0.86796625338301
4.58166373539622 -0.7
4.7 -0.591921872952037
4.9007912005623 -0.4
5 -0.305813621572904
5 -0.1
5 -0.069255345409666
4.96775806803117 -0.1
4.7 -0.355470046626826
4.65159634340206 -0.4
4.4 -0.631919791961795
4.3214224416199 -0.7
4.1 -0.892944948502605
3.96332811185659 -1
4.1 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
2 -1
2.13255191166432 -1
2 -0.844381753176836
1.91673910175907 -0.7
1.77517042854589 -0.4
1.7 -0.198836260554114
1.66923183399842 -0.1
1.60177615216803 0.2
1.55735902398092 0.5
1.52966354946632 0.8
1.51417697548506 1.1
1.50924221446258 1.4
1.51326080550218 1.7
1.52173716886422 2
1.53041195894371 2.3
1.53792658426778 2.6
1.54404126578728 2.9
1.54860561062155 3.2
1.55167983635658 3.5
1.55327621918228 3.8
1.55288059932537 4.1
1.55107808523773 4.4
1.54777635084417 4.7
1.54632677274064 5
1.4458480338532 5
1.4472200484953 4.7
1.44994549955464 4.4
1.45161469481296 4.1
1.45197159832698 3.8
1.4505762228937 3.5
1.44779607179187 3.2
1.44374378299979 2.9
1.43824961210043 2.6
1.43075900372915 2.3
1.42094566884668 2
1.41021872806536 1.7
1.40372461890144 1.4
1.40708335087601 1.1
1.42157633317805 0.8
1.44775877323889 0.5
1.48924637376458 0.2
1.55110683563086 -0.1
1.63959082590314 -0.4
1.7 -0.554368468888623
1.76656621588236 -0.7
1.93235393110316 -1
2 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
3.8 -1
3.96332811185659 -1
4.1 -0.892944948502605
4.3214224416199 -0.7
4.4 -0.631919791961795
4.65159634340206 -0.4
4.7 -0.355470046626826
4.96775806803117 -0.1
5 -0.069255345409666
5 0.147956198769544
4.73996823192509 -0.1
4.7 -0.138133999653395
4.4153540258794 -0.4
4.4 -0.414153236249691
4.1 -0.674475813731039
4.06794867852547 -0.7
3.8 -0.911585786539859
3.66896855106937 -1
3.8 -1
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
2 -0.844381753176836
2.13255191166432 -1
2.3 -1
2.40352085022768 -1
2.3 -0.939481096361835
2.0944369272347 -0.7
2 -0.570372914634479
1.91696311703446 -0.4
1.80258709060834 -0.1
1.71757120680501 0.2
1.7 0.288986030258718
1.66695927472294 0.5
1.63775076575459 0.8
1.62127060009411 1.1
1.61475981002372 1.4
1.61630288293901 1.7
1.62252866888176 2
1.63006491415827 2.3
1.63760355643513 2.6
1.64433874857477 2.9
1.64941514945122 3.2
1.65278344981946 3.5
1.65458084003757 3.8
1.65414650383778 4.1
1.65221067092082 4.4
1.64833265319303 4.7
1.64680551162808 5
1.54632677274064 5
1.54777635084417 4.7
1.55107808523773 4.4
1.55288059932537 4.1
1.55327621918228 3.8
1.55167983635658 3.5
1.54860561062155 3.2
1.54404126578728 2.9
1.53792658426778 2.6
1.53041195894371 2.3
1.52173716886422 2
1.51326080550218 1.7
1.50924221446258 1.4
1.51417697548506 1.1
1.52966354946632 0.8
1.55735902398092 0.5
1.60177615216803 0.2
1.66923183399842 -0.1
1.7 -0.198836260554114
1.77517042854589 -0.4
1.91673910175907 -0.7
2 -0.844381753176836
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
3.5 -1
3.66896855106937 -1
3.8 -0.911585786539859
4.06794867852547 -0.7
4.1 -0.674475813731039
4.4 -0.41415323624969
4.4153540258794 -0.4
4.7 -0.138133999653395
4.73996823192509 -0.1
5 0.147956198769544
5 0.2
5 0.366311583147436
4.82636834133362 0.2
4.7 0.0795136287389467
4.50625364618307 -0.1
4.4 -0.197792229319359
4.1691691135713 -0.4
4.1 -0.460071320115823
3.8 -0.698927933681128
3.79844359520025 -0.7
3.5 -0.899064421741161
3.30242181344328 -1
3.5 -1
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
2.3 -0.939481096361835
2.40352085022768 -1
2.6 -1
2.9 -1
3.2 -1
3.30242181344328 -1
3.5 -0.899064421741161
3.79844359520025 -0.7
3.8 -0.698927933681128
4.1 -0.460071320115823
4.1691691135713 -0.4
4.4 -0.197792229319359
4.50625364618307 -0.1
4.7 0.0795136287389467
4.82636834133362 0.2
5 0.366311583147436
5 0.5
5 0.593659450909031
4.90266647708241 0.5
4.7 0.306663982214258
4.58567545434174 0.2
4.4 0.029087661581041
4.25414518540406 -0.1
4.1 -0.233729717168494
3.89427824063768 -0.4
3.8 -0.474149892410528
3.5 -0.679161740057072
3.45996779414046 -0.7
3.2 -0.826641298459952
2.9 -0.901496627022772
2.6 -0.869387352557762
2.31248780404341 -0.7
2.3 -0.69125918304644
2.08765559667805 -0.4
2 -0.251563585755999
1.94130663414529 -0.1
1.8557854948005 0.2
1.79684511948947 0.5
1.75903740216506 0.8
1.73697869331156 1.1
1.72682839380754 1.4
1.7260490638591 1.7
1.73171509709649 2
1.74039949150435 2.3
1.75015216379994 2.6
1.75930533680539 2.9
1.76645151599509 3.2
1.77131726969415 3.5
1.77394708938601 3.8
1.77365124179992 4.1
1.7715320077482 4.4
1.76741729092018 4.7
1.76701516743209 5
1.7 5
1.64680551162808 5
1.64833265319303 4.7
1.65221067092082 4.4
1.65414650383778 4.1
1.65458084003757 3.8
1.65278344981946 3.5
1.64941514945122 3.2
1.64433874857477 2.9
1.63760355643513 2.6
1.63006491415827 2.3
1.62252866888176 2
1.61630288293901 1.7
1.61475981002372 1.4
1.62127060009411 1.1
1.63775076575459 0.8
1.66695927472294 0.5
1.7 0.288986030258718
1.71757120680501 0.2
1.80258709060834 -0.1
1.91696311703446 -0.4
2 -0.570372914634479
2.0944369272347 -0.7
2.3 -0.939481096361835
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
2.6 -0.869387352557762
2.9 -0.901496627022772
3.2 -0.826641298459952
3.45996779414046 -0.7
3.5 -0.679161740057072
3.8 -0.474149892410528
3.89427824063768 -0.4
4.1 -0.233729717168494
4.25414518540406 -0.1
4.4 0.029087661581041
4.58567545434174 0.2
4.7 0.306663982214258
4.90266647708241 0.5
5 0.593659450909031
5 0.8
5 0.840940293584231
4.95767460699179 0.8
4.7 0.553704896868139
4.64286077030928 0.5
4.4 0.275986189936832
4.31500934897489 0.2
4.1 0.0131876412949852
3.96181962281302 -0.1
3.8 -0.227170663944001
3.55328729169425 -0.4
3.5 -0.435296687587471
3.2 -0.581577343954689
2.9 -0.655854072757327
2.6 -0.610333547467403
2.3 -0.401109893914359
2.29919082461699 -0.4
2.12433898787461 -0.1
2 0.17900429343446
1.99399978279598 0.2
1.93548559975269 0.5
1.89824921238274 0.8
1.87659760909317 1.1
1.86643538620561 1.4
1.86480094565043 1.7
1.86879009957007 2
1.87587113878381 2.3
1.88424403488159 2.6
1.89256425710201 2.9
1.8998310731669 3.2
1.90512366457238 3.5
1.90799236223368 3.8
1.90824852499678 4.1
1.90714834171887 4.4
1.90608324142309 4.7
1.90942198231216 5
1.76701516743209 5
1.76741729092018 4.7
1.7715320077482 4.4
1.77365124179992 4.1
1.77394708938601 3.8
1.77131726969415 3.5
1.76645151599509 3.2
1.75930533680539 2.9
1.75015216379994 2.6
1.74039949150435 2.3
1.73171509709649 2
1.7260490638591 1.7
1.72682839380754 1.4
1.73697869331156 1.1
1.75903740216506 0.8
1.79684511948947 0.5
1.8557854948005 0.2
1.94130663414529 -0.1
2 -0.251563585756
2.08765559667805 -0.4
2.3 -0.69125918304644
2.31248780404341 -0.7
2.6 -0.869387352557762
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
2.3 -0.401109893914359
2.6 -0.610333547467403
2.9 -0.655854072757327
3.2 -0.581577343954689
3.5 -0.435296687587471
3.55328729169425 -0.4
3.8 -0.227170663944001
3.96181962281302 -0.1
4.1 0.0131876412949852
4.31500934897489 0.2
4.4 0.275986189936832
4.64286077030928 0.5
4.7 0.553704896868139
4.95767460699179 0.8
5 0.840940293584231
5 1.1
5 1.13279799779649
4.96632366398871 1.1
4.7 0.844435714361236
4.65314809743422 0.8
4.4 0.565423562486664
4.32764381833845 0.5
4.1 0.301311648093975
3.9779137035262 0.2
3.8 0.0598292409004596
3.57485034329561 -0.1
3.5 -0.14938223003685
3.2 -0.295085904963373
2.9 -0.363636942236166
2.6 -0.294315174386716
2.37904695873141 -0.1
2.3 -0.00588785005763724
2.21081207546153 0.2
2.11986335413307 0.5
2.06095013852652 0.8
2.02640928404263 1.1
2.00980561426349 1.4
2.00575045777126 1.7
2.00954240850964 2
2.01863061847589 2.3
2.03053354936279 2.6
2.04349075121075 2.9
2.0560234096589 3.2
2.06572680128641 3.5
2.0710646643341 3.8
2.072030535105 4.1
2.07073614264835 4.4
2.07406674873418 4.7
2.08573491663326 5
2 5
1.90942198231216 5
1.90608324142309 4.7
1.90714834171887 4.4
1.90824852499678 4.1
1.90799236223368 3.8
1.90512366457238 3.5
1.8998310731669 3.2
1.89256425710201 2.9
1.88424403488159 2.6
1.87587113878381 2.3
1.86879009957007 2
1.86480094565043 1.7
1.86643538620561 1.4
1.87659760909317 1.1
1.89824921238274 0.8
1.93548559975269 0.5
1.99399978279598 0.2
2 0.17900429343446
2.12433898787461 -0.1
2.29919082461699 -0.4
2.3 -0.401109893914359
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
2.6 -0.294315174386716
2.9 -0.363636942236166
3.2 -0.295085904963373
3.5 -0.14938223003685
3.57485034329561 -0.1
3.8 0.0598292409004596
3.9779137035262 0.2
4.1 0.301311648093975
4.32764381833845 0.5
4.4 0.565423562486664
4.65314809743422 0.8
4.7 0.844435714361236
4.96632366398871 1.1
5 1.13279799779649
5 1.4
5 1.51820809193783
4.8798806097404 1.4
4.7 1.22615866148472
4.56867862807578 1.1
4.4 0.942375890764522
4.24478658513199 0.8
4.1 0.672531113140215
3.89494077061612 0.5
3.8 0.424742978734546
3.5 0.211908406559807
3.47655644842709 0.2
3.2 0.0767485776005726
2.9 0.0309675179277776
2.6 0.148268678184881
2.55662295179469 0.2
2.38440251295829 0.5
2.3 0.73401564930199
2.28745167340987 0.8
2.25378448514593 1.1
2.2363608180548 1.4
2.23032844530419 1.7
2.23256080790472 2
2.2411439023099 2.3
2.25382771181275 2.6
2.26792210060542 2.9
2.28102298043944 3.2
2.29163620011918 3.5
2.29766833273884 3.8
2.29830971482151 4.1
2.29505624307046 4.4
2.3 4.575667054122
2.3068220227583 4.7
2.33814300997679 5
2.3 5
2.08573491663326 5
2.07406674873418 4.7
2.07073614264835 4.4
2.072030535105 4.1
2.0710646643341 3.8
2.06572680128641 3.5
2.0560234096589 3.2
2.04349075121075 2.9
2.03053354936279 2.6
2.01863061847589 2.3
2.00954240850964 2
2.00575045777126 1.7
2.00980561426349 1.4
2.02640928404263 1.1
2.06095013852652 0.8
2.11986335413307 0.5
2.21081207546153 0.2
2.3 -0.00588785005763724
2.37904695873141 -0.1
2.6 -0.294315174386716
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
2.6 0.148268678184881
2.9 0.0309675179277776
3.2 0.0767485776005726
3.47655644842709 0.2
3.5 0.211908406559807
3.8 0.424742978734546
3.89494077061612 0.5
4.1 0.672531113140215
4.24478658513198 0.8
4.4 0.942375890764522
4.56867862807578 1.1
4.7 1.22615866148472
4.8798806097404 1.4
5 1.51820809193783
5 1.7
5 2
5 2.12716823682003
4.87685174556424 2
4.7 1.82281255617532
4.57880133045507 1.7
4.4 1.52593593949518
4.26940468165709 1.4
4.1 1.24487379564146
3.9334228913981 1.1
3.8 0.99160820420055
3.53088676220456 0.8
3.5 0.779998625217848
3.2 0.672260558126029
2.9 0.715597637481955
2.82247815853516 0.8
2.66899254252907 1.1
2.6 1.37915669849477
2.59750079801549 1.4
2.58185108341317 1.7
2.58096148681319 2
2.59128426482297 2.3
2.6 2.45234711271663
2.61340996069256 2.6
2.64427102516291 2.9
2.67486159707477 3.2
2.70179946563734 3.5
2.72415867279574 3.8
2.7431361222598 4.1
2.76398653015719 4.4
2.7995031831101 4.7
2.83615044119233 5
2.6 5
2.33814300997679 5
2.3068220227583 4.7
2.3 4.575667054122
2.29505624307046 4.4
2.29830971482151 4.1
2.29766833273884 3.8
2.29163620011918 3.5
2.28102298043944 3.2
2.26792210060542 2.9
2.25382771181275 2.6
2.2411439023099 2.3
2.23256080790472 2
2.23032844530419 1.7
2.2363608180548 1.4
2.25378448514593 1.1
2.28745167340987 0.8
2.3 0.73401564930199
2.38440251295829 0.5
2.55662295179469 0.2
2.6 0.148268678184881
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
2.9 0.715597637481955
3.2 0.672260558126029
3.5 0.779998625217848
3.53088676220456 0.8
3.8 0.99160820420055
3.9334228913981 1.1
4.1 1.24487379564146
4.26940468165709 1.4
4.4 1.52593593949518
4.57880133045507 1.7
4.7 1.82281255617532
4.87685174556424 2
5 2.12716823682003
5 2.3
5 2.6
5 2.9
5 3.2
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.1 5
3.8 5
3.5 5
3.2 5
2.9 5
2.83615044119233 5
2.7995031831101 4.7
2.76398653015719 4.4
2.7431361222598 4.1
2.72415867279574 3.8
2.70179946563734 3.5
2.67486159707477 3.2
2.64427102516291 2.9
2.61340996069256 2.6
2.6 2.45234711271663
2.59128426482297 2.3
2.58096148681319 2
2.58185108341317 1.7
2.59750079801549 1.4
2.6 1.37915669849477
2.66899254252907 1.1
2.82247815853516 0.8
2.9 0.715597637481955
};
\addplot [semithick, steelblue31119180, mark=mystar, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
4.1 3.2
};
\coordinate (CVI_mean_lml_ep_t) at (axis cs:4.1,3.2);
\end{axis}



==> fig/tikz/usps/CVI_nlpd.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.7 -1
-0.4 -1
-0.1 -1
0.2 -1
0.5 -1
0.8 -1
0.925113689757841 -1
0.860469763454581 -0.7
0.821377521170356 -0.4
0.8 -0.153444584124935
0.782829659258018 -0.1
0.711957843762462 0.2
0.672773024563125 0.5
0.651279652978252 0.8
0.642778017285618 1.1
0.655591761565055 1.4
0.70939781533501 1.7
0.8 1.95690187617473
0.802696151145468 2
0.814315346631294 2.3
0.81923163041049 2.6
0.820404935498082 2.9
0.821592078953209 3.2
0.82345709738071 3.5
0.823768953921614 3.8
0.822662483446321 4.1
0.822817303375986 4.4
0.824294120535959 4.7
0.826123619076537 5
0.8 5
0.5 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
1.1 -1
1.21659310285514 -1
1.14212194116255 -0.7
1.1 -0.476614455232909
1.07279019199168 -0.4
0.992821132254586 -0.1
0.94556830511979 0.2
0.917531887171415 0.5
0.901008786481787 0.8
0.892769747023101 1.1
0.895147197483519 1.4
0.90911020987251 1.7
0.925697987528612 2
0.935714330996353 2.3
0.938528662308358 2.6
0.936820175800056 2.9
0.936856554071868 3.2
0.938667754718829 3.5
0.937234605111878 3.8
0.933802829765485 4.1
0.933789891164454 4.4
0.936821393904746 4.7
0.942315702987839 5
0.826123619076537 5
0.824294120535959 4.7
0.822817303375986 4.4
0.82266248344632 4.1
0.823768953921614 3.8
0.82345709738071 3.5
0.821592078953209 3.2
0.820404935498082 2.9
0.81923163041049 2.6
0.814315346631294 2.3
0.802696151145468 2
0.8 1.95690187617473
0.70939781533501 1.7
0.655591761565055 1.4
0.642778017285618 1.1
0.651279652978252 0.8
0.672773024563125 0.5
0.711957843762462 0.2
0.782829659258018 -0.1
0.8 -0.153444584124935
0.821377521170356 -0.4
0.860469763454581 -0.7
0.925113689757841 -1
1.1 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
1.27560486554141 -0.7
1.19859544391019 -0.4
1.14446327753077 -0.1
1.10615953019748 0.2
1.1 0.268233107532229
1.06584809021152 0.5
1.03932640860852 0.8
1.02507505328551 1.1
1.02359108677481 1.4
1.03461941021665 1.7
1.04869982391176 2
1.05711331536141 2.3
1.05782569420622 2.6
1.05323541610203 2.9
1.05212102919053 3.2
1.05387841205695 3.5
1.05070025630214 3.8
1.04494317608465 4.1
1.04476247895292 4.4
1.04934866727353 4.7
1.05850778689914 5
0.942315702987839 5
0.936821393904746 4.7
0.933789891164454 4.4
0.933802829765485 4.1
0.937234605111878 3.8
0.938667754718829 3.5
0.936856554071868 3.2
0.936820175800056 2.9
0.938528662308358 2.6
0.935714330996353 2.3
0.925697987528612 2
0.90911020987251 1.7
0.895147197483519 1.4
0.892769747023101 1.1
0.901008786481787 0.8
0.917531887171415 0.5
0.94556830511979 0.2
0.992821132254586 -0.1
1.07279019199168 -0.4
1.1 -0.476614455232909
1.14212194116255 -0.7
1.21659310285514 -1
1.39099484413736 -1
1.27560486554141 -0.7
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
1.4 -1
1.50974483263259 -1
1.40698291867947 -0.7
1.4 -0.677044248044066
1.30915667213568 -0.4
1.2423140200388 -0.1
1.19702051506529 0.2
1.16690188723253 0.5
1.14740616436698 0.8
1.13579216641432 1.1
1.13258240854128 1.4
1.13733839514132 1.7
1.14409241726953 2
1.14775151494952 2.3
1.14700072869955 2.6
1.14333813972643 2.9
1.1420944903903 3.2
1.14269700582772 3.5
1.14018408105254 3.8
1.13624582646329 4.1
1.13652104556426 4.4
1.14048559819822 4.7
1.14725622050636 5
1.1 5
1.05850778689914 5
1.04934866727353 4.7
1.04476247895292 4.4
1.04494317608465 4.1
1.05070025630214 3.8
1.05387841205695 3.5
1.05212102919053 3.2
1.05323541610203 2.9
1.05782569420622 2.6
1.05711331536141 2.3
1.04869982391176 2
1.03461941021665 1.7
1.02359108677481 1.4
1.02507505328551 1.1
1.03932640860852 0.8
1.06584809021152 0.5
1.1 0.268233107532229
1.10615953019748 0.2
1.14446327753077 -0.1
1.19859544391019 -0.4
1.27560486554141 -0.7
1.39099484413736 -1
1.4 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
5 -1
5 -0.759615580143111
4.74510557658577 -1
5 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
1.50954915471849 -0.7
1.41726673406653 -0.4
1.4 -0.332260706535237
1.34016476254684 -0.1
1.2878814999331 0.2
1.25381727564278 0.5
1.23185705991294 0.8
1.21832029235413 1.1
1.21300929814346 1.4
1.21527653594673 1.7
1.21973150669113 2
1.2215868940807 2.3
1.21970364927999 2.6
1.21577421155939 2.9
1.21409809695179 3.2
1.21389712693012 3.5
1.21124226603416 3.8
1.20807394162249 4.1
1.20923711413581 4.4
1.21411250275367 4.7
1.22076101614837 5
1.14725622050636 5
1.14048559819822 4.7
1.13652104556426 4.4
1.13624582646329 4.1
1.14018408105254 3.8
1.14269700582772 3.5
1.1420944903903 3.2
1.14333813972643 2.9
1.14700072869955 2.6
1.14775151494952 2.3
1.14409241726953 2
1.13733839514132 1.7
1.13258240854128 1.4
1.13579216641432 1.1
1.14740616436698 0.8
1.16690188723253 0.5
1.19702051506529 0.2
1.2423140200388 -0.1
1.30915667213568 -0.4
1.4 -0.677044248044066
1.40698291867947 -0.7
1.50974483263259 -1
1.62546481475493 -1
1.50954915471849 -0.7
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
4.7 -1
4.74510557658577 -1
5 -0.759615580143111
5 -0.7
5 -0.553675079684867
4.84568210960732 -0.7
4.7 -0.83893245374039
4.52369370430006 -1
4.7 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.7 -1
1.74505216679117 -1
1.7 -0.911960853705987
1.61211539075751 -0.7
1.51408390480335 -0.4
1.43696156581 -0.1
1.4 0.0872429194056387
1.37874248480091 0.2
1.34073266405303 0.5
1.3163079554589 0.8
1.30084841829394 1.1
1.29343618774563 1.4
1.29321467675215 1.7
1.29537059611273 2
1.29542227321188 2.3
1.29240656986043 2.6
1.28821028339234 2.9
1.28610170351327 3.2
1.28509724803253 3.5
1.28230045101578 3.8
1.27990205678168 4.1
1.28195318270735 4.4
1.28773940730912 4.7
1.29426581179038 5
1.22076101614837 5
1.21411250275367 4.7
1.20923711413581 4.4
1.20807394162249 4.1
1.21124226603416 3.8
1.21389712693012 3.5
1.21409809695179 3.2
1.21577421155939 2.9
1.21970364927999 2.6
1.2215868940807 2.3
1.21973150669113 2
1.21527653594673 1.7
1.21300929814346 1.4
1.21832029235413 1.1
1.23185705991294 0.8
1.25381727564278 0.5
1.2878814999331 0.2
1.34016476254684 -0.1
1.4 -0.332260706535237
1.41726673406653 -0.4
1.50954915471849 -0.7
1.62546481475493 -1
1.7 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
4.4 -1
4.52369370430006 -1
4.7 -0.83893245374039
4.84568210960732 -0.7
5 -0.553675079684867
5 -0.4
5 -0.361918382558826
4.96006943163989 -0.4
4.7 -0.647549162215944
4.64311694003414 -0.7
4.4 -0.923735587197823
4.31244566796735 -1
4.4 -1
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.7 -0.911960853705987
1.74505216679117 -1
1.87163858534707 -1
1.7180481755194 -0.7
1.7 -0.659618268498654
1.61090107554016 -0.4
1.53209950106952 -0.1
1.47300229188986 0.2
1.43051924965413 0.5
1.40086650341687 0.8
1.4 0.812811499708162
1.38337654423375 1.1
1.37386307734781 1.4
1.37115281755756 1.7
1.37100968553433 2
1.36925765234306 2.3
1.36510949044087 2.6
1.3606463552253 2.9
1.35810531007476 3.2
1.35629736913493 3.5
1.3533586359974 3.8
1.35173017194088 4.1
1.3546692512789 4.4
1.36136631186456 4.7
1.36777060743239 5
1.29426581179038 5
1.28773940730912 4.7
1.28195318270735 4.4
1.27990205678168 4.1
1.28230045101578 3.8
1.28509724803253 3.5
1.28610170351327 3.2
1.28821028339234 2.9
1.29240656986043 2.6
1.29542227321188 2.3
1.29537059611273 2
1.29321467675215 1.7
1.29343618774563 1.4
1.30084841829394 1.1
1.3163079554589 0.8
1.34073266405303 0.5
1.37874248480091 0.2
1.4 0.0872429194056387
1.43696156581 -0.1
1.51408390480335 -0.4
1.61211539075751 -0.7
1.7 -0.911960853705987
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
4.4 -0.923735587197823
4.64311694003414 -0.7
4.7 -0.647549162215944
4.96006943163989 -0.4
5 -0.361918382558826
5 -0.180725557909958
4.77007927478326 -0.4
4.7 -0.466705516491915
4.44699157047346 -0.7
4.4 -0.743245388872334
4.1052363265171 -1
4.31244566796735 -1
4.4 -0.923735587197823
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.84413321064875 -0.7
1.71044718577037 -0.4
1.7 -0.3716813939865
1.62723743632903 -0.1
1.56830012934381 0.2
1.5264606343575 0.5
1.49729780426533 0.8
1.47701368858047 1.1
1.46437898626966 1.4
1.45855748266052 1.7
1.45574432731504 2
1.45193213546915 2.3
1.44604469055925 2.6
1.44036759707949 2.9
1.4369977925225 3.2
1.43434003839393 3.5
1.43082350212106 3.8
1.42964039153516 4.1
1.43393676396246 4.4
1.44299851393898 4.7
1.45098799411297 5
1.4 5
1.36777060743239 5
1.36136631186456 4.7
1.3546692512789 4.4
1.35173017194088 4.1
1.3533586359974 3.8
1.35629736913493 3.5
1.35810531007476 3.2
1.3606463552253 2.9
1.36510949044087 2.6
1.36925765234306 2.3
1.37100968553433 2
1.37115281755756 1.7
1.37386307734781 1.4
1.38337654423375 1.1
1.4 0.812811499708162
1.40086650341687 0.8
1.43051924965413 0.5
1.47300229188986 0.2
1.53209950106952 -0.1
1.61090107554016 -0.4
1.7 -0.659618268498654
1.7180481755194 -0.7
1.87163858534707 -1
1.99822500390297 -1
1.84413321064875 -0.7
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
4.1 -1
4.1052363265171 -1
4.4 -0.743245388872334
4.44699157047346 -0.7
4.7 -0.466705516491915
4.77007927478326 -0.4
5 -0.180725557909958
5 -0.1
5 0.00733645612447965
4.8880869671635 -0.1
4.7 -0.278861409699853
4.56980752021934 -0.4
4.4 -0.555947257485403
4.23693482379043 -0.7
4.1 -0.81874262703893
3.87561225291558 -1
4.1 -1
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
2 -1
2.19304679224855 -1
2 -0.757979198377285
1.9702182457781 -0.7
1.84149599299313 -0.4
1.732572055374 -0.1
1.7 0.0143227453043903
1.66359796679775 0.2
1.62240201906086 0.5
1.5937291051138 0.8
1.57345291471605 1.1
1.55975207106414 1.4
1.5515249349368 1.7
1.54613148458791 2
1.54091239005506 2.3
1.53457603226593 2.6
1.52875501063366 2.9
1.52547571846777 3.2
1.52325778583946 3.5
1.520526503072 3.8
1.52001255855676 4.1
1.52404884112161 4.4
1.53346883378078 4.7
1.54178933845633 5
1.45098799411297 5
1.44299851393898 4.7
1.43393676396246 4.4
1.42964039153516 4.1
1.43082350212106 3.8
1.43434003839393 3.5
1.4369977925225 3.2
1.44036759707949 2.9
1.44604469055925 2.6
1.45193213546915 2.3
1.45574432731504 2
1.45855748266052 1.7
1.46437898626966 1.4
1.47701368858047 1.1
1.49729780426533 0.8
1.5264606343575 0.5
1.56830012934381 0.2
1.62723743632903 -0.1
1.7 -0.3716813939865
1.71044718577037 -0.4
1.84413321064875 -0.7
1.99822500390297 -1
2 -1
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
3.8 -1
3.87561225291558 -1
4.1 -0.81874262703893
4.23693482379043 -0.7
4.4 -0.555947257485403
4.56980752021934 -0.4
4.7 -0.278861409699853
4.8880869671635 -0.1
5 0.00733645612447965
5 0.2
5 0.201103198505991
4.9988565498253 0.2
4.7 -0.084369544383322
4.68335440676387 -0.1
4.4 -0.36030675061999
4.3556795849554 -0.4
4.1 -0.62150723331878
4.00474790551871 -0.7
3.8 -0.860915385419227
3.60399054855979 -1
3.8 -1
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
2 -0.757979198377285
2.19304679224855 -1
2.3 -1
2.49093426075718 -1
2.3 -0.876619691730594
2.16212698798939 -0.7
2 -0.464575252124623
1.97254480021588 -0.4
1.87106531271178 -0.1
1.79029154297207 0.2
1.7291571045788 0.5
1.7 0.695607278034531
1.69016040596227 0.8
1.66989214085163 1.1
1.65512515585862 1.4
1.64449238721308 1.7
1.63651864186079 2
1.62989264464098 2.3
1.62310737397261 2.6
1.61714242418784 2.9
1.61395364441303 3.2
1.61217553328498 3.5
1.61022950402294 3.8
1.61038472557836 4.1
1.61416091828075 4.4
1.62393915362258 4.7
1.63259068279969 5
1.54178933845633 5
1.53346883378078 4.7
1.52404884112161 4.4
1.52001255855676 4.1
1.520526503072 3.8
1.52325778583946 3.5
1.52547571846777 3.2
1.52875501063366 2.9
1.53457603226593 2.6
1.54091239005506 2.3
1.54613148458791 2
1.5515249349368 1.7
1.55975207106414 1.4
1.57345291471605 1.1
1.5937291051138 0.8
1.62240201906086 0.5
1.66359796679775 0.2
1.7 0.0143227453043903
1.732572055374 -0.1
1.84149599299313 -0.4
1.9702182457781 -0.7
2 -0.757979198377285
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
3.5 -1
3.60399054855979 -1
3.8 -0.860915385419227
4.00474790551871 -0.7
4.1 -0.62150723331878
4.3556795849554 -0.4
4.4 -0.36030675061999
4.68335440676387 -0.1
4.7 -0.084369544383322
4.9988565498253 0.2
5 0.201103198505991
5 0.433770600394275
4.75769996749509 0.2
4.7 0.145097025723198
4.43898487071485 -0.1
4.4 -0.135813895167619
4.10501689838765 -0.4
4.1 -0.404346374709126
3.8 -0.641712674909395
3.72000525894802 -0.7
3.5 -0.846387424626304
3.22144344083424 -1
3.5 -1
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
2.3 -0.876619691730594
2.49093426075718 -1
2.6 -1
2.9 -1
3.2 -1
3.22144344083424 -1
3.5 -0.846387424626304
3.72000525894802 -0.7
3.8 -0.641712674909395
4.1 -0.404346374709126
4.10501689838765 -0.4
4.4 -0.135813895167619
4.43898487071485 -0.1
4.7 0.145097025723198
4.75769996749509 0.2
5 0.433770600394275
5 0.5
5 0.718775086490995
4.77499796662657 0.5
4.7 0.428408933670091
4.45950976151128 0.2
4.4 0.145102578987026
4.13061575371508 -0.1
4.1 -0.126644182538081
3.8 -0.373565099903082
3.76479656037498 -0.4
3.5 -0.578047917308111
3.28535503003989 -0.7
3.2 -0.741764783376395
2.9 -0.816025305720146
2.6 -0.782035518763073
2.46707787362906 -0.7
2.3 -0.573465048386441
2.18659239678949 -0.4
2.01808337676524 -0.1
2 -0.0589510012831944
1.93639004514799 0.2
1.88165731790813 0.5
1.84131014321839 0.8
1.81064206316077 1.1
1.7864114219959 1.4
1.76655446087044 1.7
1.74970718489063 2
1.73565752178364 2.3
1.72234833553643 2.6
1.71074078694224 2.9
1.70471525161602 3.2
1.70210086302464 3.5
1.7 3.78269995264945
1.69993250497388 3.8
1.7 3.82473000005294
1.70143063178781 4.1
1.70819191955706 4.4
1.72700623178521 4.7
1.74238465923965 5
1.7 5
1.63259068279969 5
1.62393915362258 4.7
1.61416091828075 4.4
1.61038472557836 4.1
1.61022950402294 3.8
1.61217553328498 3.5
1.61395364441303 3.2
1.61714242418784 2.9
1.62310737397261 2.6
1.62989264464098 2.3
1.63651864186079 2
1.64449238721308 1.7
1.65512515585862 1.4
1.66989214085163 1.1
1.69016040596227 0.8
1.7 0.695607278034531
1.7291571045788 0.5
1.79029154297207 0.2
1.87106531271178 -0.1
1.97254480021588 -0.4
2 -0.464575252124623
2.16212698798939 -0.7
2.3 -0.876619691730594
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
2.6 -0.782035518763073
2.9 -0.816025305720146
3.2 -0.741764783376395
3.28535503003989 -0.7
3.5 -0.578047917308111
3.76479656037498 -0.4
3.8 -0.373565099903082
4.1 -0.126644182538081
4.13061575371508 -0.1
4.4 0.145102578987026
4.45950976151128 0.2
4.7 0.428408933670091
4.77499796662657 0.5
5 0.718775086490995
5 0.8
5 1.1
5 1.11965781148736
4.9805376416773 1.1
4.7 0.825314055086031
4.67467194141333 0.8
4.4 0.537703113127295
4.36107718171357 0.5
4.1 0.262839016233103
4.03037892272527 0.2
3.8 0.00970121181414806
3.65986647932606 -0.1
3.5 -0.210773828123406
3.2 -0.385074868278017
3.14930771533077 -0.4
2.9 -0.457749176206977
2.6 -0.412015999336825
2.58357607468392 -0.4
2.3 -0.138276507480658
2.28009178794997 -0.1
2.16121111423526 0.2
2.06819601440418 0.5
2 0.789152189138474
1.9986776491323 0.8
1.97150464498162 1.1
1.94961163987758 1.4
1.93172865139267 1.7
1.9166931612588 2
1.90377241118491 2.3
1.89234373575688 2.6
1.88241858684372 2.9
1.87628983997694 3.2
1.87296640801289 3.5
1.87062088232964 3.8
1.87224653734722 4.1
1.88094915686101 4.4
1.89656568400037 4.7
1.90691011977195 5
1.74238465923965 5
1.72700623178521 4.7
1.70819191955706 4.4
1.70143063178781 4.1
1.7 3.82473000005294
1.69993250497388 3.8
1.7 3.78269995264945
1.70210086302464 3.5
1.70471525161602 3.2
1.71074078694224 2.9
1.72234833553643 2.6
1.73565752178364 2.3
1.74970718489063 2
1.76655446087044 1.7
1.7864114219959 1.4
1.81064206316077 1.1
1.84131014321839 0.8
1.88165731790813 0.5
1.93639004514799 0.2
2 -0.0589510012831944
2.01808337676524 -0.1
2.18659239678949 -0.4
2.3 -0.573465048386441
2.46707787362906 -0.7
2.6 -0.782035518763073
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
2.6 -0.412015999336825
2.9 -0.457749176206976
3.14930771533077 -0.4
3.2 -0.385074868278017
3.5 -0.210773828123406
3.65986647932606 -0.1
3.8 0.00970121181414803
4.03037892272527 0.2
4.1 0.262839016233103
4.36107718171357 0.5
4.4 0.537703113127295
4.67467194141333 0.8
4.7 0.825314055086031
4.9805376416773 1.1
5 1.11965781148736
5 1.4
5 1.7
5 1.97866654945577
4.75853106804382 1.7
4.7 1.63673309092511
4.49711818372558 1.4
4.4 1.2952118694405
4.22865600400463 1.1
4.1 0.965712374603683
3.94267035480068 0.8
3.8 0.663729060982212
3.61699513949982 0.5
3.5 0.407076190738351
3.2 0.214995003465352
3.1430640564692 0.2
2.9 0.148710802830845
2.74415194170141 0.2
2.6 0.271345116509083
2.46550215419487 0.5
2.33786011269405 0.8
2.3 0.920599369939154
2.27384928465317 1.1
2.23876525952366 1.4
2.20843369614227 1.7
2.18076485845377 2
2.15470996331599 2.3
2.13177299131531 2.6
2.11322698190317 2.9
2.10085798096663 3.2
2.094896505481 3.5
2.09083157777188 3.8
2.09221764358218 4.1
2.10544738053079 4.4
2.12856763895951 4.7
2.15192092399005 5
2 5
1.90691011977195 5
1.89656568400037 4.7
1.88094915686101 4.4
1.87224653734722 4.1
1.87062088232964 3.8
1.87296640801289 3.5
1.87628983997694 3.2
1.88241858684372 2.9
1.89234373575688 2.6
1.90377241118491 2.3
1.9166931612588 2
1.93172865139267 1.7
1.94961163987758 1.4
1.97150464498162 1.1
1.9986776491323 0.8
2 0.789152189138474
2.06819601440418 0.5
2.16121111423526 0.2
2.28009178794997 -0.1
2.3 -0.138276507480658
2.58357607468392 -0.4
2.6 -0.412015999336825
};
\addplot [draw=none, fill=lavender231240249]
table{%
x  y
2.9 0.148710802830845
3.1430640564692 0.2
3.2 0.214995003465352
3.5 0.407076190738351
3.61699513949982 0.5
3.8 0.663729060982212
3.94267035480068 0.8
4.1 0.965712374603683
4.22865600400463 1.1
4.4 1.2952118694405
4.49711818372558 1.4
4.7 1.63673309092511
4.75853106804382 1.7
5 1.97866654945577
5 2
5 2.3
5 2.6
5 2.9
5 3.2
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.1 5
3.8 5
3.5 5
3.43518215041185 5
3.41802428192927 4.7
3.43790985943538 4.4
3.5 4.30704312841933
3.58464628586566 4.4
3.8 4.59860357514058
3.94635090520314 4.7
4.1 4.79969680723698
4.16287007385271 4.7
4.1807929372837 4.4
4.16040885445074 4.1
4.10857019144245 3.8
4.1 3.771109523368
3.98349510252755 3.5
3.85960711293334 3.2
3.8 3.07034306537177
3.59370772021509 2.9
3.5 2.80860722743747
3.4105722392421 2.9
3.2 3.19528638077985
3.1987920333333 3.2
3.14784643879943 3.5
3.11471723655176 3.8
3.10806273001993 4.1
3.0881750686661 4.4
3.07312069415832 4.7
3.02046269781719 5
2.9 5
2.6 5
2.3 5
2.15192092399005 5
2.12856763895951 4.7
2.10544738053079 4.4
2.09221764358218 4.1
2.09083157777188 3.8
2.094896505481 3.5
2.10085798096663 3.2
2.11322698190317 2.9
2.13177299131531 2.6
2.15470996331599 2.3
2.18076485845377 2
2.20843369614227 1.7
2.23876525952366 1.4
2.27384928465317 1.1
2.3 0.920599369939154
2.33786011269405 0.8
2.46550215419487 0.5
2.6 0.271345116509083
2.74415194170141 0.2
2.9 0.148710802830845
};
\addplot [draw=none, fill=aliceblue242247253]
table{%
x  y
3.5 2.80860722743747
3.59370772021509 2.9
3.8 3.07034306537177
3.85960711293334 3.2
3.98349510252755 3.5
4.1 3.771109523368
4.10857019144245 3.8
4.16040885445074 4.1
4.1807929372837 4.4
4.16287007385271 4.7
4.1 4.79969680723698
3.94635090520314 4.7
3.8 4.59860357514058
3.58464628586566 4.4
3.5 4.30704312841933
3.43790985943538 4.4
3.41802428192927 4.7
3.43518215041185 5
3.2 5
3.02046269781719 5
3.07312069415832 4.7
3.0881750686661 4.4
3.10806273001993 4.1
3.11471723655176 3.8
3.14784643879943 3.5
3.1987920333333 3.2
3.2 3.19528638077985
3.4105722392421 2.9
3.5 2.80860722743747
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
4.1 2.6
};
\addplot [semithick, darkorange25512714, mark=mystar, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
4.1 3.2
};
\draw (axis cs:3.8,2.1) node[
  scale=0.5,
  anchor=base west,
  text=black,
  rotate=0.0
]{$-0.064$};
\draw (axis cs:2.7,3.2) node[
  scale=0.5,
  anchor=base west,
  text=black,
  rotate=0.0
]{$-0.059$};
\coordinate (CVI_mean_lml_b) at (axis cs:4.1,2.5999999999999996);
\coordinate (CVI_mean_lml_ep_b) at (axis cs:4.1,3.2);
\end{axis}



==> fig/tikz/usps/EP_mean_lml.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.7 -1
-0.4 -1
-0.1 -1
0.2 -1
0.5 -1
0.8 -1
1.09577175043836 -1
0.969076334379931 -0.7
0.896661665765523 -0.4
0.854085724525261 -0.1
0.828487945281069 0.2
0.813045306250138 0.5
0.803867529524183 0.8
0.8 1.01466723053767
0.793604092690313 1.1
0.780602542522535 1.4
0.773456062807945 1.7
0.769530387708693 2
0.767374797953379 2.3
0.766191435441032 2.6
0.765541885559676 2.9
0.765185372633607 3.2
0.764989704391906 3.5
0.764882316429539 3.8
0.764823379772374 4.1
0.764791056830834 4.4
0.764773325297235 4.7
0.764763563106329 5
0.5 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
1.1 -1
1.4 -1
1.40684216643347 -1
1.4 -0.979814552115557
1.28155970949484 -0.7
1.19887975851464 -0.4
1.14388213247721 -0.1
1.10681693614992 0.2
1.1 0.279720933034664
1.06436516091556 0.5
1.03579237767368 0.8
1.01971550126675 1.1
1.01074719772612 1.4
1.00577618923503 1.7
1.00303223292282 2
1.00152137313147 2.3
1.00069067279336 2.6
1.00023431307458 2.9
0.999983718374034 3.2
0.999846145846758 3.5
0.999770631628827 3.8
0.999729185170814 4.1
0.999706437673827 4.4
0.999693956508217 4.7
0.999687101663904 5
0.8 5
0.764763563106329 5
0.764773325297235 4.7
0.764791056830834 4.4
0.764823379772374 4.1
0.764882316429539 3.8
0.764989704391906 3.5
0.765185372633607 3.2
0.765541885559676 2.9
0.766191435441032 2.6
0.767374797953379 2.3
0.769530387708693 2
0.773456062807945 1.7
0.780602542522535 1.4
0.793604092690313 1.1
0.8 1.01466723053767
0.803867529524183 0.8
0.813045306250138 0.5
0.828487945281069 0.2
0.854085724525261 -0.1
0.896661665765523 -0.4
0.969076334379931 -0.7
1.09577175043836 -1
1.1 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
5 -1
5 -0.94410603735685
4.9407564633128 -1
5 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
1.4 -0.979814552115557
1.40684216643347 -1
1.58805454497982 -1
1.47031733731887 -0.7
1.4 -0.466787353734326
1.37584633317065 -0.4
1.29271881828719 -0.1
1.23966097760667 0.2
1.20626610717001 0.5
1.18589520390295 0.8
1.1738801365564 1.1
1.16698201726097 1.4
1.16309376242539 1.7
1.16092691687521 2
1.15972744191548 2.3
1.15906599360731 2.6
1.15870202135406 2.9
1.15850206772379 3.2
1.15839217021941 3.5
1.15833186211499 3.8
1.15829874057624 4.1
1.1582805498714 4.4
1.15827056697589 4.7
1.15826510690672 5
1.1 5
0.999687101663904 5
0.999693956508217 4.7
0.999706437673827 4.4
0.999729185170814 4.1
0.999770631628827 3.8
0.999846145846758 3.5
0.999983718374034 3.2
1.00023431307458 2.9
1.00069067279336 2.6
1.00152137313147 2.3
1.00303223292282 2
1.00577618923503 1.7
1.01074719772612 1.4
1.01971550126675 1.1
1.03579237767368 0.8
1.06436516091556 0.5
1.1 0.279720933034664
1.10681693614992 0.2
1.14388213247721 -0.1
1.19887975851464 -0.4
1.28155970949484 -0.7
1.4 -0.979814552115557
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
4.7 -1
4.9407564633128 -1
5 -0.94410603735685
5 -0.7
5 -0.580084292090219
4.87320182110155 -0.7
4.7 -0.86601762742214
4.55231864277404 -1
4.7 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
1.7 -1
1.76425449128694 -1
1.7 -0.877875395614802
1.61785833968295 -0.7
1.51102118487919 -0.4
1.43298058838577 -0.1
1.4 0.0722852805369267
1.37250501906341 0.2
1.33008918564343 0.5
1.30467389240192 0.8
1.28985784997827 1.1
1.28141187781019 1.4
1.27667078647235 1.7
1.27403485780709 2
1.27257762804707 2.3
1.27177462550326 2.6
1.27133293714298 2.9
1.27109049516159 3.2
1.27095713893903 3.5
1.2708840164108 3.8
1.27084383083358 4.1
1.27082174557211 4.4
1.27080962334938 4.7
1.27080302905129 5
1.15826510690672 5
1.15827056697589 4.7
1.1582805498714 4.4
1.15829874057624 4.1
1.15833186211499 3.8
1.15839217021941 3.5
1.15850206772379 3.2
1.15870202135406 2.9
1.15906599360731 2.6
1.15972744191548 2.3
1.16092691687521 2
1.16309376242539 1.7
1.16698201726097 1.4
1.1738801365564 1.1
1.18589520390295 0.8
1.20626610717001 0.5
1.23966097760667 0.2
1.29271881828719 -0.1
1.37584633317065 -0.4
1.4 -0.466787353734326
1.47031733731887 -0.7
1.58805454497982 -1
1.7 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
4.4 -1
4.55231864277404 -1
4.7 -0.86601762742214
4.87320182110155 -0.7
5 -0.580084292090219
5 -0.4
5 -0.305814103302366
4.90079170868214 -0.4
4.7 -0.591922357884665
4.581664267766 -0.7
4.4 -0.867966744578961
4.24584686000063 -1
4.4 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
1.7 -0.877875395614802
1.76425449128694 -1
1.93235361574124 -1
1.76656594531523 -0.7
1.7 -0.554369317266705
1.63959042082756 -0.4
1.55110504814263 -0.1
1.48923665555804 0.2
1.44771268099445 0.5
1.42133338741613 0.8
1.40539570450434 1.1
1.4 1.27419466753539
1.39584173835941 1.4
1.39024781051931 1.7
1.38714279873896 2
1.38542781417866 2.3
1.38448325739921 2.6
1.38396385293189 2.9
1.3836789225994 3.2
1.38352210765865 3.5
1.38343617070661 3.8
1.38338892109092 4.1
1.38336294127281 4.4
1.38334867972286 4.7
1.38334095119585 5
1.27080302905129 5
1.27080962334938 4.7
1.27082174557211 4.4
1.27084383083358 4.1
1.2708840164108 3.8
1.27095713893903 3.5
1.27109049516159 3.2
1.27133293714298 2.9
1.27177462550326 2.6
1.27257762804707 2.3
1.27403485780709 2
1.27667078647235 1.7
1.28141187781019 1.4
1.28985784997827 1.1
1.30467389240192 0.8
1.33008918564343 0.5
1.37250501906341 0.2
1.4 0.0722852805369267
1.43298058838577 -0.1
1.51102118487919 -0.4
1.61785833968295 -0.7
1.7 -0.877875395614802
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
4.1 -1
4.24584686000063 -1
4.4 -0.867966744578961
4.581664267766 -0.7
4.7 -0.591922357884665
4.90079170868214 -0.4
5 -0.305814103302366
5 -0.1
5 -0.0692558323546502
4.96775857893078 -0.1
4.7 -0.355470533544465
4.65159687326159 -0.4
4.4 -0.63192027948118
4.3214230057996 -0.7
4.1 -0.892945438704428
3.96332874159446 -1
4.1 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
2 -1
2.13255145698249 -1
2 -0.84438227910187
1.91673880619902 -0.7
1.77516991022416 -0.4
1.7 -0.198842009045542
1.66922950789949 -0.1
1.601763126244 0.2
1.55729685705775 0.5
1.52937914106844 0.8
1.51263153210211 1.1
1.50292329757768 1.4
1.49742152260364 1.7
1.49434633575036 2
1.49264123152258 2.3
1.49170010201346 2.6
1.49118197593252 2.9
1.49089742773048 3.2
1.49074088191816 3.5
1.49065657257919 3.8
1.49060946899688 4.1
1.49058298565338 4.4
1.49056943288417 4.7
1.49056176247982 5
1.4 5
1.38334095119585 5
1.38334867972286 4.7
1.38336294127281 4.4
1.38338892109092 4.1
1.38343617070661 3.8
1.38352210765865 3.5
1.3836789225994 3.2
1.38396385293189 2.9
1.38448325739921 2.6
1.38542781417866 2.3
1.38714279873896 2
1.39024781051931 1.7
1.39584173835941 1.4
1.4 1.27419466753539
1.40539570450434 1.1
1.42133338741613 0.8
1.44771268099445 0.5
1.48923665555804 0.2
1.55110504814263 -0.1
1.63959042082756 -0.4
1.7 -0.554369317266705
1.76656594531523 -0.7
1.93235361574124 -1
2 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
3.8 -1
3.96332874159446 -1
4.1 -0.892945438704428
4.3214230057996 -0.7
4.4 -0.63192027948118
4.65159687326159 -0.4
4.7 -0.355470533544465
4.96775857893078 -0.1
5 -0.0692558323546502
5 0.147955695995874
4.73996876112133 -0.1
4.7 -0.138134504483667
4.41535457806235 -0.4
4.4 -0.41415374519314
4.1 -0.674476315906766
4.0679493099546 -0.7
3.8 -0.911586283196167
3.66896929200571 -1
3.8 -1
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
2 -0.84438227910187
2.13255145698249 -1
2.3 -1
2.40351993803827 -1
2.3 -0.939481621822536
2.09443649013585 -0.7
2 -0.570373777617789
1.91696255386379 -0.4
1.80258400285395 -0.1
1.7175514706563 0.2
1.7 0.288759310968228
1.66688103312106 0.5
1.63742489472075 0.8
1.61986735969987 1.1
1.60972775770742 1.4
1.60399377635843 1.7
1.60079263037351 2
1.59901885609551 2.3
1.59804017954061 2.6
1.59750149601342 2.9
1.59720552120518 3.2
1.59704284176234 3.5
1.59695692259161 3.8
1.59690806657561 4.1
1.5968799383947 4.4
1.5968666396805 4.7
1.59685872050772 5
1.49056176247982 5
1.49056943288417 4.7
1.49058298565338 4.4
1.49060946899688 4.1
1.49065657257919 3.8
1.49074088191816 3.5
1.49089742773048 3.2
1.49118197593252 2.9
1.49170010201346 2.6
1.49264123152258 2.3
1.49434633575036 2
1.49742152260364 1.7
1.50292329757768 1.4
1.51263153210211 1.1
1.52937914106844 0.8
1.55729685705775 0.5
1.601763126244 0.2
1.66922950789949 -0.1
1.7 -0.198842009045542
1.77516991022416 -0.4
1.91673880619902 -0.7
2 -0.84438227910187
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
3.5 -1
3.66896929200571 -1
3.8 -0.911586283196167
4.0679493099546 -0.7
4.1 -0.674476315906766
4.4 -0.41415374519314
4.41535457806235 -0.4
4.7 -0.138134504483667
4.73996876112133 -0.1
5 0.147955695995874
5 0.2
5 0.366311088156129
4.82636885940346 0.2
4.7 0.0795131348009327
4.50625418154112 -0.1
4.4 -0.197792721927311
4.16916967997262 -0.4
4.1 -0.460071811796439
3.8 -0.698928455554881
3.79844435289378 -0.7
3.5 -0.899064924324671
3.30242280468644 -1
3.5 -1
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
2.3 -0.939481621822536
2.40351993803827 -1
2.6 -1
2.9 -1
3.2 -1
3.30242280468644 -1
3.5 -0.899064924324671
3.79844435289378 -0.7
3.8 -0.698928455554881
4.1 -0.460071811796439
4.16916967997262 -0.4
4.4 -0.197792721927311
4.50625418154112 -0.1
4.7 0.0795131348009328
4.82636885940346 0.2
5 0.366311088156129
5 0.5
5 0.593658939957205
4.9026670089412 0.5
4.7 0.306663474440266
4.5856760000355 0.2
4.4 0.0290871589212942
4.25414575577182 -0.1
4.1 -0.233730212084695
3.89427885769353 -0.4
3.8 -0.474150377464743
3.5 -0.679162271597814
3.45996881611594 -0.7
3.2 -0.826641792512859
2.9 -0.901497139856235
2.6 -0.869387865554374
2.3124869488751 -0.7
2.3 -0.691259795428152
2.08765475282108 -0.4
2 -0.251568753617219
1.94130328764352 -0.1
1.85576425986105 0.2
1.79673522388093 0.5
1.75857855517417 0.8
1.73528994850537 1.1
1.72165674743309 1.4
1.7138882332218 1.7
1.70953292817122 2
1.7071140207382 2.3
1.70577766321217 2.6
1.70504160082833 2.9
1.70463680617235 3.2
1.70441444564573 3.5
1.70429898326529 3.8
1.70423229867603 4.1
1.70419361090148 4.4
1.70417631121615 4.7
1.7041656542374 5
1.7 5
1.59685872050772 5
1.5968666396805 4.7
1.5968799383947 4.4
1.59690806657561 4.1
1.59695692259161 3.8
1.59704284176234 3.5
1.59720552120518 3.2
1.59750149601342 2.9
1.59804017954061 2.6
1.59901885609551 2.3
1.60079263037351 2
1.60399377635843 1.7
1.60972775770742 1.4
1.61986735969987 1.1
1.63742489472075 0.8
1.66688103312106 0.5
1.7 0.288759310968228
1.7175514706563 0.2
1.80258400285395 -0.1
1.91696255386379 -0.4
2 -0.570373777617789
2.09443649013585 -0.7
2.3 -0.939481621822536
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
2.6 -0.869387865554374
2.9 -0.901497139856235
3.2 -0.826641792512859
3.45996881611594 -0.7
3.5 -0.679162271597813
3.8 -0.474150377464743
3.89427885769353 -0.4
4.1 -0.233730212084695
4.25414575577182 -0.1
4.4 0.0290871589212942
4.5856760000355 0.2
4.7 0.306663474440266
4.9026670089412 0.5
5 0.593658939957205
5 0.8
5 0.840939755006943
4.95767516434503 0.8
4.7 0.553704362218229
4.64286134012998 0.5
4.4 0.275985662094608
4.31500993969381 0.2
4.1 0.0131871265015984
3.96182025439452 -0.1
3.8 -0.227171161114294
3.55328800674496 -0.4
3.5 -0.435297161108169
3.2 -0.581577866708063
2.9 -0.655854634985614
2.6 -0.610334183385177
2.3 -0.401110931790727
2.29919006643071 -0.4
2.12433410322718 -0.1
2 0.178929272943669
1.9939770490658 0.2
1.9353688576389 0.5
1.89777085544069 0.8
1.87491732119393 1.1
1.86156763177657 1.4
1.85396925696114 1.7
1.84971187479697 2
1.84734849460883 2.3
1.84604275368623 2.6
1.84532381039649 2.9
1.84492823505831 3.2
1.84471102492625 3.5
1.84459532359356 3.8
1.84452993888433 4.1
1.8445094230352 4.4
1.84448976202343 4.7
1.8444829801734 5
1.7041656542374 5
1.70417631121615 4.7
1.70419361090148 4.4
1.70423229867603 4.1
1.70429898326529 3.8
1.70441444564573 3.5
1.70463680617235 3.2
1.70504160082833 2.9
1.70577766321217 2.6
1.7071140207382 2.3
1.70953292817122 2
1.7138882332218 1.7
1.72165674743309 1.4
1.73528994850537 1.1
1.75857855517417 0.8
1.79673522388093 0.5
1.85576425986105 0.2
1.94130328764352 -0.1
2 -0.251568753617219
2.08765475282108 -0.4
2.3 -0.691259795428152
2.3124869488751 -0.7
2.6 -0.869387865554374
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
2.3 -0.401110931790727
2.6 -0.610334183385177
2.9 -0.655854634985614
3.2 -0.581577866708063
3.5 -0.435297161108169
3.55328800674496 -0.4
3.8 -0.227171161114294
3.96182025439452 -0.1
4.1 0.0131871265015984
4.31500993969381 0.2
4.4 0.275985662094608
4.64286134012998 0.5
4.7 0.553704362218229
4.95767516434503 0.8
5 0.840939755006943
5 1.1
5 1.13279742100786
4.96632425802943 1.1
4.7 0.844435138321929
4.65314870811277 0.8
4.4 0.565422987936738
4.32764445929949 0.5
4.1 0.301311081073495
3.97791439376095 0.2
3.8 0.0598286854053308
3.57485112847553 -0.1
3.5 -0.149382752322333
3.2 -0.295086572841971
2.9 -0.363637791186145
2.6 -0.294317258134022
2.3790395961567 -0.1
2.3 -0.00591498757152575
2.21078153065859 0.2
2.11968681524452 0.5
2.06018649242406 0.8
2.02375129532756 1.1
2.00241722030755 1.4
2 1.4597701518624
1.99405028070049 1.7
1.98989082142272 2
1.98758296847946 2.3
1.9863078441603 2.6
1.98560601996466 2.9
1.98521966394427 3.2
1.98500760420677 3.5
1.98489166392184 3.8
1.98482757909262 4.1
1.98482523516891 4.4
1.98480321283071 4.7
1.98480030610939 5
1.8444829801734 5
1.84448976202343 4.7
1.8445094230352 4.4
1.84452993888433 4.1
1.84459532359356 3.8
1.84471102492625 3.5
1.84492823505831 3.2
1.84532381039649 2.9
1.84604275368623 2.6
1.84734849460883 2.3
1.84971187479697 2
1.85396925696114 1.7
1.86156763177657 1.4
1.87491732119393 1.1
1.89777085544069 0.8
1.9353688576389 0.5
1.9939770490658 0.2
2 0.178929272943669
2.12433410322718 -0.1
2.29919006643071 -0.4
2.3 -0.401110931790727
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
2.6 -0.294317258134022
2.9 -0.363637791186145
3.2 -0.295086572841971
3.5 -0.149382752322333
3.57485112847553 -0.1
3.8 0.0598286854053308
3.97791439376095 0.2
4.1 0.301311081073495
4.32764445929949 0.5
4.4 0.565422987936738
4.65314870811278 0.8
4.7 0.844435138321929
4.96632425802943 1.1
5 1.13279742100786
5 1.4
5 1.51820725314777
4.87988150635818 1.4
4.7 1.22615777364333
4.56867962238469 1.1
4.4 0.942374927165217
4.24478773846129 0.8
4.1 0.67253004951219
3.89494215819474 0.5
3.8 0.424741833498208
3.5 0.211906778413339
3.4765597535846 0.2
3.2 0.0767458919367535
2.9 0.0309603092881951
2.6 0.148238350806301
2.55658955706388 0.2
2.38415081522009 0.5
2.3 0.731349685577307
2.28683100275315 0.8
2.25176097303744 1.1
2.23115698600795 1.4
2.21939448169029 1.7
2.21279368550017 2
2.20912610371527 2.3
2.20709910941191 2.6
2.20598564786953 2.9
2.20537021911792 3.2
2.20503339589283 3.5
2.20484837421195 3.8
2.20474623647686 4.1
2.20478978568268 4.4
2.20477752260727 4.7
2.20478365109807 5
2 5
1.98480030610939 5
1.98480321283071 4.7
1.98482523516891 4.4
1.98482757909262 4.1
1.98489166392184 3.8
1.98500760420677 3.5
1.98521966394427 3.2
1.98560601996466 2.9
1.9863078441603 2.6
1.98758296847946 2.3
1.98989082142272 2
1.99405028070049 1.7
2 1.4597701518624
2.00241722030755 1.4
2.02375129532756 1.1
2.06018649242406 0.8
2.11968681524452 0.5
2.21078153065859 0.2
2.3 -0.00591498757152575
2.3790395961567 -0.1
2.6 -0.294317258134022
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
2.6 0.148238350806301
2.9 0.0309603092881951
3.2 0.0767458919367535
3.4765597535846 0.2
3.5 0.211906778413339
3.8 0.424741833498208
3.89494215819474 0.5
4.1 0.67253004951219
4.24478773846129 0.8
4.4 0.942374927165217
4.56867962238469 1.1
4.7 1.22615777364333
4.87988150635818 1.4
5 1.51820725314777
5 1.7
5 2
5 2.12715668583872
4.87686476473922 2
4.7 1.82279892908277
4.57881766366898 1.7
4.4 1.52591881903065
4.26942697829657 1.4
4.1 1.24485109420936
3.93345631505645 1.1
3.8 0.991577839298379
3.53094314106812 0.8
3.5 0.779961010353491
3.2 0.67213506256359
2.9 0.715067546980933
2.82164082397377 0.8
2.66514708042188 1.1
2.6 1.3382249611912
2.59179590788647 1.4
2.56904815099373 1.7
2.55633762063254 2
2.54929321497678 2.3
2.54540593021676 2.6
2.54327607267776 2.9
2.5421014466509 3.2
2.54145253063 3.5
2.54110327672567 3.8
2.5409069438932 4.1
2.54084192757076 4.4
2.5410078983702 4.7
2.54100661259232 5
2.3 5
2.20478365109807 5
2.20477752260727 4.7
2.20478978568268 4.4
2.20474623647686 4.1
2.20484837421195 3.8
2.20503339589283 3.5
2.20537021911792 3.2
2.20598564786954 2.9
2.20709910941191 2.6
2.20912610371527 2.3
2.21279368550017 2
2.21939448169029 1.7
2.23115698600795 1.4
2.25176097303744 1.1
2.28683100275315 0.8
2.3 0.731349685577307
2.38415081522009 0.5
2.55658955706388 0.2
2.6 0.148238350806301
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
2.9 0.715067546980933
3.2 0.67213506256359
3.5 0.779961010353491
3.53094314106812 0.8
3.8 0.991577839298379
3.93345631505645 1.1
4.1 1.24485109420936
4.26942697829657 1.4
4.4 1.52591881903065
4.57881766366898 1.7
4.7 1.82279892908277
4.87686476473922 2
5 2.12715668583872
5 2.3
5 2.6
5 2.9
5 3.2
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.1 5
3.8 5
3.5 5
3.2 5
2.9 5
2.6 5
2.54100661259232 5
2.5410078983702 4.7
2.54084192757076 4.4
2.5409069438932 4.1
2.54110327672567 3.8
2.54145253063 3.5
2.5421014466509 3.2
2.54327607267776 2.9
2.54540593021676 2.6
2.54929321497678 2.3
2.55633762063254 2
2.56904815099373 1.7
2.59179590788647 1.4
2.6 1.3382249611912
2.66514708042188 1.1
2.82164082397377 0.8
2.9 0.715067546980933
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
3.8 5
};
\coordinate (EP_mean_lml_t) at (axis cs:3.8,5.0);
\end{axis}



==> fig/tikz/usps/EP_nlpd.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.7 -1
-0.4 -1
-0.1 -1
0.2 -1
0.5 -1
0.8 -1
0.925111869992329 -1
0.860464109363407 -0.7
0.821360296922516 -0.4
0.8 -0.154097474362705
0.782597667878001 -0.1
0.71149439891784 0.2
0.672037317416943 0.5
0.650152842153157 0.8
0.638042169843416 1.1
0.631357766024902 1.4
0.6276762092353 1.7
0.62565147443861 2
0.624538943755281 2.3
0.623927959113298 2.6
0.623592515673471 2.9
0.623408386700223 3.2
0.623307318186268 3.5
0.623251849937613 3.8
0.623221404624652 4.1
0.623205822417488 4.4
0.623196988554497 4.7
0.623191615359477 5
0.5 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
1.1 -1
1.21659120065671 -1
1.14211500294561 -0.7
1.1 -0.476752123847539
1.07273285797699 -0.4
0.992692732045872 -0.1
0.945348979080062 0.2
0.917287232927436 0.5
0.900858944575605 0.8
0.891414086858923 1.1
0.886072591066407 1.4
0.883088045410405 1.7
0.881432614338328 2
0.880518654807629 2.3
0.880015043855216 2.6
0.879738401468641 2.9
0.879586539217356 3.2
0.879503082824526 3.5
0.879457267700421 3.8
0.879432099548096 4.1
0.879418652970586 4.4
0.879411449620533 4.7
0.879406951850462 5
0.8 5
0.623191615359477 5
0.623196988554497 4.7
0.623205822417488 4.4
0.623221404624652 4.1
0.623251849937613 3.8
0.623307318186268 3.5
0.623408386700223 3.2
0.623592515673471 2.9
0.623927959113298 2.6
0.624538943755281 2.3
0.62565147443861 2
0.6276762092353 1.7
0.631357766024902 1.4
0.638042169843416 1.1
0.650152842153157 0.8
0.672037317416943 0.5
0.71149439891784 0.2
0.782597667878001 -0.1
0.8 -0.154097474362705
0.821360296922516 -0.4
0.860464109363407 -0.7
0.925111869992329 -1
1.1 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
1.27559560321003 -0.7
1.19856839533764 -0.4
1.14439030600594 -0.1
1.10600354281118 0.2
1.1 0.266531254196234
1.0656508452988 0.5
1.03964053756078 0.8
1.02488543207009 1.1
1.01661185413062 1.4
1.01201326611738 1.7
1.00946995835669 2
1.00806812573201 2.3
1.00729603482083 2.6
1.00687239753159 2.9
1.00664002912206 3.2
1.00651228482101 3.5
1.00644215985446 3.8
1.00640362123462 4.1
1.00638224362866 4.4
1.00637126644567 4.7
1.00636437699568 5
0.879406951850462 5
0.879411449620533 4.7
0.879418652970586 4.4
0.879432099548096 4.1
0.879457267700421 3.8
0.879503082824526 3.5
0.879586539217356 3.2
0.879738401468641 2.9
0.880015043855216 2.6
0.880518654807629 2.3
0.881432614338328 2
0.883088045410405 1.7
0.886072591066407 1.4
0.891414086858923 1.1
0.900858944575605 0.8
0.917287232927436 0.5
0.945348979080062 0.2
0.992692732045872 -0.1
1.07273285797699 -0.4
1.1 -0.47675212384754
1.14211500294561 -0.7
1.21659120065671 -1
1.39099185709029 -1
1.27559560321003 -0.7
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
1.4 -1
1.50974289403232 -1
1.40697429732878 -0.7
1.4 -0.677077176291307
1.30912971099943 -0.4
1.24226815591762 -0.1
1.19699947884875 0.2
1.16710750335998 0.5
1.1482457863795 0.8
1.13687730155678 1.1
1.13026484533686 1.4
1.12651068921176 1.7
1.12440933604942 2
1.12324328318199 2.3
1.12259863322283 2.6
1.12224422118146 2.9
1.1220521249204 3.2
1.1219448390942 3.5
1.12188624846659 3.8
1.12185389354082 4.1
1.12183554761515 4.4
1.12182622550736 4.7
1.12182077763165 5
1.1 5
1.00636437699568 5
1.00637126644567 4.7
1.00638224362866 4.4
1.00640362123462 4.1
1.00644215985446 3.8
1.00651228482101 3.5
1.00664002912206 3.2
1.00687239753159 2.9
1.00729603482083 2.6
1.00806812573201 2.3
1.00946995835669 2
1.01201326611738 1.7
1.01661185413062 1.4
1.02488543207009 1.1
1.03964053756078 0.8
1.0656508452988 0.5
1.1 0.266531254196234
1.10600354281118 0.2
1.14439030600594 -0.1
1.19856839533764 -0.4
1.27559560321003 -0.7
1.39099185709029 -1
1.4 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
5 -1
5 -0.759615749673315
4.74510576071017 -1
5 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
1.50954288743244 -0.7
1.41724594471141 -0.4
1.4 -0.332334155551769
1.34014600582931 -0.1
1.28799541488633 0.2
1.25443249546328 0.5
1.23362509247531 0.8
1.22122162754346 1.1
1.21405396513015 1.4
1.20999927716042 1.7
1.2077346183043 2
1.20647934486826 2.3
1.20578613607042 2.6
1.20540495741906 2.9
1.20520756584437 3.2
1.20509140465289 3.5
1.20502917415681 3.8
1.2049942751179 4.1
1.20497395421088 4.4
1.20496344519759 4.7
1.20495883034158 5
1.12182077763165 5
1.12182622550736 4.7
1.12183554761515 4.4
1.12185389354082 4.1
1.12188624846659 3.8
1.1219448390942 3.5
1.1220521249204 3.2
1.12224422118146 2.9
1.12259863322283 2.6
1.12324328318199 2.3
1.12440933604942 2
1.12651068921176 1.7
1.13026484533686 1.4
1.13687730155678 1.1
1.1482457863795 0.8
1.16710750335998 0.5
1.19699947884875 0.2
1.24226815591762 -0.1
1.30912971099943 -0.4
1.4 -0.677077176291307
1.40697429732878 -0.7
1.50974289403232 -1
1.62546296110414 -1
1.50954288743244 -0.7
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
4.7 -1
4.74510576071017 -1
5 -0.759615749673315
5 -0.7
5 -0.553675096120872
4.84568213826304 -0.7
4.7 -0.838932478223108
4.52369375458121 -1
4.7 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.7 -1
1.74505051295995 -1
1.7 -0.911964912693921
1.61211147753609 -0.7
1.51407859696109 -0.4
1.43698471799589 -0.1
1.4 0.0881705722321637
1.37899135092391 0.2
1.34175748756659 0.5
1.31900439857112 0.8
1.30556595353014 1.1
1.29784308492344 1.4
1.29348786510908 1.7
1.29105990055918 2
1.28971540655453 2.3
1.28897363891801 2.6
1.28856569365666 2.9
1.28836300676834 3.2
1.28823797021158 3.5
1.28817209984703 3.8
1.28813465669497 4.1
1.2881123608066 4.4
1.28810066488782 4.7
1.28809688305151 5
1.20495883034158 5
1.20496344519759 4.7
1.20497395421088 4.4
1.2049942751179 4.1
1.20502917415681 3.8
1.20509140465289 3.5
1.20520756584437 3.2
1.20540495741906 2.9
1.20578613607042 2.6
1.20647934486826 2.3
1.2077346183043 2
1.20999927716042 1.7
1.21405396513015 1.4
1.22122162754346 1.1
1.23362509247531 0.8
1.25443249546328 0.5
1.28799541488633 0.2
1.34014600582931 -0.1
1.4 -0.332334155551769
1.41724594471141 -0.4
1.50954288743244 -0.7
1.62546296110414 -1
1.7 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
4.4 -1
4.52369375458121 -1
4.7 -0.838932478223108
4.84568213826304 -0.7
5 -0.553675096120872
5 -0.4
5 -0.361918299768017
4.96006934698688 -0.4
4.7 -0.647549114012731
4.6431168923749 -0.7
4.4 -0.923735590385226
4.31244568094043 -1
4.4 -1
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.7 -0.911964912693921
1.74505051295995 -1
1.87163781390033 -1
1.7180465588116 -0.7
1.7 -0.659613203577232
1.61091124921076 -0.4
1.53218770586976 -0.1
1.47344532100267 0.2
1.43209751112298 0.5
1.40499201169296 0.8
1.4 0.890093185339391
1.38991027951681 1.1
1.38163220471673 1.4
1.37697645305774 1.7
1.37438518281405 2
1.3729514682408 2.3
1.3721611417656 2.6
1.37172642989426 2.9
1.3715184476923 3.2
1.37138453577026 3.5
1.37131502553725 3.8
1.37127503827205 4.1
1.37125076740233 4.4
1.37123788457805 4.7
1.37123493576144 5
1.28809688305151 5
1.28810066488782 4.7
1.2881123608066 4.4
1.28813465669497 4.1
1.28817209984703 3.8
1.28823797021158 3.5
1.28836300676834 3.2
1.28856569365666 2.9
1.28897363891801 2.6
1.28971540655453 2.3
1.29105990055918 2
1.29348786510908 1.7
1.29784308492344 1.4
1.30556595353014 1.1
1.31900439857112 0.8
1.34175748756659 0.5
1.37899135092391 0.2
1.4 0.0881705722321637
1.43698471799589 -0.1
1.51407859696109 -0.4
1.61211147753609 -0.7
1.7 -0.911964912693921
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
4.4 -0.923735590385226
4.6431168923749 -0.7
4.7 -0.647549114012731
4.96006934698688 -0.4
5 -0.361918299768017
5 -0.180725565842818
4.7700792955241 -0.4
4.7 -0.466705544957981
4.44699162188193 -0.7
4.4 -0.743245445276177
4.10523642262704 -1
4.31244568094043 -1
4.4 -0.923735590385226
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
1.84413658366391 -0.7
1.7104817923327 -0.4
1.7 -0.371528419648398
1.62739069374364 -0.1
1.56893731708327 0.2
1.52847563765018 0.5
1.50221902098077 0.8
1.4861407555287 1.1
1.47670594020937 1.4
1.47132150436618 1.7
1.46830037625102 2
1.46662080339669 2.3
1.46569235859749 2.6
1.4651815121434 2.9
1.46493209848509 3.2
1.46477547691123 3.5
1.46472790780735 3.8
1.46468318477988 4.1
1.46464677368775 4.4
1.46463936185245 4.7
1.46463701199298 5
1.4 5
1.37123493576144 5
1.37123788457805 4.7
1.37125076740233 4.4
1.37127503827205 4.1
1.37131502553725 3.8
1.37138453577026 3.5
1.3715184476923 3.2
1.37172642989426 2.9
1.3721611417656 2.6
1.3729514682408 2.3
1.37438518281405 2
1.37697645305774 1.7
1.38163220471673 1.4
1.38991027951681 1.1
1.4 0.890093185339391
1.40499201169296 0.8
1.43209751112298 0.5
1.47344532100267 0.2
1.53218770586976 -0.1
1.61091124921076 -0.4
1.7 -0.659613203577232
1.7180465588116 -0.7
1.87163781390033 -1
1.9982251148407 -1
1.84413658366391 -0.7
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
4.1 -1
4.10523642262704 -1
4.4 -0.743245445276177
4.44699162188193 -0.7
4.7 -0.466705544957981
4.7700792955241 -0.4
5 -0.180725565842818
5 -0.1
5 0.00733650126471466
4.88808692995311 -0.1
4.7 -0.278861372545683
4.56980748847688 -0.4
4.4 -0.555947225732596
4.23693481156883 -0.7
4.1 -0.818742613994574
3.87561226340847 -1
4.1 -1
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
2 -1
2.19304833277649 -1
2 -0.757964166650477
1.97022660851622 -0.7
1.84155006032276 -0.4
1.73287847148143 -0.1
1.7 0.0167497110704925
1.66442931316388 0.2
1.62485376417739 0.5
1.59944603026858 0.8
1.58398632235633 1.1
1.57494796238175 1.4
1.56980042029509 1.7
1.56691590676933 2
1.56531268944887 2.3
1.5644261813692 2.6
1.56393943536908 2.9
1.56368961173867 3.2
1.56354220463796 3.5
1.56355034801321 3.8
1.56351150732394 4.1
1.56346478030329 4.4
1.56347019444175 4.7
1.56346908764604 5
1.46463701199298 5
1.46463936185245 4.7
1.46464677368775 4.4
1.46468318477988 4.1
1.46472790780735 3.8
1.46477547691123 3.5
1.46493209848509 3.2
1.4651815121434 2.9
1.46569235859749 2.6
1.46662080339669 2.3
1.46830037625102 2
1.47132150436618 1.7
1.47670594020937 1.4
1.4861407555287 1.1
1.50221902098077 0.8
1.52847563765018 0.5
1.56893731708327 0.2
1.62739069374364 -0.1
1.7 -0.371528419648398
1.7104817923327 -0.4
1.84413658366391 -0.7
1.9982251148407 -1
2 -1
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
3.8 -1
3.87561226340847 -1
4.1 -0.818742613994574
4.23693481156883 -0.7
4.4 -0.555947225732596
4.56980748847688 -0.4
4.7 -0.278861372545683
4.88808692995311 -0.1
5 0.00733650126471466
5 0.2
5 0.201103466172723
4.99885627239995 0.2
4.7 -0.0843692641537596
4.68335412090701 -0.1
4.4 -0.360306452270664
4.35567927525647 -0.4
4.1 -0.621506940111497
4.00474761031526 -0.7
3.8 -0.860915123727064
3.60399029815731 -1
3.8 -1
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
2 -0.757964166650477
2.19304833277649 -1
2.3 -1
2.49093930856486 -1
2.3 -0.876606322217959
2.16214616384184 -0.7
2 -0.464426934564666
1.97261832831282 -0.4
1.87141847460038 -0.1
1.79171353866958 0.2
1.733583671273 0.5
1.7 0.759666457053156
1.69667303955639 0.8
1.68183188918396 1.1
1.67318998455413 1.4
1.668279336224 1.7
1.66553143728764 2
1.66400457550105 2.3
1.66316000414091 2.6
1.66269735859476 2.9
1.66244712499225 3.2
1.66230893236468 3.5
1.66237278821907 3.8
1.662339829868 4.1
1.66228278691884 4.4
1.66230102703104 4.7
1.66230116329909 5
1.56346908764604 5
1.56347019444175 4.7
1.56346478030329 4.4
1.56351150732394 4.1
1.56355034801321 3.8
1.56354220463796 3.5
1.56368961173867 3.2
1.56393943536908 2.9
1.5644261813692 2.6
1.56531268944887 2.3
1.56691590676933 2
1.56980042029509 1.7
1.57494796238175 1.4
1.58398632235633 1.1
1.59944603026858 0.8
1.62485376417739 0.5
1.66442931316388 0.2
1.7 0.0167497110704925
1.73287847148143 -0.1
1.84155006032276 -0.4
1.97022660851622 -0.7
2 -0.757964166650477
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
3.5 -1
3.60399029815731 -1
3.8 -0.860915123727064
4.00474761031526 -0.7
4.1 -0.621506940111497
4.35567927525647 -0.4
4.4 -0.360306452270664
4.68335412090701 -0.1
4.7 -0.0843692641537596
4.99885627239995 0.2
5 0.201103466172723
5 0.433771834246901
4.75769869022491 0.2
4.7 0.145098244215751
4.43898377022979 -0.1
4.4 -0.135812879276891
4.10501592001309 -0.4
4.1 -0.404345526608789
3.8 -0.641711415477596
3.72000373711342 -0.7
3.5 -0.84638621082865
3.22144190237646 -1
3.5 -1
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
2.3 -0.876606322217959
2.49093930856486 -1
2.6 -1
2.9 -1
3.2 -1
3.22144190237646 -1
3.5 -0.84638621082865
3.72000373711342 -0.7
3.8 -0.641711415477596
4.1 -0.404345526608789
4.10501592001309 -0.4
4.4 -0.135812879276891
4.43898377022979 -0.1
4.7 0.145098244215751
4.75769869022491 0.2
5 0.433771834246901
5 0.5
5 0.718781653258229
4.77499162397138 0.5
4.7 0.428415036294046
4.45950410227919 0.2
4.4 0.145107797670167
4.13061032164259 -0.1
4.1 -0.126639432867176
3.8 -0.373558856171563
3.76478846401283 -0.4
3.5 -0.578040907147402
3.28534485773516 -0.7
3.2 -0.741759466211297
2.9 -0.816015755131964
2.6 -0.782017191459165
2.46712113343654 -0.7
2.3 -0.5733611358043
2.18672466005726 -0.4
2.01882446784413 -0.1
2 -0.0566081136936593
1.93787037311791 0.2
1.88603035462452 0.5
1.85156677825878 0.8
1.83015684514985 1.1
1.81749107884995 1.4
1.81022983092738 1.7
1.80614568634329 2
1.80389770319941 2.3
1.80263453939948 2.6
1.80194681167739 2.9
1.80156144190886 3.2
1.80135582994015 3.5
1.80142235898569 3.8
1.80136619444825 4.1
1.80145782704239 4.4
1.80147159398273 4.7
1.80148468691085 5
1.7 5
1.66230116329909 5
1.66230102703104 4.7
1.66228278691884 4.4
1.662339829868 4.1
1.66237278821907 3.8
1.66230893236468 3.5
1.66244712499225 3.2
1.66269735859476 2.9
1.66316000414091 2.6
1.66400457550105 2.3
1.66553143728764 2
1.668279336224 1.7
1.67318998455413 1.4
1.68183188918396 1.1
1.69667303955639 0.8
1.7 0.759666457053156
1.733583671273 0.5
1.79171353866958 0.2
1.87141847460038 -0.1
1.97261832831282 -0.4
2 -0.464426934564666
2.16214616384184 -0.7
2.3 -0.876606322217959
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
2.6 -0.782017191459165
2.9 -0.816015755131964
3.2 -0.741759466211297
3.28534485773516 -0.7
3.5 -0.578040907147402
3.76478846401283 -0.4
3.8 -0.373558856171563
4.1 -0.126639432867176
4.13061032164259 -0.1
4.4 0.145107797670167
4.45950410227919 0.2
4.7 0.428415036294046
4.77499162397138 0.5
5 0.718781653258229
5 0.8
5 1.1
5 1.11968863497696
4.98050690110547 1.1
4.7 0.825345552297462
4.67464003342456 0.8
4.4 0.537735161920702
4.36104361919285 0.5
4.1 0.262882008669513
4.03033131572087 0.2
3.8 0.00974135971312276
3.65981627389323 -0.1
3.5 -0.210737779084
3.2 -0.385031383116671
3.14914829896779 -0.4
2.9 -0.457688443544155
2.6 -0.4118806936026
2.58377247216027 -0.4
2.3 -0.137223965904237
2.28070604325565 -0.1
2.16373916541416 0.2
2.07621169449111 0.5
2.01697318897686 0.8
2 0.939176189082983
1.98999214772691 1.1
1.97907916383302 1.4
1.97283615902433 1.7
1.96932741618965 2
1.96744537449077 2.3
1.96635846678938 2.6
1.96577415250964 2.9
1.96543718291206 3.2
1.96526046304986 3.5
1.96520645235983 3.8
1.96514179604744 4.1
1.96554506133065 4.4
1.96551898563348 4.7
1.96555160739988 5
1.80148468691085 5
1.80147159398273 4.7
1.80145782704239 4.4
1.80136619444825 4.1
1.80142235898569 3.8
1.80135582994015 3.5
1.80156144190886 3.2
1.80194681167739 2.9
1.80263453939948 2.6
1.80389770319941 2.3
1.80614568634329 2
1.81022983092738 1.7
1.81749107884995 1.4
1.83015684514985 1.1
1.85156677825878 0.8
1.88603035462452 0.5
1.93787037311791 0.2
2 -0.0566081136936593
2.01882446784413 -0.1
2.18672466005726 -0.4
2.3 -0.5733611358043
2.46712113343654 -0.7
2.6 -0.782017191459165
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
2.6 -0.4118806936026
2.9 -0.457688443544155
3.14914829896779 -0.4
3.2 -0.385031383116671
3.5 -0.210737779084
3.65981627389323 -0.1
3.8 0.00974135971312276
4.03033131572087 0.2
4.1 0.262882008669513
4.36104361919285 0.5
4.4 0.537735161920702
4.67464003342456 0.8
4.7 0.825345552297462
4.98050690110547 1.1
5 1.11968863497696
5 1.4
5 1.7
5 1.97928058138705
4.75794906265337 1.7
4.7 1.63736246061163
4.49652405864205 1.4
4.4 1.29585562950932
4.22804135611424 1.1
4.1 0.966360405481502
3.94200467470086 0.8
3.8 0.664384472796597
3.6162003853074 0.5
3.5 0.40774440528117
3.2 0.215971083545027
3.13874941888128 0.2
2.9 0.150194740691094
2.75190802010795 0.2
2.6 0.278750497892145
2.47599228527857 0.5
2.36622981537367 0.8
2.30014902016927 1.1
2.3 1.10117855464299
2.28215691838711 1.4
2.27186964299571 1.7
2.2660970620186 2
2.26289296180101 2.3
2.26111245610982 2.6
2.26034675958763 2.9
2.25975772419319 3.2
2.25949786184645 3.5
2.2593340740996 3.8
2.25922992854383 4.1
2.26034977478368 4.4
2.26051488636557 4.7
2.26043580610532 5
2 5
1.96555160739988 5
1.96551898563348 4.7
1.96554506133065 4.4
1.96514179604744 4.1
1.96520645235983 3.8
1.96526046304986 3.5
1.96543718291206 3.2
1.96577415250964 2.9
1.96635846678938 2.6
1.96744537449077 2.3
1.96932741618965 2
1.97283615902433 1.7
1.97907916383302 1.4
1.98999214772691 1.1
2 0.939176189082983
2.01697318897686 0.8
2.07621169449111 0.5
2.16373916541416 0.2
2.28070604325565 -0.1
2.3 -0.137223965904237
2.58377247216027 -0.4
2.6 -0.4118806936026
};
\addplot [draw=none, fill=lavender231240249]
table{%
x  y
2.9 0.150194740691094
3.13874941888128 0.2
3.2 0.215971083545027
3.5 0.40774440528117
3.6162003853074 0.5
3.8 0.664384472796597
3.94200467470086 0.8
4.1 0.966360405481502
4.22804135611424 1.1
4.4 1.29585562950932
4.49652405864205 1.4
4.7 1.63736246061163
4.75794906265337 1.7
5 1.97928058138705
5 2
5 2.3
5 2.6
5 2.9
5 3.2
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.1 5
3.8 5
3.5 5
3.2 5
2.9 5
2.6 5
2.3 5
2.26043580610532 5
2.26051488636557 4.7
2.26034977478368 4.4
2.25922992854383 4.1
2.25933407409961 3.8
2.25949786184645 3.5
2.25975772419319 3.2
2.26034675958763 2.9
2.26111245610982 2.6
2.26289296180101 2.3
2.2660970620186 2
2.27186964299571 1.7
2.28215691838711 1.4
2.3 1.10117855464299
2.30014902016927 1.1
2.36622981537367 0.8
2.47599228527857 0.5
2.6 0.278750497892145
2.75190802010795 0.2
2.9 0.150194740691094
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
3.8 5
};
\coordinate (MCMC_mean_lml_t) at (axis cs:3.8,3.2);
\end{axis}



==> fig/tikz/usps/LA_mean_lml.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=black]
table{%
x  y
-0.7 1.9099452743957
-0.4 1.90994576563469
-0.1 1.90997034588468
0.2 1.91057494064351
0.5 1.92008449032342
0.762808216632413 2
0.8 2.0111663787553
0.999422801003941 2.3
1.1 2.45765123198343
1.14104231994138 2.6
1.21874644849234 2.9
1.28624329569137 3.2
1.34493634301256 3.5
1.39620947813599 3.8
1.4 3.82449442033577
1.43504411523782 4.1
1.46872730894041 4.4
1.49859445074182 4.7
1.5252703049149 5
1.4 5
1.1 5
0.8 5
0.5 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.90994530344982
-0.7 1.9099452743957
};
\addplot [draw=none, fill=midnightblue854116]
table{%
x  y
-0.7 1.64693283665046
-0.4 1.64693333620134
-0.1 1.64695886706337
0.2 1.64758749213387
0.5 1.65748168631773
0.635221863532554 1.7
0.8 1.74868614121473
0.977474885046705 2
1.1 2.18142308016761
1.13642489516564 2.3
1.22100655292695 2.6
1.29486660088279 2.9
1.35905538137842 3.2
1.4 3.41757839392962
1.41272888884124 3.5
1.45424995782323 3.8
1.49054054790071 4.1
1.52248999391548 4.4
1.55082802702951 4.7
1.57614553851916 5
1.5252703049149 5
1.49859445074182 4.7
1.46872730894041 4.4
1.43504411523782 4.1
1.4 3.82449442033577
1.39620947813599 3.8
1.34493634301256 3.5
1.28624329569137 3.2
1.21874644849234 2.9
1.14104231994138 2.6
1.1 2.45765123198343
0.999422801003941 2.3
0.8 2.0111663787553
0.762808216632413 2
0.5 1.92008449032342
0.2 1.91057494064351
-0.1 1.90997034588468
-0.4 1.90994576563469
-0.7 1.9099452743957
-1 1.90994530344982
-1 1.7
-1 1.64693281922641
-0.7 1.64693283665046
};
\addplot [draw=none, fill=midnightblue868137]
table{%
x  y
-0.7 1.36273859396608
-0.4 1.36273918651576
-0.1 1.36276748649882
0.2 1.36346403784821
0.5 1.37442199448722
0.573618981734039 1.4
0.8 1.46905069796843
0.958875108361359 1.7
1.1 1.90416470882386
1.13038650431349 2
1.2208265067497 2.3
1.30097078591251 2.6
1.37098675327324 2.9
1.4 3.03964667123947
1.42730638429081 3.2
1.47248355561625 3.5
1.51172677085956 3.8
1.5460369805636 4.1
1.57625267889054 4.4
1.6030616033172 4.7
1.62702077212341 5
1.57614553851916 5
1.55082802702951 4.7
1.52248999391548 4.4
1.49054054790071 4.1
1.45424995782323 3.8
1.41272888884124 3.5
1.4 3.41757839392962
1.35905538137842 3.2
1.29486660088279 2.9
1.22100655292695 2.6
1.13642489516564 2.3
1.1 2.18142308016761
0.977474885046705 2
0.8 1.74868614121473
0.635221863532554 1.7
0.5 1.65748168631773
0.2 1.64758749213387
-0.1 1.64695886706337
-0.4 1.64693333620134
-0.7 1.64693283665046
-1 1.64693281922641
-1 1.4
-1 1.36273863442245
-0.7 1.36273859396608
};
\addplot [draw=none, fill=teal882156]
table{%
x  y
-0.7 1.02466638875948
-0.4 1.02466709280379
-0.1 1.02470065649824
0.2 1.02552700936142
0.5 1.03854600799811
0.646980253945799 1.1
0.8 1.15137045402181
0.955259451329667 1.4
1.1 1.6155426460688
1.12626566342747 1.7
1.21983696076665 2
1.30522811833376 2.3
1.38093501889807 2.6
1.4 2.68343440009747
1.44050653132941 2.9
1.48969712242828 3.2
1.53223822239127 3.5
1.5692035838959 3.8
1.60153341322649 4.1
1.63001536386561 4.4
1.65529517960489 4.7
1.67789600572766 5
1.62702077212341 5
1.6030616033172 4.7
1.57625267889054 4.4
1.5460369805636 4.1
1.51172677085956 3.8
1.47248355561625 3.5
1.42730638429081 3.2
1.4 3.03964667123947
1.37098675327324 2.9
1.30097078591251 2.6
1.2208265067497 2.3
1.13038650431349 2
1.1 1.90416470882386
0.958875108361359 1.7
0.8 1.46905069796843
0.573618981734039 1.4
0.5 1.37442199448722
0.2 1.36346403784821
-0.1 1.36276748649882
-0.4 1.36273918651576
-0.7 1.36273859396608
-1 1.36273863442245
-1 1.1
-1 1.02466637987541
-0.7 1.02466638875948
};
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 0.538707066519745
-0.4 0.538707904469997
-0.1 0.538748470558278
0.2 0.539748422311958
0.5 0.555589993296955
0.8 0.717788024253921
0.830544225083271 0.8
0.982877676005411 1.1
1.1 1.29409441269817
1.12980593425888 1.4
1.22132480946454 1.7
1.30928741721982 2
1.38962972991781 2.3
1.4 2.34167615483649
1.45256426801066 2.6
1.50596112432722 2.9
1.55208786056574 3.2
1.59199288916629 3.5
1.62668039693224 3.8
1.65702984588938 4.1
1.68377804884068 4.4
1.7 4.60301879736349
1.70934287991183 4.7
1.73568666143989 5
1.7 5
1.67789600572766 5
1.65529517960489 4.7
1.63001536386561 4.4
1.60153341322649 4.1
1.5692035838959 3.8
1.53223822239127 3.5
1.48969712242828 3.2
1.44050653132941 2.9
1.4 2.68343440009747
1.38093501889807 2.6
1.30522811833376 2.3
1.21983696076665 2
1.12626566342747 1.7
1.1 1.6155426460688
0.955259451329667 1.4
0.8 1.15137045402181
0.646980253945799 1.1
0.5 1.03854600799811
0.2 1.02552700936142
-0.1 1.02470065649824
-0.4 1.02466709280379
-0.7 1.02466638875948
-1 1.02466637987541
-1 0.8
-1 0.538707010498004
-0.7 0.538707066519745
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.7 -1
-0.4 -1
-0.1 -1
0.2 -1
0.5 -1
0.8 -1
1.1 -1
1.1002828701077 -1
1.1 -0.998520023701796
0.979241511910188 -0.7
0.917112092051018 -0.4
0.895374820960183 -0.1
0.909754424719305 0.2
0.963941276875476 0.5
1.06167136127567 0.8
1.1 0.879538470274868
1.14936660463431 1.1
1.23089924122594 1.4
1.31638395550161 1.7
1.39873787367299 2
1.4 2.00474947992296
1.46416442081098 2.3
1.52158418605418 2.6
1.57141571732503 2.9
1.6144785987032 3.2
1.6517475559413 3.5
1.68415720996858 3.8
1.7 3.9649370496248
1.71555731035033 4.1
1.74660695649148 4.4
1.77416262404807 4.7
1.79879020787963 5
1.73568666143989 5
1.70934287991183 4.7
1.7 4.60301879736349
1.68377804884068 4.4
1.65702984588938 4.1
1.62668039693224 3.8
1.59199288916629 3.5
1.55208786056574 3.2
1.50596112432722 2.9
1.45256426801066 2.6
1.4 2.34167615483649
1.38962972991781 2.3
1.30928741721982 2
1.22132480946454 1.7
1.12980593425888 1.4
1.1 1.29409441269817
0.982877676005411 1.1
0.830544225083271 0.8
0.8 0.717788024253921
0.5 0.555589993296955
0.2 0.539748422311958
-0.1 0.538748470558278
-0.4 0.538707904469997
-0.7 0.538707066519745
-1 0.538707010498004
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
1.1 -0.998520023701796
1.1002828701077 -1
1.4 -1
1.40777329110599 -1
1.4 -0.976622193355596
1.2851033944728 -0.7
1.20686172360395 -0.4
1.16171494121242 -0.1
1.14469579023708 0.2
1.15604726106557 0.5
1.19512460581442 0.8
1.25676683642829 1.1
1.331992548193 1.4
1.4 1.65446513699343
1.41001346099465 1.7
1.47678732534694 2
1.53731695881635 2.3
1.5906041040977 2.6
1.63687031032284 2.9
1.67686933684067 3.2
1.7 3.39747121956668
1.71429309791287 3.5
1.7517241347109 3.8
1.78448242826701 4.1
1.81335352388136 4.4
1.8389823681843 4.7
1.86189375431937 5
1.79879020787963 5
1.77416262404807 4.7
1.74660695649148 4.4
1.71555731035033 4.1
1.7 3.9649370496248
1.68415720996858 3.8
1.6517475559413 3.5
1.6144785987032 3.2
1.57141571732503 2.9
1.52158418605418 2.6
1.46416442081098 2.3
1.4 2.00474947992296
1.39873787367299 2
1.31638395550161 1.7
1.23089924122594 1.4
1.14936660463431 1.1
1.1 0.879538470274868
1.06167136127567 0.8
0.963941276875476 0.5
0.909754424719305 0.2
0.895374820960183 -0.1
0.917112092051018 -0.4
0.979241511910188 -0.7
1.1 -0.998520023701796
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
5 -1
5 -0.944103564336623
4.94075384517856 -1
5 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
1.4 -0.976622193355596
1.40777329110599 -1
1.58896944803384 -1
1.47261266921222 -0.7
1.4 -0.446865937855011
1.38386435425266 -0.4
1.31041494846389 -0.1
1.27681044661241 0.2
1.27772443382612 0.5
1.30916013001221 0.8
1.36416706822226 1.1
1.4 1.25144318643381
1.42908969976283 1.4
1.49319642042311 1.7
1.55467360907944 2
1.61046949682171 2.3
1.65962402214121 2.6
1.7 2.88282734095797
1.70288996075553 2.9
1.74879437966968 3.2
1.78854651171214 3.5
1.82313060004079 3.8
1.85340754618369 4.1
1.88010009127124 4.4
1.90380211232054 4.7
1.92499730075911 5
1.86189375431937 5
1.8389823681843 4.7
1.81335352388136 4.4
1.78448242826701 4.1
1.7517241347109 3.8
1.71429309791287 3.5
1.7 3.39747121956669
1.67686933684067 3.2
1.63687031032284 2.9
1.5906041040977 2.6
1.53731695881635 2.3
1.47678732534694 2
1.41001346099465 1.7
1.4 1.65446513699343
1.331992548193 1.4
1.25676683642829 1.1
1.19512460581442 0.8
1.15604726106557 0.5
1.14469579023708 0.2
1.16171494121242 -0.1
1.20686172360395 -0.4
1.2851033944728 -0.7
1.4 -0.976622193355596
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
4.7 -1
4.94075384517856 -1
5 -0.944103564336623
5 -0.7
5 -0.580079191445522
4.87319641010789 -0.7
4.7 -0.866012402069831
4.55231285200284 -1
4.7 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
1.7 -1
1.76506722423223 -1
1.7 -0.874967910256895
1.62008566267842 -0.7
1.51662784623441 -0.4
1.44666390448003 -0.1
1.40747137490177 0.2
1.4 0.479642753845836
1.39940160658667 0.5
1.4 0.507082021806187
1.42038660878701 0.8
1.4630936967474 1.1
1.51797281713965 1.4
1.57637937985157 1.7
1.63255989281194 2
1.68362203482708 2.3
1.7 2.40512851355508
1.73561409579491 2.6
1.78425300211434 2.9
1.82633670138574 3.2
1.86279992551141 3.5
1.89453706537068 3.8
1.92233266410037 4.1
1.94684665866111 4.4
1.96862185645677 4.7
1.98810084719885 5
1.92499730075911 5
1.90380211232054 4.7
1.88010009127124 4.4
1.85340754618369 4.1
1.82313060004079 3.8
1.78854651171214 3.5
1.74879437966968 3.2
1.70288996075553 2.9
1.7 2.88282734095797
1.65962402214121 2.6
1.61046949682171 2.3
1.55467360907944 2
1.49319642042311 1.7
1.42908969976283 1.4
1.4 1.25144318643381
1.36416706822226 1.1
1.30916013001221 0.8
1.27772443382612 0.5
1.27681044661241 0.2
1.31041494846389 -0.1
1.38386435425266 -0.4
1.4 -0.446865937855011
1.47261266921222 -0.7
1.58896944803384 -1
1.7 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
4.4 -1
4.55231285200284 -1
4.7 -0.866012402069831
4.87319641010789 -0.7
5 -0.580079191445522
5 -0.4
5 -0.305805302911686
4.90078235112167 -0.4
4.7 -0.591913287332151
4.58165418323 -0.7
4.4 -0.867957226945939
4.24583548290512 -1
4.4 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
1.7 -0.874967910256896
1.76506722423223 -1
1.93309728652956 -1
1.76869997265298 -0.7
1.7 -0.545070069286251
1.64495396363531 -0.4
1.56404406404531 -0.1
1.51806708782016 0.2
1.50484752220051 0.5
1.52061217684361 0.8
1.55777768865253 1.1
1.60685593451647 1.4
1.65956233928003 1.7
1.7 1.93512896180884
1.71300567742466 2
1.77062261067235 2.3
1.82142917420613 2.6
1.86561604347315 2.9
1.90387902310181 3.2
1.93705333931068 3.5
1.96594353070058 3.8
1.99125778201705 4.1
2 4.21513464714217
2.02047335128557 4.4
2.05032430288969 4.7
2.07698169754867 5
2 5
1.98810084719885 5
1.96862185645677 4.7
1.94684665866111 4.4
1.92233266410037 4.1
1.89453706537068 3.8
1.86279992551141 3.5
1.82633670138574 3.2
1.78425300211434 2.9
1.73561409579491 2.6
1.7 2.40512851355508
1.68362203482708 2.3
1.63255989281194 2
1.57637937985157 1.7
1.51797281713965 1.4
1.4630936967474 1.1
1.42038660878701 0.8
1.4 0.507082021806187
1.39940160658667 0.5
1.4 0.479642753845836
1.40747137490177 0.2
1.44666390448003 -0.1
1.51662784623441 -0.4
1.62008566267842 -0.7
1.7 -0.874967910256896
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
4.1 -1
4.24583548290512 -1
4.4 -0.867957226945939
4.58165418323 -0.7
4.7 -0.591913287332151
4.90078235112167 -0.4
5 -0.305805302911686
5 -0.1
5 -0.0692414828324971
4.96774342272137 -0.1
4.7 -0.355455606797475
4.65158040709704 -0.4
4.4 -0.631904381172185
4.3214041203522 -0.7
4.1 -0.892927992188526
3.96330529726746 -1
4.1 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
2 -1
2.13338262577617 -1
2 -0.842203228662049
1.91866433246043 -0.7
1.78061915565792 -0.4
1.7 -0.16509805411487
1.68142422361059 -0.1
1.62866280073855 0.2
1.61021321998081 0.5
1.62083774490022 0.8
1.65246168055766 1.1
1.69573905189329 1.4
1.7 1.42559876640923
1.75329772611458 1.7
1.80997549960999 2
1.86161797978757 2.3
1.90724425261734 2.6
1.94697908483195 2.9
1.98142134481787 3.2
2 3.38342514548732
2.01706662290449 3.5
2.05633877950078 3.8
2.09071526328648 4.1
2.12100327083172 4.4
2.147867733207 4.7
2.17185281662802 5
2.07698169754867 5
2.05032430288969 4.7
2.02047335128557 4.4
2 4.21513464714217
1.99125778201705 4.1
1.96594353070058 3.8
1.93705333931068 3.5
1.90387902310181 3.2
1.86561604347315 2.9
1.82142917420613 2.6
1.77062261067235 2.3
1.71300567742466 2
1.7 1.93512896180884
1.65956233928003 1.7
1.60685593451647 1.4
1.55777768865253 1.1
1.52061217684361 0.8
1.50484752220051 0.5
1.51806708782016 0.2
1.56404406404531 -0.1
1.64495396363531 -0.4
1.7 -0.545070069286251
1.76869997265298 -0.7
1.93309728652956 -1
2 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
3.8 -1
3.96330529726746 -1
4.1 -0.892927992188526
4.3214041203522 -0.7
4.4 -0.631904381172185
4.65158040709704 -0.4
4.7 -0.355455606797475
4.96774342272137 -0.1
5 -0.0692414828324971
5 0.147980113739765
4.73994228464103 -0.1
4.7 -0.138109173536898
4.41532562707256 -0.4
4.4 -0.414127014513364
4.1 -0.674446995875874
4.06791153150096 -0.7
3.8 -0.911551625717313
3.66891311005595 -1
3.8 -1
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
2 -0.842203228662049
2.13338262577617 -1
2.3 -1
2.4046603573163 -1
2.3 -0.938447646765282
2.09674216769264 -0.7
2 -0.564279328955138
1.92179726418931 -0.4
1.81536775735334 -0.1
1.74766342770432 0.2
1.71931544593689 0.5
1.72632935244938 0.8
1.75899708278276 1.1
1.80572235668972 1.4
1.85701585940575 1.7
1.90694532179532 2
1.95261334890279 2.3
1.99305933102856 2.6
2 2.65652988856365
2.04284634739002 2.9
2.0890631507934 3.2
2.12914610322565 3.5
2.16404837877004 3.8
2.19460790099168 4.1
2.22153319037787 4.4
2.24541116352432 4.7
2.26672393570737 5
2.17185281662802 5
2.147867733207 4.7
2.12100327083172 4.4
2.09071526328648 4.1
2.05633877950078 3.8
2.01706662290449 3.5
2 3.38342514548732
1.98142134481787 3.2
1.94697908483195 2.9
1.90724425261734 2.6
1.86161797978757 2.3
1.80997549960999 2
1.75329772611458 1.7
1.7 1.42559876640923
1.69573905189329 1.4
1.65246168055766 1.1
1.62083774490022 0.8
1.61021321998081 0.5
1.62866280073855 0.2
1.68142422361059 -0.1
1.7 -0.16509805411487
1.78061915565792 -0.4
1.91866433246043 -0.7
2 -0.842203228662049
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
3.5 -1
3.66891311005595 -1
3.8 -0.911551625717313
4.06791153150096 -0.7
4.1 -0.674446995875874
4.4 -0.414127014513364
4.41532562707256 -0.4
4.7 -0.138109173536898
4.73994228464103 -0.1
5 0.147980113739765
5 0.2
5 0.366351033312422
4.82632535408042 0.2
4.7 0.0795552341706382
4.50620565344443 -0.1
4.4 -0.19774721569219
4.16911246586494 -0.4
4.1 -0.460021273745322
3.8 -0.698867838033142
3.79835614856065 -0.7
3.5 -0.898985424096849
3.30223556991897 -1
3.5 -1
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
2.3 -0.938447646765282
2.4046603573163 -1
2.6 -1
2.9 -1
3.2 -1
3.30223556991897 -1
3.5 -0.898985424096849
3.79835614856065 -0.7
3.8 -0.698867838033142
4.1 -0.460021273745322
4.16911246586494 -0.4
4.4 -0.19774721569219
4.50620565344443 -0.1
4.7 0.0795552341706382
4.82632535408042 0.2
5 0.366351033312422
5 0.5
5 0.593725972869883
4.90259460171272 0.5
4.7 0.306735305178195
4.58559379553849 0.2
4.4 0.0291669208912607
4.25404558096357 -0.1
4.1 -0.233638013702543
3.89414514703706 -0.4
3.8 -0.474040439803104
3.5 -0.679008833158112
3.45965295129513 -0.7
3.2 -0.826423493076494
2.9 -0.901119892512741
2.6 -0.86858636188448
2.31588540559308 -0.7
2.3 -0.68869040906624
2.09365744598458 -0.4
2 -0.231286418157099
1.95242529803673 -0.1
1.88193674261269 0.2
1.84995259739278 0.5
1.85161231772704 0.8
1.87748259835235 1.1
1.91676811124857 1.4
1.96073399269691 1.7
2 1.97108912816827
2.00595519189574 2
2.06613133003351 2.3
2.11938237193508 2.6
2.16584732167489 2.9
2.20618889784804 3.2
2.24122558354681 3.5
2.27175797803931 3.8
2.29850053869688 4.1
2.3 4.11851142566509
2.3363555636133 4.4
2.37083720128334 4.7
2.40167585197744 5
2.3 5
2.26672393570737 5
2.24541116352432 4.7
2.22153319037787 4.4
2.19460790099168 4.1
2.16404837877004 3.8
2.12914610322565 3.5
2.0890631507934 3.2
2.04284634739002 2.9
2 2.65652988856365
1.99305933102856 2.6
1.95261334890279 2.3
1.90694532179532 2
1.85701585940575 1.7
1.80572235668972 1.4
1.75899708278276 1.1
1.72632935244938 0.8
1.71931544593689 0.5
1.74766342770432 0.2
1.81536775735334 -0.1
1.92179726418931 -0.4
2 -0.564279328955138
2.09674216769264 -0.7
2.3 -0.938447646765282
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
2.6 -0.86858636188448
2.9 -0.901119892512741
3.2 -0.826423493076494
3.45965295129513 -0.7
3.5 -0.679008833158112
3.8 -0.474040439803104
3.89414514703706 -0.4
4.1 -0.233638013702543
4.25404558096357 -0.1
4.4 0.0291669208912607
4.58559379553849 0.2
4.7 0.306735305178195
4.90259460171272 0.5
5 0.593725972869883
5 0.8
5 0.841057233343683
4.95755091238139 0.8
4.7 0.553832406401999
4.64271845137813 0.5
4.4 0.27613196105923
4.31482998892758 0.2
4.1 0.0133639252056114
3.96156496404961 -0.1
3.8 -0.22694733570443
3.55287306869611 -0.4
3.5 -0.435011736106588
3.2 -0.581077317322744
2.9 -0.65495787611294
2.6 -0.608236459165252
2.30714225318556 -0.4
2.3 -0.393399932432661
2.13802764264767 -0.1
2.02547030329444 0.2
2 0.334483958421221
1.98058974884868 0.5
1.9768952830047 0.8
1.99596811392195 1.1
2 1.13588236024089
2.04280275255316 1.4
2.09850251620024 1.7
2.15345267910544 2
2.20412311378637 2.3
2.2492699702232 2.6
2.28884829595976 2.9
2.3 2.9938804908696
2.3383325276985 3.2
2.38767537757286 3.5
2.43077801061166 3.8
2.46860867656122 4.1
2.50200863327052 4.4
2.53169784479751 4.7
2.55828098681898 5
2.40167585197744 5
2.37083720128334 4.7
2.3363555636133 4.4
2.3 4.11851142566509
2.29850053869688 4.1
2.27175797803931 3.8
2.24122558354681 3.5
2.20618889784804 3.2
2.16584732167489 2.9
2.11938237193508 2.6
2.06613133003351 2.3
2.00595519189574 2
2 1.97108912816828
1.96073399269691 1.7
1.91676811124857 1.4
1.87748259835235 1.1
1.85161231772704 0.8
1.84995259739278 0.5
1.88193674261269 0.2
1.95242529803673 -0.1
2 -0.231286418157099
2.09365744598458 -0.4
2.3 -0.68869040906624
2.31588540559308 -0.7
2.6 -0.86858636188448
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
2.6 -0.608236459165252
2.9 -0.65495787611294
3.2 -0.581077317322744
3.5 -0.435011736106588
3.55287306869611 -0.4
3.8 -0.22694733570443
3.96156496404961 -0.1
4.1 0.0133639252056113
4.31482998892758 0.2
4.4 0.27613196105923
4.64271845137813 0.5
4.7 0.553832406401999
4.95755091238139 0.8
5 0.841057233343683
5 1.1
5 1.13301860054512
4.96609276809079 1.1
4.7 0.844680300693975
4.65287805661079 0.8
4.4 0.565712288607773
4.32728922491648 0.5
4.1 0.301679392060395
3.97737193433032 0.2
3.8 0.0603275732523929
3.57388388414836 -0.1
3.5 -0.148701815338422
3.2 -0.293782311656249
2.9 -0.361082397011265
2.6 -0.287629916556106
2.39695051671505 -0.1
2.3 0.0311153788052535
2.23644932361097 0.2
2.17535650621613 0.5
2.16013878155694 0.8
2.17770978277673 1.1
2.21369104213396 1.4
2.25701547365739 1.7
2.3 1.99303866460819
2.30157472377797 2
2.36945087188054 2.3
2.43024472041654 2.6
2.48389197284029 2.9
2.53090359030401 3.2
2.57202204264143 3.5
2.6 3.73101515499779
2.6130433052328 3.8
2.66450356637686 4.1
2.71005608904725 4.4
2.75057680589428 4.7
2.78677931450747 5
2.6 5
2.55828098681898 5
2.53169784479751 4.7
2.50200863327052 4.4
2.46860867656122 4.1
2.43077801061166 3.8
2.38767537757286 3.5
2.3383325276985 3.2
2.3 2.9938804908696
2.28884829595976 2.9
2.2492699702232 2.6
2.20412311378637 2.3
2.15345267910544 2
2.09850251620024 1.7
2.04280275255316 1.4
2 1.13588236024089
1.99596811392195 1.1
1.9768952830047 0.8
1.98058974884868 0.5
2 0.334483958421221
2.02547030329444 0.2
2.13802764264767 -0.1
2.3 -0.393399932432661
2.30714225318556 -0.4
2.6 -0.608236459165252
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
2.6 -0.287629916556106
2.9 -0.361082397011265
3.2 -0.293782311656249
3.5 -0.148701815338422
3.57388388414836 -0.1
3.8 0.0603275732523929
3.97737193433032 0.2
4.1 0.301679392060395
4.32728922491648 0.5
4.4 0.565712288607773
4.65287805661079 0.8
4.7 0.844680300693975
4.96609276809079 1.1
5 1.13301860054512
5 1.4
5 1.51871538047328
4.87933796188986 1.4
4.7 1.22671525988347
4.56803239356514 1.1
4.4 0.943038688852471
4.24389055489723 0.8
4.1 0.673413962797598
3.89345110256799 0.5
3.8 0.426027452091092
3.5 0.21443637445166
3.47110405458368 0.2
3.2 0.0809572661153652
2.9 0.0408077394121196
2.6 0.176516227526675
2.58248299064235 0.2
2.45067107828794 0.5
2.40105930762139 0.8
2.40707556383453 1.1
2.44357704471582 1.4
2.4932056304869 1.7
2.54602434970019 2
2.59701048270614 2.3
2.6 2.31801017779098
2.67170608364024 2.6
2.73989291058924 2.9
2.80029074577312 3.2
2.85368817185244 3.5
2.9 3.7944160142178
2.90126678200604 3.8
2.96354769820532 4.1
3.01837298254747 4.4
3.06684216589967 4.7
3.10990591026953 5
2.9 5
2.78677931450747 5
2.75057680589428 4.7
2.71005608904725 4.4
2.66450356637686 4.1
2.61304330523279 3.8
2.6 3.73101515499779
2.57202204264143 3.5
2.53090359030401 3.2
2.48389197284029 2.9
2.43024472041654 2.6
2.36945087188054 2.3
2.30157472377797 2
2.3 1.99303866460819
2.25701547365739 1.7
2.21369104213396 1.4
2.17770978277673 1.1
2.16013878155694 0.8
2.17535650621613 0.5
2.23644932361097 0.2
2.3 0.0311153788052535
2.39695051671505 -0.1
2.6 -0.287629916556106
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
2.6 0.176516227526675
2.9 0.0408077394121196
3.2 0.0809572661153652
3.47110405458368 0.2
3.5 0.21443637445166
3.8 0.426027452091092
3.89345110256799 0.5
4.1 0.673413962797598
4.24389055489723 0.8
4.4 0.943038688852471
4.56803239356514 1.1
4.7 1.22671525988347
4.87933796188986 1.4
5 1.51871538047328
5 1.7
5 2
5 2.13004826916013
4.87391546465763 2
4.7 1.82585978221997
4.57549341159389 1.7
4.4 1.52941236615156
4.26507551131274 1.4
4.1 1.24941374064615
3.9259876848315 1.1
3.8 0.998603134814834
3.51342583057886 0.8
3.5 0.791486609180668
3.2 0.704010506655856
2.9402656298958 0.8
2.9 0.841941397541882
2.83816516985402 1.1
2.83765791861314 1.4
2.87088130349083 1.7
2.9 1.87763870659192
2.93019763292012 2
3.01143309201755 2.3
3.08794273344486 2.6
3.15850077349125 2.9
3.2 3.08941582461206
3.23467271232177 3.2
3.32141988326126 3.5
3.39873587672385 3.8
3.46861328223013 4.1
3.5 4.24563475664498
3.55521462499204 4.4
3.65564746148915 4.7
3.74901871500001 5
3.5 5
3.2 5
3.10990591026953 5
3.06684216589967 4.7
3.01837298254747 4.4
2.96354769820532 4.1
2.90126678200604 3.8
2.9 3.7944160142178
2.85368817185244 3.5
2.80029074577312 3.2
2.73989291058924 2.9
2.67170608364024 2.6
2.6 2.31801017779098
2.59701048270614 2.3
2.54602434970019 2
2.4932056304869 1.7
2.44357704471582 1.4
2.40707556383453 1.1
2.40105930762139 0.8
2.45067107828794 0.5
2.58248299064235 0.2
2.6 0.176516227526675
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
3.2 0.704010506655856
3.5 0.791486609180668
3.51342583057886 0.8
3.8 0.998603134814834
3.9259876848315 1.1
4.1 1.24941374064615
4.26507551131274 1.4
4.4 1.52941236615156
4.57549341159389 1.7
4.7 1.82585978221997
4.87391546465763 2
5 2.13004826916013
5 2.3
5 2.6
5 2.9
5 3.2
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.1 5
3.8 5
3.74901871500001 5
3.65564746148915 4.7
3.55521462499204 4.4
3.5 4.24563475664498
3.46861328223013 4.1
3.39873587672385 3.8
3.32141988326126 3.5
3.23467271232177 3.2
3.2 3.08941582461206
3.15850077349125 2.9
3.08794273344486 2.6
3.01143309201755 2.3
2.93019763292012 2
2.9 1.87763870659192
2.87088130349083 1.7
2.83765791861314 1.4
2.83816516985402 1.1
2.9 0.841941397541882
2.9402656298958 0.8
3.2 0.704010506655856
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
4.1 2.6
};
\coordinate (LA_mean_lml_t) at (axis cs:4.1,2.5999999999999996);
\end{axis}



==> fig/tikz/usps/LA_nlpd.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.7 -1
-0.4 -1
-0.1 -1
0.2 -1
0.5 -1
0.8 -1
0.928355624040564 -1
0.864298486099111 -0.7
0.826187011230425 -0.4
0.802793088201124 -0.1
0.8 -0.0451642031257042
0.751213013695476 0.2
0.72582242980784 0.5
0.724819859836294 0.8
0.742526703939462 1.1
0.77710464399804 1.4
0.8 1.54323325173203
0.807641169336536 1.7
0.826609728300804 2
0.852069137073629 2.3
0.885693878271613 2.6
0.929814746795914 2.9
0.987578277604385 3.2
1.06317559629843 3.5
1.1 3.62946474218256
1.13625158944751 3.8
1.21199994736423 4.1
1.31152522346452 4.4
1.4 4.61902837534475
1.43708381029482 4.7
1.5875601483439 5
1.4 5
1.1 5
0.8 5
0.5 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
1.1 -1
1.22079985420754 -1
1.14784803362133 -0.7
1.1 -0.424374690102979
1.09183402620712 -0.4
1.01818780568283 -0.1
0.980927570989134 0.2
0.968193538715652 0.5
0.97416088715999 0.8
0.996288158837534 1.1
1.03422469981735 1.4
1.08940557053913 1.7
1.1 1.74914532848495
1.13819457289541 2
1.19710915550836 2.3
1.27448008681921 2.6
1.37580806062126 2.9
1.4 2.96595568682477
1.49580461302616 3.2
1.64819868423378 3.5
1.7 3.59306132919117
1.83804912925631 3.8
2 4.01679687821221
2.0664809453844 4.1
2.3 4.37610372992196
2.31853060204172 4.4
2.55624609161681 4.7
2.6 4.75305823488113
2.77473711352477 5
2.6 5
2.3 5
2 5
1.7 5
1.5875601483439 5
1.43708381029482 4.7
1.4 4.61902837534475
1.31152522346452 4.4
1.21199994736423 4.1
1.13625158944751 3.8
1.1 3.62946474218256
1.06317559629843 3.5
0.987578277604385 3.2
0.929814746795914 2.9
0.885693878271613 2.6
0.852069137073629 2.3
0.826609728300804 2
0.807641169336536 1.7
0.8 1.54323325173203
0.77710464399804 1.4
0.742526703939462 1.1
0.724819859836294 0.8
0.72582242980784 0.5
0.751213013695476 0.2
0.8 -0.0451642031257042
0.802793088201124 -0.1
0.826187011230425 -0.4
0.864298486099111 -0.7
0.928355624040564 -1
1.1 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
1.28549956924224 -0.7
1.21283193357432 -0.4
1.16595746873926 -0.1
1.13933324349618 0.2
1.13091312788375 0.5
1.13931480820074 0.8
1.1634494446059 1.1
1.20322743503535 1.4
1.26009125511241 1.7
1.33720244491082 2
1.4 2.19774475604229
1.43585908254005 2.3
1.55618430489447 2.6
1.7 2.88125714876753
1.71163267435499 2.9
1.90618823776391 3.2
2 3.32960558955944
2.13368560527115 3.5
2.3 3.6996802644495
2.37757468599152 3.8
2.6 4.07220567286931
2.619757077195 4.1
2.83703589829207 4.4
2.9 4.48225095324357
3.04178094222899 4.7
3.2 4.92110939426989
3.24768105281038 5
3.2 5
2.9 5
2.77473711352477 5
2.6 4.75305823488113
2.55624609161681 4.7
2.31853060204172 4.4
2.3 4.37610372992196
2.0664809453844 4.1
2 4.01679687821221
1.83804912925631 3.8
1.7 3.59306132919117
1.64819868423378 3.5
1.49580461302616 3.2
1.4 2.96595568682477
1.37580806062126 2.9
1.27448008681921 2.6
1.19710915550836 2.3
1.13819457289541 2
1.1 1.74914532848495
1.08940557053913 1.7
1.03422469981735 1.4
0.996288158837534 1.1
0.97416088715999 0.8
0.968193538715652 0.5
0.980927570989134 0.2
1.01818780568283 -0.1
1.09183402620712 -0.4
1.1 -0.424374690102979
1.14784803362133 -0.7
1.22079985420754 -1
1.39832400982989 -1
1.28549956924224 -0.7
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
5 -1
5 -0.999758066274195
4.99974346743378 -1
5 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
1.4 -1
1.51639486595695 -1
1.41767357484852 -0.7
1.4 -0.634980856322914
1.32924231552034 -0.4
1.27231038084439 -0.1
1.24283287189512 0.2
1.23681580060813 0.5
1.25223500139886 0.8
1.2882031104484 1.1
1.34538720081092 1.4
1.4 1.61220916182638
1.42476520410174 1.7
1.52527934829409 2
1.65561778404423 2.3
1.7 2.39087762501035
1.82483521198722 2.6
2 2.85477070550024
2.03442536744679 2.9
2.27362499036362 3.2
2.3 3.2320154547219
2.50674495681855 3.5
2.6 3.61470794688845
2.73204587649205 3.8
2.9 4.02109553524462
2.95190557462607 4.1
3.15807858637235 4.4
3.2 4.458791703843
3.34700597969179 4.7
3.5 4.92809959944986
3.54180147465205 5
3.5 5
3.24768105281038 5
3.2 4.92110939426989
3.04178094222899 4.7
2.9 4.48225095324357
2.83703589829207 4.4
2.619757077195 4.1
2.6 4.07220567286931
2.37757468599152 3.8
2.3 3.6996802644495
2.13368560527115 3.5
2 3.32960558955944
1.90618823776391 3.2
1.71163267435499 2.9
1.7 2.88125714876753
1.55618430489447 2.6
1.43585908254005 2.3
1.4 2.19774475604229
1.33720244491082 2
1.26009125511241 1.7
1.20322743503535 1.4
1.1634494446059 1.1
1.13931480820074 0.8
1.13091312788375 0.5
1.13933324349618 0.2
1.16595746873926 -0.1
1.21283193357432 -0.4
1.28549956924224 -0.7
1.39832400982989 -1
1.4 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
5 -0.999758066274195
5 -0.759020413561074
4.74447914811746 -1
4.99974346743378 -1
5 -0.999758066274195
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
1.52275688435749 -0.7
1.43936338998557 -0.4
1.4 -0.201530581908259
1.37866329294952 -0.1
1.34633250029405 0.2
1.3427184733325 0.5
1.36515519459699 0.8
1.4 1.02445489951407
1.41268922661139 1.1
1.48380202448812 1.4
1.58059091197356 1.7
1.7 1.98320740016521
1.70884317734798 2
1.88020489037562 2.3
2 2.48118434559917
2.08831055631625 2.6
2.3 2.86591035117268
2.32606251539268 2.9
2.56073771407419 3.2
2.6 3.24862618932621
2.77967737653456 3.5
2.9 3.6592736058766
2.99320027654859 3.8
3.2 4.09324869308828
3.20420341993212 4.1
3.38943433350997 4.4
3.5 4.5656787496021
3.57896683496917 4.7
3.76563406985666 5
3.54180147465205 5
3.5 4.92809959944986
3.34700597969179 4.7
3.2 4.458791703843
3.15807858637235 4.4
2.95190557462607 4.1
2.9 4.02109553524462
2.73204587649205 3.8
2.6 3.61470794688845
2.50674495681855 3.5
2.3 3.2320154547219
2.27362499036362 3.2
2.03442536744679 2.9
2 2.85477070550024
1.82483521198722 2.6
1.7 2.39087762501035
1.65561778404423 2.3
1.52527934829409 2
1.42476520410174 1.7
1.4 1.61220916182638
1.34538720081092 1.4
1.2882031104484 1.1
1.25223500139886 0.8
1.23681580060813 0.5
1.24283287189512 0.2
1.27231038084439 -0.1
1.32924231552034 -0.4
1.4 -0.634980856322914
1.41767357484852 -0.7
1.51639486595695 -1
1.63389907900713 -1
1.52275688435749 -0.7
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
4.7 -1
4.74447914811746 -1
5 -0.759020413561074
5 -0.7
5 -0.552826025156504
4.84478967104531 -0.7
4.7 -0.838078085915137
4.52276378423776 -1
4.7 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.7 -1
1.75586639707994 -1
1.7 -0.883256079951101
1.62784019386646 -0.7
1.53973658844308 -0.4
1.48004066312595 -0.1
1.44930315624472 0.2
1.44888604621539 0.5
1.47794592262832 0.8
1.53486680388331 1.1
1.61988071044668 1.4
1.7 1.61475669871253
1.74038154643944 1.7
1.90346732339711 2
2 2.15411875922358
2.1048118633439 2.3
2.3 2.55211622450055
2.33627014274754 2.6
2.56983892270951 2.9
2.6 2.93771031633473
2.78807081896415 3.2
2.9 3.34925689774303
3.00064573472281 3.5
3.2 3.78509203974676
3.20940621849063 3.8
3.39711794945907 4.1
3.5 4.25523669029081
3.5862773139788 4.4
3.77273304920118 4.7
3.8 4.74276420824392
3.9485533924981 5
3.8 5
3.76563406985666 5
3.57896683496917 4.7
3.5 4.5656787496021
3.38943433350997 4.4
3.20420341993212 4.1
3.2 4.09324869308828
2.99320027654859 3.8
2.9 3.6592736058766
2.77967737653456 3.5
2.6 3.24862618932621
2.56073771407419 3.2
2.32606251539268 2.9
2.3 2.86591035117268
2.08831055631625 2.6
2 2.48118434559917
1.88020489037562 2.3
1.70884317734798 2
1.7 1.98320740016521
1.58059091197356 1.7
1.48380202448812 1.4
1.41268922661139 1.1
1.4 1.02445489951407
1.36515519459699 0.8
1.3427184733325 0.5
1.34633250029405 0.2
1.37866329294952 -0.1
1.4 -0.201530581908259
1.43936338998557 -0.4
1.52275688435749 -0.7
1.63389907900713 -1
1.7 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
4.4 -1
4.52276378423776 -1
4.7 -0.838078085915137
4.84478967104531 -0.7
5 -0.552826025156504
5 -0.4
5 -0.360694235114307
4.95878595735359 -0.4
4.7 -0.646315333588922
4.64177915901591 -0.7
4.4 -0.922485814512404
4.31101160925611 -1
4.4 -1
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.7 -0.883256079951101
1.75586639707994 -1
1.88357294586497 -1
1.73987139236062 -0.7
1.7 -0.596709631019494
1.64010978690058 -0.4
1.58016931042088 -0.1
1.55170412694501 0.2
1.55536570317537 0.5
1.59067887075397 0.8
1.65704438115522 1.1
1.7 1.23827140404518
1.76520698218065 1.4
1.91317306541083 1.7
2 1.84977507082873
2.10262820626328 2
2.3 2.26556325624276
2.32566967753338 2.3
2.55469251758534 2.6
2.6 2.65742255143861
2.77440036213646 2.9
2.9 3.06920064827456
2.98813980886284 3.2
3.19522394977942 3.5
3.2 3.5068301217304
3.38497634035994 3.8
3.5 3.97519711079049
3.5756206126646 4.1
3.75976066946774 4.4
3.8 4.46376737580613
3.93855847868702 4.7
4.1 4.96387881519334
4.12131338433914 5
4.1 5
3.9485533924981 5
3.8 4.74276420824392
3.77273304920117 4.7
3.5862773139788 4.4
3.5 4.25523669029081
3.39711794945907 4.1
3.20940621849063 3.8
3.2 3.78509203974676
3.00064573472281 3.5
2.9 3.34925689774303
2.78807081896415 3.2
2.6 2.93771031633473
2.56983892270951 2.9
2.33627014274754 2.6
2.3 2.55211622450055
2.1048118633439 2.3
2 2.15411875922358
1.90346732339711 2
1.74038154643944 1.7
1.7 1.61475669871253
1.61988071044668 1.4
1.53486680388331 1.1
1.47794592262832 0.8
1.44888604621539 0.5
1.44930315624472 0.2
1.48004066312595 -0.1
1.53973658844308 -0.4
1.62784019386646 -0.7
1.7 -0.883256079951101
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
4.4 -0.922485814512404
4.64177915901591 -0.7
4.7 -0.646315333588922
4.95878595735359 -0.4
5 -0.360694235114307
5 -0.178871481853743
4.76813578863762 -0.4
4.7 -0.464852396471763
4.44498321125857 -0.7
4.4 -0.741393668656062
4.10311290613819 -1
4.31101160925611 -1
4.4 -0.922485814512404
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
2 -1
2.01724048299192 -1
2 -0.976601151870982
1.86713056694505 -0.7
1.75310236017655 -0.4
1.7 -0.198368570303977
1.6802979577158 -0.1
1.65410509764529 0.2
1.66184536013535 0.5
1.7 0.776635211872064
1.70443118732779 0.8
1.79750756671086 1.1
1.92377338962021 1.4
2 1.54742681589863
2.09642332670557 1.7
2.3 1.99147746179108
2.30617413925339 2
2.52989681448045 2.3
2.6 2.39066342373969
2.75060773561099 2.6
2.9 2.80418365493673
2.96519076459348 2.9
3.16881011752734 3.2
3.2 3.24510999783824
3.36324546086329 3.5
3.5 3.71096785073259
3.55500209576419 3.8
3.73765452619258 4.1
3.8 4.20012884414665
3.91943832936855 4.4
4.09980815217705 4.7
4.1 4.70031357841406
4.27683063051977 5
4.12131338433914 5
4.1 4.96387881519334
3.93855847868702 4.7
3.8 4.46376737580613
3.75976066946774 4.4
3.5756206126646 4.1
3.5 3.97519711079049
3.38497634035994 3.8
3.2 3.5068301217304
3.19522394977942 3.5
2.98813980886284 3.2
2.9 3.06920064827456
2.77440036213646 2.9
2.6 2.65742255143861
2.55469251758534 2.6
2.32566967753338 2.3
2.3 2.26556325624276
2.10262820626328 2
2 1.84977507082873
1.91317306541083 1.7
1.76520698218065 1.4
1.7 1.23827140404518
1.65704438115522 1.1
1.59067887075397 0.8
1.55536570317537 0.5
1.55170412694501 0.2
1.58016931042088 -0.1
1.64010978690058 -0.4
1.7 -0.596709631019494
1.73987139236062 -0.7
1.88357294586497 -1
2 -1
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
4.1 -1
4.10311290613819 -1
4.4 -0.741393668656062
4.44498321125857 -0.7
4.7 -0.464852396471763
4.76813578863762 -0.4
5 -0.178871481853743
5 -0.1
5 0.0102260032015516
4.88506574094341 -0.1
4.7 -0.275969707049589
4.56668523595602 -0.4
4.4 -0.553052236854264
4.23363227745647 -0.7
4.1 -0.815843775918512
3.87197465814831 -1
4.1 -1
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
2 -0.976601151870982
2.01724048299192 -1
2.21243740010612 -1
2 -0.711679164421502
1.99438974152948 -0.7
1.88476393823007 -0.4
1.81033471610937 -0.1
1.77825725284207 0.2
1.79263833972996 0.5
1.85084599678411 0.8
1.94788554906494 1.1
2 1.22007735855146
2.10027735004554 1.4
2.29023724676887 1.7
2.3 1.7139781365215
2.50720808418118 2
2.6 2.1238222874385
2.72620691011982 2.3
2.9 2.54263214893311
2.93934957796352 2.6
3.14189595693532 2.9
3.2 2.98532003386492
3.33971439835052 3.2
3.5 3.45154544352774
3.53058807197833 3.5
3.71449489354027 3.8
3.8 3.93969127107409
3.89792460146803 4.1
4.07494670702065 4.4
4.1 4.44166829656617
4.25597356818247 4.7
4.4 4.94479321917345
4.43433699381796 5
4.4 5
4.27683063051977 5
4.1 4.70031357841406
4.09980815217705 4.7
3.91943832936855 4.4
3.8 4.20012884414665
3.73765452619258 4.1
3.55500209576419 3.8
3.5 3.71096785073259
3.36324546086328 3.5
3.2 3.24510999783824
3.16881011752734 3.2
2.96519076459348 2.9
2.9 2.80418365493673
2.75060773561099 2.6
2.6 2.39066342373969
2.52989681448045 2.3
2.30617413925339 2
2.3 1.99147746179108
2.09642332670557 1.7
2 1.54742681589863
1.92377338962021 1.4
1.79750756671086 1.1
1.70443118732779 0.8
1.7 0.776635211872064
1.66184536013535 0.5
1.65410509764529 0.2
1.6802979577158 -0.1
1.7 -0.198368570303977
1.75310236017655 -0.4
1.86713056694505 -0.7
2 -0.976601151870982
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
3.8 -1
3.87197465814831 -1
4.1 -0.815843775918512
4.23363227745647 -0.7
4.4 -0.553052236854264
4.56668523595602 -0.4
4.7 -0.275969707049589
4.88506574094341 -0.1
5 0.0102260032015516
5 0.2
5 0.205903790586725
4.99387894120173 0.2
4.7 -0.0795631974500552
4.67822595225581 -0.1
4.4 -0.355488871522846
4.35026739614153 -0.4
4.1 -0.616669322000814
3.99878457433925 -0.7
3.8 -0.856052672473788
3.59687652527383 -1
3.8 -1
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
2 -0.711679164421502
2.21243740010612 -1
2.3 -1
2.52618686142347 -1
2.3 -0.839595873336265
2.19973184540913 -0.7
2.02816940396458 -0.4
2 -0.325962829122201
1.94769804099704 -0.1
1.92007597939647 0.2
1.93700857270079 0.5
1.99726080624044 0.8
2 0.808350096035275
2.13109797536547 1.1
2.2933871184937 1.4
2.3 1.41044164651296
2.49921147232858 1.7
2.6 1.84146499798418
2.71185069049799 2
2.9 2.2713472779883
2.91970632309711 2.3
3.1233748974159 2.6
3.2 2.71485760884347
3.32240234492404 2.9
3.5 3.18512230504286
3.50960361589656 3.2
3.69788310543303 3.5
3.8 3.67045619685216
3.88112114563859 3.8
4.05709156657462 4.1
4.1 4.17296000708495
4.24075654471118 4.4
4.4 4.67729896626893
4.41453138384834 4.7
4.59941721747988 5
4.43433699381796 5
4.4 4.94479321917345
4.25597356818247 4.7
4.1 4.44166829656617
4.07494670702065 4.4
3.89792460146803 4.1
3.8 3.93969127107409
3.71449489354027 3.8
3.53058807197833 3.5
3.5 3.45154544352774
3.33971439835052 3.2
3.2 2.98532003386492
3.14189595693532 2.9
2.93934957796352 2.6
2.9 2.54263214893311
2.72620691011982 2.3
2.6 2.1238222874385
2.50720808418118 2
2.3 1.7139781365215
2.29023724676887 1.7
2.10027735004554 1.4
2 1.22007735855146
1.94788554906494 1.1
1.85084599678411 0.8
1.79263833972996 0.5
1.77825725284207 0.2
1.81033471610937 -0.1
1.88476393823007 -0.4
1.99438974152948 -0.7
2 -0.711679164421502
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
3.5 -1
3.59687652527383 -1
3.8 -0.856052672473787
3.99878457433925 -0.7
4.1 -0.616669322000814
4.35026739614153 -0.4
4.4 -0.355488871522846
4.67822595225581 -0.1
4.7 -0.0795631974500552
4.99387894120173 0.2
5 0.205903790586725
5 0.440612027357081
4.75053309473151 0.2
4.7 0.151928527160137
4.43158698553253 -0.1
4.4 -0.129005645314834
4.1 -0.396887855721992
4.09629111734723 -0.4
3.8 -0.632949649737633
3.7076214028826 -0.7
3.5 -0.837562856306993
3.20369960292137 -1
3.5 -1
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
2.3 -0.839595873336265
2.52618686142347 -1
2.6 -1
2.9 -1
3.2 -1
3.20369960292137 -1
3.5 -0.837562856306993
3.7076214028826 -0.7
3.8 -0.632949649737633
4.09629111734723 -0.4
4.1 -0.396887855721992
4.4 -0.129005645314834
4.43158698553253 -0.1
4.7 0.151928527160137
4.75053309473151 0.2
5 0.440612027357081
5 0.5
5 0.731458529001716
4.76174126258862 0.5
4.7 0.441099939334791
4.44580466158018 0.2
4.4 0.157788089893981
4.11611746001529 -0.1
4.1 -0.114003868976004
3.8 -0.356328200690915
3.74125438860604 -0.4
3.5 -0.560654852601715
3.25090640246052 -0.7
3.2 -0.724497633196024
2.9 -0.791572051994872
2.6 -0.745916843609906
2.53347593471837 -0.7
2.3 -0.48447884468801
2.25396615304517 -0.4
2.14724297535763 -0.1
2.10426845000774 0.2
2.12918983587066 0.5
2.21018035089827 0.8
2.3 1.01785321743913
2.34283253109295 1.1
2.52441099825145 1.4
2.6 1.51551158956693
2.72533872714962 1.7
2.9 1.96543233558424
2.92353509207033 2
3.12575730706559 2.3
3.2 2.41451465151041
3.32420041818617 2.6
3.5 2.89079092351239
3.50606716947757 2.9
3.69859554128548 3.2
3.8 3.37380075372315
3.88113826328343 3.5
4.05599129290913 3.8
4.1 3.87687686165625
4.24228311958585 4.1
4.4 4.38224708274951
4.41174509682265 4.4
4.60156056648369 4.7
4.7 4.87218479782626
4.78516191253705 5
4.7 5
4.59941721747988 5
4.41453138384834 4.7
4.4 4.67729896626893
4.24075654471118 4.4
4.1 4.17296000708495
4.05709156657462 4.1
3.88112114563859 3.8
3.8 3.67045619685216
3.69788310543303 3.5
3.50960361589656 3.2
3.5 3.18512230504286
3.32240234492404 2.9
3.2 2.71485760884347
3.1233748974159 2.6
2.91970632309711 2.3
2.9 2.2713472779883
2.71185069049799 2
2.6 1.84146499798418
2.49921147232858 1.7
2.3 1.41044164651296
2.2933871184937 1.4
2.13109797536547 1.1
2 0.808350096035275
1.99726080624044 0.8
1.93700857270079 0.5
1.92007597939647 0.2
1.94769804099704 -0.1
2 -0.325962829122201
2.02816940396458 -0.4
2.19973184540913 -0.7
2.3 -0.839595873336265
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
2.6 -0.745916843609906
2.9 -0.791572051994872
3.2 -0.724497633196024
3.25090640246052 -0.7
3.5 -0.560654852601715
3.74125438860604 -0.4
3.8 -0.356328200690915
4.1 -0.114003868976004
4.11611746001529 -0.1
4.4 0.157788089893981
4.44580466158018 0.2
4.7 0.441099939334791
4.76174126258862 0.5
5 0.731458529001716
5 0.8
5 1.1
5 1.15675424261348
4.94351139674939 1.1
4.7 0.862386935652927
4.63708327978163 0.8
4.4 0.574808785049052
4.32189029184767 0.5
4.1 0.300098067340002
3.98730412562644 0.2
3.8 0.0472775702829577
3.60741650954863 -0.1
3.5 -0.172867199578749
3.2 -0.330971546937226
2.9068277406261 -0.4
2.9 -0.401258145565452
2.89497658829077 -0.4
2.6 -0.280438264004005
2.47342478931997 -0.1
2.38142994773125 0.2
2.39942156256348 0.5
2.48895115126244 0.8
2.6 1.06125668654309
2.62004938424398 1.1
2.80260150342481 1.4
2.9 1.56208089015974
2.99041615179638 1.7
3.17314568242424 2
3.2 2.04319100485484
3.37275743857306 2.3
3.5 2.51911652675776
3.55408998095484 2.6
3.73798200733273 2.9
3.8 3.00976772378168
3.92549386770091 3.2
4.08939871229436 3.5
4.1 3.51910717357295
4.284394024834 3.8
4.4 4.01341381560968
4.45928514986522 4.1
4.64237713477393 4.4
4.7 4.50359732089665
4.83623735452237 4.7
5 4.9926141426742
5 5
4.78516191253705 5
4.7 4.87218479782626
4.60156056648369 4.7
4.41174509682265 4.4
4.4 4.38224708274951
4.24228311958585 4.1
4.1 3.87687686165625
4.05599129290913 3.8
3.88113826328343 3.5
3.8 3.37380075372315
3.69859554128548 3.2
3.50606716947757 2.9
3.5 2.89079092351239
3.32420041818617 2.6
3.2 2.41451465151041
3.12575730706559 2.3
2.92353509207033 2
2.9 1.96543233558424
2.72533872714962 1.7
2.6 1.51551158956693
2.52441099825145 1.4
2.34283253109295 1.1
2.3 1.01785321743913
2.21018035089827 0.8
2.12918983587066 0.5
2.10426845000774 0.2
2.14724297535763 -0.1
2.25396615304517 -0.4
2.3 -0.48447884468801
2.53347593471837 -0.7
2.6 -0.745916843609906
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
2.9 -0.401258145565452
2.9068277406261 -0.4
3.2 -0.330971546937226
3.5 -0.172867199578749
3.60741650954863 -0.1
3.8 0.0472775702829577
3.98730412562644 0.2
4.1 0.300098067340002
4.32189029184767 0.5
4.4 0.574808785049052
4.63708327978163 0.8
4.7 0.862386935652927
4.94351139674939 1.1
5 1.15675424261348
5 1.4
5 1.7
5 2
5 2.14971135273324
4.88032197681036 2
4.7 1.78976864382541
4.62798750630714 1.7
4.4 1.43404970572513
4.3710549632801 1.4
4.10165659490701 1.1
4.1 1.0983210488395
3.8 0.803071754105016
3.7960475985311 0.8
3.5 0.582351063042486
3.29834401612111 0.5
3.2 0.464137763416859
3.12960709877605 0.5
3.03024747253045 0.8
3.10950785391485 1.1
3.2 1.34226847477905
3.22973959919525 1.4
3.40530034537912 1.7
3.5 1.89419961496514
3.56918864714886 2
3.74284330590738 2.3
3.8 2.41187477167063
3.92934001678752 2.6
4.08347685250468 2.9
4.1 2.93216571644519
4.28741498115617 3.2
4.4 3.42450734402999
4.45675108234677 3.5
4.64686645305324 3.8
4.7 3.9004054995071
4.85376796510912 4.1
5 4.36326855419346
5 4.4
5 4.7
5 4.9926141426742
4.83623735452237 4.7
4.7 4.50359732089665
4.64237713477393 4.4
4.45928514986522 4.1
4.4 4.01341381560968
4.284394024834 3.8
4.1 3.51910717357295
4.08939871229436 3.5
3.92549386770091 3.2
3.8 3.00976772378168
3.73798200733273 2.9
3.55408998095484 2.6
3.5 2.51911652675776
3.37275743857306 2.3
3.2 2.04319100485484
3.17314568242424 2
2.99041615179638 1.7
2.9 1.56208089015974
2.80260150342481 1.4
2.62004938424398 1.1
2.6 1.06125668654309
2.48895115126244 0.8
2.39942156256348 0.5
2.38142994773125 0.2
2.47342478931997 -0.1
2.6 -0.280438264004005
2.89497658829077 -0.4
2.9 -0.401258145565452
};
\addplot [draw=none, fill=lavender231240249]
table{%
x  y
3.2 0.464137763416859
3.29834401612111 0.5
3.5 0.582351063042486
3.7960475985311 0.8
3.8 0.803071754105016
4.1 1.0983210488395
4.10165659490701 1.1
4.3710549632801 1.4
4.4 1.43404970572513
4.62798750630714 1.7
4.7 1.78976864382541
4.88032197681036 2
5 2.14971135273324
5 2.3
5 2.6
5 2.9
5 3.2
5 3.5
5 3.8
5 4.1
5 4.36326855419346
4.85376796510912 4.1
4.7 3.9004054995071
4.64686645305324 3.8
4.45675108234677 3.5
4.4 3.42450734402999
4.28741498115617 3.2
4.1 2.93216571644519
4.08347685250468 2.9
3.92934001678752 2.6
3.8 2.41187477167063
3.74284330590738 2.3
3.56918864714886 2
3.5 1.89419961496514
3.40530034537912 1.7
3.22973959919525 1.4
3.2 1.34226847477905
3.10950785391485 1.1
3.03024747253045 0.8
3.12960709877605 0.5
3.2 0.464137763416859
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
4.1 2.6
};
\coordinate (MCMC_mean_lml_t) at (axis cs:3.8,3.2);
\end{axis}



==> fig/tikz/usps/MCMC_mean_lml.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=teal1996167]
table{%
x  y
-0.7 4.54766875412731
-0.4 4.51513503414221
-0.1 4.529275705577
0.2 4.54816127828554
0.5 4.57461510291747
0.599340562373571 4.7
0.8 4.8294709197334
0.856026055438696 5
0.8 5
0.5 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.57697150408672
-0.7 4.54766875412731
};
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.7 -1
-0.4 -1
-0.1 -1
0.2 -1
0.5 -1
0.8 -1
1.09484915668695 -1
0.967577086494847 -0.7
0.89578558483893 -0.4
0.853091355679454 -0.1
0.828098441921518 0.2
0.813147284688625 0.5
0.804194786782559 0.8
0.8 1.04126791492845
0.795677782799318 1.1
0.787120264788144 1.4
0.782937881345467 1.7
0.789378604290626 2
0.8 2.14671716803583
0.802748975914488 2.3
0.802473350425106 2.6
0.812466408974618 2.9
0.823810029443945 3.2
0.832325019260191 3.5
0.844635018022834 3.8
0.857720098375945 4.1
0.886407259608248 4.4
0.927957815331137 4.7
1.0110664593552 5
0.856026055438696 5
0.8 4.8294709197334
0.599340562373571 4.7
0.5 4.57461510291747
0.2 4.54816127828554
-0.1 4.529275705577
-0.4 4.51513503414221
-0.7 4.54766875412731
-1 4.57697150408672
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
1.1 -1
1.4 -1
1.40687503190484 -1
1.4 -0.97984357944367
1.28124935825887 -0.7
1.1984566012808 -0.4
1.1438257673898 -0.1
1.10557453144333 0.2
1.1 0.270126031076834
1.06552764717826 0.5
1.03797427915527 0.8
1.0214827088905 1.1
1.0132610362085 1.4
1.00909558830166 1.7
1.00737099749162 2
1.00545385412733 2.3
1.01060790698428 2.6
1.01872754201148 2.9
1.02271880037854 3.2
1.03026347268352 3.5
1.04083800079659 3.8
1.052999180931 4.1
1.07786597343877 4.4
1.1 4.64778960048812
1.10248294237288 4.7
1.14097628952589 5
1.1 5
1.0110664593552 5
0.927957815331137 4.7
0.886407259608248 4.4
0.857720098375945 4.1
0.844635018022834 3.8
0.832325019260191 3.5
0.823810029443945 3.2
0.812466408974618 2.9
0.802473350425106 2.6
0.802748975914488 2.3
0.8 2.14671716803583
0.789378604290626 2
0.782937881345468 1.7
0.787120264788144 1.4
0.795677782799318 1.1
0.8 1.04126791492845
0.804194786782559 0.8
0.813147284688625 0.5
0.828098441921518 0.2
0.853091355679454 -0.1
0.89578558483893 -0.4
0.967577086494847 -0.7
1.09484915668695 -1
1.1 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
5 -1
5 -0.943952809163039
4.94045037033084 -1
5 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
1.4 -0.97984357944367
1.40687503190484 -1
1.58866774552022 -1
1.47001199796612 -0.7
1.4 -0.468420387736983
1.37519874033213 -0.4
1.29257840014025 -0.1
1.23935833455424 0.2
1.20618379119404 0.5
1.18692464237869 0.8
1.1749886151898 1.1
1.16845236740549 1.4
1.16491451313274 1.7
1.16289811712403 2
1.16058582741755 2.3
1.16316742272475 2.6
1.1665577462332 2.9
1.16773883595469 3.2
1.17039263729046 3.5
1.17644966797087 3.8
1.18263383833149 4.1
1.19184680730542 4.4
1.20441420630189 4.7
1.23707796739527 5
1.14097628952589 5
1.10248294237288 4.7
1.1 4.64778960048812
1.07786597343877 4.4
1.052999180931 4.1
1.04083800079659 3.8
1.03026347268352 3.5
1.02271880037854 3.2
1.01872754201148 2.9
1.01060790698428 2.6
1.00545385412733 2.3
1.00737099749162 2
1.00909558830166 1.7
1.0132610362085 1.4
1.0214827088905 1.1
1.03797427915527 0.8
1.06552764717826 0.5
1.1 0.270126031076834
1.10557453144333 0.2
1.1438257673898 -0.1
1.1984566012808 -0.4
1.28124935825887 -0.7
1.4 -0.97984357944367
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
4.7 -1
4.94045037033084 -1
5 -0.943952809163039
5 -0.7
5 -0.579890922581706
4.87295292382311 -0.7
4.7 -0.865511527701911
4.55234207193003 -1
4.7 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
1.7 -1
1.76502003676788 -1
1.7 -0.877318755487771
1.6174210140642 -0.7
1.51027935579155 -0.4
1.43286856655529 -0.1
1.4 0.0741623525484656
1.37314213766516 0.2
1.3291655198277 0.5
1.30524052324225 0.8
1.29088331568618 1.1
1.28271391444452 1.4
1.2780573411365 1.7
1.27539383308921 2
1.27413230214393 2.3
1.27388875295039 2.6
1.27639390655036 2.9
1.27851839406655 3.2
1.27907594791443 3.5
1.28590344228829 3.8
1.29146071395033 4.1
1.29569977688551 4.4
1.3063454702309 4.7
1.33317964526466 5
1.23707796739527 5
1.20441420630189 4.7
1.19184680730542 4.4
1.18263383833149 4.1
1.17644966797087 3.8
1.17039263729046 3.5
1.16773883595469 3.2
1.1665577462332 2.9
1.16316742272475 2.6
1.16058582741755 2.3
1.16289811712403 2
1.16491451313274 1.7
1.16845236740549 1.4
1.1749886151898 1.1
1.18692464237869 0.8
1.20618379119404 0.5
1.23935833455424 0.2
1.29257840014025 -0.1
1.37519874033213 -0.4
1.4 -0.468420387736983
1.47001199796612 -0.7
1.58866774552022 -1
1.7 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
4.4 -1
4.55234207193003 -1
4.7 -0.865511527701911
4.87295292382311 -0.7
5 -0.579890922581706
5 -0.4
5 -0.306193780289477
4.90086452087274 -0.4
4.7 -0.591946151653569
4.58149850861839 -0.7
4.4 -0.86827807613358
4.24621428737149 -1
4.4 -1
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
1.7 -0.877318755487771
1.76502003676788 -1
1.93277609553353 -1
1.76606204620253 -0.7
1.7 -0.556393111378422
1.6385595744851 -0.4
1.5511643232271 -0.1
1.48969607074699 0.2
1.44650171511807 0.5
1.42144148670277 0.8
1.40625929520369 1.1
1.4 1.30652542188603
1.39697546148356 1.4
1.39120016914027 1.7
1.38788954905438 2
1.3876787768703 2.3
1.38461008317603 2.6
1.38623006686753 2.9
1.38929795217841 3.2
1.38775925853841 3.5
1.39535721660572 3.8
1.4 4.08240605259851
1.40027321673962 4.1
1.4 4.21408304511069
1.3995527464656 4.4
1.4 4.4151098680368
1.40848158115861 4.7
1.4295728380229 5
1.4 5
1.33317964526466 5
1.3063454702309 4.7
1.29569977688551 4.4
1.29146071395033 4.1
1.28590344228829 3.8
1.27907594791443 3.5
1.27851839406655 3.2
1.27639390655036 2.9
1.27388875295039 2.6
1.27413230214393 2.3
1.27539383308921 2
1.2780573411365 1.7
1.28271391444452 1.4
1.29088331568618 1.1
1.30524052324225 0.8
1.3291655198277 0.5
1.37314213766516 0.2
1.4 0.0741623525484656
1.43286856655529 -0.1
1.51027935579155 -0.4
1.6174210140642 -0.7
1.7 -0.877318755487771
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
4.1 -1
4.24621428737149 -1
4.4 -0.86827807613358
4.58149850861839 -0.7
4.7 -0.591946151653569
4.90086452087274 -0.4
5 -0.306193780289477
5 -0.1
5 -0.0703168557118743
4.96900823639726 -0.1
4.7 -0.355867161224841
4.65188396489177 -0.4
4.4 -0.631832304058136
4.32102324876338 -0.7
4.1 -0.892595175845542
3.96381310492898 -1
4.1 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
2 -1
2.13223451634132 -1
2 -0.844569781215913
1.91627239174403 -0.7
1.77423132151581 -0.4
1.7 -0.199395082581381
1.66946007989891 -0.1
1.60192217211717 0.2
1.556169271478 0.5
1.52913485003906 0.8
1.51328458452309 1.1
1.50354704750735 1.4
1.49757140045988 1.7
1.49503477926853 2
1.49415238072859 2.3
1.49138215328961 2.6
1.49288759833234 2.9
1.49519220415564 3.2
1.49406757786627 3.5
1.499461243834 3.8
1.50366126459298 4.1
1.50308217101314 4.4
1.51293561712388 4.7
1.5266312714943 5
1.4295728380229 5
1.40848158115861 4.7
1.4 4.4151098680368
1.3995527464656 4.4
1.4 4.21408304511069
1.40027321673962 4.1
1.4 4.08240605259851
1.39535721660572 3.8
1.38775925853841 3.5
1.38929795217841 3.2
1.38623006686753 2.9
1.38461008317603 2.6
1.3876787768703 2.3
1.38788954905438 2
1.39120016914027 1.7
1.39697546148356 1.4
1.4 1.30652542188603
1.40625929520369 1.1
1.42144148670277 0.8
1.44650171511807 0.5
1.48969607074699 0.2
1.5511643232271 -0.1
1.6385595744851 -0.4
1.7 -0.556393111378422
1.76606204620253 -0.7
1.93277609553353 -1
2 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
3.8 -1
3.96381310492898 -1
4.1 -0.892595175845542
4.32102324876338 -0.7
4.4 -0.631832304058136
4.65188396489177 -0.4
4.7 -0.355867161224841
4.96900823639726 -0.1
5 -0.0703168557118743
5 0.148042770988409
4.74102194675795 -0.1
4.7 -0.139018021178253
4.41546316973675 -0.4
4.4 -0.414232197232772
4.1 -0.673714322820465
4.06694425972761 -0.7
3.8 -0.912205881141492
3.66981431248671 -1
3.8 -1
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
2 -0.844569781215913
2.13223451634132 -1
2.3 -1
2.40195832746377 -1
2.3 -0.94060459902387
2.09392984860001 -0.7
2 -0.5707511893339
1.91669750378702 -0.4
1.802738085215 -0.1
1.71744236952118 0.2
1.7 0.286430748283445
1.66583682783793 0.5
1.63682821337534 0.8
1.62030987384249 1.1
1.60990954319701 1.4
1.603371545007 1.7
1.60153452834348 2
1.59976506877034 2.3
1.59751667086439 2.6
1.59908951175081 2.9
1.6005640332656 3.2
1.60007445712797 3.5
1.6033282947993 3.8
1.60704931244634 4.1
1.6066101961539 4.4
1.61738965308914 4.7
1.62368970496569 5
1.5266312714943 5
1.51293561712388 4.7
1.50308217101314 4.4
1.50366126459298 4.1
1.499461243834 3.8
1.49406757786627 3.5
1.49519220415564 3.2
1.49288759833234 2.9
1.49138215328961 2.6
1.49415238072859 2.3
1.49503477926853 2
1.49757140045988 1.7
1.50354704750735 1.4
1.51328458452309 1.1
1.52913485003906 0.8
1.556169271478 0.5
1.60192217211717 0.2
1.66946007989891 -0.1
1.7 -0.199395082581381
1.77423132151581 -0.4
1.91627239174403 -0.7
2 -0.844569781215913
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
3.5 -1
3.66981431248671 -1
3.8 -0.912205881141492
4.06694425972761 -0.7
4.1 -0.673714322820465
4.4 -0.414232197232772
4.41546316973675 -0.4
4.7 -0.139018021178253
4.74102194675795 -0.1
5 0.148042770988409
5 0.2
5 0.366276754238012
4.82603827316676 0.2
4.7 0.0792902107266922
4.50656843407176 -0.1
4.4 -0.197765134719028
4.16987485539682 -0.4
4.1 -0.46050446754962
3.8 -0.699011344004361
3.79857814706717 -0.7
3.5 -0.899869892089626
3.30444841656815 -1
3.5 -1
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
2.3 -0.94060459902387
2.40195832746377 -1
2.6 -1
2.9 -1
3.2 -1
3.30444841656815 -1
3.5 -0.899869892089626
3.79857814706717 -0.7
3.8 -0.699011344004361
4.1 -0.46050446754962
4.16987485539682 -0.4
4.4 -0.197765134719028
4.50656843407176 -0.1
4.7 0.0792902107266922
4.82603827316676 0.2
5 0.366276754238012
5 0.5
5 0.593384144437749
4.90268622188542 0.5
4.7 0.307129419727588
4.58603197339295 0.2
4.4 0.0285562761594149
4.25472063070511 -0.1
4.1 -0.234723466254595
3.89467665862338 -0.4
3.8 -0.474234174274494
3.5 -0.681238236732348
3.46382638930032 -0.7
3.2 -0.82757392322213
2.9 -0.90240712815632
2.6 -0.869859111871681
2.31197393227811 -0.7
2.3 -0.691627135989765
2.08741232283406 -0.4
2 -0.251621040446638
1.94123006483084 -0.1
1.8557977053697 0.2
1.79575626005112 0.5
1.75769430961453 0.8
1.73557458084123 1.1
1.72130491313892 1.4
1.71220381420492 1.7
1.71047011294629 2
1.70710185924102 2.3
1.70482984681869 2.6
1.70690997762922 2.9
1.70778170030547 3.2
1.70792819755203 3.5
1.70949600482514 3.8
1.71378775465007 4.1
1.71334048026722 4.4
1.72770356078666 4.7
1.72854801903687 5
1.7 5
1.62368970496569 5
1.61738965308914 4.7
1.6066101961539 4.4
1.60704931244634 4.1
1.6033282947993 3.8
1.60007445712797 3.5
1.6005640332656 3.2
1.59908951175081 2.9
1.59751667086439 2.6
1.59976506877034 2.3
1.60153452834348 2
1.603371545007 1.7
1.60990954319701 1.4
1.62030987384249 1.1
1.63682821337534 0.8
1.66583682783793 0.5
1.7 0.286430748283445
1.71744236952118 0.2
1.802738085215 -0.1
1.91669750378702 -0.4
2 -0.5707511893339
2.09392984860001 -0.7
2.3 -0.94060459902387
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
2.6 -0.869859111871681
2.9 -0.90240712815632
3.2 -0.82757392322213
3.46382638930032 -0.7
3.5 -0.681238236732348
3.8 -0.474234174274494
3.89467665862338 -0.4
4.1 -0.234723466254595
4.25472063070511 -0.1
4.4 0.0285562761594148
4.58603197339295 0.2
4.7 0.307129419727588
4.90268622188542 0.5
5 0.593384144437749
5 0.8
5 0.841041541536703
4.95772719075822 0.8
4.7 0.55438993106223
4.64239662971421 0.5
4.4 0.274434209915337
4.31664365041185 0.2
4.1 0.0119653665558378
3.96241725498632 -0.1
3.8 -0.226946578758194
3.55334187822246 -0.4
3.5 -0.435580474072448
3.2 -0.582250014838781
2.9 -0.657035566478838
2.6 -0.611335137660835
2.3 -0.402879079524613
2.29790123499161 -0.4
2.1235883425183 -0.1
2 0.179482038204835
1.99415304121822 0.2
1.93483897898906 0.5
1.89725123249707 0.8
1.87485963959139 1.1
1.86056488834481 1.4
1.85298107223229 1.7
1.8492584996914 2
1.84657384928185 2.3
1.8452261782056 2.6
1.84559715970707 2.9
1.84592034687325 3.2
1.84612865659735 3.5
1.84657378390743 3.8
1.85036338264608 4.1
1.84956887145659 4.4
1.86017883671503 4.7
1.86209378338732 5
1.72854801903687 5
1.72770356078666 4.7
1.71334048026722 4.4
1.71378775465007 4.1
1.70949600482514 3.8
1.70792819755203 3.5
1.70778170030547 3.2
1.70690997762922 2.9
1.70482984681869 2.6
1.70710185924102 2.3
1.71047011294629 2
1.71220381420492 1.7
1.72130491313892 1.4
1.73557458084123 1.1
1.75769430961453 0.8
1.79575626005112 0.5
1.8557977053697 0.2
1.94123006483084 -0.1
2 -0.251621040446638
2.08741232283406 -0.4
2.3 -0.691627135989765
2.31197393227811 -0.7
2.6 -0.869859111871681
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
2.3 -0.402879079524613
2.6 -0.611335137660835
2.9 -0.657035566478838
3.2 -0.582250014838781
3.5 -0.435580474072448
3.55334187822246 -0.4
3.8 -0.226946578758194
3.96241725498632 -0.1
4.1 0.0119653665558378
4.31664365041185 0.2
4.4 0.274434209915337
4.64239662971421 0.5
4.7 0.55438993106223
4.95772719075822 0.8
5 0.841041541536703
5 1.1
5 1.13385554050591
4.96530694525446 1.1
4.7 0.84420991256019
4.65323159511614 0.8
4.4 0.564225880370299
4.32893634165382 0.5
4.1 0.300665314635159
3.97929696725925 0.2
3.8 0.0596472460280267
3.57572391639402 -0.1
3.5 -0.150175906790391
3.2 -0.296106621793499
2.9 -0.364788869449337
2.6 -0.295170488203415
2.37666673919065 -0.1
2.3 -0.00879195589644733
2.21034688666717 0.2
2.11888871864571 0.5
2.05985430205172 0.8
2.02301912493802 1.1
2 1.39633024518248
1.99982486355071 1.4
1.99375833025967 1.7
1.98804688643651 2
1.98604583932269 2.3
1.9856225095925 2.6
1.98428434178491 2.9
1.98405899344103 3.2
1.98432911564268 3.5
1.98365156298972 3.8
1.9869390106421 4.1
1.98579726264597 4.4
1.9926541126434 4.7
1.99563954773777 5
1.86209378338732 5
1.86017883671503 4.7
1.84956887145659 4.4
1.85036338264608 4.1
1.84657378390743 3.8
1.84612865659735 3.5
1.84592034687325 3.2
1.84559715970707 2.9
1.8452261782056 2.6
1.84657384928185 2.3
1.8492584996914 2
1.85298107223229 1.7
1.86056488834481 1.4
1.87485963959139 1.1
1.89725123249707 0.8
1.93483897898906 0.5
1.99415304121822 0.2
2 0.179482038204835
2.1235883425183 -0.1
2.29790123499161 -0.4
2.3 -0.402879079524613
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
2.6 -0.295170488203415
2.9 -0.364788869449337
3.2 -0.296106621793499
3.5 -0.150175906790391
3.57572391639402 -0.1
3.8 0.0596472460280267
3.97929696725925 0.2
4.1 0.300665314635159
4.32893634165382 0.5
4.4 0.564225880370299
4.65323159511614 0.8
4.7 0.844209912560191
4.96530694525446 1.1
5 1.13385554050591
5 1.4
5 1.51892469193777
4.87920381842967 1.4
4.7 1.22638949294628
4.56883748034658 1.1
4.4 0.942838683894996
4.2436747037917 0.8
4.1 0.673431898178795
3.89558764512385 0.5
3.8 0.423610253286102
3.5 0.212194441975148
3.47574458383793 0.2
3.2 0.0763245134446303
2.9 0.0316840125361485
2.6 0.148794252075746
2.55704149693009 0.2
2.3822720560292 0.5
2.3 0.729739445625541
2.28678993980571 0.8
2.24969205156744 1.1
2.22932650627419 1.4
2.21816432032841 1.7
2.21117124919168 2
2.20767795292462 2.3
2.20646724126137 2.6
2.20384144455221 2.9
2.20351358745938 3.2
2.20459168473581 3.5
2.20574789263938 3.8
2.2060267024599 4.1
2.20526962997733 4.4
2.20974993430916 4.7
2.21439280426172 5
2 5
1.99563954773777 5
1.9926541126434 4.7
1.98579726264597 4.4
1.9869390106421 4.1
1.98365156298972 3.8
1.98432911564268 3.5
1.98405899344103 3.2
1.98428434178491 2.9
1.9856225095925 2.6
1.98604583932269 2.3
1.98804688643651 2
1.99375833025967 1.7
1.99982486355071 1.4
2 1.39633024518248
2.02301912493802 1.1
2.05985430205172 0.8
2.11888871864571 0.5
2.21034688666717 0.2
2.3 -0.00879195589644733
2.37666673919065 -0.1
2.6 -0.295170488203415
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
2.6 0.148794252075746
2.9 0.0316840125361485
3.2 0.0763245134446303
3.47574458383793 0.2
3.5 0.212194441975147
3.8 0.423610253286102
3.89558764512385 0.5
4.1 0.673431898178795
4.2436747037917 0.8
4.4 0.942838683894996
4.56883748034658 1.1
4.7 1.22638949294628
4.87920381842967 1.4
5 1.51892469193777
5 1.7
5 2
5 2.13866667723928
4.87056994429671 2
4.7 1.82543978232823
4.57801857100431 1.7
4.4 1.52285596849763
4.27220722463562 1.4
4.1 1.24449763300668
3.93494884349596 1.1
3.8 0.989488871736613
3.5307923217043 0.8
3.5 0.779945163189796
3.2 0.67081680227626
2.9 0.710167143775318
2.81631327936906 0.8
2.66017107152762 1.1
2.6 1.31243241855274
2.58815236957814 1.4
2.56676673171908 1.7
2.5563408488738 2
2.54751898340636 2.3
2.54561604428473 2.6
2.5424324755658 2.9
2.53805175030166 3.2
2.53865656374226 3.5
2.54140621661911 3.8
2.54746460777571 4.1
2.54093727861192 4.4
2.54905114850986 4.7
2.55640135376043 5
2.3 5
2.21439280426172 5
2.20974993430916 4.7
2.20526962997733 4.4
2.2060267024599 4.1
2.20574789263938 3.8
2.20459168473581 3.5
2.20351358745938 3.2
2.20384144455221 2.9
2.20646724126137 2.6
2.20767795292462 2.3
2.21117124919168 2
2.21816432032841 1.7
2.22932650627419 1.4
2.24969205156744 1.1
2.28678993980571 0.8
2.3 0.729739445625541
2.3822720560292 0.5
2.55704149693009 0.2
2.6 0.148794252075746
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
5 4.64070313682235
5 4.7
5 5
4.73011648558867 5
4.95258164453347 4.7
5 4.64070313682235
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
2.9 0.710167143775318
3.2 0.670816802276259
3.5 0.779945163189796
3.5307923217043 0.8
3.8 0.989488871736613
3.93494884349596 1.1
4.1 1.24449763300668
4.27220722463562 1.4
4.4 1.52285596849763
4.57801857100431 1.7
4.7 1.82543978232823
4.87056994429671 2
5 2.13866667723928
5 2.3
5 2.6
5 2.9
5 3.2
5 3.5
5 3.8
5 4.1
5 4.4
5 4.64070313682235
4.95258164453347 4.7
4.73011648558867 5
4.7 5
4.4 5
4.1 5
3.8 5
3.5 5
3.2 5
2.9 5
2.6 5
2.55640135376043 5
2.54905114850986 4.7
2.54093727861192 4.4
2.54746460777571 4.1
2.54140621661911 3.8
2.53865656374226 3.5
2.53805175030166 3.2
2.5424324755658 2.9
2.54561604428473 2.6
2.54751898340636 2.3
2.5563408488738 2
2.56676673171908 1.7
2.58815236957814 1.4
2.6 1.31243241855274
2.66017107152762 1.1
2.81631327936906 0.8
2.9 0.710167143775318
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
3.8 3.2
};
\coordinate (MCMC_mean_lml_t) at (axis cs:3.8,3.2);
\end{axis}



==> fig/tikz/usps/MCMC_nlpd.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{aliceblue242247253}{RGB}{242,247,253}
\definecolor{cornflowerblue107174214}{RGB}{107,174,214}
\definecolor{cornflowerblue89162207}{RGB}{89,162,207}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lavender210227243}{RGB}{210,227,243}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lavender231240249}{RGB}{231,240,249}
\definecolor{lightblue168206228}{RGB}{168,206,228}
\definecolor{lightblue185213234}{RGB}{185,213,234}
\definecolor{midnightblue854116}{RGB}{8,54,116}
\definecolor{midnightblue868137}{RGB}{8,68,137}
\definecolor{powderblue200220239}{RGB}{200,220,239}
\definecolor{skyblue128185218}{RGB}{128,185,218}
\definecolor{skyblue149197223}{RGB}{149,197,223}
\definecolor{steelblue30109178}{RGB}{30,109,178}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue43123186}{RGB}{43,123,186}
\definecolor{steelblue57137193}{RGB}{57,137,193}
\definecolor{steelblue72150200}{RGB}{72,150,200}
\definecolor{teal1996167}{RGB}{19,96,167}
\definecolor{teal882156}{RGB}{8,82,156}

\begin{axis}[
height=\figureheight,
tick pos=left,
width=\figurewidth,
x grid style={darkgray176},
xmin=-1, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ymin=-1, ymax=5,
ytick style={color=black}
]
\addplot [draw=none, fill=steelblue30109178]
table{%
x  y
-0.7 -1
-0.4 -1
-0.1 -1
0.2 -1
0.5 -1
0.8 -1
0.925245178749352 -1
0.860566582328153 -0.7
0.821482764219575 -0.4
0.8 -0.151094245263644
0.783687598533362 -0.1
0.711308063713757 0.2
0.672591140058874 0.5
0.650385868694352 0.8
0.638115566389705 1.1
0.631512756203757 1.4
0.627747258556063 1.7
0.626133249882703 2
0.624944870280413 2.3
0.624395281239576 2.6
0.623573849714627 2.9
0.624041776320402 3.2
0.623743922965221 3.5
0.623500259499288 3.8
0.624577271340898 4.1
0.624333649970153 4.4
0.623638903960531 4.7
0.62433440278382 5
0.5 5
0.2 5
-0.1 5
-0.4 5
-0.7 5
-1 5
-1 4.7
-1 4.4
-1 4.1
-1 3.8
-1 3.5
-1 3.2
-1 2.9
-1 2.6
-1 2.3
-1 2
-1 1.7
-1 1.4
-1 1.1
-1 0.8
-1 0.5
-1 0.2
-1 -0.1
-1 -0.4
-1 -0.7
-1 -1
-0.7 -1
};
\addplot [draw=none, fill=steelblue43123186]
table{%
x  y
1.1 -1
1.21724815588989 -1
1.14258967757635 -0.7
1.1 -0.473113126715385
1.07416836082049 -0.4
0.993304500764427 -0.1
0.94604025325011 0.2
0.918050543786769 0.5
0.901471427925183 0.8
0.891901324349755 1.1
0.886572237431246 1.4
0.883700256393163 1.7
0.881979802383875 2
0.881171591267691 2.3
0.880587437477207 2.6
0.880191700869088 2.9
0.880545466295679 3.2
0.880371319292955 3.5
0.880313408598856 3.8
0.880609721226441 4.1
0.880224489388341 4.4
0.880158125784374 4.7
0.880679579691547 5
0.8 5
0.62433440278382 5
0.623638903960531 4.7
0.624333649970153 4.4
0.624577271340898 4.1
0.623500259499288 3.8
0.623743922965221 3.5
0.624041776320402 3.2
0.623573849714627 2.9
0.624395281239576 2.6
0.624944870280413 2.3
0.626133249882703 2
0.627747258556063 1.7
0.631512756203757 1.4
0.638115566389705 1.1
0.650385868694352 0.8
0.672591140058874 0.5
0.711308063713757 0.2
0.783687598533362 -0.1
0.8 -0.151094245263644
0.821482764219575 -0.4
0.860566582328153 -0.7
0.925245178749352 -1
1.1 -1
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
1.27684108914834 -0.7
1.20010526320651 -0.4
1.14525136614435 -0.1
1.10690351189312 0.2
1.1 0.276049997930129
1.06710792872863 0.5
1.04092714069729 0.8
1.02602531148646 1.1
1.01773293478313 1.4
1.01346623638504 1.7
1.01041090778063 2
1.00940155446167 2.3
1.00834579267494 2.6
1.00813314061253 2.9
1.00837202286964 3.2
1.00835033823288 3.5
1.00845784112184 3.8
1.00831101170665 4.1
1.00750408636016 4.4
1.00792141237075 4.7
1.00873896873318 5
0.880679579691547 5
0.880158125784374 4.7
0.880224489388341 4.4
0.880609721226441 4.1
0.880313408598856 3.8
0.880371319292955 3.5
0.880545466295679 3.2
0.880191700869088 2.9
0.880587437477207 2.6
0.881171591267691 2.3
0.881979802383875 2
0.883700256393163 1.7
0.886572237431246 1.4
0.891901324349755 1.1
0.901471427925183 0.8
0.918050543786769 0.5
0.94604025325011 0.2
0.993304500764427 -0.1
1.07416836082049 -0.4
1.1 -0.473113126715385
1.14258967757635 -0.7
1.21724815588989 -1
1.39243664511501 -1
1.27684108914834 -0.7
};
\addplot [draw=none, fill=steelblue57137193]
table{%
x  y
5 -1
5 -0.99885239241713
4.99877806737892 -1
5 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
1.4 -1
1.51182885762507 -1
1.40861146256194 -0.7
1.4 -0.671682358706507
1.31160941523344 -0.4
1.24412316612924 -0.1
1.1990299365012 0.2
1.16884726724727 0.5
1.14985046195998 0.8
1.13831805687106 1.1
1.13164608126069 1.4
1.12816280263549 1.7
1.12560984295899 2
1.12478187884999 2.3
1.12381068803703 2.6
1.12371854652372 2.9
1.12381313145352 3.2
1.12385090741753 3.5
1.12404483236362 3.8
1.12375450005013 4.1
1.12310258361394 4.4
1.12356229347085 4.7
1.12419807928258 5
1.1 5
1.00873896873318 5
1.00792141237075 4.7
1.00750408636016 4.4
1.00831101170665 4.1
1.00845784112184 3.8
1.00835033823288 3.5
1.00837202286964 3.2
1.00813314061253 2.9
1.00834579267494 2.6
1.00940155446167 2.3
1.01041090778063 2
1.01346623638504 1.7
1.01773293478313 1.4
1.02602531148646 1.1
1.04092714069729 0.8
1.06710792872863 0.5
1.1 0.276049997930129
1.10690351189312 0.2
1.14525136614435 -0.1
1.20010526320651 -0.4
1.27684108914834 -0.7
1.39243664511501 -1
1.4 -1
};
\addplot [draw=none, fill=steelblue72150200]
table{%
x  y
5 -0.99885239241713
5 -0.758480645113283
4.74283859503635 -1
4.99877806737892 -1
5 -0.99885239241713
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
1.51283512085038 -0.7
1.42042795089389 -0.4
1.4 -0.320664489448313
1.34299496611414 -0.1
1.29115636110927 0.2
1.25718855684582 0.5
1.23633571851156 0.8
1.22376162287297 1.1
1.21653897846137 1.4
1.21269637480882 1.7
1.21028878133534 2
1.20922650428048 2.3
1.20806733218951 2.6
1.20783830511613 2.9
1.20790346432666 3.2
1.2078715444358 3.5
1.2082257067062 3.8
1.20798905676837 4.1
1.207638988322 4.4
1.20792327006101 4.7
1.20840812115104 5
1.12419807928258 5
1.12356229347085 4.7
1.12310258361394 4.4
1.12375450005013 4.1
1.12404483236362 3.8
1.12385090741753 3.5
1.12381313145352 3.2
1.12371854652372 2.9
1.12381068803703 2.6
1.12478187884999 2.3
1.12560984295899 2
1.12816280263549 1.7
1.13164608126069 1.4
1.13831805687106 1.1
1.14985046195998 0.8
1.16884726724727 0.5
1.1990299365012 0.2
1.24412316612924 -0.1
1.31160941523344 -0.4
1.4 -0.671682358706507
1.40861146256194 -0.7
1.51182885762507 -1
1.62870350590636 -1
1.51283512085038 -0.7
};
\addplot [draw=none, fill=cornflowerblue89162207]
table{%
x  y
4.7 -1
4.74283859503635 -1
5 -0.758480645113283
5 -0.7
5 -0.551281627645962
4.84340872005949 -0.7
4.7 -0.836272749963011
4.52109906903895 -1
4.7 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
1.7 -1
1.75014796411691 -1
1.7 -0.901336758791208
1.61705877913882 -0.7
1.51897618952844 -0.4
1.44117747389893 -0.1
1.4 0.110005874577512
1.38328278571735 0.2
1.34552984644438 0.5
1.32282097506313 0.8
1.30920518887487 1.1
1.30143187566205 1.4
1.29722994698215 1.7
1.29496771971169 2
1.29367112971097 2.3
1.29232397634199 2.6
1.29195806370853 2.9
1.29199379719981 3.2
1.29189218145407 3.5
1.29240658104877 3.8
1.29222361348662 4.1
1.29217539303006 4.4
1.29228424665116 4.7
1.29261816301951 5
1.20840812115104 5
1.20792327006101 4.7
1.207638988322 4.4
1.20798905676837 4.1
1.2082257067062 3.8
1.2078715444358 3.5
1.20790346432666 3.2
1.20783830511613 2.9
1.20806733218951 2.6
1.20922650428048 2.3
1.21028878133534 2
1.21269637480882 1.7
1.21653897846137 1.4
1.22376162287297 1.1
1.23633571851156 0.8
1.25718855684582 0.5
1.29115636110927 0.2
1.34299496611414 -0.1
1.4 -0.320664489448313
1.42042795089389 -0.4
1.51283512085038 -0.7
1.62870350590636 -1
1.7 -1
};
\addplot [draw=none, fill=cornflowerblue107174214]
table{%
x  y
4.4 -1
4.52109906903895 -1
4.7 -0.836272749963011
4.84340872005949 -0.7
5 -0.551281627645962
5 -0.4
5 -0.358041913787561
4.95596439554439 -0.4
4.7 -0.644025341633572
4.63931086536621 -0.7
4.4 -0.920508617641848
4.30889366578314 -1
4.4 -1
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
1.7 -0.901336758791208
1.75014796411691 -1
1.87874083437786 -1
1.72618794418394 -0.7
1.7 -0.641158780789914
1.617524428163 -0.4
1.5384214538516 -0.1
1.47997820806746 0.2
1.43789107877931 0.5
1.41074514420662 0.8
1.4 0.989630047697422
1.39464875487678 1.1
1.38632477286273 1.4
1.38176351915549 1.7
1.37964665808804 2
1.37811575514146 2.3
1.37658062049447 2.6
1.37607782230094 2.9
1.37608413007295 3.2
1.37591281847234 3.5
1.37658745539134 3.8
1.37645817020486 4.1
1.37671179773813 4.4
1.37664522324131 4.7
1.37682820488797 5
1.29261816301951 5
1.29228424665116 4.7
1.29217539303006 4.4
1.29222361348662 4.1
1.29240658104877 3.8
1.29189218145407 3.5
1.29199379719981 3.2
1.29195806370853 2.9
1.29232397634199 2.6
1.29367112971097 2.3
1.29496771971169 2
1.29722994698215 1.7
1.30143187566205 1.4
1.30920518887487 1.1
1.32282097506313 0.8
1.34552984644438 0.5
1.38328278571735 0.2
1.4 0.110005874577512
1.44117747389893 -0.1
1.51897618952844 -0.4
1.61705877913882 -0.7
1.7 -0.901336758791208
};
\addplot [draw=none, fill=skyblue128185218]
table{%
x  y
4.4 -0.920508617641848
4.63931086536621 -0.7
4.7 -0.644025341633572
4.95596439554439 -0.4
5 -0.358041913787561
5 -0.175813664636508
4.76471327270659 -0.4
4.7 -0.461694824574586
4.44162352576331 -0.7
4.4 -0.738353236128254
4.10012249367287 -1
4.30889366578314 -1
4.4 -0.920508617641848
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
2 -1
2.01135247754124 -1
2 -0.985647567276083
1.85443469013267 -0.7
1.7218856709094 -0.4
1.7 -0.340669448425406
1.63566543380427 -0.1
1.5776865161643 0.2
1.53671701598445 0.5
1.51060259369506 0.8
1.49432004044019 1.1
1.48486287413182 1.4
1.47948269617899 1.7
1.47693749641429 2
1.47501672197927 2.3
1.47351009501911 2.6
1.47283439020502 2.9
1.47310643599077 3.2
1.47275192153488 3.5
1.47316061817056 3.8
1.47322317153139 4.1
1.47377393126262 4.4
1.47344457723853 4.7
1.47320916712703 5
1.4 5
1.37682820488797 5
1.37664522324131 4.7
1.37671179773813 4.4
1.37645817020486 4.1
1.37658745539134 3.8
1.37591281847234 3.5
1.37608413007295 3.2
1.37607782230094 2.9
1.37658062049447 2.6
1.37811575514146 2.3
1.37964665808804 2
1.38176351915549 1.7
1.38632477286273 1.4
1.39464875487678 1.1
1.4 0.989630047697422
1.41074514420662 0.8
1.43789107877931 0.5
1.47997820806746 0.2
1.5384214538516 -0.1
1.617524428163 -0.4
1.7 -0.641158780789914
1.72618794418394 -0.7
1.87874083437786 -1
2 -1
};
\addplot [draw=none, fill=skyblue149197223]
table{%
x  y
4.1 -1
4.10012249367287 -1
4.4 -0.738353236128254
4.44162352576331 -0.7
4.7 -0.461694824574586
4.76471327270659 -0.4
5 -0.175813664636508
5 -0.1
5 0.0139218733199164
4.88130642137034 -0.1
4.7 -0.272242675558395
4.56249153501155 -0.4
4.4 -0.549273725372781
4.22926219933754 -0.7
4.1 -0.812268392982272
3.86726890431748 -1
4.1 -1
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
2 -0.985647567276083
2.01135247754124 -1
2.21041253565647 -1
2 -0.733984784263326
1.98268143608139 -0.7
1.85607586763425 -0.4
1.74835367687883 -0.1
1.7 0.0720074291815603
1.67539482426113 0.2
1.63554295318958 0.5
1.61046004318349 0.8
1.59494192918356 1.1
1.58602112942734 1.4
1.58082886535937 1.7
1.57821888167597 2
1.57627504123256 2.3
1.57531799111014 2.6
1.57461275455702 2.9
1.57526845350874 3.2
1.57474275022358 3.5
1.57450822525484 3.8
1.57484855085014 4.1
1.57559868139469 4.4
1.57500566903265 4.7
1.57421054505853 5
1.47320916712703 5
1.47344457723853 4.7
1.47377393126262 4.4
1.47322317153139 4.1
1.47316061817056 3.8
1.47275192153488 3.5
1.47310643599077 3.2
1.47283439020502 2.9
1.47351009501911 2.6
1.47501672197927 2.3
1.47693749641429 2
1.47948269617899 1.7
1.48486287413182 1.4
1.49432004044019 1.1
1.51060259369506 0.8
1.53671701598445 0.5
1.5776865161643 0.2
1.63566543380427 -0.1
1.7 -0.340669448425406
1.7218856709094 -0.4
1.85443469013267 -0.7
2 -0.985647567276083
};
\addplot [draw=none, fill=lightblue168206228]
table{%
x  y
3.8 -1
3.86726890431748 -1
4.1 -0.812268392982272
4.22926219933754 -0.7
4.4 -0.549273725372781
4.56249153501155 -0.4
4.7 -0.272242675558395
4.88130642137034 -0.1
5 0.0139218733199164
5 0.2
5 0.210905209286124
4.98866294349258 0.2
4.7 -0.0747579492660866
4.6732255777182 -0.1
4.4 -0.350423123777311
4.34421143683926 -0.4
4.1 -0.611075954250498
3.99223611298582 -0.7
3.8 -0.850689150583445
3.58870220661419 -1
3.8 -1
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
2 -0.733984784263326
2.21041253565647 -1
2.3 -1
2.5331271590733 -1
2.3 -0.845190873901491
2.1879340020585 -0.7
2 -0.423212337072807
1.99026606435911 -0.4
1.89123388798713 -0.1
1.81323225813127 0.2
1.75522095265292 0.5
1.71693992920891 0.8
1.7 1.01027538051821
1.69556381792692 1.1
1.68717938472287 1.4
1.68217503453975 1.7
1.67950026693764 2
1.67753336048585 2.3
1.67712588720117 2.6
1.67639111890901 2.9
1.67743047102671 3.2
1.67673357891227 3.5
1.67585583233913 3.8
1.67647393016889 4.1
1.67742343152676 4.4
1.67656676082676 4.7
1.67521192299003 5
1.57421054505853 5
1.57500566903265 4.7
1.57559868139469 4.4
1.57484855085014 4.1
1.57450822525484 3.8
1.57474275022358 3.5
1.57526845350874 3.2
1.57461275455702 2.9
1.57531799111014 2.6
1.57627504123256 2.3
1.57821888167597 2
1.58082886535937 1.7
1.58602112942734 1.4
1.59494192918356 1.1
1.61046004318349 0.8
1.63554295318958 0.5
1.67539482426113 0.2
1.7 0.0720074291815603
1.74835367687883 -0.1
1.85607586763425 -0.4
1.98268143608139 -0.7
2 -0.733984784263326
};
\addplot [draw=none, fill=lightblue185213234]
table{%
x  y
3.2 -1
3.5 -1
3.58870220661419 -1
3.8 -0.850689150583445
3.99223611298582 -0.7
4.1 -0.611075954250498
4.34421143683926 -0.4
4.4 -0.350423123777311
4.6732255777182 -0.1
4.7 -0.0747579492660866
4.98866294349258 0.2
5 0.210905209286124
5 0.447132199181305
4.74308134457469 0.2
4.7 0.158993898753508
4.4252833342768 -0.1
4.4 -0.123173275364555
4.1 -0.387243472601369
4.08484238598548 -0.4
3.8 -0.624934102231373
3.69557901734589 -0.7
3.5 -0.828941348743235
3.2 -0.993345188965422
3.17648122078441 -1
3.2 -1
};
\addplot [draw=none, fill=powderblue200220239]
table{%
x  y
2.3 -0.845190873901491
2.5331271590733 -1
2.6 -1
2.9 -1
3.17648122078441 -1
3.2 -0.993345188965422
3.5 -0.828941348743235
3.69557901734589 -0.7
3.8 -0.624934102231373
4.08484238598548 -0.4
4.1 -0.387243472601369
4.4 -0.123173275364555
4.4252833342768 -0.1
4.7 0.158993898753508
4.74308134457469 0.2
5 0.447132199181305
5 0.5
5 0.743443018404427
4.75026634295587 0.5
4.7 0.452212877224532
4.43444660399827 0.2
4.4 0.168071047954314
4.10448457612201 -0.1
4.1 -0.103861912105287
3.8 -0.343887892537381
3.72444253077138 -0.4
3.5 -0.54780696649047
3.22887271348967 -0.7
3.2 -0.71401757004736
2.9 -0.783202417616175
2.6 -0.742602574554383
2.53293900152644 -0.7
2.3 -0.516782364607889
2.22509341088107 -0.4
2.06446730363442 -0.1
2 0.0514911729039385
1.96457642092054 0.2
1.91400589847486 0.5
1.8808923718327 0.8
1.85951445665076 1.1
1.84748888662395 1.4
1.84067380681391 1.7
1.83673941139696 2
1.83393493950272 2.3
1.83282223886277 2.6
1.83195261352389 2.9
1.83298554353535 3.2
1.83216337532231 3.5
1.83090190689718 3.8
1.83245307297467 4.1
1.83332848239442 4.4
1.83108621461313 4.7
1.8300401031698 5
1.7 5
1.67521192299003 5
1.67656676082676 4.7
1.67742343152676 4.4
1.67647393016889 4.1
1.67585583233913 3.8
1.67673357891227 3.5
1.67743047102671 3.2
1.67639111890901 2.9
1.67712588720117 2.6
1.67753336048585 2.3
1.67950026693764 2
1.68217503453975 1.7
1.68717938472287 1.4
1.69556381792692 1.1
1.7 1.01027538051821
1.71693992920891 0.8
1.75522095265292 0.5
1.81323225813127 0.2
1.89123388798713 -0.1
1.99026606435911 -0.4
2 -0.423212337072807
2.1879340020585 -0.7
2.3 -0.845190873901491
};
\addplot [draw=none, fill=lavender210227243]
table{%
x  y
2.6 -0.742602574554383
2.9 -0.783202417616175
3.2 -0.71401757004736
3.22887271348967 -0.7
3.5 -0.54780696649047
3.72444253077138 -0.4
3.8 -0.343887892537381
4.1 -0.103861912105286
4.10448457612201 -0.1
4.4 0.168071047954314
4.43444660399827 0.2
4.7 0.452212877224532
4.75026634295587 0.5
5 0.743443018404427
5 0.8
5 1.1
5 1.18093505709419
4.9189735231449 1.1
4.7 0.885387733031289
4.61438186465087 0.8
4.4 0.598429094937477
4.29642527929621 0.5
4.1 0.322215029016766
3.96238052622675 0.2
3.8 0.0684296981018558
3.57911689117036 -0.1
3.5 -0.153730008740175
3.2 -0.311879075228259
2.9 -0.389764780672966
2.6 -0.313931784797733
2.37980647393424 -0.1
2.3 0.00335822876539257
2.22776325834805 0.2
2.14599159084063 0.5
2.09037251782066 0.8
2.05411403032324 1.1
2.0338025578734 1.4
2.02317342644439 1.7
2.01669634590857 2
2.01240458136531 2.3
2.00851023755901 2.6
2.00773441182586 2.9
2.0075366059349 3.2
2.00699677437269 3.5
2.00560347734263 3.8
2.00984052281716 4.1
2.00955457645204 4.4
2.00312519310739 4.7
2.00494455582115 5
2 5
1.8300401031698 5
1.83108621461313 4.7
1.83332848239442 4.4
1.83245307297467 4.1
1.83090190689718 3.8
1.83216337532231 3.5
1.83298554353535 3.2
1.83195261352389 2.9
1.83282223886277 2.6
1.83393493950272 2.3
1.83673941139696 2
1.84067380681391 1.7
1.84748888662395 1.4
1.85951445665076 1.1
1.8808923718327 0.8
1.91400589847486 0.5
1.96457642092054 0.2
2 0.0514911729039385
2.06446730363442 -0.1
2.22509341088107 -0.4
2.3 -0.516782364607889
2.53293900152644 -0.7
2.6 -0.742602574554383
};
\addplot [draw=none, fill=lavender221234246]
table{%
x  y
2.6 -0.313931784797733
2.9 -0.389764780672966
3.2 -0.311879075228259
3.5 -0.153730008740175
3.57911689117036 -0.1
3.8 0.0684296981018558
3.96238052622675 0.2
4.1 0.322215029016766
4.29642527929621 0.5
4.4 0.598429094937477
4.61438186465087 0.8
4.7 0.885387733031289
4.9189735231449 1.1
5 1.18093505709419
5 1.4
5 1.7
5 2
5 2.19465996785494
4.84164301570199 2
4.7 1.84102734788913
4.58519568868821 1.7
4.4 1.47936815216285
4.33412664041122 1.4
4.1 1.14265716941137
4.05954392336933 1.1
3.8 0.844930785587071
3.74840379486689 0.8
3.5 0.597928105076769
3.3294719469142 0.5
3.2 0.436608217045656
2.9 0.410119566080854
2.76716874335304 0.5
2.6 0.699195789381847
2.5664219120842 0.8
2.50662477680292 1.1
2.47050606831179 1.4
2.45121229123114 1.7
2.44065279942708 2
2.43330174905465 2.3
2.43027172275761 2.6
2.42696059904818 2.9
2.42482952041606 3.2
2.42743603530415 3.5
2.4210566167586 3.8
2.42914003291413 4.1
2.42853538808549 4.4
2.42636476513306 4.7
2.42706172207503 5
2.3 5
2.00494455582115 5
2.00312519310739 4.7
2.00955457645204 4.4
2.00984052281716 4.1
2.00560347734263 3.8
2.00699677437269 3.5
2.0075366059349 3.2
2.00773441182586 2.9
2.00851023755901 2.6
2.01240458136531 2.3
2.01669634590857 2
2.02317342644439 1.7
2.0338025578734 1.4
2.05411403032324 1.1
2.09037251782066 0.8
2.14599159084063 0.5
2.22776325834805 0.2
2.3 0.00335822876539257
2.37980647393424 -0.1
2.6 -0.313931784797733
};
\addplot [draw=none, fill=lavender231240249]
table{%
x  y
2.9 0.410119566080854
3.2 0.436608217045656
3.3294719469142 0.5
3.5 0.597928105076769
3.74840379486689 0.8
3.8 0.84493078558707
4.05954392336933 1.1
4.1 1.14265716941137
4.33412664041122 1.4
4.4 1.47936815216285
4.58519568868821 1.7
4.7 1.84102734788913
4.84164301570199 2
5 2.19465996785494
5 2.3
5 2.6
5 2.9
5 3.2
5 3.5
5 3.8
5 4.1
5 4.4
5 4.7
5 5
4.7 5
4.4 5
4.1 5
3.8 5
3.5 5
3.2 5
2.9 5
2.6 5
2.42706172207503 5
2.42636476513306 4.7
2.42853538808549 4.4
2.42914003291413 4.1
2.4210566167586 3.8
2.42743603530415 3.5
2.42482952041606 3.2
2.42696059904818 2.9
2.43027172275761 2.6
2.43330174905465 2.3
2.44065279942708 2
2.45121229123114 1.7
2.47050606831179 1.4
2.50662477680292 1.1
2.5664219120842 0.8
2.6 0.699195789381847
2.76716874335304 0.5
2.9 0.410119566080854
};
\addplot [semithick, steelblue31119180, mark=*, mark size=2.5, mark options={solid,fill=black,draw=white}]
table {%
3.8 3.2
};
\coordinate (CVI_mean_lml_b) at (axis cs:4.1,2.5999999999999996);
\coordinate (CVI_mean_lml_ep_b) at (axis cs:4.1,3.2);
\end{axis}



==> table/3_isotropic_sparse_test_acc.tex <==
\begin{tabular}{lc|ccc}
%test acc (this table has been automatically generated, do not alter manually)
\toprule
{} &($n$, $d$)     &      VI(Scipy)      &          VI         &         Ours        \\
\hline
   {\sc titanic}     &      (2201, 4)       & $\bf 0.997{\pm}0.002 $ & $\bf 0.996{\pm}0.003 $ & $\bf 0.993{\pm}0.001 $ \\
    {\sc ozone}      &      (2536, 73)      & $\bf 0.971{\pm}0.009 $ & $\bf 0.971{\pm}0.009 $ & $\bf 0.945{\pm}0.035 $ \\
 {\sc chess-krvkp}   &      (3196, 37)      & $  0.989{\pm}0.005   $ & $\bf 0.991{\pm}0.005 $ & $  0.875{\pm}0.013   $ \\
     {\sc bank}      &      (4521, 17)      & $\bf 0.897{\pm}0.003 $ & $\bf 0.896{\pm}0.003 $ & $\bf 0.897{\pm}0.004 $ \\
    {\sc musk-2}     &     (6598, 167)      & $\bf 1.000{\pm}0.000 $ & $\bf 1.000{\pm}0.000 $ & $  0.927{\pm}0.004   $ \\
   {\sc twonorm}     &      (7400, 21)      & $\bf 0.977{\pm}0.003 $ & $\bf 0.977{\pm}0.003 $ & $  0.971{\pm}0.005   $ \\
   {\sc ringnorm}    &      (7400, 21)      & $\bf 0.985{\pm}0.005 $ & $\bf 0.986{\pm}0.005 $ & $\bf 0.986{\pm}0.005 $ \\
   {\sc mushroom}    &      (8124, 22)      & $\bf 1.000{\pm}0.000 $ & $\bf 1.000{\pm}0.000 $ & $\bf 1.000{\pm}0.000 $ \\
\hline
    {Bold Count}     & {}& $7$            & $8$            & $5$            \\
\bottomrule\end{tabular}


==> table/3_isotropic_sparse_test_lpd.tex <==
\begin{tabular}{lc|ccc}
%test lpd (this table has been automatically generated, do not alter manually)
\toprule
{} &($n$, $d$)     &      VI(Scipy)      &          VI         &         Ours        \\
\hline
   {\sc titanic}     &      (2201, 4)       & $\bf -0.010{\pm}0.003$ & $  -0.020{\pm}0.004  $ & $  -0.045{\pm}0.005  $ \\
    {\sc ozone}      &      (2536, 73)      & $\bf -0.086{\pm}0.021$ & $\bf -0.085{\pm}0.022$ & $  -0.691{\pm}0.001  $ \\
 {\sc chess-krvkp}   &      (3196, 37)      & $\bf -0.038{\pm}0.010$ & $  -0.047{\pm}0.010  $ & $  -0.693{\pm}0.000  $ \\
     {\sc bank}      &      (4521, 17)      & $\bf -0.249{\pm}0.006$ & $\bf -0.249{\pm}0.006$ & $\bf -0.247{\pm}0.007$ \\
    {\sc musk-2}     &     (6598, 167)      & $\bf -0.006{\pm}0.000$ & $  -0.017{\pm}0.001  $ & $  -0.645{\pm}0.005  $ \\
   {\sc twonorm}     &      (7400, 21)      & $\bf -0.060{\pm}0.008$ & $\bf -0.060{\pm}0.008$ & $  -0.566{\pm}0.255  $ \\
   {\sc ringnorm}    &      (7400, 21)      & $\bf -0.045{\pm}0.007$ & $\bf -0.047{\pm}0.006$ & $\bf -0.048{\pm}0.005$ \\
   {\sc mushroom}    &      (8124, 22)      & $\bf -0.001{\pm}0.000$ & $  -0.003{\pm}0.000  $ & $  -0.006{\pm}0.001  $ \\
\hline
    {Bold Count}     & {}& $8$            & $4$            & $2$            \\
\bottomrule\end{tabular}


==> table/ard_test_acc_order.tex <==
\begin{tabular}{l|ccccc|c}
%test acc order (this table has been automatically generated, do not alter manually)
\toprule
{} &         LA          &         EP          &         VI          &        CVI          &       EPCVI         &($n$, $d$)     \\
\hline
  {\sc fertility}    & $       2.200        $ & $     \bf 3.000      $ & $       1.400        $ & $       1.400        $ & $       1.400        $ &      (100, 10)       \\
{\sc statlog-heart}  & $       2.800        $ & $     \bf 4.400      $ & $       1.400        $ & $       1.600        $ & $       2.000        $ &      (270, 14)       \\
  {\sc ionosphere}   & $       2.200        $ & $       1.600        $ & $       2.200        $ & $       2.800        $ & $     \bf 3.000      $ &      (351, 34)       \\
   {\sc planning}    & $       2.600        $ & $     \bf 2.800      $ & $       2.200        $ & $       1.800        $ & $       1.200        $ &      (182, 13)       \\
{\sc pittsburg-bridges-T-OR-D} & $       1.200        $ & $     \bf 2.600      $ & $       1.600        $ & $       1.600        $ & $       1.600        $ &       (102, 8)       \\
{\sc heart-hungarian} & $     \bf 1.000      $ & $     \bf 1.000      $ & $     \bf 1.000      $ & $     \bf 1.000      $ & $     \bf 1.000      $ &      (294, 13)       \\
{\sc conn-bench-sonar-mines-rocks} & $     \bf 1.400      $ & $     \bf 1.400      $ & $     \bf 1.400      $ & $       1.000        $ & $       1.000        $ &      (208, 61)       \\
{\sc congressional-voting} & $       1.800        $ & $       2.600        $ & $       1.800        $ & $     \bf 2.800      $ & $     \bf 2.800      $ &      (435, 17)       \\
{\sc echocardiogram} & $       1.800        $ & $     \bf 4.000      $ & $       1.800        $ & $       1.400        $ & $       1.200        $ &      (131, 11)       \\
{\sc molec-biol-promoter} & $       1.400        $ & $       2.200        $ & $       2.200        $ & $     \bf 3.200      $ & $     \bf 3.200      $ &      (106, 58)       \\
{\sc haberman-survival} & $       1.000        $ & $     \bf 2.000      $ & $       1.200        $ & $       1.200        $ & $       1.200        $ &       (306, 4)       \\
  {\sc parkinsons}   & $       2.000        $ & $       1.000        $ & $       1.800        $ & $       1.800        $ & $     \bf 2.200      $ &      (195, 23)       \\
{\sc vertebral-column-2clases} & $     \bf 2.000      $ & $       1.200        $ & $       1.000        $ & $       1.200        $ & $       1.200        $ &       (310, 7)       \\
    {\sc spectf}     & $     \bf 3.200      $ & $       2.000        $ & $       2.600        $ & $       2.000        $ & $       2.600        $ &      (267, 45)       \\
{\sc breast-cancer}  & $       1.000        $ & $     \bf 1.800      $ & $       1.000        $ & $       1.000        $ & $       1.000        $ &      (286, 10)       \\
\hline
  {\sc Bold Count}   & $4$            & $9$            & $2$            & $3$            & $5$            & {}\\
\bottomrule\end{tabular}


==> table/ard_test_lpd_order.tex <==
\begin{tabular}{l|ccccc|c}
%test lpd order (this table has been automatically generated, do not alter manually)
\toprule
{} &         LA          &         EP          &         VI          &        CVI          &       EPCVI         &($n$, $d$)     \\
\hline
  {\sc fertility}    & $       3.800        $ & $     \bf 4.600      $ & $       2.200        $ & $       2.600        $ & $       1.800        $ &      (100, 10)       \\
{\sc statlog-heart}  & $       3.400        $ & $     \bf 5.000      $ & $       3.200        $ & $       2.200        $ & $       1.200        $ &      (270, 14)       \\
  {\sc ionosphere}   & $       1.800        $ & $       2.000        $ & $       3.000        $ & $       4.000        $ & $     \bf 4.200      $ &      (351, 34)       \\
   {\sc planning}    & $     \bf 4.000      $ & $       3.000        $ & $       3.600        $ & $       3.000        $ & $       1.400        $ &      (182, 13)       \\
{\sc pittsburg-bridges-T-OR-D} & $     \bf 3.600      $ & $       2.600        $ & $       3.000        $ & $       2.800        $ & $       3.000        $ &       (102, 8)       \\
{\sc heart-hungarian} & $       1.000        $ & $       2.000        $ & $     \bf 4.600      $ & $       3.200        $ & $       4.200        $ &      (294, 13)       \\
{\sc conn-bench-sonar-mines-rocks} & $       1.000        $ & $       2.000        $ & $     \bf 4.600      $ & $       3.400        $ & $       4.000        $ &      (208, 61)       \\
{\sc congressional-voting} & $       2.800        $ & $       3.000        $ & $       1.400        $ & $     \bf 4.200      $ & $       3.600        $ &      (435, 17)       \\
{\sc echocardiogram} & $       3.600        $ & $     \bf 3.800      $ & $       3.000        $ & $       3.000        $ & $       1.600        $ &      (131, 11)       \\
{\sc molec-biol-promoter} & $       1.400        $ & $       2.200        $ & $       3.200        $ & $       3.600        $ & $     \bf 4.600      $ &      (106, 58)       \\
{\sc haberman-survival} & $       3.200        $ & $     \bf 3.400      $ & $       2.400        $ & $       2.600        $ & $     \bf 3.400      $ &       (306, 4)       \\
  {\sc parkinsons}   & $       1.400        $ & $       1.600        $ & $       4.000        $ & $       3.400        $ & $     \bf 4.600      $ &      (195, 23)       \\
{\sc vertebral-column-2clases} & $       1.000        $ & $       2.000        $ & $     \bf 4.600      $ & $       4.000        $ & $       3.400        $ &       (310, 7)       \\
    {\sc spectf}     & $       1.400        $ & $       1.600        $ & $       3.800        $ & $       3.600        $ & $     \bf 4.600      $ &      (267, 45)       \\
{\sc breast-cancer}  & $       1.000        $ & $       2.000        $ & $     \bf 5.000      $ & $       3.400        $ & $       3.600        $ &      (286, 10)       \\
\hline
  {\sc Bold Count}   & $2$            & $4$            & $4$            & $1$            & $5$            & {}\\
\bottomrule\end{tabular}


==> table/foo.tex <==
A & B & C \\


==> table/isotropic_sparse_test_acc.tex <==
\begin{tabular}{lc|ccc}
%test acc (this table has been automatically generated, do not alter manually)
\toprule
{} &($n$, $d$)     &          VI         &         Ours        \\
\hline
   {\sc titanic}     &      (2201, 4)       & $\bf 0.996{\pm}0.002 $ & $\bf 0.994{\pm}0.002 $ \\
     {\sc bank}      &      (4521, 17)      & $\bf 0.897{\pm}0.003 $ & $\bf 0.898{\pm}0.006 $ \\
\hline
    {Bold Count}     & {}& $2$            & $2$            \\
\bottomrule\end{tabular}


==> table/isotropic_sparse_test_acc_order.tex <==
\begin{tabular}{lc|ccc}
%test acc order (this table has been automatically generated, do not alter manually)
\toprule
{} &($n$, $d$)     &          VI         &         Ours        \\
\hline
   {\sc titanic}     &      (2201, 4)       & $      \bf 1.8       $ & $        1.2         $ \\
     {\sc bank}      &      (4521, 17)      & $        1.4         $ & $      \bf 1.6       $ \\
\hline
    {Bold Count}     & {}& $1$            & $1$            \\
\bottomrule\end{tabular}


==> table/isotropic_sparse_test_lpd_order.tex <==
\begin{tabular}{lc|cccc}
%test lpd order (this table has been automatically generated, do not alter manually)
\toprule
{} &($n$, $d$)     &          LA         &          EP         &          VI         &         Ours        \\
\hline
   {\sc titanic}     &      (2201, 4)       & $        1.0         $ & $        3.0         $ & $      \bf 4.0       $ & $        2.0         $ \\
     {\sc bank}      &      (4521, 17)      & $        2.6         $ & $      \bf 3.8       $ & $        1.2         $ & $        2.4         $ \\
   {\sc twonorm}     &      (7400, 21)      & $        3.0         $ & $        2.8         $ & $      \bf 3.2       $ & $        1.0         $ \\
   {\sc mushroom}    &      (8124, 22)      & $        1.0         $ & $        3.0         $ & $      \bf 4.0       $ & $        2.0         $ \\
    {\sc magic}      &     (19020, 11)      & $        2.2         $ & $        1.4         $ & $      \bf 4.0       $ & $        2.4         $ \\
\hline
    {Bold Count}     & {}& $0$            & $1$            & $4$            & $0$            \\
\bottomrule\end{tabular}


==> table/isotropic_test_acc.tex <==
\begin{tabular}{lc|cccc}
%test acc (this table has been automatically generated, do not alter manually)
\toprule
{} &($n$, $d$)     &          LA         &          EP         &          VI         &         Ours        \\
\hline
    {\sc trains}     &       (10, 30)       & $\bf 0.700{\pm}0.400 $ & $\bf 0.800{\pm}0.245 $ & $\bf 0.800{\pm}0.245 $ & $\bf 0.800{\pm}0.245 $ \\
   {\sc balloons}    &       (16, 5)        & $\bf 0.667{\pm}0.298 $ & $\bf 0.667{\pm}0.298 $ & $\bf 0.667{\pm}0.298 $ & $\bf 0.667{\pm}0.298 $ \\
  {\sc fertility}    &      (100, 10)       & $\bf 0.880{\pm}0.060 $ & $\bf 0.880{\pm}0.060 $ & $\bf 0.880{\pm}0.060 $ & $\bf 0.880{\pm}0.060 $ \\
{\sc pittsburg-bridges-T-OR-D} &       (102, 8)       & $\bf 0.863{\pm}0.036 $ & $\bf 0.883{\pm}0.066 $ & $\bf 0.863{\pm}0.036 $ & $\bf 0.863{\pm}0.036 $ \\
{\sc acute-inflammation} &       (120, 7)       & $\bf 1.000{\pm}0.000 $ & $\bf 1.000{\pm}0.000 $ & $\bf 1.000{\pm}0.000 $ & $\bf 1.000{\pm}0.000 $ \\
{\sc acute-nephritis} &       (120, 7)       & $\bf 1.000{\pm}0.000 $ & $\bf 1.000{\pm}0.000 $ & $\bf 1.000{\pm}0.000 $ & $\bf 1.000{\pm}0.000 $ \\
{\sc echocardiogram} &      (131, 11)       & $  0.808{\pm}0.061   $ & $\bf 0.847{\pm}0.043 $ & $\bf 0.785{\pm}0.076 $ & $  0.778{\pm}0.063   $ \\
  {\sc hepatitis}    &      (155, 20)       & $\bf 0.813{\pm}0.024 $ & $\bf 0.813{\pm}0.032 $ & $\bf 0.813{\pm}0.024 $ & $\bf 0.832{\pm}0.024 $ \\
   {\sc planning}    &      (182, 13)       & $\bf 0.714{\pm}0.038 $ & $\bf 0.714{\pm}0.038 $ & $\bf 0.714{\pm}0.038 $ & $\bf 0.714{\pm}0.038 $ \\
{\sc breast-cancer-wisc-prog} &      (198, 34)       & $\bf 0.793{\pm}0.051 $ & $\bf 0.793{\pm}0.069 $ & $\bf 0.793{\pm}0.051 $ & $\bf 0.793{\pm}0.051 $ \\
    {\sc spect}      &      (265, 23)       & $\bf 0.706{\pm}0.031 $ & $\bf 0.698{\pm}0.027 $ & $\bf 0.702{\pm}0.028 $ & $\bf 0.706{\pm}0.023 $ \\
{\sc statlog-heart}  &      (270, 14)       & $\bf 0.830{\pm}0.036 $ & $\bf 0.833{\pm}0.039 $ & $\bf 0.830{\pm}0.036 $ & $\bf 0.826{\pm}0.034 $ \\
{\sc haberman-survival} &       (306, 4)       & $\bf 0.725{\pm}0.039 $ & $\bf 0.719{\pm}0.036 $ & $\bf 0.725{\pm}0.039 $ & $\bf 0.725{\pm}0.039 $ \\
  {\sc ionosphere}   &      (351, 34)       & $\bf 0.932{\pm}0.025 $ & $\bf 0.932{\pm}0.024 $ & $\bf 0.946{\pm}0.024 $ & $\bf 0.946{\pm}0.028 $ \\
 {\sc horse-colic}   &      (368, 26)       & $\bf 0.799{\pm}0.035 $ & $\bf 0.807{\pm}0.032 $ & $\bf 0.791{\pm}0.045 $ & $\bf 0.802{\pm}0.039 $ \\
{\sc congressional-voting} &      (435, 17)       & $\bf 0.605{\pm}0.024 $ & $\bf 0.593{\pm}0.014 $ & $\bf 0.595{\pm}0.013 $ & $\bf 0.591{\pm}0.016 $ \\
{\sc ilpd-indian-liver} &      (583, 10)       & $\bf 0.719{\pm}0.025 $ & $\bf 0.712{\pm}0.020 $ & $\bf 0.717{\pm}0.029 $ & $\bf 0.719{\pm}0.028 $ \\
{\sc credit-approval} &      (690, 16)       & $\bf 0.859{\pm}0.026 $ & $\bf 0.864{\pm}0.020 $ & $\bf 0.864{\pm}0.024 $ & $\bf 0.862{\pm}0.026 $ \\
{\sc statlog-australian-credit} &      (690, 15)       & $\bf 0.678{\pm}0.028 $ & $\bf 0.677{\pm}0.021 $ & $\bf 0.678{\pm}0.028 $ & $\bf 0.678{\pm}0.028 $ \\
{\sc breast-cancer-wisc} &      (699, 10)       & $\bf 0.969{\pm}0.016 $ & $\bf 0.969{\pm}0.016 $ & $\bf 0.969{\pm}0.016 $ & $\bf 0.969{\pm}0.016 $ \\
    {\sc blood}      &       (748, 5)       & $\bf 0.785{\pm}0.042 $ & $\bf 0.785{\pm}0.041 $ & $\bf 0.786{\pm}0.044 $ & $\bf 0.786{\pm}0.044 $ \\
     {\sc pima}      &       (768, 9)       & $\bf 0.764{\pm}0.027 $ & $\bf 0.766{\pm}0.025 $ & $\bf 0.767{\pm}0.026 $ & $\bf 0.767{\pm}0.026 $ \\
 {\sc mammographic}  &       (961, 6)       & $\bf 0.824{\pm}0.019 $ & $\bf 0.823{\pm}0.017 $ & $\bf 0.823{\pm}0.019 $ & $\bf 0.823{\pm}0.019 $ \\
{\sc statlog-german-credit} &      (1000, 25)      & $\bf 0.770{\pm}0.039 $ & $\bf 0.763{\pm}0.038 $ & $\bf 0.768{\pm}0.038 $ & $\bf 0.769{\pm}0.037 $ \\
\hline
    {Bold Count}     & {}& $23$           & $24$           & $24$           & $23$           \\
\bottomrule\end{tabular}


==> table/isotropic_test_acc_order.tex <==
\begin{tabular}{lc|cccc}
%test acc order (this table has been automatically generated, do not alter manually)
\toprule
{} &($n$, $d$)     &          LA         &          EP         &          VI         &         Ours        \\
\hline
    {\sc trains}     &       (10, 30)       & $       1.000        $ & $     \bf 1.200      $ & $     \bf 1.200      $ & $     \bf 1.200      $ \\
   {\sc balloons}    &       (16, 5)        & $     \bf 1.000      $ & $     \bf 1.000      $ & $     \bf 1.000      $ & $     \bf 1.000      $ \\
  {\sc fertility}    &      (100, 10)       & $     \bf 1.000      $ & $     \bf 1.000      $ & $     \bf 1.000      $ & $     \bf 1.000      $ \\
{\sc pittsburg-bridges-T-OR-D} &       (102, 8)       & $       1.200        $ & $     \bf 1.600      $ & $       1.200        $ & $       1.200        $ \\
{\sc acute-inflammation} &       (120, 7)       & $     \bf 1.000      $ & $     \bf 1.000      $ & $     \bf 1.000      $ & $     \bf 1.000      $ \\
{\sc acute-nephritis} &       (120, 7)       & $     \bf 1.000      $ & $     \bf 1.000      $ & $     \bf 1.000      $ & $     \bf 1.000      $ \\
{\sc echocardiogram} &      (131, 11)       & $       2.000        $ & $     \bf 3.600      $ & $       1.200        $ & $       1.000        $ \\
  {\sc hepatitis}    &      (155, 20)       & $       1.400        $ & $       1.600        $ & $       1.400        $ & $     \bf 2.200      $ \\
   {\sc planning}    &      (182, 13)       & $     \bf 1.000      $ & $     \bf 1.000      $ & $     \bf 1.000      $ & $     \bf 1.000      $ \\
{\sc breast-cancer-wisc-prog} &      (198, 34)       & $       1.400        $ & $     \bf 2.800      $ & $       1.400        $ & $       1.400        $ \\
    {\sc spect}      &      (265, 23)       & $       1.800        $ & $       1.400        $ & $       1.400        $ & $     \bf 2.000      $ \\
{\sc statlog-heart}  &      (270, 14)       & $       1.200        $ & $     \bf 1.600      $ & $       1.200        $ & $       1.000        $ \\
{\sc haberman-survival} &       (306, 4)       & $     \bf 1.400      $ & $       1.000        $ & $     \bf 1.400      $ & $     \bf 1.400      $ \\
  {\sc ionosphere}   &      (351, 34)       & $       1.800        $ & $       1.600        $ & $     \bf 2.600      $ & $       2.400        $ \\
 {\sc horse-colic}   &      (368, 26)       & $       1.800        $ & $     \bf 2.800      $ & $       1.400        $ & $       2.400        $ \\
{\sc congressional-voting} &      (435, 17)       & $     \bf 1.600      $ & $       1.200        $ & $       1.400        $ & $       1.000        $ \\
{\sc ilpd-indian-liver} &      (583, 10)       & $     \bf 2.200      $ & $       1.400        $ & $       1.600        $ & $     \bf 2.200      $ \\
{\sc credit-approval} &      (690, 16)       & $       1.000        $ & $       1.600        $ & $     \bf 2.200      $ & $       1.800        $ \\
{\sc statlog-australian-credit} &      (690, 15)       & $     \bf 1.600      $ & $     \bf 1.600      $ & $     \bf 1.600      $ & $     \bf 1.600      $ \\
{\sc breast-cancer-wisc} &      (699, 10)       & $     \bf 1.000      $ & $     \bf 1.000      $ & $     \bf 1.000      $ & $     \bf 1.000      $ \\
    {\sc blood}      &       (748, 5)       & $       1.400        $ & $     \bf 2.200      $ & $       1.800        $ & $       1.800        $ \\
     {\sc pima}      &       (768, 9)       & $       1.000        $ & $       1.200        $ & $     \bf 1.600      $ & $     \bf 1.600      $ \\
 {\sc mammographic}  &       (961, 6)       & $     \bf 1.800      $ & $       1.600        $ & $       1.200        $ & $       1.200        $ \\
{\sc statlog-german-credit} &      (1000, 25)      & $     \bf 2.200      $ & $       1.200        $ & $       1.600        $ & $       1.800        $ \\
\hline
    {Bold Count}     & {}& $12$           & $14$           & $12$           & $13$           \\
\bottomrule\end{tabular}


==> table/isotropic_test_lpd.tex <==
\begin{tabular}{lc|cccc}
%test lpd (this table has been automatically generated, do not alter manually)
\toprule
{} &($n$, $d$)     &          LA         &          EP         &          VI         &         Ours        \\
\hline
    {\sc trains}     &       (10, 30)       & $\bf -0.695{\pm}0.011$ & $\bf -0.687{\pm}0.023$ & $\bf -0.692{\pm}0.023$ & $\bf -0.681{\pm}0.042$ \\
   {\sc balloons}    &       (16, 5)        & $\bf -0.707{\pm}0.146$ & $\bf -0.684{\pm}0.161$ & $\bf -0.711{\pm}0.239$ & $\bf -0.657{\pm}0.267$ \\
  {\sc fertility}    &      (100, 10)       & $\bf -0.379{\pm}0.099$ & $\bf -0.384{\pm}0.138$ & $\bf -0.378{\pm}0.103$ & $\bf -0.379{\pm}0.103$ \\
{\sc pittsburg-bridges-T-OR-D} &       (102, 8)       & $\bf -0.306{\pm}0.044$ & $\bf -0.316{\pm}0.060$ & $\bf -0.295{\pm}0.057$ & $\bf -0.296{\pm}0.059$ \\
{\sc acute-inflammation} &       (120, 7)       & $  -0.172{\pm}0.033  $ & $  -0.055{\pm}0.005  $ & $  -0.008{\pm}0.001  $ & $\bf -0.007{\pm}0.001$ \\
{\sc acute-nephritis} &       (120, 7)       & $  -0.203{\pm}0.010  $ & $  -0.047{\pm}0.009  $ & $  -0.006{\pm}0.002  $ & $\bf -0.005{\pm}0.001$ \\
{\sc echocardiogram} &      (131, 11)       & $\bf -0.420{\pm}0.073$ & $\bf -0.412{\pm}0.084$ & $\bf -0.420{\pm}0.085$ & $\bf -0.421{\pm}0.086$ \\
  {\sc hepatitis}    &      (155, 20)       & $\bf -0.369{\pm}0.043$ & $\bf -0.376{\pm}0.046$ & $\bf -0.361{\pm}0.051$ & $\bf -0.361{\pm}0.052$ \\
   {\sc planning}    &      (182, 13)       & $\bf -0.602{\pm}0.032$ & $  -0.638{\pm}0.020  $ & $\bf -0.602{\pm}0.032$ & $\bf -0.602{\pm}0.032$ \\
{\sc breast-cancer-wisc-prog} &      (198, 34)       & $\bf -0.460{\pm}0.063$ & $\bf -0.478{\pm}0.083$ & $\bf -0.458{\pm}0.071$ & $\bf -0.458{\pm}0.070$ \\
    {\sc spect}      &      (265, 23)       & $\bf -0.587{\pm}0.045$ & $\bf -0.587{\pm}0.052$ & $\bf -0.589{\pm}0.050$ & $\bf -0.590{\pm}0.051$ \\
{\sc statlog-heart}  &      (270, 14)       & $\bf -0.392{\pm}0.071$ & $\bf -0.380{\pm}0.058$ & $\bf -0.394{\pm}0.080$ & $\bf -0.395{\pm}0.080$ \\
{\sc haberman-survival} &       (306, 4)       & $\bf -0.535{\pm}0.050$ & $\bf -0.539{\pm}0.059$ & $\bf -0.537{\pm}0.054$ & $\bf -0.537{\pm}0.054$ \\
  {\sc ionosphere}   &      (351, 34)       & $  -0.221{\pm}0.021  $ & $  -0.227{\pm}0.016  $ & $\bf -0.169{\pm}0.031$ & $\bf -0.169{\pm}0.033$ \\
 {\sc horse-colic}   &      (368, 26)       & $  -0.465{\pm}0.058  $ & $\bf -0.455{\pm}0.060$ & $\bf -0.466{\pm}0.068$ & $\bf -0.469{\pm}0.068$ \\
{\sc congressional-voting} &      (435, 17)       & $\bf -0.636{\pm}0.026$ & $\bf -0.633{\pm}0.027$ & $\bf -0.636{\pm}0.029$ & $\bf -0.636{\pm}0.029$ \\
{\sc ilpd-indian-liver} &      (583, 10)       & $\bf -0.516{\pm}0.033$ & $\bf -0.521{\pm}0.033$ & $\bf -0.516{\pm}0.037$ & $\bf -0.516{\pm}0.037$ \\
{\sc credit-approval} &      (690, 16)       & $\bf -0.342{\pm}0.008$ & $\bf -0.343{\pm}0.012$ & $\bf -0.341{\pm}0.008$ & $\bf -0.341{\pm}0.009$ \\
{\sc statlog-australian-credit} &      (690, 15)       & $\bf -0.627{\pm}0.022$ & $\bf -0.636{\pm}0.030$ & $\bf -0.627{\pm}0.023$ & $\bf -0.627{\pm}0.023$ \\
{\sc breast-cancer-wisc} &      (699, 10)       & $\bf -0.091{\pm}0.030$ & $\bf -0.092{\pm}0.028$ & $\bf -0.091{\pm}0.037$ & $\bf -0.091{\pm}0.037$ \\
    {\sc blood}      &       (748, 5)       & $\bf -0.475{\pm}0.043$ & $\bf -0.476{\pm}0.045$ & $\bf -0.476{\pm}0.044$ & $\bf -0.476{\pm}0.044$ \\
     {\sc pima}      &       (768, 9)       & $\bf -0.470{\pm}0.031$ & $\bf -0.472{\pm}0.035$ & $\bf -0.471{\pm}0.033$ & $\bf -0.471{\pm}0.033$ \\
 {\sc mammographic}  &       (961, 6)       & $\bf -0.408{\pm}0.037$ & $\bf -0.408{\pm}0.041$ & $\bf -0.408{\pm}0.039$ & $\bf -0.408{\pm}0.039$ \\
{\sc statlog-german-credit} &      (1000, 25)      & $\bf -0.493{\pm}0.040$ & $\bf -0.493{\pm}0.041$ & $\bf -0.493{\pm}0.043$ & $\bf -0.494{\pm}0.043$ \\
\hline
    {Bold Count}     & {}& $20$           & $20$           & $22$           & $24$           \\
\bottomrule\end{tabular}


==> table/isotropic_test_lpd_order.tex <==
\begin{tabular}{lc|cccc}
%test lpd order (this table has been automatically generated, do not alter manually)
\toprule
{} &($n$, $d$)     &          LA         &          EP         &          VI         &         Ours        \\
\hline
    {\sc trains}     &       (10, 30)       & $       1.800        $ & $       3.000        $ & $       1.800        $ & $     \bf 3.400      $ \\
   {\sc balloons}    &       (16, 5)        & $       2.200        $ & $       2.400        $ & $       2.400        $ & $     \bf 3.000      $ \\
  {\sc fertility}    &      (100, 10)       & $       2.600        $ & $       2.200        $ & $       2.200        $ & $     \bf 3.000      $ \\
{\sc pittsburg-bridges-T-OR-D} &       (102, 8)       & $       2.600        $ & $       1.600        $ & $     \bf 3.000      $ & $       2.800        $ \\
{\sc acute-inflammation} &       (120, 7)       & $       1.000        $ & $       2.000        $ & $       3.000        $ & $     \bf 4.000      $ \\
{\sc acute-nephritis} &       (120, 7)       & $       1.000        $ & $       2.000        $ & $       3.000        $ & $     \bf 4.000      $ \\
{\sc echocardiogram} &      (131, 11)       & $       2.000        $ & $     \bf 2.800      $ & $       2.600        $ & $       2.600        $ \\
  {\sc hepatitis}    &      (155, 20)       & $       2.600        $ & $       1.600        $ & $       2.800        $ & $     \bf 3.000      $ \\
   {\sc planning}    &      (182, 13)       & $     \bf 3.200      $ & $       1.000        $ & $       3.000        $ & $       2.800        $ \\
{\sc breast-cancer-wisc-prog} &      (198, 34)       & $       2.400        $ & $       1.600        $ & $     \bf 3.000      $ & $     \bf 3.000      $ \\
    {\sc spect}      &      (265, 23)       & $       2.200        $ & $       2.600        $ & $     \bf 2.800      $ & $       2.400        $ \\
{\sc statlog-heart}  &      (270, 14)       & $       2.000        $ & $     \bf 3.400      $ & $       2.400        $ & $       2.200        $ \\
{\sc haberman-survival} &       (306, 4)       & $       2.600        $ & $     \bf 2.800      $ & $       2.200        $ & $       2.400        $ \\
  {\sc ionosphere}   &      (351, 34)       & $       1.800        $ & $       1.200        $ & $       3.400        $ & $     \bf 3.600      $ \\
 {\sc horse-colic}   &      (368, 26)       & $       2.400        $ & $     \bf 3.600      $ & $       1.600        $ & $       2.400        $ \\
{\sc congressional-voting} &      (435, 17)       & $       2.000        $ & $     \bf 3.000      $ & $       2.400        $ & $       2.600        $ \\
{\sc ilpd-indian-liver} &      (583, 10)       & $       2.600        $ & $       1.600        $ & $       2.800        $ & $     \bf 3.000      $ \\
{\sc credit-approval} &      (690, 16)       & $       2.400        $ & $       2.200        $ & $       2.600        $ & $     \bf 2.800      $ \\
{\sc statlog-australian-credit} &      (690, 15)       & $       2.400        $ & $       1.000        $ & $     \bf 3.400      $ & $       3.200        $ \\
{\sc breast-cancer-wisc} &      (699, 10)       & $       2.200        $ & $       1.600        $ & $       3.000        $ & $     \bf 3.200      $ \\
    {\sc blood}      &       (748, 5)       & $       2.400        $ & $       2.200        $ & $       2.600        $ & $     \bf 2.800      $ \\
     {\sc pima}      &       (768, 9)       & $       2.200        $ & $     \bf 2.800      $ & $       2.600        $ & $       2.400        $ \\
 {\sc mammographic}  &       (961, 6)       & $       2.600        $ & $     \bf 3.200      $ & $       2.200        $ & $       2.000        $ \\
{\sc statlog-german-credit} &      (1000, 25)      & $       2.000        $ & $       2.600        $ & $     \bf 2.800      $ & $       2.600        $ \\
\hline
    {Bold Count}     & {}& $1$            & $7$            & $5$            & $12$           \\
\bottomrule\end{tabular}


==> table/new_isotropic_test_acc_order.tex <==
\begin{tabular}{lc|ccccc}
%test acc order (this table has been automatically generated, do not alter manually)
\toprule
{} &($n$, $d$)     &          LA         &          EP         &          VI         &         Ours        \\
\hline
    {\sc trains}     &       (10, 30)       & $        1.0         $ & $      \bf 1.2       $ & $      \bf 1.2       $ & $      \bf 1.2       $ \\
   {\sc balloons}    &       (16, 5)        & $      \bf 1.0       $ & $      \bf 1.0       $ & $      \bf 1.0       $ & $      \bf 1.0       $ \\
  {\sc fertility}    &      (100, 10)       & $      \bf 1.0       $ & $      \bf 1.0       $ & $      \bf 1.0       $ & $      \bf 1.0       $ \\
{\sc pittsburg-bridges-T-OR-D} &       (102, 8)       & $        1.2         $ & $      \bf 1.6       $ & $        1.2         $ & $        1.2         $ \\
{\sc acute-nephritis} &       (120, 7)       & $      \bf 1.0       $ & $      \bf 1.0       $ & $      \bf 1.0       $ & $      \bf 1.0       $ \\
{\sc acute-inflammation} &       (120, 7)       & $      \bf 1.0       $ & $      \bf 1.0       $ & $      \bf 1.0       $ & $      \bf 1.0       $ \\
{\sc echocardiogram} &      (131, 11)       & $        2.0         $ & $      \bf 3.6       $ & $        1.2         $ & $        1.0         $ \\
  {\sc hepatitis}    &      (155, 20)       & $        1.4         $ & $        1.6         $ & $        1.4         $ & $      \bf 2.2       $ \\
  {\sc parkinsons}   &      (195, 23)       & $      \bf 2.2       $ & $        1.0         $ & $        1.8         $ & $      \bf 2.2       $ \\
{\sc breast-cancer-wisc-prog} &      (198, 34)       & $        1.4         $ & $      \bf 2.8       $ & $        1.4         $ & $        1.4         $ \\
    {\sc spect}      &      (265, 23)       & $        1.8         $ & $        1.4         $ & $        1.4         $ & $      \bf 2.0       $ \\
{\sc statlog-heart}  &      (270, 14)       & $        1.2         $ & $      \bf 1.6       $ & $        1.2         $ & $        1.0         $ \\
{\sc haberman-survival} &       (306, 4)       & $      \bf 1.4       $ & $        1.0         $ & $      \bf 1.4       $ & $      \bf 1.4       $ \\
  {\sc ionosphere}   &      (351, 34)       & $        1.8         $ & $        1.6         $ & $      \bf 2.6       $ & $        2.4         $ \\
 {\sc horse-colic}   &      (368, 26)       & $        1.8         $ & $      \bf 2.8       $ & $        1.4         $ & $        2.4         $ \\
{\sc congressional-voting} &      (435, 17)       & $      \bf 1.6       $ & $        1.2         $ & $        1.4         $ & $        1.0         $ \\
{\sc cylinder-bands} &      (512, 36)       & $        1.8         $ & $        1.6         $ & $        2.0         $ & $      \bf 3.2       $ \\
{\sc breast-cancer-wisc-diag} &      (569, 31)       & $        1.2         $ & $        1.8         $ & $        2.2         $ & $      \bf 2.4       $ \\
{\sc ilpd-indian-liver} &      (583, 10)       & $      \bf 2.2       $ & $        1.4         $ & $        1.6         $ & $      \bf 2.2       $ \\
   {\sc monks-2}     &       (601, 7)       & $        1.8         $ & $        1.2         $ & $        2.2         $ & $      \bf 3.6       $ \\
{\sc statlog-australian-credit} &      (690, 15)       & $      \bf 1.6       $ & $      \bf 1.6       $ & $      \bf 1.6       $ & $      \bf 1.6       $ \\
{\sc credit-approval} &      (690, 16)       & $        1.0         $ & $        1.6         $ & $      \bf 2.2       $ & $        1.8         $ \\
{\sc breast-cancer-wisc} &      (699, 10)       & $      \bf 1.0       $ & $      \bf 1.0       $ & $      \bf 1.0       $ & $      \bf 1.0       $ \\
    {\sc blood}      &       (748, 5)       & $        1.4         $ & $      \bf 2.2       $ & $        1.8         $ & $        1.8         $ \\
     {\sc pima}      &       (768, 9)       & $        1.0         $ & $        1.2         $ & $      \bf 1.6       $ & $      \bf 1.6       $ \\
 {\sc mammographic}  &       (961, 6)       & $      \bf 1.8       $ & $        1.6         $ & $        1.2         $ & $        1.2         $ \\
{\sc statlog-german-credit} &      (1000, 25)      & $      \bf 2.2       $ & $        1.2         $ & $        1.6         $ & $        1.8         $ \\
\hline
    {Bold Count}     & {}& $12$           & $13$           & $11$           & $16$           \\
\bottomrule\end{tabular}


==> table/new_isotropic_test_lpd_order.tex <==
\begin{tabular}{lc|ccccc}
%test lpd order (this table has been automatically generated, do not alter manually)
\toprule
{} &($n$, $d$)     &          LA         &          EP         &          VI         &         Ours        \\
\hline
    {\sc trains}     &       (10, 30)       & $        1.8         $ & $        3.0         $ & $        1.8         $ & $      \bf 3.4       $ \\
   {\sc balloons}    &       (16, 5)        & $        2.2         $ & $        2.4         $ & $        2.4         $ & $      \bf 3.0       $ \\
  {\sc fertility}    &      (100, 10)       & $        2.6         $ & $        2.2         $ & $        2.2         $ & $      \bf 3.0       $ \\
{\sc pittsburg-bridges-T-OR-D} &       (102, 8)       & $        2.6         $ & $        1.6         $ & $      \bf 3.0       $ & $        2.8         $ \\
{\sc acute-nephritis} &       (120, 7)       & $        1.0         $ & $        2.0         $ & $        3.0         $ & $      \bf 4.0       $ \\
{\sc acute-inflammation} &       (120, 7)       & $        1.0         $ & $        2.0         $ & $        3.0         $ & $      \bf 4.0       $ \\
{\sc echocardiogram} &      (131, 11)       & $        2.0         $ & $      \bf 2.8       $ & $        2.6         $ & $        2.6         $ \\
  {\sc hepatitis}    &      (155, 20)       & $        2.6         $ & $        1.6         $ & $        2.8         $ & $      \bf 3.0       $ \\
  {\sc parkinsons}   &      (195, 23)       & $        1.6         $ & $        1.4         $ & $        3.2         $ & $      \bf 3.8       $ \\
{\sc breast-cancer-wisc-prog} &      (198, 34)       & $        2.4         $ & $        1.6         $ & $      \bf 3.0       $ & $      \bf 3.0       $ \\
    {\sc spect}      &      (265, 23)       & $        2.2         $ & $        2.6         $ & $      \bf 2.8       $ & $        2.4         $ \\
{\sc statlog-heart}  &      (270, 14)       & $        2.0         $ & $      \bf 3.4       $ & $        2.4         $ & $        2.2         $ \\
{\sc haberman-survival} &       (306, 4)       & $        2.6         $ & $      \bf 2.8       $ & $        2.2         $ & $        2.4         $ \\
  {\sc ionosphere}   &      (351, 34)       & $        1.8         $ & $        1.2         $ & $        3.4         $ & $      \bf 3.6       $ \\
 {\sc horse-colic}   &      (368, 26)       & $        2.4         $ & $      \bf 3.6       $ & $        1.6         $ & $        2.4         $ \\
{\sc congressional-voting} &      (435, 17)       & $        2.0         $ & $      \bf 3.0       $ & $        2.4         $ & $        2.6         $ \\
{\sc cylinder-bands} &      (512, 36)       & $        2.0         $ & $        1.0         $ & $        3.0         $ & $      \bf 4.0       $ \\
{\sc breast-cancer-wisc-diag} &      (569, 31)       & $        2.4         $ & $        1.0         $ & $        3.0         $ & $      \bf 3.6       $ \\
{\sc ilpd-indian-liver} &      (583, 10)       & $        2.6         $ & $        1.6         $ & $        2.8         $ & $      \bf 3.0       $ \\
   {\sc monks-2}     &       (601, 7)       & $        2.0         $ & $        1.0         $ & $        3.0         $ & $      \bf 4.0       $ \\
{\sc statlog-australian-credit} &      (690, 15)       & $        2.4         $ & $        1.0         $ & $      \bf 3.4       $ & $        3.2         $ \\
{\sc credit-approval} &      (690, 16)       & $        2.4         $ & $        2.2         $ & $        2.6         $ & $      \bf 2.8       $ \\
{\sc breast-cancer-wisc} &      (699, 10)       & $        2.2         $ & $        1.6         $ & $        3.0         $ & $      \bf 3.2       $ \\
    {\sc blood}      &       (748, 5)       & $        2.4         $ & $        2.2         $ & $        2.6         $ & $      \bf 2.8       $ \\
     {\sc pima}      &       (768, 9)       & $        2.2         $ & $      \bf 2.8       $ & $        2.6         $ & $        2.4         $ \\
 {\sc mammographic}  &       (961, 6)       & $        2.6         $ & $      \bf 3.2       $ & $        2.2         $ & $        2.0         $ \\
{\sc statlog-german-credit} &      (1000, 25)      & $        2.0         $ & $        2.6         $ & $      \bf 2.8       $ & $        2.6         $ \\
\hline
    {Bold Count}     & {}& $0$            & $7$            & $5$            & $16$           \\
\bottomrule\end{tabular}


==> table/old_isotropic_test_acc.tex <==
\begin{tabular}{lc|cccc}
%test acc (this table has been automatically generated, do not alter manually)
\toprule
{} &($n$, $d$)     &          LA         &          EP         &         CVI         &      OLD\_EPCVI     \\
\hline
    {\sc trains}     &       (10, 30)       & $\bf 0.700{\pm}0.400 $ & $\bf 0.800{\pm}0.245 $ & $\bf 0.800{\pm}0.245 $ & $\bf 0.800{\pm}0.245 $ \\
   {\sc balloons}    &       (16, 5)        & $\bf 0.667{\pm}0.298 $ & $\bf 0.667{\pm}0.298 $ & $\bf 0.667{\pm}0.298 $ & $\bf 0.617{\pm}0.256 $ \\
  {\sc fertility}    &      (100, 10)       & $\bf 0.880{\pm}0.060 $ & $\bf 0.880{\pm}0.060 $ & $\bf 0.880{\pm}0.060 $ & $\bf 0.880{\pm}0.060 $ \\
{\sc pittsburg-bridges-T-OR-D} &       (102, 8)       & $\bf 0.863{\pm}0.036 $ & $\bf 0.883{\pm}0.066 $ & $\bf 0.863{\pm}0.036 $ & $\bf 0.863{\pm}0.036 $ \\
{\sc acute-inflammation} &       (120, 7)       & $\bf 1.000{\pm}0.000 $ & $\bf 1.000{\pm}0.000 $ & $\bf 1.000{\pm}0.000 $ & $\bf 1.000{\pm}0.000 $ \\
{\sc acute-nephritis} &       (120, 7)       & $\bf 1.000{\pm}0.000 $ & $\bf 1.000{\pm}0.000 $ & $\bf 1.000{\pm}0.000 $ & $\bf 1.000{\pm}0.000 $ \\
{\sc echocardiogram} &      (131, 11)       & $  0.808{\pm}0.061   $ & $\bf 0.847{\pm}0.043 $ & $\bf 0.785{\pm}0.076 $ & $  0.778{\pm}0.063   $ \\
  {\sc hepatitis}    &      (155, 20)       & $\bf 0.813{\pm}0.024 $ & $\bf 0.813{\pm}0.032 $ & $\bf 0.813{\pm}0.024 $ & $\bf 0.832{\pm}0.032 $ \\
   {\sc planning}    &      (182, 13)       & $\bf 0.714{\pm}0.038 $ & $\bf 0.714{\pm}0.038 $ & $\bf 0.714{\pm}0.038 $ & $\bf 0.714{\pm}0.038 $ \\
{\sc breast-cancer-wisc-prog} &      (198, 34)       & $\bf 0.793{\pm}0.051 $ & $\bf 0.793{\pm}0.069 $ & $\bf 0.793{\pm}0.051 $ & $\bf 0.793{\pm}0.051 $ \\
    {\sc spect}      &      (265, 23)       & $\bf 0.706{\pm}0.031 $ & $\bf 0.698{\pm}0.027 $ & $\bf 0.702{\pm}0.028 $ & $\bf 0.706{\pm}0.023 $ \\
{\sc statlog-heart}  &      (270, 14)       & $\bf 0.830{\pm}0.036 $ & $\bf 0.833{\pm}0.039 $ & $\bf 0.830{\pm}0.036 $ & $\bf 0.826{\pm}0.034 $ \\
{\sc haberman-survival} &       (306, 4)       & $\bf 0.725{\pm}0.039 $ & $\bf 0.719{\pm}0.036 $ & $\bf 0.725{\pm}0.039 $ & $\bf 0.725{\pm}0.039 $ \\
  {\sc ionosphere}   &      (351, 34)       & $\bf 0.932{\pm}0.025 $ & $\bf 0.932{\pm}0.024 $ & $\bf 0.946{\pm}0.024 $ & $\bf 0.949{\pm}0.026 $ \\
 {\sc horse-colic}   &      (368, 26)       & $\bf 0.799{\pm}0.035 $ & $\bf 0.807{\pm}0.032 $ & $\bf 0.791{\pm}0.045 $ & $\bf 0.788{\pm}0.050 $ \\
{\sc congressional-voting} &      (435, 17)       & $\bf 0.605{\pm}0.024 $ & $\bf 0.593{\pm}0.014 $ & $\bf 0.595{\pm}0.013 $ & $\bf 0.591{\pm}0.016 $ \\
{\sc ilpd-indian-liver} &      (583, 10)       & $\bf 0.719{\pm}0.025 $ & $\bf 0.712{\pm}0.020 $ & $\bf 0.717{\pm}0.029 $ & $\bf 0.719{\pm}0.028 $ \\
{\sc credit-approval} &      (690, 16)       & $\bf 0.859{\pm}0.026 $ & $\bf 0.864{\pm}0.020 $ & $\bf 0.864{\pm}0.024 $ & $\bf 0.862{\pm}0.026 $ \\
{\sc statlog-australian-credit} &      (690, 15)       & $\bf 0.678{\pm}0.028 $ & $\bf 0.677{\pm}0.021 $ & $\bf 0.678{\pm}0.028 $ & $\bf 0.678{\pm}0.028 $ \\
{\sc breast-cancer-wisc} &      (699, 10)       & $\bf 0.969{\pm}0.016 $ & $\bf 0.969{\pm}0.016 $ & $\bf 0.969{\pm}0.016 $ & $\bf 0.969{\pm}0.016 $ \\
    {\sc blood}      &       (748, 5)       & $\bf 0.785{\pm}0.042 $ & $\bf 0.785{\pm}0.041 $ & $\bf 0.786{\pm}0.044 $ & $\bf 0.786{\pm}0.044 $ \\
     {\sc pima}      &       (768, 9)       & $\bf 0.764{\pm}0.027 $ & $\bf 0.766{\pm}0.025 $ & $\bf 0.767{\pm}0.026 $ & $\bf 0.767{\pm}0.026 $ \\
 {\sc mammographic}  &       (961, 6)       & $\bf 0.824{\pm}0.019 $ & $\bf 0.823{\pm}0.017 $ & $\bf 0.823{\pm}0.019 $ & $\bf 0.823{\pm}0.019 $ \\
{\sc statlog-german-credit} &      (1000, 25)      & $\bf 0.770{\pm}0.039 $ & $\bf 0.763{\pm}0.038 $ & $\bf 0.768{\pm}0.038 $ & $\bf 0.769{\pm}0.037 $ \\
\hline
  {\sc Bold Count}   & {}& $23$           & $24$           & $24$           & $23$           \\
\bottomrule\end{tabular}


==> table/old_isotropic_test_acc_order.tex <==
\begin{tabular}{l|ccccc|c}
%test acc order (this table has been automatically generated, do not alter manually)
\toprule
{} &         LA          &         EP          &         VI          &        CVI          &       EPCVI         &($n$, $d$)     \\
\hline
  {\sc fertility}    & $     \bf 1.000      $ & $     \bf 1.000      $ & $     \bf 1.000      $ & $     \bf 1.000      $ & $     \bf 1.000      $ &      (100, 10)       \\
{\sc statlog-german-credit} & $     \bf 2.600      $ & $       1.400        $ & $       1.600        $ & $       1.600        $ & $       2.000        $ &      (1000, 25)      \\
  {\sc hepatitis}    & $       1.400        $ & $       1.800        $ & $       1.400        $ & $       1.400        $ & $     \bf 3.200      $ &      (155, 20)       \\
{\sc breast-cancer-wisc-prog} & $       1.400        $ & $     \bf 3.400      $ & $       1.400        $ & $       1.400        $ & $       1.400        $ &      (198, 34)       \\
    {\sc trains}     & $       1.000        $ & $     \bf 1.200      $ & $     \bf 1.200      $ & $     \bf 1.200      $ & $     \bf 1.200      $ &       (10, 30)       \\
 {\sc horse-colic}   & $       2.600        $ & $     \bf 4.000      $ & $       1.400        $ & $       1.400        $ & $       1.800        $ &      (368, 26)       \\
{\sc statlog-heart}  & $       1.200        $ & $     \bf 1.800      $ & $       1.200        $ & $       1.200        $ & $       1.000        $ &      (270, 14)       \\
    {\sc blood}      & $       1.400        $ & $     \bf 2.200      $ & $       1.800        $ & $     \bf 2.200      $ & $     \bf 2.200      $ &       (748, 5)       \\
{\sc cylinder-bands} & $       2.400        $ & $       2.000        $ & $       2.000        $ & $       2.000        $ & $     \bf 4.600      $ &      (512, 36)       \\
{\sc credit-approval} & $       1.000        $ & $       1.800        $ & $     \bf 2.000      $ & $     \bf 2.000      $ & $       1.400        $ &      (690, 16)       \\
  {\sc ionosphere}   & $       1.800        $ & $       1.800        $ & $       2.600        $ & $       2.600        $ & $     \bf 2.800      $ &      (351, 34)       \\
   {\sc planning}    & $     \bf 1.000      $ & $     \bf 1.000      $ & $     \bf 1.000      $ & $     \bf 1.000      $ & $     \bf 1.000      $ &      (182, 13)       \\
{\sc pittsburg-bridges-T-OR-D} & $       1.200        $ & $     \bf 1.800      $ & $       1.200        $ & $       1.200        $ & $       1.200        $ &       (102, 8)       \\
{\sc statlog-australian-credit} & $       1.600        $ & $     \bf 1.800      $ & $       1.600        $ & $       1.600        $ & $       1.600        $ &      (690, 15)       \\
{\sc congressional-voting} & $     \bf 1.800      $ & $       1.200        $ & $       1.400        $ & $       1.400        $ & $       1.000        $ &      (435, 17)       \\
{\sc echocardiogram} & $       2.400        $ & $     \bf 4.400      $ & $       1.200        $ & $       1.200        $ & $       1.000        $ &      (131, 11)       \\
   {\sc balloons}    & $     \bf 1.000      $ & $     \bf 1.000      $ & $     \bf 1.000      $ & $     \bf 1.000      $ & $     \bf 1.000      $ &       (16, 5)        \\
{\sc haberman-survival} & $     \bf 1.400      $ & $       1.000        $ & $     \bf 1.400      $ & $     \bf 1.400      $ & $     \bf 1.400      $ &       (306, 4)       \\
    {\sc spect}      & $       2.000        $ & $       1.600        $ & $       1.400        $ & $       1.400        $ & $     \bf 2.200      $ &      (265, 23)       \\
  {\sc parkinsons}   & $     \bf 2.800      $ & $       1.000        $ & $       2.000        $ & $       2.000        $ & $       2.600        $ &      (195, 23)       \\
{\sc ilpd-indian-liver} & $     \bf 2.400      $ & $       1.800        $ & $       2.200        $ & $       1.800        $ & $     \bf 2.400      $ &      (583, 10)       \\
{\sc breast-cancer-wisc} & $       1.000        $ & $       1.000        $ & $     \bf 1.400      $ & $     \bf 1.400      $ & $     \bf 1.400      $ &      (699, 10)       \\
 {\sc mammographic}  & $     \bf 2.000      $ & $       1.800        $ & $       1.200        $ & $       1.200        $ & $       1.200        $ &       (961, 6)       \\
     {\sc pima}      & $       1.000        $ & $       1.200        $ & $     \bf 1.600      $ & $     \bf 1.600      $ & $     \bf 1.600      $ &       (768, 9)       \\
\hline
  {\sc Bold Count}   & $9$            & $11$           & $8$            & $9$            & $13$           & {}\\
\bottomrule\end{tabular}


==> table/old_isotropic_test_lpd.tex <==
\begin{tabular}{lc|cccc}
%test lpd (this table has been automatically generated, do not alter manually)
\toprule
{} &($n$, $d$)     &          LA         &          EP         &         CVI         &      OLD\_EPCVI     \\
\hline
    {\sc trains}     &       (10, 30)       & $\bf -0.695{\pm}0.011$ & $\bf -0.687{\pm}0.023$ & $\bf -0.692{\pm}0.023$ & $\bf -0.681{\pm}0.042$ \\
   {\sc balloons}    &       (16, 5)        & $\bf -0.707{\pm}0.146$ & $\bf -0.684{\pm}0.161$ & $\bf -0.711{\pm}0.239$ & $\bf -0.661{\pm}0.267$ \\
  {\sc fertility}    &      (100, 10)       & $\bf -0.379{\pm}0.099$ & $\bf -0.384{\pm}0.138$ & $\bf -0.378{\pm}0.103$ & $\bf -0.379{\pm}0.103$ \\
{\sc pittsburg-bridges-T-OR-D} &       (102, 8)       & $\bf -0.306{\pm}0.044$ & $\bf -0.316{\pm}0.060$ & $\bf -0.295{\pm}0.057$ & $\bf -0.296{\pm}0.059$ \\
{\sc acute-inflammation} &       (120, 7)       & $  -0.172{\pm}0.033  $ & $  -0.055{\pm}0.005  $ & $  -0.008{\pm}0.001  $ & $\bf -0.007{\pm}0.001$ \\
{\sc acute-nephritis} &       (120, 7)       & $  -0.203{\pm}0.010  $ & $  -0.047{\pm}0.009  $ & $  -0.006{\pm}0.002  $ & $\bf -0.004{\pm}0.001$ \\
{\sc echocardiogram} &      (131, 11)       & $\bf -0.420{\pm}0.073$ & $\bf -0.412{\pm}0.084$ & $\bf -0.420{\pm}0.085$ & $\bf -0.421{\pm}0.086$ \\
  {\sc hepatitis}    &      (155, 20)       & $\bf -0.369{\pm}0.043$ & $\bf -0.376{\pm}0.046$ & $\bf -0.361{\pm}0.051$ & $\bf -0.354{\pm}0.053$ \\
   {\sc planning}    &      (182, 13)       & $\bf -0.602{\pm}0.032$ & $  -0.638{\pm}0.020  $ & $\bf -0.602{\pm}0.032$ & $\bf -0.602{\pm}0.032$ \\
{\sc breast-cancer-wisc-prog} &      (198, 34)       & $\bf -0.460{\pm}0.063$ & $\bf -0.478{\pm}0.083$ & $\bf -0.458{\pm}0.071$ & $\bf -0.458{\pm}0.070$ \\
    {\sc spect}      &      (265, 23)       & $\bf -0.587{\pm}0.045$ & $\bf -0.587{\pm}0.052$ & $\bf -0.589{\pm}0.050$ & $\bf -0.590{\pm}0.051$ \\
{\sc statlog-heart}  &      (270, 14)       & $\bf -0.392{\pm}0.071$ & $\bf -0.380{\pm}0.058$ & $\bf -0.394{\pm}0.080$ & $\bf -0.395{\pm}0.080$ \\
{\sc haberman-survival} &       (306, 4)       & $\bf -0.535{\pm}0.050$ & $\bf -0.539{\pm}0.059$ & $\bf -0.537{\pm}0.054$ & $\bf -0.537{\pm}0.054$ \\
  {\sc ionosphere}   &      (351, 34)       & $  -0.221{\pm}0.021  $ & $  -0.227{\pm}0.016  $ & $\bf -0.169{\pm}0.031$ & $\bf -0.190{\pm}0.051$ \\
 {\sc horse-colic}   &      (368, 26)       & $  -0.465{\pm}0.058  $ & $\bf -0.455{\pm}0.060$ & $\bf -0.466{\pm}0.068$ & $\bf -0.487{\pm}0.080$ \\
{\sc congressional-voting} &      (435, 17)       & $\bf -0.636{\pm}0.026$ & $\bf -0.633{\pm}0.027$ & $\bf -0.636{\pm}0.029$ & $\bf -0.636{\pm}0.029$ \\
{\sc ilpd-indian-liver} &      (583, 10)       & $\bf -0.516{\pm}0.033$ & $\bf -0.521{\pm}0.033$ & $\bf -0.516{\pm}0.037$ & $\bf -0.516{\pm}0.037$ \\
{\sc credit-approval} &      (690, 16)       & $\bf -0.342{\pm}0.008$ & $\bf -0.343{\pm}0.012$ & $\bf -0.341{\pm}0.008$ & $\bf -0.341{\pm}0.009$ \\
{\sc statlog-australian-credit} &      (690, 15)       & $\bf -0.627{\pm}0.022$ & $\bf -0.636{\pm}0.030$ & $\bf -0.627{\pm}0.023$ & $\bf -0.627{\pm}0.023$ \\
{\sc breast-cancer-wisc} &      (699, 10)       & $\bf -0.091{\pm}0.030$ & $\bf -0.092{\pm}0.028$ & $\bf -0.091{\pm}0.037$ & $\bf -0.091{\pm}0.037$ \\
    {\sc blood}      &       (748, 5)       & $\bf -0.475{\pm}0.043$ & $\bf -0.476{\pm}0.045$ & $\bf -0.476{\pm}0.044$ & $\bf -0.476{\pm}0.044$ \\
     {\sc pima}      &       (768, 9)       & $\bf -0.470{\pm}0.031$ & $\bf -0.472{\pm}0.035$ & $\bf -0.471{\pm}0.033$ & $\bf -0.471{\pm}0.033$ \\
 {\sc mammographic}  &       (961, 6)       & $\bf -0.408{\pm}0.037$ & $\bf -0.408{\pm}0.041$ & $\bf -0.408{\pm}0.039$ & $\bf -0.408{\pm}0.039$ \\
{\sc statlog-german-credit} &      (1000, 25)      & $\bf -0.493{\pm}0.040$ & $\bf -0.493{\pm}0.041$ & $\bf -0.493{\pm}0.043$ & $\bf -0.494{\pm}0.043$ \\
\hline
  {\sc Bold Count}   & {}& $20$           & $20$           & $22$           & $24$           \\
\bottomrule\end{tabular}


==> table/old_isotropic_test_lpd_order.tex <==
\begin{tabular}{l|ccccc|c}
%test lpd order (this table has been automatically generated, do not alter manually)
\toprule
{} &         LA          &         EP          &         VI          &        CVI          &       EPCVI         &($n$, $d$)     \\
\hline
  {\sc fertility}    & $       2.800        $ & $       2.600        $ & $       2.800        $ & $       3.000        $ & $     \bf 3.800      $ &      (100, 10)       \\
{\sc statlog-german-credit} & $       2.400        $ & $       3.000        $ & $       3.200        $ & $     \bf 3.400      $ & $       3.000        $ &      (1000, 25)      \\
  {\sc hepatitis}    & $       2.800        $ & $       1.800        $ & $       3.000        $ & $     \bf 3.800      $ & $       3.600        $ &      (155, 20)       \\
{\sc breast-cancer-wisc-prog} & $       2.800        $ & $       1.800        $ & $     \bf 3.800      $ & $       3.200        $ & $       3.400        $ &      (198, 34)       \\
    {\sc trains}     & $       2.200        $ & $     \bf 4.200      $ & $       2.400        $ & $       2.600        $ & $       3.600        $ &       (10, 30)       \\
 {\sc horse-colic}   & $       2.800        $ & $     \bf 4.400      $ & $       2.000        $ & $       2.600        $ & $       3.200        $ &      (368, 26)       \\
{\sc statlog-heart}  & $       2.400        $ & $     \bf 4.200      $ & $       2.600        $ & $       3.200        $ & $       2.600        $ &      (270, 14)       \\
    {\sc blood}      & $       2.800        $ & $       2.600        $ & $     \bf 3.400      $ & $       3.200        $ & $       3.000        $ &       (748, 5)       \\
{\sc cylinder-bands} & $       2.000        $ & $       1.000        $ & $       3.600        $ & $       3.400        $ & $     \bf 5.000      $ &      (512, 36)       \\
{\sc credit-approval} & $       1.800        $ & $       2.600        $ & $     \bf 3.600      $ & $       3.400        $ & $     \bf 3.600      $ &      (690, 16)       \\
  {\sc ionosphere}   & $       1.800        $ & $       1.200        $ & $     \bf 4.200      $ & $       4.000        $ & $       3.800        $ &      (351, 34)       \\
   {\sc planning}    & $       3.400        $ & $       1.000        $ & $       3.200        $ & $     \bf 3.800      $ & $       3.600        $ &      (182, 13)       \\
{\sc pittsburg-bridges-T-OR-D} & $       3.000        $ & $       1.800        $ & $       3.400        $ & $     \bf 3.600      $ & $       3.200        $ &       (102, 8)       \\
{\sc statlog-australian-credit} & $       2.600        $ & $       1.000        $ & $       3.600        $ & $     \bf 4.200      $ & $       3.600        $ &      (690, 15)       \\
{\sc congressional-voting} & $       2.400        $ & $     \bf 3.600      $ & $       2.800        $ & $       3.000        $ & $       3.200        $ &      (435, 17)       \\
{\sc echocardiogram} & $       2.200        $ & $     \bf 3.400      $ & $     \bf 3.400      $ & $       2.800        $ & $       3.200        $ &      (131, 11)       \\
   {\sc balloons}    & $       2.600        $ & $       2.800        $ & $       3.200        $ & $       3.000        $ & $     \bf 3.400      $ &       (16, 5)        \\
{\sc haberman-survival} & $       3.200        $ & $     \bf 3.400      $ & $       2.400        $ & $       3.000        $ & $       3.000        $ &       (306, 4)       \\
    {\sc spect}      & $       2.600        $ & $       3.000        $ & $       3.200        $ & $     \bf 3.400      $ & $       2.800        $ &      (265, 23)       \\
  {\sc parkinsons}   & $       1.600        $ & $       1.400        $ & $       3.200        $ & $       3.800        $ & $     \bf 5.000      $ &      (195, 23)       \\
{\sc ilpd-indian-liver} & $       2.600        $ & $       1.800        $ & $     \bf 3.600      $ & $       3.400        $ & $     \bf 3.600      $ &      (583, 10)       \\
{\sc breast-cancer-wisc} & $       2.400        $ & $       1.800        $ & $     \bf 3.800      $ & $       3.200        $ & $     \bf 3.800      $ &      (699, 10)       \\
 {\sc mammographic}  & $       2.600        $ & $     \bf 4.000      $ & $       3.000        $ & $       2.800        $ & $       2.600        $ &       (961, 6)       \\
     {\sc pima}      & $       2.600        $ & $     \bf 3.400      $ & $       3.000        $ & $       3.200        $ & $       2.800        $ &       (768, 9)       \\
\hline
  {\sc Bold Count}   & $0$            & $8$            & $7$            & $6$            & $7$            & {}\\
\bottomrule\end{tabular}


==> table/t_test_lpd_full.tex <==
\begin{tabular}{lc|cccc|c}
%test lpd (this table has been automatically generated, do not alter manually)
\toprule
{} &($n$, $d$)     &          LA         &          EP         &          VI         &         Ours   & MCMC     \\
\hline
     {\sc neal}      &       (100, 1)       & $\bf 0.317{\pm}0.440 $ & $\bf 0.303{\pm}0.432 $ & $\bf 0.295{\pm}0.426 $ & $\bf 0.301{\pm}0.436 $ & $0.309 {\pm} 0.454 $ \\
    {\sc boston}     &      (506, 13)       & $\bf -0.210{\pm}0.069$ & $\bf -0.190{\pm}0.053$ & $  -0.206{\pm}0.056  $ & $\bf -0.195{\pm}0.061$ & $-0.191 {\pm} 0.051 $ \\
    {\sc stock}      &      (1000, 1)       & $  1.910{\pm}0.079   $ & $  1.389{\pm}0.242   $ & $  1.917{\pm}0.082   $ & $\bf 1.921{\pm}0.083 $ & $1.586 {\pm} 0.034 $ \\
\hline
    {Bold Count}     & {}& $2$            & $2$            & $1$            & $3$     & $/$      \\
\bottomrule\end{tabular}


==> table/t_test_lpd_order.tex <==
\begin{tabular}{lc|ccccc}
%test lpd order (this table has been automatically generated, do not alter manually)
\toprule
{} &($n$, $d$)     &          LA         &          EP         &          VI         &         Ours        \\
\hline
     {\sc neal}      &       (100, 1)       & $      \bf 3.0       $ & $        2.0         $ & $        2.6         $ & $        2.4         $ \\
    {\sc boston}     &      (506, 13)       & $        1.8         $ & $      \bf 3.4       $ & $        1.8         $ & $        3.0         $ \\
    {\sc stock}      &      (1000, 1)       & $        2.0         $ & $        1.6         $ & $        2.6         $ & $      \bf 3.8       $ \\
\hline
    {Bold Count}     & {}& $1$            & $1$            & $0$            & $1$            \\
\bottomrule\end{tabular}


==> table/test_lpd_order_copy.tex <==
A & B & C \\
